Distributing Labels on Infinite Trees

Sturmian words are infinite binary words with many equivalent definitions: They have a minimal factor complexity among all aperiodic sequences; they are balanced sequences (the labels 0 and 1 are as evenly distributed as possible) and they can be constructed using a mechanical definition. All this properties make them good candidates for being extremal points in scheduling problems over two processors. In this paper, we consider the problem of generalizing Sturmian words to trees. The problem is to evenly distribute labels 0 and 1 over infinite trees. We show that (strongly) balanced trees exist and can also be constructed using a mechanical process as long as the tree is irrational. Such trees also have a minimal factor complexity. Therefore they bring the hope that extremal scheduling properties of Sturmian words can be extended to such trees, as least partially. Such possible extensions are illustrated by one such example.

==> pgf.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfatcode{\the\catcode`\@}
\catcode`\@=11


\input pgfrcs.tex
\ProvidesPackageRCS $Header: /cvsroot/pgf/pgf/plain/pgf/basiclayer/pgf.tex,v 1.10 2008/01/15 17:17:22 tantau Exp $

\input pgfcore.tex

\usepgfmodule{shapes,plot}

%\input pgfbasesnakes.tex
%\input pgfbasedecorations.tex
%\input pgfbasematrix.tex

\catcode`\@=\pgfatcode

\endinput


==> pgfbaseimage.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfbaseimageatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfcore.tex

\PackageWarning{pgf}{This package is obsolete and no longer needed}

\catcode`\@=\pgfbaseimageatcode

\endinput


==> pgfbaselayers.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfbaselayersatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfcore.tex

\PackageWarning{pgf}{This package is obsolete and no longer needed}

\catcode`\@=\pgfbaselayersatcode

\endinput


==> pgfbasematrix.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfbasematrixatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfcore.tex

\PackageWarning{pgf}{This package is obsolete. Use \string\usepgfmodule{matrix} instead}

\usepgfmodule{matrix}

\catcode`\@=\pgfbasematrixatcode

\endinput


==> pgfbasepatterns.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfbasepatternsatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfcore.tex

\PackageWarning{pgf}{This package is obsolete and no longer needed}

\catcode`\@=\pgfbasepatternsatcode

\endinput


==> pgfbaseplot.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfbaseplotatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfcore.tex

\PackageWarning{pgf}{This package is obsolete. Use \string\usepgfmodule{plot} instead}

\usepgfmodule{plot}

\catcode`\@=\pgfbaseplotatcode

\endinput


==> pgfbaseshapes.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfbaseshapesatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfcore.tex

\PackageWarning{pgf}{This package is obsolete. Use \string\usepgfmodule{shapes} instead}

\usepgfmodule{shapes}

\catcode`\@=\pgfbaseshapesatcode

\endinput


==> pgfbasesnakes.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\edef\pgfbasesnakesatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfcore.tex

\PackageWarning{pgf}{This package is obsolete. Use \string\usepgfmodule{decorations} instead}

\usepgfmodule{decorations}

\catcode`\@=\pgfbasesnakesatcode

\endinput


==> pgfcalendar.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/utilities/pgfcalendar.code.tex,v 1.11 2007/07/23 21:23:14 tantau Exp $


% Translation stuff

\ifx\translate\@undefined
  \def\translate#1{#1}
\fi

% Load month dictionary, if possible

\ifx\usedictionary\@undefined
\else
  \usedictionary{translator-months-dictionary}
\fi




% Typeset a calendar
%
% #1 = prefix for the calendar nodes
% #2 = begin date in ISO format
% #3 = end date in ISO format
% #4 = date rendering code
%
% Description:
%
% First note that this macro need not be called inside a pgfpicture
% (even though it often will be). You can use it to typeset
% calendars also using packages other than pgf. You do not even need
% to load pgf to use this file.
%
% A calendar is typeset as follows: You specify a range of dates (by
% providing a begin and an end date). Then, for each date the code #4
% is executed. When the code is called, lots of information about the
% current date (like its day of week) is available. The job of
% #4 is to render the date. Typically, this is done by placing nodes
% somewhere, but the function could do other things as well. 
% It is also the job of #4 to position the calendar correctly.
%
% The different calls of #4 are not surrounded by TeX groups (though
% you can do so yourself, of course). This means that settings can
% accumulate between different calls, which is often desirable and
% useful. 
%
% Inside #4 code, different macros can be access:
%
% \pgfcalendarprefix
% The parameter #1. This prefix is recomended for nodes inside the
% calendar, but you have to use it yourself explicitly.
%
% \pgfcalendarbeginiso
% Start date of range being typeset in ISO format (like 2006-01-10)
%
% \pgfcalendarbeginjulian
% Julian day number of start date begin typeset
%
% \pgfcalendarendiso
% End date of range begin typeset
%
% \pgfcalendarendjulian
% Same as Julian day number
%
% \pgfcalendarcurrentjulian (a TeX-count)
% Julian day number of day to be rendered/considered
%
% \pgfcalendarcurrentweekday
% Weekday (0 = Monday) of day to be checked
%
% \pgfcalendarcurrentyear
% Year of day to be checked
%
% \pgfcalendarcurrentmonth
% Month of day to be chjeck
%
% \pgfcalendarcurrentday
% Day of monath of day to be checked
%
%
% Inside the \pgfcalendar macro the macro \ifdate is available, which
% has the same effect as \pgfcalendarifdate{\pgfcalendarcurrentjulian}
% (only faster). This means that you
% can write, say, \ifdate{Monday}{current date is a Monday}{Not a Monday}.
%
% Example:
%
% \begin{tikzpicture}
%   \pgfcalendar{cal}{2007-01-20}{2007-02-10}
%     {\node[anchor=base] {\pgfcalendaronday}; \pgftransformyshift{-1.5em}}
% \end{tikzpicture}
%
% \pgfcalendar{cal}{2007-01-20}{2007-02-10}{ \pgfcalendaronday\ }

\long\def\pgfcalendar#1#2#3#4{%
  \begingroup%
    % Setup local \ifdate
    \let\ifdate=\pgfcalendar@local@ifdate%
    % Let's start with computing start and end dates... 
    \def\pgfcalendarprefix{#1}%
    \pgfcalendardatetojulian{#2}{\pgfcalendarcurrentjulian}%
    \edef\pgfcalendarbeginjulian{\the\pgfcalendarcurrentjulian}%
    \edef\pgfcalendarbeginiso{#2}%
    \pgfcalendardatetojulian{#3}{\pgfutil@tempcnta}%
    \edef\pgfcalendarendjulian{\the\pgfutil@tempcnta}%
    \advance\pgfutil@tempcnta by1\relax%
    \edef\pgfcalendarendjulianplus{\the\pgfutil@tempcnta}%
    \edef\pgfcalendarendiso{#3}%
    %
    % Start main loop
    %
    \loop%
    \ifnum\pgfcalendarcurrentjulian<\pgfcalendarendjulianplus\relax%
      % Setup information about current date
      \pgfcalendarjuliantodate{\pgfcalendarcurrentjulian}%
      {\pgfcalendarcurrentyear}{\pgfcalendarcurrentmonth}{\pgfcalendarcurrentday}%
      \pgfcalendarjuliantoweekday{\pgfcalendarcurrentjulian}{\pgfutil@tempcntb}%
      \edef\pgfcalendarcurrentweekday{\the\pgfutil@tempcntb}%
      % Render:
      #4%
      % Advance day:
      \advance\pgfcalendarcurrentjulian by1\relax%
    \repeat%
  \endgroup%
}

\newcount\pgfcalendarcurrentjulian

\def\pgfcalendar@local@ifdate{%
  \let\pgfcalendarifdatejulian=\pgfcalendarcurrentjulian%
  \let\pgfcalendarifdateyear=\pgfcalendarcurrentyear%
  \let\pgfcalendarifdatemonth=\pgfcalendarcurrentmonth%
  \let\pgfcalendarifdateday=\pgfcalendarcurrentday%
  \let\pgfcalendarifdateweekday=\pgfcalendarcurrentweekday%
  \pgfcalendar@launch@ifdate%
}



% Execute on specific kinds of dates
%
% #1 = ISO-format date
% #2 = date specification
% #3 = code
%
% Description:
%
% The given code #3 is execute on every day that matches the date
% specification #2. This specification is a comma-separated list of
% key-value pairs with the path /pgf/calendar. The code for a
% key-value should check whether the given day matches its
% specification. If so, it should set \pgfcalendarmatches to true.
%
% When the key-value code is executed, the following macros will have
% been setup:
%
% \pgfcalendarifdatejulian 
% Julian day number of day to be checked
%
% \pgfcalendarifdateweekday
% Weekday (0 = Monday) of day to be checked
%
% \pgfcalendarifdateyear
% Year of day to be checked
%
% \pgfcalendarifdatemonth
% Month of day to be chjeck
%
% \pgfcalendarifdateday
% Day of month of day to be checked
%
% The setting of these macros will persist after the call, so a
% sideeffect of callling this macro is to setup these macros.
%
% By setting \ifpgfcalendar@do@not@recompute to false, the computation
% of the year, month etc. is suppressed.
%
% Examples:
%
% \pgfcalendarifdate{2007-01-10}{all}{}
% % Simply setup the macros
%
% \pgfcalendarifdate{2007-01-10}{mondays}{Is a monday}
%
% \pgfcalendarifdate{\mydate}{date=05-01}{\mydate is a Worker's Day}

\def\pgfcalendarifdate#1#2#3#4{%
  \pgfcalendardatetojulian{#1}{\pgfutil@tempcnta}%
  \pgfcalendarjuliantodate{\pgfutil@tempcnta}
    {\pgfcalendarifdateyear}{\pgfcalendarifdatemonth}{\pgfcalendarifdateday}%
  \edef\pgfcalendarifdatejulian{\the\pgfutil@tempcnta}%
  % Compute info about date
  \pgfcalendarjuliantoweekday{\pgfutil@tempcnta}{\pgfutil@tempcntb}%
  \edef\pgfcalendarifdateweekday{\the\pgfutil@tempcntb}%
  %
  \pgfcalendar@launch@ifdate{#2}{#3}{#4}%
}


\long\def\pgfcalendar@launch@ifdate#1#2#3{%
  % When this macro is called, the pgfcalendarifdatexxxx macros must
  % be setup correctly
  %
  % Set match to false
  \pgfcalendarmatchesfalse%
  \pgfqkeys{/pgf/calendar}{#1}% 
  \ifpgfcalendarmatches%
    #2%
  \else%
    #3%
  \fi%
}

\newif\ifpgfcalendarmatches


% Keys for matching

\pgfkeys{/pgf/calendar/all/.code=\pgfcalendarmatchestrue}

\pgfkeys{/pgf/calendar/Monday/.code={\ifnum\pgfcalendarifdateweekday=0\relax\pgfcalendarmatchestrue\fi}}
\pgfkeys{/pgf/calendar/Tuesday/.code={\ifnum\pgfcalendarifdateweekday=1\relax\pgfcalendarmatchestrue\fi}}
\pgfkeys{/pgf/calendar/Wednesday/.code={\ifnum\pgfcalendarifdateweekday=2\relax\pgfcalendarmatchestrue\fi}}
\pgfkeys{/pgf/calendar/Thursday/.code={\ifnum\pgfcalendarifdateweekday=3\relax\pgfcalendarmatchestrue\fi}}
\pgfkeys{/pgf/calendar/Friday/.code={\ifnum\pgfcalendarifdateweekday=4\relax\pgfcalendarmatchestrue\fi}}
\pgfkeys{/pgf/calendar/Saturday/.code={\ifnum\pgfcalendarifdateweekday=5\relax\pgfcalendarmatchestrue\fi}}
\pgfkeys{/pgf/calendar/Sunday/.code={\ifnum\pgfcalendarifdateweekday=6\relax\pgfcalendarmatchestrue\fi}}

\pgfkeys{/pgf/calendar/workday/.code={\ifnum\pgfcalendarifdateweekday<5\relax\pgfcalendarmatchestrue\fi}}
\pgfkeys{/pgf/calendar/weekend/.code={\ifnum\pgfcalendarifdateweekday>4\relax\pgfcalendarmatchestrue\fi}}

\pgfkeys{/pgf/calendar/equals/.cd,.value required,.code={%
  \pgfcalendar@special@datetojulian{#1}%
  \ifnum\pgfcalendarifdatejulian=\pgfutil@tempcnta\relax%
    \pgfcalendarmatchestrue%
  \fi}%
}

\pgfkeys{/pgf/calendar/day of month/.cd,.value required,.code={\ifnum#1=\pgfcalendarifdateday\relax\pgfcalendarmatchestrue\fi}}
\pgfkeys{/pgf/calendar/end of month/.cd,.default=1,.code={%
  % Tricky and expensive ... do only if necessary
  \ifpgfcalendarmatches%
  \else% sigh
    {%
      \pgfutil@tempcnta=\pgfcalendarifdatejulian\relax%
      \advance\pgfutil@tempcnta by#1\relax%
      \pgfcalendarjuliantodate{\pgfutil@tempcnta}{\pgf@dummy}{\pgf@dummy}{\pgf@cal@temp}%
      \global\let\pgf@cal@temp=\pgf@cal@temp%
    }%
    \ifnum\pgf@cal@temp=1\relax\pgfcalendarmatchestrue\fi%
  \fi}%
}

\pgfkeys{/pgf/calendar/at least/.cd,.value required,.code={%
  \pgfcalendar@special@datetojulian{#1}%
  \ifnum\pgfcalendarifdatejulian<\pgfutil@tempcnta\relax%
  \else%
    \pgfcalendarmatchestrue%
  \fi%
}}

\pgfkeys{/pgf/calendar/at most/.cd,.value required,.code={%
  \pgfcalendar@special@datetojulian{#1}%
  \ifnum\pgfcalendarifdatejulian>\pgfutil@tempcnta\relax%
  \else%
    \pgfcalendarmatchestrue%
  \fi%
}}

\pgfkeys{/pgf/calendar/between/.cd,.value required,.code args={#1and#2}{%
  \pgfcalendar@special@datetojulian{#1}%
  \ifnum\pgfcalendarifdatejulian<\pgfutil@tempcnta\relax%
  \else%
    \pgfcalendar@special@datetojulian{#2}%
    \ifnum\pgfcalendarifdatejulian>\pgfutil@tempcnta\relax%
    \else%
      \pgfcalendarmatchestrue%
    \fi%
  \fi%
}}

\def\pgfcalendar@special@datetojulian#1{%
  \edef\pgf@temp{#1}%
  \expandafter\pgfcalendar@special@split@test\pgf@temp-\relax{#1}%  
}

\def\pgfcalendar@special@split@test#1-#2-#3\relax#4{%
  \def\pgf@temp{#3}%
  \ifx\pgf@temp\pgfutil@empty%
    \def\pgf@temp{\pgfcalendarifdateyear-#1-#2}%
  \else%
    \def\pgf@temp{#4}%
  \fi%
  \pgfcalendardatetojulian{\pgf@temp}{\pgfutil@tempcnta}%
}


% Suggested name for nodes inside a calendar
%
% Description:
%
% It is suggested that (main) nodes (if present) in a calendar should
% get this name.
%
% Example:
%
% \pgfcalendar{cal}{2007-01-20}{2007-02-10}{}
% { \node[anchor=base] (\pgfcalendarsuggestedname) {\pgfcalendarifdateday};
%   \pgftransformyshift{-1.5em} }
%
% \draw (cal-2007-01-30) -- (cal-2007-02-08);

\def\pgfcalendarsuggestedname{%
  \ifx\pgfcalendarprefix\pgfutil@empty\else\pgfcalendarprefix-%
  \pgfcalendarcurrentyear-\pgfcalendarcurrentmonth-\pgfcalendarcurrentday\fi%
}



%
%
% Date conversion functions
%
%



% Convert a date to the Julian day number (number of days since
% January 1st, -4712)
%
% #1 = date specification
% #2 = counter that should be set to the number of days
%
% Description:
%
% The conversion is taken from the Wikipedia entry on Julian days. 
%
% The date specification works as follows:
%
% - It starts with a year. Use \year for the current year (the year
%   the file is being typeset).
% - Next comes a hyphen.
% - Next comes a month (number). Use \month for the current month.
% - Next comes a hyphen.
% - Next comes either a day of month (number, use \day for current
%   day) or "last". The keyword "last" refers the last day of the
%   month. Thus, 2006-01-last is the same as 2006-01-31 and
%   2000-02-last is the same as 2002-02-29.
% - Next may come a plus sign, followed by a number (positive or
%   negative). This will adjust the date by the given number of
%   days. Thus, 2006-01-31+1 is the same as 2006-02-01 and
%   2006-02-01+-2 is the same as 2006-01-30. And \year-\month-day+1 is
%   tomorrow. You may add a space before the +.
%
% Example:
%
% \pgfcalendardatetojulian{2006-01-10}{\mycount}

\def\pgfcalendardatetojulian#1#2{\edef\pgf@temp{#1}\expandafter\pgfcalendar@datetojulian\pgf@temp+/{#2}}
\def\pgfcalendar@datetojulian#1-#2-#3+#4/#5{%
  {%
    %
    % Store year, month and days.
    % 
    \count1=#1\relax%
    \count2=#2\relax%
    % If #3=="last", then calculate first day of next month
    \edef\pgf@temp{#3}%
    \ifx\pgf@temp\pgfcalendar@last@text%
      \advance\count2 by1\relax%
      \count3=1\relax%
    \else%
      \count3=#3\relax%
    \fi%
    %
    % Store offset
    %
    \edef\pgf@@temp{#4}%
    \ifx\pgf@@temp\pgfutil@empty%
      \count8=0\relax%
    \else%
      \pgfcalendar@unpack#4%
    \fi%
    %
    %
    % 4) a = \lfloor (14-month) /12 \rfloor
    %
    \ifnum\count2<3\relax%
      \count4=1\relax%
    \else%
      \count4=0\relax%
    \fi%
    %
    % 5) y = year + 4800 - a
    %
    \count5=\count1\relax%
    \advance\count5 by 4800\relax%
    \advance\count5 by-\count4\relax%
    %
    % 6) m = month + 12a - 3
    %
    \count6=\count2\relax%
    \count0=\count4\relax%
    \multiply\count0 by12\relax
    \advance\count6 by\count0\relax%
    \advance\count6 by-3\relax%
    %
    % 7) jdn = day + \floor{(153 m+2)/5} + 365y + \floor{y/4} -
    % \floor{y/100} + \florr{y/400} - 32045
    %
    \count7=\count3\relax%
    % + \floor{(153 m+2)/5} :
    \count0=\count6\relax%
    \multiply\count0 by 153\relax%
    \advance\count0 by 2\relax%
    \divide\count0 by 5\relax%
    \advance\count7 by \count0\relax%
    % + 365y :
    \count0=\count5%
    \multiply\count0by365\relax%
    \advance\count7 by\count0\relax%
    % + \floor{y/4}
    \count0=\count5\relax%
    \divide\count0 by 4\relax%
    \advance\count7 by\count0%
    % - \floor{y/100}
    \count0=\count5\relax%
    \divide\count0 by 100\relax%
    \advance\count7 by-\count0\relax%
    % + \floor{y/400}
    \count0=\count5\relax%
    \divide\count0 by 400\relax%
    \advance\count7 by\count0%
    %  - 32045
    \advance\count7 by-32045\relax%
    %
    % Undo "last" advance
    \ifx\pgf@temp\pgfcalendar@last@text%
      \advance\count7by-1\relax%
    \fi%
    % Add offset  
    \advance\count7by\count8\relax%
    \expandafter%
  }%
  \expandafter#5\the\count7\relax%  
}
\def\pgfcalendar@last@text{last}
\def\pgfcalendar@unpack#1+{%
  \count8=#1\relax%
}

% Convert Julian day number date. 
%
% #1 = the number of Julian days
% #2 = a macro in which the year should be stored.
% #3 = a macro in which the month should be stored.
% #4 = a macro in which the day should be stored.
%
% Formula used:
%
% 1) J = Julian day number
% 2) j = J + 32044
% 3) g = j div 146097
% 4) dg = j mod 146097
% 5) c = (dg div 36524 + 1) * 3 div 4
% 6) dc = dg - c * 36524
% 7) b = dc div 1461
% 8) db = dc mod 1461
% 9) a = (db div 365 + 1) * 3 div 4
% 10)da = db - a * 365
% 11)y = g * 400 + c * 100 + b * 4 + a
% 12)m = (da * 5 + 308) div 153 - 2
% 13)d = da - (m + 4) * 153 div 5 + 122
% 14)Y = y - 4800 + (m + 2) div 12
% 15)M = (m + 2) mod 12 + 1
% 16)D = d + 1
%
% Example
%
% \pgfcalendarjuliantodate{\mynumber}{\myyear}{\mymonth}{\myday}

\def\pgfcalendarjuliantodate#1#2#3#4{%
  {%
    % 1) J = Julian day number
    \count1=#1\relax%
    % 2) j = J + 32044     
    \count2=\count1\relax%
    \advance\count2 by 32044\relax%
    % 3) g = j div 146097  
    \count3=\count2\relax%
    \divide\count3 by 146097\relax%
    % 4) dg = j mod 146097 
    \count4=\count3\relax%
    \multiply\count4 by-146097\relax%
    \advance\count4 by\count2\relax%
    % 5) c = (dg div 36524 + 1) * 3 div 4 
    \count5=\count4\relax%
    \divide\count5 by36524\relax%
    \advance\count5 by1\relax%
    \multiply\count5 by3\relax%
    \divide\count5 by4\relax%
    % 6) dc = dg - c * 36524 
    \count6=\count4\relax%
    \count0=\count5\relax%
    \multiply\count0 by-36524\relax%
    \advance\count6 by\count0\relax%
    % 7) b = dc div 1461
    \count7=\count6\relax%
    \divide\count7 by1461\relax%
    % 8) db = dc mod 1461
    \count8=\count7\relax%
    \multiply\count8 by-1461\relax%
    \advance\count8 by\count6\relax%
    % 9) a = (db div 365 + 1) * 3 div 4
    \count9=\count8\relax%
    \divide\count9 by 365\relax%
    \advance\count9 by 1\relax%
    \multiply\count9 by3\relax%
    \divide\count9 by4\relax%
    % 10)da = db - a * 365
    \count10=\count8\relax%
    \count0=\count9\relax%
    \multiply\count0 by-365\relax%
    \advance\count10 by\count0\relax%
    % 11)y = g * 400 + c * 100 + b * 4 + a
    \count11=\count3\relax%
    \multiply\count11 by400\relax%
    \count0=\count5\relax%
    \multiply\count0 by100\relax%
    \advance\count11 by\count0\relax%
    \count0=\count7\relax%
    \multiply\count0 by4\relax%
    \advance\count11 by\count0\relax%
    \advance\count11 by\count9\relax%
    % 12)m = (da * 5 + 308) div 153 - 2
    \count12=\count10\relax%
    \multiply\count12 by5\relax%
    \advance\count12 by 308\relax%
    \divide\count12 by 153\relax%
    \advance\count12 by -2\relax%
    % 13)d = - (m + 4) * 153 div 5 + 122 + da
    \count13=\count12\relax%
    \advance\count13 by 4\relax%
    \multiply\count13 by153\relax%
    \divide\count13 by5\relax%
    \count13=-\count13\relax%
    \advance\count13 by 122\relax%
    \advance\count13 by \count10\relax%
    % 14)Y =  (m + 2) div 12 + y - 4800
    \count14=\count12\relax%
    \advance\count14 by 2\relax%
    \divide\count14 by12\relax%
    \advance\count14 by\count11\relax%
    \advance\count14 by-4800\relax%
    % 15)M = (m + 2) mod 12 + 1
    \count15=\count12\relax%
    \advance\count15 by2\relax%
    \count0=\count15\relax%
    \divide\count0 by12\relax%
    \multiply\count0 by12\relax%
    \advance\count15 by-\count0\relax%
    \advance\count15 by1\relax%
    % 16)D = d + 1
    \count16=\count13%
    \advance\count16by 1\relax%    
    %
    \xdef\pgf@temp@year{\the\count14}%
    \xdef\pgf@temp@month{\ifnum\count15<10 0\fi\the\count15}%
    \xdef\pgf@temp@day{\ifnum\count16<10 0\fi\the\count16}%
  }%
  \let#2=\pgf@temp@year%
  \let#3=\pgf@temp@month%  
  \let#4=\pgf@temp@day%  
}



% Returns the day of week as a number between 0 = Monday and 6 =
% Sunday
%
% #1 = a Julian day number
% #2 = a counter into which the weekday should be put.
%
% Example:
%
% \pgfcalendardatetojulian{2006-01-10}{\mycount}
% \pgfcalendarjuliantoweekday{\mycount}{\myweekday}

\def\pgfcalendarjuliantoweekday#1#2{%
  {%
    \pgfutil@tempcnta=#1\relax%
    #2=\pgfutil@tempcnta%
    \divide#2by7\relax%
    \multiply#2by-7\relax%
    \advance#2by\pgfutil@tempcnta\relax%
    \expandafter%
  }%
  \expandafter#2\the#2\relax%
}



% Converts a day of week into a weekday name (long or short)
%
% #1 = a number representing a weekday (0=Monday)
%
% Example:
%
% \pgfcalendardatetojulian{2006-01-10}{\mycount}
% \pgfcalendarjuliantoweekday{\mycount}{\myweekday}
% October 1st, 2006 was a \pgfcalendarweekdayname{\myweekday}

\def\pgfcalendarweekdayname#1{%
  \translate{\ifcase#1Monday\or Tuesday\or Wednesday\or Thursday\or Friday\or Saturday\or Sunday\fi}%
}

\def\pgfcalendarweekdayshortname#1{%
  \translate{\ifcase#1Mon\or Tue\or Wed\or Thu\or Fri\or Sat\or Sun\fi}%
}


% Converts a month of year number into a month name (long or short)
%
% #1 = a number representing a month (1=January)
%
% Example:
%
% \pgfcalendarmonthname

\def\pgfcalendarmonthname#1{%
  \translate{\ifcase#1\or January\or February\or March\or April\or
    May\or June\or July\or August\or September\or October\or
    November\or December\fi}%
}

\def\pgfcalendarmonthshortname#1{%
  \translate{\ifcase#1\or Jan\or Feb\or Mar\or Apr\or
    May\or Jun\or Jul\or Aug\or Sep\or Oct\or
    Nov\or Dec\fi}%
}






% Macro for easy typesetting of days, etc.
%
% #1 = kind selection
% #2 = length and representation selection
%
% Description:
%
% Replaces the shorthand according to the following rules: The
% first letter of the shorthand describes the kind of
% shorthand. Possible kinds are:
%
% d = day of current date (in an invocation of \pgfcalendar)
% m = month of current date
% y = year of current date
% w = week day of current date
%
% The second parameter determines how the kind is represented:
%
% - = shortest possible numerical way (allowed only for d, m, y)
% = = same, but always of the same length (padded with blanks as
%     needed, allowed only for d, m, y)
% 0 = numerical representation for d and m padded with leading zeros.
% t = textual representation (allowed only for d, m, w)
% . = abbreviated textual representation (allowed only for d, m, w)
%
% It is adivsed that you say, for example,
% \let\%=\pgfcalendarshorthand.
%
% With this setting, you can typeset an ISO-date by saying \%y0-\%m0-\%d0.
% For another example, on 2007-02-09, which is a
% Friday, you can write "\%wt, \%mt \%d-, \%y0" to get "Friday, February 9, 2007"

\def\pgfcalendarshorthand#1#2{\csname pgfcalendar@shorthand@#1#2\endcsname}
\expandafter\def\csname pgfcalendar@shorthand@d-\endcsname{%
  {\pgfutil@tempcnta=\pgfcalendarcurrentday\relax\the\pgfutil@tempcnta}}
\expandafter\def\csname pgfcalendar@shorthand@d=\endcsname{%
  {\pgfutil@tempcnta=\pgfcalendarcurrentday\relax\ifnum\pgfutil@tempcnta<10\relax\setbox0=\hbox{1}\kern\wd0\relax\fi\the\pgfutil@tempcnta}}
\expandafter\def\csname pgfcalendar@shorthand@d0\endcsname{%
  \pgfcalendarcurrentday}
\expandafter\def\csname pgfcalendar@shorthand@m-\endcsname{%
  {\pgfutil@tempcnta=\pgfcalendarcurrentmonth\relax\the\pgfutil@tempcnta}}
\expandafter\def\csname pgfcalendar@shorthand@m=\endcsname{%
  {\pgfutil@tempcnta=\pgfcalendarcurrentmonth\relax\ifnum\pgfutil@tempcnta<10\relax\setbox0=\hbox{1}\kern\wd0\relax\fi\the\pgfutil@tempcnta}}
\expandafter\def\csname pgfcalendar@shorthand@m0\endcsname{%
  \pgfcalendarcurrentmonth}
\expandafter\def\csname pgfcalendar@shorthand@y-\endcsname{%
  \pgfcalendarcurrentyear}
\expandafter\def\csname pgfcalendar@shorthand@y=\endcsname{%
  \pgfcalendarcurrentyear}
\expandafter\def\csname pgfcalendar@shorthand@y0\endcsname{%
  \pgfcalendarcurrentyear}
\expandafter\def\csname pgfcalendar@shorthand@w.\endcsname{%
  \pgfcalendarweekdayshortname{\pgfcalendarcurrentweekday}}
\expandafter\def\csname pgfcalendar@shorthand@wt\endcsname{%
  \pgfcalendarweekdayname{\pgfcalendarcurrentweekday}}
\expandafter\def\csname pgfcalendar@shorthand@m.\endcsname{%
  \pgfcalendarmonthshortname{\pgfcalendarcurrentmonth}}
\expandafter\def\csname pgfcalendar@shorthand@mt\endcsname{%
  \pgfcalendarmonthname{\pgfcalendarcurrentmonth}}


\endinput


==> pgfcalendar.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\edef\pgfcalendaratcode{\the\catcode`\@}
\catcode`\@=11

\input pgfrcs.tex
\input pgfcalendar.code.tex

\catcode`\@=\pgfcalendaratcode

\endinput


==> pgfcore.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcore.code.tex,v 1.6 2008/01/15 10:27:34 tantau Exp $

\newif\ifpgf@draftmode

\input pgfmath.code.tex

\input pgfcorepoints.code.tex
\input pgfcorepathconstruct.code.tex
\input pgfcorepathusage.code.tex
\input pgfcorescopes.code.tex
\input pgfcoregraphicstate.code.tex
\input pgfcoretransformations.code.tex
\input pgfcorequick.code.tex
\input pgfcoreobjects.code.tex
\input pgfcorepathprocessing.code.tex
\input pgfcorearrows.code.tex
\input pgfcoreshade.code.tex
\input pgfcoreimage.code.tex
\input pgfcorelayers.code.tex
\input pgfcoretransparency.code.tex
\input pgfcorepatterns.code.tex

\endinput


==> pgfcore.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\ifx\pgfcoreincluded\undefined
\def\pgfcoreincluded{}

\edef\pgfcoreatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfsys.tex
\input pgfcore.code.tex
\catcode`\@=\pgfcoreatcode

\fi

\endinput


==> pgfcorearrows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorearrows.code.tex,v 1.8 2007/06/07 07:41:10 tantau Exp $


% Sets the end arrow
%
% #1 = An arrow name
%
% Example:
%
% \pgfsetarrowsend{stealth}

\def\pgfsetarrowsend#1{\pgf@arrowset{end}{#1}}
\def\pgf@arrowset#1#2{%
  \pgfutil@ifundefined{pgf@arrow@code@#2}
  {\PackageError{pgf}{Arrow #1 type ``#2'' unknown}{}}
  {%
    \edef\pgf@arrow@temp{#2}%
    \ifx\pgf@arrow@temp\pgfutil@empty% ah. clear!
      \expandafter\let\csname pgf@#1arrow\endcsname=\pgfutil@empty%
      \expandafter\let\csname pgf@shorten@#1\endcsname=\pgfutil@empty%
    \else%
      %\pgf@arrow@prepare{#2}%
      \expandafter\def\csname pgf@#1arrow\endcsname{\pgf@arrow@call{#2}}%
      \expandafter\edef\csname pgf@shorten@#1\endcsname{\expandafter\noexpand\csname pgf@arrow@right@#2\endcsname}%
    \fi%
  }%
}


% Sets the start arrow
%
% #1 = An arrow name
%
% Example:
%
% \pgfsetarrowsstart{stealth}

\def\pgfsetarrowsstart#1{\pgf@arrowset{start}{\csname pgf@arrows@invert#1\endcsname}}

\def\pgf@arrows@invname#1#2{\expandafter\def\csname pgf@arrows@invert#1\endcsname{#2}}
\pgf@arrows@invname{}{}




% Sets arrows
%
% #1 = An arrow specification of the form ``left''-``right''. The last
%      and right should be arrow types that have been defined using
%      the \pgfarrowsdef command
%
% Example:
%
% \pgfsetarrows{-to}

\def\pgfsetarrows#1{\pgf@arrows#1\pgf@stop}
\def\pgf@arrows#1-#2\pgf@stop{%
  \pgfsetarrowsstart{#1}
  \pgfsetarrowsend{#2}
}

\def\pgf@arrows@checked#1#2#3{%
  \pgfutil@ifundefined{pgf@arrow@code@#2}%
  {%
    \PackageError{pgf}{Arrow end type ``#2'' unknown}{}}%
  {%
    \pgfutil@ifundefined{pgf@arrow@code@\csname pgf@arrows@invert#1\endcsname}
    {\PackageError{pgf}{Arrow start type ``#1'' unknown}{}}%
    {#3}%
  }%
}

\def\pgf@arrows@check@already#1#2#3{%
  \pgfutil@ifundefined{pgf@arrow@code@#2}
  {#3}%
  {\PackageError{pgf}{Arrow end type ``#2'' already defined}{}}%
}


% Called when an arrow needs to be rendered

\def\pgf@arrow@call#1{%
  \expandafter\ifx\csname pgf@arrow@prot@#1@\the\pgflinewidth\endcsname\relax%
    \pgfsysprotocol@getcurrentprotocol\pgf@arrow@temp%
    {%
      \pgfinterruptpath%
        \let\pgfusepath=\pgf@nousepath@here%
        \pgf@relevantforpicturesizefalse%
        \pgftransformreset%
        \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
        \pgfsysprotocol@bufferedtrue%
        \pgfsys@beginscope%
        \csname pgf@arrow@code@#1\endcsname%
        \pgfsys@endscope%
        \pgfsysprotocol@getcurrentprotocol\pgf@@arrow@temp%
        \global\let\pgf@@arrow@temp=\pgf@@arrow@temp%
      \endpgfinterruptpath%
      \expandafter\def\expandafter\pgf@temp\expandafter{\expandafter\pgfsys@invoke\expandafter{\pgf@@arrow@temp}}%
      \expandafter\global\expandafter\let\csname pgf@arrow@prot@#1@\the\pgflinewidth\endcsname=\pgf@temp%
    }%
    \pgfsysprotocol@setcurrentprotocol\pgf@arrow@temp%
  \fi%
  \csname pgf@arrow@prot@#1@\the\pgflinewidth\endcsname%
} 

\def\pgf@arrow@code@{} % dummy

\def\pgf@nousepath@here#1{%
  \PackageError{pgf}{The definition of an arrow may not use \string\pgfusepath}{}
}



% Define an arrow type.
%
% #1 = name or mnemonic for arrow when used at the start (examples: ``to'' or ``<'')
% #2 = name or mnemonic for arrow when used at the end (examples: ``to'' or ``>'')
% #3 = code to setup the left and right extend of the arrow. To set
%      the left extend, call \pgfarrowsleftextend, for the right \pgfarrowsrightextend.
% #4 = protocolable code
%
% Description:
%
% When you define an arrow using this command, you must give two
% names. The first is used for the arrow when it is ``at the start'',
% the other when it is at the end. For example, a simple arrow might
% have the names ``<'' and ``>'', though these particular names are
% not used by pgf and left for the user.
%
% The code should be ``protocolable'' code. This means that it uses
% only pretty simple commands. 
%
% The arrow code will be protocolled once for each line width at which
% the arrow is used. Thus, the code can (and often should) depend on
% the line width.
%
% The arrow should ``point right'' in the coordinate system. The end
% of the line at which the arrow should be drawn will be at the origin
% of the coordinate system. The coordinate system will be scaled and
% rotated appropriately before the arrow is drawn.
%
% The right extend of the arrow should be set to how much the arrow
% ``protrudes over the right''. Prior to drawing the arrow, the line
% will be shortened by this amount so that the arrow tip will exactly
% touch the original right end of the unshortened line.
%
% The left extend specifies the leftmost point of the arrow. This is
% important only if you use the swapping command, when this end is
% used to compute the shortening. 
%
% The definition of an arrow should normally take care of the fact
% that the line cap of the main line may be a butt cap, a round cap or
% a rect cap. In all cases, the arrow should ``cover'' the cap
% completely or not at all.
%
% Example:
%
% \pgfarrowsdeclare{stealth}{stealth}
% {
%   \pgfarrowsleftextend{-6\pgflinewidth}
%   \pgfarrowsrightextend{2\pgflinewidth}
% {
%   \pgfpathmoveto{\pgfpoint{2\pgflinewidth}{0pt}}
%   \pgfpathlineto{\pgfpoint{-6\pgflinewidth}{4\pgflinewidth}}
%   \pgfpathlineto{\pgfpoint{-3\pgflinewidth}{0pt}}
%   \pgfpathlineto{\pgfpoint{-6\pgflinewidth}{-4\pgflinewidth}}
%   \pgfusepathqfill
% }

\def\pgfarrowsdeclare#1#2#3#4{%
  \pgf@arrows@check@already{#1}{#2}
  {%
    \expandafter\def\csname pgf@arrow@code@#2\endcsname{#4}%
    \expandafter\def\csname pgf@arrow@left@#2\endcsname{#3\advance\pgf@x by-\pgf@xa}%
    \expandafter\def\csname pgf@arrow@right@#2\endcsname{#3\advance\pgf@x by\pgf@xb}%
    \pgf@arrows@invname{#1}{#2}%
  }%
}

\def\pgfarrowsleftextend#1{\pgfmathsetlength\pgf@xa{#1}}
\def\pgfarrowsrightextend#1{\pgfmathsetlength\pgf@xb{#1}}

\def\pgf@arrows@repeat#1#2{%
  \edef\pgf@arrows@marshal{\noexpand\let\expandafter\noexpand\csname#2\endcsname=\expandafter\noexpand\csname#1\endcsname}%
  \pgf@arrows@marshal}



% Declare a new arrow type to be the same as another one.
%
% #1 = name of new start
% #2 = name or new end
% #3 = name or old start
% #4 = name or old end
%
% Example:
%
% \pgfarrowsdeclarealias{<}{>}{to}{to}

\def\pgfarrowsdeclarealias#1#2#3#4{%
  \pgf@arrows@check@already{#1}{#2}
  {%
    \pgf@arrows@checked{#3}{#4}%
    {%
      \pgf@arrows@repeat{pgf@arrow@code@#4}{pgf@arrow@code@#2}%
      \pgf@arrows@repeat{pgf@arrow@left@#4}{pgf@arrow@left@#2}%
      \pgf@arrows@repeat{pgf@arrow@right@#4}{pgf@arrow@right@#2}%
      \pgf@arrows@invname{#1}{#2}%
    }%
  }%
}




% Creates a new arrows by ``swapping'' an existing arrow.
%
% #1 = name of new start
% #2 = name of new end
% #3 = name of old start
% #4 = name of old end
%
% Example:
%
% \pgfarrowsdeclarealias{]}{[}{[}{]}

\def\pgfarrowsdeclarereversed#1#2#3#4{%
  \pgf@arrows@check@already{#1}{#2}%
  {%
    \pgf@arrows@checked{#3}{#4}%
    {%
      \expandafter\def\csname pgf@arrow@code@#2\endcsname{%
        \pgflowlevel{\pgftransformxscale{-1}}%
        \csname pgf@arrow@code@#4\endcsname}%
      \pgf@arrows@repeat{pgf@arrow@right@#4}{pgf@arrow@left@#2}%
      \pgf@arrows@repeat{pgf@arrow@left@#4}{pgf@arrow@right@#2}%
      \pgf@arrows@invname{#1}{#2}%
    }%
  }%
}



% Creates new arrows by combining two existing arrows.
%
% #1 = optional additional space
% #2 = name of new start
% #3 = name of new end
% #4 = name of second (innermost) start
% #5 = name of second end
% #6 = name of first (outermost) start
% #7 = name of first end
%
% In the star form, the line will end at the innermost arrows,
% otherwise the line will end at the outermost arrows.
%
% Example:
%
% \pgfarrowsdeclarecombine*{|<}{>|}{|}{|}{<}{>}
% \pgfarrowsdeclarecombine{<<}{>>}{<}{>}{<}{>}

\def\pgfarrowsdeclarecombine{\pgfutil@ifnextchar*{\pgfarrowsdeclarecombine@star}{\pgf@@arrowsdeclarecombine}}

\def\pgf@@arrowsdeclarecombine{\pgfutil@ifnextchar[{\pgf@arrowsdeclarecombine}{\pgf@arrowsdeclarecombine[0pt]}}
\def\pgf@arrowsdeclarecombine[#1]#2#3#4#5#6#7{%
  \pgf@arrows@check@already{#2}{#3}%
  {%
    \pgf@arrows@checked{#4}{#5}%
    {%
      \pgf@arrows@checked{#6}{#7}%
      {%
        \expandafter\edef\csname pgf@arrow@code@#3\endcsname{%
          \noexpand\pgfscope%
          {\expandafter\noexpand\csname pgf@arrow@code@#7\endcsname}%
          \noexpand\endpgfscope%
          {%
            \noexpand\pgfmathsetlength\pgf@x{#1}%
            \noexpand\pgf@process{\expandafter\noexpand\csname pgf@arrow@left@#7\endcsname}%
            \noexpand\pgf@process{\expandafter\noexpand\csname pgf@arrow@right@#5\endcsname}%
            \pgf@x=-\pgf@x%
            \noexpand\pgflowlevel{\noexpand\pgftransformxshift{\pgf@x}}%
            \expandafter\noexpand\csname pgf@arrow@code@#5\endcsname}%
          }%
        \pgf@arrows@repeat{pgf@arrow@right@#7}{pgf@arrow@right@#3}%
        \expandafter\def\csname pgf@arrow@left@#3\endcsname{%
          \pgf@process{%
            \pgfmathsetlength\pgf@y{#1}%
            \advance\pgf@x by\pgf@y%
            \pgf@process{\csname pgf@arrow@left@#7\endcsname}%
            \pgf@process{\csname pgf@arrow@right@#5\endcsname}%
            \pgf@process{\csname pgf@arrow@left@#5\endcsname}%
          }%
        }%
        \pgf@arrows@invname{#2}{#3}%
      }%
    }%
  }%
}

\def\pgfarrowsdeclarecombine@star*{\pgfutil@ifnextchar[{\pgf@arrowsdeclarecombine@star}{\pgf@arrowsdeclarecombine@star[0pt]}}
\def\pgf@arrowsdeclarecombine@star[#1]#2#3#4#5#6#7{%
  \pgf@arrows@check@already{#2}{#3}%
  {%
    \pgf@arrows@checked{#4}{#5}%
    {%
      \pgf@arrows@checked{#6}{#7}%
      {%
        \expandafter\edef\csname pgf@arrow@code@#3\endcsname{%
          \noexpand\pgfscope%
            {%
              \noexpand\pgfmathsetlength\pgf@x{#1}%
              \pgf@process{\expandafter\noexpand\csname pgf@arrow@left@#7\endcsname}%
              \pgf@process{\expandafter\noexpand\csname pgf@arrow@right@#5\endcsname}%
              \noexpand\pgflowlevel{\noexpand\pgftransformxshift{\pgf@x}}%
            }%
            {\expandafter\noexpand\csname pgf@arrow@code@#7\endcsname}%
          \noexpand\endpgfscope%
          \expandafter\noexpand\csname pgf@arrow@code@#5\endcsname%
        }%
        \pgf@arrows@repeat{pgf@arrow@left@#7}{pgf@arrow@left@#3}%
        \expandafter\def\csname pgf@arrow@right@#3\endcsname{%
          \pgf@process{%
            \pgfmathsetlength\pgf@y{#1}%
            \advance\pgf@x by\pgf@y%
            \pgf@process{\csname pgf@arrow@left@#7\endcsname}%
            \pgf@process{\csname pgf@arrow@right@#5\endcsname}%
            \pgf@process{\csname pgf@arrow@right@#7\endcsname}%
          }%
        }%
        \pgf@arrows@invname{#2}{#3}%
      }%
    }%
  }%
}



% Creates new arrows by doubling/tripling existing arrows.
%
% #1 = optional additional space in multiples of line width
% #2 = name of new start
% #3 = name of new end
% #4 = name of old start
% #5 = name of old end
%
% Example:
%
% \pgfarrowsdeclaredouble{<<}{>>}{<}{>}

\def\pgfarrowsdeclaredouble{\pgfutil@ifnextchar[{\pgf@arrowsdeclaredouble}{\pgf@arrowsdeclaredouble[0pt]}}
\def\pgf@arrowsdeclaredouble[#1]#2#3#4#5{\pgfarrowsdeclarecombine[#1]{#2}{#3}{#4}{#5}{#4}{#5}}
\def\pgfarrowsdeclaretriple{\pgfutil@ifnextchar[{\pgf@arrowsdeclaretriple}{\pgf@arrowsdeclaretriple[0pt]}}
\def\pgf@arrowsdeclaretriple[#1]#2#3#4#5{%
  \pgfarrowsdeclarecombine[#1]{pgf@trip@#2}{pgf@trip@#3}{#4}{#5}{#4}{#5}%
  \pgfarrowsdeclarecombine[#1]{#2}{#3}{pgf@trip@#2}{pgf@trip@#3}{#4}{#5}%
}


% A stealth-fighter-like pointed arrow
%
% Example:
%
% \pgfsetarrows{-stealth}

\pgfarrowsdeclare{stealth}{stealth}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-3\pgfutil@tempdima}
  \pgfarrowsrightextend{+5\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfqpoint{5\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqfill
}

\pgfarrowsdeclarereversed{stealth reversed}{stealth reversed}{stealth}{stealth}


% An arrow similar to the $\to$ arrow
%
% Example:
%
% \pgfsetarrow{-to}

\pgfarrowsdeclare{to}{to}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
  {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
  {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
  {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
  {\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}

\pgfarrowsdeclare{to reversed}{to reversed}
{
  \pgfutil@tempdima=-0.21pt%
  \advance\pgfutil@tempdima by-0.475\pgflinewidth%
  \pgfutil@tempdimb=0.98pt%
  \advance\pgfutil@tempdimb by1.45\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{+0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{3.5\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{3.25\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{0.25\pgfutil@tempdima}}
  {\pgfqpoint{-0.25\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{0.5\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}
  {\pgfqpoint{3.25\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
  {\pgfqpoint{3.5\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfusepathqstroke
}



% LaTeX's orginal arrow type
%
% Example:
%
% \pgfsetarrows{-latex}

\pgfarrowsdeclare{latex}{latex}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-1\pgfutil@tempdima}
  \pgfarrowsrightextend{+9\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{6.3333\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{2\pgfutil@tempdima}{2\pgfutil@tempdima}}
  {\pgfqpoint{-1\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-1\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{2\pgfutil@tempdima}{-2\pgfutil@tempdima}}
  {\pgfqpoint{6.3333\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{9\pgfutil@tempdima}{0pt}}
  \pgfusepathqfill
}
\pgfarrowsdeclarereversed{latex reversed}{latex reversed}{latex}{latex}



% A bar shaped arrow
%
% Example:
%
% \pgfsetarrows{-|}

\pgfarrowsdeclare{|}{|}
{
  \pgfarrowsleftextend{+-0.25\pgflinewidth}
  \pgfarrowsrightextend{+.75\pgflinewidth}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetrectcap
  \pgfpathmoveto{\pgfqpoint{0.25\pgflinewidth}{-\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.25\pgflinewidth}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}



\endinput


==> pgfcoregraphicstate.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoregraphicstate.code.tex,v 1.8 2007/12/12 16:57:17 tantau Exp $

% Globals

\newdimen\pgflinewidth


% Set the line width to #1.
% 
% #1 = new line width.
% 
% Example:
%
% \pgfsetlinewidth{3pt}

\def\pgfsetlinewidth#1{%
  \pgfmathsetlength\pgflinewidth{#1}%
  \global\pgflinewidth=\pgflinewidth%
  \pgfsys@setlinewidth{\the\pgflinewidth}%
  \ignorespaces}


% Set the miter limit to #1.
% 
% #1 = new miter limit factor.
% 
% Example:
%
% \pgfsetmiterlimit{3}

\def\pgfsetmiterlimit#1{%
  \pgfsys@setmiterlimit{#1}%
  \ignorespaces}


% Set the dash pattern to #1 with phase #2/
% 
% #1 = a row of numbers of length of ``on'' and ``off'' points.
% #2 = a phase
% 
% Example:
%
% \pgfsetdash{}          {0pt} % solid line
% \pgfsetdash{{.1cm}}    {0pt} % long dashes
% \pgfsetdash{{1pt}{1ex}}{0pt} % dotted

\def\pgfsetdash#1#2{%
  \def\pgf@temp{}%
  \def\pgf@next{\pgf@strip}%
  \pgf@strip#1{pgf@stop}%
  \pgfmathsetlength\pgf@x{#2}%
  \pgfsys@setdash{\pgf@temp}{\the\pgf@x}%
  \ignorespaces}

\def\pgf@strip#1{%
  \def\pgf@@temp{#1}%
  \ifx\pgf@@temp\pgf@stop%
    \let\pgf@next=\relax%
  \else%
    \pgfmathsetlength\pgf@x{#1}%
    \ifx\pgf@temp\pgfutil@empty%
      \edef\pgf@temp{\the\pgf@x}%
    \else%
      \edef\pgf@temp{\pgf@temp,\the\pgf@x}%
    \fi%
  \fi\pgf@next}

\def\pgf@stop{pgf@stop}


% Set color of strokes. This will overrule the normal color.
% 
% Example:
%
% \pgfsetstrokecolor{red}

\def\pgfsetstrokecolor#1{%
  \pgfutil@colorlet{pgf@tempcolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
  \expandafter\expandafter\expandafter\pgf@setstrokecolor\csname\string\color@pgf@tempcolor\endcsname%
}
\def\pgf@setstrokecolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4@stroke\endcsname\relax%
    \PackageError{pgfbase}{Unsupported color model `#4'. Sorry}{}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4@stroke\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}

\def\pgf@uncomma#1,{%
  \def\pgf@coltest{#1}%
  \ifx\pgf@coltest\pgfutil@empty%
    \let\pgf@colnext=\relax%
  \else%
    \expandafter\def\expandafter\pgf@colmarshal\expandafter{\pgf@colmarshal{#1}}%
    \let\pgf@colnext=\pgf@uncomma%
  \fi%
  \pgf@colnext%  
}


% Set color of fills. This will overrule the normal color.
% 
% Example:
%
% \pgfsetfillcolor{gray}

\def\pgfsetfillcolor#1{%
  \pgfutil@colorlet{pgf@tempcolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
  \expandafter\expandafter\expandafter\pgf@setfillcolor\csname\string\color@pgf@tempcolor\endcsname%
}
\def\pgf@setfillcolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4@fill\endcsname\relax%
    \PackageError{pgfbase}{Unsupported color model `#4'. Sorry}{}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4@fill\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}



% Sets both the stroke and fill color.
% 
% Example:
%
% \pgfsetcolor{blue}

\def\pgfsetcolor#1{%
  \pgfutil@colorlet{pgf@tempcolor}{#1}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
  \expandafter\expandafter\expandafter\pgf@setcolor\csname\string\color@pgf@tempcolor\endcsname%
}
\def\pgf@setcolor#1#2#3#4#5{%
  \expandafter\ifx\csname pgfsys@color@#4\endcsname\relax%
    \PackageError{pgfbase}{Unsupported color model `#4'. Sorry}{}%
  \else%
    \edef\pgf@colmarshal{\expandafter\noexpand\csname pgfsys@color@#4\endcsname}%
    \pgf@uncomma#5,,%
    \pgf@colmarshal%
  \fi}

% Code for ensuring the stroke/fill colors are correctly reset.
\def\XC@bcolor{\pgfsys@color@reset}

% Set a butt line cap.
% 
% Example:
%
% \pgfsetbuttcap

\def\pgfsetbuttcap{\pgfsys@buttcap\ignorespaces}


% Set a round line cap.
% 
% Example:
%
% \pgfsetroundcap

\def\pgfsetroundcap{\pgfsys@roundcap\ignorespaces}


% Set a rectangular line cap.
% 
% Example:
%
% \pgfsetrectcap

\def\pgfsetrectcap{\pgfsys@rectcap\ignorespaces}


% Set a miter line join.
% 
% Example:
%
% \pgfsetmiterjoin

\def\pgfsetmiterjoin{\pgfsys@miterjoin\ignorespaces}


% Set a bevel line join.
% 
% Example:
%
% \pgfsetbeveljoin

\def\pgfsetbeveljoin{\pgfsys@beveljoin\ignorespaces}


% Set a round line join.
% 
% Example:
%
% \pgfsetroundjoin

\def\pgfsetroundjoin{\pgfsys@roundjoin\ignorespaces}


% Sets the even-odd rule for filling and clipping.
% 
% Example:
%
% \pgfseteorule

\def\pgfseteorule{\pgfsys@eoruletrue\ignorespaces}


% Sets the non-zero winding number rule for filling and clipping.
% 
% Example:
%
% \pgfsetnonzerorule

\def\pgfsetnonzerorule{\pgfsys@eorulefalse\ignorespaces}



\endinput


==> pgfcoreimage.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoreimage.code.tex,v 1.1 2008/01/15 10:27:34 tantau Exp $



% Declare an image
%
% #1 = optional argument: width, height, page specification
% #2 = name of the image for later use
% #4 = filename without extension, automatic extensions are .pdf,
%      .jpg, and .png for PDF and .ps, .eps, .epsi for postscript.
%
% Description:
%
% This command declares an image file for later use. Even if the image
% is used several times in the document, in PDF it will only be stored
% once. 
%
% Example:
%
% \pgfdeclareimage[width=2cm,page=2]{myimage}{imagefilename}

\def\pgfdeclareimage{\pgfutil@ifnextchar[{\pgf@declareimage}{\pgf@declareimage[]}}
\def\pgf@declareimage[#1]#2#3{%
  \pgfqkeys{/pgf/images}{height=,width=,page=,interpolate=false,mask=,#1}%
  % Try to find the file
  \gdef\pgf@filename{}%
  % If page= parameter is not empty, try that file first:
  \ifx\pgf@imagepage\pgfutil@empty%
  \else%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3.page\pgf@imagepage}%
  \fi%
  \ifx\pgf@filename\pgfutil@empty%
    \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3}%
  \else%
    \pgfkeys{/pgf/images/page=}% make page empty     
  \fi%
  \ifx\pgf@filename\pgfutil@empty%
    \PackageWarning{pgf}%
    {File "#3" not found when defining image "#2".\MessageBreak
      Tried all extensions in "\pgfsys@imagesuffixlist"}%
    \pgf@declaredraftimage{#2}%
  \else%
    \ifpgf@draftmode%
      \pgf@declaredraftimage{#2}%
    \else%
      \pgfsys@defineimage%
    \fi%
  \fi%
  \expandafter\global\expandafter\let\csname pgf@image@#2!\endcsname=\pgf@image%
}

\pgfkeys{/pgf/images/width/.estore in=\pgf@imagewidth}
\pgfkeys{/pgf/images/height/.estore in=\pgf@imageheight}
\pgfkeys{/pgf/images/page/.estore in=\pgf@imagepage}
\pgfkeys{/pgf/images/interpolate/.cd,.code=\edef\pgf@imageinterpolate{/Interpolate #1},.default=true}
\pgfkeys{/pgf/images/mask/.code=%
  {%
    \edef\pgf@imagemask{#1}%
    \ifx\pgf@imagemask\pgfutil@empty%
    \else%
      \pgfutil@ifundefined{pgf@mask@#1}%
      {\PackageError{pgf}{Undefined mask "#1".}{}%
        \edef\pgf@imagemask{}}%
      {\edef\pgf@imagemask{\csname pgf@mask@#1\endcsname}%
        \ifx\pgf@imagemask\pgfutil@empty%
        \else
          \edef\pgf@imagemask{/SMask \pgf@imagemask\space 0 R}%
        \fi%
      }%
    \fi%
  }}


\def\pgf@findfile#1:#2+#3{%
  \pgfutil@IfFileExists{#3#1}%
  {\xdef\pgf@filename{#3#1}}%
  {\def\pgf@mightbeempty{#2}%
    \ifx\pgf@mightbeempty\pgfutil@empty\else%
    \pgf@findfile#2+{#3}%
    \fi}}

\def\pgf@declaredraftimage#1{%
  \ifx\pgf@imagewidth\pgfutil@empty%
    \PackageWarning{pgf}{Missing width for image "#1" in draft mode.\MessageBreak  Using 1cm instead}%
    \edef\pgf@imagewidth{1cm}%
  \fi%
  \ifx\pgf@imageheight\pgfutil@empty%
    \PackageWarning{pgf}{Missing height for image "#1" in draft mode.\MessageBreak Using 1cm instead}%
    \edef\pgf@imageheight{1cm}%
  \fi%  
  \ifx\pgf@imagepage\pgfutil@empty\else\edef\pgf@imagepagetext{ page \pgf@imagepage}\fi%
  \edef\pgf@image{%
    \hbox to \pgf@imagewidth{%
      \vrule\kern-0.4pt%
      \vbox to \pgf@imageheight{%
        \hrule\vfil%
        \hbox to \pgf@imagewidth{\hskip-10cm\hfil\noexpand\tiny#1\pgf@imagepage\hfil\hskip-10cm}%
        \vfil\hrule}%
      \kern-0.4pt\vrule}%
  }%
}



% Declare a soft mask
%
% #1 = optional argument: matte specification. default matte is
%      white. 
% #2 = name of the mask for later use
% #3 = filename without extension, automatic extensions are .pdf,
%      .jpg, and .png for PDF. Postscript is not supported.
%
% Description:
%
% This command declares a soft mask for later masking an image. The
% declared mask should be used together with an image of exactly the
% same height/width if matte is defined. Matte should be the
% preblended background color (see pdf spec for details).
%
% Example:
%
% \pgfdeclaremask[matte=white]{maskname}{maskfilename}
% \pgfdeclareimage[mask=maskname]{image}{imagefilename}

\def\pgfdeclaremask{\pgfutil@ifnextchar[\pgf@declaremask{\pgf@declaremask[]}}
\def\pgf@declaremask[#1]#2#3{%
  \pgfqkeys{/pgf/images/mask}{matte={1 1 1},#1}% defaults
  \def\pgf@mask{}%
  % Try to find the file
  \gdef\pgf@filename{}%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#3}%
  \ifx\pgf@filename\pgfutil@empty%
    \PackageWarning{pgf}%
    {File "#3" not found when defining mask "#2".\MessageBreak
      Tried all extensions in "\pgfsys@imagesuffixlist"}%
  \else%
    \pgfsys@definemask%
  \fi%
  \expandafter\global\expandafter\let\csname pgf@mask@#2\endcsname=\pgf@mask%
}

\pgfkeys{/pgf/images/mask/matte/.cd,.estore in=\pgf@maskmatte,.value required}



% Create an alias name for an image
%
% #1 = name of the alias
% #2 = name of the original
%
% Example:
%
% \pgfdeclareimage{image}{1cm}{1cm}{filename
% \pgfaliasimage{alias}{image}
% \pgfuseimage{alias}

\def\pgfaliasimage#1#2{%
  \expandafter\global\expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@image@#2!\endcsname%
  \expandafter\global\expandafter\let\csname pgf@image@#1!\endcsname=\pgf@temp%
  }

  
% Use an image
%
% #1 = name of a previously declared image
%
% Example:
%
% \pgfputat{\pgforigin}{\pgfbox[left,base]{\pgfuseimage{myimage}}}

\def\pgfuseimage#1{%
  \def\pgf@imagename{pgf@image@#1}%
  \pgf@tryextensions{\pgf@imagename}{\pgfalternateextension}%
  \expandafter\pgfutil@ifundefined\expandafter{\pgf@imagename}%
  {\PackageError{pgf}{Undefined image "#1"}{}}%
  {{\leavevmode\csname\pgf@imagename\endcsname}}}

\def\pgf@tryextensions#1#2{%
  \edef\pgf@args{[#2!]}\expandafter\pgf@@tryextensions\pgf@args{#1}}
\def\pgf@@tryextensions[#1!#2]#3{%
  \expandafter\pgfutil@ifundefined\expandafter{#3#1!#2}%
  {\def\pgf@temp{#2}%
    \ifx\pgf@temp\pgfutil@empty%
    \edef#3{#3!}%
    \else%
    \pgf@@tryextensions[#2]{#3}%
    \fi}%
  {\edef#3{#3#1!#2}}}


% Alternate image
%
% Description:
%
% When an image is used, pgf first attempts to use the image with the
% alternate extension added. If this fails, the original image is
% used. If the alternate extension contains ``!'', then the text up to
% the ! is successively removed and the remainder is tried as an
% alternate extension.
%
% Example:
%
% \def\pgfalternateextension{20!white}

\def\pgfalternateextension{}



% Directly insert an image
%
% #1 = optional argument: width, height, page specification
% #2 = file name
%
% Description:
%
% Directly inserts an image without declaration. You can, however,
% still access this image using the name pgflastimage. By using
% pgfaliasimage, you can also save this image for later.
%
% Example:
%
% \pgfimage[height=2cm]{filename}

\def\pgfimage{\pgfutil@ifnextchar[\pgf@imagecom{\pgf@imagecom[]}}
\def\pgf@imagecom[#1]#2{%
  \pgfdeclareimage[#1]{pgflastimage}{#2}%
  \pgfuseimage{pgflastimage}}








% The external read/write mechanism is used as follows:
%
% In your document, you put a number or all of your pgfpicture (or
% tikzpicture) environments inside a pair of \beginpgfexternal and
% \endpgfexternal. The \beginpgfexternal gets one parameter called the
% graphics name.
%
% Once this is done, the next step is to declare the names of your
% graphics in the document at the beginning using the
% \pgfdeclaregraphicname command.
%
% Now, when you typeset your document, each time a \beginpgfexternal
% command is encountered, it will be checked whether the corresponding
% graphics file exists. If this is the case, it will be included and
% the code between \beginpgfexternal and \endpgfexternal is
% ignored. Otherwise, the code is executed normally.
%
% Things change when you run tex on your file with the \jobname set to
% the name of a decalred graphics name. In this case, only your
% graphic will be typeset, the rest of the document will be "thrown away". 
% To be more precise, everything is gobbled up to the beginning
% of the first \beginpgfexternal with the given graphics name. Then,
% the content of the "environment" is put in a box (this "environment"
% need not contain a graphics, it may contain anything that can be put
% in a box). Then a single page is output whose size is exactly the
% size of the picture.
%
% So, once you have run tex repeatedly, each time with the jobname set
% to each of the graphics, you can then run tex on the whole document
% and this will cause all graphics to be included rather than begin
% typeset.
%
% Finally, once all the graphics have been created, you can also say
% \input pgfexternal.tex instead of including pgf/TikZ.



% Tells pgf which jobname is the name of the real file
%
% #1 = name
%
% Description:
%
% This command is used to tell pgf that the file named #1 should be
% typeset normally. If \jobname is not equal to #1, only
% the graphic called \jobname will be typeset. 
%
% Example:
%
% \pgfrealjobname{survey}

\def\pgfrealjobname#1{%
  \edef\pgf@tempa{\expandafter\string\csname #1\endcsname}%
  \edef\pgf@tempb{\expandafter\string\csname\jobname\endcsname}%
  \ifx\pgf@tempa\pgf@tempb%
  \else%
    \pgf@external@grabshipouttrue%
  \fi%
}


\newif\ifpgf@external@grabshipout
\newbox\pgfexternal@startupbox

\AtBeginDocument{%
  \ifpgf@external@grabshipout%
    \global\let\pgfexternal@originalshipout=\shipout%
    \global\def\shipout{\setbox\pgfpic=}%
    \maxdeadcycles=10000%
    % Ok, gather everything we have seen up to now in a box. This box
    % will contain any specials that have been used.
    {%
      \output{\global\setbox\pgfexternal@startupbox=\vbox{\csname @begindvi\endcsname\unvbox255}}%
      \hbox{}\eject%
    }%
  \fi%
}


% "Environment" for an external graphic.
%
% #1 = graphic name
%
% Example:
%
% \beginpgfgraphicnamed{main-graphic2}
%   \begin{tikzpicture}
%     ...
%   \end{tikzpicture}
% \endpgfgraphicnamed

\def\pgf@externalbegin#1{%
  % First, check whether we wish to grab this graphic:
  \let\pgf@next=\pgf@external@normal%
  \ifpgf@external@grabshipout%
    \edef\pgf@tempa{\expandafter\string\csname #1\endcsname}%
    \edef\pgf@tempb{\expandafter\string\csname\jobname\endcsname}%
    \ifx\pgf@tempa\pgf@tempb%
      \let\pgf@next=\pgf@external@grab%
    \fi%
  \fi%
  \pgf@next{#1}%
}


\AtBeginDocument{
  \let\beginpgfgraphicnamed=\pgf@externalbegin% overwrite definition of pgfexternal.tex if necessary   
  \let\endpgfgraphicnamed=\unskip
}


% Normal operation: Include an external graphic instead of the
% picture, if such an external picture exists.
\def\pgf@external@normal#1{%
  \let\pgf@filename=\pgfutil@empty%
  \expandafter\pgf@findfile\pgfsys@imagesuffixlist:+{#1}%
  \ifx\pgf@filename\pgfutil@empty%
    % Ok, no such image... Just typeset the picture normally.
    \let\pgf@next=\relax%
  \else%
    \let\pgf@next=\pgf@replacepicturebygraphic%
  \fi%
  \pgf@next%  
}

\long\def\pgf@replacepicturebygraphic#1\endpgfgraphicnamed{\includegraphics{\pgf@filename}\unskip}


% Grab operation: If jobname matches the graphic name, typeset this
% picture normall.

\def\pgf@external@grab#1{%
  \setbox\pgfpic=\hbox\bgroup\bgroup%
    \let\endpgfgraphicnamed=\pgf@externalend%
}

\def\pgf@externalend{%
  \unskip\egroup\egroup%
  {%
    \parindent0pt%
    \leftmargin0pt%
    \rightmargin0pt%
    \dimen0\ht\pgfpic%
    \advance\dimen0\dp\pgfpic%
    \pgfsys@papersize{\the\wd\pgfpic}{\the\dimen0}%
    \setbox0=\vbox{%
      \kern -1truein%
      \hbox{%
        \kern -1truein%
        \hbox to0pt{%
          \wd\pgfexternal@startupbox=0pt%
          \ht\pgfexternal@startupbox=0pt%
          \dp\pgfexternal@startupbox=0pt%
          \box\pgfexternal@startupbox%
          \pgfsys@atbegindocument\hss}%
        \box\pgfpic%
        \kern 1truein}%
      \kern1truein}%
    \pgfexternal@originalshipout\box0%
  }%
}


\endinput


==> pgfcorelayers.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorelayers.code.tex,v 1.1 2008/01/15 10:27:34 tantau Exp $


% Creates a new pgf layer
%
% #1 = layer name
%
% Declares a new layer for pgf.
%
% Example:
%
% \pgfdeclarelayer{background}

\def\pgfdeclarelayer#1{%
  \expandafter\pgf@newbox\csname pgf@layerbox@#1\endcsname%
  \expandafter\pgf@newbox\csname pgf@layerboxsaved@#1\endcsname%
}
\let\pgf@newbox=\newbox % avoid plain TeX outer problem

% Sets the layers that compose the picture
%
% #1 = List of layers
%
% Description:
%
% Sets the list of layers that make up the picture. The layers will be
% put on top of each other in the order given. 
%
% Example:
%
% \pgfsetlayers{background,main}

\def\pgfsetlayers#1{\edef\pgf@layerlist{#1}}
\pgfsetlayers{main}



% Adds code to a layer
%
% #1 = layer name
%
% Note:
%
% You cannot anything to the ``main'' layer using this command.
%
% Example:
%
% \begin{pgfonlayer}{background}
%   \fill[red] (0,0) -- (1,1);
% \end{pgfonlayer}

\def\pgfonlayer#1{%
  \expandafter\global\expandafter%
  \setbox\csname pgf@layerbox@#1\endcsname=\hbox to 0pt%
    \bgroup%
      \expandafter\box\csname pgf@layerbox@#1\endcsname%
      \begingroup%
}
\def\endpgfonlayer{%
      \endgroup%
      \hss
    \egroup%
}

\let\startpgfonlayer=\pgfonlayer
\let\stoppgfonlayer=\endpgfonlayer




% Hooks into the scoping:

\def\pgf@insertlayers{%
  \expandafter\pgf@dolayer\pgf@layerlist,,\relax%
}
\def\pgf@maintext{main}%
\def\pgf@dolayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
    \box\pgf@layerbox@main%
  \else%
    \pgfsys@beginscope%
      \expandafter\box\csname pgf@layerbox@#1\endcsname%
    \pgfsys@endscope%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dolayer#2,\relax%
  \fi%
}

\def\pgf@savelayers{%
  \expandafter\pgf@dosavelayer\pgf@layerlist,,\relax%
}
\def\pgf@dosavelayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
  \else%
    \setbox\csname pgf@layerboxsaved@#1\endcsname=\box\csname pgf@layerbox@#1\endcsname%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dosavelayer#2,\relax%
  \fi%
}

\def\pgf@restorelayers{%
  \expandafter\pgf@dorestorelayer\pgf@layerlist,,\relax%
}
\def\pgf@dorestorelayer#1,#2,\relax{%
  \def\pgf@test{#1}%
  \ifx\pgf@test\pgf@maintext%
  \else%
    \global\setbox\csname pgf@layerbox@#1\endcsname=\box\csname pgf@layerboxsaved@#1\endcsname%
  \fi%
  \def\pgf@test{#2}%
  \ifx\pgf@test\pgfutil@empty%
  \else%
    \pgf@dorestorelayer#2,\relax%
  \fi%
}

\endinput


==> pgfcoreobjects.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoreobjects.code.tex,v 1.2 2006/10/11 15:22:25 tantau Exp $


% Object reuse


% Define a pgf object for reuse. Such objects will be stored
% efficiently internally.
%
% #1 = name for later reuse
% #2 = lower left corner point of bounding box
% #3 = upper right left corner point of bounding box
% #4 = pure pgf code (nothing too fancy!)
%
% Description:
% 
% Used to define reusable objects. The object must be composed of
% basic pgf graphic primitives. Nothing fancy can be used. The
% created object will be stored as an xform object in pdf or as a
% postscript procedure in postscript.
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfpathqmoveto{0pt}{0pt}
%  \pgfpathqmoveto{10pt}{0pt}
%  \pgfpathqmoveto{10pt}{10pt}
%  \pgfpathqmoveto{0pt}{10pt}
%  \pgfpathclose
%  \pgfusepath{stroke}}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgfuseobject{myrect}
% \end{pgfpicture}

\def\pgfdefobject#1#2#3#4{%
  \pgfinterruptpath%
    \pgf@relevantforpicturesizefalse%
    \pgfsys@defobject{#1}{#2}{#3}{#4}%
  \endpgfinterruptpath%
  \ignorespaces%
}


% Use an object that was previously defined using pgfdefobject
%
% #1 = name of previously defined object
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfqmoveto{0}{0}
%  \pgfqmoveto{10}{0}
%  \pgfqmoveto{10}{10}
%  \pgfqmoveto{0}{10}
%  \pgfclosestroke}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgfuseobject{myrect}
% \end{pgfpicture}

\def\pgfuseobject#1{\pgfsys@beginscope\pgfsys@useobject{#1}{}\pgfsys@endscope}


% Use an object that was previously defined using pgfdefobject, but
% magnify the object by the current x and y register values
%
% #1 = name of previously defined object
%  
% Example:
%
% \pgfdefobject{myrect}{\pgfpoint{-1pt}{-1pt}}{\pgfpoint{11pt}{11pt}}
% {\pgfqmoveto{0}{0}
%  \pgfqmoveto{10}{0}
%  \pgfqmoveto{10}{10}
%  \pgfqmoveto{0}{10}
%  \pgfclosestroke}
%
% \begin{pgfpicture}{0cm}{0cm}{1cm}{1cm}
%   \pgf@x=2pt% Scale by factor two in x-direction
%   \pgf@y=2pt% Scale by factor two in y-direction
%   \pgfuseobjectmagnify{myrect}
% \end{pgfpicture}

\def\pgfuseobjectmagnify#1{%
  \pgfsys@beginscope%
  \pgfsys@useobject{#1}{\pgfsys@transformxyscale{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}}%
  \pgfsys@endscope%
}


\endinput


==> pgfcorepathconstruct.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepathconstruct.code.tex,v 1.14 2008/02/13 15:10:06 tantau Exp $


\newdimen\pgf@path@lastx
\newdimen\pgf@path@lasty



% Replace corners by arcs.
%
% #1 = in-size of arc
% #2 = out-size of arc
% 
% Description:
% 
% This command influences path construction command like
% \pgfpathlineto or \pgfpatharc. It will cause the corners at the end
% of these commands to be replaced by little arcs. If the
% corner is a 90 degrees corner and if #1=#2, a quarter-circle of
% radius #1 is put in place of the corner. If #1 and #2 are different,
% the quarter circle will instead by a quarter ellipse. If the angle
% is different from 90 degrees, a deformed quarter circle will
% result, which may or may not be desirable. For a ``perfect'' arc you
% must use the \pgfpatharc command. 
% 
% 
% Example: One rounded corner.
%
% \pgfpathmoveto{\pgfpointxy{0}{0}}
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathlineto{\pgfpointxy{0}{1}}
% \pgfpathlineto{\pgfpointxy{1}{1}}
% \pgfstroke
%
% Example: A rounded rectangle
%
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% \pgfstroke
%
% Example: A rounded triangles
%
% \pgfsetcornersarced{4pt}{4pt}
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{1cm}{0cm}}
% \pgfpathlineto{\pgfpoint{1cm}{1cm}}
% \pgfpathclose
% \pgfstroke

\newif\ifpgf@arccorners

\def\pgfsetcornersarced#1{%
  \pgf@process{#1}%
  \edef\pgf@corner@arc{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@arccornerstrue%
  \ifdim\pgf@x=0pt%
    \ifdim\pgf@y=0pt\relax%
      \pgf@arccornersfalse%
    \fi%
  \fi%
}

\def\pgf@roundcornerifneeded{%
  \ifpgf@arccorners\expandafter\pgfsyssoftpath@specialround\pgf@corner@arc\fi%
}


% Move current point to #1.
%
% #1 = new current point
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfstroke

\def\pgfpathmoveto#1{%
  \pgfpointtransformed{#1}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgfsyssoftpath@moveto{\the\pgf@x}{\the\pgf@y}%
  \global\pgf@path@lastx=\pgf@x%
  \global\pgf@path@lasty=\pgf@y%
}

\def\pgf@protocolsizes#1#2{%
  \ifpgf@relevantforpicturesize%
    \ifdim#1<\pgf@picminx\global\pgf@picminx#1\fi%
    \ifdim#1>\pgf@picmaxx\global\pgf@picmaxx#1\fi%
    \ifdim#2<\pgf@picminy\global\pgf@picminy#2\fi%
    \ifdim#2>\pgf@picmaxy\global\pgf@picmaxy#2\fi%
  \fi%
  \ifdim#1<\pgf@pathminx\global\pgf@pathminx#1\fi%
  \ifdim#1>\pgf@pathmaxx\global\pgf@pathmaxx#1\fi%
  \ifdim#2<\pgf@pathminy\global\pgf@pathminy#2\fi%
  \ifdim#2>\pgf@pathmaxy\global\pgf@pathmaxy#2\fi%
  \ifpgf@size@hooked%
    \let\pgf@size@hook@x#1\let\pgf@size@hook@y#2\pgf@path@size@hook%
  \fi%
}
\newif\ifpgf@size@hooked
\let\pgf@path@size@hook=\pgfutil@empty%

\def\pgf@resetpathsizes{%
  \global\pgf@pathmaxx=-16000pt\relax%
  \global\pgf@pathminx=16000pt\relax%
  \global\pgf@pathmaxy=-16000pt\relax%
  \global\pgf@pathminy=16000pt\relax%
}

\def\pgf@getpathsizes#1{%
  \edef#1{{\the\pgf@pathmaxx}{\the\pgf@pathminx}{\the\pgf@pathmaxy}{\the\pgf@pathminy}}%
}
\def\pgf@setpathsizes#1{%
  \expandafter\pgf@@setpathsizes#1%
}
\def\pgf@@setpathsizes#1#2#3#4{%
  \global\pgf@pathmaxx=#1\relax%
  \global\pgf@pathminx=#2\relax%
  \global\pgf@pathmaxy=#3\relax%
  \global\pgf@pathminy=#4\relax%
}





% Append a line from the current point to #1 to the current path.
%
% #1 = end of line
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfstroke

\def\pgfpathlineto#1{%
  \pgfpointtransformed{#1}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@roundcornerifneeded%
  \pgfsyssoftpath@lineto{\the\pgf@x}{\the\pgf@y}%
  \global\pgf@path@lastx=\pgf@x%
  \global\pgf@path@lasty=\pgf@y%
}



% Close the current path.
%
% Example:
%
% % Draws two triangles
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfclosepath
% \pgfpathmoveto{\pgfxy(2,0)}
% \pgfpathlineto{\pgfxy(2,1)}
% \pgfpathlineto{\pgfxy(3,0)}
% \pgfpathclose
% \pgfstroke

\def\pgfpathclose{%
  \pgf@roundcornerifneeded%
  \pgfsyssoftpath@closepath%
}


% Append a bezier spline from the current point to #3 with control
% points #1 and #2 to the current path.
%
% #1 = first control point
% #2 = second control point
% #3 = end point
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathcurveto{\pgfxy(0,1)}{\pgfxy(1,1)}{\pgfxy(1,2)}
% \pgfstroke

\def\pgfpathcurveto#1#2#3{%
  \pgfpointtransformed{#3}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgfpointtransformed{#2}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpointtransformed{#1}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@roundcornerifneeded%
  \pgfsyssoftpath@curveto{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xb}{\the\pgf@yb}%
  \global\pgf@path@lastx=\pgf@xb%
  \global\pgf@path@lasty=\pgf@yb%
}


% Append an arc to the current point, where the current point is at
% angle #1 and the end is at angle #2. If #2 > #1, the arc is drawn
% counter-clockwise, otherwise it is clockwise.
%
% #1 = angle of first point
% #2 = angle of second point
% #3 = radius or x-radius/y-radius
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpatharc{0}{90}{2cm}
% \pgfstroke

\def\pgfpatharc#1#2#3{%
  {%
    \pgfmathparse{#1}\let\pgf@temp@a=\pgfmathresult%
    \pgfmathparse{#2}\let\pgf@temp@b=\pgfmathresult%
    \pgfutil@in@{and }{#3}%
    \ifpgfutil@in@%
      \pgf@arc@get@radii#3\pgf@arc@stop%
    \else
      \pgf@arc@get@radii#3and #3\pgf@arc@stop%
    \fi%
    \pgf@arc@local@angle@a=\pgf@temp@a pt%
    \pgf@arc@local@angle@b=\pgf@temp@b pt%
    \relax%
    \ifdim\pgf@arc@local@angle@a>360pt\relax%
      \advance\pgf@arc@local@angle@a by-360pt\relax%
    \fi%
    \ifdim\pgf@arc@local@angle@a<-360pt\relax%
      \advance\pgf@arc@local@angle@a by360pt\relax%
    \fi%
    \ifdim\pgf@arc@local@angle@b>360pt\relax%
      \advance\pgf@arc@local@angle@b by-360pt\relax%
    \fi%
    \ifdim\pgf@arc@local@angle@b<-360pt\relax%
      \advance\pgf@arc@local@angle@b by360pt\relax%
    \fi%
    \loop%
      \pgfutil@tempdima=\pgf@arc@local@angle@a%
      \advance\pgfutil@tempdima by-\pgf@arc@local@angle@b\relax%
      \ifdim\pgfutil@tempdima<0pt\relax%
        \pgfutil@tempdima=-\pgfutil@tempdima\relax%
      \fi%
    \ifdim\pgfutil@tempdima>90pt\relax%
      \ifdim\pgfutil@tempdima>115pt\relax%
        \pgf@arc@temp=90pt% big skip
      \else%
        \pgf@arc@temp=60pt% smaller skip to ensure wide segments
                          % (important shortened end segments because
                          % of arrow tips)
      \fi%
      \ifdim\pgf@arc@local@angle@b>\pgf@arc@local@angle@a\relax%
        {%
          \pgf@arc@local@angle@b=\pgf@arc@local@angle@a\relax%
          \advance\pgf@arc@local@angle@b by\pgf@arc@temp\relax%
          \pgf@arc%
        }
        \advance\pgf@arc@local@angle@a by\pgf@arc@temp\relax%
      \else
        {%
          \pgf@arc@local@angle@b=\pgf@arc@local@angle@a\relax%
          \advance\pgf@arc@local@angle@b by-\pgf@arc@temp\relax%
          \pgf@arc%
        }%
        \advance\pgf@arc@local@angle@a by-\pgf@arc@temp\relax%
      \fi%
    \repeat%
    \pgf@roundcornerifneeded%
    \pgf@arc%
  }%
}
\dimendef\pgf@arc@local@angle@a=0
\dimendef\pgf@arc@local@angle@b=1
\dimendef\pgf@arc@temp=2

\def\pgf@arc@get@radii#1and #2\pgf@arc@stop{%
  \pgfmathparse{#1}\let\pgf@arc@radius@a=\pgfmathresult%
  \pgfmathparse{#2}\let\pgf@arc@radius@b=\pgfmathresult%
}


\def\pgf@arc{%
  {%
  % \pgfmathsetlength{\pgfutil@tempdima}{#3}%
  % \pgfmathsetlength{\pgfutil@tempdimb}{#4}%
  \pgfutil@tempdima=\pgf@arc@radius@a pt%
  \pgfutil@tempdimb=\pgf@arc@radius@b pt%
  %
  \pgf@xa=\pgf@arc@local@angle@a\relax% 
  \pgf@xb=\pgf@arc@local@angle@b\relax%
  % \pgfutil@tempcnta=#1\relax%
  %    \pgfutil@tempcntb=#2\relax%
  \advance\pgf@xb by-\pgf@xa\relax%
  \ifdim\pgf@xb<0pt\relax%
    \pgf@xb=-\pgf@xb\relax%
  \fi%
  \ifdim\pgf@xb>85pt\relax% hackery to correct the control points
    \pgfutil@tempdima=0.0555\pgfutil@tempdima\relax%
    \pgfutil@tempdimb=0.0555\pgfutil@tempdimb\relax%
  \else%
    \ifdim\pgf@xb>75pt\relax%  
      \pgfutil@tempdima=0.055\pgfutil@tempdima\relax%
      \pgfutil@tempdimb=0.055\pgfutil@tempdimb\relax%
    \else%
      \ifdim\pgf@xb>60pt\relax%  
        \pgfutil@tempdima=0.0545\pgfutil@tempdima\relax%
        \pgfutil@tempdimb=0.0545\pgfutil@tempdimb\relax%
      \else%
        \pgfutil@tempdima=0.054\pgfutil@tempdima\relax%
        \pgfutil@tempdimb=0.054\pgfutil@tempdimb\relax%
      \fi%
    \fi%
  \fi
  \pgfutil@tempdima=\pgf@sys@tonumber{\pgf@xb}\pgfutil@tempdima\relax%
  \divide\pgfutil@tempdima by 9\relax%
  \pgfutil@tempdimb=\pgf@sys@tonumber{\pgf@xb}\pgfutil@tempdimb\relax%
  \divide\pgfutil@tempdimb by 9\relax%
  %.. controls +(\pgf@xa+90:\pgfutil@tempdima) and +(\pgf@xb-90:\pgfutil@tempdima) .. +(-(#1:#3)+(#2:#3))%
  % store first support vector in xa/ya:
  \pgf@xa=\pgf@arc@local@angle@a\relax%
  \ifdim\pgf@arc@local@angle@b>\pgf@arc@local@angle@a\relax%
    \advance\pgf@xa by 90pt\relax%
  \else%
    \advance\pgf@xa by -90pt\relax%
  \fi%
  \edef\pgf@arc@angle{\pgf@sys@tonumber{\pgf@xa}}%  
  \pgfpointtransformed{\pgfpointpolar{\pgf@arc@angle}{\pgfutil@tempdima and \pgfutil@tempdimb}}%
  \advance\pgf@x by-\pgf@pt@x%
  \advance\pgf@y by-\pgf@pt@y%
  \pgf@xa=\pgf@path@lastx%
  \pgf@ya=\pgf@path@lasty%
  \advance\pgf@xa by \pgf@x%
  \advance\pgf@ya by \pgf@y%
  % store target in xb/yb:
  \pgfpointtransformed{\pgfpointpolar{\pgf@sys@tonumber{\pgf@arc@local@angle@a}}{\pgf@arc@radius@a pt and \pgf@arc@radius@b pt}}%
  \pgf@xb=\pgf@path@lastx%
  \pgf@yb=\pgf@path@lasty%
  \advance\pgf@xb by -\pgf@x%
  \advance\pgf@yb by -\pgf@y%
  \pgfpointtransformed{\pgfpointpolar{\pgf@sys@tonumber{\pgf@arc@local@angle@b}}{\pgf@arc@radius@a pt and \pgf@arc@radius@b pt}}%
  \advance\pgf@xb by \pgf@x%
  \advance\pgf@yb by \pgf@y%
  % store second support xc/yc:
  \ifdim\pgf@arc@local@angle@b>\pgf@arc@local@angle@a\relax%
    \advance\pgf@arc@local@angle@b by -90pt\relax%
  \else%
    \advance\pgf@arc@local@angle@b by 90pt\relax%
  \fi%
  \pgfpointtransformed{\pgfpointpolar{\pgf@sys@tonumber{\pgf@arc@local@angle@b}}{\pgfutil@tempdima and \pgfutil@tempdimb}}%
  \advance\pgf@x by-\pgf@pt@x%
  \advance\pgf@y by-\pgf@pt@y%
  \pgf@xc=\pgf@xb\relax%
  \pgf@yc=\pgf@yb\relax%
  \advance \pgf@xc by \pgf@x\relax%
  \advance \pgf@yc by \pgf@y\relax%
  \pgfsyssoftpath@curveto{\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xc}{\the\pgf@yc}{\the\pgf@xb}{\the\pgf@yb}%
  \global\pgf@path@lastx=\pgf@xb%
  \global\pgf@path@lasty=\pgf@yb%
  \pgf@protocolsizes{\pgf@xa}{\pgf@ya}%
  \pgf@protocolsizes{\pgf@xb}{\pgf@yb}%
  \pgf@protocolsizes{\pgf@xc}{\pgf@yc}%
  }%
}

% Append an arc to the current point, where the arc is on an ellipse
% given by two axis vectors.
%
% #1 = angle of first point
% #2 = angle of second point
% #3 = first axis
% #4 = second axis
% 
% Example:
%
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpatharcaxes{0}{90}{\pgfpointxy{2}{0}}{\pgfpointxy{0}{2}}
% \pgfstroke

\def\pgfpatharcaxes#1#2#3#4{%
  {%
    \pgftransformtriangle{\pgfpointorigin}{#3}{#4}%
    \pgfpatharc{#1}{#2}{1pt}%
  }%
}




% Append  an ellipse to the current path.
%
% #1 = center
% #2 = first axis
% #3 = second axis
%  
% Example:
%
% % Add a circle of radius 3cm around the origin
% \pgfpathellipse{\pgforigin}{\pgfxy(2,0)}{\pgfxy(0,1)}
%
% % Draw a non-filled circle of radius 1cm around the point (1,1)
% \pgfpathellipse{\pgfxy(1,1)}{\pgfxy(1,1)}{\pgfxy(-2,2)}
% \pgfstroke

\def\pgfpathellipse#1#2#3{%
  \pgfpointtransformed{#1}% store center in xc/yc
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgfpointtransformed{#2}%
  \pgf@xa=\pgf@x% store first axis in xa/ya
  \pgf@ya=\pgf@y%
  \advance\pgf@xa by-\pgf@pt@x%
  \advance\pgf@ya by-\pgf@pt@y%
  \pgfpointtransformed{#3}%
  \pgf@xb=\pgf@x% store second axis in xb/yb
  \pgf@yb=\pgf@y%
  \advance\pgf@xb by-\pgf@pt@x%
  \advance\pgf@yb by-\pgf@pt@y%
  {%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%
    \pgfsyssoftpath@moveto{\the\pgf@xa}{\the\pgf@ya}%
    \pgf@protocolsizes{\pgf@xa}{\pgf@ya}%
  }%
  \pgf@x=0.555\pgf@xb% first arc
  \pgf@y=0.555\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@x=0.555\pgf@xa%
  \pgf@y=0.555\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xb by\pgf@xc%
    \advance\pgf@yb by\pgf@yc%    
    \expandafter\pgfsyssoftpath@curveto\pgf@temp{\the\pgf@x}{\the\pgf@y}{\the\pgf@xb}{\the\pgf@yb}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@xb}{\pgf@yb}%
  }%
  \pgf@xa=-\pgf@xa% flip first axis
  \pgf@ya=-\pgf@ya%
  \pgf@x=0.555\pgf@xa% second arc
  \pgf@y=0.555\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@x=0.555\pgf@xb%
  \pgf@y=0.555\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%    
    \expandafter\pgfsyssoftpath@curveto\pgf@temp{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}%  
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@xa}{\pgf@ya}%
  }%
  \pgf@xb=-\pgf@xb% flip second axis
  \pgf@yb=-\pgf@yb%
  \pgf@x=0.555\pgf@xb% third arc
  \pgf@y=0.555\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@x=0.555\pgf@xa%
  \pgf@y=0.555\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xb by\pgf@xc%
    \advance\pgf@yb by\pgf@yc%    
    \expandafter\pgfsyssoftpath@curveto\pgf@temp{\the\pgf@x}{\the\pgf@y}{\the\pgf@xb}{\the\pgf@yb}%  
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@xb}{\pgf@yb}%
  }%
  \pgf@xa=-\pgf@xa% flip first axis once more
  \pgf@ya=-\pgf@ya%
  \pgf@x=0.555\pgf@xa% fourth arc
  \pgf@y=0.555\pgf@ya%
  \advance\pgf@x by\pgf@xb%
  \advance\pgf@y by\pgf@yb%
  \advance\pgf@x by\pgf@xc%
  \advance\pgf@y by\pgf@yc%
  \edef\pgf@temp{{\the\pgf@x}{\the\pgf@y}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@x=0.555\pgf@xb%
  \pgf@y=0.555\pgf@yb%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya%
  {%
    \advance\pgf@x by\pgf@xc%
    \advance\pgf@y by\pgf@yc%
    \advance\pgf@xa by\pgf@xc%
    \advance\pgf@ya by\pgf@yc%    
    \expandafter\pgfsyssoftpath@curveto\pgf@temp{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@xa}{\pgf@ya}%
  }%
  \pgfsyssoftpath@closepath%
  \pgfsyssoftpath@moveto{\the\pgf@xc}{\the\pgf@yc}%
}



% Append a circle to the current path
%
% #1 = center
% #2 = radius
%  
% Example:
%
% % Append a circle of radius 3cm around the the point (1,1)
% \pgfpathcircle{\pgxy(1,1)}{3cm}

\def\pgfpathcircle#1#2{\pgfpathellipse{#1}{\pgfpoint{#2}{0pt}}{\pgfpoint{0pt}{#2}}}




% Append a rectangle to the current path
%
% #1 = lower left corner point of rectangle
% #2 = width and height vector
%  
% Example:
%
% % A rectangle with corners (2,2) and (3,3)
% \pgfpathrectangle{\pgfpointxy{2}{2}}{\pgfpointxy{1}{1}}

\def\pgfpathrectangle{%
  \let\pgfrect@next=\pgf@specialrect%
  \ifpgf@pt@identity%
    \ifpgf@arccorners%
    \else%
      \let\pgfrect@next=\pgf@normalrect%
    \fi%
  \fi%
  \pgfrect@next%
}

\def\pgf@normalrect#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpointtransformed{#1}%
  \pgfsyssoftpath@rect{\the\pgf@x}{\the\pgf@y}{\the\pgf@xa}{\the\pgf@ya}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \advance\pgf@x by\pgf@xa\relax%
  \advance\pgf@y by\pgf@ya\relax%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
}

\def\pgf@specialrect#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#1}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \advance\pgf@xa by\pgf@xb%
  \advance\pgf@ya by\pgf@yb%
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}%
  \pgfpathclose%
  \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
}

% Append a rectangle to the current path
%
% #1 = one corner of the rectangle
% #2 = opposite corner of the rectangle
%  
% Example:
%
% % A rectangle with corners (2,2) and (3,3)
% \pgfpathrectanglecorners{\pgfpointxy{2}{2}}{\pgfpointxy{3}{3}}

\def\pgfpathrectanglecorners#1#2{%
  \pgf@process{#2}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xc by-\pgf@x%
  \advance\pgf@yc by-\pgf@y%
  \pgfpathrectangle{#1}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
}


% Append a grid to the current path.
%
% #1 = lower left point of grid
% #2 = upper right point of grid
%  
% Options: 
%  
% stepx = x-step dimension (default 1cm)
% stepy = y-step dimension (default 1cm)
% step  = dimesion vector
%  
% Example:
%
% \pgfsetlinewidth{0.8pt}
% \pgfgrid{\pgfxy(0,0)}{\pgfxy(3,2)}
% \pgfsetlinewidth{0.4pt}
% \pgfgrid[stepx=1cm,stepy=1cm]{\pgfxy(0,0)}{\pgfxy(3,2)}

\pgfkeys{
  /pgf/stepx/.initial=1cm,
  /pgf/stepy/.initial=1cm,
  /pgf/step/.code={\pgf@process{#1}\pgfkeysalso{/pgf/stepx/.expanded=\the\pgf@x,/pgf/stepy/.expanded=\the\pgf@y}},
  /pgf/step/.value required
}

\def\pgfpathgrid{\pgfutil@ifnextchar[{\pgf@pathgrid}{\pgf@pathgrid[]}}
\def\pgf@pathgrid[#1]#2#3{%
  \pgfset{#1}%
  \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/stepx}}%
  \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/stepy}}%
  \pgf@process{#3}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x\relax%
  \pgf@ya=\pgf@y\relax%
  {%
    % compute bounding box
    % first corner
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    % second corner
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@ya%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    % third corner
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@yb%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
    % fourth corner
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  }%
  \c@pgf@counta=\pgf@y\relax%
  \c@pgf@countb=\pgf@yc\relax%
  \divide\c@pgf@counta by\c@pgf@countb\relax%
  \pgf@y=\c@pgf@counta\pgf@yc\relax%
  \ifdim\pgf@y<\pgf@ya%
    \advance\pgf@y by\pgf@yc%
  \fi%
  \loop% horizontal lines
    {%
      \pgf@xa=\pgf@x%
      \pgf@ya=\pgf@y%
      \pgf@pos@transform{\pgf@xa}{\pgf@ya}
      \pgfsyssoftpath@moveto{\the\pgf@xa}{\the\pgf@ya}%
      \pgf@xa=\pgf@xb%
      \pgf@ya=\pgf@y%
      \pgf@pos@transform{\pgf@xa}{\pgf@ya}
      \pgfsyssoftpath@lineto{\the\pgf@xa}{\the\pgf@ya}%
    }%
    \advance\pgf@y by\pgf@yc%
  \ifdim\pgf@y<\pgf@yb%
  \repeat%
  \advance\pgf@y by-0.01pt\relax%
  \ifdim\pgf@y<\pgf@yb%
    {%
      \pgf@xa=\pgf@x%
      \pgf@ya=\pgf@y%
      \pgf@pos@transform{\pgf@xa}{\pgf@ya}
      \pgfsyssoftpath@moveto{\the\pgf@xa}{\the\pgf@ya}%
      \pgf@xa=\pgf@xb%
      \pgf@ya=\pgf@y%
      \pgf@pos@transform{\pgf@xa}{\pgf@ya}
      \pgfsyssoftpath@lineto{\the\pgf@xa}{\the\pgf@ya}%
    }%
  \fi%
  \c@pgf@counta=\pgf@x\relax%
  \c@pgf@countb=\pgf@xc\relax%
  \divide\c@pgf@counta by\c@pgf@countb\relax%
  \pgf@x=\c@pgf@counta\pgf@xc\relax%
  \ifdim\pgf@x<\pgf@xa%
    \advance\pgf@x by\pgf@xc%
  \fi%
  \loop% vertical lines
    {%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@ya%
      \pgf@pos@transform{\pgf@xc}{\pgf@yc}
      \pgfsyssoftpath@moveto{\the\pgf@xc}{\the\pgf@yc}%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@yb%
      \pgf@pos@transform{\pgf@xc}{\pgf@yc}
      \pgfsyssoftpath@lineto{\the\pgf@xc}{\the\pgf@yc}%
    }%
    \advance\pgf@x by\pgf@xc%
  \ifdim\pgf@x<\pgf@xb%
  \repeat%
  \advance\pgf@x by-0.01pt\relax%
  \ifdim\pgf@x<\pgf@xb%
    {%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@ya%
      \pgf@pos@transform{\pgf@xc}{\pgf@yc}
      \pgfsyssoftpath@moveto{\the\pgf@xc}{\the\pgf@yc}%
      \pgf@xc=\pgf@x%
      \pgf@yc=\pgf@yb%
      \pgf@pos@transform{\pgf@xc}{\pgf@yc}
      \pgfsyssoftpath@lineto{\the\pgf@xc}{\the\pgf@yc}%
    }%
  \fi%
}



% Append two half-parabolas to the path
%
% #1 = bend (relative to current point)
% #2 = end point (relative to bend point)
%  
% Description:
%  
% This command appends a half-parabola that starts at the current point
% and has its bend at #1+current point. Then, a second parabola is
% appended that starts at #1+current point, where it also has its
% minimum/maximum, and ends at #1+current point+#2, which becomes the
% new current point. 
%  
% By setting #2 = (0,0) you draw only a half parabola that goes from the
% current point to the bend; by setting #1 = (0,0)
% you draw a half parabola that going to current point + #2 and has its
% bend at the current point. 
%  
% Examples:
%
% % Half-parabola going ``up and right''
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpointorigin}{\pgfpoint{2cm}{4cm}}
%
% % Half-parabola going ``down and right''
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpoint{-2cm}{4cm}}}{\pgfpointorigin}
%
% % Full parabola
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathparabola{\pgfpoint{-2cm}{4cm}}{\pgfpoint{2cm}{4cm}}

\def\pgfpathparabola#1#2{%
  {%
    \pgf@process{#2}% untransformed
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempswatrue%
    \ifdim\pgf@xb=0pt\relax%
      \ifdim\pgf@yb=0pt\relax%
        \pgfutil@tempswafalse%
      \fi%
    \fi%  
    {%
      \ifpgfutil@tempswa%
        \pgf@arccornersfalse
      \else%
      \fi%
      \pgfutil@tempswatrue%
      \ifdim\pgf@xc=0pt\relax%
        \ifdim\pgf@yc=0pt\relax%
          \pgfutil@tempswafalse%
        \fi%
      \fi%
      \ifpgfutil@tempswa  
      {%
        \pgf@pt@x=\pgf@path@lastx%
        \pgf@pt@y=\pgf@path@lasty%
        \pgfpathcurveto%
          {\pgfqpoint{.1125\pgf@xc}{.225\pgf@yc}}% found by trial and error
          {\pgfqpoint{.5\pgf@xc}{\pgf@yc}}% found by trial and error
          {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
      }%
      \fi%
    }%
    \ifpgfutil@tempswa%
      \pgf@xc=\pgf@xb%
      \pgf@yc=\pgf@yb%
      {%
        \pgf@pt@x=\pgf@path@lastx%
        \pgf@pt@y=\pgf@path@lasty%
        \pgfpathcurveto%
          {\pgfqpoint{.5\pgf@xc}{0\pgf@yc}}% found by trial and error
          {\pgfqpoint{.8875\pgf@xc}{.775\pgf@yc}}% found by trial and error
          {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
      }%
    \fi%
  }%  
}  




% Append a sine curve between 0 and \pi/2 to the path.
%
% #1 = vector, describing the width and height of the curve
%  
% Description:
%  
% This command appends a sine curve in the interval 0 and \pi/2 to the
% current path. The sine curve ends at currentpoint+#1.
%  
% Examples:
%
% % One complete sine in the interval [0,\pi]
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathsine{\pgfpoint{1.57cm}{1cm}}
% \pgfpathcosine{\pgfpoint{3.141cm}{0cm}}

\def\pgfpathsine#1{%
  {%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@pt@x=\pgf@path@lastx% evil trickery to transform to the last point
    \pgf@pt@y=\pgf@path@lasty%
    \pgfpathcurveto%
      {\pgfqpoint{.31831\pgf@xc}{.5\pgf@yc}}% found by trial and error
      {\pgfqpoint{.63503\pgf@xc}{\pgf@yc}}% found by trial and error
      {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  }%  
}  

% Append a cosine curve between 0 and \pi/2 to the path.
%
% #1 = vector, describing the width and height of the curve
%  
% Examples:
%
% % One complete sine in the interval [0,\pi]
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathsine{\pgfpoint{1.57cm}{1cm}}
% \pgfpathcosine{\pgfpoint{3.141cm}{0cm}}

\def\pgfpathcosine#1{%
  {%
    \pgf@process{#1}% untransformed
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@pt@x=\pgf@path@lastx% evil trickery to transform to the last point
    \pgf@pt@y=\pgf@path@lasty%
    \pgfpathcurveto%
      {\pgfqpoint{.36497\pgf@xc}{0pt}}% found by trial and error
      {\pgfqpoint{.68169\pgf@xc}{.5\pgf@yc}}% found by trial and error
      {\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  }%  
}  


\endinput


==> pgfcorepathprocessing.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepathprocessing.code.tex,v 1.7 2008/01/23 15:22:29 tantau Exp $





% Extract start and end vectors of a path
%
% #1 = a macro that stores a path
%
% Description:
%
% This command will extract the first and second coordinate on the
% path as well as the last and second-last. These coordinates will be
% put in the pgfpoint-macros \pgfpointfirstonpath,
% \pgfpointsecondonpath, \pgfpointsecondlastonpath, and
% \pgfpointlastonpath. If the path is empty, these macros are set to
% \pgfpointorigin. 
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{30}{40}{40}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfprocesspathextractpoints\mypath
% 
% % \pgfpointfirstonpath is now \pgfpoint{0}{0}
% % \pgfpointsecondonpath is now \pgfpoint{10bp}{10bp}
% % \pgfpointsecondlastonpath is now \pgfpoint{30bp}{30bp}
% % \pgfpointlastonpath is now \pgfpoint{40bp}{40bp}

\def\pgfprocesspathextractpoints#1{%
  \ifx#1\pgfutil@empty%
    \let\pgfpointfirstonpath=\pgfpointorigin%
    \let\pgfpointsecondonpath=\pgfpointorigin%
    \let\pgfpointsecondlastonpath=\pgfpointorigin%
    \let\pgfpointlastonpath=\pgfpointorigin%
  \else%
    \expandafter\pgf@extractprocessorfirst#1\pgf@stop%
  \fi%
}

\def\pgf@extractprocessorfirst#1#2#3#4{%
  \def\pgfpointfirstonpath{\pgfqpoint{#2}{#3}}%
  \ifx#4\pgf@stop%
    % pretty short path...
    \let\pgfpointsecondonpath=\pgfpointfirstonpath%
    \let\pgfpointsecondlastonpath=\pgfpointfirstonpath%
    \let\pgfpointlastonpath=\pgfpointfirstonpath%
    \let\next=\pgfutil@gobble%
  \else
    \let\next=\pgf@extractprocessorsecond%
  \fi%
  \next#4%
}

\def\pgf@extractprocessorsecond#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    % Reset things...
    \let\pgf@next=\pgf@extractprocessorfirst%
  \else%
    \let\pgf@next=\pgf@@extractprocessorsecond%
  \fi%
  \pgf@next#1%
}
\def\pgf@@extractprocessorsecond#1#2#3#4{%
  \def\pgfpointsecondonpath{\pgfqpoint{#2}{#3}}%
  \let\pgfpointsecondlastonpath=\pgfpointfirstonpath%
  \let\pgfpointlastonpath=\pgfpointsecondonpath%
  \ifx#4\pgf@stop%
    % short path...
    \let\next=\pgfutil@gobble%
  \else
    \let\next=\pgf@extractprocessorother%
  \fi%
  \next#4%
}

\def\pgf@extractprocessorother#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    % Reset things...
    \let\pgf@next=\pgf@extractprocessorfirst%
  \else%
    \let\pgf@next=\pgf@@extractprocessorother%
  \fi%
  \pgf@next#1%
}
\def\pgf@@extractprocessorother#1#2#3#4{%
  \let\pgfpointsecondlastonpath=\pgfpointlastonpath%
  \def\pgfpointlastonpath{\pgfqpoint{#2}{#3}}%
  \ifx#4\pgf@stop%
    % end!
    \let\next=\pgfutil@gobble%
  \fi%
  \next#4%
}



% Check for closepath and rectangles
%
% #1 = a macro that stores a path
% #2 = command to be executed when a closepath or a rectangle is encountered
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{30}{40}{40}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfprocesscheckclosed{\mypath}{\pgf@drawarrowsfalse}

\def\pgfprocesscheckclosed#1#2{%
  {%
    \global\let\pgf@proc@todo=\relax%
    \let\pgfsyssoftpath@movetotoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@linetotoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetosupportatoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetosupportbtoken=\pgfutil@gobbletwo%
    \let\pgfsyssoftpath@curvetotoken=\pgfutil@gobbletwo%
    \def\pgfsyssoftpath@rectcornertoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    \def\pgfsyssoftpath@rectsizetoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    \def\pgfsyssoftpath@closepathtoken{\gdef\pgf@proc@todo{#2}\pgfutil@gobbletwo}%
    #1%
  }%
  \pgf@proc@todo%
}

  
% Resolve specialround
%
% #1 = a macro that stores a path
% #2 = a macro that stores the new path
%
% Description:
%
% Resolves all specialround tokens. When such a token is encountered,
% the objective is to replace the next corner by a rounded corner. 
%

\def\pgfprocessround#1#2{%
  % first, check whether #1 contains \pgfsyssoftpath@specialroundtoken.
  % if not, do quick assignment!
  \expandafter\pgf@processroundcheck\expandafter#1\expandafter#2#1\pgfsyssoftpath@specialroundtoken\pgf@stop%
}

\def\pgf@processroundcheck#1#2#3\pgfsyssoftpath@specialroundtoken#4\pgf@stop{%
  \def\pgf@test{#4}%
  \ifx\pgf@test\pgfutil@empty%
    % ok, nothing to be done!
    \let#2=#1%
  \else%
    % very well...
    \pgf@@processround#1#2%
  \fi%
}


\def\pgf@@processround#1#2{%  
  \let\pgfprocess@newpath\pgfutil@empty%
  \let\pgfprocess@moveto\pgfutil@empty%
  \let\pgfprocess@firstto\pgfutil@empty%
  \let\pgfprocess@segment\pgfutil@empty%
  \pgf@xa=0pt%
  \pgf@ya=0pt%
  \expandafter\pgfprocess@round#1\pgf@stop{0pt}{0pt}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@moveto}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@segment}%
  \let#2=\pgfprocess@newpath%
}

\def\pgfprocess@round#1#2#3{%
  \ifx#1\pgf@stop%
    \let\next=\relax%
  \else%
    \ifx#1\pgfsyssoftpath@specialroundtoken%
      \def\pgfprocess@savex{#2}%
      \def\pgfprocess@savey{#3}%
      \let\next=\pgfprocess@specialround%
      \ifdim#2=0pt%
        \ifdim#3=0pt%
          \let\next=\pgfprocess@round% skip!
        \fi%
      \fi%
    \else%
      \ifx\pgfprocess@firstto\pgfutil@empty%
        \def\pgfprocess@firstto{{#2}{#3}}%
      \fi%
      \pgf@xa=#2%
      \pgf@ya=#3%
      \ifx#1\pgfsyssoftpath@movetotoken%
        % ok, move old segment to newpath
        \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@moveto}%
        \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@newpath\expandafter{\pgfprocess@segment}%
        \def\pgfprocess@moveto{#1{#2}{#3}}%
        \let\pgfprocess@firstto=\pgfutil@empty%
        \let\pgfprocess@segment=\pgfutil@empty%
      \else%
        \pgfutil@g@addto@macro\pgfprocess@segment{#1{#2}{#3}}%
      \fi%
      \let\next=\pgfprocess@round%
    \fi%
  \fi%
  \next%  
}

\def\pgfprocess@specialround#1#2#3{%
  \ifx\pgfprocess@firstto\pgfutil@empty%
    \def\pgfprocess@firstto{{#2}{#3}}%
  \fi%
  \let\next=\pgfprocess@round% default: do nothing
  \ifx#1\pgfsyssoftpath@linetotoken%
    % Ok, round a lineto
    \let\next=\pgfprocess@specialroundcope%
  \else%
    \ifx#1\pgfsyssoftpath@curvetosupportatoken%
      % Ok, round a curveto. 
      \let\next=\pgfprocess@specialroundcurveto%
    \else%
      \ifx#1\pgfsyssoftpath@closepathtoken%
        % Ok, round a closepath (this is tricky...)
        \let\next=\pgfprocess@specialroundclose%
      \fi%
    \fi%
  \fi%
  \next#1{#2}{#3}%
}%

\def\pgfprocess@specialroundcope#1#2#3#4#5#6{%
  \let\next=\pgfprocess@round% do nothing by default
  \let\pgfprocess@continueafterrounding=\pgfprocess@round%
  \ifx#4\pgfsyssoftpath@linetotoken%
    % ok, let's get kicking...
    \pgf@xc=#5%
    \pgf@yc=#6%
    \let\next=\pgfprocess@@specialround%
  \else%
    \ifx#4\pgfsyssoftpath@curvetosupportatoken%  
      \pgf@xc=#5%
      \pgf@yc=#6%
      \let\next=\pgfprocess@@specialround%
    \else%
      \ifx#4\pgfsyssoftpath@closepathtoken%  
        \pgf@xc=#5%
        \pgf@yc=#6%
        \let\next=\pgfprocess@@specialround%
      \else
        \ifx#4\pgfsyssoftpath@specialroundtoken%  
          \let\next=\pgfprocess@@findrightcoordinates%
        \fi%
      \fi%
    \fi%
  \fi%
  \next#1{#2}{#3}#4{#5}{#6}%
}

\def\pgfprocess@@findrightcoordinates#1#2#3#4#5#6#7#8#9{%
  \pgf@xc=#8%
  \pgf@yc=#9%
  \pgfprocess@@specialround#1{#2}{#3}#4{#5}{#6}#7{#8}{#9}%
}

\def\pgfprocess@@specialround#1#2#3{%
  \pgfutil@g@addto@macro\pgfprocess@segment{#1}%
  % calculate start coordinate of the curve
  \pgf@xb=#2%
  \pgf@yb=#3%
  %
  \edef\pgf@marshal%
  {\noexpand\pgfpointlineatdistance{\pgfprocess@savex}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
    {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}}%
  \pgf@process{\pgf@marshal}%
  \pgf@xa=\pgf@x% save start point of added curve
  \pgf@ya=\pgf@y%
  \edef\pgfprocess@addition{{\the\pgf@x}{\the\pgf@y}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  %
  % now add curve
  %
  \edef\pgf@marshal%
  {\noexpand\pgfpointlineatdistance{\pgfprocess@savey}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
    {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}}%
  \pgf@process{\pgf@marshal}%
  \pgf@xc=\pgf@x% save end point of added curve
  \pgf@yc=\pgf@y%
  % calculate first support:
  {%
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \advance\pgf@xa by 0.555\pgf@x%
    \advance\pgf@ya by 0.555\pgf@y%
    \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetosupportatoken{\the\pgf@xa}{\the\pgf@ya}}%
    \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  }%
  % calculate second support:
  {%
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by-\pgf@xc%
    \advance\pgf@y by-\pgf@yc%
    \advance\pgf@xc by 0.555\pgf@x%
    \advance\pgf@yc by 0.555\pgf@y%
    \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetosupportbtoken{\the\pgf@xc}{\the\pgf@yc}}%
    \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  }%
  % add end:
  \edef\pgfprocess@addition{\noexpand\pgfsyssoftpath@curvetotoken{\the\pgf@xc}{\the\pgf@yc}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfprocess@segment\expandafter{\pgfprocess@addition}%
  %
  % continue!
  %
  \pgf@xa=#2%
  \pgf@ya=#3%
  \pgfprocess@continueafterrounding%
}

\def\pgfprocess@specialroundcurveto#1#2#3#4#5#6{%
  \pgfutil@g@addto@macro\pgfprocess@segment{#1{#2}{#3}#4{#5}{#6}}% supports
  \pgf@xa=#5%
  \pgf@ya=#6%
  \pgfprocess@specialroundcope}

\def\pgfprocess@specialroundclose{%
  \let\next=\pgfprocess@round%
  \ifx\pgfprocess@moveto\pgfutil@empty%
  \else%
    \ifx\pgfprocess@firstto\pgfutil@empty%
    \else%
      \expandafter\pgfprocess@@specialclosetarget\pgfprocess@firstto%
      \let\pgfprocess@continueafterrounding=\pgfprocess@cleanupafterclose%
      \edef\next{%
        \noexpand\pgfprocess@@specialround%
        \expandafter\expandafter\expandafter\noexpand\expandafter\pgfprocess@@specialclosemoveto\pgfprocess@moveto%
      }%
    \fi%
  \fi%  
  \next%
}

\def\pgfprocess@@specialclosetarget#1#2{%
  \pgf@xc=#1%
  \pgf@yc=#2%
}

\def\pgfprocess@@specialclosemoveto#1#2#3{%
  \pgfsyssoftpath@linetotoken{#2}{#3}%
}


\def\pgfprocess@cleanupafterclose#1#2#3{%
  \edef\pgfprocess@moveto{\noexpand\pgfsyssoftpath@movetotoken{\the\pgf@xc}{\the\pgf@yc}}%
  \edef\pgf@marshal{\noexpand\pgfprocess@round\noexpand\pgfsyssoftpath@closepathtoken{\the\pgf@xc}{\the\pgf@yc}}%
  \pgf@marshal%  
}


% Replace start and end coordinates of a path
%
% #1 = new start coordinate
% #2 = new end coordinate
%
% Description:
%
% This command will replace the first and last coordinates on a path
% by the given coordinates.
%
% Example:
%
% \pgfsyssoftpath@moveto{0}{0}
% \pgfsyssoftpath@lineto{10}{10}
% \pgfsyssoftpath@curveto{20}{20}{30}{10}{40}{0}
% \pgfsyssoftpath@getcurrentpath\mypath
% \pgfsetlinewidth{2pt}
% \pgfusepath{stroke}
% \pgfprocesspathextractpoints{\mypath}
% \pgfprocesspathreplacestartandend{\mypath}
%   {\pgfpointlineatdistance{2pt}{\pgfpointfirstonpath}{\pgfpointsecondonpath}}%
%   {\pgfpointlineatdistance{2pt}{\pgfpointlastonpath}{\pgfpointsecondlastonpath}}%
% \pgfsyssoftpath@setcurrentpath\mypath
% \pgfsetlinewidth{1pt}
% \color{red}
% \pgfusepath{stroke}

\def\pgfprocesspathreplacestartandend#1#2#3{%
  \ifx#1\pgfutil@empty%
  \else%
  {%
    % We (mis)use the current path to store (in a buffered manner) the
    % rest path.
    \pgfsyssoftpath@getcurrentpath\pgf@replace@origpath%
    \let\pgf@prepath=\pgfutil@empty%
    \pgf@process{#3}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#2}%
    \expandafter\pgf@replaceprocessfirst#1\pgf@stop%
    \pgfsyssoftpath@getcurrentpath\pgf@restpath%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter#1%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
      \expandafter\expandafter\expandafter\pgf@prepath%
      \expandafter\pgf@newstart\pgf@restpath}%
    % Restore current path
    \pgfsyssoftpath@setcurrentpath\pgf@replace@origpath%
  }%
  \fi%
}

\def\pgf@replaceprocessfirst#1#2#3#4{%
  \def\pgf@origstart{#1{#2}{#3}}%
  \edef\pgf@newstart{\noexpand#1{\the\pgf@x}{\the\pgf@y}}%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \ifx#4\pgf@stop%
    \let\pgf@next=\pgfutil@gobble%
  \else%
    \let\pgf@next=\pgf@replaceprocessother%
    \let\pgf@@next=\pgf@@replaceprocessother%
  \fi%
  \pgf@next#4%
}

\def\pgf@replaceprocessother#1{%
  \ifx#1\pgfsyssoftpath@movetotoken%
    \pgf@replace@handle@move%
  \fi%
  \pgf@@next#1%
}
\def\pgf@@replaceprocessother#1#2#3#4{%
  \ifx#4\pgf@stop%
    \edef\pgf@restpathaddition{{\noexpand#1{\the\pgf@xa}{\the\pgf@ya}}}%
    \expandafter\pgfsyssoftpath@addtocurrentpath\pgf@restpathaddition%
    \let\pgf@next=\pgfutil@gobble%
  \else%
    \pgfsyssoftpath@addtocurrentpath{#1{#2}{#3}}%
  \fi%
  \pgf@next#4%
}  

\def\pgf@replace@handle@move{%
  \pgfsyssoftpath@getcurrentpath\pgf@restpath%
  % Arggghh! Must reset everything!
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgf@prepath%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
    \expandafter\expandafter\expandafter\pgf@prepath%
    \expandafter\pgf@origstart\pgf@restpath}%
  % Redo first.
  \let\pgf@@next=\pgf@replaceprocessfirst%
}
  
\endinput


==> pgfcorepathusage.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepathusage.code.tex,v 1.11 2008/01/23 13:15:28 tantau Exp $


% Stroke/fill/clip/etc. the current path. Depending on the options,
% the current path will be stroked/filled/clipped/etc. If no options
% are given, the path is stroked. If multiple options are given, all
% of them are performed (in a sensible order).
%
% #1 = action(s) to be applied to the current path. Valid actions are: 
%      stroke -  strokes the path. If no options are given, this is the
%                default. 
%      draw -    same as stroke.
%      fill -    fills the path.
%      clip -    clip the path.
%      discard - Discards the path. Same effect as having an empty
%                options list.
%
% Example:
%
% % Draws an edge.
% \pgfpathmoveto{\pgfxy(0,0)}
% \pgfpathlineto{\pgfxy(0,1)}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfusepath{stroke}

\pgfkeys{
  /pgf/stroke/.code=\def\pgf@up@stroke{stroke},
  /pgf/draw/.code=\def\pgf@up@stroke{stroke},
  /pgf/fill/.code=\def\pgf@up@fill{fill},
  /pgf/clip/.code=\def\pgf@up@clip{clip},
  /pgf/discard/.code=,
  /pgf/use as bounding box/.code=\def\pgf@up@bb{\pgf@relevantforpicturesizefalse}
}

\def\pgfusepath#1{%
  \let\pgf@up@stroke\pgfutil@empty%
  \let\pgf@up@fill\pgfutil@empty%
  \let\pgf@up@clip\pgfutil@empty%
  \let\pgf@up@discard\pgfutil@empty%
  \let\pgf@up@bb\pgfutil@empty%
  \pgfset{#1}%
  \expandafter\def\expandafter\pgf@up@action\expandafter{\csname pgfsys@\pgf@up@fill\pgf@up@stroke\endcsname}%
  \ifx\pgf@up@stroke\pgfutil@empty%
    \ifx\pgf@up@fill\pgfutil@empty%
      \ifx\pgf@up@clip\pgfutil@empty%
        \let\pgf@up@action=\pgfutil@empty%
        \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
      \else%
        % only clipping  
        \let\pgf@up@action=\pgfsys@discardpath%
      \fi%
    \fi%
  \fi%  
  \pgfsyssoftpath@getcurrentpath\pgf@last@processed@path
  \pgfprocessround{\pgf@last@processed@path}{\pgf@last@processed@path}% change the path
  \pgfsyssoftpath@setcurrentpath\pgf@last@processed@path%
  %
  % Check whether the path is stroked. If so, add half the line width
  % to the bounding box.
  %
  \ifpgf@relevantforpicturesize%
    \ifx\pgf@up@stroke\pgfutil@empty%
    \else%
      \ifdim\pgf@picmaxx=-16000pt\relax%
      \else%
        \pgf@x=\pgf@pathminx\advance\pgf@x by-.5\pgflinewidth%
        \ifdim\pgf@x<\pgf@picminx\global\pgf@picminx\pgf@x\fi%
        \pgf@y=\pgf@pathminy\advance\pgf@y by-.5\pgflinewidth%
        \ifdim\pgf@y<\pgf@picminy\global\pgf@picminy\pgf@y\fi%
        \pgf@x=\pgf@pathmaxx\advance\pgf@x by.5\pgflinewidth%
        \ifdim\pgf@x>\pgf@picmaxx\global\pgf@picmaxx\pgf@x\fi%
        \pgf@y=\pgf@pathmaxy\advance\pgf@y by.5\pgflinewidth%
        \ifdim\pgf@y>\pgf@picmaxy\global\pgf@picmaxy\pgf@y\fi%
      \fi%
    \fi%
  \fi%
  %
  \ifx\pgf@up@clip\pgfutil@empty%
    \ifx\pgf@up@stroke\pgfutil@empty%
      \pgfsyssoftpath@invokecurrentpath%
      \pgfsyssoftpath@getcurrentpath\pgf@last@used@path%
      \pgf@up@action%
    \else%
      \pgf@check@for@arrows%
      \ifpgf@drawarrows%
        \pgf@shorten@path@as@needed%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfsyssoftpath@getcurrentpath\pgf@last@used@path%
        \pgf@up@action%
        \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
        \pgf@add@arrows@as@needed%
      \else%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfsyssoftpath@getcurrentpath\pgf@last@used@path%
        \pgf@up@action%
      \fi%
    \fi%
  \else%
    \pgfsyssoftpath@invokecurrentpath%
    \pgfsyssoftpath@getcurrentpath\pgf@last@used@path%
    \pgfsys@clipnext%
    \pgf@up@action%
    \pgf@relevantforpicturesizefalse%
  \fi%
  \pgf@up@bb%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \pgf@resetpathsizes%
  \ignorespaces%
}


% Shorten start/end of paths by a certain amount.
%
% #1 = amount by which paths should be shortened.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{10pt}{0pt}
%
% % The following has the same effect:
% \pgfsetshortenstart{1pt}
% \pgfpathmoveto{\pgfpointorigin}
% \pgfpathlineto{\pgfpoint{11pt}{0pt}

\def\pgfsetshortenstart#1{\pgfmathsetlength\pgf@shorten@start@additional{#1}}
\def\pgfsetshortenend#1{\pgfmathsetlength\pgf@shorten@end@additional{#1}}

\newif\ifpgf@drawarrows

\def\pgf@check@for@arrows{%
  \pgf@drawarrowsfalse%
  \ifx\pgf@startarrow\pgfutil@empty\else\pgf@drawarrowstrue\fi%
  \ifx\pgf@endarrow\pgfutil@empty\else\pgf@drawarrowstrue\fi%
  \ifdim\pgf@shorten@end@additional=0pt\relax\else\pgf@drawarrowstrue\fi%
  \ifdim\pgf@shorten@start@additional=0pt\relax\else\pgf@drawarrowstrue\fi%
  \ifpgf@drawarrows%
    \pgfsyssoftpath@getcurrentpath\pgf@arrowpath%
    \ifx\pgf@arrowpath\pgfutil@empty%
      \pgf@drawarrowsfalse%
    \else%
      \pgfprocesscheckclosed{\pgf@arrowpath}{\pgf@drawarrowsfalse}%
    \fi%
  \fi%
}

\newdimen\pgf@shorten@end@additional
\newdimen\pgf@shorten@start@additional

\let\pgf@shorten@end=\pgfutil@empty
\let\pgf@shorten@start=\pgfutil@empty

\def\pgf@shorten@path@as@needed{%
  \pgfprocesspathextractpoints{\pgf@arrowpath}%
  \let\pgf@arrow@next=\pgf@shorten@now%
  \ifx\pgf@shorten@start\pgfutil@empty%
    \ifx\pgf@shorten@end\pgfutil@empty%
      \ifdim\pgf@shorten@end@additional=0pt\relax%
        \ifdim\pgf@shorten@start@additional=0pt\relax%
          \let\pgf@arrow@next=\relax%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgf@arrow@next%
}

\def\pgf@shorten@now{%
  {%
    \pgf@x=0pt%
    \pgf@shorten@start%
    \advance\pgf@x by\pgf@shorten@start@additional%
    \pgf@xc=\pgf@x%
    \pgfpointlineatdistance{\pgf@xc}{\pgfpointfirstonpath}{\pgfpointsecondonpath}%
    \global\pgf@xb=\pgf@x%
    \global\pgf@yb=\pgf@y%
    \pgf@process{\pgfpointsecondonpath}%
    \global\advance\pgf@x by\pgf@xa%
    \global\advance\pgf@y by\pgf@ya%
  }%
  \edef\pgfpointfirstonpath{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \edef\pgfpointsecondonpath{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  {%
    \pgf@x=0pt%
    \pgf@shorten@end%
    \advance\pgf@x by\pgf@shorten@end@additional%
    \pgf@xc=\pgf@x%
    \pgfpointlineatdistance{\pgf@xc}{\pgfpointlastonpath}{\pgfpointsecondlastonpath}%
    \global\pgf@xb=\pgf@x%
    \global\pgf@yb=\pgf@y%
    \pgf@process{\pgfpointsecondlastonpath}%
    \global\advance\pgf@x by\pgf@xa%
    \global\advance\pgf@y by\pgf@ya%
  }%
  \edef\pgfpointlastonpath{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \edef\pgfpointsecondlastonpath{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgfprocesspathreplacestartandend{\pgf@arrowpath}{\pgfpointfirstonpath}{\pgfpointlastonpath}%
  \pgfsyssoftpath@setcurrentpath\pgf@arrowpath%
}

\def\pgf@add@arrows@as@needed{%
  \ifx\pgf@startarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondonpath}{\pgfpointfirstonpath}}
      {\pgf@startarrow}%
  \fi%
  \ifx\pgf@endarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondlastonpath}{\pgfpointlastonpath}}
      {\pgf@endarrow}%
  \fi%      
}

\let\pgf@startarrow=\pgfutil@empty
\let\pgf@endarrow=\pgfutil@empty

\endinput


==> pgfcorepatterns.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepatterns.code.tex,v 1.1 2008/01/15 10:27:34 tantau Exp $


% Creates a new uncolored pattern
%
% #1 = pattern name
% #2 = lower left of bounding box
% #3 = upper right of bounding box
% #4 = step vector
% #5 = pattern code
%
% Description:
%
% Declares a new uncolored pattern. An uncolored pattern is a pattern
% that has no inherent color. When the pattern is used, a color for
% the pattern must be supplied.
%
% See the pdf-manual for more details on uncolored patterns.
%
% The bounding box must be a bounding box of the pattern cell.
%
% The step vector must provide the x- and y-step by which the cells
% are spaced.
%
% The pattern code should be pgf code that can be protocolled.
%
% The transformation matrix will be reset prior to invoking the
% pattern code.
%
% Example:
%
% \pgfdeclarepatternformonly{stars}{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% {\pgfpoint{1cm}{1cm}}{
%   \pgftransformshift{\pgfpoint{.5cm}{.5cm}}
%   \pgfpathmoveto{\pgfpointpolar{0}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{144}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{288}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{72}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{216}{4mm}}
%   \pgfpathclose%
%   \pgfusepath{stroke}
% }

\def\pgfdeclarepatternformonly#1#2#3#4#5{\pgf@declarepattern{#1}{#2}{#3}{#4}{#5}{0}}

% Creates a new colored pattern
%
% #1 = pattern name
% #2 = lower left of bounding box
% #3 = upper right of bounding box
% #4 = step vector
% #5 = pattern code
%
% Description:
%
% Declares a new colored pattern. Such patterns have a one or more
% fixed inherent colors. See the pdf-manual for more details on
% uncolored patterns.
%
% The parameters have the same effect as for uncolored patterns.
%
% Example:
%
% \pgfdeclarepatterninherentlycolored{red stars}{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
% {\pgfpoint{1cm}{1cm}}{
%   \pgfsetfillcolor{red}
%   \pgfsetstrokecolor{black}
%   \pgftransformshift{\pgfpoint{.5cm}{.5cm}}
%   \pgfpathmoveto{\pgfpointpolar{0}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{144}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{288}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{72}{4mm}}
%   \pgfpathlineto{\pgfpointpolar{216}{4mm}}
%   \pgfpathclose%
%   \pgfusepath{stroke,fill}
% }

\def\pgfdeclarepatterninherentlycolored#1#2#3#4#5{\pgf@declarepattern{#1}{#2}{#3}{#4}{#5}{1}}

\def\pgf@declarepattern#1#2#3#4#5#6{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}{%
  \pgfsysprotocol@getcurrentprotocol\pgf@pattern@temp%
  {%
    \pgfinterruptpath%
      \pgfpicturetrue%
      \pgf@relevantforpicturesizefalse%
      \pgftransformreset%
      \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
      \pgfsysprotocol@bufferedtrue%
      \pgfsys@beginscope%
      #5%
      \pgfsys@endscope%
      \pgfsysprotocol@getcurrentprotocol\pgf@pattern@code%
      \global\let\pgf@pattern@code=\pgf@pattern@code%
    \endpgfinterruptpath%
    \pgf@process{#2}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#3}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#4}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    % Now, build a name for the pattern
    \pgfutil@tempcnta=\pgf@pattern@number%
    \advance\pgfutil@tempcnta by1\relax%
    \xdef\pgf@pattern@number{\the\pgfutil@tempcnta}%
    \expandafter\xdef\csname pgf@pattern@name@#1\endcsname{\the\pgfutil@tempcnta}%
    \expandafter\gdef\csname pgf@pattern@type@#1\endcsname{#6}%
    \xdef\pgf@marshal{\noexpand\pgfsys@declarepattern
      {\csname pgf@pattern@name@#1\endcsname}
      {\the\pgf@xa}{\the\pgf@ya}{\the\pgf@xb}{\the\pgf@yb}{\the\pgf@xc}{\the\pgf@yc}{\pgf@pattern@code}{#6}}%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgf@pattern@temp%
  \expandafter\global\expandafter\let\csname pgf@pattern@instantiate@#1\endcsname=\pgf@marshal%
  }
  {%
    \PackageError{pgfbasepatterns}{Pattern `#1' already defined}{}%
  }%
}

\def\pgf@pattern@number{0}%

\def\pgf@ifpatternisinherentlycolored#1#2#3{%
  \expandafter\ifnum\csname pgf@pattern@type@#1\endcsname=1\relax#2\else#3\fi%
}



% Set an pattern as fill color
%
% #1 = Name of the pattern
% #2 = Color to be used for the pattern. If the pattern is already
%      colored, this parameter is ignored.
%
% Description:
%
% Sets the pattern for subsequent filling operations.
%
% Example:
%
% \pgfsetfillpattern{stars}{red}

\def\pgfsetfillpattern#1#2{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}{%
    \PackageError{pgfbasepatterns}{Undefined pattern `#1'}{}}
  {%
    \csname pgf@pattern@instantiate@#1\endcsname%
    \expandafter\global\expandafter\let\csname pgf@pattern@instantiate@#1\endcsname=\relax%
    \pgf@ifpatternisinherentlycolored{#1}{%
      \pgfsys@setpatterncolored{\csname pgf@pattern@name@#1\endcsname}%
    }{%
      \pgfutil@colorlet{pgf@tempcolor}{#2}%
      \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
      \pgfutil@extractcolorspec{pgf@tempcolor}{\pgf@tempcolor}%
      \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
      \expandafter\pgf@set@fill@patternuncolored\pgf@rgbcolor\relax{#1}%
    }%
  }%
}
\def\pgf@set@fill@patternuncolored#1,#2,#3\relax#4{%
  \pgfsys@setpatternuncolored{\csname pgf@pattern@name@#4\endcsname}{#1}{#2}{#3}%
}




\endinput


==> pgfcorepoints.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorepoints.code.tex,v 1.13 2008/02/03 19:37:26 tantau Exp $

\newdimen\pgf@picminx
\newdimen\pgf@picmaxx
\newdimen\pgf@picminy
\newdimen\pgf@picmaxy

\newdimen\pgf@pathminx
\newdimen\pgf@pathmaxx
\newdimen\pgf@pathminy
\newdimen\pgf@pathmaxy

\newif\ifpgf@relevantforpicturesize

\def\pgf@process#1{{#1\global\pgf@x=\pgf@x\global\pgf@y=\pgf@y}}

% Save a point.
%
% #1 = macro for storing point.
% #2 = code for point (should define x and y)
%
% Example:
%
% \pgfextract@process\mypoint{\pgf@x=10pt \pgf@y10pt}
% \pgfextract@process\myarcpoint{\pgfpointpolar{30}{5cm and 2cm}}

\def\pgfextract@process#1#2{%
	\pgf@process{#2}%
	\edef#1{\noexpand\pgf@x\the\pgf@x\noexpand\pgf@y\the\pgf@y}%
}
% This needed until old shapes code changed.
\let\pgfsavepgf@process\pgfextract@process%


% Return a point
%  
% #1 = x-coordinate of the point 
% #2 = y-coordinate of the point 
%  
% x = #1
% y = #2
%
% Example:
%
% \pgfpathmoveto{\pgfpoint{2pt+3cm}{3cm}}

\def\pgfpoint#1#2{%
  \pgfmathsetlength\pgf@x{#1}%
  \pgfmathsetlength\pgf@y{#2}\ignorespaces}


% Quickly a point
%  
% #1 = x-coordinate of the point (no calculations done)
% #2 = y-coordinate of the point (no calculations done)
%  
% x = #1
% y = #2
%
% Example:
%
% \pgfpathmoveto{\pgfqpoint{2pt}{3cm}}

\def\pgfqpoint#1#2{\pgf@x=#1\pgf@y=#2}



% Return the origin.
%  
% x = 0
% y = 0
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}

\def\pgfpointorigin{\pgf@x=0pt\pgf@y=\pgf@x\ignorespaces}



% Return a transformed point
%  
% #1 = a point
%
% Description:
%
% This command applies pgf's current transformation matrix to the
% given point. Normally, this is done automatically by commands like
% lineto or moveto, but sometimes you may wish to access a transformed
% point yourself. In the below example, this command is used for a low level
% coordinate system shift.
%
% In addition to applying the transformation matrix to the given
% point, this function also applies the pre- and post-morphing
% macros. 
%
% Example:
%
% \begin{pgflowleveltransformshiftscope}{\pgfpointtransformed{\pgfpointorigin}}
%   \pgfbox[center,center]{Hi!}
% \end{pgflowleveltransformshiftscope}

\def\pgfpointtransformed#1{%
  \pgf@process{%
    #1%
    \pgfmorph@prelist%
    \pgf@pos@transform{\pgf@x}{\pgf@y}%
    \pgfmorph@postlist%
  }%
}


% Return the difference vector of two points.
%  
% #1 = start of vector  
% #2 = end of vector  
%  
% x = x-component of difference 
% y = y-component of difference 
%
% Example:
%
% \pgfpathmoveto{\pgfpointdiff{\pgfpointxy{1}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointdiff#1#2{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \advance\pgf@x by-\pgf@xa\relax%
  \advance\pgf@y by-\pgf@ya\relax\ignorespaces}

% Add two vectors. 
%  
% #1 = first vector  
% #2 = second vector  
%  
% x = x-component of addition
% y = y-component of addition
%
% Example:
%
% \pgfpathmoveto{\pgfpointadd{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointadd#1#2{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya}



% Multiply a vector by a factor.
%  
% #1 = factor  
% #2 = vector  
%
% Example:
%
% \pgfpointscale{2}{\pgfpointxy{0}{1}}

\def\pgfpointscale#1#2{%
  \pgf@process{#2}%
  \pgf@x=#1\pgf@x%
  \pgf@y=#1\pgf@y%
}


% The intersection of two lines
%  
% #1 = point on first line
% #2 = another point on first line
% #3 = point on second line
% #4 = another point on second line
%
% Returns the intersection of the two lines. If there is no
% intersection or if the points #1 and #2 or the points #3 and #4 are
% identical, the behaviour is not specified.
%
% Example:
%
% \pgfpointintersectionoflines{\pgfpointxy{0}{1}}{\pgfpointxy{1}{0}}{\pgfpointxy{2}{2}}{\pgfpointxy{3}{4}}

\def\pgfpointintersectionoflines#1#2#3#4{%
  {
    % 
    % Compute orthogonal vector to #1--#2
    % 
    \pgf@process{#2}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{#1}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgf@ya=-\pgf@ya%
    % Normalise a bit
    \c@pgf@counta=\pgf@xa%
    \ifnum\c@pgf@counta<0\relax%
      \c@pgf@counta=-\c@pgf@counta\relax%
    \fi%
    \c@pgf@countb=\pgf@ya%
    \ifnum\c@pgf@countb<0\relax%
      \c@pgf@countb=-\c@pgf@countb\relax%
    \fi%
    \advance\c@pgf@counta by\c@pgf@countb\relax%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta>0\relax%
      \divide\pgf@xa by\c@pgf@counta\relax%
      \divide\pgf@ya by\c@pgf@counta\relax%
    \fi%
    %
    % Compute projection
    %
    \pgf@xc=\pgf@sys@tonumber{\pgf@ya}\pgf@x%
    \advance\pgf@xc by\pgf@sys@tonumber{\pgf@xa}\pgf@y%
    % 
    % The orthogonal vector is (\pgf@ya,\pgf@xa)
    % 
    % 
    % Compute orthogonal vector to #3--#4
    % 
    \pgf@process{#4}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{#3}%
    \advance\pgf@xb by-\pgf@x%
    \advance\pgf@yb by-\pgf@y%
    \pgf@yb=-\pgf@yb%
    % Normalise a bit
    \c@pgf@counta=\pgf@xb%
    \ifnum\c@pgf@counta<0\relax%
      \c@pgf@counta=-\c@pgf@counta\relax%
    \fi%
    \c@pgf@countb=\pgf@yb%
    \ifnum\c@pgf@countb<0\relax%
      \c@pgf@countb=-\c@pgf@countb\relax%
    \fi%
    \advance\c@pgf@counta by\c@pgf@countb\relax%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta>0\relax%
      \divide\pgf@xb by\c@pgf@counta\relax%
      \divide\pgf@yb by\c@pgf@counta\relax%
    \fi%
    %
    % Compute projection
    %
    \pgf@yc=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
    \advance\pgf@yc by\pgf@sys@tonumber{\pgf@xb}\pgf@y%
    % 
    % The orthogonal vector is (\pgf@yb,\pgf@xb)
    % 
    % Setup transformation matrx (this is just to use the matrix
    % inversion)
    % 
    \pgfsettransform{{\pgf@sys@tonumber\pgf@ya}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@xb}{0pt}{0pt}}%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{\pgfpoint{\pgf@xc}{\pgf@yc}}}%
  }%
}


% The intersection of two circles
%  
% #1 = center of first circle
% #2 = center of second circle
% #3 = radius of first circle
% #4 = radius of second circle
% #5 = solution number
%
% Returns the intersection of the two circles. If #5 is to "1", the
% first intersection is returned, otherwise the second. If the circles
% do not intersect, an error may occur.
%
% Example:
%
% \pgfpointintersectionofcircles{\pgfpointxy{0}{1}}{\pgfpointxy{1}{0}}{1cm}{1cm}{1}

\def\pgfpointintersectionofcircles#1#2#3#4#5{%
  {%
    % Store first point in (xa,ya) and radius in xc.
    \pgf@process{#1}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgfmathsetlength{\pgf@xc}{#3}%
    % Store second point in (xb,yb) and radius in yc.
    \pgf@process{#2}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgfmathsetlength{\pgf@yc}{#4}%
    %
    % Ok, now make numbers smaller, in case they are too large
    %
    \c@pgf@counta=1\relax%
    \loop%
      \pgf@scale@downfalse%
      \ifdim\pgf@xc>50pt\relax%
        \pgf@scale@downtrue%
      \fi%
      \ifdim\pgf@yc>50pt\relax%
        \pgf@scale@downtrue%
      \fi%
    \ifpgf@scale@down%
      \multiply\c@pgf@counta by2\relax%
      \divide\pgf@xa by2\relax%
      \divide\pgf@ya by2\relax%
      \divide\pgf@xb by2\relax%
      \divide\pgf@yb by2\relax%
      \divide\pgf@xc by2\relax%
      \divide\pgf@yc by2\relax%
    \repeat%
    % The following code is taken from the Dr. Math internet forum:
    %
    % Let the centers be: (a,b), (c,d)
    % Let the radii be: r, s
    %
    % e = c - a                          [difference in x coordinates]
    % f = d - b                          [difference in y coordinates]
    % p = sqrt(e^2 + f^2)                [distance between centers]
    % k = (p^2 + r^2 - s^2)/(2p)         [distance from center 1 to line
    %                                     joining points of intersection]
    % x = a + ek/p + (f/p)sqrt(r^2 - k^2)
    % y = b + fk/p - (e/p)sqrt(r^2 - k^2)
    % OR
    % x = a + ek/p - (f/p)sqrt(r^2 - k^2)
    % y = b + fk/p + (e/p)sqrt(r^2 - k^2)
    %
    % Since we are running low on registers, use
    % \dimen0 for e
    % \dimen1 for f
    % \dimen2 for p
    % \dimen3 for p^2
    % \dimen4 for k
    % \dimen5 for 1/p
    % \dimen6 for sqrt(r^2 - k^2)
    % \dimen7 for k^2
    % \dimen8 for k/p
    % \dimen9 for sqrt(r^2 - k^2)/p
    % Also note that:
    % \pgf@xa for a
    % \pgf@ya for b
    % \pgf@xb for c
    % \pgf@yb for d
    % \pgf@xc for r
    % \pgf@yc for s
    %
    % Now:
    % e = c - a
    \dimen0=\pgf@xb%
    \advance\dimen0 by-\pgf@xa%
    % f = d - b
    \dimen1=\pgf@yb%
    \advance\dimen1 by-\pgf@ya%
    % p^2 = e^2 + f^2
    \pgf@x=\dimen0\relax%
    \pgf@x=\pgf@sys@tonumber{\pgf@x}\pgf@x%
    \dimen3=\pgf@x%
    \pgf@x=\dimen1\relax%
    \advance\dimen3 by\pgf@sys@tonumber{\pgf@x}\pgf@x%
    % p = sqrt(p^2)
    \pgfmathparse{sqrt(\the\dimen3)}%
    \dimen2=\pgfmathresult pt%
    % 1/p = 1/p
    \pgfmathreciprocal@{\pgfmathresult}%
    \dimen5=\pgfmathresult pt%
    % k = (p^2 + r^2 - s^2)/(2p)
    \dimen4=\dimen3\relax%
    \pgf@x=\pgf@xc%
    \advance\dimen4 by\pgf@sys@tonumber{\pgf@x}\pgf@x\relax%
    \pgf@x=\pgf@yc%
    \advance\dimen4 by-\pgf@sys@tonumber{\pgf@x}\pgf@x\relax%
    \dimen4=.5\dimen4%
    \dimen4=\pgf@sys@tonumber{\dimen5}\dimen4%
    % dimen7 is k^2
    \dimen7=\pgf@sys@tonumber{\dimen4}\dimen4\relax%
    % dimen6 is sqrt(r^2 - k^2)
    \pgfmathparse{sqrt(\pgf@sys@tonumber{\pgf@xc}\pgf@xc-\the\dimen7)}%
    \dimen6=\pgfmathresult pt%
    % dimen8 is k/p
    \dimen8=\pgf@sys@tonumber{\dimen4}\dimen5\relax%
    % dimen9 is sqrt(r^2 - k^2)/p
    \dimen9=\pgf@sys@tonumber{\dimen6}\dimen5\relax%
    \ifnum#5=1\relax%
      % x = a + ek/p + (f/p)sqrt(r^2 - k^2)
      \pgf@x=\pgf@xa%
      \advance\pgf@x by\pgf@sys@tonumber{\dimen0}\dimen8\relax%
      \advance\pgf@x by\pgf@sys@tonumber{\dimen1}\dimen9\relax%
      % y = b + fk/p - (e/p)sqrt(r^2 - k^2)
      \pgf@y=\pgf@ya%
      \advance\pgf@y by\pgf@sys@tonumber{\dimen1}\dimen8\relax%
        %temp
        \pgf@xb=\pgf@sys@tonumber{\dimen0}\dimen9%
        \pgf@xb=-\pgf@xb%
      \advance\pgf@y by\pgf@xb\relax%
    \else%  
      % x = a + ek/p - (f/p)sqrt(r^2 - k^2)
      \pgf@x=\pgf@xa%
      \advance\pgf@x by\pgf@sys@tonumber{\dimen0}\dimen8\relax%
        %temp
        \pgf@xb=\pgf@sys@tonumber{\dimen1}\dimen9%
        \pgf@xb=-\pgf@xb%
      \advance\pgf@x by\pgf@xb\relax%
      % y = b + fk/p + (e/p)sqrt(r^2 - k^2)
      \pgf@y=\pgf@ya%
      \advance\pgf@y by\pgf@sys@tonumber{\dimen1}\dimen8\relax%
      \advance\pgf@y by\pgf@sys@tonumber{\dimen0}\dimen9\relax%
    \fi%
    \pgf@x=\c@pgf@counta\pgf@x%
    \pgf@y=\c@pgf@counta\pgf@y%
    \pgf@process{}% get results outside
  }%
}
\newif\ifpgf@scale@down


% Returns point on a line from #2 to #3 at time #1.
%  
% #1 = a time, where 0 is the start and 1 is the end
% #2 = start point
% #3 = end point 
%  
% x = x-component of #1*start + (1-#1)*end
% y = y-component of #1*start + (1-#1)*end 
%
% Example:
%
% % Middle of (1,1) and (2,3)
% \pgfpathmoveto{\pgfpointlineattime{0.5}{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointlineattime#1#2#3{%
  \pgf@process{#3}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \advance\pgf@xa by-\pgf@x\relax%
  \advance\pgf@ya by-\pgf@y\relax%
  \advance\pgf@x by #1\pgf@xa\relax%
  \advance\pgf@y by #1\pgf@ya\relax%  
  \ignorespaces}


% Move point #2 #1 many units in the direction of #3.
%  
% #1 = a distance
% #2 = start point
% #3 = end point 
%  
% x = x-component of start + #1*(normalise(end-start))
% y = y-component of start + #1*(normalise(end-start))
% xa = #1*(normalise(end-start))
% ya = #1*(normalise(end-start))
%
% Example:
%
%
% \pgfpathmoveto{\pgfpointlineatdistance{2pt}{\pgfpointxy{0}{1}}{\pgfpointxy{2}{3}}}
% \pgfpathlineto{\pgfpointlineatdistance{3pt}{\pgfpointxy{2}{3}}{\pgfpointxy{0}{1}}}

\def\pgfpointlineatdistance#1#2#3{%
  \pgf@process{#2}%
  \pgf@xb=\pgf@x\relax% xb/yb = start point
  \pgf@yb=\pgf@y\relax%
  \pgf@process{#3}%
  \advance\pgf@x by-\pgf@xb\relax%
  \advance\pgf@y by-\pgf@yb\relax%
  \pgf@process{\pgfpointnormalised{}}% x/y = normalised vector
  \pgfmathsetlength\pgf@xa{#1}%
  \pgf@ya=\pgf@xa\relax%
  \pgf@xa=\pgf@sys@tonumber{\pgf@x}\pgf@xa%
  \pgf@ya=\pgf@sys@tonumber{\pgf@y}\pgf@ya%
  \pgf@x=\pgf@xb\relax%
  \pgf@y=\pgf@yb\relax%
  \advance\pgf@x by\pgf@xa\relax%
  \advance\pgf@y by\pgf@ya\relax%
  \ignorespaces}


% Returns point on a curve from #2 to #5 with controls #3 and #4 at time #1.
%  
% #1 = a time
% #2 = start point
% #3 = first control point
% #4 = second control point
% #5 = end point 
%  
% x = x-component of place on the curve at time t
% y = y-component of place on the curve at time t
%
% Additionally, (\pgf@xa,\pgf@ya) and (\pgf@xb,\pgf@yb) will be on a
% tangent to the point on the curve (this can be useful for computing
% a label rotation).
%
% Example:
%
% % Middle of (1,1) and (2,3)
% \pgfpathmoveto{\pgfpointcurveattime{0.5}{\pgfpointxy{0}{1}}{\pgfpointxy{1}{1}}{\pgfpointxy{1}{1}}{\pgfpointxy{2}{3}}}

\def\pgfpointcurveattime#1#2#3#4#5{%
  \pgfmathparse{#1}%
  \let\pgf@time@s=\pgfmathresult%
  \pgf@x=\pgfmathresult pt%
  \pgf@x=-\pgf@x%
  \advance\pgf@x by 1pt%
  \edef\pgf@time@t{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@process{#5}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgf@process{#4}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#3}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  % First iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  \pgf@xb=\pgf@time@t\pgf@xb\advance\pgf@xb by\pgf@time@s\pgf@xc%
  \pgf@yb=\pgf@time@t\pgf@yb\advance\pgf@yb by\pgf@time@s\pgf@yc%
  % Second iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  % Save x/y
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  % Third iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
}






% Internal registers
\newdimen\pgf@xx
\newdimen\pgf@xy
\newdimen\pgf@yx
\newdimen\pgf@yy
\newdimen\pgf@zx
\newdimen\pgf@zy



% A polar coordinate
%
% #1 = a degree
% #2 = a radius -- either a dimension or two dimensions separated by 
%      " and ". 
%
% x = (first dimension in #2) * cos(#1)
% y = (second dimension in #2) * sin(#2)
% 
% Example:
%
% \pgfpathmoveto{\pgfpointpolar{30}{1cm}}
% \pgfpathlineto{\pgfpointpolar{30}{1cm and 2cm}}

\def\pgfpointpolar#1#2{%
  \pgfutil@in@{and }{#2}%
  \ifpgfutil@in@%
    \pgf@polar@#2\@@%
  \else%
    \pgf@polar@#2 and #2\@@%
  \fi%  
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \pgf@x=\pgfmathresult\pgf@x%
  \pgfmathsin@{\pgfpoint@angle}%
  \pgf@y=\pgfmathresult\pgf@y%
}

\def\pgf@polar@#1and #2\@@{%
  \pgfmathsetlength{\pgf@y}{#2}%
  \pgfmathsetlength{\pgf@x}{#1}%  
}

% Quick version of the polar coordinate method

\def\pgfqpointpolar#1#2{%
  \pgf@x=#2%
  \pgf@y=\pgf@x%
  \pgfmathcos@{#1}%
  \pgf@x=\pgfmathresult\pgf@x%
  \pgfmathsin@{#1}%
  \pgf@y=\pgfmathresult\pgf@y\relax%
}




% A polar coordinate in the xy plane.
%
% #1 = a degree
% #2 = a radius given as a number or two radi
%
% result = (first dim in #2) * x-vector * cos(#1) +
%          (second dim in #2) * y-vector * sin(#1)
% 
% Example:
%
% \pgfpathmoveto{\pgfpointpolarxy{30}{2}}

\def\pgfpointpolarxy#1#2{%
  \pgfutil@in@{and }{#2}%
  \ifpgfutil@in@%
    \pgf@polarxy@#2\@@%
  \else%
    \pgf@polarxy@#2and #2\@@%
  \fi%  
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \pgf@xa=\pgfmathresult\pgf@xa%
  \pgfmathsin@{\pgfpoint@angle}%
  \pgf@ya=\pgfmathresult\pgf@ya%
  \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@xx%
  \advance\pgf@x by \pgf@sys@tonumber{\pgf@ya}\pgf@yx%
  \pgf@y=\pgf@sys@tonumber{\pgf@xa}\pgf@xy%
  \advance\pgf@y by \pgf@sys@tonumber{\pgf@ya}\pgf@yy}

\def\pgf@polarxy@#1and #2\@@{%
  \pgfmathsetlength{\pgf@xa}{#1}%
  \pgfmathsetlength{\pgf@ya}{#2}%
}



% A cylindrical coordinate.
%
% #1 = a degree
% #2 = a radius given as a number
% #3 = a height given as a number
%
% result = #2*(x-vector * cos(#1) + y-vector * sin(#1)) + #3*z-vector
% 
% Example:
%
% \pgfpathmoveto{\pgfpointcylindrical{30}{2}{1}}

\def\pgfpointcylindrical#1#2#3{%
  \pgfpointpolarxy{#1}{#2}%
  \pgfmathparse{#3}%
  \advance\pgf@x by \pgfmathresult\pgf@zx%
  \advance\pgf@y by \pgfmathresult\pgf@zy}


% A spherical coordinate.
%
% #1 = a longitude
% #2 = a latitude
% #3 = a radius
%
% result = #3*(cos(#2)*(x-vector * cos(#1) + y-vector * sin(#1)) + sin(#2)*z-vector)
% 
% Example:
%
% \pgfpathmoveto{\pgfpointspherical{30}{30}{2}}

\def\pgfpointspherical#1#2#3{%
  \pgfmathparse{#1}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathsin@{\pgfpoint@angle}%
  \pgf@xb=\pgfmathresult\pgf@xx%
  \pgf@yb=\pgfmathresult\pgf@xy%
  \pgfmathcos@{\pgfpoint@angle}%
  \advance\pgf@xb by \pgfmathresult\pgf@yx%
  \advance\pgf@yb by \pgfmathresult\pgf@yy%
  %
  \pgfmathparse{#2}%
  \let\pgfpoint@angle=\pgfmathresult%
  \pgfmathcos@{\pgfpoint@angle}%
  \pgf@xc=\pgfmathresult\pgf@xb%
  \pgf@yc=\pgfmathresult\pgf@yb%
  \pgfmathsin@{\pgfpoint@angle}%
  \advance\pgf@xc by \pgfmathresult\pgf@zx%
  \advance\pgf@yc by \pgfmathresult\pgf@zy%
  \pgfmathparse{#3}%
  \pgf@x=\pgfmathresult\pgf@xc%
  \pgf@y=\pgfmathresult\pgf@yc\relax%
}


% Store the vector #1 * x-vec + #2 * y-vec
%
% #1 = a factor for the x-vector
% #2 = a factor fot the y-vector
%
% x = x-component of result vector
% y = y-component of result vector
%
% Description:
% 
% This command can be used to create a new coordinate system
% without using the rotate/translate/scale commands. This
% may be useful, if you do not want arrows and line width to
% be scaled/transformed together with the coordinate system.
% 
% Example:
%
% % Create a slanted rectangle
%
% \pgfsetxvec{\pgfpoint{1cm}{1cm}}
% \pgfsetyvec{\pgfpoint{0cm}{1cm}}
% 
% \pgfpathmoveto{\pgfpointxy{0}{0}}
% \pgfpathlineto{\pgfpointxy{1}{0}}
% \pgfpathlineto{\pgfpointxy{1}{1}}
% \pgfpathlineto{\pgfpointxy{0}{1}}
% \pgfclosestroke

\def\pgfpointxy#1#2{%
  \pgfmathparse{#1}%
  \let\pgftemp@x=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgftemp@y=\pgfmathresult%
  \pgf@x=\pgftemp@x\pgf@xx%
  \advance\pgf@x by \pgftemp@y\pgf@yx%
  \pgf@y=\pgftemp@x\pgf@xy%
  \advance\pgf@y by \pgftemp@y\pgf@yy}


% Store the vector #1 * x-vec + #2 * y-vec + #3 * z-vec
%
% #1 = a factor for the x-vector
% #2 = a factor fot the y-vector
% #3 = a factor fot the z-vector
%
% x = x-component of result vector
% y = y-component of result vector
%
%
% Description:
% 
% This command allows you to use a 3d coordinate system.
% 
%
% Example:
%
% % Draw a cubus
% 
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{0}{0}{1}}
% \pgfline{\pgfpointxyz{0}{1}{0}}{\pgfpointxyz{0}{1}{1}}
% \pgfline{\pgfpointxyz{1}{0}{0}}{\pgfpointxyz{1}{0}{1}}
% \pgfline{\pgfpointxyz{1}{1}{0}}{\pgfpointxyz{1}{1}{1}}
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{0}{1}{0}}
% \pgfline{\pgfpointxyz{0}{0}{1}}{\pgfpointxyz{0}{1}{1}}
% \pgfline{\pgfpointxyz{1}{0}{0}}{\pgfpointxyz{1}{1}{0}}
% \pgfline{\pgfpointxyz{1}{0}{1}}{\pgfpointxyz{1}{1}{1}}
% \pgfline{\pgfpointxyz{0}{0}{0}}{\pgfpointxyz{1}{0}{0}}
% \pgfline{\pgfpointxyz{0}{0}{1}}{\pgfpointxyz{1}{0}{1}}
% \pgfline{\pgfpointxyz{0}{1}{0}}{\pgfpointxyz{1}{1}{0}}
% \pgfline{\pgfpointxyz{0}{1}{1}}{\pgfpointxyz{1}{1}{1}}

\def\pgfpointxyz#1#2#3{%
  \pgfmathparse{#1}%
  \let\pgftemp@x=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\pgftemp@y=\pgfmathresult%
  \pgfmathparse{#3}%
  \let\pgftemp@z=\pgfmathresult%
  \pgf@x=\pgftemp@x\pgf@xx%
  \advance\pgf@x by \pgftemp@y\pgf@yx%
  \advance\pgf@x by \pgftemp@z\pgf@zx%
  \pgf@y=\pgftemp@x\pgf@xy%
  \advance\pgf@y by \pgftemp@y\pgf@yy%
  \advance\pgf@y by \pgftemp@z\pgf@zy}




% Set the x-vector
%
% #1 = a point the is the new x-vector
%
% Example:
%
% \pgfsetxvec{\pgfpoint{1cm}{0cm}}

\def\pgfsetxvec#1{%
  \pgf@process{#1}%
  \pgf@xx=\pgf@x%
  \pgf@xy=\pgf@y%
  \ignorespaces}


% Set the y-vector
%
% #1 = a point the is the new y-vector
%
% Example:
%
% \pgfsetyvec{\pgfpoint{0cm}{1cm}}

\def\pgfsetyvec#1{%
  \pgf@process{#1}%
  \pgf@yx=\pgf@x%
  \pgf@yy=\pgf@y%
  \ignorespaces}


% Set the z-vector
%
% #1 = a point the is the new z-vector
%
% Example:
%
% \pgfsetzvec{\pgfpoint{-0.385cm}{-0.385cm}}

\def\pgfsetzvec#1{%
  \pgf@process{#1}%
  \pgf@zx=\pgf@x%
  \pgf@zy=\pgf@y%
  \ignorespaces}



% Default values
\pgfsetxvec{\pgfpoint{1cm}{0cm}}
\pgfsetyvec{\pgfpoint{0cm}{1cm}}
\pgfsetzvec{\pgfpoint{-0.385cm}{-0.385cm}}




% Normalise a point.
%
% #1 = point with coordinates (a,b)
%
% x  = a/\sqrt(a*a+b*b)
% y  = b/\sqrt(a*a+b*b)
%
% Example:
%
% \pgfpointnormalised{\pgfpointxy{2}{1}}

\def\pgfpointnormalised#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifdim\pgf@x<0pt\relax% move into first quadrant
    \pgf@x=-\pgf@x%
  \fi%
  \ifdim\pgf@y<0pt\relax%
    \pgf@y=-\pgf@y%
  \fi%
  \ifdim\pgf@x>\pgf@y% x > y
    % make point small
    \c@pgf@counta=\pgf@x%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta=0\relax%
      \c@pgf@counta=1\relax%
    \fi%
    \divide\pgf@x by\c@pgf@counta%
    \divide\pgf@y by\c@pgf@counta%
    \divide\pgf@xa by\c@pgf@counta%
    \divide\pgf@ya by\c@pgf@counta%
    % ok.
    \pgf@x=.125\pgf@x%
    \pgf@y=.125\pgf@y%
    \c@pgf@counta=\pgf@x%
    \c@pgf@countb=\pgf@y%
    \multiply\c@pgf@countb by 100%
    \ifnum\c@pgf@counta<64\relax%
      \pgf@x=1pt\relax%
      \pgf@y=0pt\relax%
    \else%
      \divide\c@pgf@countb by \c@pgf@counta%
      \pgf@x=\csname pgf@cosfrac\the\c@pgf@countb\endcsname pt%
      \pgf@xc=8192pt%
      \divide\pgf@xc by\c@pgf@counta%
      \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@ya%
      \pgf@y=\pgf@sys@tonumber{\pgf@x}\pgf@y%
    \fi%
    \ifdim\pgf@xa<0pt%
      \pgf@x=-\pgf@x%
    \fi%
  \else% x <= y
    % make point small
    \c@pgf@counta=\pgf@y%
    \divide\c@pgf@counta by 65536\relax%
    \ifnum\c@pgf@counta=0\relax%
      \c@pgf@counta=1\relax%
    \fi%
    \divide\pgf@x by\c@pgf@counta%
    \divide\pgf@y by\c@pgf@counta%
    \divide\pgf@xa by\c@pgf@counta%
    \divide\pgf@ya by\c@pgf@counta%
    % ok.
    \pgf@x=.125\pgf@x%
    \pgf@y=.125\pgf@y%
    \c@pgf@counta=\pgf@y%
    \c@pgf@countb=\pgf@x%
    \multiply\c@pgf@countb by 100%
    \ifnum\c@pgf@counta<64\relax%
      \pgf@y=1pt\relax%
      \pgf@x=0pt\relax%
    \else%
      \divide\c@pgf@countb by \c@pgf@counta%
      \pgf@y=\csname pgf@cosfrac\the\c@pgf@countb\endcsname pt%
      \pgf@xc=8192pt%
      \divide\pgf@xc by\c@pgf@counta%
      \pgf@x=\pgf@sys@tonumber{\pgf@xc}\pgf@xa%
      \pgf@x=\pgf@sys@tonumber{\pgf@y}\pgf@x%
    \fi%
    \ifdim\pgf@ya<0pt%
      \pgf@y=-\pgf@y%
    \fi%
  \fi\ignorespaces%
}





% A point on a rectangle in a certain direction.
%
% #1 = a point pointing in some direction (length should be about 1pt,
%      but need not be exact)
% #2 = upper right corner of a rectangle centered at the origin
%
% Returns the intersection of a line starting at the origin going in
% the given direction and the rectangle's border.
%
% Example:
%
% \pgfpointborderrectangle{\pgfpointnormalised{\pgfpointxy{2}{1}}
%   {\pgfpoint{1cm}{2cm}}

\def\pgfpointborderrectangle#1#2{%
  \pgf@process{#2}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#1}%
  % Ok, let's find out about the direction:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifnum\pgf@xa<0\relax% move into first quadrant
    \pgf@x=-\pgf@x%
  \fi%
  \ifnum\pgf@ya<0\relax%
    \pgf@y=-\pgf@y%
  \fi%
  \pgf@xc=.125\pgf@x%
  \pgf@yc=.125\pgf@y%
  \c@pgf@counta=\pgf@xc%
  \c@pgf@countb=\pgf@yc%
  \ifnum\c@pgf@countb<\c@pgf@counta%
    \ifnum\c@pgf@counta<255\relax%
      \pgf@y=\pgf@yb\relax%
      \pgf@x=0pt\relax%
    \else%
      \pgf@xc=8192pt%
      \divide\pgf@xc by\c@pgf@counta% \pgf@xc = 1/\pgf@x
      \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
      \pgf@y=\pgf@sys@tonumber{\pgf@xb}\pgf@y%
      \ifnum\pgf@y<\pgf@yb%
        \pgf@x=\pgf@xb%
      \else% rats, calculate intersection on upper side
        \ifnum\c@pgf@countb<255\relax%
          \pgf@x=\pgf@xb\relax%
          \pgf@y=0pt\relax%
        \else%
          \pgf@yc=8192pt%
          \divide\pgf@yc by\c@pgf@countb% \pgf@xc = 1/\pgf@x
          \pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
          \pgf@x=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
          \pgf@y=\pgf@yb%
        \fi%
      \fi%  
    \fi%
  \else%
    \ifnum\c@pgf@countb<255\relax%
      \pgf@x=\pgf@xb\relax%
      \pgf@y=0pt\relax%
    \else%
      \pgf@yc=8192pt%
      \divide\pgf@yc by\c@pgf@countb% \pgf@xc = 1/\pgf@x
      \pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
      \pgf@x=\pgf@sys@tonumber{\pgf@yb}\pgf@x%
      \ifnum\pgf@x<\pgf@xb%
        \pgf@y=\pgf@yb%
      \else%
        \ifnum\c@pgf@counta<255\relax%
          \pgf@y=\pgf@yb\relax%
          \pgf@x=0pt\relax%
        \else%
          \pgf@xc=8192pt%
          \divide\pgf@xc by\c@pgf@counta% \pgf@xc = 1/\pgf@x
          \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
          \pgf@y=\pgf@sys@tonumber{\pgf@xb}\pgf@y%
          \pgf@x=\pgf@xb%
        \fi%
      \fi%  
    \fi%
  \fi%  
  \ifnum\pgf@xa<0\relax\pgf@x=-\pgf@x\fi%
  \ifnum\pgf@ya<0\relax\pgf@y=-\pgf@y\fi%    
}




% An approximation to a point on an ellipse in a certain
% direction. Will be exact only if the ellipse is a circle. 
%
% #1 = a point pointing in some direction
% #2 = upper right corner of a bounding box for the ellipse
%
% Returns the intersection of a line starting at the origin going in
% the given direction and the ellipses border.
%
% Example:
%
% \pgfpointborderellipse{\pgfpointnormalised{\pgfpointxy{2}{1}}
%   {\pgfpoint{1cm}{2cm}}

\def\pgfpointborderellipse#1#2{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \ifdim\pgf@xa=\pgf@ya% circle. that's easy!
    \pgf@process{\pgfpointnormalised{#1}}%
    \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
    \pgf@y=\pgf@sys@tonumber{\pgf@xa}\pgf@y%
  \else%
    \ifdim\pgf@xa<\pgf@ya%
      % Ok, first, let's compute x/y:
      \c@pgf@countb=\pgf@ya%
      \divide\c@pgf@countb by65536\relax%
      \divide\pgf@x by\c@pgf@countb%
      \divide\pgf@y by\c@pgf@countb%
      \pgf@xc=\pgf@x%
      \pgf@yc=8192pt%
      \pgf@y=.125\pgf@y%
      \c@pgf@countb=\pgf@y%
      \divide\pgf@yc by\c@pgf@countb%
      \pgf@process{#1}%
      \pgf@y=\pgf@sys@tonumber{\pgf@yc}\pgf@y%
      \pgf@y=\pgf@sys@tonumber{\pgf@xc}\pgf@y%
      \pgf@process{\pgfpointnormalised{}}%
      \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
      \pgf@y=\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \else%
      % Ok, now let's compute y/x:
      \c@pgf@countb=\pgf@xa%
      \divide\c@pgf@countb by65536\relax%
      \divide\pgf@x by\c@pgf@countb%
      \divide\pgf@y by\c@pgf@countb%
      \pgf@yc=\pgf@y%
      \pgf@xc=8192pt%
      \pgf@x=.125\pgf@x%
      \c@pgf@countb=\pgf@x%
      \divide\pgf@xc by\c@pgf@countb%
      \pgf@process{#1}%
      \pgf@x=\pgf@sys@tonumber{\pgf@yc}\pgf@x%
      \pgf@x=\pgf@sys@tonumber{\pgf@xc}\pgf@x%
      \pgf@process{\pgfpointnormalised{}}%
      \pgf@x=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
      \pgf@y=\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \fi%  
  \fi%
}





% Extract the x-coordinate of a point to a dimensions
%  
% #1 = a TeX dimension
% #2 = a point
%
% Example:
%
% \newdimen\mydim
% \pgfextractx{\mydim}{\pgfpoint{2cm}{4pt}}
% % \mydim is now 2cm

\def\pgfextractx#1#2{%
  \pgf@process{#2}%
  #1=\pgf@x\relax}


% Extract the y-coordinate of a point to a dimensions
%  
% #1 = a TeX dimension
% #2 = a point
%
% Example:
%
% \newdimen\mydim
% \pgfextracty{\mydim}{\pgfpoint{2cm}{4pt}}
% % \mydim is now 4pt

\def\pgfextracty#1#2{%
  \pgf@process{#2}%
  #1=\pgf@y\relax}



\def\pgf@def#1#2#3{\expandafter\def\csname pgf@#1#2\endcsname{#3}}
\pgf@def{cosfrac}{0}{1}
\pgf@def{cosfrac}{1}{0.99995}    \pgf@def{cosfrac}{2}{0.9998}
\pgf@def{cosfrac}{3}{0.99955}    \pgf@def{cosfrac}{4}{0.999201}
\pgf@def{cosfrac}{5}{0.998752}   \pgf@def{cosfrac}{6}{0.998205}
\pgf@def{cosfrac}{7}{0.997559}   \pgf@def{cosfrac}{8}{0.996815}
\pgf@def{cosfrac}{9}{0.995974}   \pgf@def{cosfrac}{10}{0.995037}
\pgf@def{cosfrac}{11}{0.994004}  \pgf@def{cosfrac}{12}{0.992877}
\pgf@def{cosfrac}{13}{0.991656}  \pgf@def{cosfrac}{14}{0.990342}
\pgf@def{cosfrac}{15}{0.988936}  \pgf@def{cosfrac}{16}{0.987441}
\pgf@def{cosfrac}{17}{0.985856}  \pgf@def{cosfrac}{18}{0.984183}
\pgf@def{cosfrac}{19}{0.982424}  \pgf@def{cosfrac}{20}{0.980581}
\pgf@def{cosfrac}{21}{0.978653}  \pgf@def{cosfrac}{22}{0.976644}
\pgf@def{cosfrac}{23}{0.974555}  \pgf@def{cosfrac}{24}{0.972387}
\pgf@def{cosfrac}{25}{0.970143}  \pgf@def{cosfrac}{26}{0.967823}
\pgf@def{cosfrac}{27}{0.965429}  \pgf@def{cosfrac}{28}{0.962964}
\pgf@def{cosfrac}{29}{0.960429}  \pgf@def{cosfrac}{30}{0.957826}
\pgf@def{cosfrac}{31}{0.955157}  \pgf@def{cosfrac}{32}{0.952424}
\pgf@def{cosfrac}{33}{0.949629}  \pgf@def{cosfrac}{34}{0.946773}
\pgf@def{cosfrac}{35}{0.943858}  \pgf@def{cosfrac}{36}{0.940887}
\pgf@def{cosfrac}{37}{0.937862}  \pgf@def{cosfrac}{38}{0.934784}
\pgf@def{cosfrac}{39}{0.931655}  \pgf@def{cosfrac}{40}{0.928477}
\pgf@def{cosfrac}{41}{0.925252}  \pgf@def{cosfrac}{42}{0.921982}
\pgf@def{cosfrac}{43}{0.918669}  \pgf@def{cosfrac}{44}{0.915315}
\pgf@def{cosfrac}{45}{0.911922}  \pgf@def{cosfrac}{46}{0.90849}
\pgf@def{cosfrac}{47}{0.905024}  \pgf@def{cosfrac}{48}{0.901523}
\pgf@def{cosfrac}{49}{0.89799}   \pgf@def{cosfrac}{50}{0.894427}
\pgf@def{cosfrac}{51}{0.890835}  \pgf@def{cosfrac}{52}{0.887217}
\pgf@def{cosfrac}{53}{0.883573}  \pgf@def{cosfrac}{54}{0.879905}
\pgf@def{cosfrac}{55}{0.876216}  \pgf@def{cosfrac}{56}{0.872506}
\pgf@def{cosfrac}{57}{0.868777}  \pgf@def{cosfrac}{58}{0.865031}
\pgf@def{cosfrac}{59}{0.861269}  \pgf@def{cosfrac}{60}{0.857493}
\pgf@def{cosfrac}{61}{0.853704}  \pgf@def{cosfrac}{62}{0.849903}
\pgf@def{cosfrac}{63}{0.846092}  \pgf@def{cosfrac}{64}{0.842271}
\pgf@def{cosfrac}{65}{0.838444}  \pgf@def{cosfrac}{66}{0.834609}
\pgf@def{cosfrac}{67}{0.83077}   \pgf@def{cosfrac}{68}{0.826927}
\pgf@def{cosfrac}{69}{0.82308}   \pgf@def{cosfrac}{70}{0.819232}
\pgf@def{cosfrac}{71}{0.815383}  \pgf@def{cosfrac}{72}{0.811534}
\pgf@def{cosfrac}{73}{0.807687}  \pgf@def{cosfrac}{74}{0.803842}
\pgf@def{cosfrac}{75}{0.8}       \pgf@def{cosfrac}{76}{0.796162}
\pgf@def{cosfrac}{77}{0.792329}  \pgf@def{cosfrac}{78}{0.788502}
\pgf@def{cosfrac}{79}{0.784682}  \pgf@def{cosfrac}{80}{0.780869}
\pgf@def{cosfrac}{81}{0.777064}  \pgf@def{cosfrac}{82}{0.773268}
\pgf@def{cosfrac}{83}{0.769481}  \pgf@def{cosfrac}{84}{0.765705}
\pgf@def{cosfrac}{85}{0.761939}  \pgf@def{cosfrac}{86}{0.758185}
\pgf@def{cosfrac}{87}{0.754443}  \pgf@def{cosfrac}{88}{0.750714}
\pgf@def{cosfrac}{89}{0.746997}  \pgf@def{cosfrac}{90}{0.743294}
\pgf@def{cosfrac}{91}{0.739605}  \pgf@def{cosfrac}{92}{0.735931}
\pgf@def{cosfrac}{93}{0.732272}  \pgf@def{cosfrac}{94}{0.728628}
\pgf@def{cosfrac}{95}{0.724999}  \pgf@def{cosfrac}{96}{0.721387}
\pgf@def{cosfrac}{97}{0.717792}  \pgf@def{cosfrac}{98}{0.714213}
\pgf@def{cosfrac}{99}{0.710651}  \pgf@def{cosfrac}{100}{0.707107}



\endinput


==> pgfcorequick.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorequick.code.tex,v 1.2 2006/10/11 15:22:25 tantau Exp $

% Quick version of basic drawing commands. Most high-level commands
% are not available if these commands are used.

% Move current point to (#1,#2).
%
% #1 = x dimension of new current point
% #2 = y dimension of new current point
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqmoveto#1#2{\pgfsyssoftpath@moveto{#1}{#2}}


% Append a line to (#1,#2) to the current path.
%
% #1 = x dimension of target
% #2 = y dimension of target
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqlineto#1#2{\pgfsyssoftpath@lineto{#1}{#2}}


% Append a bezier spline to the current path.
%
% #1 = x dimension of first support point
% #2 = y dimension of first support point
% #3 = x dimension of second support point
% #4 = y dimension of second support point
% #5 = x dimension of target point
% #6 = y dimension of target point
% 
% Example:
%
% \pgfpathqmoveto{0pt}{0pt}
% \pgfpathqlineto{1pt}{1pt}
% \pgfpathqcurveto{2pt}{1pt}{2pt}{2pt}{3pt}{2pt}
% \pgfqstroke

\def\pgfpathqcurveto#1#2#3#4#5#6{\pgfsyssoftpath@curveto{#1}{#2}{#3}{#4}{#5}{#6}}




% Append a circle of the given radius around the origin.
%
% #1 = radius
% 
% Example:
%
% \pgfpathqcircle{10pt}
% is quicker than
% \pgfpathcircle{\pgforigin}{10pt}

\def\pgfpathqcircle#1{%
  {%
    \pgf@x=#1%
    \pgf@y=0.555\pgf@x%
    \pgfsyssoftpath@moveto{\the\pgf@x}{0pt}%
    \pgfsyssoftpath@curveto{\the\pgf@x}{\the\pgf@y}{\the\pgf@y}{\the\pgf@x}{0pt}{\the\pgf@x}%
    \pgfsyssoftpath@curveto{-\the\pgf@y}{\the\pgf@x}{-\the\pgf@x}{\the\pgf@y}{-\the\pgf@x}{0pt}%
    \pgfsyssoftpath@curveto{-\the\pgf@x}{-\the\pgf@y}{-\the\pgf@y}{-\the\pgf@x}{0pt}{-\the\pgf@x}%
    \pgfsyssoftpath@curveto{\the\pgf@y}{-\the\pgf@x}{\the\pgf@x}{-\the\pgf@y}{\the\pgf@x}{0pt}%
    \pgfsyssoftpath@closepath%
  }%
}



% Stroke current path. No hooks called.
% 
% Example:
%
% \pgfpathqmoveto{0cm}{0cm}
% \pgfpathqlineto{1cm}{1cm}
% \pgfpathqcurveto{2cm}{1cm}{2cm}{2cm}{3cm}{2cm}
% \pgfqstroke

\def\pgfusepathqstroke{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@stroke%
  \pgf@resetpathsizes%
}


% Quickly fill current path.

\def\pgfusepathqfill{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@fill%
  \pgf@resetpathsizes%
}


% Quickly fill and stroke current path.

\def\pgfusepathqfillstroke{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@fillstroke%
  \pgf@resetpathsizes%
}

% Quickly clip current path.

\def\pgfusepathqclip{%
  \pgfsyssoftpath@flushcurrentpath%
  \pgfsys@clipnext%
  \pgfsys@discardpath%
  \pgf@resetpathsizes%
}


\endinput


==> pgfcorescopes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcorescopes.code.tex,v 1.26 2008/01/15 10:27:34 tantau Exp $

% Globals

\newbox\pgfpic
\newbox\pgf@hbox

\newbox\pgf@layerbox@main

\newcount\pgf@picture@serial@count



% This if decides whether the position of pictures on the page is
% protocolled or not. Normally,
% this is switched off as it works only with certain drivers and it
% causes external files to be written. When switched on, the position
% of pgfpictures are protocolled and can be referenced using
% \pgfsys@getposition{XXX} where XXX is the value of \pgfpictureid
% inside the picture.
\newif\ifpgfrememberpicturepositiononpage



% Library files inclusion


% Include a library file.
%
% #1 = List of names of library file.
%  
% Description:
%
% This command includes a list of library files. For each file X in the
% list, the file pgflibraryX.code.tex is included, provided this has
% not been done earlier. 
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgflibrary{arrows}
% \usepgflibrary[patterns,snakes]

\def\usepgflibrary{\pgfutil@ifnextchar[{\use@pgflibrary}{\use@@pgflibrary}}%}
\def\use@pgflibrary[#1]{\use@@pgflibrary{#1}}
\def\use@@pgflibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\ifx\csname pgf@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \input pgflibrary\pgf@temp.code.tex
      \catcode`\@=\csname pgf@library@#1@atcode\endcsname
      \catcode`\|=\csname pgf@library@#1@barcode\endcsname
    \fi%
  }%
}


% Include a module file.
%
% #1 = List of names of module files.
%  
% Description:
%
% This command includes a list of module files. For each file X in the
% list, the file pgfmoduleX.code.tex is included, provided this has
% not been done earlier. 
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgfmodule{matrix}

\def\usepgfmodule{\pgfutil@ifnextchar[{\use@pgfmodule}{\use@@pgfmodule}}%}
\def\use@pgfmodule[#1]{\use@@pgfmodule{#1}}
\def\use@@pgfmodule#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\ifx\csname pgf@module@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@module@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@module@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@module@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \input pgfmodule\pgf@temp.code.tex
      \catcode`\@=\csname pgf@module@#1@atcode\endcsname
      \catcode`\|=\csname pgf@module@#1@barcode\endcsname
    \fi%
  }%
}



% Scopes


% Pgf scope environment. All changes of the graphic state are local to
% the scope.
%  
% Example:
%
% \begin{pgfscope}
%    \pgfsetlinewidth{3pt}
%    \pgfline{\pgfxy(0,0)}{\pgfxy(3,3)}
% \end{pgfscope}

\def\pgfscope{%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \pgfsys@beginscope%
    \pgf@resetpathsizes%
    \edef\pgfscope@linewidth{\the\pgflinewidth}%
    \begingroup}
\def\endpgfscope{%
    \endgroup%
    \global\pgflinewidth=\pgfscope@linewidth%
  \pgfsys@endscope}




% Quickly insert a box can contain normal TeX text at the origin.
% 
% #1 = box of width/height and depth 0pt
% 
% Example:
%
% \pgfqbox{\mybox}

\def\pgfqbox#1{%
  \pgfsys@hbox#1%
} 


% Insert a box that can contain normal TeX text at the origin, but
% with the current coordinate transformation matrix synced with the
% low-level transformation matrix.
% 
% #1 = box of width/height and depth 0pt
%
% In essence, this command does the same as if you first said
% \pgflowlevelsynccm and then \pgfqbox. However, pgf will use a
% ``TeX-translation'' for the translation part of the transformation
% cm. This will ensure that hyperlinks ``survive'' at least
% translations. 
% 
% Example:
%
% \pgfqboxsynced{\mybox}

\def\pgfqboxsynced#1{%
  \pgfsys@hboxsynced#1%
}


% Puts some text in a box and inserts it with the current
% transformations applied.
% 
% #1 = List of optional positioning. Possible values are ``left'', ``right'',
%      ``top'', ``bottom'' and ``base''.
% #2 = TeX text. May contain verbatims.
% 
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{0cm}}
% \pgftext{Hello World!}

\def\pgftext{\pgfutil@ifnextchar[\pgf@text{\pgf@text[]}}%
\def\pgf@text[#1]{%
  \def\pgf@text@options{#1}%
  \pgf@maketext\pgf@after@text}
\def\pgf@after@text{%
  {%
  \def\pgf@text@hshift{center}%
  \def\pgf@text@vshift{center}%
  \expandafter\pgf@text@setkeys\expandafter{\pgf@text@options}%
  \csname pgf@halign\pgf@text@hshift\endcsname%
  \csname pgf@valign\pgf@text@vshift\endcsname%
  % Protocol sizes:
  \pgf@process{\pgfpointtransformed{\pgfqpoint{0pt}{\dp\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{\wd\pgf@hbox}{\dp\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{0pt}{\ht\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgf@process{\pgfpointtransformed{\pgfqpoint{\wd\pgf@hbox}{\ht\pgf@hbox}}}%
  \pgf@protocolsizes{\pgf@x}{\pgf@y}%
  \pgfqboxsynced{\pgf@hbox}%
  }%
}
\def\pgf@text@setkeys{\pgfqkeys{/pgf/text}}%

\pgfkeys{/pgf/text/left/.code=\def\pgf@text@hshift{left}}
\pgfkeys{/pgf/text/center/.code=}
\pgfkeys{/pgf/text/right/.code=\def\pgf@text@hshift{right}}
\pgfkeys{/pgf/text/top/.code=\def\pgf@text@vshift{top}}
\pgfkeys{/pgf/text/bottom/.code=\def\pgf@text@vshift{bottom}}
\pgfkeys{/pgf/text/base/.code=\def\pgf@text@vshift{base}}
\pgfkeys{/pgf/text/at/.cd,.code=\pgftransformshift{#1},.value required}
\pgfkeys{/pgf/text/x/.cd,.code=\pgftransformxshift{#1},.value required}
\pgfkeys{/pgf/text/y/.cd,.code=\pgftransformyshift{#1},.value required}
\pgfkeys{/pgf/text/rotate/.cd,.code=\pgftransformrotate{#1},.value required}

\def\pgf@halignleft{}% do nothing
\def\pgf@haligncenter{\pgftransformxshift{+-.5\wd\pgf@hbox}}
\def\pgf@halignright{\pgftransformxshift{+-\wd\pgf@hbox}}%
\def\pgf@valignbase{}% do nothing
\def\pgf@valignbottom{\pgftransformyshift{+\dp\pgf@hbox}}%
\def\pgf@valigncenter{\pgftransformyshift{+.5\dp\pgf@hbox}\pgftransformyshift{+-.5\ht\pgf@hbox}}%
\def\pgf@valigntop{\pgftransformyshift{+-\ht\pgf@hbox}}%


% Internal function for creating a hbox.
\def\pgf@maketext#1{%
  \def\pgf@@maketextafter{#1}%
  \setbox\pgf@hbox=\hbox\bgroup%
    \pgfinterruptpicture%
      \bgroup%
        \aftergroup\pgf@collectresetcolor%
        \let\next=%
}
\def\pgf@collectresetcolor{%
  \pgfutil@ifnextchar\reset@color%
  {\reset@color\afterassignment\pgf@collectresetcolor\let\pgf@temp=}%
  {\pgf@textdone}%
}
\def\pgf@textdone{%
    \endpgfinterruptpicture%
  \egroup%
  \pgf@@maketextafter%  
}

\long\def\pgf@makehbox#1{%
  \setbox\pgf@hbox=\hbox{{%
    \pgfinterruptpicture%
      #1%
    \endpgfinterruptpicture%
    }}}



% Picture environment
%
% Example:
%
% \begin{pgfpicture}
%   \pgfsetendarrow{\pgfarrowto}
%   \pgfpathmoveto{\pgfpointxy{-0.9}{0.2}}
%   \pgfpathlineto{\pgfpointxy{0.9}{0.4}}
%   \pgfusepath{stroke}
% \end{pgfpicture}

\newif\ifpgfpicture

\def\pgfpicture{%
  \begingroup%
    \pgfpicturetrue%
    \global\advance\pgf@picture@serial@count by1\relax%
    \edef\pgfpictureid{pgfid\the\pgf@picture@serial@count}%
    \let\pgf@nodecallback=\pgfutil@gobble%
    \pgf@picmaxx=-16000pt\relax%
    \pgf@picminx=16000pt\relax%
    \pgf@picmaxy=-16000pt\relax%
    \pgf@picminy=16000pt\relax%
    \pgf@relevantforpicturesizetrue%
    \pgf@resetpathsizes%
    \pgfutil@ifnextchar\bgroup\pgf@oldpicture\pgf@picture}
\def\pgf@oldpicture#1#2#3#4{%
  \pgfmathsetlength\pgf@picminx{#1}%
  \pgfmathsetlength\pgf@picminy{#2}%
  \pgfmathsetlength\pgf@picmaxx{#3}%
  \pgfmathsetlength\pgf@picmaxy{#4}%
  \pgf@relevantforpicturesizefalse%
  \pgf@picture}

\def\pgf@picture{%
  \setbox\pgfpic\hbox to0pt\bgroup%
    \begingroup%
    \pgfsys@beginpicture%
      \pgfsys@beginscope%
        \begingroup%
        \pgfsetcolor{.}%
        \pgfsetlinewidth{0.4pt}%
        \pgftransformreset%
        \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
        \begingroup%
          \let\pgf@setlengthorig=\setlength%
          \let\pgf@addtolengthorig=\addtolength%
          \let\pgf@selectfontorig=\selectfont%
          \let\setlength=\pgf@setlength%
          \let\addtolength=\pgf@addtolength%
          \let\selectfont=\pgf@selectfont%
          \nullfont\spaceskip\z@\xspaceskip\z@%
          \setbox\pgf@layerbox@main\hbox to0pt\bgroup%
            \begingroup%
  }
\def\endpgfpicture{%
              \ifpgfrememberpicturepositiononpage%
                \hbox to0pt{\pgfsys@markposition{\pgfpictureid}}%
              \fi%    
              % ok, now let's position the box
              \ifdim\pgf@picmaxx=-16000pt\relax%
                % empty picture. make size 0.  
                \global\pgf@picmaxx=0pt\relax%
                \global\pgf@picminx=0pt\relax%
                \global\pgf@picmaxy=0pt\relax%
                \global\pgf@picminy=0pt\relax%
              \fi%
              % Shift baseline outside:
              \pgf@relevantforpicturesizefalse%
              \pgf@process{\pgf@baseline}%
              \gdef\pgf@shift@baseline{\the\pgf@y}%
            \endgroup%
            \hss%
          \egroup%
          \pgf@insertlayers%
        \endgroup%    
        \pgfsys@discardpath%
        \endgroup%
      \pgfsys@endscope%
    \pgfsys@endpicture%
    \endgroup%
    \hss
  \egroup%
  \pgfsys@typesetpicturebox\pgfpic%
  \endgroup%
}

\def\pgf@insertlayers{%
  \box\pgf@layerbox@main%
}

\def\pgf@selectfont{\pgf@selectfontorig\nullfont}

\def\pgf@setlength#1#2{% these will be used only when \nullfont is active
  \begingroup% keep font setting local
    \pgfutil@selectfont% restore font
    \pgf@setlengthorig#1{#2}% calculate dimension (possibly using calc)
    \expandafter%
  \endgroup%
  \expandafter#1\expandafter=\the#1\relax}
\def\pgf@addtolength#1#2{%
  \begingroup% keep font setting local
    \pgfutil@selectfont% restore font
    \pgf@addtolengthorig#1{#2}% calculate dimension (possibly using calc)
    \expandafter%
  \endgroup%
  \expandafter#1\expandafter=\the#1\relax}


% Sets the baseline at the y-coordinate of a given point
%
% #1 = point
%
% Sets the baseline of the picture to the y-coordinate of a given
% point. However, the point will be evaluated *at the end of the
% picture*. 
%
% Example:
%
% \pgfsetbaselinepointlater{\pgfpointanchor{mynode}{base}}

\def\pgfsetbaselinepointlater#1{\def\pgf@baseline{#1}}


% Sets the baseline at the y-coordinate of a given point, now
%
% #1 = point
%
% Sets the baseline of the picture to the y-coordinate of a given
% point.
%
% Example:
%
% \pgfsetbaselinepointnow{\pgfpoint{1cm}{2pt}}

\def\pgfsetbaselinepointnow#1{%
  \pgf@process{#1}%
  \edef\pgf@setter@baseline{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}%
  \pgfsetbaselinepointlater{\pgf@setter@baseline}%
}


% Sets the baseline
%
% #1 = baseline
%
% Sets the baseline of the picture. Default is the lower border, which
% is the same as \pgf@picminy
%
% Example:
%
% \pgfsetbaseline{1cm+2pt}

\def\pgfsetbaseline#1{\pgfsetbaselinepointlater{\pgfpoint{0pt}{#1}}}
\pgfsetbaseline{\pgf@picminy}




% Interrupt path
%
% Description:
%
% The environment can be used to insert some drawing commands while
% constructing a path. The drawing commands inside the environment
% will not interfere with the path being constructed ``outside.''
% However, you must ward against graphic state changes using a scope. 
%
% Example: Draw two parallel lines
%
% \pgfmoveto{\pgfpoint{0cm}{0cm}}
% \begin{pgfinterruptpath}
%   \pgfmoveto{\pgfpoint{1cm}{0cm}}
%   \pgfmoveto{\pgfpoint{1cm}{1cm}}
%   \pgfusepath{stroke}
% \end{pgfinterruptpath}
% \pgflineto{\pgfpoint{0cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfinterruptpath
{%
  \begingroup%
  % save all sorts of things...
  \edef\pgf@interrupt@savex{\the\pgf@path@lastx}%
  \edef\pgf@interrupt@savey{\the\pgf@path@lasty}%
  \pgf@getpathsizes\pgf@interrupt@pathsizes%
  \pgfsyssoftpath@getcurrentpath\pgf@interrupt@path%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
  \edef\pgfscope@linewidth{\the\pgflinewidth}%
  \let\pgf@interrupt@lastmoveto=\pgfsyssoftpath@lastmoveto%
  \begingroup%
}
\def\endpgfinterruptpath
{%
  \endgroup%
  \global\pgflinewidth=\pgfscope@linewidth%
  \pgfsyssoftpath@setcurrentpath\pgf@interrupt@path%
  \pgf@setpathsizes\pgf@interrupt@pathsizes%
  \global\pgf@path@lastx=\pgf@interrupt@savex%
  \global\pgf@path@lasty=\pgf@interrupt@savey%
  \global\let\pgfsyssoftpath@lastmoveto=\pgf@interrupt@lastmoveto%
  \endgroup%
}



% Interrupt bounding box
%
% Description:
%
% The environment can be used to temporarily setup a new bounding box
% computation. The bounding box will be made empty at the beginning of
% the environment and will be reset to its old value after the
% environment. 
%
% Example: 
%
% \begin{pgfinterruptboundinbox}
%   \pgfmoveto{\pgfpoint{1cm}{0cm}}
%   \pgfmoveto{\pgfpoint{1cm}{1cm}}
%   \pgfusepath{stroke}
% \end{pgfinterruptboundinbox}

\def\pgfinterruptboundingbox
{%
  \begingroup%
    \edef\pgf@interrupt@savemaxx{\the\pgf@picmaxx}%
    \edef\pgf@interrupt@saveminx{\the\pgf@picminx}%
    \edef\pgf@interrupt@savemaxy{\the\pgf@picmaxy}%
    \edef\pgf@interrupt@saveminy{\the\pgf@picminy}%
    \pgf@picmaxx=-16000pt\relax%
    \pgf@picminx=16000pt\relax%
    \pgf@picmaxy=-16000pt\relax%
    \pgf@picminy=16000pt\relax%
}
\def\endpgfinterruptboundingbox
{%
    \global\pgf@picmaxx=\pgf@interrupt@savemaxx%
    \global\pgf@picmaxy=\pgf@interrupt@savemaxy%
    \global\pgf@picminx=\pgf@interrupt@saveminx%
    \global\pgf@picminy=\pgf@interrupt@saveminy%
  \endgroup%
}





% Interrupts a picture
%
% Description:
%
% This environment interrupts a picture and temporarily returns to
% normal TeX mode. All sorts of things are saved and restored by this
% environment.
%
% WARNING: Using this environment in conjuction with low level
% transformations can *strongly* upset the typesetting. Typically, the
% contents of this environment should have size/height/depth 0pt in
% the end.
%
% WARNING: This environment should only be used inside typesetting a
% box and this box must in turn be inserted using \pgfqbox.
%
% Example: Draw two parallel lines
%
% \pgfmoveto{\pgfpoint{0cm}{0cm}}
% \setbox\mybox=\hbox{
%    \begin{pgfinterruptpicture}
%      This is normal text.
%      \begin{pgfpicture} % a subpicture
%        \pgfmoveto{\pgfpoint{1cm}{0cm}}
%        \pgfmoveto{\pgfpoint{1cm}{1cm}}
%        \pgfusepath{stroke}
%      \end{pgfpicture}
%      More text.
%    \end{pgfinterruptpicture}
%  }
% \ht\mybox=0pt
% \wd\mybox=0pt
% \dp\mybox=0pt
% \pgfqbox{\mybox}%
% \pgfpathlineto{\pgfpoint{0cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfinterruptpicture
{%
  \begingroup%
    \pgfinterruptboundingbox%
      \pgftransformreset%
      \pgfinterruptpath%
        \ifx\pgf@selectfontorig\@undefined%
        \else%
          \let\setlength\pgf@setlengthorig%
          \let\addtolength\pgf@addtolengthorig%
          \let\selectfont\pgf@selectfontorig%
        \fi%
        \pgfutil@selectfont%
        \pgfpicturefalse%
        \pgf@savelayers%
}
\def\endpgfinterruptpicture
{%
        \pgf@restorelayers%
      \endpgfinterruptpath%
    \endpgfinterruptboundingbox%
  \endgroup%
}

\let\pgf@savelayers=\relax
\let\pgf@restorelayers=\relax


\endinput


==> pgfcoreshade.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoreshade.code.tex,v 1.9 2007/12/10 13:19:32 tantau Exp $

%
% Parsing functions
%
\newdimen\pgf@max
\newcount\pgf@sys@shading@range@num
\def\pgf@parsefunc#1{%
  \edef\temp{{#1}}%
  \expandafter\pgf@convertrgbstring\temp%
  \edef\temp{{\pgf@rgbconv}}%
  \expandafter\pgf@@parsefunc\temp}
\def\pgf@@parsefunc#1{%
  \let\pgf@bounds=\pgfutil@empty%
  \let\pgf@funcs=\pgfutil@empty%
  \let\pgf@psfuncs=\pgfutil@empty%
  \let\pgf@encode=\pgfutil@empty%
  \let\pgf@sys@shading@ranges=\pgfutil@empty%
  \pgf@sys@shading@range@num=0\relax%
  \pgf@parsefirst[#1; ]%
  \pgf@parselastdom[#1; ]%
  \pgf@parsemid[#1; ]%
  \ifx\pgf@bounds\pgfutil@empty%
    \edef\pgf@pdfparseddomain{0 1}%
    \edef\pgf@pdfparsedfunction{\pgf@singlefunc\space}%
  \else%
    \edef\pgf@pdfparseddomain{\pgf@doma\space\pgf@domb}%
    \edef\pgf@pdfparsedfunction{%
      << /FunctionType 3 /Domain [\pgf@doma\space\pgf@domb] /Functions
      [\pgf@funcs\space] /Bounds [\pgf@bounds] /Encode [0 1 \pgf@encode]
      >> }% <<
  \fi%
  \xdef\pgf@psfuncs{\pgf@psfuncs}%
  }
\def\pgf@parsefirst[rgb(#1)=(#2,#3,#4)#5]{%
  \pgfmathsetlength\pgf@x{#1}%
  \edef\pgf@sys@shading@start@pos{\the\pgf@x}%
  \pgf@sys@bp@correct\pgf@x%
  \edef\pgf@doma{\pgf@sys@tonumber{\pgf@x}}%
  \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
  \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
  \edef\pgf@sys@shading@start@rgb{\pgf@sys@rgb}%
  \let\pgf@sys@prevcolor=\pgf@sys@shading@start@rgb%
  \let\pgf@sys@prevpos=\pgf@sys@shading@start@pos%
  \edef\pgf@prevcolor{\pgf@rgb}%
  \edef\pgf@firstcolor{\pgf@rgb}}
\def\pgf@parselastdom[rgb(#1)=(#2,#3,#4); {%
  \pgfutil@ifnextchar]{%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@end@pos{\the\pgf@x}%
    \pgf@max=\pgf@x\relax%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@domb{\pgf@sys@tonumber{\pgf@x}}%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@sys@shading@end@rgb{\pgf@sys@rgb}%
    \pgfutil@gobble}{\pgf@parselastdom[}}
\def\pgf@parsemid[rgb(#1)=(#2,#3,#4); {\pgf@parserest[}
\def\pgf@parserest[rgb(#1)=(#2,#3,#4); {%
  \advance\pgf@sys@shading@range@num by1\relax%
  \pgfutil@ifnextchar]{%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@rgb\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgfmathsetlength\pgf@x{#1}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{{\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@rgb}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@rgb%
    \pgfutil@gobble}{%
    \pgfmathsetlength\pgf@x{#1}%
    \pgf@getrgbtuplewithmixin{#2}{#3}{#4}%
    \edef\pgf@sys@shading@ranges{\pgf@sys@shading@ranges{{\pgf@sys@prevpos}{\the\pgf@x}{\pgf@sys@prevcolor}{\pgf@sys@rgb}}}%
    \edef\pgf@sys@prevpos{\the\pgf@x}%
    \let\pgf@sys@prevcolor=\pgf@sys@rgb%
    \edef\pgf@psfuncs{\pgf@prevx\space \pgf@rgb\space \pgf@prevcolor\space pgfshade \pgf@psfuncs}%
    \pgf@sys@bp@correct\pgf@x%
    \edef\pgf@prevx{\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@bounds{\pgf@bounds\space\pgf@sys@tonumber{\pgf@x}}%
    \edef\pgf@encode{\pgf@encode\space0 1}%
    \edef\pgf@singlefunc{\space%
      << /FunctionType 2 /Domain [0 1] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@funcs{\pgf@funcs\space%
      << /FunctionType 2 /Domain [\pgf@doma\space\pgf@domb] /C0
      [\pgf@prevcolor] /C1 [\pgf@rgb] /N 1 >> }% <<
    \edef\pgf@prevcolor{\pgf@rgb}%
    \pgf@parserest[}}

\def\pgf@getrgbtuplewithmixin#1#2#3{%
  \pgfutil@definecolor{pgfshadetemp}{rgb}{#1,#2,#3}%
  \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgfshadetemp}}%
  \pgfutil@extractcolorspec{pgfshadetemp}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgf@getrgb@@\pgf@rgbcolor!}
\def\pgf@getrgb@@#1,#2,#3!{%
  \def\pgf@rgb{#1 #2 #3}%
  \def\pgf@sys@rgb{{#1}{#2}{#3}}%
}


\def\pgf@convertrgbstring#1{%
  \def\pgf@rgbconv{}%
  \pgf@converttorgb#1]%
  }
\def\pgf@converttorgb{%
  \pgfutil@ifnextchar]{\pgfutil@gobble}%done!
  {%
    \pgfutil@ifnextchar;{\pgf@grabsemicolor}%
    {%
      \pgfutil@ifnextchar r{\pgf@grabrgb}%
      {%
        \pgfutil@ifnextchar g{\pgf@grabgray}%
        {%
          \pgfutil@ifnextchar c{\pgf@grabcolor}%
          {\PackageError{pgfshade}{Illformed shading
              specification}{}\pgf@converttorgb}%
        }%
      }%
    }%
  }%
}
\def\pgf@grabsemicolor;{%
  \edef\pgf@rgbconv{\pgf@rgbconv; }\pgf@converttorgb}
\def\pgf@grabrgb rgb(#1)=(#2,#3,#4){%
  \edef\pgf@rgbconv{\pgf@rgbconv rgb(#1)=(#2,#3,#4)}\pgf@converttorgb}
\def\pgf@grabgray gray(#1)=(#2){%
  \edef\pgf@rgbconv{\pgf@rgbconv rgb(#1)=(#2,#2,#2)}\pgf@converttorgb}
\def\pgf@grabcolor color(#1)=(#2){%
  \pgfutil@colorlet{pgf@tempcol}{#2}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgf@convgetrgb@\expandafter{\pgf@rgbcolor}{#1}%
}
\def\pgf@convgetrgb@#1#2{%
  \edef\pgf@rgbconv{\pgf@rgbconv rgb(#2)=(#1)}\pgf@converttorgb}




% Declares a horizontal shading for later use. The shading is a
% horizontal bar that changes its color.
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = height of the shading
% #4 = color specification in the following format: A list of colors
%      that the bar should have at certain points. If the bar should
%      be red at 1cm, this is specified as
%      "rgb(1cm)=(1,0,0)". Multiple specifications are separated by a
%      semicolon and a space. At least two specifications must be
%      given. The specified positions must be given in increasing
%      order. 
%
% Description:
%
% The optional dependecies have the following effect: If present, it
% should consist of a list of colors, separated by commas. Each time
% the shading is used, these colors will be reevaluated. It will be
% checked whether the colors still have their "original meaning". If
% the colors have changed, a new shading will be created internally to
% reflect the changed color's values.
%
% Example:
%
% \pgfdeclarehorizontalshading{redtogreentoblue}{1cm}{%
%   rgb(0cm)=(1,0,0); % red
%   rgb(1cm)=(0,1,0); % green
%   rgb(2cm)=(0,0,1)}
%
% \begin{document}
%   The following bar is 2cm long: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclarehorizontalshading{\pgfutil@ifnextchar[\pgf@declarehorizontalshading{\pgf@declarehorizontalshading[]}}%
\def\pgf@declarehorizontalshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \pgfsys@horishading{#2}{#3}{#4}%
  \else%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@horishading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}


% Declares a vertical shading for later use. 
%
% #1 = optinal dependecies
% #2 = name of the shading for later use
% #3 = height of the shading
% #4 = color specification 
%
% Example:
%
% \pgfdeclareverticalshading{redtogreentoblue}{1cm}{%
%   rgb(0cm)=(1,0,0); % red
%   rgb(1cm)=(0,1,0); % green
%   rgb(2cm)=(0,0,1)}
%
% \begin{document}
%   The following bar is 2cm high: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclareverticalshading{\pgfutil@ifnextchar[\pgf@declareverticalshading{\pgf@declareverticalshading[]}}%
\def\pgf@declareverticalshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \pgfsys@vertshading{#2}{#3}{#4}%
  \else%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@vertshading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}


% Declares a radial shading for later use. 
%
% #1 = optional dependencies
% #2 = name of the shading for later use
% #3 = center of inner circle
% #4 = color specification 
%
% Description:
%
% A radial shading creates a smooth color transition between two
% circles. The center of the inner circle is at the give position. Its
% radius is the start of the color specification. The
% center of the outer circle is at the center of the whole shading,
% whose radius is the end of the color specification. For example,
% suppose the color specification is "rgb(1cm)=(1,1,1); rgb(2cm)=(0,0,0)".  
% Then the shading would be 4cm times 4cm large. The inner circle would
% have diameter 1cm and the outer circle would have diameter 2cm. The
% outer circle would be centered in the middle of the shading, whereas
% the outer circle would be centered at the given position.
%
% Example:
%
% \pgfdeclareradialshading{redtogreentoblue}{\pgfpoint{2cm}{2cm}}{%
%   rgb(10pt)=(1,0,0); % red
%   rgb(2cm)=(0,1,0); % green
%   rgb(3cm)=(0,0,1)}
%
% \begin{document}
%   The following ball has diameter 3cm: \pgfuseshading{redtogreentoblue}.
% \end{document}

\def\pgfdeclareradialshading{\pgfutil@ifnextchar[\pgf@declareradialshading{\pgf@declareradialshading[]}}%
\def\pgf@declareradialshading[#1]#2#3#4{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \pgfsys@radialshading{#2}{#3}{#4}%
  \else%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfsys@radialshading}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}




% Declares a functional shading for later use. 
%
% #1 = optional dependecies
% #2 = name of the shading for later use
% #3 = lower left corner of the shading as a pgfpoint.
% #4 = upper right corner of the shading as a pgfpoint.
% #5 = Preparation code
% #6 = a PDF type 4 function (restricted Postscript function), see the 
%      PDF-specification 1.7, section 3.9.4
%
% Description:
%
% This command creates a so-called functional shading. For such a
% shading the color of each point is calculated by calling a function
% for each point that gets the coordinates as input and yields the
% color as an output. Note that the function is evaluated by the
% *renderer*, not by PGF or TeX or someone else at compile-time. This
% means that the evaluation of this function has to be done *extremely
% quickly* and the funciton should be *very simple*. For this reason,
% only a very restricted set of operations are possible in the
% function (see 3.9.4 of the PDF-spec 1.7). Also functions should be
% kept small. Any errors in the function will only be noticed by the
% renderer.
%
% The function gets the coordinates of a point as input (as bp). This
% input consists of the top two elements of an otherwise empty
% (virtual, PostScript) stack. The function should then replace these
% two values by three values, representing the red, green, and blue
% color of the point. The numbers should be real values, not integers
% since Apple's PDF renderer is broken in this regard (use cvr at the
% end if necessary).
%
% Conceptually, the function will be evaluated once for each point of
% the rectangle (#3) to (#4). A renderer may choose to evaluate the
% function at less points, but, in principle, the function will be
% evaluated for each pixel independently.
%
% Because of the rather difficult PostScript syntax, use this macro
% only *if you know what you are doing* (or if you are advanterous, of
% course). 
%
% As for other shadings, the optional depencies argument is used to
% determine whether a shading needs to be recalculated when a color
% has changed.
%
% The code #5 is executed each time a shading is
% (re)calculated. Typically, it will contain code to extract
% coordinates from colors (see below).
%
% Inside the PostScript function #6 you cannot use colors
% directly. Rather, you must push the color components on the
% stack. For this, it is useful to call \pgfshadergb in the startup
% code #4. The macro takes a color name as input and stores the color's 
% red/green/blue components real numbers between 0.0 and 1.0 separated
% by spaces (which is exactly what you need if you want to push it on
% a stack) in a macro. 
%
% Example:
%
%\pgfdeclarefunctionalshading{twospots}{\pgfpointorigin}{\pgfpoint{200bp}{200bp}}{}{
%  2 copy
%  90 sub dup mul exch
%  80 sub dup mul add sqrt
%  dup mul neg 1.0005 exch exp 1.0 exch sub
%  3 1 roll
%  120 sub dup mul exch
%  100 sub dup mul add sqrt
%  dup mul neg 1.002 exch exp 1.0 exch sub
%  1.0
%}
%
% \pgfdeclarefunctionalshading[mycol]{sweep}{\pgfpointorigin}{\pgfpoint{100bp}{100bp}}
% {\pgfshadecolortorgb{mycol}{\myrgb}}{
%   add 150 div   % not very useful...
%   dup
%   \myrgb        % push mycol
%   5 4 roll      % multiply all components by calculated value
%   mul
%   3 1 roll
%   3 index
%   mul
%   3 1 roll
%   4 3 roll
%   mul
%   3 1 roll
% }
%
% \begin{document}
%   Have a look at this: \pgfuseshading{twospots}.
%   Here is \colorlet{mycol}{green!50}\pgfuseshading{sweep} in green
%   and in \colorlet{mycol}{red!50!blue}\pgfuseshading{sweep} in red/blue.
% \end{document}

\def\pgfdeclarefunctionalshading{\pgfutil@ifnextchar[\pgf@declarefunctionalshading{\pgf@declarefunctionalshading[]}}%
\def\pgf@declarefunctionalshading[#1]#2#3#4#5#6{%
  \expandafter\def\csname pgf@deps@pgfshading#2!\endcsname{#1}%
  \expandafter\ifx\csname pgf@deps@pgfshading#2!\endcsname\pgfutil@empty%
    \pgfshade@functionaldo{#2}{#3}{#4}{#5}{#6}%
  \else%
    \expandafter\def\csname pgf@func@pgfshading#2!\endcsname{\pgfshade@functionaldo}%
    \expandafter\def\csname pgf@args@pgfshading#2!\endcsname{{#3}{#4}{#5}{#6}}%
    \expandafter\let\csname @pgfshading#2!\endcsname=\pgfutil@empty%
  \fi}
\def\pgfshade@functionaldo#1#2#3#4#5{%
  {%
    #4%
    \pgfsys@functionalshading{#1}{#2}{#3}{#5}%
  }%
}

\def\pgfshadecolortorgb#1#2{%
  \pgfutil@colorlet{pgf@tempcol}{#1}%
  \pgfutil@extractcolorspec{pgf@tempcol}{\pgf@tempcolor}%
  \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
  \expandafter\pgfshading@rgb\pgf@rgbcolor\relax%
  \edef#2{\pgf@sys@tonumber{\pgf@xa}\space\pgf@sys@tonumber{\pgf@xb}\space\pgf@sys@tonumber{\pgf@xc}\space}%
}
\def\pgfshading@rgb#1,#2,#3\relax{%
  \pgf@xa=#1pt%
  \pgf@xb=#2pt%
  \pgf@xc=#3pt%
}




% Inserts a box into the text that contains a previously defined
% shading. 
%
% #1 = Name of a shading
%
% Example:
%
% \pgfuseshading{redtogreentoblue}

\def\pgfuseshading#1{%
  \edef\pgf@shadingname{@pgfshading#1}%
  \pgf@tryextensions{\pgf@shadingname}{\pgfalternateextension}%
  \expandafter\pgfutil@ifundefined\expandafter{\pgf@shadingname}%
  {\PackageError{pgfshade}{Undefined shading "#1"}{}}%
  {%
    {%
      \pgfutil@globalcolorsfalse%
      \def\pgf@shade@adds{}%
      \pgfutil@ifundefined{pgf@deps\pgf@shadingname}%
      {}%
      {%
        \edef\@list{\csname pgf@deps\pgf@shadingname\endcsname}%
        \pgfutil@for\@temp:=\@list\do{%
          {%
            \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{\@temp}}%
            \pgfutil@extractcolorspec{\@temp}{\pgf@tempcolor}%
            \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{rgb}{\pgf@rgbcolor}%
            \xdef\pgf@shade@adds{\pgf@shade@adds,\pgf@rgbcolor}%
          }%
        }%
      }%
      \expandafter\pgf@strip@shadename\pgf@shadingname!!%
      \pgfutil@ifundefined{@pgfshading\pgf@basename\pgf@shade@adds!}%
      {%
        {%
          \expandafter\def\expandafter\@temp\expandafter{\csname pgf@func\pgf@shadingname\endcsname}%
          \edef\@args{{\pgf@basename\pgf@shade@adds}}%
          \expandafter\expandafter\expandafter\def%
          \expandafter\expandafter\expandafter\@@args%
          \expandafter\expandafter\expandafter{\csname pgf@args\pgf@shadingname\endcsname}%
          \expandafter\expandafter\expandafter\@temp\expandafter\@args\@@args%
          %
        }%
      }%
      {}%
      \pgf@invokeshading{\csname @pgfshading\pgf@basename\pgf@shade@adds!\endcsname}%
    }%
  }%
}

\def\pgf@strip@shadename @pgfshading#1!!!{\def\pgf@basename{#1}}

\def\pgf@invokeshading#1{%
  \ifpgfpicture%
    \pgfsys@shadinginsidepgfpicture{#1}%
  \else%
    \pgfsys@shadingoutsidepgfpicture{#1}%  
  \fi%
}


% Create an alias name for a shading
%
% #1 = name of the alias
% #2 = name of the original
%
% Example:
%
% \pgfaliasshading{shading!25}{shadingshaded}

\def\pgfaliasshading#1#2{%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname @pgfshading#2!\endcsname%
  \expandafter\let\csname @pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@deps@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@deps@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@func@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@func@pgfshading#1!\endcsname=\pgf@temp%
  \expandafter\let\expandafter\pgf@temp\expandafter=\csname pgf@args@pgfshading#2!\endcsname%
  \expandafter\let\csname pgf@args@pgfshading#1!\endcsname=\pgf@temp%
}




% Shades the current path, but does not discard it.
%
% #1 - a shading (see below)
% #2 - an angle
%
% Description:
%
% \pgfshadepath  ``tries'' to fill the
% current path with a shading. The shading's original size should
% completely cover the area between (0,0) and (100bp,100bp). The
% shading will be rotated by #2 and then rescaled so that it
% completely covers the path. Then the path will be used (locally) for
% clipping and the shading is drawn.
%
% In addition to the rotation, any transformation set by the
%\pgfsetadditionalshadetransform will also be applied.
%
% After all this, the path can still be used for the normal
% stroking/clipping operations.
%
% The shading is rotated around its middle. If no rotation occurs, the
% lower left corner of the path will lie on (25bp, 25bp), the upper
% right corner on (75bp, 75bp).
%
% Example:
%
% \pgfdeclareverticalshading{myshading}{100bp}{color(0pt)=(red); color(100bp)=(green)}
%
% \pgfpathmoveto{\pgforigin}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfpathlineto{\pgfxy(1,1)}
% \pgfshadepath{myshading}{0}
% \pgfusepath{stroke}

\def\pgfshadepath#1#2{%
  \ifdim\pgf@pathminx=16000pt%
    \PackageWarning{pgfshade}{No path specified that can be filled}%
  \else%
    \begingroup%  
      \pgfsys@beginscope%
        % Calculate center:
        \pgf@xb=.5\pgf@pathmaxx%
        \advance\pgf@xb by.5\pgf@pathminx%
        \pgf@yb=.5\pgf@pathmaxy%
        \advance\pgf@yb by.5\pgf@pathminy%
        % Calculate scaling:
        \pgf@xc=\pgf@pathmaxx%
        \advance\pgf@xc by-\pgf@pathminx%
        \pgf@yc=\pgf@pathmaxy%
        \advance\pgf@yc by-\pgf@pathminy%
        \pgf@xc=.02\pgf@xc%
        \pgf@yc=.02\pgf@yc%
        \pgfsyssoftpath@invokecurrentpath%
        \pgfsys@clipnext%
        \pgfsys@discardpath%
        % Compute new transformation matrix:
        \pgfsys@transformcm{1}{0}{0}{1}{\pgf@xb}{\pgf@yb}%
        \pgfsys@transformcm%
        {\pgf@sys@tonumber{\pgf@xc}}{0}%
        {0}{\pgf@sys@tonumber{\pgf@yc}}{0pt}{0pt}%
        \pgfmathparse{#2}%
        \let\pgfshade@angle=\pgfmathresult%
        \pgfmathsin@{\pgfshade@angle}%
        \let\pgfshade@sin=\pgfmathresult%
        \pgfmathcos@{\pgfshade@angle}%
        \let\pgfshade@cos=\pgfmathresult%
        \pgf@x=\pgfshade@sin pt%
        \pgf@xa=-\pgf@x%
        \pgfsys@transformcm{\pgfshade@cos}{\pgfshade@sin}{\pgf@sys@tonumber{\pgf@xa}}{\pgfshade@cos}{0pt}{0pt}%
        \ifx\pgf@shade@extra@transform\pgfutil@empty%
        \else%
          \pgflowlevel{\pgf@shade@extra@transform}%
        \fi%
        \pgfuseshading{#1}%
      \pgfsys@endscope%
    \endgroup%
  \fi%
}


% Additionally transform shade paths
%
% #1 = Transformation code that is used in addition to the normal
%      shading transformation.
%
% Example:
%
% \pgfsetadditionalshadetransform{\pgftransformrotate{30}}

\def\pgfsetadditionalshadetransform#1{\def\pgf@shade@extra@transform{#1}}
\let\pgf@shade@extra@transform=\pgfutil@empty





\endinput


==> pgfcoretransformations.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoretransformations.code.tex,v 1.10 2008/02/04 17:19:54 tantau Exp $


% Position transformations

\newdimen\pgf@pt@x
\newdimen\pgf@pt@y

\newdimen\pgf@pt@temp

\newif\ifpgf@pt@identity
\pgf@pt@identitytrue

\def\pgf@pt@aa{1.0} \def\pgf@pt@ab{0.0}
\def\pgf@pt@ba{0.0} \def\pgf@pt@bb{1.0}



% Store the current transformation matrix in a macro.
%
% #1 = macro name
%
% Example:
%
% \pgfgettransform\mytransform

\def\pgfgettransform#1{%
  \edef#1{{\pgf@pt@aa}{\pgf@pt@ab}{\pgf@pt@ba}{\pgf@pt@bb}{\the\pgf@pt@x}{\the\pgf@pt@y}}
}


% Restore the current transformation matrix from a macro.
%
% #1 = macro name, previously used with \pgfgettransform
%
% Example:
%
% \pgfsettransform\mytransform

\def\pgfsettransform#1{%
  \edef\pgf@temp{#1}%
  \expandafter\pgf@settransform\pgf@temp%
}
\def\pgf@settransform#1#2#3#4#5#6{%
  \def\pgf@pt@aa{#1}%
  \def\pgf@pt@ab{#2}%
  \def\pgf@pt@ba{#3}%
  \def\pgf@pt@bb{#4}%
  \pgf@pt@x=#5%
  \pgf@pt@y=#6%
  \edef\pgf@idtest{#1,#2,#3,#4}%
  \ifx\pgf@idtest\pgf@idmatrixtext%
    \pgf@pt@identitytrue%
  \else%
    \pgf@pt@identityfalse%
  \fi%
}

\def\pgf@idmatrixtext{1.0,0.0,0.0,1.0}
\def\pgf@zerozerotext{0.0,0.0}

% Transformation command
%
% #1 = x dimension
% #2 = y dimension
%
% Description:
%
% Applies the pgfs transformation matrix to the point (#1,#2). The
% result is once more stored in the point.
%
%
% Example:
%
% \pgf@pos@transform{\pgf@x}{\pgf@y}

\def\pgf@pos@transform#1#2{%
  \ifpgf@pt@identity%
  \else%
    \pgf@pt@temp=#1%
    #1=\pgf@pt@aa#1%
    \advance#1 by\pgf@pt@ba#2%
    #2=\pgf@pt@bb#2%
    \advance#2 by\pgf@pt@ab\pgf@pt@temp%
  \fi%
  \advance#1 by\pgf@pt@x%
  \advance#2 by\pgf@pt@y%
}


% Invert the current transformation matrix
%
% Description:
%
% This command replaces the current transformation matrix by its
% inverse. The inversion is not very exact if the matrix is nearly
% singular. 
%
% Example:
%
% \pgftransforminvert

\def\pgftransforminvert{%
  % First, invert the shift. That's easy
  \pgf@pt@x=-\pgf@pt@x
  \pgf@pt@y=-\pgf@pt@y
  \ifpgf@pt@identity%
  \else%
    % Sigh. Have to calculate the inverse of the matrix.
    % Perhaps we are lucky and ba and bb are zero?
    \edef\pgf@zerotest{\pgf@pt@ab,\pgf@pt@ba}%
    \ifx\pgf@zerotest\pgf@zerozerotext%
      % Ha! Just invert aa and bb
      \pgfmathreciprocal@{\pgf@pt@aa}%
      \let\pgf@pt@aa\pgfmathresult%
      \pgfmathreciprocal@{\pgf@pt@bb}%
      \let\pgf@pt@bb\pgfmathresult%
    \else%
      % Start with determinant
      % Matrix = (aa ab
      %           ba bb)
      {%
        \pgfutil@tempdima=\pgf@pt@aa pt%
        \pgfutil@tempdima=\pgf@pt@bb\pgfutil@tempdima% aa * bb
        \pgfutil@tempdimb=\pgf@pt@ba pt%
        \pgfutil@tempdimb=\pgf@pt@ab\pgfutil@tempdimb% ba * ab
        \advance\pgfutil@tempdima by -\pgfutil@tempdimb% aa*bb - ba*ab
        % Invert
        \pgfmathreciprocal@{\pgf@sys@tonumber{\pgfutil@tempdima}}%
        \pgfutil@tempdima=\pgfmathresult pt%
        \pgf@x=\pgf@pt@bb\pgfutil@tempdima% bb/(det A)
        \xdef\pgf@new@pt@aa{\pgf@sys@tonumber{\pgf@x}}%
        \pgf@x=\pgf@pt@aa\pgfutil@tempdima% aa/(det A)
        \xdef\pgf@new@pt@bb{\pgf@sys@tonumber{\pgf@x}}%
        \pgfutil@tempdima=-\pgfutil@tempdima%
        \pgf@x=\pgf@pt@ba\pgfutil@tempdima% -ba/(det A)
        \xdef\pgf@new@pt@ba{\pgf@sys@tonumber{\pgf@x}}%
        \pgf@x=\pgf@pt@ab\pgfutil@tempdima% -ab/(det A)
        \xdef\pgf@new@pt@ab{\pgf@sys@tonumber{\pgf@x}}%
      }%
      \let\pgf@pt@aa\pgf@new@pt@aa%
      \let\pgf@pt@ab\pgf@new@pt@ab%
      \let\pgf@pt@ba\pgf@new@pt@ba%
      \let\pgf@pt@bb\pgf@new@pt@bb%
    \fi%
    \pgf@pt@temp=\pgf@pt@x%
    \pgf@pt@x=\pgf@pt@aa\pgf@pt@x%
    \advance\pgf@pt@x by\pgf@pt@ba\pgf@pt@y%
    \pgf@pt@y=\pgf@pt@bb\pgf@pt@y%
    \advance\pgf@pt@y by\pgf@pt@ab\pgf@pt@temp%
  \fi%
}




% PGF-Level concatenation of the transformation matrix with a given
% matrix. 
%
% #1 - #5 = a concatenation matrix (see pdf spec). Entry #5 is a
%           translation point.
%
% Description:
%
% All coordinates given to subsequent path construction commands will
% be transformed additionally by the given transformation matrix. If
% the command is followed by a 6th argument, the transformation is
% only applied to this argument.
%
%
% Example:
%
% \pgftransformcm{1}{0}{0}{1}{\pgfpoint{100pt}{0pt}} % 100pt to the right.
%
% \pgftransformcm{2}{0}{0}{2}{\pgfpointorigin} % double in in size
% \pgfpathmoveto{\pgfpoint{0cm}{0cm}}
% \pgfpathlineto{\pgflineto{1cm}{1cm}} % actually 2cm/2cm

\def\pgftransformcm#1#2#3#4#5{%
  \edef\pgf@marshal{\noexpand\pgf@transformcm{#1}{#2}{#3}{#4}}%
  \pgf@marshal{#5}%
}
\def\pgf@transformcm#1#2#3#4#5{%
  {%
    \pgf@process{#5}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    %
    \pgfmathsetlength\pgf@x{#1}%
    \pgfmathsetlength\pgf@y{#2}%
    %
    \pgf@xa=\pgf@pt@aa\pgf@x%
    \advance\pgf@xa by \pgf@pt@ba\pgf@y%
    %
    \pgf@ya=\pgf@pt@ab\pgf@x%
    \advance\pgf@ya by \pgf@pt@bb\pgf@y%
    %
    \pgfmathsetlength\pgf@x{#3}%
    \pgfmathsetlength\pgf@y{#4}%
    %
    \pgf@xb=\pgf@pt@aa\pgf@x%
    \advance\pgf@xb by \pgf@pt@ba\pgf@y%
    %
    \pgf@yb=\pgf@pt@ab\pgf@x%
    \advance\pgf@yb by \pgf@pt@bb\pgf@y%
    %
    \pgf@x=\pgf@pt@aa\pgf@xc%
    \advance\pgf@x by\pgf@pt@ba\pgf@yc%
    \advance\pgf@x by\pgf@pt@x%
    %
    \pgf@y=\pgf@pt@ab\pgf@xc%
    \advance\pgf@y by\pgf@pt@bb\pgf@yc%
    \advance\pgf@y by\pgf@pt@y%
    %
    \global\pgf@x=\pgf@x%
    \global\pgf@y=\pgf@y%
    \xdef\pgf@tempaa{\pgf@sys@tonumber{\pgf@xa}}%
    \xdef\pgf@tempab{\pgf@sys@tonumber{\pgf@ya}}%
    \xdef\pgf@tempba{\pgf@sys@tonumber{\pgf@xb}}%
    \xdef\pgf@tempbb{\pgf@sys@tonumber{\pgf@yb}}%
  }%
  \pgf@pt@x=\pgf@x%
  \pgf@pt@y=\pgf@y%
  \let\pgf@pt@aa=\pgf@tempaa%
  \let\pgf@pt@ba=\pgf@tempba%
  \let\pgf@pt@ab=\pgf@tempab%
  \let\pgf@pt@bb=\pgf@tempbb%
  \edef\pgf@idtest{\pgf@pt@aa,\pgf@pt@ba,\pgf@pt@ab,\pgf@pt@bb}%
  \ifx\pgf@idtest\pgf@idmatrixtext%
    \pgf@pt@identitytrue%
  \else%
    \pgf@pt@identityfalse%
  \fi%
}


% Add a pre-morph
%
% #1 = morphing code
%
% Description:
%
% This function adds code to the pre-morphing list. When a
% coordinate is transformed, the current pre-morphing code is
% called first. Then the transformation matrix is applied. Finally, all
% post-morphing code is called. The morphing list is local to the
% current TeX group.
%
% The job of the #1 macro is to modify the values of \pgf@x and
% \pgf@y. It should not have any other sideeffects.
%
% Example:
%
% \pgfmorphaddmorph{\advance\pgf@x by 1cm\relax}

\def\pgfmorphaddpre#1{\expandafter\def\expandafter\pgfmorph@prelist\expandafter{\pgfmorph@prelist#1}}
\let\pgfmorph@prelist=\pgfutil@empty


% Add a post-morph
%
% #1 = morphing macro
%
% Description:
%
% The only difference to the pre-morphs is that post morphs are
% executed after the transformation matrix has been applied.

\def\pgfmorphaddpost#1{\expandafter\def\expandafter\pgfmorph@postlist\expandafter{\pgfmorph@postlist#1}}
\let\pgfmorph@postlist=\pgfutil@empty


% Transformation into a given triangle. The three corners of the
% triangle are called "origin", "x" and "y" are given. After this
% transformation has been applied, the canvas origin is at "origin",
% the vector (1pt,0pt) lies at "x" and the vector (0pt,1pt) lies at
% "y". 
%
% #1 = origin
% #2 = x
% #3 = y
%
% Example:
%
% \pgftransformtriangle{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}{\pgfpoint{-1cm}{1cm}}

\def\pgftransformtriangle#1#2#3{%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#3}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  \advance\pgf@xb by-\pgf@x%
  \advance\pgf@yb by-\pgf@y%
  \pgftransformcm%
  {\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
  {\pgf@sys@tonumber\pgf@xb}{\pgf@sys@tonumber\pgf@yb}%
  {\pgfpoint{\pgf@x}{\pgf@y}}%
}



% Undo all transformations
%
% Example:
%
% \pgftansformreset

\def\pgftransformreset{%
  \pgf@pt@x=0pt%
  \pgf@pt@y=0pt%
  \def\pgf@pt@aa{1.0}%
  \def\pgf@pt@ba{0.0}%
  \def\pgf@pt@ab{0.0}%
  \def\pgf@pt@bb{1.0}%
  \pgf@pt@identitytrue%
}


% Undo all slanting/rotation, but not translations
%
% Example:
%
% \pgftansformreset

\def\pgftransformresetnontranslations{%
  \def\pgf@pt@aa{1.0}%
  \def\pgf@pt@ba{0.0}%
  \def\pgf@pt@ab{0.0}%
  \def\pgf@pt@bb{1.0}%
  \pgf@pt@identitytrue%
}




% Shifting command and environment
%
% #1 = vector by which all subsequent points should be moved.
%
% Example:
%
% \pgftansformshift{\pgfpoint{1cm}{1cm}}

\def\pgftransformshift#1{\pgftransformcm{1.0}{0}{0}{1.0}{#1}}
\def\pgftransformxshift#1{\pgftransformcm{1.0}{0}{0}{1.0}{\pgfpoint{#1}{0pt}}}
\def\pgftransformyshift#1{\pgftransformcm{1.0}{0}{0}{1.0}{\pgfpoint{0pt}{#1}}}




% Scaling commands
%
% #1 = scaling for all subsequent points.
%
% Example:
%
% \pgftransformscale{2}
% \pgftransformxscale{2}
% \pgftransformyscale{2}

\def\pgftransformscale#1{\pgftransformcm{#1}{0}{0}{#1}{\pgfpointorigin}}
\def\pgftransformxscale#1{\pgftransformcm{#1}{0}{0}{1.0}{\pgfpointorigin}}
\def\pgftransformyscale#1{\pgftransformcm{1.0}{0}{0}{#1}{\pgfpointorigin}}



% Slanting commands
%
% #1 = slanting in x-direction. 1 means 45 degrees.
%
% Example:
%
% \pgftransformxslant{2}
% \pgftransformyslant{2}

\def\pgftransformxslant#1{\pgftransformcm{1.0}{0}{#1}{1.0}{\pgfpointorigin}}
\def\pgftransformyslant#1{\pgftransformcm{1.0}{#1}{0}{1.0}{\pgfpointorigin}}



% Rotation commands
%
% #1 = degrees for the rotation
%
% Example:
%
% \pgftransformrotate{30}

\def\pgftransformrotate#1{%
  \pgfmathparse{#1}%
  \let\pgftransform@angle=\pgfmathresult%
  \pgfmathsin@{\pgftransform@angle}%
  \let\pgftransform@sin=\pgfmathresult%
  \pgfmathcos@{\pgftransform@angle}%
  \let\pgftransform@cos=\pgfmathresult%
  \pgf@x=\pgftransform@sin pt%
  \pgf@xa=-\pgf@x%
  \pgftransformcm{\pgftransform@cos}{\pgftransform@sin}{\pgf@sys@tonumber{\pgf@xa}}{\pgftransform@cos}{\pgfpointorigin}%
}



% The following if's have the following effect:
%
% \ifpgfslopedattime decides whether the coordinate system of an
% xxxattime transformation command should be rotated such that text
% drawn on the line should be tangent to the line
%
% \ifpgfallowupsidedowattime decides whether the transformation should
% be done in such a way that the text is always ``upright,'' that is,
% text drawn in this coordiante system is never upside-down. 
%
% \ifpgfresetnontranslationattime decides whether the coordinate
% system of an xxxattime transformation command should be reset
% (concerning the non-translations) before a possible rotation is
% applied. This is useful, for example, if the main coordinate system
% is scaled by, say, a factor of 2 and you do not want that to apply
% to the text, but you do want the rotation to applyu.

\newif\ifpgfslopedattime
\newif\ifpgfallowupsidedownattime
\newif\ifpgfresetnontranslationattime


% Transform to the coordinate system of a point on a line
%
% #1 = a time fraction of line where to put the label, where 0 means start,
%      1 means end, and for example 0.5 means the middle.
% #2 = start of line
% #3 = end of line
%
% Example:
%
% {
%   \pgftransformlineattime{.5}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftext{Hi!}
% }
%
% {
%   \pgftransformlineattime{.75}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftransformresetnontranslations
%   \pgftext{Hi!}
% }
%
\def\pgftransformlineattime#1#2#3{%
  \pgftransformshift{\pgfpointlineattime{#1}{#2}{#3}}%
  \ifpgfresetnontranslationattime%
    \pgftransformresetnontranslations%
  \fi%
  \ifpgfslopedattime%
    \pgf@process{#2}%
    \pgf@xa=\pgf@x% xb/yb = start point
    \pgf@ya=\pgf@y%
    \pgf@process{#3}%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \ifpgfallowupsidedownattime%
    \else%
      \ifdim\pgf@x<0pt%   
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      \fi%
    \fi%
    \pgfpointnormalised{}% x/y = normalised vector
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
    {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
  \fi%
}




% Transform to the coordinate system of a point on a curve
%
% #1 = a time fraction of line where to put the label, where 0 means start,
%      1 means end, and for example 0.5 means the middle.
% #2 = start of line
% #3 = first control
% #4 = second control
% #5 = end of line
%
% Example:
%
% {
%   \pgftransformcurveattime{.5}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftext{Hi!}
% }
%
% {
%   \pgftransformcurveattime{.75}{\pgfxy(0,0)}{\pgfxy(3,2)}
%   \pgftransformresetnontranslations
%   \pgftext{Hi!}
% }
%
\def\pgftransformcurveattime#1#2#3#4#5{%
  \pgfpointcurveattime{#1}{#2}{#3}{#4}{#5}%
  \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \ifpgfresetnontranslationattime%
    \pgftransformresetnontranslations%
  \fi%
  \ifpgfslopedattime%
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
    \advance\pgf@x by-\pgf@xb%
    \advance\pgf@y by-\pgf@yb%
    \ifpgfallowupsidedownattime%
    \else%
      \ifdim\pgf@x<0pt%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      \fi%
    \fi%
    \pgfpointnormalised{}% x/y = normalised vector
    \pgf@ya=-\pgf@y%
    \pgftransformcm%
    {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
    {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
  \fi%
}





% Transform to the coordinate system of an arrow at the end of the
% line going from point #1 to point #2 with the correct rotation.
%
% #1 = a start point an (invisible) line
% #2 = an end point an (invisible) line
%
% Example:
%
% \pgftransformarrow{\pgfpointorigin}{\pgfpoint{1cm}{0cm}}

\def\pgftransformarrow#1#2{%
  \pgftransformshift{#2}%
  \pgf@process{#2}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#1}%
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  \pgf@x=\pgf@xa%
  \pgf@y=\pgf@ya%
  \pgfpointnormalised{}%
  \pgf@ya=-\pgf@y%
  \pgftransformcm%
  {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
  {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfqpoint{0pt}{0pt}}%
}



% Low-level transformations

% Causes the current high-level transformation command to be applied
% to the low-level.
%
% Description:
%
% All subsequent drawing will be transformed additionally by the
% current high-level transformation. Thus, the high-level
% transformation becomes the low-level transformation. The high-level
% transformation is reset at this point.

\def\pgflowlevelsynccm{%
  \pgfsys@transformcm%
  {\pgf@pt@aa}{\pgf@pt@ab}%
  {\pgf@pt@ba}{\pgf@pt@bb}%
  {\pgf@pt@x}{\pgf@pt@y}%
  \pgftransformreset%
  \pgf@relevantforpicturesizefalse%
}  



% Causes a transformation command to be applied to the ``lowlevel''
% transformation matrix. 
%
% #1 - a high-level transformation command
%
% Description:
%
% All subsequent drawing will be transformed additionally by the given
% transformation matrix. Note that PGF will no longer be able to
% ``keep track'' of the coordinates. Also, transformations are applied
% to *everything*, including line thickness and line endings. Most
% often, this is not desirable.
%
% Example:
%
% \pgflowlevel{\pgftransformcm{1}{0}{0}{1}{\pgfpoint{100pt}{0pt}}} % 100bp to the right.
%
% \begin{pgflowlevelscope}{\pgftransformcm{2}{0}{0}{2}{\pgfpointorigin}} % double in in size
%  \pgfmoveto{\pgfpoint{0cm}{0cm}}
%  \pgflineto{\pgflineto{1cm}{1cm}} % actually 2cm/2cm
% \end{pgflowlevelscope}

\def\pgflowlevel#1{%
  {%
    \pgftransformreset%
    #1%
    \pgflowlevelsynccm%
  }%
  \pgf@relevantforpicturesizefalse%
}

\def\pgflowlevelscope#1{\pgfscope\pgflowlevel{#1}}
\def\endpgflowlevelscope{\endpgfscope}

\long\def\pgflowlevelobj#1#2{\pgfscope{\pgflowlevel{#1}#2}\endpgfscope}




\endinput


==> pgfcoretransparency.code.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/basiclayer/pgfcoretransparency.code.tex,v 1.2 2008/01/17 20:09:16 tantau Exp $


% Sets the opacity of stroking operations.
% 
% #1 = opacity, where 1 means fully opaque and 0 means fully
% transparent. 
%
% Example:
%
% \pgfsetstrokeopacity{0.5}

\def\pgfsetstrokeopacity#1{%
  \pgfmathparse{#1}%
  \expandafter\pgfsys@stroke@opacity\expandafter{\pgfmathresult}}


% Sets the opacity of stroking operations.
% 
% #1 = opacity, where 1 means fully opaque and 0 means fully
% transparent. 
%
% Example:
%
% \pgfsetfillopacity{0.5}

\def\pgfsetfillopacity#1{%
  \pgfmathparse{#1}%
  \expandafter\pgfsys@fill@opacity\expandafter{\pgfmathresult}}



% Declares a new fading based on the contents of a box.
%
% #1 = name of the fading
% #2 = content of a TeX box that specifies the fading
%
% Description:
%
% This command declares a new fading based on the contents of
% the TeX box. The mask can later be used to mask other graphics.
%
% The box is used to determine where the mask is opaque: At the
% beginning, the mask is completely transparent. Whereever the box
% contains something (like text or a picture or whatever), the
% luminosity of the text/graphic is used to determine how opaque the
% point will be. The greater the luminosity, the more opaque. The net
% effect is that white corresponds to "completely opaque" and black to
% "completely transparent". This is rather counterintuitive. Because
% of this, the special color "pgftransparent" is defined, which is the
% same as black. By setting the color to, say,
% \color{pgftransparent!10} you get something that is 10% transparent
% and \color{pgftransparent!90} gives you 90% transparency.
%
% By default, the drawing color is set to opaque.
%
% Example:
%
% \pgfdeclarefading{mymask}{
%  \fontsize{200}{200}\bfseries
%  Ti\emph{k}Z
% }
% \pgfdeclarefading{myothermask}{
%  \tikz \shade [left color=transparent,right color=transparent!0]
%    (0,0) rectangle (5,5);
% }

\def\pgfdeclarefading#1#2{%
  \setbox\pgfutil@tempboxa=\hbox{{\pgfsys@beginscope\pgfutil@color{white}\ignorespaces#2\pgfsys@endscope}}%
  \pgfsys@fadingfrombox{#1}\pgfutil@tempboxa%
}

\pgfutil@colorlet{pgftransparent}{black}


% Use a previously declared fading.
%
% #1 = name of the fading
% #2 = transformation code
%
% Description:
%
% The command should be used *inside* a pgfpicture to install a
% fading. The fading is a part of the graphic state. (This command 
% works much like \pgfsetstrokeopacity).
%
% The mask will be centered on the origin. The transformation code #2 is
% applied to the mask (but not the contents of the actual picture).

\def\pgfsetfading#1#2{%
  {%
    \pgftransformreset%
    #2%
    \pgfgettransform{\pgftrans@temp}%
    \edef\pgf@marshal{\noexpand\pgfsys@usefading{#1}\pgftrans@temp}%
    \pgf@marshal%
  }%
}



% Use a previously declared fading scaled for the current path.
%
% #1 - an fading
% #2 - extra transformations
%
% Description:
%
% This command works a bit like \pgfshadepath. "Works a bit like"
% means the following: The masks's original size should
% completely cover the area between (0,0) and (100bp,100bp). The
% mask is then rescaled so that it completely covers the path. Then
% the additional transformation #2 is applied. Finally, the mask is
% made part of the graphic state (as with \pgfsetfading). The path
% used for computation purposes only -- it is not drawn or otherwise
% used.  
%
% If no transformations occur, the lower left corner of the path will
% lie on (25bp, 25bp), the upper right corner on (75bp, 75bp).
%
% If the path was empty, the fading will be used at its natural size,
% centered on the origin.
%
% Example:
%
% \pgfdeclarefading{fade right}
% {\tikz[left color=transparent!0,right color=transparent!100]
%    (0,0) rectangle (100bp,100bp);}
%
% \pgfpathmoveto{\pgforigin}
% \pgfpathlineto{\pgfxy(1,0)}
% \pgfpathlineto{\pgfxy(1,1)}
% \pgfsetfadingforcurrentpath{fade right}{}
% \pgfusepath{fill}

\def\pgfsetfadingforcurrentpath#1#2{%
  \ifdim\pgf@pathminx=16000pt%
    % Path was empty -> use natural size
    \pgfsetfading{#1}{#2}%
  \else%
    \pgfsetfading{#1}{%
      % Calculate center:
      \pgf@xb=.5\pgf@pathmaxx%
      \advance\pgf@xb by.5\pgf@pathminx%
      \pgf@yb=.5\pgf@pathmaxy%
      \advance\pgf@yb by.5\pgf@pathminy%
      % Calculate scaling:
      \pgf@xc=\pgf@pathmaxx%
      \advance\pgf@xc by-\pgf@pathminx%
      \pgf@yc=\pgf@pathmaxy%
      \advance\pgf@yc by-\pgf@pathminy%
      \pgf@xc=.02\pgf@xc%
      \pgf@yc=.02\pgf@yc%
      % Compute new transformation matrix:
      \pgftransformcm{1}{0}{0}{1}{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
      \pgftransformcm{\pgf@sys@tonumber{\pgf@xc}}{0}{0}{\pgf@sys@tonumber{\pgf@yc}}{\pgfpointorigin}%
      #2%
    }%
  \fi%
}




% Group things in a a transparency group
%
% Description:
%
% This takes groups pgf commands inside a pgfpicture in a transparency
% group. This means that any transparency settings apply to commands a
% whole. For instance, if a box contains two overlapping black 
% circles and you draw them normally with 50% transparency, then the
% overlap will be darker than the rest. By comparison, if the circles
% are part of a transparency group, the overlap will get the same
% color as the rest.
%
% 

\def\pgftransparencygroup{%
  \begingroup%
    \setbox\pgfutil@tempboxa=\hbox\bgroup%
}
\def\endpgftransparencygroup{%
    \egroup%
    % Now compute the correct position. This is a bit tricky...
    \ifdim\pgf@picminx=16000pt%
      % Nothing needs to be done
    \else%
      % Safety margin to avoid clipping:
      \advance\pgf@picminx by-1cm%
      \advance\pgf@picmaxx by1cm%
      \advance\pgf@picminy by-1cm%
      \advance\pgf@picmaxy by1cm%
      % Ok, set the box size to current picture size.
      \setbox\pgfutil@tempboxa=\hbox{%
        \vrule width0pt height\pgf@picmaxy depth-\pgf@picminy%
        \hskip-\pgf@picminx%
        \box\pgfutil@tempboxa%
        \hskip\pgf@picmaxx%
      }%
      \pgfsys@transparencygroupfrombox\pgfutil@tempboxa%
      \wd\pgfutil@tempboxa=0pt%
      \ht\pgfutil@tempboxa=0pt%
      \dp\pgfutil@tempboxa=0pt%
      \hskip\pgf@picminx\box\pgfutil@tempboxa\hskip-\pgf@picminx%
    \fi%
  \endgroup%
}

\let\startpgftransparencygroup=\pgftransparencygroup
\let\stoppgftransparencygroup=\endpgftransparencygroup

\endinput


==> pgfexternal.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% In addition to the above licenses, this particular file may also be
% directly inlined into other documents and this copyright notice may
% be removed. Additionally, when you inline this file, you may modify
% it as needed and you may remove comments.
%
% This file is intended to be distributed or even inlined into a file
% when a document needs to be typeset on a system that does not have
% pgf/TikZ installed. 

% "environment" for reading an external graphic. Note that there are
% no (!) braces around the "name" of the environment
%
% #1 = name of the graphics file
%
% Example:
%
% \beginpgfgraphicnamed{mygraph}
%   \begin{tikzpicture}
%     ...
%   \end{tikzpicture}
% \endpgfgraphicnamed

\long\def\beginpgfgraphicnamed#1#2\endpgfgraphicnamed{\includegraphics{#1}}


==> pgffor.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/utilities/pgffor.code.tex,v 1.8 2007/11/07 23:21:48 tantau Exp $



\newdimen\pgffor@iter
\newdimen\pgffor@skip
\newif\ifpgffor@continue

\let\pgffor@beginhook=\pgfutil@empty
\let\pgffor@endhook=\pgfutil@empty
\let\pgffor@afterhook=\pgfutil@empty

\def\pgffor@emptyvalues{, \pgffor@stop,}%

\def\foreach#1in{%
  \def\pgffor@var{#1}%
  \pgfutil@ifnextchar\bgroup{\pgffor@normal@list}{\pgffor@macro@list}}
\def\pgffor@macro@list#1{%
  \expandafter\pgffor@normal@list\expandafter{#1}}
\def\pgffor@normal@list#1{%
  \def\pgffor@values{#1, \pgffor@stop,}%
  \ifx\pgffor@values\pgffor@emptyvalues
    \def\pgffor@values{\pgffor@stop,}%
  \fi%
  \let\pgffor@body\pgfutil@empty%
  \global\pgffor@continuetrue%
  \pgffor@collectbody}

\def\pgffor@collectbody{%
  \pgfutil@ifnextchar\foreach{\pgffor@collectforeach}{%
    \pgfutil@ifnextchar\bgroup{\pgffor@collectargument}{\pgffor@collectsemicolon}}%
}

\def\pgffor@collectforeach\foreach#1in{%
  \pgfutil@ifnextchar\bgroup{\pgffor@collectforeach@normal{#1}}{\pgffor@collectforeach@macro{#1}}}
\def\pgffor@collectforeach@macro#1#2{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body\foreach#1in#2}%
  \pgffor@collectbody%
}
\def\pgffor@collectforeach@normal#1#2{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body\foreach#1in{#2}}%
  \pgffor@collectbody%
}

\long\def\pgffor@collectargument#1{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body{#1}}%
  \pgffor@iterate%
}


\def\pgffor@collectsemicolon{%
  \let\pgffor@next=\pgffor@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\pgffor@next=\pgffor@collectactivesemicolon%
  \fi%
  \pgffor@next%
}

\def\pgffor@collectnormalsemicolon#1;{%
  \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body#1;}%
  \pgffor@iterate%
}

{
  \catcode`\;=\active
  
  \gdef\pgffor@collectactivesemicolon#1;{%
    \expandafter\long\expandafter\def\expandafter\pgffor@body\expandafter{\pgffor@body#1;}%
    \pgffor@iterate%
  }
}

\def\pgffor@iterate{%
  \let\pgffor@last\pgfutil@empty%
  \let\pgffor@prevlast\pgfutil@empty%
  \expandafter\pgffor@scan\pgffor@values}

\def\pgffor@stop{\pgffor@stop}%
\def\pgffor@dots{...}%

\def\pgffor@scan{\pgfutil@ifnextchar({\pgffor@scanround}{\pgffor@scanone}}
\def\pgffor@scanround(#1)#2,{\def\pgffor@value{(#1)}\pgffor@scanned}
\def\pgffor@scanone#1,{\def\pgffor@value{#1}\pgffor@scanned}

\def\pgffor@scanned{%
  \ifx\pgffor@value\pgffor@stop%
    \let\pgffor@next=\pgffor@after% done!
  \else%
    \ifx\pgffor@value\pgffor@dots%
      \let\pgffor@next=\pgffor@handledots%
    \else%
      \let\pgffor@next=\pgffor@handlevalue%
    \fi%
    \ifpgffor@continue%
    \else%
      \let\pgffor@next=\pgffor@scan% done!
    \fi%
  \fi%
  \pgffor@next}

\def\pgffor@after{%
  \global\pgffor@continuetrue%
  \pgffor@afterhook}

\def\pgffor@handlevalue{%
  \let\pgffor@prevlast\pgffor@last%
  \let\pgffor@last\pgffor@value%
  \pgffor@invokebody%
  \pgffor@scan%
}

\def\pgffor@invokebody{%
  \begingroup%
    \expandafter\pgfutil@in@\expandafter/\expandafter{\pgffor@var}%
    \ifpgfutil@in@%
      \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@value//\relax}%
      \expandafter\pgffor@multiassign\pgffor@var/\pgffor@stop/\pgffor@stop/\relax%
    \else%
      \expandafter\expandafter\expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@value}%
    \fi%
    \expandafter\pgffor@beginhook\pgffor@body\pgffor@endhook%
  \endgroup%
}


\def\pgffor@multiassign#1/#2/\relax{%
  \def\pgffor@currentvar{#1}%
  \def\pgffor@rest{#2}%
  \ifx\pgffor@currentvar\pgffor@stop%
    \let\pgffor@next=\relax%
  \else%
    \let\pgffor@next=\pgffor@multiassignrest%
  \fi%
  \pgffor@next%
}

\def\pgffor@multiassignrest{\expandafter\pgffor@multiassignfinal\pgffor@valuerest}
\def\pgffor@multiassignfinal#1/#2/\relax{%
  \def\pgffor@test{#2}%
  \ifx\pgffor@test\pgfutil@empty%
    \def\pgffor@valuerest{#1//\relax}% repeat
  \else%
    \def\pgffor@valuerest{#2/\relax}%
  \fi%
  \expandafter\def\pgffor@currentvar{#1}%
  \expandafter\pgffor@multiassign\pgffor@rest/\relax%
}
  



\def\pgffor@handledots{%
  \ifx\pgffor@last\pgfutil@empty%
    \PackageError{pgffor}{``...'' not allowed without prior value}{}%
  \fi%
  \pgffor@dotsscanend%
}
\def\pgffor@dotsscanend#1,{%
  \def\pgffor@dotsend{#1}%
  % calculate skip%
  \ifx\pgffor@prevlast\pgfutil@empty%
    \ifdim\pgffor@dotsend pt>\pgffor@last pt%
      \pgffor@skip=1pt%
    \else%
      \pgffor@skip=-1pt%
    \fi%
  \else%
    \pgffor@skip=\pgffor@last pt%
    \pgffor@iter=\pgffor@prevlast pt%
    \advance\pgffor@skip by-\pgffor@iter%
  \fi%
  \pgffor@iter=\pgffor@last pt%
  % do loop
  \pgffor@loop%
}

\def\pgffor@loop{%
  \advance\pgffor@iter by\pgffor@skip%
  \let\pgffor@next=\pgffor@doloop%
  \ifdim\pgffor@skip<0pt%
    \ifdim\pgffor@iter<\pgffor@dotsend pt%
      \let\pgffor@next=\pgffor@endloop%
    \fi%
  \else%
    \ifdim\pgffor@iter>\pgffor@dotsend pt%
      \let\pgffor@next=\pgffor@endloop%
    \fi%
  \fi%
  \ifpgffor@continue%
  \else%
    \let\pgffor@next=\pgffor@endloop% done!
  \fi%
  \pgffor@next%
}

\def\pgffor@endloop{%
  \pgffor@scan%
}

{\catcode`\p=12\catcode`\t=12\gdef\Pgffor@geT#1pt{#1}}

\def\pgffor@doloop{%
  \begingroup%
    \edef\pgffor@temp{\expandafter\Pgffor@geT\the\pgffor@iter}%
    \edef\pgffor@incheck{{.0/}{\pgffor@temp/}}%
    \expandafter\pgfutil@in@\pgffor@incheck%
    \ifpgfutil@in@%
      \expandafter\pgffor@strip\pgffor@temp%
    \fi%
    \expandafter\pgfutil@in@\expandafter/\expandafter{\pgffor@var}%
    \ifpgfutil@in@%
      \expandafter\def\expandafter\pgffor@valuerest\expandafter{\pgffor@temp//\relax}%
      \expandafter\pgffor@multiassign\pgffor@var/\pgffor@stop/\pgffor@stop/\relax%
    \else%
      \expandafter\expandafter\expandafter\def\expandafter\pgffor@var\expandafter{\pgffor@temp}%
    \fi%
    \expandafter\pgffor@beginhook\pgffor@body\pgffor@endhook%
  \endgroup%
  \pgffor@loop%  
}

\def\pgffor@strip#1.0{\def\pgffor@temp{#1}}


\def\breakforeach{\global\pgffor@continuefalse}
  
\endinput


==> pgffor.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\edef\pgfforatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfrcs.tex
\input pgffor.code.tex

\catcode`\@=\pgfforatcode

\endinput


==> pgfkeys.code.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% This file is perfectly self-contained, except that the catcode of @ should be made a letter. 


% Guard against reading twice
\ifx\pgfkeysloaded\undefined
  \let\pgfkeysloaded=\relax
\else
  \expandafter\endinput
\fi
  
% The purpose of this file is to provide a general settings engine that 
% works with all TeX formats and has no save-stack impact


% This is useful:

\def\pgfkeys@ifcsname#1\endcsname#2\else#3\fi{\expandafter\ifx\csname#1\endcsname\relax#3\else#2\fi}%
\ifx\eTeXrevision\undefined%
\else%
  \expandafter\let\expandafter\pgfkeys@ifcsname\csname ifcsname\endcsname%
\fi

\def\pgfkeys@empty{}

% This also:

\ifx\PackageError\undefined
  \def\pgfkeys@error#1{\immediate\write-1{Package pgfkeys: Error! #1.}}%
\else
  \def\pgfkeys@error#1{\PackageError{pgfkeys}{#1}{}}%
\fi

% Set a key to a value
%
% #1 = key
% #2 = tokens
%
% Description:
%
% This command sets the key to the given tokens. The tokens are stored as
% is and can even contain things like #9. 
%
% Keys are organized hierarchically using something similar to Unix
% paths. Thus, a typically key might be called "/tikz/length" or
% "/tikz/length dimension/.@cmd". Some keys starting with a dot are
% special, so they should not be used as normal key names (they are
% similar to Unix files starting with a dot -- you can use them, but
% be careful).
%
% Keys are always local to the current TeX group.
%
% Example:
%
% \pgfkeyssetvalue{/tikz/length}{2cm-3cm}
% \pgfkeyssetvalue{/algo/swap}{{#2}{#1}}

\def\pgfkeyssetvalue#1#2{%
  \pgfkeys@temptoks{#2}\expandafter\edef\csname pgfk@#1\endcsname{\the\pgfkeys@temptoks}%
}



% Add text to a key at the end
%
% #1 = key
% #2 = a value to be added at the beginning
% #3 = a value to be added at the end
%
% Description:
%
% This command adds #2 to the definition of the key. The key should
% have been set previously using \pgfkeyssetvalue.
%
% Example:
%
% \pgfkeysaddvalue{/tikz/length}{}{-3cm}

\def\pgfkeysaddvalue#1#2#3{%
  {%
    \toks0{#1}%
    \pgfkeysifdefined{#1}
    {\pgfkeys@temptoks\expandafter\expandafter\expandafter{\csname pgfk@#1\endcsname}}%
    {\pgfkeys@temptoks{}}%
    \toks1{#2}%
    \xdef\pgfkeys@global@temp{\the\toks0 \the\pgfkeys@temptoks \the\toks1}% believe or don't: the spaces are important
  }%
  \pgfkeyslet{#1}\pgfkeys@global@temp%
}



% Makes a key equal a given code
%
% #1 = key
% #2 = a code name
%
% Description:
%
% This command executes a \let command so that a key gets the same
% value as the parameter #2.
%
% Keys are always local to the current TeX group.
%
% Example:
%
% \pgfkeyslet{/algo/swap}{\myswap}

\def\pgfkeyslet#1#2{%
  \expandafter\let\csname pgfk@#1\endcsname#2%
}


% Retrieve the code stored in a key into a code
%
% #1 = key
% #2 = code
%
% Description:
%
% This command will set #2 to "point" to the value stored in the key.
%
% Example:
%
% \pgfkeysgetvalue{/tikz/swap}{\myswap}

\def\pgfkeysgetvalue#1#2{\expandafter\let\expandafter#2\csname pgfk@#1\endcsname}



% Retrieve the value stored in a key
%
% #1 = key
%
% Description:
%
% This command will expand to the value stored in the key. The key
% should previously have been set using \pgfkeyasetkey or \pgfkeyslet. 
%
% Example:
%
% The length is \pgfkeysvalue{/tikz/length}.

\def\pgfkeysvalueof#1{\csname pgfk@#1\endcsname}



% If for testing whether a key exists
%
% #1 = key
% #2 = if-case
% #3 = else-case
%
% Description:
%
% This if will be executed if the key exists. In eTeX mode this works
% like a normal if, in normal TeX mode you need to provide an \else.
%
% Example:
%
% \pgfkeysifdefined{/tikz/length}{key exists}{does not exist}

\def\pgfkeysifdefined#1#2#3{\pgfkeys@ifcsname pgfk@#1\endcsname#2\else#3\fi}




% Execute settings
%
% #1 = list of settings
%
% Description:
%
% The list of settings should contain comma-separated settings. Each
% setting has the following form:
%
% /path/key=value
%
% The parts "/path/" and "=value" are optional. When the path is not
% specified, the value of the token register "\pgfkeypath" is used. If
% "=value" is missing, the value of the setting "/path/key/.@def" is used
% instead. If this key is set to "\pgfvaluerequired", the key
% "/errors/value required/.@cmd" is executed. Theis error handler,
% like all other error handlers, will get the current key as its first
% parameter (unexpanded) and the current value as its second value
% (also unexpanded).
%
% Any spaces at the beginning and at the end and around the
% equals-sign are removed. The key with the complete path is set to
% the code \pgfcurrentkey.
%
% The setting is then processed according to the following rules:
%
% 1) If the key /path/key/.@cmd" is present, its code is executed
%    with the value computed above, followed by \pgfeov (end of
%    value). So, to handle
%
%    "/stuff/height=  1.5 ,"
%
%    /stuff/height/.@cmd should be set to some code, that can
%    handle the parameter
%
%    "1.5\pgfeov"
%
%    For instance, saying
%
%    \pgfkeys{/stuff/height/.@cmd}{#1\pgfeov}{\def\myheight{#1}}
%
%    will do nicely.
%
% 2) Otherwise, if the key /path/key is present, this key is
%    set to the value computed above.
%
% 3) Otherwise, if the key /handlers/key/.@cmd is present, it is executed
%    with the same parameters as in 1). Additionally, the
%    token register \pgfcurrentkeypath will be set to "/path/" and the
%    macor \pgfcurrentkeywithoutpath to "key". So, in the above
%    example if neither "/stuff/height/.@cmd" nor
%    "/stuff/height" is present, but "/handlers/height" is,
%    then "/handlers/height" is executed with the parameters:
%
%    "1.5\pgfeov"
%
%    and \pgfcurrentkey is set to "/stuff/height" and \pgfcurrentkeypath
%    is set to "/stuff/" and \pgfcurrentkeywithoutpath to "height".
%
% 4) Otherwise, if the key "/path/.unknown/.@cmd" is present, its code is
%    executed with the same parameters as in 3).
%
% 5) Otherwise, the key "/handlers/.unknown/.@cmd" is executed with the same
%    parameters as in 1).
%
% After all settings have been processed, the value of the token
% register \pgfdefaultkeypath is set to its original value. Thus, any local
% change of this token register has no effect outside the call.
%
% Example:
%
% \pgfkeys{/tikz/.is family}
% \pgfkeys{/tikz/line width/.cd,
%         .def=\pgfsetlinewidth{##1},
%         .set default=.4pt}
% \pgfkeys{tikz,line width=1pt}

\newtoks\pgfkeys@pathtoks
\def\pgfkeyscurrentpath{\the\pgfkeys@pathtoks}
\newtoks\pgfkeys@temptoks

\def\pgfkeys@root{/}
\let\pgfkeysdefaultpath\pgfkeys@root

\def\pgfkeys{\expandafter\pgfkeys@@set\expandafter{\pgfkeysdefaultpath}}%
\def\pgfkeys@@set#1#2{%
  \let\pgfkeysdefaultpath\pgfkeys@root%
  \pgfkeys@parse#2,\pgfkeys@mainstop%
  \def\pgfkeysdefaultpath{#1}}

\def\pgfkeys@parse{\futurelet\pgfkeys@possiblerelax\pgfkeys@parse@main}
\def\pgfkeys@parse@main{%
  \ifx\pgfkeys@possiblerelax\pgfkeys@mainstop%
    \expandafter\pgfkeys@cleanup%
  \else%
    \expandafter\pgfkeys@normal%
  \fi%
}
\def\pgfkeys@normal#1,{%
  \pgfkeys@unpack#1=\pgfkeysnovalue=\pgfkeys@stop%
  \pgfkeys@parse%
}
\def\pgfkeys@cleanup\pgfkeys@mainstop{}

\def\pgfkeys@mainstop{\pgfkeys@mainstop} % equals only itself
\def\pgfkeys@novalue{} % equals only itself
\def\pgfkeysnovalue{\pgfkeys@novalue} % equals only itself
\def\pgfkeysnovalue@text{\pgfkeysnovalue}
\def\pgfkeysvaluerequired{\pgfkeysvaluerequired} % equals only itself

\def\pgfkeys@unpack#1=#2=#3\pgfkeys@stop{%
  \pgfkeys@spdef\pgfkeyscurrentkey{#1}%
  \edef\pgfkeyscurrentkey{\pgfkeyscurrentkey}%
  \ifx\pgfkeyscurrentkey\pgfkeys@empty%
    % Skip
  \else%
    \pgfkeys@add@path@as@needed%
    \pgfkeys@spdef\pgfkeyscurrentvalue{#2}%
    \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
      \pgfkeysifdefined{\pgfkeyscurrentkey/.@def}%
      {\pgfkeysgetvalue{\pgfkeyscurrentkey/.@def}{\pgfkeyscurrentvalue}}
      {}% no default, so leave it
    \fi%
    \ifx\pgfkeyscurrentvalue\pgfkeysvaluerequired%
      \pgfkeysvalueof{/errors/value required/.@cmd}\pgfkeyscurrentkey\pgfkeyscurrentvalue\pgfeov%
    \else%
      \pgfkeys@case@one%
    \fi%
  \fi}

\def\pgfkeys@case@one{%
  \pgfkeysifdefined{\pgfkeyscurrentkey/.@cmd}%
  {\pgfkeysgetvalue{\pgfkeyscurrentkey/.@cmd}{\pgfkeys@code}%
   \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {\pgfkeys@case@two}%
}

\def\pgfkeys@case@two{%
  \pgfkeysifdefined{\pgfkeyscurrentkey}%
  {\pgfkeys@case@two@extern}%
  {\pgfkeys@case@three}%
}

\def\pgfkeys@case@two@extern{%
  \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
    \pgfkeysvalueof{\pgfkeyscurrentkey}%
  \else%
    \pgfkeyslet{\pgfkeyscurrentkey}\pgfkeyscurrentvalue%
  \fi%
}


\def\pgfkeys@case@three{%
  \pgfkeys@split@path%
  \pgfkeysifdefined{/handlers/\pgfkeyscurrentname/.@cmd}%
  {\pgfkeysgetvalue{/handlers/\pgfkeyscurrentname/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {\pgfkeys@unknown}%
}

\def\pgfkeys@unknown{%
  \pgfkeysifdefined{\pgfkeyscurrentpath/.unknown/.@cmd}%
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.unknown/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov}
  {%
    \pgfkeysgetvalue{/handlers/.unknown/.@cmd}{\pgfkeys@code}%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
  }%
}


\def\pgfkey@argumentisspace#1{%
  \def\pgfkeys@spdef##1##2{%
    \futurelet\pgfkeys@possiblespace\pgfkeys@sp@a##2\pgfkeys@stop\pgfkeys@stop#1\pgfkeys@stop\relax##1}%
  \def\pgfkeys@sp@a{%
    \ifx\pgfkeys@possiblespace\pgfkeys@sptoken%
      \expandafter\pgfkeys@sp@b%
    \else%
      \expandafter\pgfkeys@sp@b\expandafter#1%
    \fi}%
  \def\pgfkeys@sp@b#1##1 \pgfkeys@stop{\pgfkeys@sp@c##1}%
}
\pgfkey@argumentisspace{ }
\def\pgfkeys@sp@c#1\pgfkeys@stop#2\relax#3{\pgfkeys@temptoks{#1}\edef#3{\the\pgfkeys@temptoks}}
{\def\:{\global\let\pgfkeys@sptoken= } \: }



\def\pgfkeys@add@path@as@needed{% Should add the path if the
  % \pgfkeyscurrentkey does not start with /
  \expandafter\futurelet\expandafter\pgfkeys@possibleslash\expandafter\pgfkeys@check@slash\pgfkeyscurrentkey\relax%
}
\def\pgfkeys@check@slash{%
  \ifx\pgfkeys@possibleslash/%
    \expandafter\pgfkeys@nevermind%
  \else%
    \expandafter\pgfkeys@addpath%
  \fi%
}

\def\pgfkeys@nevermind#1\relax{}
\def\pgfkeys@addpath#1\relax{\edef\pgfkeyscurrentkey{\pgfkeysdefaultpath#1}}

\def\pgfkeys@split@path{% Should assign the two codes
                       % \pgfkeyscurrentname and \pgfcurrentlkeypath
  \pgfkeys@pathtoks{}%
  \expandafter\pgfkeys@splitter\pgfkeyscurrentkey//%
}
\def\pgfkeys@splitter#1/#2/{%
  \def\pgfkeys@temp{#2}%
  \ifx\pgfkeys@temp\pgfkeys@empty%
    % Ah. done
    \def\pgfkeyscurrentname{#1}%
    \expandafter\pgfkeys@gobbletoslash%
  \else%
    \expandafter\pgfkeys@pathtoks\expandafter{\the\pgfkeys@pathtoks#1/}%
  \fi%
  \pgfkeys@splitter#2/%
}
\def\pgfkeys@gobbletoslash\pgfkeys@splitter/{\expandafter\pgfkeys@remove@slash\the\pgfkeys@pathtoks\relax}%
\def\pgfkeys@remove@slash#1/\relax{\pgfkeys@pathtoks{#1}}



% Quickly set keys
%
% #1 = default path
% #2 = key-value pairs
%
% Desscription:
%
% This command starts the execution with the default path set to
% #1. This command should only be used when speed is important (like
% in a heavily used macro like \tikzset). Normally, keys should be
% used to set the path. Note that if #1 equals /, then \pgfkeys will
% actually be quicker!
%
% Example:
%
% \pgfqkeys{/tikz}{myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\def\pgfqkeys{\expandafter\pgfkeys@@qset\expandafter{\pgfkeysdefaultpath}}%
\def\pgfkeys@@qset#1#2#3{\def\pgfkeysdefaultpath{#2/}\pgfkeys@parse#3,\pgfkeys@mainstop\def\pgfkeysdefaultpath{#1}}


% Sets keys while setting keys
%
% #1 = key-value pairs
%
% Desscription:
%
% This code may only be called inside the code that is executed for a
% key. The #1 should be a list of settings pairs. They will be executed
% as if they had been given as the argument to the \pgfkeys command.
%
% Example:
%
% \pgfkeys{tikz,myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\def\pgfkeysalso#1{\pgfkeys@parse#1,\pgfkeys@mainstop}



% Quickly sets keys while setting keys
%
% #1 = default path
% #2 = key-value pairs
%
% Desscription:
%
% This command executes #2 with the default path set to #1. This
% command will cause chaos if used incorrectly. The only safe
% place to use it instead of \pgfkeys is at the beginning of a TeX group.
%
% Example:
%
% \begingroup
%   \pgfqkeysalso{/tikz}{myother length/.code=\def\myotherlength{#1}\pgfkeysalso{length=#1}}

\def\pgfqkeysalso#1#2{\def\pgfkeysdefaultpath{#1/}\pgfkeys@parse#2,\pgfkeys@mainstop}




% Now setup the default handelers and keys:

% Define a key macro with one argument (\def or \edef)
%
% #1 = key
% #2 = code
%
% Description:
%
% This command will setup things so the key/.@cmd contains a macro
% that takes one parameter and has #2 as its code.
%
% Example:
%
% \pgfkeysdef{/my key}{\show#1}

\def\pgfkeysdef#1#2{%
  \def\pgfkeys@temp##1\pgfeov{#2}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
}
\def\pgfkeysedef#1#2{%
  \edef\pgfkeys@temp##1\pgfeov{#2}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
}


% Define a key macro with mutliple arguments (\def or \edef)
%
% #1 = key
% #2 = argument pattern
% #2 = code
%
% Description:
%
% This command will setup things so the key/.@cmd contains a macro
% that takes #2 as its parameter pattern and has #3 as its code.
%
% Example:
%
% \pgfkeysdefargs{/swap}{#1#2}{#2#1}

\def\pgfkeysdefargs#1#2#3{%
  \def\pgfkeys@temp#2\pgfeov{#3}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetvalue{#1/.@args}{#2\pgfeov}%
  \pgfkeyssetvalue{#1/.@body}{#3}%
}
\def\pgfkeysedefargs#1#2#3{%
  \edef\pgfkeys@temp#2\pgfeov{#3}%
  \pgfkeyslet{#1/.@cmd}{\pgfkeys@temp}%
  \pgfkeyssetvalue{#1/.@args}{#2\pgfeov}%
  \pgfkeyssetvalue{#1/.@body}{#3}%
}



% Defining a key command

\pgfkeysdef{/handlers/.code}{\pgfkeysdef{\pgfkeyscurrentpath}{#1}}
\pgfkeysdef{/handlers/.code 2 args}{\pgfkeysdefargs{\pgfkeyscurrentpath}{##1##2}{#1}}
\pgfkeysdef{/handlers/.ecode}{\pgfkeysedef{\pgfkeyscurrentpath}{#1}}
\pgfkeysdef{/handlers/.ecode 2 args}{\pgfkeysedefargs{\pgfkeyscurrentpath}{##1##2}{#1}}
\pgfkeysdefargs{/handlers/.code args}{#1#2}{\pgfkeysdefargs{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeysdefargs{/handlers/.ecode args}{#1#2}{\pgfkeysedefargs{\pgfkeyscurrentpath}{#1}{#2}}

% Adding to a key command

\pgfkeys{/handlers/.add code/.code 2 args=%
  % Find out, whether with args or not.
  \pgfkeysifdefined{\pgfkeyscurrentpath/.@args}%
  {% Yes, so add to body and reuse args
    \pgfkeysaddvalue{\pgfkeyscurrentpath/.@body}{#1}{#2}%
    % Redefine code
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@args}{\pgfkeys@tempargs}
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@body}{\pgfkeys@tempbody}
    \expandafter\expandafter\expandafter\def\expandafter\pgfkeys@temp\expandafter\pgfkeys@tempargs\expandafter{\pgfkeys@tempbody}%
    \pgfkeyslet{\pgfkeyscurrentpath/.@cmd}{\pgfkeys@temp}%
  }%
  {%
    % No, so single argument. Redefine accordingly.
    {%
      \toks0{#1}%
      \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}%
      {\pgfkeys@temptoks\expandafter\expandafter\expandafter{\csname pgfk@\pgfkeyscurrentpath/.@cmd\endcsname##1\pgfeov}}%
      {\pgfkeys@temptoks{}}%
      \toks1{#2}%
      \xdef\pgfkeys@global@temp{\the\toks0 \the\pgfkeys@temptoks \the\toks1}%
    }%
    \expandafter\def\expandafter\pgfkeys@temp\expandafter##\expandafter1\expandafter\pgfeov\expandafter{\pgfkeys@global@temp}%
    \pgfkeyslet{\pgfkeyscurrentpath/.@cmd}\pgfkeys@temp%
  }%
}
\pgfkeys{/handlers/.prefix code/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={#1}{}}}%
\pgfkeys{/handlers/.append code/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={}{#1}}}%


% Defining a style

\pgfkeys{/handlers/.style/.code=\pgfkeys{\pgfkeyscurrentpath/.code=\pgfkeysalso{#1}}}
\pgfkeys{/handlers/.estyle/.code=\pgfkeys{\pgfkeyscurrentpath/.ecode=\noexpand\pgfkeysalso{#1}}}
\pgfkeys{/handlers/.style args/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.code args={#1}{\pgfkeysalso{#2}}}}
\pgfkeys{/handlers/.estyle args/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.ecode args={#1}{\noexpand\pgfkeysalso{#2}}}}
\pgfkeys{/handlers/.style 2 args/.code=\pgfkeys{\pgfkeyscurrentpath/.code 2 args=\pgfkeysalso{#1}}}

% Adding to a style

\pgfkeys{/handlers/.add style/.code 2 args=\pgfkeys{\pgfkeyscurrentpath/.add code={\pgfkeysalso{#1}}{\pgfkeysalso{#2}}}}%
\pgfkeys{/handlers/.prefix style/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={\pgfkeysalso{#1}}{}}}%
\pgfkeys{/handlers/.append style/.code=\pgfkeys{\pgfkeyscurrentpath/.add code={}{\pgfkeysalso{#1}}}}%


% Defining a value

\pgfkeys{/handlers/.initial/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath}{#1}}
\pgfkeys{/handlers/.add/.code 2 args=\pgfkeysaddvalue{\pgfkeyscurrentpath}{#1}{#2}}
\pgfkeys{/handlers/.get/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath}{#1}}

% Defining a default

\pgfkeys{/handlers/.default/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath/.@def}{#1}}
\pgfkeys{/handlers/.value required/.code=\pgfkeyssetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeysvaluerequired}}
\pgfkeys{/handlers/.value forbidden/.code=\pgfkeys{\pgfkeyscurrentpath/.add code=%
{%
  \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
  \else%
    \pgfkeysvalueof{/errors/value forbidden/.@cmd}\pgfkeyscurrentkey\pgfkeyscurrentvalue\pgfeov%
  \fi%
}{}}}


% High-level cmds

\pgfkeys{/handlers/.store in/.code=\pgfkeysalso{\pgfkeyscurrentpath/.code=\def#1{##1}}}
\pgfkeys{/handlers/.estore in/.code=\pgfkeysalso{\pgfkeyscurrentpath/.code=\edef#1{##1}}}

\pgfkeys{/handlers/.is if/.code=\pgfkeysalso{%
    \pgfkeyscurrentpath/.code=\pgfkeys@handle@boolean{#1}{##1},
    \pgfkeyscurrentpath/.default=true%
  }%
}
\def\pgfkeys@handle@boolean#1#2{%
  \pgfkeys@ifcsname#1#2\endcsname%
    \csname#1#2\endcsname%
  \else%
    \pgfkeysvalueof{/errors/boolean expected/.@cmd}\pgfkeyscurrentkey{#2}\pgfeov%
  \fi
}

\pgfkeys{/handlers/.is choice/.code=%
  \pgfkeys{%
    \pgfkeyscurrentpath/.cd,%
    .code=\expandafter\pgfkeysalso\expandafter{\pgfkeyscurrentkey/##1},
    .unknown/.style={/errors/unknown choice value=\pgfkeyscurrentkey\pgfkeyscurrentvalue}}}


% Inspection handlers

\pgfkeys{/handlers/.show value/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath}{\pgfkeysshower}\show\pgfkeysshower} % inspect the value 
\pgfkeys{/handlers/.show code/.code=\pgfkeysgetvalue{\pgfkeyscurrentpath/.@cmd}{\pgfkeysshower}\show\pgfkeysshower} % inspect the body of the command


% Path handling

\pgfkeys{/handlers/.is family/.code=\pgfkeys{\pgfkeyscurrentpath/.ecode=\edef\noexpand\pgfkeysdefaultpath{\pgfkeyscurrentpath/}}}
\pgfkeys{/handlers/.cd/.code=\edef\pgfkeysdefaultpath{\pgfkeyscurrentpath/}}


% Value expansion

\pgfkeys{/handlers/.expand once/.code=\expandafter\pgfkeys@exp@call\expandafter{#1}}
\pgfkeys{/handlers/.expand twice/.code=\expandafter\expandafter\expandafter\pgfkeys@exp@call\expandafter\expandafter\expandafter{#1}}
\pgfkeys{/handlers/.expanded/.code=\edef\pgfkeys@temp{#1}\expandafter\pgfkeys@exp@call\expandafter{\pgfkeys@temp}}

\def\pgfkeys@exp@call#1{\pgfkeysalso{\pgfkeyscurrentpath=#1}}

% Try to set a key and do nothing if not define

\newif\ifpgfkeyssuccess
\pgfkeys{/handlers/.try/.code=\pgfkeys@try}
\pgfkeys{/handlers/.retry/.code=\ifpgfkeyssuccess\else\pgfkeys@try\fi}
\def\pgfkeys@try{%
  \pgfkeysifdefined{\pgfkeyscurrentpath/.@cmd}%
  {%
    \pgfkeysgetvalue{\pgfkeyscurrentpath/.@cmd}{\pgfkeys@code}%
    \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text% Hmm... no value
      \pgfkeysifdefined{\pgfkeyscurrentpath/.@def}%
      {\pgfkeysgetvalue{\pgfkeyscurrentpath/.@def}{\pgfkeyscurrentvalue}}
      {}% no default, so leave it
    \fi%
    \expandafter\pgfkeys@code\pgfkeyscurrentvalue\pgfeov%
    \pgfkeyssuccesstrue%
  }%
  {%
    \pgfkeysifdefined{\pgfkeyscurrentpath}%
    {%
      \ifx\pgfkeyscurrentvalue\pgfkeysnovalue@text%
        \pgfkeysvalueof{\pgfkeyscurrentpath}%
      \else%
        \pgfkeyslet{\pgfkeyscurrentpath}\pgfkeyscurrentvalue%
      \fi%
      \pgfkeyssuccesstrue%
    }%
    {\pgfkeyssuccessfalse}%
  }%
}

% Utilities

\pgfkeys{/utils/exec/.code=#1} % simply execute the given code directly.


% Errors

\pgfkeys{/errors/boolean expected/.code 2 args=\pgfkeys@error{%
    Boolean parameter of key '#1' must be 'true' or 'false', not
    '#2'. I am going to ignore it}}  
\pgfkeys{/errors/value required/.code 2 args=\pgfkeys@error{%
    The key '#1' requires a value. I am going to ignore this key}{}}  
\pgfkeys{/errors/value forbidden/.code 2 args=\pgfkeys@error{%
    You may not specify a value for the key '#1'. I am going to ignore
    the value '#2' that you provided}}
\pgfkeys{/errors/unknown choice value/.code 2 args=\pgfkeys@error{%
    Choice '\pgfkeyscurrentname' unknown in key
    '\pgfkeyscurrentpath'. I am going to ignore this key}}
\pgfkeys{/errors/unknown key/.code 2 args=\pgfkeys@error{%
    I do not know the key '#1' and I am going to ignore it. Perhaps
    you misspelled it}}

\pgfkeys{/handlers/.unknown/.code=%
  {%
    \let\pgfkeys@orig@key=\pgfkeyscurrentkey%
    \pgfkeysalso{/errors/unknown key=\pgfkeys@orig@key{}}%
  }
}



\endinput


==> pgfkeys.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\edef\pgfkeysatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfrcs.tex
\input pgfkeys.code.tex

\catcode`\@=\pgfkeysatcode

\endinput


==> pgflibraryarrows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryarrows.code.tex,v 1.7 2007/06/07 07:41:11 tantau Exp $


% A square bracket shaped arrow

\pgfarrowsdeclare{[}{]}
{
  \pgfutil@tempdima=1pt%
  \advance\pgfutil@tempdima by1.25\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdima}
  \pgfarrowsrightextend{+.5\pgflinewidth}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfutil@tempdimb=\pgfutil@tempdima%
  \advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{-.5\pgfutil@tempdimb}{-1\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{-1\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-.5\pgfutil@tempdimb}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{]}{[}{[}{]}


% A round bracket shaped arrow

\pgfarrowsdeclare{(}{)}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfutil@tempdimb=0.0625\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
  \pgfutil@tempdimb=0.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=2pt%
  \advance\pgfutil@tempdima by1.5\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{-.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{.25\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{.25\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-.5\pgfutil@tempdima}{\pgfutil@tempdima}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{)}{(}{(}{)}




% A pointed bracket shaped arrow

\pgfarrowsdeclare{angle 90}{angle 90}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=5.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpoint{-5.5\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-5.5\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{angle 90 reversed}{angle 90 reversed}{angle 90}{angle 90}


\pgfarrowsdeclare{angle 60}{angle 60}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=7.29\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{angle 60 reversed}{angle 60 reversed}{angle 60}{angle 60}



\pgfarrowsdeclare{angle 45}{angle 45}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=8.705\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.3pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
  \pgfusepathqstroke
}

\pgfarrowsdeclarereversed{angle 45 reversed}{angle 45 reversed}{angle 45}{angle 45}



% A dot shaped arrow

\pgfarrowsdeclare{*}{*}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfutil@tempdimb=5.5\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=1.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfpathcircle{\pgfqpoint{-3\pgfutil@tempdima}{0pt}}{+4.5\pgfutil@tempdima}
  \pgfusepathqfillstroke
}


% An open dot shaped arrow

\pgfarrowsdeclare{o}{o}
{
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfutil@tempdimb=9\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfpathcircle{\pgfqpoint{4.5\pgfutil@tempdima}{0bp}}{4.5\pgfutil@tempdima}
  \pgfusepathqstroke
}



% A diamond shaped arrow

\pgfarrowsdeclare{diamond}{diamond}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.275\pgflinewidth%
  \pgfutil@tempdimb=13\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=1\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.275\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{1\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-6\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-13\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-6\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclare{open diamond}{open diamond}%{{-.5bp}{14.5bp}}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.275\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=14\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.275\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{14\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{7\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{7\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}



% A triangle shaped arrow

\pgfarrowsdeclare{triangle 90}{triangle 90}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=5.5\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpoint{-5.5\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{-5.5\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclarereversed{triangle 90 reversed}{triangle 90 reversed}{triangle 90}{triangle 90}


\pgfarrowsdeclare{triangle 60}{triangle 60}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=7.29\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclarereversed{triangle 60 reversed}{triangle 60 reversed}{triangle 60}{triangle 60}




\pgfarrowsdeclare{triangle 45}{triangle 45}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfutil@tempdimb=8.705\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclarereversed{triangle 45 reversed}{triangle 45 reversed}{triangle 45}{triangle 45}




\pgfarrowsdeclare{open triangle 90}{open triangle 90}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=6\pgfutil@tempdima\advance\pgfutil@tempdimb by0.707\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}

\pgfarrowsdeclare{open triangle 90 reversed}{open triangle 90 reversed}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-.707\pgflinewidth}
  \pgfutil@tempdimb=6\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{6\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}



\pgfarrowsdeclare{open triangle 60}{open triangle 60}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=7.794\pgfutil@tempdima\advance\pgfutil@tempdimb by\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{150}{9\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{7.794\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-150}{9\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqstroke
}



\pgfarrowsdeclare{open triangle 60 reversed}{open triangle 60 reversed}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-\pgflinewidth}
  \pgfutil@tempdimb=7.794\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpointpolar{30}{9\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpointpolar{-30}{9\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}



\pgfarrowsdeclare{open triangle 45}{open triangle 45}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=9.205\pgfutil@tempdima\advance\pgfutil@tempdimb by1.28\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{157}{10\pgfutil@tempdima}}}
  \pgfpathlineto{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}
  \pgfpathlineto{\pgfpointadd{\pgfqpoint{9.205\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-157}{10\pgfutil@tempdima}}}
  \pgfpathclose
  \pgfusepathqstroke
}



\pgfarrowsdeclare{open triangle 45 reversed}{open triangle 45 reversed}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfarrowsleftextend{+-1.28\pgflinewidth}
  \pgfutil@tempdimb=9.205\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.5pt%
  \advance\pgfutil@tempdima by.25\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetmiterjoin
  \pgfpathmoveto{\pgfqpointpolar{23}{10\pgfutil@tempdima}}
  \pgfpathlineto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpointpolar{-23}{10\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqstroke
}



% A less fleshy variant of LaTeX's orginal arrow type

\pgfarrowsdeclare{latex'}{latex'}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-4\pgfutil@tempdima}
  \pgfarrowsrightextend{+6\pgfutil@tempdima}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfpathmoveto{\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{3.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-1\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
  {\pgfqpoint{-4\pgfutil@tempdima}{3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-1.5\pgfutil@tempdima}{1\pgfutil@tempdima}}
  {\pgfqpoint{-1.5\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  {\pgfqpoint{-4\pgfutil@tempdima}{-3.75\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-1\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
  {\pgfqpoint{3.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{6\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfusepathqfill
}

\pgfarrowsdeclarereversed{latex' reversed}{latex' reversed}{latex'}{latex'}


% A rounded variant of the stealth arrow

\pgfarrowsdeclare{stealth'}{stealth'}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfutil@tempdimb=6\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
  \pgfarrowsleftextend{+-\pgfutil@tempdimb}
  \pgfutil@tempdimb=2\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-.5\pgfutil@tempdima}{.5\pgfutil@tempdima}}
  {\pgfqpoint{-3\pgfutil@tempdima}{1.5\pgfutil@tempdima}}
  {\pgfqpoint{-6\pgfutil@tempdima}{3.25\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-3\pgfutil@tempdima}{1\pgfutil@tempdima}}
  {\pgfqpoint{-3\pgfutil@tempdima}{-1\pgfutil@tempdima}}
  {\pgfqpoint{-6\pgfutil@tempdima}{-3.25\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-3\pgfutil@tempdima}{-1.5\pgfutil@tempdima}}
  {\pgfqpoint{-.5\pgfutil@tempdima}{-.5\pgfutil@tempdima}}
  {\pgfqpoint{2\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\pgfarrowsdeclarereversed{stealth' reversed}{stealth' reversed}{stealth'}{stealth'}



% The two half of the $\to$ arrow

\pgfarrowsdeclare{left to}{left to}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-2.75\pgfutil@tempdima}{2.5\pgfutil@tempdima}}
  {\pgfqpoint{0pt}{0.25\pgfutil@tempdima}}
  {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{0.55\pgfutil@tempdima}{-0.125\pgflinewidth}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{-0.125\pgflinewidth}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{-0.125\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{0pt}{-0.125\pgflinewidth}}
  \pgfusepathqstroke
}


\pgfarrowsdeclare{right to}{right to}
{
  \pgfutil@tempdima=-0.84pt%
  \advance\pgfutil@tempdima by-1.3\pgflinewidth%
  \pgfutil@tempdimb=0.21pt%
  \advance\pgfutil@tempdimb by.625\pgflinewidth%
  \pgfarrowsleftextend{+\pgfutil@tempdima}
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfqpoint{-3\pgfutil@tempdima}{-4\pgfutil@tempdima}}
  \pgfpathcurveto
  {\pgfqpoint{-2.75\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}
  {\pgfqpoint{0pt}{-0.25\pgfutil@tempdima}}
  {\pgfqpoint{0.75\pgfutil@tempdima}{0pt}}
  \pgfpathcurveto
  {\pgfqpoint{0.55\pgfutil@tempdima}{0.125\pgflinewidth}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{0.125\pgflinewidth}}
  {\pgfqpoint{0.5\pgfutil@tempdima}{0.125\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{0pt}{0.125\pgflinewidth}}
  \pgfusepathqstroke
}



% The halfs of the $\to$ arrow reversed

\pgfarrowsdeclare{left to reversed}{left to reversed}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.9\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{4\pgfutil@tempdima}}
    \pgfpathcurveto{\pgfqpoint{3.5\pgfutil@tempdima}{2.5\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{0.25\pgfutil@tempdima}}{\pgfqpoint{0pt}{0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{4\pgfutil@tempdima}}
    \pgfpathcurveto{\pgfqpoint{3.5\pgfutil@tempdima}{2.5\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{0.25\pgfutil@tempdima}}{\pgfqpoint{0pt}{-0.125\pgflinewidth}}
  }
  \pgfusepathqstroke%
}

\pgfarrowsdeclare{right to reversed}{right to reversed}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfarrowsleftextend{+-.1\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.9\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.28pt%
  \advance\pgfutil@tempdima by.3\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundjoin
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{-0.1\pgflinewidth}{0pt}}
  \pgfusepathqstroke
  \pgfsetroundcap
  \pgfsetlinewidth{.8\pgflinewidth}
  {\pgftransformxshift{0.625\pgflinewidth}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4\pgfutil@tempdima}}
    \pgfpathcurveto{\pgfqpoint{3.5\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}{\pgfqpoint{0pt}{-0.125\pgflinewidth}}
    \pgfpathmoveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4\pgfutil@tempdima}}
    \pgfpathcurveto{\pgfqpoint{3.5\pgfutil@tempdima}{-2.5\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{-0.25\pgfutil@tempdima}}{\pgfqpoint{0pt}{0.125\pgflinewidth}}
  }
  \pgfusepathqstroke%
}



% A left hook

\pgfarrowsdeclare{left hook}{left hook}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{1.665\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{3\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{3.75\pgfutil@tempdima}{4.665\pgfutil@tempdima}}{\pgfqpoint{2.415\pgfutil@tempdima}{6\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}

\pgfarrowsdeclarereversed{left hook reversed}{left hook reversed}{left hook}{left hook}



% A right hook

\pgfarrowsdeclare{right hook}{right hook}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{-1.665\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{-3\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4.665\pgfutil@tempdima}}{\pgfqpoint{2.415\pgfutil@tempdima}{-6\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}

\pgfarrowsdeclarereversed{right hook reversed}{right hook reversed}{right hook}{right hook}


% Hooks in both directions

\pgfarrowsdeclare{hooks}{hooks}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfarrowsleftextend{+-.5\pgflinewidth}
  \pgfutil@tempdimb=3.75\pgfutil@tempdima\advance\pgfutil@tempdimb by0.5\pgflinewidth%
  \pgfarrowsrightextend{+\pgfutil@tempdimb}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.2\pgflinewidth%
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfqpoint{0\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{1.665\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{3\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{3.75\pgfutil@tempdima}{4.665\pgfutil@tempdima}}{\pgfqpoint{2.415\pgfutil@tempdima}{6\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{6\pgfutil@tempdima}}
  \pgfpathmoveto{\pgfqpoint{0.75\pgfutil@tempdima}{0\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{2.415\pgfutil@tempdima}{0\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{-1.665\pgfutil@tempdima}}{\pgfqpoint{3.75\pgfutil@tempdima}{-3\pgfutil@tempdima}}
  \pgfpathcurveto{\pgfqpoint{3.75\pgfutil@tempdima}{-4.665\pgfutil@tempdima}}{\pgfqpoint{2.415\pgfutil@tempdima}{-6\pgfutil@tempdima}}{\pgfqpoint{0.75\pgfutil@tempdima}{-6\pgfutil@tempdima}}
  \pgfusepathqstroke%
}

\pgfarrowsdeclarereversed{hooks reversed}{hooks reversed}{hooks}{hooks}


% An arrow that looks like a serif of the computer modern font

\pgfarrowsdeclare{serif cm}{serif cm}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.45\pgflinewidth%
  \pgfarrowsleftextend{+-.75\pgfutil@tempdima}
  \pgfarrowsrightextend{+.04\pgflinewidth}
}
{
  \pgfutil@tempdima=0.4pt%
  \advance\pgfutil@tempdima by.45\pgflinewidth%
  \pgftransformxshift{.04\pgflinewidth}
  \pgfpathmoveto{\pgfqpoint{-.75\pgfutil@tempdima}{.5\pgflinewidth}}
  \pgfpathcurveto
    {\pgfqpoint{-.375\pgfutil@tempdima}{.5\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{.7\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{1.95\pgfutil@tempdima}}
  \pgfpathlineto{\pgfqpoint{0pt}{1.95\pgfutil@tempdima}}
  \pgfpathcurveto
    {\pgfqpoint{-.04\pgflinewidth}{.5\pgfutil@tempdima}}
    {\pgfqpoint{-.04\pgflinewidth}{-.5\pgfutil@tempdima}}
    {\pgfqpoint{0pt}{-1.95\pgfutil@tempdima}}  
  \pgfpathlineto{\pgfqpoint{-.375\pgfutil@tempdima}{-1.95\pgfutil@tempdima}}  
  \pgfpathcurveto
    {\pgfqpoint{-.375\pgfutil@tempdima}{-.7\pgflinewidth}}
    {\pgfqpoint{-.375\pgfutil@tempdima}{-.5\pgflinewidth}}
    {\pgfqpoint{-.75\pgfutil@tempdima}{-.5\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}



% Round cap

\pgfarrowsdeclare{round cap}{round cap}
{\pgfarrowsleftextend{+0pt}\pgfarrowsrightextend{+\pgflinewidth}}
{
  \pgfsetdash{}{+0pt}
  \pgfsetroundcap
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}


% Butt cap

\pgfarrowsdeclare{butt cap}{butt cap}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+.5\pgflinewidth}}
{
  \pgfsetdash{}{+0pt}
  \pgfsetbuttcap
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0pt}}
  \pgfusepathqstroke
}



% 90 degrees cap

\pgfarrowsdeclare{triangle 90 cap}{triangle 90 cap}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+\pgflinewidth}}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{\pgflinewidth}{0pt}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfusepathqfill
}


% reversed 90 degrees cap

\pgfarrowsdeclare{triangle 90 cap reversed}{triangle 90 cap reversed}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+\pgflinewidth}}
{
  \pgfpathmoveto{\pgfqpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{0.5\pgflinewidth}{0\pgflinewidth}}
  \pgfusepathqfill
}



% fast

\pgfarrowsdeclare{fast cap}{fast cap}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+2\pgflinewidth}}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfqpoint{1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}


\pgfarrowsdeclare{fast cap reversed}{fast cap reversed}
{\pgfarrowsleftextend{+-.1\pgflinewidth}\pgfarrowsrightextend{+2\pgflinewidth}}
{
  \pgfpathmoveto{\pgfqpoint{-.1\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{-.1\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathclose
  \pgfpathmoveto{\pgfqpoint{1.5\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{0\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{2\pgflinewidth}{-.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1.5\pgflinewidth}{-0.5\pgflinewidth}}
  \pgfpathlineto{\pgfqpoint{1\pgflinewidth}{0\pgflinewidth}}
  \pgfpathclose
  \pgfusepathqfill
}


\endinput


==> pgflibrarydecorations.footprints.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}


% Parameters
\pgfset{
  % Length of a footprint:
  /pgf/decoration/foot length/.initial=10pt,
  % Distance between two footprints on the same side of the path
  /pgf/decoration/stride length/.initial=30pt,
  % Double distance between footprint and input path
  /pgf/decoration/foot sep/.initial=4pt,
  % Rotate feet by this much
  /pgf/decoration/foot angle/.initial=10,
  % What animal?
  /pgf/decoration/foot of/.initial=human,
}



\pgfdeclaredecoration{footprints}{left}
{
  \state{left}[width=\pgfkeysvalueof{/pgf/decoration/stride length}/2,next state=right]
  {
    \pgftransformyshift{\pgfkeysvalueof{/pgf/decoration/foot sep}/2}
    \pgfmathparse{\pgfkeysvalueof{/pgf/decoration/foot length}}
    \pgftransformscale{\pgfmathresult}
    \pgftransformrotate{\pgfkeysvalueof{/pgf/decoration/foot angle}}
    \csname pgf@lib@foot@of@\pgfkeysvalueof{/pgf/decoration/foot of}\endcsname
  }
  \state{right}[width=\pgfkeysvalueof{/pgf/decoration/stride length}/2,next state=left]
  {
    \pgftransformyscale{-1}
    \pgftransformyshift{\pgfkeysvalueof{/pgf/decoration/foot sep}/2}
    \pgfmathparse{\pgfkeysvalueof{/pgf/decoration/foot length}}
    \pgftransformscale{\pgfmathresult}
    \pgftransformrotate{\pgfkeysvalueof{/pgf/decoration/foot angle}}
    \csname pgf@lib@foot@of@\pgfkeysvalueof{/pgf/decoration/foot of}\endcsname
  }
}



% Actual footprints. 
%
% A footprint must be name \pgf@lib@foot@of@XXX, be a left foot and
% should fill a rectangle of (0,0) rectangle (1pt,1pt) (more or less)
% and point right. 
%


\def\pgf@lib@foot@of@gnome{
  % Coordinates from a Gnome logo on wikimedia commons. LGPL
  % license... Unknown author.
  % 
  % Flip and rotate
  \pgftransformcm{0}{-1}{-1}{0}{\pgfqpoint{1pt}{0.8pt}}
  \pgftransformscale{0.83333}
  \pgfpathmoveto{\pgfqpoint{.86068pt}{0pt}}
  \pgfpathcurveto{\pgfqpoint{.61466pt}{0pt}}{\pgfqpoint{.56851pt}{.35041pt}}{\pgfqpoint{.70691pt}{.35041pt}}
  \pgfpathcurveto{\pgfqpoint{.84529pt}{.35041pt}}{\pgfqpoint{1.10671pt}{0pt}}{\pgfqpoint{.86068pt}{0pt}}
  \pgfpathclose
  % 
  \pgfpathmoveto{\pgfqpoint{.45217pt}{.30699pt}}
  \pgfpathcurveto{\pgfqpoint{.52586pt}{.31149pt}}{\pgfqpoint{.60671pt}{.02577pt}}{\pgfqpoint{.46821pt}{.04374pt}}
  \pgfpathcurveto{\pgfqpoint{.32976pt}{.06171pt}}{\pgfqpoint{.37845pt}{.30249pt}}{\pgfqpoint{.45217pt}{.30699pt}}
  \pgfpathclose
  % 
  \pgfpathmoveto{\pgfqpoint{.11445pt}{.48453pt}}
  \pgfpathcurveto{\pgfqpoint{.16686pt}{.46146pt}}{\pgfqpoint{.1212pt}{.23581pt}}{\pgfqpoint{.03208pt}{.29735pt}}
  \pgfpathcurveto{\pgfqpoint{-.057pt}{.3589pt}}{\pgfqpoint{.06204pt}{.50759pt}}{\pgfqpoint{.11445pt}{.48453pt}}
  \pgfpathclose
  % 
  \pgfpathmoveto{\pgfqpoint{.26212pt}{.36642pt}}
  \pgfpathcurveto{\pgfqpoint{.32451pt}{.3537pt}}{\pgfqpoint{.32793pt}{.09778pt}}{\pgfqpoint{.21667pt}{.14369pt}}
  \pgfpathcurveto{\pgfqpoint{.10539pt}{.18961pt}}{\pgfqpoint{.19978pt}{.37916pt}}{\pgfqpoint{.26212pt}{.36642pt}}
  \pgfpathlineto{\pgfqpoint{.26212pt}{.36642pt}}
  \pgfpathclose
  % 
  \pgfpathmoveto{\pgfqpoint{.58791pt}{.93913pt}}
  \pgfpathcurveto{\pgfqpoint{.59898pt}{1.02367pt}}{\pgfqpoint{.52589pt}{1.06542pt}}{\pgfqpoint{.45431pt}{1.01092pt}}
  \pgfpathcurveto{\pgfqpoint{.22644pt}{.83743pt}}{\pgfqpoint{.8316pt}{.75088pt}}{\pgfqpoint{.79171pt}{.51386pt}}
  \pgfpathcurveto{\pgfqpoint{.7586pt}{.31712pt}}{\pgfqpoint{.15495pt}{.37769pt}}{\pgfqpoint{.08621pt}{.68553pt}}
  \pgfpathcurveto{\pgfqpoint{.03968pt}{.89374pt}}{\pgfqpoint{.27774pt}{1.1826pt}}{\pgfqpoint{.52614pt}{1.1826pt}}
  \pgfpathcurveto{\pgfqpoint{.64834pt}{1.1826pt}}{\pgfqpoint{.78929pt}{1.07226pt}}{\pgfqpoint{.81566pt}{.93248pt}}
  \pgfpathcurveto{\pgfqpoint{.8358pt}{.82589pt}}{\pgfqpoint{.57867pt}{.8686pt}}{\pgfqpoint{.58791pt}{.93913pt}}
  \pgfpathlineto{\pgfqpoint{.58791pt}{.93913pt}}
  \pgfpathclose
}  



\def\pgf@lib@foot@of@bird{
  % Coordinates derived from vector image created by Mark Wibrow.
  %
  \pgftransformcm{0}{.11}{.11}{0}{\pgfqpoint{.37pt}{.52pt}}
  \pgfpathmoveto{\pgfqpoint{-.886pt}{1.652pt}}
  \pgfpathcurveto{\pgfqpoint{-.4632pt}{2.669pt}}{\pgfqpoint{-.5092pt}{4.3712pt}}{\pgfqpoint{-.4512pt}{5.6734pt}}
  \pgfpathcurveto{\pgfqpoint{-.4374pt}{5.9842pt}}{\pgfqpoint{-.3182pt}{6.0686pt}}{\pgfqpoint{-.2484pt}{5.644pt}}
  \pgfpathcurveto{\pgfqpoint{-.0534pt}{4.459pt}}{\pgfqpoint{.087pt}{3.0132pt}}{\pgfqpoint{.5206pt}{1.8464pt}}
  \pgfpathcurveto{\pgfqpoint{.714pt}{1.326pt}}{\pgfqpoint{.692pt}{1.416pt}}{\pgfqpoint{1.0864pt}{1.759pt}}
  \pgfpathcurveto{\pgfqpoint{1.7662pt}{2.3504pt}}{\pgfqpoint{2.665pt}{3.1756pt}}{\pgfqpoint{3.2028pt}{4.02pt}}
  \pgfpathcurveto{\pgfqpoint{3.4708pt}{4.4408pt}}{\pgfqpoint{3.4258pt}{4.0814pt}}{\pgfqpoint{3.3366pt}{3.8708pt}}
  \pgfpathcurveto{\pgfqpoint{2.9068pt}{2.8562pt}}{\pgfqpoint{.8502pt}{.645pt}}{\pgfqpoint{.4808pt}{-.0864pt}}
  \pgfpathcurveto{\pgfqpoint{.0808pt}{-.8788pt}}{\pgfqpoint{.1664pt}{-2.1246pt}}{\pgfqpoint{.0024pt}{-2.7868pt}}
  \pgfpathcurveto{\pgfqpoint{-.172pt}{-3.4908pt}}{\pgfqpoint{-.2726pt}{-3.704pt}}{\pgfqpoint{-.3812pt}{-2.9558pt}}
  \pgfpathcurveto{\pgfqpoint{-.5316pt}{-1.9202pt}}{\pgfqpoint{-.88pt}{-.256pt}}{\pgfqpoint{-1.332pt}{.128pt}}
  \pgfpathcurveto{\pgfqpoint{-1.716pt}{.4542pt}}{\pgfqpoint{-3.7928pt}{2.3136pt}}{\pgfqpoint{-4.5044pt}{3.3524pt}}
  \pgfpathcurveto{\pgfqpoint{-4.7618pt}{3.728pt}}{\pgfqpoint{-4.709pt}{3.7864pt}}{\pgfqpoint{-4.4212pt}{3.5818pt}}
  \pgfpathcurveto{\pgfqpoint{-3.4844pt}{2.9162pt}}{\pgfqpoint{-2.6164pt}{1.654pt}}{\pgfqpoint{-1.454pt}{1.3886pt}}
  \pgfpathcurveto{\pgfqpoint{-1.0876pt}{1.305pt}}{\pgfqpoint{-1.0296pt}{1.3066pt}}{\pgfqpoint{-.886pt}{1.652pt}}
  \pgfpathclose
}


\expandafter\def\csname pgf@lib@foot@of@felis silvestris\endcsname{
  % Coordinates derived from vector image created by Mark Wibrow, based
  % on the forefoot of `felis silvestris' shown in
  % Pearson, B. and Burton, J. A. (1980), `Wild Animals', Collins, 155.
  % 
  \pgftransformcm{0}{.1}{.1}{0}{\pgfqpoint{.48pt}{.5pt}}
  \pgfpathmoveto{\pgfqpoint{2.7312pt}{-1.992pt}}
  \pgfpathcurveto{\pgfqpoint{1.8716pt}{-1.4226pt}}{\pgfqpoint{2.1404pt}{.0436pt}}{\pgfqpoint{.9202pt}{.0436pt}}
  \pgfpathcurveto{\pgfqpoint{-.1146pt}{.0436pt}}{\pgfqpoint{-.7386pt}{.0178pt}}{\pgfqpoint{-1.319pt}{-1.0288pt}}
  \pgfpathcurveto{\pgfqpoint{-1.7922pt}{-1.8822pt}}{\pgfqpoint{-2.072pt}{-1.5488pt}}{\pgfqpoint{-2.9638pt}{-1.968pt}}
  \pgfpathcurveto{\pgfqpoint{-3.9244pt}{-2.4198pt}}{\pgfqpoint{-4.4394pt}{-3.348pt}}{\pgfqpoint{-4.1136pt}{-4.041pt}}
  \pgfpathcurveto{\pgfqpoint{-3.3862pt}{-5.5882pt}}{\pgfqpoint{-1.6156pt}{-3.83pt}}{\pgfqpoint{-1.1684pt}{-4.312pt}}
  \pgfpathcurveto{\pgfqpoint{-.5806pt}{-4.9454pt}}{\pgfqpoint{.5032pt}{-4.8822pt}}{\pgfqpoint{1.1748pt}{-4.2878pt}}
  \pgfpathcurveto{\pgfqpoint{1.5822pt}{-3.9272pt}}{\pgfqpoint{2.6524pt}{-5.0652pt}}{\pgfqpoint{3.3506pt}{-4.1066pt}}
  \pgfpathcurveto{\pgfqpoint{3.839pt}{-3.4356pt}}{\pgfqpoint{3.1192pt}{-2.249pt}}{\pgfqpoint{2.7312pt}{-1.992pt}}
  \pgfpathclose
  %
  \pgfpathmoveto{\pgfqpoint{5.0576pt}{.4996pt}}
  \pgfpathcurveto{\pgfqpoint{4.6056pt}{.6536pt}}{\pgfqpoint{4.0596pt}{.2516pt}}{\pgfqpoint{3.8382pt}{-.398pt}}
  \pgfpathcurveto{\pgfqpoint{3.6168pt}{-1.0478pt}}{\pgfqpoint{3.8038pt}{-1.6996pt}}{\pgfqpoint{4.2558pt}{-1.8536pt}}
  \pgfpathcurveto{\pgfqpoint{4.7078pt}{-2.0076pt}}{\pgfqpoint{5.2538pt}{-1.6056pt}}{\pgfqpoint{5.4752pt}{-.9558pt}}
  \pgfpathcurveto{\pgfqpoint{5.6966pt}{-.3062pt}}{\pgfqpoint{5.5096pt}{.3456pt}}{\pgfqpoint{5.0576pt}{.4996pt}}
  \pgfpathclose
  %
  \pgfpathmoveto{\pgfqpoint{3.1212pt}{3.5542pt}}
  \pgfpathcurveto{\pgfqpoint{2.5874pt}{3.6726pt}}{\pgfqpoint{1.975pt}{3.1756pt}}{\pgfqpoint{1.7538pt}{2.4442pt}}
  \pgfpathcurveto{\pgfqpoint{1.5324pt}{1.7128pt}}{\pgfqpoint{1.7858pt}{1.0238pt}}{\pgfqpoint{2.3196pt}{.9052pt}}
  \pgfpathcurveto{\pgfqpoint{2.8534pt}{.7868pt}}{\pgfqpoint{3.4658pt}{1.2838pt}}{\pgfqpoint{3.6872pt}{2.0152pt}}
  \pgfpathcurveto{\pgfqpoint{3.9084pt}{2.7466pt}}{\pgfqpoint{3.655pt}{3.4358pt}}{\pgfqpoint{3.1212pt}{3.5542pt}}
  \pgfpathclose
  % 
  \pgfpathmoveto{\pgfqpoint{-.6182pt}{5.0456pt}}
  \pgfpathcurveto{\pgfqpoint{-1.2132pt}{5.0456pt}}{\pgfqpoint{-1.6956pt}{4.3104pt}}{\pgfqpoint{-1.6956pt}{3.4038pt}}
  \pgfpathcurveto{\pgfqpoint{-1.6956pt}{2.4972pt}}{\pgfqpoint{-1.2132pt}{1.7618pt}}{\pgfqpoint{-.6182pt}{1.7618pt}}
  \pgfpathcurveto{\pgfqpoint{-.0232pt}{1.7618pt}}{\pgfqpoint{.4592pt}{2.4972pt}}{\pgfqpoint{.4592pt}{3.4038pt}}
  \pgfpathcurveto{\pgfqpoint{.4592pt}{4.3104pt}}{\pgfqpoint{-.0232pt}{5.0456pt}}{\pgfqpoint{-.6182pt}{5.0456pt}}
  \pgfpathclose
  % 
  \pgfpathmoveto{\pgfqpoint{-4.1176pt}{1.8248pt}}
  \pgfpathcurveto{\pgfqpoint{-4.6334pt}{1.7534pt}}{\pgfqpoint{-4.9806pt}{1.0312pt}}{\pgfqpoint{-4.8928pt}{.212pt}}
  \pgfpathcurveto{\pgfqpoint{-4.8052pt}{-.6072pt}}{\pgfqpoint{-4.3158pt}{-1.2136pt}}{\pgfqpoint{-3.8pt}{-1.1422pt}}
  \pgfpathcurveto{\pgfqpoint{-3.2842pt}{-1.0708pt}}{\pgfqpoint{-2.9372pt}{-.3486pt}}{\pgfqpoint{-3.0248pt}{.4706pt}}
  \pgfpathcurveto{\pgfqpoint{-3.1126pt}{1.2898pt}}{\pgfqpoint{-3.6018pt}{1.8962pt}}{\pgfqpoint{-4.1176pt}{1.8248pt}}
  \pgfpathclose
}



\def\pgf@lib@foot@of@human{%
  % Coordinates derived from vector image created by Mark Wibrow.
  \pgftransformcm{0}{.5}{.5}{0}{\pgfqpoint{.48pt}{.2pt}}
  % 
  % Draw main part of foot.
  % 
  \pgfpathmoveto{\pgfqpoint{.20175pt}{-.72633pt}}
  \pgfpathcurveto{\pgfqpoint{.16314pt}{-.88194pt}}{\pgfqpoint{.07386pt}{-1.0167pt}}{\pgfqpoint{-.08385pt}{-1.0167pt}}
  \pgfpathcurveto{\pgfqpoint{-.24153pt}{-1.0167pt}}{\pgfqpoint{-.36942pt}{-.84897pt}}{\pgfqpoint{-.36942pt}{-.72633pt}}
  \pgfpathcurveto{\pgfqpoint{-.36942pt}{-.60372pt}}{\pgfqpoint{-.32505pt}{-.54825pt}}{\pgfqpoint{-.27633pt}{-.51192pt}}
  \pgfpathcurveto{\pgfqpoint{-.23937pt}{-.48435pt}}{\pgfqpoint{-.17031pt}{-.46539pt}}{\pgfqpoint{-.10611pt}{-.40323pt}}
  \pgfpathcurveto{\pgfqpoint{-.04191pt}{-.3411pt}}{\pgfqpoint{.00495pt}{-.27783pt}}{\pgfqpoint{.00495pt}{-.14787pt}}
  \pgfpathcurveto{\pgfqpoint{.00495pt}{-.01794pt}}{\pgfqpoint{-.08526pt}{.12648pt}}{\pgfqpoint{-.22194pt}{.22467pt}}
  \pgfpathcurveto{\pgfqpoint{-.35862pt}{.32286pt}}{\pgfqpoint{-.40863pt}{.50226pt}}{\pgfqpoint{-.32703pt}{.5979pt}}
  \pgfpathcurveto{\pgfqpoint{-.24543pt}{.69354pt}}{\pgfqpoint{-.00564pt}{.66543pt}}{\pgfqpoint{.17172pt}{.53484pt}}
  \pgfpathcurveto{\pgfqpoint{.34908pt}{.40422pt}}{\pgfqpoint{.39363pt}{.27192pt}}{\pgfqpoint{.37416pt}{.10971pt}}
  \pgfpathcurveto{\pgfqpoint{.35472pt}{-.0525pt}}{\pgfqpoint{.26736pt}{-.46203pt}}{\pgfqpoint{.20175pt}{-.72633pt}}
  \pgfpathclose
  %
  % Draw toe.s
  % 
  \pgfpathmoveto{\pgfqpoint{-.27138pt}{1.01451pt}}
  \pgfpathcurveto{\pgfqpoint{-.21198pt}{1.01451pt}}{\pgfqpoint{-.1638pt}{.94509pt}}{\pgfqpoint{-.1638pt}{.8595pt}}
  \pgfpathcurveto{\pgfqpoint{-.1638pt}{.77388pt}}{\pgfqpoint{-.21198pt}{.70446pt}}{\pgfqpoint{-.27138pt}{.70446pt}}
  \pgfpathcurveto{\pgfqpoint{-.33078pt}{.70446pt}}{\pgfqpoint{-.37896pt}{.77388pt}}{\pgfqpoint{-.37896pt}{.8595pt}}
  \pgfpathcurveto{\pgfqpoint{-.37896pt}{.94509pt}}{\pgfqpoint{-.33078pt}{1.01451pt}}{\pgfqpoint{-.27138pt}{1.01451pt}}
  \pgfpathclose
  %
  \pgfpathmoveto{\pgfqpoint{-.05769pt}{.90573pt}}
  \pgfpathcurveto{\pgfqpoint{-.01659pt}{.90573pt}}{\pgfqpoint{.01674pt}{.86445pt}}{\pgfqpoint{.01674pt}{.81354pt}}
  \pgfpathcurveto{\pgfqpoint{.01674pt}{.7626pt}}{\pgfqpoint{-.01659pt}{.72132pt}}{\pgfqpoint{-.05769pt}{.72132pt}}
  \pgfpathcurveto{\pgfqpoint{-.09879pt}{.72132pt}}{\pgfqpoint{-.13209pt}{.7626pt}}{\pgfqpoint{-.13209pt}{.81354pt}}
  \pgfpathcurveto{\pgfqpoint{-.13209pt}{.86445pt}}{\pgfqpoint{-.09879pt}{.90573pt}}{\pgfqpoint{-.05769pt}{.90573pt}}
  \pgfpathclose
  %
  \pgfpathmoveto{\pgfqpoint{.10497pt}{.81636pt}}
  \pgfpathcurveto{\pgfqpoint{.14214pt}{.81096pt}}{\pgfqpoint{.16722pt}{.77193pt}}{\pgfqpoint{.16104pt}{.72918pt}}
  \pgfpathcurveto{\pgfqpoint{.15483pt}{.68646pt}}{\pgfqpoint{.11964pt}{.65619pt}}{\pgfqpoint{.08247pt}{.66159pt}}
  \pgfpathcurveto{\pgfqpoint{.0453pt}{.66699pt}}{\pgfqpoint{.02019pt}{.70602pt}}{\pgfqpoint{.0264pt}{.74874pt}}
  \pgfpathcurveto{\pgfqpoint{.03261pt}{.79149pt}}{\pgfqpoint{.0678pt}{.82176pt}}{\pgfqpoint{.10497pt}{.81636pt}}
  \pgfpathclose
  % 
  \pgfpathmoveto{\pgfqpoint{.24054pt}{.70842pt}}
  \pgfpathcurveto{\pgfqpoint{.27513pt}{.70842pt}}{\pgfqpoint{.30318pt}{.67686pt}}{\pgfqpoint{.30318pt}{.63795pt}}
  \pgfpathcurveto{\pgfqpoint{.30318pt}{.59904pt}}{\pgfqpoint{.27513pt}{.56751pt}}{\pgfqpoint{.24054pt}{.56751pt}}
  \pgfpathcurveto{\pgfqpoint{.20598pt}{.56751pt}}{\pgfqpoint{.17793pt}{.59904pt}}{\pgfqpoint{.17793pt}{.63795pt}}
  \pgfpathcurveto{\pgfqpoint{.17793pt}{.67686pt}}{\pgfqpoint{.20598pt}{.70842pt}}{\pgfqpoint{.24054pt}{.70842pt}}
  \pgfpathclose
  % 
  \pgfpathmoveto{\pgfqpoint{.35973pt}{.57501pt}}
  \pgfpathcurveto{\pgfqpoint{.3918pt}{.57501pt}}{\pgfqpoint{.41781pt}{.54852pt}}{\pgfqpoint{.41781pt}{.51585pt}}
  \pgfpathcurveto{\pgfqpoint{.41781pt}{.48318pt}}{\pgfqpoint{.3918pt}{.45669pt}}{\pgfqpoint{.35973pt}{.45669pt}}
  \pgfpathcurveto{\pgfqpoint{.32769pt}{.45669pt}}{\pgfqpoint{.30168pt}{.48318pt}}{\pgfqpoint{.30168pt}{.51585pt}}
  \pgfpathcurveto{\pgfqpoint{.30168pt}{.54852pt}}{\pgfqpoint{.32769pt}{.57501pt}}{\pgfqpoint{.35973pt}{.57501pt}}
  \pgfpathclose
}


\endinput

==> pgflibrarydecorations.fractals.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}



\pgfdeclaredecoration{Koch curve type 1}{init}
{
  \state{init}[width=\pgfdecoratedinputsegmentremainingdistance]
  {
    \pgfpathlineto{\pgfpoint{.33333\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathlineto{\pgfpoint{.33333\pgfdecoratedinputsegmentremainingdistance}{.33333\pgfdecoratedinputsegmentremainingdistance}}
    \pgfpathlineto{\pgfpoint{.66666\pgfdecoratedinputsegmentremainingdistance}{.33333\pgfdecoratedinputsegmentremainingdistance}}
    \pgfpathlineto{\pgfpoint{.66666\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgfdecoratedinputsegmentremainingdistance}{0pt}}
  }
}

\pgfdeclaredecoration{Koch curve type 2}{init}
{
  \state{init}[width=\pgfdecoratedinputsegmentremainingdistance]
  {
    \pgfpathlineto{\pgfpoint{.25\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathlineto{\pgfpoint{.25\pgfdecoratedinputsegmentremainingdistance}{.25\pgfdecoratedinputsegmentremainingdistance}}
    \pgfpathlineto{\pgfpoint{.5\pgfdecoratedinputsegmentremainingdistance}{.25\pgfdecoratedinputsegmentremainingdistance}}
    \pgfpathlineto{\pgfpoint{.5\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathlineto{\pgfpoint{.5\pgfdecoratedinputsegmentremainingdistance}{-.25\pgfdecoratedinputsegmentremainingdistance}}
    \pgfpathlineto{\pgfpoint{.75\pgfdecoratedinputsegmentremainingdistance}{-.25\pgfdecoratedinputsegmentremainingdistance}}
    \pgfpathlineto{\pgfpoint{.75\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgfdecoratedinputsegmentremainingdistance}{0pt}}
  }
}

\pgfdeclaredecoration{Koch snowflake}{init}
{
  \state{init}[width=\pgfdecoratedinputsegmentremainingdistance]
  {
    \pgfpathlineto{\pgfpoint{.3333\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathlineto{\pgfpoint{.5\pgfdecoratedinputsegmentremainingdistance}{0.2886751347\pgfdecoratedinputsegmentremainingdistance}}
    \pgfpathlineto{\pgfpoint{.6666\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgfdecoratedinputsegmentremainingdistance}{0pt}}
  }
}


\pgfdeclaredecoration{Cantor set}{init}
{
  \state{init}[width=\pgfdecoratedinputsegmentremainingdistance]
  {
    \pgfpathlineto{\pgfpoint{.3333\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathmoveto{\pgfpoint{.6666\pgfdecoratedinputsegmentremainingdistance}{0pt}}
    \pgfpathlineto{\pgfpoint{\pgfdecoratedinputsegmentremainingdistance}{0pt}}
  }
}



\endinput

==> pgflibrarydecorations.markings.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}


% A marking decoration is used to add markings (which are just pgf
% scopes, essentially) at certain positions of a path.

\pgfkeys{
  /pgf/decoration/reset marks/.code=\let\pgf@lib@dec@mark@marks=\pgfutil@empty,
  /pgf/decoration/mark/.code=\pgf@lib@dec@parsemark#1\pgf@lib@dec@stop,
}

\let\pgf@lib@dec@mark@marks=\pgfutil@empty

\def\pgf@lib@dec@parsemark at position#1with#2\pgf@lib@dec@stop{%
  \expandafter\def\expandafter\pgf@lib@dec@mark@marks\expandafter{\pgf@lib@dec@mark@marks%
    \pgf@lib@dec@domark{#1}{#2}%
  }%
}

\def\pgf@lib@dec@arrowhead#1#2{%
  \expandafter\ifx\csname tikz@special@arrow@end#2\endcsname\relax% be nice to TikZ
    \pgfsetarrowsend{#2}
  \else%
    \pgfsetarrowsend{\csname tikz@special@arrow@end#2\endcsname}%
  \fi%
  \pgf@x=0pt%
  \pgf@shorten@end%
  \pgftransformxshift{-\pgf@x}
  \pgftransformxscale{#1}
  \pgflowlevelsynccm%
  \pgflowlevelobj{}{\pgf@endarrow}%
}

\def\pgf@lib@dec@doarrowhead#1{%
  \pgf@lib@dec@arrowhead{1}{#1}%
}
\def\pgf@lib@dec@doarrowheadrev#1{%
  \pgf@lib@dec@arrowhead{-1}{#1}%
}


\pgfdeclaredecoration{markings}{pre}
{
  \state{pre}
  [
    width=0pt,
    persistent precomputation={%
      \pgf@lib@dec@mark@marks\pgf@lib@dec@mark@last%
      \let\arrow=\pgf@lib@dec@doarrowhead%
      \let\arrowreversed=\pgf@lib@dec@doarrowheadrev%
    },
    next state=skipper
  ]
  {}

  \state{skipper}[width=\pgf@lib@dec@computed@width-\pgfdecoratedcompleteddistance-1sp,
                  next state=\pgf@lib@dec@next@state]{}
  
  \state{main}
  [
    width=1sp,
    next state=pre
  ]
  {%
    \pgfinterruptpath%
      \pgfscope%
        \let\pgf@lib@dec@mark@marks=\pgfutil@empty%
        \pgf@lib@dec@computed@action%
      \endpgfscope%
    \endpgfinterruptpath%
  }%

  \state{final}[width=\pgfdecoratedremainingdistance]{}
}

\def\pgf@lib@dec@domark#1#2#3\pgf@lib@dec@mark@last{%
  \def\pgf@lib@dec@mark@marks{#3}%
  \pgf@lib@dec@parsenum{#1}%
  \def\pgf@lib@dec@computed@action{#2}%
  \def\pgf@lib@dec@next@state{main}%
}

\def\pgf@lib@dec@parsenum#1{%
  \pgfmathparse{#1}%
  \ifpgfmathunitsdeclared%
    \ifdim\pgfmathresult pt<0pt\relax%
      \edef\pgf@lib@dec@computed@width{\pgfdecoratedpathlength\pgfmathresult pt}%
    \else%
      \edef\pgf@lib@dec@computed@width{\pgfmathresult pt}%
    \fi%
  \else%  
    \ifdim\pgfmathresult pt<0pt\relax%
      \edef\pgf@lib@dec@computed@width{\pgfdecoratedpathlength\pgfmathresult*\pgfdecoratedpathlength}%
    \else%
      \edef\pgf@lib@dec@computed@width{\pgfmathresult*\pgfdecoratedpathlength}%
    \fi%
  \fi%
}

\def\pgf@lib@dec@mark@last{%
  \def\pgf@lib@dec@next@state{final}%
}


\endinput

==> pgflibrarydecorations.pathmorphing.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}


%
% These decorations "morph" paths. That means that the
% orginal characteristic of the path is kept and the number of
% subpaths remains the same -- only, the lines are slightly offset or
% changed by the decoration. For instance a line might be turned into
% a squiggly line or a snaking line or a bumping line.
%


%
%
% Kind 1: Path morphing straight line decorations
%
%


% zigzag decoration.
%
\pgfdeclaredecoration{zigzag}{up from center}{
  \state{up from center}[width=+.5\pgfdecorationsegmentlength, next state=big down]
  {
    \pgfpathlineto{\pgfqpoint{.25\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
  }
  \state{big down}[switch if less than=+.5\pgfdecorationsegmentlength to center finish,
                   width=+.5\pgfdecorationsegmentlength,
                   next state=big up]
  {
    \pgfpathlineto{\pgfqpoint{.25\pgfdecorationsegmentlength}{-\pgfdecorationsegmentamplitude}}
  }
  \state{big up}[switch if less than=+.5\pgfdecorationsegmentlength to center finish,
                 width=+.5\pgfdecorationsegmentlength,
                 next state=big down]
  {
    \pgfpathlineto{\pgfqpoint{.25\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
  }
  \state{center finish}[width=0pt, next state=final]{
    \pgfpathlineto{\pgfpointorigin}
  }
  \state{final}
  {
    \pgfpathlineto{\pgfpointdecoratedpathlast}
  }
}




% saw decoration
%
% Parameters: \pgfdecorationsegmentamplitude, \pgfdecorationsegmentlength

\pgfdeclaredecoration{saw}{initial}
{
  \state{initial}[auto end on length=+\pgfdecorationsegmentlength,
                  auto corner on length=+\pgfdecorationsegmentlength,
                  width=+\pgfdecorationsegmentlength]
  {
    \pgfpathlineto{\pgfqpoint{\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{\pgfdecorationsegmentlength}{0pt}}
  }
  \state{final}
  {}
}




% random steps decoration
%
% A decoration that consists of random steps heading towards the target
%
% Parameters: \pgfdecorationsegmentamplitude, \pgfdecorationsegmentlength

\pgfdeclaredecoration{random steps}{start}
{
  \state{start}[width=+0pt,next state=step,persistent precomputation=\pgfdecoratepathhascornerstrue]{}
  \state{step}[auto end on length=1.5\pgfdecorationsegmentlength,
               auto corner on length=1.5\pgfdecorationsegmentlength,               
               width=+\pgfdecorationsegmentlength]
  {
    \pgfpathlineto{
      \pgfpointadd
      {\pgfpoint{\pgfdecorationsegmentlength}{0pt}}
      {\pgfpoint{rand*\pgfdecorationsegmentamplitude}{rand*\pgfdecorationsegmentamplitude}}
    }
  }
  \state{final}
  {}
}



% Meta-decoration line zigzag

\pgfdeclaremetadecoration{straight zigzag}{line to}{
  \state{line to}[width=\pgfmetadecorationsegmentlength, next state=zigzag]
  {
    \decoration{curveto}
  }
  \state{zigzag}[width=\pgfmetadecorationsegmentlength, next state=line to]
  {
    \decoration{zigzag}	
  }
  \state{final}
  {
    \decoration{curveto}
  }
}





%
%
% Kind 2: Path morphing curved decorations
%
%



% bent decoration
%
% A decoration that looks like someone bent the line a bit.
%
% Parameters: \pgfdecorationsegmentamplitude, \pgfdecorationsegmentaspect

\pgfdeclaredecoration{bent}{bent}
{
  \state{bent}[width=+\pgfdecoratedinputsegmentremainingdistance]
  {
    \pgfpathcurveto
    {\pgfqpoint{\pgfdecorationsegmentaspect\pgfdecoratedinputsegmentremainingdistance}{\pgfdecorationsegmentamplitude}}
    {\pgfpointadd{\pgfqpoint{\pgfdecoratedinputsegmentremainingdistance}{0pt}}
       {\pgfqpoint{-\pgfdecorationsegmentaspect\pgfdecoratedinputsegmentremainingdistance}{\pgfdecorationsegmentamplitude}}}
    {\pgfqpoint{\pgfdecoratedinputsegmentremainingdistance}{0pt}}
  }
  \state{final}
  {}
}



% decoration snake
%
% This decoration produces a hopefully optically pleasing squiggly snake. 
%
% Parameters: \pgfdecorationsegmentamplitude, \pgfdecorationsegmentlength

\pgfdeclaredecoration{snake}{initial}
{
  \state{initial}[switch if less than=+.625\pgfdecorationsegmentlength to final,
                  width=+.3125\pgfdecorationsegmentlength,
                  next state=down]
  { 
    \pgfpathcurveto
    {\pgfqpoint{.125\pgfdecorationsegmentlength}{0pt}}
    {\pgfqpoint{.1875\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{.3125\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
  }
  \state{down}[switch if less than=+.8125\pgfdecorationsegmentlength to end down,
               width=+.5\pgfdecorationsegmentlength,
               next state=up]
  {
    \pgfpathcosine{\pgfqpoint{.25\pgfdecorationsegmentlength}{-1\pgfdecorationsegmentamplitude}}
    \pgfpathsine{\pgfqpoint{.25\pgfdecorationsegmentlength}{-1\pgfdecorationsegmentamplitude}}
  }               
  \state{up}[switch if less than=+.8125\pgfdecorationsegmentlength to end up,
             width=+.5\pgfdecorationsegmentlength,
             next state=down]
  {
    \pgfpathcosine{\pgfqpoint{.25\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
    \pgfpathsine{\pgfqpoint{.25\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
  }               
  \state{end down}[width=+.3125\pgfdecorationsegmentlength,
                   next state=final]
  {
    \pgfpathcurveto
    {\pgfqpoint{.125\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{.1875\pgfdecorationsegmentlength}{0pt}}
    {\pgfqpoint{.3125\pgfdecorationsegmentlength}{0pt}}
  }  
  \state{end up}[width=+.3125\pgfdecorationsegmentlength,
                 next state=final]
  {
    \pgfpathcurveto
    {\pgfqpoint{.125\pgfdecorationsegmentlength}{-\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{.1875\pgfdecorationsegmentlength}{0pt}}
    {\pgfqpoint{.3125\pgfdecorationsegmentlength}{0pt}}
  }  
  \state{final}
  {
    \pgfpathlineto{\pgfpointdecoratedpathlast}
  }
}


% coil decoration
%
% Parameters: \pgfdecorationsegmentamplitude, \pgfdecorationsegmentlength,

\pgfdeclaredecoration{coil}{coil}
{
  \state{coil}[switch if less than=%
    1.5\pgfdecorationsegmentlength+%
    \pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude+%
    \pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude to last,
               width=+\pgfdecorationsegmentlength]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{2    }{-0.555}{7}}
    {\pgfpoint@oncoil{1.555}{-1    }{8}}
    {\pgfpoint@oncoil{1    }{-1    }{9}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{0.445}{-1    }{10}}
    {\pgfpoint@oncoil{0    }{-0.555}{11}}
    {\pgfpoint@oncoil{0    }{ 0    }{12}}
  }
  \state{last}[width=.5\pgfdecorationsegmentlength+%
    \pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude+%
    \pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude,next state=final]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
  }
  \state{final}
  {
    \pgfpathlineto{\pgfpointdecoratedpathlast}
  }
}

\def\pgfpoint@oncoil#1#2#3{%
  \pgf@x=#1\pgfdecorationsegmentamplitude%
  \pgf@x=\pgfdecorationsegmentaspect\pgf@x%
  \pgf@y=#2\pgfdecorationsegmentamplitude%
  \pgf@xa=0.083333333333\pgfdecorationsegmentlength%
  \advance\pgf@x by#3\pgf@xa%
}


% bumps decoration
%
% Parameters: \pgfdecorationsegmentamplitude, \pgfdecorationsegmentlength

\pgfdeclaredecoration{bumps}{initial}
{
  \state{initial}[auto end on length=+.51\pgfdecorationsegmentlength,
                  auto corner on length=+.51\pgfdecorationsegmentlength,
                  width=+.5\pgfdecorationsegmentlength]
  {
    \pgfpathcurveto
    {\pgfqpoint{0pt}{.555\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{0.11125\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{.25\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
    \pgfpathcurveto
    {\pgfqpoint{.38875\pgfdecorationsegmentlength}{\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{.5\pgfdecorationsegmentlength}{.5\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{.5\pgfdecorationsegmentlength}{0\pgfdecorationsegmentamplitude}}
  }
  \state{final}
  {
    \pgfpathlineto{\pgfpointdecoratedpathlast}
  }
}








\endinput

==> pgflibrarydecorations.pathreplacing.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}


%
% Path replacing decorations
%
% These decorations change the path by replacing it by another path.
% For instance, a line in the path might be replaced by small
% ticks or unconnected curves or crosses. Applying a chopping
% decoration to a path means that the path can no longer be used for
% filling in the original manner.
%



%
%
% Kind 1: Path chopping with open subpaths
%
%


% ticks decoration
%
% Parameters: \pgfdecorationsegmentlength, \pgfdecorationsegmentamplitude

\pgfdeclaredecoration{ticks}{ticks}
{
  \state{ticks}[width=+\pgfdecorationsegmentlength]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfdecorationsegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfdecorationsegmentamplitude}}
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgfdecorationsegmentamplitude}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgfdecorationsegmentamplitude}}
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }
}



% expanding waves decoration
%
% Parameters: \pgfdecorationsegmentangle, \pgfdecorationsegmentlength

\pgfdeclaredecoration{expanding waves}{initial}
{
  \state{initial}[width=+\pgfdecorationsegmentlength,next state=wave]
  {}

  \state{wave}[switch if less than=+\pgfdecorationsegmentlength to last,
               width=+\pgfdecorationsegmentlength]
  {
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfdecoratedcompleteddistance}{0pt}}%
      {\pgfpointpolar{\pgfdecorationsegmentangle}{+\pgfdecoratedcompleteddistance}}}%
    \pgfpatharc{\pgfdecorationsegmentangle}{-\pgfdecorationsegmentangle}{+\pgfdecoratedcompleteddistance}%
  }
  \state{last}[width=+0pt,next state=final]
  {
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfdecoratedcompleteddistance}{0pt}}%
      {\pgfpointpolar{\pgfdecorationsegmentangle}{+\pgfdecoratedcompleteddistance}}}%
    \pgfpatharc{\pgfdecorationsegmentangle}{-\pgfdecorationsegmentangle}{+\pgfdecoratedcompleteddistance}%
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }
}



% waves decoration

\pgfdeclaredecoration{waves}{wave}
{
  \state{wave}[width=\pgfdecorationsegmentlength]
  {
    \pgftransformxshift{+\pgfdecorationsegmentlength}
    \pgfpathmoveto{
      \pgfpointadd
      {\pgfqpoint{-\pgfkeysvalueof{/pgf/decoration/start radius}}{0pt}}%
      {\pgfpointpolar{\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}}}%
    \pgfpatharc{\pgfdecorationsegmentangle}{-\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}%
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }
}



% border decoration
%
% Parameters: \pgfdecorationsegmentlength, \pgfdecorationsegmentamplitude, \pgfdecorationsegmentangle

\pgfdeclaredecoration{border}{tick}
{
  \state{tick}[switch if less than=+\pgfdecorationsegmentlength to last,
               width=+\pgfdecorationsegmentlength]
  {
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpointpolar{\pgfdecorationsegmentangle}{+\pgfdecorationsegmentamplitude}}
  }
  \state{last}[width=+\pgfdecorationsegmentamplitude,next state=final]
  {
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathlineto{\pgfpointpolar{\pgfdecorationsegmentangle}{+\pgfdecorationsegmentamplitude}}
  }  
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }
}






% brace decorations
%
% Parameters: \pgfdecorationsegmentamplitude

\pgfdeclaredecoration{brace}{brace}
{
  \state{brace}[width=+\pgfdecoratedremainingdistance,next state=final]
  {
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathcurveto
    {\pgfqpoint{.15\pgfdecorationsegmentamplitude}{.3\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{.5\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}}
    {\pgfqpoint{\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}}
    {
      \pgftransformxshift{+\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance}
      \pgfpathlineto{\pgfqpoint{-\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{-.5\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{-.15\pgfdecorationsegmentamplitude}{.7\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{0\pgfdecorationsegmentamplitude}{1\pgfdecorationsegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{.15\pgfdecorationsegmentamplitude}{.7\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{.5\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}}
    }
    {
      \pgftransformxshift{+\pgfdecoratedremainingdistance}
      \pgfpathlineto{\pgfqpoint{-\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}}
      \pgfpathcurveto
      {\pgfqpoint{-.5\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{-.15\pgfdecorationsegmentamplitude}{.3\pgfdecorationsegmentamplitude}}
      {\pgfqpoint{0pt}{0pt}}
    }
  }
  \state{final}
  {}
}




\endinput

==> pgflibrarydecorations.shapes.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}


% Options for shape decorations

\pgfkeys{
  /pgf/decoration/.cd,
  shape/.initial=circle,
  anchor/.initial=center,
  shape start width/.initial=2.5pt,
  shape start height/.initial=2.5pt,
  shape end width/.initial=2.5pt,
  shape end height/.initial=2.5pt,
  shape sep/.store in=\pgf@lib@shapedecoration@sep,
  shape sloped/.is if=pgfshapedecorationsloped,
  shape scaled/.is if=pgfshapedecorationscaled,
  shape evenly spread/.store in=\pgf@lib@shapedecoration@spread,
  shape start size/.style={%
    shape start width=#1,
    shape start height=#1%
  },%
  shape end size/.style={%
    shape end width=#1,
    shape end height=#1%
  },%
  shape size/.style={%
    shape start size=#1,
    shape end size=#1%
  },%
  shape width/.style={%
    shape start width=#1,
    shape end width=#1
  },
  shape height/.style={%
    shape start height=#1,
    shape end height=#1
  }
}

\def\pgf@lib@shapedecoration@sep{.25cm, between centers}
\newif\ifpgfshapedecorationsloped
\pgfshapedecorationslopedtrue
\newif\ifpgfshapedecorationscaled
\let\pgf@lib@shapedecoration@spread\pgfutil@empty%



% triangle decoration

\pgfdeclaredecoration{triangles}{init}
{
  \state{init}[width=+0pt,next state=triangle,persistent precomputation={
    \pgfmathparse{\pgfkeysvalueof{/pgf/decoration/shape start width}}
    \edef\pgf@lib@dec@ssw{\pgfmathresult pt}
    \pgfmathparse{\pgfkeysvalueof{/pgf/decoration/shape start height}/2}
    \edef\pgf@lib@dec@ssh{\pgfmathresult pt}
  }]{}  
  \state{triangle}[switch if less than=+\pgfdecorationsegmentlength to last,
                   width=+\pgfdecorationsegmentlength]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgf@lib@dec@ssh}}
    \pgfpathlineto{\pgfqpoint{\pgf@lib@dec@ssw}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgf@lib@dec@ssh}}
    \pgfpathclose
  }
  \state{last}[switch if less than=\pgf@lib@dec@ssw to skip,
               width=\pgfdecoratedremainingdistance,next state=final]
  {
    \pgfpathmoveto{\pgfqpoint{0pt}{\pgf@lib@dec@ssh}}
    \pgfpathlineto{\pgfqpoint{\pgf@lib@dec@ssw}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgf@lib@dec@ssh}}
    \pgfpathclose
  }
  \state{skip}[width=\pgfdecoratedremainingdistance]
  {}
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }
}




% crosses decoration

\pgfdeclaredecoration{crosses}{init}
{
  \state{init}[width=+0pt,next state=crosses,persistent precomputation={
    \pgfmathparse{\pgfkeysvalueof{/pgf/decoration/shape start width}/2}
    \edef\pgf@lib@dec@ssw{\pgfmathresult pt}
    \pgfmathparse{\pgfkeysvalueof{/pgf/decoration/shape start height}/2}
    \edef\pgf@lib@dec@ssh{\pgfmathresult pt}
  }]{}  
  \state{crosses}[switch if less than=+\pgfdecorationsegmentlength to last,
                  width=+\pgfdecorationsegmentlength]
  {
    \pgfpathmoveto{\pgfqpoint{-\pgf@lib@dec@ssw}{\pgf@lib@dec@ssh}}
    \pgfpathlineto{\pgfqpoint{\pgf@lib@dec@ssw}{-\pgf@lib@dec@ssh}}
    \pgfpathmoveto{\pgfqpoint{-\pgf@lib@dec@ssw}{-\pgf@lib@dec@ssh}}
    \pgfpathlineto{\pgfqpoint{\pgf@lib@dec@ssw}{\pgf@lib@dec@ssh}}
  }
  \state{last}[width=+\pgfdecoratedremainingdistance]
  {
    \pgfpathmoveto{\pgfqpoint{-\pgf@lib@dec@ssw}{\pgf@lib@dec@ssh}}
    \pgfpathlineto{\pgfqpoint{\pgf@lib@dec@ssw}{-\pgf@lib@dec@ssh}}
    \pgfpathmoveto{\pgfqpoint{-\pgf@lib@dec@ssw}{-\pgf@lib@dec@ssh}}
    \pgfpathlineto{\pgfqpoint{\pgf@lib@dec@ssw}{\pgf@lib@dec@ssh}}
  }
  \state{final}{
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }
}






% The shape background decoration
%	
% The shape background decoration adds repeated instances of 
% the background path of a specified shape along the path. The shape
% must have been declared  by \pgfdeclareshape. If a shape has
% specialized keys (e.g. the number of points on a star, or the apex
% angle the isosceles triangle), these can be specified in the usual manner. 
%	
% The sepatation between shapes in the path can be specified and can 
% be between the center of the shape or the border of the shape. 
%	
% The height and width of the shape can be independently or
% simultaneously scaled (linearly) along the path. It is also
% possible to prevent the shapes being sloped parallel to the
% path.

% internal if
\newif\ifpgf@lib@shapedecoration@betweenborders

\edef\pgf@lib@shapedecoration@initialise{0pt}%

\pgfdeclaredecoration{shape backgrounds}{initialise}
{
  \state{initialise}
  [
    width=+\pgf@lib@shapedecoration@initialise,
    next state=shape,
    persistent precomputation=
    {
      % 
      % \egroup ends the group started by the automaton before executing
      % a decoration state. This prevents the need for (most) \global variables. 
      % 
      % 
      % Check the shape exists.
      % 
      \pgfutil@ifundefined{pgf@sh@bg@\pgfkeysvalueof{/pgf/decoration/shape}}{%
        \PackageError{PGF}{I do not know the shape `\pgfkeysvalueof{/pgf/decoration/shape}',
          so I cannot use it in a decoration. Check if its library been loaded or if you 
          simply mistyped the name}{}}{}%
      % 
      % Calculate a `default' path size.
      % 
      \pgfinterruptpath%
        \pgfinterruptboundingbox%
          \pgftransformreset%
          \pgf@relevantforpicturesizetrue%
          % 
          % This size of this shape is unimportant, but it should
          % be just large/small enough to avoid huge errors when
          % calculting the scaling factors later on.
          % 
          \pgfkeys{/pgf/inner sep=50pt, /pgf/minimum size=1pt}% Arbitrary lengths.
          \setbox\pgfnodeparttextbox\hbox{}% Assume shape does nothing special if box is empty.
          \let\pgf@sh@savedmacros\pgfutil@empty% 
          \let\pgf@sh@savedpoints\pgfutil@empty%
          \csname pgf@sh@s@\pgfkeysvalueof{/pgf/decoration/shape}\endcsname%
          \pgf@sh@savedpoints%
          \pgf@sh@savedmacros%
          % 
          % Save the macros and pionts.
          % 
          \expandafter\gdef\expandafter\pgf@lib@shapedecoration@points\expandafter{\pgf@sh@savedpoints}%
          \expandafter\gdef\expandafter\pgf@lib@shapedecoration@macros\expandafter{\pgf@sh@savedmacros}%
          \csname pgf@sh@bg@\pgfkeysvalueof{/pgf/decoration/shape}\endcsname% 
          % 
          % Save the dimensions of the shape path.
          % 
          \pgf@x\pgf@picmaxx%
          \pgf@y\pgf@picmaxy%
          \advance\pgf@x-\pgf@picminx%
          \advance\pgf@y-\pgf@picminy%
          \xdef\pgf@lib@shapedecoration@shapepathsize{%
            \noexpand\pgf@x\the\pgf@x%
            \noexpand\pgf@y\the\pgf@y%
          }%
        \endpgfinterruptboundingbox%
      \endpgfinterruptpath%
      % 
      \edef\pgf@lib@shapedecoration@beforeshape{0pt}%
      \edef\pgf@lib@shapedecoration@aftershape{0pt}%
      % 
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/decoration/shape start width}}%
      \edef\pgf@lib@shapedecoration@startwidth{\the\pgf@x}%
      \edef\pgf@lib@shapedecoration@width{\the\pgf@x}%
      \pgf@x-\pgf@x%
      \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/decoration/shape end width}}%
      \edef\pgf@lib@shapedecoration@widthchange{\the\pgf@x}%
      % 
      \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/decoration/shape start height}}%
      \edef\pgf@lib@shapedecoration@initialheight{\the\pgf@y}%
      \edef\pgf@lib@shapedecoration@height{\the\pgf@y}%
      \pgf@y-\pgf@y%
      \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/decoration/shape end height}}%
      \edef\pgf@lib@shapedecoration@heightchange{\the\pgf@y}%		
      % 
      % Calculate the sep.
      % 
      \ifx\pgf@lib@shapedecoration@spread\pgfutil@empty%
        % 
        % Not spreading, so easy:
        % 
        \def\pgf@lib@shapedecoration@borderstext{between borders}%
        \afterassignment\pgf@lib@shapedecoration@setkeyword%
        \expandafter\pgf@x\pgf@lib@shapedecoration@sep,\pgf@stop%
        \edef\pgf@lib@shapedecoration@sep{\the\pgf@x}%
      \else%
        % 
        % Spreading (a bit of a nuiscence actually).
        % 
        \def\pgf@lib@shapedecoration@borderstext{by borders}%
        \afterassignment\pgf@lib@shapedecoration@setkeyword%
        \expandafter\c@pgf@counta\pgf@lib@shapedecoration@spread,\pgf@stop%
        \ifpgf@lib@shapedecoration@betweenborders%
          %  
          % Ok. The required sep between borders is:
          % 
          % (r -(n-1)((a+b)/2))/(n-1)
          % 
          % r = decoration length (here, the remaining distance)
          % a = initial width
          % b = end width
          % n = the number of shapes
          % 
          \ifnum\c@pgf@counta>1\relax%
            \advance\c@pgf@counta-1\relax%
            \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/decoration/shape start width}}%
            \ifpgfshapedecorationscaled%
              \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/decoration/shape end width}}%
            \else%
              \advance\pgf@x\pgf@x%
            \fi%
            \pgf@x.5\pgf@x% (a+b)/2
            \multiply\pgf@x-\c@pgf@counta% -(n-1)((a+b)/2)
            \advance\pgf@x\pgfdecoratedremainingdistance%
            \divide\pgf@x\c@pgf@counta%
            \pgf@x.9999\pgf@x% Hackery to control some native TeX inaccuracies.
            % 
            % Unfortunately if the shape is scaled, and evenly spread by borders,
            % it is necessary to do something a bit different to control for 
            % (most) inaccuracies.
            % 
            \ifpgfshapedecorationscaled%
              \pgf@xa\pgf@lib@shapedecoration@widthchange\relax%
              \divide\pgf@xa\c@pgf@counta%
              \edef\pgf@lib@shapedecoration@specialwidth{\the\pgf@xa}%		
            \fi%
          \else%
            \pgf@lib@shapedecoration@betweenbordersfalse%
            \pgf@x\pgfdecoratedremainingdistance%
            \ifnum\c@pgf@counta=1\relax%
              \pgf@y.5\pgf@x%
              \edef\pgf@lib@shapedecoration@initialise{\the\pgf@y}%
            \else%
              \advance\pgf@x5pt\relax% An arbitrary value >0pt.
              \edef\pgf@lib@shapedecoration@initialise{\the\pgf@x}%
            \fi%
          \fi%	
        \else%
          %  
          % Between centers.
          % 
          \pgf@x\pgfdecoratedremainingdistance%
          \ifnum\c@pgf@counta>1\relax%
            \advance\c@pgf@counta-1\relax%
            \divide\pgf@x\c@pgf@counta\relax%
          \else%
            \ifnum\c@pgf@counta=1\relax%
              \pgf@y.5\pgf@x%
              \edef\pgf@lib@shapedecoration@initialise{\the\pgf@y}%
            \else%
              \advance\pgf@x5pt\relax% An arbitrary value >0pt.
              \edef\pgf@lib@shapedecoration@initialise{\the\pgf@x}%
            \fi%
          \fi%
        \fi%
        \edef\pgf@lib@shapedecoration@sep{\the\pgf@x}%
      \fi%
    }]
  {}
  \state{before shape}
  [
    width=\pgf@lib@shapedecoration@beforeshape-1sp,
    next state=shape,
    persistent precomputation=
    {
      \ifpgfshapedecorationscaled%
        \ifpgf@lib@shapedecoration@betweenborders%
          \ifx\pgf@lib@shapedecoration@spread\pgfutil@empty%
            % 
            % Not so straightforward. The required ratio is given by
            % 
            % R = (c+W/2)/(c+r-.5*w)
            % 
            % c = completed distance
            % r = remaining distance
            % W = initial width
            % w = the change in width (i.e., end - start)
            % 
            \pgf@x\pgfdecoratedcompleteddistance%
            \advance\pgf@x\pgfdecoratedremainingdistance%
            \pgf@xa\pgf@lib@shapedecoration@startwidth\relax%
            \pgf@xa.5\pgf@xa%
            \advance\pgf@xa\pgfdecoratedcompleteddistance% c+W/2
            % 
            \pgf@xb\pgf@lib@shapedecoration@widthchange\relax%
            \pgf@xb-.5\pgf@xb%
            \advance\pgf@xb\pgf@x% c+r-.5*w
            % 
            \pgfmathdivide@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgf@xb}}%
          \fi%
        \else%
          % 
          % Easy peasy. The required ratio is 
          % 
          % R = c / (c+r)
          % 
          \pgf@y\pgfdecoratedcompleteddistance%
          \advance\pgf@y\pgfdecoratedremainingdistance%
          \pgfmathdivide@{\pgfmath@tonumber{\pgfdecoratedcompleteddistance}}{\pgfmath@tonumber{\pgf@y}}%			
        \fi%
        % 
        % Get the new width.
        % 
        \ifx\pgf@lib@shapedecoration@spread\pgfutil@empty%
          \pgf@x\pgf@lib@shapedecoration@widthchange\relax%
          \pgf@x\pgfmathresult\pgf@x%
          \advance\pgf@x\pgf@lib@shapedecoration@startwidth\relax%
        \else%
          \ifpgf@lib@shapedecoration@betweenborders%
            % 
            % Specical case when decoration is scaled, and evenly spread by borders.
            % 
            \pgf@x\pgf@lib@shapedecoration@width\relax%
            \advance\pgf@x\pgf@lib@shapedecoration@specialwidth\relax%
            \pgf@xa\pgf@x%
            \advance\pgf@xa-\pgf@lib@shapedecoration@startwidth\relax%
            \pgf@xb\pgf@lib@shapedecoration@widthchange\relax%
            \pgfmathdivide@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgf@xb}}%
          \else%
            \pgf@x\pgf@lib@shapedecoration@widthchange\relax%
            \pgf@x\pgfmathresult\pgf@x%
            \advance\pgf@x\pgf@lib@shapedecoration@startwidth\relax%
          \fi%
        \fi%		
        \edef\pgf@lib@shapedecoration@width{\the\pgf@x}%		
        % 
        % New height = R*h + H
        % 
        \pgf@y\pgf@lib@shapedecoration@heightchange\relax%
        \pgf@y\pgfmathresult\pgf@y%
        \advance\pgf@y\pgf@lib@shapedecoration@initialheight\relax%
        \edef\pgf@lib@shapedecoration@height{\the\pgf@y}%
      \fi%
      % 
      \ifpgf@lib@shapedecoration@betweenborders%
        \pgf@x\pgf@lib@shapedecoration@width\relax%
        \pgf@x.5\pgf@x%
        \edef\pgf@lib@shapedecoration@beforeshape{\the\pgf@x}%
      \else%
        \def\pgf@lib@shapedecoration@beforeshape{0pt}%
      \fi%	
    }]
  {}
  \state{shape}[width=+0sp,next state=after shape]
  {
    \ifpgfshapedecorationsloped%
    \else%
      \pgftransformrotate{-\pgfdecoratedangle}%
    \fi%
    % 
    % Scale the path when it is actually drawn.
    % 
    \pgf@lib@shapedecoration@shapepathsize%
    \pgfutil@tempdima\pgf@x%
    \pgfutil@tempdimb\pgf@y%
    \pgf@xa\pgf@lib@shapedecoration@width\relax%
    \pgf@xb\pgfutil@tempdima%
    \pgfmathdivide@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgf@xb}}%
    \expandafter\pgftransformxscale\expandafter{\pgfmathresult}%
    % 
    \pgf@ya\pgf@lib@shapedecoration@height\relax%
    \pgf@yb\pgfutil@tempdimb%
    \pgfmathdivide@{\pgfmath@tonumber{\pgf@ya}}{\pgfmath@tonumber{\pgf@yb}}%
    \expandafter\pgftransformyscale\expandafter{\pgfmathresult}%
    % 
    % Move to the center anchor.
    % 
    \pgf@lib@shapedecoration@points%
    \pgf@lib@shapedecoration@macros%
    \pgftransformshift{%
      \pgf@sh@reanchor{\pgfkeysvalueof{/pgf/decoration/shape}}{\pgfkeysvalueof{/pgf/decoration/anchor}}%
      \pgf@x-\pgf@x%
      \pgf@y-\pgf@y%
    }%
    % 
    % And draw the shape path.
    % 
    \csname pgf@sh@bg@\pgfkeysvalueof{/pgf/decoration/shape}\endcsname%	
  }
  \state{after shape}
  [
    width=\pgf@lib@shapedecoration@aftershape-1sp,
    next state=sep,
    persistent precomputation=
    {
      \ifpgf@lib@shapedecoration@betweenborders%
        \pgf@x\pgf@lib@shapedecoration@width\relax%
        \pgf@x.5\pgf@x%
        \edef\pgf@lib@shapedecoration@aftershape{\the\pgf@x}%
      \else%
        \edef\pgf@lib@shapedecoration@aftershape{0pt}%
      \fi%
    }
  ]
  {}
  \state{sep}[width=\pgf@lib@shapedecoration@sep,next state=before shape,
              persistent precomputation=\def\pgf@lib@shapedecoration@beforeshape{0pt}]
  {}
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}%
  }
}

\def\pgf@lib@shapedecoration@setkeyword,{%
  \pgfutil@ifnextchar\pgf@stop{\def\pgf@temp{}\pgf@lib@@@shapedecoration@setkeyword}{\pgf@lib@@shapedecoration@setkeyword}%
}
\def\pgf@lib@@shapedecoration@setkeyword#1,{\def\pgf@temp{#1}\pgf@lib@@@shapedecoration@setkeyword}
\def\pgf@lib@@@shapedecoration@setkeyword\pgf@stop{%
  \ifx\pgf@temp\pgf@lib@shapedecoration@borderstext%
    \pgf@lib@shapedecoration@betweenborderstrue%
  \else%
    \pgf@lib@shapedecoration@betweenbordersfalse%
  \fi%
}



\endinput

==> pgflibrarydecorations.text.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}


% Options for text decorations

\pgfkeys{
  /pgf/decoration/.cd,
  text/.store in=\pgfdecorationtext,%                                                 
  text color/.store in=\pgf@lib@decorationtextcolor,%
  text format delimiters/.code={\expandafter\pgfsetdecoratetextformatdelimiters#1}
}
\def\pgf@lib@decorationtextcolor{black}

% Decorates a path with a text. The path is removed during this
% process

\pgfdeclaredecoration{text along path}{initial}{
  \state{initial}[width=+0pt,
                  next state=scan,
                  persistent precomputation=\let\pgfdecorationrestoftext\pgfdecorationtext]
  {}
  \state{scan}[width=+0pt,
               next state=before typeset,
               persistent precomputation=
               {
                 \pgf@lib@decorations@text@scanchar%
                 \ifvoid\pgf@lib@decorations@text@box%
                   \setbox\pgf@lib@decorations@text@box\hbox{}%
                   \wd\pgf@lib@decorations@text@box16383pt\relax%
                 \fi%
               }]
  {}
  \state{before typeset}[width=+.5\wd\pgf@lib@decorations@text@box, next state=typeset]{}
  \state{typeset}[width=+0pt, next state=after typeset]
  {
    \pgftransformxshift{+-.5\wd\pgf@lib@decorations@text@box}%
    \setbox\pgf@hbox\hbox{\copy\pgf@lib@decorations@text@box}%
    \pgfqboxsynced\pgf@hbox%
  }
  \state{after typeset}[width=+.5\wd\pgf@lib@decorations@text@box, next state=scan]{}
  \state{final}{}
}


% \pgfsetdecoratetextformatdelimiters
% 
% Set the delimiters for formatting in the text decoration.
% NB: Catcodes for delimiters should be 11 or 12.
%
% Examples:
%
% \pgfsetdecoratetextformatdelimiters{|}{}% 2nd argument can be empty.
%
% \def\pgfdecoratetext{A big |\color{red}|red|| apple.}
%
% \pgfsetdecoratetextformatdelimiters{[}{]}
%
% \def\pgfdecoratetext{The [\it]very[+\color{green}]green[] sprouts.}
%
\def\pgfsetdecoratetextformatdelimiters#1#2{%
	\def\pgf@lib@decorations@text@formatchar{#1}%
	\def\pgf@test{#2}%
	\ifx\pgf@test\pgfutil@empty%
		\def\pgf@lib@decorations@text@collectformat##1#1{%
		\pgf@lib@decorations@text@@collectformat##1\pgf@stop}%
	\else%
		\def\pgf@lib@decorations@text@collectformat##1#2{%
			\pgf@lib@decorations@text@@collectformat##1\pgf@stop}%
	\fi%
}

\pgfsetdecoratetextformatdelimiters{|}{}

\newbox\pgf@lib@decorations@text@box
\newif\ifpgf@lib@decorate@textmathmode

\let\pgfdecorationtext\pgfutil@empty
\let\pgfdecorationrestoftext\pgfutil@empty%
\let\pgf@lib@decorations@text@format\pgfutil@empty

\def\pgf@lib@decorations@text@scanchar{%
	\ifx\pgfdecorationrestoftext\pgfutil@empty%
		\let\pgf@lib@decorations@text@char\pgfutil@empty%
		\setbox\pgf@lib@decorations@text@box\box\voidb@x%
		\let\pgf@next\relax%
	\else%
		\let\pgf@next\pgf@lib@decorations@text@@scanchar%
	\fi%
	\pgf@next}

\def\pgf@lib@decorations@text@@scanchar{%
	\expandafter\pgf@lib@decorations@text@@@scanchar\pgfdecorationrestoftext\pgf@stop}

\def\pgf@lib@decorations@text@@@scanchar{%
	\futurelet\pgf@lib@decorations@lettoken%
	\pgf@lib@decorations@text@@@@scanchar}
	
\def\pgf@lib@decorations@text@@@@scanchar{%
	\ifx\pgf@lib@decorations@lettoken\pgfutil@sptoken%
		\let\pgf@next\pgf@lib@decorations@text@insertspace%
	\else%
		\let\pgf@next\pgf@lib@decorations@text@@@@@scanchar%
	\fi%
	\pgf@next}

\def\pgf@lib@decorations@text@@@@@scanchar{%
	\pgfutil@ifnextchar\bgroup{\pgf@lib@decorations@text@collectgroup}%
		{\pgf@lib@decorations@text@@@@@@scanchar}}
		
\def\pgf@lib@decorations@text@collectgroup#1{%
	\def\pgf@lib@decorations@text@char{#1}%
	\pgf@lib@decorations@text@collectrestoftext}
	
\def\pgf@lib@decorations@text@@@@@@scanchar#1{%
	\ifx#1\pgf@stop%
		\pgf@lib@decorations@text@box\box\voidb@x%
		\let\pgf@next\pgf@lib@decorations@text@endoftext%
	\else%
		\def\pgf@lib@decorations@text@char{#1}%
		\ifx#1\space%
			\let\pgf@next\pgf@lib@decorations@text@collectrestoftext%
		\else%
			\ifx#1\ %
				\let\pgf@next\pgf@lib@decorations@text@collectrestoftext%
			\else%
				\ifx\pgf@lib@decorations@text@char\pgf@lib@decorations@text@formatchar%
					\let\pgf@next\pgf@lib@decorations@text@collectformat%
				\else%
					\expandafter\ifcat\noexpand#1\relax%
						\let\pgf@next\pgf@lib@decorations@text@expandcs%
					\else%
						\ifnum\catcode`#1=3\relax%
							\ifpgf@lib@decorate@textmathmode%
								\pgf@lib@decorate@textmathmodefalse%
							\else%
								\pgf@lib@decorate@textmathmodetrue%
							\fi%
							\let\pgf@next\pgf@lib@decorations@text@@@scanchar%
						\else%
							\let\pgf@next\pgf@lib@decorations@text@collectrestoftext%
						\fi%
					\fi%
				\fi%
			\fi%
		\fi%
	\fi%
	\pgf@next%
}

\def\pgf@lib@decorations@text@@collectformat{%
	\pgfutil@ifnextchar+{\pgf@lib@decorations@text@addtoformat}{\pgf@lib@decorations@text@setformat}}
	
\def\pgf@lib@decorations@text@setformat#1\pgf@stop{%
	\def\pgf@lib@decorations@text@format{#1}%
	\pgf@lib@decorations@text@@@scanchar%
}

\def\pgf@lib@decorations@text@addtoformat+#1\pgf@stop{%
	\expandafter\def\expandafter\pgf@lib@decorations@text@format\expandafter{\pgf@lib@decorations@text@format#1}%
	\pgf@lib@decorations@text@@@scanchar%
}

\def\pgf@lib@decorations@text@insertspace{%
	\pgfutil@ifnextchar\bgroup{\pgf@lib@decorations@text@@insertspacegrp}%
		{\pgf@lib@decorations@text@@insertspace}}
		
\def\pgf@lib@decorations@text@@insertspacegrp#1{%
	\pgf@lib@decorations@text@@@@@@scanchar\space{#1}}
	
\def\pgf@lib@decorations@text@@insertspace#1{%
	\pgf@lib@decorations@text@@@@@@scanchar\space#1}
	
\def\pgf@lib@decorations@text@expandcs{%
	\expandafter\expandafter\expandafter\pgf@lib@decorations@text@@@@@scanchar%
		\pgf@lib@decorations@text@char}

\def\pgf@lib@decorations@text@endoftext{%
	\let\pgfdecoraterestoftext\pgfutil@empty%
	\let\pgf@lib@decorations@text@char\pgfutil@empty%
}
\def\pgf@lib@decorations@text@collectrestoftext{%
	\pgf@lib@decorations@text@dobox%
	\futurelet\pgf@lib@decorations@text@lettoken%
	\pgf@lib@decorations@text@@collectrestoftext}

\def\pgf@lib@decorations@text@@collectrestoftext{%
	\ifx\bgroup\pgf@lib@decorations@text@lettoken%
		\let\pgf@next\pgf@lib@decorations@text@@@collectrestoftextgrp%
	\else%
		\let\pgf@next\pgf@lib@decorations@text@@@collectrestoftext%
	\fi%
	\pgf@next}
	
\def\pgf@lib@decorations@text@@@collectrestoftextgrp#1#2\pgf@stop{\def\pgfdecorationrestoftext{{#1}#2}%
}

\def\pgf@lib@decorations@text@@@collectrestoftext#1\pgf@stop{\def\pgfdecorationrestoftext{#1}}

{%
	\catcode`\$3 %
	\gdef\pgf@lib@decorations@mathshift{$}%
	\catcode`\$9 $% For editors with annoying syntax highlighting.
}%

\def\pgf@lib@decorations@text@dobox{%
	\setbox\pgf@lib@decorations@text@box\hbox{%
		\pgfinterruptpicture%
		\begingroup%
			\pgfsetcolor{\pgf@lib@decorationtextcolor}%
			\ifpgf@lib@decorate@textmathmode\pgf@lib@decorations@mathshift\fi%
				\pgf@lib@decorations@text@format\relax%
				\pgf@lib@decorations@text@char%
			\ifpgf@lib@decorate@textmathmode\pgf@lib@decorations@mathshift\fi%
		\endgroup%
		\endpgfinterruptpicture%
	}%
}






\endinput

==> pgflibraryfadings.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryfadings.code.tex,v 1.3 2008/02/07 19:25:41 tantau Exp $


% Axial fadings

\pgfdeclarehorizontalshading{pgf@lib@fade@east}{100bp}
{color(0bp)=(pgftransparent!0); color(25bp)=(pgftransparent!0);
 color(75bp)=(pgftransparent!100); color(100bp)=(pgftransparent!100)}

\pgfdeclarehorizontalshading{pgf@lib@fade@west}{100bp}
{color(0bp)=(pgftransparent!100); color(25bp)=(pgftransparent!100);
 color(75bp)=(pgftransparent!0); color(100bp)=(pgftransparent!0)}

\pgfdeclareverticalshading{pgf@lib@fade@north}{100bp}
{color(0bp)=(pgftransparent!0); color(25bp)=(pgftransparent!0);
 color(75bp)=(pgftransparent!100); color(100bp)=(pgftransparent!100)}

\pgfdeclareverticalshading{pgf@lib@fade@south}{100bp}
{color(0bp)=(pgftransparent!100); color(25bp)=(pgftransparent!100);
 color(75bp)=(pgftransparent!0); color(100bp)=(pgftransparent!0)}

\pgfdeclarefading{east}{\pgfuseshading{pgf@lib@fade@east}}
\pgfdeclarefading{west}{\pgfuseshading{pgf@lib@fade@west}}
\pgfdeclarefading{north}{\pgfuseshading{pgf@lib@fade@north}}
\pgfdeclarefading{south}{\pgfuseshading{pgf@lib@fade@south}}


% Circular fadings

\pgfdeclareradialshading{tikz@lib@fade@circle@10}{\pgfpointorigin}{
  color(0pt)=(pgftransparent!0); color(22.5bp)=(pgftransparent!0);
  color(25bp)=(pgftransparent!100); color(50bp)=(pgftransparent!100)}
\pgfdeclarefading{circle with fuzzy edge 10 percent}{\pgfuseshading{tikz@lib@fade@circle@10}}

\pgfdeclareradialshading{tikz@lib@fade@circle@15}{\pgfpointorigin}{
  color(0pt)=(pgftransparent!0); color(21.25bp)=(pgftransparent!0);
  color(25bp)=(pgftransparent!100); color(50bp)=(pgftransparent!100)}
\pgfdeclarefading{circle with fuzzy edge 15 percent}{\pgfuseshading{tikz@lib@fade@circle@15}}

\pgfdeclareradialshading{tikz@lib@fade@circle@20}{\pgfpointorigin}{
  color(0pt)=(pgftransparent!0); color(20bp)=(pgftransparent!0);
  color(25bp)=(pgftransparent!100); color(50bp)=(pgftransparent!100)}
\pgfdeclarefading{circle with fuzzy edge 20 percent}{\pgfuseshading{tikz@lib@fade@circle@20}}

\pgfdeclareradialshading{tikz@lib@fade@fuzzy@15}{\pgfpointorigin}{
  color(0pt)=(pgftransparent!100); color(21.25bp)=(pgftransparent!100); color(23.125bp)=(pgftransparent!0);
  color(25bp)=(pgftransparent!100); color(50bp)=(pgftransparent!100)}
\pgfdeclarefading{fuzzy ring 15 percent}{\pgfuseshading{tikz@lib@fade@fuzzy@15}}


==> pgflibrarypatterns.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarypatterns.code.tex,v 1.12 2008/01/15 10:27:34 tantau Exp $


% Lines in different directions

\pgfdeclarepatternformonly{horizontal lines}{\pgfpointorigin}{\pgfqpoint{100pt}{1pt}}{\pgfqpoint{100pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{0.5pt}}
  \pgfpathlineto{\pgfqpoint{100pt}{0.5pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{vertical lines}{\pgfpointorigin}{\pgfqpoint{1pt}{100pt}}{\pgfqpoint{3pt}{100pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfqpoint{0.5pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{0.5pt}{100pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{north east lines}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{3.1pt}{3.1pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{north west lines}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{3pt}}
  \pgfpathlineto{\pgfqpoint{3.1pt}{-0.1pt}}
  \pgfusepath{stroke}
}

% Crossed lines in different directions

\pgfdeclarepatternformonly{grid}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{0pt}{3.1pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{3.1pt}{0pt}}
  \pgfusepath{stroke}
}

\pgfdeclarepatternformonly{crosshatch}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{4pt}{4pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfsetlinewidth{0.4pt}
  \pgfpathmoveto{\pgfqpoint{3.1pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{0pt}{3.1pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{3.1pt}{3.1pt}}
  \pgfusepath{stroke}
}


% Dotted regions

\pgfdeclarepatternformonly{dots}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{1pt}{1pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{.5pt}
  \pgfusepath{fill}
}

\pgfdeclarepatternformonly{crosshatch dots}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{2.5pt}{2.5pt}}{\pgfqpoint{3pt}{3pt}}%
{
  \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{.5pt}
  \pgfpathcircle{\pgfqpoint{1.5pt}{1.5pt}}{.5pt}
  \pgfusepath{fill}
}




% Star shaped patterns

\pgfdeclarepatternformonly{fivepointed stars}{\pgfpointorigin}{\pgfqpoint{3mm}{3mm}}{\pgfqpoint{3mm}{3mm}}%
{
  \pgftransformshift{\pgfqpoint{1mm}{1mm}}
  \pgfpathmoveto{\pgfqpointpolar{18}{1mm}}
  \pgfpathlineto{\pgfqpointpolar{162}{1mm}}
  \pgfpathlineto{\pgfqpointpolar{306}{1mm}}
  \pgfpathlineto{\pgfqpointpolar{90}{1mm}}
  \pgfpathlineto{\pgfqpointpolar{234}{1mm}}
  \pgfpathclose%
  \pgfusepath{fill}
}

\pgfdeclarepatternformonly{sixpointed stars}{\pgfpointorigin}{\pgfqpoint{3mm}{3mm}}{\pgfqpoint{3mm}{3mm}}%
{
  \pgftransformshift{\pgfqpoint{1mm}{1mm}}
  \pgfpathmoveto{\pgfqpointpolar{30}{1mm}}
  \pgfpathlineto{\pgfqpointpolar{150}{1mm}}
  \pgfpathlineto{\pgfqpointpolar{270}{1mm}}
  \pgfpathclose%
  \pgfpathmoveto{\pgfqpointpolar{-30}{1mm}}
  \pgfpathlineto{\pgfqpointpolar{-270}{1mm}}
  \pgfpathlineto{\pgfqpointpolar{-150}{1mm}}
  \pgfpathclose%
  \pgfsetnonzerorule
  \pgfusepath{fill}
}



% Bricks

\pgfdeclarepatternformonly{bricks}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{5mm}{5mm}}{\pgfqpoint{4mm}{4mm}}%
{
  \pgfsetlinewidth{0.8pt}
  \pgfpathmoveto{\pgfqpoint{0mm}{1mm}}
  \pgfpathlineto{\pgfqpoint{4mm}{1mm}}
  \pgfpathmoveto{\pgfqpoint{0mm}{3mm}}
  \pgfpathlineto{\pgfqpoint{4mm}{3mm}}
  \pgfpathmoveto{\pgfqpoint{1mm}{0mm}}
  \pgfpathlineto{\pgfqpoint{1mm}{1mm}}
  \pgfpathmoveto{\pgfqpoint{3mm}{1mm}}
  \pgfpathlineto{\pgfqpoint{3mm}{3mm}}
  \pgfpathmoveto{\pgfqpoint{1mm}{3mm}}
  \pgfpathlineto{\pgfqpoint{1mm}{4mm}}
  \pgfusepath{stroke}
}


% Checkerboards

\pgfdeclarepatternformonly{checkerboard}{\pgfpointorigin}{\pgfqpoint{4mm}{4mm}}{\pgfqpoint{4mm}{4mm}}%
{
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{2mm}{2mm}}
  \pgfpathrectangle{\pgfqpoint{2mm}{2mm}}{\pgfqpoint{2mm}{2mm}}
  \pgfusepath{fill}
}



% Backgrounds

\pgfdeclarepatterninherentlycolored{checkerboard light gray}
{\pgfpointorigin}{\pgfqpoint{4mm}{4mm}}{\pgfqpoint{4mm}{4mm}}%
{
  \pgfsetfillcolor{black!10}
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{4.1mm}{4.1mm}}% make
                                % slightly larger to ensure that tiles
                                % are really solid
  \pgfusepath{fill}
  \pgfsetfillcolor{black!20}
  \pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{2mm}{2mm}}
  \pgfpathrectangle{\pgfqpoint{2mm}{2mm}}{\pgfqpoint{2mm}{2mm}}
  \pgfusepath{fill}
}

\pgfdeclarepatterninherentlycolored{horizontal lines light gray}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{
  \pgfsetfillcolor{black!10}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
  \pgfsetfillcolor{black!15}
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
}

\pgfdeclarepatterninherentlycolored{horizontal lines gray}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{
  \pgfsetfillcolor{black!30}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
  \pgfsetfillcolor{black!35}
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
}

\pgfdeclarepatterninherentlycolored{horizontal lines dark gray}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{
  \pgfsetfillcolor{black!90}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
  \pgfsetfillcolor{black!85}
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
}

\pgfdeclarepatterninherentlycolored{horizontal lines light blue}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{
  \pgfsetfillcolor{blue!10}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
  \pgfsetfillcolor{blue!15}
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
}

\pgfdeclarepatterninherentlycolored{horizontal lines dark blue}
{\pgfpointorigin}{\pgfpoint{100pt}{4pt}}
{\pgfpoint{100pt}{4pt}}
{
  \pgfsetfillcolor{blue!90}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
  \pgfsetfillcolor{blue!85}
  \pgfpathrectangle{\pgfpoint{0pt}{2pt}}{\pgfpoint{100pt}{2.5pt}}
  \pgfusepath{fill}
}


\pgfdeclarepatterninherentlycolored{crosshatch dots gray}
{\pgfpointorigin}{\pgfpoint{8pt}{8pt}}
{\pgfpoint{8pt}{8pt}}
{
  \pgfsetfillcolor{black!20}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{8pt}{8pt}}
  \pgfusepath{fill}
  \pgfsetfillcolor{black!10}
  \pgfpathcircle{\pgfpoint{2pt}{1.75pt}}{1pt}
  \pgfpathcircle{\pgfpoint{6pt}{5.75pt}}{1pt}
  \pgfusepath{fill}
  \pgfsetfillcolor{black!70}
  \pgfpathcircle{\pgfpoint{2pt}{2.25pt}}{1pt}
  \pgfpathcircle{\pgfpoint{6pt}{6.25pt}}{1pt}
  \pgfusepath{fill}
}

\pgfutil@definecolor{pgf@lightsteelblue}{rgb}{0.6875,0.765625,0.8671875}

\pgfdeclarepatterninherentlycolored{crosshatch dots light steel blue}
{\pgfpointorigin}{\pgfpoint{8pt}{8pt}}
{\pgfpoint{8pt}{8pt}}
{
  \pgfsetfillcolor{pgf@lightsteelblue}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{8pt}{8pt}}
  \pgfusepath{fill}
  \pgfsetfillcolor{black!80!pgf@lightsteelblue!10}
  \pgfpathcircle{\pgfpoint{2pt}{1.75pt}}{1pt}
  \pgfpathcircle{\pgfpoint{6pt}{5.75pt}}{1pt}
  \pgfusepath{fill}
  \pgfsetfillcolor{black!80!pgf@lightsteelblue!70}
  \pgfpathcircle{\pgfpoint{2pt}{2.25pt}}{1pt}
  \pgfpathcircle{\pgfpoint{6pt}{6.25pt}}{1pt}
  \pgfusepath{fill}
}




\endinput


==> pgflibraryplothandlers.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryplothandlers.code.tex,v 1.9 2007/03/09 17:49:32 tantau Exp $

\newif\ifpgf@plot@started


% This handler converts each plot stream command into a curveto
% command, except for the first, which is converted to the previously
% specified action.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfsetlinetofirstplotpoint
% \pgfplothandlercurveto
% \pgfplotxyfile{mytable}

\def\pgfplothandlercurveto{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@initial%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgf@plot@curveto@handler@finish%
    \global\pgf@plot@startedfalse%
  }%
}

\def\pgf@plot@curveto@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@plot@first@action{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \xdef\pgf@plot@curveto@first{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plot@curveto@first@support=\pgf@plot@curveto@first%
  \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@second%
}

\def\pgf@plot@curveto@handler@second#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@curveto@second{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@curveto@handler@third%
  \global\pgf@plot@startedtrue%
}

\def\pgf@plot@curveto@handler@third#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@curveto@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@curveto@first}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@curveto@second}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@curveto@first@support}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@curveto@second}}%
  {\pgf@marshal}%
  % Prepare next:
  \global\let\pgf@plot@curveto@first=\pgf@plot@curveto@second%
  \global\let\pgf@plot@curveto@second=\pgf@plot@curveto@current%
  \xdef\pgf@plot@curveto@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
}

\def\pgf@plot@curveto@handler@finish{%
  \ifpgf@plot@started%
    \pgfpathcurveto{\pgf@plot@curveto@first@support}{\pgf@plot@curveto@second}{\pgf@plot@curveto@second}%
  \fi%
}


% This commands sets the tension for smoothing of plots.
%
% #1 = tension of curves. A value of 1 will yield a circle when the
%      control points are at quarters of a circle. A smaller value
%      will result in a tighter curve. Default is 0.5. 
%
% Example:
%
% \pgfsetplottension{0.2}

\def\pgfsetplottension#1{%
  \pgf@x=#1pt\relax%
  \pgf@x=0.2775\pgf@x\relax%
  \edef\pgf@plottension{\pgf@sys@tonumber\pgf@x}}
\pgfsetplottension{0.5}


% This handler converts the plot stream command into a curveto
% command that is closed using a closepath.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
% \pgfplothandlerclosedcurve
% \pgfplotxyfile{mytable}

\def\pgfplothandlerclosedcurve{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@initial%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\pgf@plot@closedcurve@handler@finish%
  }%
}

\def\pgf@plot@closedcurve@handler@initial#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \xdef\pgf@plot@closedcurve@initial{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@second%
  \global\pgf@plot@startedfalse%
}

\def\pgf@plot@closedcurve@handler@second#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@after@initial{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  {\pgfpathmoveto{}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@third%
}

\def\pgf@plot@closedcurve@handler@third#1{%
  \global\pgf@plot@startedtrue%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@closedcurve@initial}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@closedcurve@after@initial}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \global\let\pgf@plot@closedcurve@first=\pgf@plot@closedcurve@after@initial%
  \global\let\pgf@plot@closedcurve@second=\pgf@plot@closedcurve@current%
  \xdef\pgf@plot@closedcurve@after@initial@presupport{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
  \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
  \global\let\pgf@plotstreampoint=\pgf@plot@closedcurve@handler@fourth%
}

\def\pgf@plot@closedcurve@handler@fourth#1{%
  \pgf@process{#1}%
  \xdef\pgf@plot@closedcurve@current{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
  % compute difference vector:
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\pgf@plot@closedcurve@first}
  \advance\pgf@xa by-\pgf@x%
  \advance\pgf@ya by-\pgf@y%
  % compute support directions:
  \pgf@xa=\pgf@plottension\pgf@xa%
  \pgf@ya=\pgf@plottension\pgf@ya%
  % first marshal:
  \pgf@process{\pgf@plot@closedcurve@second}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \advance\pgf@xc by\pgf@xa%
  \advance\pgf@yc by\pgf@ya%
  \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
    {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@second}}%
  {\pgf@marshal}%
  % Prepare next:
  \global\let\pgf@plot@closedcurve@first=\pgf@plot@closedcurve@second%
  \global\let\pgf@plot@closedcurve@second=\pgf@plot@closedcurve@current%
  \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
}

\def\pgf@plot@closedcurve@handler@finish{%
  \ifpgf@plot@started
    %
    % first, draw line from 2nd last to last:
    %
    \pgf@process{\pgf@plot@closedcurve@initial}%
    % compute difference vector:
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgf@plot@closedcurve@first}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    % compute support directions:
    \pgf@xa=\pgf@plottension\pgf@xa%
    \pgf@ya=\pgf@plottension\pgf@ya%
    % first marshal:
    \pgf@process{\pgf@plot@closedcurve@second}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xb by-\pgf@xa%
    \advance\pgf@yb by-\pgf@ya%
    \advance\pgf@xc by\pgf@xa%
    \advance\pgf@yc by\pgf@ya%
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@second}}%
    {\pgf@marshal}%
    \xdef\pgf@plot@closedcurve@first@support{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    %
    % second, draw line from last point to start:
    %
    \pgf@process{\pgf@plot@closedcurve@after@initial}%
    % compute difference vector:
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgf@plot@closedcurve@second}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    % compute support directions:
    \pgf@xa=\pgf@plottension\pgf@xa%
    \pgf@ya=\pgf@plottension\pgf@ya%
    % first marshal:
    \pgf@process{\pgf@plot@closedcurve@initial}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \advance\pgf@xb by-\pgf@xa%
    \advance\pgf@yb by-\pgf@ya%
    \advance\pgf@xc by\pgf@xa%
    \advance\pgf@yc by\pgf@ya%
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgf@plot@closedcurve@first@support}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}{\noexpand\pgf@plot@closedcurve@initial}}%
    {\pgf@marshal}%
    %
    % third, draw line from first to second point:
    %
    \edef\pgf@marshal{\noexpand\pgfpathcurveto{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      {\noexpand\pgf@plot@closedcurve@after@initial@presupport}{\noexpand\pgf@plot@closedcurve@after@initial}}%
    {\pgf@marshal}%
    \pgfpathclose%
  \fi%
}





% This handler converts each point in a stream into a line from the
% $y$-axis to the given points coordinate, resulting in a
% ``comb.'' 
%
% Example:
%
% \pgfplothandlerxcomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerxcomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@xcomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@xcomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgf@ya}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}


% This handler converts each point in a stream into a line from the
% $x$-axis straight up to the given points coordinate, resulting in a
% ``comb.'' 
%
% Example:
%
% \pgfplothandlerycomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerycomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@ycomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@ycomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{0pt}}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}






% This handler converts each point in a stream into a line from the
% origin to the point's coordinate, resulting in a ``star''.
%
% Example:
%
% \pgfplothandlerpolarcomb
% \pgfplotxyfile{mytable}

\def\pgfplothandlerpolarcomb{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@polarcomb@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@polarcomb@handler#1{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfpathmoveto{\pgfpointorigin}%
  \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
}




% This handler draws a given mark at each point. 
%
% #1 = some code to be executed at each point (with the coordinate
%      system translated to that point).
%      Typically, this code will be \pgfuseplotmark{whatever}.
%
% Example:
%
% \pgfplothandlermark{\pgfuseplotmark{*}}
% \pgfplotxyfile{mytable}

\def\pgfplothandlermark#1{%
  \pgf@plothandlermark{%
    \ifnum\pgf@plot@mark@count<\pgf@plot@mark@repeat\relax%
    \else%
      \global\pgf@plot@mark@count=0\relax%
      #1%
    \fi%
    }%
}

\newcount\pgf@plot@mark@count
\def\pgf@plot@mark@phase{0}

\def\pgf@plothandlermark#1{%
  \def\pgf@plot@mark{#1}%
  \def\pgf@plotstreamstart{%
    \global\pgf@plot@mark@count=\pgf@plot@mark@repeat\relax%
    \global\advance\pgf@plot@mark@count by-\pgf@plot@mark@phase\relax%
    \global\let\pgf@plotstreampoint=\pgf@plot@mark@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@mark@handler#1{%
  \global\advance\pgf@plot@mark@count by1\relax%
  {\pgftransformshift{#1}\pgf@plot@mark}%
}


% Set the repeat count for marks. For example, if 3 is given as a
% value, only every third point will get a mark.
%
% #1 = repeat count
%
% Example:
%
% \pgfsetplotmarkrepeat{2}

\def\pgfsetplotmarkrepeat#1{\def\pgf@plot@mark@repeat{#1}}
\pgfsetplotmarkrepeat{1}


% Set the phase for marks. For example, if 3 is the repeat and 3 is 
% the phase, already the first point will be marked. 
%
% #1 = the index of the first point that should be marked.
%
% Example:
%
% \pgfsetplotmarkphase{3}

\def\pgfsetplotmarkphase#1{\def\pgf@plot@mark@phase{#1}}
\pgfsetplotmarkphase{1}



% This handler draws a given mark at those points whose number is
% given in the (pgffor-like) list.
%
% #1 = some code to be executed at each point (with the coordinate
%      system translated to that point).
%      Typically, this code will be \pgfuseplotmark{whatever}.
% #2 = list of positions like "1,2,4,...,9,10"
%
% Example:
%
% \pgfplothandlermarklisted{\pgfuseplotmark{*}}{1,2,4,...,9}
% \pgfplotxyfile{mytable}

\def\pgfplothandlermarklisted#1#2{%
  \let\pgf@plot@mark@list=\pgfutil@empty%
  \edef\pgf@marshal{\noexpand\foreach\noexpand\pgf@temp in{#2}}
  \pgf@marshal{\xdef\pgf@plot@mark@list{\pgf@plot@mark@list(\pgf@temp)}}%
  \pgf@plothandlermark{%
    \edef\pgf@marshal{\noexpand\pgfutil@in@{(\the\pgf@plot@mark@count)}{\pgf@plot@mark@list}}%
    \pgf@marshal%
    \ifpgfutil@in@#1\fi}%
}


% Define a new plot mark for use with \pgfplotmark.
%
% #1 = a plot mark mnemonic
% #2 = code for drawing the mark
%
% Example:
%
% \pgfdeclareplotmark{*}{\pgfpathcircle{\pgfpointorigin}{2pt}\pgfusepathqfill}

\def\pgfdeclareplotmark#1#2{\expandafter\def\csname pgf@plot@mark@#1\endcsname{#2}}


% Set the size of plot marks. For circles, this will be the radius,
% for other shapes it should be about half the width/height.
%
% Example:
%
% \pgfsetplotmarksize{1pt}

\def\pgfsetplotmarksize#1{\pgfmathsetlength\pgfplotmarksize{#1}}

\newdimen\pgfplotmarksize
\pgfplotmarksize=2pt


% Insert a plot mark's code at the origin.
%
% #1 = plot mark mnemonic
%
% Example:
%
% \pgfuseplotmark{*}

\def\pgfuseplotmark#1{\csname pgf@plot@mark@#1\endcsname}


% A stroke-filled circle mark

\pgfdeclareplotmark{*}
{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfusepathqfillstroke
}


% A plus-sign like mark

\pgfdeclareplotmark{+}
{%
  \pgfpathmoveto{\pgfqpoint{-\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{0pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfusepathqstroke
}


% An x-shaped mark

\pgfdeclareplotmark{x}
{%
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfusepathqstroke
}

% See pgflibraryplotmarks for more plot marks






\endinput


==> pgflibraryplotmarks.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryplotmarks.code.tex,v 1.5 2007/03/09 17:49:32 tantau Exp $


% A stroked circle mark

\pgfdeclareplotmark{o}
{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfusepathqstroke
}



% A six-pointed star mark

\pgfdeclareplotmark{asterisk}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpointpolar{30}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{210}{\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpointpolar{-30}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{-210}{\pgfplotmarksize}}
  \pgfusepathqstroke
}


% A five-pointed star mark

\pgfdeclareplotmark{star}
{%
  \pgfpathmoveto{\pgfpointorigin}\pgfpathlineto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathmoveto{\pgfpointorigin}\pgfpathlineto{\pgfqpointpolar{18}{\pgfplotmarksize}}
  \pgfpathmoveto{\pgfpointorigin}\pgfpathlineto{\pgfqpointpolar{-54}{\pgfplotmarksize}}
  \pgfpathmoveto{\pgfpointorigin}\pgfpathlineto{\pgfqpointpolar{234}{\pgfplotmarksize}}
  \pgfpathmoveto{\pgfpointorigin}\pgfpathlineto{\pgfqpointpolar{162}{\pgfplotmarksize}}
  \pgfusepathqstroke
}


% An \oplus mark

\pgfdeclareplotmark{oplus}
{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfpathmoveto{\pgfqpoint{-\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{0pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfusepathqstroke
}

\pgfdeclareplotmark{oplus*}
{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfpathmoveto{\pgfqpoint{-\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpoint{\pgfplotmarksize}{0pt}}
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfusepathqfillstroke
}


% An \otimes mark

\pgfdeclareplotmark{otimes}
{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfusepathqstroke
}

\pgfdeclareplotmark{otimes*}
{%
  \pgfpathcircle{\pgfpointorigin}{\pgfplotmarksize}
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathmoveto{\pgfqpoint{-.70710678\pgfplotmarksize}{.70710678\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.70710678\pgfplotmarksize}{-.70710678\pgfplotmarksize}}
  \pgfusepathqfillstroke
}


% A vertical bar mark

\pgfdeclareplotmark{|}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfusepathqstroke
}



% A horizontal bar mark

\pgfdeclareplotmark{-}
{%
  \pgfpathmoveto{\pgfqpoint{\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpoint{-\pgfplotmarksize}{0pt}}
  \pgfusepathqstroke
}


% A square stroked mark

\pgfdeclareplotmark{square}
{%
  \pgfpathrectangle{\pgfqpoint{-\pgfplotmarksize}{-\pgfplotmarksize}}{\pgfqpoint{2\pgfplotmarksize}{2\pgfplotmarksize}}%
  \pgfusepathqstroke
}

% A square stroked-filled mark

\pgfdeclareplotmark{square*}
{%
  \pgfpathrectangle{\pgfqpoint{-\pgfplotmarksize}{-\pgfplotmarksize}}{\pgfqpoint{2\pgfplotmarksize}{2\pgfplotmarksize}}%
  \pgfusepathqfillstroke
}


% A triangle mark

\pgfdeclareplotmark{triangle}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{-30}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{-150}{\pgfplotmarksize}}
  \pgfpathclose
  \pgfusepathqstroke
}


% A stroke-filled triangle mark

\pgfdeclareplotmark{triangle*}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{-30}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{-150}{\pgfplotmarksize}}
  \pgfpathclose
  \pgfusepathqfillstroke
}



% A diamond-shaped mark

\pgfdeclareplotmark{diamond}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.75\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{-.75\pgfplotmarksize}{0pt}}
  \pgfpathclose
  \pgfusepathqstroke
}


% A stroke-filled diamond-shaped mark

\pgfdeclareplotmark{diamond*}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{.75\pgfplotmarksize}{0pt}}
  \pgfpathlineto{\pgfqpoint{0pt}{-\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpoint{-.75\pgfplotmarksize}{0pt}}
  \pgfpathclose
  \pgfusepathqfillstroke
}



% A pentagon-shaped mark

\pgfdeclareplotmark{pentagon}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{18}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{-54}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{234}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{162}{\pgfplotmarksize}}
  \pgfpathclose
  \pgfusepathqstroke
}

% A stroke-filled pentagon-shaped mark

\pgfdeclareplotmark{pentagon*}
{%
  \pgfpathmoveto{\pgfqpoint{0pt}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{18}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{-54}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{234}{\pgfplotmarksize}}
  \pgfpathlineto{\pgfqpointpolar{162}{\pgfplotmarksize}}
  \pgfpathclose
  \pgfusepathqfillstroke
}

\endinput


==> pgflibraryshapes.arrows.code.tex <==
% Copyright 2007 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryshapes.arrows.code.tex,v 1.3 2007/11/10 09:16:33 vibrovski Exp $


% keys for shape single arrow
%
% /pgf/single arrow tip angle
% /pgf/single arrow head extend
% /pgf/single arrow head indent

\pgfkeys{/pgf/.cd,
	single arrow tip angle/.initial=90, 
	single arrow head extend/.initial=.25cm,
	single arrow head indent/.initial=0cm}

% Shape single arrow
%
%
\pgfdeclareshape{single arrow}{%
	\savedmacro\getsinglearrowpoints{%
		%
		% Get the outer sep.
		% 
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\edef\xoutersep{\the\pgf@x}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\edef\youtersep{\the\pgf@y}%
		%
		% Get the node dimensions.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@xa.5\wd\pgfnodeparttextbox%
		\advance\pgf@xa.5\pgflinewidth%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@ya.5\ht\pgfnodeparttextbox%
		\advance\pgf@ya.5\dp\pgfnodeparttextbox%
		\advance\pgf@ya.5\pgflinewidth%
		\ifpgfshapeborderusesincircle%
			\ifdim\pgf@xa<\pgf@ya%
				\pgf@xa\pgf@ya%
			\fi%			
			\pgf@xa1.41421\pgf@xa%
			\pgf@ya\pgf@xa%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			\ifdim\xoutersep>\youtersep\relax%
				\let\youtersep\xoutersep%
			\else%
				\let\xoutersep\youtersep%
			\fi%
		\else%
			%
			% Round the rotation.
			%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			\pgfmathmod@{\rotate}{360}%
			\afterassignment\pgfmath@gobbletilpgfmath@%
			\expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\ifnum\c@pgf@counta<0\relax%
				\advance\c@pgf@counta360\relax%
			\fi%
			\edef\rotate{\the\c@pgf@counta}%
			%
			% Calculate the width and height of the node
			% contents, according to any border rotation.
			%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@x\pgf@xa%
				\pgf@xa\pgf@ya%
				\pgf@ya\pgf@x%
				\let\pgfmathresult\xoutersep%
				\let\xoutersep\youtersep%
				\let\youtersep\pgfmathresult%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@x\pgf@xa%
					\pgf@xa\pgf@ya%
					\pgf@ya\pgf@x%
					\let\pgfmathresult\xoutersep%
					\let\xoutersep\youtersep%
					\let\youtersep\pgfmathresult%
				\fi%
			\fi%
		\fi%
		\addtosavedmacro\rotate%
		%
		% Get some useful trig stuff.
		%
		\pgfmathdivide{\pgfkeysvalueof{/pgf/single arrow tip angle}}{2}%
		\let\halftipangle\pgfmathresult%
		\pgfmathcosec@{\halftipangle}%
		\let\cosechalftipangle\pgfmathresult%
		\pgfmathcos@{\halftipangle}%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\pgfutil@tempdima\cosechalftipangle\pgfutil@tempdima%
		\edef\cothalftipangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgfmathreciprocal@{\pgfmathresult}%
		\let\sechalftipangle\pgfmathresult%
		\pgfmathsin@{\halftipangle}%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\pgfutil@tempdima\sechalftipangle\pgfutil@tempdima%
		\edef\tanhalftipangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
		%
		% Get the single arrow head extend, and adjust for minimum width.
		%
		\pgf@xb\pgf@ya%
		\pgf@xb\cothalftipangle\pgf@xb%
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/single arrow head extend}}%
		\pgf@yc\pgf@xc%
		\advance\pgf@xc\pgf@ya%
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@xc<.5\pgfutil@tempdimb%
			\pgfutil@tempdimb.5\pgfutil@tempdimb%
			\pgfmathdivide@{\pgfmath@tonumber{\pgfutil@tempdimb}}{\pgfmath@tonumber{\pgf@xc}}%
			\pgf@ya\pgfmathresult\pgf@ya%
			\pgf@xc\pgfmathresult\pgf@xc%
			\pgf@yc\pgfmathresult\pgf@yc%
			\pgf@xb\pgfmathresult\pgf@xb%
		\fi%
		%
		% Now calculate the height of the arrow and adjust for minimum height.
		%
		\advance\pgf@xc-\pgf@ya%
		\pgf@xc\cothalftipangle\pgf@xc%
		\pgf@xa2.0\pgf@xa%
		\advance\pgf@xa\pgf@xb%
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@xa<\pgfutil@tempdimb%
			\pgf@xa\pgfutil@tempdimb%
		\fi%
		\advance\pgf@xa-\pgf@xb%
		\pgf@xa.5\pgf@xa%		
		\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/single arrow head indent}}%
		%
		% Now:
		%
		% xa - .5 * width of the node minus xb.
		% ya - .5 * height of the node contents.
		% xb - distance from the end of the node contents to the arrow tip.
		% xc - distance from the end of the node contents to the back end of the arrow head.
		% yc - distance from the top of the node contents to the top end of the arrow head.
		%
		\pgfsavepgf@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		\pgfsavepgf@process\basepoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y0pt%
		}%
		\pgfsavepgf@process\midpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgfmathsetlength\pgf@y{+.5ex}%
		}%
		%
		% As the arrow is symmetrical it can be described by only four points:
		%
		\pgfsavepgf@process\arrowtip{%
			\pgf@x\pgf@xa%
			\advance\pgf@x\pgf@xb%
			\pgf@y0pt\relax%
		}%
		\pgfsavepgf@process\beforearrowtip{%
			\pgf@x\pgf@xa%
			\advance\pgf@x-\pgf@xc%
			\pgf@y\pgf@ya%
			\advance\pgf@y\pgf@yc%
		}%
		\pgfsavepgf@process\beforearrowhead{%
			\pgf@x\pgf@xa%
			\advance\pgf@x-\pgf@xc%
			\advance\pgf@x\pgfutil@tempdima%
			\pgf@y\pgf@ya%
		}%
		\pgfsavepgf@process\afterarrowtail{%
			\pgf@x-\pgf@xa%
			\pgf@y\pgf@ya%
		}%
		%
		% Calculate the anchor point at the arrow tip...
		%
		\pgfsavepgf@process\arrowtipanchor{%
			\pgfpointadd{\centerpoint}{\arrowtip}%
			\pgf@xa\xoutersep\relax%
			\advance\pgf@x\cosechalftipangle\pgf@xa%
		}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\edef\externalradius{\the\pgf@x}%
		\addtosavedmacro\externalradius%
		%
		% ...and the rest of the points.
		%
		\pgfmathanglebetweenlines{\beforearrowtip}{\beforearrowhead}{\beforearrowtip}{\arrowtip}%
		\pgf@xa\xoutersep\relax%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\pgfutil@tempdima.5\pgfutil@tempdima%
		\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgf@xa\pgfmathresult\pgf@xa%
		\pgfutil@tempdima-\pgfutil@tempdima%
		\advance\pgfutil@tempdima180pt\relax%
		\advance\pgfutil@tempdima-\halftipangle pt\relax%
		%
		\pgfsavepgf@process\beforearrowtipanchor{%
			\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgf@xa}%
			\pgf@xb\pgf@x%
			\pgf@yb\pgf@y%
			\pgf@process{\pgfpointadd{\centerpoint}{\beforearrowtip}}%
			\advance\pgf@x\pgf@xb%
			\advance\pgf@y\pgf@yb%
		}%
		\pgfmathanglebetweenpoints{\beforearrowhead}{\beforearrowtip}%
		\pgfutil@tempdima-\pgfmathresult pt\relax%
		\advance\pgfutil@tempdima180pt\relax%
		\pgfutil@tempdima.5\pgfutil@tempdima%
		\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgf@xa\xoutersep\relax%
		\pgf@xa\pgfmathresult\pgf@xa%
		\pgfutil@tempdima-\pgfutil@tempdima%
		\advance\pgfutil@tempdima180pt\relax%
		\pgfsavepgf@process\beforearrowheadanchor{%
			\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgf@xa}%
			\pgf@xb\pgf@x%
			\pgf@yb\pgf@y%
			\pgf@process{\pgfpointadd{\centerpoint}{\beforearrowhead}}%
			\advance\pgf@x\pgf@xb%
			\advance\pgf@y\pgf@yb%
		}%
		\pgfsavepgf@process\afterarrowtailanchor{%
			\pgfpointadd{\centerpoint}{\afterarrowtail}%
			\advance\pgf@x-\xoutersep\relax%
			\advance\pgf@y\youtersep\relax%
		}%
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\beforearrowtipanchor}%
		\let\center@angle@beforearrowtip\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\beforearrowheadanchor}%
		\let\center@angle@beforearrowhead\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\afterarrowtailanchor}%
		\let\center@angle@afterarrowtail\pgfmathresult%
		\addtosavedmacro\center@angle@beforearrowtip%
		\addtosavedmacro\center@angle@beforearrowhead%
		\addtosavedmacro\center@angle@afterarrowtail%
		%
		\pgfmathanglebetweenpoints{\midpoint}{\beforearrowtipanchor}%
		\let\mid@angle@beforearrowtip\pgfmathresult%
		\pgfmathanglebetweenpoints{\midpoint}{\beforearrowheadanchor}%
		\let\mid@angle@beforearrowhead\pgfmathresult%
		\pgfmathanglebetweenpoints{\midpoint}{\afterarrowtailanchor}%
		\let\mid@angle@afterarrowtail\pgfmathresult%
		\addtosavedmacro\mid@angle@beforearrowtip%
		\addtosavedmacro\mid@angle@beforearrowhead%
		\addtosavedmacro\mid@angle@afterarrowtail%
		%
		\pgfmathanglebetweenpoints{\basepoint}{\beforearrowtipanchor}%
		\let\base@angle@beforearrowtip\pgfmathresult%
		\pgfmathanglebetweenpoints{\basepoint}{\beforearrowheadanchor}%
		\let\base@angle@beforearrowhead\pgfmathresult%
		\pgfmathanglebetweenpoints{\basepoint}{\afterarrowtailanchor}%
		\let\base@angle@afterarrowtail\pgfmathresult%
		\addtosavedmacro\base@angle@beforearrowtip%
		\addtosavedmacro\base@angle@beforearrowhead%
		\addtosavedmacro\base@angle@afterarrowtail%
		%
		\addtosavedmacro\arrowtipanchor%
		\addtosavedmacro\beforearrowtipanchor%
		\addtosavedmacro\beforearrowheadanchor%
		\addtosavedmacro\afterarrowtailanchor%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}%
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\getsinglearrowpoints%
		\let\pgf@singlearrow@referencepoint\midpoint%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}	
	\anchor{mid west}{%
		\getsinglearrowpoints%
		\let\pgf@singlearrow@referencepoint\midpoint%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}	
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\getsinglearrowpoints%
		\let\pgf@singlearrow@referencepoint\basepoint%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}	
	\anchor{base west}{%
		\getsinglearrowpoints%
		\let\pgf@singlearrow@referencepoint\basepoint%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}	
	\anchor{north}{%
		\getsinglearrowpoints%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
	}
	\anchor{south}{%
		\getsinglearrowpoints%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
	}
	\anchor{east}{%
		\getsinglearrowpoints%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{west}{%
		\getsinglearrowpoints%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}
	\anchor{north east}{%
		\getsinglearrowpoints%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
	}
	\anchor{south east}{%
		\getsinglearrowpoints%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
	}
	\anchor{south west}{%
		\getsinglearrowpoints%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
	}
	\anchor{north west}{%
		\getsinglearrowpoints%
		\csname pgf@anchor@single arrow@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
	}
	\anchor{before head}{%
		\getsinglearrowpoints%
		\pgfmathrotatepointaround{\beforearrowheadanchor}{\centerpoint}{\rotate}%
	}%
	\anchor{before tip}{%
		\getsinglearrowpoints%
		\pgfmathrotatepointaround{\beforearrowtipanchor}{\centerpoint}{\rotate}%
	}%
	\anchor{tip}{%
		\getsinglearrowpoints%
		\pgfmathrotatepointaround{\arrowtipanchor}{\centerpoint}{\rotate}%
	}%
	\anchor{after tip}{%
		\getsinglearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
				\pgf@y-\pgf@y%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}
	\anchor{after head}{%
		\getsinglearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
				\pgf@y-\pgf@y%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}
	\anchor{before tail}{%
		\getsinglearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\afterarrowtailanchor}%
				\pgf@y-\pgf@y%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}
	\anchor{after tail}{%
		\getsinglearrowpoints%
		\pgfmathrotatepointaround{\afterarrowtailanchor}{\centerpoint}{\rotate}%
	}
	\anchor{tail}{%
		\getsinglearrowpoints%
		\pgfpointlineattime{0.5}{%
			\pgfmathrotatepointaround{\afterarrowtailanchor}{\centerpoint}{\rotate}%
		}%
		{%
			\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\afterarrowtailanchor}%
				\pgf@y-\pgf@y%
			}{\centerpoint}}%
			{\centerpoint}{\rotate}%
		}%	
	}%
	\backgroundpath{%
		{%
			\pgftransformshift{\centerpoint}%
			\pgftransformrotate{\rotate}%
			\pgfpathmoveto{\arrowtip}%
			\pgfpathlineto{\beforearrowtip}%
			\pgfpathlineto{\beforearrowhead}%
			\pgfpathlineto{\afterarrowtail}%
			\pgfpathlineto{\afterarrowtail\pgf@y-\pgf@y}%
			\pgfpathlineto{\beforearrowhead\pgf@y-\pgf@y}%
			\pgfpathlineto{\beforearrowtip\pgf@y-\pgf@y}%			
		}%
		\pgfpathclose%
	}%
	\anchorborder{%
		\pgfsavepgf@process\externalpoint{}%			
		\getsinglearrowpoints%
		\pgfutil@ifundefined{pgf@singlearrow@referencepoint}{\let\referencepoint\centerpoint}%
			{\let\referencepoint\pgf@singlearrow@referencepoint}%
		\pgfsavepgf@process\externalpoint{%
			\externalpoint%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\referencepoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya}% 
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\externalangle\pgfmathresult%
		\pgf@x\externalangle pt\relax%
		\ifx\referencepoint\midpoint%
			\pgf@xa\mid@angle@beforearrowtip pt\relax%
			\pgf@xb\mid@angle@beforearrowhead pt\relax%
			\pgf@xc\mid@angle@afterarrowtail pt\relax%
		\else%
			\ifx\referencepoint\basepoint%
				\pgf@xa\base@angle@beforearrowtip pt\relax%
				\pgf@xb\base@angle@beforearrowhead pt\relax%
				\pgf@xc\base@angle@afterarrowtail pt\relax%
			\else%
				\pgf@xa\center@angle@beforearrowtip pt\relax%
				\pgf@xb\center@angle@beforearrowhead pt\relax%
				\pgf@xc\center@angle@afterarrowtail pt\relax%
			\fi%
		\fi%
		\ifdim\pgf@x<\pgf@xa%
			\let\firstpoint\arrowtipanchor%
			\let\secondpoint\beforearrowtipanchor%
		\else%
			\ifdim\pgf@x<\pgf@xb%
				\ifdim\pgf@xb<\pgf@xa%
					\let\firstpoint\arrowtipanchor%
					\let\secondpoint\beforearrowtipanchor%
				\else%
					\let\firstpoint\beforearrowheadanchor%
					\let\secondpoint\beforearrowtipanchor%
				\fi%
			\else%
				\ifdim\pgf@x<\pgf@xc%
					\let\firstpoint\beforearrowheadanchor%
					\let\secondpoint\afterarrowtailanchor%
				\else%
					\pgf@xc-\pgf@xc%
					\advance\pgf@xc360pt\relax%
					\ifdim\pgf@x<\pgf@xc%
						\let\firstpoint\afterarrowtailanchor%
						\pgfsavepgf@process\secondpoint{%
							\pgfpointadd{%
								\pgfpointdiff{\centerpoint}{\afterarrowtailanchor}%
								\pgf@y-\pgf@y%
							}{\centerpoint}%
						}%
					\else%
						\pgf@xa-\pgf@xa%
						\advance\pgf@xa360pt\relax%
						\pgf@xb-\pgf@xb%
						\advance\pgf@xb360pt\relax%
						\ifdim\pgf@x<\pgf@xa%
							\ifdim\pgf@x<\pgf@xb%
								\pgfsavepgf@process\firstpoint{%
									\pgfpointadd{%
											\pgfpointdiff{\centerpoint}{\afterarrowtailanchor}%
											\pgf@y-\pgf@y%
									}{\centerpoint}%
								}%
								\pgfsavepgf@process\secondpoint{%
									\pgfpointadd{%
										\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
										\pgf@y-\pgf@y%
									}{\centerpoint}%
								}%
							\else%
								\ifdim\pgf@xb<\pgf@xa%
									\pgfsavepgf@process\firstpoint{%
										\pgfpointadd{%
												\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
												\pgf@y-\pgf@y%
										}{\centerpoint}%
									}%									
								\else%
									\pgfsavepgf@process\firstpoint{%
										\pgfpointadd{%
												\pgfpointdiff{\centerpoint}{\arrowtipanchor}%
												\pgf@y-\pgf@y%
										}{\centerpoint}%
									}%	
								\fi%
								\pgfsavepgf@process\secondpoint{%
										\pgfpointadd{%
											\pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
											\pgf@y-\pgf@y%
										}{\centerpoint}%
									}%
							\fi%
						\else%
							\pgfsavepgf@process\firstpoint{%
								\pgfpointadd{%
									\pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
									\pgf@y-\pgf@y%
								}{\centerpoint}%
							}%
							\let\secondpoint\arrowtipanchor%
						\fi%
					\fi%
				\fi%
			\fi%
		\fi%
		\pgfsavepgf@process\firstpoint{%
			\pgfmathrotatepointaround{\firstpoint}{\centerpoint}{\rotate}%
		}%
		\pgfsavepgf@process\secondpoint{%
			\pgfmathrotatepointaround{\secondpoint}{\centerpoint}{\rotate}%
		}%
		\pgfpointintersectionoflines{\referencepoint}{\externalpoint}%
			{\firstpoint}{\secondpoint}%			
	}%
}







% keys for shape double arrow
%
% /pgf/double arrow tip angle
% /pgf/double arrow head sep

\pgfkeys{/pgf/.cd,
	double arrow tip angle/.initial=90,
	double arrow head extend/.initial=.25cm,
	double arrow head indent/.initial=0cm}

% Shape double arrow
%
%
\pgfdeclareshape{double arrow}{%
	\savedmacro\getdoublearrowpoints{%
		%
		% Get the outer sep.
		% 
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\edef\xoutersep{\the\pgf@x}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\edef\youtersep{\the\pgf@y}%
		%
		% Get the node dimensions.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@xa.5\wd\pgfnodeparttextbox%
		\advance\pgf@xa.5\pgflinewidth%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@ya.5\ht\pgfnodeparttextbox%
		\advance\pgf@ya.5\dp\pgfnodeparttextbox%
		\advance\pgf@ya.5\pgflinewidth%
		\ifpgfshapeborderusesincircle%
			\ifdim\pgf@xa<\pgf@ya%
				\pgf@xa\pgf@ya%
			\fi%			
			\pgf@xa1.41421\pgf@xa%
			\pgf@ya\pgf@xa%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			\ifdim\xoutersep>\youtersep\relax%
				\let\youtersep\xoutersep%
			\else%
				\let\xoutersep\youtersep%
			\fi%
		\else%
			%
			% Round the rotation.
			%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}
			\pgfmathmod@{\rotate}{360}%
			\afterassignment\pgfmath@gobbletilpgfmath@%
			\expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\ifnum\c@pgf@counta<0\relax%
				\advance\c@pgf@counta360\relax%
			\fi%
			\edef\rotate{\the\c@pgf@counta}%
			%
			% Calculate the width and height of the node
			% contents, according to any border rotation.
			%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@x\pgf@xa%
				\pgf@xa\pgf@ya%
				\pgf@ya\pgf@x%
				\let\pgfmathresult\xoutersep%
				\let\xoutersep\youtersep%
				\let\youtersep\pgfmathresult%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@x\pgf@xa%
					\pgf@xa\pgf@ya%
					\pgf@ya\pgf@x%
					\let\pgfmathresult\xoutersep%
					\let\xoutersep\youtersep%
					\let\youtersep\pgfmathresult%
				\fi%
			\fi%
		\fi%
		\addtosavedmacro\rotate%
		%
		% Get some useful trig stuff.
		%
		\pgfmathdivide{\pgfkeysvalueof{/pgf/double arrow tip angle}}{2}%
		\let\halftipangle\pgfmathresult%
		\pgfmathcosec@{\halftipangle}%
		\let\cosechalftipangle\pgfmathresult%
		\pgfmathcos@{\halftipangle}%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\pgfutil@tempdima\cosechalftipangle\pgfutil@tempdima%
		\edef\cothalftipangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgfmathreciprocal@{\pgfmathresult}%
		\let\sechalftipangle\pgfmathresult%
		\pgfmathsin@{\halftipangle}%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\pgfutil@tempdima\sechalftipangle\pgfutil@tempdima%
		\edef\tanhalftipangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
		%
		% Get the double arrow head extend, and adjust for minimum width.
		%
		\pgf@xb\pgf@ya%
		\pgf@xb\cothalftipangle\pgf@xb%
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/double arrow head extend}}%
		\pgf@yc\pgf@xc%
		\advance\pgf@xc\pgf@ya%
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@xc<.5\pgfutil@tempdimb%
			\pgfutil@tempdimb.5\pgfutil@tempdimb%
			\pgfmathdivide@{\pgfmath@tonumber{\pgfutil@tempdimb}}{\pgfmath@tonumber{\pgf@xc}}%
			\pgf@ya\pgfmathresult\pgf@ya%
			\pgf@xc\pgfmathresult\pgf@xc%
			\pgf@yc\pgfmathresult\pgf@yc%
			\pgf@xb\pgfmathresult\pgf@xb%
		\fi%
		%
		% Now calculate the height of the arrow and adjust for minimum height.
		%
		\advance\pgf@xc-\pgf@ya%
		\pgf@xc\cothalftipangle\pgf@xc%
		\advance\pgf@xa\pgf@xb%
		\pgf@xa2.0\pgf@xa%
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@xa<\pgfutil@tempdimb%
			\pgf@xa\pgfutil@tempdimb%
		\fi%
		\pgf@xa.5\pgf@xa%	
		\advance\pgf@xa-\pgf@xb%
		\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/double arrow head indent}}%
		%
		% Now:
		%
		% xa - .5 * width of the node minus xb.
		% ya - .5 * height of the node contents.
		% xb - distance from the end of the node contents to the arrow tip.
		% xc - distance from the end of the node contents to the back end of the arrow head.
		% yc - distance from the top of the node contents to the top end of the arrow head.
		%
		\pgfsavepgf@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		\pgfsavepgf@process\basepoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y0pt%
		}%
		\pgfsavepgf@process\midpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgfmathsetlength\pgf@y{+.5ex}%
		}%
		%
		% As the arrow is symmetrical it can be described by only 3 points:
		%
		\pgfsavepgf@process\arrowtip{%
			\pgf@x\pgf@xa%
			\advance\pgf@x\pgf@xb%
			\pgf@y0pt\relax%
		}%
		\pgfsavepgf@process\beforearrowtip{%
			\pgf@x\pgf@xa%
			\advance\pgf@x-\pgf@xc%
			\pgf@y\pgf@ya%
			\advance\pgf@y\pgf@yc%
		}%
		\pgfsavepgf@process\beforearrowhead{%
			\pgf@x\pgf@xa%
			\advance\pgf@x-\pgf@xc%
			\advance\pgf@x\pgfutil@tempdima%
			\pgf@y\pgf@ya%
		}%
		%
		% Calculate the anchor point at the arrow tip.
		%
		\pgfsavepgf@process\arrowtipanchor{%
			\pgfpointadd{\centerpoint}{\arrowtip}%
			\pgf@xa\xoutersep\relax%
			\advance\pgf@x\cosechalftipangle\pgf@xa%
		}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\edef\externalradius{\the\pgf@x}%
		\addtosavedmacro\externalradius%
		%
		%
		\pgfmathanglebetweenlines{\beforearrowtip}{\beforearrowhead}{\beforearrowtip}{\arrowtip}%
		\pgf@xa\xoutersep\relax%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\pgfutil@tempdima.5\pgfutil@tempdima%
		\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgf@xa\pgfmathresult\pgf@xa%
		\pgfutil@tempdima-\pgfutil@tempdima%
		\advance\pgfutil@tempdima180pt\relax%
		\advance\pgfutil@tempdima-\halftipangle pt\relax%
		\pgfsavepgf@process\beforearrowtipanchor{%
			\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgf@xa}%
			\pgf@xb\pgf@x%
			\pgf@yb\pgf@y%
			\pgf@process{\pgfpointadd{\centerpoint}{\beforearrowtip}}%
			\advance\pgf@x\pgf@xb%
			\advance\pgf@y\pgf@yb%
		}%
		\pgfmathanglebetweenpoints{\beforearrowhead}{\beforearrowtip}%
		\pgfutil@tempdima-\pgfmathresult pt\relax%
		\advance\pgfutil@tempdima180pt\relax%
		\pgfutil@tempdima.5\pgfutil@tempdima%
		\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgf@xa\xoutersep\relax%
		\pgf@xa\pgfmathresult\pgf@xa%
		\pgfutil@tempdima-\pgfutil@tempdima%
		\advance\pgfutil@tempdima180pt\relax%
		\pgfsavepgf@process\beforearrowheadanchor{%
			\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgf@xa}%
			\pgf@xb\pgf@x%
			\pgf@yb\pgf@y%
			\pgf@process{\pgfpointadd{\centerpoint}{\beforearrowhead}}%
			\advance\pgf@x\pgf@xb%
			\advance\pgf@y\pgf@yb%
		}%
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\beforearrowtipanchor}%
		\let\center@angle@beforearrowtip\pgfmathresult%
		\addtosavedmacro\center@angle@beforearrowtip%
		%
		\pgfmathanglebetweenpoints{\midpoint}{\beforearrowtipanchor}%
		\let\mid@angle@beforearrowtip\pgfmathresult%
		\addtosavedmacro\mid@angle@beforearrowtip%
		%
		\pgfmathanglebetweenpoints{\basepoint}{\beforearrowtipanchor}%
		\let\base@angle@beforearrowtip\pgfmathresult%
		\addtosavedmacro\base@angle@beforearrowtip%
		%
		\addtosavedmacro\arrowtipanchor%
		\addtosavedmacro\beforearrowtipanchor%
		\addtosavedmacro\beforearrowheadanchor%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}%
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\getdoublearrowpoints%
		\let\pgf@singlearrow@referencepoint\midpoint%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}	
	\anchor{mid west}{%
		\getdoublearrowpoints%
		\let\pgf@singlearrow@referencepoint\midpoint%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}	
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\getdoublearrowpoints%
		\let\pgf@singlearrow@referencepoint\basepoint%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}	
	\anchor{base west}{%
		\getdoublearrowpoints%
		\let\pgf@singlearrow@referencepoint\basepoint%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}	
	\anchor{north}{%
		\getdoublearrowpoints%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
	}
	\anchor{south}{%
		\getdoublearrowpoints%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
	}
	\anchor{east}{%
		\getdoublearrowpoints%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{west}{%
		\getdoublearrowpoints%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}
	\anchor{north east}{%
		\getdoublearrowpoints%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
	}
	\anchor{south east}{%
		\getdoublearrowpoints%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
	}
	\anchor{south west}{%
		\getdoublearrowpoints%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
	}
	\anchor{north west}{%
		\getdoublearrowpoints%
		\csname pgf@anchor@double arrow@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
	}
	\anchor{before head 1}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{\beforearrowheadanchor}{\centerpoint}{\rotate}%
	}%
	\anchor{before tip 1}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{\beforearrowtipanchor}{\centerpoint}{\rotate}%
	}%
	\anchor{tip 1}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{\arrowtipanchor}{\centerpoint}{\rotate}%
	}%
	\anchor{after tip 1}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
				\pgf@y-\pgf@y%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}
	\anchor{after head 1}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
				\pgf@y-\pgf@y%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}
	\anchor{before head 2}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
				\pgf@x-\pgf@x%
				\pgf@y-\pgf@y%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}%
	\anchor{before tip 2}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
				\pgf@x-\pgf@x%
				\pgf@y-\pgf@y%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}%
	\anchor{tip 2}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\arrowtipanchor}%
				\pgf@x-\pgf@x%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}%
	\anchor{after tip 2}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
				\pgf@x-\pgf@x%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}
	\anchor{after head 2}{%
		\getdoublearrowpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
				\pgf@x-\pgf@x%
			}{\centerpoint}}%
		{\centerpoint}{\rotate}%
	}
	\backgroundpath{%
		{%
			\pgftransformshift{\centerpoint}%
			\pgftransformrotate{\rotate}%
			\pgfpathmoveto{\arrowtip}%
			\pgfpathlineto{\beforearrowtip}%
			\pgfpathlineto{\beforearrowhead}%
			\pgfpathlineto{\beforearrowhead\pgf@x-\pgf@x}%
			\pgfpathlineto{\beforearrowtip\pgf@x-\pgf@x}%
			\pgfpathlineto{\arrowtip\pgf@x-\pgf@x}%
			\pgfpathlineto{\beforearrowtip\pgf@x-\pgf@x\pgf@y-\pgf@y}%
			\pgfpathlineto{\beforearrowhead\pgf@x-\pgf@x\pgf@y-\pgf@y}%
			\pgfpathlineto{\beforearrowhead\pgf@y-\pgf@y}%
			\pgfpathlineto{\beforearrowtip\pgf@y-\pgf@y}%			
		}%
		\pgfpathclose%
	}%
	\anchorborder{%
		\pgfsavepgf@process\externalpoint{}%			
		\getdoublearrowpoints%
		\pgfutil@ifundefined{pgf@singlearrow@referencepoint}{\let\referencepoint\centerpoint}%
			{\let\referencepoint\pgf@singlearrow@referencepoint}%
		\pgfsavepgf@process\externalpoint{%
			\externalpoint%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\referencepoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya}% 
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\externalangle\pgfmathresult%
		\pgf@x\externalangle pt\relax%
		\ifx\referencepoint\midpoint%
			\pgf@xa\mid@angle@beforearrowtip pt\relax%
		\else%
			\ifx\referencepoint\basepoint%
				\pgf@xa\base@angle@beforearrowtip pt\relax%
			\else%
				\pgf@xa\center@angle@beforearrowtip pt\relax%
			\fi%
		\fi%
		\ifdim\pgf@x<180pt\relax%
			\ifdim\pgf@x<\pgf@xa%
				\let\firstpoint\arrowtipanchor%
				\let\secondpoint\beforearrowtipanchor%
			\else%
				\pgf@xa-\pgf@xa%
				\advance\pgf@xa180pt\relax%
				\ifdim\pgf@x<\pgf@xa%
					\let\firstpoint\beforearrowheadanchor%
					\pgfsavepgf@process\secondpoint{%
						\pgfpointadd{%
							\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
							\pgf@x-\pgf@x
							}{\centerpoint}}%
				\else%
					\pgfsavepgf@process\firstpoint{%
						\pgfpointadd{%
							\pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
							\pgf@x-\pgf@x
							}{\centerpoint}}%
					\pgfsavepgf@process\secondpoint{%
						\pgfpointadd{%
							\pgfpointdiff{\centerpoint}{\arrowtipanchor}%
							\pgf@x-\pgf@x%
							\pgf@y-\pgf@y%
						}{\centerpoint}}%
				\fi%
			\fi%
		\else%
			\pgf@xa-\pgf@xa%
			\advance\pgf@xa360pt\relax%
			\ifdim\pgf@x<\pgf@xa%
				\pgf@xa-\pgf@xa%
				\advance\pgf@xa540pt\relax%
				\ifdim\pgf@x<\pgf@xa%
					\pgfsavepgf@process\firstpoint{%
						\pgfpointadd{%
							\pgfpointdiff{\centerpoint}{\arrowtipanchor}%
							\pgf@x-\pgf@x%
						}{\centerpoint}}%
					\pgfsavepgf@process\secondpoint{%
						\pgfpointadd{%
							\pgfpointdiff{\centerpoint}{\beforearrowtipanchor}%
							\pgf@x-\pgf@x%
							\pgf@y-\pgf@y%
						}{\centerpoint}}%
				\else%
					\pgfsavepgf@process\firstpoint{%
						\pgfpointadd{%
							\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
							\pgf@x-\pgf@x%
							\pgf@y-\pgf@y%
						}{\centerpoint}}%
					\pgfsavepgf@process\secondpoint{%
						\pgfpointadd{%
							\pgfpointdiff{\centerpoint}{\beforearrowheadanchor}%
							\pgf@y-\pgf@y%
						}{\centerpoint}}%
				\fi%
			\else%
				\pgfsavepgf@process\firstpoint{%
						\pgfpointadd{%
							\pgfpointdiff{\beforearrowtipanchor}{\centerpoint}%
							\pgf@x-\pgf@x%
						}{\centerpoint}}%
				\let\secondpoint\arrowtipanchor%
			\fi%
		\fi%
		\pgfsavepgf@process\firstpoint{%
			\pgfmathrotatepointaround{\firstpoint}{\centerpoint}{\rotate}%
		}%
		\pgfsavepgf@process\secondpoint{%
			\pgfmathrotatepointaround{\secondpoint}{\centerpoint}{\rotate}%
		}%
		\pgfpointintersectionoflines{\referencepoint}{\externalpoint}%
			{\firstpoint}{\secondpoint}%			
	}%
}




%
% Internal macros for the arrow box/shape.
%
\def\pgf@lib@arrowbox@parsearrowlength#1#2#3{%
	\edef\pgf@lib@temp{#3}%
	\edef\pgf@lib@marshal{%
		\noexpand\pgfutil@in@{none}{\pgf@lib@temp}%
	}%
	\pgf@lib@marshal%
	\ifpgfutil@in@%
		#10pt\relax%
	\else%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter#1\pgf@lib@temp\relax\pgfmath@%
		%
		\edef\pgf@lib@marshal{%
			\noexpand\pgfutil@in@{from center}{\pgf@lib@temp}%
		}%
		\pgf@lib@marshal%
		\ifpgfutil@in@%
		\else%
			\ifdim#1>0pt\relax%
				\advance#1#2\relax%
			\fi%
		\fi%
	\fi}

\def\pgf@lib@arrowbox@parsearrows#1{%
	\pgfkeys{/pgf/.cd,%
		arrow box west arrow=0pt,
		arrow box east arrow=0pt,
		arrow box south arrow=0pt,
		arrow box north arrow=0pt
	}%
	\def\pgf@lib@arrowbox@extend{0pt}%
	\edef\pgf@lib@temp{#1}%
	\expandafter\pgf@lib@arrowbox@@parsearrows\pgf@lib@temp,\pgf@lib@arrowbox@parsearrows,}


\def\pgf@lib@arrowbox@@parsearrows#1,{%
	\ifx\pgf@lib@arrowbox@parsearrows#1%
		\let\pgflib@next\relax%
	\else%
		\pgfutil@in@:{#1}%
		\ifpgfutil@in@%
			\pgf@lib@arrowbox@getextend#1\pgf@lib%
		\else%
			\def\pgf@lib@arrowbox@direction{#1}%
		\fi%
		\edef\pgf@marshal{%
			\noexpand\pgfkeys{/pgf/arrow box  \pgf@lib@arrowbox@direction\space arrow=\pgf@lib@arrowbox@extend}%
		}%
		\pgf@marshal%
		\let\pgflib@next\pgf@lib@arrowbox@@@parsearrows%
	\fi%
	\pgflib@next%
}
\def\pgf@lib@arrowbox@@@parsearrows{%
	\pgfutil@ifnextchar x{\relax\pgf@lib@arrowbox@@parsearrows}{\relax\pgf@lib@arrowbox@@parsearrows}%
}

\def\pgf@lib@arrowbox@getextend#1:#2\pgf@lib{%
	\def\pgf@lib@arrowbox@direction{#1}%
	\def\pgf@lib@arrowbox@extend{#2}%
}%

%
% /pgf/arrow box north arrow  
% /pgf/arrow box south arrow  
% /pgf/arrow box west arrow   
% /pgf/arrow box east arrow   
% /pgf/arrow box arrows       
% /pgf/arrow box shaft width  
% /pgf/arrow box head extend   
% /pgf/arrow box head indent 
% /pgf/arrow box tip angle   
%
\pgfkeys{/pgf/.cd,
	arrow box west arrow/.initial=.5cm,
	arrow box east arrow/.initial=.5cm,
	arrow box south arrow/.initial=.5cm,
	arrow box north arrow/.initial=.5cm,
	arrow box shaft width/.initial=.125cm,
	arrow box head extend/.initial=.125cm,
	arrow box head indent/.initial=0cm,
	arrow box tip angle/.initial=90,
}	

%
% arrow box/Shape.
%
\pgfdeclareshape{arrow box}{%
	\saveddimen\shaftwidth{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/arrow box shaft width}}%
	}%
	%
	% Calculate far the arrows extend from the center of the node.
	%
	\savedmacro\arrowboxpoints{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@x<.5\pgf@xa%
			\pgf@x.5\pgf@xa%
		\fi%
		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@y<.5\pgf@ya%
			\pgf@y.5\pgf@ya%
		\fi%	
		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%	
		%
		\edef\halfboxwidth{\the\pgf@x}%
		\edef\halfboxheight{\the\pgf@y}%
		\pgfextract@process\arrowboxcorner{}%
		\addtosavedmacro\arrowboxcorner%
		%
		\pgf@lib@arrowbox@parsearrowlength\pgf@x{\halfboxwidth}%
			{\pgfkeysvalueof{/pgf/arrow box west arrow}}%
		\edef\westextend{\the\pgf@x}%
		\addtosavedmacro\westextend%
		%
		\pgf@lib@arrowbox@parsearrowlength\pgf@x{\halfboxwidth}%
			{\pgfkeysvalueof{/pgf/arrow box east arrow}}%
		\edef\eastextend{\the\pgf@x}%
		\addtosavedmacro\eastextend%
		%
		\pgf@lib@arrowbox@parsearrowlength\pgf@x{\halfboxheight}%
			{\pgfkeysvalueof{/pgf/arrow box north arrow}}%
		\edef\northextend{\the\pgf@x}%
		\addtosavedmacro\northextend%
		%
		\pgf@lib@arrowbox@parsearrowlength\pgf@x{\halfboxheight}%
			{\pgfkeysvalueof{/pgf/arrow box south arrow}}%
		\edef\southextend{\the\pgf@x}%
		\addtosavedmacro\southextend%
	}%
	\saveddimen\arrowheadextend{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/arrow box head extend}}%
	}%
	\saveddimen\arrowheadindent{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/arrow box head indent}}%
	}%
	%
	% Calculate the `miter' angle for the outer sep at the arrow tip.
	%
	\savedmacro\arrowtipmiterangle{%
		\pgfmathparse{\pgfkeysvalueof{/pgf/arrow box tip angle}}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\arrowtipmiterangle\pgfmathresult%
	}%
	%
	% Calculate the `miter' angle for the outer sep at the point just 
	% before the arrow tip. 
	% 
	\savedmacro\arrowheadangles{%
		%
		% Calculate the `miter' angle and its cosecant at the arrow tip...
		%
		\pgfmathparse{\pgfkeysvalueof{/pgf/arrow box tip angle}}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\arrowtipmiterangle\pgfmathresult%
		\addtosavedmacro\arrowtipmiterangle%
		\pgfmathcosec@{\arrowtipmiterangle}%
		\let\cosecarrowtipmiterangle\pgfmathresult%
		\addtosavedmacro\cosecarrowtipmiterangle%
		%
		% ...before the arrow head...
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/arrow box head extend}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/arrow box head indent}}%
		\ifdim\pgf@y=0pt\relax%
			\def\pgfmathresult{90}%
		\else%
			\ifdim\pgf@y<0pt\relax%
				\pgfmathdivide@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
				\pgfmathatan@{\pgfmathresult}%
				\pgfmathadd@{\pgfmathresult}{180}%
			\else%
				\pgfmathdivide@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
				\pgfmathatan@{\pgfmathresult}%
			\fi%			
		\fi%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\beforearrowheadmiterangle\pgfmathresult%
		\addtosavedmacro\beforearrowheadmiterangle%
		\pgfmathcosec@{\beforearrowheadmiterangle}%
		\let\cosecbeforearrowheadmiterangle\pgfmathresult%
		\addtosavedmacro\cosecbeforearrowheadmiterangle%
		%
		% ...and before the arrow tip.
		%
		\pgfutil@tempdima-\arrowtipmiterangle pt\relax%
		\advance\pgfutil@tempdima90pt\relax%
		\pgfutil@tempdimb\beforearrowheadmiterangle pt\relax%
		\pgfutil@tempdimb2.0\pgfutil@tempdimb%
		\advance\pgfutil@tempdimb-90pt\relax%
		\advance\pgfutil@tempdima\pgfutil@tempdimb%
		\divide\pgfutil@tempdima2\relax%	
		\edef\beforearrowtipmiterangle{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\addtosavedmacro\beforearrowtipmiterangle%
		\pgfmathcosec@{\beforearrowtipmiterangle}%
		\let\cosecbeforearrowtipmiterangle\pgfmathresult%
		\addtosavedmacro\cosecbeforearrowtipmiterangle%
	}
	\saveddimen\outerxsep{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
	}%
	\saveddimen\outerysep{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer ysep}}%
	}%
	%
	% Calculate the (path) point immediately prior to an arrow tip. 
	%
	\savedanchor\beforearrowtip{%
		\pgfmathparse{\pgfkeysvalueof{/pgf/arrow box tip angle}}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\pgfmathcot@{\pgfmathresult}%
		\let\cothalfangle\pgfmathresult%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/arrow box shaft width}}%
		\pgf@y.5\pgf@y%
		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/arrow box head extend}}%
		\pgf@y\pgf@y%	
		\pgf@x\cothalfangle\pgf@y%	
	}%
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt\relax%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\anchor{center}{\centerpoint}
	\anchor{mid}{\midpoint}
	\anchor{mid east}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\let\pgf@lib@shapes@arrowbox@referencepoint\midpoint%
			\csname pgf@anchor@arrow box@border\endcsname{\pgfqpoint{\eastextend}{0pt}};
		\else%
			\arrowboxcorner%
			\pgf@xa\pgf@x%
			\midpoint%
			\advance\pgf@x\pgf@xa%
		\fi%
	}
	\anchor{mid west}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\let\pgf@lib@shapes@arrowbox@referencepoint\midpoint%
			\csname pgf@anchor@arrow box@border\endcsname{\pgfqpoint{-\westextend}{0pt}};
		\else%
			\arrowboxcorner%
			\pgf@xa\pgf@x%
			\midpoint%
			\advance\pgf@x-\pgf@xa%
		\fi%
	}
	\anchor{base}{\basepoint}
	\anchor{base east}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\let\pgf@lib@shapes@arrowbox@referencepoint\basepoint%
			\csname pgf@anchor@arrow box@border\endcsname{\pgfqpoint{\eastextend}{0pt}};
		\else%
			\arrowboxcorner%
			\pgf@xa\pgf@x%
			\basepoint%
			\advance\pgf@x\pgf@xa%
		\fi%
	}
	\anchor{base west}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\let\pgf@lib@shapes@arrowbox@referencepoint\basepoint%
			\csname pgf@anchor@arrow box@border\endcsname{\pgfqpoint{-\westextend}{0pt}};
		\else%
			\arrowboxcorner%
			\pgf@xa\pgf@x%
			\basepoint%
			\advance\pgf@x-\pgf@xa%
		\fi%
	}
	\anchor{north}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\csname pgf@anchor@arrow box@north arrow tip\endcsname%
		\else%
			\pgfpointadd{\centerpoint}{\arrowboxcorner}%
			\pgf@ya\pgf@y%
			\centerpoint%
			\pgf@y\pgf@ya%
		\fi%
	}%
	\anchor{south}{%
		\arrowboxpoints%
		\ifdim\southextend>0pt\relax%
			\csname pgf@anchor@arrow box@south arrow tip\endcsname%
		\else%
			\pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@y-\pgf@y}%
			\pgf@ya\pgf@y%
			\centerpoint%
			\pgf@y\pgf@ya%
		\fi%
	}%
	\anchor{east}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\csname pgf@anchor@arrow box@east arrow tip\endcsname%
		\else%
			\pgfpointadd{\centerpoint}{\arrowboxcorner}%
			\pgf@xa\pgf@x%
			\centerpoint%
			\pgf@x\pgf@xa%
		\fi%
	}%
	\anchor{west}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\csname pgf@anchor@arrow box@west arrow tip\endcsname%
		\else%
			\pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@x-\pgf@x}%
			\pgf@xa\pgf@x%
			\centerpoint%
			\pgf@x\pgf@xa%
		\fi%
	}%
	\anchor{north east}{%
		\arrowboxpoints%
		\pgfpointadd{\centerpoint}{\arrowboxcorner}%
	}%
	\anchor{north west}{%
		\arrowboxpoints%
		\pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@x-\pgf@x}%
	}%
	\anchor{south west}{%
		\arrowboxpoints%
		\pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@x-\pgf@x\pgf@y-\pgf@y}%
	}%
	\anchor{south east}{%
		\arrowboxpoints%
		\pgfpointadd{\centerpoint}{\arrowboxcorner\pgf@y-\pgf@y}%
	}%
	\anchor{before east arrow}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\arrowboxcorner%
				\pgf@y\shaftwidth\relax%
				\pgf@y.5\pgf@y%
				\advance\pgf@y\outerysep\relax%
			}%
		\else%
			\csname pgf@anchor@arrow box@east\endcsname%
		\fi%
	}%
	\anchor{before east arrow head}{%
		\arrowboxpoints%	
		\ifdim\eastextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
					\pgfutil@tempdimb\outerxsep\relax%
					\pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\eastextend\relax%
					\advance\pgf@x\arrowheadindent\relax%
					\pgf@y\shaftwidth\relax%
					\pgf@y.5\pgf@y%
				}%
			}%
		\else%
			\csname pgf@anchor@arrow box@east\endcsname%
		\fi%			
	}
	\anchor{before east arrow tip}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\arrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima-\beforearrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
					\pgfutil@tempdimb\outerysep\relax%
					\pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\eastextend\relax%
				}%
			}%
		\else%
			\csname pgf@anchor@arrow box@east\endcsname%
		\fi%
	}
	\anchor{east arrow tip}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\centerpoint%
			\advance\pgf@x\eastextend\relax%
			\pgf@xa\outerxsep\relax%
			\pgfmathcosec@{\arrowtipmiterangle}%
			\advance\pgf@x\pgfmathresult\pgf@xa%
		\else%
			\csname pgf@anchor@arrow box@east\endcsname%
		\fi%	
	}
	\anchor{after east arrow tip}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\arrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima-\beforearrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
					\pgfutil@tempdimb\outerysep\relax%
					\pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\eastextend\relax%
				}%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@east\endcsname%
		\fi%
	}
	\anchor{after east arrow head}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
					\pgfutil@tempdimb\outerxsep\relax%
					\pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\eastextend\relax%
					\advance\pgf@x\arrowheadindent\relax%
					\pgf@y\shaftwidth\relax%
					\pgf@y.5\pgf@y%
				}%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@east\endcsname%
		\fi%
	}
	\anchor{after east arrow}{%
		\arrowboxpoints%
		\ifdim\eastextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\arrowboxcorner%
				\pgf@y\shaftwidth\relax%
				\pgf@y.5\pgf@y%
				\advance\pgf@y\outerysep\relax%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@east\endcsname%
		\fi%
	}%
	%
	\anchor{before west arrow}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\arrowboxcorner%
				\pgf@x-\pgf@x%
				\pgf@y\shaftwidth\relax%
				\pgf@y.5\pgf@y%
				\advance\pgf@y\outerysep\relax%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@west\endcsname%
		\fi%
	}%
	\anchor{before west arrow head}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
					\pgfutil@tempdimb\outerxsep\relax%
					\pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\westextend\relax%
					\advance\pgf@x\arrowheadindent\relax%
					\pgf@y\shaftwidth\relax%
					\pgf@y.5\pgf@y%
				}%
				\pgf@x-\pgf@x%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@west\endcsname%
		\fi%			
	}
	\anchor{before west arrow tip}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\arrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima-\beforearrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
					\pgfutil@tempdimb\outerysep\relax%
					\pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\westextend\relax%
				}%
				\pgf@x-\pgf@x%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@west\endcsname%
		\fi%
	}
	\anchor{west arrow tip}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\centerpoint%
			\advance\pgf@x-\westextend\relax%
			\pgf@xa\outerxsep\relax%
			\pgfmathcosec@{\arrowtipmiterangle}%
			\advance\pgf@x-\pgfmathresult\pgf@xa%
		\else%
			\csname pgf@anchor@arrow box@west\endcsname%
		\fi%	
	}
	\anchor{after west arrow tip}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\arrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima-\beforearrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
					\pgfutil@tempdimb\outerysep\relax%
					\pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\westextend\relax%
				}%
				\pgf@x-\pgf@x%
			}%
		\else%
			\csname pgf@anchor@arrow box@west\endcsname%
		\fi%
	}
	\anchor{after west arrow head}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
					\pgfutil@tempdimb\outerxsep\relax%
					\pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\westextend\relax%
					\advance\pgf@x\arrowheadindent\relax%
					\pgf@y\shaftwidth\relax%
					\pgf@y.5\pgf@y%
				}%
				\pgf@x-\pgf@x%
			}%
		\else%
			\csname pgf@anchor@arrow box@west\endcsname%
		\fi%
	}
	\anchor{after west arrow}{%
		\arrowboxpoints%
		\ifdim\westextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\arrowboxcorner%
				\pgf@y\shaftwidth\relax%
				\pgf@y.5\pgf@y%
				\advance\pgf@y\outerysep\relax%
				\pgf@x-\pgf@x%
			}%
		\else%
			\csname pgf@anchor@arrow box@west\endcsname%
		\fi%
	}%
	%
	\anchor{before north arrow}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\arrowboxcorner%
				\pgf@x-\shaftwidth\relax%
				\pgf@x.5\pgf@x%
				\advance\pgf@x-\outerxsep\relax%
			}%
		\else%
			\csname pgf@anchor@arrow box@north\endcsname%
		\fi%
	}
	\anchor{before north arrow head}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
					\advance\pgfutil@tempdima270pt\relax%
					\pgfutil@tempdimb\outerysep\relax%
					\pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@y-\pgf@x%
					\advance\pgf@y\northextend\relax%
					\advance\pgf@y\arrowheadindent\relax%
					\pgf@x-\shaftwidth\relax%
					\pgf@x.5\pgf@x%
				}%
			}%
		\else%
			\csname pgf@anchor@arrow box@north\endcsname%
		\fi%			
	}
	\anchor{before north arrow tip}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima\arrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima\beforearrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima-90pt\relax%
					\pgfutil@tempdimb\outerxsep\relax%
					\pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@xa\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y-\pgf@xa%
					\advance\pgf@y\northextend\relax%
				}%
				\pgf@x-\pgf@x%
			}%
		\else%
			\csname pgf@anchor@arrow box@north\endcsname%
		\fi%
	}
	\anchor{north arrow tip}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\centerpoint%
			\advance\pgf@y\northextend\relax%
			\pgf@ya\outerysep\relax%
			\pgfmathcosec@{\arrowtipmiterangle}%
			\advance\pgf@y\pgfmathresult\pgf@ya%
		\else%
			\csname pgf@anchor@arrow box@north\endcsname%
		\fi%	
	}
	\anchor{after north arrow tip}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima\arrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima\beforearrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima-90pt\relax%
					\pgfutil@tempdimb\outerxsep\relax%
					\pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@xa\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y-\pgf@xa%
					\advance\pgf@y\northextend\relax%
				}%
			}%
		\else%
			\csname pgf@anchor@arrow box@north\endcsname%
		\fi%
		}
	\anchor{after north arrow head}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
					\advance\pgfutil@tempdima270pt\relax%
					\pgfutil@tempdimb\outerysep\relax%
					\pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@y-\pgf@x%
					\advance\pgf@y\northextend\relax%
					\advance\pgf@y\arrowheadindent\relax%
					\pgf@x-\shaftwidth\relax%
					\pgf@x.5\pgf@x%
				}%
				\pgf@x-\pgf@x%
			}%
		\else%
			\csname pgf@anchor@arrow box@north\endcsname%
		\fi%	
		}
	\anchor{after north arrow}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\arrowboxcorner%
				\pgf@x\shaftwidth\relax%
				\pgf@x.5\pgf@x%
				\advance\pgf@x\outerxsep\relax%
			}%
		\else%
			\csname pgf@anchor@arrow box@north\endcsname%
		\fi%
	}
	%
	\anchor{before south arrow}{%
		\arrowboxpoints%
		\ifdim\southextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\arrowboxcorner%
				\pgf@x\shaftwidth\relax%
				\pgf@x.5\pgf@x%
				\advance\pgf@x\outerxsep\relax%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@south\endcsname%
		\fi%
	}%
	\anchor{before south arrow head}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
					\advance\pgfutil@tempdima270pt\relax%
					\pgfutil@tempdimb\outerysep\relax%
					\pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@y-\pgf@x%
					\advance\pgf@y\northextend\relax%
					\advance\pgf@y\arrowheadindent\relax%
					\pgf@x-\shaftwidth\relax%
					\pgf@x.5\pgf@x%
				}%
				\pgf@x-\pgf@x%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@south\endcsname%
		\fi%	
		}
	\anchor{before south arrow tip}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima\arrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima\beforearrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima-90pt\relax%
					\pgfutil@tempdimb\outerxsep\relax%
					\pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@xa\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y-\pgf@xa%
					\advance\pgf@y\northextend\relax%
				}%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@south\endcsname%
		\fi%
		}
	\anchor{south arrow tip}{%
		\arrowboxpoints%
		\ifdim\southextend>0pt\relax%
			\centerpoint%
			\advance\pgf@y-\southextend\relax%
			\pgf@ya\outerysep\relax%
			\pgfmathcosec@{\arrowtipmiterangle}%
			\advance\pgf@y-\pgfmathresult\pgf@ya%
		\else%
			\csname pgf@anchor@arrow box@east\endcsname%
		\fi%	
	}
	\anchor{after south arrow tip}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima\arrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima\beforearrowtipmiterangle pt\relax%
					\advance\pgfutil@tempdima-90pt\relax%
					\pgfutil@tempdimb\outerxsep\relax%
					\pgfutil@tempdimb\cosecbeforearrowtipmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@xa\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y-\pgf@xa%
					\advance\pgf@y\northextend\relax%
				}%
				\pgf@x-\pgf@x%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@south\endcsname%
		\fi%
		}
	\anchor{after south arrow head}{%
		\arrowboxpoints%
		\ifdim\northextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\pgfpointadd{%
					\arrowheadangles%
					\pgfutil@tempdima-\beforearrowheadmiterangle pt\relax%
					\advance\pgfutil@tempdima270pt\relax%
					\pgfutil@tempdimb\outerysep\relax%
					\pgfutil@tempdimb\cosecbeforearrowheadmiterangle\pgfutil@tempdimb%
					\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
				}%
				{%
					\beforearrowtip%
					\pgf@y-\pgf@x%
					\advance\pgf@y\northextend\relax%
					\advance\pgf@y\arrowheadindent\relax%
					\pgf@x-\shaftwidth\relax%
					\pgf@x.5\pgf@x%
				}%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@south\endcsname%
		\fi%	
		}
	\anchor{after south arrow}{%
		\arrowboxpoints%
		\ifdim\southextend>0pt\relax%
			\pgfpointadd{\centerpoint}{%
				\arrowboxcorner%
				\pgf@x-\shaftwidth\relax%
				\pgf@x.5\pgf@x%
				\advance\pgf@x-\outerxsep\relax%
				\pgf@y-\pgf@y%
			}%
		\else%
			\csname pgf@anchor@arrow box@south\endcsname%
		\fi%
	}%
	%
	\backgroundpath{%
		\arrowboxpoints%
		\pgfextract@process\arrowboxcorner{%
			\arrowboxcorner%
			\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
			\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
		}%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\arrowboxcorner}%
			\ifdim\eastextend>0pt\relax%
				\pgfpathlineto{%
					\arrowboxcorner%
					\pgf@y\shaftwidth\relax%
					\pgf@y.5\pgf@y%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\eastextend\relax%
					\advance\pgf@x\arrowheadindent\relax%
					\pgf@y\shaftwidth\relax%
					\pgf@y.5\pgf@y%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\eastextend\relax%
				}%
				\pgfpathlineto{%
					\pgf@x\eastextend\relax%
					\pgf@y0pt\relax%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\eastextend\relax%
					\pgf@y-\pgf@y%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@x-\pgf@x%
					\advance\pgf@x\eastextend\relax%
					\advance\pgf@x\arrowheadindent\relax%
					\pgf@y\shaftwidth\relax%
					\pgf@y-.5\pgf@y%
				}%
				\pgfpathlineto{%
					\arrowboxcorner%
					\pgf@y\shaftwidth\relax%
					\pgf@y-.5\pgf@y%
				}%
			\fi%
			\pgfpathlineto{\arrowboxcorner\pgf@y-\pgf@y}%
			\ifdim\southextend>0pt\relax%
				\pgfpathlineto{%
					\arrowboxcorner%
					\pgf@x\shaftwidth\relax%
					\pgf@x.5\pgf@x%
					\pgf@y-\pgf@y%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@y\pgf@x%
					\advance\pgf@y-\southextend\relax%
					\advance\pgf@y-\arrowheadindent\relax%
					\pgf@x\shaftwidth\relax%
					\pgf@x.5\pgf@x%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@xa\pgf@y%
					\pgf@y\pgf@x%
					\advance\pgf@y-\southextend\relax%
					\pgf@x\pgf@xa%
				}%
				\pgfpathlineto{%
					\pgf@x0pt\relax%
					\pgf@y-\southextend\relax%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@xa\pgf@y%
					\pgf@y\pgf@x%
					\advance\pgf@y-\southextend\relax%
					\pgf@x-\pgf@xa%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@y\pgf@x%
					\advance\pgf@y-\southextend\relax%
					\advance\pgf@y-\arrowheadindent\relax%
					\pgf@x\shaftwidth\relax%
					\pgf@x-.5\pgf@x%
				}%
				\pgfpathlineto{%
					\arrowboxcorner%
					\pgf@x\shaftwidth\relax%
					\pgf@x-.5\pgf@x%
					\pgf@y-\pgf@y%
				}%
			\fi%
			\pgfpathlineto{\arrowboxcorner\pgf@x-\pgf@x\pgf@y-\pgf@y}%
			\ifdim\westextend>0pt\relax%
				\pgfpathlineto{%
					\arrowboxcorner%
					\pgf@x-\pgf@x
					\pgf@y\shaftwidth\relax%
					\pgf@y-.5\pgf@y%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\advance\pgf@x-\westextend\relax%
					\advance\pgf@x-\arrowheadindent\relax%
					\pgf@y\shaftwidth\relax%
					\pgf@y-.5\pgf@y%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\advance\pgf@x-\westextend\relax%
					\pgf@y-\pgf@y%
				}%
				\pgfpathlineto{%
					\pgf@x-\westextend\relax%
					\pgf@y0pt\relax%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\advance\pgf@x-\westextend\relax%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\advance\pgf@x-\westextend\relax%
					\advance\pgf@x-\arrowheadindent\relax%
					\pgf@y\shaftwidth\relax%
					\pgf@y.5\pgf@y%
				}%
				\pgfpathlineto{%
					\arrowboxcorner%
					\pgf@x-\pgf@x%
					\pgf@y\shaftwidth\relax%
					\pgf@y.5\pgf@y%
				}%
			\fi%
			\pgfpathlineto{\arrowboxcorner\pgf@x-\pgf@x}%
			\ifdim\northextend>0pt\relax%
				\pgfpathlineto{%
					\arrowboxcorner%
					\pgf@x\shaftwidth\relax%
					\pgf@x-.5\pgf@x%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@y-\pgf@x%
					\advance\pgf@y\northextend\relax%
					\advance\pgf@y\arrowheadindent\relax%
					\pgf@x\shaftwidth\relax%
					\pgf@x-.5\pgf@x%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@xa\pgf@y%
					\pgf@y-\pgf@x%
					\advance\pgf@y\northextend\relax%
					\pgf@x-\pgf@xa%
				}%
				\pgfpathlineto{%
					\pgf@x0pt\relax%
					\pgf@y\northextend\relax%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@xa\pgf@y%
					\pgf@y-\pgf@x%
					\advance\pgf@y\northextend\relax%
					\pgf@x\pgf@xa%
				}%
				\pgfpathlineto{%
					\beforearrowtip%
					\pgf@y-\pgf@x%
					\advance\pgf@y\northextend\relax%
					\advance\pgf@y\arrowheadindent\relax%
					\pgf@x\shaftwidth\relax%
					\pgf@x.5\pgf@x%
				}%				
				\pgfpathlineto{%
					\arrowboxcorner%
					\pgf@x\shaftwidth\relax%
					\pgf@x.5\pgf@x%
				}%
			\fi%
			\pgfpathclose%	
		}%
	}
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\pgfutil@ifundefined{pgf@lib@shapes@arrowbox@referencepoint}%
			{\let\referencepoint\centerpoint}{\let\referencepoint\pgf@lib@shapes@arrowbox@referencepoint}%
		\pgfextract@process\externalpoint{%
			\pgfpointadd{\referencepoint}{\externalpoint}%
		}%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\let\externalangle\pgfmathresult%
		\pgfmathanglebetweenpoints{\referencepoint}%
			{\csname pgf@anchor@arrow box@west\endcsname}%
		\ifdim\externalangle pt<\pgfmathresult pt\relax%
			\pgfmathanglebetweenpoints{\referencepoint}%
				{\csname pgf@anchor@arrow box@north\endcsname}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathanglebetweenpoints{\referencepoint}%
					{\csname pgf@anchor@arrow box@north east\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\pgfmathanglebetweenpoints{\referencepoint}%
						{\csname pgf@anchor@arrow box@before east arrow tip\endcsname}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax%
						\def\firstpoint{east arrow tip}%
						\def\secondpoint{before east arrow tip}%
					\else%
						\pgfmathanglebetweenpoints{\referencepoint}%
							{\csname pgf@anchor@arrow box@before east arrow\endcsname}%
						\ifdim\externalangle pt<\pgfmathresult pt\relax%
							\def\firstpoint{before east arrow head}%
							\def\secondpoint{before east arrow}%
						\else%
							\def\firstpoint{before east arrow}%
							\def\secondpoint{north east}%
						\fi%
					\fi%
				\else%
					\pgfmathanglebetweenpoints{\referencepoint}%
						{\csname pgf@anchor@arrow box@after north arrow tip\endcsname}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax%
						\pgfmathanglebetweenpoints{\referencepoint}%
							{\csname pgf@anchor@arrow box@after north arrow\endcsname}%
						\ifdim\externalangle pt<\pgfmathresult pt\relax%
							\def\firstpoint{north east}%
							\def\secondpoint{after north arrow}%
						\else%
							\def\firstpoint{after north arrow}%
							\def\secondpoint{after north arrow head}%
						\fi%
					\else%
						\def\firstpoint{after north arrow tip}%
						\def\secondpoint{north arrow tip}%
					\fi%
				\fi%
			\else%	
				\pgfmathanglebetweenpoints{\referencepoint}%
					{\csname pgf@anchor@arrow box@north west\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\pgfmathanglebetweenpoints{\referencepoint}%
						{\csname pgf@anchor@arrow box@before north arrow tip\endcsname}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax%
						\def\firstpoint{north arrow tip}%
						\def\secondpoint{before north arrow tip}%
					\else%
						\pgfmathanglebetweenpoints{\referencepoint}%
							{\csname pgf@anchor@arrow box@before north arrow\endcsname}%
						\ifdim\externalangle pt<\pgfmathresult pt\relax%
							\def\firstpoint{before north head}%
							\def\secondpoint{before north arrow}%
						\else%
							\def\firstpoint{before north arrow}%
							\def\secondpoint{north west}%
						\fi%
					\fi%
				\else%
					\pgfmathanglebetweenpoints{\referencepoint}%
						{\csname pgf@anchor@arrow box@after west arrow tip\endcsname}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax%
						\pgfmathanglebetweenpoints{\referencepoint}%
							{\csname pgf@anchor@arrow box@after west arrow\endcsname}%
						\ifdim\externalangle pt<\pgfmathresult pt\relax%
							\def\firstpoint{north west}%
							\def\secondpoint{after west arrow}%
						\else%
							\def\firstpoint{after west arrow}%
							\def\secondpoint{after west arrow head}%
						\fi%
					\else%
						\def\firstpoint{after west arrow tip}%
						\def\secondpoint{west arrow tip}%
					\fi%
				\fi%
			\fi%
		\else%
			\pgfmathanglebetweenpoints{\referencepoint}%
				{\csname pgf@anchor@arrow box@south arrow tip\endcsname}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathanglebetweenpoints{\referencepoint}%
					{\csname pgf@anchor@arrow box@south west\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\pgfmathanglebetweenpoints{\referencepoint}%
						{\csname pgf@anchor@arrow box@before west arrow tip\endcsname}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax%
						\def\firstpoint{west arrow tip}%
						\def\secondpoint{before west arrow tip}%
					\else%
						\pgfmathanglebetweenpoints{\referencepoint}%
							{\csname pgf@anchor@arrow box@before west arrow\endcsname}%
						\ifdim\externalangle pt<\pgfmathresult pt\relax%
							\def\firstpoint{before west arrow head}%
							\def\secondpoint{before west arrow}%
						\else%
							\def\firstpoint{before west arrow}%
							\def\secondpoint{south west}%
						\fi%
					\fi%
				\else%
					\pgfmathanglebetweenpoints{\referencepoint}%
						{\csname pgf@anchor@arrow box@after south arrow tip\endcsname}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax%
						\pgfmathanglebetweenpoints{\referencepoint}%
							{\csname pgf@anchor@arrow box@after south arrow\endcsname}%
						\ifdim\externalangle pt<\pgfmathresult pt\relax%
							\def\firstpoint{south west}%
							\def\secondpoint{after south arrow}%
						\else%
							\def\firstpoint{after south arrow}%
							\def\secondpoint{after south arrow head}%
						\fi%
					\else%
						\def\firstpoint{after south arrow tip}%
						\def\secondpoint{south arrow tip}%
					\fi%
				\fi%
			\else%
				\pgfmathanglebetweenpoints{\referencepoint}%
					{\csname pgf@anchor@arrow box@south east\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\pgfmathanglebetweenpoints{\referencepoint}%
						{\csname pgf@anchor@arrow box@before south arrow tip\endcsname}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax%
						\def\firstpoint{south arrow tip}%
						\def\secondpoint{before south arrow tip}%
					\else%
						\pgfmathanglebetweenpoints{\referencepoint}%
							{\csname pgf@anchor@arrow box@before south arrow\endcsname}%
						\ifdim\externalangle pt<\pgfmathresult pt\relax%
							\def\firstpoint{before south arrow head}%
							\def\secondpoint{before south arrow}%
						\else%
							\def\firstpoint{before south arrow}%
							\def\secondpoint{south east}%
						\fi%
					\fi%
				\else%
					\pgfmathanglebetweenpoints{\referencepoint}%
						{\csname pgf@anchor@arrow box@after east arrow tip\endcsname}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax%
						\pgfmathanglebetweenpoints{\referencepoint}%
							{\csname pgf@anchor@arrow box@after east arrow\endcsname}%
						\ifdim\externalangle pt<\pgfmathresult pt\relax%
							\def\firstpoint{south east}%
							\def\secondpoint{after east arrow}%
						\else%
							\def\firstpoint{after east arrow}%
							\def\secondpoint{after east arrow head}%
						\fi%
					\else%
						\def\firstpoint{after east arrow tip}%
						\def\secondpoint{east arrow tip}%
					\fi%
				\fi%
			\fi%
		\fi%
		\pgfpointintersectionoflines{\referencepoint}{\externalpoint}%
			{\csname pgf@anchor@arrow box@\firstpoint\endcsname}%
			{\csname pgf@anchor@arrow box@\secondpoint\endcsname}%					
	}
}


		
 
\endinput


==> pgflibraryshapes.callouts.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.



% Keys for callouts
%
% Common to all callouts:
%	/pgf/callout absolute pointer
%	/pgf/callout relative pointer
%
% ellipse callout only:
%	/pgf/callout pointer arc    
%
% rectangle callout only:    
%	/pgf/callout pointer width      
%
% cloud callout only:
%	/pgf/callout pointer start size
%	/pgf/callout pointer end size
%	/pgf/callout pointer segments
%
\newif\ifpgf@lib@callout@absolutepointer
\pgfkeys{/pgf/.cd,
	callout pointer arc/.initial=15,
	callout pointer width/.initial=.25cm,
	callout pointer start size/.initial=.2 of callout,
	callout pointer end size/.initial=.1 of callout,
	callout pointer segments/.initial=2,
	callout absolute pointer/.code={\pgf@lib@callout@makeabsolutepointer{#1}},
	callout relative pointer/.code={\pgf@lib@callout@makerelativepointer{#1}},
	callout pointer shorten/.initial=0cm
}



\def\pgf@lib@callout@makeabsolutepointer#1{%
	\pgf@lib@callout@absolutepointertrue%
	{%
		\pgftransformshift{#1}%
		\pgfmultipartnode{coordinate}{center}{pgf@lib@callout@pointer}{}%
	}%
}

\def\pgf@lib@callout@makerelativepointer#1{%
	\pgf@lib@callout@absolutepointerfalse%
	\def\pgf@lib@callout@relativepointer{#1}%
}
\pgfkeys{/pgf/callout relative pointer=\pgfpointpolar{300}{.5cm}}


% Shape ellipse callout
%
%
\pgfdeclareshape{ellipse callout}{%
	\savedmacro\ellipsecalloutpoints{%
		%
		% Get the larger of the outer sep.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@x>\pgf@y%
			\edef\outersep{\the\pgf@x}%
		\else%
			\edef\outersep{\the\pgf@y}%
		\fi%
		\addtosavedmacro\outersep%
		%
		% Calculate the node dimensions...
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@x1.4142136\pgf@x%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<.5\pgf@xa%
      \pgf@x.5\pgf@xa%
    \fi%
    %
   	\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%    
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y.5\dp\pgfnodeparttextbox%
    \pgf@y1.4142136\pgf@y%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<.5\pgf@ya%
      \pgf@y.5\pgf@ya%
    \fi%
    %
    % ...without outer sep...
    %
    \edef\xpathradius{\the\pgf@x}%
    \edef\ypathradius{\the\pgf@y}%
    %
    % ...and width outer sep.
    %
    \pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
    \edef\xradius{\the\pgf@x}%
    \pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
    \edef\yradius{\the\pgf@y}%
    %
    \addtosavedmacro\xradius%
    \addtosavedmacro\xpathradius%
    \addtosavedmacro\yradius% 
    \addtosavedmacro\ypathradius%
  	%
	  \pgfmathsetmacro\pointerarc{\pgfkeysvalueof{/pgf/callout pointer arc}}%
		\addtosavedmacro\pointerarc%
	  %
	  \pgfextract@process\centerpoint{%
	    \pgf@x.5\wd\pgfnodeparttextbox%
	    \pgf@y.5\ht\pgfnodeparttextbox%
	    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
	  }%
	  %
	  % Get the realtive pointer.
	  %
	  \ifpgf@lib@callout@absolutepointer%
	  \else%
	   	\pgfextract@process\calloutpointer{%
				\pgfextract@process\borderpoint{%
					\expandafter\pgfpointborderellipse\expandafter{\pgf@lib@callout@relativepointer}{\pgfqpoint{\xpathradius}{\ypathradius}}%
				}%
				\pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
				\let\pointerangle\pgfmathresult%
				\expandafter\pgf@process\expandafter{\pgf@lib@callout@relativepointer}%
				\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
				\edef\pointerradius{\pgfmathresult pt}%
				\pgfpointadd{\borderpoint}{\pgfqpointpolar{\pointerangle}{\pointerradius}}%
				\pgf@xa\pgf@x%
				\pgf@ya\pgf@y%
				\centerpoint%
				\advance\pgf@x\pgf@xa%
				\advance\pgf@y\pgf@ya%
			}%
			%
			\addtosavedmacro\calloutpointer%
			\pgf@lib@callouts@shortenpointer%
			\pgf@lib@ellipsecallout@getpoints%
	  	\addtosavedmacro\calloutpointeranchor%
	  	\addtosavedmacro\beforecalloutangle%
	  	\addtosavedmacro\aftercalloutangle%
  	\fi%
  }%
  \savedanchor\centerpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y.5\ht\pgfnodeparttextbox%
    \advance\pgf@y-.5\dp\pgfnodeparttextbox%
  }
  \savedanchor\midpoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@y{+.5ex}%
  }
  \savedanchor\basepoint{%
    \pgf@x.5\wd\pgfnodeparttextbox%
    \pgf@y0pt\relax%
  }
  \anchor{center}{\centerpoint}%
  \anchor{mid}{\midpoint}%
  \anchor{mid east}{%
  	\ellipsecalloutpoints%
  	\pgfmathpointintersectionoflineandarc{\midpoint\advance\pgf@x\xradius}{\midpoint}%
  		{\centerpoint}{270}{450}{\xradius and \yradius}%
  }%
  \anchor{mid west}{%
  	\ellipsecalloutpoints%
  	\pgfmathpointintersectionoflineandarc{\midpoint\advance\pgf@x-\xradius}{\midpoint}%
  		{\centerpoint}{90}{270}{\xradius and \yradius}%
  }%
  \anchor{base}{\basepoint}%
  \anchor{base east}{%
  	\ellipsecalloutpoints%
  	\pgfmathpointintersectionoflineandarc{\basepoint\advance\pgf@x\xradius}{\basepoint}%
  		{\centerpoint}{270}{450}{\xradius and \yradius}%
  }%
  \anchor{base west}{%
  	\ellipsecalloutpoints%
  	\pgfmathpointintersectionoflineandarc{\basepoint\advance\pgf@x-\xradius}{\basepoint}%
  		{\centerpoint}{90}{270}{\xradius and \yradius}%
  }%
  \anchor{north}{%
  	\ellipsecalloutpoints%
  	\centerpoint%
  	\advance\pgf@y\yradius\relax%
  }
  \anchor{south}{%
  	\ellipsecalloutpoints%
  	\centerpoint%
  	\advance\pgf@y-\yradius\relax%
  }
  \anchor{east}{%
  	\ellipsecalloutpoints%
  	\centerpoint%
  	\advance\pgf@x\xradius\relax%
  }
  \anchor{west}{%
  	\ellipsecalloutpoints%
  	\centerpoint%
  	\advance\pgf@x-\xradius\relax%
  }
  \anchor{north west}{%
  	\ellipsecalloutpoints%
  	\pgf@xa\xradius\relax%
  	\pgf@ya\yradius\relax%
  	\centerpoint%
  	\advance\pgf@y0.7071067\pgf@ya%
  	\advance\pgf@x-0.7071067\pgf@xa%
  }
  \anchor{north east}{%
  	\ellipsecalloutpoints%
  	\pgf@xa\xradius\relax%
  	\pgf@ya\yradius\relax%
  	\centerpoint%
  	\advance\pgf@y0.7071067\pgf@ya%
  	\advance\pgf@x0.7071067\pgf@xa%
  }
  \anchor{south west}{%
  	\ellipsecalloutpoints%
  	\pgf@xa\xradius\relax%
  	\pgf@ya\yradius\relax%
  	\centerpoint%
  	\advance\pgf@y-0.7071067\pgf@ya%
  	\advance\pgf@x-0.7071067\pgf@xa%
  }
  \anchor{south east}{%
  	\ellipsecalloutpoints%
  	\pgf@xa\xradius\relax%
  	\pgf@ya\yradius\relax%
  	\centerpoint%
  	\advance\pgf@y-0.7071067\pgf@ya%
  	\advance\pgf@x0.7071067\pgf@xa%
  }
  \anchor{pointer}{%
  	\ellipsecalloutpoints%
  	\calloutpointeranchor%
	}%
  \backgroundpath{%
  	\ellipsecalloutpoints%
   	\ifpgf@lib@callout@absolutepointer%
   		\pgfextract@process\calloutpointer{%
				\pgfpointanchor{pgf@lib@callout@pointer}{center}%
			}%
			\pgf@lib@callouts@shortenpointer%
			\pgf@lib@ellipsecallout@getpoints%	
			\calloutpointeranchor%	
			\ifx\pgf@test\pgfutil@empty%
			\else%
				\edef\pgf@sh@@temp{\noexpand\expandafter\noexpand\pgfutil@g@addto@macro\noexpand\csname pgf@sh@np@\pgf@test\noexpand\endcsname}%
				\edef\pgf@sh@@@temp{%
					\noexpand\def\noexpand\calloutpointeranchor{%
						\noexpand\pgf@x\the\pgf@x%
						\noexpand\pgf@y\the\pgf@y%
					}%
				}%
				\expandafter\pgf@sh@@temp\expandafter{\pgf@sh@@@temp}
			\fi%
		\fi%
		\pgfpathmoveto{\calloutpointer}%
		\pgfpathlineto{\aftercalloutpointer}%
		\ifdim\aftercalloutangle pt<\beforecalloutangle pt\relax%
			\pgfpatharc{\aftercalloutangle}{\beforecalloutangle}{\xpathradius and \ypathradius}%
		\else%
			\pgfpatharc{\aftercalloutangle}{360}{\xpathradius and \ypathradius}%
			\pgfpatharc{0}{\beforecalloutangle}{\xpathradius and \ypathradius}%
		\fi%
		\pgfpathclose%
  }%    
  \anchorborder{%
  	\pgfextract@process\externalpoint{}%
  	\ellipsecalloutpoints%
   	\pgfpointadd{\pgfpointborderellipse{\externalpoint}{\pgfpoint{\xradius}{\yradius}}%
  	}{\centerpoint}%  		
  }%
}

% Internal macro for calculating the points for the
% ellipse callout pointer.
%
% The following must be set up:
%
% \centerpoint    - the center of the ellipse.
% \calloutpointer - the location of the callout point.
% \pointerarc     - the width of the pointer.
% \xpathradius    - the x radius of the ellipse.
% \ypathradius    - the y radius of the ellipse.
%
\def\pgf@lib@ellipsecallout@getpoints{%
	\pgfextract@process\borderpoint{%
		\pgfpointborderellipse{%
			\centerpoint%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\calloutpointer%
			\advance\pgf@x-\pgf@xa%
			\advance\pgf@y-\pgf@ya%
		}{\pgfqpoint{\xpathradius}{\ypathradius}}%
	}%
	\pgfmathangleonellipse{\borderpoint}{\xpathradius and \ypathradius}%
	\pgfutil@tempdima\pointerarc pt\relax%
	\pgfutil@tempdimb\pgfmathresult pt\relax%
	\advance\pgfutil@tempdimb-.5\pgfutil@tempdima%
	\ifdim\pgfutil@tempdimb<0pt\relax%
		\advance\pgfutil@tempdimb360pt\relax%
	\fi%
	\edef\beforecalloutangle{\pgfmath@tonumber{\pgfutil@tempdimb}}%
	\advance\pgfutil@tempdimb\pgfutil@tempdima%
	\ifdim\pgfutil@tempdimb<360pt\relax%
	\else%
		\advance\pgfutil@tempdimb-360pt\relax%
	\fi%
	\edef\aftercalloutangle{\pgfmath@tonumber{\pgfutil@tempdimb}}%	
	%
	\pgfextract@process\beforecalloutpointer{%
		\pgfpointadd{\centerpoint}{%
			\pgfpointpolar{\beforecalloutangle}{\xpathradius and \ypathradius}%
		}%
	}%
	\pgfextract@process\aftercalloutpointer{%
		\pgfpointadd{\centerpoint}{%
			\pgfpointpolar{\aftercalloutangle}{\xpathradius and \ypathradius}%
		}%
	}%
	%
	% Calculate the pointer anchor.
	%
	\pgf@lib@callouts@pointeranchor%
}


% If the callout pointer is very pointed and stroked, the anchor will be 
% miles away from the end of the pointer which will (typically) be
% bevelled. 
% Using outer sep=0pt is one solution, however, another is provided
% using this special key:
%
% /pgf/callout pointer anchor aspect
% 
% which takes a value from 0 (ignore any outer sep) to 1 (use
% the full outer sep).

\pgfkeys{/pgf/callout pointer anchor aspect/.initial=1}

% Internal macro for calculating the anchor for the callout pointer.
%
% Requires the following to be set up (points are anti-clockwise)
%
% \beforecalloutpointer - point on the border before the callout pointer 
% \calloutpointer    
% \aftercalloutpointer  - point on the border after the callout pointer
% \outersep             - the largest of the outer xsep or ysep.
%
\def\pgf@lib@callouts@pointeranchor{%
	\pgfutil@tempdimb\outersep\relax%
	%
	\pgfmathanglebetweenlines{\calloutpointer}{\aftercalloutpointer}{\calloutpointer}{\beforecalloutpointer}%
	\pgfmathdivide@{\pgfmathresult}{2}%
	\pgfutil@tempdima\pgfmathresult pt\relax%
	\pgfmathcosec@{\pgfmathresult}%
	\pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
	\pgfmathanglebetweenpoints{\calloutpointer}{\aftercalloutpointer}%
	\advance\pgfutil@tempdima\pgfmathresult pt\relax%
	\advance\pgfutil@tempdima180pt\relax%
	%	
	\pgfextract@process\calloutpointeranchor{%
		\pgfpointadd{%
			\pgfmathparse{\pgfkeysvalueof{/pgf/callout pointer anchor aspect}}%
			\pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
			\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
		}{%
			\calloutpointer%
		}%
	}%	
}%

\def\pgf@lib@callouts@shortenpointer{%
	\pgfextract@process\calloutpointer{%
		\pgfmathanglebetweenpoints{\calloutpointer}{\centerpoint}%
		\let\angle\pgfmathresult%
		\pgfmathsin@{\angle}%
		\let\sinpointerangle\pgfmathresult%
		\pgfmathcos@{\angle}%
		\let\cospointerangle\pgfmathresult%	
		\pgfpointadd{\calloutpointer}{%
			\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/callout pointer shorten}}%
			\pgf@x\cospointerangle\pgfutil@tempdima%
			\pgf@y\sinpointerangle\pgfutil@tempdima%
		}%
	}%
}%
	

\pgfdeclareshape{rectangle callout}{%
	\savedmacro\rectanglecalloutpoints{%
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@x<.5\pgf@xa%
			\pgf@x.5\pgf@xa%
		\fi%
		\edef\xtemp{\the\pgf@x}%
		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@y<.5\pgf@ya%
			\pgf@y.5\pgf@ya%
		\fi%
		\edef\ytemp{\the\pgf@y}%
		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		%
		\edef\xlength{\the\pgf@x}%
		\edef\ylength{\the\pgf@y}%
		\addtosavedmacro\xlength%
		\addtosavedmacro\ylength%
		%
		\pgfmathsetlengthmacro\pointerwidth{\pgfkeysvalueof{/pgf/callout pointer width}}%
		\addtosavedmacro\pointerwidth%
		%
		\pgfextract@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		%
		% Process the relative callout pointer.
		%
		\ifpgf@lib@callout@absolutepointer%
		\else%
			\pgfextract@process\calloutpointer{%
				\pgfextract@process\borderpoint{%
					\expandafter\pgfpointborderrectangle\expandafter{\pgf@lib@callout@relativepointer}%
						{\pgfqpoint{\xtemp}{\ytemp}}%
				}%
				\pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
				\let\pointerangle\pgfmathresult%
				\expandafter\pgf@process\expandafter{\pgf@lib@callout@relativepointer}%
				\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
				\edef\pointerradius{\pgfmathresult pt}%
				\pgfpointadd{\borderpoint}{\pgfqpointpolar{\pointerangle}{\pointerradius}}%
				\pgf@xa\pgf@x%
				\pgf@ya\pgf@y%
				\centerpoint%
				\advance\pgf@x\pgf@xa%
				\advance\pgf@y\pgf@ya%
			}%
			\pgf@lib@callouts@shortenpointer%
			\addtosavedmacro\calloutpointer%
			\pgf@lib@rectanglecallout@pointer%
			\addtosavedmacro\calloutpointeranchor%
			\addtosavedmacro\beforecalloutpointer%
			\addtosavedmacro\aftercalloutpointer%
			\addtosavedmacro\firstpoint%
			\addtosavedmacro\secondpoint%
			\addtosavedmacro\thirdpoint%
			\addtosavedmacro\fourthpoint%
		\fi%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt\relax%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5em}%
	}
	\anchor{center}{\centerpoint}
	\anchor{mid}{\midpoint}
	\anchor{mid east}{%
		\rectanglecalloutpoints%
		\midpoint%
		\advance\pgf@x\xlength\relax%		
	}
	\anchor{mid west}{%
		\rectanglecalloutpoints%
		\midpoint%
		\advance\pgf@x-\xlength\relax%		
	}
	\anchor{base}{\basepoint}
	\anchor{base east}{%
		\rectanglecalloutpoints%
		\basepoint%
		\advance\pgf@x\xlength\relax%		
	}
	\anchor{base west}{%
		\rectanglecalloutpoints%
		\basepoint%
		\advance\pgf@x-\xlength\relax%		
	}
	\anchor{north}{%
		\rectanglecalloutpoints%
		\centerpoint%
		\advance\pgf@y\ylength\relax%
	}%
	\anchor{south}{%
		\rectanglecalloutpoints%
		\centerpoint%
		\advance\pgf@y-\ylength\relax%
	}%
	\anchor{east}{%
		\rectanglecalloutpoints%
		\centerpoint%
		\advance\pgf@x\xlength\relax%
	}%
	\anchor{west}{%
		\rectanglecalloutpoints%
		\centerpoint%
		\advance\pgf@x-\xlength\relax%
	}%
	\anchor{north east}{%
		\rectanglecalloutpoints%
		\centerpoint%
		\advance\pgf@x\xlength\relax%
		\advance\pgf@y\ylength\relax%
	}%
	\anchor{south west}{%
		\rectanglecalloutpoints%
		\centerpoint%
		\advance\pgf@x-\xlength\relax%
		\advance\pgf@y-\ylength\relax%
	}%
	\anchor{south east}{%
		\rectanglecalloutpoints%
		\centerpoint%
		\advance\pgf@x\xlength\relax%
		\advance\pgf@y-\ylength\relax%
	}%
	\anchor{north west}{%
		\rectanglecalloutpoints%
		\centerpoint%
		\advance\pgf@x-\xlength\relax%
		\advance\pgf@y\ylength\relax%
	}%
	\anchor{pointer}{%
		\rectanglecalloutpoints%
		\calloutpointeranchor%
	}%
	\backgroundpath{%
		\rectanglecalloutpoints%
		\pgf@x\xlength\relax%
		\pgf@y\ylength\relax%
		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
		\edef\xtemp{\the\pgf@x}%
		\edef\ytemp{\the\pgf@y}%
		%
		% The absolute pointer must be calculated here because the
		% anchor of the shape (which is calculated after the saved
		% macros and points) affects how the pointer joins the 
		% main rectangle. 
		%
		\ifpgf@lib@callout@absolutepointer%
			\pgfextract@process\calloutpointer{%
				\pgfpointanchor{pgf@lib@callout@pointer}{center}%
			}%
			\pgf@lib@callouts@shortenpointer%
			\pgfmathsetlengthmacro\pointerwidth{\pgfkeysvalueof{/pgf/callout pointer width}}%
			\pgf@lib@rectanglecallout@pointer%
			%
			% \pgf@test = the shape name (from \pgfmultipartnode)
			%
			\ifx\pgf@test\pgfutil@empty%
			\else%
				%
				% Now hack an extra saved anchor \calloutpointeranchor,
				% with the new anchor for the callout pointer.
				%
				\edef\pgf@sh@@temp{\noexpand\expandafter\noexpand\pgfutil@g@addto@macro\noexpand\csname pgf@sh@np@\pgf@test\noexpand\endcsname}%
				\edef\pgf@sh@@@temp{%
					\noexpand\def\noexpand\calloutpointeranchor{%
						\noexpand\pgf@x\the\pgf@x%
						\noexpand\pgf@y\the\pgf@y%
					}%
				}%
				\expandafter\pgf@sh@@temp\expandafter{\pgf@sh@@@temp}%
			\fi%
		\fi%
		{%
			\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
			\pgfpathmoveto{\beforecalloutpointer}%
		}%
		\pgfpathlineto{\calloutpointer}%
		{%
			\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
			\pgfpathlineto{\aftercalloutpointer}%
		}%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathlineto{\firstpoint}%
			\pgfpathlineto{\secondpoint}%
			\pgfpathlineto{\thirdpoint}%
			\pgfpathlineto{\fourthpoint}%
			{%
				\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
				\pgfpathclose%
			}%
		}			
	}
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\rectanglecalloutpoints%
		\pgfpointadd{\centerpoint}%
		{%
			\pgfpointborderrectangle{\pgfpointadd{\centerpoint}{\externalpoint}}%
			{\pgfqpoint{\xlength}{\ylength}}%
		}%
	}%
}



% \pgf@lib@rectanglecallout@pointer
%
% Internal macro for calculations relating to the rectangle callout.
%
% Requires the following to be set up:
%
% \calloutpointer - the location of the callout point.
% \xtemp          - the half width of the rectangle
% \ytemp          - the half height of the rectangle
% \pointerwidth   - the width of the pointer.
%
\def\pgf@lib@rectanglecallout@pointer{%
	%
	% Ensure that the pointer never connects to the main shape
	% too near to a corner. This is done for two reasons:
	% 1. It can look ugly.
	% 2. If the corners are rounded, a mess can result.
	%
	\pgfextract@process\borderpoint{%
			\pgfpointborderrectangle{%
				\centerpoint%
				\pgf@xa\pgf@x%
				\pgf@ya\pgf@y%
				\calloutpointer%
				\advance\pgf@x-\pgf@xa%
				\advance\pgf@y-\pgf@ya%
			}{\pgfqpoint{\xtemp}{\ytemp}}%
		}%
	\pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
	\let\borderangle\pgfmathresult%
	%
	\pgfutil@tempdima\pointerwidth\relax%
	\pgf@xa\xtemp\relax%
	\advance\pgf@xa-\pgfutil@tempdima%
	\pgf@ya\ytemp\relax%
	\advance\pgf@ya-\pgfutil@tempdima%
	%
	\pgf@process{%
		\pgfutil@ifundefined{pgf@corner@arc}{\pgfpointorigin}{%
			\expandafter\pgfqpoint\pgf@corner@arc}%
	}%
	\advance\pgf@xa-\pgf@x%
	\advance\pgf@ya-\pgf@y%
	%
	\borderpoint%
	\pgf@xb\pgf@x%
	\pgf@yb\pgf@y%
	%
	\pgf@xc0pt\relax%
	\pgf@yc0pt\relax%
	%
	\pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{\xtemp}{\ytemp}}%
	\ifdim\borderangle pt<\pgfmathresult pt\relax%
		\pgf@yc.5\pgfutil@tempdima%
		\ifdim\pgf@yb>\pgf@ya%
			\pgf@yb\pgf@ya%
		\fi%
		%
		% Establish the order for drawing the rectangle corners.
		%
		\edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
		\edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
		\edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
		\edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
	\else%
		\pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{-\xtemp}{\ytemp}}%
		\ifdim\borderangle pt<\pgfmathresult pt\relax%
			\pgf@xc-.5\pgfutil@tempdima%
			\ifdim\pgf@xb>\pgf@xa%
				\pgf@xb\pgf@xa%
			\else%
				\ifdim\pgf@xb<-\pgf@xa%
					\pgf@xb-\pgf@xa%
				\fi%
			\fi%
			\edef\firstpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
			\edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
			\edef\thirdpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
			\edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
		\else%
			\pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{-\xtemp}{-\ytemp}}%
			\ifdim\borderangle pt<\pgfmathresult pt\relax%
				\pgf@yc-.5\pgfutil@tempdima%
				\ifdim\pgf@yb>\pgf@ya%
					\pgf@yb\pgf@ya%
				\else%
					\ifdim\pgf@yb<-\pgf@ya%
						\pgf@yb-\pgf@ya%
					\fi%
				\fi%
				\edef\firstpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
				\edef\secondpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
				\edef\thirdpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
				\edef\fourthpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
			\else%
				\pgfmathanglebetweenpoints{\pgfpointorigin}{\pgfqpoint{\xtemp}{-\ytemp}}%
				\ifdim\borderangle pt<\pgfmathresult pt\relax%
					\pgf@xc.5\pgfutil@tempdima%
					\ifdim\pgf@xb>\pgf@xa%
						\pgf@xb\pgf@xa%
					\else%
						\ifdim\pgf@xb<-\pgf@xa%
							\pgf@xb-\pgf@xa%
						\fi%
					\fi%
					\edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
					\edef\secondpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
					\edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
					\edef\fourthpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
				\else%
					\pgf@yc.5\pgfutil@tempdima%
					\ifdim\pgf@yb<-\pgf@ya%
						\pgf@yb-\pgf@ya%
					\fi%
					\edef\firstpoint{\noexpand\pgfqpoint{\xtemp}{\ytemp}}%
					\edef\secondpoint{\noexpand\pgfqpoint{-\xtemp}{\ytemp}}%
					\edef\thirdpoint{\noexpand\pgfqpoint{-\xtemp}{-\ytemp}}%
					\edef\fourthpoint{\noexpand\pgfqpoint{\xtemp}{-\ytemp}}%
				\fi%
			\fi%
		\fi%
	\fi%
	\pgfextract@process\beforecalloutpointer{%
		\centerpoint%
		\advance\pgf@x\pgf@xb%
		\advance\pgf@y\pgf@yb%
		\advance\pgf@x-\pgf@xc%		
		\advance\pgf@y-\pgf@yc%
	}%	
	\pgfextract@process\aftercalloutpointer{%
		\centerpoint%
		\advance\pgf@x\pgf@xb%
		\advance\pgf@y\pgf@yb%
		\advance\pgf@x\pgf@xc%		
		\advance\pgf@y\pgf@yc%
	}%	
	%
	% Now calculate the pointer anchor.
	%
	\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
	\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
	\ifdim\pgf@x>\pgf@y%
		\edef\outersep{\the\pgf@x}%
	\else%
		\edef\outersep{\the\pgf@y}%
	\fi%
	\pgf@lib@callouts@pointeranchor%
}


% Internal macro for parsing the size of 
% the cloud callout pointer.
%
% \pgf@x and \pgf@y should be set up as the
% width and height of the main shape.
%
% \pgf@xa and \pgf@ya are returned appropriately.
%
\def\pgf@lib@callout@setpointersize#1{%
	\edef\pgf@lib@callout@temp{#1}%
	\edef\pgf@marshall{\noexpand\pgfutil@in@{of callout}{\pgf@lib@callout@temp}}%
	\pgf@marshall%
	\ifpgfutil@in@%
		\expandafter\pgf@xa\expandafter\pgf@lib@callout@setpointerrelativesize%
			\pgf@lib@callout@temp\pgf@lib@stop\pgf@x%
		\expandafter\pgf@ya\expandafter\pgf@lib@callout@setpointerrelativesize%
			\pgf@lib@callout@temp\pgf@lib@stop\pgf@y%
	\else%
		\edef\pgf@marshall{\noexpand\pgfutil@in@{and}{\pgf@lib@callout@temp}}%
		\pgf@marshall%
		\ifpgfutil@in@%
			\expandafter\pgf@lib@callout@setpointerbothsizes\pgf@lib@callout@temp\pgf@lib@stop%
		\else%
			\pgfmathsetlength\pgf@xa{#1}%
			\pgfmathsetlength\pgf@ya{#1}%
		\fi%
	\fi%		 
}
\def\pgf@lib@callout@setpointerrelativesize#1of callout#2\pgf@lib@stop{#1}%
\def\pgf@lib@callout@setpointerbothsizes#1and#2\pgf@lib@stop{%
	\pgfmathsetlength\pgf@xa{#2}%
	\pgfmathsetlength\pgf@ya{#2}%
}

% Shape: cloud callout.
%
\pgfdeclareshape{cloud callout}{%
	\savedanchor\calloutpointer{%
		\pgfutil@ifundefined{pgf@sh@s@cloud}{%
			\PackageError{PGF}{I cannot find the cloud shape. Please load the `symbol shapes' library}{}}{}%
		\pgf@sh@s@cloud%
		\pgf@sh@savedmacros%
		%
		\pgfextract@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		\ifpgf@lib@callout@absolutepointer%
	  \else%
	  	\pgfextract@process\calloutpointer{%
				\pgfextract@process\borderpoint{%
					\expandafter\pgfpointborderellipse\expandafter{\pgf@lib@callout@relativepointer}%
						{\pgfqpoint{\xouterradius}{\youterradius}}%
				}%
				\pgfmathanglebetweenpoints{\pgfpointorigin}{\borderpoint}%
				\let\pointerangle\pgfmathresult%
				\expandafter\pgf@process\expandafter{\pgf@lib@callout@relativepointer}%
				\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
				\edef\pointerradius{\pgfmathresult pt}%
				\pgfpointadd{\borderpoint}{\pgfqpointpolar{\pointerangle}{\pointerradius}}%
				\pgf@xa\pgf@x%
				\pgf@ya\pgf@y%
				\centerpoint%
				\advance\pgf@x\pgf@xa%
				\advance\pgf@y\pgf@ya%
			}%
			\pgf@lib@callouts@shortenpointer%
		\fi%
	}
	\anchor{pointer}{%
		\calloutpointer%
	}%
	\inheritsavedanchors[from=cloud]
	\inheritanchor[from=cloud]{center}
	\inheritanchor[from=cloud]{base}
	\inheritanchor[from=cloud]{mid}
	\inheritanchor[from=cloud]{north}
	\inheritanchor[from=cloud]{south}
	\inheritanchor[from=cloud]{east}
	\inheritanchor[from=cloud]{west}
	\inheritanchor[from=cloud]{north east}
	\inheritanchor[from=cloud]{south west}
	\inheritanchor[from=cloud]{south east}
	\inheritanchor[from=cloud]{north west}
	\inheritanchorborder[from=cloud]
	\backgroundpath{%
		\pgf@sh@bg@cloud%
		\ifpgf@lib@callout@absolutepointer%
   		\pgfextract@process\calloutpointer{%
				\pgfpointanchor{pgf@lib@callout@pointer}{center}%
			}%
			\ifx\pgf@test\pgfutil@empty%
			\else%
				\edef\pgf@sh@@temp{\noexpand\expandafter\noexpand\pgfutil@g@addto@macro\noexpand\csname pgf@sh@np@\pgf@test\noexpand\endcsname}%
				\edef\pgf@sh@@@temp{%
					\noexpand\def\noexpand\calloutpointeranchor{%
						\noexpand\pgf@x\the\pgf@x%
						\noexpand\pgf@y\the\pgf@y%
					}%
				}%
				\expandafter\pgf@sh@@temp\expandafter{\pgf@sh@@@temp}
			\fi%
		\fi%
		%
		\pgfextract@process\borderpoint{%
			\pgfpointadd{%
				\pgfpointborderellipse{\pgfpointdiff{\centerpoint}{\calloutpointer}}%
						{\pgfqpoint{\xouterradius}{\youterradius}}%
			}{\centerpoint}%
		}%
		\pgf@lib@callouts@shortenpointer%
		\pgfmathanglebetweenpoints{\calloutpointer}{\centerpoint}%
		\let\angle\pgfmathresult%
		\pgfmathsin@{\angle}%
		\let\sinpointerangle\pgfmathresult%
		\pgfmathcos@{\angle}%
		\let\cospointerangle\pgfmathresult%	
		%
		\pgf@x\xouterradius\relax%
		\pgf@x2.0\pgf@x%
		\pgf@y\yinnerradius\relax%
		\pgf@y2.0\pgf@y%
		\pgf@lib@callout@setpointersize{\pgfkeysvalueof{/pgf/callout pointer start size}}%
		\pgf@xb\pgf@xa%
		\pgf@yb\pgf@ya%
		\pgf@lib@callout@setpointersize{\pgfkeysvalueof{/pgf/callout pointer end size}}%
		\advance\pgf@xb-\pgf@xa%
		\advance\pgf@yb-\pgf@ya%
		%
		\pgfmathsetcount\c@pgf@counta{\pgfkeysvalueof{/pgf/callout pointer segments}}%
		\divide\pgf@xb\c@pgf@counta%
		\divide\pgf@yb\c@pgf@counta%
		%
		\pgf@process{\pgfpointdiff{\borderpoint}{\calloutpointer}}%
		\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\divide\pgfutil@tempdima\c@pgf@counta%
		%
		\pgfutil@tempdimb0pt\relax%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\c@pgf@counta%
		\else%
			{%
				\pgf@xa.5\pgf@xa%
				\pgf@ya.5\pgf@ya%
				\edef\tempxradius{\the\pgf@xa}%
				\edef\tempyradius{\the\pgf@ya}%
				\pgfpathellipse%
					{%
						\calloutpointer%
						\advance\pgf@x\cospointerangle\pgfutil@tempdimb%
						\advance\pgf@y\sinpointerangle\pgfutil@tempdimb%
					}%
					{\pgfqpoint{\tempxradius}{0pt}}{\pgfqpoint{0pt}{\tempyradius}}%
			}%
			\advance\pgf@xa\pgf@xb%
			\advance\pgf@ya\pgf@yb%
			\advance\pgfutil@tempdimb\pgfutil@tempdima%
		\repeatpgfmathloop%
	}%
	%
	% Hack the puff anchors for the callout.
	%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@cloud callout\endcsname{%
		\c@pgf@counta\puffs\relax%
		\pgfmathloop%
			\ifnum\c@pgf@counta>0\relax%
				\pgfutil@ifundefined{pgf@anchor@cloud callout@puff\space\the\c@pgf@counta}{%
				\expandafter\xdef\csname pgf@anchor@cloud callout@puff\space\the\c@pgf@counta\endcsname{%
					\noexpand\pgf@sh@@cloudpuffanchor{\the\c@pgf@counta}%
				}%
			}{\c@pgf@counta0\relax}%
			\advance\c@pgf@counta-1\relax%
		\repeatpgfmathloop%	
	}%
}

\endinput


==> pgflibraryshapes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryshapes.code.tex,v 1.14 2007/12/17 16:20:50 tantau Exp $

% Only the following are loaded by default and only for historical
% reasons. 

\usepgflibrary{shapes.geometric}
\usepgflibrary{shapes.misc}
\usepgflibrary{shapes.symbols}

% Further libraries should be included directly

\endinput


==> pgflibraryshapes.gates.logic.IEC.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\pgfkeys{/pgf/.cd,
	logic gate input sep/.initial=0.125cm,
	logic gate inputs/.initial={normal,normal},%
	logic gate inverted radius/.initial=2pt,%
	logic gate anchors use bounding box/.is if=pgfgateanchorsuseboundingrectangle,%
	and gate IEC symbol/.initial=$\char`\&$,
	nand gate IEC symbol/.initial=$\char`\&$,
	or gate IEC symbol/.initial=$\geq1$,
	nor gate IEC symbol/.initial=$\geq1$,
	xor gate IEC symbol/.initial={$=1$},
	xnor gate IEC symbol/.initial={$=1$},
	not gate IEC symbol/.initial=1,
	buffer gate IEC symbol/.initial=1,
	logic gate IEC symbol align/.initial=top,
	logic gate IEC symbol color/.initial=% no value
}

\pgfkeys{/pgf/logic gate IEC symbol align/.cd,
	top/.code=\pgftransformyshift{\innerhalfheight},
	bottom/.code=\pgftransformyshift{-\innerhalfheight},
	left/.code=\pgftransformxshift{-\innerhalfwidth},
	right/.code=\pgftransformxshift{\innerhalfwidth}
}

% Internal macro for parsing inputs.
%
\expandafter\ifx\csname pgf@lib@sh@logicgate@parseinputs\endcsname\relax%
\def\pgf@lib@sh@logicgate@parseinputs#1{%
	\edef\pgf@lib@sh@temp{\pgfkeysvalueof{/pgf/logic gate inputs}}%
	\c@pgf@counta#1\relax%
	\c@pgf@countb0\relax%
	\expandafter\pgfutil@in@\expandafter,\expandafter{\pgf@lib@sh@temp}%
	\ifpgfutil@in@%
		\let\pgf@lib@sh@next\pgf@lib@sh@logicgate@parseinputs@long%
	\else%
		\let\pgf@lib@sh@next\pgf@lib@sh@logicgate@parseinputs@short%
	\fi%
	\pgf@lib@sh@next%
}	
\def\pgf@lib@sh@itext{i}
\def\pgf@lib@sh@invertedtext{inverted}
%
%	The `short' version for input specifcation is an extension of
%	ideas due to Juergen Werber and Christoph Bartoschek.
%
\def\pgf@lib@sh@logicgate@parseinputs@short{%
	\expandafter\pgf@lib@sh@logicgate@parseinputs@@short\pgf@lib@sh@temp\pgf@stop%
}
\def\pgf@lib@sh@logicgate@parseinputs@@short#1{%
	\ifx#1\pgf@stop%
		\edef\pgf@lib@sh@logicgate@numinputs{\the\c@pgf@countb}%
		\let\pgf@lib@sh@next\relax%
	\else%
		\ifnum\c@pgf@countb=\c@pgf@counta%
			\edef\pgf@lib@sh@logicgate@numinputs{\the\c@pgf@countb}%
			\let\pgf@lib@sh@next\relax%
		\else%
			\advance\c@pgf@countb1\relax%
			\expandafter\ifx\pgf@lib@sh@itext#1%
				\expandafter\pgf@sh@resavedmacro\expandafter{\csname input-\the\c@pgf@countb\endcsname}{%
					\expandafter\def\csname input-\the\c@pgf@countb\endcsname{i}}%
			\else%
				\expandafter\pgf@sh@resavedmacro\expandafter{\csname input-\the\c@pgf@countb\endcsname}{%
					\expandafter\def\csname input-\the\c@pgf@countb\endcsname{n}}%
			\fi%		
			\let\pgf@lib@sh@next\pgf@lib@sh@logicgate@parseinputs@@short%
		\fi%
	\fi%
	\pgf@lib@sh@next%
}
\def\pgf@lib@sh@logicgate@parseinputs@long{%
	\expandafter\pgf@lib@sh@logicgate@parseinputs@@long\pgf@lib@sh@temp,\pgf@stop,%
}
\def\pgf@lib@sh@logicgate@parseinputs@@long#1,{%
	\ifx#1\pgf@stop%
		\edef\pgf@lib@sh@logicgate@numinputs{\the\c@pgf@countb}%
		\let\pgf@lib@sh@next\relax%
	\else%
		\ifnum\c@pgf@countb=\c@pgf@counta%
			\edef\pgf@lib@sh@logicgate@numinputs{\the\c@pgf@countb}%
			\let\pgf@lib@sh@next\relax%
		\else%
			\advance\c@pgf@countb1\relax%
			\def\pgf@lib@sh@temp{#1}%
			\ifx\pgf@lib@sh@invertedtext\pgf@lib@sh@temp%
				\expandafter\pgf@sh@resavedmacro\expandafter{\csname input-\the\c@pgf@countb\endcsname}{%
					\expandafter\def\csname input-\the\c@pgf@countb\endcsname{i}}%
			\else%
				\expandafter\pgf@sh@resavedmacro\expandafter{\csname input-\the\c@pgf@countb\endcsname}{%
					\expandafter\def\csname input-\the\c@pgf@countb\endcsname{n}}%
			\fi%		
			\let\pgf@lib@sh@next\pgf@lib@sh@logicgate@parseinputs@@@long%
		\fi%
	\fi%
	\pgf@lib@sh@next%
}
\def\pgf@lib@sh@logicgate@parseinputs@@@long{%
	\pgfutil@ifnextchar x{\pgf@lib@sh@logicgate@parseinputs@@long}%
		{\pgf@lib@sh@logicgate@parseinputs@@long}%
}
\fi%

\def\pgf@lib@sh@logicgates@IEC@foregroundpath#1{%
	\dimensions%
	{%
		\pgftransformshift{\centerpoint}%
		\edef\pgf@lib@sh@temp{\pgfkeysvalueof{/pgf/logic gate IEC symbol align}}%
		\edef\pgf@lib@sh@@temp{/pgf/logic gate IEC symbol align/.cd, \pgf@lib@sh@temp}%
		\expandafter\pgfkeys\expandafter{\pgf@lib@sh@@temp}%
		\expandafter\pgftext\expandafter[\pgf@lib@sh@temp]{%
			\pgfkeysgetvalue{/pgf/logic gate IEC symbol color}{\pgf@lib@sh@temp}%
			\ifx\pgf@lib@sh@temp\pgfutil@empty%
			\else%
				\expandafter\color\expandafter{\pgf@lib@sh@temp}%
			\fi%
			\pgfkeysvalueof{/pgf/#1 gate IEC symbol}%
		}%
	}%
}	


\def\pgf@lib@sh@logicgates@dimensions@IEC#1{%
	\pgf@x.5\wd\pgfnodeparttextbox%
	\pgf@y.5\ht\pgfnodeparttextbox%
	\advance\pgf@y.5\dp\pgfnodeparttextbox%
	%
	% Adjust for the width of the gate symbol.
	%
	\setbox\pgf@hbox\hbox{{\pgfkeysvalueof{/pgf/#1 gate IEC	symbol}}}% add braces as color-aftergroup-fix TT
	\pgf@xa.5\wd\pgf@hbox%
	\pgf@ya.5\ht\pgf@hbox%
	\advance\pgf@ya.5\dp\pgf@hbox%
	\ifdim\pgf@x<\pgf@xa%
		\pgf@x\pgf@xa%
	\fi%
	\ifdim\pgf@y<\pgf@ya%
		\pgf@y\pgf@ya%
	\fi%
	\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
	\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
	%
	% Adjust for minimum height and width.
	%
	\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
	\ifdim\pgf@x<.5\pgf@xa%
		\pgf@x.5\pgf@xa%
	\fi%
	\ifdim\pgf@y<.5\pgf@ya%
		\pgf@y.5\pgf@ya%
	\fi%
	%
	% Adjust the height for the number of inputs.
	%
	\c@pgf@counta\pgf@lib@sh@logicgate@numinputs%
	\advance\c@pgf@counta1\relax%
	\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	\pgf@yb2.0\pgf@yb%
	\advance\pgf@yb\pgflinewidth%
	\pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/logic gate input sep}}%
	\edef\inputsep{\the\pgf@yc}%
	\addtosavedmacro\inputsep%
	\ifdim\pgf@yb<\pgf@yc%
		\pgf@yb\pgf@yc%
	\fi%
	\multiply\pgf@yb\c@pgf@counta%
	\ifdim\pgf@y<.5\pgf@yb%
		\pgf@y.5\pgf@yb%
	\fi%
	%
	\pgf@xa\pgf@y%
	\pgfmathaddtolength\pgf@xa{-\pgfkeysvalueof{/pgf/inner xsep}}%
	\edef\innerhalfwidth{\the\pgf@xa}%
	\addtosavedmacro\innerhalfwidth%
	%
	\pgf@ya\pgf@y%
	\pgfmathaddtolength\pgf@ya{-\pgfkeysvalueof{/pgf/inner ysep}}%
	\edef\innerhalfheight{\the\pgf@ya}%
	\addtosavedmacro\innerhalfheight%
	%
	% Take into account the outer sep.
	%
	\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
	\pgfmathaddtolength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
	%
	\edef\halfwidth{\the\pgf@x}%
	\edef\halfheight{\the\pgf@y}%
	\addtosavedmacro\halfwidth%
	\addtosavedmacro\halfheight%
}%

\def\pgf@lib@sh@logicgate@IEC@inputanchor#1{%
	\dimensions%
	\centerpoint%
	\advance\pgf@x-\halfwidth%
	\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-#1\endcsname%
		\advance\pgf@x-\invertedradius%
		\advance\pgf@x-\outerinvertedradius%
	\fi%
	%
	\pgfutil@tempdima\halfheight%
	\multiply\pgfutil@tempdima2\relax%
	\c@pgf@counta\numinputs%
	\advance\c@pgf@counta1\relax%
	\divide\pgfutil@tempdima\c@pgf@counta%
	\multiply\pgfutil@tempdima#1\relax%
	\advance\pgf@y\halfheight%
	\advance\pgf@y-\pgfutil@tempdima%
}



% Shape and gate IEC
%
\pgfdeclareshape{and gate IEC}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@and gate IEC\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@and gate IEC@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@and gate IEC@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{An and gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{and}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}
	\anchor{mid west}{%
		\dimensions%
		\midpoint%
		\advance\pgf@x-\halfwidth}%
	\anchor{mid east}{%
		\dimensions%
		\midpoint%
		\advance\pgf@x\halfwidth}%
	\anchor{base}{\basepoint}
	\anchor{base west}{%
		\dimensions%
		\basepoint%
		\advance\pgf@x-\halfwidth}%
	\anchor{base east}{%
		\dimensions%
		\basepoint%
		\advance\pgf@x\halfwidth}%
	\anchor{north}{\dimensions\centerpoint\advance\pgf@y\halfheight}%
	\anchor{south}{\dimensions\centerpoint\advance\pgf@y-\halfheight}%
	\anchor{east}{\dimensions\centerpoint\advance\pgf@x\halfwidth}%
	\anchor{west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth}%
	\anchor{north east}{\dimensions\centerpoint\advance\pgf@x\halfwidth\advance\pgf@y\halfheight}%
	\anchor{north west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y\halfheight}%
	\anchor{south east}{\dimensions\centerpoint\advance\pgf@x\halfwidth\advance\pgf@y-\halfheight}%
	\anchor{south west}{\dimensions\centerpoint\advance\pgf@x-\halfwidth\advance\pgf@y-\halfheight}%
	\anchor{output}{\dimensions\centerpoint\advance\pgf@x\halfwidth} 
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\pgfmathaddtolength\pgf@xc{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@yc{-\pgfkeysvalueof{/pgf/outer xsep}}%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathrectangle{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
				{%
					\pgf@xc2.0\pgf@xc%
					\pgf@yc2.0\pgf@yc%
					\pgfqpoint{\pgf@xc}{\pgf@yc}%
				}%
			\pgfpathclose%
			%
			% Draw inputs.
			%
			\pgf@xc-\halfwidth%
			\advance\pgf@xc-\invertedradius%
			\pgf@yc\halfheight%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\invertedradius}%			
					}%
				\fi%
			\repeatpgfmathloop%
		}%
	}
	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{and}}
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\dimensions%
		\pgfpointadd{\centerpoint}{\pgfpointborderrectangle{\externalpoint}{\pgfqpoint{\halfwidth}{\halfheight}}}%
	}%	
}





% Shape nand gate IEC
%
\pgfdeclareshape{nand gate IEC}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@nand gate IEC\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@nand gate IEC@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@nand gate IEC@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A nand gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{nand}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\inheritanchor[from=and gate IEC]{center}
	\inheritanchor[from=and gate IEC]{mid}
	\inheritanchor[from=and gate IEC]{mid west}
	\inheritanchor[from=and gate IEC]{mid east}
	\inheritanchor[from=and gate IEC]{base}
	\inheritanchor[from=and gate IEC]{base west}
	\inheritanchor[from=and gate IEC]{base east}
	\inheritanchor[from=and gate IEC]{north}
	\inheritanchor[from=and gate IEC]{south}
	\inheritanchor[from=and gate IEC]{east}
	\inheritanchor[from=and gate IEC]{west}
	\inheritanchor[from=and gate IEC]{north east}
	\inheritanchor[from=and gate IEC]{north west}
	\inheritanchor[from=and gate IEC]{south east}
	\inheritanchor[from=and gate IEC]{south west}
	\anchor{output}{%
		\csname pgf@anchor@and gate IEC@east\endcsname%
		\advance\pgf@x\invertedradius%
		\advance\pgf@x\outerinvertedradius%
	}
	\backgroundpath{%
		\csname pgf@sh@bg@and gate IEC\endcsname%
		\pgfpathcircle{%
			\centerpoint%
			\advance\pgf@x\halfwidth%
			\advance\pgf@x\invertedradius%
		}{+\invertedradius}%
	}
	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{nand}}
	\inheritanchorborder[from=and gate IEC]
}





% Shape or gate IEC
%
\pgfdeclareshape{or gate IEC}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@or gate IEC\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@or gate IEC@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@or gate IEC@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{An or gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{or}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\inheritanchor[from=and gate IEC]{center}
	\inheritanchor[from=and gate IEC]{mid}
	\inheritanchor[from=and gate IEC]{mid west}
	\inheritanchor[from=and gate IEC]{mid east}
	\inheritanchor[from=and gate IEC]{base}
	\inheritanchor[from=and gate IEC]{base west}
	\inheritanchor[from=and gate IEC]{base east}
	\inheritanchor[from=and gate IEC]{north}
	\inheritanchor[from=and gate IEC]{south}
	\inheritanchor[from=and gate IEC]{east}
	\inheritanchor[from=and gate IEC]{west}
	\inheritanchor[from=and gate IEC]{north east}
	\inheritanchor[from=and gate IEC]{north west}
	\inheritanchor[from=and gate IEC]{south east}
	\inheritanchor[from=and gate IEC]{south west}
	\inheritanchor[from=and gate IEC]{output}
	\inheritbackgroundpath[from=and gate IEC]
	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{or}}
	\inheritanchorborder[from=and gate IEC]
}





% Shape nor gate IEC
%
\pgfdeclareshape{nor gate IEC}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@nor gate IEC\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@nor gate IEC@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@nor gate IEC@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A nor gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{nor}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\inheritanchor[from=and gate IEC]{center}
	\inheritanchor[from=and gate IEC]{mid}
	\inheritanchor[from=and gate IEC]{mid west}
	\inheritanchor[from=and gate IEC]{mid east}
	\inheritanchor[from=and gate IEC]{base}
	\inheritanchor[from=and gate IEC]{base west}
	\inheritanchor[from=and gate IEC]{base east}
	\inheritanchor[from=and gate IEC]{north}
	\inheritanchor[from=and gate IEC]{south}
	\inheritanchor[from=and gate IEC]{east}
	\inheritanchor[from=and gate IEC]{west}
	\inheritanchor[from=and gate IEC]{north east}
	\inheritanchor[from=and gate IEC]{north west}
	\inheritanchor[from=and gate IEC]{south east}
	\inheritanchor[from=and gate IEC]{south west}
	\inheritanchor[from=nand gate IEC]{output}%
	\inheritbackgroundpath[from=nand gate IEC]
	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{nor}}
	\inheritanchorborder[from=and gate IEC]
}





% Shape xor gate IEC
%
\pgfdeclareshape{xor gate IEC}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@xor gate IEC\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{2}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@xor gate IEC@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@xor gate IEC@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{An xor gate must have two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{xor}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\inheritanchor[from=and gate IEC]{center}
	\inheritanchor[from=and gate IEC]{mid}
	\inheritanchor[from=and gate IEC]{mid west}
	\inheritanchor[from=and gate IEC]{mid east}
	\inheritanchor[from=and gate IEC]{base}
	\inheritanchor[from=and gate IEC]{base west}
	\inheritanchor[from=and gate IEC]{base east}
	\inheritanchor[from=and gate IEC]{north}
	\inheritanchor[from=and gate IEC]{south}
	\inheritanchor[from=and gate IEC]{east}
	\inheritanchor[from=and gate IEC]{west}
	\inheritanchor[from=and gate IEC]{north east}
	\inheritanchor[from=and gate IEC]{north west}
	\inheritanchor[from=and gate IEC]{south east}
	\inheritanchor[from=and gate IEC]{south west}
	\inheritanchor[from=and gate IEC]{output}
	\inheritbackgroundpath[from=and gate IEC]
	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{xor}}
	\inheritanchorborder[from=and gate IEC]
}




% Shape xnor gate IEC
%

\pgfdeclareshape{xnor gate IEC}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@xnor gate IEC\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@xnor gate IEC@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@xnor gate IEC@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@IEC@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A xnor gate must have two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{xnor}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\inheritanchor[from=and gate IEC]{center}
	\inheritanchor[from=and gate IEC]{mid}
	\inheritanchor[from=and gate IEC]{mid west}
	\inheritanchor[from=and gate IEC]{mid east}
	\inheritanchor[from=and gate IEC]{base}
	\inheritanchor[from=and gate IEC]{base west}
	\inheritanchor[from=and gate IEC]{base east}
	\inheritanchor[from=and gate IEC]{north}
	\inheritanchor[from=and gate IEC]{south}
	\inheritanchor[from=and gate IEC]{east}
	\inheritanchor[from=and gate IEC]{west}
	\inheritanchor[from=and gate IEC]{north east}
	\inheritanchor[from=and gate IEC]{north west}
	\inheritanchor[from=and gate IEC]{south east}
	\inheritanchor[from=and gate IEC]{south west}
	\inheritanchor[from=nand gate IEC]{output}
	\inheritbackgroundpath[from=nand gate IEC]
	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{xnor}}
	\inheritanchorborder[from=and gate IEC]
}




% Shape buffer gate IEC
%
\pgfdeclareshape{buffer gate IEC}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@buffer gate IEC\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1}% Maximum 1 input.
		%
		\expandafter\gdef\csname pgf@anchor@buffer gate IEC@input\endcsname{%
			\pgf@lib@sh@logicgate@IEC@inputanchor{1}%
		}%
		\ifnum\pgf@lib@sh@logicgate@numinputs=0\relax%
			\PackageError{PGF}{A buffer gate must have one inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{xor}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\inheritanchor[from=and gate IEC]{center}
	\inheritanchor[from=and gate IEC]{mid}
	\inheritanchor[from=and gate IEC]{mid west}
	\inheritanchor[from=and gate IEC]{mid east}
	\inheritanchor[from=and gate IEC]{base}
	\inheritanchor[from=and gate IEC]{base west}
	\inheritanchor[from=and gate IEC]{base east}
	\inheritanchor[from=and gate IEC]{north}
	\inheritanchor[from=and gate IEC]{south}
	\inheritanchor[from=and gate IEC]{east}
	\inheritanchor[from=and gate IEC]{west}
	\inheritanchor[from=and gate IEC]{north east}
	\inheritanchor[from=and gate IEC]{north west}
	\inheritanchor[from=and gate IEC]{south east}
	\inheritanchor[from=and gate IEC]{south west}
	\inheritanchor[from=and gate IEC]{output}
	\inheritbackgroundpath[from=and gate IEC]
	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{buffer}}
	\inheritanchorborder[from=and gate IEC]
}





% Shape not gate IEC
%
\pgfdeclareshape{not gate IEC}{
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@not gate IEC\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1}%
		%
		\pgfutil@ifundefined{pgf@anchor@not gate IEC@input}{%
			\expandafter\gdef\csname pgf@anchor@not gate IEC@input\endcsname{%
					\pgf@lib@sh@logicgate@IEC@inputanchor{1}%
				}}{}%
		\ifnum\pgf@lib@sh@logicgate@numinputs=0\relax%
			\PackageError{PGF}{A not gate must have one input}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{%
		\pgf@lib@sh@logicgates@dimensions@IEC{not}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\inheritanchor[from=and gate IEC]{center}
	\inheritanchor[from=and gate IEC]{mid}
	\inheritanchor[from=and gate IEC]{mid west}
	\inheritanchor[from=and gate IEC]{mid east}
	\inheritanchor[from=and gate IEC]{base}
	\inheritanchor[from=and gate IEC]{base west}
	\inheritanchor[from=and gate IEC]{base east}
	\inheritanchor[from=and gate IEC]{north}
	\inheritanchor[from=and gate IEC]{south}
	\inheritanchor[from=and gate IEC]{east}
	\inheritanchor[from=and gate IEC]{west}
	\inheritanchor[from=and gate IEC]{north east}
	\inheritanchor[from=and gate IEC]{north west}
	\inheritanchor[from=and gate IEC]{south east}
	\inheritanchor[from=and gate IEC]{south west}
	\inheritanchor[from=nand gate IEC]{output}
	\inheritbackgroundpath[from=nand gate IEC]
	\foregroundpath{\pgf@lib@sh@logicgates@IEC@foregroundpath{not}}
	\inheritanchorborder[from=and gate IEC]
}

\endinput

==> pgflibraryshapes.gates.logic.US.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\newif\ifpgfgateanchorsuseboundingrectangle%


% Keys for US/CDH logic gates.
%
\pgfkeys{/pgf/.cd,%
	logic gate input sep/.initial=0.125cm,
	logic gate inputs/.initial={normal,normal},%
	logic gate inverted radius/.initial=2pt,%
	logic gate anchors use bounding box/.is if=pgfgateanchorsuseboundingrectangle,%
}

% An internal macro for calculating internal dimensions of 
% the US + CDH gates (excluding and gate US and nand gate US).
%
\def\pgf@lib@sh@logicgates@dimensions@orUS{%
	\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
	\advance\pgf@x.5\wd\pgfnodeparttextbox%
	\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
	\advance\pgf@y.5\ht\pgfnodeparttextbox%
	\advance\pgf@y.5\dp\pgfnodeparttextbox%
	%
	% Adjust the height for the number of inputs.
	%
	\c@pgf@counta\pgf@lib@sh@logicgate@numinputs%
	\advance\c@pgf@counta1\relax%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	\advance\pgf@ya\pgflinewidth%
	\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/logic gate input sep}}%
	\pgf@yb.5\pgf@yb%
	\ifdim\pgf@ya<\pgf@yb%
		\pgf@ya\pgf@yb%
	\fi%	
	\multiply\pgf@ya\c@pgf@counta%
	\ifdim\pgf@y<\pgf@ya%
		\pgf@y\pgf@ya%
	\fi%
	%
	\ifdim\pgf@x>\pgf@y%
		\pgf@y\pgf@x%
	\else%
		\pgf@x\pgf@y%
	\fi%
	%
	% Adjust for minimum height and width.
	%
	\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
	\ifdim\pgf@y<.5\pgf@ya%
		\pgf@y.5\pgf@ya%
	\fi%
	\pgf@xb\pgf@x%
	\advance\pgf@xb1.732051\pgf@y% 2y*cos(30)
	\ifdim\pgf@xb<\pgf@xa%
		\pgf@xb\pgf@xa%
		\pgf@x0.366025\pgf@xb% xb / (1 + 2*cos(30))
	\fi%
	%
	\ifdim\pgf@x>\pgf@y%
		\pgf@y\pgf@x%
	\else%
		\pgf@x\pgf@y%
	\fi%
	\edef\halfside{\the\pgf@x}%
	\addtosavedmacro\halfside%
	%
	% Take into account the outer sep.
	%
	\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
	\edef\outerxsep{\the\pgf@xa}%
	\edef\outerysep{\the\pgf@ya}%
	\addtosavedmacro\outerxsep%
	\addtosavedmacro\outerysep%
	\advance\pgf@x\pgf@xa%
	\advance\pgf@y\pgf@ya%
	%
	\edef\halfwidth{\the\pgf@x}%
	\edef\halfheight{\the\pgf@y}%
	\addtosavedmacro\halfwidth%
	\addtosavedmacro\halfheight%
	%
	\pgfextract@process\tipanchor{%
		\advance\pgf@x-\pgf@xa%
		\advance\pgf@y-\pgf@ya%	
		\pgf@x-.16666\pgf@x%
		\pgf@yb2.0\pgf@y%
		\advance\pgf@x.866025\pgf@yb%	
		\advance\pgf@x1.154701\pgf@xa%
		\pgf@y0pt%
	}%
	\addtosavedmacro\tipanchor%		
}%


% An internal macro for calculating internal dimensions of 
% the and gate US and nand gate US.
%
\def\pgf@lib@sh@logicgates@dimensions@andUS{%
	\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
	\advance\pgf@x.5\wd\pgfnodeparttextbox%
	\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
	\advance\pgf@y.5\ht\pgfnodeparttextbox%
	\advance\pgf@y.5\dp\pgfnodeparttextbox%
	%
	% Adjust the height for the number of inputs.
	%
	\c@pgf@counta\pgf@lib@sh@logicgate@numinputs%
	\advance\c@pgf@counta1\relax%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	\advance\pgf@ya\pgflinewidth%
	\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/logic gate input sep}}%
	\pgf@yb.5\pgf@yb%
	\ifdim\pgf@ya<\pgf@yb%
		\pgf@ya\pgf@yb%
	\fi%	
	\multiply\pgf@ya\c@pgf@counta%
	\ifdim\pgf@y<\pgf@ya%
		\pgf@y\pgf@ya%
	\fi%
	%
	\ifdim\pgf@x>\pgf@y%
		\pgf@y\pgf@x%
	\else%
		\pgf@x\pgf@y%
	\fi%
	%
	% Adjust for minimum height and width.
	%
	\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
	\ifdim\pgf@y<.5\pgf@ya%
		\pgf@y.5\pgf@ya%
	\fi%
	\pgf@xb2.5\pgf@x%
	\ifdim\pgf@xb<\pgf@xa%
		\pgf@xb\pgf@xa%
		\pgf@x0.4\pgf@xb% 
	\fi% 
	%
	\ifdim\pgf@x>\pgf@y%
		\pgf@y\pgf@x%
	\else%
		\pgf@x\pgf@y%
	\fi%
	\edef\halfside{\the\pgf@x}%
	\addtosavedmacro\halfside%
	%
	% Take into account the outer sep.
	%
	\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
	\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
	\edef\outerxsep{\the\pgf@xa}%
	\edef\outerysep{\the\pgf@ya}%
	\addtosavedmacro\outerxsep%
	\addtosavedmacro\outerysep%
	\advance\pgf@x\pgf@xa%
	\advance\pgf@y\pgf@ya%
	%
	\edef\halfwidth{\the\pgf@x}%
	\edef\halfheight{\the\pgf@y}%
	\addtosavedmacro\halfwidth%
	\addtosavedmacro\halfheight%
	%
}%


% Internal macro for parsing inputs.
%
\expandafter\ifx\csname pgf@lib@sh@logicgate@parseinputs\endcsname\relax%
\def\pgf@lib@sh@logicgate@parseinputs#1{%
	\edef\pgf@lib@sh@temp{\pgfkeysvalueof{/pgf/logic gate inputs}}%
	\c@pgf@counta#1\relax%
	\c@pgf@countb0\relax%
	\expandafter\pgfutil@in@\expandafter,\expandafter{\pgf@lib@sh@temp}%
	\ifpgfutil@in@%
		\let\pgf@lib@sh@next\pgf@lib@sh@logicgate@parseinputs@long%
	\else%
		\let\pgf@lib@sh@next\pgf@lib@sh@logicgate@parseinputs@short%
	\fi%
	\pgf@lib@sh@next%
}	
\def\pgf@lib@sh@itext{i}
\def\pgf@lib@sh@invertedtext{inverted}
%
%	The `short' version for input specifcation is an extension of
%	ideas due to Juergen Werber and Christoph Bartoschek.
%
\def\pgf@lib@sh@logicgate@parseinputs@short{%
	\expandafter\pgf@lib@sh@logicgate@parseinputs@@short\pgf@lib@sh@temp\pgf@stop%
}
\def\pgf@lib@sh@logicgate@parseinputs@@short#1{%
	\ifx#1\pgf@stop%
		\edef\pgf@lib@sh@logicgate@numinputs{\the\c@pgf@countb}%
		\let\pgf@lib@sh@next\relax%
	\else%
		\ifnum\c@pgf@countb=\c@pgf@counta%
			\edef\pgf@lib@sh@logicgate@numinputs{\the\c@pgf@countb}%
			\let\pgf@lib@sh@next\relax%
		\else%
			\advance\c@pgf@countb1\relax%
			\expandafter\ifx\pgf@lib@sh@itext#1%
				\expandafter\pgf@sh@resavedmacro\expandafter{\csname input-\the\c@pgf@countb\endcsname}{%
					\expandafter\def\csname input-\the\c@pgf@countb\endcsname{i}}%
			\else%
				\expandafter\pgf@sh@resavedmacro\expandafter{\csname input-\the\c@pgf@countb\endcsname}{%
					\expandafter\def\csname input-\the\c@pgf@countb\endcsname{n}}%
			\fi%		
			\let\pgf@lib@sh@next\pgf@lib@sh@logicgate@parseinputs@@short%
		\fi%
	\fi%
	\pgf@lib@sh@next%
}
\def\pgf@lib@sh@logicgate@parseinputs@long{%
	\expandafter\pgf@lib@sh@logicgate@parseinputs@@long\pgf@lib@sh@temp,\pgf@stop,%
}
\def\pgf@lib@sh@logicgate@parseinputs@@long#1,{%
	\ifx#1\pgf@stop%
		\edef\pgf@lib@sh@logicgate@numinputs{\the\c@pgf@countb}%
		\let\pgf@lib@sh@next\relax%
	\else%
		\ifnum\c@pgf@countb=\c@pgf@counta%
			\edef\pgf@lib@sh@logicgate@numinputs{\the\c@pgf@countb}%
			\let\pgf@lib@sh@next\relax%
		\else%
			\advance\c@pgf@countb1\relax%
			\def\pgf@lib@sh@temp{#1}%
			\ifx\pgf@lib@sh@invertedtext\pgf@lib@sh@temp%
				\expandafter\pgf@sh@resavedmacro\expandafter{\csname input-\the\c@pgf@countb\endcsname}{%
					\expandafter\def\csname input-\the\c@pgf@countb\endcsname{i}}%
			\else%
				\expandafter\pgf@sh@resavedmacro\expandafter{\csname input-\the\c@pgf@countb\endcsname}{%
					\expandafter\def\csname input-\the\c@pgf@countb\endcsname{n}}%
			\fi%		
			\let\pgf@lib@sh@next\pgf@lib@sh@logicgate@parseinputs@@@long%
		\fi%
	\fi%
	\pgf@lib@sh@next%
}
\def\pgf@lib@sh@logicgate@parseinputs@@@long{%
	\pgfutil@ifnextchar x{\pgf@lib@sh@logicgate@parseinputs@@long}%
		{\pgf@lib@sh@logicgate@parseinputs@@long}%
}
\fi%

% Internal macro for calculation input anchors. Used by
% both and gates and nand gates, and also the not gate and buffer.
%
\def\pgf@lib@sh@logicgate@AND@inputanchor#1{%
	\dimensions%
	\centerpoint%
	\pgf@xa\halfside%
	\advance\pgf@x-.166666\pgf@xa%
	\advance\pgf@x-\halfwidth%
	\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-#1\endcsname%
		\advance\pgf@x-\invertedradius%
		\advance\pgf@x-\outerinvertedradius%
	\fi%
	%
	\pgfutil@tempdima\halfside%
	\multiply\pgfutil@tempdima2\relax%
	\c@pgf@counta\numinputs%
	\advance\c@pgf@counta1\relax%
	\divide\pgfutil@tempdima\c@pgf@counta%
	\multiply\pgfutil@tempdima#1\relax%
	\advance\pgf@y\halfside%
	\advance\pgf@y-\pgfutil@tempdima%
}




% Shape and gate US
%
\pgfdeclareshape{and gate US}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@and gate US\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@and gate US@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@and gate US@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@AND@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{An and gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@andUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\csname pgf@anchor@and gate US@east\endcsname%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa}
	\anchor{mid west}{%
		\csname pgf@anchor@and gate US@west\endcsname%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa}
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\csname pgf@anchor@and gate US@east\endcsname%
		\pgf@xa\pgf@x%
		\basepoint%
		\pgf@x\pgf@xa}
	\anchor{base west}{%
		\csname pgf@anchor@and gate US@west\endcsname%
		\pgf@xa\pgf@x%
		\basepoint%
		\pgf@x\pgf@xa}
	\anchor{east}{%
		\dimensions%
		\pgf@xa\halfwidth%
		\pgf@xb\pgf@xa%
		\advance\pgf@xb-\outerxsep%
		\centerpoint%
		\advance\pgf@x.333333\pgf@xb%
		\advance\pgf@x\pgf@xa%
	}
	\anchor{output}{\csname pgf@anchor@and gate US@east\endcsname}
	\anchor{north east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@nand gate US@east\endcsname%
			\advance\pgf@y\halfheight%
		\else
			\pgf@xa\halfwidth%
			\pgf@ya\halfheight%
			\pgf@xb\pgf@xa%
			\advance\pgf@xb-\outerxsep%
			\centerpoint%
			\advance\pgf@x.333333\pgf@xb%
			\advance\pgf@x.707106\pgf@xa%
			\advance\pgf@y.707106\pgf@ya%
		\fi%
	}
	\anchor{south east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@nand gate US@east\endcsname%
			\advance\pgf@y-\halfheight%
		\else
			\pgf@xa\halfwidth%
			\pgf@ya\halfheight%
			\pgf@xb\pgf@xa%
			\advance\pgf@xb-\outerxsep%
			\centerpoint%
			\advance\pgf@x.333333\pgf@xb%
			\advance\pgf@x.707106\pgf@xa%
			\advance\pgf@y-.707106\pgf@ya%
		\fi%
	}
	\anchor{north}{%
		\dimensions%
		\centerpoint%
		\advance\pgf@y\halfheight%		
	}
	\anchor{south}{%
		\dimensions%
		\centerpoint%
		\advance\pgf@y-\halfheight%
	}
	\anchor{south west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\advance\pgf@x-1.16666\pgf@xa%
		\advance\pgf@x-\outerxsep%
		\advance\pgf@y-\halfheight%
	}
	\anchor{north west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\advance\pgf@x-1.16666\pgf@xa%
		\advance\pgf@x-\outerxsep%
		\advance\pgf@y\halfheight%
	}
	\anchor{west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\advance\pgf@x-1.16666\pgf@xa%
		\advance\pgf@x-\outerxsep%
	}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		\pgf@xb.333333\pgf@xc%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yc}}%
			{%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{90}{-90}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{-\pgf@yc}}%
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{\pgf@yc}}%
			\pgfpathclose%
			%
			% Draw the inputs.
			%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{%
							\pgf@xa\halfside%
							\pgf@x-1.16666\pgf@xa%
							\advance\pgf@x-.5\pgflinewidth%
							\advance\pgf@x-\invertedradius%
							\pgf@y\pgf@yc%
						}{+\invertedradius}%				
					}%
				\fi%				
			\repeatpgfmathloop%
		}%
	}%
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\pgfextract@process\externalpoint{\pgfpointadd{\centerpoint}{\externalpoint}}%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\let\externalangle\pgfmathresult%
		\dimensions%
		\pgf@xb\halfside%
		\pgf@xc1.66666\pgf@xb%
		\advance\pgf@xc\outerxsep%
		\pgf@yc\halfheight%
		\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@and gate US@north west\endcsname}%
		\ifdim\externalangle pt<\pgfmathresult pt\relax%
			\pgfmathanglebetweenpoints{\centerpoint}{\centerpoint\advance\pgf@x.333333\pgf@xb\advance\pgf@y\pgf@yc}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
					{%
						\centerpoint%
						\advance\pgf@x.333333\pgf@xb%	
					}%
					{0}{90}{+\halfwidth and +\halfheight}%
			\else%
				\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
					{\centerpoint\advance\pgf@x.333333\pgf@xb\advance\pgf@y\pgf@yc}%
					{\centerpoint\advance\pgf@x-\pgf@xc\advance\pgf@y\pgf@yc}%			
			\fi%
		\else%
			\pgfmathanglebetweenpoints{\centerpoint}{\centerpoint\advance\pgf@x.333333\pgf@xb\advance\pgf@y-\pgf@yc}%
			\ifdim\externalangle pt>\pgfmathresult pt\relax%
					\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
					{%
						\centerpoint%
						\advance\pgf@x.333333\pgf@xb%		
					}%
					{270}{360}{+\halfwidth and +\halfheight}%
			\else%
				\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@and gate US@south west\endcsname}%
				\ifdim\externalangle pt>\pgfmathresult pt\relax%
					\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
						{\centerpoint\advance\pgf@x.333333\pgf@xb\advance\pgf@y-\pgf@yc}%
						{\csname pgf@anchor@and gate US@south west\endcsname}%	
				\else%
					\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
						{\csname pgf@anchor@and gate US@north west\endcsname}%
						{\csname pgf@anchor@and gate US@south west\endcsname}%
				\fi%
			\fi%
		\fi%
	}
}





% Shape nand gate US
%
\pgfdeclareshape{nand gate US}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@nand gate US\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@nand gate US@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@nand gate US@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@AND@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A nand gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@andUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\inheritanchor[from=and gate US]{mid}
	\inheritanchor[from=and gate US]{mid east}
	\inheritanchor[from=and gate US]{mid west}
	\inheritanchor[from=and gate US]{base}
	\inheritanchor[from=and gate US]{base east}
	\inheritanchor[from=and gate US]{base west}
	\anchor{output}{%
		\dimensions
		\pgfpointadd{\centerpoint}{%
			\pgf@xa\halfside%
			\pgf@x1.33333\pgf@xa%
			\advance\pgf@x\invertedradius%
			\advance\pgf@x\outerinvertedradius%
			\advance\pgf@x\outerxsep%
			\pgf@y0pt%
		}%
	}
	\inheritanchor[from=and gate US]{east}
	\inheritanchor[from=and gate US]{north east}
	\inheritanchor[from=and gate US]{south east}
	\inheritanchor[from=and gate US]{north}
	\inheritanchor[from=and gate US]{south}
	\inheritanchor[from=and gate US]{south west}
	\inheritanchor[from=and gate US]{north west}
	\inheritanchor[from=and gate US]{west}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		\pgf@xb.333333\pgf@xc%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yc}}%
			{%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{90}{-90}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{-\pgf@yc}}%
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{\pgf@yc}}%
			\pgfpathclose%
			%
			% Draw the inputs.
			%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{%
							\pgf@xa\halfside%
							\pgf@x-1.166666\pgf@xa%
							\advance\pgf@x-.5\pgflinewidth%
							\advance\pgf@x-\invertedradius%
							\pgf@y\pgf@yc%
						}{+\invertedradius}%				
					}%
				\fi%				
			\repeatpgfmathloop%
			%
			% Draw the output inverter.
			%
			{%
				\pgfpathcircle{%
					\pgf@x1.33333\pgf@xc%
					\advance\pgf@x\outerinvertedradius%
					\pgf@y0pt%
				}{+\invertedradius}%			
			}%
		}%
	}		
	\inheritanchorborder[from=and gate US]
}


% Internal macro for calculation input anchors. Used by
% or, nor xnor gates (US).
%
\def\pgf@lib@sh@logicgate@OR@inputanchor#1{%
	\dimensions%
	\pgf@ya\halfside%
	\pgf@yb2.0\pgf@ya%
	%
	\pgfutil@tempdima\halfside%
	\multiply\pgfutil@tempdima2\relax%
	\c@pgf@counta\numinputs%
	\advance\c@pgf@counta1\relax%
	\divide\pgfutil@tempdima\c@pgf@counta%
	\multiply\pgfutil@tempdima#1\relax%
	\pgf@yc\pgf@ya%
	\advance\pgf@yc-\pgfutil@tempdima%
	%
	\pgf@xb\pgf@yb%
	\advance\pgf@yb-\halflinewidth%
	\pgfmathdivide@{\pgfmath@tonumber{\pgf@yc}}{\pgfmath@tonumber{\pgf@yb}}%
	\pgfmathasin@{\pgfmathresult}%
	\pgfmathcos@{\pgfmathresult}%
	%
	\pgf@xc-1.166666\pgf@ya%
	\advance\pgf@xc-.866025\pgf@xb%
	\advance\pgf@xc\pgfmathresult\pgf@yb%
	\advance\pgf@xc\halflinewidth%
	\advance\pgf@xc-\outerxsep%
	%
	\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-#1\endcsname%
		\advance\pgf@xc-\invertedradius%
		\advance\pgf@xc-\outerinvertedradius%
	\fi%
	%
	\centerpoint%
	\advance\pgf@x\pgf@xc%
	\advance\pgf@y\pgf@yc%
}


% Shape or gate US
%
\pgfdeclareshape{or gate US}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@or gate US\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@or gate US@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@or gate US@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@OR@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{An or gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\halflinewidth{%
		\pgf@x.5\pgflinewidth%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\csname pgf@anchor@or gate US@east\endcsname%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa}
	\anchor{mid west}{%
		\csname pgf@anchor@or gate US@north west\endcsname%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa}
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\csname pgf@anchor@or gate US@east\endcsname%
		\pgf@xa\pgf@x%
		\basepoint%
		\pgf@x\pgf@xa}
	\anchor{base west}{%
		\csname pgf@anchor@or gate US@north west\endcsname%
		\pgf@xa\pgf@x%
		\basepoint%
		\pgf@x\pgf@xa}
	\anchor{east}{%
		\dimensions%
		\pgfpointadd{\centerpoint}{\tipanchor}%
	}
	\anchor{output}{\csname pgf@anchor@or gate US@east\endcsname}
	\anchor{north east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\tipanchor%
			\pgf@xa\pgf@x%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\halfheight%
		\else%
			\centerpoint%
			\pgf@xa\halfwidth%
			\pgf@ya\halfheight%
			\pgf@xb\halfside%
			\advance\pgf@x-.166666\pgf@xb%
			\advance\pgf@xa\pgf@xb%
			\advance\pgf@x.5\pgf@xa%
			\advance\pgf@y-\pgf@xb%
			\advance\pgf@ya\pgf@xb%
			\advance\pgf@y.866025\pgf@ya%
		\fi%
	}
	\anchor{south east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\tipanchor%
			\pgf@xa\pgf@x%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y-\halfheight%
		\else
			\centerpoint%
			\pgf@xa\halfwidth%
			\pgf@ya\halfheight%
			\pgf@xb\halfside%
			\advance\pgf@x-.166666\pgf@xb%
			\advance\pgf@xa\pgf@xb%
			\advance\pgf@x.5\pgf@xa%
			\advance\pgf@y\pgf@xb%
			\advance\pgf@ya\pgf@xb%
			\advance\pgf@y-.866025\pgf@ya%
		\fi%
	}
	\anchor{north}{%
		\dimensions%
		\centerpoint%
		\ifpgfgateanchorsuseboundingrectangle%
			\advance\pgf@y\halfheight%
		\else%
			\pgf@ya\halfheight%
			\advance\pgf@y.993043\pgf@ya%
		\fi%	
	}
	\anchor{south}{%
		\dimensions%
		\centerpoint%
		\ifpgfgateanchorsuseboundingrectangle%
			\advance\pgf@y-\halfheight%
		\else%
			\pgf@ya\halfheight%
			\advance\pgf@y-.993043\pgf@ya%
		\fi%	
	}
	\anchor{south west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\advance\pgf@x-1.16666\pgf@xa%
		\pgf@xa\outerxsep%
		\advance\pgf@x-1.732050\pgf@xa%
		\advance\pgf@y-\halfheight%
	}
	\anchor{north west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\advance\pgf@x-1.16666\pgf@xa%
		\pgf@xa\outerxsep%
		\advance\pgf@x-1.732050\pgf@xa%
		\advance\pgf@y\halfheight%
	}
	\anchor{west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\ifpgfgateanchorsuseboundingrectangle%			
			\advance\pgf@x-1.16666\pgf@xa%
			\advance\pgf@x-\outerxsep%
		\else%
			\advance\pgf@x-1.16666\pgf@xa%
			\advance\pgf@x-\outerxsep%
			\advance\pgf@x0.267949\pgf@xa%
		\fi%
	}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{-.16666\pgf@xc}{\pgf@yc}}%
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{90}{30}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{-30}{-90}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{-\pgf@yc}}%
			{%
				\pgf@yc2.0\pgf@yc%
				\pgfpatharc{-30}{0}{+\pgf@yc}%			
			}
			{%
				\pgf@yc2.0\pgf@yc%
				\pgfpatharc{0}{30}{+\pgf@yc}%			
			}%
			\pgfpathclose%
			%
			% Draw the inputs.
			%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{%
							\pgf@ya\halfside%
							\pgf@yb2.0\pgf@ya%
							\pgf@xa\pgf@yb%
							\advance\pgf@yb-\halflinewidth%
							\pgfmathdivide@{\pgfmath@tonumber{\pgf@yc}}{\pgfmath@tonumber{\pgf@yb}}%
							\let\sineangle\pgfmathresult%
							\pgfmathasin@{\pgfmathresult}%
							\pgfmathcos@{\pgfmathresult}%
							%
							\pgf@x-1.166666\pgf@ya%
							\advance\pgf@x-.866025\pgf@xa%
							\advance\pgf@x\pgfmathresult\pgf@yb%
							\advance\pgf@x-\invertedradius%
							\pgf@y\pgf@yc%
						}{+\invertedradius}%				
					}%
				\fi%				
			\repeatpgfmathloop%
		}%
	}%
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\pgfextract@process\externalpoint{\pgfpointadd{\centerpoint}{\externalpoint}}%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\centerpoint%
		\pgf@xb\pgf@x%
		\pgf@yb\pgf@y%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\let\externalangle\pgfmathresult%
		\dimensions%
		\pgf@xc\halfside%
		%
		\pgf@xc-.166666\pgf@xc%
		\ifdim\pgf@xa<\pgf@xc%
			\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@or gate US@north west\endcsname}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
					{%
						\pgfgateanchorsuseboundingrectangletrue%
						\csname pgf@anchor@or gate US@north\endcsname%
					}%
					{\csname pgf@anchor@or gate US@north west\endcsname}%
			\else%
				\pgfmathsubtract@{360}{\pgfmathresult}%
				\ifdim\externalangle pt>\pgfmathresult pt\relax%
					\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
					{%
						\pgfgateanchorsuseboundingrectangletrue%
						\csname pgf@anchor@or gate US@south\endcsname%
					}%
					{\csname pgf@anchor@or gate US@south west\endcsname}%
				\else%
					\ifdim\pgf@ya>\pgf@yb%
						\pgf@yc\halfheight%
						\advance\pgf@yc\halfside%
						\advance\pgf@yc-\outerxsep%
						\pgfextract@process\point{%
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
							{%
								\centerpoint%
								\pgf@xa\halfside%
								\advance\pgf@x-1.166666\pgf@xa%
								\pgf@xa2.0\pgf@xa%
								\advance\pgf@x-.866025\pgf@xa%
								\advance\pgf@x-\outerxsep%
							}%
							{0}{90}{+\pgf@yc}%
						}%
					\else%
						\pgf@yc\halfheight%
						\advance\pgf@yc\halfside%
						\advance\pgf@yc-\outerxsep%
						\pgfextract@process\point{%
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
							{%
								\centerpoint%
								\pgf@xa\halfside%
								\advance\pgf@x-1.166666\pgf@xa%
								\pgf@xa2.0\pgf@xa%
								\advance\pgf@x-.866025\pgf@xa%
								\advance\pgf@x-\outerxsep%
							}%
							{270}{360}{+\pgf@yc}%
						}%
					\fi%
				\fi%
			\fi%
		\else%
			\ifdim\pgf@y=0pt\relax%
				\csname pgf@anchor@and gate US@east\endcsname%
			\else%
				\pgf@xc\halfwidth%
				\advance\pgf@xc\halfside%
				\pgf@yc\halfheight%
				\advance\pgf@yc\halfside%
				\pgf@xb\halfside%
				\pgf@xb-.166666\pgf@xb%
				\ifdim\pgf@ya<0pt%
					\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
					{%
						\centerpoint%
						\advance\pgf@y\halfside%	
						\advance\pgf@x\pgf@xb%		
					}%
					{270}{330}{+\pgf@yc}%
				\else%
					\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
					{%
						\centerpoint%
						\advance\pgf@y-\halfside%	
						\advance\pgf@x\pgf@xb%
					}%
					{30}{90}{+\pgf@xc and +\pgf@yc}%
				\fi%
			\fi%
		\fi%
	}%
}




% Shape nor gate US
%
\pgfdeclareshape{nor gate US}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@nor gate US\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@nor gate US@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@nor gate US@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@OR@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A nor gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\halflinewidth{%
		\pgf@x.5\pgflinewidth%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\inheritanchor[from=or gate US]{center}
	\inheritanchor[from=or gate US]{mid}
	\inheritanchor[from=or gate US]{mid east}
	\inheritanchor[from=or gate US]{mid west}
	\inheritanchor[from=or gate US]{base}
	\inheritanchor[from=or gate US]{base east}
	\inheritanchor[from=or gate US]{base west}
	\inheritanchor[from=or gate US]{east}
	\inheritanchor[from=or gate US]{north east}
	\inheritanchor[from=or gate US]{south east}
	\inheritanchor[from=or gate US]{north}
	\inheritanchor[from=or gate US]{south}
	\inheritanchor[from=or gate US]{south west}
	\inheritanchor[from=or gate US]{north west}
	\inheritanchor[from=or gate US]{west}
	\anchor{output}{%
		\dimensions%
		\centerpoint%
		\pgf@xc\halfside%
		\pgf@yc\pgf@xc%
		\advance\pgf@x-.166666\pgf@xc%
		\pgf@yc2.0\pgf@yc%
		\advance\pgf@x.866025\pgf@yc%
		\advance\pgf@x\outerinvertedradius%
		\advance\pgf@x\invertedradius%
		\advance\pgf@x\outerxsep%
	}%
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{-.16666\pgf@xc}{\pgf@yc}}%
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{90}{30}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{-30}{-90}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{-\pgf@yc}}%
			{%
				\pgf@yc2.0\pgf@yc%
				\pgfpatharc{-30}{0}{+\pgf@yc}%			
			}
			{%
				\pgf@yc2.0\pgf@yc%
				\pgfpatharc{0}{30}{+\pgf@yc}%			
			}%
			\pgfpathclose%
			% Draw the output inverter.
			%
			{%
				\pgfpathcircle{%
					\pgf@x-.166666\pgf@xc%
					\pgf@yc2.0\pgf@yc%
					\advance\pgf@x.866025\pgf@yc%
					\advance\pgf@x\outerinvertedradius%
					\pgf@y0pt%
				}{+\invertedradius}%			
			}%
			%
			% Draw the inputs.
			%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{%
							\pgf@ya\halfside%
							\pgf@yb2.0\pgf@ya%
							\pgf@xa\pgf@yb%
							\advance\pgf@yb-\halflinewidth%
							\pgfmathdivide@{\pgfmath@tonumber{\pgf@yc}}{\pgfmath@tonumber{\pgf@yb}}%
							\let\sineangle\pgfmathresult%
							\pgfmathasin@{\pgfmathresult}%
							\pgfmathcos@{\pgfmathresult}%
							%
							\pgf@x-1.166666\pgf@ya%
							\advance\pgf@x-.866025\pgf@xa%
							\advance\pgf@x\pgfmathresult\pgf@yb%
							\advance\pgf@x-\invertedradius%
							\pgf@y\pgf@yc%
						}{+\invertedradius}%				
					}%
				\fi%				
			\repeatpgfmathloop%
		}%
	}%
	\inheritanchorborder[from=or gate US]
}



% Internal macro for calculation input anchors. Used by
% xor and xnor gates (US).
%
\def\pgf@lib@sh@logicgate@XOR@inputanchor#1{%
	\dimensions%
	\pgf@ya\halfside%
	\pgf@yb2.0\pgf@ya%
	%
	\pgfutil@tempdima\halfside%
	\multiply\pgfutil@tempdima2\relax%
	\c@pgf@counta\numinputs%
	\advance\c@pgf@counta1\relax%
	\divide\pgfutil@tempdima\c@pgf@counta%
	\multiply\pgfutil@tempdima#1\relax%
	\pgf@yc\pgf@ya%
	\advance\pgf@yc-\pgfutil@tempdima%
	%
	\pgf@xb\pgf@yb%
	\advance\pgf@yb-\halflinewidth%
	\pgfmathdivide@{\pgfmath@tonumber{\pgf@yc}}{\pgfmath@tonumber{\pgf@yb}}%
	\pgfmathasin@{\pgfmathresult}%
	\pgfmathcos@{\pgfmathresult}%
	%
	\pgf@xc-1.166666\pgf@ya%
	\advance\pgf@xc-.866025\pgf@xb%
	\advance\pgf@xc\pgfmathresult\pgf@yb%
	\advance\pgf@xc\halflinewidth%
	\advance\pgf@xc-\outerxsep%
	%
	\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-#1\endcsname%
		\advance\pgf@xc-\invertedradius%
		\advance\pgf@xc-\outerinvertedradius%
	\fi%
	%
	\centerpoint%
	\advance\pgf@x\pgf@xc%
	\advance\pgf@y\pgf@yc%
	\pgf@xa\halfside%
	\advance\pgf@x-.333333\pgf@xa%
}





% Shape xor gate US
%
\pgfdeclareshape{xor gate US}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@xor gate US\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{2}% 
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@xor gate US@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@xor gate US@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@XOR@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{An xor gate must have at two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\halflinewidth{%
		\pgf@x.5\pgflinewidth%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\inheritanchor[from=or gate US]{mid east}
	\anchor{mid west}{%
		\csname pgf@anchor@xor gate US@north west\endcsname%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa}
	\anchor{base}{\basepoint}%
	\inheritanchor[from=or gate US]{base east}
	\anchor{base west}{%
		\csname pgf@anchor@xor gate US@north west\endcsname%
		\pgf@xa\pgf@x%
		\basepoint%
		\pgf@x\pgf@xa}
	\inheritanchor[from=or gate US]{base}
	\inheritanchor[from=or gate US]{output}
	\inheritanchor[from=or gate US]{east}
	\inheritanchor[from=or gate US]{north east}
	\inheritanchor[from=or gate US]{south east}
	\inheritanchor[from=or gate US]{north}
	\inheritanchor[from=or gate US]{south}
	\anchor{south west}{%
		\dimensions%
		\pgf@xa\halfside%
		\pgf@xa-3.232051\pgf@xa% (7/6 + 2*cos(30) + 1/3) * x
		\pgf@xb\halfside%
		\pgf@xb2.0\pgf@xb%
		\advance\pgf@xb-\halflinewidth%
		\advance\pgf@xa.866025\pgf@xb%
		\pgf@ya.5\pgf@xb%
		\centerpoint%
		\advance\pgf@x\pgf@xa%
		\ifpgfgateanchorsuseboundingrectangle%
			\advance\pgf@y-\halfheight%
		\else%
			\advance\pgf@y-\pgf@ya%
		\fi%
	}
	\anchor{north west}{%
		\dimensions%
		\pgf@xa\halfside%
		\pgf@xa-3.232051\pgf@xa% (7/6 + 2*cos(30) + 1/3) * x
		\pgf@xb\halfside%
		\pgf@xb2.0\pgf@xb%
		\advance\pgf@xb-\halflinewidth%
		\advance\pgf@xa.866025\pgf@xb%
		\pgf@ya.5\pgf@xb%
		\centerpoint%
		\advance\pgf@x\pgf@xa%
		\ifpgfgateanchorsuseboundingrectangle%
			\advance\pgf@y\halfheight%
		\else%
			\advance\pgf@y\pgf@ya%
		\fi%
	}
	\anchor{west}{%
		\dimensions%
		\pgf@ya\halfside%
		\pgf@yb2.0\pgf@ya%
		%
		\pgf@xb\pgf@yb%
		\advance\pgf@yb-\halflinewidth%
		\pgfmathdivide@{0}{\pgfmath@tonumber{\pgf@yb}}%
		\pgfmathasin@{\pgfmathresult}%
		\pgfmathcos@{\pgfmathresult}%
		%
		\pgf@xc-1.166666\pgf@ya%
		\advance\pgf@xc-.866025\pgf@xb%
		\advance\pgf@xc\pgfmathresult\pgf@yb%
		\advance\pgf@xc\halflinewidth%
		\advance\pgf@xc-\outerxsep%
		%
		\centerpoint%
		\advance\pgf@x\pgf@xc%
		\pgf@xa\halfside%
		\advance\pgf@x-.333333\pgf@xa%
		\ifpgfgateanchorsuseboundingrectangle%
			\pgf@xa2.0\pgf@xa%
			\advance\pgf@x-0.133974\pgf@xa%
		\fi%
	}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{-.16666\pgf@xc}{\pgf@yc}}%
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{90}{30}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{-30}{-90}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{-\pgf@yc}}%
			{%
				\pgf@yc2.66666\pgf@yc%
				\pgfpatharc{-22}{0}{+1.166666\pgf@yc and +\pgf@yc}%			
			}
			{%
				\pgf@yc2.66666\pgf@yc%
				\pgfpatharc{0}{22}{+1.166666\pgf@yc and +\pgf@yc}%			
			}%
			\pgfpathclose%
			%
			% Draw the inputs.
			%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{%
							\pgf@ya\halfside%
							\pgf@yb2.0\pgf@ya%
							\pgf@xa\pgf@yb%
							\advance\pgf@yb-\halflinewidth%
							\pgfmathdivide@{\pgfmath@tonumber{\pgf@yc}}{\pgfmath@tonumber{\pgf@yb}}%
							\pgfmathasin@{\pgfmathresult}%
							\pgfmathcos@{\pgfmathresult}%
							%
							\pgf@x-1.5\pgf@ya%
							\advance\pgf@x-.866025\pgf@xa%
							\advance\pgf@x\pgfmathresult\pgf@yb%
							\advance\pgf@x-\invertedradius%
							\pgf@y\pgf@yc%
						}{+\invertedradius}%				
					}%
				\fi%				
			\repeatpgfmathloop%
			%
			% Now, some fooling around to stop the `tail' being filled.
			% Technically it still is, but it isn't visible.
			%
			\pgf@xc\halfside%
			\pgf@yc\halfside%
			\pgfpathmoveto{\pgfqpoint{-1.5\pgf@xc}{-\pgf@yc}}%
			\pgf@yc2.0\pgf@yc%
			\pgfmathloop%
			\ifnum\pgfmathcounter<61\relax%
				{%
					\pgfextract@process\point{%
						\pgfpointadd{%
							\pgf@x\halfside%
							\pgf@x-3.232051\pgf@x% (7/6 + 2*cos(30) + 1/3) * x
							\pgf@y0pt%
						}{%
							\pgfpointpolar{\pgfmathcounter-30}{+\pgf@yc}%
						}%
					}%
					\pgfpathlineto{\point}%
					\pgfpathmoveto{\point}%
				}
			\repeatpgfmathloop%
		}%
	}%
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\pgfextract@process\externalpoint{\pgfpointadd{\centerpoint}{\externalpoint}}%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\centerpoint%
		\pgf@xb\pgf@x%
		\pgf@yb\pgf@y%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\let\externalangle\pgfmathresult%
		\dimensions%
		\pgf@xc\halfside%
		%
		\pgf@xc-.166666\pgf@xc%
		\ifdim\pgf@xa<\pgf@xc%
			\pgfmathanglebetweenpoints{\centerpoint}%
			{%
				\pgfgateanchorsuseboundingrectangletrue%
				\csname pgf@anchor@xor gate US@north west\endcsname%
			}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
					{%
						\pgfgateanchorsuseboundingrectangletrue%
						\csname pgf@anchor@xor gate US@north\endcsname%
					}%
					{%
						\pgfgateanchorsuseboundingrectangletrue%
						\csname pgf@anchor@xor gate US@north west\endcsname%
					}%
			\else%
				\pgfmathsubtract@{360}{\pgfmathresult}%
				\ifdim\externalangle pt>\pgfmathresult pt\relax%
					\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
					{%
						\pgfgateanchorsuseboundingrectangletrue%
						\csname pgf@anchor@xor gate US@south\endcsname%
					}%
					{%
						\pgfgateanchorsuseboundingrectangletrue%
						\csname pgf@anchor@xor gate US@south west\endcsname%
					}%
				\else%
					\ifdim\pgf@ya>\pgf@yb%
						\pgf@yc\halfheight%
						\advance\pgf@yc\halfside%
						\advance\pgf@yc-\outerxsep%
						\pgf@process{%
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
							{%
								\centerpoint%
								\pgf@xa\halfside%
								\advance\pgf@x-1.166666\pgf@xa%
								\pgf@xa2.0\pgf@xa%
								\advance\pgf@x-.866025\pgf@xa%
								\advance\pgf@x-\outerxsep%
								\advance\pgf@x-.166666\pgf@xa%
							}%
							{0}{90}{+\pgf@yc}%
						}%
					\else%
						\pgf@yc\halfheight%
						\advance\pgf@yc\halfside%
						\advance\pgf@yc-\outerxsep%
						\pgf@process{%
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
							{%
								\centerpoint%
								\pgf@xa\halfside%
								\advance\pgf@x-1.166666\pgf@xa%
								\pgf@xa2.0\pgf@xa%
								\advance\pgf@x-.866025\pgf@xa%
								\advance\pgf@x-\outerxsep%
								\advance\pgf@x-.166666\pgf@xa%
							}%
							{270}{360}{+\pgf@yc}%
						}%
					\fi%
				\fi%
			\fi%
		\else%
			\ifdim\pgf@y=0pt\relax%
				\csname pgf@anchor@and gate US@east\endcsname%
			\else%
				\pgf@xc\halfwidth%
				\advance\pgf@xc\halfside%
				\pgf@yc\halfheight%
				\advance\pgf@yc\halfside%
				\pgf@xb\halfside%
				\pgf@xb-.166666\pgf@xb%
				\ifdim\pgf@ya<0pt%
					\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
					{%
						\centerpoint%
						\advance\pgf@y\halfside%	
						\advance\pgf@x\pgf@xb%		
					}%
					{270}{330}{+\pgf@yc}%
				\else%
					\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
					{%
						\centerpoint%
						\advance\pgf@y-\halfside%	
						\advance\pgf@x\pgf@xb%
					}%
					{30}{90}{+\pgf@xc and +\pgf@yc}%
				\fi%
			\fi%
		\fi%
	}%
}




% Shape xnor gate US
%
\pgfdeclareshape{xnor gate US}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@xnor gate US\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{2}% 
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@xnor gate US@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@xnor gate US@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@XOR@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{An xnor gate must have two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\halflinewidth{%
		\pgf@x.5\pgflinewidth%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\inheritanchor[from=xor gate US]{mid east}
	\inheritanchor[from=xor gate US]{mid west}
	\anchor{base}{\basepoint}%
	\inheritanchor[from=xor gate US]{base east}
	\inheritanchor[from=xor gate US]{base west}
	\inheritanchor[from=xor gate US]{base}
	\inheritanchor[from=nor gate US]{output}
	\inheritanchor[from=xor gate US]{east}
	\inheritanchor[from=xor gate US]{north east}
	\inheritanchor[from=xor gate US]{south east}
	\inheritanchor[from=xor gate US]{north}
	\inheritanchor[from=xor gate US]{south}
	\inheritanchor[from=xor gate US]{south west}
	\inheritanchor[from=xor gate US]{north west}
	\inheritanchor[from=xor gate US]{west}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{-.16666\pgf@xc}{\pgf@yc}}%
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{90}{30}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{-30}{-90}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{-\pgf@yc}}%
			{%
				\pgf@yc2.66666\pgf@yc%
				\pgfpatharc{-22}{0}{+1.166666\pgf@yc and +\pgf@yc}%			
			}
			{%
				\pgf@yc2.66666\pgf@yc%
				\pgfpatharc{0}{22}{+1.166666\pgf@yc and +\pgf@yc}%			
			}%
			\pgfpathclose%
			%
			% Draw the output inverter.
			%
			{%
				\pgfpathcircle{%
					\pgf@x-.166666\pgf@xc%
					\pgf@yc2.0\pgf@yc%
					\advance\pgf@x.866025\pgf@yc%
					\advance\pgf@x\outerinvertedradius%
					\pgf@y0pt%
				}{+\invertedradius}%			
			}%
			%
			% Draw the inputs.
			%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{%
							\pgf@ya\halfside%
							\pgf@yb2.0\pgf@ya%
							\pgf@xa\pgf@yb%
							\advance\pgf@yb-\halflinewidth%
							\pgfmathdivide@{\pgfmath@tonumber{\pgf@yc}}{\pgfmath@tonumber{\pgf@yb}}%
							\pgfmathasin@{\pgfmathresult}%
							\pgfmathcos@{\pgfmathresult}%
							%
							\pgf@x-1.5\pgf@ya%
							\advance\pgf@x-.866025\pgf@xa%
							\advance\pgf@x\pgfmathresult\pgf@yb%
							\advance\pgf@x-\invertedradius%
							\pgf@y\pgf@yc%
						}{+\invertedradius}%				
					}%
				\fi%				
			\repeatpgfmathloop%
			%
			% Now, some fooling around to stop the `tail' being filled.
			%
			\pgf@xc\halfside%
			\pgf@yc\halfside%
			\pgfpathmoveto{\pgfqpoint{-1.5\pgf@xc}{-\pgf@yc}}%
			\pgf@yc2.0\pgf@yc%
			\pgfmathloop%
			\ifnum\pgfmathcounter<61\relax%
				{%
					\pgfextract@process\point{%
						\pgfpointadd{%
							\pgf@x\halfside%
							\pgf@x-3.232051\pgf@x% (7/6 + 2*cos(30) + 1/3) * x
							\pgf@y0pt%
						}{%
							\pgfpointpolar{\pgfmathcounter-30}{+\pgf@yc}%
						}%
					}%
					\pgfpathlineto{\point}%
					\pgfpathmoveto{\point}%
				}
			\repeatpgfmathloop%
		}%
	}%
	\inheritanchorborder[from=xor gate US]
}






% Shape not gate US
%
\pgfdeclareshape{not gate US}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@not gate US\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1}% 
		\ifnum\pgf@lib@sh@logicgate@numinputs=0\relax%
			\PackageError{PGF}{A not gate must have one input}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\halflinewidth{%
		\pgf@x.5\pgflinewidth%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\midpoint%
		\pgfutil@tempdima\pgf@y%
		\csname pgf@anchor@not gate US@east\endcsname%
		\pgf@y\pgfutil@tempdima%
	}
	\anchor{mid west}{%
		\dimensions%
		\pgf@xc\halfside%
		\pgf@xc-.833333\pgf@xc%
		\advance\pgf@xc-\outerxsep%
		\midpoint%
		\advance\pgf@x\pgf@xc%	
	}%
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\basepoint%
		\pgfutil@tempdima\pgf@y%
		\csname pgf@anchor@not gate US@east\endcsname%
		\pgf@y\pgfutil@tempdima%
	}
	\anchor{base west}{%
		\dimensions%
		\pgf@xc\halfside%
		\pgf@xc-.833333\pgf@xc%
		\advance\pgf@xc-\outerxsep%
		\basepoint%
		\advance\pgf@x\pgf@xc%	
	}%
	\inheritanchor[from=and gate US]{base}
	\anchor{output}{%
		\dimensions%
		\pgf@xc\halfside%
		\centerpoint%
		\advance\pgf@x-.166666\pgf@xc%
		\pgf@xc2.0\pgf@xc%
		\advance\pgf@x.866025\pgf@xc%
		\advance\pgf@x\invertedradius%
		\advance\pgf@x\outerinvertedradius%
		\advance\pgf@x\outerxsep%
	}
	\anchor{east}{%
		\dimensions%
		\tipanchor%
		\pgf@xa\pgf@x%
		\centerpoint%
		\advance\pgf@x\pgf@xa%
	}%
	\anchor{north}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@not gate US@north west\endcsname%
			\pgf@ya\pgf@y%
			\centerpoint%
			\pgf@y\pgf@ya%
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y1pt}%
				{\csname pgf@anchor@not gate US@north west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
		\fi%
	}
	\anchor{south}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@not gate US@south west\endcsname%
			\pgf@ya\pgf@y%
			\centerpoint%
			\pgf@y\pgf@ya%
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y-1pt}%
				{\csname pgf@anchor@not gate US@south west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
		\fi%
	}
	\anchor{south east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@not gate US@south west\endcsname%
			\pgf@ya\pgf@y%
			\pgf@process{%	
				\dimensions%
				\tipanchor%
				\pgf@xa\pgf@x%
				\centerpoint%
				\advance\pgf@x\pgf@xa%
			}%
			\pgf@y\pgf@ya%
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y-1pt}%
				{\csname pgf@anchor@not gate US@south west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
		\fi%
	}
	\anchor{north east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@not gate US@north west\endcsname%
			\pgf@ya\pgf@y%
			\pgf@process{%	
				\dimensions%
				\tipanchor%
				\pgf@xa\pgf@x%
				\centerpoint%
				\advance\pgf@x\pgf@xa%
			}%
			\pgf@y\pgf@ya%
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y1pt}%
				{\csname pgf@anchor@not gate US@north west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
		\fi%
	}
	\anchor{south west}{%
		\dimensions%
		\pgf@xa\halfside%
		\centerpoint%
		\advance\pgf@x-.833333\pgf@xa
		\advance\pgf@x-\outerxsep%
		\advance\pgf@y-1.166666\pgf@xa%
		\pgf@ya\outerysep%
		\advance\pgf@y-1.565\pgf@ya% Selected by trial and error.	
	}%
	\anchor{north west}{%
		\dimensions%
		\pgf@xa\halfside%
		\centerpoint%
		\advance\pgf@x-.833333\pgf@xa
		\advance\pgf@x-\outerxsep%
		\advance\pgf@y1.166666\pgf@xa%
		\pgf@ya\outerysep%
		\advance\pgf@y1.565\pgf@ya% Selected by trial and error.	
	}%
	\anchor{input}{%
		\dimensions%
		\pgf@lib@sh@logicgate@AND@inputanchor{1}%
		\pgf@xc\halfside%
		\advance\pgf@x.333333\pgf@xc%
	}%
	\anchor{west}{%
		\dimensions%
		\pgf@xc\halfside%
		\pgf@xc-.833333\pgf@xc%
		\advance\pgf@xc-\outerxsep%
		\centerpoint%
		\advance\pgf@x\pgf@xc%
	}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\tipanchor}%
			\pgfpathlineto{\pgfqpoint{-.833333\pgf@xc}{1.166666\pgf@yc}}%
			\pgfpathlineto{\pgfqpoint{-.833333\pgf@xc}{-1.166666\pgf@yc}}%
			\pgfpathlineto{\tipanchor}%
			%
			% Draw the output inverter.
			%
			{%
				\pgfpathcircle{%
					\pgf@x-.166666\pgf@xc%
					\pgf@yc2.0\pgf@yc%
					\advance\pgf@x.866025\pgf@yc%
					\advance\pgf@x\outerinvertedradius%
					\pgf@y0pt%
				}{+\invertedradius}%			
			}%
			%
			% Draw the input.
			%
			\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-1\endcsname%
				{%
					\pgfpathcircle{%
						\pgf@xa\halfside%
						\pgf@x-.833333\pgf@xa%
						\advance\pgf@x-.5\pgflinewidth%
						\advance\pgf@x-\invertedradius%
						\pgf@y0pt%
					}{+\invertedradius}%				
				}%
			\fi%				
		}%
	}%
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\pgfextract@process\externalpoint{\pgfpointadd{\centerpoint}{\externalpoint}}%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\let\externalangle\pgfmathresult%
		\dimensions%
		\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@not gate US@north west\endcsname}%
		\ifdim\externalangle pt<\pgfmathresult pt%
			\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
				{\csname pgf@anchor@not gate US@north west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
		\else%
			\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@not gate US@south west\endcsname}%
			\ifdim\externalangle pt<\pgfmathresult pt%
				\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
					{\csname pgf@anchor@not gate US@north west\endcsname}%
					{\csname pgf@anchor@not gate US@south west\endcsname}%
			\else%
				\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
				{\csname pgf@anchor@not gate US@south west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
			\fi%
		\fi%		
	}%
}





% Shape buffer gate US.
%
\pgfdeclareshape{buffer gate US}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@buffer gate US\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1}% 
		\ifnum\pgf@lib@sh@logicgate@numinputs=0\relax%
			\PackageError{PGF}{A buffer gate must have one input}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\halflinewidth{%
		\pgf@x.5\pgflinewidth%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\midpoint%
		\pgfutil@tempdima\pgf@y%
		\csname pgf@anchor@buffer gate US@east\endcsname%
		\pgf@y\pgfutil@tempdima%
	}
	\anchor{mid west}{%
		\dimensions%
		\pgf@xc\halfside%
		\pgf@xc-.833333\pgf@xc%
		\advance\pgf@xc-\outerxsep%
		\midpoint%
		\advance\pgf@x\pgf@xc%	
	}%
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\basepoint%
		\pgfutil@tempdima\pgf@y%
		\csname pgf@anchor@buffer gate US@east\endcsname%
		\pgf@y\pgfutil@tempdima%
	}
	\inheritanchor[from=not gate US]{base west}
	\inheritanchor[from=and gate US]{base}
	\anchor{output}{\csname pgf@anchor@buffer gate US@east\endcsname}
	\anchor{east}{%
		\dimensions%
		\pgfpointadd{\centerpoint}{%
			\tipanchor%
			\pgf@xa\outerxsep%
			\advance\pgf@x2.350943\pgf@xa%	
		}%
	}%
	\anchor{north}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@not gate US@north west\endcsname%
			\pgf@ya\pgf@y%
			\centerpoint%
			\pgf@y\pgf@ya%
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y1pt}%
				{\csname pgf@anchor@buffer gate US@north west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
		\fi%
	}
	\anchor{south}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@not gate US@south west\endcsname%
			\pgf@ya\pgf@y%
			\centerpoint%
			\pgf@y\pgf@ya%
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@y-1pt}%
				{\csname pgf@anchor@not gate US@south west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
		\fi%
	}
	\anchor{south east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@not gate US@south west\endcsname%
			\pgfutil@tempdima\pgf@y%
			\csname pgf@anchor@buffer gate US@east\endcsname%
			\pgf@y\pgfutil@tempdima%
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y-1pt}%
				{\csname pgf@anchor@buffer gate US@south west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xc\outerxsep%
						\advance\pgf@x2.350943\pgf@xc%	
					}%
				}%	
		\fi%
	}
	\anchor{north east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\csname pgf@anchor@not gate US@north west\endcsname%
			\pgfutil@tempdima\pgf@y%
			\csname pgf@anchor@buffer gate US@east\endcsname%
			\pgf@y\pgfutil@tempdima%
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\centerpoint\advance\pgf@x1pt\advance\pgf@y1pt}%
				{\csname pgf@anchor@buffer gate US@north west\endcsname}%
				{%
					\pgfpointadd{\centerpoint}{%
						\tipanchor%
						\pgf@xa\outerxsep%
						\advance\pgf@x2.350943\pgf@xa%	
					}%
				}%	
		\fi%
	}
	\inheritanchor[from=not gate US]{south west}
	\inheritanchor[from=not gate US]{north west}
	\inheritanchor[from=not gate US]{input}
	\inheritanchor[from=not gate US]{west}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\tipanchor}%
			\pgfpathlineto{\pgfqpoint{-.833333\pgf@xc}{1.166666\pgf@yc}}%
			\pgfpathlineto{\pgfqpoint{-.833333\pgf@xc}{-1.166666\pgf@yc}}%
			\pgfpathclose%
			%
			% Draw the input.
			%
			\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-1\endcsname%
				{%
					\pgfpathcircle{%
						\pgf@xa\halfside%
						\pgf@x-.833333\pgf@xa%
						\advance\pgf@x-.5\pgflinewidth%
						\advance\pgf@x-\invertedradius%
						\pgf@y0pt%
					}{+\invertedradius}%				
				}%
			\fi%				
		}%
	}%
	\inheritanchorborder[from=not gate US]
}





\pgfdeclareshape{and gate CDH}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@and gate CDH\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@and gate CDH@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@and gate CDH@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@AND@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{An and gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\csname pgf@anchor@and gate CDH@east\endcsname%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa}
	\anchor{mid west}{%
		\csname pgf@anchor@and gate CDH@west\endcsname%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa}
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\csname pgf@anchor@and gate CDH@east\endcsname%
		\pgf@xa\pgf@x%
		\basepoint%
		\pgf@x\pgf@xa}
	\anchor{base west}{%
		\csname pgf@anchor@and gate CDH@west\endcsname%
		\pgf@xa\pgf@x%
		\basepoint%
		\pgf@x\pgf@xa}
	\anchor{east}{%
		\dimensions%
		\pgfpointadd{\centerpoint}{\tipanchor}%
	}
	\anchor{output}{\csname pgf@anchor@and gate CDH@east\endcsname}
	\anchor{north east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\tipanchor%
			\pgf@xa\pgf@x%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\halfheight%
		\else%
			\centerpoint%
			\pgf@xa\halfwidth%
			\pgf@ya\halfheight%
			\pgf@xb\halfside%
			\advance\pgf@x-.166666\pgf@xb%
			\advance\pgf@xa\pgf@xb%
			\advance\pgf@x.5\pgf@xa%
			\advance\pgf@y-\pgf@xb%
			\advance\pgf@ya\pgf@xb%
			\advance\pgf@y.866025\pgf@ya%
		\fi%
	}
	\anchor{south east}{%
		\dimensions%
		\ifpgfgateanchorsuseboundingrectangle%
			\tipanchor%
			\pgf@xa\pgf@x%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y-\halfheight%
		\else
			\centerpoint%
			\pgf@xa\halfwidth%
			\pgf@ya\halfheight%
			\pgf@xb\halfside%
			\advance\pgf@x-.166666\pgf@xb%
			\advance\pgf@xa\pgf@xb%
			\advance\pgf@x.5\pgf@xa%
			\advance\pgf@y\pgf@xb%
			\advance\pgf@ya\pgf@xb%
			\advance\pgf@y-.866025\pgf@ya%
		\fi%
	}
	\anchor{north}{%
		\dimensions%
		\centerpoint%
		\ifpgfgateanchorsuseboundingrectangle%
			\advance\pgf@y\halfheight%
		\else%
			\pgf@ya\halfheight%
			\advance\pgf@y.993043\pgf@ya%
		\fi%	
	}
	\anchor{south}{%
		\dimensions%
		\centerpoint%
		\ifpgfgateanchorsuseboundingrectangle%
			\advance\pgf@y-\halfheight%
		\else%
			\pgf@ya\halfheight%
			\advance\pgf@y-.993043\pgf@ya%
		\fi%	
	}
	\anchor{south west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\advance\pgf@x-1.16666\pgf@xa%
		\advance\pgf@x-\outerxsep%
		\advance\pgf@y-\halfheight%
	}
	\anchor{north west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\advance\pgf@x-1.16666\pgf@xa%
		\advance\pgf@x-\outerxsep%
		\advance\pgf@y\halfheight%
	}
	\anchor{west}{%
		\dimensions%
		\centerpoint%
		\pgf@xa\halfside%
		\advance\pgf@x-1.16666\pgf@xa%
		\advance\pgf@x-\outerxsep%
	}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{-.16666\pgf@xc}{\pgf@yc}}%
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{90}{30}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{-30}{-90}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{-\pgf@yc}}%
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{\pgf@yc}}%
			\pgfpathclose%
			%
			% Draw the inputs.
			%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{%
							\pgf@xa\halfside%
							\pgf@x-1.16666\pgf@xa%
							\advance\pgf@x-.5\pgflinewidth%
							\advance\pgf@x-\invertedradius%
							\pgf@y\pgf@yc%
						}{+\invertedradius}%				
					}%
				\fi%				
			\repeatpgfmathloop%
		}%
	}%
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\dimensions%
		\pgf@xb\halfside%
		%
		\pgf@xb-.166666\pgf@xb%
		\ifdim\pgf@xa<\pgf@xb%
			\pgfpointadd{\centerpoint}{%
				\pgfpointborderrectangle{\externalpoint}{%
					\pgf@xc\halfside%
					\pgf@xc.166666\pgf@xc%
					\advance\pgf@xc\halfwidth%
					\pgfqpoint{\pgf@xc}{\halfheight}%
				}%
			}%
		\else%
			\ifdim\pgf@y=0pt\relax%
				\csname pgf@anchor@and gate CDH@east\endcsname%
			\else%
				\pgfextract@process\externalpoint{\pgfpointadd{\centerpoint}{\externalpoint}}%
				\pgf@xc\halfwidth%
				\advance\pgf@xc\halfside%
				\pgf@yc\halfheight%
				\advance\pgf@yc\halfside%
				\ifdim\pgf@ya<0pt%
					\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
					{%
						\centerpoint%
						\advance\pgf@y\halfside%	
						\advance\pgf@x\pgf@xb%		
					}%
					{270}{330}{+\pgf@yc}%
				\else%
					\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
					{%
						\centerpoint%
						\advance\pgf@y-\halfside%	
						\advance\pgf@x\pgf@xb%
					}%
					{30}{90}{+\pgf@xc and +\pgf@yc}%
				\fi%
			\fi%
		\fi%
	}
}


\pgfdeclareshape{nand gate CDH}{%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@nand gate CDH\endcsname{%
		\pgf@lib@sh@logicgate@parseinputs{1024}% Maximum 1024 (!) inputs.
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\pgf@lib@sh@logicgate@numinputs%
		\else%
			\pgfutil@ifundefined{pgf@anchor@nand gate CDH@input \pgfmathcounter}{%
				\expandafter\xdef\csname pgf@anchor@nand gate CDH@input \pgfmathcounter\endcsname{%
					\noexpand\pgf@lib@sh@logicgate@AND@inputanchor{\pgfmathcounter}%
				}%
			}{}%
		\repeatpgfmathloop%
		\ifnum\pgf@lib@sh@logicgate@numinputs<2\relax%
			\PackageError{PGF}{A nand gate must have at least two inputs}{}%
		\fi%
	}%
	\savedmacro\numinputs{\let\numinputs\pgf@lib@sh@logicgate@numinputs}%
	\saveddimen\invertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
	}%
	\saveddimen\outerinvertedradius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/logic gate inverted radius}}%
		\advance\pgf@x.5\pgflinewidth%
	}
	\savedmacro\dimensions{\pgf@lib@sh@logicgates@dimensions@orUS}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\inheritanchor[from=and gate CDH]{mid east}
	\inheritanchor[from=and gate CDH]{mid west}
	\anchor{base}{\basepoint}%
	\inheritanchor[from=and gate CDH]{base east}
	\inheritanchor[from=and gate CDH]{base west}
	\anchor{output}{%
		\dimensions
		\pgfpointadd{\centerpoint}{%
			\pgf@xa\halfside%
			\pgf@x-.166666\pgf@xa%
			\pgf@xb2.0\pgf@xa%
			\advance\pgf@x.866025\pgf@xb%
			\advance\pgf@x\invertedradius%
			\advance\pgf@x\outerinvertedradius%
			\advance\pgf@x\outerxsep%
			\pgf@y0pt%
		}%
	}
	\inheritanchor[from=and gate CDH]{east}
	\inheritanchor[from=and gate CDH]{north east}
	\inheritanchor[from=and gate CDH]{south east}
	\inheritanchor[from=and gate CDH]{north}
	\inheritanchor[from=and gate CDH]{south}
	\inheritanchor[from=and gate CDH]{south west}
	\inheritanchor[from=and gate CDH]{north west}
	\inheritanchor[from=and gate CDH]{west}
	\backgroundpath{%
		\dimensions%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%
		\advance\pgf@xc-\outerxsep%
		\advance\pgf@yc-\outerysep%
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{-.16666\pgf@xc}{\pgf@yc}}%
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{90}{30}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			{%
				\pgf@yc2.0\pgf@yc%
				\edef\pgf@marshal{%
					\noexpand\pgfpatharc{-30}{-90}{\the\pgf@yc}%
				}%
				\pgf@marshal%
			}
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{-\pgf@yc}}%
			\pgfpathlineto{\pgfqpoint{-1.16666\pgf@xc}{\pgf@yc}}%
			\pgfpathclose%
			%
			% Draw the output inverter.
			%
			{%
				\pgfpathcircle{%
					\pgf@x-.166666\pgf@xc%
					\pgf@yc2.0\pgf@yc%
					\advance\pgf@x.866025\pgf@yc%
					\advance\pgf@x\outerinvertedradius%
					\pgf@y0pt%
				}{+\invertedradius}%			
			}%
			%
			% Draw the inputs.
			%
			\pgfutil@tempdima2.0\pgf@yc%
			\c@pgf@counta\numinputs%
			\advance\c@pgf@counta1\relax%
			\divide\pgfutil@tempdima\c@pgf@counta%
			\pgfmathloop%
			\ifnum\pgfmathcounter>\numinputs%
			\else%
				\advance\pgf@yc-\pgfutil@tempdima%
				\expandafter\ifx\expandafter\pgf@lib@sh@itext\csname input-\pgfmathcounter\endcsname%
					{%
						\pgfpathcircle{%
							\pgf@xa\halfside%
							\pgf@x-1.16666\pgf@xa%
							\advance\pgf@x-.5\pgflinewidth%
							\advance\pgf@x-\invertedradius%
							\pgf@y\pgf@yc%
						}{+\invertedradius}%				
					}%
				\fi%				
			\repeatpgfmathloop%
		}%
	}%
	\inheritanchorborder[from=and gate CDH]
}

==> pgflibraryshapes.geometric.code.tex <==
% Copyright 2006 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryshapes.geometric.code.tex,v 1.22 2008/02/01 17:09:04 vibrovski Exp $

\pgfdeclareshape{ellipse}
%
% Draws a circle around the text
%
{
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
  }
  \savedanchor\radius{%
    % 
    % Caculate ``height radius''
    % 
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by\pgf@yb%
    % 
    % Caculate ``width radius''
    % 
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by\pgf@xb%
    % 
    % Adjust
    % 
    \pgf@x=1.4142136\pgf@x%
    \pgf@y=1.4142136\pgf@y%
    % 
    % Adjust hieght, if necessary
    % 
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<.5\pgf@yc%
      \pgf@y=.5\pgf@yc%
    \fi%
    % 
    % Adjust width, if necessary
    % 
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<.5\pgf@xc%
      \pgf@x=.5\pgf@xc%
    \fi%
    % 
    % Add outer sep
    % 
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \advance\pgf@x by\pgf@xb%
    \advance\pgf@y by\pgf@yb%
  }

  %
  % Anchors
  % 
  \anchor{center}{\centerpoint}
  \anchor{mid}{\centerpoint\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base}{\centerpoint\pgf@y=0pt}
  \anchor{north}
  {
    \pgf@process{\radius}
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@y by\pgf@ya
  }
  \anchor{south}
  {
    \pgf@process{\radius}
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@y by-\pgf@ya
  }
  \anchor{west}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-\pgf@xa
  }
  \anchor{mid west}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-\pgf@xa%
    \pgfmathsetlength\pgf@y{.5ex}
  }
  \anchor{base west}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-\pgf@xa%
    \pgf@y=0pt
  }
  \anchor{north west}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@ya
  }
  \anchor{south west}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@ya
  }
  \anchor{east}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by\pgf@xa
  }
  \anchor{mid east}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength\pgf@y{.5ex}
  }
  \anchor{base east}
  {%
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@process{\centerpoint}
    \advance\pgf@x by\pgf@xa%
    \pgf@y=0pt
  }
  \anchor{north east}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@ya
  }
  \anchor{south east}
  {
    \pgf@process{\radius}
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\centerpoint}
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@ya
  }
  \anchorborder{
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderellipse
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      {\noexpand\radius}%
    }%
    \pgf@marshal%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \centerpoint%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }

  %
  % Background path
  %
  \backgroundpath
  {
    \pgf@process{\radius}%
    \pgfutil@tempdima=\pgf@x%
    \pgfutil@tempdimb=\pgf@y%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \advance\pgfutil@tempdima by-\pgf@xb%
    \advance\pgfutil@tempdimb by-\pgf@yb%
    \pgfpathellipse{\centerpoint}{\pgfqpoint{\pgfutil@tempdima}{0pt}}{\pgfqpoint{0pt}{\pgfutil@tempdimb}}%
  }
}




% Set the recommended shape aspect ratio
%
% #1 = aspect ratio
%
% Example:
%
% \pgfsetshapeaspect{1.5}

% Keys for shape aspect ratio.
%
% /pgf/aspect         : recommended width/height quotient.
%
\pgfkeys{/pgf/.cd,
	aspect/.code={\pgfsetshapeaspect{#1}},% this for tikz...
	shape aspect/.initial=1,% but this is consistent with other pgfset stuff. 
	shape aspect/.code={%
		\pgfkeys{/pgf/aspect=#1}%
		\pgfkeyssetvalue{/pgf/shape aspect}{#1}
	}%
}
	

\def\pgfsetshapeaspect#1{%
  \def\pgfshapeaspect{#1}%
  % Invert
  \pgfutil@tempdima=#1pt%
  \pgfutil@tempdima=.125\pgfutil@tempdima%
  \c@pgf@counta=\pgfutil@tempdima\relax% 8192*determinant
  \pgfutil@tempdima=8192pt%
  \divide\pgfutil@tempdima by\c@pgf@counta%
  \edef\pgfshapeaspectinverse{\pgf@sys@tonumber{\pgfutil@tempdima}}
}

\pgfsetshapeaspect{1}

\pgfdeclareshape{diamond}
{
  \savedanchor\outernortheast{%
    %
    % Calculate width and height of the inner rectangle
    %
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa by\pgf@xc%
    \pgf@ya=.5\ht\pgfnodeparttextbox%
    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya by\pgf@yc%
    %
    % Calculate width and height of diamond
    %
    \pgf@x=\pgf@xa%
    \advance\pgf@x by\pgfshapeaspect\pgf@ya%
    \pgf@y=\pgfshapeaspectinverse\pgf@xa%
    \advance\pgf@y by\pgf@ya%
    %
    % Check against minimum height/width
    %
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
    \pgf@xb=.5\pgf@xb%   
    \ifdim\pgf@x<\pgf@xb%
      % yes, too small. Enlarge...
      \pgf@x=\pgf@xb%
    \fi%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
    \pgf@yb=.5\pgf@yb%   
    \ifdim\pgf@y<\pgf@yb%
      % yes, too small. Enlarge...
      \pgf@y=\pgf@yb%
    \fi%
    %
    % Add outer border
    %
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }
  \savedanchor\text{%
    \pgf@x=-.5\wd\pgfnodeparttextbox%
    \pgf@y=-.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by.5\dp\pgfnodeparttextbox%
  }

  %
  % Anchors
  %
  \anchor{text}{\text}%
  \anchor{center}{\pgfpointorigin}%
  \anchor{mid}{%
    \pgf@process{\text}%
    \pgf@x=0pt%
    \pgfmathsetlength\pgf@ya{.5ex}
    \advance\pgf@y by\pgf@ya%
  }
  \anchor{base}{\pgf@process{\text}\pgf@x=0pt  }
  \anchor{north}{\pgf@process{\outernortheast}\pgf@x=0pt}
  \anchor{south}{\pgf@process{\outernortheast}\pgf@x=0pt\pgf@y=-\pgf@y}
  \anchor{west}{\pgf@process{\outernortheast}\pgf@x=-\pgf@x\pgf@y=0pt}
  \anchor{north west}{\pgf@process{\outernortheast}\pgf@x=-.5\pgf@x\pgf@y=.5\pgf@y}
  \anchor{south west}{\pgf@process{\outernortheast}\pgf@x=-.5\pgf@x\pgf@y=-.5\pgf@y}
  \anchor{east}{\pgf@process{\outernortheast}\pgf@y=0pt}
  \anchor{north east}{\pgf@process{\outernortheast}\pgf@x=.5\pgf@x\pgf@y=.5\pgf@y}
  \anchor{south east}{\pgf@process{\outernortheast}\pgf@x=.5\pgf@x\pgf@y=-.5\pgf@y}
  \anchorborder{%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\outernortheast}%
    \ifdim\pgf@xa>0pt%
    \else%
      \pgf@x=-\pgf@x%
    \fi%
    \ifdim\pgf@ya>0pt%
    \else%
      \pgf@y=-\pgf@y%
    \fi%
    \edef\pgf@marshal{%
      \noexpand\pgfpointintersectionoflines
      {\noexpand\pgfpointorigin}
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
      {\noexpand\pgfqpoint{\the\pgf@x}{0pt}}
      {\noexpand\pgfqpoint{0pt}{\the\pgf@y}}%
    }%
    \pgf@process{\pgf@marshal}%
  }

  %
  % Background path
  %
  \backgroundpath{
    \pgf@process{\outernortheast}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/pgf/outer xsep}}%
    \pgfmathsetlength{\pgf@ya}{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@xc by-1.414213\pgf@xa%
    \advance\pgf@yc by-1.414213\pgf@ya%
    \pgfpathmoveto{\pgfqpoint{\pgf@xc}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{\pgf@yc}}%
    \pgfpathlineto{\pgfqpoint{-\pgf@xc}{0pt}}%
    \pgfpathlineto{\pgfqpoint{0pt}{-\pgf@yc}}%
    \pgfpathclose%
  }
}






\newif\ifpgf@lib@shapes@starouterradiususesratio
\pgf@lib@shapes@starouterradiususesratiotrue

% Keys for star shape
%
% /pgf/star points       : Number of points on the star.
% /pgf/star point height : The height of the outer star points.
% /pgf/star point ratio  : The ratio of the outer point and inner point radii.

\pgfkeys{/pgf/.cd,
	star points/.initial=5,
	star point height/.initial=.5cm,
	star point height/.code={%
		\def\pgf@lib@temp{#1}%
		\pgfkeyslet{/pgf/star point height}{\pgf@lib@temp}%
		\pgf@lib@shapes@starouterradiususesratiofalse%	
	},
	star point ratio/.initial=1.5,
	star point ratio/.code={%
		\def\pgf@lib@temp{#1}%
		\pgfkeyslet{/pgf/star point ratio}{\pgf@lib@temp}%
		\pgf@lib@shapes@starouterradiususesratiotrue%	
	}%
	star rotate/.style={/pgf/shape border rotate=#1}% For compatability with 1.18
}


% Shape star.
%
\pgfdeclareshape{star}{
	\savedmacro\totalstarpoints{%
		\pgfmathsetcounter{pgf@counta}{\pgfkeysvalueof{/pgf/star points}}%
		\multiply\c@pgf@counta2\relax%
		\edef\totalstarpoints{\the\c@pgf@counta}%
	}
	\savedmacro\anglestep{%
		\pgfmathdivide{180}{\pgfkeysvalueof{/pgf/star points}}%
		\let\anglestep\pgfmathresult%
	}
	\savedmacro\calculateradii{%
		%
		% Get the node dimensions.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		\ifdim\pgf@y>\pgf@x%
			\pgf@x\pgf@y%
		\fi%
		%
		% Calculate the incircle radius.
		%
		\pgf@x1.41421\pgf@x%
		\edef\innerradius{\the\pgf@x}%
		%
		% Calculate the circumcircle radius.
		%
		% Use the star point height or the star point ratio?
		%
		\ifpgf@lib@shapes@starouterradiususesratio%
			\pgfmathparse{\pgfkeysvalueof{/pgf/star point ratio}}%
			\expandafter\pgf@x\pgfmathresult\pgf@x%
		\else%
			\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/star point height}}%
		\fi%
		\pgf@xc\pgf@x%
		%
		% Accommodate the larger of the minimum height/width.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@ya>\pgf@xa%
			\pgf@xa\pgf@ya%
		\fi%
		\ifdim\pgf@x<.5\pgf@xa%
	   	\pgf@x.5\pgf@xa%
	   \fi%
	   \edef\outerradius{\the\pgf@x}%
	   %
	   % If the outer radius has been enlarged, adjust the inner radius...
	   %
	   \ifdim\pgf@x>\pgf@xc%
	   	%
	   	% ...using the star point ratio, or...
	   	%
	   	\ifpgf@lib@shapes@starouterradiususesratio%
	   		\pgfmathreciprocal{\pgfkeysvalueof{/pgf/star point ratio}}%
	   		\pgf@xa\pgfmathresult\pgf@x\relax%
	   		\edef\innerradius{\the\pgf@xa}%
			\else%
				%
				% The star point height.
				%
				\pgf@xa\pgf@x\relax%
				\pgfmathaddtolength\pgf@xa{-\pgfkeysvalueof{/pgf/star point height}}%
				\edef\innerradius{\the\pgf@xa}%
			\fi%
		\fi%
		\edef\outerradius{\the\pgf@x}%
		%
		% Now calculate the anchor radii from the outer sep.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@ya>\pgf@xa%
			\pgf@xa\pgf@ya%
		\fi
		%
		% Take into account the miter length...
		%
		\pgfmathdivide{180}{\pgfkeysvalueof{/pgf/star points}}%
		\let\angletofirstpoint\pgfmathresult%
		\pgfmathmultiply@{\angletofirstpoint}{2}%
		\let\angletosecondpoint\pgfmathresult%
		%
		% ...for the outer radius...
		%
		\pgfmathanglebetweenlines%
			{\pgfqpointpolar{\angletofirstpoint}{\outerradius}}%
			{\pgfqpointpolar{\angletosecondpoint}{\innerradius}}%
			{\pgfqpointpolar{\angletofirstpoint}{\outerradius}}%		
			{\pgfqpointpolar{0}{\innerradius}}%		
		\pgfmathdivide@{\pgfmathresult}{2}%
		\pgfmathcosec@{\pgfmathresult}%
		\pgf@x\outerradius\relax%
		\advance\pgf@x\pgfmathresult\pgf@xa%
		\edef\anchorouterradius{\the\pgf@x}%
		%
		% ...and for the inner radius.
		%
		\pgfmathanglebetweenlines%
			{\pgfqpointpolar{\angletofirstpoint}{\innerradius}}%		
			{\pgfqpointpolar{0}{\outerradius}}%	
			{\pgfqpointpolar{\angletofirstpoint}{\innerradius}}%
			{\pgfqpointpolar{\angletosecondpoint}{\outerradius}}%						
		\pgfmathdivide@{\pgfmathresult}{2}%
		\pgfmathcosec@{\pgfmathresult}%
		\pgf@x\innerradius\relax%
		\advance\pgf@x\pgfmathresult\pgf@xa%
		\edef\anchorinnerradius{\the\pgf@x}%
		%	
		% Save all radii.
		%
		\addtosavedmacro{\innerradius}%
		\addtosavedmacro{\outerradius}%
		\addtosavedmacro{\anchorinnerradius}%
		\addtosavedmacro{\anchorouterradius}%
	}
	\savedmacro\startangle{%
		\pgfmathadd{90}{\pgfkeysvalueof{/pgf/shape border rotate}}%
		\let\startangle\pgfmathresult%
	}
	%
	% Saved anchors.
	%
	\savedanchor{\centerpoint}{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor{\midpoint}{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%	
	%
	% Other anchors.
	%
%
	% Other anchors.
	%
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\centerpoint\pgfmathsetlength\pgf@y{.5ex}}%
 	\anchor{base}{\centerpoint\pgf@y=0pt}%
 	\anchor{north}{%
 		\calculateradii%
 		\csname pgf@anchor@star@border\endcsname{\pgfqpoint{0pt}{\anchorouterradius}}}%
 	\anchor{south}{%
 		\calculateradii%
 		\csname pgf@anchor@star@border\endcsname{\pgfqpoint{0pt}{-\anchorouterradius}}}%
 	\anchor{east}{%
 		\calculateradii%
 		\csname pgf@anchor@star@border\endcsname{\pgfqpoint{\anchorouterradius}{0pt}}}%
 	\anchor{west}{%
 		\calculateradii%
 		\csname pgf@anchor@star@border\endcsname{\pgfqpoint{-\anchorouterradius}{0pt}}}%
 	\anchor{north east}{%
 		\calculateradii%
 		\csname pgf@anchor@star@border\endcsname{\pgfqpoint{\anchorouterradius}{\anchorouterradius}}}%
 	\anchor{north west}{%
 		\calculateradii%
 		\csname pgf@anchor@star@border\endcsname{\pgfqpoint{-\anchorouterradius}{\anchorouterradius}}}%
 	\anchor{south east}{%
 		\calculateradii%
 		\csname pgf@anchor@star@border\endcsname{\pgfqpoint{\anchorouterradius}{-\anchorouterradius}}}%
 	\anchor{south west}{%
 		\calculateradii%
 		\csname pgf@anchor@star@border\endcsname{\pgfqpoint{-\anchorouterradius}{-\anchorouterradius}}}%	 	
 	%
 	% Background path.
 	%
	\backgroundpath{%
		\calculateradii%
		\let\angle\startangle%
		\pgfpathmoveto{\pgfpointadd{\centerpoint}{\pgfqpointpolar{\startangle}{\outerradius}}}%
		\pgfmathloop%
			\pgfmathadd@{\angle}{\anglestep}%
			\let\angle\pgfmathresult%
		\ifnum\pgfmathcounter=\totalstarpoints%
			\pgfpathclose%
		\else%
			\ifodd\pgfmathcounter
				\pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpointpolar{\angle}{\innerradius}}}%
			\else%
				\pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpointpolar{\angle}{\outerradius}}}%
			\fi%
		\repeatpgfmathloop%
	}%
	%
	% Define points on the anchor border.
	%
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% Adjust the location of the external 
		% point relative to \centerpoint.
		%
		\centerpoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Get the angle of the external point to the \centerpoint.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
		%
		% Locate the appropriate sides on the star border...
		%
		\pgfmathsubtract@{\pgfmathresult}{\startangle}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\pgfmathdivide@{\pgfmathresult}{\anglestep}%
		\pgfmathfloor@{\pgfmathresult}%
		\afterassignment\pgfmath@gobbletilpgfmath@
		\c@pgf@counta\pgfmathresult\relax\pgfmath@
		\pgfmathmultiply@{\pgfmathresult}{\anglestep}%
		\pgfmathadd@{\pgfmathresult}{\startangle}%
		\let\firstangle\pgfmathresult%
		\pgfmathadd@{\pgfmathresult}{\anglestep}%
		\let\secondangle\pgfmathresult%
		\calculateradii%
		%
		% ...and thus, the point on the star border.
		%
		\ifodd\c@pgf@counta
			\pgfpointintersectionoflines{\centerpoint}{\pgfpoint{+\externalx}{+\externaly}}%
				{%
					\pgfpointadd{\centerpoint}%
						{\pgfqpointpolar{+\firstangle}{+\anchorinnerradius}}%
					}%	
					{%
						\pgfpointadd{\centerpoint}%
							{\pgfqpointpolar{+\secondangle}{+\anchorouterradius}}%
					}%	
		\else%
			\pgfpointintersectionoflines{\centerpoint}{\pgfpoint{+\externalx}{+\externaly}}%
				{%
					\pgfpointadd{\centerpoint}%
						{\pgfqpointpolar{+\firstangle}{+\anchorouterradius}}%
					}%	
					{%
						\pgfpointadd{\centerpoint}%
							{\pgfqpointpolar{+\secondangle}{+\anchorinnerradius}}%
					}%	
		\fi%
	}
	%
	% Some hackery. This is needed if a star is positioned using 
	% a `...point <n+1>' anchor, where n is the maximum number of 
	% points of any previously drawn star.
	%
	\pgfutil@g@addto@macro\pgf@sh@s@star{%
		\c@pgf@counta\totalstarpoints\relax%
		\divide\c@pgf@counta2\relax%
		\pgfmathloop%
			\ifnum\c@pgf@counta>0\relax%
				\c@pgf@countb\c@pgf@counta\relax%
				\advance\c@pgf@countb-1\relax%
				\pgfutil@ifundefined{pgf@anchor@star@inner point\space\the\c@pgf@counta}{%
					\expandafter\xdef\csname pgf@anchor@star@inner point\space\the\c@pgf@counta\endcsname{%
						\noexpand\calculateradii%
						\noexpand\pgfmathmultiply@{\the\c@pgf@countb}{\noexpand\anglestep}%
						\noexpand\pgfmathmultiply@{\noexpand\pgfmathresult}{2}%
						\noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\anglestep}%
						\noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\startangle}%
						\noexpand\let\noexpand\angle\noexpand\pgfmathresult%
						\noexpand\pgfpointadd{\noexpand\centerpoint}%
							{\noexpand\pgfqpointpolar{\noexpand\angle}{\noexpand\anchorinnerradius}}%
					}%
					\expandafter\xdef\csname pgf@anchor@star@outer point\space\the\c@pgf@counta\endcsname{%
						\noexpand\calculateradii%
						\noexpand\pgfmathmultiply@{\the\c@pgf@countb}{\noexpand\anglestep}%
						\noexpand\pgfmathmultiply@{\noexpand\pgfmathresult}{2}%
						\noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\startangle}%
						\noexpand\let\noexpand\angle\noexpand\pgfmathresult%
						\noexpand\pgfpointadd{\noexpand\centerpoint}%
							{\noexpand\pgfqpointpolar{\noexpand\angle}{\noexpand\anchorouterradius}}%
					}%
				}{\c@pgf@counta0\relax}%
			\advance\c@pgf@counta-1\relax%
		\repeatpgfmathloop%	
	}%
}




% Keys for shape regular polygon
%
% /pgf/regular polygon sides 
%
\pgfkeys{/pgf/.cd,
	regular polygon sides/.initial=5,
	regular polygon rotate/.style={/pgf/shape border rotate=#1}% For compatability with 1.18
}


% Shape Regular Polygon.
%
\pgfdeclareshape{regular polygon}{
	\savedmacro\sides{%
		\pgfmathtruncatemacro\sides{\pgfkeysvalueof{/pgf/regular polygon sides}}%
	}
	\savedmacro\anglestep{%
		\pgfmathdivide{360}{\pgfkeysvalueof{/pgf/regular polygon sides}}%
		\let\anglestep\pgfmathresult%
	}
	\savedmacro\calculateradii{%
		%
		% Get the node dimensions.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		\ifdim\pgf@y>\pgf@x%
			\pgf@x\pgf@y%
		\fi%
		%
		% Calculate i, the incircle radius 
		%
		\pgf@x1.41421\pgf@x%
		%
		% Calculate r, the polygon radius
		%
		% r = i / cos(360 / s / 2)
		%
		% (s = polygon sides)
		%
		\pgfmathdivide{180}{\pgfkeysvalueof{/pgf/regular polygon sides}}%
		\pgfmathsec@{\pgfmathresult}%
		\pgf@x\pgfmathresult\pgf@x%
		%
		% Accommodate the minimum width/height.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@ya>\pgf@xa%
			\pgf@xa\pgf@ya%
		\fi%
		\ifdim\pgf@x<.5\pgf@xa%
			\pgf@x.5\pgf@xa%
		\fi%
		\edef\radius{\the\pgf@x}%
		%
		% Now calculate the anchor radius from the outer sep.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@ya>\pgf@xa%
			\pgf@xa\pgf@ya%
		\fi
		%
		% Take into account the miter length.
		%
		% m = o / sin (90 - (360 / s / 2))
		%
		% (o = outer sep, s = sides)
		%
		\pgfmathdivide{180}{\pgfkeysvalueof{/pgf/regular polygon sides}}%
		\pgfmathsubtract@{90}{\pgfmathresult}%
		\pgfmathcosec@{\pgfmathresult}%
		\advance\pgf@x\pgfmathresult\pgf@xa%
		\edef\anchorradius{\the\pgf@x}%
		%
		% Save both radii.
		%
		\addtosavedmacro{\radius}%
		\addtosavedmacro{\anchorradius}%
	}
	\savedmacro\startangle{%
		\pgfmathdivide{360}{\pgfkeysvalueof{/pgf/regular polygon sides}}%
		\let\anglestep\pgfmathresult%
		\pgfmathtruncatemacro\sides{\pgfkeysvalueof{/pgf/regular polygon sides}}%
		\expandafter\ifodd\sides\relax%
			\edef\pgfmathresult{90}%
		\else%
			\pgfmathdivide@{\anglestep}{2}%
			\pgfmathsubtract@{90}{\pgfmathresult}%
		\fi%
		\pgfmathadd{\pgfmathresult}{\pgfkeysvalueof{/pgf/shape border rotate}}%
		\let\startangle\pgfmathresult%
	}
	%
	% Saved anchors.
	%
	\savedanchor{\centerpoint}{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor{\midpoint}{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%	
	%
	% Other anchors.
	%
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
 	\anchor{base}{\centerpoint\pgf@y=0pt}%
 	\anchor{north}{%
 		\calculateradii%
 		\csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{0pt}{\anchorradius}}}%
 	\anchor{south}{%
 		\calculateradii%
 		\csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{0pt}{-\anchorradius}}}%
 	\anchor{east}{%
 		\calculateradii%
 		\csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{\anchorradius}{0pt}}}%
 	\anchor{west}{%
 		\calculateradii%
 		\csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{-\anchorradius}{0pt}}}%
 	\anchor{north east}{%
 		\calculateradii%
 		\csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{\anchorradius}{\anchorradius}}}%
 	\anchor{north west}{%
 		\calculateradii%
 		\csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{-\anchorradius}{\anchorradius}}}%
 	\anchor{south east}{%
 		\calculateradii%
 		\csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{\anchorradius}{-\anchorradius}}}%
 	\anchor{south west}{%
 		\calculateradii%
 		\csname pgf@anchor@regular polygon@border\endcsname{\pgfqpoint{-\anchorradius}{-\anchorradius}}}%	
 	%
 	% Background path.
 	%
	\backgroundpath{%
		\calculateradii%
		\pgfpathmoveto{%
			\pgfpointadd{\centerpoint}{\pgfqpointpolar{\startangle}{\radius}}%
		}%
		\let\angle\startangle%
		\pgfmathloop%
			\ifnum\pgfmathcounter=\sides\relax% 
				\pgfpathclose%
			\else%
				\pgfmathadd@{\angle}{\anglestep}%
				\let\angle\pgfmathresult%
				\pgfpathlineto{%
					\pgfpointadd{\centerpoint}{\pgfqpointpolar{\angle}{\radius}}%
				}%
		\repeatpgfmathloop%	
	}%
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% Adjust the location of the external 
		% point relative to \centerpoint.
		%
		\centerpoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Get the angle of the external point to the \centerpoint.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
		%
		% Locate the appropriate sides on the polygon border...
		%
		\pgfmathsubtract@{\pgfmathresult}{\startangle}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\pgfmathdivide@{\pgfmathresult}{\anglestep}%
		\pgfmathfloor@{\pgfmathresult}%
		\pgfmathmultiply@{\pgfmathresult}{\anglestep}%
		\pgfmathadd@{\pgfmathresult}{\startangle}%
		\let\firstangle\pgfmathresult%
		\pgfmathadd@{\pgfmathresult}{\anglestep}%
		\let\secondangle\pgfmathresult%
		\calculateradii%
		%
		% ...and thus, the point on the polygon border.
		%
		\pgfpointintersectionoflines{\centerpoint}{\pgfpoint{+\externalx}{+\externaly}}%
			{%
				\pgfpointadd{\centerpoint}%
					{\pgfqpointpolar{+\firstangle}{+\anchorradius}}%
				}%	
				{%
					\pgfpointadd{\centerpoint}%
						{\pgfqpointpolar{+\secondangle}{+\anchorradius}}%
				}%	
	}
	%
	% More hackery for when the recuglar polygon is positioned using 
	% a `corner <n+1>' or `side <n+1>' anchor, where n is the maximum 
	% number of sides of any previously drawn regular polygon.
	%
	\expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@regular polygon\endcsname{%
		\c@pgf@counta\sides\relax%
		\pgfmathloop%
			\ifnum\c@pgf@counta>0\relax%
				\pgfutil@ifundefined{pgf@anchor@regular polygon@corner\space\the\c@pgf@counta}{%
				%
				% ...(manually \xdef as \gdef is normally used by \anchor)...
				%
				\expandafter\xdef\csname pgf@anchor@regular polygon@corner\space\the\c@pgf@counta\endcsname{%
					\noexpand\calculateradii%
					\noexpand\pgfmathsubtract@{\the\c@pgf@counta}{1}%
					\noexpand\pgfmathmultiply@{\noexpand\pgfmathresult}{\noexpand\anglestep}%
					\noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\startangle}%
					\noexpand\let\noexpand\angle\noexpand\pgfmathresult%
					\noexpand\pgfpointadd{\noexpand\centerpoint}%
						{\noexpand\pgfqpointpolar{\noexpand\angle}{\noexpand\anchorradius}}%
				}%
				\expandafter\xdef\csname pgf@anchor@regular polygon@side\space\the\c@pgf@counta\endcsname{%
					\noexpand\calculateradii%
					\noexpand\pgfmathsubtract@{\the\c@pgf@counta}{1}%
					\noexpand\pgfmathmultiply@{\noexpand\pgfmathresult}{\noexpand\anglestep}%
					\noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\startangle}%
					\noexpand\let\noexpand\firstangle\noexpand\pgfmathresult%
					\noexpand\pgfmathadd@{\noexpand\pgfmathresult}{\noexpand\anglestep}%
					\noexpand\let\noexpand\secondangle\noexpand\pgfmathresult%
					\noexpand\pgfpointlineattime{0.5}%
						{\noexpand\pgfpointadd{\noexpand\centerpoint}%
							{\noexpand\pgfqpointpolar{\noexpand\firstangle}{\noexpand\anchorradius}}}%
						{\noexpand\pgfpointadd{\noexpand\centerpoint}%
							{\noexpand\pgfqpointpolar{\noexpand\secondangle}{\noexpand\anchorradius}}}%
				}%
			}{\c@pgf@counta0\relax}% 
			\advance\c@pgf@counta-1\relax%
		\repeatpgfmathloop%	
	}%
}



% Keys for shape trapezium
%
% /pgf/trapezium left angle  : angle of the left side.
% /pgf/trapezium right angle : angle of the right side.

\pgfkeys{/pgf/.cd,
	trapezium left angle/.initial=60,
	trapezium right angle/.initial=60,
	trapezium angle/.style={
		/pgf/trapezium left angle=#1,
		/pgf/trapezium right angle=#1
	},%
	trapezium stretches/.is if=pgf@lib@sh@trapeziumstretches,%
	trapezium stretches body/.is if=pgf@lib@sh@trapeziumstretchesbody%
}

\newif\ifpgf@lib@sh@trapeziumstretchesbody
\newif\ifpgf@lib@sh@trapeziumstretches


% Shape trapezium.
%
\pgfdeclareshape{trapezium}{
	\savedmacro\installtrapeziumparameters{%
		%
		% Get the node dimensions.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		\ifpgfshapeborderusesincircle%
			%
			% Get the rotation (no rounding).
			%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			%
			% Use the radius of the incircle if required...
			%
			\ifdim\pgf@x<\pgf@y%
				\pgf@x\pgf@y%
			\fi%			
			\pgf@x1.41421\pgf@x%
			\pgf@y\pgf@x%
		\else%
			%
			% Get the rotation (with rounding).
			%
			\pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
			\afterassignment\pgfmath@gobbletilpgfmath@%
			\expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\ifnum\c@pgf@counta<0\relax%
				\advance\c@pgf@counta360\relax%
			\fi%
			\edef\rotate{\the\c@pgf@counta}%
			%
			% Calculate the width and height of the node
			% contents, according to any border rotation.
			%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@xc\pgf@x%
				\pgf@x\pgf@y%
				\pgf@y\pgf@xc%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@xc\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y\pgf@xc%
				\fi%
			\fi%
		\fi%
		\pgfmathmod{\pgfkeysvalueof{/pgf/trapezium left angle}}{360}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\leftangle\pgfmathresult%
		\ifdim\leftangle pt=0pt\relax%
			\def\pgfmathresult{0}%
		\else%
			\pgfmathcot@{\leftangle}%
		\fi%
		\pgf@xa2\pgf@y%
		\pgf@xa\pgfmathresult\pgf@xa%
		\pgfmathmod{\pgfkeysvalueof{/pgf/trapezium right angle}}{360}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\rightangle\pgfmathresult%
		\ifdim\rightangle pt=0pt\relax%
			\def\pgfmathresult{0}%
		\else%
			\pgfmathcot@{\rightangle}%
		\fi%
		\pgf@xb2\pgf@y%
		\pgf@xb\pgfmathresult\pgf@xb%
		%
		% Take into account minimum height and width.
		%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@y<.5\pgf@ya%
			\ifpgf@lib@sh@trapeziumstretches%
				\pgf@y.5\pgf@ya%
			\else%
				\ifpgf@lib@sh@trapeziumstretchesbody%
					\pgf@y.5\pgf@ya%
				\else%
					\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@y}}%
					\pgf@yb.5\pgf@ya%
					\pgf@yb\pgfmathresult\pgf@yb%
					\pgf@y.5\pgf@ya%
					\pgf@x\pgfmath@tonumber{\pgf@yb}\pgf@x%
					\pgf@xa\pgfmath@tonumber{\pgf@yb}\pgf@xa%
					\pgf@xb\pgfmath@tonumber{\pgf@yb}\pgf@xb%
				\fi%
			\fi%
		\fi%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgf@xc2\pgf@x%
		\ifdim\pgf@xa<0pt\relax%
			\advance\pgf@xc-\pgf@xa%
		\else%
			\advance\pgf@xc\pgf@xa%
		\fi%
		\ifdim\pgf@xb<0pt\relax%
			\advance\pgf@xc-\pgf@xb%
		\else%
			\advance\pgf@xc\pgf@xb%
		\fi%
		\ifdim\pgf@xc<\pgf@ya%
			\ifpgf@lib@sh@trapeziumstretchesbody%
				\pgf@xc-\pgf@xc%
				\advance\pgf@xc\pgf@ya%
				\advance\pgf@x.5\pgf@xc%
			\else%
				\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@xc}}%
				\pgf@ya\pgfmathresult\pgf@ya%
				\pgf@x\pgfmath@tonumber{\pgf@ya}\pgf@x%
				\pgf@xa\pgfmath@tonumber{\pgf@ya}\pgf@xa%
				\pgf@xb\pgfmath@tonumber{\pgf@ya}\pgf@xb%
				\ifpgf@lib@sh@trapeziumstretches%	
				\else%					
					\pgf@y\pgfmath@tonumber{\pgf@ya}\pgf@y%
				\fi%				
			\fi%
		\fi%
		\edef\halfheight{\the\pgf@y}%
		\edef\halfwidth{\the\pgf@x}%
		\edef\leftextension{\the\pgf@xa}%
		\edef\rightextension{\the\pgf@xb}%
		\pgf@xc2\pgf@x%
		%
		% Take the larger of the outer sep.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@y>\pgf@x%
			\pgf@x\pgf@y%
		\fi%
		\edef\outersep{\the\pgf@x}%
		%
		% The \externalradius is a length that is
		% guarenteed to produce a point outside the trapezium.
		%
		\advance\pgf@xc2.0\pgf@x%
		\pgf@yc\halfheight\relax%
		\multiply\pgf@yc2\relax%
		\advance\pgf@yc2.0\pgf@x%
		\ifdim\pgf@xc<\pgf@yc%
			\edef\externalradius{\the\pgf@yc}%
		\else%
			\edef\externalradius{\the\pgf@xc}%
		\fi%
		%
		% Calculate the centre base and mid poins of the node.
		%
		\pgfextract@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		\pgfextract@process\basepoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y0pt\relax%
		}%
		\pgfextract@process\midpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgfmathsetlength\pgf@y{+.5ex}%
		}%
		%
		% Calculate each point on the trapezium (without rotation).
		%
		\pgfextract@process\lowerleftpoint{%
			\centerpoint%
			\advance\pgf@x-\halfwidth\relax%
			\ifdim\leftextension>0pt\relax%
				\advance\pgf@x-\leftextension\relax%
			\fi%
			\advance\pgf@y-\halfheight\relax%
		}%
		\pgfextract@process\upperleftpoint{%
			\centerpoint%
			\advance\pgf@x-\halfwidth\relax%
			\ifdim\leftextension<0pt\relax%
				\advance\pgf@x\leftextension\relax%
			\fi%
			\advance\pgf@y\halfheight\relax%
		}%
		\pgfextract@process\upperrightpoint{%
			\centerpoint%
			\advance\pgf@x\halfwidth\relax%
			\ifdim\rightextension<0pt\relax%
				\advance\pgf@x-\rightextension\relax%
			\fi%
			\advance\pgf@y\halfheight\relax%
		}%
		\pgfextract@process\lowerrightpoint{%
			\centerpoint%
			\advance\pgf@x\halfwidth\relax%
			\ifdim\rightextension>0pt\relax%
				\advance\pgf@x\rightextension\relax%
			\fi%
			\advance\pgf@y-\halfheight\relax%
		}%
		%
		% Now calculate the adjustment for the miter length at each corner 
		% of the trapezium. This ensures more accurate anchor positioning
		% when the line width is particularly thick.
		%
		\pgfextract@process\lowerleftmiter{%
			\pgfmathanglebetweenlines{\lowerleftpoint}{\lowerrightpoint}{\lowerleftpoint}{\upperleftpoint}%
			\pgfmathmultiply@{\pgfmathresult}{.5}%
			\pgfmathtan@{\pgfmathresult}%	
			\pgfmathreciprocal@{\pgfmathresult}%
			\pgf@x-\outersep\relax%
			\pgf@x\pgfmathresult\pgf@x%
			\pgf@y-\outersep\relax%
		}%
		\pgfextract@process\upperleftmiter{%
			\pgfmathanglebetweenlines{\upperleftpoint}{\lowerleftpoint}{\upperleftpoint}{\upperrightpoint}%
			\pgfmathmultiply@{\pgfmathresult}{.5}%
			\pgfmathtan@{\pgfmathresult}%
			\pgfmathreciprocal@{\pgfmathresult}%
			\pgf@x-\outersep\relax%
			\pgf@x\pgfmathresult\pgf@x%
			\pgf@y\outersep\relax%
		}%
		\pgfextract@process\upperrightmiter{%
			\pgfmathanglebetweenlines{\upperrightpoint}{\upperleftpoint}{\upperrightpoint}{\lowerrightpoint}%
			\pgfmathmultiply@{\pgfmathresult}{.5}%
			\pgfmathtan@{\pgfmathresult}%
			\pgfmathreciprocal@{\pgfmathresult}%
			\pgf@x\outersep\relax%
			\pgf@x\pgfmathresult\pgf@x%
			\pgf@y\outersep\relax%
		}%
		\pgfextract@process\lowerrightmiter{%
			\pgfmathanglebetweenlines{\lowerrightpoint}{\upperrightpoint}{\lowerrightpoint}{\lowerleftpoint}%
			\pgfmathmultiply@{\pgfmathresult}{.5}%
			\pgfmathtan@{\pgfmathresult}%
			\pgfmathreciprocal@{\pgfmathresult}%
			\pgf@x\outersep\relax%
			\pgf@x\pgfmathresult\pgf@x%
			\pgf@y-\outersep\relax%
		}%
		%
		% Now calculate the corners for determining anchor border
		% points, by adding the adjustment for the miter length.
		%
		\pgfextract@process\lowerleftborderpoint{%
			\pgfpointadd{\lowerleftpoint}{\lowerleftmiter}%
		}%
		\pgfextract@process\upperleftborderpoint{%
			\pgfpointadd{\upperleftpoint}{\upperleftmiter}%
		}%
		\pgfextract@process\upperrightborderpoint{%
			\pgfpointadd{\upperrightpoint}{\upperrightmiter}%
		}%
		\pgfextract@process\lowerrightborderpoint{%
			\pgfpointadd{\lowerrightpoint}{\lowerrightmiter}%
		}%
		%
		% Calulate the angle from the centerpoint to each corner.
		% Rotation is not important here (see \anchorborder code).
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\lowerleftborderpoint}%
		\let\angletolowerleft\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\upperleftborderpoint}%
		\let\angletoupperleft\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\upperrightborderpoint}%
		\let\angletoupperright\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\lowerrightborderpoint}%
		\let\angletolowerright\pgfmathresult%
		%
		% Do the same for the *inversely rotated* base point...
		%
		\pgfextract@process\rotatedbasepoint{%
			\pgfmathrotatepointaround{\basepoint}{\centerpoint}{-\rotate}%
		}%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\lowerleftborderpoint}%
		\let\baseangletolowerleft\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\upperleftborderpoint}%
		\let\baseangletoupperleft\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\upperrightborderpoint}%
		\let\baseangletoupperright\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\lowerrightborderpoint}%
		\let\baseangletolowerright\pgfmathresult%
		%
		% And the *inversely rotated* mid point...
		%
		\pgfextract@process\rotatedmidpoint{%
			\pgfmathrotatepointaround{\midpoint}{\centerpoint}{-\rotate}%
		}%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\lowerleftborderpoint}%
		\let\midangletolowerleft\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\upperleftborderpoint}%
		\let\midangletoupperleft\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\upperrightborderpoint}%
		\let\midangletoupperright\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\lowerrightborderpoint}%
		\let\midangletolowerright\pgfmathresult%
		%
		% Now rotate the border points around the centerpoint...
		%
		\pgfextract@process\lowerleftborderpoint{%
			\pgfmathrotatepointaround%
				{\lowerleftborderpoint}%
				{\centerpoint}%
				{\rotate}%
		}%
		\pgfextract@process\upperleftborderpoint{%
			\pgfmathrotatepointaround%
				{\upperleftborderpoint}%
				{\centerpoint}%
				{\rotate}%
		}%
		\pgfextract@process\upperrightborderpoint{%
			\pgfmathrotatepointaround%
				{\upperrightborderpoint}%
				{\centerpoint}%
				{\rotate}%
		}%
		\pgfextract@process\lowerrightborderpoint{%
			\pgfmathrotatepointaround%
				{\lowerrightborderpoint}%
				{\centerpoint}%
				{\rotate}%
		}%
		%
		% ...and the points for drawing the border (i.e. no outer sep).
		%
		\pgfextract@process\lowerleftpoint{%
			\pgfmathrotatepointaround{\lowerleftpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\upperleftpoint{%
			\pgfmathrotatepointaround{\upperleftpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\upperrightpoint{%
			\pgfmathrotatepointaround{\upperrightpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\lowerrightpoint{%
			\pgfmathrotatepointaround{\lowerrightpoint}{\centerpoint}{\rotate}%
		}%			
		%
		% And finally, save all the relevant stuff.
		%
		\addtosavedmacro{\lowerleftpoint}%
		\addtosavedmacro{\upperleftpoint}%
		\addtosavedmacro{\upperrightpoint}%
		\addtosavedmacro{\lowerrightpoint}%
    %
		\addtosavedmacro{\lowerleftborderpoint}%
		\addtosavedmacro{\upperleftborderpoint}%
		\addtosavedmacro{\upperrightborderpoint}%
		\addtosavedmacro{\lowerrightborderpoint}%
    %
		\addtosavedmacro{\angletolowerleft}%
		\addtosavedmacro{\angletoupperleft}%
		\addtosavedmacro{\angletoupperright}%
		\addtosavedmacro{\angletolowerright}%
		%
		\addtosavedmacro{\baseangletolowerleft}%
		\addtosavedmacro{\baseangletoupperleft}%
		\addtosavedmacro{\baseangletoupperright}%
		\addtosavedmacro{\baseangletolowerright}%
		%
		\addtosavedmacro{\midangletolowerleft}%
		\addtosavedmacro{\midangletoupperleft}%
		\addtosavedmacro{\midangletoupperright}%
		\addtosavedmacro{\midangletolowerright}%
    %
    \addtosavedmacro{\rotate}%
    \addtosavedmacro{\externalradius}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt\relax%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\anchor{center}{\centerpoint}%
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\installtrapeziumparameters%
		\let\pgf@trapeziumanchorborderreferencepoint\basepoint%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{base west}{%
		\installtrapeziumparameters%
		\let\pgf@trapeziumanchorborderreferencepoint\basepoint%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\installtrapeziumparameters%
		\let\pgf@trapeziumanchorborderreferencepoint\midpoint%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{mid west}{%
		\installtrapeziumparameters%
		\let\pgf@trapeziumanchorborderreferencepoint\midpoint%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}%
	\anchor{north}{%
		\installtrapeziumparameters%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
	}
	\anchor{south}{%
		\installtrapeziumparameters%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
	}
	\anchor{east}{%
		\installtrapeziumparameters%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{west}{%
		\installtrapeziumparameters%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}
	\anchor{north east}{%
		\installtrapeziumparameters%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
	}
	\anchor{south west}{%
		\installtrapeziumparameters%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
	}
	\anchor{south east}{%
		\installtrapeziumparameters%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
	}
	\anchor{north west}{%
		\installtrapeziumparameters%
		\csname pgf@anchor@trapezium@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
	}
	\anchor{bottom left corner}{%
		\installtrapeziumparameters%
		\lowerleftborderpoint%
	}%
	\anchor{top left corner}{%
		\installtrapeziumparameters%
		\upperleftborderpoint%
	}%
	\anchor{top right corner}{%
		\installtrapeziumparameters%
		\upperrightborderpoint%
	}%
	\anchor{bottom right corner}{%
		\installtrapeziumparameters%
		\lowerrightborderpoint%
	}%	
	\anchor{left side}{%
		\installtrapeziumparameters%
		\pgfpointlineattime{0.5}{\lowerleftborderpoint}{\upperleftborderpoint}%
	}%	
	\anchor{right side}{%
		\installtrapeziumparameters%
		\pgfpointlineattime{0.5}{\lowerrightborderpoint}{\upperrightborderpoint}%
	}%	
	\anchor{top side}{%
		\installtrapeziumparameters%
		\pgfpointlineattime{0.5}{\upperleftborderpoint}{\upperrightborderpoint}%
	}%	
	\anchor{bottom side}{%
		\installtrapeziumparameters%
		\pgfpointlineattime{0.5}{\lowerleftborderpoint}{\lowerrightborderpoint}%
	}%		
	\backgroundpath{%
		\installtrapeziumparameters%
		\pgfpathmoveto{\lowerleftpoint}%
		\pgfpathlineto{\upperleftpoint}%
		\pgfpathlineto{\upperrightpoint}%
		\pgfpathlineto{\lowerrightpoint}%
		\pgfpathclose%			
	}
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% This allows anchors base east, base west, mid east and mid west,
		% to redefine the `center' of the node to correctly calculate the
		% border points.
		%
		\pgfutil@ifundefined{pgf@trapeziumanchorborderreferencepoint}%
			{\let\referencepoint\centerpoint}%
			{\let\referencepoint\pgf@trapeziumanchorborderreferencepoint}%
		%
		% Adjust the location of the external 
		% point relative to the reference point.
		%
		\referencepoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Install the required points and angles.
		%
		\installtrapeziumparameters%
		%
		% Get the angle of the external point to the \referencepoint.
		%
		\pgfmathanglebetweenpoints{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
		%
		% *Subtract* the rotation from the external angle. This is 
		% why the border point angles do not neeed to be rotated.
		%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		%
		% Get the relevant angles for the reference point.
		%
		\let\externalangle\pgfmathresult%
		\ifx\referencepoint\basepoint%
			\let\angletoupperright\baseangletoupperright%
			\let\angletoupperleft\baseangletoupperleft%
			\let\angletolowerright\baseangletolowerright%
			\let\angletolowerleft\baseangletolowerleft%
		\else%
			\ifx\referencepoint\midpoint%
				\let\angletoupperright\midangletoupperright%
				\let\angletoupperleft\midangletoupperleft%
				\let\angletolowerright\midangletolowerright%
				\let\angletolowerleft\midangletolowerleft%
		\fi\fi%
		%
		% Find the line on the border...
		%			
		\ifdim\externalangle pt<\angletoupperright pt\relax%
			\let\firstpoint\upperrightborderpoint%
			\let\secondpoint\lowerrightborderpoint%
		\else%
			\ifdim\externalangle pt<\angletoupperleft pt\relax%
				\let\firstpoint\upperleftborderpoint%
				\let\secondpoint\upperrightborderpoint%
			\else%
				\ifdim\externalangle pt<\angletolowerleft pt\relax%
					\let\firstpoint\upperleftborderpoint%
					\let\secondpoint\lowerleftborderpoint%
				\else%
					\ifdim\externalangle pt<\angletolowerright pt\relax%
						\let\firstpoint\lowerleftborderpoint%
						\let\secondpoint\lowerrightborderpoint%
					\else%
						\let\firstpoint\upperrightborderpoint%
						\let\secondpoint\lowerrightborderpoint%
					\fi%
				\fi%
			\fi%
		\fi%
		%
		% ...and thus the point on the border.
		%
		\pgfpointintersectionoflines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
				{\firstpoint}{\secondpoint}%
	}%
}




% Shape semicircle.
%
\pgfdeclareshape{semicircle}{
	\savedmacro\installsemicircleparameters{%
		%
		% Get the larger of the outer sep.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@x<\pgf@y%
			\pgf@x\pgf@y%
		\fi%
		\edef\outersep{\the\pgf@x}%
		%
		% Get the node dimensions.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x+.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y+.5\ht\pgfnodeparttextbox%
		\advance\pgf@y+.5\dp\pgfnodeparttextbox%
		%
		% Use the radius of the incircle if required...
		%
		\ifpgfshapeborderusesincircle%
			%
			% Get the rotation (no rounding).
			%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			\ifdim\pgf@x<\pgf@y%
				\pgf@x\pgf@y%
			\fi%			
			\pgf@x1.41421\pgf@x%
			\edef\halfheight{\the\pgf@x}%
			\advance\pgf@x\pgf@x%
		\else%
			%
			% Get the rotation (with rounding).
			%
			\pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
			\afterassignment\pgfmath@gobbletilpgfmath@%
			\expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\ifnum\c@pgf@counta<0\relax%
				\advance\c@pgf@counta360\relax%
			\fi%
			\edef\rotate{\the\c@pgf@counta}%
			%
			% Calculate the width and height of the node
			% contents, according to any border rotation.
			%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@xc\pgf@x%
				\pgf@x\pgf@y%
				\pgf@y\pgf@xc%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@xc\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y\pgf@xc%
				\fi%
			\fi%
			\advance\pgf@y\pgf@y%
			\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
			\pgf@x\pgfmathresult pt\relax%
			\pgf@y.5\pgf@y%
			\edef\halfheight{\the\pgf@y}%
		\fi%
		\edef\defaultradius{\the\pgf@x}%
		%
		% Take into account minimum height and width.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@x<.5\pgf@xa%
			\pgf@x.5\pgf@xa%
		\fi%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@x<\pgf@ya%
			\pgf@x\pgf@ya%
		\fi%
		\edef\semicircleradius{\the\pgf@x}%
		%
		% Find the center/base/mid of the semi circle node.
		%		
		\pgfextract@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y+-.5\dp\pgfnodeparttextbox%
		}%
		\pgfextract@process\basepoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y0pt\relax%
		}%
		\pgfextract@process\midpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgfmathsetlength\pgf@y{+.5ex}%
		}%
		\pgfextract@process\semicirclecenterpoint{%
			\centerpoint%
			\pgf@ya\semicircleradius\relax%
			\advance\pgf@ya-\defaultradius\relax%
			%
			% The point is adjusted to make the node contents
			% appear more centered if the node is enlarged to
			% some minimum size. The factor .4 just seems OK.
			%
			\pgf@ya.4\pgf@ya% 
			\advance\pgf@y-\pgf@ya%
			\pgf@ya\halfheight\relax%
			\advance\pgf@y-\pgf@ya%	
		}%
		%
		% Add the outer sep to the radius here.
		%
		\pgf@x\semicircleradius\relax%
		\advance\pgf@x\outersep\relax%
		\edef\semicircleradius{\the\pgf@x}%
		\pgfpointdiff{\centerpoint}{\semicirclecenterpoint}%
		\ifdim\pgf@y<0pt\pgf@y-\pgf@y\fi%
		\edef\centerpointdiff{\the\pgf@y}%
		%
		% Calculate the start and end points on the border.
		%		
		\pgfextract@process\arcstartborder{%
			\semicirclecenterpoint%
			\advance\pgf@x\semicircleradius\relax%
		}%
		\pgfextract@process\arcendborder{%
			\semicirclecenterpoint%
			\advance\pgf@x-\semicircleradius\relax%
		}%
		%
		% Calculate the start and end *corner* points on the border.
		% This is needed to accommodate the outer sep.
		%
		\pgfextract@process\arcstartcorner{%
			\arcstartborder%
			\advance\pgf@y-\outersep\relax%
		}%
		\pgfextract@process\arcendcorner{%
			\arcendborder%
			\advance\pgf@y-\outersep\relax%
		}
		%
		% Now calculate all the relevant angles.
		%
		% For the center point.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\arcstartborder}%
		\let\angletoarcstartborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\arcendborder}%
		\let\angletoarcendborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\arcstartcorner}%
		\let\angletoarcstartcorner\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\arcendcorner}%
		\let\angletoarcendcorner\pgfmathresult%
		%
		% For the basepoint (rotated about the center point).
		%
		\pgfextract@process\rotatedbasepoint{%
			\pgfmathrotatepointaround{\basepoint}{\centerpoint}{-\rotate}%
		}%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\arcstartborder}%
		\let\baseangletoarcstartborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\arcendborder}%
		\let\baseangletoarcendborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\arcstartcorner}%
		\let\baseangletoarcstartcorner\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\arcendcorner}%
		\let\baseangletoarcendcorner\pgfmathresult%
		%
		% For the midpoint (rotated about the center point).
		%
		\pgfextract@process\rotatedmidpoint{%
			\pgfmathrotatepointaround{\midpoint}{\centerpoint}{-\rotate}%
		}%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\arcstartborder}%
		\let\midangletoarcstartborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\arcendborder}%
		\let\midangletoarcendborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\arcstartcorner}%
		\let\midangletoarcstartcorner\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\arcendcorner}%
		\let\midangletoarcendcorner\pgfmathresult%
		%
		% Now, rotate the semicircle points around the centerpoint.
		%
		\pgfextract@process\semicirclecenterpoint{%
			\pgfmathrotatepointaround{\semicirclecenterpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcstartborder{%
			\pgfmathrotatepointaround{\arcstartborder}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcendborder{%
			\pgfmathrotatepointaround{\arcendborder}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcstartcorner{%
			\pgfmathrotatepointaround{\arcstartcorner}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcendcorner{%
			\pgfmathrotatepointaround{\arcendcorner}{\centerpoint}{\rotate}%
		}%
		%
		% Calculate the distance between the base point and the (rotated) semicircle center.
		%
		\pgfpointdiff{\basepoint}{\semicirclecenterpoint}%
		\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
		\edef\basesemicirclecenterdiff{\pgfmathresult pt}%
		%
		% Calculate the distance between the base point and the (rotated) semicircle center.
		%
		\pgfpointdiff{\midpoint}{\semicirclecenterpoint}%
		\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
		\edef\midsemicirclecenterdiff{\pgfmathresult pt}%
		%
		% And save all the stuff.
		%
		\addtosavedmacro{\rotate}%
		\addtosavedmacro{\outersep}%
		\addtosavedmacro{\semicircleradius}%
		%
		\addtosavedmacro{\arcstartborder}%
		\addtosavedmacro{\arcendborder}%
		\addtosavedmacro{\arcstartcorner}%
		\addtosavedmacro{\arcendcorner}%
		\addtosavedmacro{\semicirclecenterpoint}%
		%
		\addtosavedmacro{\angletoarcstartborder}%
		\addtosavedmacro{\angletoarcendborder}%
		\addtosavedmacro{\angletoarcstartcorner}%
		\addtosavedmacro{\angletoarcendcorner}%
		%
		\addtosavedmacro{\centerpointdiff}%
		\addtosavedmacro{\basesemicirclecenterdiff}%
		\addtosavedmacro{\midsemicirclecenterdiff}%
		%
		\addtosavedmacro{\baseangletoarcstartborder}%
		\addtosavedmacro{\baseangletoarcendborder}%
		\addtosavedmacro{\baseangletoarcstartcorner}%
		\addtosavedmacro{\baseangletoarcendcorner}%
		%
		\addtosavedmacro{\midangletoarcstartborder}%
		\addtosavedmacro{\midangletoarcendborder}%
		\addtosavedmacro{\midangletoarcstartcorner}%
		\addtosavedmacro{\midangletoarcendcorner}%
	}
	\savedanchor{\centerpoint}{%
		\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
		\pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
		\pgfmathaddtolength\pgf@y{-.5\dp\pgfnodeparttextbox}%	
	}
	\savedanchor{\basepoint}{%
		\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
		\pgf@y0pt\relax%
	}
	\savedanchor{\midpoint}{%
		\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}
	\anchor{center}{\centerpoint}
	\anchor{base}{\basepoint}
	\anchor{base west}{%
		\installsemicircleparameters%
		\let\pgf@semicirclereferencepoint\basepoint%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpoint{-\semicircleradius}{0pt}}%
	}
	\anchor{base east}{%
		\installsemicircleparameters%
		\let\pgf@semicirclereferencepoint\basepoint%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpoint{\semicircleradius}{0pt}}%
	}
	\anchor{mid}{\midpoint}
	\anchor{mid west}{%
		\installsemicircleparameters%
		\let\pgf@semicirclereferencepoint\midpoint%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpoint{-\semicircleradius}{0pt}}%
	}
	\anchor{mid east}{%
		\installsemicircleparameters%
		\let\pgf@semicirclereferencepoint\midpoint%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpoint{\semicircleradius}{0pt}}%
	}
	\anchor{apex}{%
		\installsemicircleparameters%
		\pgfmathadd@{\rotate}{90}%
		\let\angle\pgfmathresult%
		\pgfpointadd{\semicirclecenterpoint}{\pgfqpointpolar{\angle}{\semicircleradius}}%
	}
	\anchor{arc start}{%
		\installsemicircleparameters%
		\arcstartcorner%
	}
	\anchor{arc end}{%
		\installsemicircleparameters%
		\arcendcorner%
	}
	\anchor{chord center}{%
		\installsemicircleparameters%
		\pgfpointlineattime{0.5}{\arcstartcorner}{\arcendcorner}%
	}
	\anchor{north}{%
		\installsemicircleparameters%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{90}{\semicircleradius}}%
	}
	\anchor{south}{%
		\installsemicircleparameters%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{270}{\semicircleradius}}%
	}
	\anchor{east}{%
		\installsemicircleparameters%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{0}{\semicircleradius}}%
	}
	\anchor{west}{%
		\installsemicircleparameters%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{180}{\semicircleradius}}%
	}
	\anchor{north west}{%
		\installsemicircleparameters%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{135}{\semicircleradius}}%
	}
	\anchor{south west}{%
		\installsemicircleparameters%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{225}{\semicircleradius}}%
	}
	\anchor{north east}{%
		\installsemicircleparameters%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{45}{\semicircleradius}}%
	}
	\anchor{south east}{%
		\installsemicircleparameters%
		\csname pgf@anchor@semicircle@border\endcsname{\pgfqpointpolar{315}{\semicircleradius}}%
	}
	\backgroundpath{%
		\installsemicircleparameters%
		\pgf@x\semicircleradius\relax%
		\advance\pgf@x-\outersep\relax%
		\edef\semicircleradius{\the\pgf@x}%
		\pgfpathmoveto{\pgfpointadd{\semicirclecenterpoint}{\pgfqpointpolar{\rotate}{\semicircleradius}}}%
		{%
			\pgftransformrotate{\rotate}%
			\pgfpatharc{0}{180}{\semicircleradius}%
			\pgfpathclose%	
		}%
	}
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% Check if a reference point has been defined (i.e. \midpoint or \basepoint).
		%
		\pgfutil@ifundefined{pgf@semicirclereferencepoint}%
			{\let\referencepoint\centerpoint}%
			{\let\referencepoint\pgf@semicirclereferencepoint}%
		%
		% Adjust the location of the external  point relative to the reference point.
		%
		\referencepoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Install the required points and angles.
		%
		\installsemicircleparameters%
		%
		% Get the angle of the external point to the \referencepoint.
		%
		\pgfmathanglebetweenpoints{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
		\let\externalangle\pgfmathresult%
		%
		% *Subtract* the rotation from the external angle.
		%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\angle\pgfmathresult%
		\ifx\referencepoint\basepoint%
			\let\angletoarcstartborder\baseangletoarcstartborder%
			\let\angletoarcendborder\baseangletoarcendborder%
			\let\angletoarcstartcorner\baseangletoarcstartcorner%
			\let\angletoarcendcorner\baseangletoarcendcorner%
			\let\centerpointdiff\basesemicirclecenterdiff%
		\else%
			\ifx\referencepoint\midpoint%
				\let\angletoarcstartborder\midangletoarcstartborder%
				\let\angletoarcendborder\midangletoarcendborder%
				\let\angletoarcstartcorner\midangletoarcstartcorner%
				\let\angletoarcendcorner\midangletoarcendcorner%
				\let\centerpointdiff\midsemicirclecenterdiff%
		\fi\fi%
		%
		% Determine if the line will cross the semicircle arc, or the chord.
		% 
		\ifdim\angle pt>\angletoarcstartborder pt\relax%
			\let\firstpoint\pgfutil@empty%
			\let\secondpoint\pgfutil@empty%
		\else%
			\ifdim\angle pt>\angletoarcstartcorner pt\relax%
				\let\firstpoint\arcstartcorner%
				\let\secondpoint\arcstartborder%
			\else%
				\ifdim\angle pt>\angletoarcendcorner pt\relax%
					\let\firstpoint\arcendcorner%
					\let\secondpoint\arcstartcorner%
				\else%
					\ifdim\angle pt>\angletoarcendborder pt\relax%
						\let\firstpoint\arcendborder%
						\let\secondpoint\arcendcorner%
					\else%
						\let\firstpoint\pgfutil@empty%
						\let\secondpoint\pgfutil@empty%
					\fi%
				\fi%
			\fi%
		\fi%
		\ifx\firstpoint\pgfutil@empty
			%
			% Calculate the angle from the centre of the semicircle to the
			% point on the semicircle arc which intersects the line from 
			% the external point to the reference point...
			%
			\pgfmathanglebetweenlines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
				{\semicirclecenterpoint}{\referencepoint}%
			\pgfmathsin@{\pgfmathresult}%
			\let\sineangle\pgfmathresult%
			\pgf@x\semicircleradius\relax%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@x}}%
			\let\reciprocalradius\pgfmathresult%
			\pgf@x\centerpointdiff\relax%
			\pgf@x\sineangle\pgf@x%
			\pgf@x\reciprocalradius\pgf@x%
			\pgfmathasin@{\pgfmath@tonumber{\pgf@x}}%
			\pgf@x\pgfmathresult pt\relax%
			\advance\pgf@x\externalangle pt\relax%
			\edef\angle{\pgfmath@tonumber{\pgf@x}}%
			%
			% ...and thus the point on the border.
			%
			\pgfpointadd{\semicirclecenterpoint}{\pgfqpointpolar{\angle}{\semicircleradius}}%
		\else%
			%
			% Calculate the the point where the semicircle chord intersects 
			% the line from the external point to the reference point.
			%
			\pgfpointintersectionoflines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
				{\firstpoint}{\secondpoint}%
		\fi%
	}		
}


% Keys for shape isosceles triangle
%
% /pgf/isosceles triangle apex angle : angle at the apex of the triangle.
\pgfkeys{/pgf/.cd,
	isosceles triangle apex angle/.initial=45,
	isosceles triangle stretches/.is if=pgf@lib@sh@isosceslestrianglestretches
}
\newif\ifpgf@lib@sh@isosceslestrianglestretches

\pgfdeclareshape{isosceles triangle}{
	\savedmacro\trianglepoints{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/isosceles triangle apex angle}}%
		\divide\pgf@x2\relax%
		\edef\halfapexangle{\pgfmath@tonumber{\pgf@x}}%
		\addtosavedmacro\halfapexangle%
		%
		\pgfmathtan@{\halfapexangle}%
		\let\tanhalfapexangle\pgfmathresult%
		%
		\pgfmathcot@{\halfapexangle}%
		\let\cothalfapexangle\pgfmathresult%
		%
		\pgfmathsin@{\halfapexangle}%
		\let\sinhalfapexangle\pgfmathresult%
		%
		\pgfmathreciprocal@{\pgfmathresult}%
		\let\cosechalfapexangle\pgfmathresult%
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		%
		\ifpgfshapeborderusesincircle%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			\ifdim\pgf@x<\pgf@y%
				\pgf@x\pgf@y%
			\else%
				\pgf@y\pgf@x%
			\fi%
			\pgf@x1.414213\pgf@x%
			\pgf@y1.414213\pgf@y%
			%
			\pgf@xa\pgf@x%
			\advance\pgf@xa\cosechalfapexangle\pgf@x%
			\pgf@ya\tanhalfapexangle\pgf@xa%
		\else%
			\pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
			\ifdim\pgfmathresult pt<0pt\relax%
				\pgfmathadd@{\pgfmathresult}{360}%
			\fi%
			\pgfmathsetcount\c@pgf@counta{+\pgfmathresult}%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\edef\rotate{\the\c@pgf@counta}%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@xa\pgf@x%
				\pgf@x\pgf@y%
				\pgf@y\pgf@xa%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@xa\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y\pgf@xa%
				\fi%
			\fi%
			%
			\pgf@xa2.0\pgf@x%
			\pgf@ya\tanhalfapexangle\pgf@xa%
			\advance\pgf@xa\cothalfapexangle\pgf@y%
			\advance\pgf@ya\pgf@y%			
		\fi%
		\addtosavedmacro\rotate%
		\ifdim\pgf@xa=0pt\relax%
			\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum height}}%
		\fi%
		% Adjust for minimum height and width.
		%
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@ya<.5\pgf@yb%
			\ifpgf@lib@sh@isosceslestrianglestretches%
				\pgf@ya.5\pgf@yb%
				%
				\pgfmathdivide@{\pgfmath@tonumber{\pgf@ya}}{\pgfmath@tonumber{\pgf@xa}}%
				\pgfmathatan@{\pgfmathresult}%
				\let\halfapexangle\pgfmathresult%
				%				
			\else%
				\pgf@ya.5\pgf@yb%
				\pgf@xa\cothalfapexangle\pgf@ya%
			\fi%
		\fi%
		%
		\pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@xa<\pgf@xb%
			\ifpgf@lib@sh@isosceslestrianglestretches%
				\pgf@xa\pgf@xb%
				%
				\pgfmathdivide@{\pgfmath@tonumber{\pgf@ya}}{\pgfmath@tonumber{\pgf@xa}}%
				\pgfmathatan@{\pgfmathresult}%
				\let\halfapexangle\pgfmathresult%
				%		
			\else%
				\pgf@xa\pgf@xb%
				\pgf@ya\tanhalfapexangle\pgf@xa%
			\fi%
		\fi%
		%
		%
		% Now find the ``offset height'' (h'). This is the distance from the
		% center of the node contents to the base of the triangle. 
		%
		\ifpgfshapeborderusesincircle%
			%
			% h' = H*sin(a/2) / (1+sin(a/2))
			%
			% where:
			%   H = the height of the triangle.
			%   a = the apex angle.
			%
			\pgf@xc\pgf@xa%
			\pgfmathsin@{\halfapexangle}%
			\pgf@xc\pgfmathresult\pgf@xc%
			\pgf@yc1pt\relax%
			\advance\pgf@yc\pgfmathresult pt\relax%
			\pgfmathdivide@{\pgfmath@tonumber{\pgf@xc}}{\pgfmath@tonumber{\pgf@yc}}
			\pgfutil@tempdima\pgfmathresult pt\relax%
		\else%
			%
			% h' = 0.5*h + (0.5*(W-w)*cos(a/2) - h*sin(a/2))/(1+sin(a/2))
			%
			% where:
			%   h = the height of the node contents.
			%   w = the width of the node contents.
			%   W = the width of the triangle.
			%   a = the apex angle.
			%
			\pgf@xc\pgf@ya%
			\advance\pgf@xc-\pgf@y%
			\pgfmathcos@{\halfapexangle}%
			\pgf@xc\pgfmathresult\pgf@xc%
			\pgfmathsin@{\halfapexangle}%
			\advance\pgf@xc-\pgfmathresult\pgf@x%
			\advance\pgf@xc-\pgfmathresult\pgf@x%
			\pgf@yc\pgfmathresult pt\relax%
			\advance\pgf@yc1pt\relax%
			\pgfmathdivide@{\pgfmath@tonumber{\pgf@xc}}{\pgfmath@tonumber{\pgf@yc}}%
			\pgfutil@tempdima\pgfmathresult pt\relax%
			\advance\pgfutil@tempdima\pgf@x%	
		\fi%
		\pgfextract@process\apex{%
			\pgf@y0pt%
			\pgf@x\pgf@xa%
			\advance\pgf@x-\pgfutil@tempdima%
		}%
		\addtosavedmacro\apex%
		%
		\pgfextract@process\lowerleft{%
			\pgf@y\pgf@ya%
			\pgf@x-\pgfutil@tempdima%
		}%
		\addtosavedmacro\lowerleft%
		%
		\pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@xb<\pgf@yb%
			\pgf@xb\pgf@yb%
		\fi%
		\pgfextract@process\apexanchor{%
			\apex%
			\advance\pgf@x\cosechalfapexangle\pgf@xb%
		}%
		\addtosavedmacro\apexanchor%
		%
		\pgf@yc-\halfapexangle pt\relax%
		\advance\pgf@yc90pt\relax%
		\divide\pgf@yc2\relax%
		\pgfmathcot@{\pgfmath@tonumber{\pgf@yc}}%
		\pgfextract@process\lowerleftanchor{%
			\lowerleft%
			\advance\pgf@y\pgfmathresult\pgf@xb%
			\advance\pgf@x-\pgf@xb%
		}%
		\addtosavedmacro\lowerleftanchor%	
		%
		\pgfextract@process\lowerrightanchor{%
			\lowerleftanchor%
			\pgf@y-\pgf@y%
		}%	
		\addtosavedmacro\lowerrightanchor%	
	}
	\anchor{apex}{%
		\trianglepoints%
		\pgfpointadd{\centerpoint}{%
			\pgfmathrotatepointaround{\apexanchor}{\pgfpointorigin}{\rotate}%
		}%
	}%
	\anchor{left corner}{%
		\trianglepoints%
		\pgfpointadd{\centerpoint}{%
			\pgfmathrotatepointaround{\lowerleftanchor}{\pgfpointorigin}{\rotate}%
		}%
	}%
	\anchor{right corner}{%
		\trianglepoints%
		\pgfpointadd{\centerpoint}{%
			\pgfmathrotatepointaround{\lowerrightanchor}{\pgfpointorigin}{\rotate}%
		}%
	}%
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}%
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid west}{%
		\trianglepoints%
		\let\pgf@isoscelestriangle@referencepoint\midpoint%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{0pt}}%
	}%
	\anchor{mid east}{%
		\trianglepoints%
		\let\pgf@isoscelestriangle@referencepoint\midpoint%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{0pt}}%
	}%
	\anchor{base}{\basepoint}%
	\anchor{base west}{%
		\trianglepoints%
		\let\pgf@isoscelestriangle@referencepoint\basepoint%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{0pt}}%
	}%
	\anchor{base east}{%
		\trianglepoints%
		\let\pgf@isoscelestriangle@referencepoint\basepoint%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{0pt}}%
	}%
	\anchor{north}{%
		\trianglepoints%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{0pt}{1pt}}%
	}
	\anchor{south}{%
		\trianglepoints%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{0pt}{-1pt}}%
	}
	\anchor{east}{%
		\trianglepoints%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{0pt}}%
	}
	\anchor{west}{%
		\trianglepoints%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{0pt}}%
	}
	\anchor{north east}{%
		\trianglepoints%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{1pt}}%
	}
	\anchor{south west}{%
		\trianglepoints%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{-1pt}}%
	}
	\anchor{south east}{%
		\trianglepoints%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{1pt}{-1pt}}%
	}
	\anchor{north west}{%
		\trianglepoints%
		\csname pgf@anchor@isosceles triangle@border\endcsname{\pgfqpoint{-1pt}{1pt}}%
	}
	\anchor{left side}{%
		\trianglepoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{\pgfpointlineattime{0.5}{\lowerleftanchor}{\apexanchor}}{\centerpoint}}%
				{\centerpoint}{\rotate}%
	}
	\anchor{right side}{%
		\trianglepoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{\pgfpointlineattime{0.5}{\lowerrightanchor}{\apexanchor}}{\centerpoint}}%
				{\centerpoint}{\rotate}%
	}
	\anchor{lower side}{%
		\trianglepoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{\pgfpointlineattime{0.5}{\lowerleftanchor}{\lowerrightanchor}}{\centerpoint}}%
				{\centerpoint}{\rotate}%
	}
	\backgroundpath{%
		\trianglepoints%
		{%
			\pgftransformshift{\centerpoint}%
			\pgftransformrotate{\rotate}%
			\pgfpathmoveto{\apex}%
			\pgfpathlineto{\lowerleft}%
			\pgfpathlineto{\lowerleft\pgf@y-\pgf@y}%
			\pgfpathclose%
		}%
	}
	\anchorborder{%
		\pgfutil@ifundefined{pgf@isoscelestriangle@referencepoint}{\let\referencepoint\centerpoint}%
			{\let\referencepoint\pgf@isoscelestriangle@referencepoint}%
		\pgfextract@process\externalpoint{%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\referencepoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%		
		\trianglepoints%
		\pgfmathanglebetweenpoints{\referencepoint}{\externalpoint}%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
			\pgfmathmod@{\pgfmathresult}{360}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\externalangle\pgfmathresult%
		%
		\pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\centerpoint}{\lowerrightanchor}}%
		\ifdim\externalangle pt<\pgfmathresult pt\relax%
			\pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\centerpoint}{\lowerleftanchor}}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\centerpoint}{\apexanchor}}%
				\ifdim\externalangle pt>\pgfmathresult pt\relax%
					\let\firstpoint\apexanchor%
					\let\secondpoint\lowerleftanchor%
				\else%
					\let\firstpoint\apexanchor%
					\let\secondpoint\lowerrightanchor%
				\fi%
			\else%
				\let\firstpoint\lowerleftanchor%
				\let\secondpoint\lowerrightanchor%
			\fi%
		\else%
			\let\firstpoint\lowerrightanchor%
			\let\secondpoint\apexanchor%
		\fi%
		\pgfpointintersectionoflines{\referencepoint}{\externalpoint}%
			{\pgfmathrotatepointaround{\pgfpointadd{\centerpoint}{\firstpoint}}{\centerpoint}{\rotate}}%
			{\pgfmathrotatepointaround{\pgfpointadd{\centerpoint}{\secondpoint}}{\centerpoint}{\rotate}}%	
	}%
}




% Keys for shape kite
%
%
\pgfkeys{/pgf/.cd,
	kite upper vertex angle/.initial=120,
	kite lower vertex angle/.initial=60,
	kite vertex angles/.code={%
		\pgfutil@in@{and}{#1}%
		\ifpgfutil@in@%
			\def\pgf@marshal##1and##2\@@{%
				\pgfkeys{/pgf/kite upper vertex angle=##1}%
				\pgfkeys{/pgf/kite lower vertex angle=##2}%
			}%
			\expandafter\pgf@marshal#1\@@%
		\else%
			\pgfkeys{/pgf/kite upper vertex angle=#1}%
			\pgfkeys{/pgf/kite lower vertex angle=#1}%
		\fi%
	}%
}

% Shape kite.
%
\pgfdeclareshape{kite}{
	\savedmacro\installkiteparameters{%
		%
		% Get the larger of the outer sep.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@x<\pgf@y%
			\pgf@x\pgf@y%
		\fi%
		\edef\outersep{\the\pgf@x}%
		%
		% Calculate the centre, base and mid points of the node.
		%
		\pgfextract@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		\pgfextract@process\basepoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y0pt\relax%
		}%
		\pgfextract@process\midpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgfmathsetlength\pgf@y{+.5ex}%
		}%
		%
		% Halve the vertex angles.
		%
		\pgfmathdivide{\pgfkeysvalueof{/pgf/kite upper vertex angle}}{2}%
		\let\halfuppervertexangle\pgfmathresult%
		\pgfmathdivide{\pgfkeysvalueof{/pgf/kite lower vertex angle}}{2}%
		\let\halflowervertexangle\pgfmathresult%
		%
		% Get the node dimensions.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		\ifpgfshapeborderusesincircle%
			%
			% Get the rotation.
			%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			%
			% Get the radis of the incircle.
			%
			\ifdim\pgf@x<\pgf@y%
				\pgf@x\pgf@y%
			\fi%			
			\pgf@x1.41421\pgf@x%
			%
			% Get the distances from the upper and lower verticies
			% to the center of the incircle.
			%
			\pgfmathsin@{\halfuppervertexangle}%
			\let\sinehalfuppervertexangle\pgfmathresult%
			\pgfmathreciprocal@{\pgfmathresult}%
			\let\cosechalfuppervertexangle\pgfmathresult%
			\pgf@ya\pgfmathresult\pgf@x%
			\pgfmathsin@{\halflowervertexangle}%
			\let\sinehalflowervertexangle\pgfmathresult%
			\pgfmathreciprocal@{\pgfmathresult}%
			\pgf@yb\pgfmathresult\pgf@x%
			%
			% Now calculate vertical offset (yc) between the center of 
			% the incircle, and the intersection of the kite diagonals.
			%
		   % yc = x * cosec(a/2) - x * cot(a/2) * (sin(a/2) + sin(b/2)) * cosec(a/2 + b/2)
		   %
		   % where:
		   %   x = the incircle radius.
		   %   a = the upper vertex angle.
		   %   b = the lower vertex angle.
		   %
		   \pgf@yc\pgf@x%
		   \pgfmathadd@{\halfuppervertexangle}{\halflowervertexangle}%
		   \pgfmathcosec@{\pgfmathresult}%
		   \pgf@yc\pgfmathresult\pgf@yc%
		   \pgfmathadd@{\sinehalfuppervertexangle}{\sinehalflowervertexangle}%
        \pgf@yc\pgfmathresult\pgf@yc%
		  	\pgfmathcos@{\halfuppervertexangle}%
		  	\pgf@yc\pgfmathresult\pgf@yc%
		  	\pgf@yc-\cosechalfuppervertexangle\pgf@yc%
		  	\advance\pgf@yc\cosechalfuppervertexangle\pgf@x%
			\edef\deltay{\the\pgf@yc}%
			%
			% Now calculate the height of the kite...
			%
			\advance\pgf@ya-\pgf@yc%
			%
			% ...and the depth.
			%
			\advance\pgf@yb\pgf@yc%
			%
			% Get the half width of the widest part of the kite.
			%
			\pgfmathtan@{\halfuppervertexangle}%
			\pgf@xa\pgfmathresult\pgf@ya%			
		\else%
			\multiply\pgf@x2\relax%
			\multiply\pgf@y2\relax%
			%
			% Get the rotation (with rounding).
			%
			\pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
			\afterassignment\pgfmath@gobbletilpgfmath@%
			\expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\ifnum\c@pgf@counta<0\relax%
				\advance\c@pgf@counta360\relax%
			\fi%
			\edef\rotate{\the\c@pgf@counta}%
			%
			% Calculate the width and height of the node
			% contents, according to any border rotation.
			%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@xc\pgf@x%
				\pgf@x\pgf@y%
				\pgf@y\pgf@xc%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@xc\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y\pgf@xc%
				\fi%
			\fi%
			%
			% The node contents (total height y) extends a distance ya into the 
			% upper isosceles triangle of the kite and a distance yb into the 
			% lower isosceles triangle. Thus, the following relationships hold:
			%
			%   ya/yb = tan(b/2)/tan(a/2)
			%
			% and   y = ya + yb
			%
			% so   ya = y * sin(a/2 + b/2) / (cos(a/2) * sin(b/2))
			%
			% where:
			%   a = upper vertex angle.
			%   b = lower vertex angle.
			%
			\pgfmathadd@{\halfuppervertexangle}{\halflowervertexangle}%
			\pgfmathsin@{\pgfmathresult}%
			\pgfmathreciprocal@{\pgfmathresult}%
			\pgf@ya\pgfmathresult\pgf@y%
			\pgfmathcos@{\halfuppervertexangle}%
			\pgf@ya\pgfmathresult\pgf@ya%
			\pgfmathsin@{\halflowervertexangle}%
			\pgf@ya\pgfmathresult\pgf@ya%
			\pgf@yb\pgf@y%
			\advance\pgf@yb-\pgf@ya%
			%
			% The vertical offset between the center of the node, and
			% the intersection of the kite diagonals is given by:
			% 
			% yc = y/2 - ya
			%
			\pgf@yc.5\pgf@y%
			\advance\pgf@yc-\pgf@ya%
			\edef\deltay{\the\pgf@yc}%
			%
			% Get the half width of the widest part of the kite.
			%
			\pgfmathtan@{\halfuppervertexangle}%
			\pgf@xa.5\pgf@x%
			\advance\pgf@xa\pgfmathresult\pgf@ya%
			%
			% Now calculate the height of the kite...
			%
			\pgf@xb.5\pgf@x%
			\pgfmathreciprocal@{\pgfmathresult}%
			\advance\pgf@ya\pgfmathresult\pgf@xb%
			%
			% ...and the depth.
			%
			\pgfmathtan@{\halflowervertexangle}%
			\pgfmathreciprocal@{\pgfmathresult}%
			\advance\pgf@yb\pgfmathresult\pgf@xb%
		\fi%
		%
		% Take into account minimum height and width.
		%
		% ya is the kite height.
		% yb is the kite depth.
		% xa is the kite (half) width.
		%
		\pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/minimum height}}%
		\pgf@y\pgf@ya%
		\advance\pgf@y\pgf@yb%
		\ifdim\pgf@y<\pgf@yc%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@y}}%
			\pgf@yc\pgfmathresult\pgf@yc%
			\pgf@xa\pgfmath@tonumber{\pgf@yc}\pgf@xa%
			\pgf@ya\pgfmath@tonumber{\pgf@yc}\pgf@ya%
			\pgf@yb\pgfmath@tonumber{\pgf@yc}\pgf@yb%
		\fi%
		\pgf@x2.0\pgf@xa%	
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@x<\pgf@xc%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@x}}%
			\pgf@xc\pgfmathresult\pgf@xc%
			\pgf@xa\pgfmath@tonumber{\pgf@xc}\pgf@xa%
			\pgf@ya\pgfmath@tonumber{\pgf@xc}\pgf@ya%
			\pgf@yb\pgfmath@tonumber{\pgf@xc}\pgf@yb%
		\fi%
		\edef\kitehalfwidth{\the\pgf@xa}%
		\edef\kiteheight{\the\pgf@ya}%
		\edef\kitedepth{\the\pgf@yb}%
		%
		% Calculate the basic points on the kite (for the background path).
		%
		\pgfextract@process\toppoint{%
			\centerpoint%
			\advance\pgf@y\deltay\relax%
			\advance\pgf@y\kiteheight%
		}%
		\pgfextract@process\bottompoint{%
			\centerpoint%
			\advance\pgf@y\deltay\relax%
			\advance\pgf@y-\kitedepth%
		}%
		\pgfextract@process\leftpoint{%
			\centerpoint%
			\advance\pgf@y\deltay\relax%
			\advance\pgf@x-\kitehalfwidth%
		}%
		\pgfextract@process\rightpoint{%
			\centerpoint%
			\advance\pgf@y\deltay\relax%
				\advance\pgf@x\kitehalfwidth%
		}%
		%
		% Now calculate the miter length. At the top...
		%
		\pgfmathsin@{\halfuppervertexangle}%
		\pgfmathreciprocal@{\pgfmathresult}%
		\pgf@y\outersep\relax%
		\pgf@y\pgfmathresult\pgf@y%
		\edef\topmiter{\the\pgf@y}%
		%
		% ...at the bottom...
		%
		\pgfmathsin@{\halflowervertexangle}%
		\pgfmathreciprocal@{\pgfmathresult}%
		\pgf@y\outersep\relax%
		\pgf@y\pgfmathresult\pgf@y%
		\edef\bottommiter{\the\pgf@y}%
		%
		% ...to the right...
		%
		\pgfmathsubtract@{180}{\halflowervertexangle}%
		\pgfmathsubtract@{\pgfmathresult}{\halfuppervertexangle}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\pgfmathsin@{\pgfmathresult}%
		\pgfmathreciprocal@{\pgfmathresult}%
		\pgf@xa\outersep\relax%
		\pgf@xa\pgfmathresult\pgf@xa%
		\pgfmathsubtract@{\halfuppervertexangle}{\halflowervertexangle}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\angle\pgfmathresult%
		\pgfextract@process\rightmiter{%
			\pgfqpointpolar{\angle}{\the\pgf@xa}%
		}%
		%
		% ...and to the left.
		%
		\pgfmathsubtract@{180}{\angle}%
		\let\angle\pgfmathresult%
		\pgfextract@process\leftmiter{%
			\pgfqpointpolar{\angle}{\the\pgf@xa}%
		}%
		%
		% Create the border points.
		%
		\pgfextract@process\topborderpoint{%
			\toppoint%
			\advance\pgf@y\topmiter\relax%
		}%
		\pgfextract@process\bottomborderpoint{%
			\bottompoint%
			\advance\pgf@y-\bottommiter\relax%
		}%
		\pgfextract@process\leftborderpoint{%
			\leftpoint%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\leftmiter%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfextract@process\rightborderpoint{%
			\rightpoint%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\rightmiter%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		%
		% Get the angle from the \centerpoint to the *unrotated points*.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\topborderpoint}%
		\let\angletotoppoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\leftborderpoint}%
		\let\angletoleftpoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\bottomborderpoint}%
		\let\angletobottompoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\rightborderpoint}%
		\let\angletorightpoint\pgfmathresult%
		%
		% ...from the *inversly rotated* \basepoint...
		%
		\pgfextract@process\rotatedbasepoint{%
			\pgfmathrotatepointaround{\basepoint}{\centerpoint}{-\rotate}%
		}%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\topborderpoint}%
		\let\baseangletotoppoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\leftborderpoint}%
		\let\baseangletoleftpoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\bottomborderpoint}%
		\let\baseangletobottompoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\rightborderpoint}%
		\let\baseangletorightpoint\pgfmathresult%
		%
		% ...and from the *inversely rotated* \midpoint.
		%
		\pgfextract@process\rotatedmidpoint{%
			\pgfmathrotatepointaround{\midpoint}{\centerpoint}{-\rotate}%
		}%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\topborderpoint}%
		\let\midangletotoppoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\leftborderpoint}%
		\let\midangletoleftpoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\bottomborderpoint}%
		\let\midangletobottompoint\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\rightborderpoint}%
		\let\midangletorightpoint\pgfmathresult%
		%
		% Calculate a radius guaranteed to be outside the kite.
		%
		\pgfextractx\pgf@xa{\pgfpointdiff{\leftborderpoint}{\rightborderpoint}}%
		\ifdim\pgf@xa<0pt\relax%
			\pgf@xa-\pgf@xa%
		\fi%
		\pgfextracty\pgf@ya{\pgfpointdiff{\topborderpoint}{\bottomborderpoint}}%
		\ifdim\pgf@ya<0pt\relax%
			\pgf@ya-\pgf@ya%
		\fi%
		\ifdim\pgf@ya>\pgf@xa%
			\edef\externalradius{\the\pgf@ya}%
		\else%
			\edef\externalradius{\the\pgf@xa}%
		\fi%
		%
		% Now rotate the points...
		%
		\pgfextract@process\toppoint{%
			\pgfmathrotatepointaround{\toppoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\bottompoint{%
			\pgfmathrotatepointaround{\bottompoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\leftpoint{%
			\pgfmathrotatepointaround{\leftpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\rightpoint{%
			\pgfmathrotatepointaround{\rightpoint}{\centerpoint}{\rotate}%
		}%
		%
		% ...and the border points.
		%
		\pgfextract@process\topborderpoint{%
			\pgfmathrotatepointaround{\topborderpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\bottomborderpoint{%
			\pgfmathrotatepointaround{\bottomborderpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\leftborderpoint{%
			\pgfmathrotatepointaround{\leftborderpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\rightborderpoint{%
			\pgfmathrotatepointaround{\rightborderpoint}{\centerpoint}{\rotate}%
		}%
		%
		% Now save it all.
		%
		\addtosavedmacro{\rotate}%
		\addtosavedmacro{\externalradius}%
		%
		\addtosavedmacro\toppoint%
		\addtosavedmacro\bottompoint%
		\addtosavedmacro\leftpoint%
		\addtosavedmacro\rightpoint%
		%
		\addtosavedmacro\topborderpoint%
		\addtosavedmacro\bottomborderpoint%
		\addtosavedmacro\leftborderpoint%
		\addtosavedmacro\rightborderpoint%
		%
		\addtosavedmacro\angletotoppoint%
		\addtosavedmacro\angletobottompoint%
		\addtosavedmacro\angletoleftpoint%
		\addtosavedmacro\angletorightpoint%
		%
		\addtosavedmacro\baseangletotoppoint%
		\addtosavedmacro\baseangletobottompoint%
		\addtosavedmacro\baseangletoleftpoint%
		\addtosavedmacro\baseangletorightpoint%
		%
		\addtosavedmacro\midangletotoppoint%
		\addtosavedmacro\midangletobottompoint%
		\addtosavedmacro\midangletoleftpoint%
		\addtosavedmacro\midangletorightpoint%			
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt\relax%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\anchor{center}{\centerpoint}%
	\anchor{base}{\basepoint}%
	\anchor{base west}{%
		\installkiteparameters%
		\let\pgf@kiteanchorborderreferencepoint\basepoint%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}%
	\anchor{base east}{%
		\installkiteparameters%
		\let\pgf@kiteanchorborderreferencepoint\basepoint%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}%
	\anchor{mid}{\midpoint}%
	\anchor{mid west}{%
		\installkiteparameters%
		\let\pgf@kiteanchorborderreferencepoint\midpoint%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}%
	\anchor{mid east}{%
		\installkiteparameters%
		\let\pgf@kiteanchorborderreferencepoint\midpoint%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}%
	\anchor{north}{%
		\installkiteparameters%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
	}
	\anchor{south}{%
		\installkiteparameters%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
	}
	\anchor{east}{%
		\installkiteparameters%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{west}{%
		\installkiteparameters%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}
	\anchor{north east}{%
		\installkiteparameters%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
	}
	\anchor{south west}{%
		\installkiteparameters%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
	}
	\anchor{south east}{%
		\installkiteparameters%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
	}
	\anchor{north west}{%
		\installkiteparameters%
		\csname pgf@anchor@kite@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
	}
	\anchor{upper vertex}{%
		\installkiteparameters%
		\topborderpoint}
	\anchor{lower vertex}{%
		\installkiteparameters%
		\bottomborderpoint}
	\anchor{left vertex}{%
		\installkiteparameters%
		\leftborderpoint}
	\anchor{right vertex}{%
		\installkiteparameters%
		\rightborderpoint}
	\anchor{upper left side}{%
		\installkiteparameters%
		\pgfpointlineattime{0.5}{\topborderpoint}{\leftborderpoint}}
	\anchor{lower left side}{%
		\installkiteparameters%
		\pgfpointlineattime{0.5}{\bottomborderpoint}{\leftborderpoint}}
	\anchor{upper right side}{%
		\installkiteparameters%
		\pgfpointlineattime{0.5}{\topborderpoint}{\rightborderpoint}}
	\anchor{lower right side}{%
		\installkiteparameters%
		\pgfpointlineattime{0.5}{\bottomborderpoint}{\rightborderpoint}}
	\backgroundpath{%
		\installkiteparameters%
		\pgfpathmoveto{\toppoint}%
		\pgfpathlineto{\leftpoint}%
		\pgfpathlineto{\bottompoint}%
		\pgfpathlineto{\rightpoint}%
		\pgfpathclose%
	}
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% This allows anchors base east, base west, mid east and mid west,
		% to redefine the `center' of the node to correctly calculate the
		% border points.
		%
		\pgfutil@ifundefined{pgf@kiteanchorborderreferencepoint}%
			{\let\referencepoint\centerpoint}%
			{\let\referencepoint\pgf@kiteanchorborderreferencepoint}%
		%
		% Adjust the location of the external 
		% point relative to the reference point.
		%
		\referencepoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Install the required points and angles.
		%
		\installkiteparameters%
		%
		% Get the angle of the external point relative to \referencepoint.
		%
		\pgfmathanglebetweenpoints{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
		%
		% *Subtract* the rotation from the external angle.
		%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\externalangle\pgfmathresult%
		\ifx\referencepoint\basepoint%
			\let\angletotoppoint\baseangletotoppoint%
			\let\angletobottompoint\baseangletobottompoint%
			\let\angletoleftpoint\baseangletoleftpoint%
			\let\angletorightpoint\baseangletorightpoint%
		\else%
			\ifx\referencepoint\midpoint%
				\let\angletotoppoint\midangletotoppoint%
				\let\angletobottompoint\midangletobottompoint%
				\let\angletoleftpoint\midangletoleftpoint%
				\let\angletorightpoint\midangletorightpoint%
		\fi\fi%
		%
		%  Depending on the rotation, the angle to \rightborderpoint
		%  may be smaller than the angle to \topborderpoint.
		%
		\ifdim\angletorightpoint pt<\angletotoppoint pt\relax%
			\ifdim\externalangle pt<\angletorightpoint pt\relax%
				\let\firstpoint\rightborderpoint%
				\let\secondpoint\bottomborderpoint%
			\else%
				\ifdim\externalangle pt<\angletotoppoint pt\relax%
					\let\firstpoint\rightborderpoint%
					\let\secondpoint\topborderpoint%
				\else%
					\ifdim\externalangle pt<\angletoleftpoint pt\relax%
						\let\firstpoint\topborderpoint%
						\let\secondpoint\leftborderpoint%
					\else%
						\ifdim\externalangle pt<\angletobottompoint pt\relax%
							\let\firstpoint\leftborderpoint%
							\let\secondpoint\bottomborderpoint%
						\else%
							\let\firstpoint\rightborderpoint%
							\let\secondpoint\bottomborderpoint%
						\fi%
					\fi%
				\fi%
			\fi%
		\else%
			\ifdim\externalangle pt<\angletotoppoint pt\relax%
				\let\firstpoint\rightborderpoint%
				\let\secondpoint\topborderpoint%
			\else%
				\ifdim\externalangle pt<\angletoleftpoint pt\relax%
					\let\firstpoint\leftborderpoint%
					\let\secondpoint\topborderpoint%
				\else%
					\ifdim\externalangle pt<\angletobottompoint pt\relax%
						\let\firstpoint\bottomborderpoint%
						\let\secondpoint\leftborderpoint%
					\else%
						\ifdim\externalangle pt<\angletorightpoint pt\relax%
							\let\firstpoint\rightborderpoint%
							\let\secondpoint\bottomborderpoint%
						\else%
							\let\firstpoint\rightborderpoint%
							\let\secondpoint\topborderpoint%
						\fi%
					\fi%
				\fi%
			\fi%
		\fi%
		\pgfpointintersectionoflines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
				{\firstpoint}{\secondpoint}%
	}
}




% Keys for shape dart.
%
%

\pgfkeys{/pgf/.cd,
	dart tip angle/.initial=45,
	dart tail angle/.initial=135
}

% Shape dart.
%
\pgfdeclareshape{dart}{%
	\savedmacro\installdartparameters{%
		%
		% Get the halved angles (more useful).
		%
		\pgfmathdivide{\pgfkeysvalueof{/pgf/dart tip angle}}{2}%
		\let\halftipangle\pgfmathresult%
		\pgfmathdivide{\pgfkeysvalueof{/pgf/dart tail angle}}{2}%
		\let\halftailangle\pgfmathresult%
		%
		% Calculate some common results.
		%
		\pgfmathcot@{\halftipangle}%
		\let\cothalftipangle\pgfmathresult%
		%
		% Get the larger of the outer sep.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@x<\pgf@y%
			\pgf@x\pgf@y%
		\fi%
		\edef\outersep{\the\pgf@x}%
		%
		% Calculate the centre, base and mid points of the node.
		%
		\pgfextract@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		\pgfextract@process\basepoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y0pt\relax%
		}%
		\pgfextract@process\midpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgfmathsetlength\pgf@y{+.5ex}%
		}%
		%
		% Get the (halved) dimension of the node.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		%
		% Get the length of the dart tip.
		%
		\ifpgfshapeborderusesincircle%
			%
			% Get the (unrounded) rotation.
			%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			%
			% Get the radius of the incircle.
			%
			\ifdim\pgf@x<\pgf@y%
				\pgf@x\pgf@y%
			\fi%			
			\pgf@x1.41421\pgf@x%
			%
			% Calculate the length of the dart tip.
			%
			\pgf@xa\cothalftipangle\pgf@x%
			\advance\pgf@xa\pgf@x%
		\else%
			%
			% Get the rotation (with rounding).
			%
			\pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
			\afterassignment\pgfmath@gobbletilpgfmath@%
			\expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\ifnum\c@pgf@counta<0\relax%
				\advance\c@pgf@counta360\relax%
			\fi%
			\edef\rotate{\the\c@pgf@counta}%
			%
			% Flip the width and height of the node contents, 
			% according to the appropriate border rotation.
			%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@xc\pgf@x%
				\pgf@x\pgf@y%
				\pgf@y\pgf@xc%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@xc\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y\pgf@xc%
				\fi%
			\fi%
			%
			% Calculate the length of the dart tip.
			%
			\pgf@xa\cothalftipangle\pgf@y%
			\advance\pgf@xa2.0\pgf@x% 
		\fi%
		%
		% Get the (half) separation of the dart tails.
		%
		\pgfmathsubtract@{\halftailangle}{\halftipangle}%
		\pgfmathcosec@{\pgfmathresult}%
		\pgf@ya\pgfmathresult\pgf@xa%
		\pgfmathsin@{\halftipangle}%
		\pgf@ya\pgfmathresult\pgf@ya%
		\pgfmathcos@{\halftipangle}%
		\pgf@ya\pgfmathresult\pgf@ya%
		%
		% Get the total length of the dart...
		%
		\pgf@xb\cothalftipangle\pgf@ya%
		%
		% and hence the length of the tails. 
		%
		\pgf@xc-\pgf@xa%
		\advance\pgf@xc\pgf@xb%
		%
		% Adjust for minimum height (length of the dart).
		%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@xb<\pgf@y%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@xb}}%
			\pgf@y\pgfmathresult\pgf@y%
			\pgf@xa\pgfmath@tonumber{\pgf@y}\pgf@xa%
			\pgf@xc\pgfmath@tonumber{\pgf@y}\pgf@xc%
			\pgf@ya\pgfmath@tonumber{\pgf@y}\pgf@ya%
			\pgf@x\pgfmath@tonumber{\pgf@y}\pgf@x%
		\fi%
		%
		% Adjust for minimum width (tail separation length).
		%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgf@y.5\pgf@y%
		\ifdim\pgf@ya<\pgf@y%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@ya}}%
			\pgf@ya\pgf@y%
			\pgf@y\pgfmathresult\pgf@y%
			\pgf@xa\pgfmath@tonumber{\pgf@y}\pgf@xa%
			\pgf@xc\pgfmath@tonumber{\pgf@y}\pgf@xc%
			\pgf@x\pgfmath@tonumber{\pgf@y}\pgf@x%
		\fi%
		\edef\dartlength{\the\pgf@xa}%
		\edef\deltax{\the\pgf@x}%
		\edef\taillength{\the\pgf@xc}%
		\edef\halftailseparation{\the\pgf@ya}
		%
		% Create the basic points on the dart (for the backgroundo path).
		%
		\pgfextract@process\tippoint{%
			\centerpoint%
			\advance\pgf@x\dartlength\relax%
			\advance\pgf@x-\deltax\relax%
		}%
		\pgfextract@process\tailcenterpoint{%
			\centerpoint%
			\advance\pgf@x-\deltax\relax%
		}%
		\pgfextract@process\lefttailpoint{%
			\centerpoint%
			\advance\pgf@x-\deltax\relax%
			\advance\pgf@x-\taillength\relax%
			\advance\pgf@y\halftailseparation\relax%
		}%
		\pgfextract@process\righttailpoint{%
			\centerpoint%
			\advance\pgf@x-\deltax\relax%
			\advance\pgf@x-\taillength\relax%
			\advance\pgf@y-\halftailseparation\relax%
		}%
		%
		% Calculate the miter vectors. At the dart tip...
		%
		\pgfextract@process\tipmiter{%
			\pgfmathcosec@{\halftipangle}%
			\pgf@x\outersep\relax%
			\pgf@x\pgfmathresult\pgf@x%
			\pgf@y0pt\relax%
		}%
		%
		% ...at the tail center...
		%
		\pgfextract@process\tailcentermiter{%
			\pgfmathcosec@{\halftailangle}%
			\pgf@x-\outersep\relax%
			\pgf@x\pgfmathresult\pgf@x%
			\pgf@y0pt\relax%
		}%
		%
		% ...at the left tail...
		%
		\pgfmathsubtract@{\halftailangle}{\halftipangle}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\angle\pgfmathresult%
		\pgfmathcosec@{\pgfmathresult}%
		\pgf@x\outersep\relax%
		\pgf@x\pgfmathresult\pgf@x%
		\pgfmathadd@{\angle}{90}%
		\pgfmathsubtract{\pgfmathresult}{\halftailangle}%
		\pgfmathsincos@{\pgfmathresult}%
		\pgf@ya\pgfmathresultx\pgf@x%
		\pgf@xa\pgfmathresulty\pgf@x%
		\pgfextract@process\lefttailmiter{%
			\pgf@x-\pgf@xa%
			\pgf@y\pgf@ya%
		}%
		%
		% ...and the right tail.
		%
		\pgfextract@process\righttailmiter{%
			\pgf@x-\pgf@xa%
			\pgf@y-\pgf@ya%
		}%
		%
		% Create the border points.
		%
		\pgfextract@process\tipborderpoint{%
			\pgfpointadd{\tippoint}{\tipmiter}
		}%
		\pgfextract@process\tailcenterborderpoint{%
			\pgfpointadd{\tailcenterpoint}{\tailcentermiter}%
		}%
		\pgfextract@process\lefttailborderpoint{%
			\pgfpointadd{\lefttailpoint}{\lefttailmiter}%
		}%
		\pgfextract@process\righttailborderpoint{%
			\pgfpointadd{\righttailpoint}{\righttailmiter}%
		}%
		%
		% Calculate the angles between the centerpoint
		% and the *unrotated* borderpoints.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\tipborderpoint}%
		\let\angletotip\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\tailcenterborderpoint}%
		\let\angletotailcenter\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\lefttailborderpoint}%
		\let\angletolefttail\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\righttailborderpoint}%
		\let\angletorighttail\pgfmathresult%
		%
		% Calculate the angles between the *inversly rotated* 
		% basepoint and the *unrotated* borderpoints.
		%
		\pgfextract@process\rotatedbasepoint{%
			\pgfmathrotatepointaround{\basepoint}{\centerpoint}{-\rotate}%
		}%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\tipborderpoint}%
		\let\baseangletotip\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\tailcenterborderpoint}%
		\let\baseangletotailcenter\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\lefttailborderpoint}%
		\let\baseangletolefttail\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedbasepoint}{\righttailborderpoint}%
		\let\baseangletorighttail\pgfmathresult%
		%
		% Calculate the angles between the *inversly rotated* 
		% midpoint and the *unrotated* borderpoints.
		%
		\pgfextract@process\rotatedmidpoint{%
			\pgfmathrotatepointaround{\midpoint}{\centerpoint}{-\rotate}%
		}%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\tipborderpoint}%
		\let\midangletotip\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\tailcenterborderpoint}%
		\let\midangletotailcenter\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\lefttailborderpoint}%
		\let\midangletolefttail\pgfmathresult%
		\pgfmathanglebetweenpoints{\rotatedmidpoint}{\righttailborderpoint}%
		\let\midangletorighttail\pgfmathresult%
		%
		% Rotate the background path points.
		%
		\pgfextract@process\tippoint{%
			\pgfmathrotatepointaround{\tippoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\tailcenterpoint{%
			\pgfmathrotatepointaround{\tailcenterpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\lefttailpoint{%
			\pgfmathrotatepointaround{\lefttailpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\righttailpoint{%
			\pgfmathrotatepointaround{\righttailpoint}{\centerpoint}{\rotate}%
		}%
		%
		% Calculate a radius guaranteed to be outside the dart.
		%
		\pgfextractx\pgf@xa{\pgfpointdiff{\lefttailborderpoint}{\tipborderpoint}}%
		\pgfextracty\pgf@ya{\pgfpointdiff{\lefttailborderpoint}{\righttailborderpoint}}%
		\ifdim\pgf@xa<0pt\relax%
			\pgf@xa-\pgf@xa%
		\fi%
		\ifdim\pgf@ya<0pt\relax%
			\pgf@ya-\pgf@ya%
		\fi%
		\ifdim\pgf@xa>\pgf@ya%
			\edef\externalradius{\the\pgf@xa}%
		\else%
			\edef\externalradius{\the\pgf@ya}%
		\fi%
		%
		% Rotate the border anchor points.
		%
		\pgfextract@process\tipborderpoint{%
			\pgfmathrotatepointaround{\tipborderpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\tailcenterborderpoint{%
			\pgfmathrotatepointaround{\tailcenterborderpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\lefttailborderpoint{%
			\pgfmathrotatepointaround{\lefttailborderpoint}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\righttailborderpoint{%
			\pgfmathrotatepointaround{\righttailborderpoint}{\centerpoint}{\rotate}%
		}%
		%
		% Save everything.
		%
		\addtosavedmacro{\rotate}%
		\addtosavedmacro{\externalradius}%
		%
		\addtosavedmacro{\tippoint}%
		\addtosavedmacro{\tailcenterpoint}%
		\addtosavedmacro{\lefttailpoint}%
		\addtosavedmacro{\righttailpoint}%
		%
		\addtosavedmacro{\tipborderpoint}%
		\addtosavedmacro{\tailcenterborderpoint}%
		\addtosavedmacro{\lefttailborderpoint}%
		\addtosavedmacro{\righttailborderpoint}%
		%
		\addtosavedmacro{\angletotip}%
		\addtosavedmacro{\angletotailcenter}%
		\addtosavedmacro{\angletolefttail}%
		\addtosavedmacro{\angletorighttail}%
		%
		\addtosavedmacro{\baseangletotip}%
		\addtosavedmacro{\baseangletotailcenter}%
		\addtosavedmacro{\baseangletolefttail}%
		\addtosavedmacro{\baseangletorighttail}%
		%
		\addtosavedmacro{\midangletotip}%
		\addtosavedmacro{\midangletotailcenter}%
		\addtosavedmacro{\midangletolefttail}%
		\addtosavedmacro{\midangletorighttail}%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt\relax%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\anchor{center}{\centerpoint}%
	\anchor{base}{\basepoint}%
	\anchor{base west}{%
		\installdartparameters%
		\let\pgf@dartanchorborderreferencepoint\basepoint%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}
	\anchor{base east}{%
		\installdartparameters%
		\let\pgf@dartanchorborderreferencepoint\basepoint%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{mid}{\midpoint}%
	\anchor{mid west}{%
		\installdartparameters%
		\let\pgf@dartanchorborderreferencepoint\midpoint%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}
	\anchor{mid east}{%
		\installdartparameters%
		\let\pgf@dartanchorborderreferencepoint\midpoint%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{north}{%
		\installdartparameters%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
	}
	\anchor{south}{%
		\installdartparameters%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
	}
	\anchor{east}{%
		\installdartparameters%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{west}{%
		\installdartparameters%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}
	\anchor{north east}{%
		\installdartparameters%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
	}
	\anchor{south west}{%
		\installdartparameters%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
	}
	\anchor{south east}{%
		\installdartparameters%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
	}
	\anchor{north west}{%
		\installdartparameters%
		\csname pgf@anchor@dart@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
	}
	\anchor{tip}{%
		\installdartparameters%
		\tipborderpoint}
	\anchor{left tail}{%
		\installdartparameters%
		\lefttailborderpoint}
	\anchor{right tail}{%
		\installdartparameters%
		\righttailborderpoint}
	\anchor{tail center}{%
		\installdartparameters%
		\tailcenterborderpoint}
	\anchor{left side}{%
		\installdartparameters%
		\pgfpointlineattime{0.5}{\tipborderpoint}{\lefttailborderpoint}}
	\anchor{right side}{%
		\installdartparameters%
		\pgfpointlineattime{0.5}{\tipborderpoint}{\righttailborderpoint}}
	\backgroundpath{%
		\installdartparameters%
		\pgfpathmoveto{\tippoint}%
		\pgfpathlineto{\lefttailpoint}%
		\pgfpathlineto{\tailcenterpoint}%
		\pgfpathlineto{\righttailpoint}%
		\pgfpathclose%
	}
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% This allows anchors base east, base west, mid east and mid west,
		% to redefine the `center' of the node to correctly calculate the
		% border points.
		%
		\pgfutil@ifundefined{pgf@dartanchorborderreferencepoint}%
			{\let\referencepoint\centerpoint}%
			{\let\referencepoint\pgf@dartanchorborderreferencepoint}%
		%
		% Adjust the location of the external 
		% point relative to the reference point.
		%
		\referencepoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Install the required points and angles.
		%
		\installdartparameters%
		%
		% Get the angle of the external point relative to \referencepoint.
		%
		\pgfmathanglebetweenpoints{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
		%
		% *Subtract* the rotation from the external angle.
		%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\externalangle\pgfmathresult%
		%
		% Get the set of angles for the appropriate border point.
		%
		\ifx\referencepoint\basepoint%
			\let\angletotip\baseangletotip%
			\let\angletotailcenter\baseangletotailcenter%
			\let\angletolefttail\baseangletolefttail%
			\let\angletorighttail\baseangletorighttail%
		\else%
			\ifx\referencepoint\midpoint%
				\let\angletotip\midangletotip%
				\let\angletotailcenter\midangletotailcenter%
				\let\angletolefttail\midangletolefttail%
				\let\angletorighttail\midangletorighttail%
		\fi\fi%
		%
		% Locate the appropriate line on the border...
		%
		\ifdim\externalangle pt<\angletotip pt\relax%
			\let\firstpoint\tipborderpoint%
			\let\secondpoint\righttailborderpoint%
		\else%
			\ifdim\externalangle pt<\angletolefttail pt\relax%
				\let\firstpoint\lefttailborderpoint%
				\let\secondpoint\tipborderpoint%
			\else%
				\ifdim\externalangle pt<\angletotailcenter pt\relax%
					\let\firstpoint\lefttailborderpoint%
					\let\secondpoint\tailcenterborderpoint%
				\else%
					\ifdim\externalangle pt<\angletorighttail pt\relax%
						\let\firstpoint\righttailborderpoint%
						\let\secondpoint\tailcenterborderpoint%
					\else%
						\let\firstpoint\tipborderpoint%
						\let\secondpoint\righttailborderpoint%
					\fi%
				\fi%
			\fi%
		\fi%
		%
		% ...and thus the point on the border.
		%
		\pgfpointintersectionoflines{\referencepoint}{\pgfqpoint{\externalx}{\externaly}}%
				{\firstpoint}{\secondpoint}%
	}%
}



% Keys for shape circular sector:
%
% /pgf/circular sector angle : the angle at the center of the sector.
%
\pgfkeys{/pgf/circular sector angle/.initial=60}

% Shape circular sector
%
\pgfdeclareshape{circular sector}{%
	\savedmacro\installcircularsectorparameters{%
		%
		% Define a \centerpoint, \basepoint and \midpoint.
		%
		\pgfextract@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		%
		% Get the larger of the outer sep.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@x<\pgf@y%
			\pgf@x\pgf@y%
		\fi%
		\edef\outersep{\the\pgf@x}%
		%
		% Half of the sector angle is more useful.
		%
		\pgfmathmod{\pgfkeysvalueof{/pgf/circular sector angle}}{360}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\angle\pgfmathresult%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\halfangle\pgfmathresult%
		%
		% Get some useful trigonometric stuff.
		%
		\pgfmathsin@{\halfangle}%
		\let\sinehalfangle\pgfmathresult%
		\pgfmathreciprocal@{\pgfmathresult}%
		\let\cosechalfangle\pgfmathresult%
		\pgfmathabs@{\halfangle}%
		\pgfmathcos@{\pgfmathresult}%
		\let\coshalfangle\pgfmathresult%
		\pgf@x\pgfmathresult pt\relax%
		\pgf@x\cosechalfangle\pgf@x%
		\edef\cothalfangle{\pgfmath@tonumber{\pgf@x}}%
		%
		% Calculate the miter length at the center, 
		% according to the outer sep.
		%
		\pgf@x\outersep\relax%
		\pgf@x\cosechalfangle\pgf@x%
		\edef\centermiter{\the\pgf@x}%
		%
		% Get the start and end angles of the arc.
		%
		\pgfmathsubtract@{180}{\halfangle}%
		\let\startangle\pgfmathresult%
		\pgfmathadd@{180}{\halfangle}%
		\let\endangle\pgfmathresult%
		%
		% Get (half) the node dimensions.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		%
		% Calculate the radius of the sector and the `center offset', 
		% which is the distance between the center of the node and the 
		% center of the sector.
		%
		\ifpgfshapeborderusesincircle%
			%
			% Get the rotation.
			%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			%
			% Calculate the incircle radius.
			%	
			\ifdim\pgf@x<\pgf@y%
				\pgf@x\pgf@y%
			\fi%
			\pgf@x1.41421\pgf@x%
			\pgf@xa\cosechalfangle\pgf@x% 
			%
			% xa is the radius, xb the offset.
			%
			\pgf@xb\pgf@xa%
			\advance\pgf@xa\pgf@x%
		\else%
			%
			% Get the rotation (with rounding).
			%
			\pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
			\afterassignment\pgfmath@gobbletilpgfmath@%
			\expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\ifnum\c@pgf@counta<0\relax%
				\advance\c@pgf@counta360\relax%
			\fi%
			\edef\rotate{\the\c@pgf@counta}%
			%
			% Swap the height and width for relevant angles.
			%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@xc\pgf@x%
				\pgf@x\pgf@y%
				\pgf@y\pgf@xc%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@xc\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y\pgf@xc%
				\fi%
			\fi%
			%
			% xa is the radius, xb the offset.
			%
			\pgf@xa\cosechalfangle\pgf@y%
			\pgf@xa\coshalfangle\pgf@xa%
			\advance\pgf@xa\pgf@x%
			\pgf@xb\pgf@xa% 
			\advance\pgf@xa\pgf@x%
			\pgfmathveclen@{\the\pgf@xa}{\the\pgf@y}%
			\pgf@xa\pgfmathresult pt\relax% 
		\fi%
		%
		% Adjust for minimum height and width.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgf@x.5\pgf@x%
		\pgfmathsec@{\halfangle}%
		\pgf@xc\pgfmathresult\pgf@xb%
		\ifdim\pgf@xc<0pt\relax%
			\pgf@xc-\pgf@xc%
		\fi%
		\ifdim\pgf@xc<\pgf@x%
			\pgfmathreciprocal{\pgfmath@tonumber{\pgf@xc}}% 
			\pgf@xc\pgfmathresult\pgf@x% Increase by ratio.
			\pgf@xa\pgfmath@tonumber{\pgf@xc}\pgf@xa%
			\pgf@xb\pgfmath@tonumber{\pgf@xc}\pgf@xb%
		\fi%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@xa<\pgf@y%
			\pgfmathreciprocal{\pgfmath@tonumber{\pgf@xa}}%
			\pgf@xc\pgfmathresult\pgf@y% Increase by ratio.
			\pgf@xa\pgf@y%
			\pgf@xb\pgfmath@tonumber{\pgf@xc}\pgf@xb%
		\fi%
		\edef\centeroffset{\the\pgf@xb}%
		\edef\radius{\the\pgf@xa}%
		%
		% Calculate the radius at sector border and the arc corners.
		%
		\advance\pgf@xa\outersep\relax%
		\edef\borderradius{\the\pgf@xa}%
		\pgf@x\outersep\relax%
		\pgf@x\cosechalfangle\pgf@x%
		\pgf@x\coshalfangle\pgf@x%
		\advance\pgf@xa\pgf@x%		
		\edef\cornerradius{\the\pgf@xa}%
		%
		% Calculate the *unrotated* points for the background path.
		%
		\pgfextract@process\sectorcenter{%
			\centerpoint%
			\advance\pgf@x\centeroffset%
		}%
		\pgfextract@process\arcstart{%
			\pgfqpointpolar{\startangle}{\radius}%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\sectorcenter%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		%
		% Calculate the *unrotated* points for the anchor border.
		%
		\pgfextract@process\sectorcenterborder{%
			\sectorcenter%
			\advance\pgf@x\centermiter\relax%
		}%
		\pgfextract@process\arcstartborder{%
			\pgfqpointpolar{\startangle}{\borderradius}%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\sectorcenter%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfextract@process\arcendborder{%
			\pgfqpointpolar{\endangle}{\borderradius}%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\sectorcenter%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfextract@process\arcstartcorner{%
			\pgfqpointpolar{\startangle}{\cornerradius}%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\sectorcenterborder%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfextract@process\arcendcorner{%
			\pgfqpointpolar{\endangle}{\cornerradius}%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\sectorcenterborder%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		%
		% Calculate the *unrotated* corner angles to the \centerpoint.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\sectorcenterborder}%
		\let\angletosectorcenterborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\arcstartborder}%
		\let\angletoarcstartborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\arcendborder}%
		\let\angletoarcendborder\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\arcstartcorner}%
		\let\angletoarcstartcorner\pgfmathresult%
		\pgfmathanglebetweenpoints{\centerpoint}{\arcendcorner}%
		\let\angletoarcendcorner\pgfmathresult%
		%
		% Rotate the background path points around the note center.
		%
		\pgfextract@process\sectorcenter{%
			\pgfmathrotatepointaround{\sectorcenter}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcstart{%
			\pgfmathrotatepointaround{\arcstart}{\centerpoint}{\rotate}%
		}%
		%
		% Rotate the border points around the note center.
		%
		\pgfextract@process\sectorcenterborder{%
			\pgfmathrotatepointaround{\sectorcenterborder}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcstartborder{%
			\pgfmathrotatepointaround{\arcstartborder}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcendborder{%
			\pgfmathrotatepointaround{\arcendborder}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcstartcorner{%
			\pgfmathrotatepointaround{\arcstartcorner}{\centerpoint}{\rotate}%
		}%
		\pgfextract@process\arcendcorner{%
			\pgfmathrotatepointaround{\arcendcorner}{\centerpoint}{\rotate}%
		}%
		%
		% Add the rotation to the start and end angles.
		%
		\pgfmathadd@{\startangle}{\rotate}%
		\let\startangle\pgfmathresult%
		\pgfmathadd@{\endangle}{\rotate}%
		\let\endangle\pgfmathresult%
		%
		% Save everything. 
		%
		% NB \addtosavedmacro is currently experimental. May get changed.
		%
		\addtosavedmacro{\rotate}%
		\addtosavedmacro{\centeroffset}%
		%
		\addtosavedmacro{\radius}%
		\addtosavedmacro{\borderradius}%
		\addtosavedmacro{\cornerradius}%
		%
		\addtosavedmacro{\endangle}%
		\addtosavedmacro{\startangle}%
		%
		\addtosavedmacro{\sectorcenter}%
		\addtosavedmacro{\arcstart}%
		%
		\addtosavedmacro{\sectorcenterborder}%
		\addtosavedmacro{\arcstartborder}%
		\addtosavedmacro{\arcendborder}%
		\addtosavedmacro{\arcstartcorner}%
		\addtosavedmacro{\arcendcorner}%
		%
		\addtosavedmacro{\angletosectorcenterborder}%
		\addtosavedmacro{\angletoarcstartborder}%
		\addtosavedmacro{\angletoarcendborder}%
		\addtosavedmacro{\angletoarcstartcorner}%
		\addtosavedmacro{\angletoarcendcorner}%
	}%
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt\relax%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\anchor{center}{\centerpoint}
	\anchor{base}{\basepoint}
	\anchor{mid}{\midpoint}	
	\anchor{arc start}{%
		\installcircularsectorparameters%
		\arcstartcorner%
	}
	\anchor{arc end}{%
		\installcircularsectorparameters%
		\arcendcorner%
	}
	\anchor{sector center}{%
		\installcircularsectorparameters%
		\sectorcenterborder%
	}
	\anchor{arc center}{%
		\installcircularsectorparameters%
		\pgfmathadd@{\rotate}{180}%
		\let\angle\pgfmathresult%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpointpolar{\angle}{\cornerradius}}%
	}
	\anchor{north}{%
		\installcircularsectorparameters%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{0pt}{\cornerradius}}%
	}
	\anchor{south}{%
		\installcircularsectorparameters%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{0pt}{-\cornerradius}}%
	}
	\anchor{east}{%
		\installcircularsectorparameters%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{\cornerradius}{0pt}}%
	}
	\anchor{west}{%
		\installcircularsectorparameters%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{-\cornerradius}{0pt}}%
	}
	\anchor{north west}{%
		\installcircularsectorparameters%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{-\cornerradius}{\cornerradius}}%
	}
	\anchor{south west}{%
		\installcircularsectorparameters%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{-\cornerradius}{-\cornerradius}}%
	}
	\anchor{north east}{%
		\installcircularsectorparameters%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{\cornerradius}{\cornerradius}}%
	}
	\anchor{south east}{%
		\installcircularsectorparameters%
		\csname pgf@anchor@circular sector@border\endcsname{\pgfqpoint{\cornerradius}{-\cornerradius}}%
	}
	\backgroundpath{%
		\installcircularsectorparameters%
		\pgfpathmoveto{\sectorcenter}%
		\pgfpathlineto{\arcstart}%
		\ifdim\endangle pt>360pt\relax%
			\ifdim\startangle pt>360pt\relax%
				\pgfpatharc{\startangle}{\endangle}{\radius}%
			\else%
				\pgfpatharc{\startangle}{360}{\radius}%
				\pgfpatharc{0}{\endangle}{\radius}%
			\fi%
		\else%
			\pgfpatharc{\startangle}{\endangle}{\radius}%
		\fi%
		\pgfpathclose%
	}%
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% Adjust the location of the external  point relative to \centerpoint.
		%
		\centerpoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Install the required points and angles.
		%
		\installcircularsectorparameters%
		%
		% Get the angle of the external point to the \centerpoint.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
		\let\externalangle\pgfmathresult%
		%
		% *Subtract* the rotation from the external angle.
		%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\angle\pgfmathresult%
		%
		% Determine if the line will cross the sector arc.
		% 
		\ifdim\angle pt>\angletoarcendcorner pt\relax%
			\let\firstpoint\arcendcorner%
			\let\secondpoint\sectorcenterborder%
		\else%
			\ifdim\angle pt>\angletoarcendborder pt\relax%
				\let\firstpoint\arcendborder%
				\let\secondpoint\arcendcorner%
			\else%
				\ifdim\angle pt>\angletoarcstartborder pt\relax%
					\let\firstpoint\pgfutil@empty%
					\let\secondpoint\pgfutil@empty%
				\else%
					\ifdim\angle pt>\angletoarcstartcorner pt\relax%
						\let\firstpoint\arcstartborder
						\let\secondpoint\arcstartcorner
					\else%		
						\let\firstpoint\sectorcenterborder%
						\let\secondpoint\arcstartcorner%
					\fi%
				\fi%
			\fi%
		\fi%
		\ifx\firstpoint\pgfutil@empty
			%
			% Calculate the angle from the centre of the semicircle to the
			% point on the semicircle arc which intersects the line from 
			% the external point to the reference point...
			%
			\pgfmathanglebetweenlines{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
				{\sectorcenter}{\centerpoint}%
			\pgfmathsin@{\pgfmathresult}%
			\let\sineangle\pgfmathresult%
			\pgf@x\borderradius\relax%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@x}}%
			\let\reciprocalradius\pgfmathresult%
			\pgf@x\centeroffset\relax%
			\pgf@x\sineangle\pgf@x%
			\pgf@x\reciprocalradius\pgf@x%
			\pgfmathasin@{\pgfmath@tonumber{\pgf@x}}%
			\pgf@x\pgfmathresult pt\relax%
			\advance\pgf@x\externalangle pt\relax%
			\edef\angle{\pgfmath@tonumber{\pgf@x}}%
			%
			% ...and thus the point on the border.
			%
			\pgfpointadd{\sectorcenter}{\pgfqpointpolar{\angle}{\borderradius}}%
		\else%
			%
			% Calculate the the point where the semicircle chord intersects 
			% the line from the external point to the reference point.
			%
			\pgfpointintersectionoflines{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
				{\firstpoint}{\secondpoint}%
		\fi%		
	}%
}



% Keys for shape cylinder
%
% /pgf/shape aspect              : Ratio between the x and y radii of the cylinder end.
% /pgf/cylinder uses custom fill : Use a custom fill for the cylinder.
% /pgf/cylinder end fill         : Custom color for the cylinder end.
% /pgf/cylinder body fill        : Custom color for the cylinderbody.
%

\newif\ifpgfcylinderusescustomfill
\pgfkeys{/pgf/.cd,
	cylinder uses custom fill/.is if=pgfcylinderusescustomfill,
	cylinder end fill/.initial=white,
	cylinder body fill/.initial=white
}


\pgfdeclareshape{cylinder}{%
	\savedmacro\getcylinderpoints{%
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
		\pgf@x\pgf@xc%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
		\pgf@y\pgf@yc%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		\ifpgfshapeborderusesincircle%
			\pgfmathsetmacro\rotate{\pgfkeysvalueof{/pgf/shape border rotate}}%
			\ifdim\pgf@x<\pgf@y%
				\pgf@x\pgf@y%
			\else%
				\pgf@y\pgf@x%
			\fi%
			\pgf@x1.414213\pgf@x%
			\pgf@y1.414213\pgf@y%			
		\else%
			\pgfmathmod{\pgfkeysvalueof{/pgf/shape border rotate}}{360}%
			\ifdim\pgfmathresult pt<0pt\relax%
				\pgfmathadd@{\pgfmathresult}{360}%
			\fi%
			\pgfmathsetcount\c@pgf@counta{+\pgfmathresult}%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\edef\rotate{\the\c@pgf@counta}%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@xa\pgf@x%
				\pgf@x\pgf@y%
				\pgf@y\pgf@xa%
				\pgf@yc\pgf@xc%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@xa\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y\pgf@xa%
					\pgf@yc\pgf@xc%
				\fi%
			\fi%
		\fi%
		\addtosavedmacro\rotate%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\pgfutil@tempdima\pgfshapeaspect\pgf@ya%
		\pgfutil@tempdimb\pgf@ya%
		%
		% Adjust for minimum height.
		%
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgfutil@tempdimb<.5\pgf@xc\relax%
			\pgfutil@tempdimb.5\pgf@xc%
			\pgf@ya\pgfutil@tempdimb%
		\fi%
		%
		% Calculate how far the node contents can extend into the cylinder bottom.
		%
		\pgf@yb\pgfutil@tempdimb%
		\advance\pgf@yb-\pgf@yc%
		\pgfmathdivide@{\pgfmath@tonumber{\pgf@yb}}{\pgfmath@tonumber{\pgfutil@tempdimb}}%
		\pgfmathasin@{\pgfmathresult}%
		\pgfmathcos@{\pgfmathresult}%
		\let\angle\pgfmathresult%
		\pgf@xb\pgfmathresult\pgfutil@tempdima%
		%
		% Adjust for minimum width.
		%
		\pgf@x.5\pgflinewidth%
		\advance\pgf@x2.0\pgf@xa%
		\advance\pgf@x3.0\pgfutil@tempdima%
		\advance\pgf@x-\pgf@xb%
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@x<\pgf@xc%
			\advance\pgf@xc-\pgf@x%
			\advance\pgf@xa.5\pgf@xc%
		\fi%		
		%
		% Add the larger of the outer sep to the radii.
		%
		\pgf@x\pgfutil@tempdima\relax%
		\pgf@y\pgfutil@tempdimb\relax%
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@xc>\pgf@yc%
			\advance\pgf@x\pgf@xc%
			\advance\pgf@y\pgf@xc%
			\edef\outersep{\the\pgf@xc}%
		\else%
			\advance\pgf@x\pgf@yc%
			\advance\pgf@y\pgf@yc%
			\edef\outersep{\the\pgf@yc}%
		\fi%
		\edef\xradius{\the\pgf@x}%
		\edef\yradius{\the\pgf@y}%
		\addtosavedmacro\xradius%
		\addtosavedmacro\yradius%
		\addtosavedmacro\outersep%
		%
		\pgfextract@process\cylindercenter{%
			\pgf@x\pgfutil@tempdima%
			\advance\pgf@x.5\pgflinewidth%
			\advance\pgf@x\pgf@xb%
			\pgf@x.5\pgf@x%	
			\pgf@y0pt%
		}%
		\addtosavedmacro\cylindercenter%
		%
		\pgfextract@process\beforetop{%
			\pgf@x\pgf@xa%
			\advance\pgf@x\pgfutil@tempdima%
			\advance\pgf@x.5\pgflinewidth%
			\pgf@y\pgf@ya%
		}%
		\pgfextract@process\afterbottom{%
			\pgf@x-\pgf@xa%
			\advance\pgf@x\pgf@xb%
			\pgf@y\pgf@ya%
		}%
		\addtosavedmacro\beforetop%
		\addtosavedmacro\afterbottom%		
		\pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/outer ysep}}%
		\pgfextract@process\beforetopanchor{%
			\beforetop%
			\advance\pgf@y\pgf@yc%
		}%
		\pgfextract@process\afterbottomanchor{%
			\afterbottom%
			\advance\pgf@y\pgf@yc%
		}%
		\addtosavedmacro\beforetopanchor%		
		\addtosavedmacro\afterbottomanchor%	
		%
		\beforetopanchor%
		\advance\pgf@x\xradius\relax%
		\ifdim\pgf@x>\pgf@y%
			\edef\externalradius{\the\pgf@x}%
		\else%
			\edef\externalradius{\the\pgf@y}%
		\fi%
		\addtosavedmacro\externalradius%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}%
	\anchor{center}{\centerpoint}
	\anchor{shape center}{%
		\getcylinderpoints%
		\pgfmathrotatepointaround{\pgfpointadd{\cylindercenter}{\centerpoint}}%
			{\centerpoint}{\rotate}%	
	}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\getcylinderpoints%
		\let\pgf@cylinder@referencepoint\midpoint%
		\pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{0pt}}%
	}%
	\anchor{mid west}{%
		\getcylinderpoints%
		\let\pgf@cylinder@referencepoint\midpoint%
		\pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{0pt}}%
	}%
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\getcylinderpoints%
		\let\pgf@cylinder@referencepoint\basepoint%
		\pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{0pt}}%
	}%
	\anchor{base west}{%
		\getcylinderpoints%
		\let\pgf@cylinder@referencepoint\basepoint%
		\pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{0pt}}%
	}%
	\anchor{north}{%
		\getcylinderpoints%
		\pgf@anchor@cylinder@border{\pgfqpoint{0pt}{\externalradius}}%
	}%
	\anchor{south}{%
		\getcylinderpoints%
		\pgf@anchor@cylinder@border{\pgfqpoint{0pt}{-\externalradius}}%
	}%
	\anchor{east}{%
		\getcylinderpoints%
		\pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{0pt}}%
	}%
	\anchor{west}{%
		\getcylinderpoints%
		\pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{0pt}}%
	}%
	\anchor{north east}{%
		\getcylinderpoints%
		\pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{\externalradius}}%
	}%
	\anchor{south west}{%
		\getcylinderpoints%
		\pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{-\externalradius}}%
	}%
	\anchor{south east}{%
		\getcylinderpoints%
		\pgf@anchor@cylinder@border{\pgfqpoint{\externalradius}{-\externalradius}}%
	}%
	\anchor{north west}{%
		\getcylinderpoints%
		\pgf@anchor@cylinder@border{\pgfqpoint{-\externalradius}{\externalradius}}%
	}%
	\anchor{before top}{%
		\getcylinderpoints%
		\pgfmathrotatepointaround{\pgfpointadd{\beforetopanchor}{\centerpoint}}{\centerpoint}{\rotate}%
	}
	\anchor{top}{%
		\getcylinderpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\beforetop%
				\pgf@y0pt\relax%
				\advance\pgf@x\xradius\relax%
			}{\centerpoint}}{\centerpoint}{\rotate}%
	}
	\anchor{after top}{%
		\getcylinderpoints%
		\pgfmathrotatepointaround{\pgfpointadd{\beforetopanchor\pgf@y-\pgf@y}{\centerpoint}}{\centerpoint}{\rotate}%
	}
	\anchor{before bottom}{%
		\getcylinderpoints%
		\pgfmathrotatepointaround{\pgfpointadd{\afterbottomanchor\pgf@y-\pgf@y}{\centerpoint}}{\centerpoint}{\rotate}%
	}
	\anchor{bottom}{%
		\getcylinderpoints%
		\pgfmathrotatepointaround{%
			\pgfpointadd{%
				\afterbottom%
				\pgf@y0pt\relax%
				\advance\pgf@x-\xradius\relax%
			}{\centerpoint}}{\centerpoint}{\rotate}%
	}
	\anchor{after bottom}{%
		\getcylinderpoints%
		\pgfmathrotatepointaround{\pgfpointadd{\afterbottomanchor}{\centerpoint}}{\centerpoint}{\rotate}%
	}	
	\backgroundpath{%
		\getcylinderpoints%
		{%
			\pgf@x\xradius\relax%
			\advance\pgf@x-\outersep\relax%
			\edef\xradius{\the\pgf@x}%
			\pgf@y\yradius\relax%
			\advance\pgf@y-\outersep\relax%
			\edef\yradius{\the\pgf@y}%
			\pgftransformshift{\centerpoint}%
			\pgftransformrotate{\rotate}%
			\pgfpathmoveto{\afterbottom}%
			\pgfpatharc{90}{270}{\xradius and \yradius}%
			\pgfpathlineto{\beforetop\pgf@y-\pgf@y}%
			\pgfpatharc{-90}{90}{\xradius and \yradius}%
			\pgfpathclose%
			\pgfpathmoveto{\beforetop}%
			\pgfpatharc{90}{270}{\xradius and \yradius}%
		}%
	}%
	\behindbackgroundpath{%
		\ifpgfcylinderusescustomfill%
			\getcylinderpoints%
			\pgf@x\xradius\relax%
			\advance\pgf@x-\outersep\relax%
			\edef\xradius{\the\pgf@x}%
			\pgf@y\yradius\relax%
			\advance\pgf@y-\outersep\relax%
			\edef\yradius{\the\pgf@y}%
			{%				
				\pgftransformshift{\centerpoint}%
				\pgftransformrotate{\rotate}%
				\pgfpathmoveto{\afterbottom}%
				\pgfpatharc{90}{270}{\xradius and \yradius}%
				\pgfpathlineto{\beforetop\pgf@y-\pgf@y}%
				\pgfpatharc{270}{90}{\xradius and \yradius}%
				\pgfpathclose%
				\expandafter\pgfsetfillcolor\expandafter{\pgfkeysvalueof{/pgf/cylinder body fill}}%
				\pgfusepath{fill}%
				%
				\pgfpathmoveto{\beforetop}%
				\pgfpatharc{90}{-270}{\xradius and \yradius}%
				\pgfpathclose
				\expandafter\pgfsetfillcolor\expandafter{\pgfkeysvalueof{/pgf/cylinder end fill}}%
				\pgfusepath{fill}%
			}%		
		\fi%	
	}%
	\anchorborder{%
		\pgfextract@process\externalpoint{}%
		\getcylinderpoints%
		\pgfutil@ifundefined{pgf@cylinder@referencepoint}{\let\referencepoint\centerpoint}{%
			\let\referencepoint\pgf@cylinder@referencepoint}%
		\pgfextract@process\externalpoint{%
			\externalpoint%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\referencepoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\externalangle\pgfmathresult%
		%
		\pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\afterbottomanchor}{\centerpoint}}%
		\ifdim\externalangle pt<\pgfmathresult pt\relax%
			\pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\beforetopanchor}{\centerpoint}}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathrotatepointaround{%
					\pgfmathpointintersectionoflineandarc%
						{\pgfmathrotatepointaround{\externalpoint}{\centerpoint}{-\rotate}}%
						{\pgfmathrotatepointaround{\referencepoint}{\centerpoint}{-\rotate}}%
						{%
							\beforetop%
							\pgf@xa\pgf@x%
							\centerpoint%
							\advance\pgf@x\pgf@xa%
						}%
						{0}{90}{\xradius and \yradius}%
					}{\centerpoint}{\rotate}%
			\else%
				\pgfpointintersectionoflines{%
					\pgfmathrotatepointaround{\pgfpointadd{\afterbottomanchor}{\centerpoint}}%
						{\centerpoint}{\rotate}}{%
					\pgfmathrotatepointaround{\pgfpointadd{\beforetopanchor}{\centerpoint}}%
						{\centerpoint}{\rotate}}%
					{\referencepoint}{\externalpoint}%
			\fi%
		\else%
			\pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\afterbottomanchor\pgf@y-\pgf@y}{\centerpoint}}%
			\ifdim\externalangle pt>\pgfmathresult pt\relax%
				\pgfmathanglebetweenpoints{\referencepoint}{\pgfpointadd{\beforetopanchor\pgf@y-\pgf@y}{\centerpoint}}%
				\ifdim\externalangle pt>\pgfmathresult pt\relax%
					\pgfmathrotatepointaround{%
						\pgfmathpointintersectionoflineandarc%
							{\pgfmathrotatepointaround{\externalpoint}{\centerpoint}{-\rotate}}%
							{\pgfmathrotatepointaround{\referencepoint}{\centerpoint}{-\rotate}}%
							{%
								\beforetop%
								\pgf@xa\pgf@x%
								\centerpoint
								\advance\pgf@x\pgf@xa%
							}%
							{270}{360}{\xradius and \yradius}%
						}{\centerpoint}{\rotate}%
				\else%
					\pgfpointintersectionoflines{%
						\pgfmathrotatepointaround{\pgfpointadd{\afterbottomanchor\pgf@y-\pgf@y}{\centerpoint}}%
							{\centerpoint}{\rotate}}{%
						\pgfmathrotatepointaround{\pgfpointadd{\beforetopanchor\pgf@y-\pgf@y}{\centerpoint}}%
							{\centerpoint}{\rotate}}%
						{\referencepoint}{\externalpoint}%
				\fi%
			\else%
				\pgfmathrotatepointaround{%
					\pgfmathpointintersectionoflineandarc%
						{\pgfmathrotatepointaround{\externalpoint}{\centerpoint}{-\rotate}}%
						{\pgfmathrotatepointaround{\referencepoint}{\centerpoint}{-\rotate}}%
						{%
							\afterbottom%
							\pgf@xa\pgf@x%
							\centerpoint
							\advance\pgf@x\pgf@xa%
						}%
						{90}{270}{\xradius and \yradius}%
					}{\centerpoint}{\rotate}%
			\fi%
		\fi%
	}
}


==> pgflibraryshapes.misc.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryshapes.misc.code.tex,v 1.10 2008/02/12 18:02:25 tantau Exp $


\pgfdeclareshape{cross out}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \foregroundpath{
    % store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
 }
}


\pgfdeclareshape{strike out}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \foregroundpath{
    \pgfpathmoveto{\southwest}
    \pgfpathlineto{\northeast}
 }
}

\pgfkeys{/pgf/.cd,
	rounded rectangle west arc/.initial=convex,
	rounded rectangle east arc/.initial=convex,
	rounded rectangle left arc/.style={/pgf/rounded rectangle west arc=#1},%
	rounded rectangle right arc/.code={/pgf/rounded rectangle east arc=#1},%
	rounded rectangle arc length/.initial=180%
}%

\def\pgf@lib@shapes@roundedrectangle@concave{concave}%
\def\pgf@lib@shapes@roundedrectangle@convex{convex}%

\pgfdeclareshape{rounded rectangle}{
	\savedmacro\leftarc{%
		\edef\leftarc{\pgfkeysvalueof{/pgf/rounded rectangle west arc}}%
	}
	\savedmacro\rightarc{%
		\edef\rightarc{\pgfkeysvalueof{/pgf/rounded rectangle east arc}}%
	}
	\savedmacro\roundedrectanglepoints{%
		%
		% Get half the arc angle.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/rounded rectangle arc length}}%
		\pgf@x.5\pgf@x%
		\edef\halfarcangle{\pgfmath@tonumber{\pgf@x}}%
		\addtosavedmacro\halfarcangle%		
		%
		% Get the (half) node dimensions x & y.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
                %
                % Adjust for minimum height
                %
		%
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@y<.5\pgf@yb%
		  \pgf@y.5\pgf@yb%
		\fi%
		%
		% Calculate the radii xa & ya of the arc ends.
		%
		\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rounded rectangle arc length}}%
		\pgfutil@tempdima.5\pgfutil@tempdima%
		\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgf@ya\pgfmathresult\pgf@y%
		\pgf@xa\pgf@ya%
		%
		% Calculate the width of the arc end.
		%
		\pgfmathcos@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgf@xb-\pgfmathresult\pgf@xa%
		\advance\pgf@xb\pgf@xa\relax%
		\edef\arcwidth{\the\pgf@xb}%
		\addtosavedmacro{\arcwidth}%
		%
		% Adjust for minimum width
		%
		\pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
		\advance\pgf@x\arcwidth\relax%
		\ifdim\pgf@x<.5\pgf@xb%
			\pgf@x.5\pgf@xb%
		\fi%
		\advance\pgf@x-\arcwidth\relax%
		%
		% Get the outer sep.
		%
		\pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/outer ysep}}%
		\edef\outerxsep{\the\pgf@xb}%
		\edef\outerysep{\the\pgf@yb}%
		\addtosavedmacro\outerxsep%
		\addtosavedmacro\outerysep%
		%
		\edef\xpathradius{\the\pgf@xa}%
		\edef\ypathradius{\the\pgf@ya}%
		\addtosavedmacro\xpathradius%
		\addtosavedmacro\ypathradius%
		%
		\advance\pgf@xa\pgf@xb%
		\advance\pgf@ya\pgf@yb%
		\edef\xradius{\the\pgf@xa}%
		\edef\yradius{\the\pgf@ya}%
		\addtosavedmacro\xradius%
		\addtosavedmacro\yradius%
		%
		\advance\pgf@xa-2.0\pgf@xb%
		\advance\pgf@ya-2.0\pgf@yb%
		\edef\xinnerradius{\the\pgf@xa}%
		\edef\yinnerradius{\the\pgf@ya}%
		\addtosavedmacro\xinnerradius%
		\addtosavedmacro\yinnerradius%		
		%
		\pgfextract@process\pathcornernoarc{}%
		\addtosavedmacro\pathcornernoarc%
		%
		\pgfextract@process\pathcornerconvexarc{%
			\pathcornernoarc%
			\pgf@xc\arcwidth\relax%
			\advance\pgf@x-.707106\pgf@xc
		}%
		\addtosavedmacro\pathcornerconvexarc%
		%
		\pgfextract@process\pathcornerconcavearc{%
			\pathcornernoarc%
			\advance\pgf@x\arcwidth\relax%
		}%
		\addtosavedmacro\pathcornerconcavearc%
		%
		\pgfextract@process\anchorcornernoarc{%
			\pathcornernoarc%
			\advance\pgf@x\pgf@xb%
			\advance\pgf@y\pgf@yb%
		}%
		\addtosavedmacro\anchorcornernoarc%
		%
		\pgfextract@process\anchorcornerconvexarc{%
			\pathcornerconvexarc%
			\ifdim\halfarcangle pt=90pt\relax%
			\else%
				\pgfmathsin@{\halfarcangle}%
				\pgf@xa\xpathradius\relax%
				\pgf@xa\pgfmathresult\pgf@xa%
				\pgfmathcos@{\halfarcangle}%
				\pgf@ya\ypathradius\relax%
				\pgf@ya\pgfmathresult\pgf@ya%
				%
				\pgfmathdivide@{\pgfmath@tonumber{\pgf@ya}}{\pgfmath@tonumber{\pgf@xa}}%
				\pgfmathatan@{\pgfmathresult}%
				\let\angle\pgfmathresult%				
				\pgfmathadd@{90}{\angle}%
				\pgfmathcosec@{\pgfmathresult}%
				\pgf@xb\pgfmathresult\pgf@xb%
				\pgfmathadd@{90}{\halfarcangle}%
				\pgfmathdivide@{\pgfmathresult}{2}%
				\pgfmathcos@{\pgfmathresult}%
				\advance\pgf@x\pgfmathresult\pgf@xb%
			\fi%
			\advance\pgf@y\pgf@yb%
		}%
		\addtosavedmacro\anchorcornerconvexarc%
		%
		\pgfextract@process\anchorcornerconcavearc{%
			\pathcornerconcavearc%
			\ifdim\halfarcangle pt=90pt\relax%
			\else%
				\pgfmathsin@{\halfarcangle}%
				\pgf@xa\xpathradius\relax%
				\pgf@xa\pgfmathresult\pgf@xa%
				\pgfmathcos@{\halfarcangle}%
				\pgf@ya\ypathradius\relax%
				\pgf@ya\pgfmathresult\pgf@ya%
				%
				\pgfmathdivide@{\pgfmath@tonumber{\pgf@ya}}{\pgfmath@tonumber{\pgf@xa}}%
				\pgfmathatan@{\pgfmathresult}%
				\pgfmathdivide@{\pgfmathresult}{2}%
				\let\angle\pgfmathresult%
				\pgfmathcosec@{\pgfmathresult}%
				\pgf@xb\pgfmathresult\pgf@xb%
				\pgfmathcos@{\angle}%
				\advance\pgf@x\pgfmathresult\pgf@xb%
			\fi%
			\advance\pgf@y\pgf@yb%
		}%
		\addtosavedmacro\anchorcornerconcavearc%
		%	
	}%
	\saveddimen\halflinewidth{\pgf@x.5\pgflinewidth}%
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%		
	}	
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%	
	}	
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt\relax%
	}	
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\roundedrectanglepoints%
		\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
			\csname pgf@anchor@rounded rectangle@east\endcsname%
		\else%
			\csname pgf@anchor@rounded rectangle@south east\endcsname%
		\fi%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa%
	}%
	\anchor{mid west}{%
		\roundedrectanglepoints%
		\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
			\csname pgf@anchor@rounded rectangle@west\endcsname%
		\else%
			\csname pgf@anchor@rounded rectangle@south west\endcsname%
		\fi%
		\pgf@xa\pgf@x%
		\midpoint%
		\pgf@x\pgf@xa%
	}%
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\roundedrectanglepoints%
		\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
			\csname pgf@anchor@rounded rectangle@east\endcsname%
		\else%
			\csname pgf@anchor@rounded rectangle@south east\endcsname%
		\fi%
		\pgf@y0pt%
	}%
	\anchor{base west}{%
		\roundedrectanglepoints%
		\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
			\csname pgf@anchor@rounded rectangle@west\endcsname%
		\else%
			\csname pgf@anchor@rounded rectangle@south west\endcsname%
		\fi%
		\pgf@y0pt%
	}%
	\anchor{north}{%
		\pgfpointadd{\centerpoint}{%
			\roundedrectanglepoints%
			\anchorcornernoarc%
			\pgf@x0pt%
		}%
	}%
	\anchor{east}{%
		\pgfpointadd{\centerpoint}{%
			\roundedrectanglepoints%
			\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
				\pathcornerconvexarc%
				\advance\pgf@x\arcwidth\relax%
				\advance\pgf@x\outerxsep\relax%
			\else%
				\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
					\pathcornerconcavearc%
					\advance\pgf@x-\arcwidth\relax%
					\advance\pgf@x\outerxsep\relax%
				\else%
					\anchorcornernoarc%
				\fi%
			\fi%	
			\pgf@y0pt\relax%	
		}%
	}%
	\anchor{west}{%
		\pgfpointadd{\centerpoint}{%
			\roundedrectanglepoints%
			\ifx\leftarc\pgf@lib@shapes@roundedrectangle@convex%
				\pathcornerconvexarc%
				\advance\pgf@x\arcwidth\relax%
				\advance\pgf@x\outerxsep\relax%
			\else%
				\ifx\leftarc\pgf@lib@shapes@roundedrectangle@concave%
					\pathcornerconcavearc%
					\advance\pgf@x-\arcwidth\relax%
					\advance\pgf@x\outerxsep\relax%
				\else%
					\anchorcornernoarc%
				\fi%
			\fi%	
			\pgf@x-\pgf@x%
			\pgf@y0pt\relax%	
		}%
	}%
	\anchor{south}{%
		\pgfpointadd{\centerpoint}{%
			\roundedrectanglepoints%
			\anchorcornernoarc%
			\pgf@x0pt%
			\pgf@y-\pgf@y
		}%
	}%
	\anchor{north east}{%
		\pgfpointadd{\centerpoint}{%
			\roundedrectanglepoints%
			\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
				\anchorcornerconvexarc%
			\else%
				\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
					\anchorcornerconcavearc%
				\else%
					\anchorcornernoarc%
				\fi%
			\fi%		
		}%
	}%
	\anchor{north west}{%
		\pgfpointadd{\centerpoint}{%
			\roundedrectanglepoints%
			\ifx\leftarc\pgf@lib@shapes@roundedrectangle@convex%
				\anchorcornerconvexarc%
			\else%
				\ifx\leftarc\pgf@lib@shapes@roundedrectangle@concave%
					\anchorcornerconcavearc%
				\else%
					\anchorcornernoarc%
				\fi%
			\fi%
			\pgf@x-\pgf@x%		
		}%
	}%
	\anchor{south west}{%
		\pgfpointadd{\centerpoint}{%
			\roundedrectanglepoints%
			\ifx\leftarc\pgf@lib@shapes@roundedrectangle@convex%
				\anchorcornerconvexarc%
			\else%
				\ifx\leftarc\pgf@lib@shapes@roundedrectangle@concave%
					\anchorcornerconcavearc%
				\else%
					\anchorcornernoarc%
				\fi%
			\fi%
			\pgf@x-\pgf@x%
			\pgf@y-\pgf@y%		
		}%
	}%
	\anchor{south east}{%
		\pgfpointadd{\centerpoint}{%
			\roundedrectanglepoints%
			\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
				\anchorcornerconvexarc%
			\else%
				\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
					\anchorcornerconcavearc%
				\else%
					\anchorcornernoarc%
				\fi%
			\fi%
			\pgf@y-\pgf@y%		
		}%
	}%
	\anchor{shape center}{%
		\roundedrectanglepoints%
		\pgfpointadd{\centerpoint}{%
			\pgfpointadd{%
				\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
					\pathcornerconvexarc%
				\else%
					\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
						\pathcornerconcavearc%
					\else%
						\pathcornernoarc%
					\fi%
				\fi}%
			{%
				\pgfpointadd{%
					\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
						\pathcornerconvexarc%
					\else%
						\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
							\pathcornerconcavearc%
						\else%
							\pathcornernoarc%
						\fi%
					\fi
					\pgf@x-\pgf@x}%
				{%
					\pgfpointadd{%
						\ifx\leftarc\pgf@lib@shapes@roundedrectangle@convex%
							\pathcornerconvexarc%
						\else%
							\ifx\leftarc\pgf@lib@shapes@roundedrectangle@concave%
								\pathcornerconcavearc%
							\else%
								\pathcornernoarc%
							\fi%
						\fi
						\pgf@x-\pgf@x%
						\pgf@y-\pgf@y}% 
					{%
						\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
							\pathcornerconvexarc%
						\else%
							\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
								\pathcornerconcavearc%
							\else%
								\pathcornernoarc%
							\fi%
						\fi
						\pgf@y-\pgf@y%
					}%
				}%
			}%
			\divide\pgf@x4\relax%
			\divide\pgf@y4\relax%
		}%
	}%
	\backgroundpath{%
		{%
			\pgftransformshift{\centerpoint}%
			\roundedrectanglepoints%
			%
			\pgf@x\xradius\relax%
			\pgf@y\yradius\relax%
			\advance\pgf@x-\outerxsep\relax%
			\advance\pgf@y-\outerysep\relax%
			\edef\xradius{\the\pgf@x}%
			\edef\yradius{\the\pgf@y}%
			%
			\pgfpathmoveto{%
				\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
					\pathcornerconvexarc%
				\else%
					\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
						\pathcornerconcavearc%
					\else%
						\pathcornernoarc%
					\fi%
				\fi%			
			}%
			\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
				\pgfpatharc{\halfarcangle}{-\halfarcangle}{\xradius and \yradius}%
			\else%
				\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
					\pgfpatharc{180-\halfarcangle}{180+\halfarcangle}{\xradius and \yradius}%
				\else%
					\pgfpathlineto{\pathcornernoarc\pgf@y-\pgf@y}%
				\fi%
			\fi%
			\pgfpathlineto{%
				\ifx\leftarc\pgf@lib@shapes@roundedrectangle@convex%
					\pathcornerconvexarc%
				\else%
					\ifx\leftarc\pgf@lib@shapes@roundedrectangle@concave%
						\pathcornerconcavearc%
					\else%
						\pathcornernoarc%
					\fi%
				\fi%	
				\pgf@x-\pgf@x%
				\pgf@y-\pgf@y%		
			}%
			\ifx\leftarc\pgf@lib@shapes@roundedrectangle@convex%
				\pgfpatharc{180+\halfarcangle}{180-\halfarcangle}{\xradius and \yradius}%
			\else%
				\ifx\leftarc\pgf@lib@shapes@roundedrectangle@concave%
					\pgfpatharc{-\halfarcangle}{\halfarcangle}{\xradius and \yradius}%
				\else%
					\pgfpathlineto{\pathcornernoarc\pgf@x-\pgf@x}%
				\fi%
			\fi%
			\pgfpathclose%
		}%
	}
	\anchorborder{%
		\pgfextract@process\externalpoint{%
			\pgfextract@process\externalpoint{}%
			\pgfpointadd{\centerpoint}{\externalpoint}%
		}%
		\roundedrectanglepoints%
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\let\externalangle\pgfmathresult%
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@west\endcsname}%
		\ifdim\externalangle pt<\pgfmathresult pt\relax%
			\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@north\endcsname}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@north east\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
						\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
						{%
							\csname pgf@anchor@rounded rectangle@east\endcsname%
							\advance\pgf@x-\xradius\relax%
						}%
						{0}{\halfarcangle}{\xradius and \yradius}%
					\else%
						\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
							{%
								\centerpoint%
								\pgf@xa\pgf@x%
								\pgf@ya\pgf@y%
								\pathcornernoarc%
								\advance\pgf@x\pgf@xa%
								\pgf@y\pgf@ya%
								\advance\pgf@x\xpathradius\relax%
							}%
							{180-\halfarcangle}{180}{\xinnerradius and \yinnerradius}%
						\else%
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\csname pgf@anchor@rounded rectangle@north east\endcsname}%
							{\csname pgf@anchor@rounded rectangle@south east\endcsname}%
						\fi%
					\fi%
				\else%
					\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
						{\csname pgf@anchor@rounded rectangle@north east\endcsname}%
						{\csname pgf@anchor@rounded rectangle@north west\endcsname}%
				\fi%
			\else%
				\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@north west\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
						{\csname pgf@anchor@rounded rectangle@north east\endcsname}%
						{\csname pgf@anchor@rounded rectangle@north west\endcsname}%
				\else%
					\ifx\leftarc\pgf@lib@shapes@roundedrectangle@convex%
							\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
							{%
								\csname pgf@anchor@rounded rectangle@west\endcsname%
								\advance\pgf@x\xradius\relax%
							}%
							{180-\halfarcangle}{180}{\xradius and \yradius}%
					\else%
						\ifx\leftarc\pgf@lib@shapes@roundedrectangle@concave%
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
								{%
									\centerpoint%
									\pgf@xa\pgf@x%
									\pgf@ya\pgf@y%
									\pathcornernoarc%
									\pgf@x-\pgf@x%
									\advance\pgf@x\pgf@xa%
									\pgf@y\pgf@ya%
									\advance\pgf@x-\xpathradius\relax%
								}%
								{0}{\halfarcangle}{\xinnerradius and \yinnerradius}%
						\else%
							\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
								{\csname pgf@anchor@rounded rectangle@north west\endcsname}%
								{\csname pgf@anchor@rounded rectangle@south west\endcsname}%
						\fi%
					\fi%
				\fi%
			\fi%
		\else%
			\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@south\endcsname}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@south west\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\ifx\leftarc\pgf@lib@shapes@roundedrectangle@convex%
						\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
						{%
							\csname pgf@anchor@rounded rectangle@west\endcsname%
							\advance\pgf@x\xradius\relax%
						}%
						{180}{180+\halfarcangle}{\xradius and \yradius}%
					\else%
						\ifx\leftarc\pgf@lib@shapes@roundedrectangle@concave%
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
								{%
									\centerpoint%
									\pgf@xa\pgf@x%
									\pgf@ya\pgf@y%
									\pathcornernoarc%
									\pgf@x-\pgf@x%
									\advance\pgf@x\pgf@xa%
									\pgf@y\pgf@ya%
									\advance\pgf@x-\xpathradius\relax%
								}%
								{360-\halfarcangle}{360}{\xinnerradius and \yinnerradius}%
						\else%
							\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
								{\csname pgf@anchor@rounded rectangle@north west\endcsname}%
								{\csname pgf@anchor@rounded rectangle@south west\endcsname}%
						\fi%
					\fi%
				\else%
					\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
						{\csname pgf@anchor@rounded rectangle@south west\endcsname}%
						{\csname pgf@anchor@rounded rectangle@south east\endcsname}%
				\fi%
			\else%
				\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@rounded rectangle@south east\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
						{\csname pgf@anchor@rounded rectangle@south west\endcsname}%
						{\csname pgf@anchor@rounded rectangle@south east\endcsname}%
				\else%
					\ifx\rightarc\pgf@lib@shapes@roundedrectangle@convex%
						\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
						{%
							\csname pgf@anchor@rounded rectangle@east\endcsname%
							\advance\pgf@x-\xradius\relax%
						}%
						{360-\halfarcangle}{360}{\xradius and \yradius}%
					\else%
						\ifx\rightarc\pgf@lib@shapes@roundedrectangle@concave%
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
								{%
									\centerpoint%
									\pgf@xa\pgf@x%
									\pgf@ya\pgf@y%
									\pathcornernoarc%
									\advance\pgf@x\pgf@xa%
									\pgf@y\pgf@ya%
									\advance\pgf@x\xpathradius\relax%
								}%
								{180}{180+\halfarcangle}{\xinnerradius and \yinnerradius}%
						\else%
							\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
								{\csname pgf@anchor@rounded rectangle@south east\endcsname}%
								{\csname pgf@anchor@rounded rectangle@north east\endcsname}%
						\fi%
					\fi%
				\fi%
			\fi%
		\fi%
	}%
}




% Keys for chamfered rectangle
%
% /pgf/chamfered rectangle corners : specify the corners to chamfer.
% /pgf/chamfered rectangle angle   : set the angle of the chamfer.
% /pgf/chamfered rectangle xsep    : set the extent of the x chamferling.
% /pgf/chamfered rectangle ysep    : set the extent of the y chamferling.

\pgfkeys{/pgf/chamfered rectangle corners/.store in=\pgf@chamferedrectangle@corners}
\pgfkeys{/tikz/chamfered rectangle corners/.store in=\pgf@chamferedrectangle@corners}

\def\pgf@chamferedrectangle@chamferall{chamfer all}%
\def\pgf@chamferedrectangle@chamfer{chamfer}
\let\pgf@chamferedrectangle@corners\pgf@chamferedrectangle@chamferall


\def\pgf@chamferedrectangle@getcorners{%
	\let\northeastcorner\pgfutil@empty%
	\let\southeastcorner\pgfutil@empty%
	\let\southwestcorner\pgfutil@empty%
	\let\northwestcorner\pgfutil@empty%
	\expandafter\pgfutil@in@\expandafter{\pgf@chamferedrectangle@corners}{chamfer all}%
	\ifpgfutil@in@%
		\let\northeastcorner\pgf@chamferedrectangle@round%
		\let\southeastcorner\pgf@chamferedrectangle@round%
		\let\southwestcorner\pgf@chamferedrectangle@round%
		\let\northwestcorner\pgf@chamferedrectangle@round%
		\let\pgf@next\relax%
	\else%	
		\let\pgf@next\pgf@chamferedrectangle@parsecorners%
	\fi%
	\pgf@next}

\def\pgf@chamferedrectangle@parsecorners{%
	\expandafter\pgf@@chamferedrectangle@parsecorners\pgf@chamferedrectangle@corners,\pgf@stop,%
}
		
\def\pgf@@chamferedrectangle@parsecorners#1,{%
	\ifx#1\pgf@stop%
		\let\pgf@next\relax%
	\else%
		\pgfutil@in@{@#1@}{@north east@@top left@}%
		\ifpgfutil@in@%
			\let\northeastcorner\pgf@chamferedrectangle@chamfer%
		\else%
			\pgfutil@in@{@#1@}{@south east@@bottom right@}%
			\ifpgfutil@in@%
				\let\southeastcorner\pgf@chamferedrectangle@chamfer%
			\else%
				\pgfutil@in@{@#1@}{@south west@@bottom left@}%
				\ifpgfutil@in@%
					\let\southwestcorner\pgf@chamferedrectangle@chamfer%
				\else%
					\pgfutil@in@{@#1@}{@north west@@top right@}%
					\ifpgfutil@in@%
						\let\southeastcorner\pgf@chamferedrectangle@round%
					\fi%
				\fi%
			\fi%
		\fi%
		\let\pgf@next\pgf@@@chamferedrectangle@parsecorners%
	\fi%
	\pgf@next%
}
\def\pgf@@@chamferedrectangle@parsecorners{%
	\pgfutil@ifnextchar x{\pgf@@chamferedrectangle@parsecorners}{\pgf@@chamferedrectangle@parsecorners}%
}%

\pgfkeys{/pgf/.cd,
	chamfered rectangle angle/.initial=45,%
	chamfered rectangle xsep/.initial=.666ex,%
	chamfered rectangle ysep/.initial=.666ex%
}
 \pgfkeys{/pgf/chamfered rectangle sep/.style={%
	/pgf/chamfered rectangle xsep=#1,/pgf/chamfered rectangle ysep=#1}%
}




% Shape chamfered rectangle.
%
%
\pgfdeclareshape{chamfered rectangle}{%
	\savedmacro\getchamferedrectanglepoints{%
		\pgf@chamferedrectangle@getcorners%
		%
		% Get the node dimensions.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@xa.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@ya.5\ht\pgfnodeparttextbox%
		\advance\pgf@ya.5\dp\pgfnodeparttextbox%
		%
		% Get chamfer stuff. 
		%
		\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/chamfered rectangle angle}}%
		\ifdim\pgfutil@tempdima<89pt\relax%
			\ifdim\pgfutil@tempdima<1pt\relax%
				\pgfutil@tempdima1pt\relax%
			\fi%
		\else%		
			\pgfutil@tempdima89pt\relax%
		\fi%
		\pgfutil@tempdima-\pgfutil@tempdima%
		\advance\pgfutil@tempdima90pt\relax%
		\pgfmathtan@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\let\tanangle\pgfmathresult%
		\pgfmathcot@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\let\cotangle\pgfmathresult%
		\pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/chamfered rectangle xsep}}%
		\pgf@yc\tanangle\pgf@xb%
		\ifdim\pgf@yc>\pgf@ya%
			\pgf@yc\pgf@ya%
			\pgf@xb\cotangle\pgf@yc%
		\fi%
		\pgfmathcot@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/chamfered rectangle ysep}}%
		\pgf@xc\cotangle\pgf@yb%
			\ifdim\pgf@xc>\pgf@xa%
			\pgf@xc\pgf@xa%
			\pgf@yb\tanangle\pgf@xc%
		\fi%
		%
		% Check for minimum width and height%
		%
		\pgfutil@tempdima\pgf@xa%
		\advance\pgfutil@tempdima\pgf@xb%
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgfutil@tempdima<.5\pgfutil@tempdimb%
			\pgf@xa.5\pgfutil@tempdimb%
			\advance\pgf@xa-\pgf@xb%
		\fi%
		\pgfutil@tempdima\pgf@ya%
		\advance\pgfutil@tempdima\pgf@yb%
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgfutil@tempdima<.5\pgfutil@tempdimb%
			\pgf@ya.5\pgfutil@tempdimb%
			\advance\pgf@ya-\pgf@yb%
		\fi%		
		%
		% Define the background path points.
		%
		\pgfextract@process\centerpoint{%
			\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
			\pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
			\pgfmathaddtolength\pgf@y{+-.5\dp\pgfnodeparttextbox}%
		}%
		\pgfextract@process\beforenortheast{%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@x\pgf@xb%
			\advance\pgf@y\pgf@ya%
			\advance\pgf@y-\pgf@yc%
		}%
		\pgfextract@process\northeast{%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
			\ifx\northeastcorner\pgfutil@empty%
				\advance\pgf@x\pgf@xb%
				\advance\pgf@y\pgf@yb%
			\fi%
		}%
		\pgfextract@process\afternortheast{%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@x-\pgf@xc%
			\advance\pgf@y\pgf@ya%
			\advance\pgf@y\pgf@yb%
		}%	
		\pgfextract@process\northwest{%
			\centerpoint%
			\advance\pgf@x-\pgf@xa%
			\advance\pgf@y\pgf@ya%
			\ifx\northwestcorner\pgfutil@empty%
				\advance\pgf@x-\pgf@xb%
				\advance\pgf@y\pgf@yb%
			\fi%
		}%
		\pgfextract@process\beforesouthwest{%
			\centerpoint%
			\advance\pgf@x-\pgf@xa%
			\advance\pgf@x-\pgf@xb%
			\advance\pgf@y-\pgf@ya%
			\advance\pgf@y\pgf@yc%
		}%
		\pgfextract@process\southwest{%
			\centerpoint%
			\advance\pgf@x-\pgf@xa%
			\advance\pgf@y-\pgf@ya%
			\ifx\southwestcorner\pgfutil@empty%
				\advance\pgf@x-\pgf@xb%
				\advance\pgf@y-\pgf@yb%
			\fi%
		}%
		\pgfextract@process\aftersouthwest{%
			\centerpoint%
			\advance\pgf@x-\pgf@xa%
			\advance\pgf@x\pgf@xc%
			\advance\pgf@y-\pgf@ya%
			\advance\pgf@y-\pgf@yb%
		}%
		\pgfextract@process\southeast{%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y-\pgf@ya%
			\ifx\southeastcorner\pgfutil@empty%
				\advance\pgf@x\pgf@xb%
				\advance\pgf@y-\pgf@yb%
			\fi%
		}%
		%
		% Calculate the `miter' vectors.
		%
		\pgfmathanglebetweenlines{\beforenortheast}{\afternortheast}{\beforenortheast}%
			{\beforesouthwest\pgf@ya\pgf@y\beforenortheast\pgf@y\pgf@ya}%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\ifdim\pgfutil@tempdima>180pt\relax%
			\advance\pgfutil@tempdima-180pt\relax%
		\fi%
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/outer xsep}}%
		\ifdim\pgfutil@tempdima<90pt\relax%
			\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
			\pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
			\pgfutil@tempdima0pt\relax%
		\else%
			\pgfutil@tempdima.5\pgfutil@tempdima%
			\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
			\pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
			\pgfutil@tempdima-\pgfutil@tempdima%
			\advance\pgfutil@tempdima90pt\relax%
		\fi%
		\pgfextract@process\before@ne@anchor{%
			\beforenortheast%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfutil@tempdima-\pgfutil@tempdima%
		\advance\pgfutil@tempdima180pt\relax%
		\pgfextract@process\before@sw@anchor{%
			\beforesouthwest%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\pgfqpointpolar{-\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		%
		\pgfmathanglebetweenlines{\afternortheast}{\aftersouthwest\pgf@xa\pgf@x\afternortheast\pgf@x\pgf@xa}%
			{\afternortheast}{\beforenortheast}%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\ifdim\pgfutil@tempdima>270pt\relax%
			\advance\pgfutil@tempdima-270pt\relax%
		\fi%
		\pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgfutil@tempdima<90pt\relax%
			\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
			\pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
			\pgfutil@tempdima90pt\relax%
		\else%
			\pgfutil@tempdima.5\pgfutil@tempdima%
			\pgfmathcosec@{\pgfmath@tonumber{\pgfutil@tempdima}}%
			\pgfutil@tempdimb\pgfmathresult\pgfutil@tempdimb%
		\fi%		
		%
		\pgfextract@process\after@ne@anchor{%
			\afternortheast%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\pgfqpointpolar{\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfutil@tempdima-\pgfutil@tempdima%
		\advance\pgfutil@tempdima180pt\relax%
		\pgfextract@process\after@sw@anchor{%
			\aftersouthwest
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\pgfqpointpolar{-\pgfmath@tonumber{\pgfutil@tempdima}}{\the\pgfutil@tempdimb}%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\addtosavedmacro\before@ne@anchor%
		\addtosavedmacro\after@ne@anchor%
		\addtosavedmacro\before@sw@anchor%
		\addtosavedmacro\after@sw@anchor%
		\pgfextract@process\ne@anchor{%
			\ifx\northeastcorner\pgfutil@empty%
				\northeast%
				\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
				\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
			\else%
				\pgfpointlineattime{0.5}{\before@ne@anchor}{\after@ne@anchor}%
			\fi%
		}%
		\pgfextract@process\nw@anchor{%
			\ifx\northwestcorner\pgfutil@empty%
				\northwest%
				\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
				\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
			\else%
				\pgfpointlineattime{0.5}{%
					\before@ne@anchor%
					\pgf@ya\pgf@y
					\before@sw@anchor%
					\pgf@y\pgf@ya%
				}{%
					\after@ne@anchor%
					\pgf@ya\pgf@y
					\after@sw@anchor%
					\pgf@y\pgf@ya%
				}%
			\fi%
		}%
		\pgfextract@process\sw@anchor{%
			\ifx\southwestcorner\pgfutil@empty%
				\southwest%
				\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
				\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
			\else%
				\pgfpointlineattime{0.5}{\before@sw@anchor}{\after@sw@anchor}%
			\fi%
		}%
		\pgfextract@process\se@anchor{%
			\ifx\southeastcorner\pgfutil@empty%
				\southeast%
				\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
				\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
			\else%
				\pgfpointlineattime{0.5}{%
					\before@ne@anchor%
					\pgf@xa\pgf@x
					\before@sw@anchor%
					\pgf@x\pgf@xa%
				}{%
					\after@ne@anchor%
					\pgf@xa\pgf@x
					\after@sw@anchor%
					\pgf@x\pgf@xa%
				}%
			\fi%
		}%
		\addtosavedmacro\ne@anchor%
		\addtosavedmacro\nw@anchor%
		\addtosavedmacro\sw@anchor%
		\addtosavedmacro\se@anchor%
	}%
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}%
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\getchamferedrectanglepoints%
		\midpoint%
		\pgf@ya\pgf@y%
		\pgf@process{%
			\before@sw@anchor%
			\pgf@ya\pgf@y%
			\before@ne@anchor%
			\pgf@y\pgf@ya		
		}%
		\ifdim\pgf@ya<\pgf@y%
			\pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
				{\before@sw@anchor\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
				{\after@sw@anchor\pgf@ya\pgf@y\after@ne@anchor\pgf@y\pgf@ya}%
		\else%
			\pgf@process{\before@ne@anchor}%
			\ifdim\pgf@ya<\pgf@y%
				\pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
					{\before@sw@anchor\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
					{\before@ne@anchor}%
			\else%
				\pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
					{\before@ne@anchor}%
					{\after@ne@anchor}%
			\fi%
		\fi%			
	}%
	\anchor{mid west}{%
		\getchamferedrectanglepoints%
		\midpoint%
		\pgf@ya\pgf@y%
		\pgf@process{\before@sw@anchor}%
		\ifdim\pgf@ya<\pgf@y%
			\pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
				{\before@sw@anchor}{\after@sw@anchor}%
		\else%
			\pgf@process{\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
			\ifdim\pgf@ya<\pgf@y%
				\pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
					{\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
					{\before@sw@anchor}%
			\else%
				\pgfpointintersectionoflines{\midpoint}{\midpoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
					{\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
					{\after@ne@anchor\pgf@ya\pgf@y\after@sw@anchor\pgf@y\pgf@ya}%
			\fi%
		\fi%			
	}%
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\getchamferedrectanglepoints%
		\basepoint%
		\pgf@ya\pgf@y%
		\pgf@process{%
			\before@sw@anchor%
			\pgf@ya\pgf@y%
			\before@ne@anchor%
			\pgf@y\pgf@ya		
		}%
		\ifdim\pgf@ya<\pgf@y%
			\pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
				{\before@sw@anchor\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
				{\after@sw@anchor\pgf@ya\pgf@y\after@ne@anchor\pgf@y\pgf@ya}%
		\else%
			\pgf@process{\before@ne@anchor}%
			\ifdim\pgf@ya<\pgf@y%
				\pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
					{\before@sw@anchor\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
					{\before@ne@anchor}%
			\else%
				\pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
					{\before@ne@anchor}%
					{\after@ne@anchor}%
			\fi%
		\fi%			
	}%
	\anchor{base west}{%
		\getchamferedrectanglepoints%
		\basepoint%
		\pgf@ya\pgf@y%
		\pgf@process{\before@sw@anchor}%
		\ifdim\pgf@ya<\pgf@y%
			\pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
				{\before@sw@anchor}{\after@sw@anchor}%
		\else%
			\pgf@process{\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
			\ifdim\pgf@ya<\pgf@y%
				\pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
					{\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
					{\before@sw@anchor}%
			\else%
				\pgfpointintersectionoflines{\basepoint}{\basepoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
					{\before@ne@anchor\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
					{\after@ne@anchor\pgf@ya\pgf@y\after@sw@anchor\pgf@y\pgf@ya}%
			\fi%
		\fi%			
	}%
	\anchor{before north east}{\getchamferedrectanglepoints\before@ne@anchor}%
	\anchor{north east}{\getchamferedrectanglepoints\ne@anchor}%
	\anchor{after north east}{\getchamferedrectanglepoints\after@ne@anchor}%
	\anchor{north}{%
		\getchamferedrectanglepoints%
		\centerpoint%
		\pgf@xa\pgf@x%
		\after@ne@anchor%
		\pgf@x\pgf@xa}%	
	\anchor{before north west}{%
		\getchamferedrectanglepoints%
		\after@sw@anchor%
		\pgf@xa\pgf@x%
		\after@ne@anchor%
		\pgf@x\pgf@xa}%
	\anchor{north west}{\getchamferedrectanglepoints\nw@anchor}%
	\anchor{after north west}{%
		\getchamferedrectanglepoints%
		\before@sw@anchor%
		\pgf@xa\pgf@x%
		\before@ne@anchor%
		\pgf@x\pgf@xa}%
	\anchor{west}{%
		\getchamferedrectanglepoints%
		\centerpoint%
		\pgf@ya\pgf@y%
		\before@sw@anchor%
		\pgf@y\pgf@ya}%	
	\anchor{before south west}{\getchamferedrectanglepoints\before@sw@anchor}%
	\anchor{south west}{\getchamferedrectanglepoints\sw@anchor}%
	\anchor{after south west}{\getchamferedrectanglepoints\after@sw@anchor}%
		\anchor{south}{%
		\getchamferedrectanglepoints%
		\centerpoint%
		\pgf@xa\pgf@x%
		\after@sw@anchor%
		\pgf@x\pgf@xa}%	
	\anchor{before south east}{%
		\getchamferedrectanglepoints%
		\after@sw@anchor%
		\pgf@ya\pgf@y%
		\after@ne@anchor%
		\pgf@y\pgf@ya}%
	\anchor{south east}{\getchamferedrectanglepoints\se@anchor}%
	\anchor{after south east}{%
		\getchamferedrectanglepoints%
		\before@sw@anchor%
		\pgf@ya\pgf@y%
		\before@ne@anchor%
		\pgf@y\pgf@ya}%
	\anchor{east}{%
		\getchamferedrectanglepoints%
		\centerpoint%
		\pgf@ya\pgf@y%
		\before@ne@anchor%
		\pgf@y\pgf@ya}%	
	\backgroundpath{%
		\pgfpathmoveto{\beforenortheast}%
		\pgfpathlineto{\northeast}%
		\pgfpathlineto{\afternortheast}%
		\pgfpathlineto{\aftersouthwest\pgf@xa\pgf@x\afternortheast\pgf@x\pgf@xa}%
		\pgfpathlineto{\northwest}%
		\pgfpathlineto{\beforesouthwest\pgf@xa\pgf@x\beforenortheast\pgf@x\pgf@xa}%
		\pgfpathlineto{\beforesouthwest}%
		\pgfpathlineto{\southwest}%
		\pgfpathlineto{\aftersouthwest}%
		\pgfpathlineto{\aftersouthwest\pgf@ya\pgf@y\afternortheast\pgf@y\pgf@ya}%
		\pgfpathlineto{\southeast}%
		\pgfpathlineto{\beforesouthwest\pgf@ya\pgf@y\beforenortheast\pgf@y\pgf@ya}%		
		\pgfpathclose%
	}
	\anchorborder{%
		\pgfextract@process\externalpoint{%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\let\externalangle\pgfmathresult%
		\getchamferedrectanglepoints%
		\pgfmathanglebetweenpoints{\centerpoint}{\centerpoint\pgf@ya\pgf@y\before@sw@anchor\pgf@y\pgf@ya}%
		\ifdim\externalangle pt<\pgfmathresult pt\relax% west.
			\pgfmathanglebetweenpoints{\centerpoint}{\centerpoint\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax% north.
				\pgfmathanglebetweenpoints{\centerpoint}{\ne@anchor}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax% north east.
					\pgfmathanglebetweenpoints{\centerpoint}{\before@ne@anchor}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax% before north east.
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\centerpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}{\before@ne@anchor}%
					\else% 
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\before@ne@anchor}{\ne@anchor}%
					\fi%
				\else%
					\pgfmathanglebetweenpoints{\centerpoint}{\after@ne@anchor}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax% after north east.
							\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\ne@anchor}{\after@ne@anchor}%
					\else% 
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\after@ne@anchor}{\centerpoint\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
					\fi%
				\fi%
			\else%
				\pgfmathanglebetweenpoints{\centerpoint}{\nw@anchor}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax% north west.
					\pgfmathanglebetweenpoints{\centerpoint}{\after@sw@anchor\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax% before north west.
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\centerpoint\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
							{\after@sw@anchor\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
					\else%
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\after@sw@anchor\pgf@xa\pgf@x\after@ne@anchor\pgf@x\pgf@xa}%
							{\nw@anchor}%
					\fi%
				\else%
					\pgfmathanglebetweenpoints{\centerpoint}{\before@sw@anchor\pgf@xa\pgf@x\before@ne@anchor\pgf@x\pgf@xa}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax% after north west.
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\nw@anchor}{\before@sw@anchor\pgf@xa\pgf@x\before@ne@anchor\pgf@x\pgf@xa}%
					\else%
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\before@sw@anchor\pgf@xa\pgf@x\before@ne@anchor\pgf@x\pgf@xa}%
							{\before@sw@anchor\pgf@xa\pgf@x\centerpoint\pgf@x\pgf@xa}%
					\fi%
				\fi%
			\fi%
		\else%
			\pgfmathanglebetweenpoints{\centerpoint}{\centerpoint\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax% south.
				\pgfmathanglebetweenpoints{\centerpoint}{\sw@anchor}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax% south west.
					\pgfmathanglebetweenpoints{\centerpoint}{\before@sw@anchor}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax% before south west.
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\before@sw@anchor\pgf@xa\pgf@x\centerpoint\pgf@x\pgf@xa}%
							{\before@sw@anchor}%
					\else%
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\before@sw@anchor}{\sw@anchor}%
					\fi%
				\else%
					\pgfmathanglebetweenpoints{\centerpoint}{\after@sw@anchor}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax% after south west.
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\before@sw@anchor}{\after@sw@anchor}%
					\else%
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\after@sw@anchor}{\centerpoint\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
					\fi%
				\fi%
			\else%
				\pgfmathanglebetweenpoints{\centerpoint}{\se@anchor}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax% south east.
					\pgfmathanglebetweenpoints{\centerpoint}{\after@ne@anchor\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax% before south east.
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\after@ne@anchor\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
							{\centerpoint\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}%
					\else%
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\after@ne@anchor\pgf@xa\pgf@x\after@sw@anchor\pgf@x\pgf@xa}{\se@anchor}
					\fi%
				\else%
					\pgfmathanglebetweenpoints{\centerpoint}{\before@ne@anchor\pgf@xa\pgf@x\before@sw@anchor\pgf@x\pgf@xa}%
					\ifdim\externalangle pt<\pgfmathresult pt\relax% after south east.
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\se@anchor}{\before@ne@anchor\pgf@xa\pgf@x\before@sw@anchor\pgf@x\pgf@xa}%					
					\else%
						\pgfpointintersectionoflines{\centerpoint}{\externalpoint}%
							{\before@ne@anchor\pgf@xa\pgf@x\before@sw@anchor\pgf@x\pgf@xa}%
							{\centerpoint\pgf@ya\pgf@y\before@ne@anchor\pgf@y\pgf@ya}%
					\fi%
				\fi%
			\fi%			
		\fi%
	}%			
}


\endinput


==> pgflibraryshapes.multipart.code.tex <==
% Copyright 2007 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryshapes.multipart.code.tex,v 1.7 2008/01/15 15:41:18 vibrovski Exp $

\newbox\pgfnodepartlowerbox

%
% A circle that is split in the middle into an upper and a lower part.
%
% This node consists of two parts: The upper (main) part is shown in
% the upper half of the circle. The second part is the (optional)
% lower part.
%
% Parts: text, lower

\pgfdeclareshape{circle split}
{
  %
  % Node parts
  %
  \nodeparts{text,lower}

  %
  % Anchors
  %
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength{\pgf@y}{\pgfkeysvalueof{/pgf/inner ysep}}%
    \pgf@y=-\pgf@y%
    \advance\pgf@y by-\dp\pgfnodeparttextbox%
    \advance\pgf@y by-.5\pgflinewidth%
  }%
  \savedanchor\loweranchor{%
    \pgf@x=-.5\wd\pgfnodepartlowerbox%
    \advance\pgf@x by.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength{\pgf@y}{\pgfkeysvalueof{/pgf/inner ysep}}%
    \pgf@y=-2\pgf@y%
    \advance\pgf@y by-\ht\pgfnodepartlowerbox%
    \advance\pgf@y by-.5\pgflinewidth%
    \advance\pgf@y by-\dp\pgfnodeparttextbox%
    \advance\pgf@y by-.5\pgflinewidth%
  }
    
  \saveddimen\radius{%
    % 
    % Caculate ``height radius''
    %
    %\pgf@ya=.5\ht\pgfnodeparttextbox%
%    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
%    \advance\pgf@ya by.5\ht\pgfnodepartlowerbox%
%    \advance\pgf@ya by.5\dp\pgfnodepartlowerbox%
%    \advance\pgf@ya by.5\pgflinewidth%
		%
		% MW: Suggested correction for above calculation:	Use the tallest box * 2.
		%
		\pgf@ya=.5\ht\pgfnodeparttextbox%
		\advance\pgf@ya by.5\dp\pgfnodeparttextbox%
		\pgf@yb=.5\ht\pgfnodepartlowerbox%
		\advance\pgf@yb by.5\dp\pgfnodepartlowerbox%
		\ifdim\pgf@ya>\pgf@yb\relax%
			\pgf@ya2.0\pgf@ya\relax%
		\else%
			\pgf@ya2.0\pgf@yb\relax%
		\fi%
		\advance\pgf@ya by.5\pgflinewidth%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya by2\pgf@yb%
    % 
    % Caculate ``width radius''
    % 
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \ifdim\pgf@xa<.5\wd\pgfnodepartlowerbox%
      \pgf@xa=.5\wd\pgfnodepartlowerbox%
    \fi%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa by\pgf@xb%
    % 
    % Calculate length of radius vector:
    % 
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \ifdim\pgf@x>\pgf@y%
        \c@pgf@counta=\pgf@x%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@xa=16\pgf@xa\relax%
          \divide\pgf@xa by\c@pgf@counta%
          \pgf@xa=16\pgf@xa\relax%
        \fi%
      \else%
        \c@pgf@counta=\pgf@y%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@ya=16\pgf@ya\relax%
          \divide\pgf@ya by\c@pgf@counta%
          \pgf@xa=16\pgf@ya\relax%
        \fi%
    \fi%
    \pgf@x=\pgf@xa%
    % 
    % If necessary, adjust radius so that the size requirements are
    % met: 
    % 
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/minimum width}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/minimum height}}%  
    \ifdim\pgf@x<.5\pgf@xb%
        \pgf@x=.5\pgf@xb%
    \fi%
    \ifdim\pgf@x<.5\pgf@yb%
        \pgf@x=.5\pgf@yb%
    \fi%
    % 
    % Now, add larger of outer sepearations.
    % 
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgf@x by\pgf@yb%
    \else%
      \advance\pgf@x by\pgf@xb%
    \fi%
  }

  %
  % Anchors
  % 
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \anchor{lower}{\loweranchor}

  %
  % Background path
  %
  \inheritbackgroundpath[from=circle]
  \beforebackgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \advance\pgfutil@tempdima by-.5\pgflinewidth%  
    \pgfsetshortenstart{0pt}%
    \pgfsetshortenend{0pt}%
    \pgfsetarrows{-}%  
    \pgfpathmoveto{\pgfpointadd{\centerpoint}{\pgfqpoint{-1\pgfutil@tempdima}{0pt}}}%
    \pgfpathlineto{\pgfpointadd{\centerpoint}{\pgfqpoint{\pgfutil@tempdima}{0pt}}}%
    \pgfusepath{stroke}%
  }
}





% (Most) keys for shape rectangle split.
%
% /pgf/rectangle split parts             : Set the number of rectangles to split into.
% /pgf/rectangle split part align        : Align the for the boxes in each part
%                                          (also keys for each part)
% /pgf/rectangle split use custom fill   : Use a custom (behindbackground path) fill.
% /pgf/rectangle split part fill         : Custom fill for ech part.
%                                          (also keys for each part)
% /pgf/rectangle split draw splits       : Draw the line between node parts.
% /pgf/rectangle split empty part height : Set the default height for empty boxes.


\newif\ifpgfrectanglesplitdrawsplits
\pgfrectanglesplitdrawsplitstrue

\newif\ifpgfrectanglesplitusecustomfill
\pgfrectanglesplitusecustomfillfalse

\pgfkeys{/pgf/.cd,
	rectangle split parts/.initial=4,
	rectangle split empty part height/.initial=1ex,
	rectangle split draw splits/.is if=pgfrectanglesplitdrawsplits,
	%
	rectangle split part align/.code=\pgf@lib@shapes@rectanglesplit@assigntoparts{#1}{align},
	rectangle split text part align/.initial=center,
	rectangle split second part align/.initial=center,
	rectangle split third part align/.initial=center,
	rectangle split fourth part align/.initial=center,
	%
	rectangle split use custom fill/.is if=pgfrectanglesplitusecustomfill,
	rectangle split part fill/.code={%
		\pgfrectanglesplitusecustomfilltrue%
		\pgf@lib@shapes@rectanglesplit@assigntoparts{#1}{fill}%
	},
	rectangle split text part fill/.initial=white,
	rectangle split second part fill/.initial=white,
	rectangle split third part fill/.initial=white,
	rectangle split fourth part fill/.initial=white
}

% Internal macros for the rectangle split shape.
%
\def\pgf@lib@shapes@rectanglesplit@left{left}
\def\pgf@lib@shapes@rectanglesplit@right{right}

\def\pgf@lib@shapes@rectanglesplit@assigntoparts#1#2{%
	\expandafter\pgf@lib@shapes@rectanglesplit@@assigntoparts#1,\@@,\@@,\@@,\@@,\pgf@lib#2\pgf@lib}
\def\pgf@lib@shapes@rectanglesplit@@assigntoparts#1,#2,#3,#4,#5\pgf@lib#6\pgf@lib{%
	\pgfkeys{/pgf/.cd,%
		rectangle split text part #6=#1,
		rectangle split second part #6=#1,
		rectangle split third part #6=#1,
		rectangle split fourth part #6=#1
	}%
	\ifx#2\@@\else%
	\pgfkeys{/pgf/.cd,%
			rectangle split second part #6=#2,
			rectangle split third part #6=#2,
			rectangle split fourth part #6=#2
		}%
	\fi%
	\ifx#3\@@\else%
		\pgfkeys{/pgf/.cd,%
			rectangle split third part #6=#3,
			rectangle split fourth part #6=#3
		}%
	\fi%
	\ifx#4\@@\else%
		\pgfkeys{/pgf/rectangle split fourth part #6=#4}%
	\fi%
}%

\newbox\pgfnodepartsecondbox
\newbox\pgfnodepartthirdbox
\newbox\pgfnodepartfourthbox

\pgfdeclareshape{rectangle split}{%
	\nodeparts{text,second,third,fourth}
	\savedmacro\getrectanglesplitparameters{%
		%
		% If the height+depth of any box is 0pt use the default empty height.
		%
		\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/rectangle split empty part height}}
		\pgf@y\ht\pgfnodeparttextbox%
		\advance\pgf@y\dp\pgfnodeparttextbox%
		\ifdim\pgf@y=0pt\relax%
			\setbox\pgfnodeparttextbox=\hbox{%				
				\vrule width0pt height\the\pgfutil@tempdima depth0pt%
			}%
		\fi%
		\pgf@y\ht\pgfnodepartsecondbox%
		\advance\pgf@y\dp\pgfnodepartsecondbox%
		\ifdim\pgf@y=0pt\relax%
			\setbox\pgfnodepartsecondbox=\hbox{%
				\vrule width0pt height\the\pgfutil@tempdima depth0pt%
			}%
		\fi%
		\pgf@y\ht\pgfnodepartthirdbox%
		\advance\pgf@y\dp\pgfnodepartthirdbox%
		\ifdim\pgf@y=0pt\relax%
			\setbox\pgfnodepartthirdbox=\hbox{%
				\vrule width0pt height\the\pgfutil@tempdima depth0pt%
			}%
		\fi%
		\pgf@y\ht\pgfnodepartfourthbox%
		\advance\pgf@y\dp\pgfnodepartfourthbox%
		\ifdim\pgf@y=0pt\relax%
			\setbox\pgfnodepartfourthbox=\hbox{%
					\vrule width0pt height\the\pgfutil@tempdima depth0pt%
			}%
		\fi%
		%
		% Empty boxes (without voiding them) if they are not used.
		%
		\pgfmathtruncatemacro\parts{\pgfkeysvalueof{/pgf/rectangle split parts}}%
	  \addtosavedmacro{\parts}%
	  \ifnum\parts<2\relax%
	  	\setbox\pgfnodepartsecondbox=\hbox{}%
	  \fi%
	  \ifnum\parts<3\relax%
	  	\setbox\pgfnodepartthirdbox=\hbox{}%
	  \fi%
	  \ifnum\parts<4\relax%
	  	\setbox\pgfnodepartfourthbox=\hbox{}%
	  \fi%	  
	  %
		% Save the line width.
		%
		\pgfmathsetlength\pgf@x{\pgflinewidth}
		\edef\linewidth{\the\pgf@x}%
	  \addtosavedmacro{\linewidth}%
	  %
	  \pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
  	\edef\innerysep{\the\pgf@y}%
  	%
	  \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
  	\edef\innerxsep{\the\pgf@x}%
  	%
  	% Get the widths.
  	%
  	\pgf@x.5\wd\pgfnodeparttextbox%
  	\pgf@xa.5\wd\pgfnodepartsecondbox%
  	\pgf@xb.5\wd\pgfnodepartthirdbox%
  	\pgf@xc.5\wd\pgfnodepartfourthbox%
  	%
  	% Find the maximum width%
  	%
  	\pgfutil@tempdima\pgf@x%
  	\ifdim\pgfutil@tempdima<\pgf@xa%
  		\pgfutil@tempdima\pgf@xa%
  	\fi%
  	\ifdim\pgfutil@tempdima<\pgf@xb%
  		\pgfutil@tempdima\pgf@xb%
  	\fi%
  	\ifdim\pgfutil@tempdima<\pgf@xc%
  		\pgfutil@tempdima\pgf@xc%
  	\fi%
  	%
  	% Adjust for alignment.
	  %
	  \edef\pgf@lib@temp{\pgfkeysvalueof{/pgf/rectangle split text part align}}%
	  \ifx\pgf@lib@temp\pgf@lib@shapes@rectanglesplit@left%
  		\pgf@x-\pgfutil@tempdima%
	  \else%
	  	\ifx\pgf@lib@temp\pgf@lib@shapes@rectanglesplit@right%
	  		\pgf@x-2.0\pgf@x%
  			\advance\pgf@x\pgfutil@tempdima%	  		
	  	\else%
	  		\pgf@x-\pgf@x%
  		\fi%
	  \fi%
  	%
  	\edef\pgf@lib@temp{\pgfkeysvalueof{/pgf/rectangle split second part align}}%
  	\ifx\pgf@lib@temp\pgf@lib@shapes@rectanglesplit@left%
  		\pgf@xa-\pgfutil@tempdima%
	  \else%
	  	\ifx\pgf@lib@temp\pgf@lib@shapes@rectanglesplit@right%
	  		\pgf@xa-2.0\pgf@xa%
  			\advance\pgf@xa\pgfutil@tempdima%
	  	\else%
  			\pgf@xa-\pgf@xa%
  		\fi%
	  \fi%
  	%
  	\edef\pgf@lib@temp{\pgfkeysvalueof{/pgf/rectangle split third part align}}%
  	\ifx\pgf@lib@temp\pgf@lib@shapes@rectanglesplit@left%
  		\pgf@xb-\pgfutil@tempdima%
	  \else%
	  	\ifx\pgf@lib@temp\pgf@lib@shapes@rectanglesplit@right%
	  		\pgf@xb-2.0\pgf@xb%
	  		\advance\pgf@xb\pgfutil@tempdima%
	  	\else%
	  		\pgf@xb-\pgf@xb%
	  	\fi%
	  \fi%
  	%
  	\edef\pgf@lib@temp{\pgfkeysvalueof{/pgf/rectangle split fourth part align}}%
  	\ifx\pgf@lib@temp\pgf@lib@shapes@rectanglesplit@left%
  		\pgf@xc-\pgfutil@tempdima%
	  \else%
	  	\ifx\pgf@lib@temp\pgf@lib@shapes@rectanglesplit@right%
	  		\pgf@xc-2.0\pgf@xc%
	  		\advance\pgf@xc\pgfutil@tempdima%
	  	\else%
	  		\pgf@xc-\pgf@xc%
	  	\fi%
	  \fi%
  	%
  	% Make relative to x.
  	%
  	\advance\pgf@xa-\pgf@x%
  	\advance\pgf@xb-\pgf@x%
  	\advance\pgf@xc-\pgf@x%
  	\pgf@x0pt%
  	%
  	% Find the minimum.
  	%
  	\pgfutil@tempdimb\pgf@x%
  	\ifdim\pgfutil@tempdimb>\pgf@xa%
  		\pgfutil@tempdimb\pgf@xa%
  	\fi%
  	\ifdim\pgfutil@tempdimb>\pgf@xb%
  		\pgfutil@tempdimb\pgf@xb%
  	\fi%
  	\ifdim\pgfutil@tempdimb>\pgf@xc%
  		\pgfutil@tempdimb\pgf@xc%
  	\fi%
  	%
  	% Anchor for the text box is (0pt, 0pt)
  	%
  	\pgfsavepgf@process\textanchor{\pgfqpoint{0pt}{0pt}}%
  	%
  	% Anchor for second box.
  	%
  	\pgfsavepgf@process\lowestanchor{\pgfqpoint{0pt}{0pt}}%
  	\let\lowestbox\pgfnodeparttextbox%
  	\ifnum\parts>1\relax%
  	  \pgfsavepgf@process\secondanchor{%
  	  	\pgf@x\pgf@xa%
	  		\pgf@y-\dp\pgfnodeparttextbox%
	  		\advance\pgf@y-\innerysep\relax%
	  		\advance\pgf@y-\pgflinewidth%
	  		\advance\pgf@y-\innerysep\relax%
	  		\advance\pgf@y-\ht\pgfnodepartsecondbox%
	  	}%
	  	\let\lowestanchor\secondanchor%
	  	\let\lowestbox\pgfnodepartsecondbox%
  	\else%
  		\let\secondanchor\textanchor%
  	\fi%
  	%
  	% Anchor for third box.
  	%
  	\ifnum\parts>2\relax%
  	  \pgfsavepgf@process\thirdanchor{%
  	  	\lowestanchor%
  	  	\pgf@x\pgf@xb%
	  		\advance\pgf@y-\dp\pgfnodepartsecondbox%
	  		\advance\pgf@y-\innerysep\relax%
	  		\advance\pgf@y-\pgflinewidth%
	  		\advance\pgf@y-\innerysep\relax%
	  		\advance\pgf@y-\ht\pgfnodepartthirdbox%
	  	}%
	  	\let\lowestanchor\thirdanchor%
	  	\let\lowestbox\pgfnodepartthirdbox%
  	\else%
  		\let\thirdanchor\secondanchor%
  	\fi%
  	%
  	% Anchor for fourth box.
  	%
  	\ifnum\parts>3\relax%
  		\pgfsavepgf@process\fourthanchor{%
  			\lowestanchor%
  	  	\pgf@x\pgf@xc%
  	  	\advance\pgf@y-\dp\lowestbox%
	  		\advance\pgf@y-\innerysep\relax%
	  		\advance\pgf@y-\pgflinewidth%
	  		\advance\pgf@y-\innerysep\relax%
	  		\advance\pgf@y-\ht\pgfnodepartfourthbox%
	  	}%
	  	\let\lowestanchor\fourthanchor%
	  	\let\lowestbox\pgfnodepartfourthbox%
	  \else%
  		\let\fourthanchor\thirdanchor%
  	\fi%
  	%
  	\addtosavedmacro{\textanchor}%
	  \addtosavedmacro{\secondanchor}%
	  \addtosavedmacro{\thirdanchor}%
	  \addtosavedmacro{\fourthanchor}%
	  %
	  % Adjust the boxwidth for minimum width
	  %
	  \pgfmathaddtolength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/inner xsep}}%
  	\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/minimum width}}%
  	\ifdim\pgfutil@tempdima<.5\pgf@x%
  		\pgfutil@tempdima.5\pgf@x%
  	\fi%
  	\pgfmathaddtolength\pgfutil@tempdima{-\pgfkeysvalueof{/pgf/inner xsep}}%
  	%
  	% Get some important points.
  	%
  	\pgfsavepgf@process\southwest{%
  		\lowestanchor%
  		\pgf@x\pgfutil@tempdimb%
  		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/inner xsep}}%
  		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
  		\pgf@ya\linewidth\relax%
  		\advance\pgf@x-.5\pgf@ya%
  		\advance\pgf@y-\dp\lowestbox%
  		\advance\pgf@y-.5\pgf@ya%
  		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/inner ysep}}%
  		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
  	}%
  	\pgfsavepgf@process\northeast{%
  		\pgf@x\pgfutil@tempdimb%
  		\advance\pgf@x2.0\pgfutil@tempdima%
  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
  		\pgf@ya\linewidth\relax%
  		\advance\pgf@x.5\pgf@ya%
  		\pgf@y\ht\pgfnodeparttextbox%
  		\advance\pgf@y.5\pgf@ya%
  		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
  		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
  	}%
  	\addtosavedmacro{\northeast}%
  	\addtosavedmacro{\southwest}%  	
  	\pgfsavepgf@process\centerpoint{%
  	  \pgfpointadd{\southwest}{%
  			\pgfpointdiff{\southwest}{\northeast}%
  			\pgf@x.5\pgf@x%
  			\pgf@y.5\pgf@y%
  		}%
  	}%
  	\addtosavedmacro{\centerpoint}%  
  	\pgfsavepgf@process\south{%
  		\centerpoint%
  		\pgf@xa\pgf@x%
  		\southwest%
  		\pgf@x\pgf@xa%
  	}%
  	%
  	% Get the split points.
  	%
  	\let\lastsplit\south%
  	\ifnum\parts>1\relax%
	  	\pgfsavepgf@process\textsplit{%
	  		\pgf@x\pgfutil@tempdimb%
	  		\advance\pgf@x\pgfutil@tempdima%
	  		\pgf@y-\dp\pgfnodeparttextbox%
	  		\advance\pgf@y-\innerysep%
	  		\advance\pgf@y-.5\pgflinewidth%
	  	}%
	  \else%
	  	\let\textsplit\south%
	  \fi%
  	\addtosavedmacro{\textsplit}%
  	\pgfsavepgf@process\textspliteast{%
  		\textsplit%
  		\pgf@ya\pgf@y%
  		\northeast%
  		\pgf@y\pgf@ya%
  	}%
  	\addtosavedmacro{\textspliteast}%
  	\pgfsavepgf@process\textsplitwest{%
  		\textsplit%
  		\pgf@ya\pgf@y%
  		\southwest%
  		\pgf@y\pgf@ya%
  	}%
  	\addtosavedmacro{\textsplitwest}%
  	\ifnum\parts>2\relax%
  		\pgfsavepgf@process\secondsplit{%
  		  \secondanchor%
  			\pgf@x\pgfutil@tempdimb%
  			\advance\pgf@x\pgfutil@tempdima%
  			\advance\pgf@y-\dp\pgfnodepartsecondbox%
  			\advance\pgf@y-\innerysep%
  			\advance\pgf@y-.5\pgflinewidth%
  		}%
  	\else%
  		\let\secondsplit\south%
  	\fi%
  	\addtosavedmacro{\secondsplit}%
  	\pgfsavepgf@process\secondspliteast{%
  		\secondsplit%
  		\pgf@ya\pgf@y%
  		\northeast%
  		\pgf@y\pgf@ya%
  	}%
  	\addtosavedmacro{\secondspliteast}%
  	\pgfsavepgf@process\secondsplitwest{%
  		\secondsplit%
  		\pgf@ya\pgf@y%
  		\southwest%
  		\pgf@y\pgf@ya%
  	}%
  	\addtosavedmacro{\secondsplitwest}%
  	\ifnum\parts>3\relax%
  		\pgfsavepgf@process\thirdsplit{%
  		  \thirdanchor%
  			\pgf@x\pgfutil@tempdimb%
  			\advance\pgf@x\pgfutil@tempdima%
  			\advance\pgf@y-\dp\pgfnodepartthirdbox%
  			\advance\pgf@y-\innerysep%
  			\advance\pgf@y-.5\pgflinewidth%
  		}%
  		\let\lastsplit\thirdsplit%
  	\else%
  		\let\thirdsplit\south%
  	\fi%
  	\addtosavedmacro{\thirdsplit}%
  	\pgfsavepgf@process\thirdspliteast{%
  		\thirdsplit%
  		\pgf@ya\pgf@y%
  		\northeast%
  		\pgf@y\pgf@ya%
  	}%
  	\addtosavedmacro{\thirdspliteast}%
  	\pgfsavepgf@process\thirdsplitwest{%
  		\thirdsplit%
  		\pgf@ya\pgf@y%
  		\southwest%
  		\pgf@y\pgf@ya%
  	}%
  	\addtosavedmacro{\thirdsplitwest}%
	}%
	\savedanchor\basepoint{%
		\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
		\pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
		\pgf@y0pt\relax%
	}%
	\savedanchor\midpoint{%
		\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\anchor{center}{\getrectanglesplitparameters\centerpoint}%
	\anchor{base}{\basepoint}%
	\anchor{mid}{\midpoint}%
	\anchor{second}{\getrectanglesplitparameters\secondanchor}%
	\anchor{third}{\getrectanglesplitparameters\thirdanchor}%
	\anchor{fourth}{\getrectanglesplitparameters\fourthanchor}%
	\anchor{north east}{\getrectanglesplitparameters\northeast}
	\anchor{south west}{\getrectanglesplitparameters\southwest}
	\anchor{south east}{%
		\getrectanglesplitparameters%
		\northeast%
		\pgf@xa\pgf@x%
		\southwest%
		\pgf@x\pgf@xa}
	\anchor{north west}{%
		\getrectanglesplitparameters%
		\northeast%
		\pgf@ya\pgf@y%
		\southwest%
		\pgf@y\pgf@ya}
	\anchor{south}{%
		\getrectanglesplitparameters%
		\centerpoint%
		\pgf@xa\pgf@x%
		\southwest%
		\pgf@x\pgf@xa}
	\anchor{north}{%
		\getrectanglesplitparameters%
		\centerpoint%
		\pgf@xa\pgf@x%
		\northeast%
		\pgf@x\pgf@xa}
	\anchor{west}{%
		\getrectanglesplitparameters%
		\centerpoint%
		\pgf@ya\pgf@y%
		\southwest%
		\pgf@y\pgf@ya}
	\anchor{east}{%
		\getrectanglesplitparameters%
		\centerpoint%
		\pgf@ya\pgf@y%
		\northeast%
		\pgf@y\pgf@ya}
	\anchor{text split}{\getrectanglesplitparameters\textsplit}
	\anchor{text split east}{\getrectanglesplitparameters\textspliteast}
	\anchor{text split west}{\getrectanglesplitparameters\textsplitwest}
	\anchor{second split}{\getrectanglesplitparameters\secondsplit}
	\anchor{second split east}{\getrectanglesplitparameters\secondspliteast}
	\anchor{second split west}{\getrectanglesplitparameters\secondsplitwest}
	\anchor{third split}{\getrectanglesplitparameters\thirdsplit}
	\anchor{third split east}{\getrectanglesplitparameters\thirdspliteast}
	\anchor{third split west}{\getrectanglesplitparameters\thirdsplitwest}	
	\anchor{text east}{%
		\getrectanglesplitparameters%
		\ifnum\parts>1\relax%
			\textsplit%
			\pgf@ya\pgf@y
			\northeast%
			\advance\pgf@y\pgf@ya%
			\pgf@y.5\pgf@y%
			\pgf@ya\linewidth\relax%
			\advance\pgf@y-.25\pgf@ya%
		\else%
			\centerpoint%
			\pgf@ya\pgf@y%
			\northeast%
			\pgf@y\pgf@ya%
		\fi%
	}
	\anchor{text west}{%
		\getrectanglesplitparameters%
		\ifnum\parts>1\relax%
			\textsplit%
			\pgf@ya\pgf@y
			\southwest%
			\pgf@xa\pgf@x%
			\northeast%
			\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
			\pgf@y.5\pgf@y%
			\pgf@ya\linewidth\relax%
			\advance\pgf@y-.25\pgf@ya%
		\else%
			\centerpoint%
			\pgf@ya\pgf@y%
			\southwest%
			\pgf@y\pgf@ya%
		\fi%
	}
	\anchor{second east}{%
		\getrectanglesplitparameters%
		\ifnum\parts>1\relax%
			\northeast%
			\pgf@xa\pgf@x%
			\secondsplit%
			\pgf@ya\pgf@y
			\textsplit%
			\advance\pgf@y\pgf@ya%
			\pgf@y.5\pgf@y%
			\pgf@x\pgf@xa%
		\else%
			\southwest%
			\pgf@ya\pgf@y%
			\northeast%
			\pgf@y\pgf@ya%
		\fi%
	}
	\anchor{second west}{%
		\getrectanglesplitparameters%
		\ifnum\parts>1\relax%
			\southwest%
			\pgf@xa\pgf@x%
			\secondsplit%
			\pgf@ya\pgf@y
			\textsplit%
			\advance\pgf@y\pgf@ya%
			\pgf@y.5\pgf@y%
			\pgf@x\pgf@xa%
		\else%
			\southwest%
		\fi%
	}
	\anchor{third east}{%
		\getrectanglesplitparameters%
		\ifnum\parts>2\relax%
			\northeast%
			\pgf@xa\pgf@x%
			\thirdsplit%
			\pgf@ya\pgf@y
			\secondsplit%
			\advance\pgf@y\pgf@ya%
			\pgf@y.5\pgf@y%
			\pgf@x\pgf@xa%
		\else%
			\southwest%
			\pgf@ya\pgf@y%
			\northeast%
			\pgf@y\pgf@ya%
		\fi%
	}
	\anchor{third west}{%
		\getrectanglesplitparameters%
		\ifnum\parts>2\relax%
			\southwest%
			\pgf@xa\pgf@x%
			\thirdsplit%
			\pgf@ya\pgf@y
			\secondsplit%
			\advance\pgf@y\pgf@ya%
			\pgf@y.5\pgf@y%
			\pgf@x\pgf@xa%
		\else%
			\southwest
		\fi%
	}
	\anchor{fourth east}{%
		\getrectanglesplitparameters%
		\ifnum\parts>3\relax%
			\northeast%
			\pgf@xa\pgf@x%
			\southwest%
			\pgf@ya\linewidth\relax%
			\pgf@ya.5\pgf@ya%
			\advance\pgf@ya\pgf@y%
			\thirdsplit%
			\advance\pgf@y\pgf@ya%
			\pgf@y.5\pgf@y%
			\pgf@x\pgf@xa%
		\else%
			\northeast%
			\pgf@xa\pgf@x%
			\southwest%
			\pgf@x\pgf@xa%
		\fi%
	}
	\anchor{fourth west}{%
		\getrectanglesplitparameters%
		\ifnum\parts>3\relax%
			\southwest%
			\pgf@xa\pgf@x%
			\pgf@ya\linewidth\relax%
			\pgf@ya.5\pgf@ya%
			\advance\pgf@ya\pgf@y%
			\thirdsplit%
			\advance\pgf@y\pgf@ya%
			\pgf@y.5\pgf@y%
			\pgf@x\pgf@xa%
		\else%
			\southwest%
		\fi%
	}
	\backgroundpath{%
		\getrectanglesplitparameters%
		%
		% Remove outer sep.
		%
		\pgfsavepgf@process\southwest{%
			\southwest%
  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
  		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
  	}%
  	\pgfsavepgf@process\northeast{%
			\northeast%
  		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
  		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
  	}%
  	\pgfsavepgf@process\textsplit{%
			\textsplit%
  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
  	}%
  	\pgfsavepgf@process\secondsplit{%
			\secondsplit%
  		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
  	}%
  	\pgfsavepgf@process\thirdsplit{%
			\thirdsplit%
  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
  	}%
  	\pgfpathrectangle{\southwest}{\pgfpointdiff{\southwest}{\northeast}}%
  	{%
  		\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
  		\ifnum\parts>1\relax%
  			\pgfpathmoveto{\textsplit\pgf@ya\pgf@y\southwest\pgf@y\pgf@ya}%
  			\pgfpathlineto{\textsplit\pgf@ya\pgf@y\northeast\pgf@y\pgf@ya}%
  		\fi%
  		\ifnum\parts>2\relax%
  			\pgfpathmoveto{\secondsplit\pgf@ya\pgf@y\southwest\pgf@y\pgf@ya}%
  			\pgfpathlineto{\secondsplit\pgf@ya\pgf@y\northeast\pgf@y\pgf@ya}%
  		\fi%
  		\ifnum\parts>3\relax%
  			\pgfpathmoveto{\thirdsplit\pgf@ya\pgf@y\southwest\pgf@y\pgf@ya}%
  			\pgfpathlineto{\thirdsplit\pgf@ya\pgf@y\northeast\pgf@y\pgf@ya}%
  		\fi%
  	}%
  }
  \behindbackgroundpath{%
  	\ifpgfrectanglesplitusecustomfill%
  		%
			% Remove outer sep.
			%
			\getrectanglesplitparameters%
			\pgfsavepgf@process\southwest{%
				\southwest%
	  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
	  		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
	  	}%
	  	\pgfsavepgf@process\northeast{%
				\northeast%
	  		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
	  		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
	  	}%
	  	\pgfsavepgf@process\textspliteast{%
				\textspliteast%
	  		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
	  	}%
	  	\pgfsavepgf@process\textsplitwest{%
				\textsplitwest%
	  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
	  	}%
	  	\pgfsavepgf@process\secondspliteast{%
				\secondspliteast%
	  		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
	  	}%
	  	\pgfsavepgf@process\secondsplitwest{%
				\secondsplitwest%
	  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
	  	}%
	  	\pgfsavepgf@process\thirdspliteast{%
				\thirdspliteast%
	  		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
	  	}%
	  	\pgfsavepgf@process\thirdsplitwest{%
				\thirdsplitwest%
	  		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
	  	}%
	  	%
  		% Always fill the text box.
  		%
  		\pgfpathmoveto{\textsplitwest}%
  		\pgfpathlineto{\northeast\pgf@ya\pgf@y\southwest\pgf@y\pgf@ya}%
  		\pgfpathlineto{\northeast}%
  		\ifnum\parts>1\relax%
  			\bgroup%
  				\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
  		\fi%  		
  		\pgfpathlineto{\textspliteast}%
  		\pgfpathclose%
  		\ifnum\parts>1\relax%
  			\egroup%
  		\fi% 
  		\pgfsetfillcolor{\pgfkeysvalueof{/pgf/rectangle split text part fill}}%
  		\pgfusepath{fill}%
  		%
  		% Second box.
  		%
  		\ifnum\parts>1\relax%
  			\bgroup%
  				\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
  				\pgfpathmoveto{\textsplitwest}%
  				\pgfpathlineto{\textspliteast}%
	  			\ifnum\parts=2\relax%
	  				\egroup%
	  			\fi%
  				\pgfpathlineto{\secondspliteast}%
  				\pgfpathlineto{\secondsplitwest}%
  				\ifnum\parts=2\relax%
	  				\bgroup%
	  				\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
	  			\fi%
  				\pgfpathclose%
  				\pgfsetfillcolor{\pgfkeysvalueof{/pgf/rectangle split second part fill}}%
  				\pgfusepath{fill}%
  			\egroup%
  		\fi%
  		%
  		% Third box.
  		%
  		\ifnum\parts>2\relax%
  			\bgroup%
  				\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
  				\pgfpathmoveto{\secondsplitwest}%
  				\pgfpathlineto{\secondspliteast}%
  				\ifnum\parts=3\relax%
  					\egroup%
  				\fi%
  				\pgfpathlineto{\thirdspliteast}%
  				\pgfpathlineto{\thirdsplitwest}%
  				\ifnum\parts=3\relax%
  					\bgroup%
  					\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
  				\fi%
  				\pgfpathclose%
  				\pgfsetfillcolor{\pgfkeysvalueof{/pgf/rectangle split third part fill}}%
  				\pgfusepath{fill}%
  			\egroup%
  		\fi%
	  	%
			% And the fourth box.
			%
			\ifnum\parts>3\relax%
				\pgfpathmoveto{\thirdsplitwest}%
				\pgfpathlineto{\southwest}%
				\pgfpathlineto{\southwest\pgf@ya\pgf@y\northeast\pgf@y\pgf@ya}%
				\bgroup%
						\pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
						\pgfpathlineto{\thirdspliteast}%
					\pgfpathclose%
				\egroup%
				\pgfsetfillcolor{\pgfkeysvalueof{/pgf/rectangle split fourth part fill}}%
				\pgfusepath{fill}%
			\fi%
		\fi%
  }
  \anchorborder{%
  	\pgfutil@tempdima\pgf@x%
  	\pgfutil@tempdimb\pgf@y%
  	\getrectanglesplitparameters%
  	\pgfpointdiff{\southwest}{\northeast}%
  	\pgf@x.5\pgf@x%
  	\pgf@y.5\pgf@y%
  	\edef\pgf@marshall{%
  		\noexpand\pgfpointborderrectangle{%
  				\noexpand\pgfqpoint{\the\pgfutil@tempdima}{\the\pgfutil@tempdimb}%
  			}%
      	{%
      		\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}%
      	}%
    }%
    \pgf@marshall%
    \pgf@xa\pgf@x%
    \pgf@ya\pgf@y%
    \centerpoint%
    \advance\pgf@x\pgf@xa%
    \advance\pgf@y\pgf@ya%
   }%
}


% Shape: ellipse split.
%
\pgfdeclareshape{ellipse split}{%
	\nodeparts{text,lower}
	\savedanchor\radii{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\pgf@y2.0\pgf@y%
		\advance\pgf@y.5\pgflinewidth%
		\pgf@xa.5\wd\pgfnodeparttextbox%
		\pgf@xb.5\wd\pgfnodepartlowerbox%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@xb\pgf@x%
		\pgf@ya\ht\pgfnodeparttextbox%
		\advance\pgf@ya\dp\pgfnodeparttextbox%
		\pgf@yb\ht\pgfnodepartlowerbox%
		\advance\pgf@yb\dp\pgfnodepartlowerbox%
		\advance\pgf@ya\pgf@y%
		\advance\pgf@yb\pgf@y%
		\ifdim\pgf@xa>\pgf@xb%
			\pgf@x1.414213\pgf@xa%
		\else%
			\pgf@x1.414213\pgf@xb%
		\fi%
		\ifdim\pgf@ya>\pgf@yb%
			\pgf@y1.414213\pgf@ya%
		\else%
			\pgf@y1.414213\pgf@yb%
		\fi%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@x<.5\pgf@xa%
			\pgf@x.5\pgf@xa%
		\fi%
		\ifdim\pgf@y<.5\pgf@ya%
			\pgf@y.5\pgf@ya%
		\fi%
		\pgfmathaddtolength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
	}
	\savedanchor\lower{%
		\pgf@x-.5\wd\pgfnodepartlowerbox%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\pgf@y-2.0\pgf@y%
		\advance\pgf@y-\pgflinewidth%
		\advance\pgf@y-\dp\pgfnodeparttextbox%
		\advance\pgf@y-\ht\pgfnodepartlowerbox%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{-\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y-\dp\pgfnodeparttextbox%
		\advance\pgf@y-.5\pgflinewidth%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt\relax%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{.5ex}%
	}%
	\anchor{center}{\centerpoint}
	\anchor{lower}{\lower}
	\anchor{mid}{\midpoint}
	\anchor{mid east}{\radii\pgf@xa\pgf@x\midpoint\advance\pgf@x\pgf@xa}
	\anchor{mid west}{\radii\pgf@xa\pgf@x\midpoint\advance\pgf@x-\pgf@xa}
	\anchor{base}{\basepoint}
	\anchor{base east}{\radii\pgf@xa\pgf@x\basepoint\advance\pgf@x\pgf@xa}
	\anchor{base west}{\radii\pgf@xa\pgf@x\basepoint\advance\pgf@x-\pgf@xa}
	\anchor{north}{\pgfpointadd{\centerpoint}{\radii\pgf@x0pt}}%
	\anchor{south}{\pgfpointadd{\centerpoint}{\radii\pgf@x0pt\pgf@y-\pgf@y}}%
	\anchor{east}{\pgfpointadd{\centerpoint}{\radii\pgf@y0pt}}%
	\anchor{west}{\pgfpointadd{\centerpoint}{\radii\pgf@x-\pgf@x\pgf@y0pt}}%	
	\anchor{north west}{\pgfpointadd{\centerpoint}{\radii\pgf@x-0.707106\pgf@x\pgf@y0.707106\pgf@y}}%
	\anchor{south west}{\pgfpointadd{\centerpoint}{\radii\pgf@x-0.707106\pgf@x\pgf@y-0.707106\pgf@y}}%
	\anchor{north east}{\pgfpointadd{\centerpoint}{\radii\pgf@x0.707106\pgf@x\pgf@y0.707106\pgf@y}}%
	\anchor{south east}{\pgfpointadd{\centerpoint}{\radii\pgf@x0.707106\pgf@x\pgf@y-0.707106\pgf@y}}%
	\backgroundpath{%
		\radii%
		\pgfmathaddtolength\pgf@x{-\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathaddtolength\pgf@y{-\pgfkeysvalueof{/pgf/outer ysep}}%
		\pgfutil@tempdima\pgf@x%
		\pgfutil@tempdimb\pgf@y%
		\pgfpathellipse{\centerpoint}{\pgfqpoint{\the\pgfutil@tempdima}{0pt}}{\pgfqpoint{0pt}{\the\pgfutil@tempdimb}}%
		\pgfpathmoveto{\centerpoint\advance\pgf@x-\pgfutil@tempdima}%
		\pgfpathlineto{\centerpoint\advance\pgf@x\pgfutil@tempdima}%
	}
	\anchorborder{%
  	\pgfextract@process\externalpoint{}%
  	\radii%
  	\edef\pgf@marshal{%
   		\noexpand\pgfpointadd{\noexpand\pgfpointborderellipse{\noexpand\externalpoint}%
   			{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}}{\noexpand\centerpoint}%
   	}%  
   	\pgf@marshal%		
  }%
}

\endinput


==> pgflibraryshapes.symbols.code.tex <==
% Copyright 2007 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibraryshapes.symbols.code.tex,v 1.13 2008/01/30 07:56:38 vibrovski Exp $

\pgfdeclareshape{forbidden sign}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  \foregroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.707107\pgfutil@tempdima}{-0.707107\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{0.707107\pgfutil@tempdima}{0.707107\pgfutil@tempdima}}}
  }
}





% Keys for starburst shape
%
% /pgf/starburst point height : The maximum height of the outer points.
% /pgf/starburst points       : The number of points.
% /pgf/random starburst       : The seed for the random number generator.
%
\pgfkeys{/pgf/random starburst/%
	.code={%
		\ifx\pgfkeysnovalue#1%
			\pgfmathgeneratepseudorandomnumber%
		\else%
			\pgfmathtruncatemacro\pgfmathresult{#1}%
		\fi%
		\pgfkeyslet{/pgf/random starburst}{\pgfmathresult}%
	}%
}
\pgfkeys{/pgf/random starburst=100}

\pgfkeys{/pgf/starburst point height/.value required}
\pgfkeys{/pgf/starburst point height/.code={%
		\pgfmathparse{#1}%
		\edef\pgfmathresult{\pgfmathresult pt}%
		\pgfkeyslet{/pgf/starburst point height}{\pgfmathresult}%
	}%
}%
\pgfkeys{/pgf/starburst point height=.5cm}

\pgfkeys{/pgf/starburst points/.value required}
\pgfkeys{/pgf/starburst points/.code={%
		\pgfmathtruncatemacro\pgfmathresult{#1}%
		\pgfkeyslet{/pgf/starburst points}{\pgfmathresult}%
	}%	
}%
\pgfkeys{/pgf/starburst points=17}

\pgfdeclareshape{starburst}{%
	\savedmacro\anglestep{%
		\pgfmathdivide@{180}{\pgfkeysvalueof{/pgf/starburst points}}%
		\let\anglestep\pgfmathresult%
	}
	\savedmacro\calculatestarburstpoints{%
		%
		% Get the angle step.
		%
		\pgfmathdivide@{180}{\pgfkeysvalueof{/pgf/starburst points}}%
		\let\anglestep\pgfmathresult%
		%
		% Get the total number of points.
		%
		\pgfmathsetcounter{pgf@counta}{\pgfkeysvalueof{/pgf/starburst points}}%
		\multiply\c@pgf@counta2\relax%
		\edef\totalpoints{\the\c@pgf@counta}%
		\addtosavedmacro{\totalpoints}%
		%
		% Calculate the centerpoint.
		%
		\pgfextract@process\centerpoint{%
			\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
			\pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
			\pgfmathaddtolength\pgf@y{+-.5\dp\pgfnodeparttextbox}%
		}%
		%
		% Get the larger of the outer sep.
		%
		\pgfmathsetlength\pgf@x{+\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{+\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@x<\pgf@y%
			\pgf@x\pgf@y%
		\fi%
		\edef\outersep{\the\pgf@x}%
		% 
		% Get the node dimensions.
		% 
		\pgfmathsetlength\pgf@x{+\pgfkeysvalueof{/pgf/inner xsep}}%
		\pgfmathaddtolength\pgf@x{+.5\wd\pgfnodeparttextbox}%		
		\pgfmathsetlength\pgf@y{+\pgfkeysvalueof{/pgf/inner ysep}}%
		\pgfmathaddtolength\pgf@y{+.5\ht\pgfnodeparttextbox}%
		\pgfmathaddtolength\pgf@y{+.5\dp\pgfnodeparttextbox}%
		%
		%  Calculate the inner radii.
		%
		\ifpgfshapeborderusesincircle%
			\pgfkeysgetvalue{/pgf/shape border rotate}{\rotate}%
			%
			% Use the incircle...
			%
			\ifdim\pgf@y>\pgf@x%
				\pgf@x\pgf@y%
			\fi%
			\pgf@x1.41421\pgf@x%
			\pgf@y\pgf@x%
		\else%
			%
			% Get the rotation (with rounding).
			%
			\pgfkeysgetvalue{/pgf/shape border rotate}{\rotate}%
			\pgfmathmod@{\rotate}{360}%
			\afterassignment\pgfmath@gobbletilpgfmath@%
			\expandafter\c@pgf@counta\pgfmathresult\relax\pgfmath@%
			\advance\c@pgf@counta45\relax%
			\divide\c@pgf@counta90\relax%
			\multiply\c@pgf@counta90\relax%
			\ifnum\c@pgf@counta<0\relax%
				\advance\c@pgf@counta360\relax%
			\fi%
			%
			% Calculate the width and height of the node
			% contents, according to any border rotation.
			%
			\ifnum\c@pgf@counta=90\relax%
				\pgf@xc\pgf@x%
				\pgf@x\pgf@y%
				\pgf@y\pgf@xc%
			\else%
				\ifnum\c@pgf@counta=270\relax%
					\pgf@xc\pgf@x%
					\pgf@x\pgf@y%
					\pgf@y\pgf@xc%
				\fi%
			\fi%
			\edef\rotate{\the\c@pgf@counta}%
			%
			% ...or not.
			%		
			\pgf@x=1.41421\pgf@x%
			\pgf@y=1.41421\pgf@y%
		\fi%
		\addtosavedmacro{\rotate}%
		% 
		% Adjust innerradius for minimum width and height.
		%
		\pgf@xa\pgf@x% 
		\pgfmathsetlength\pgf@xb{+\pgfkeysvalueof{/pgf/starburst point height}}%
		\advance\pgf@xa\pgf@xb%
		\pgfmathsetlength\pgf@xc{+\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@xa<.5\pgf@xc%
			\pgf@x.5\pgf@xc%
			\advance\pgf@x-\pgf@xb%
		\fi%
		\pgf@ya\pgf@y% 
		\pgfmathsetlength\pgf@yb{+\pgfkeysvalueof{/pgf/starburst point height}}%
		\advance\pgf@ya\pgf@yb%
		\pgfmathsetlength\pgf@yc{+\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@ya<.5\pgf@yc%
			\pgf@y.5\pgf@yc%
			\advance\pgf@y-\pgf@yb%
		\fi%	
		\edef\xinnerradius{\the\pgf@x}%
		\edef\yinnerradius{\the\pgf@y}%
		\addtosavedmacro{\xinnerradius}%
		\addtosavedmacro{\yinnerradius}%
		%
		% Calculate a radius outside the starburst.
		%
		\ifdim\pgf@y>\pgf@x%
			\pgf@x\pgf@y%
		\fi%
		\pgfmathaddtolength\pgf@x{+\pgfkeysvalueof{/pgf/starburst point height}}%
		\edef\externalradius{\the\pgf@x}%
		\addtosavedmacro{\externalradius}%
		%
		% Set the seed for the random number generator.
		%
		\pgfmathsetseed{\pgfkeysvalueof{/pgf/random starburst}}%	
		%
		% Now create the points on the shape and also 
		% the miter length and angle for each point.
		%
		\def\angle{90}% Start at the top.
		%
		% At point a, the miter length and angle are calculated for point b = a - 1.
		%
		\c@pgf@counta1\relax%
		\c@pgf@countb0\relax%
		%
		% As 3 consecutive points are required to be defined for miter
		% calculations, it is necessary to go over the first two points
		% again.
		% 
		\c@pgf@countc\totalpoints\relax%
		\advance\c@pgf@countc2\relax%
		\edef\looppoints{\the\c@pgf@countc}%
		\let\secondpoint\pgfutil@empty%
		\let\thirdpoint\pgfutil@empty%
		\pgfmathloop%
			%
			% Cycle the point definitions.
			%
			\let\firstpoint\secondpoint%	
			\let\secondpoint\thirdpoint%	
			\ifnum\pgfmathcounter>\looppoints%
			\else%
				\ifnum\pgfmathcounter>\totalpoints%
					\expandafter\let\expandafter\thirdpoint\csname point@\the\c@pgf@counta @\endcsname%
				\else%
					\ifodd\pgfmathcounter%
						%
						% An outer point.
						%
						\ifnum\pgfkeysvalueof{/pgf/random starburst}=0\relax%
							\pgf@xa\pgfkeysvalueof{/pgf/starburst point height}\relax%
						\else%
							\pgf@x\pgfkeysvalueof{/pgf/starburst point height}\relax%
							\pgf@xa.75\pgf@x%
							\pgf@xb.25\pgf@x%
							\pgfmathrnd%
							\pgf@xa\pgfmathresult\pgf@xa%
							\advance\pgf@xa\pgf@xb%
						\fi%
						\pgf@x\xinnerradius\relax%
						\advance\pgf@x\pgf@xa%
						\pgf@y\yinnerradius\relax%
						\advance\pgf@y\pgf@xa%
						\expandafter\pgfextract@process\csname point@\the\c@pgf@counta @\endcsname{%
							\pgfpointpolar{\angle}{\the\pgf@x and \the\pgf@y}%
							\pgf@xa\pgf@x%
							\pgf@ya\pgf@y%
							\centerpoint%
							\advance\pgf@x\pgf@xa%
							\advance\pgf@y\pgf@ya%
						}%
					\else%
						%
						% An inner point.
						%
						\expandafter\pgfextract@process\csname point@\the\c@pgf@counta @\endcsname{%
							\pgfpointpolar{\angle}{\xinnerradius and \yinnerradius}%
							\pgf@xa\pgf@x%
							\pgf@ya\pgf@y%
							\centerpoint%
							\advance\pgf@x\pgf@xa%
							\advance\pgf@y\pgf@ya%
						}%						
					\fi%
					%
					% Add the points to the saved macro.
					%
					\expandafter\let\expandafter\thirdpoint\csname point@\the\c@pgf@counta @\endcsname%
					\expandafter\addtosavedmacro\expandafter{\csname point@\the\c@pgf@counta @\endcsname}%
				\fi%				
				%
				% It is only possible to do the miter calculations if three points are defined.
				%
				\ifx\firstpoint\pgfutil@empty%
				\else%
					%
					% Calculate the miter length...
					%
					\pgfmathanglebetweenlines{\secondpoint}{\thirdpoint}{\secondpoint}{\firstpoint}%
					\pgfmathdivide@{\pgfmathresult}{2}%
					\let\defaultmiterangle\pgfmathresult%
					\pgfmathcosec@{\pgfmathresult}%
					\pgf@x\outersep\relax%
					\pgf@x\pgfmathresult\pgf@x%
					\edef\miterlength{\the\pgf@x}%
					%
					% ...the miter angle...
					%
					\pgfmathanglebetweenlines{\firstpoint}{\secondpoint}{\firstpoint}{\thirdpoint}%
					\pgfmathadd@{\pgfmathresult}{\defaultmiterangle}%
					\pgfmathsubtract@{180}{\pgfmathresult}%
					\let\angletemp\pgfmathresult%
					\pgfmathanglebetweenpoints{\firstpoint}{\thirdpoint}%
					\pgfmathsubtract@{180}{\pgfmathresult}%
					\pgfmathsubtract@{\angletemp}{\pgfmathresult}%
					\edef\miterangle{\pgfmathresult}%
					%
					% ...and thus the border point.
					%
					\pgfextract@process\borderpoint{%
						\secondpoint%
						\pgf@xa\pgf@x
						\pgf@ya\pgf@y%
						\pgfpointpolar{\miterangle}{\miterlength}%
						\advance\pgf@x\pgf@xa%
						\advance\pgf@y\pgf@ya%
					}%
					%
					% Get the angle from the centerpoint to the *unrotated* border points.
					%
					\pgfmathanglebetweenpoints{\centerpoint}{\borderpoint}%
					\expandafter\edef\csname angletoborderpoint@\the\c@pgf@countb @\endcsname{\pgfmathresult}%
					\expandafter\addtosavedmacro\expandafter{\csname angletoborderpoint@\the\c@pgf@countb @\endcsname}%
					%
					% Rotatee the border points and save.
					%
					\expandafter\pgfextract@process\csname borderpoint@\the\c@pgf@countb @\endcsname{%
						\pgfmathrotatepointaround{\borderpoint}{\centerpoint}{\rotate}%
					}%
					\expandafter\addtosavedmacro\expandafter{\csname borderpoint@\the\c@pgf@countb @\endcsname}%				
					%
					% Now create the anchors.
					%
					\c@pgf@countc\c@pgf@countb%
					\advance\c@pgf@countc1\relax%
					\divide\c@pgf@countc2\relax%
					\ifodd\c@pgf@countb\relax%
						\pgfutil@ifundefined{pgf@anchor@starburst@outer point\space\the\c@pgf@countc}{%
							\expandafter\xdef\csname pgf@anchor@starburst@outer point\space\the\c@pgf@countc\endcsname{%
								\noexpand\calculatestarburstpoints%
								\noexpand\csname borderpoint@\the\c@pgf@countb @\noexpand\endcsname%
							}%
						}{}%
					\else%
						\pgfutil@ifundefined{pgf@anchor@starburst@inner point\space\the\c@pgf@countc}{%
							\expandafter\xdef\csname pgf@anchor@starburst@inner point\space\the\c@pgf@countc\endcsname{%
								\noexpand\calculatestarburstpoints%
								\noexpand\csname borderpoint@\the\c@pgf@countb @\noexpand\endcsname%
							}%
						}{}%
					\fi%
				\fi%
				\pgfmathadd@{\angle}{\anglestep}%
				\pgfmathmod@{\pgfmathresult}{360}%	
				\let\angle\pgfmathresult%
				\advance\c@pgf@counta1\relax%
				\ifnum\c@pgf@counta>\totalpoints%
					\c@pgf@counta1\relax%
				\fi%
				\advance\c@pgf@countb1\relax%
				\ifnum\c@pgf@countb>\totalpoints%
					\c@pgf@countb1\relax%
				\fi%
		\repeatpgfmathloop%
	}
	\savedanchor\centerpoint{%
		\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
		\pgfmathsetlength\pgf@y{+.5\ht\pgfnodeparttextbox}%
		\pgfmathaddtolength\pgf@y{+-.5\dp\pgfnodeparttextbox}%
	}%
	\savedanchor\midpoint{%
		\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\savedanchor\basepoint{%
		\pgfmathsetlength\pgf@x{+.5\wd\pgfnodeparttextbox}%
		\pgf@y0pt\relax%
	}%
	\anchor{center}{\centerpoint}
	\anchor{base}{\basepoint}
	\anchor{mid}{\midpoint}
	\anchor{north}{%
		\calculatestarburstpoints%
		\csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{0pt}{\externalradius}}%
	}
	\anchor{south}{%
		\calculatestarburstpoints%
		\csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{0pt}{-\externalradius}}%
	}
	\anchor{east}{%
		\calculatestarburstpoints%
		\csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{\externalradius}{0pt}}%
	}
	\anchor{west}{%
		\calculatestarburstpoints%
		\csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{-\externalradius}{0pt}}%
	}
	\anchor{north west}{%
		\calculatestarburstpoints%
		\csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{-\externalradius}{\externalradius}}%
	}
	\anchor{south west}{%
		\calculatestarburstpoints%
		\csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{-\externalradius}{-\externalradius}}%
	}
	\anchor{north east}{%
		\calculatestarburstpoints%
		\csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{\externalradius}{\externalradius}}%
	}
	\anchor{south east}{%
		\calculatestarburstpoints%
		\csname pgf@anchor@starburst@border\endcsname{\pgfqpoint{\externalradius}{-\externalradius}}%
	}
	\backgroundpath{%	
		\calculatestarburstpoints%
		\pgfmathloop%
			\ifnum\pgfmathcounter>\totalpoints%
			\else%
				\ifnum\pgfmathcounter=1\relax%
					\let\starburstaction\pgfpathmoveto%
				\else%
					\let\starburstaction\pgfpathlineto%
				\fi%
				\starburstaction{%
					%\pgfmathrotatepointaround{\csname point@\pgfmathcounter @\endcsname}{\centerpoint}{\rotate}}%
					\csname point@\pgfmathcounter @\endcsname}
			\repeatpgfmathloop%
		\pgfpathclose%		
	}
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% Adjust the location of the external 
		% point relative to \centerpoint.
		%
		\centerpoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Get the starburst points.
		%
		\calculatestarburstpoints%
		%
		% Get the angle of the external point to the \centerpoint.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
		\pgfmathsubtract@{\pgfmathresult}{\rotate}%
		\ifdim\pgfmathresult pt<0pt\relax%
			\pgfmathadd@{\pgfmathresult}{360}%
		\fi%
		\let\externalangle\pgfmathresult%
		%
		% Locate the appropriate sides on the starburst border...
		%
		\ifdim\externalangle pt<90pt\relax%
			\c@pgf@counta0\relax%
			\c@pgf@countb\totalpoints\relax%
			\pgfmathloop%
			\ifnum\c@pgf@counta>0\relax%
			\else%
				\ifdim\csname angletoborderpoint@\the\c@pgf@countb @\endcsname pt>90pt\relax%
					\c@pgf@counta\c@pgf@countb%
				\else%
					\ifdim\externalangle pt>\csname angletoborderpoint@\the\c@pgf@countb @\endcsname pt\relax%
						\c@pgf@counta\c@pgf@countb%
					\fi%
				\fi%
				\advance\c@pgf@countb-1\relax%
			\repeatpgfmathloop%
			\edef\first{\the\c@pgf@counta}%
			\advance\c@pgf@counta1\relax%
			\ifnum\c@pgf@counta>\totalpoints\relax%
				\c@pgf@counta1\relax%
			\fi%
			\edef\second{\the\c@pgf@counta}%
		\else%
			\c@pgf@counta0\relax%
			\pgfmathloop%
			\ifnum\c@pgf@counta>0\relax%
			\else%
				\ifdim\csname angletoborderpoint@\pgfmathcounter @\endcsname pt<90pt\relax%
					\c@pgf@counta\pgfmathcounter%
				\else%
					\ifdim\externalangle pt<\csname angletoborderpoint@\pgfmathcounter @\endcsname pt\relax%
						\c@pgf@counta\pgfmathcounter%	
					\fi%
				\fi%					
			\repeatpgfmathloop%
			\edef\first{\the\c@pgf@counta}%
			\advance\c@pgf@counta-1\relax%
			\ifnum\c@pgf@counta=0\relax%
				\c@pgf@counta\totalpoints\relax%
			\fi%
			\edef\second{\the\c@pgf@counta}%
		\fi%
		%
		% ...and thus, the point on the star border.
		%
		\pgfpointintersectionoflines{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
				{\csname borderpoint@\first @\endcsname}{\csname borderpoint@\second @\endcsname}%
	}%
}




% Keys for shape cloud.
%
% /pgf/cloud puffs    : the number of cloud puffs.
% /pgf/cloud puff arc : the length of the cloud puff arc.

\newif\ifpgfcloudanchorsuseellipse%
\newif\ifpgfcloudignoresaspect%
\pgfcloudignoresaspectfalse%
\pgfkeys{/pgf/.cd,
	cloud puffs/.initial=10,
	cloud puff arc/.initial=150,
	cloud ignores aspect/.is if=pgfcloudignoresaspect,
	cloud anchors use ellipse/.is if=pgfcloudanchorsuseellipse
}%


% If symbol library is loaded separately these need to be defined.
%
\pgfkeys{/pgf/.cd,
	aspect/.code={\pgfsetshapeaspect{#1}},% this for tikz...
	shape aspect/.initial=1,% but this is consistent with other pgfset stuff. 
	shape aspect/.code={%
		\pgfkeys{/pgf/aspect=#1}%
		\pgfkeyssetvalue{/pgf/shape aspect}{#1}
	}%
}

\def\pgfsetshapeaspect#1{%
  \def\pgfshapeaspect{#1}%
  % Invert
  \pgfutil@tempdima=#1pt%
  \pgfutil@tempdima=.125\pgfutil@tempdima%
  \c@pgf@counta=\pgfutil@tempdima\relax% 8192*determinant
  \pgfutil@tempdima=8192pt%
  \divide\pgfutil@tempdima by\c@pgf@counta%
  \edef\pgfshapeaspectinverse{\pgf@sys@tonumber{\pgfutil@tempdima}}
}

\pgfsetshapeaspect{1}
%

% Shape cloud.
%
\pgfdeclareshape{cloud}{%
	\savedmacro\getradii{%
		\pgfmathtruncatemacro\puffs{\pgfkeysvalueof{/pgf/cloud puffs}}%
		\addtosavedmacro\puffs%
		\pgfmathdivide{360}{\pgfkeysvalueof{/pgf/cloud puffs}}%
		\let\anglestep\pgfmathresult%
		\addtosavedmacro\anglestep%
		\pgfmathsetmacro\arc{\pgfkeysvalueof{/pgf/cloud puff arc}}%
		\addtosavedmacro\arc%
		%
		% x radius.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@x1.4142135\pgf@x%
		%
		% y radius.
		%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		\pgf@y1.4142135\pgf@y%
		%
		% Adjust for shape aspect.
		%
		\ifpgfcloudignoresaspect%
			\pgf@xc\pgf@x%
			\pgf@yc\pgf@y%
		\else%
			\pgf@xc\pgfshapeaspect\pgf@y%
			\ifdim\pgf@xc<\pgf@x%
				\pgf@xc\pgf@x%
			\fi%
	    \pgf@yc\pgfshapeaspectinverse\pgf@xc%
	  	\ifdim\pgf@yc<\pgf@y%
	  		\pgf@yc\pgf@y%
				\pgf@xc\pgfshapeaspect\pgf@y%
			\fi%
		\fi%
    %
		\edef\xinnerradius{\the\pgf@xc}%
		\edef\yinnerradius{\the\pgf@yc}%
		%
		% Get the larger of the outer sep.
		%	
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@x<\pgf@y%
			\pgf@x\pgf@y%
		\fi%
		\edef\outersep{\the\pgf@x}%
		\addtosavedmacro\outersep%
		%
		% For a given cloud, with puff arc length a, the quotient of the
		% distance between the start and end point of a puffs circular arc
		% and the radius of that arc, is constant:
		%
		% g = .5 * sec((180-a)/2)
		% 
		\pgfmathsubtract{180}{\arc}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\tempangle\pgfmathresult%
		\pgfmathsec@{\pgfmathresult}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\arcradiusquotient\pgfmathresult%
		\addtosavedmacro\arcradiusquotient%
		%
		% In addition, the quotient of the distance between the start and
		% end point of a puffs circular arc and the height of that arc 
		% (ignoring rotation), is also constant:
		%
		% h = .5 * (1-sin((180-a)/2))/cos((180-a)/2)
		%   = g  * (1 - sin((180-a)/2))
		\pgfmathsin@{\tempangle}%
		\pgfmathsubtract@{1}{\pgfmathresult}%
		\pgfmathmultiply@{\pgfmathresult}{\arcradiusquotient}%
		\let\archeightquotient\pgfmathresult%
		\addtosavedmacro\archeightquotient%
		%
		% Minimum size is applied to the circum-ellipse (i.e. the ellipse 
		% that passes through the extremeties of each puff). Thus, the
		% relationship between the radii of the elliptical incircle ("inellipse"?) 
		% of the cloud (x and y) and the radii of the circum-ellispe (X and Y), 
		% is given by 
		%
		% X = 2(x*cos(p/2) + ky)  
		% Y = 2(y*cos(p/2) + kx)
		% 
		% where:
		% k = sin(p/2)*((1-cos(a/2))/sin(a/2))
		% p = the angle between each puff (i.e. 360/<puffs>) 
		% a = the length of arc of the puff.
		% 
		\pgfmathdivide{\arc}{2}%
		\let\halfarcangle\pgfmathresult%
		\pgfmathcos@{\pgfmathresult}%
		\pgfmathsubtract@{1}{\pgfmathresult}%
		\let\pgf@temp\pgfmathresult%
		\pgfmathsin@{\halfarcangle}%
		\pgfmathdivide@{\pgf@temp}{\pgfmathresult}%
		\let\pgf@temp\pgfmathresult%
		\pgfmathdivide@{\anglestep}{2}%
		\pgfmathsin@{\pgfmathresult}%
		\pgfmathmultiply@{\pgfmathresult}{\pgf@temp}%
		\let\k\pgfmathresult%
		%
		\pgfmathdivide@{\anglestep}{2}%
		\pgfmathcos@{\pgfmathresult}%
		\let\coshalfanglestep\pgfmathresult%
		%
		% Calculate the actual radii of the circum-ellipse.
		%
		\pgf@x\xinnerradius\relax%
		\pgf@y\yinnerradius\relax%
		\pgf@xa\coshalfanglestep\pgf@x%
		\advance\pgf@xa\k\pgf@y%
		\pgf@ya\coshalfanglestep\pgf@y%
		\advance\pgf@ya\k\pgf@x%
		%
		% Adjust for minimum height (Y').
		%
		\pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@ya<.5\pgf@yb%
			\pgf@ya.5\pgf@yb%
		\fi%
		%
		% Adjust for minimum width (X').
		%
		\pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgf@xa<.5\pgf@xb%
			\pgf@xa.5\pgf@xb%
		\fi%
		%
		\edef\xouterradius{\the\pgf@xa}%
		\addtosavedmacro\xouterradius%
		\edef\youterradius{\the\pgf@ya}%
		\addtosavedmacro\youterradius%
		%
		% Now recalculate `in-ellispe' radii: 
		%
		% x = (X'cos(p/2)-kY')/cos^2(p/2)-k^2, 
		% y = (Y'cos(p/2)-kX')/cos^2(p/2)-k^2, 
		%
		\pgf@xc\k pt\relax%
		\pgf@xc-\k\pgf@xc%
		\pgf@yc\coshalfanglestep pt\relax%
		\pgf@yc\coshalfanglestep\pgf@yc%
		\advance\pgf@xc\pgf@yc\relax%
		\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@xc}}% cos^2(p/2)-k^2
		%
		\pgf@x\coshalfanglestep\pgf@xa%
		\advance\pgf@x-\k\pgf@ya%
		\pgf@x\pgfmathresult\pgf@x%
		\pgf@y\coshalfanglestep\pgf@ya%
		\advance\pgf@y-\k\pgf@xa%
		\pgf@y\pgfmathresult\pgf@y%
		%
		\edef\xinnerradius{\the\pgf@x}%
		\edef\yinnerradius{\the\pgf@y}%
		\addtosavedmacro\xinnerradius%
		\addtosavedmacro\yinnerradius%
		%
		% Get some useful trig. constants.
		%
		\pgfmathdivide@{\arc}{4}%
		\let\quarterarc\pgfmathresult%
		\pgfmathsubtract@{180}{\arc}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\halfcomplementarc\pgfmathresult%
		%
		\addtosavedmacro\arc%
		\addtosavedmacro\quarterarc%
		\addtosavedmacro\halfcomplementarc%
		%
		\pgfmathsec@{\halfcomplementarc}% 1/cos((180-a)/2)
		\let\sechalfcomplementarc\pgfmathresult%
		\pgfmathsin@{\halfcomplementarc}% sin((180-a)/2)
		\let\sinhalfcomplementarc\pgfmathresult%
		%
		\addtosavedmacro\sechalfcomplementarc%
		\addtosavedmacro\sinhalfcomplementarc%
		%
		\pgfmathsin@{\quarterarc}% sin(a/4)
		\let\sinquarterarc\pgfmathresult%
		\pgfmathcos@{\quarterarc}% cos(a/4)
		\let\cosquarterarc\pgfmathresult%
		\pgfmathreciprocal@{\cosquarterarc}%
		\pgfmathmultiply@{\pgfmathresult}{\sinquarterarc}% tan(a/4)
		\let\tanquarterarc\pgfmathresult%
		%
		\addtosavedmacro\sinquarterarc%
		\addtosavedmacro\cosquarterarc%
		\addtosavedmacro\tanquarterarc%
		%
	}
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}
	\anchor{mid}{\midpoint}
	\anchor{base}{\basepoint}
	\anchor{north}{%
		\getradii%
		\csname pgf@anchor@cloud@border\endcsname{\pgfqpoint{0pt}{\youterradius}}%
	}%
	\anchor{south}{%
		\getradii%
		\csname pgf@anchor@cloud@border\endcsname{\pgfqpoint{0pt}{-\youterradius}}%
	}%
	\anchor{east}{%
		\getradii%
		\csname pgf@anchor@cloud@border\endcsname{\pgfqpoint{\xouterradius}{0pt}}%
	}%
	\anchor{west}{%
		\getradii%
		\csname pgf@anchor@cloud@border\endcsname{\pgfqpoint{-\xouterradius}{0pt}}%
	}%
	\anchor{north west}{%
		\getradii%
		\pgfextract@process\pgf@sh{%
			\pgf@x\xouterradius\relax%
			\pgf@x-0.707106\pgf@x%
			\pgf@y\youterradius\relax%
			\pgf@y0.707106\pgf@y%
		}%
		\csname pgf@anchor@cloud@border\endcsname{\pgf@sh}%
	}%
	\anchor{north east}{%
		\getradii%
		\pgfextract@process\pgf@sh{%
			\pgf@x\xouterradius\relax%
			\pgf@x0.707106\pgf@x%
			\pgf@y\youterradius\relax%
			\pgf@y0.707106\pgf@y%
		}%
		\csname pgf@anchor@cloud@border\endcsname{\pgf@sh}%
	}%
	\anchor{south west}{%
		\getradii%
		\pgfextract@process\pgf@sh{%
			\pgf@x\xouterradius\relax%
			\pgf@x-0.707106\pgf@x%
			\pgf@y\youterradius\relax%
			\pgf@y-0.707106\pgf@y%
		}%
		\csname pgf@anchor@cloud@border\endcsname{\pgf@sh}%
	}%
	\anchor{south east}{%
		\getradii%
		\pgfextract@process\pgf@sh{%
			\pgf@x\xouterradius\relax%
			\pgf@x0.707106\pgf@x%
			\pgf@y\youterradius\relax%
			\pgf@y-0.707106\pgf@y%
		}%
		\csname pgf@anchor@cloud@border\endcsname{\pgf@sh}%
	}%
	%
	% Each `puff' is a circular arc of length a, drawn using two a/2 
	% arcs (a < 180), approximated by Bezier curves. 
	% Due to TeX rounding errors, it is sometimes necessary to `force' 
	% the arc to end at a specific point. So...
	%
	% @article{riskus2006,
	%   author  = {Aleskus Ri\v{s}kus},
	% 	title   = {Approximation of a cubic Bezier curve by circular arcs and vice versa},
	%   journal = {Information Technology and Control},
	%   year    = {2006},
	%   volume  = {35},
	%   number  = {4}
	% }
	%
	\backgroundpath{%
		{%
		\getradii%
		%
		% Get the start angle.
		%
		\pgfmathdivide@{\anglestep}{2}%
		\pgfmathsubtract@{90}{\pgfmathresult}%
		\let\angle\pgfmathresult%
		%
		% Calculate the first arc point.
		%
		\pgfextract@process\arcfirstpoint{%
			\pgfpointadd{\centerpoint}{%
				\pgfpointpolar{+\angle}{+\xinnerradius and +\yinnerradius}%
			}%
		}%
		\pgfpathmoveto{\arcfirstpoint}%
		\let\arcendpoint\arcfirstpoint%
		%
		\pgfmathloop%
		\ifnum\pgfmathcounter>\puffs\relax%
		\else
			\let\arcstartpoint\arcendpoint%
			%
			% Make sure beginning and end of path are exactly the same.
			%
			\ifnum\pgfmathcounter=\puffs\relax%
				\let\arcendpoint\arcfirstpoint%
			\else%
				\pgfmathadd@{\angle}{\anglestep}%
				\let\angle\pgfmathresult%
				\pgfextract@process\arcendpoint{%
					\pgfpointadd{\centerpoint}{%
						\pgfpointpolar{+\angle}{+\xinnerradius and +\yinnerradius}%
					}%
				}%	
			\fi%
			%
			% Get some useful cloud parameters from \arcstartpoint and \arcendpoint.
			%
			\pgf@sh@getcloudpuffparameters%
			%
			% Get the rotation for the Bezier curve.
			%
			\pgfmathsubtract@{90}{\quarterarc}%
			\pgfmathadd@{\pgfmathresult}{\arcslope}%
			\let\arcrotate\pgfmathresult%
			\pgfmathsin@{\arcrotate}%
			\let\sinarcrotate\pgfmathresult%
			\pgfmathcos@{\arcrotate}%
			\let\cosarcrotate\pgfmathresult%
			%
			% Calculate the amount by which to scale the control 
			% points, in order to approximate an a/2 arc with radius x.
			%
			\pgf@x\arcradius\relax%
			\pgf@x\tanquarterarc\pgf@x% tan(a/4)
			\edef\controlscale{\pgfmath@tonumber{\pgf@x}}%
			%
			% Get the first control point for the first arc (length a/2)...
			%
			\pgfextract@process\controlone{%
				%
				% k = 0.552284745 (a `magic' number)...
				%
				\pgf@x0.55228475pt\relax%
				\pgf@x\sinquarterarc\pgf@x% k * sin(a/2)
				\pgf@y0.55228475pt\relax%
				\pgf@y\cosquarterarc\pgf@y% k * cos(a/2)
				%
				% ...scale the control points up...
				%
				\pgf@x\controlscale\pgf@x%
				\pgf@y\controlscale\pgf@y%
				%
				% ...rotate...
				%
				\pgf@xa\cosarcrotate\pgf@x%
				\advance\pgf@xa-\sinarcrotate\pgf@y%
				\pgf@ya\cosarcrotate\pgf@y%
				\advance\pgf@ya\sinarcrotate\pgf@x%
				%
				% ...and shift.
				%
				\arcstartpoint%
				\advance\pgf@x\pgf@xa%
				\advance\pgf@y\pgf@ya%
			}%
			%
			% Get the midpoint of the 150° arc.
			%
			\pgfextract@process\arcmidpoint{%
				\pgfextract@process\arcmidpoint{%
					\pgf@x-\halfchordlength\relax%
					\pgf@y\segmentheight\relax%
				}%
				\pgfpointadd{\arcstartpoint}{%
					\pgfmathrotatepointaround{\arcmidpoint}{\pgfpointorigin}{\arcslope}%
				}%
			}%
			%
			% Get the second control point for the first arc (length a/2)...
			%
			\pgfextract@process\controltwo{%		
				\pgf@x0.55228475pt\relax%
				\pgf@x\sinquarterarc\pgf@x%  k * sin(a/2)
				\pgf@y-0.55228475pt\relax%
				\pgf@y\cosquarterarc\pgf@y% -k * cos(a/2)		
				%
				% ...scale, rotate and shift.
				%
				\pgf@x\controlscale\pgf@x%
				\pgf@y\controlscale\pgf@y%
				%
				\pgf@xa\cosarcrotate\pgf@x%
				\advance\pgf@xa-\sinarcrotate\pgf@y%
				\pgf@ya\cosarcrotate\pgf@y%
				\advance\pgf@ya\sinarcrotate\pgf@x%
				%
				\arcmidpoint%
				\advance\pgf@x\pgf@xa%
				\advance\pgf@y\pgf@ya%
			}%
			{%
				\pgfsetcornersarced{\pgfpointorigin}%
				\pgfpathcurveto{\controlone}{\controltwo}{\arcmidpoint}%
			}%
			%
			% Do the same for the second arc...
			%
			\pgfmathadd@{\quarterarc}{90}%
			\pgfmathadd@{\pgfmathresult}{\arcslope}%
			\let\arcrotate\pgfmathresult%
			\pgfmathsin@{\arcrotate}%
			\let\sinarcrotate\pgfmathresult%
			\pgfmathcos@{\arcrotate}%
			\let\cosarcrotate\pgfmathresult%
			%
			% First control point for the second arc...
			%
			\pgfextract@process\controlone{%				
				\pgf@x0.55228475pt\relax%
				\pgf@x\sinquarterarc\pgf@x% k * sin(a/2)
				\pgf@y0.55228475pt\relax%
				\pgf@y\cosquarterarc\pgf@y% k * cos(a/2)
				%
				% ...scale, rotate and shift.
				%
				\pgf@x\controlscale\pgf@x%
				\pgf@y\controlscale\pgf@y%
				%
				\pgf@xa\cosarcrotate\pgf@x%
				\advance\pgf@xa-\sinarcrotate\pgf@y%
				\pgf@ya\cosarcrotate\pgf@y%
				\advance\pgf@ya\sinarcrotate\pgf@x%
				%
				\arcmidpoint%
				\advance\pgf@x\pgf@xa%
				\advance\pgf@y\pgf@ya%
			}%
			%
			% Second control point for the second arc.
			%
			\pgfextract@process\controltwo{%				
				\pgf@x0.55228475pt\relax%
				\pgf@x\sinquarterarc\pgf@x%  k * sin(a/2)
				\pgf@y-0.55228475pt\relax%
				\pgf@y\cosquarterarc\pgf@y% -k * cos(a/2)		
				%
				% ...scale, rotate and shift.
				%
				\pgf@x\controlscale\pgf@x%
				\pgf@y\controlscale\pgf@y%
				%
				\pgf@xa\cosarcrotate\pgf@x%
				\advance\pgf@xa-\sinarcrotate\pgf@y%
				\pgf@ya\cosarcrotate\pgf@y%
				\advance\pgf@ya\sinarcrotate\pgf@x%
				%
				\arcendpoint%
				\advance\pgf@x\pgf@xa%
				\advance\pgf@y\pgf@ya%
			}%
			\pgfpathcurveto{\controlone}{\controltwo}{\arcendpoint}%
			\repeatpgfmathloop%
		\pgfpathclose% Phew!
		}%
	}%
	%
	% Calculate a point on the border of the cloud. This is a two-stage process:
	%
	% 1. Locate the correct puff.
	% 2. Locate the angle on the circular arc which forms the puff.
	%
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
	 	%
		% Get the inner radii and trig. constants.
		%
		\getradii%		
		%
		%
		%
		\ifpgfcloudanchorsuseellipse%
			\pgfpointadd{\centerpoint}{%
				\pgfpointborderellipse{%
					\pgfpoint{\externalx}{\externaly}
					}{%
						\pgfpoint{\xouterradius}{\youterradius}
					}%
			}%
		\else%
			\pgfextract@process\externalpoint{%
				\centerpoint%
				\advance\pgf@x\externalx\relax%
				\advance\pgf@y\externaly\relax%
			}%
			\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
			\let\externalangle\pgfmathresult%
			%
			% 1. Locate the correct puff: 
			%
			% Get end angle of the relavent puff arc.
			%
			\pgfmathdivide@{\anglestep}{2}%
			\let\halfanglestep\pgfmathresult%
			\pgfmathsubtract@{90}{\halfanglestep}%
			\let\endangle\pgfmathresult%
			\pgfmathloop%
				\pgfmathsubtract@{\endangle}{\anglestep}%
				\ifdim\pgfmathresult pt<-\anglestep pt\relax%
				\else%
					\let\endangle\pgfmathresult%
			\repeatpgfmathloop%
			\def\angle{0}%
			\let\lastangle\angle%
			\pgfmathloop%
				\pgfmathadd@{\endangle}{\anglestep}%
				\let\endangle\pgfmathresult%
				%
				% Calculate the `miter point'. This is the point between 
				% each puff, and takes into account the outer sep.
				%
				\pgfextract@process\miterpoint{%
					%
					\pgfextract@process\secondpoint{%
						\pgfpointpolar{+\endangle}{+\xinnerradius and +\yinnerradius}%
					}%
					%
					\pgfmathadd@{\endangle}{\anglestep}%
					\let\angletemp\pgfmathresult%
					\pgfextract@process\thirdpoint{%
						\pgfpointpolar{+\angletemp}{+\xinnerradius and +\yinnerradius}%
					}%
					%
					\pgfmathsubtract@{\endangle}{\anglestep}%
					\let\angletemp\pgfmathresult%
					\pgfextract@process\firstpoint{%
						\pgfpointpolar{+\angletemp}{+\xinnerradius and +\yinnerradius}%
					}%
					%
					\pgfmathanglebetweenpoints{\firstpoint}{\secondpoint}%
					\let\anglealpha\pgfmathresult%
					\pgfmathanglebetweenpoints{\secondpoint}{\thirdpoint}%
					\let\anglebeta\pgfmathresult%
					%
					\pgfmathsubtract@{\anglebeta}{\anglealpha}%
					\pgfmathdivide@{\pgfmathresult}{2}%
					\pgfmathadd@{\pgfmathresult}{\halfcomplementarc}%
					\pgfmathcosec@{\pgfmathresult}%
					\pgf@x\outersep\relax%
					\pgf@x\pgfmathresult\pgf@x%
					\edef\miterradius{\the\pgf@x}%
					%
					\pgfmathadd@{\anglealpha}{\anglebeta}%
					\pgfmathsubtract@{\pgfmathresult}{180}%
					\pgfmathdivide@{\pgfmathresult}{2}%
					\let\miterangle\pgfmathresult%
					\pgfpointadd{\secondpoint}{%
						\pgfqpointpolar{\miterangle}{\miterradius}%
					}%
				}%
				%
				% Get the angle of the miter point...
				%
				\pgfmathanglebetweenpoints{\pgfpointorigin}{\miterpoint}%
				\let\angle\pgfmathresult%
				\ifdim\angle pt<\lastangle pt\relax% Guard against 360° = 0°
					\pgfmathadd@{\angle}{360}%
					\let\angle\pgfmathresult%
				\fi%
				\let\lastangle\angle%
				%
				% ...and see if it is greater than the external point.
				%
			\ifdim\externalangle pt>\angle pt\relax%
			\repeatpgfmathloop%
			%
			% Get the start angle of the relevant arc and ensure angles are in the range.
			%
			\pgfmathmod@{\endangle}{360}%
			\let\endangle\pgfmathresult%
			\pgfmathsubtract@{\endangle}{\anglestep}%
			\ifdim\pgfmathresult pt<0pt\relax%
				\pgfmathadd@{\pgfmathresult}{360}%
			\fi%
			\let\startangle\pgfmathresult%
			%
			% Now, get the start and end points of the arc.
			%
			\pgfextract@process\arcstartpoint{%
				\pgfpointadd{\centerpoint}{%
					\pgfpointpolar{+\startangle}{+\xinnerradius and +\yinnerradius}%
				}%
			}%	
			\pgfextract@process\arcendpoint{%
				\pgfpointadd{\centerpoint}{%
					\pgfpointpolar{+\endangle}{+\xinnerradius and +\yinnerradius}%
				}%
			}%	
			%
			% Get some useful cloud parameters from \arcstartpoint and \arcendpoint.
			%
			\pgf@sh@getcloudpuffparameters%
			%
			% Hackery, for when an arc straddles 0°.
			%
			\ifdim\endangle pt<\startangle pt\relax%
				\pgfmathadd@{\externalangle}{180}%
				\pgfmathmod@{\pgfmathresult}{360}%
				\let\x\pgfmathresult%
			\else%
				\let\x\externalangle%
			\fi%
			%
			% 2. Locate the angle on the circular arc which forms the puff.
			% 
			% Essentially a binary search to find the angle on the circular  
			% arc, which provides the nearset estimate to the border point.
			%
			\let\s\halfcomplementarc% The start of the arc.
			\pgfmathadd@{\s}{\arc}%
			\let\e\pgfmathresult% The end of the arc.
			\pgfmathadd@{\e}{\s}%
			\pgfmathdivide@{\pgfmathresult}{2}%
			\let\n\pgfmathresult% The nearest estimate (default to middle of arc).
			\def\m{360}% Measure of `nearness'.
			\pgfmathloop%
				\pgfmathadd@{\e}{\s}%
				\pgfmathdivide@{\pgfmathresult}{2}%
				\let\p\pgfmathresult% The point halfway between \s and \e.
				\ifdim\p pt=\s pt\relax% 
				\else%
					%
					% Get the point on the circular arc.
					%
					\pgfmathadd@{\p}{\arcslope}%
					\let\a\pgfmathresult%
					\pgfextract@process\arcpoint{%
						\pgfpointadd{\circlecenterpoint}{%
							\pgfqpointpolar{\a}{\outerarcradius}%
						}%
					}%
					%
					% Find the angle between the node centre and the point on the arc.
					%
					\pgfmathanglebetweenpoints{\centerpoint}{\arcpoint}%
					%
					% Hackery, for when an arc straddles 0°.
					%
					\ifdim\endangle pt<\startangle pt\relax%
						\pgfmathadd@{\pgfmathresult}{180}%
						\pgfmathmod@{\pgfmathresult}{360}%
					\fi%
					\let\q\pgfmathresult%
					\ifdim\x pt=\q pt% Found it!
						\pgfmathbreakloop% Breaks after current iteration is complete.
					\else
						\ifdim\x pt<\q pt\relax%
							\let\e\p%
						\else%
							\let\s\p%
						\fi%
					\fi%
					\pgfmathsubtract@{\x}{\q}%
					\pgfmathabs@{\pgfmathresult}%
					%
					% Save the estimate if it is better than any previous estimate.
					%
					\ifdim\pgfmathresult pt<\m pt\relax%
						\let\m\pgfmathresult%
						\let\n\p%
					\fi%				
			\repeatpgfmathloop%
			%
			% Use the nearest estimate as the anchor angle.
			%
			\pgfmathadd@{\n}{\arcslope}%
			\let\anchorangle\pgfmathresult%
			%
			% Finally, the required point.
			%
			\pgfpointadd{\circlecenterpoint}{%
				\pgfqpointpolar{\anchorangle}{\outerarcradius}%
			}%
		\fi%
	}% Again, Phew!
	%
	% Now, a sneaky hack. This means an arbitrary `puff' anchors 
	% can be used for positiong the cloud shape. This is needed
	% if a cloud is positioned using the `puff <n+1>' anchor, where
	% n is the number of puffs of any previously drawn cloud.
	%
	\pgfutil@g@addto@macro\pgf@sh@s@cloud{%
		\c@pgf@counta\puffs\relax%
		\pgfmathloop%
			\ifnum\c@pgf@counta>0\relax%
				\pgfutil@ifundefined{pgf@anchor@cloud@puff\space\the\c@pgf@counta}{%
				\expandafter\xdef\csname pgf@anchor@cloud@puff\space\the\c@pgf@counta\endcsname{%
					\noexpand\pgf@sh@@cloudpuffanchor{\the\c@pgf@counta}%
				}%
			}{\c@pgf@counta0\relax}%
			\advance\c@pgf@counta-1\relax%
		\repeatpgfmathloop%	
	}%
}

% \pgf@sh@@cloudpuffanchor
% 
% Internal macro for calculating the anchors puff 1, puff 2, ... etc.
%
\def\pgf@sh@@cloudpuffanchor#1{%
		\getradii%
		\pgfmathdivide@{\anglestep}{2}%
		\let\halfanglestep\pgfmathresult%
		\c@pgf@counta#1\relax%
		\advance\c@pgf@counta-1\relax%
		\pgfmathmultiply@{\anglestep}{\the\c@pgf@counta}%
		\pgfmathadd@{\pgfmathresult}{90}%
		\pgfmathsubtract@{\pgfmathresult}{\halfanglestep}%
		\let\angle\pgfmathresult%
		%
		% Calculate the first arc point.
		%
		\pgfextract@process\arcstartpoint{%
			\pgfpointadd{\centerpoint}{%
				\pgfpointpolar{+\angle}{+\xinnerradius and +\yinnerradius}%
			}%
		}%
		%
		\pgfmathadd@{\angle}{\anglestep}%
		\let\angle\pgfmathresult%
		\pgfextract@process\arcendpoint{%
			\pgfpointadd{\centerpoint}{%
				\pgfpointpolar{+\angle}{+\xinnerradius and +\yinnerradius}%
			}%
		}%	
		%
		% Get some useful cloud parameters from \arcstartpoint and \arcendpoint.
		%
		\pgf@sh@getcloudpuffparameters%
		%
		% Calculate the point.
		%
		\pgfmathadd@{\arcslope}{90}%
		\let\anchorangle\pgfmathresult%
		\pgfpointadd{\circlecenterpoint}{%
			\pgfqpointpolar{\anchorangle}{\outerarcradius}%
		}%
}  

% \pgf@sh@cloudpuffparameters
%
% Internal macro to calculate some common arc parameters which 
% are required when calculating radii, drawing the background
% path and calculating border anchors.
%
\def\pgf@sh@getcloudpuffparameters{%
  %
	% Calculate the angle to which the entire arc is sloped.
	%
	\pgfmathanglebetweenpoints{\arcendpoint}{\arcstartpoint}%
	\let\arcslope\pgfmathresult%
	%
  % Calculate the chord length and arc radius.
  %
  \pgfpointdiff{\arcendpoint}{\arcstartpoint}%
  \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}
  \pgf@x\pgfmathresult pt\relax%
  \pgf@xa.5\pgf@x%
  \edef\halfchordlength{\the\pgf@xa}%
	\pgf@x\arcradiusquotient\pgf@x%
  \edef\arcradius{\the\pgf@x}%
  \pgf@xa\outersep\relax%
  \advance\pgf@xa\pgf@x%
  \edef\outerarcradius{\the\pgf@xa}%
  %
  % Calculate the height of the resulting segment.
  %
  \pgf@y-\sinhalfcomplementarc\pgf@x% sin((180-a)/2)
  \advance\pgf@y\pgf@x%
  \edef\segmentheight{\the\pgf@y}%
  %
  % Calculate the center of the circle of which the arc is a part.
  %
  \pgfextract@process\circlecenterpoint{%
    \pgfextract@process\circlecenterpoint{%
      \pgf@x-\halfchordlength\relax%
      \pgf@y\segmentheight\relax%
      \advance\pgf@y-\arcradius
    }%
    \pgfpointadd{\arcstartpoint}{%
      \pgfmathrotatepointaround{\circlecenterpoint}{\pgfpointorigin}{\arcslope}%
    }%
  }%
}





% Internal macros for signal shape.
%
\def\pgf@lib@shapes@signal@nowhere{nowhere}%
\def\pgf@lib@shapes@signal@from{from}%
\def\pgf@lib@shapes@signal@to{to}%

\let\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@nowhere%
\let\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@nowhere%
\let\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@nowhere%
\let\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@nowhere%

\def\pgf@lib@shapes@signal@parsedirection#1#2{%
	\let\pgf@lib@shapes@signal@direction#2%
	\pgfutil@in@{and}{#1}%
	\ifpgfutil@in@%
		\pgf@lib@shapes@signal@@parsedirection#1\pgf@lib%
	\else%
		\pgf@lib@shapes@signal@@parsedirection#1 and #1\pgf@lib%
	\fi
}
\def\pgf@lib@shapes@signal@@parsedirection#1 and #2\pgf@lib{%
	\pgfutil@in@{nowhere}{#1}%
	\ifpgfutil@in@
		\pgf@lib@shapes@signal@@donowhere%
	\else%
		\pgf@lib@shapes@signal@@@parsedirection{#1}%
		\pgf@lib@shapes@signal@@@parsedirection{#2}%
	\fi%
}
\def\pgf@lib@shapes@signal@@@parsedirection#1{%
	\pgfutil@in@{ #1 }{ east right }%
	\ifpgfutil@in@%
		\let\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@direction%
		\let\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@nowhere%
		\let\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@nowhere%
	\fi%
	\pgfutil@in@{ #1 }{ left west }%
	\ifpgfutil@in@%
		\let\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@direction%
		\let\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@nowhere%
		\let\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@nowhere%
	\fi%
	\pgfutil@in@{ #1 }{ above up north }%
	\ifpgfutil@in@%
		\let\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@direction%
		\let\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@nowhere%
		\let\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@nowhere%
	\fi%
	\pgfutil@in@{ #1 }{ below down south }%
	\ifpgfutil@in@%
		\let\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@direction%
		\let\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@nowhere%
		\let\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@nowhere%
	\fi%
}

\def\pgf@lib@shapes@signal@@donowhere{%
	\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@direction%
		\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@nowhere%
	\fi%
	\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@direction%
		\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@nowhere%
	\fi%
	\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@direction%
		\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@nowhere%
	\fi%
	\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@direction%
		\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@nowhere%
	\fi%
}


% Keys for signal shape:
%
\pgfkeys{/pgf/.cd,
	signal pointer angle/.initial=90,
	signal from/.code={\pgf@lib@shapes@signal@parsedirection{#1}{\pgf@lib@shapes@signal@from}},
	signal to/.code={\pgf@lib@shapes@signal@parsedirection{#1}{\pgf@lib@shapes@signal@to}}
}


\pgfkeys{/pgf/.cd,
	signal to=east,
	signal from=nowhere
}


% Shape signal
%
%
\pgfdeclareshape{signal}{%
	\savedmacro\installsignalparameters{%
		%
		% Define a centerpoint.
		%
		\pgfextract@process\centerpoint{%
			\pgf@x.5\wd\pgfnodeparttextbox%
			\pgf@y.5\ht\pgfnodeparttextbox%
			\advance\pgf@y-.5\dp\pgfnodeparttextbox%
		}%
		%
		% Get some useful trig. stuff
		%
		\pgfmathsetmacro\pointerangle{\pgfkeysvalueof{/pgf/signal pointer angle}}%
		\pgfmathdivide@{\pointerangle}{2}%
		\let\halfpointerangle\pgfmathresult%
		\pgfmathcosec@{\halfpointerangle}%
		\let\cosechalfpointerangle\pgfmathresult%
		\pgfmathdivide@{\halfpointerangle}{2}%
		\let\quarterpointerangle\pgfmathresult%
		\pgfmathcosec@{\quarterpointerangle}%
		\let\cosecquarterpointerangle\pgfmathresult%
		\pgfmathsec@{\quarterpointerangle}%
		\let\secquarterpointerangle\pgfmathresult%
		\pgfmathsubtract@{90}{\quarterpointerangle}%
		\let\complementquarterpointerangle\pgfmathresult%
		%
		% Get the larger of the outer sep.
		%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/outer ysep}}%
		\ifdim\pgf@x>\pgf@y%
			\pgf@y\pgf@x%
		\fi%
		\pgf@yc\pgf@y%
		%
		% Calculate the miter due to the line width, at the pointer apex... 
		%
		\pgf@x\cosechalfpointerangle\pgf@y%
		\edef\pointerapexmiter{\the\pgf@x}%
		%
		% ...at a corner by a `to' pointer (i.e. sticks out)...
		%
		\pgf@x\secquarterpointerangle\pgf@y%
		\edef\tocornermiter{\the\pgf@x}%
		%
		% ...at a corner by a `from' pointer (i.e. sticks in).
		%
		\pgf@x\cosecquarterpointerangle\pgf@y
		\edef\fromcornermiter{\the\pgf@x}%
		%
		% Get the (half) dimensions of the node.
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@xa.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@ya.5\ht\pgfnodeparttextbox%
		\advance\pgf@ya.5\dp\pgfnodeparttextbox%
		%
		% Get the distance a pointer sticks out to the side...
		%
		\pgfmathsubtract@{90}{\halfpointerangle}%
		\pgfmathtan@{\pgfmathresult}%
		\pgf@xb\pgfmathresult\pgf@ya%
		% 
		% ...and up.
		%
		\pgf@yb\pgfmathresult\pgf@xa%
		%
		% Adjust for minimum height.
		%
		\pgfutil@tempdima2.0\pgf@ya%
		\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@nowhere%
		\else%
			\advance\pgfutil@tempdima\pgf@yb%
		\fi%
		\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@nowhere%
		\else%
			\advance\pgfutil@tempdima\pgf@yb%
		\fi%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgfutil@tempdima<\pgf@y%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgfutil@tempdima}}%
			\pgfutil@tempdima\pgfmathresult\pgf@y%
			\pgf@xa\pgfmath@tonumber{\pgfutil@tempdima}\pgf@xa%
			\pgf@ya\pgfmath@tonumber{\pgfutil@tempdima}\pgf@ya%
			\pgf@xb\pgfmath@tonumber{\pgfutil@tempdima}\pgf@xb%
			\pgf@yb\pgfmath@tonumber{\pgfutil@tempdima}\pgf@yb%
		\fi%
		%
		% Adjust for minimum width.
		%
		\pgfutil@tempdima2.0\pgf@xa%
		\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@nowhere%
		\else%
			\advance\pgfutil@tempdima\pgf@xb%
		\fi%
		\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@nowhere%
		\else%
			\advance\pgfutil@tempdima\pgf@xb%
		\fi%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/minimum width}}%
		\ifdim\pgfutil@tempdima<\pgf@x%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgfutil@tempdima}}%
			\pgfutil@tempdima\pgfmathresult\pgf@x%
			\pgf@xa\pgfmath@tonumber{\pgfutil@tempdima}\pgf@xa%
			\pgf@ya\pgfmath@tonumber{\pgfutil@tempdima}\pgf@ya%
			\pgf@xb\pgfmath@tonumber{\pgfutil@tempdima}\pgf@xb%
			\pgf@yb\pgfmath@tonumber{\pgfutil@tempdima}\pgf@yb%
		\fi%
		%
		% So, define the points for the background path.
		%
		\pgfextract@process\north{%
			\centerpoint%
			\advance\pgf@y\pgf@ya%
			\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@to%
				\advance\pgf@y\pgf@yb%
			\fi%
		}%
		\pgfextract@process\south{%
			\centerpoint%
			\advance\pgf@y-\pgf@ya%
			\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@to%
				\advance\pgf@y-\pgf@yb%
			\fi%
		}%
		\pgfextract@process\east{%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@to%
				\advance\pgf@x\pgf@xb%
			\fi%
		}%
		\pgfextract@process\west{%
			\centerpoint%
			\advance\pgf@x-\pgf@xa%
			\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@to%
				\advance\pgf@x-\pgf@xb%
			\fi%
		}%
		\pgfextract@process\northeast{%
			\centerpoint%
			\advance\pgf@y\pgf@ya%
			\advance\pgf@x\pgf@xa%
			\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@from%
				\advance\pgf@y\pgf@yb%
			\fi%
			\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@from%
				\advance\pgf@x\pgf@xb%
			\fi%
		}%
		\pgfextract@process\southeast{%
			\centerpoint%
			\advance\pgf@y-\pgf@ya%
			\advance\pgf@x\pgf@xa%
			\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@from%
				\advance\pgf@y-\pgf@yb%
			\fi%
			\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@from%
				\advance\pgf@x\pgf@xb%
			\fi%
		}%
		\pgfextract@process\southwest{%
			\centerpoint%
			\advance\pgf@y-\pgf@ya%
			\advance\pgf@x-\pgf@xa%
			\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@from%
				\advance\pgf@y-\pgf@yb%
			\fi%
			\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@from%
				\advance\pgf@x-\pgf@xb%
			\fi%
		}%
		\pgfextract@process\northwest{%
			\centerpoint%
			\advance\pgf@y\pgf@ya%
			\advance\pgf@x-\pgf@xa%
			\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@from%
				\advance\pgf@y\pgf@yb%
			\fi%
			\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@from%
				\advance\pgf@x-\pgf@xb%
			\fi%
		}%
		\addtosavedmacro{\north}%
		\addtosavedmacro{\south}%
		\addtosavedmacro{\east}%
		\addtosavedmacro{\west}%
		\addtosavedmacro{\northeast}%
		\addtosavedmacro{\southwest}%
		\addtosavedmacro{\southeast}%
		\addtosavedmacro{\northwest}%
		%
		% Calculate the `miter vectors' (i.e. +outer sep). 
		%
		\pgfextract@process\northmiter{%
			\pgf@x0pt%
			\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@nowhere%
				\pgf@y\pgf@yc%
			\else%
				\pgf@y\pointerapexmiter\relax%
			\fi%
		}%
		\pgfextract@process\southmiter{%
			\pgf@x0pt%
			\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@nowhere%
				\pgf@y-\pgf@yc%
			\else%
				\pgf@y-\pointerapexmiter\relax%
			\fi%
		}%
		\pgfextract@process\eastmiter{%
			\pgf@y0pt%
			\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@nowhere%
				\pgf@x\pgf@yc%
			\else%
				\pgf@x\pointerapexmiter\relax%
			\fi%
		}%
		\pgfextract@process\westmiter{%
			\pgf@y0pt%
			\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@nowhere%
				\pgf@x-\pgf@yc%
			\else%
				\pgf@x-\pointerapexmiter\relax%
			\fi%
		}%
		\pgfextract@process\northeastmiter{%
			\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@nowhere%
				\pgf@x\pgf@yc
				\pgf@y\pgf@yc%
			\else
				\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@from%
					\pgfqpointpolar{\quarterpointerangle}{\fromcornermiter}
				\else%
					\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@to%
						\pgfqpointpolar{\complementquarterpointerangle}{\tocornermiter}%
					\fi%
				\fi%	
			\fi%
			\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@from%
				\pgfqpointpolar{\complementquarterpointerangle}{\fromcornermiter}%
			\else%
				\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@to%
					\pgfqpointpolar{\quarterpointerangle}{\tocornermiter}%
				\fi%
			\fi%	
		}%
		\pgfextract@process\southeastmiter{%
			\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@nowhere%
				\pgf@x\pgf@yc%
				\pgf@y\pgf@yc%
			\else
				\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@from%
					\pgfqpointpolar{-\quarterpointerangle}{\fromcornermiter}
				\else%
					\ifx\pgf@lib@shapes@signal@east\pgf@lib@shapes@signal@to%
						\pgfqpointpolar{-\complementquarterpointerangle}{\tocornermiter}%
					\fi%
				\fi%	
			\fi%
			\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@from%
				\pgfqpointpolar{-\complementquarterpointerangle}{\fromcornermiter}
			\else%
				\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@to%
					\pgfqpointpolar{-\quarterpointerangle}{\tocornermiter}%
				\fi%
			\fi%	
		}%
		\pgfextract@process\southwestmiter{%
			\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@nowhere%
				\pgf@x-\pgf@yc
				\pgf@y-\pgf@yc%
			\else
				\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@from%
					\pgfmathadd@{\quarterpointerangle}{180}%
					\expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\fromcornermiter}
				\else%
					\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@to%
						\pgfmathadd@{\complementquarterpointerangle}{180}%
						\expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\tocornermiter}%
					\fi%
				\fi%	
			\fi%
			\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@from%
				\pgfmathadd@{\complementquarterpointerangle}{180}%
				\expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\fromcornermiter}%
			\else%
				\ifx\pgf@lib@shapes@signal@south\pgf@lib@shapes@signal@to%
					\pgfmathadd@{\quarterpointerangle}{180}%
					\expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\tocornermiter}%
				\fi%
			\fi%	
		}%
		\pgfextract@process\northwestmiter{%
			\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@nowhere%
				\pgf@x-\pgf@yc%
				\pgf@y\pgf@yc%
			\else
				\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@from%
					\pgfmathsubtract@{180}{\quarterpointerangle}%
					\expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\fromcornermiter}
				\else%
					\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@to%
						\pgfmathsubtract@{180}{\complementquarterpointerangle}%
						\expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\tocornermiter}%
					\fi%
				\fi%	
			\fi%
			\ifx\pgf@lib@shapes@signal@north\pgf@lib@shapes@signal@from%
				\pgfmathsubtract@{180}{\complementquarterpointerangle}%
				\expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\fromcornermiter}%
			\else%
				\ifx\pgf@lib@shapes@signal@west\pgf@lib@shapes@signal@to%
					\pgfmathsubtract@{180}{\quarterpointerangle}%
					\expandafter\pgfqpointpolar\expandafter{\pgfmathresult}{\tocornermiter}%
				\fi%
			\fi%	
		}%
		\addtosavedmacro{\northmiter}%
		\addtosavedmacro{\southmiter}%
		\addtosavedmacro{\eastmiter}%
		\addtosavedmacro{\westmiter}%
		\addtosavedmacro{\northeastmiter}%
		\addtosavedmacro{\southeastmiter}%
		\addtosavedmacro{\southwestmiter}%
		\addtosavedmacro{\northwestmiter}%
		%
		% Now calculate the anchor points
		%
		\pgfextract@process\anchornorth{%
			\pgfpointadd{\north}{\northmiter}%
		}%
		\pgfextract@process\anchorsouth{%
			\pgfpointadd{\south}{\southmiter}%
		}%
		\pgfextract@process\anchoreast{%
			\pgfpointadd{\east}{\eastmiter}%
		}%
		\pgfextract@process\anchorwest{%
			\pgfpointadd{\west}{\westmiter}%
		}%
		\pgfextract@process\anchornortheast{%
			\pgfpointadd{\northeast}{\northeastmiter}%
		}%
		\pgfextract@process\anchorsoutheast{%
			\pgfpointadd{\southeast}{\southeastmiter}%
		}%
		\pgfextract@process\anchorsouthwest{%
			\pgfpointadd{\southwest}{\southwestmiter}%
		}%
		\pgfextract@process\anchornorthwest{%
			\pgfpointadd{\northwest}{\northwestmiter}%
		}%
		\addtosavedmacro{\anchornorth}%
		\addtosavedmacro{\anchorsouth}%
		\addtosavedmacro{\anchoreast}%
		\addtosavedmacro{\anchorwest}%
		\addtosavedmacro{\anchornortheast}%
		\addtosavedmacro{\anchorsouthwest}%
		\addtosavedmacro{\anchorsoutheast}%
		\addtosavedmacro{\anchornorthwest}%		
	}%
	\savedanchor\centerpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%
	}%
	\savedanchor\basepoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}%
	\savedanchor\midpoint{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+.5ex}%
	}%
	\anchor{center}{\centerpoint}%
	\anchor{base}{\basepoint}%
	\anchor{base east}{%
		\installsignalparameters%
		\anchoreast%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\anchorsoutheast%
		\ifdim\pgf@xa>\pgf@x%
			\pgfutil@tempdima\pgf@xa%
		\else%
			\pgfutil@tempdima\pgf@x%
		\fi%
		\pgfextract@process\externalpoint{%
			\basepoint%
			\pgf@x\pgfutil@tempdima%
		}
		\basepoint%
		\let\firstpoint\anchoreast%
		\ifdim\pgf@y<\pgf@ya%
			\let\secondpoint\anchorsoutheast%
		\else%
			\let\secondpoint\anchornortheast%
		\fi%
		\pgfpointintersectionoflines{\basepoint}{\externalpoint}%
			{\firstpoint}{\secondpoint}%		
	}%
	\anchor{base west}{%
		\installsignalparameters%
		\anchorwest%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\anchorsouthwest%
		\ifdim\pgf@xa<\pgf@x%
			\pgfutil@tempdima\pgf@xa%
		\else%
			\pgfutil@tempdima\pgf@x%
		\fi%
		\pgfextract@process\externalpoint{%
			\basepoint%
			\pgf@x\pgfutil@tempdima%
		}
		\basepoint%
		\let\firstpoint\anchorwest%
		\ifdim\pgf@y<\pgf@ya%
			\let\secondpoint\anchorsouthwest%
		\else%
			\let\secondpoint\anchornorthwest%
		\fi%
		\pgfpointintersectionoflines{\basepoint}{\externalpoint}%
			{\firstpoint}{\secondpoint}%		
	}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{%
		\installsignalparameters%
		\anchoreast%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\anchorsoutheast%
		\ifdim\pgf@xa>\pgf@x%
			\pgfutil@tempdima\pgf@xa%
		\else%
			\pgfutil@tempdima\pgf@x%
		\fi%
		\pgfextract@process\externalpoint{%
			\midpoint%
			\pgf@x\pgfutil@tempdima%
		}
		\midpoint%
		\let\firstpoint\anchoreast%
		\ifdim\pgf@y<\pgf@ya%
			\let\secondpoint\anchorsoutheast%
		\else%
			\let\secondpoint\anchornortheast%
		\fi%
		\pgfpointintersectionoflines{\midpoint}{\externalpoint}%
			{\firstpoint}{\secondpoint}%		
	}%
	\anchor{mid west}{%
		\installsignalparameters%
		\anchorwest%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\anchorsouthwest%
		\ifdim\pgf@xa<\pgf@x%
			\pgfutil@tempdima\pgf@xa%
		\else%
			\pgfutil@tempdima\pgf@x%
		\fi%
		\pgfextract@process\externalpoint{%
			\midpoint%
			\pgf@x\pgfutil@tempdima%
		}
		\midpoint%
		\let\firstpoint\anchorwest%
		\ifdim\pgf@y<\pgf@ya%
			\let\secondpoint\anchorsouthwest%
		\else%
			\let\secondpoint\anchornorthwest%
		\fi%
		\pgfpointintersectionoflines{\midpoint}{\externalpoint}%
			{\firstpoint}{\secondpoint}%		
	}%
	\anchor{north}{\installsignalparameters\anchornorth}%
	\anchor{south}{\installsignalparameters\anchorsouth}%
	\anchor{east}{\installsignalparameters\anchoreast}%
	\anchor{west}{\installsignalparameters\anchorwest}%
	\anchor{north east}{\installsignalparameters\anchornortheast}%
	\anchor{south east}{\installsignalparameters\anchorsoutheast}%
	\anchor{south west}{\installsignalparameters\anchorsouthwest}%
	\anchor{north west}{\installsignalparameters\anchornorthwest}%
	\backgroundpath{%
		\installsignalparameters%
		\pgfpathmoveto{\north}%
		\pgfpathlineto{\northeast}%
		\pgfpathlineto{\east}%
		\pgfpathlineto{\southeast}%
		\pgfpathlineto{\south}%
		\pgfpathlineto{\southwest}%
		\pgfpathlineto{\west}%
		\pgfpathlineto{\northwest}%
		\pgfpathclose%
	}
	\anchorborder{%
		%
		% Save x and y.
		%
		\edef\externalx{\the\pgf@x}%
		\edef\externaly{\the\pgf@y}%
		%
		% Adjust the location of the external 
		% point relative to \centerpoint.
		%
		\centerpoint%
		\pgf@xa\externalx\relax%
		\pgf@ya\externaly\relax%
		\advance\pgf@xa\pgf@x%
		\advance\pgf@ya\pgf@y%
		\edef\externalx{\the\pgf@xa}%
		\edef\externaly{\the\pgf@ya}%
		%
		% Get the shape parameters.
		%
		\installsignalparameters%
		%
		% Get the angle of the external point to the \centerpoint.
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
		\let\externalangle\pgfmathresult%
		%
		%
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\anchorwest}%
		\ifdim\externalangle pt<\pgfmathresult pt\relax%
			\pgfmathanglebetweenpoints{\centerpoint}{\anchornorth}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathanglebetweenpoints{\centerpoint}{\anchornortheast}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\let\firstpoint\anchoreast%
					\let\secondpoint\anchornortheast%
				\else%
					\let\secondpoint\anchornortheast%
					\let\firstpoint\anchornorth%
				\fi%
			\else%
				\pgfmathanglebetweenpoints{\centerpoint}{\anchornorthwest}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\let\firstpoint\anchornorth%
					\let\secondpoint\anchornorthwest%
				\else%
					\let\secondpoint\anchornorthwest%
					\let\firstpoint\anchorwest%
				\fi%
			\fi%
		\else%
			\pgfmathanglebetweenpoints{\centerpoint}{\anchorsouth}%
			\ifdim\externalangle pt<\pgfmathresult pt\relax%
				\pgfmathanglebetweenpoints{\centerpoint}{\anchorsouthwest}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\let\firstpoint\anchorwest%
					\let\secondpoint\anchorsouthwest%
				\else%
					\let\secondpoint\anchorsouthwest%
					\let\firstpoint\anchorsouth%
				\fi%
			\else%
				\pgfmathanglebetweenpoints{\centerpoint}{\anchorsoutheast}%
				\ifdim\externalangle pt<\pgfmathresult pt\relax%
					\let\firstpoint\anchorsouth%
					\let\secondpoint\anchorsoutheast%
				\else%
					\let\secondpoint\anchorsoutheast%
					\let\firstpoint\anchoreast%
				\fi%
			\fi%
		\fi%
		%
		% Now locate the point.
		%
		\pgfpointintersectionoflines{\centerpoint}{\pgfqpoint{\externalx}{\externaly}}%
			{\firstpoint}{\secondpoint}%
	}%
}%







% Keys for shape tape
%
% /pgf/tape bend top : Type of bend for north side.
% /pgf/tape bend bottom : Type of bend for south side.
% /pgf/tape bend height : The height of the bends.
\pgfkeys{/pgf/.cd,
	tape bend top/.initial=in and out,
	tape bend bottom/.initial=in and out,
	tape bend/.style={/pgf/tape bend top=#1, /pgf/tape bend bottom=#1},
	tape bend height/.initial=5pt
}

\def\pgf@lib@sh@inandouttext{in and out}
\def\pgf@lib@sh@outandintext{out and in}
\def\pgf@lib@sh@nonetext{none}

\pgfdeclareshape{tape}{
	\savedmacro\tapedimensions{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/pgf/inner xsep}}%
		\advance\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{\pgfkeysvalueof{/pgf/inner ysep}}%
		\advance\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y.5\dp\pgfnodeparttextbox%
		%
		\pgfmathsetlengthmacro\outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}%
		\pgfmathsetlengthmacro\outerysep{\pgfkeysvalueof{/pgf/outer ysep}}%
		\addtosavedmacro\outerxsep%
		\addtosavedmacro\outerysep%
		%
		\pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/tape bend height}}%
		\pgfutil@tempdima.5\pgfutil@tempdima%
		\edef\halfbendheight{\the\pgfutil@tempdima}%
		\addtosavedmacro\halfbendheight%
		%
		\pgfkeysgetvalue{/pgf/tape bend top}{\topbendstyle}%
		\pgfkeysgetvalue{/pgf/tape bend bottom}{\bottombendstyle}%
		\addtosavedmacro\topbendstyle%
		\addtosavedmacro\bottombendstyle%
		%
		\ifx\topbendstyle\pgf@lib@sh@nonetext%
		\else%
			\advance\pgf@y\pgfutil@tempdima%
		\fi%
		\ifx\bottombendstyle\pgf@lib@sh@none%
		\else%
			\advance\pgf@y\pgfutil@tempdima%
		\fi%
		%
		\pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/minimum width}}%
		\pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/minimum height}}%
		\ifdim\pgf@x<.5\pgf@xa%
			\pgf@x.5\pgf@xa%
		\fi%
		\ifdim\pgf@y<.5\pgf@ya%
			\pgf@y.5\pgf@ya%
		\fi%
		\ifx\topbendstyle\pgf@lib@sh@nonetext%
		\else%
			\advance\pgf@y-\pgfutil@tempdima%
		\fi%
		\ifx\bottombendstyle\pgf@lib@sh@nonetext%
		\else%
			\advance\pgf@y-\pgfutil@tempdima%
		\fi%	
		%
		\pgfutil@tempdima3.414213\pgfutil@tempdima% 1 / (1-sin(45))
		\edef\bendyradius{\the\pgfutil@tempdima}%
		\addtosavedmacro\bendyradius%
		\advance\pgfutil@tempdima\outerysep%
		\edef\outerbendyradius{\the\pgfutil@tempdima}%
		\addtosavedmacro\outerbendyradius%
		\advance\pgfutil@tempdima-\outerysep%
		\advance\pgfutil@tempdima-\outerysep%
		\edef\innerbendyradius{\the\pgfutil@tempdima}%
		\addtosavedmacro\innerbendyradius%
		%
		\pgfutil@tempdima0.707106\pgf@x% cos(45) 
		\edef\bendxradius{\the\pgfutil@tempdima}%
		\addtosavedmacro\bendxradius%
		\advance\pgfutil@tempdima\outerxsep%
		\edef\outerbendxradius{\the\pgfutil@tempdima}%
		\addtosavedmacro\outerbendxradius%
		\advance\pgfutil@tempdima-\outerxsep%
		\advance\pgfutil@tempdima-\outerxsep%
		\edef\innerbendxradius{\the\pgfutil@tempdima}%
		\addtosavedmacro\innerbendxradius%
		%
		\edef\halfwidth{\the\pgf@x}%
		\edef\halfheight{\the\pgf@y}%
		\addtosavedmacro\halfwidth%
		\addtosavedmacro\halfheight%
		%
		\advance\pgf@x\outerxsep%
		\edef\outerhalfwidth{\the\pgf@x}%
		\addtosavedmacro\outerhalfwidth%
		%
		\pgf@xc\bendxradius%
		\pgf@yc\bendyradius%
		\pgfmathdivide@{\pgfmath@tonumber{\pgf@yc}}{\pgfmath@tonumber{\pgf@xc}}%
		\pgfmathatan{\pgfmathresult}%
		\pgf@xc\pgfmathresult pt\relax%
		\pgf@xc.5\pgf@xc%
		\edef\halfangle{\pgfmath@tonumber{\pgf@xc}}%
		\addtosavedmacro\halfangle%
		%
		\pgf@xc45pt\relax%
		\advance\pgf@xc-\halfangle pt%
		\pgfmathcot@{\pgfmath@tonumber{\pgf@xc}}%
		\let\cothalfanglein\pgfmathresult%
		\addtosavedmacro\cothalfanglein%
		%
		\pgf@xc90pt\relax%
		\advance\pgf@xc-\halfangle pt%
		\pgfmathcot@{\pgfmath@tonumber{\pgf@xc}}%
		\let\cothalfangleout\pgfmathresult%
		\addtosavedmacro\cothalfangleout%
		%
	}
	\savedanchor{\centerpoint}{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y.5\ht\pgfnodeparttextbox%
		\advance\pgf@y-.5\dp\pgfnodeparttextbox%	
	}
		\savedanchor{\midpoint}{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgfmathsetlength\pgf@y{+0.5ex}%
	}
	\savedanchor{\basepoint}{%
		\pgf@x.5\wd\pgfnodeparttextbox%
		\pgf@y0pt%
	}
	\anchor{center}{\centerpoint}%
	\anchor{mid}{\midpoint}%
	\anchor{mid east}{\tapedimensions\midpoint\advance\pgf@x\outerhalfwidth}%
	\anchor{mid west}{\tapedimensions\midpoint\advance\pgf@x-\outerhalfwidth}%
	\anchor{base}{\basepoint}%
	\anchor{base east}{\tapedimensions\basepoint\advance\pgf@x\outerhalfwidth}%
	\anchor{base west}{\tapedimensions\basepoint\advance\pgf@x-\outerhalfwidth}%
	\anchor{north}{%
		\csname pgf@anchor@tape@north east\endcsname%
		\pgf@ya\pgf@y%	
		\csname pgf@anchor@tape@north west\endcsname%
		\advance\pgf@ya\pgf@y%	
		\centerpoint%
		\pgf@y.5\pgf@ya%
	}
	\anchor{south}{%
		\csname pgf@anchor@tape@south east\endcsname%
		\pgf@ya\pgf@y%	
		\csname pgf@anchor@tape@south west\endcsname%
		\advance\pgf@ya\pgf@y%	
		\centerpoint%
		\pgf@y.5\pgf@ya%
	}
	\anchor{east}{%
		\tapedimensions%
		\centerpoint%
		\advance\pgf@x\outerhalfwidth%
	}
	\anchor{west}{%
		\tapedimensions%
		\centerpoint%
		\advance\pgf@x-\outerhalfwidth%
	}
	\anchor{north east}{%
		\tapedimensions%
		\centerpoint%
		\advance\pgf@x\outerhalfwidth%
		\advance\pgf@y\halfheight%
		\pgf@yc\outerysep%
		\ifx\topbendstyle\pgf@lib@sh@inandouttext%
			\advance\pgf@y\halfbendheight%
			\advance\pgf@y\cothalfangleout\pgf@yc%	
		\else%
			\ifx\topbendstyle\pgf@lib@sh@outandintext%	
				\advance\pgf@y\halfbendheight%
				\advance\pgf@y\cothalfanglein\pgf@yc%	
			\else%
				\advance\pgf@y\pgf@yc%
			\fi%
		\fi%		
	}%
	\anchor{north west}{%
		\tapedimensions%
		\centerpoint%
		\advance\pgf@x-\outerhalfwidth%
		\advance\pgf@y\halfheight%
		\pgf@yc\outerysep%
		\ifx\topbendstyle\pgf@lib@sh@inandouttext%
			\advance\pgf@y\halfbendheight%
			\advance\pgf@y\cothalfanglein\pgf@yc%	
		\else%
			\ifx\topbendstyle\pgf@lib@sh@outandintext%
				\advance\pgf@y\halfbendheight%
				\advance\pgf@y\cothalfangleout\pgf@yc%	
			\else%
				\advance\pgf@y\pgf@yc%
			\fi%
		\fi%			
	}%
	\anchor{south east}{%
		\tapedimensions%
		\centerpoint%
		\advance\pgf@x\outerhalfwidth%
		\advance\pgf@y-\halfheight%
		\pgf@yc\outerysep%
		\ifx\topbendstyle\pgf@lib@sh@outandintext%
			\advance\pgf@y-\halfbendheight%
			\advance\pgf@y-\cothalfangleout\pgf@yc%	
		\else%
			\ifx\topbendstyle\pgf@lib@sh@inandouttext%	
				\advance\pgf@y-\halfbendheight%
				\advance\pgf@y-\cothalfanglein\pgf@yc%	
			\else%
				\advance\pgf@y-\pgf@yc%
			\fi%
		\fi%			
	}%
	\anchor{south west}{%
		\tapedimensions%
		\centerpoint%
		\advance\pgf@x-\outerhalfwidth%
		\advance\pgf@y-\halfheight%
		\pgf@yc\outerysep%
		\ifx\topbendstyle\pgf@lib@sh@outandintext%
			\advance\pgf@y-\halfbendheight%
			\advance\pgf@y-\cothalfanglein\pgf@yc%	
		\else%
			\ifx\topbendstyle\pgf@lib@sh@inandouttext%
				\advance\pgf@y-\halfbendheight%
				\advance\pgf@y-\cothalfangleout\pgf@yc%	
			\else%
				\advance\pgf@y-\pgf@yc%
			\fi%
		\fi%			
	}%
	\backgroundpath{%
		\tapedimensions%
		%
		\pgf@xc\halfwidth%
		\pgf@yc\halfheight%		
		%
		\pgf@xc\bendxradius%
		\pgf@yc\bendyradius%		
		{%
			\pgftransformshift{\centerpoint}%
			\pgfpathmoveto{\pgfqpoint{-\halfwidth}{0pt}}%
			\pgfpathlineto{\pgfqpoint{-\halfwidth}{\halfheight}}%
			\ifx\topbendstyle\pgf@lib@sh@inandouttext%
				\pgfpathlineto{\pgf@x-\halfwidth\pgf@y\halfheight\advance\pgf@y\halfbendheight}%
				\pgfpatharc{225}{315}{\bendxradius and \bendyradius}%
				\pgfpatharc{135}{45}{\bendxradius and \bendyradius}%
			\else%
				\ifx\topbendstyle\pgf@lib@sh@outandintext%
					\pgfpathlineto{\pgf@x-\halfwidth\pgf@y\halfheight\advance\pgf@y\halfbendheight}%
					\pgfpatharc{135}{45}{\bendxradius and \bendyradius}%
					\pgfpatharc{225}{315}{\bendxradius and \bendyradius}%
				\else%
					\pgfpathlineto{\pgfqpoint{\halfwidth}{\halfheight}}%
				\fi%
			\fi%
			\pgfpathlineto{\pgfqpoint{\halfwidth}{-\halfheight}}%
			\ifx\bottombendstyle\pgf@lib@sh@inandouttext%
				\pgfpathlineto{\pgf@x\halfwidth\pgf@y-\halfheight\advance\pgf@y-\halfbendheight}%
				\pgfpatharc{45}{135}{\bendxradius and \bendyradius}%
				\pgfpatharc{315}{225}{\bendxradius and \bendyradius}%
			\else%
				\ifx\bottombendstyle\pgf@lib@sh@outandintext%
					\pgfpathlineto{\pgf@x\halfwidth\pgf@y-\halfheight\advance\pgf@y-\halfbendheight}%
					\pgfpatharc{315}{225}{\bendxradius and \bendyradius}%
					\pgfpatharc{45}{135}{\bendxradius and \bendyradius}%
				\else%
					\pgfpathlineto{\pgfqpoint{-\halfwidth}{-\halfheight}}%
				\fi%
			\fi%
			\pgfpathclose%
		}%	
	}
	\anchorborder{%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\pgfextract@process\externalpoint{%
			\centerpoint%
			\advance\pgf@x\pgf@xa%
			\advance\pgf@y\pgf@ya%
		}%
		\pgfmathanglebetweenpoints{\centerpoint}{\externalpoint}%
		\let\externalangle\pgfmathresult%
		\tapedimensions%
		%
		\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@tape@north west\endcsname}%
		\ifdim\externalangle pt<\pgfmathresult pt%
			\ifdim\externalangle pt<90pt%
				\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@tape@north east\endcsname}%
				\ifdim\externalangle pt<\pgfmathresult pt%
					\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
						{\csname pgf@anchor@tape@north east\endcsname}%
						{\csname pgf@anchor@tape@south east\endcsname}%
				\else%
					% Between north and north east.
					\ifx\topbendstyle\pgf@lib@sh@inandouttext%
						% in and out.
						\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
						{%
							\centerpoint%
							\pgf@xc\halfwidth%
							\advance\pgf@x.5\pgf@xc%
							\advance\pgf@y\halfheight%
							\advance\pgf@y\halfbendheight%
							\pgf@yc\bendyradius%
							\advance\pgf@y-.707106\pgf@yc%
						}%
						{5}{175}{\outerbendxradius and \outerbendyradius}%
					\else%
						\ifx\topbendstyle\pgf@lib@sh@outandintext%
							% out and in.
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
							{%
								\centerpoint%
								\pgf@xc\halfwidth%
								\advance\pgf@x.5\pgf@xc%
								\advance\pgf@y\halfheight%
								\advance\pgf@y\halfbendheight%
								\pgf@yc\bendyradius%
								\advance\pgf@y.707106\pgf@yc%
							}%
							{185}{355}{\innerbendxradius and \innerbendyradius}%
						\else%
							\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
								{\csname pgf@anchor@tape@north east\endcsname}%
								{\csname pgf@anchor@tape@north west\endcsname}%
						\fi%
					\fi%
				\fi%
			\else%
				% Between north and north west.
				\ifx\topbendstyle\pgf@lib@sh@inandouttext%
					% in and out.
					\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
						{%
							\centerpoint%
							\pgf@xc\halfwidth%
							\advance\pgf@x-.5\pgf@xc%
							\advance\pgf@y\halfheight%
							\advance\pgf@y\halfbendheight%
							\pgf@yc\bendyradius%
							\advance\pgf@y.707106\pgf@yc%
						}%
						{185}{355}{\innerbendxradius and \innerbendyradius}%
				\else%
					\ifx\topbendstyle\pgf@lib@sh@outandintext%
						% out and in.
						\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
						{%
							\centerpoint%
							\pgf@xc\halfwidth%
							\advance\pgf@x-.5\pgf@xc%
							\advance\pgf@y\halfheight%
							\advance\pgf@y\halfbendheight%
							\pgf@yc\bendyradius%
							\advance\pgf@y-.707106\pgf@yc%
						}%
						{5}{175}{\outerbendxradius and \outerbendyradius}%
					\else%
						\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
							{\csname pgf@anchor@tape@north east\endcsname}%
							{\csname pgf@anchor@tape@north west\endcsname}%
					\fi%
				\fi%
			\fi%
		\else%
			\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@tape@south west\endcsname}%
				\ifdim\externalangle pt>\pgfmathresult pt%
				\ifdim\externalangle pt>270pt%
					\pgfmathanglebetweenpoints{\centerpoint}{\csname pgf@anchor@tape@south east\endcsname}%
					\ifdim\externalangle pt>\pgfmathresult pt%
						\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
							{\csname pgf@anchor@tape@north east\endcsname}%
							{\csname pgf@anchor@tape@south east\endcsname}%
					\else%
						% Between south and south east.
						\ifx\bottombendstyle\pgf@lib@sh@inandouttext%
							% in and out.
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
							{%
								\centerpoint%
								\pgf@xc\halfwidth%
								\advance\pgf@x.5\pgf@xc%
								\advance\pgf@y-\halfheight%
								\advance\pgf@y-\halfbendheight%
								\pgf@yc\bendyradius%
								\advance\pgf@y-.707106\pgf@yc%
							}%
							{5}{175}{\innerbendxradius and \innerbendyradius}%
						\else%
							\ifx\bottombendstyle\pgf@lib@sh@outandintext%
								% out and in.
								\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
							{%
								\centerpoint%
								\pgf@xc\halfwidth%
								\advance\pgf@x.5\pgf@xc%
								\advance\pgf@y-\halfheight%
								\advance\pgf@y-\halfbendheight%
								\pgf@yc\bendyradius%
								\advance\pgf@y.707106\pgf@yc%
							}%
							{185}{355}{\outerbendxradius and \outerbendyradius}%
							\else%
								\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
									{\csname pgf@anchor@tape@south east\endcsname}%
									{\csname pgf@anchor@tape@south west\endcsname}%
							\fi%
						\fi%
					\fi%
				\else%
					% Between south and south west.
					\ifx\bottombendstyle\pgf@lib@sh@inandouttext%
						% in and out.
						\pgfmathpointintersectionoflineandarc{\externalpoint}{\centerpoint}%
							{%
								\centerpoint%
								\pgf@xc\halfwidth%
								\advance\pgf@x-.5\pgf@xc%
								\advance\pgf@y-\halfheight%
								\advance\pgf@y-\halfbendheight%
								\pgf@yc\bendyradius%
								\advance\pgf@y.707106\pgf@yc%
							}%
							{185}{355}{\outerbendxradius and \outerbendyradius}%
					\else%
						\ifx\bottombendstyle\pgf@lib@sh@outandintext%
							% out and in.
							\pgfmathpointintersectionoflineandarc{\centerpoint}{\externalpoint}%
							{%
								\centerpoint%
								\pgf@xc\halfwidth%
								\advance\pgf@x-.5\pgf@xc%
								\advance\pgf@y-\halfheight%
								\advance\pgf@y-\halfbendheight%
								\pgf@yc\bendyradius%
								\advance\pgf@y-.707106\pgf@yc%
							}%
							{5}{175}{\innerbendxradius and \innerbendyradius}%
						\else%
							\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
								{\csname pgf@anchor@tape@south east\endcsname}%
								{\csname pgf@anchor@tape@south west\endcsname}%
						\fi%
					\fi%
				\fi%
			\else%
				\pgfpointintersectionoflines{\externalpoint}{\centerpoint}%
					{\csname pgf@anchor@tape@north west\endcsname}%
					{\csname pgf@anchor@tape@south west\endcsname}%
			\fi%
		\fi%
	}%
}

==> pgflibrarysnakes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/libraries/pgflibrarysnakes.code.tex,v 1.24 2008/01/19 16:52:30 tantau Exp $

\PackageWarning{pgf}{Snakes have been superseded by decorations. Use
the decoration libraries instead of the snakes library}

\usepgflibrary{decorations.pathmorphing,decorations.pathreplacing,decorations.shapes}

\endinput


==> pgfmanual-en-base-actions.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Using Paths}

\subsection{Overview}

Once a path has been constructed, it can be \emph{used} in different
ways. For example, you can draw the path or fill it or use it for
clipping.

Numerous graph parameters influence how a path will be rendered. For
example, when you draw a path, the line width is important as well as
the dashing pattern. The options that govern how paths are rendered
can all be set with commands starting with |\pgfset|. \emph{All
  options that influence how a path is rendered always influence the
  complete path.} Thus, it is not possible to draw part of a path
using, say, a red color and drawing another part using a green
color. To achieve such an effect, you must use two paths.

In detail, paths can be used in the following ways:

\begin{enumerate}
\item
  You can \emph{stroke} (also known as \emph{draw}) a path.
\item
  You can \emph{fill} a path with a uniform color.
\item
  You can \emph{clip} subsequent renderings against the path.
\item
  You can \emph{shade} a path.
\item
  You can \emph{use the path as bounding box} for the whole picture.
\end{enumerate}
You can also perform any combination of the above, though it makes no
sense to fill and shade a path at the same time.

To perform (a combination of) the first three actions, you can use the
following command:
\begin{command}{\pgfusepath\marg{actions}}
  Applies the given \meta{actions} to the current path. Afterwards,
  the current path is (globally) empty. The following actions are
  possible:
  \begin{itemize}
  \item \declare{|fill|}
    fills the path. See Section~\ref{section-fill} for further details.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{1cm}}
  \pgfpathlineto{\pgfpoint{1cm}{0cm}}
  \pgfusepath{fill}
\end{pgfpicture}
\end{codeexample}
  \item \declare{|stroke|}
    strokes the path. See Section~\ref{section-stroke} for further details.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{1cm}}
  \pgfpathlineto{\pgfpoint{1cm}{0cm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
  \item \declare{|clip|}
    clips all subsequent drawings against the path. See
    Section~\ref{section-clip} for further details.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{1cm}}
  \pgfpathlineto{\pgfpoint{1cm}{0cm}}
  \pgfusepath{stroke,clip}
  \pgfpathcircle{\pgfpoint{1cm}{1cm}}{0.5cm}
  \pgfusepath{fill}
\end{pgfpicture}
\end{codeexample}
  \item \declare{|discard|}
    discards the path, that is, it is not used at all. Giving this
    option (alone) has the same effect as giving an empty options
    list.
  \end{itemize}
  When more than one of the first three actions are given, they are
  applied in the above ordering, regardless of their ordering in
  \meta{actions}. Thus, |{stroke,fill}| and |{fill,stroke}| have the
  same effect. 
\end{command}

To shade a path, use the |\pgfshadepath| command, which is explained
in Section~\ref{section-shadings}.



\subsection{Stroking a Path}
\label{section-stroke}

When you use |\pgfusepath{stroke}| to stroke a path, several graphic
parameters influence how the path is drawn. The commands for setting
these parameters are explained in the following.

Note that all graphic parameters apply to the path as a whole, never
only to a part of it.

All graphic parameters are local to the current |{pgfscope}|, but they
persists past \TeX\ groups, \emph{except} for the interior rule
(even-odd or nonzero) and the arrow tip kinds. The latter graphic
parameters only persist till the end of the current \TeX\ group, but 
this may change in the future, so do not count on this.

\subsubsection{Graphic Parameter: Line Width}

\begin{command}{\pgfsetlinewidth\marg{line width}}
  This command sets the line width for subsequent strokes (in the
  current |pgfscope|). The line width is given as a normal \TeX\
  dimension like |0.4pt| or |1mm|.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetlinewidth{1mm}
  \pgfpathmoveto{\pgfpoint{0mm}{0mm}}
  \pgfpathlineto{\pgfpoint{2cm}{0mm}}
  \pgfusepath{stroke}
  \pgfsetlinewidth{2\pgflinewidth} % double in size
  \pgfpathmoveto{\pgfpoint{0mm}{5mm}}
  \pgfpathlineto{\pgfpoint{2cm}{5mm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{textoken}{\pgflinewidth}
  You can access the current line width via the \TeX\ dimension
  |\pgflinewidth|. It will be set to the correct line width, that is,
  even when a \TeX\ group closed, the value will be correct since it
  is set globally, but when a |{pgfscope}| closes, the value is set to
  the correct value it had before the scope.
\end{textoken}


\subsubsection{Graphic Parameter: Caps and Joins}

\begin{command}{\pgfsetbuttcap}
  Sets the line cap to a butt cap. See Section~\ref{section-cap-joins}
  for an explanation of what this is.
\end{command}
\begin{command}{\pgfsetroundcap}
  Sets the line cap to a round cap. See again
  Section~\ref{section-cap-joins}.
\end{command}
\begin{command}{\pgfsetrectcap}
  Sets the line cap to a square cap. See again
  Section~\ref{section-cap-joins}. 
\end{command}
\begin{command}{\pgfsetroundjoin}
  Sets the line join to a round join. See again
  Section~\ref{section-cap-joins}. 
\end{command}
\begin{command}{\pgfsetbeveljoin}
  Sets the line join to a bevel join. See again
  Section~\ref{section-cap-joins}. 
\end{command}
\begin{command}{\pgfsetmiterjoin}
  Sets the line join to a miter join. See again
  Section~\ref{section-cap-joins}. 
\end{command}
\begin{command}{\pgfsetmiterlimit\marg{miter limit factor}}
  Sets the miter limit to  \meta{miter limit factor}. See again 
  Section~\ref{section-cap-joins}. 
\end{command}

\subsubsection{Graphic Parameter: Dashing}

\begin{command}{\pgfsetdash\marg{list of even length of dimensions}\marg{phase}}
  Sets the dashing of a line. The first entry in the list specifies
  the length of the first solid part of the list. The second entry
  specifies the length of the following gap. Then comes the length of
  the second solid part, following by the length of the second gap,
  and so on. The \meta{phase} specifies where the first solid part
  starts relative to the beginning of the line.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetdash{{0.5cm}{0.5cm}{0.1cm}{0.2cm}}{0cm}
  \pgfpathmoveto{\pgfpoint{0mm}{0mm}}
  \pgfpathlineto{\pgfpoint{2cm}{0mm}}
  \pgfusepath{stroke}
  \pgfsetdash{{0.5cm}{0.5cm}{0.1cm}{0.2cm}}{0.1cm}
  \pgfpathmoveto{\pgfpoint{0mm}{1mm}}
  \pgfpathlineto{\pgfpoint{2cm}{1mm}}
  \pgfusepath{stroke}
  \pgfsetdash{{0.5cm}{0.5cm}{0.1cm}{0.2cm}}{0.2cm}
  \pgfpathmoveto{\pgfpoint{0mm}{2mm}}
  \pgfpathlineto{\pgfpoint{2cm}{2mm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}

  Use |\pgfsetdash{}{0pt}| to get a solid dashing.
\end{command}

\subsubsection{Graphic Parameter: Stroke Color}

\begin{command}{\pgfsetstrokecolor\marg{color}}
  Sets the color used for stroking lines to \meta{color}, where
  \meta{color} is a \LaTeX\ color like |red| or |black!20!red|. Unlike
  the |\color| command, the effect of this command lasts till the end
  of the current |{pgfscope}| and not till the end of the current
  \TeX\ group.

  The color used for stroking may be different from the color used for
  filling. However, a |\color| command will always ``immediately
  override'' any special settings for the stroke and fill colors.

  In plain \TeX, this command will also work, but the problem of
  \emph{defining} a color arises. After all, plain \TeX\ does not
  provide \LaTeX\ colors. For this reason, \pgfname\ implements a
  minimalistic ``emulation'' of the |\definecolor|, |\colorlet|, and
  |\color| commands. Only gray-scale and rgb colors are supported. For
  most cases this turns out to be enough.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetlinewidth{1pt}
  \color{red}
  \pgfpathcircle{\pgfpoint{0cm}{0cm}}{3mm} \pgfusepath{fill,stroke}
  \pgfsetstrokecolor{black}
  \pgfpathcircle{\pgfpoint{1cm}{0cm}}{3mm} \pgfusepath{fill,stroke}
  \color{red}
  \pgfpathcircle{\pgfpoint{2cm}{0cm}}{3mm} \pgfusepath{fill,stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfsetcolor\marg{color}}
  Sets both the stroke and fill color. The difference to the normal
  |\color| command is that the effect lasts till the end of the
  current |{pgfscope}|, not only till the end of the current \TeX\
  group. 
\end{command}


\subsubsection{Graphic Parameter: Stroke Opacity}

You can set the stroke opacity using |\pgfsetstrokeopacity|. This
command is described in Section~\ref{section-transparency}.

\subsubsection{Graphic Parameter: Arrows}

After a path has been drawn, \pgfname\ can add arrow tips at the
ends. Currently, it will only add arrows correctly at the end of paths
that consist of a single open part. For other paths, like closed paths
or path consisting of multiple parts, the result is not defined.

\begin{command}{\pgfsetarrowsstart\marg{arrow kind}}
  Sets the arrow tip kind used at the start of a (possibly curved)
  path. When this option is used, the line will often be slightly
  shortened to ensure that the tip of the arrow will exactly ``touch''
  the ``real'' start of the line.

  To ``clear'' the start arrow, say |\pgfsetarrowsstart{}|.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetarrowsstart{latex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{0cm}}
  \pgfusepath{stroke}
  \pgfsetarrowsstart{to}
  \pgfpathmoveto{\pgfpoint{0cm}{2mm}}
  \pgfpathlineto{\pgfpoint{1cm}{2mm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}

  The effect of this command persists only till the end of the current
  \TeX\ scope.

  The different possible arrow kinds are explained in
  Section~\ref{section-arrows}.  
\end{command}

\begin{command}{\pgfsetarrowsend\marg{arrow kind}}
  Sets the arrow tip kind used at the end of a path.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetarrowsstart{latex}
  \pgfsetarrowsend{to}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{0cm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfsetarrows{\texttt{\char`\{}}\meta{start kind}|-|\meta{end kind}{\texttt{\char`\}}}}
  Sets the start arrow kind to \meta{start kind} and the end kind to
  \meta{end kind}.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetarrows{latex-to}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{0cm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfsetshortenstart\marg{dimension}}
  This command will shortened the start of every stroked path by the
  given dimension. This shortening is done in addition to automatic
  shortening done by a start arrow, but it can be used even if no
  start arrow is given.

  This command is useful if you wish arrows or lines to ``stop shortly
  before'' a given point.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathcircle{\pgfpointorigin}{5mm}
  \pgfusepath{stroke}
  \pgfsetarrows{latex-}
  \pgfsetshortenstart{4pt}
  \pgfpathmoveto{\pgfpoint{5mm}{0cm}} % would be on the circle
  \pgfpathlineto{\pgfpoint{2cm}{0cm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}
  
\begin{command}{\pgfsetshortenend\marg{dimension}}
  Works like |\pgfsetshortenstart|.
\end{command}



\subsection{Filling a Path}
\label{section-fill}

Filling a path means coloring every interior point of the path with
the current fill color. It is not always obvious whether a point is
``inside'' a  path when the path is self-intersecting and/or consists
or multiple parts. In this case either the nonzero winding number rule
or the even-odd crossing number rule is used to decide, which points
lie ``inside.'' These rules are explained in
Section~\ref{section-rules}. 

\subsubsection{Graphic Parameter: Interior Rule}

You can set which rule is used using the following commands:

\begin{command}{\pgfseteorule}
  Dictates that the even-odd rule is used in subsequent fillings in
  the current \emph{\TeX\ scope}. Thus, for once, the effect of this
  command does not persist past the current \TeX\ scope.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfseteorule
  \pgfpathcircle{\pgfpoint{0mm}{0cm}}{7mm}
  \pgfpathcircle{\pgfpoint{5mm}{0cm}}{7mm}
  \pgfusepath{fill}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfsetnonzerorule}
  Dictates that the nonzero winding number rule is used in subsequent
  fillings in the current \TeX\ scope. This is the default.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetnonzerorule
  \pgfpathcircle{\pgfpoint{0mm}{0cm}}{7mm}
  \pgfpathcircle{\pgfpoint{5mm}{0cm}}{7mm}
  \pgfusepath{fill}
\end{pgfpicture}
\end{codeexample}
\end{command}

\subsubsection{Graphic Parameter: Filling Color}

\begin{command}{\pgfsetfillcolor\marg{color}}
  Sets the color used for filling paths to \meta{color}. Like the
  stroke color, the effect lasts only till the next use of |\color|. 
\end{command}


\subsubsection{Graphic Parameter: Fill Opacity}

You can set the fill opacity using |\pgfsetfillopacity|. This
command is described in Section~\ref{section-transparency}.

\subsection{Clipping a Path}
\label{section-clip}

When you add the |clip| option, the current path is used for
clipping subsequent drawings. The same rule as for filling is used to
decide whether a point is inside or outside the path, that is, either
the even-odd rule or the nonzero rule.

Clipping never enlarges the clipping area. Thus, when you clip against
a certain path and then clip again against another path, you clip
against the intersection of both.

The only way to enlarge the clipping path is to end the |{pgfscope}|
in which the clipping was done. At the end of a |{pgfscope}| the
clipping path that was in force at the beginning of the scope is
reinstalled. 

\subsection{Using a Path as a Bounding Box}
\label{section-using-bb}

When you add the |use as bounding box| option, the bounding box of the
picture will be enlarged such that the path in encompassed, but any
\emph{subsequent} paths of the current \TeX\ scope will not have any
effect on the size of the bounding box. Typically, you use this
command at the very beginning of a |{pgfpicture}| environment.

\begin{codeexample}[]
Left
\begin{pgfpicture}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{2ex}{1ex}}
  \pgfusepath{use as bounding box} % draws nothing

  \pgfpathcircle{\pgfpointorigin}{2ex}
  \pgfusepath{stroke}
\end{pgfpicture}
right.
\end{codeexample}



==> pgfmanual-en-base-arrows.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Arrow Tips}
\label{section-arrows}


\subsection{Overview}

\subsubsection{When Does PGF Draw Arrow Tips?}

\pgfname\ offers an interface for placing \emph{arrow tips} at the end
of lines. The interface works as follows:

\begin{enumerate}
\item
  You (or someone else) assigns a name to a certain kind of arrow
  tips. For example, the 
  arrow tip |latex| is the arrow tip used by the standard \LaTeX\
  picture environment; the arrow tip |to| looks like the tip of the
  arrow in \TeX's |\to| command; and so on.

  This is done once at the beginning of the document.
\item
  Inside some picture, at some point you specify that in the current
  scope from now on you would like tips of, say, kind |to| to be added
  at the end and/or beginning of all paths.

  When an arrow kind has been installed and when \pgfname\ is about to
  stroke a path, the following things happen:
  \begin{enumerate}
  \item
    The beginning and/or end of the path is shortened appropriately.
  \item
    The path is stroked.
  \item
    The arrow tip is drawn at the beginning and/or end of the path,
    appropriately rotated and appropriately resized.
  \end{enumerate}
\end{enumerate}

In the above description, there are a number of ``appropriately.''
The exact details are not quite trivial and described later on.

\subsubsection{Meta-Arrow Tips}

In \pgfname, arrows are ``meta-arrows'' in the same way that fonts in
\TeX\ are ``meta-fonts.'' When a meta-arrow is resized, it is not
simply scaled, but a possibly complicated transformation is applied to
the size.

A meta-font is not one particular font at a specific size with a
specific stroke width (and with a large number of other parameters
being fixed). Rather, it is a ``blueprint'' (actually, more like a
program) for generating such a font at a particular size and
width. This allows the designer of a meta-font to make sure that, say,
the font is somewhat thicker and wider at very small sizes. To
appreciate the difference: Compare the following texts: ``Berlin'' and
``\tikz{\node [scale=2,inner sep=0pt,outer sep=0pt]{\tiny
    Berlin};}''. The first is a ``normal'' text, the second is the tiny
version scaled by a factor of two. Obviously, the first look
better. Now, compare  ``\tikz{\node [scale=.5,inner sep=0pt,outer
  sep=0pt]{Berlin};}'' and ``{\tiny Berlin}''. This time, the normal
text was scaled down, while the second text is a ``normal'' tiny
text. The second text is easier to read. 

\pgfname's meta-arrows work in a similar fashion: The shape of an
arrow tip can vary according to the line width of the arrow tip is
used. Thus, an arrow tip drawn at a line width of 5pt will typically
\emph{not} be five times as large as an arrow tip of line width
1pt. Instead, the size of the arrow will get bigger only slowly as the
line width increases.

To appreciate the difference, here are the |latex| and |to| arrows, as
drawn by \pgfname\ at four different sizes:

\medskip
\begin{tikzpicture}
  \draw[-latex,line width=0.1pt] (0pt,0ex) -- +(3,0)  node[thin,right] {line width is 0.1pt};
  \draw[-latex,line width=0.4pt] (0pt,-2em) -- +(3,0) node[thin,right] {line width is 0.4pt};
  \draw[-latex,line width=1.2pt] (0pt,-4em) -- +(3,0) node[thin,right] {line width is 1.2pt};
  \draw[-latex,line width=5pt]   (0pt,-6em) -- +(3,0) node[thin,right] {line width is 5pt};

  \draw[-to,line width=0.1pt] (6cm,0ex) -- +(3,0)  node[thin,right] {line width is 0.1pt};
  \draw[-to,line width=0.4pt] (6cm,-2em) -- +(3,0) node[thin,right] {line width is 0.4pt};
  \draw[-to,line width=1.2pt] (6cm,-4em) -- +(3,0) node[thin,right] {line width is 1.2pt};
  \draw[-to,line width=5pt]   (6cm,-6em) -- +(3,0) node[thin,right] {line width is 5pt};
\end{tikzpicture}

\medskip
Here, by comparison, is the same arrow when it is simply ``resized''
(as done by most programs):

\pgfarrowsdeclare{bad latex}{bad latex}
{
  \pgfarrowsleftextend{-1\pgflinewidth}
  \pgfarrowsrightextend{9\pgflinewidth}
}
{
  \pgfpathmoveto{\pgfpoint{9\pgflinewidth}{0pt}}
  \pgfpathcurveto
  {\pgfpoint{6.3333\pgflinewidth}{.5\pgflinewidth}}
  {\pgfpoint{2\pgflinewidth}{2\pgflinewidth}}
  {\pgfpoint{-1\pgflinewidth}{3.75\pgflinewidth}}
  \pgfpathlineto{\pgfpoint{-1\pgflinewidth}{-3.75\pgflinewidth}}
  \pgfpathcurveto
  {\pgfpoint{2\pgflinewidth}{-2\pgflinewidth}}
  {\pgfpoint{6.3333\pgflinewidth}{-.5\pgflinewidth}}
  {\pgfpoint{9\pgflinewidth}{0pt}}
  \pgfusepathqfill
}

\pgfarrowsdeclare{bad to}{bad to}
{
  \pgfarrowsleftextend{-2\pgflinewidth}
  \pgfarrowsrightextend{\pgflinewidth}
}
{
  \pgfsetlinewidth{0.8\pgflinewidth}
  \pgfsetdash{}{0pt}
  \pgfsetroundcap
  \pgfsetroundjoin
  \pgfpathmoveto{\pgfpoint{-3\pgflinewidth}{4\pgflinewidth}}
  \pgfpathcurveto
  {\pgfpoint{-2.75\pgflinewidth}{2.5\pgflinewidth}}
  {\pgfpoint{0pt}{0.25\pgflinewidth}}
  {\pgfpoint{0.75\pgflinewidth}{0pt}}
  \pgfpathcurveto
  {\pgfpoint{0pt}{-0.25\pgflinewidth}}
  {\pgfpoint{-2.75\pgflinewidth}{-2.5\pgflinewidth}}
  {\pgfpoint{-3\pgflinewidth}{-4\pgflinewidth}}
  \pgfusepathqstroke
}

\medskip
\begin{tikzpicture}
  \draw[-bad latex,line width=0.1pt] (0pt,0ex) -- +(3,0)  node[thin,right] {line width is 0.1pt};
  \draw[-bad latex,line width=0.4pt] (0pt,-2em) -- +(3,0) node[thin,right] {line width is 0.4pt};
  \draw[-bad latex,line width=1.2pt] (0pt,-4em) -- +(3,0) node[thin,right] {line width is 1.2pt};
  \draw[-bad latex,line width=5pt]   (0pt,-6em) -- +(3,0) node[thin,right] {line width is 5pt};

  \draw[-bad to,line width=0.1pt] (6cm,0ex) -- +(3,0)  node[thin,right] {line width is 0.1pt};
  \draw[-bad to,line width=0.4pt] (6cm,-2em) -- +(3,0) node[thin,right] {line width is 0.4pt};
  \draw[-bad to,line width=1.2pt] (6cm,-4em) -- +(3,0) node[thin,right] {line width is 1.2pt};
  \draw[-bad to,line width=5pt]   (6cm,-6em) -- +(3,0) node[thin,right] {line width is 5pt};
\end{tikzpicture}

\bigskip
As can be seen, simple scaling produces arrow tips that are way too
large at larger sizes and way too small at smaller sizes.



\subsection{Declaring an Arrow Tip Kind}

To declare an arrow kind ``from scratch,'' the following command is
used:

\begin{command}{\pgfarrowsdeclare\marg{start name}\marg{end
      name}\marg{extend code}\marg{arrow tip code}}
  This command declares a new arrow kind. An arrow kind has two names,
  which will typically be the same. When the arrow tip needs to be
  drawn, the \meta{arrow tip code} will be invoked, but the canvas
  transformation is setup beforehand to a rotation such that when an
  arrow tip pointing right is specified, the arrow tip that is
  actually drawn points in the direction of the line.

  \medskip
  \textbf{Naming the arrow kind.}
  The \meta{start name} is the name
  used for the arrow tip when it is at the start of a path, the \meta{end
    name} is the name used at the end of a path. For example, the
  arrow kind that looks like a parenthesis has the \meta{start
    name} |(| and the \meta{end name} |)| so that you can say
  |\pgfsetarrows{(-)}| to specify that you want parenthesis arrows and
  both ends.

  The \meta{end name} and \meta{start name} can be quite arbitrary and
  may contain spaces.

  \medskip
  \textbf{Basics of the arrow tip code.}
  Let us next have a look at the \meta{arrow tip code}. This code will
  be used to draw the arrow tip when \pgfname\ thinks this is
  necessary. The code should draw an arrow that ``points right,''
  which means that is should draw an arrow at the end of a line coming
  from the left and ending at the origin.

  As an example, suppose we wanted to declare an arrow tip consisting
  of two arcs, that is, we want the arrow tip to look more or less
  like the red part of the following picture:
\begin{codeexample}[]
\begin{tikzpicture}[line width=3pt]
  \draw (-2,0) -- (0,0);
  \draw[red,line join=round,line cap=round]
        (-10pt,10pt) arc (180:270:10pt) arc (90:180:10pt);
\end{tikzpicture}
\end{codeexample}

  We could use the following as \meta{arrow tip code} for this:
\begin{codeexample}[code only]
\pgfarrowsdeclare{arcs}{arcs}{...}
{
  \pgfsetdash{}{0pt} % do not dash
  \pgfsetroundjoin   % fix join
  \pgfsetroundcap    % fix cap
  \pgfpathmoveto{\pgfpoint{-10pt}{10pt}}
  \pgfpatharc{180}{270}{10pt}
  \pgfpatharc{90}{180}{10pt}
  \pgfusepathqstroke
}
\end{codeexample}

  Indeed, when the |...| is set appropriately (in a moment), we can
  write the following:
\pgfarrowsdeclare{arcs}{arcs}{\pgfarrowsleftextend{0pt}\pgfarrowsrightextend{0pt}}
{
  \pgfsetdash{}{0pt} % do not dash
  \pgfsetroundjoin   % fix join
  \pgfsetroundcap    % fix cap
  \pgfpathmoveto{\pgfpoint{-10pt}{10pt}}
  \pgfpatharc{180}{270}{10pt}
  \pgfpatharc{90}{180}{10pt}
  \pgfusepathqstroke
}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[-arcs,line width=3pt] (-2,0)  -- (0,0);
  \draw[arcs-arcs,line width=1pt] (-2,-1.5) -- (0,-1);
  \useasboundingbox (-2,-2) rectangle (0,0.75);
\end{tikzpicture}
\end{codeexample}

  As can be seen in the second example, the arrow tip is automatically
  rotated as needed when the arrow is drawn. This is achieved by a
  canvas rotation.

  \medskip
  \textbf{Special considerations about the arrow tip code.}
  There are several things you need to be aware of when designing
  arrow tip code:
  \begin{itemize}
  \item
    Inside the code, you may not use the |\pgfusepath|
    command. The reason is that this command internally calls arrow
    construction commands, which is something you obviously do not want
    to happen.

    Instead of |\pgfusepath|, use the quick versions. Typically, you
    will use |\pgfusepathqstroke|, |\pgfusepathqfill|, or
    |\pgfusepathqfillstroke|.
  \item
    The code will be executed only once, namely the first time the
    arrow tip needs to be drawn. The resulting low-level driver
    commands are protocoled and stored away. In all subsequent 
    uses of the arrow tip, the protocoled code is directly inserted.
  \item
    However, the code will be executed anew for each line width. Thus,
    an arrow of line width 2pt may result in a different protocol than
    the same arrow for a line width of 0.4pt.
  \item
    If you stroke the path that you construct, you should first set
    the dashing to solid and setup fixed joins and caps, as
    needed. This will ensure that the arrow tip will always look the
    same.
  \item
    When the arrow tip code is executed, it is automatically put
    inside a low-level scope, so nothing will ``leak out'' from the
    scope.
  \item
    The high-level coordinate transformation matrix will be set to the
    identity matrix when the code is executed for the first time.
  \end{itemize}

  \medskip
  \textbf{Designing meta-arrows.}
  The \meta{arrow tip code} should adjust the size of the arrow in
  accordance with the line width. For a small line width, the arrow
  tip should be small, for a large line width, it should be
  larger. However, the size of the arrow typically \emph{should not}
  grow in direct proportion to the line width. On the other hand, the
  size of the arrow head typically \emph{should} grow ``a bit'' with
  the line width. 

  For these reasons, \pgfname\ will not simply executed your arrow
  code within a scaled scope, where the scaling depends on the line
  width. Instead, your \meta{arrow tip code} is reexecuted again for
  each different line width.

  In our example, we could use the following code for the new arrow
  tip kind |arc'| (note the prime):
\begin{codeexample}[code only]
\newdimen\arrowsize    
\pgfarrowsdeclare{arcs'}{arcs'}{...}
{
  \arrowsize=0.2pt
  \advance\arrowsize by .5\pgflinewidth
  \pgfsetdash{}{0pt} % do not dash
  \pgfsetroundjoin   % fix join
  \pgfsetroundcap    % fix cap
  \pgfpathmoveto{\pgfpoint{-4\arrowsize}{4\arrowsize}}
  \pgfpatharc{180}{270}{4\arrowsize}
  \pgfpatharc{90}{180}{4\arrowsize}
  \pgfusepathqstroke
}
\end{codeexample}
\newdimen\arrowsize    
\pgfarrowsdeclare{arcs'}{arcs'}{\pgfarrowsleftextend{0pt}\pgfarrowsrightextend{0pt}}
{
  \arrowsize=0.2pt
  \advance\arrowsize by .5\pgflinewidth
  \pgfsetdash{}{0pt} % do not dash
  \pgfsetroundjoin   % fix join
  \pgfsetroundcap    % fix cap
  \pgfpathmoveto{\pgfpoint{-4\arrowsize}{4\arrowsize}}
  \pgfpatharc{180}{270}{4\arrowsize}
  \pgfusepathqstroke
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpatharc{90}{180}{4\arrowsize}
  \pgfusepathqstroke
}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[-arcs',line width=3pt] (-2,0)  -- (0,0);
  \draw[arcs'-arcs',line width=1pt] (-2,-1.5) -- (0,-1);
  \useasboundingbox (-2,-1.75) rectangle (0,0.5);
\end{tikzpicture}
\end{codeexample}
  
  However, sometimes, it can also be useful to have arrows that do not
  resize at all when the line width changes. This can be achieved by
  giving absolute size coordinates in the code, as done for |arc|. On
  the other hand, you can also have the arrow resize linearly with the
  line width by specifying all coordinates as multiples of
  |\pgflinewidth|.

  \textbf{The left and right extend.}
  Let us have another look at the exact left and right ``ends'' of our
  arrow tip. Let us draw the arrow tip |arc'| at a very large size:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (-2,-1) grid (1,1);
  \draw[line width=10pt,-arcs'] (-2,0) -- (0,0);
  \draw[line width=2pt,white] (-2,0) -- (0,0);
\end{tikzpicture}
\end{codeexample}

  As one can see, the arrow tip does not ``touch'' the origin as it
  should, but protrudes a little over the origin. One remedy to this
  undesirable effect is to change the code of the arrow tip such that
  everything is shifted half an |\arrowsize| to the left. While this
  will cause the arrow tip to touch the origin, the line itself will
  then interfere with the arrow: The arrow tip will be partly
  ``hidden'' by the line itself.

  \pgfname\ uses a different approach to solving the problem: The
  \meta{extend code} argument can be used to ``tell'' \pgfname\ how
  much the arrow protrudes over the origin. The argument is also used
  to tell \pgfname\ where the ``left'' end of the arrow is. However,
  this number is important only when the arrow is being reversed or
  composed with other arrow tips.

  Once \pgfname\ knows the right extend of an arrow kind, it can
  \emph{shorten} lines by this amount when drawing arrows.

  Here is a picture that shows what the visualizes the extends. The
  arrow tip itself is shown in red once more:

  \medskip
  \begin{tikzpicture}
    \draw[line width=1cm,-arcs',red] (-6,0) -- (0,0);
    \draw[line width=1cm,black]      (-6,0) -- (0,0);
    \draw[help lines] (-6,0) -- (2,0)     (0,-3) -- (0,3) coordinate (a);
    \draw[help lines,xshift=0.5cm]        (0,-3) -- (0,3) coordinate (b);
    \draw[help lines,xshift=-2.5cm-0.8pt] (0,-3) -- (0,3) coordinate (c);

    \coordinate (xline 1) at (0,1.5);
    \coordinate (xline 2) at (0,2.8);
    
    \draw[|->|] (xline 1 -| a) -- node[above=2pt] {right extend} (xline 1 -| b);    
    \draw[|<-|] (xline 2 -| c) -- node[above=2pt] {left extend}  (xline 2 -| a);

    \draw (0,0) -- (1,-1) node[below right] {origin};
   \end{tikzpicture}
  

  The \meta{extend code} is normal \TeX\ code that is executed
  whenever \pgfname\ wants to know how far the arrow tip will protrude
  to the right and left. The code should call the following two
  commands: \declare{|\pgfarrowsrightextend|} and
  \declare{|\pgfarrowsleftextend|}. Both arguments take one argument
  that specifies the size. Here is the final code for the |arc''| arrow
  tip: 
\begin{codeexample}[]
\pgfarrowsdeclare{arcs''}{arcs''}
{
  \arrowsize=0.2pt
  \advance\arrowsize by .5\pgflinewidth
  \pgfarrowsleftextend{-4\arrowsize-.5\pgflinewidth}
  \pgfarrowsrightextend{.5\pgflinewidth}
}
{
  \arrowsize=0.2pt
  \advance\arrowsize by .5\pgflinewidth
  \pgfsetdash{}{0pt} % do not dash
  \pgfsetroundjoin   % fix join
  \pgfsetroundcap    % fix cap
  \pgfpathmoveto{\pgfpoint{-4\arrowsize}{4\arrowsize}}
  \pgfpatharc{180}{270}{4\arrowsize}
  \pgfusepathqstroke
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpatharc{90}{180}{4\arrowsize}
  \pgfusepathqstroke
}
\begin{tikzpicture}
  \draw[help lines] (-2,-1) grid (1,1);
  \draw[line width=10pt,-arcs''] (-2,0) -- (0,0);
  \draw[line width=2pt,white] (-2,0) -- (0,0);
\end{tikzpicture}
\end{codeexample}
\end{command}

\pgfarrowsdeclare{arcs''}{arcs''}
{
  \arrowsize=0.2pt
  \advance\arrowsize by .5\pgflinewidth
  \pgfarrowsleftextend{-4\arrowsize-.5\pgflinewidth}
  \pgfarrowsrightextend{.5\pgflinewidth}
}
{
  \arrowsize=0.2pt
  \advance\arrowsize by .5\pgflinewidth
  \pgfsetdash{}{0pt} % do not dash
  \pgfsetroundjoin   % fix join
  \pgfsetroundcap    % fix cap
  \pgfpathmoveto{\pgfpoint{-4\arrowsize}{4\arrowsize}}
  \pgfpatharc{180}{270}{4\arrowsize}
  \pgfusepathqstroke
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpatharc{90}{180}{4\arrowsize}
  \pgfusepathqstroke
}


\subsection{Declaring a Derived Arrow Tip Kind}

It is possible to declare arrow kinds in terms of existing ones. For
these command to work correctly, the left and right extends must be
set correctly.

\begin{command}{\pgfarrowsdeclarealias\marg{start name}\marg{end
      name}\marg{old start name}\marg{old end name}}
  This command can be used to create an alias (another name) for an
  existing arrow kind.

\begin{codeexample}[]
\pgfarrowsdeclarealias{<}{>}{arcs''}{arcs''}%
\begin{tikzpicture}
  \pgfsetarrows{<->}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgfarrowsdeclarereversed\marg{start name}\marg{end
      name}\marg{old start name}\marg{old end name}}
  This command creates a new arrow kind that is the ``reverse'' of an
  existing arrow kind. The (automatically cerated) code of the new
  arrow kind will contain a flip of the canvas and the meanings of the
  left and right extend will be reversed. 

\begin{codeexample}[]
\pgfarrowsdeclarereversed{arcs reversed}{arcs reversed}{arcs''}{arcs''}%
\begin{tikzpicture}
  \pgfsetarrows{arcs reversed-arcs reversed}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample}
\end{command}



\begin{command}{\pgfarrowsdeclarecombine\opt{|*|}\opt{\oarg{offset}}\marg{start
      name}\marg{end name}\marg{first start name}\marg{first end
      name}\penalty0\marg{second start name}\marg{second end name}}
  This command creates a new arrow kind that combines two existing
  arrow kinds. The first arrow kind is the ``innermost'' arrow kind,
  the second arrow kind is the ``outermost.''

  The code for the combined arrow kind will install a canvas
  translation before the innermost arrow kind in drawn. This
  translation is calculated such that the right tip of the innermost
  arrow touches the right  end of the outermost arrow. The optional
  \meta{offset} can be used to increase (or decrease) the distance
  between the inner and outermost arrow.

\begin{codeexample}[]
\pgfarrowsdeclarecombine[\pgflinewidth]
  {combined}{combined}{arcs''}{arcs''}{latex}{latex}%
\begin{tikzpicture}
  \pgfsetarrows{combined-combined}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample}

  In the star variant, the end of the line is not in the outermost
  arrow, but inside the innermost arrow.

\begin{codeexample}[]
\pgfarrowsdeclarecombine*[\pgflinewidth]
  {combined'}{combined'}{arcs''}{arcs''}{latex}{latex}%
\begin{tikzpicture}
  \pgfsetarrows{combined'-combined'}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgfarrowsdeclaredouble\opt{\oarg{offset}}\marg{start
      name}\marg{end name}\marg{old start name}\marg{old end
      name}}
  This command is a shortcut for combining an arrow kind with itself.

\begin{codeexample}[]
\pgfarrowsdeclaredouble{<<}{>>}{arcs''}{arcs''}%
\begin{tikzpicture}
  \pgfsetarrows{<<->>}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample} 
\end{command}


\begin{command}{\pgfarrowsdeclaretriple\opt{\oarg{offset}}\marg{start
      name}\marg{end name}\marg{old start name}\marg{old end
      name}}
  This command is a shortcut for combining an arrow kind with itself
  and then again.

\begin{codeexample}[]
\pgfarrowsdeclaretriple{<<<}{>>>}{arcs''}{arcs''}%
\begin{tikzpicture}
  \pgfsetarrows{<<<->>>}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample} 
\end{command}





\subsection{Using an Arrow Tip Kind}

The following commands install the arrow kind that will be used when
stroking is done.

\begin{command}{\pgfsetarrowsstart\marg{start arrow kind}}
  Installs the given \meta{start arrow kind} for all subsequent
  strokes in the in the current \TeX-group. If \meta{start arrow kind}
  is empty, no arrow tips will be drawn at the start of the last
  segment of paths.
\begin{codeexample}[]
\begin{tikzpicture}
  \pgfsetarrowsstart{latex}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample} 
\end{command}

\begin{command}{\pgfsetarrowsend\marg{start arrow kind}}
  Like |\pgfsetarrowsstart|, only for the end of the arrow.
\begin{codeexample}[]
\begin{tikzpicture}
  \pgfsetarrowsend{latex}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample} 
\end{command}

\emph{Warning:} If the compatibility mode is active (which is the
default), there also exist old commands called |\pgfsetstartarrow| and 
|\pgfsetendarrow|, which are incompatible with the meta-arrow
management.


\begin{command}{\pgfsetarrows\texttt{\char`\{}\meta{start kind}|-|\meta{end kind}\texttt{\char`\}}}
  Calls |\pgfsetarrowsstart| for \meta{start kind} and
  |\pgfsetarrowsend| for \meta{end kind}.
\begin{codeexample}[]
\begin{tikzpicture}
  \pgfsetarrows{latex-to}
  \pgfsetlinewidth{1ex}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3.5cm}{2cm}}
  \pgfusepath{stroke}
  \useasboundingbox (-0.25,-0.25) rectangle (3.75,2.25);
\end{tikzpicture}
\end{codeexample} 
\end{command}


\subsection{Predefined Arrow Tip Kinds}

\label{standard-arrows}

The following arrow tip kinds are always defined:

{
\bigskip
\catcode`\|=12
\begin{tabular}{ll}
  \sarrow{stealth}{stealth} \\
  \sarrow{stealth reversed}{stealth reversed}  \\
  \sarrow{to}{to} \\
  \sarrow{to reversed}{to reversed}  \\
  \sarrow{latex}{latex} \\
  \sarrow{latex reversed}{latex reversed}  \\
  \index{*vbar@\protect\texttt{\protect\myvbar} arrow tip}%
  \index{Arrow tips!*vbar@\protect\texttt{\protect\myvbar}}
  \texttt{|-|}& yields thick  
  \begin{tikzpicture}[arrows={|-|},thick]
    \useasboundingbox (0pt,-0.5ex) rectangle (1cm,2ex);
    \draw (0,0) -- (1,0);
  \end{tikzpicture} and thin
  \begin{tikzpicture}[arrows={|-|},thin]
    \useasboundingbox (0pt,-0.5ex) rectangle (1cm,2ex);
    \draw (0,0) -- (1,0);
  \end{tikzpicture}
\end{tabular}
}

For further arrow tips, see page~\pageref{section-library-arrows}.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-decorations.tex <==
 % Copyright 2008 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Decorations}
\label{section-base-decorations}


\begin{pgfmodule}{decorations}
  The commands for creating decorations are defined in this
  module, so you need to load this module to use decorations. This
  module is automatically loaded by the different decoration
  libraries. 
\end{pgfmodule}


\subsection{Overview}

Decorations are a general way of creating graphics by ``moving along''
a path and, while doing so, either drawing something or constructing a
new path. This could be as simple as extending a path with a
``zigzagged'' line\ldots 

\begin{codeexample}[]
\tikz \draw decorate[decoration=zigzag] {(0,0) -- (3,0)};
\end{codeexample}
\ldots but could also be as complex as typesetting text along a path:
{\catcode`\|12
\begin{codeexample}[]
\tikz \path decorate [decoration={text along path,
     text={Some text along a path}}]
   { (0,2) .. controls (2,2) and (1,0) .. (3,0) };
\end{codeexample}
}

The workflow for using decorations is the following:
\begin{enumerate}
\item You define a decoration using the |\pgfdeclaredecoration|
  command. Different useful decorations are already declared in
  libraries like |decorations.shapes|.
\item You use normal path construction commands like |\pgfpathlineto|
  to construct a path. Let us call this path the
  \emph{to-be-decorated} path.
\item You place the path construction commands inside the environment
  |{pgfdecoration}|. This environment takes the name of a previously
  declared decoration as a parameter. It will then starting ``walking
  along'' the to-be-decorated path. As it does this, a special finite
  automaton called a \emph{decoration automaton} produces as its
  output new path construction commands (or even other outputs). These
  outputs replace the to-be-decorated path; indeed, after the
  to-be-decorated path has been fully walked along it is thrown away,
  only the output of the automaton persists.
\end{enumerate}

In the present section the process of how decoration automata work is
explained first. Then the command(s) for declaring decoration automata
and for using them are covered.



\subsection{Decoration Automata}

Decoration automata (and the closely related meta-decoration automata)
are a general concept for creating graphics ``along paths.'' For
straight lines, this idea was first proposed by Till Tantau in an
earlier version of \pgfname, the idea to extend this to arbitrary path
was proposed and implemented by Mark Wibrow. Further versitility is
provided by ``meta-decorations''. These are automata that decorate a
path with decorations. 

In the present subsection the different ideas underlying decoration
automata are presented.



\subsubsection{The Different Paths}

In order to prevent confusion with different types of path, such
as those that are extended, those that are decorated and those that 
are created, the following conventions will be used:

\begin{itemize}
\item 
  The \emph{preexisting} path refers to the current path in existence 
  before a decoration environment. (Possibly this path has been
  created by another decoration used earlier, but we will still call
  this path the preexisting path also in this case.)
\item
  The \emph{input} path refers to the to-be-decorated path that the
  decoration automaton moves along. The input path may consist of many
  line and curve input segments (for example, a circle or an ellipse
  consists of four curves). It is specified inside the decoration
  environment. 
\item
  The \emph{output} path refers to the path that the decoration 
  creates. Depending on the decoration, this path may or may not be
  empty (a decoration can also choose to use side-effects instead of
  producing an output path). The input path is always consumed by the
  decoration automaton, that is, it is no longer available in any way
  after the decoration automaton has finished. 
\end{itemize}

The effect of a decoration environment is the following: The input
path, which is specified inside the environment, is constructed and
stored. This process does not alter the preexisting path in any
way. Then the decoration automaton is started (as described later) and
it produces an output path (possibly empty). Whenever part of the
output path is produced, it is concatenated with the preexisting
path. After the environment, the current path will equal the original
preexisting path followed by the output path.

It is permissible that a decoration issues a |\pgfusepath|
command. As usual, this causes the current path to be
filled or stroked or some other action to be taken and the current
path is set to the empty path. As described above, when the decoration
automaton starts the current path is the preexisting path and as the
automaton progresses, the current path is constantly being extend by
the output path. This means that first time e |\pgfusepath| command is
used on a decoration, the preexisting path is part of the path this
command operates on; in subsequent calls only the part of the output
path constructed since the last |\pgfusepath| command will be used. 

You can use this mechanism to stroke or fill different part of the
output path in different colors, line widths, fills and shades; all 
within the same decoration. Alternatively, a decoration can choose to
produce no output path at all: the |text| decoration simply typesets
text along a path.


\subsubsection{Segments and States}

The most common use a decoration is to ``repeat something along a
path'' (for example, the |zigzag| decoration  
repeats \tikz\draw decorate[decoration=zigzag]
{(0,0)--(\pgfdecorationsegmentlength,0)}; along a path). However, it
not necessarily the case that only one thing be repeated: a decoration
can consist of different parts, or \emph{segments}, repeated in a
particular order. 

When you declare a decoration, you provide a description 
of how their different segments will be rendered. The description of
each segment should be given in a way as if the ``x-axis'' of the
segment is the tangent to the path at a particular point,
and that point is the origin of the segment.
Thus, for example, the segment of the |zigzag| decoration might be
defined using the following code: 
\begin{codeexample}[code only]
\pgfpathlineto{\pgfpoint{5pt}{5pt}}
\pgfpathlineto{\pgfpoint{15pt}{-5pt}}
\pgfpathlineto{\pgfpoint{20pt}{0pt}}
\end{codeexample}

\pgfname\ will ensure that an appropriate coordinate transformation
is in place when the segment is rendered such that
the segment actually points in the right direction. Also
subsequent segments will be transformed such that they are
``further along the path'' toward the end of the path.
All transformations are setup automatically.

Note that we did not use a |\pgfpathmoveto{\pgfpointorigin}| at the
beginning of the segment code. Doing so would subdivide the path into
numerous subpaths. Rather, we assume that the previous segment caused
the current point to be at the origin.

The width of a segment can (and must) be specified
explicitly. \pgfname\ will use this width to find out the start point
of the next segment and the correct rotation. The width the you
provide need not be the ``real'' width of the segment, which allows
decoration segments to overlap or to be spaced far apart. 

The |zigzag| decoration only has one segment that is repeated again and
again. However, we might also like to have \emph{different} segments
and use rules to describe which segment should be used where. For
example, we might have special segments at the start and at the end.

Decorations use a mechanism known in theoretical in computer science
as \emph{finite state automata} to describe which segment is used at a
particular point. The idea is the following: For the first segment we 
start in a special \emph{state} called the \emph{initial state}. In
this state, and also in all other state later, \pgfname\ first
computes how much space is left on the input path. That is, \pgfname\ keeps
track of the distance to the end of the input path. Attached to each state 
there is a set of rules of the following form: ``If the remaining 
distance on the input path is less than $x$, switch to state~$q$.''
\pgfname\ checks for each of these rules whether it applies and, if
so, immediately switches to state~$q$.

Only if none of the rules tell us to switch to another
state, \pgfname\ will execute the state's code. This code will
(typically) add a segment to the output path. In addition to the rules
there is also width parameter attached to each state. \pgfname\ then
translates the coordinate system by this width and reduces the
remaining distance on the input path. Then, \pgfname\ either stays in
the current state or switches to another state, depending on yet
another property attached of the state.

The whole process stops when a special state called |final| is
reached. The segment of this state is immediately added to the output
path (it is often empty, though) and the process ends.




\subsection{Declaring Decorations}

The following command is used to declare a decoration. Essentially,
this command describes the decoration automaton.


\begin{command}{\pgfdeclaredecoration\marg{name}\marg{initial
      state}\marg{states}}
  This command declares a new decoration called \meta{name}. The
  \meta{states} argument contains a description of the decoration
  automaton's states and the transitions between them. The
  \meta{initial state} is the state in which the automaton starts.

  When the automaton is later applied to an input path, it keeps track
  of a certain position on the input path. This current point
  will ``travel along the path,'' each time being moved along by a
  certain distance. This will also work if the path is not a straight
  line. That is, it is permissible that the path curves are veers at a
  sharp angle.  It is also permissible that while travelling along the
  input path the current input segment ends and a new input segment starts. In this
  case, the remaining distance on the first input segment is subtracted
  from the \meta{dimension} and then we travelled along the second
  input segment for the remaining distance. This input segment may also end
  early, in which case we travel along the next input segment, and so
  on. Note that it cannot happen that we travel past the end of the
  input path since this would have caused an immediate switch to
  the |final| state.

  Note note that the computation of the path lengths has only a low
  accuracy because of \TeX's small math capabilities. Do not
  expect high accuracy alignments when using decorations (unless the
  input path consists only of horizontal and vertical lines).

  The \meta{states} argument should consist of |\state| commands, one
  for each state of the decoration automaton. The |\state| command is
  defined only when the \meta{states} argument is executed.

  \begin{command}{\state\marg{name}\oarg{options}\marg{code}}
    This command declares a new state inside the current decoration
    automaton. The state is named \meta{name}.
    
    When the decoration automaton is in state \meta{name}, the following things
    happen:
    \begin{enumerate}
    \item
      The \meta{options} are parsed. This may lead, see below, to a 
      state switch. When this happens, the following steps are not
      executed. The \meta{options} are executed one after the other in
      the given order. If an option causes a state switch, the switch
      is immediate, even if later options might cause a different
      state switch.
    \item
      The \meta{code} is executed in a \TeX-group with the current
      transformation matrix setup in such a way that the origin is on
      the input path at the current point (the point at the distance
      travelled up to now) and the coordinate system is rotated in
      such a way that the positive $x$-axis points in the direction of
      the tangent to the input path at the current point, while the
      positive $y$-axis points to the left of this tangent.
      
      As described earlier, the \meta{code} can have two different
      effects: If it just contains path construction commands, the
      decoration will produce an output path, which is extends the
      preexisting path. Here is an example:

\begin{codeexample}[]
\pgfdeclaredecoration{example}{initial}
{
  \state{initial}[width=10pt]
  {
    \pgfpathlineto{\pgfpoint{0pt}{5pt}}
    \pgfpathlineto{\pgfpoint{5pt}{5pt}}
    \pgfpathlineto{\pgfpoint{5pt}{-5pt}}
    \pgfpathlineto{\pgfpoint{10pt}{-5pt}}
    \pgfpathlineto{\pgfpoint{10pt}{0pt}}
  }
  \state{final}
  {
    \pgfpathlineto{\pgfpointdecoratedpathlast}
  }
}
\tikz[decoration=example]
{
  \draw [decorate]     (0,0) -- (3,0);
  \draw [red,decorate] (0,0) to [out=45,in=135] (3,0);
}
\end{codeexample}

    Alternatively, the \meta{code} can also contain the
    |\pgfusepath| command. This will use the path in usual manner,
    where ``the path'' is the preexisting path plus a part of the
    output path for the first invocation and the different parts of
    the rest of the output path for the following invocation. Here is
    an example:
            
\begin{codeexample}[]
\pgfdeclaredecoration{stars}{initial}{
  \state{initial}[width=15pt]
  {
    \pgfmathparse{round(rnd*100)}
    \pgfsetfillcolor{yellow!\pgfmathresult!orange}
    \pgfsetstrokecolor{yellow!\pgfmathresult!red}
    \pgfnode{star}{center}{}{}{\pgfusepath{stroke,fill}}
  }
  \state{final}
  {
    \pgfpathmoveto{\pgfpointdecoratedpathlast}
  }
}
\tikz\path[decorate, decoration=stars, star point ratio=2, star points=5,
           inner sep=0, minimum size=rnd*10pt+2pt]            
  (0,0) .. controls (0,2)  and (3,2)  .. (3,0)
        .. controls (3,-3) and (0,0)  .. (0,-3)
        .. controls (0,-5) and (3,-5) .. (3,-3);
\end{codeexample}

    \item
      After the \meta{code} has been executed (possibly more than
      once, if the |repeat state| option is used), the state switches to
      whatever state has been specified inside the \meta{options}
      using the |next state| option. If no |next state| has been
      specified, the state stays the same.
    \end{enumerate}

    The \meta{options} are executed with the key path set to
    |/pgf/decoration automaton|. The following keys are defined:
    \begin{key}{/pgf/decoration automaton/switch if less than=\meta{dimension}| to |\meta{new state}}
      When this key is encountered, \pgfname\ checks whether the
      remaining distance to the end of the input path is less than
      \meta{dimension}. If so, an immediate state switch to \meta{new
        state} occurs.
    \end{key}
    \begin{key}{/pgf/decoration automaton/switch if input segment less than=\\\meta{dimension}| to |\meta{new state}}
      When this key is encountered, \pgfname\ checks whether the
      remaining distance to the end of the current input segment of the
      input path is less than \meta{dimension}. If so, an immediate
      state switch to \meta{new state} occurs.
    \end{key}
    \begin{key}{/pgf/decoration automaton/width=\meta{dimension}}
      First, this option causes an immediate switch to the
      state |final| if the remaining distance on the input path is
      less than \meta{dimension}. The effect is the same as if you had
      said |switch if less than=|\meta{dimension}| to final| just
      before the |width| option.

      If no switch occurs, this option tells \pgfname\ the width of
      the segment. The current point will travel along the input path
      (as described earlier)   by this distance.
    \end{key}
    \begin{key}{/pgf/decoration automaton/repeat state=\meta{repetitions} (initially 0)}
      Tells \pgfname\ how long the automaton stays ``normally'' in the
      current state. This count is reset to \meta{repetitions} each
      time one of the |switch if| keys causes a state switch. If no
      state switches occur, the \meta{code} is executed and the
      repetition counter is decreased. Then, there is once more a
      chance of a state change caused by any of the \meta{options}. If
      no repetition occurs, the \meta{code} is executed 
      once more and the counter is decreased once more. When the
      counter reaches zero, the \meta{code} is executed once more,
      but, then, a different state is entered, as specified by the
      |next state| option.

      Note, that the maximum number of times the state will be executed 
      is $\meta{repetitions}+1$.
    \end{key}
    \begin{key}{/pgf/decoration automaton/next state=\meta{new state}}
      After the \meta{code} for state has been executed for the last
      time, a state switch to \meta{new state} is performed. If this
      option is not given, the next state is the same as the current state.
    \end{key}

    \begin{key}{/pgf/decoration automaton/if input segment is closepath=\meta{options}}
      This key checks whether the current input segment is a closepath
      operation. If so, the \meta{options} get executed; otherwise
      nothing happens. You can use this option to handle a closepath
      in some special way, for instance, switching to a new state in
      which |\pgfpathclose| is executed.
    \end{key}

    \begin{key}{/pgf/decoration automaton/auto end on length=\meta{dimension}}
      This key is just included for convenience, it does nothing that
      cannot be achieved using the previous options. The effect is the
      following: If the remaingin input path's length is at most
      \meta{dimension}, the decorated path is ended with a straight
      line to the end of the input path and, possibly, it is closed,
      namely if the input path ended with a closepath
      operation. Otherwise, it is checked whether the current input
      segment is a closepath segment and whether the remaining
      distance on the current input segment is at most
      \meta{distance}. If so, the a closepath operation is used to
      close the decorated path and the automaton continues with the
      next subpath, remaining in the current state.

      In all other cases, nothing happens.
    \end{key}

    \begin{key}{/pgf/decoration automaton/auto corner on length=\meta{dimension}}
      This key has the following effect: Firstly, the \TeX-if
      |\ifpgfdecoratepathhascorners| is false, nothing
      happens. Otherwise, it is tested whether the remaining distance
      on the current input segment is at most \meta{dimension}. If so,
      a lineto operation is used to reach the end of this input
      segment and the automaton continues with the next input segment,
      but remains in the current state.

      The main idea behind this option is to avoid having decoration
      segments ``overshoot'' past a corner.
    \end{key}

    You may sometimes wish to do computations outside the
    transformational \TeX-group of the current segment,
    so that these results of these computations are available in the
    next state. For this, the following two options are useful:
    
    \begin{key}{/pgf/decoration automaton/persistent precomputation=\meta{precode}}
      If the \meta{code} of state is executed, the \meta{precode} is
      executed first and it executed outside the \TeX-group of the
      \meta{code}. Note that when the \meta{precode} is executed, the
      transformation matrix is not setup.
    \end{key}

    \begin{key}{/pgf/decoration automaton/persistent postcomputation=\meta{postcode}}
      Works like the |persistent precomputation| option, only the
      \meta{postcode} is executed after (and also outside) the
      \TeX-group of the main \meta{code}.
    \end{key}
    
    There are a number of macros and dimensions which may be useful
    inside a decoration automaton. The following macros are available:
    
    \begin{command}{\pgfdecoratedpathlength}
      The length of the input path. If the input path consists of
      several input segments, this number is the sum of the lengths of the
      input segments. 
    \end{command}
    
    \begin{command}{\pgfdecoratedinputsegmentlength}
      The length of the current input segment of the input path. ``Current
      input segment''  refers to the input segment on which the current point
      lies. 
    \end{command}
		
    \begin{command}{\pgfpointdecoratedpathlast}
      The final point of the input path.
    \end{command}
    
    \begin{command}{\pgfpointdecoratedinputsegmentlast}
      The final point of the current input segment of the input path.
    \end{command}
		
    \begin{command}{\pgfdecoratedangle}
      The angle of the tangent to the decorated path at the \emph{origin}
      of the current segment. The transformation matrix applied at 
      the beginning of a state includes a rotation equivalent to 
      this angle.
    \end{command}
		
    The following \TeX\ dimension registers are also available inside the 
    automaton:
    
    \begin{command}{\pgfdecoratedremainingdistance}
      The remaining distance on the input path.
    \end{command}
		
    \begin{command}{\pgfdecoratedcompleteddistance}
      The completed distance on the input path.
    \end{command}
    
    \begin{command}{\pgfdecoratedinputsegmentremainingdistance}
      The remaining distance on the current input segment of the input path.
    \end{command}
    
    \begin{command}{\pgfdecoratedinputsegmentcompleteddistance}
      The completed distance on the current input segment of the input path.
    \end{command}

    Further keys and macros are defined and used by the decoration
    libraries, see Section~\ref{section-library-decorations}.
    
    The following example shows how these options can be used:
\begin{codeexample}[]
\pgfdeclaredecoration{complicated example decoration}{initial}
{
  \state{initial}[width=5pt,next state=up]
  { \pgfpathlineto{\pgfpoint{5pt}{0pt}} }
  
  \state{up}[width=5pt,next state=down]
  {
    \ifdim\pgfdecoratedremainingdistance>\pgfdecoratedcompleteddistance
      % Growing
      \pgfpathlineto{\pgfpoint{0pt}{\pgfdecoratedcompleteddistance}}
      \pgfpathlineto{\pgfpoint{5pt}{\pgfdecoratedcompleteddistance}}
      \pgfpathlineto{\pgfpoint{5pt}{0pt}}
    \else
      % Shrinking
      \pgfpathlineto{\pgfpoint{0pt}{\pgfdecoratedremainingdistance}}
      \pgfpathlineto{\pgfpoint{5pt}{\pgfdecoratedremainingdistance}}
      \pgfpathlineto{\pgfpoint{5pt}{0pt}}
    \fi%      
  }
  \state{down}[width=5pt,next state=up]
  {
    \ifdim\pgfdecoratedremainingdistance>\pgfdecoratedcompleteddistance
      % Growing
      \pgfpathlineto{\pgfpoint{0pt}{-\pgfdecoratedcompleteddistance}}
      \pgfpathlineto{\pgfpoint{5pt}{-\pgfdecoratedcompleteddistance}}
      \pgfpathlineto{\pgfpoint{5pt}{0pt}}
    \else
      % Shrinking
      \pgfpathlineto{\pgfpoint{0pt}{-\pgfdecoratedremainingdistance}}
      \pgfpathlineto{\pgfpoint{5pt}{-\pgfdecoratedremainingdistance}}
      \pgfpathlineto{\pgfpoint{5pt}{0pt}}
    \fi%      
  }
  \state{final}
  {
    \pgfpathlineto{\pgfpointdecoratedpathlast}
  }
}
\begin{tikzpicture}[decoration=complicated example decoration]
  \draw decorate{ (0,0) -- (3,0)};
  \fill [red!50,rounded corners=2pt]
    decorate {(.5,-2) -- ++(2.5,-2.5)} -- (3,-5) -| (0,-2) -- cycle;
\end{tikzpicture}
\end{codeexample}
  \end{command}
\end{command}



\subsubsection{Predefined Decorations}

The three decorations |moveto|, |lineto|, and |curveto| are predefined
and ``always available.'' They are mostly useful in conjunction with
meta-decorations. They are documented in
Section~\ref{section-library-decorations} alongside the other
decorations.



\subsection{Using Decorations}

Once a decoration has been declared, it can be used. 

\begin{environment}{{pgfdecoration}\marg{decoration list}}
  The \meta{environment contents} should contain commands for creating
  an path. This path is the basis for the \emph{input paths}
  for the decorations in the \meta{decoration list}. In detail, the
  following happens: 
  \begin{enumerate}
  \item
    The preexisting unused path is saved.
  \item 
    The path commands specified in \meta{environment contents} are
    executed and this resulting path is saved. The path is then
    divided into different \emph{input paths} as follows:
    The format for each item in \marg{decoration list} is 
    \begin{quote}
      \marg{decoration}\marg{length}\opt{\marg{before code}\marg{after code}}
    \end{quote}
    The \meta{before code} and the \meta{after code} are optional. The
    input path is divided into input paths as follows: The first input
    path consists of the first lines of the path specified in the
    \meta{environment contents} until the \meta{length}  of the first
    element of the \meta{decoration list} is reached. If this length
    is reached in the middle of a line, the line is broken up at this
    exact position. Then the second input path has the \meta{length}
    of the second element in the \meta{decoration list} and consists
    of the lines making up the following \meta{length} part of the
    path in the \meta{environment contents}, and so on.

    If the lengths in the \meta{decoration list}
    do not add up to the total length of the path in the
    \meta{environment contents}, either some  decorations are dropped
    (if their lengths add up to more than the length of the
    \meta{environment contents}) or
    the input path is not fully used (if their lengths  add up to less).
  \item
    The preexisting path is reinstalled.
  \item
    The decoration automata move along the input paths, thus creating
    (and  possibly using) the output paths. These output paths extend
    (unless they are used) the current path.
  \end{enumerate}
	 
  Some important points should be noted regarding the use of this
  environment:
  
  \begin{itemize}
  \item
    If \meta{environment contents} does not begin with 
    |\pgfpathmoveto|,	he last known point on the preexisting path is 
    assumed as the starting point.
  \item
    All except the last of any sequence of consecutive move-to commands 
    in \meta{environment contents} are discarded.
  \item
    Any move-to commands at end of \meta{environment contents} are 
    ignored.
  \item
    Any close-path commands on the input path are interpreted as 
    straight lines.
    Internally somthing a little more complicated is going on,
    however, a closed path on the input path has no effect on the 
    output path, other than causing the automaton to travel in a 
    straight line towards the location of the last move-to command on 
    the input path.
  \item
    Although tangent computations for the input path work with the
    last point on the preexisting path, no automatic move-to
    operations are issued for the output path. 
    If an output path commences with a line-to or curve-to when the 
    existing path is empty, an appropriate move-to command should be 
    inserted before the decoration commences.
  \item
    If a decoration uses its own path, the first time this happens the
    preexisting path is part of the path that is used at this point.
  \end{itemize}

  When the decoration automata ``work on'' their respective input
  paths, before the automaton starts, \meta{before code} is
  executed. After the decoration automaton has finished, \meta{after
    code} is executed. 
        
\begin{codeexample}[]
\begin{tikzpicture}[decoration={segment length=5pt}]
  \draw [help lines] grid (3,2);
  \begin{pgfdecoration}{{curveto}{1cm},{zigzag}{2cm},{curveto}{1cm}}
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathcurveto
      {\pgfpoint{0cm}{2cm}}{\pgfpoint{3cm}{2cm}}{\pgfpoint{3cm}{0cm}}
  \end{pgfdecoration}
\pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}

  When the lengths are evaluated, the dimension
  |\pgfdecoratedremainingdistance| holds the remaining distance on
  the entire decorated path, and |\pgfdecoratedpathlength| holds the
  total length of the path. Thus, it is possible to specify lengths
  like |\pgfdecoratedpathlength/3|.

\begin{codeexample}[]
\begin{tikzpicture}[decoration={segment length=5pt}]
  \draw [help lines] grid (3,2);
  \begin{pgfdecoration}{
      {curveto}{\pgfdecoratedpathlength/3},
      {zigzag}{\pgfdecoratedpathlength/3},
      {curveto}{\pgfdecoratedremainingdistance}
    }
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathcurveto
      {\pgfpoint{0cm}{2cm}}{\pgfpoint{3cm}{2cm}}{\pgfpoint{3cm}{0cm}}
  \end{pgfdecoration}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}

  When \meta{before code} is executed, the following macro is useful:
  \begin{command}{\pgfpointdecoratedpathfirst}
    Returns the point corresponding to the start of the current
    input path.
  \end{command}
  When \meta{after code} is executed, the following macro can be used:
  \begin{command}{\pgfpointdecoratedpathlast}
    Returns the point corresponding to the end of the current input
    path.
  \end{command}
  This means that if decorations do not use their own path, it is 
  possible to do something with them and and continue from the
  correct place. 
	
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \begin{pgfdecoration}{
      {curveto}{\pgfdecoratedpathlength/3}
      {}
      {
        \pgfusepath{stroke}
      },
      {zigzag}{\pgfdecoratedpathlength/3}
      {
        \pgfpathmoveto{\pgfpointdecoratedpathfirst}
        \pgfdecorationsegmentlength=5pt
      }
      {
        \pgfsetstrokecolor{red}
        \pgfusepath{stroke}
        \pgfpathmoveto{\pgfpointdecoratedpathlast}
        \pgfsetstrokecolor{black}
      },
      {curveto}{\pgfdecoratedremainingdistance}
    }
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathcurveto
      {\pgfpoint{0cm}{2cm}}{\pgfpoint{3cm}{2cm}}{\pgfpoint{3cm}{0cm}}
  \end{pgfdecoration}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
	
  After the |{decoration}| environment has finished, the following 
  macros are available:
	
  \begin{command}{\pgfdecorateexistingpath}
    The preexisting path before the environment was entered.
  \end{command}
	
  \begin{command}{\pgfdecoratedpath}
    The (total) input path (that is, the path created by the environment contents).
  \end{command}
	
  \begin{command}{\pgfdecorationpath}
    The output path. If the path is used, this macro contains only the
    last unused part of the output path.
  \end{command}
	
  \begin{command}{\pgfpointdecoratedpathlast}
    The final point of the input path.
  \end{command}
  
  \begin{command}{\pgfpointdecorationpathlast}
    The final point of the output path.
  \end{command}

  The following style is executed each time a decoration is used. You
  may use it to setup default options for decorations.
  \begin{stylekey}{/pgf/every decoration (initially \normalfont empty)}
    This sytle is executed for every decoration.
  \end{stylekey}
\end{environment}

\begin{plainenvironment}{{pgfdecoration}\marg{name}}
  The plain-\TeX{} version of the |{pgfdecorate}| environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgfdecoration}\marg{name}}
  The Con\TeX t version of the |{pgfdecoration}| environment.
\end{contextenvironment}

For convenience, the following macros provide a ``shorthand''
for decorations (internally, they all use the |{pgfdecoration}|
environment).

\begin{command}{\pgfdecoratepath\marg{name}\marg{path commands}}
  Decorate the path described by \meta{path commands} with the
  decoration \meta{name}. This is equivalent to
\begin{codeexample}[code only]
\pgfdecorate{{name}{\pgfdecoratedpathlength}
             {\pgfdecoratebeforecode}{\pgfdecorateaftercode}}
  // the path commands.
\endpgfdecorate    
\end{codeexample}
\end{command}

\begin{command}{\pgfdecoratecurrentpath\marg{name}}
  Decorate the preexisting path with the decoration \meta{name}.
\end{command}

Both the above commands use the current definitons of the following
macros:

\begin{command}{\pgfdecoratebeforecode}
  Code executed as \meta{before code}, see the description of
  |\pgfdecorate|. 
\end{command}

\begin{command}{\pgfdecorateaftercode}
  Code executed as \meta{after code}, see the description of
  |\pgfdecorate|. 
\end{command}

It may sometimes be useful to add an additional transformation
for each segment of a decoration. The following command allows 
you to define such a ``last minute transformation.''

\begin{command}{\pgfsetdecorationsegmenttransformation\marg{code}}
  The \meta{code} will be executed at the very beginning of each
  segment. Note when applying multiple decorations, this will
  be reset between decorations, so it needs to be specified for
  each segment.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \begin{pgfdecoration}{
      {curveto}{\pgfdecoratedpathlength/3},
      {zigzag}{\pgfdecoratedpathlength/3}
      {
        \pgfdecorationsegmentlength=5pt
        \pgfsetdecorationsegmenttransformation{\pgftransformyshift{.5cm}}
      },
      {curveto}{\pgfdecoratedremainingdistance}
    }
    \pgfpathmoveto{\pgfpointorigin}
    \pgfpathcurveto
      {\pgfpoint{0cm}{2cm}}{\pgfpoint{3cm}{2cm}}{\pgfpoint{3cm}{0cm}}
  \end{pgfdecoration}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}




\subsection{Meta-Decorations}

\label{section-base-meta-decorations}

A meta-decoration provides an alternative way to decorate a path with 
mutiple decorations. It is, in essence, an automaton that decorates
an input path with decoration automatons. In general, however, the end
effect is still that a path is decorated with other paths, and the input 
path should be thought of as being divided into sub-input-paths, each with 
their own decoration. Like ordinary decorations, before a
meta-decoration can be used it must be declared.

\subsubsection{Declaring Meta-Decorations}

\begin{command}{\pgfdeclaremetadecorate\marg{name}\marg{initial state}\marg{states}}

  This command declares a new meta-decoration called \meta{name}. The
  \meta{states} argument contains a description of the meta-decoration
  automaton's states and the transitions between them. The
  \meta{initial state} is the state in which the automaton starts.
  
  The |\state| command is similar to the one found in 
  decoration declarations, and takes the same form:
  
  \begin{command}{\state\marg{name}\oarg{options}\marg{code}}
    Declares the state \meta{name} inside the current meta-decoration
    automaton. Unlike decorations, states in meta-decorations are not
    executed within a group, which makes the persistent computation
    options superfluous. Consider using an initial state with
    |width=0pt| to do precalculations that could speed the execution
    of the meta-decoration. 
    
    The \meta{options} are executed with the key path set to
    |/pgf/meta-decorations automaton/|, and the following keys are defined for 
    this path: 
    
    \begin{key}{/pgf/meta-decoration automaton/switch if less than=\meta{dimension}| to |\meta{new state}}
      This causes \pgfname\ to check whether the
      remaining distance to the end of the input path is less than
      \meta{dimension}, and, if so, to immediately switch to the state 
      \meta{new state}. When this key is evaluated, the macro 
      |\pgfmetadecoratedpathlength| will be defined as the total length of 
      the decoration path, allowing for values such as
      |\pgfmetadecoratedpathlength/8|.
    \end{key}
    
    \begin{key}{/pgf/meta-decoration automaton/width=\meta{dimension}}
      As always, this option will cause an immediate switch to the
      state |final| if the remaining distance on the input path is less than
      \meta{dimension}. 

      Otherwise, this option tells \pgfname\ the width of the
      ``meta-segment'', that is, the length of the sub-input-path
      which the decoration automaton specified  in \meta{code} will decorate.
    \end{key}
    
    \begin{key}{/pgf/meta-decoration automaton/next state=\meta{new state}}
      After the code for a state has been executed, a state switch to
      \meta{new state} is performed. If this option is not given, the
      next state is the same as the current state.
    \end{key}
    
    The code in \meta{code} is quite different from the code in a 
    decoration state. In almost all cases only the following three
    macros will be required: 
    
    \begin{command}{\decoration\marg{name}}
      This sets the decoration for the current state to \meta{name}.
      If this command is omitted, the |moveto| decoration will be
      used.
    \end{command}
    
    \begin{command}{\beforedecoration\marg{before code}}
      Defines \marg{before code} as (typically) \pgfname{} commands to be
      executed before the decoration is applied to the current segment.
      This command can be omitted.
      If you wish to set up some decoration specific parameters 
      such as segment length, or segment amplitude, then they
      can be set in \meta{before code}.
    \end{command}
   
    \begin{command}{\afterdecoration\marg{after code}}
      Defines \marg{after code} as commands to be executed afer the 
      decoration has been applied to the current segment.
      This command can be omitted.
    \end{command}
    
    There are some macros that may be usedful when creating 
    meta-decorations (note that they are all macros):
    
    \begin{command}{\pgfpointmetadecoratedpathfirst}
      When the \meta{before code} is executed,
      this macro stores the first point on the current
      sub-input-path. 
    \end{command}

    \begin{command}{\pgfpointmetadecoratedpathlast}
      When the \meta{after code} is executed,
      this macro stores the last point on the current
      sub-input-path. 
    \end{command}
    
    \begin{command}{\pgfmetadecoratedpathlength}
      The entire length of the entire input path.
    \end{command}    
    
    \begin{command}{\pgfmetadecoratedcompleteddistance}
      The completed distance on the entire input path.
    \end{command}
    
    \begin{command}{\pgfmetadecoratedremainingdistance}
      The remaining distance on the entire input path.
    \end{command}
    
    \begin{command}{\pgfmetadecoratedinputsegmentcompleteddistance}
      The completed distance on the current input segment of the entire
      input path.
    \end{command}
    
    \begin{command}{\pgfmetadecoratedinputsegmentremainingdistance}
      The remaining distance on the current input segment of the entire
      input path.
    \end{command}
  \end{command}

  Here is a complete example of a meta-decoration:

\begin{codeexample}[]
\pgfdeclaremetadecoration{arrows}{initial}{
  \state{initial}[width=0pt, next state=arrow]
  {	
    \pgfmathdivide{100}{\pgfmetadecoratedpathlength}
    \let\factor\pgfmathresult
    \pgfsetlinewidth{1pt}
    \pgfset{/pgf/decoration/segment length=4pt}
  }
  \state{arrow}[
    switch if less than=\pgfmetadecorationsegmentlength to final,
    width=\pgfmetadecorationsegmentlength/3, 
    next state=zigzag]
  {
    \decoration{curveto}
    \beforedecoration
    {   
      \pgfmathparse{\pgfmetadecoratedcompleteddistance*\factor}
      \pgfsetcolor{red!\pgfmathresult!yellow}
      \pgfpathmoveto{\pgfpointmetadecoratedpathfirst}
    }	
  }
  \state{zigzag}[width=\pgfmetadecorationsegmentlength/3, next state=end arrow]
  {
  	\decoration{zigzag}
  }
  \state{end arrow}[width=\pgfmetadecorationsegmentlength/3, next state=move]
  {
    \decoration{curveto}
    \beforedecoration{\pgfpathmoveto{\pgfpointmetadecoratedpathfirst}}
    \afterdecoration
    {	
      \pgfsetarrowsend{to}
      \pgfusepath{stroke}	
    }
  }  
  \state{move}[width=\pgfmetadecorationsegmentlength/2, next state=arrow]{}
  \state{final}{}
}

\tikz\draw[decorate,decoration={arrows,meta-segment length=2cm}]
  (0,0) .. controls (0,2)   and (3,2)   .. (3,0)
        .. controls (3,-2)  and (0,-2)  .. (0,-4)
        .. controls (0,-6)  and (3,-6)  .. (3,-8)
        .. controls (3,-10) and (0,-10) .. (0,-8);
\end{codeexample}

\end{command}


\subsubsection{Predefined Meta-decorations}

There are no predefined meta-decorations loaded with \pgfname{}.


\subsubsection{Using Meta-Decorations}

Using meta-decorations is ``simpler'' than using decorations, because
you can only use one meta-decoration per path.

\begin{environment}{{pgfmetadecoration}\marg{name}}
  This environment decorates the input path described in 
  \meta{environment contents}, with the	meta-decoration \meta{name}.
\end{environment}

\begin{plainenvironment}{{pgfmetadecoration}\marg{name}}
  The plain \TeX{} version of the |{pgfmetadecoration}| environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgfmetadecoration}\marg{name}}
  The Con\TeX t version of the |{pgfmetadecoration}| environment.
\end{contextenvironment}


==> pgfmanual-en-base-design.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Design Principles}

This section describes the basic layer of \pgfname. This layer is
build on top of the system layer. Whereas the system layer just
provides the absolute minimum for drawing graphics, the basic
layer provides numerous commands that make it possible to create
sophisticated graphics easily and also quickly.

The basic layer does not provide a convenient syntax for describing
graphics, which is left to frontends like \tikzname. For this reason, the
basic layer is typically used only by ``other programs.'' For example,
the \textsc{beamer} package uses the basic layer extensively, but does
not need a convenient input syntax. Rather, speed and flexibility are
needed when \textsc{beamer} creates graphics.

The following basic design principles underlie the basic layer:
\begin{enumerate}
\item Structuring into a core and modules.
\item Consistently named \TeX\ macros for all graphics commands.
\item Path-centered description of graphics.
\item Coordinate transformation system.
\end{enumerate}



\subsection{Core and Modules}

The basic layer consists of a \emph{core package}, called |pgfcore|,
which provides the most basic commands, and several
\emph{modules} like commands for plotting (in the |plot| module).
Modules are loaded using the |\usepgfmodule| command. 

If you say |\usepackage{pgf}| or |\input pgf.tex| or
|\usemodule[pgf]|, the |plot| and |shapes| modules are preloaded (as
well as the core and the system layer).



\subsection{Communicating with the Basic Layer via Macros}

In order to ``communicate'' with the basic layer you use long
sequences of commands that start with |\pgf|. You are only allowed to
give these commands inside a |{pgfpicture}| environment. (Note that
|{tikzpicture}| opens a |{pgfpicture}| internally, so you can freely
mix \pgfname\ commands and \tikzname\ commands inside a
|{tikzpicture}|.) It is possible to ``do other things'' between the
commands. For example, you might use one command to move to a certain
point, then have a complicated computation of the next point, and then
move there. 

\begin{codeexample}[]
\newdimen\myypos
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpoint{0cm}{\myypos}}
  \pgfpathlineto{\pgfpoint{1cm}{\myypos}}
  \advance \myypos by 1cm
  \pgfpathlineto{\pgfpoint{1cm}{\myypos}}
  \pgfpathclose
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}

The following naming conventions are used in the basic layer:

\begin{enumerate}
\item
  All commands and environments start with |pgf|.
\item
  All commands that specify a point (a coordinate) start with |\pgfpoint|.
\item
  All commands that extend the current path start with |\pgfpath|.
\item
  All commands that set/change a graphics parameter start with |\pgfset|.
\item
  All commands that use a previously declared object (like a path,
  image or shading) start with |\pgfuse|.
\item
  All commands having to do with coordinate transformations start with
  |\pgftransform|. 
\item
  All commands having to do with arrow tips start with |\pgfarrows|.
\item
  All commands for ``quickly'' extending or drawing a path start with
  |\pgfpathq| or |\pgfusepathq|.
\item
  All commands having to do with matrices start with |\pgfmatrix|.
\end{enumerate}


\subsection{Path-Centered Approach}

In \pgfname\ the most important entity is the \emph{path}. All
graphics are composed of numerous paths that can be stroked,
filled, shaded, or clipped against. Paths can be closed or open, they
can self-intersect and consist of unconnected parts.

Paths are first \emph{constructed} and then \emph{used}. In order to
construct a path, you can use commands starting with |\pgfpath|. Each
time such a command is called, the current path is extended in some
way.

Once a path has been completely constructed, you can use it using the
command |\pgfusepath|. Depending on the parameters given to this
command, the path will be stroked (drawn) or filled or subsequent
drawings will be clipped against this path.




\subsection{Coordinate Versus Canvas Transformations}

\label{section-design-transformations}

\pgfname\ provides two transformation systems: \pgfname's own
\emph{coordinate} transformation matrix and \pdf's or PostScript's
\emph{canvas} transformation matrix. These two systems are quite
different. Whereas a scaling by a factor of, say, $2$ of the canvas
causes \emph{everything} to be scaled by this factor (including
the thickness of lines and text), a scaling of two in the coordinate 
system causes only the \emph{coordinates} to be scaled, but not the
line width nor text.

By default, all transformations only apply to the coordinate
transformation system. However, using the command |\pgflowlevel|
it is possible to apply a transformation to the canvas.

Coordinate transformations are often preferable over canvas
transformations. Text and lines that are transformed using canvas 
transformations suffer from differing sizes and lines whose thickness 
differs depending on whether the line is horizontal or vertical. To
appreciate the difference, consider the following two ``circles'' both
of which have been scaled in the $x$-direction by a factor of $3$ and
by a factor of $0.5$ in the $y$-direction. The left circle uses a
canvas transformation, the right uses \pgfname's coordinate
transformation (some viewers will render the left graphic incorrectly
since they do no apply the low-level transformation the way they
should):  

\begin{tikzpicture}[line width=5pt]
  \useasboundingbox (-1.75,-1) rectangle (14,1);
  
  \begin{scope}
    \pgflowlevel{\pgftransformxscale{3}}
    \pgflowlevel{\pgftransformyscale{.5}}

    \draw (0,0) circle (0.5cm);
    \draw (.55cm,0pt) node[right] {canvas};
  \end{scope}
  \begin{scope}[xshift=9cm,xscale=3,yscale=.5]
    \draw (0,0) circle (0.5cm);
    \draw (.55cm,0pt) node[right] {coordinate};
  \end{scope}
\end{tikzpicture}



==> pgfmanual-en-base-images.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Declaring and Using Images}
\label{section-images}


This section describes the commands for creating images.


\subsection{Overview}

To be quite frank, \LaTeX's |\includegraphics| is designed better than
\pgfname's image mechanism. For this reason, \emph{I recommend that you use the
  standard image inclusion mechanism of your format}. Thus, \LaTeX\
users are encouraged to use |\includegraphics| to include images.

However, there are reasons why you might need to use the image
inclusion facilities of \pgfname:
\begin{itemize}
\item
  There is no standard image inclusion mechanism in your format. For
  example, plain \TeX\ does not have one, so \pgfname's inclusion
  mechanism is ``better than nothing.''

  However, this applies only to the |pdftex| backend. For all other
  backends, \pgfname\ currently maps its commands back to the |graphicx|
  package. Thus, in plain \TeX, this does not really help. It might be
  a good idea to fix this in the future such that \pgfname\ becomes
  independent of \LaTeX, thereby providing a uniform image abstraction
  for all formats. 
\item
  You wish to use masking. This is a feature that is only supported by
  \pgfname, though I hope that someone will implement this also for
  the graphics package in \LaTeX\ in the future.
\end{itemize}

Whatever your choice, you can still use the usual image inclusion
facilities of the |graphics| package.

The general approach taken by \pgfname\ to including an image is the
following: First, |\pgfdeclareimage| declares the
image. This must be done prior to the first use of the image. Once you
have declared an image, you can insert it into the text using
|\pgfuseimage|. The advantage of this two-phase approach is that, at
least for \textsc{pdf}, the image data will only be included once in the
file. This can drastically reduce the file size if you use an image
repeatedly, for example in an overlay. However, there is also a
command called |\pgfimage| that declares and then immediately uses the
image.

To speedup the compilation, you may wish to use the following class
option:
\begin{packageoption}{draft}
  In draft mode boxes showing the image name replace the
  images. It is checked whether the image files exist, but they are
  not read. If either height or width is not given, 1cm is used
  instead. 
\end{packageoption}

\subsection{Declaring an Image}

\begin{command}{\pgfdeclareimage\oarg{options}\marg{image
      name}\marg{filename}}
  Declares an image, but does not paint anything. To draw the image,
  use |\pgfuseimage{|\meta{image name}|}|. The \meta{filename} may not
  have an extension.  For \textsc{pdf}, the extensions |.pdf|, |.jpg|,
  and |.png| will automatically tried. For PostScript, the extensions
  |.eps|, |.epsi|, and |.ps| will be tried. 

  The following options are possible:
  \begin{itemize}
  \item
    \declare{|height=|\meta{dimension}} sets the height of the
    image. If the width is not specified simultaneously, the aspect
    ratio of the image is kept.
  \item
    \declare{|width=|\meta{dimension}} sets the width of the
    image. If the height is not specified simultaneously, the aspect
    ratio of the image is kept.
  \item
    \declare{|page=|\meta{page number}} selects a given page number
    from a multipage document. Specifying this option will have the
    following effect: first, \pgfname\ tries to find a file named
    \begin{quote}
      \meta{filename}|.page|\meta{page number}|.|\meta{extension}
    \end{quote}
    If such a file is found, it will be used instead of the originally
    specified filename. If not, \pgfname\ inserts the image stored in
    \meta{filename}|.|\meta{extension} and if a recent version of
    |pdflatex| is used, only the selected page is inserted. For older
    versions of |pdflatex| and for |dvips| the complete document is
    inserted and a warning is printed.    
  \item
    \declare{|interpolate=|\meta{true or false}} selects whether the
    image should ``smoothed'' when zoomed. False by default.
  \item
    \declare{|mask=|\meta{mask name}} selects a transparency mask. The
    mask must previously be declared using |\pgfdeclaremask| (see
    below). This option only has an effect for |pdf|. Not all viewers
    support masking. 
  \end{itemize}

\begin{codeexample}[code only]
\pgfdeclareimage[interpolate=true,height=1cm]{image1}{brave-gnu-world-logo}
\pgfdeclareimage[interpolate=true,width=1cm,height=1cm]{image2}{brave-gnu-world-logo}
\pgfdeclareimage[interpolate=true,height=1cm]{image3}{brave-gnu-world-logo}
\end{codeexample}
\end{command}


\begin{command}{\pgfaliasimage\marg{new image name}\marg{existing image name}}
  The \marg{existing image name} is ``cloned'' and the \marg{new image
    name} can now be used whenever original image is used. This
  command is useful for creating aliases for alternate extensions
  and for accessing the last image inserted using |\pgfimage|.

  \example |\pgfaliasimage{image.!30!white}{image.!25!white}|
\end{command}


\subsection{Using an Image}

\begin{command}{\pgfuseimage\marg{image name}}
  Inserts a previously declared image into the \emph{normal text}. If
  you wish to use it in a |{pgfpicture}| environment, you must put a
  |\pgftext| around it.

  If the macro |\pgfalternateextension| expands to some nonempty
  \meta{alternate extension}, \pgfname\ will first try to use the image
  names \meta{image name}|.|\meta{alternate extension}. If this
  image is not defined, \pgfname\ will next check whether \meta{alternate
    extension} contains a |!| character. If so, everything up to this
  exclamation mark and including it is deleted from \meta{alternate
    extension} and the \pgfname\ again tries to use the image \meta{image
    name}|.|\meta{alternate extension}. This is repeated until
  \meta{alternate extension} no longer contains a~|!|. Then the
  original image is used.

  The |xxcolor| package sets the alternate extension to the current
  color mixin. 

\begin{codeexample}[]
\pgfdeclareimage[interpolate=true,width=1cm,height=1cm]
  {image1}{brave-gnu-world-logo}
\pgfdeclareimage[interpolate=true,width=1cm]{image2}{brave-gnu-world-logo}
\pgfdeclareimage[interpolate=true,height=1cm]{image3}{brave-gnu-world-logo}
\begin{pgfpicture}
  \pgftext[at=\pgfpoint{1cm}{5cm},left,base]{\pgfuseimage{image1}}
  \pgftext[at=\pgfpoint{1cm}{3cm},left,base]{\pgfuseimage{image2}}
  \pgftext[at=\pgfpoint{1cm}{1cm},left,base]{\pgfuseimage{image3}}

  \pgfpathrectangle{\pgfpoint{1cm}{5cm}}{\pgfpoint{1cm}{1cm}}
  \pgfpathrectangle{\pgfpoint{1cm}{3cm}}{\pgfpoint{1cm}{1cm}}
  \pgfpathrectangle{\pgfpoint{1cm}{1cm}}{\pgfpoint{1cm}{1cm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}

  The following example demonstrates the effect of using
  |\pgfuseimage| inside a color mixin environment.

\begin{codeexample}[]
\pgfdeclareimage[interpolate=true,width=1cm,height=1cm]
  {image1.!25!white}{brave-gnu-world-logo.25}
\pgfdeclareimage[interpolate=true,width=1cm]
  {image2.25!white}{brave-gnu-world-logo.25}
\pgfdeclareimage[interpolate=true,height=1cm]
  {image3.white}{brave-gnu-world-logo.25}
\begin{colormixin}{25!white}
\begin{pgfpicture}
  \pgftext[at=\pgfpoint{1cm}{5cm},left,base]{\pgfuseimage{image1}}
  \pgftext[at=\pgfpoint{1cm}{3cm},left,base]{\pgfuseimage{image2}}
  \pgftext[at=\pgfpoint{1cm}{1cm},left,base]{\pgfuseimage{image3}}

  \pgfpathrectangle{\pgfpoint{1cm}{5cm}}{\pgfpoint{1cm}{1cm}}
  \pgfpathrectangle{\pgfpoint{1cm}{3cm}}{\pgfpoint{1cm}{1cm}}
  \pgfpathrectangle{\pgfpoint{1cm}{1cm}}{\pgfpoint{1cm}{1cm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{colormixin}
\end{codeexample}
\end{command}

\begin{command}{\pgfalternateextension}
  You should redefine this command to install a different alternate
  extension.

  \example |\def\pgfalternateextension{!25!white}|
\end{command}


\begin{command}{\pgfimage\oarg{options}\marg{filename}}
  Declares the image under the name |pgflastimage| and
  immediately uses it. You can ``save'' the image for later usage by
  invoking |\pgfaliasimage| on |pgflastimage|.
  
\begin{codeexample}[]
\begin{colormixin}{25!white}
\begin{pgfpicture}
  \pgftext[at=\pgfpoint{1cm}{5cm},left,base]
    {\pgfimage[interpolate=true,width=1cm,height=1cm]{brave-gnu-world-logo}}
  \pgftext[at=\pgfpoint{1cm}{3cm},left,base]
    {\pgfimage[interpolate=true,width=1cm]{brave-gnu-world-logo}}
  \pgftext[at=\pgfpoint{1cm}{1cm},left,base]
    {\pgfimage[interpolate=true,height=1cm]{brave-gnu-world-logo}}

  \pgfpathrectangle{\pgfpoint{1cm}{5cm}}{\pgfpoint{1cm}{1cm}}
  \pgfpathrectangle{\pgfpoint{1cm}{3cm}}{\pgfpoint{1cm}{1cm}}
  \pgfpathrectangle{\pgfpoint{1cm}{1cm}}{\pgfpoint{1cm}{1cm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{colormixin}
\end{codeexample}
\end{command}



\subsection{Masking an Image}


\begin{command}{\pgfdeclaremask\oarg{options}\marg{mask  name}\marg{filename}}
  Declares a transparency mask named \meta{mask name} (called a
  \emph{soft mask} in the \textsc{pdf} specification). This mask is
  read from the file \meta{filename}. This file should contain a
  grayscale image that is as large as the actual image. A white
  pixel in the mask will correspond to ``transparent,'' a black pixel
  to ``solid,'' and gray values correspond to intermediate values. The
  mask must have a single ``color channel.'' This means that the
  mask must be a ``real'' grayscale image, not an \textsc{rgb}-image
  in which all \textsc{rgb}-triples happen to have the same
  components.

  You can only mask images the are in a ``pixel format.'' These are
  |.jpg| and |.png|.  You cannot mask |.pdf| images in this way. Also,
  again, the mask file and the image file must have the same size.

  The following options may be given:
  \begin{itemize}
  \item |matte=|\marg{color components} sets the so-called
    \emph{matte} of the actual image (strangely, this has to be
    specified together with the mask, not with the image itself). The
    matte is the color that has been used to preblend the image. For
    example, if the image has been preblended with a red background,
    then \meta{color components} should be set to |{1 0 0}|. The
    default is |{1 1 1}|, which is white in the rgb model.

    The matte is specified in terms of the parent's image color
    space. Thus, if the parent is a grayscale image, the matte has to
    be set to |{1}|.
  \end{itemize}
  \example
\begin{codeexample}[]
%% Draw a large colorful background
\pgfdeclarehorizontalshading{colorful}{5cm}{color(0cm)=(red);
color(2cm)=(green); color(4cm)=(blue); color(6cm)=(red);
color(8cm)=(green); color(10cm)=(blue); color(12cm)=(red);
color(14cm)=(green)}
\hbox{\pgfuseshading{colorful}\hskip-14cm\hskip1cm
\pgfimage[height=4cm]{brave-gnu-world-logo}\hskip1cm
\pgfimage[height=4cm]{brave-gnu-world-logo-mask}\hskip1cm
\pgfdeclaremask{mymask}{brave-gnu-world-logo-mask}
\pgfimage[mask=mymask,height=4cm,interpolate=true]{brave-gnu-world-logo}}
\end{codeexample}
\end{command}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-layers.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Layered Graphics}

\label{section-layers}

\subsection{Overview}

\pgfname\ provides a layering mechanism for composing graphics from
multiple layers. (This mechanism is not be confused with the
conceptual ``software layers'' the \pgfname\ system is composed of.)
Layers are often used in graphic programs. The idea is that you can
draw on the different layers in any order. So you might start drawing
something on the ``background'' layer, then something on the
``foreground'' layer, then something on the ``middle'' layer, and then
something on the background layer once more, and so on. At the end, no
matter in which ordering you drew on the different layers, the layers
are ``stacked on top of each other'' in a fixed ordering to produce
the final picture. Thus, anything drawn on the middle layer would come
on top of everything of the background layer.

Normally, you do not need to use different layers since you will have
little trouble ``ordering'' your graphic commands in such a way that
layers are superfluous. However, in certain situations you only
``know'' what you should draw behind something else after the
``something else'' has been drawn.

For example, suppose you wish to draw a yellow background behind your
picture. The background should be as large as the bounding box of the
picture, plus a little border. If you know the size of the bounding box
of the picture at its beginning, this is easy to accomplish. However,
in general this is not the case and you need to create a
``background'' layer in addition to the standard ``main'' layer. Then,
at the end of the picture, when the bounding box has been established,
you can add a rectangle of the appropriate size to the picture.



\subsection{Declaring Layers}

In \pgfname\ layers are referenced using names. The standard layer,
which is a bit special in certain ways, is called |main|. If nothing
else is specified, all graphic commands are added to the |main|
layer. You can declare a new layer using the following command:

\begin{command}{\pgfdeclarelayer\marg{name}}
  This command declares a layer named \meta{name} for later
  use. Mainly, this will setup some internal bookkeeping.
\end{command}

The next step toward using a layer is to tell \pgfname\ which layers
will be part of the actual picture and which will be their
ordering. Thus, it is possible to have more layers declared than are
actually used.

\begin{command}{\pgfsetlayers\marg{layer list}}
  This command, which should be used \emph{outside} a |{pgfpicture}|
  environment, tells \pgfname\ which layers will be used in
  pictures. They are stacked on top of each other in the order
  given. The layer |main| should always be part of the list. Here is
  an example:
\begin{codeexample}[code only]
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}  
\pgfsetlayers{background,main,foreground}
\end{codeexample}
\end{command}


\subsection{Using Layers}

Once the layers of your picture have been declared, you can start to
``fill'' them. As said before, all graphics commands are normally
added to the |main| layer. Using the |{pgfonlayer}| environment, you
can tell \pgfname\ that certain commands should, instead, be added to
the given layer.

\begin{environment}{{pgfonlayer}\marg{layer name}}
  The whole \meta{environment contents} is added to the layer with the
  name \meta{layer name}. This environment can be used anywhere inside
  a picture. Thus, even if it is used inside a |{pgfscope}| or a \TeX\
  group, the contents will still be added to the ``whole'' picture.
  Using this environment multiple times inside the same picture will
  cause the \meta{environment contents} to accumulate.

  \emph{Note:} You can \emph{not} add anything to the |main| layer
  using this environment. The only way to add anything to the main
  layer is to give graphic commands outside all |{pgfonlayer}|
  environments. 

\begin{codeexample}[]
\pgfdeclarelayer{background layer}
\pgfdeclarelayer{foreground layer}
\pgfsetlayers{background layer,main,foreground layer}
\begin{tikzpicture}
  % On main layer:
  \fill[blue] (0,0) circle (1cm);
  
  \begin{pgfonlayer}{background layer}
    \fill[yellow] (-1,-1) rectangle (1,1);
  \end{pgfonlayer}
  
  \begin{pgfonlayer}{foreground layer}
    \node[white] {foreground};
  \end{pgfonlayer}
  
  \begin{pgfonlayer}{background layer}
    \fill[black] (-.8,-.8) rectangle (.8,.8);
  \end{pgfonlayer}

  % On main layer again:
  \fill[blue!50] (-.5,-1) rectangle (.5,1);
\end{tikzpicture}
\end{codeexample}
\end{environment}

\begin{plainenvironment}{{pgfonlayer}\marg{layer name}}
  This is the plain \TeX\ version of the environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgfonlayer}\marg{layer name}}
  This is the Con\TeX t version of the environment.
\end{contextenvironment}






%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-matrices.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Matrices}

\label{section-base-matrices}

\begin{pgfmodule}{matrix}
  The present section documents the commands of this module.
\end{pgfmodule}

\subsection{Overview}

Matrices are a mechanism for aligning several so-called cell pictures 
horizontally and vertically. The resulting alignment is placed in a
normal node and the command for creating matrices, |\pgfmatrix|, takes
options very similar to the |\pgfnode| command.

In the following, the basic idea behind the alignment mechanism is
explained first. Then the command |\pgfmatrix| is explained. At the
end of the section additional ways of modifying the width of columns
and rows is discussed.


\subsection{Cell Pictures and Their Alignment}

A matrix consists of rows of \emph{cells}. Cells are separated using
the special command |\pgfmatrixnextcell|, rows are ended using the
command |\pgfmatrixendrow| (the command |\\| is setup to mean the same
as |\pgfmatrixendrow| by default). Each cell contains a \emph{cell
  picture}, although cell pictures are not complete pictures as they
lack layers. However, each cell picture has its own bouding box like a
normal picture does. These bounding boxes are important for the
alignment as explained in the following.

Each cell picture will have an origin somewhere in the picture (or
even outside the picture). The position of these origins is important
for the alignment: On each row the origins will be on the same
horizontal line and for each column the origins will also be on the
same vertical line. These two requirements mean that the cell pictures
may need to be shifted around so that the origins wind up on the same
lines. The top of a row is given by the top of the cell picture whose
bounding box's maximum $y$-position is largest. Similarly, the bottom
of a row is given by the bottom of the cell picture whose bounding
box's minimum $y$-position is the most negative. Similarly, the left
end of a row is given by the left end of the cell whose bounding box's
$x$-position is the most negative; and similarly for the right end of
a row.

\begin{codeexample}[]
\begin{tikzpicture}[x=3mm,y=3mm,fill=blue!50]
  \def\atorig#1{\node[black] at (0,0) {\tiny #1};}

  \pgfmatrix{rectangle}{center}{mymatrix}
    {\pgfusepath{}}{\pgfpointorigin}{}
    {
      \fill (0,-3)  rectangle (1,1);\atorig1 \pgfmatrixnextcell
      \fill (-1,0)  rectangle (1,1);\atorig2 \pgfmatrixnextcell
      \fill (-1,-2) rectangle (0,0);\atorig3 \pgfmatrixnextcell
      \fill (-1,-1) rectangle (0,3);\atorig4 \\
      \fill (-1,0)  rectangle (4,1);\atorig5 \pgfmatrixnextcell
      \fill (0,-1)  rectangle (1,1);\atorig6 \pgfmatrixnextcell
      \fill (0,0)   rectangle (1,4);\atorig7 \pgfmatrixnextcell
      \fill (-1,-1) rectangle (0,0);\atorig8 \\
    }
\end{tikzpicture}
\end{codeexample}


\subsection{The Matrix Command}

All matrices are typeset using the following command:

\begin{command}{\pgfmatrix\marg{shape}\marg{anchor}\marg{name}%
    \marg{usage}\marg{shift}\marg{pre-code}\marg{matrix cells}}

  This command creates a node that contains a matrix. The name of the
  node is \meta{name}, its shape is \meta{shape} and the node is
  anchored at \meta{anchor}.

  The \meta{matrix cell} parameter contains the cells of the
  matrix. In each cell drawing commands may be given, which create a
  so-called cell picture. For each cell picture a bounding box is
  computed and the cells are aligned according to the rules outlined
  in the previous section.

  The resulting matrix is used as the |text| box of the node. As for a
  normal node, the \meta{usage} commands are applied, so that the
  path(s) of the resulting node are stroked or filled or whatever.

  \medskip
  \textbf{Specifiying the cells and rows.\ }
  Even though this command uses |\halign| internally, there are two
  special rules for indicating cells:
  \begin{enumerate}
  \item Cells in the same row must be separated using the macro
    |\pgfmatrixnextcell| rather than |&|. Using |&| will result in an
    error message.

    However, you can make |&| an active character and have it expand
    to |\pgfmatrixnextcell|. This way, it will ``look'' as if |&| is
    used.
  \item Rows are ended using the command |\pgfmatrixendrow|, but |\\|
    is setup to mean the same by default. However, some environments
    like |{minipage}| redefine |\\|, so it is good to have
    |\pgfmatrixendrow| as a ``fallback.''
  \item Every row \emph{including the last row} must be ended using
    the command |\\| or |\pgfmatrixendrow|. 
  \end{enumerate}

  Both |\pgfmatrixnextcell| and |\pgfmatrixendrow| (and, thus, also
  |\\|) take an optional argument as explained in the
  Section~\ref{section-matrix-spacing} 

\begin{codeexample}[]
\begin{tikzpicture}
  \pgfmatrix{rectangle}{center}{mymatrix}
    {\pgfusepath{}}{\pgfpointorigin}{}
    {
      \node {a}; \pgfmatrixnextcell \node {b}; \pgfmatrixendrow
      \node {c}; \pgfmatrixnextcell \node {d}; \pgfmatrixendrow
    }
\end{tikzpicture}
\end{codeexample}

  \medskip
  \textbf{Anchoring matrices at nodes inside the matrix.\ }
  The parameter \meta{shift} is an additional negative shift for the
  node. Normally, such a shift could be given beforehand (that is, the
  shift could be preapplied to the current transformation
  matrix). However, when \meta{shift} is evaluated, you can refer to
  \emph{temporary} positions of nodes inside the matrix. In detail,
  the following happens: When the matrix has been typeset, all nodes
  in the matrix temporarily get assigned their positions in the matrix
  box. The origin of this coordinate system is at the left baseline
  end of the matrix box, which corresponds to the |text| anchor. The
  position \meta{shift} is then interpreted inside this coordinate
  system and then used for shifting. 

  This allows you to use the parameter \meta{shift} in the following
  way: If you use |text| as the \meta{anchor} and specify
  |\pgfpointanchor{inner node}{some anchor}| for the parameter
  \meta{shift}, where |inner node| is a node that 
  is created in the matrix, then the whole matrix will be shifted such
  that |inner node.some anchor| lies at the origin of the whole
  picture. 

  \medskip
  \textbf{Rotations and scaling.\ }
  The matrix node is never rotated or shifted, because the current
  coordinate transformation matrix is reset (except for the
  translational part) at the beginning of |\pgfmatrix|. This is
  intentional and will not change in the future. If you need to rotate
  the matrix, you must install an appropriate canvas transformation
  yourself.

  However, nodes and stuff inside the cell pictures can be rotated and
  scaled normally.

  \medskip
  \textbf{Callbacks.\ }
  At the beginning and at the end of each cell the special macros 
  |\pgfmatrixbegincode|, |\pgfmatrixendcode| and possibly
  |\pgfmatrixemptycode| are called. The effect is explained in
  Section~\ref{section-matrix-callbacks}. 

  \medskip
  \textbf{Executing extra code.\ }
  The parameter \meta{pre-code} is executed at the beginning of the
  outermost \TeX-group enclosing the matrix node. It is inside this
  \TeX-group, but outside the matrix itself. It can be used
  for different purposes:
  \begin{enumerate}
  \item It can be used to simplify the next cell macro. For example,
    saying |\let\&=\pgfmatrixnextcell| allows you to use |\&| instead
    of |\pgfmatrixnextcell|. You can also set the catcode of |&| to 
    active.
  \item It can be used to issue an |\aftergroup| command. This allows
    you to regain control after the |\pgfmatrix| command. (If you do
    not know the |\aftergroup| command, you are probably blessed with
    a simple and happy life.)
  \end{enumerate}
  
  \medskip
  \textbf{Special considerations concerning macro expansion.\ }
  As said before, the matrix is typeset using |\halign|
  internally. This command does a lot of strange and magic things like
  expanding the first macro of every cell in a most unusual
  manner. Here are some effects you may wish to be aware of:
  \begin{itemize}
  \item It is not necessary to actually mention |\pgfmatrixnextcell|
    or |\pgfmatrixendrow| inside the \meta{matrix cells}. It suffices
    that the  macros inside \meta{matrix cells} expand to these macros
    sooner or later.
  \item In particular, you can define clever macros that insert
    columns and rows as needed for special effects. 
  \end{itemize}
\end{command}


\subsection{Row and Column Spacing}
\label{section-matrix-spacing}

It is possible to control the space between columns and rows rather
detailedly. Two commands are important for the row spacing and two
commands for the column spacing.

\begin{command}{\pgfsetmatrixcolumnsep\marg{sep list}}
  This macro sets the default separation list for columns. The details of the
  format of this list are explained in the description of the next command.
\end{command}

\begin{command}{\pgfmatrixnextcell\opt{\oarg{additional sep list}}}
  This command has two puposes: First, it is used to separate
  cells. Second, by providing the optional argument \meta{additional
    sep list} you can modify the spacing between the columns that are
  separated by this command.

  The optional \meta{additional sep list} may only be provided when
  the |\pgfmatrixnextcell| command starts a new column. Normally, this
  will only be the case in the first row, but sometimes a later row
  has more elements than the first row. In this case, the
  |\pgfmatrixnextcell| commands that start the new columns in the
  later row may also have the optional argument. Once a column has
  been started, subsequent uses of this optional argument for the
  column have no effect.

  To determine the space between the two columns the are separated by
  |\pgfmatrixnextcell|, the following algorithm is executed:
  \begin{enumerate}
  \item Both the default separation list (as setup by
    |\pgfsetmatrixcolumnsep|) and the \meta{additional sep list} are
    processed, in this order. If the \meta{additional sep list}
    argument is missing, only the default separation list is
    processed.
  \item Both lists may contain dimensions, separated by commas, as
    well as occurences of the keywords |between origins| and
    |between borders|.
  \item All dimensions occuring in either list are added together to
    arrive at an dimension $d$.
  \item The last occurence of either of the keywords is located. If
    neither keyword is present, we proceed as if |between borders|
    were present.
  \end{enumerate}
  At the end of the algorithm, a dimension $d$ has been computed and
  one of the two \emph{modes} |between borders| and |between origins|
  has been determined. Depending on which mode has been determined,
  the following happens:
  \begin{itemize}
  \item For the |between borders| mode, an additional horizontal space
    of $d$ is added between the two columns. Note that $d$ may be
    negative.
  \item For the |between origins| mode, the spacing between the two
    columns is computed differently: Recall that the origins of the
    cell pictures in both pictures lie on two vertical lines. The
    spacing between the two columns is setup such that the horizontal
    distance between these two lines is exactly $d$.

    This mode may only be used between columns \emph{already
      introduced in the first row}. 
  \end{itemize}
  All of the above rules boil down to the following effects:
  \begin{itemize}
  \item A default spacing between columns should be setup using
    |\pgfsetmatrixcolumnsep|. For example, you might say
    |\pgfsetmatrixcolumnsep{5pt}| to have columns be spaced apart by
    |5pt|. You could say
\begin{verbatim}
\pgfsetmatrixcolumnsep{1cm,between origins}
\end{verbatim}
    to specify that horizontal space between the origins of cell
    pictures in adjacent columns should be 1cm by default --
    regardless of the actual size of the cell pictures.
  \item You can now use the optional argument of |\pgfmatrixnextcell|
    to locally overrule the spacing between two columns. By saying
    |\pgfmatrixnextcell[5pt]| you \emph{add} 5pt to the space between
    of the two columns, regadless of the mode.

    You can also (locally) change the spacing mode for these two
    columns. For example, even if the normal spacing mode is
    |between origins|, you can say
\begin{verbatim}
\pgfmatrixnextcell[5pt,between borders]
\end{verbatim}
    to locally change the mode for these columns to
    |between borders|.
  \end{itemize}

    \begin{codeexample}[]
\begin{tikzpicture}[every node/.style=draw]
  \pgfsetmatrixcolumnsep{1mm}
  \pgfmatrix{rectangle}{center}{mymatrix}
    {\pgfusepath{}}{\pgfpointorigin}{\let\&=\pgfmatrixnextcell}
  {
    \node {8}; \&[2mm] \node{1}; \&[-1mm] \node {6}; \\
    \node {3}; \&      \node{5}; \&       \node {7}; \\
    \node {4}; \&      \node{9}; \&       \node {2}; \\
  }
\end{tikzpicture}
    \end{codeexample}
    \begin{codeexample}[]
\begin{tikzpicture}[every node/.style=draw]
  \pgfsetmatrixcolumnsep{1mm}
  \pgfmatrix{rectangle}{center}{mymatrix}
    {\pgfusepath{}}{\pgfpointorigin}{\let\&=\pgfmatrixnextcell}
  {
    \node {8}; \&[2mm] \node(a){1}; \&[1cm,between origins] \node(b){6}; \\
    \node {3}; \&      \node   {5}; \&                      \node   {7}; \\
    \node {4}; \&      \node   {9}; \&                      \node   {2}; \\
  }
  \draw [<->,red,thick,every node/.style=] (a.center) -- (b.center)
        node [above,midway] {11mm};
\end{tikzpicture}
    \end{codeexample}
    \begin{codeexample}[]
\begin{tikzpicture}[every node/.style=draw]
  \pgfsetmatrixcolumnsep{1cm,between origins}
  \pgfmatrix{rectangle}{center}{mymatrix}
    {\pgfusepath{}}{\pgfpointorigin}{\let\&=\pgfmatrixnextcell}
  {
    \node (a) {8}; \& \node (b) {1}; \&[between borders] \node (c) {6}; \\
    \node     {3}; \& \node     {5}; \&                  \node     {7}; \\
    \node     {4}; \& \node     {9}; \&                  \node     {2}; \\
  }
  \begin{scope}[every node/.style=]
    \draw [<->,red,thick] (a.center) -- (b.center) node [above,midway] {10mm};
    \draw [<->,red,thick] (b.east) -- (c.west) node [above,midway]
    {10mm};
  \end{scope}
\end{tikzpicture}
    \end{codeexample}
\end{command}

The mechanism for the between-row-spacing is the same, only the
commands are called differently.


\begin{command}{\pgfsetmatrixrowsep\marg{sep list}}
  This macro sets the default separation list for rows.
\end{command}



\begin{command}{\pgfmatrixendrow\opt{\oarg{additional sep list}}}
  This command ends a line. The optional \meta{additional sep list} is
  used to determine the spacing between the row being ended and the
  next row. The modes and the computation of $d$ is done in the same
  way as for columns. For the last row the optional argument has no
  effect.

  Inside matrices (and only there) the command |\\| is setup to mean
  the same as this command.
\end{command}


\subsection{Callbacks}
\label{section-matrix-callbacks}

There are three macros that get called at the beginning and end of
cells. By redefining these macros, which are empty by default, you can
change the appearance of cells in a very general manner.

\begin{command}{\pgfmatrixemptycode}
  This macro is executed for empty cells. This means that \pgfname\
  uses some macro magic to determine whether a cell is empty (it
  immediatly ends with |\pgfmatrixemptycode| or |\pgfmatrixendrow|)
  and, if so, put this macro inside the cell.
  \begin{codeexample}[]
\begin{tikzpicture}
  \def\pgfmatrixemptycode{\node{empty};}
  \pgfmatrix{rectangle}{center}{mymatrix}
    {\pgfusepath{}}{\pgfpointorigin}{\let\&=\pgfmatrixnextcell}
  {
    \node {a}; \&           \& \node {b}; \\
               \& \node{c}; \& \node {d}; \& \\
  }
\end{tikzpicture}
  \end{codeexample}
  As can be seen, the macro is not executed for empty cells at the end
  of row when columns are added only later on.
\end{command}


\begin{command}{\pgfmatrixbegincode}
  This macro is executed at the beginning of non-empty
  cells. Correspondingly, |\pgfmatrixendcode| is added at
  the end of every non-empty cell.
  \begin{codeexample}[]
\begin{tikzpicture}
  \def\pgfmatrixbegincode{\node[draw]\bgroup}
  \def\pgfmatrixendcode{\egroup;}
  \pgfmatrix{rectangle}{center}{mymatrix}
    {\pgfusepath{}}{\pgfpointorigin}{\let\&=\pgfmatrixnextcell}
  {
    a \& b \& c \\
    d \&   \& e \\
  }
\end{tikzpicture}
  \end{codeexample}
  Note that between |\pgfmatrixbegincode| and |\pgfmatrixendcode|
  there will \emph{not} only be the contents of the cell. Rather,
  \pgfname\ will add some (invisible) commands for book-keeping
  purposes that involve |\let| and |\gdef|. In particular, it is not a
  good idea to have |\pgfmatrixbegincode| end with |\csname| and
  |\pgfmatrixendcode| start with |\endcsname|.
\end{command}

\begin{command}{\pgfmatrixendcode}
  See the explanation above.
\end{command}


The following two counters allow you to access the current row and
current column in a callback:

\begin{command}{\pgfmatrixcurrentrow}
  This counter stores the current row of the current cell of the
  matrix. Do not even think of changing this counter.  
\end{command}

\begin{command}{\pgfmatrixcurrentcolumn}
  This counter stores the current column of the current cell of the
  matrix. 
\end{command}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-nodes.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Nodes and Shapes}

\label{section-shapes}

This section describes the |shapes| module.

\begin{pgfmodule}{shapes}
  This module defines commands both for creating nodes and for
  creating shapes. The package is loaded automatically by |pgf|, but
  you can load it manually if you have  only included |pgfcore|.  
\end{pgfmodule}


\subsection{Overview}

\pgfname\ comes with a sophisticated set of commands for creating
\emph{nodes} and \emph{shapes}. A \emph{node} is a graphical object
that consists (typically) of (one or more) text labels and some
additional stroked or filled paths. Each node has a certain
\emph{shape}, which may be something simple like a |rectangle| or a
|circle|, but it may also be something complicated like a
|uml class diagram| (this shape is currently not implemented,
though). Different nodes that have the same shape may look quite
different, however, since shapes (need not) specify whether the shape
path is stroked or filled.


\subsubsection{Creating and Referencing Nodes}

You create a node by calling the macro |\pgfnode| or the more general
|\pgfmultipartnode|. These macro takes several parameters and draws
the requested shape at a certain position. In addition, it will
``remember'' the node's position within the current
|{pgfpicture}|. You can then, later on, refer to the 
node's position. Coordinate transformations are ``fully supported,''
which means that if you used coordinate transformations to shift or
rotate the shape of a node, the node's position will still be correctly
determined by \pgfname. This is \emph{not} the case if you use canvas
transformations, instead.


\subsubsection{Anchors}

An important property of a node or a shape in general are its
\emph{anchors}. Anchors are ``important'' positions in a shape. For
example, the |center| anchor lies at the center of a shape, the
|north| anchor is usually ``at the top, in the middle'' of a shape,
the |text| anchor is the lower left corner of the shape's text label
(if present), and so on.

Anchors are important both when you create a node and when you
reference it. When you create a node, you specify the node's
``position'' by asking \pgfname\ to place the shape in such a way that
a certain anchor lies at a certain point. For example, you might ask
that the node is placed such that the |north| anchor is at the
origin. This will effectively cause the node to be placed below the
origin.

When you reference a node, you always reference an anchor of the
node. For example, when you request the ``|north| anchor of the node
just placed'' you will get the origin. However, you can also request
the ``|south| anchor of this node,'' which will give you a point
somewhere below the origin. When a coordinate transformation was in
force at the time of creation of a node, all anchors are also
transformed accordingly.

\subsubsection{Layers of a Shape}

The simplest shape, the |coordinate|, has just one anchor, namely the
|center|, and a label (which is usually empty). More complicated
shapes like the |rectangle| shape also have a \emph{background
  path}. This is a \pgfname-path that is defined by the shape. The
shape does not prescribe what should happen with the path: When a node
is created this path may be stroked (resulting in a frame around the
label), filled (resulting in a background color for the text), or just
discarded.

Although most shapes consist just of a background path plus some label
text, when a shape is drawn, up to seven different layers are drawn:

\begin{enumerate}
\item
  The ``behind the background layer.'' Unlike the background path,
  which be used in different ways by different nodes, the graphic
  commands given for this layer will always stroke or
  always fill the path they construct. They might also insert some
  text that is ``behind everything.''
\item
  The background path layer. How this path is used depends on how the
  arguments of the |\pgfnode| command.
\item
  The ``before the background path layer.'' This layer works like the
  first one, only the commands of this layer are executed after the
  background path has been used (in whatever way the creator of the
  node chose).
\item
  The label layer. This layer inserts the node's text box(es).
\item
  The ``behind the foreground layer.'' This layer, like the
  first layer, once more contains graphic commands that are ``simply
  executed.''
\item
  The foreground path layer. This path is treated in the same way as the
  background path, only it is drawn only after the label text has been
  drawn.
\item
  The ``before the foreground layer.''
\end{enumerate}

Which of these layers are actually used depends on the shape.



\subsubsection{Node Parts}

A shape typically does not consist only of different background and
foreground paths, but it may also have text labels. Indeed, for many
shapes the text labels are the more important part of the shape.

Most shapes will have only one text label. In this case, this text
label is simply passed as a parameter to the |\pgfnode| command. When
the node is drawn, the text label is shifted around such that its
lower left corner is at the |text| anchor of the node.

More complicated shapes may have more than one text label. Nodes of
such shapes are called \emph{multipart nodes}. The different
\emph{node parts} are simply the different text labels. For example, a
|uml class| shape might have a |class name| part, a |method| part and
an |attributes| part. Indeed, single part nodes are a special case of
multipart nodes: They only have one part named |text|.

When a shape is declared, you must specify the node parts. There is a
simple command called |\nodeparts| that takes a list of the part names
as input. When you create a node of a multipart shape, for each part
of the node you must have setup a \TeX-box containing the text of the
part. For a part named |XYZ| you must setup the box
|\pgfnodepartXYZbox|. The box will be placed at the anchor |XYZ|. See
the description of |\pgfmultipartnode| for more details.


\subsection{Creating Nodes}

You create a node using one of the following commands:

\begin{command}{\pgfnode\marg{shape}\marg{anchor}\marg{label
      text}\marg{name}\marg{path usage command}} 
  This command creates a new node. The \meta{shape} of the node must
  have been declared previously using |\pgfdeclareshape|.

  The shape is shifted such that the \meta{anchor} is at the
  origin. In order to place the shape somewhere else, use the
  coordinate transformation prior to calling this command.

  The \meta{name} is a name for later reference. If no name is given,
  nothing will be ``saved'' for the node, it will just be drawn.

  The \meta{path usage command} is executed for the background and the
  foreground path (if the shape defines them).

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (4,3);
  {
    \pgftransformshift{\pgfpoint{1.5cm}{1cm}}
    \pgfnode{rectangle}{north}{Hello World}{hellonode}{\pgfusepath{stroke}}
  }
  {
    \color{red!20}
    \pgftransformrotate{10}
    \pgftransformshift{\pgfpoint{3cm}{1cm}}
    \pgfnode{rectangle}{center}
      {\color{black}Hello World}{hellonode}{\pgfusepath{fill}}
  }
\end{tikzpicture}
\end{codeexample}

  As can be seen, all coordinate transformations are also applied to
  the text of the shape. Sometimes, it is desirable that the
  transformations are applied to the point where the shape will be
  anchored, but you do not wish the shape itself to the
  transformed. In this case, you should call
  |\pgftransformresetnontranslations| prior to calling the |\pgfnode|
  command. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (4,3);
  {
    \color{red!20}
    \pgftransformrotate{10}
    \pgftransformshift{\pgfpoint{3cm}{1cm}}
    \pgftransformresetnontranslations
    \pgfnode{rectangle}{center}
      {\color{black}Hello World}{hellonode}{\pgfusepath{fill}}
  }
\end{tikzpicture}
\end{codeexample}

  The \meta{label text} is typeset inside the \TeX-box
  |\pgfnodeparttextbox|. This box is shown at the |text| anchor of the
  node, if the node has a |text| part. See the description of
  |\pgfmultipartnode| for details.
\end{command}

\begin{command}{\pgfmultipartnode\marg{shape}\marg{anchor}\marg{name}\marg{path
      usage command}}
  This command is the more general (and less user-friendly) version of
  the |\pgfnode| command. While the |\pgfnode| command can only be
  used for shapes that have a single part (which is the case for most
  shapes), this command can also be used with multi-part nodes.

  When this command is called, for each node part of the node you must
  have setup one \TeX-box. Suppose the shape has two parts: The |text|
  part and the |lower| part. Then, prior to calling
  |\pgfmultipartnode|, you must have setup the boxes
  |\pgfnodeparttextbox| and |\pgfnodepartlowerbox|. These boxes may 
  contain any \TeX-text. The shape code will then compute the
  positions of the shape's anchors based on the sizes of the these
  shapes. Finally, when the node is drawn, the boxes are placed at the
  anchor positions |text| and |lower|.

\begin{codeexample}[]
\setbox\pgfnodeparttextbox=\hbox{$q_1$}
\setbox\pgfnodepartlowerbox=\hbox{01}
\begin{pgfpicture}
  \pgfmultipartnode{circle split}{center}{my state}{\pgfusepath{stroke}}
\end{pgfpicture}
\end{codeexample}

  \emph{Note:\/} Be careful when using the |\setbox| command inside a
  |{pgfpicture}| command. You will have to use |\pgfinterruptpath| at
  the beginning of the box and |\endpgfinterruptpath| at the end of
  the box to make sure that the box is typeset correctly. In the above
  example this problem was sidestepped by moving the box construction
  outside the environment.

  \emph{Note:\/} It is not necessary to use |\newbox| for every node
  part name. Although you need a different box for each part of a
  single shape, two different shapes may very well use the same box
  even when the names of the parts are different. Suppose you have a
  |circle split| shape that has an |lower| part and you have a
  |uml class| shape that has a |methods| part. Then, in order to avoid
  exhausting \TeX's limited number of box registers, you can say
\begin{codeexample}[code only]
\newbox\pgfnodepartlowerbox
\let\pgfnodepartmethodsbox=\pgfnodepartlowerbox  
\end{codeexample}
  Also, when you have a node part name with spaces like |class name|,
  it may be useful to create an alias:
\begin{codeexample}[code only]
\newbox\mybox
\expandafter\let\csname pgfnodepartclass namebox\endcsname=\mybox
\end{codeexample}
\end{command}

\begin{command}{\pgfnodealias\marg{new name}\marg{existing node}}
  This command does not actually create a new node. Rather, it allows
  you to subsequently access the node \meta{existing node} using the
  name \meta{new name}.
\end{command}

There are a number of values that have an influence on the size of a
node. These values are stored in the following keys.

\begin{key}{/pgf/minimum width=\meta{dimension} (initially 1pt)}
  \keyalias{tikz}
  This key stores the \emph{recommended} minimum width of a
  shape. Thus, when a shape is drawn and when the shape's width would
  be smaller than \meta{dimension}, the shape's width is enlarged by
  adding some empty space. 

  Note that this value is just a recommendation. A shape may choose to
  ignore this key.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (-2,0) grid (2,1);

  \pgfset{minimum width=3cm}
  \pgfnode{rectangle}{center}{Hello World}{}{\pgfusepath{stroke}}
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/minimum height=\meta{dimension} (initially 1pt)}
  \keyalias{tikz}
  Works like |/pgf/minimum width|.
\end{key}

\begin{key}{/pgf/minimum size=\meta{dimension}}
  \keyalias{tikz}
  This sytle both |/pgf/minimum width| and |/pgf/minimum height| to \meta{dimension}.
\end{key}


\begin{key}{/pgf/inner xsep=\meta{dimension} (initially 0.3333em)}
  \keyalias{tikz}
  This key stores the \emph{recommended} horizontal
  inner separation between the label text and the background path. As
  before, this value is just a recommendation and a shape may choose
  to ignore this key.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (-2,0) grid (2,1);

  \pgfset{inner xsep=1cm}
  \pgfnode{rectangle}{center}{Hello World}{}{\pgfusepath{stroke}}
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/inner ysep=\meta{dimension} (initially 0.3333em)}
  \keyalias{tikz}
  Works like |/pgf/inner xsep|.
\end{key}

\begin{key}{/pgf/inner sep=\meta{dimension}}
  \keyalias{tikz}
  This style sets both |/pgf/inner xsep| and |/pgf/inner ysep| to \meta{dimension}.
\end{key}



\begin{key}{/pgf/outer xsep=\meta{dimension} (initially .5\string\pgflinewidth)}
  \keyalias{tikz}
  This key stores the recommended horizontal separation between the
  background path and the ``outer anchors.'' For example, if
  \meta{dimension} is |1cm| then the |east| anchor will be 1cm to the
  right of the right border of the background path. 
  As before, this value is just a recommendation.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (-2,0) grid (2,1);

  \pgfset{outer xsep=.5cm}
  \pgfnode{rectangle}{center}{Hello World}{x}{\pgfusepath{stroke}}

  \pgfpathcircle{\pgfpointanchor{x}{north}}{2pt}
  \pgfpathcircle{\pgfpointanchor{x}{south}}{2pt}
  \pgfpathcircle{\pgfpointanchor{x}{east}}{2pt}
  \pgfpathcircle{\pgfpointanchor{x}{west}}{2pt}
  \pgfpathcircle{\pgfpointanchor{x}{north east}}{2pt}
  \pgfusepath{fill}
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/outer ysep=\meta{dimension} (initially .5\string\pgflinewidth)}
  \keyalias{tikz}
  Works like |/pgf/outer xsep|.
\end{key}

\begin{key}{/pgf/outer sep=\meta{dimension}}
  \keyalias{tikz}
  This style sets both |/pgf/outer xsep| and |/pgf/outer ysep| to \meta{dimension}.
\end{key}



\subsection{Using Anchors}

Each shape defines a set of anchors. We saw already that the anchors
are used when the shape is drawn: the shape is placed in such a way
that the given anchor is at the origin (which in turn is typically
translated somewhere else).

One has to look up the set of anchors of each shape, there is no
``default'' set of anchors, except for the |center| anchor, which
should always be present. Also, most shapes will declare anchors like
|north| or |east|, but this is not guaranteed.


\subsubsection{Referencing Anchors of Nodes in the Same Picture}

Once a node has been defined, you can refer to its anchors using the
following commands:

\begin{command}{\pgfpointanchor\marg{node}\marg{anchor}}
  This command is another ``point command'' like the commands
  described in Section~\ref{section-points}. It returns the coordinate
  of the given \meta{anchor} in the given \meta{node}. The command can
  be used in commands like |\pgfpathmoveto|.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgftransformrotate{30}
  \pgfnode{rectangle}{center}{Hello World!}{x}{\pgfusepath{stroke}}

  \pgfpathcircle{\pgfpointanchor{x}{north}}{2pt}
  \pgfpathcircle{\pgfpointanchor{x}{south}}{2pt}
  \pgfpathcircle{\pgfpointanchor{x}{east}}{2pt}
  \pgfpathcircle{\pgfpointanchor{x}{west}}{2pt}
  \pgfpathcircle{\pgfpointanchor{x}{north east}}{2pt}
  \pgfusepath{fill}
\end{pgfpicture}
\end{codeexample}

  In the above example, you may have noticed something curious: The
  rotation transformation is still in force when the anchors are
  invoked, but it does not seem to have an effect. You might expect
  that the rotation should apply to the already rotated points once
  more.

  However, |\pgfpointanchor| returns a point that takes the current
  transformation matrix into account: \emph{The inverse transformation
    to the current coordinate transformation is applied to an anchor
    point before returning it.}

  This behavior may seem a bit strange, but you will find it very
  natural in most cases. If you really want to apply a transformation
  to an anchor point (for example, to ``shift it away'' a little bit),
  you have to invoke |\pgfpointanchor| without any transformations in
  force. Here is an example:

\makeatletter
\begin{codeexample}[]
\begin{pgfpicture}
  \pgftransformrotate{30}
  \pgfnode{rectangle}{center}{Hello World!}{x}{\pgfusepath{stroke}}

  {
    \pgftransformreset
    \pgfpointanchor{x}{east}
    \xdef\mycoordinate{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}
  }
    
  \pgfpathcircle{\mycoordinate}{2pt}
  \pgfusepath{fill}
\end{pgfpicture}
\end{codeexample}

  A special situation arises when the \meta{node} lies in a picture
  different from the current picture. In this case, if you have not
  told \pgfname\ that the picture should be ``remembered,'' the
  \meta{node} will be treated as if it lied in the current
  picture. For example, if the \meta{node} was at position $(3,2)$ in
  the original picture, it is treated as if it lied at position
  $(3,2)$ in the current picture. However, if you have told \pgfname\
  to remember the picture position of the node's picture and also of
  the current picture,
  then |\pgfpointanchor| will return a coordinate that corresponds to
  the position of the node's anchor on the page, transformed into the
  current coordinate system. For examples and more details see
  Section~\ref{section-cross-pictures-pgf}. 
\end{command}

\begin{command}{\pgfpointshapeborder\marg{node}\marg{point}}
  This command returns the point on the border of the shape that lies
  on a straight line from the center of the node to \meta{point}. For
  complex shapes it is not guaranteed that this point will actually
  lie on the border, it may be on the border of a ``simplified''
  version of the shape.

\begin{codeexample}[]
\begin{pgfpicture}
  \begin{pgfscope}
    \pgftransformrotate{30}
    \pgfnode{rectangle}{center}{Hello World!}{x}{\pgfusepath{stroke}}
  \end{pgfscope}
  \pgfpathcircle{\pgfpointshapeborder{x}{\pgfpoint{2cm}{1cm}}}{2pt}
  \pgfpathcircle{\pgfpoint{2cm}{1cm}}{2pt}
  \pgfpathcircle{\pgfpointshapeborder{x}{\pgfpoint{-1cm}{1cm}}}{2pt}
  \pgfpathcircle{\pgfpoint{-1cm}{1cm}}{2pt}
  \pgfusepath{fill}
\end{pgfpicture}
\end{codeexample}
\end{command}


\subsubsection{Referencing Anchors of Nodes in Different Pictures}
\label{section-cross-pictures-pgf}

As a picture is typeset, \pgfname\ keeps track of the positions of all
nodes inside the picture. What \pgfname\ does not remember is the
position of the picture \emph{itself} on the page. Thus, if you define
a node in one picture and then try to reference this node while
another picture is typeset, \pgfname\ will only know the position of
the nodes that you try to typeset inside the original picture, but it
will not know where this picture lies. What is missing is the relative
positioning of the two pictures.

To overcome this problem, you need to tell \pgfname\ that it should
remember the position of pictures on a page. If these positions are
remembered, then \pgfname\ can compute the offset between the pictures
and make nodes in different pictures accessible.

Determining the positions of pictures on the page is, alas,
not-so-easy. Because of this, \pgfname\ does not do so
automatically. Rather, you have to proceed as follows:
\begin{enumerate}
\item You have to use a backend driver that supports position
  tracking. pdf\TeX\ is one such drivers, |dvips| currently is not.
\item You have to say |\pgfrememberpicturepositiononpagetrue|
  somewhere before or inside every picture
  \begin{itemize}
  \item in which you wish to reference a node and
  \item from which you wish to reference a node in another picture.
  \end{itemize}
  The second item is important since \pgfname\ does not only need to
  know the position of the picture in which the node you wish to
  reference lies, but it also needs to know where the current picture
  lies.
\item You typically have to run \TeX\ twice (depending on the backend
  driver) since the position information typically gets written into
  an external file on the first run and is available only on the
  second run.
\item You have to switch off automatic bounding bound
  computations. The reason is that the node in the other picture
  should not influence the size of the bouding box of the current
  picture. You should say |\pgfusepath{use as bounding box}| before
  using a coordinate in another picture.
\end{enumerate}



\subsection{Special Nodes}

There are several special nodes that are always defined and which you
should not attempt to redefine.

\begin{predefinednode}{current bounding box}
  This node is of shape |rectangle|. Unlike normal nodes, its size
  changes constantly and always reflects the size of the bounding box
  of the current picture. This means that, for instance, that
\begin{codeexample}[code only]
\pgfpointanchor{current bounding box}{south east}
\end{codeexample}
  returns the lower left corner of the bounding box of the current
  picture. 
\end{predefinednode}

\begin{predefinednode}{current path bounding box}
  This node is also of shape |rectangle|. Its size is the size of the
  bounding box of the current path.
\end{predefinednode}

\begin{predefinednode}{current page}
  This node is inside a virtual remembered picture. The size of this
  node is the size of the current page. This means that if you create
  a remembered picture and inside this picture you reference an anchor
  of this node, you reference an absolute position on the page. To
  demonstrate the effect, the following code puts some text in the
  lower left corner of the current page. Note that this works only if
  the backend driver supports it, otherwise the text is inserted right
  here.%
{%
\pgfrememberpicturepositiononpagetrue%
\begin{pgfpicture}
  \pgfusepath{use as bounding box}
  \pgftransformshift{\pgfpointanchor{current page}{south west}}
  \pgftransformshift{\pgfpoint{1cm}{1cm}}
  \pgftext[left,base]{
    \textcolor{red}{
      Text absolutely positioned in
      the lower left corner.}
  }
\end{pgfpicture}
}%
\begin{codeexample}[code only]
\pgfrememberpicturepositiononpagetrue
\begin{pgfpicture}
  \pgfusepath{use as bounding box}
  \pgftransformshift{\pgfpointanchor{current page}{south west}}
  \pgftransformshift{\pgfpoint{1cm}{1cm}}
  \pgftext[left,base]{
    \textcolor{red}{
      Text absolutely positioned in
      the lower left corner.}
  }
\end{pgfpicture}  
\end{codeexample}
\end{predefinednode}


There is also an option that allows you to create new special nodes
quite similar to the above:
\begin{key}{/pgf/local bounding box=\meta{node name}}
  \keyalias{tikz}
  This defines a new node \meta{node name} whose size is the bouding
  box around all objects in the current scope starting at the position
  where this option was given. After the end of the scope, the \meta{node
    name} is still available. You can use this option to keep track of
  the size of a certain area. Note that excessive use of this option
  (keeping track of dozens of bounding boxes at the same time)
  will slow things down.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);
  { [local bounding box=outer box]
    \draw (1,1) circle (.5) [local bounding box=inner box] (2,2) circle (.5);
  }
  \draw      (outer box.south west) rectangle (outer box.north east);
  \draw[red] (inner box.south west) rectangle (inner box.north east);
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsection{Declaring New Shapes}

There are only three predefined shapes, see
Section~\ref{section-predefined-shapes}, so there must be some way of
defining new shapes. Defining a shape is, unfortunately, a
not-quite-trivial process. The reason is that shapes need to be both
very flexible (their size will vary greatly according to
circumstances) and they need to be constructed reasonably ``fast.''
\pgfname\ must be able to handle pictures with several hundreds of
nodes and documents with thousands of nodes in total. It would not do
if \pgfname\ had to compute and store, say, dozens of anchor positions
for every node. 


\subsubsection{What Must Be Defined For a Shape?}

In order to define a new shape, you must provide:
\begin{itemize}
\item
  a \emph{shape name},
\item
  code for computing the  \emph{saved anchors} and \emph{saved
    dimensions}, 
\item
  code for computing \emph{anchor} positions in terms of the saved anchors,
\item
  optionally code for the \emph{background path} and \emph{foreground path},
\item
  optionally code for \emph{things to be drawn before or behind} the
  background and foreground paths.
\item
  optionally a list of node parts.
\end{itemize}


\subsubsection{Normal Anchors Versus Saved Anchors}

Anchors  are special places in shape. For example, the |north east|
anchor, which is a normal anchor, lies at the upper right corner of
the  |rectangle| shape, as does |\northeast|, which is a saved
anchor. The difference is the following: \emph{saved anchors are 
  computed and stored for each node, anchors are only computed as
  needed.} The user only has access to the normal anchors, but a
normal anchor can just ``copy'' or ``pass through'' the location of a
saved anchor. 

The idea behind all this is that a shape can declare a very large
number of normal anchors, but when a node of this shape is created,
these anchors are not actually computed. However, this causes a
problem: When we wish to reference an anchor of a node at some later
time, we must still able to compute the position of the anchor. For 
this, we may need a lot of information: What was the transformation
matrix that was in force when the node was created? What was the size
of the text box? What were the values of the different separation
dimensions? And so on. 

To solve this problem, \pgfname\ will always compute the locations of
all \emph{saved anchors} and store these positions. Then, when an
normal anchor position is requested later on, the anchor position can
be given just from knowing where the locations of the saved anchors.

As an example, consider the |rectangle| shape. For this shape two
anchors are saved: The |\northeast| corner and the |\southwest|
corner. A normal anchor like |north west| can now easily be expressed
in terms of these coordinates: Take the $x$-position of the
|\southwest| point  and the $y$-position of the |\northeast| point. 
The |rectangle| shape currently defines 13 normal anchors, but needs
only two saved anchors. Adding new anchors like a  |south south east|
anchor would not increase the memory and computation requirements of
pictures. 

All anchors (both saved and normal) are specified in a local
\emph{shape coordinate space}. This is also true for the background
and foreground paths. The |\pgfnode| macro will automatically apply
appropriate transformations to the coordinates so that the shape is
shifted to the right anchor or otherwise transformed. 


\subsubsection{Command for Declaring New Shapes}

The following command declares a new shape:
\begin{command}{\pgfdeclareshape\marg{shape name}\marg{shape
      specification}}
  This command declares a new shape named \meta{shape name}. The shape
  name can later be used in commands like |\pgfnode|.

  The \meta{shape specification} is some \TeX\ code containing calls
  to special commands that are only defined inside the \meta{shape
    specification} (similarly to commands like |\draw| that are only
  available inside the |{tikzpicture}| environment).

  \example Here is the code of the |coordinate| shape:
\begin{codeexample}[code only]
\pgfdeclareshape{coordinate}
{
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by -.5\dp\pgfnodeparttextbox%
  }
  \anchor{center}{\centerpoint}
  \anchorborder{\centerpoint}
}
\end{codeexample}

  The special commands are explained next. In the examples given for
  the special commands a new shape will be constructed, which we might
  call |simple rectangle|. It should behave like the normal rectangle
  shape, only without bothering about the fine details like inner and
  outer separations. The skeleton for the shape is the following.
\begin{codeexample}[code only]
\pgfdeclareshape{simple rectangle}{
  ...
}
\end{codeexample}

  \begin{command}{\nodeparts\marg{list of node parts}}
    This command declares which parts make up nodes of this shape. A
    \emph{node part} is a (possibly empty) text label that is drawn
    when a node of the shape is created.

    By default, a shape has just one node part called |text|. However,
    there can be several node parts. For example, the
    |circle split| shape has two parts: the |text| part, which
    shows that upper text, and a |lower| part, which shows the
    lower text. For the |circle split| shape the |\nodeparts| command
    was called with the argument |{text,lower}|.

    When a multipart node is created, the text labels are drawn in the
    sequences listed in the \meta{list of node parts}. For each node
    part there you must have declared one anchor and the \TeX-box of
    the part is placed at this anchor. For a node part called |XYZ|
    the \TeX-box |\pgfnodepartXYZbox| is placed at anchor |XYZ|.
  \end{command}

  \begin{command}{\savedanchor\marg{command}\marg{code}}
    This command declares a saved anchor. The argument \meta{command}
    should be a \TeX\ macro name like |\centerpoint|.

    The \meta{code} will be executed each time |\pgfnode| (or
    |\pgfmultipartnode|) is called to  create a node of the shape
    \meta{shape name}. When the \meta{code} 
    is executed, the \TeX-boxes of the node parts will contain the
    text labels of the node. Possibly, these box are void. For
    example, if there is just a |text| part, the node
    |\pgfnodeparttextbox| will be setup when the \meta{code} is
    executed. 

    The \meta{code} can use the width, height, and depth of the
    box(es) to compute the location of the saved anchor. In addition,
    the \meta{code} can take into account the values of dimensions like
    |\pgfshapeminwidth| or |\pgfshapeinnerxsep|. Furthermore, the
    \meta{code} can take into consideration the values of any further
    shape-specific variables that are set at the moment when
    |\pgfnode| is called.

    The net effect of the \meta{code} should be to set the two \TeX\
    dimensions |\pgf@x| and |\pgf@y|. One way to achieve this is to
    say |\pgfpoint{|\meta{x value}|}{|\meta{y value}|}| at the end of
    the \meta{code}, but you can also just set these variables.
    The values that |\pgf@x| and |\pgf@y| have after the code has been
    executed, let us call them $x$ and $y$, will be recorded and
    stored together with the node that is created by the command
    |\pgfnode|.

    The macro \meta{command} is defined to be
    |\pgfpoint{|$x$|}{|$y$|}|. However, the \meta{command} is only
    locally defined while anchor positions are being computed. Thus,
    it is possible to use very simple names for \meta{command}, like
    |\center| or |\a|, without causing a name-clash. (To be precise,
    very simple \meta{command} names will clash with existing names,
    but only locally inside the computation of anchor positions; and
    we do not need the normal |\center| command during these
    computations.)

    For our |simple rectangle| shape, we will need only one saved
    anchor: The upper right corner. The lower left corner could either
    be the origin or the ``mirrored'' upper right corner, depending on
    whether we want the text label to have its lower left corner at
    the origin or whether the text label should be centered on the
    origin. Either will be fine, for the final shape this will make no
    difference since the shape will be shifted anyway. So, let us
    assume that the text label is centered on the origin (this will be
    specified later on using the |text| anchor). We get 
    the following code for the upper right corner:
\begin{codeexample}[code only]
\savedanchor{\upperrightcorner}{
  \pgf@y=.5\ht\pgfnodeparttextbox % height of the box, ignoring the depth
  \pgf@x=.5\wd\pgfnodeparttextbox % width of the box
}
\end{codeexample}

    If we wanted to take, say, the |\pgfshapeminwidth| into account,
    we could use the following code:
    
\begin{codeexample}[code only]
\savedanchor{\upperrightcorner}{
  \pgf@y=.\ht\pgfnodeparttextbox % height of the box
  \pgf@x=.\wd\pgfnodeparttextbox % width of the box
  \setlength{\pgf@xa}{\pgfshapeminwidth}
  \ifdim\pgf@x<.5\pgf@xa
    \pgf@x=.5\pgf@xa
  \fi
}
\end{codeexample}
    Note that we could not have written |.5\pgfshapeminwidth| since
    the minium width is stored in a ``plain text macro,'' not as a
    real dimension. So if |\pgfshapeminwidth| depth were 
    2cm, writing |.5\pgfshapeminwidth| would yield the same as |.52cm|.

    In the ``real'' |rectangle| shape the code is somewhat more
    complex, but you get the basic idea.
  \end{command}  
  \begin{command}{\saveddimen\marg{command}\marg{code}}
    This command is similar to |\savedanchor|, only instead of setting
    \meta{command} to |\pgfpoint{|$x$|}{|$y$|}|, the \meta{command} is
    set just to (the value of) $x$.

    In the |simple rectangle| shape we might use a saved dimension to
    store the depth of the shape box.
  
\begin{codeexample}[code only]
\saveddimen{\depth}{
  \pgf@x=\dp\pgfnodeparttextbox 
}
\end{codeexample}
  \end{command}  
  \begin{command}{\savedmacro\marg{command}\marg{code}}
    This command is similar to |\saveddimen|, only at some point
    in \meta{code}, \meta{command} should be defined appropriately,
    (this could be a value, or some text).

    In the |regular polygon| shape, a saved macro is used to
    store the number of sides of the polygon.
  
\begin{codeexample}[code only]
\savedmacro{\sides}{\let\sides\pgfpolygonsides}
\end{codeexample}
  \end{command}  
  \begin{command}{\anchor\marg{name}\marg{code}}
    This command declares an anchor named \meta{name}. Unlike for saved
    anchors, the \meta{code} will not be executed each time a node is
    declared. Rather, the \meta{code} is only executed when the anchor
    is specifically requested; either for anchoring the node during
    its creation or as a  position in the shape referenced later on.

    The \meta{name} is a quite arbitrary string that is not ``passed
    down'' to the system level. Thus, names like |south| or |1| or
    |::| would all be fine.

    A saved anchor is not automatically also a normal anchor. If you
    wish to give the users access to a saved anchor you must declare a
    normal anchor that just returns the position of the saved anchor.

    When the \meta{code} is executed, all saved anchor macros will be
    defined. Thus, you can reference them in your \meta{code}. The
    effect of the \meta{code} should be to set the values of |\pgf@x|
    and |\pgf@y| to the coordinates of the anchor.

    Let us consider some example for the |simple rectangle|
    shape. First, we would like to make the upper right corner
    publicly available, for example as |north east|:
    
\begin{codeexample}[code only]
\anchor{north east}{\upperrightcorner}
\end{codeexample}

    The |\upperrightcorner| macro will set |\pgf@x| and |\pgf@y| to
    the coordinates of the upper right corner. Thus, |\pgf@x| and
    |\pgf@y| will have exactly the right values at the end of the
    anchor's code.

    Next, let us define a |north west| anchor. For this anchor, we can
    negate the |\pgf@x| variable:
   
\begin{codeexample}[code only]
\anchor{north west}{
  \upperrightcorner
  \pgf@x=-\pgf@x
}
\end{codeexample}

    Finally, it is a good idea to always define a |center| anchor,
    which will be the default location for a shape.

\begin{codeexample}[code only]
\anchor{center}{\pgfpointorigin}
\end{codeexample}

    You might wonder whether we should not take into consideration
    that the node is not placed at the origin, but has been shifted
    somewhere. However, the anchor positions are always specified in
    the shape's ``private'' coordinate system. The ``outer''
    transformation that has been applied to the shape upon its
    creation is applied automatically to the coordinates returned by
    the anchor's \meta{code}.

    Out |simple rectangle| only has one text label (node
    part) called |text|. This is the default situation, so we need not
    do anything. For the |text| node part we must setup a |text|
    anchor. This   anchor is used upon creation of a node to determine
    the lower left  corner of the text label (within the private
    coordinate system of the shape). By default, the |text| anchor is
    at the origin, but you may change this. For example, we would say
\begin{codeexample}[code only]
\anchor{text}{%
  \upperrightcorner%
  \pgf@x=-\pgf@x%
  \pgf@y=-\pgf@y%
}
\end{codeexample}
    to center the text label on the origin in the shape coordinate
    space. Note that we could \emph{not} have written the following:
    
\begin{codeexample}[code only]
\anchor{text}{\pgfpoint{-.5\wd\pgfnodeparttextbox}{-.5\ht\pgfnodeparttextbox}}
\end{codeexample}
    Do you see why this is wrong? The problem is that the box
    |\pgfnodeparttextbox| will most likely not have the correct size
    when the anchor is computed. After all, the anchor position might
    be recomputed at a time when several other nodes have been created. 

    If a shape has several node parts, we would have to define an
    anchor for each part.    
  \end{command}  
  \begin{command}{\anchorborder\marg{code}}
    A \emph{border anchor} is an anchor point on the border of the
    shape. What exactly is considered as the ``border'' of the shape
    depends on the shape.

    When the user request a point on the border of the shape using the
    |\pgfpointshapeborder| command, the \meta{code} will be executed
    to discern this point. When the execution of  the \meta{code}
    starts, the dimensions |\pgf@x| and |\pgf@y| will have been set to
    a location $p$ in the shape's coordinate system. It is now the job of
    the \meta{code} to setup |\pgf@x| and |\pgf@y| such that they
    specify the point on the shape's border that lies on a straight
    line from the shape's center to the point $p$. Usually, this is a
    somewhat complicated computation, involving many case distinctions
    and some basic math.

    For our |simple rectangle| we must compute a point on the border
    of a rectangle whose one corner is the origin (ignoring the depth
    for simplicity) and whose other corner is |\upperrightcorner|. The
    following code might be used:
\begin{codeexample}[code only]
\anchorborder{%
  % Call a function that computes a border point. Since this
  % function will modify dimensions like \pgf@x, we must move them to
  % other dimensions.
  \@tempdima=\pgf@x
  \@tempdimb=\pgf@y
  \pgfpointborderrectangle{\pgfpoint{\@tempdima}{\@tempdimb}}{\upperrightcorner}
}
\end{codeexample}
  \end{command}  
  \begin{command}{\backgroundpath\marg{code}}
    This command specifies the path that ``makes up'' the background
    of the shape. Note that the shape cannot prescribe what is going
    to happen with the path: It might be drawn, shaded, filled, or
    even thrown away. If you want to specify that something should
    ``always'' happen when this shape is drawn (for example, if the
    shape is a stop-sign, we \emph{always} want it to be filled with a
    red color), you can use commands like |\beforebackgroundpath|,
    explained below.

    When the \meta{code} is executed, all saved anchors will be in
    effect. The \meta{code} should contain path construction
    commands.

    For our |simple rectangle|, the following code might be used:
\begin{codeexample}[code only]
\backgroundpath{
  \pgfpathrectanglecorners
    {\upperrightcorner}
    {\pgfpointscale{-1}{\upperrightcorner}}
}  
\end{codeexample}
    As the name suggests, the background path is used ``behind'' the
    text labels. Thus, this path is used first, then the text labels are
    drawn, possibly obscuring part of the path.
  \end{command}  
  \begin{command}{\foregroundpath\marg{code}}
    This command works like |\backgroundpath|, only it is invoked
    after the text labels have been drawn. This means that this path can
    possibly obscure (part of) the text labels.
  \end{command}  
  \begin{command}{\behindbackgroundpath\marg{code}}
    Unlike the previous two commands, \meta{code} should not only
    construct a path, it should also use this path in whatever way is
    appropriate. For example, the \meta{code} might fill some area
    with a uniform color.

    Whatever the \meta{code} does, it does it first. This means that
    any drawing done by \meta{code} will be even behind the background
    path.

    Note that the \meta{code} is protected with a |{pgfscope}|.
  \end{command}  
  \begin{command}{\beforebackgroundpath\marg{code}}
    This command works like |\behindbackgroundpath|, only the
    \meta{code} is executed after the background path has been used,
    but before the texts label are drawn.
  \end{command}  
  \begin{command}{\behindforegroundpath\marg{code}}
    The \meta{code} is executed after the text labels have been drawn,
    but before the foreground path is used.
  \end{command}  
  \begin{command}{\beforeforegroundpath\marg{code}}
    This \meta{code} is executed at the very end.
  \end{command}  
  \begin{command}{\inheritsavedanchors|[from=|\marg{another shape name}|]|}
    This command allows you to inherit the code for saved anchors from
    \meta{another shape name}. The idea is that if you wish to create
    a new shape that is just a small modification of a another shape,
    you can recycle the code used for \meta{another shape name}.

    The effect of this command is the same as if you had called
    |\savedanchor| and |\saveddimen| for each saved anchor or saved
    dimension declared in \meta{another shape name}. Thus, it is not
    possible to ``selectively'' inherit only some saved anchors, you
    always have to inherit all saved anchors from another
    shape. However, you can inherit the saved anchors of more than one
    shape by calling this command several times.
  \end{command}  
  \begin{command}{\inheritbehindbackgroundpath|[from=|\marg{another shape name}|]|}
    This command can be used to inherit the code used for the
    drawings behind the background path from \meta{another shape name}. 
  \end{command}  
  \begin{command}{\inheritbackgroundpath|[from=|\marg{another shape name}|]|}
    Inherits the background path code from \meta{another shape name}.
  \end{command}  
  \begin{command}{\inheritbeforebackgroundpath|[from=|\marg{another shape name}|]|}
    Inherits the before background path code from \meta{another shape name}.
  \end{command}  
  \begin{command}{\inheritbehindforegroundpath|[from=|\marg{another shape name}|]|}
    Inherits the behind foreground path code from \meta{another shape name}.
  \end{command}  
  \begin{command}{\inheritforegroundpath|[from=|\marg{another shape name}|]|}
    Inherits the foreground path code from \meta{another shape name}.
  \end{command}  
  \begin{command}{\inheritbeforeforegroundpath|[from=|\marg{another shape name}|]|}
    Inherits the before foreground path code from \meta{another shape name}.
  \end{command}  
  \begin{command}{\inheritanchor|[from=|\marg{another shape name}|]|\marg{name}}
    Inherits the code of one specific anchor named \meta{name} from
    \meta{another shape name}. Thus, unlike saved anchors, which must
    be inherited collectively, normal anchors can and must be
    inherited individually.
  \end{command}  
  \begin{command}{\inheritanchorborder|[from=|\marg{another shape name}|]|}
    Inherits the border anchor code from \meta{another shape name}.
  \end{command}

  The following example shows how a shape can be defined that relies
  heavily on inheritance:
\makeatletter
\begin{codeexample}[]
\pgfdeclareshape{document}{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  % ... and possibly more
  \backgroundpath{% this is new
    % store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    % compute corner of ``flipped page''
    \pgf@xc=\pgf@xb \advance\pgf@xc by-5pt % this should be a parameter
    \pgf@yc=\pgf@yb \advance\pgf@yc by-5pt
    % construct main path
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathclose
    % add little corner
    \pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
 }
}\hskip-1.2cm
\begin{tikzpicture}
  \node[shade,draw,shape=document,inner sep=2ex] (x) {Remark};
  \node[fill=examplefill,draw,ellipse,double]
    at ([shift=(-80:3cm)]x) (y) {Use Case};

  \draw[dashed] (x) -- (y);  
\end{tikzpicture}
\end{codeexample}
  
\end{command}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-paths.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Constructing Paths}

\subsection{Overview}

The ``basic entity of drawing'' in \pgfname\ is the \emph{path}. A
path consists of several parts, each of which is either a closed or
open curve. An open curve has a starting point and an end point and,
in between, consists of several \emph{segments}, each of which is
either a straight line or a Bézier curve. Here is an example of a
path (in red) consisting of two parts, one open, one closed:

\begin{codeexample}[]
\begin{tikzpicture}[scale=2]
  \draw[thick,red]
       (0,0) coordinate (a)
    -- coordinate (ab) (1,.5) coordinate (b)
    .. coordinate (bc) controls +(up:1cm) and +(left:1cm) .. (3,1)  coordinate (c)
       (0,1) -- (2,1) -- coordinate (x) (1,2) -- cycle;

  \draw (a)  node[below] {start part 1}
        (ab) node[below right] {straight segment}
        (b)  node[right] {end first segment}
        (c)  node[right] {end part 1}
        (x)  node[above right]  {part 2 (closed)};        
\end{tikzpicture}
\end{codeexample}

A path, by itself, has no ``effect,'' that is, it does not leave any
marks on the page. It is just a set of points on the plane. However,
you can \emph{use} a path in different ways. The most natural actions
are \emph{stroking} (also known as \emph{drawing}) and
\emph{filling}. Stroking can be imagined as picking up a pen of a
certain diameter and ``moving it along the path.'' Filling means that
everything ``inside'' the path is filled with a uniform
color. Naturally, the open parts of a path must first be closed before
a path can be filled.

In \pgfname, there are numerous commands for constructing paths, all
of which start with |\pgfpath|. There are also commands for
\emph{using} paths, though most operations can be performed by calling
|\pgfusepath| with an appropriate parameter.

As a side-effect, the path construction commands keep track of two
bounding boxes. One is the bounding box for the current path, the
other is a bounding box for all paths in the current picture. See
Section~\ref{section-bb} for more details.

Each path construction command extends the current path in some
way. The ``current path'' is a global entity that persists across
\TeX\ groups. Thus, between calls to the path construction commands
you can perform arbitrary computations and even open and closed \TeX\
groups. The current path only gets ``flushed'' when the |\pgfusepath|
command is called (or when the soft-path subsystem is used directly,
see Section~\ref{section-soft-paths}).

\subsection{The Move-To Path Operation}

The most basic operation is the move-to operation. It must be given at
the beginning of paths, though some path construction command (like
|\pgfpathrectangle|) generate move-tos implicitly. A move-to operation
can also be used to start a new part of a path. 

\begin{command}{\pgfpathmoveto\marg{coordinate}}
  This command expects a \pgfname-coordinate like |\pgfpointorigin| as
  its parameter. When the current path is empty, this operation will
  start the path at the given \meta{coordinate}. If a path has already
  been partly constructed, this command will end the current part of
  the path and start a new one.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{1cm}}
  \pgfpathlineto{\pgfpoint{2cm}{1cm}}
  \pgfpathlineto{\pgfpoint{3cm}{0.5cm}}
  \pgfpathlineto{\pgfpoint{3cm}{0cm}}
  \pgfsetfillcolor{examplefill}
  \pgfusepath{fill,stroke}
\end{pgfpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{1cm}}
  \pgfpathlineto{\pgfpoint{2cm}{1cm}}
  \pgfpathmoveto{\pgfpoint{2cm}{1cm}} % New part
  \pgfpathlineto{\pgfpoint{3cm}{0.5cm}}
  \pgfpathlineto{\pgfpoint{3cm}{0cm}}
  \pgfsetfillcolor{examplefill}
  \pgfusepath{fill,stroke}
\end{pgfpicture}
\end{codeexample}
  The command will apply the current coordinate transformation matrix
  to \meta{coordinate} before using it.

  The command will update the bounding box of the current path and
  picture, if necessary. 
\end{command}


\subsection{The Line-To Path Operation}

\begin{command}{\pgfpathlineto\marg{coordinate}}
  This command extends the current path in a straight line to the
  given \meta{coordinate}. If this command is given at the beginning
  of path without any other path construction command given before (in
  particular without a move-to operation), the \TeX\ file may compile
  without an error message, but a viewer application may display an
  error message when trying to render the picture. 
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{1cm}{1cm}}
  \pgfpathlineto{\pgfpoint{2cm}{1cm}}
  \pgfsetfillcolor{examplefill}
  \pgfusepath{fill,stroke}
\end{pgfpicture}
\end{codeexample}
  The command will apply the current coordinate transformation matrix
  to \meta{coordinate} before using it.

  The command will update the bounding box of the current path and
  picture, if necessary. 
\end{command}


\subsection{The Curve-To Path Operation}

\begin{command}{\pgfpathcurveto\marg{support 1}\marg{support 2}\marg{coordinate}}
  This command extends the current path with a Bézier curve from the
  last point of the path to  \meta{coordinate}. The \meta{support 1}
  and \meta{support 2} are the first and second support point of the
  Bézier curve. For more information on Bézier curve, please consult a
  standard textbook on computer graphics.

  Like the line-to command, this command may not be the first path
  construction command in a path.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathcurveto
    {\pgfpoint{1cm}{1cm}}{\pgfpoint{2cm}{1cm}}{\pgfpoint{3cm}{0cm}}
  \pgfsetfillcolor{examplefill}
  \pgfusepath{fill,stroke}
\end{pgfpicture}
\end{codeexample}
  The command will apply the current coordinate transformation matrix
  to \meta{coordinate} before using it.

  The command will update the bounding box of the current path and
  picture, if necessary. However, the bounding box is simply made
  large enough such that it encompasses all of the support points and
  the \meta{coordinate}. This will guarantee that the curve is
  completely inside the bounding box, but the bounding box will
  typically be quite a bit too large. It is not clear (to me) how this 
  can be avoided without resorting to ``some serious math'' in order
  to calculate a precise bounding box. 
\end{command}


\subsection{The Close Path Operation}

\begin{command}{\pgfpathclose}
  This command closes the current part of the path by appending a
  straight line to the start point of the current part. Note that there
  \emph{is} a difference between closing a path and using the line-to
  operation to add a straight line to the start of the current
  path. The difference is demonstrated by the upper corners of the triangles
  in the following example: 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfsetlinewidth{5pt}
  \pgfpathmoveto{\pgfpoint{1cm}{1cm}}
  \pgfpathlineto{\pgfpoint{0cm}{-1cm}}
  \pgfpathlineto{\pgfpoint{1cm}{-1cm}}
  \pgfpathclose
  \pgfpathmoveto{\pgfpoint{2.5cm}{1cm}}
  \pgfpathlineto{\pgfpoint{1.5cm}{-1cm}}
  \pgfpathlineto{\pgfpoint{2.5cm}{-1cm}}
  \pgfpathlineto{\pgfpoint{2.5cm}{1cm}}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}


\subsection{Arc, Ellipse and Circle Path Operations}

The path construction commands that we have discussed up to now are
sufficient to create all paths that can be created ``at all.''
However, it is useful to have special commands to create certain
shapes, like circles, that arise often in practice.

In the following, the commands for adding (parts of) (transformed)
circles to a path are described.

\begin{command}{\pgfpatharc\marg{start angle}\marg{end
      angle}{\ttfamily\char`\{}\meta{radius}\opt{| and |\meta{y-radius}}{\ttfamily\char`\}}}
  This command appends a part of a circle (or an ellipse) to the current
  path. Imaging the curve between \meta{start angle} and \meta{end
    angle} on a circle of radius \meta{radius} (if $\meta{start angle}
  < \meta{end angle}$, the curve goes around the circle
  counterclockwise, otherwise clockwise). This curve is now moved such
  that the point where the curve starts is the previous last point of the
  path. Note that this command will \emph{not} start a new part of the
  path, which is important for example for filling purposes. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{0cm}{1cm}}
  \pgfpatharc{180}{90}{.5cm}
  \pgfpathlineto{\pgfpoint{3cm}{1.5cm}}
  \pgfpatharc{90}{-45}{.5cm}
  \pgfusepath{fill}
\end{tikzpicture}
\end{codeexample}

  Saying |\pgfpatharc{0}{360}{1cm}| ``nearly'' gives you a full
  circle. The ``nearly'' refers to the fact that the circle will not
  be closed. You can close it using |\pgfpathclose|.

  If the optional \meta{y-radius} is given, the \meta{radius} is the
  $x$-radius and the \meta{y-radius} the $y$-radius of the ellipse
  from which the curve is taken:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpatharc{180}{45}{2cm and 1cm}
  \pgfusepath{draw}
\end{tikzpicture}
\end{codeexample}

  The axes of the circle or ellipse from which the arc is ``taken''
  always point up and right. However, the current coordinate
  transformation matrix will have an effect on the arc. This can be
  used to, say, rotate an arc:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgftransformrotate{30}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpatharc{180}{45}{2cm and 1cm}
  \pgfusepath{draw}
\end{tikzpicture}
\end{codeexample}

  The command will update the bounding box of the current path and
  picture, if necessary. Unless rotation or shearing transformations
  are applied, the bounding box will be tight.
\end{command}

\begin{command}{\pgfpatharcaxes\marg{start angle}\marg{end
      angle}\marg{first axis}\marg{second axis}}
  This command is similar to |\pgfpatharc|. The main difference is how
  the ellipse or circle is specified from which the arc is taken. The
  two parameters \meta{first axis} and \meta{second axis} are the
  $0^\circ$-axis and the $90^\circ$-axis of the ellipse from which the
  path is taken. Thus, |\pgfpatharc{0}{90}{1cm and 2cm}| has the same effect
  as
\begin{verbatim}
\pgfpatharcaxes{0}{90}{\pgfpoint{1cm}{0cm}}{\pgfpoint{0cm}{2cm}}
\end{verbatim}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw (0,0) -- (2cm,5mm) (0,0) -- (0cm,1cm);
  
  \pgfpathmoveto{\pgfpoint{2cm}{5mm}}
  \pgfpatharcaxes{0}{90}{\pgfpoint{2cm}{5mm}}{\pgfpoint{0cm}{1cm}}
  \pgfusepath{draw}
\end{tikzpicture}
\end{codeexample}
\end{command}  


\begin{command}{\pgfpathellipse\marg{center}\marg{first
      axis}\marg{second axis}}
  The effect of this command is to append an ellipse to the current
  path (if the path is not empty, a new part is started). The
  ellipse's center will be \meta{center} and \meta{first axis} and
  \meta{second axis} are the axis \emph{vectors}. The same effect as
  this command can also be achieved using an appropriate sequence of
  move-to, arc, and close operations, but this command is easier and
  faster. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathellipse{\pgfpoint{1cm}{0cm}}
                 {\pgfpoint{1.5cm}{0cm}}
                 {\pgfpoint{0cm}{1cm}}
  \pgfusepath{draw}
  \color{red}               
  \pgfpathellipse{\pgfpoint{1cm}{0cm}}
                 {\pgfpoint{1cm}{1cm}}
                 {\pgfpoint{-0.5cm}{0.5cm}}
  \pgfusepath{draw}
\end{tikzpicture}
\end{codeexample}

  The command will apply coordinate transformations to all coordinates
  of the ellipse. However, the coordinate transformations are applied
  only after the ellipse is ``finished conceptually.'' Thus, a
  transformation of 1cm to the right will simply shift the ellipse one
  centimeter to the right; it will not add 1cm to the $x$-coordinates
  of the two axis vectors.

  The command will update the bounding box of the current path and
  picture, if necessary. 
\end{command}

\begin{command}{\pgfpathcirlce\marg{center}\marg{radius}}
  A shorthand for |\pgfpathellipse| applied to \meta{center} and the
  two axis vectors $(\meta{radius},0)$ and $(0,\meta{radius})$. 
\end{command}


\subsection{Rectangle Path Operations}

Another shape that arises frequently is the rectangle. Two commands
can be used to add a rectangle to the current path. Both commands will
start a new part of the path.


\begin{command}{\pgfpathrectangle\marg{corner}\marg{diagonal vector}}
  Adds a rectangle to the path whose one corner is \meta{corner} and
  whose opposite corner is given by $\meta{corner} + \meta{diagonal
    vector}$.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathrectangle{\pgfpoint{1cm}{0cm}}{\pgfpoint{1.5cm}{1cm}}
  \pgfpathrectangle{\pgfpoint{1.5cm}{0.25cm}}{\pgfpoint{1.5cm}{1cm}}
  \pgfpathrectangle{\pgfpoint{2cm}{0.5cm}}{\pgfpoint{1.5cm}{1cm}}
  \pgfusepath{draw}
\end{tikzpicture}
\end{codeexample}
  The command will apply coordinate transformations and update the
  bounding boxes tightly.
\end{command}


\begin{command}{\pgfpathrectanglecorners\marg{corner}\marg{opposite corner}}
  Adds a rectangle to the path whose two opposing corners are
  \meta{corner} and \meta{opposite corner}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathrectanglecorners{\pgfpoint{1cm}{0cm}}{\pgfpoint{1.5cm}{1cm}}
  \pgfusepath{draw}
\end{tikzpicture}
\end{codeexample}
  The command will apply coordinate transformations and update the
  bounding boxes tightly.
\end{command}



\subsection{The Grid Path Operation}

\begin{command}{\pgfpathgrid\oarg{options}\marg{lower left}\marg{upper right}}
  Appends a grid to the current path. That is, a (possibly large)
  number of parts are added to the path, each part consisting of a
  single horizontal or vertical straight line segment.

  Conceptually, the origin is part of the grid and the grid is clipped 
  to the rectangle specified by the \meta{lower left} and
  the \meta{upper right} corner. However, no clipping occurs (this
  command just adds parts to the current path). Rather, the points
  where the lines enter and leave the ``clipping area'' are computed
  and used to add simple lines to the current path.

  The following keys influence the grid:
  \begin{key}{/pgf/stepx=\meta{dimension} (initially 1cm)}
    The horizontal stepping.
  \end{key}
  \begin{key}{/pgf/stepy=\meta{dimension} (initially 1cm)}
    The vertical stepping.
  \end{key}
  \begin{key}{/pgf/step=\meta{vector}}
    Sets the horizontal stepping to the $x$-coordinate of
    \meta{vector} and the vertical stepping to its $y$-coordinate.
  \end{key}
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetlinewidth{0.8pt}
  \pgfpathgrid[step={\pgfpoint{1cm}{1cm}}]
    {\pgfpoint{-3mm}{-3mm}}{\pgfpoint{33mm}{23mm}}
  \pgfusepath{stroke}
  \pgfsetlinewidth{0.4pt}
  \pgfpathgrid[stepx=1mm,stepy=1mm]
    {\pgfpoint{-1.5mm}{-1.5mm}}{\pgfpoint{31.5mm}{21.5mm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
  The command will apply coordinate transformations and update the
  bounding boxes tightly. As for ellipses, the transformations are
  applied to the ``conceptually finished'' grid. 
\begin{codeexample}[]
\begin{pgfpicture}
  \pgftransformrotate{10}
  \pgfpathgrid[stepx=1mm,stepy=2mm]{\pgfpoint{0mm}{0mm}}{\pgfpoint{30mm}{30mm}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}


\subsection{The Parabola Path Operation}

\begin{command}{\pgfpathparabola\marg{bend vector}\marg{end vector}}
  This command appends two half-parabolas to the  current path. The
  first starts at the current point and ends at the current point plus
  \meta{bend vector}. At his point, it has its bend. The second half
  parabola starts at that bend point and end at point that is given by
  the bend plus \meta{end vector}.

  If you set \meta{end vector} to the null vector, you append only a
  half parabola that goes from the current point to the bend; by
  setting \meta{bend vector} to the null vector, you append only a
  half parabola that goes to current point plus \meta{end vector} and
  has its bend at the current point.

  It is not possible to use this command to draw a part of a parabola
  that does not contain the bend.

\begin{codeexample}[]
\begin{pgfpicture}
  % Half-parabola going ``up and right''
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathparabola{\pgfpointorigin}{\pgfpoint{2cm}{4cm}}
  \color{red}
  \pgfusepath{stroke}

  % Half-parabola going ``down and right''
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathparabola{\pgfpoint{-2cm}{4cm}}{\pgfpointorigin}
  \color{blue}
  \pgfusepath{stroke}

  % Full parabola
  \pgfpathmoveto{\pgfpoint{-2cm}{2cm}}
  \pgfpathparabola{\pgfpoint{1cm}{-1cm}}{\pgfpoint{2cm}{4cm}}
  \color{orange}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
  The command will apply coordinate transformations and update the
  bounding boxes.
\end{command}


\subsection{Sine and Cosine Path Operations}

Sine and cosine curves often need to be drawn and the following commands
may help with this. However, they only allow you to append sine and
cosine curves in intervals that are multiples of $\pi/2$.

\begin{command}{\pgfpathsine\marg{vector}}
  This command appends a sine curve in the interval $[0,\pi/2]$ to the
  current path. The sine curve is squeezed or stretched such that the
  curve starts at the current point and ends at the current point plus
  \meta{vector}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,1);
  \pgfpathmoveto{\pgfpoint{1cm}{0cm}}
  \pgfpathsine{\pgfpoint{1cm}{1cm}}
  \pgfusepath{stroke}

  \color{red}
  \pgfpathmoveto{\pgfpoint{1cm}{0cm}}
  \pgfpathsine{\pgfpoint{-2cm}{-2cm}}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
  The command will apply coordinate transformations and update the
  bounding boxes.  
\end{command}

\begin{command}{\pgfpathcosine\marg{vector}}
  This command appends a cosine curve in the interval $[0,\pi/2]$ to the
  current path. The curve is squeezed or stretched such that the
  curve starts at the current point and ends at the current point plus
  \meta{vector}. Using several sine and cosine operations in sequence
  allows you to produce a complete sine or cosine curve
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpoint{0cm}{0cm}}
  \pgfpathsine{\pgfpoint{1cm}{1cm}}
  \pgfpathcosine{\pgfpoint{1cm}{-1cm}}
  \pgfpathsine{\pgfpoint{1cm}{-1cm}}
  \pgfpathcosine{\pgfpoint{1cm}{1cm}}
  \pgfsetfillcolor{examplefill}
  \pgfusepath{fill,stroke}
\end{pgfpicture}
\end{codeexample}
  The command will apply coordinate transformations and update the
  bounding boxes.  
\end{command}


\subsection{Plot Path Operations}

There exist several commands for appending
plots to a path. These
commands are available through the module |plot|. They are
documented in Section~\ref{section-plots}.


\subsection{Rounded Corners}

Normally, when you connect two straight line segments or when you
connect two curves that end and start ``at different angles'' you get
``sharp corners'' between the lines or curves. In some cases it is
desirable to produce ``rounded corners'' instead. Thus, the lines
or curves should be shortened a bit and then connected by arcs.

\pgfname\ offers an easy way to achieve this effect, by calling the
following two commands.

\begin{command}{\pgfsetcornersarced\marg{point}}
  This command causes all subsequent corners to be replaced by little
  arcs. The effect of this command lasts till the end of the current
  \TeX\ scope.

  The \meta{point} dictates how large the corner arc will be. Consider
  a corner made by two lines $l$ and~$r$ and assume that the line $l$
  comes first on the path. The $x$-dimension of the \meta{point}
  decides by how much the line~$l$ will be shortened, the
  $y$-dimension of \meta{point} decides by how much the line $r$ will
  be shortened. Then, the shortened lines are connected by an arc.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \pgfsetcornersarced{\pgfpoint{5mm}{5mm}}
  \pgfpathrectanglecorners{\pgfpointorigin}{\pgfpoint{3cm}{2cm}}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \pgfsetcornersarced{\pgfpoint{10mm}{5mm}}
  % 10mm entering,
  % 5mm leaving.
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{0cm}{2cm}}
  \pgfpathlineto{\pgfpoint{3cm}{2cm}}
  \pgfpathcurveto
    {\pgfpoint{3cm}{0cm}}
    {\pgfpoint{2cm}{0cm}}
    {\pgfpoint{1cm}{0cm}}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}

  If the $x$- and $y$-coordinates of \meta{point} are the same and the
  corner is a right angle, you will get a perfect quarter circle
  (well, not quite perfect, but perfect up to six decimals). When the
  angle is not $90^\circ$, you only get a fair approximation.

  More or less ``all'' corners will be rounded, even the corner
  generated by a |\pgfpathclose| command. (The author is a bit proud
  of this feature.)
  
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetcornersarced{\pgfpoint{4pt}{4pt}}
  \pgfpathmoveto{\pgfpointpolar{0}{1cm}}
  \pgfpathlineto{\pgfpointpolar{72}{1cm}}
  \pgfpathlineto{\pgfpointpolar{144}{1cm}}
  \pgfpathlineto{\pgfpointpolar{216}{1cm}}
  \pgfpathlineto{\pgfpointpolar{288}{1cm}}
  \pgfpathclose
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}

  To return to normal (unrounded) corners, use
  |\pgfsetcornersarced{\pgfpointorigin}|.

  Note that the rounding will produce strange and undesirable effects
  if the lines at the corners are too short. In this case the
  shortening may cause the lines to ``suddenly extend over the other
  end'' which is rarely desirable. 
\end{command}




\subsection{Internal Tracking of Bounding Boxes for Paths and Pictures}

\label{section-bb}

\makeatletter

The path construction commands keep track of two bounding boxes: One
for the current path, which is reset whenever the path is used and
thereby flushed, and a bounding box for the current |{pgfpicture}|. 

The bounding boxes are not accessible by ``normal'' macros. Rather,
two sets of four dimension variables are used for this, all of which
contain the letter~|@|.

\begin{textoken}{\pgf@pathminx}
  The minimum $x$-coordinate ``mentioned'' in the current
  path. Initially, this is set to $16000$pt.
\end{textoken}

\begin{textoken}{\pgf@pathmaxx}
  The maximum $x$-coordinate ``mentioned'' in the current
  path. Initially, this is set to $-16000$pt.
\end{textoken}

\begin{textoken}{\pgf@pathminy}
  The minimum $y$-coordinate ``mentioned'' in the current
  path. Initially, this is set to $16000$pt.
\end{textoken}

\begin{textoken}{\pgf@pathmaxy}
  The maximum $y$-coordinate ``mentioned'' in the current
  path. Initially, this is set to $-16000$pt.
\end{textoken}

\begin{textoken}{\pgf@picminx}
  The minimum $x$-coordinate ``mentioned'' in the current
  picture. Initially, this is set to $16000$pt.
\end{textoken}

\begin{textoken}{\pgf@picmaxx}
  The maximum $x$-coordinate ``mentioned'' in the current
  picture. Initially, this is set to $-16000$pt.
\end{textoken}

\begin{textoken}{\pgf@picminy}
  The minimum $y$-coordinate ``mentioned'' in the current
  picture. Initially, this is set to $16000$pt.
\end{textoken}

\begin{textoken}{\pgf@picmaxy}
  The maximum $y$-coordinate ``mentioned'' in the current
  picture. Initially, this is set to $-16000$pt.
\end{textoken}


Each time a path construction command is called, the above variables
are (globally) updated. To facilitate this, you can use the following
command:

\begin{command}{\pgf@protocolsizes\marg{x-dimension}\marg{y-dimension}}
  Updates all of the above dimension in such a way that the point
  specified by the two arguments is inside both bounding boxes. For
  the picture's bounding box this updating occurs only if
  |\ifpgf@relevantforpicturesize| is true, see below.
\end{command}

For the bounding box of the picture it is not always desirable that
every path construction command affects this bounding box. For
example, if you have just used a clip command, you do not want anything
outside the clipping area to affect the bounding box. For this reason,
there exists a special ``\TeX\ if'' that (locally) decides whether
updating should be applied to the picture's bounding box. Clipping
will set this if to false, as will certain other commands.

\begin{command}{\pgf@relevantforpicturesizefalse}
  Suppresses updating of the picture's bounding box.
\end{command}

\begin{command}{\pgf@relevantforpicturesizetrue}
  Causes updating of the picture's bounding box.
\end{command}



==> pgfmanual-en-base-patterns.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Patterns}

\label{section-patterns}

\subsection{Overview}

There are many ways of filling a path. First, you can fill it using a
solid color and this is also the fasted method. Second, you can also
fill it using a shading, which means that the color changes smoothly
between two (or more) different colors. Third, you can fill it using a
tiling pattern and it is explained in the following how this is done.

A tiling pattern can be imagined as a rectangular tile (hence the
name) on which a small picture is painted. There is not a single tile,
but (conceptually) an infinite number of tiles, all showing the same 
picture, and these tiles are arranged horizontally and vertically to
fill the plane. When you use a tiling pattern to fill a path, what
happens is that the path clips out a ``window'' through which we see
part of this infinite plane.

Patterns come in two versions: \emph{inherently colored patterns} and
\emph{form-only patterns}. (These are often called ``color patterns''
and ``uncolored patterns,'' but these names are misleading since
uncolored patterns do have a color and the color changes. As I said, 
the name is misleading\dots) An inherently colored pattern is just a
colored tile like, say, a red star with a black outline. A form-only
pattern can be imagined as a tile that is a kind of rubber stamp. When
this pattern is used, the stamp is used to print copies of the stamp
picture onto the plane, but we can use a different stamp color each
time we use a form-only pattern.

\pgfname\ provides a special support for patterns. You can declare a
pattern and then use it very much like a fill color. \pgfname\
directly maps patterns to the pattern facilities of the underlying
graphic languages (PostScript, \textsc{pdf}, and \textsc{svg}). This
means that filling a path using a pattern will be nearly as fast as if
you used a uniform color.

There are a number of pitfalls and restrictions when using
patterns. First, once a pattern has been declared, you cannot change
it anymore. In particular, it is not possible to enlarge it or change
the line width. Such flexibility would require that the repeating of
the pattern were not done by the graphic language, but on the
\pgfname\ level. This would make patterns orders of magnitude slower
to produce and to render.

Second, the phase of patterns is not well-defined, that is, it is not
clear where origin of the ``first'' tile is. To be more precise,
PostScript and \textsc{pdf} on the one hand and \textsc{svg} on the
other hand define the origin differently. PostScript and \textsc{pdf}
define a fixed origin that is independent of where the path lies. This
has the highly desirable effect that if you use the same pattern to
fill multiple paths, this has the same effect as if you used the
pattern to will a single path that is the union of all the paths. By
comparison, \textsc{svg} uses the upper-left (?) corner of the path to
be filled as the origin. However, the \textsc{svg} specification is a
bit vague on this question.


\subsection{Declaring a Pattern}

Before a pattern can be used, it must be declared. The following
command is used for this:

\begin{command}{\pgfdeclarepatternformonly%
    \marg{name}%
    \marg{lower left}%
    \marg{upper right}%
    \marg{tile size}%
    \marg{code}}
  This command declares a new form-only pattern. The \marg{name} is a
  name for later reference. The two parameters \marg{lower left} and
  \marg{upper right} must describe a bounding box that is large enough
  to encompass the complete tile.

  The size of a tile is given by \meta{tile size}, that is, a tile is
  a rectangle whose lower left   corner is the origin and whose upper
  right corner is given by \meta{tile size}. This might make you
  wonder why the second and third parameters are needed. First, the
  bounding box might be smaller than the tile size if the tile is
  larger than the picture on the tile. Second, the bounding box might
  be bigger, in which case the picture will ``bleed'' over the tile.

  The \meta{code} should be \pgfname\ code than can be protocolled. It
  should not contain any color code.

  
\begin{codeexample}[]
\pgfdeclarepatternformonly{stars}
{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
{\pgfpoint{1cm}{1cm}}
{
  \pgftransformshift{\pgfpoint{.5cm}{.5cm}}
  \pgfpathmoveto{\pgfpointpolar{0}{4mm}}
  \pgfpathlineto{\pgfpointpolar{144}{4mm}}
  \pgfpathlineto{\pgfpointpolar{288}{4mm}}
  \pgfpathlineto{\pgfpointpolar{72}{4mm}}
  \pgfpathlineto{\pgfpointpolar{216}{4mm}}
  \pgfpathclose%
  \pgfusepath{fill}
}
\begin{tikzpicture}
  \filldraw[pattern=stars] (0,0)   rectangle (1.5,2);  
  \filldraw[pattern=stars,pattern color=red]
                           (1.5,0) rectangle (3,2);  
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfdeclarepatterninherentlycolored
    \marg{name}
    \marg{lower left}
    \marg{upper right}
    \marg{tile size}
    \marg{code}}
  This command works like |\pgfdeclarepatternuncolored|, only the
  pattern will have an inherent color. To set the color, you should
  use \pgfname's color commands, not the |\color| command, since this
  fill not be protocolled.
  
\begin{codeexample}[]
\pgfdeclarepatterninherentlycolored{green stars}
{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
{\pgfpoint{1cm}{1cm}}
{
  \pgfsetfillcolor{green!50!black}
  \pgftransformshift{\pgfpoint{.5cm}{.5cm}}
  \pgfpathmoveto{\pgfpointpolar{0}{4mm}}
  \pgfpathlineto{\pgfpointpolar{144}{4mm}}
  \pgfpathlineto{\pgfpointpolar{288}{4mm}}
  \pgfpathlineto{\pgfpointpolar{72}{4mm}}
  \pgfpathlineto{\pgfpointpolar{216}{4mm}}
  \pgfpathclose%
  \pgfusepath{stroke,fill}
}
\begin{tikzpicture}
  \filldraw[pattern=green stars] (0,0) rectangle (3,2);  
\end{tikzpicture}
\end{codeexample}
\end{command}


\subsection{Setting a Pattern}

Once a pattern has been declared, it can be used.

\begin{command}{\pgfsetfillpattern\marg{name}\marg{color}}
  This command specifies that paths that are filled should be filled
  with the ``color'' by the pattern \meta{name}. For an inherently
  colored pattern, the \meta{color} parameter is ignored. For
  form-only patterns, the \meta{color} parameter specified the color
  to be used for the pattern.
\begin{codeexample}[]
\begin{tikzpicture}
  \pgfsetfillpattern{stars}{red}
  \filldraw (0,0) rectangle (1.5,2);  

  \pgfsetfillpattern{green stars}{red}
  \filldraw (1.5,0) rectangle (3,2);  
\end{tikzpicture}
\end{codeexample} 
\end{command}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-plots.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Creating Plots}

\label{section-plots}

This section describes the |plot| module.

\begin{pgfmodule}{plot}
  This module provides a set of commands that are intended to make it
  reasonably easy to plot functions using \pgfname. It is loaded
  automatically by |pgf|, but you can load it manually if you have
  only included |pgfcore|.  
\end{pgfmodule}


\subsection{Overview}

There are different reasons for using \pgfname\ for creating plots
rather than some more powerful program such as \textsc{gnuplot} or
\textsc{mathematica}, as discussed in
Section~\ref{section-why-pgname-for-plots}. So, let us assume that --
for whatever reason -- you wish to use \pgfname\ for generating a plot.

\pgfname\ (conceptually) uses a two-stage process for generating
plots. First, a \emph{plot stream} must be produced. This stream
consists (more or less) of a large number of coordinates. Second a 
\emph{plot handler} is applied to the stream. A plot handler ``does
something'' with the stream. The standard handler will issue
line-to operations to the coordinates in the stream. However, a
handler might also try to issue appropriate curve-to operations in
order to smooth the curve. A handler may even do something else
entirely, like writing each coordinate to another stream, thereby
duplicating the original stream.

Both for the creation of streams and the handling of streams different
sets of commands exist. The commands for creating streams start with
|\pgfplotstream|, the commands for setting the handler start with
|\pgfplothandler|.



\subsection{Generating Plot Streams}

\subsubsection{Basic Building Blocks of Plot Streams}
A \emph{plot stream} is a (long) sequence of the following three
commands:
\begin{enumerate}
\item
  |\pgfplotstreamstart|,
\item
  |\pgfplotstreampoint|, and
\item
  |\pgfplotstreamend|.
\end{enumerate}
Between calls of these commands arbitrary other code may be
called. Obviously, the stream should start with the first command and
end with the last command. Here is an example of a plot stream:
\begin{codeexample}[code only]
\pgfplotstreamstart
\pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
\newdimen\mydim
\mydim=2cm
\pgfplotstreampoint{\pgfpoint{\mydim}{2cm}}
\advance \mydim by 3cm
\pgfplotstreampoint{\pgfpoint{\mydim}{2cm}}
\pgfplotstreamend
\end{codeexample}

\begin{command}{\pgfplotstreamstart}
  This command signals that a plot stream starts. The effect of this
  command is to call the internal command |\pgf@plotstreamstart|,
  which is set by the current plot handler to do whatever needs to be
  done at the beginning of the plot.
\end{command}

\begin{command}{\pgfplotstreampoint\marg{point}}
  This command adds a \meta{point} to the current plot stream. The
  effect of this command is to call the internal command |\pgf@plotstreampoint|,
  which is also set by the current plot handler. This command should
  now ``handle'' the point in some sensible way. For example, a
  line-to command might be issued for the point.
\end{command}

\begin{command}{\pgfplotstreamend}
  This command signals that a plot stream ends. It calls
  |\pgf@plotstreamend|, which should now do any necessary ``cleanup.''
\end{command}

Note that plot streams are not buffered, that is, the different points
are handled immediately. However, using the recording handler, it is
possible to record a stream.

\subsubsection{Commands That Generate Plot Streams}

Plot streams can be created ``by hand'' as in the earlier
example. However, most of the time the coordinates will be produced
internally by some command. For example, the |\pgfplotxyfile| reads a
file and converts it into a plot stream.

\begin{command}{\pgfplotxyfile\marg{filename}}
  This command will try to open the file \meta{filename}. If this
  succeeds, it will convert the file contents into a plot stream as
  follows: A |\pgfplotstreamstart| is issued. Then, each nonempty line
  of the file should start with two numbers separated by a space, such
  as |0.1 1| or |100 -.3|. Anything following the numbers is ignored.

  Each pair \meta{x} and \meta{y} of numbers is converted into one
  plot stream point in the xy-coordinate system. Thus, a line like
\begin{codeexample}[code only]
2 -5 some text
\end{codeexample}
  is turned into 
\begin{codeexample}[code only]
\pgfplotstreampoint{\pgfpointxy{2}{-5}}
\end{codeexample}

  The two characters |%| and |#| are also allowed in a file and they
  are both treated as comment characters. Thus, a line starting with
  either of them is empty and, hence, ignored.

  When the file has been read completely, |\pgfplotstreamend| is
  called. 
\end{command}


\begin{command}{\pgfplotxyzfile\marg{filename}}
  This command works like |\pgfplotxyfile|, only \emph{three} numbers
  are expected on each non-empty line. They are converted into points
  in the xyz-coordinate system. Consider, the following file:
\begin{codeexample}[code only]
% Some comments
# more comments
2 -5  1 first entry
2 -.2 2 second entry
2 -5  2 third entry
\end{codeexample}
  It is turned into the following stream:
\begin{codeexample}[code only]
\pgfplotstreamstart
\pgfplotstreampoint{\pgfpointxyz{2}{-5}{1}}
\pgfplotstreampoint{\pgfpointxyz{2}{-.2}{2}}
\pgfplotstreampoint{\pgfpointxyz{2}{-5}{2}}
\pgfplotstreamend
\end{codeexample}
\end{command}


Currently, there is no command that can decide automatically whether
the xy-coordinate system should be used or whether the xyz-system
should be used. However, it would not be terribly difficult to write a
``smart file reader'' that parses coordinate files a bit more
intelligently. 


\begin{command}{\pgfplotfunction\marg{variable}\marg{sample list}\marg{point}} 
  This command will produce coordinates by iterating the
  \meta{variable} over all values in \meta{sample list}, which should
  be a list in the |\foreach| syntax. For each value of
  \meta{variable}, the \meta{point} is evaluated and the resulting
  coordinate is inserted into the plot stream.

\begin{codeexample}[]
\begin{tikzpicture}[x=3.8cm/360]
  \pgfplothandlerlineto
  \pgfplotfunction{\x}{0,5,...,360}{\pgfpointxy{\x}{sin(\x)+sin(3*\x)}}
  \pgfusepath{stroke}  
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[y=3cm/360]
  \pgfplothandlerlineto
  \pgfplotfunction{\y}{0,5,...,360}{\pgfpointxyz{sin(2*\y)}{\y}{cos(2*\y)}}
  \pgfusepath{stroke}  
\end{tikzpicture}
\end{codeexample}

  Be warnded that if the expressions that need to evaluated for each
  point are complex, then this command can be very slow.
\end{command}



\begin{command}{\pgfplotgnuplot\oarg{prefix}\marg{function}}
  This command will ``try'' to call the \textsc{gnuplot} program to
  generate the coordinates of the \meta{function}. In detail, the
  following happens:

  This command works with two files: \meta{prefix}|.gnuplot| and
  \meta{prefix}|.table|.  If the optional argument \meta{prefix} is
  not given, it is set to |\jobname|.

  Let us start with the situation where none of these files
  exists. Then \pgfname\ will first generate the file
  \meta{prefix}|.gnuplot|. In this file it writes
\begin{codeexample}[code only]
set terminal table; set output "#1.table"; set format "%.5f"
\end{codeexample}
  where |#1| is replaced by \meta{prefix}. Then, in a second line, it
  writes the text \meta{function}.

  Next, \pgfname\ will try to invoke the program |gnuplot| with the
  argument \meta{prefix}|.gnuplot|. This call may or may not succeed,
  depending on whether the |\write18| mechanism (also known as
  shell escape) is switched on and whether the |gnuplot| program is
  available.

  Assuming that the call succeeded, the next step is to invoke
  |\pgfplotxyfile| on the file \meta{prefix}|.table|; which is exactly
  the file that has just been created by |gnuplot|.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,-1) grid (4,1);
  \pgfplothandlerlineto
  \pgfplotgnuplot[plots/pgfplotgnuplot-example]{plot [x=0:3.5] x*sin(x)}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}

  The more difficult situation arises when the |.gnuplot| file exists,
  which will be the case on the second run of \TeX\ on the \TeX\
  file. In this case \pgfname\ will read this file and check whether
  it contains exactly what \pgfname\ ``would have written'' into
  this file. If this is not the case, the file contents is overwritten
  with what ``should be there'' and, as above, |gnuplot| is invoked to
  generate a new |.table| file. However, if the file contents is ``as
  expected,'' the external |gnuplot| program is \emph{not}
  called. Instead, the \meta{prefix}|.table| file is immediately
  read.

  As explained in Section~\ref{section-tikz-gnuplot}, the net effect
  of the above mechanism is that |gnuplot| is called as little as
  possible and that when you pass along the |.gnuplot| and |.table|
  files with your |.tex| file to someone else, that person can
  \TeX\ the |.tex| file without having |gnuplot| installed and without
  having the |\write18| mechanism switched on.
\end{command}



\subsection{Plot Handlers}

\label{section-plot-handlers}

A \emph{plot handler}  prescribes what ``should be done'' with a
plot stream. You must set the plot handler before the stream starts.
The following commands install the most basic plot handlers; more plot
handlers are defined in the file |pgflibraryplothandlers|, which is
documented in Section~\ref{section-library-plothandlers}.

All plot handlers work by setting redefining the following three
macros: |\pgf@plotstreamstart|, |\pgf@plotstreampoint|, and
|\pgf@plotstreamend|.

\begin{command}{\pgfplothandlerlineto}
  This handler will issue a |\pgfpathlineto| command for each point of
  the plot, \emph{except} possibly for the first. What happens with
  the first point can be specified using the two commands described
  below.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfplothandlerlineto
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{1cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{3cm}{2cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{2cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfsetmovetofirstplotpoint}
  Specifies that the line-to plot handler (and also some other plot 
  handlers) should issue a move-to command for the
  first point of the plot instead of a line-to. This will start a new
  part of the current path, which is not always, but often,
  desirable. This is the default.
\end{command}

\begin{command}{\pgfsetlinetofirstplotpoint}
  Specifies that  plot handlers should issue a line-to command for the
  first point of the plot.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfsetlinetofirstplotpoint
  \pgfplothandlerlineto
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{1cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{3cm}{2cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{2cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfplothandlerdiscard}
  This handler will simply throw away the stream.
\end{command}

\begin{command}{\pgfplothandlerrecord\marg{macro}}
  When this handler is installed, each time a plot stream command is
  called, this command will be appended to \meta{macros}. Thus, at
  the end of the stream, \meta{macro} will contain all the
  commands that were issued on the stream. You can then install
  another handler and invoke \meta{macro} to ``replay'' the stream
  (possibly many times).
 
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfplothandlerrecord{\mystream}
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{1cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{3cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{2cm}}
  \pgfplotstreamend
  \pgfplothandlerlineto
  \mystream
  \pgfplothandlerclosedcurve
  \mystream
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample} 
\end{command}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-points.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Specifying Coordinates}

\label{section-points}

\subsection{Overview}

Most \pgfname\ commands expect you to provide the coordinates of a
\emph{point} (also called \emph{coordinate}) inside your
picture. Points are always ``local'' to your picture, that is, they
never refer to an absolute position on the page, but to a position
inside the current |{pgfpicture}| environment. To specify a coordinate
you can use commands that start with |\pgfpoint|.


\subsection{Basic Coordinate Commands}

The following commands are the most basic  for specifying a
coordinate.

\begin{command}{\pgfpoint\marg{x coordinate}\marg{y coordinate}}
  Yields a point location. The coordinates are given as \TeX\
  dimensions.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathcircle{\pgfpoint{1cm}{1cm}} {2pt}
  \pgfpathcircle{\pgfpoint{2cm}{5pt}} {2pt}
  \pgfpathcircle{\pgfpoint{0pt}{.5in}}{2pt}
  \pgfusepath{fill}
\end{tikzpicture}   
\end{codeexample}
\end{command}

\begin{command}{\pgfpointorigin}
  Yields the origin. Same as |\pgfpoint{0pt}{0pt}|.
\end{command}

\begin{command}{\pgfpointpolar\marg{degree}{\ttfamily\char`\{}\meta{radius}\opt{|/|\meta{y-radius}}{\ttfamily\char`\}}}
  Yields a point location given in polar coordinates. You can specify
  the angle only in degrees, radians are not supported, currently.

  If the optional \meta{y-radius} is given, the polar coordinate is
  actually a coordinate on an ellipse whose $x$-radius is given by
  \meta{radius} and whose $y$-radius is given by \meta{y-radius}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \foreach \angle in {0,10,...,90}
    {\pgfpathcircle{\pgfpointpolar{\angle}{1cm}}{2pt}}
  \pgfusepath{fill}
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \foreach \angle in {0,10,...,90}
    {\pgfpathcircle{\pgfpointpolar{\angle}{1cm/2cm}}{2pt}}
  \pgfusepath{fill}
\end{tikzpicture}   
\end{codeexample}
\end{command}



\subsection{Coordinates in the XY-Coordinate System}

Coordinates can also be specified as multiples of an $x$-vector and a
$y$-vector. Normally, the $x$-vector points one centimeter in the
$x$-direction and the $y$-vector points one centimeter in the
$y$-direction, but using the commands |\pgfsetxvec| and
|\pgfsetyvec| they can be changed. Note that the $x$- and
$y$-vector do not necessarily point ``horizontally'' and
``vertically.''

\begin{command}{\pgfpointxy\marg{$s_x$}\marg{$s_y$}}
  Yields a point that is situated at $s_x$ times the
  $x$-vector plus $s_y$ times the $y$-vector.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathmoveto{\pgfpointxy{1}{0}}
  \pgfpathlineto{\pgfpointxy{2}{2}}
  \pgfusepath{stroke}
\end{tikzpicture}   
\end{codeexample}
\end{command}


\begin{command}{\pgfsetxvec\marg{point}}
  Sets that current $x$-vector for usage in the $xyz$-coordinate
  system. 
  \example
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  
  \pgfpathmoveto{\pgfpointxy{1}{0}}
  \pgfpathlineto{\pgfpointxy{2}{2}}
  \pgfusepath{stroke}

  \color{red}
  \pgfsetxvec{\pgfpoint{0.75cm}{0cm}}
  \pgfpathmoveto{\pgfpointxy{1}{0}}
  \pgfpathlineto{\pgfpointxy{2}{2}}
  \pgfusepath{stroke}
\end{tikzpicture}   
\end{codeexample}
\end{command}

\begin{command}{\pgfsetyvec\marg{point}}
  Works like |\pgfsetyvec|.
\end{command}



\begin{command}{\pgfpointpolarxy\marg{degree}{\ttfamily\char`\{}\meta{radius}\opt{|/|\meta{y-radius}}{\ttfamily\char`\}}}
  This command is similar to the |\pgfpointpolar| command, but the
  \meta{radius} is now a factor to be interpreted in the
  $xy$-coordinate system. This means that a degree of |0| is the same
  as the $x$-vector of the $xy$-coordinate  system times \meta{radius}
  and a degree of |90| is the $y$-vecotr times \meta{radius}. As for
  |\pgfpointpolar|, a \meta{radius} can also be a pair separated by a
  slash. In this case, the $x$- and $y$-vectors are multiplied by
  different factors.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \begin{scope}[x={(1cm,-5mm)},y=1.5cm]
    \foreach \angle in {0,10,...,90}
      {\pgfpathcircle{\pgfpointpolarxy{\angle}{1}}{2pt}}
    \pgfusepath{fill}
  \end{scope}
\end{tikzpicture}
\end{codeexample}
\end{command}



\subsection{Three Dimensional Coordinates}

It is also possible to specify a point as a multiple of three vectors,
the $x$-, $y$-, and $z$-vector. This is useful for creating simple
three dimensional graphics.

\begin{command}{\pgfpointxyz\marg{$s_x$}\marg{$s_y$}\marg{$s_z$}}
  Yields a point that is situated at $s_x$ times the
  $x$-vector plus $s_y$ times the $y$-vector plus  $s_z$ times the
  $z$-vector.
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetarrowsend{to}
  
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpointxyz{0}{0}{1}}
  \pgfusepath{stroke}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpointxyz{0}{1}{0}}
  \pgfusepath{stroke}
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpointxyz{1}{0}{0}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfsetzvec\marg{point}}
  Works like |\pgfsetzvec|.
\end{command}

Inside the $xyz$-coordinate system, you can also specify points
using spherical and cylindrical coordinates.


\begin{command}{\pgfpointcylindrical\marg{degree}\marg{radius}\marg{height}}
  This command yields the same as
\begin{verbatim}
\pgfpointadd{\pgfpointpolarxy{degree}{radius}}{\pgfpointxyz{0}{0}{height}}
\end{verbatim}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [->] (0,0) -- (1,0,0) node [right] {$x$};
  \draw [->] (0,0) -- (0,1,0) node [above] {$y$};
  \draw [->] (0,0) -- (0,0,1) node [below left] {$z$};

  \pgfpathcircle{\pgfpointcylindrical{80}{1}{.5}}{2pt}
  \pgfusepath{fill}

  \draw[red] (0,0) -- (0,0,.5) -- +(80:1);
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfpointspherical\marg{longitude}\marg{latitude}\marg{radius}}
  This command yields a point ``on the surface of the earth''
  specified by the \meta{longitude} and the \marg{latitude}. The
  radius of the earth is given by \meta{radius}. The equator lies in
  the $xy$-plane.
\begin{codeexample}[]
\begin{tikzpicture}
  \pgfsetfillcolor{lightgray}

  \foreach \latitude in {-90,-75,...,30}
  {  
    \foreach \longitude in {0,20,...,360}
    {
      \pgfpathmoveto{\pgfpointspherical{\longitude}{\latitude}{1}}
      \pgfpathlineto{\pgfpointspherical{\longitude+20}{\latitude}{1}}
      \pgfpathlineto{\pgfpointspherical{\longitude+20}{\latitude+15}{1}}
      \pgfpathlineto{\pgfpointspherical{\longitude}{\latitude+15}{1}}
      \pgfpathclose
    }
    \pgfusepath{fill,stroke}
  }
\end{tikzpicture}
\end{codeexample}
\end{command}



\subsection{Building Coordinates From Other Coordinates}

Many commands allow you to construct a coordinate in terms of other
coordinates.


\subsubsection{Basic Manipulations of Coordinates}

\begin{command}{\pgfpointadd\marg{$v_1$}\marg{$v_2$}}
  Returns the sum vector $\meta{$v_1$} + \meta{$v_2$}$.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathcircle{\pgfpointadd{\pgfpoint{1cm}{0cm}}{\pgfpoint{1cm}{1cm}}}{2pt}
  \pgfusepath{fill} 
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfpointscale\marg{factor}\marg{coordinate}}
  Returns the vector $\meta{factor}\meta{coordinate}$.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathcircle{\pgfpointscale{1.5}{\pgfpoint{1cm}{0cm}}}{2pt}
  \pgfusepath{fill} 
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfpointdiff\marg{start}\marg{end}}
  Returns the difference vector $\meta{end} - \meta{start}$.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathcircle{\pgfpointdiff{\pgfpoint{1cm}{0cm}}{\pgfpoint{1cm}{1cm}}}{2pt}
  \pgfusepath{fill} 
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgfpointnormalised\marg{point}}
  This command returns a normalized version of \meta{point}, that is,
  a vector of length 1pt pointing in the direction of \meta{point}. If
  \meta{point} is the $0$-vector or extremely short, a vector of
  length 1pt pointing upwards is returned.

  This command is \emph{not} implemented by calculating the length of
  the vector, but rather by calculating the angle of the vector and
  then using (something equivalent to) the |\pgfpointpolar|
  command. This ensures that the point will really have length 1pt,
  but it is not guaranteed that the vector will \emph{precisely} point
  in the direction of \meta{point} due to the fact that the polar
  tables are accurate only up to one degree. Normally, this is not a
  problem.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathcircle{\pgfpoint{2cm}{1cm}}{2pt}
  \pgfpathcircle{\pgfpointscale{20}
    {\pgfpointnormalised{\pgfpoint{2cm}{1cm}}}}{2pt}
  \pgfusepath{fill} 
\end{tikzpicture}
\end{codeexample}  
\end{command}


\subsubsection{Points Traveling along Lines and Curves}

\label{section-pointsattime}

The commands in this section allow you to specify points on a line or
a curve. Imaging a point ``traveling'' along a curve from some point
$p$ to another point $q$. At time $t=0$ the point is at $p$ and at
time $t=1$ it is at $q$ and at time, say, $t=1/2$ it is ``somewhere in
the middle.'' The exact location at time $t=1/2$ will not necessarily
be the ``halfway point,'' that is, the point whose distance on the
curve from $p$ and $q$ is equal. Rather, the exact location will
depend on the ``speed'' at which the point is traveling, which in
turn depends on the lengths of the support vectors in a complicated
manner. If you are interested in the details, please see a good book
on Bézier curves.



\begin{command}{\pgfpointlineattime\marg{time $t$}\marg{point $p$}\marg{point $q$}}
  Yields a point that is the $t$th fraction between $p$
  and~$q$, that is, $p + t(q-p)$. For $t=1/2$ this is the middle of
  $p$ and $q$.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{2cm}{2cm}}
  \pgfusepath{stroke}
  \foreach \t in {0,0.25,...,1.25}
    {\pgftext[at=
      \pgfpointlineattime{\t}{\pgfpointorigin}{\pgfpoint{2cm}{2cm}}]{\t}}
\end{tikzpicture}    
\end{codeexample}
\end{command}

\begin{command}{\pgfpointlineatdistance\marg{distance}\marg{start point}\marg{end point}}
  Yields a point that is located \meta{distance} many units removed
  from the start point in the direction of the end point. In other
  words, this is the point that results if we travel \meta{distance}
  steps from \meta{start point} towards \meta{end point}.
  \example
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathlineto{\pgfpoint{3cm}{2cm}}
  \pgfusepath{stroke}
  \foreach \d in {0pt,20pt,40pt,70pt}
    {\pgftext[at=
      \pgfpointlineatdistance{\d}{\pgfpointorigin}{\pgfpoint{3cm}{2cm}}]{\d}}
\end{tikzpicture}    
\end{codeexample}
\end{command}

\begin{command}{\pgfpointcurveattime\marg{time $t$}\marg{point
      $p$}\marg{point $s_1$}\marg{point $s_2$}\marg{point $q$}} 
  Yields a point that is on the Bézier curve from $p$ to $q$ with the
  support points $s_1$ and $s_2$. The time $t$ is used to determine
  the location, where $t=0$ yields $p$ and $t=1$ yields $q$.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathmoveto{\pgfpointorigin}
  \pgfpathcurveto
    {\pgfpoint{0cm}{2cm}}{\pgfpoint{0cm}{2cm}}{\pgfpoint{3cm}{2cm}}
  \pgfusepath{stroke}
  \foreach \t in {0,0.25,0.5,0.75,1}
    {\pgftext[at=\pgfpointcurveattime{\t}{\pgfpointorigin}
                                         {\pgfpoint{0cm}{2cm}}
                                         {\pgfpoint{0cm}{2cm}}
                                         {\pgfpoint{3cm}{2cm}}]{\t}}
\end{tikzpicture}    
\end{codeexample}
\end{command}

\subsubsection{Points on Borders of Objects}

The following commands are useful for specifying a point that lies on
the border of special shapes. They are used, for example, by the shape
mechanism to determine border points of shapes.

\begin{command}{\pgfpointborderrectangle\marg{direction point}\marg{corner}}
  This command returns a point that lies on the intersection of a line
  starting at the origin and going towards the point \meta{direction
    point} and a rectangle whose center is in the origin and whose
  upper right corner is at \meta{corner}.

  The \meta{direction point} should have length ``about 1pt,'' but it
  will be normalized automatically. Nevertheless, the ``nearer'' the
  length is to 1pt, the less rounding errors.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,1.5);
  \pgfpathrectanglecorners{\pgfpoint{-1cm}{-1.25cm}}{\pgfpoint{1cm}{1.25cm}}
  \pgfusepath{stroke}

  \pgfpathcircle{\pgfpoint{5pt}{5pt}}{2pt}
  \pgfpathcircle{\pgfpoint{-10pt}{5pt}}{2pt}
  \pgfusepath{fill}
  \color{red}
  \pgfpathcircle{\pgfpointborderrectangle
    {\pgfpoint{5pt}{5pt}}{\pgfpoint{1cm}{1.25cm}}}{2pt}
  \pgfpathcircle{\pgfpointborderrectangle
    {\pgfpoint{-10pt}{5pt}}{\pgfpoint{1cm}{1.25cm}}}{2pt}
  \pgfusepath{fill}
\end{tikzpicture}    
\end{codeexample}
\end{command}


\begin{command}{\pgfpointborderellipse\marg{direction point}\marg{corner}}
  This command works like the corresponding command for rectangles,
  only this time the \meta{corner} is the corner of the bounding
  rectangle of an ellipse.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,1.5);
  \pgfpathellipse{\pgfpointorigin}{\pgfpoint{1cm}{0cm}}{\pgfpoint{0cm}{1.25cm}}
  \pgfusepath{stroke}

  \pgfpathcircle{\pgfpoint{5pt}{5pt}}{2pt}
  \pgfpathcircle{\pgfpoint{-10pt}{5pt}}{2pt}
  \pgfusepath{fill}
  \color{red}
  \pgfpathcircle{\pgfpointborderellipse
    {\pgfpoint{5pt}{5pt}}{\pgfpoint{1cm}{1.25cm}}}{2pt}
  \pgfpathcircle{\pgfpointborderellipse
    {\pgfpoint{-10pt}{5pt}}{\pgfpoint{1cm}{1.25cm}}}{2pt}
  \pgfusepath{fill}
\end{tikzpicture}    
\end{codeexample}
\end{command}


\subsubsection{Points on the Intersection of Lines}


\begin{command}{\pgfpointintersectionoflines\marg{$p$}\marg{$q$}\marg{$s$}\marg{$t$}}
  This command returns the intersection of a line going through $p$
  and $q$ and a line going through $s$ and $t$. If the lines do not
  intersection, an arithmetic overflow will occur.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,2);
  \draw (.5,0) -- (2,2);
  \draw (1,2) -- (2,0);
  \pgfpathcircle{%
    \pgfpointintersectionoflines
      {\pgfpointxy{.5}{0}}{\pgfpointxy{2}{2}}
      {\pgfpointxy{1}{2}}{\pgfpointxy{2}{0}}}
    {2pt}
  \pgfusepath{stroke}
\end{tikzpicture}    
\end{codeexample}
\end{command}


\subsubsection{Points on the Intersection of Two Circles}


\begin{command}{\pgfpointintersectionofcircles\marg{$p_1$}\marg{$p_2$}\marg{$r_1$}\marg{$r_2$}\marg{solution}}
  This command returns the intersection of the two circles centered at
  $p_1$ and $p_2$ with radii $r_1$ and $r_2$. If \meta{solution} is
  |1|, the first intersection is returned, otherwise the second one is
  returned.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,2);
  \draw (0.5,0) circle (1);
  \draw (1.5,1) circle (.8);
  \pgfpathcircle{%
    \pgfpointintersectionofcircles
      {\pgfpointxy{.5}{0}}{\pgfpointxy{1.5}{1}}
      {1cm}{0.8cm}{1}}
    {2pt}
  \pgfusepath{stroke}
\end{tikzpicture}    
\end{codeexample}
\end{command}


\subsection{Extracting Coordinates}

There are two commands that can be used to ``extract'' the $x$- or
$y$-coordinate of a coordinate. 

\begin{command}{\pgfextractx\marg{dimension}\marg{point}}
  Sets the \TeX-\meta{dimension} to the $x$-coordinate of the point.

\begin{codeexample}[code only]
\newdimen\mydim
\pgfextractx{\mydim}{\pgfpoint{2cm}{4pt}}
%% \mydim is now 2cm
\end{codeexample}
\end{command}

\begin{command}{\pgfextracty\marg{dimension}\marg{point}}
  Like |\pgfextractx|, except for the $y$-coordinate.
\end{command}




\subsection{Internals of How Point Commands Work}

As a normal user of \pgfname\ you do not need to read this section. It
is relevant only if you need to understand how the point commands work
internally. 

When a command like |\pgfpoint{1cm}{2pt}| is called, all that happens
is that the two \TeX-dimension variables |\pgf@x| and |\pgf@y| are set
to |1cm| and |2pt|, respectively. A command like |\pgfpathmoveto| that
takes a coordinate as parameter will just execute this parameter and
then use the values of |\pgf@x| and |\pgf@y| as the coordinates to
which it will move the pen on the current path.

since commands like |\pgfpointnormalised| modify other variables
besides |\pgf@x| and |\pgf@y| during the computation of the final values of
|\pgf@x| and |\pgf@y|, it is a good idea to enclose a call of a
command like |\pgfpoint| in a \TeX-scope and then make the changes of
|\pgf@x| and |\pgf@y| global as in the following example:
\begin{codeexample}[code only]
...
{ % open scope
  \pgfpointnormalised{\pgfpoint{1cm}{1cm}}
  \global\pgf@x=\pgf@x % make the change of \pgf@x persist past the scope
  \global\pgf@y=\pgf@y % make the change of \pgf@y persist past the scope
}
% \pgf@x and \pgf@y are now set correctly, all other variables are
% unchanged 
\end{codeexample}

\makeatletter
Since this situation arises very often, the macro |\pgf@process| can
be used to perform the above code:
\begin{command}{\pgf@process\marg{code}}
  Executes the \meta{code} in a scope and then makes |\pgf@x| and
  |\pgf@y| global.
\end{command}

Note that this macro is used often internally. For this reason, it is
not a good idea to keep anything important in the variables |\pgf@x|
and |\pgf@y| since they will be overwritten and changed
frequently. Instead, intermediate values can ge stored in the
\TeX-dimensions |\pgf@xa|, |\pgf@xb|, |\pgf@xc| and their
|y|-counterparts |\pgf@ya|, |\pgf@yb|, |pgf@yc|. For example, here is
the code of the command |\pgfpointadd|:
\begin{codeexample}[code only]
\def\pgfpointadd#1#2{%
  \pgf@process{#1}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{#2}%
  \advance\pgf@x by\pgf@xa%
  \advance\pgf@y by\pgf@ya}
\end{codeexample}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-quick.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Quick Commands}

This section explains the ``quick'' commands of \pgfname. These
commands are executed more quickly than the normal commands of
\pgfname, but offer less functionality. You should use these commands
only if you either have a very large number of commands that need to
be processed or if you expect your commands to be executed very often.


\subsection{Quick Coordiante Commands}

\begin{command}{\pgfqpoint\marg{x}\marg{y}}
  This command does the same as |\pgfpoint|, but \meta{x} and \meta{y}
  must be simple dimensions like |1pt| or |1cm|. Things like |2ex| or
  |2cm+1pt| are not allowed.
\end{command}

\subsection{Quick Path Construction Commands}

The difference between the quick and the normal path commands is that
the quick path commands
\begin{itemize}
\item
  do not keep track of the bounding boxes,
\item
  do not allow you to arc corners,
\item
  do not apply coordinate transformations.
\end{itemize}

However, they do use the soft-path subsystem (see
Section~\ref{section-soft-paths} for details), which allows you to mix
quick and normal path commands arbitrarily.

All quick path construction commands start with |\pgfpathq|.

\begin{command}{\pgfpathqmoveto\marg{x dimension}\marg{y dimension}}
  Either starts a path or starts a new part of a path at the coordinate
  $(\meta{x dimension},\meta{y dimension})$. The coordinate is
  \emph{not} transformed by the current coordinate transformation
  matrix. However, any low-level transformations apply.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgftransformxshift{1cm}
  \pgfpathqmoveto{0pt}{0pt} % not transformed
  \pgfpathqlineto{1cm}{1cm} % not transformed
  \pgfpathlineto{\pgfpoint{2cm}{0cm}}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfpathqlineto\marg{x dimension}\marg{y dimension}}
  The quick version of the line-to operation.
\end{command}

\begin{command}{\pgfpathqcurveto\marg{$s^1_x$}\marg{$s^1_y$}\marg{$s^2_x$}\marg{$s^2_y$}\marg{$t_x$}\marg{$t_y$}}
  The quick version of the curve-to operation. The first support point
  is $(s^1_x,s^1_y)$, the second support point is  $(s^2_x,s^2_y)$,
  and the target is $(t_x,t_y)$.
 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfpathqmoveto{0pt}{0pt}
  \pgfpathqcurveto{1cm}{1cm}{2cm}{1cm}{3cm}{0cm}
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfpathqcircle\marg{radius}}
  Adds a radius around the origin of the given \meta{radius}. This
  command is orders of magnitude faster than
  |\pgfcircle{\pgfpointorigin}{|\meta{radius}|}|. 
 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (1,1);
  \pgfpathqcircle{10pt}
  \pgfsetfillcolor{examplefill}
  \pgfusepath{stroke,fill}
\end{tikzpicture}
\end{codeexample}
\end{command}



\subsection{Quick Path Usage Commands}

The quick path usage commands perform similar tasks as |\pgfusepath|,
but they
\begin{itemize}
\item
  do not add arrows,
\item
  do not modify the path in any way, in particular,
\item
  ends are not shortened,
\item
  corners are not replaced by arcs.
\end{itemize}

Note that you \emph{have to} use the quick versions in the code of
arrow tip definitions since, inside these definition, you obviously do
not want arrows to be drawn.

\begin{command}{\pgfusepathqstroke}
  Strokes the path without further ado. No arrows are drawn, no
  corners are arced.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathqcircle{5pt}
  \pgfusepathqstroke
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfusepathqfill}
  Fills the path without further ado.
\end{command}

\begin{command}{\pgfusepathqfillstroke}
  Fills and then strokes the path without further ado.
\end{command}

\begin{command}{\pgfusepathqclip}
  Clips all subsequent drawings against the current path. The path is
  not processed.
\end{command}


\subsection{Quick Text Box Commands}

\begin{command}{\pgfqbox\marg{box number}}
  This command inserts a \TeX\ box into a |{pgfpicture}| by
  ``escaping'' to \TeX, inserting the box number \meta{box number} at
  the origin, and then returning to the typesetting the picture.
\end{command}

\begin{command}{\pgfqboxsynced\marg{box number}}
  This command works similarly to the |\pgfqbox| command. However,
  before inserting the text in \meta{box number}, the current
  coordinate transformation matrix is applied to the current canvas
  transformation matrix (is it ``synced'' with this matrix, hence the
  name).

  Thus, this command basically has the same effect as if you first
  called |\pgflowlevelsynccm| followed by |\pgfqbox|. However, this
  command will use |\hskip| and |\raise| commands for the
  ``translational part'' of the coordinate transformation matrix,
  instead of adding the translational part to the current
  canvas transformation matrix directly. Both methods have the same
  effect (box \meta{box number} is translated where it should), but
  the method used by |\pgfqboxsynced| ensures that hyperlinks are
  placed correctly. Note that scaling and rotation will not (cannot,
  even) apply to hyperlinks.
\end{command}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-scopes.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section[Hierarchical Structures: Package, Environments, Scopes, and Text]
{Hierarchical Structures:\\
  Package, Environments, Scopes, and Text}


\subsection{Overview}

\pgfname\ uses two kinds of hierarchical structuring: First, the
package itself is structured hierarchically, consisting of different
packages that are built on top of each other. Second, \pgfname\ allows you
to structure your graphics hierarchically using environments and scopes.

\subsubsection{The  Hierarchical Structure of the Package}

The \pgfname\ system consists of several layers:

\begin{description}
\item[System layer.]
  The lowest layer is called the \emph{system layer}, though it might
  also be called ``driver layer'' or perhaps ``backend layer.'' Its
  job is to provide an abstraction of the details of which driver
  is used to transform the |.dvi| file. The system layer is
  implemented by the package |pgfsys|, which will load appropriate
  driver files as needed.

  The system layer is documented in Part~\ref{part-system}.
\item[Basic layer.]
  The basic layer is loaded by the package |pgfcore| and subsequent
  use of the command |\usepgfmodule| to load additional modules of the
  basic layer.

  The basic layer is documented in the present part.
\item[Frontend layer.]
  The frontend layer is not loaded by a single packages. Rather,
  different packages, like \tikzname\ or \textsc{pgfpict2e}, are
  different frontends to the basic layer.

  The \tikzname\ frontend is documented in Part~\ref{part-tikz}.
\end{description}

Each layer will automatically load the necessary files of the layers below
it. 

In addition to the packages of these layers, there are also some
library packages. These packages provide additional definitions of
things like new arrow tips or new plot handlers.

The library packages are documented in Part~\ref{part-libraries}.




\subsubsection{The Hierarchical Structure of Graphics}

Graphics in \pgfname\ are typically structured
hierarchically. Hierarchical structuring can be used to identify
groups of graphical elements that are to be treated ``in the same
way.'' For example, you might group together a number of paths, all of
which are to be drawn in red. Then, when you decide later on that you
like them to be drawn in, say, blue, all you have to do is to change
the color once.

The general mechanism underlying hierarchical structuring is known as
\emph{scoping} in computer science. The idea is that all changes to
the general ``state'' of the graphic that are done inside a scope are
local to that scope. So, if you change the color inside a scope, this
does not affect the color used outside the scope. Likewise, when you
change the line width in a scope, the line width outside is not
changed, and so on.

There are different ways of starting and ending scopes of graphic
parameters. Unfortunately, these scopes are sometimes ``in conflict''
with each other and it is sometimes not immediately clear which scopes
apply. In essence, the following scoping mechanisms are available:

\begin{enumerate}
\item
  The ``outermost'' scope supported by \pgfname\ is the |{pgfpicture}|
  environment. All changes to the graphic state done inside a
  |{pgfpicture}| are local to that picture.

  In general, it is \emph{not} possible to set graphic parameters
  globally outside any |{pgfpicture}| environments. Thus, you can
  \emph{not} say |\pgfsetlinewidth{1pt}| at the beginning of your
  document to have a default line width of one point. Rather, you have
  to (re)set all graphic parameters inside each |{pgfpicture}|. (If
  this is too bothersome, try defining some macro that does the job
  for you.)
\item
  Inside a |{pgfpicture}| you can use a |{pgfscope}| environment to
  keep changes of the graphic state local to that environment.

  The effect of commands that change the graphic state are local to
  the current |{pgfscope}| but not always to the current \TeX\
  group. Thus, if you open a \TeX\ group (some text in curly braces)
  inside a |{pgfscope}|, and if you change, for example, the dash
  pattern, the effect of this changed dash pattern will persist till
  the end of the |{pgfscope}|.

  Unfortunately, this is not always the case. \emph{Some} graphic
  parameters only persist till the end of the current \TeX\ group. For
  example, when you use |\pgfsetarrows| to set the arrow tip 
  inside a \TeX\ group, the effect lasts only till the end of the
  current \TeX\ group.
\item
  Some graphic parameters are not scoped by |{pgfscope}| but
  ``already'' by \TeX\ groups. For example, the effect of coordinate
  transformation commands is always local to the current \TeX\
  group.

  Since every |{pgfscope}| automatically creates a \TeX\ group, all
  graphic parameters that are local to the current \TeX\ group are
  also local to the current |{pgfscope}|.
\item
  Some graphic parameters can only be scoped using \TeX\ groups, since
  in some situations it is not possible to introduce a
  |{pgfscope}|. For example, a path always has to be completely
  constructed and used in the same |{pgfscope}|. However, we might
  wish to have different coordinate transformations apply to different
  points on the path. In this case, we can use \TeX\ groups to keep
  the effect local, but we could not use |{pgfscope}|.  
\item
  The |\pgftext| command can be used to create a scope in which \TeX\
  ``escapes back'' to normal \TeX\ mode. The text passed to the
  |\pgftext| is ``heavily guarded'' against having any effect on the
  scope in which it is used. For example, it is possibly to use
  another  |{pgfpicture}| environment inside the argument of
  |\pgftext|. 
\end{enumerate}


Most of the complications can be avoided if you stick to the following
rules:

\begin{itemize}
\item
  Give graphic commands only inside |{pgfpicture}| environments.
\item
  Use |{pgfscope}| to structure graphics.
\item
  Do not use \TeX\ groups inside graphics, \emph{except} for keeping
  the effect of coordinate transformations local.
\end{itemize}



\subsection{The Hierarchical Structure of the Package}

Before we come to the structuring commands provided by \pgfname\ to
structure your graphics, let us first have a look at the structure of
the package itself.

\subsubsection{The Core Package}

To use \pgfname, include the following package:

\begin{package}{pgfcore}
  This package loads the complete core of the ``basic layer'' of
  \pgfname, but not any modules. That is, it will load all of the
  commands described in the current part of this manual, but it will
  not load frontends like \tikzname. It will also load the system
  layer. To load additional modules, use the |\usepgfmodule| command 
  explained below.
\end{package}

The following package is just a convenience.

\begin{package}{pgf}
  This package loads the |pgfcore| and the two modules |shapes| and
  |plot|. 

  In \LaTeX, the package takes two options:
  \begin{packageoption}{draft}
    When this option is set, all images will be replaced by empty
    rectangles. This can speedup compilation.
  \end{packageoption}
  
  \begin{packageoption}{version=\meta{version}}
    Indicates that the commands of version \meta{version} need to be
    defined. If you set \meta{version} to |0.65|, then a large bunch of
    ``compatibility commands'' are loaded. If you set \meta{version} to
    |0.96|, then these compatibility commands will not be loaded.
    
    If this option is not given at all, then the commands of all
    versions are defined.
  \end{packageoption}
\end{package}



\subsubsection{The Modules}

\begin{command}{\usepgflibrary\marg{module names}}
  Once the core has been loaded, you can use this command to load
  further modules. The modules in the \meta{module names} list should
  be separated by commas. Instead of curly braces, you can also
  use square brackets, which is something Con\TeX t users will
  like. If you try to load a module a second time, nothing will
  happen. 

  \example |\usepgfmodule{matrix,shapes}|

  What this command does is to load the file
  |pgfmodule|\meta{module}|.code.tex| for each \meta{module} in
  the \meta{module names}. Thus, to write your own module,
  all you need to do is to place a file of the appropriate name
  somewhere where \TeX\ can find it. \LaTeX, plain \TeX, and Con\TeX t
  users can then use your library.
\end{command}

The following modules are available for use with |pgfcore|:

\begin{itemize}
\item The |plot| module provides commands for plotting functions.  The
  commands are explained in Section~\ref{section-plots}.
\item The |shapes| module provides commands for drawing shapes and
  nodes. These commands are explained in
  Section~\ref{section-shapes}. 
\item The |decorations| module provides commands for adding
  decorations to paths. These commands are explained in
  Section~\ref{section-base-decorations}. 
\item The |matrix| module provides the |\pgfmatrix| command. The
  commands are documented in Section~\ref{section-base-matrices}.  
\end{itemize}



\subsubsection{The Library Packages}

There is a special command for loading library packages. The
difference between a library and module is the following: A library
just defines additional objects using the basic layer, whereas a
module adds completely new functionality. For instance, a decoration
library defines additional decorations, while a decoration module
defines the whole code for handling decorations.

\begin{command}{\usepgflibrary\marg{list of libraries}}
  Use this command to load further libraries. The list of libraries
  should contain the names of libraries separated by commas. Instead
  of curly braces, you can also use square brackets. If you try to
  load a library a second time, nothing will happen. 

  \example |\usepgflibrary{arrows}|

  This command causes the the file
  |pgflibrary|\meta{library}|.code.tex| to be loaded for each \meta{library} in
  the \meta{list of libraries}. This means that in order to write your
  own library file, place a file of the appropriate name somewhere
  where \TeX\ can find it. \LaTeX, plain \TeX, and Con\TeX t 
  users can then use your library.

  You should also consider adding a \tikzname\ library that simply
  includes your \pgfname\ library.
\end{command}



\subsection{The Hierarchical Structure of the Graphics}

\subsubsection{The Main Environment}


Most, but not all, commands of the \pgfname\ package must be given
within a |{pgfpicture}| environment. The only commands that (must) be
given outside are commands having to do with including images (like
|\pgfuseimage|) and with inserting complete shadings (like
|\pgfuseshading|). However, just to keep life entertaining, the
|\pgfshadepath| command must be given \emph{inside} a |{pgfpicture}|
environment.

\begin{environment}{{pgfpicture}}
  This environment will insert a \TeX\ box containing the graphic drawn by
  the \meta{environment contents} at the current position. 

  \medskip
  \textbf{The size of the bounding box.}
  The size of the box is determined in the following
  manner: While \pgfname\ parses the \meta{environment contents}, it
  keeps track of a bounding box for the graphic. Essentially, this
  bounding box is the smallest box that contains all coordinates
  mentioned in the graphics. Some coordinates may be ``mentioned'' by
  \pgfname\ itself; for example, when you add circle to the current
  path, the support points of the curve making up the circle are also
  ``mentioned'' despite the fact that you will not ``see'' them in
  your code.

  Once the \meta{environment contents} has been parsed completely, a
  \TeX\ box is created whose size is the size of the computed bounding
  box and this box is inserted at the current position.

\begin{codeexample}[]
Hello \begin{pgfpicture}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{2ex}{1ex}}
  \pgfusepath{stroke}
\end{pgfpicture} World!
\end{codeexample}

  Sometimes, you may need more fine-grained control over the size of
  the bounding box. For example, the computed bounding box may be too
  large or you intensionally wish the box to be ``too small.'' In
  these cases, you can use the command
  |\pgfusepath{use as bounding box}|, as described in
  Section~\ref{section-using-bb}.


  \medskip
  \textbf{The baseline of the bounding box.}
  When the box containing the graphic is inserted into the normal
  text, the baseline of the graphic is normally at the bottom of the
  graphic. For this reason, the following two sets of code lines have
  the same effect, despite the fact that the second graphic uses
  ``higher'' coordinates than the first:
 
\begin{codeexample}[]
Rectangles \begin{pgfpicture}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{2ex}{1ex}}
  \pgfusepath{stroke}
\end{pgfpicture} and \begin{pgfpicture}
  \pgfpathrectangle{\pgfpoint{0ex}{1ex}}{\pgfpoint{2ex}{1ex}}
  \pgfusepath{stroke}
\end{pgfpicture}.
\end{codeexample}

  You can change the baseline using the |\pgfsetbaseline| command, see
  below. 

\begin{codeexample}[]
Rectangles \begin{pgfpicture}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{2ex}{1ex}}
  \pgfusepath{stroke}
  \pgfsetbaseline{0pt}
\end{pgfpicture} and \begin{pgfpicture}
  \pgfpathrectangle{\pgfpoint{0ex}{1ex}}{\pgfpoint{2ex}{1ex}}
  \pgfusepath{stroke}
  \pgfsetbaseline{0pt}
\end{pgfpicture}.
\end{codeexample}

  \medskip
  \textbf{Including text and images in a picture.}
  You cannot directly include text and images in a picture. Thus, you
  should \emph{not} simply write some text in a |{pgfpicture}| or use
  a command like |\includegraphics| or even |\pgfimage|. In all these
  cases, you need to place the text inside a |\pgftext| command. This
  will ``escape back'' to normal \TeX\ mode, see
  Section~\ref{section-text-command} for details.

  \medskip
  \textbf{Remembering a picture position for later reference.}
  After a picture has been typset, its position on the page is
  normally forgotten by \pgfname\ and also by \TeX. This means that is
  not possible to reference a node in this picture later on. In
  particular, it is normally impossible to draw lines between nodes in
  different pictures automatically.

  In order to make \pgfname\ ``remember'' a picture, the \TeX-if
  |\||ifpgfrememberpicturepositiononpage| should be set to |true|. It
  is only important that this \TeX-if is |true| at the end of the
  |{pgfpicture}|-environment, so you can switch it on inside the
  environment. However, you can also just switch it on globally, then
  the positions of all pictures are remembered.

  There are several reasons why the remembering is not switched on by
  default. First, it does not work for all backend drivers (currently, it
  works only for pdf\TeX). Second, it requires two passes of \TeX\
  over the file; on the first pass all positions will be wrong. Third,
  for every remembered picture a line is added to the |.aux|-file,
  which may result in a large number of extra lines.

  Despite all these ``problems,'' for documents that are processed
  with pdf\TeX\ and in which there is only a small number of pictures
  (less than a hundred or so), you can switch on this option globally,
  it will not cause any significant slowing of \TeX.
\end{environment}

\begin{plainenvironment}{{pgfpicture}}
  The plain \TeX\ version of the environment. Note that in this
  version, also, a \TeX\ group is created around the environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgfpicture}}
  This is the Con\TeX t version of the environment.
\end{contextenvironment}


{\let\ifpgfrememberpicturepositiononpage=\relax
\begin{command}{\ifpgfrememberpicturepositiononpage}
  Determines whether the position of pictures on the page should be
  recorded. The value of this \TeX-if at the end of a |{pgfpicture}|
  environment is important, not the value at the beginning.

  If this option is set to true of a picture, \pgfname\ will attempt
  to record the position of the picture on the page. (This attempt
  will fail with most drivers and when it works it typically requires
  two runs of \TeX.) The position is not directly accessible. Rather,
  the nodes mechanism will use this position if you access a node from
  another picture. See Sections~\ref{section-cross-pictures-pgf}
  and~\ref{section-cross-picture-tikz} for more details. 
\end{command}
}


\makeatletter
\begin{command}{\pgfsetbaseline\marg{dimension}}
  This command specifies a $y$-coordinate of the picture that should
  be used as the baseline of the whole picture. When a \pgfname\
  picture has been typeset completely, \pgfname\ must decide at which
  height the baseline of the picture should lie. Normally, the
  baseline is set to the $y$-coordinate of the bottom of the picture,
  but it is often desirable to use another height.

\begin{codeexample}[]
Text \tikz{\pgfpathcircle{\pgfpointorigin}{1ex}\pgfusepath{stroke}},
     \tikz{\pgfsetbaseline{0pt}
          \pgfpathcircle{\pgfpointorigin}{1ex}\pgfusepath{stroke}},
     \tikz{\pgfsetbaseline{.5ex}
          \pgfpathcircle{\pgfpointorigin}{1ex}\pgfusepath{stroke}},
     \tikz{\pgfsetbaseline{-1ex}
          \pgfpathcircle{\pgfpointorigin}{1ex}\pgfusepath{stroke}}.
\end{codeexample}
\end{command}

\begin{command}{\pgfsetbaselinepointnow\marg{point}}
  This command specifies the baseline indirectly, namely as the
  $y$-coordinate that the given \meta{point} has when the command is
  called.
\end{command}

\begin{command}{\pgfsetbaselinepointlater\marg{point}}
  This command also specifies the baseline indirectly, but the
  $y$-coordinate of the given \meta{point} is only computed at the end
  of the picture.

\begin{codeexample}[]
Hello
\tikz{
  \pgfsetbaselinepointlater{\pgfpointanchor{X}{base}}
  % Note: no shape X, yet
  \node [cross out,draw] (X) {world.};
}
\end{codeexample}
\end{command}



\subsubsection{Graphic Scope Environments}

Inside a |{pgfpicture}| environment you can substructure your picture
using the following environment:

\begin{environment}{{pgfscope}}
  All changes to the graphic state done inside this environment are
  local to the environment. The graphic state includes the following:
  \begin{itemize}
  \item
    The line width.
  \item
    The stroke and fill colors.
  \item
    The dash pattern.
  \item
    The line join and cap.
  \item
    The miter limit.
  \item
    The canvas transformation matrix.
  \item
    The clipping path.
  \end{itemize}
  Other parameters may also influence how graphics are rendered, but they
  are \emph{not} part of the graphic state. For example, the arrow tip
  kind is not part of the graphic state and the effect of commands
  setting the arrow tip kind are local to the current \TeX\ group, not
  to the current |{pgfscope}|. However, since |{pgfscope}| starts and
  ends a \TeX\ group automatically, a |{pgfscope}| can be used to
  limit the effect of, say, commands that set the arrow tip kind.

\begin{codeexample}[]
\begin{pgfpicture}
  \begin{pgfscope}
    {
      \pgfsetlinewidth{2pt}
      \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{2ex}{2ex}}
      \pgfusepath{stroke}
    }
    \pgfpathrectangle{\pgfpoint{3ex}{0ex}}{\pgfpoint{2ex}{2ex}}
    \pgfusepath{stroke}
  \end{pgfscope}
  \pgfpathrectangle{\pgfpoint{6ex}{0ex}}{\pgfpoint{2ex}{2ex}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
  
\begin{codeexample}[]
\begin{pgfpicture}
  \begin{pgfscope}
    {
      \pgfsetarrows{-to}
      \pgfpathmoveto{\pgfpointorigin}\pgfpathlineto{\pgfpoint{2ex}{2ex}}
      \pgfusepath{stroke}
    }
    \pgfpathmoveto{\pgfpoint{3ex}{0ex}}\pgfpathlineto{\pgfpoint{5ex}{2ex}}
    \pgfusepath{stroke}
  \end{pgfscope}
  \pgfpathmoveto{\pgfpoint{6ex}{0ex}}\pgfpathlineto{\pgfpoint{8ex}{2ex}}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}

  At the start of the scope, the current path must be empty, that is,
  you cannot open a scope while constructing a path.

  It is usually a good idea \emph{not} to introduce \TeX\ groups
  inside a |{pgfscope}| environment.
\end{environment}

\begin{plainenvironment}{{pgfscope}}
  Plain \TeX\ version of the |{pgfscope}| environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgfscope}}
  This is the Con\TeX t version of the environment.
\end{contextenvironment}


The following scopes also encapsulate certain properties of the
graphic state. However, they are typically not used directly by the
user.

\begin{environment}{{pgfinterruptpath}}
  This environment can be used to temporarily interrupt the
  construction of the current path. The effect will be that the path
  currently under construction will be ``stored away'' and restored at
  the end of the environment. Inside the environment you can construct
  a new path and do something with it.

  An example application of this environment is the arrow tip
  caching. Suppose you ask \pgfname\ to use a specific arrow tip
  kind. When the arrow tip needs to be rendered for the first time,
  \pgfname\ will ``cache'' the path that makes up the arrow tip. To do
  so, it interrupts the current path construction and then protocols
  the path of the arrow tip. The |{pgfinterruptpath}| environment is
  used to ensure that this does not interfere with the path to which
  the arrow tips should be attached.

  This command does \emph{not} install a |{pgfscope}|. In particular,
  it does not call any |\pgfsys@| commands at all, which would,
  indeed, be dangerous in the middle of a path construction.
\end{environment}

\begin{plainenvironment}{{pgfinterruptpath}}
  Plain \TeX\ version of the environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgfinterruptpath}}
  Con\TeX t version of the environment.
\end{contextenvironment}


\begin{environment}{{pgfinterruptpicture}}
  This environment can be used to temporarily interrupt a
  |{pgfpicture}|. However, the environment is intended only to be used
  at the beginning and end of a box that is (later) inserted into a
  |{pgfpicture}| using |\pgfqbox|. You cannot use this environment
  directly inside a |{pgfpicture}|.

\begin{codeexample}[]
\begin{pgfpicture}
  \pgfpathmoveto{\pgfpoint{0cm}{0cm}} % In the middle of path, now
  \newbox\mybox
  \setbox\mybox=\hbox{
    \begin{pgfinterruptpicture}
      Sub-\begin{pgfpicture} % a subpicture
        \pgfpathmoveto{\pgfpoint{1cm}{0cm}}
        \pgfpathlineto{\pgfpoint{1cm}{1cm}}
        \pgfusepath{stroke}
      \end{pgfpicture}-picture.
    \end{pgfinterruptpicture}
  }
  \pgfqbox{\mybox}%
  \pgfpathlineto{\pgfpoint{0cm}{1cm}}
  \pgfusepath{stroke}
\end{pgfpicture}\hskip3.9cm
\end{codeexample}
\end{environment}

\begin{plainenvironment}{{pgfinterruptpicture}}
  Plain \TeX\ version of the environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgfinterruptpicture}}
  Con\TeX t version of the environment.
\end{contextenvironment}



\begin{environment}{{pgfinterruptboundingbox}}
  This environment temporarily interrupts the computation of the
  bounding box and sets up a new bounding box. At the beginning of the
  environment the old bounding box is saved and an empty bounding box
  is installed. After the environment the orginal bounding box is
  reinstalled as if nothing has happened.
\end{environment}

\begin{plainenvironment}{{pgfinterruptboundingbox}}
  Plain \TeX\ version of the environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgfinterruptboundingbox}}
  Con\TeX t version of the environment.
\end{contextenvironment}


\subsubsection{Inserting Text and Images}

\label{section-text-command}

Often, you may wish to add normal \TeX\ text at a certain point inside
a |{pgfpicture}|. You cannot do so ``directly,'' that is, you cannot
simply write this text inside the |{pgfpicture}| environment. Rather,
you must pass the text as an argument to the |\pgftext| command.

You must \emph{also} use the |\pgftext| command to insert an image or
a shading into a |{pgfpicture}|.

\begin{command}{\pgftext\opt{\oarg{options}}\marg{text}}
  This command will typeset \meta{text} in normal \TeX\ mode and
  insert the resulting box into the |{pgfpicture}|. The bounding box
  of the graphic will be updated so that all of the text box is
  inside. Be default, the text box is centered at the origin, but this
  can be changed either by giving appropriate \meta{options} or by
  applying an appropriate coordinate transformation beforehand.

  The \meta{text} may contain verbatim text. (In other words, the
  \meta{text} ``argument'' is not a normal argument, but is put in a
  box and some |\aftergroup| hackery is used to find the end of the
  box.)

  \pgfname's current (high-level) coordinate transformation is
  synchronized with the canvas transformation matrix temporarily
  when the text box is inserted. The effect is that if there is
  currently a high-level rotation of, say, 30 degrees, the \meta{text}
  will also be rotated by thirty degrees. If you do not want this
  effect, you have to (possibly temporarily) reset the high-level
  transformation matrix.

  The \meta{options} keys are used with the path |/pgf/text/|. The
  following keys are defined for this path:
  \begin{key}{/pgf/text/left}
    The key causes the text box to be placed such that its left
    border is on the origin. 
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[left] {lovely}}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/text/right}
    Thie key causes the text box to be placed such that its right
    border is on the origin. 
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[right] {lovely}}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/text/right}
    This key causes the text box to be placed such that its top is on the
    origin. This option can be used together with the |left| or
    |right| option.
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[top] {lovely}}
\end{codeexample}
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[top,right] {lovely}}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/text/bottom}
    This key causes the text box to be placed such that its bottom is
    on the origin.
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[bottom] {lovely}}
\end{codeexample}
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[bottom,right] {lovely}}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/text/base}
    This key causes the text box to be placed such that its baseline
    is on the origin.
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[base] {lovely}}
\end{codeexample}
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[base,right] {lovely}}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/text/at=\meta{point}}
    Translates the origin (that is, the point where the text is
    shown) to \meta{point}. 
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[base,at={\pgfpoint{1cm}{0cm}}] {lovely}}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/text/x=\meta{dimension}}
    Translates the origin by \meta{dimension} along the $x$-axis.
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[base,x=1cm,y=-0.5cm] {lovely}}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/text/y=\meta{dimension}}
    This key works like the |x| option.
  \end{key}
  \begin{key}{/pgf/text/rotate=\meta{degree}}
    Rotates the coordinate system by \meta{degree}. This will also
    rotate the text box.
\begin{codeexample}[]
\tikz{\draw[help lines] (-1,-.5) grid (1,.5);
     \pgftext[base,x=1cm,y=-0.5cm,rotate=30] {lovely}}
\end{codeexample}
\end{key}
  
\end{command}




==> pgfmanual-en-base-shadings.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Shadings}

\label{section-shadings}

\subsection{Overview}

A shading is an area in which the color changes smoothly between different
colors. Similarly to an image, a shading must first be declared before
it can be used. Also similarly to an image, a shading is put into a
\TeX-box. Hence, in order to include a shading in a |{pgfpicture}|,
you have to use |\pgftext| around it.

There are different kinds of shadings: horizontal, vertical, radial,
and functional shadings. However, you can rotate and clip shadings
like any other graphics object, which allows you to create more
complicated shadings. Horizontal shadings could be created by rotating
a vertical shading by 90 degrees, but explicit commands for creating both
horizontal and vertical shadings are included for convenience.

Once you have declared a shading, you can insert it into text using
the command |\pgfuseshading|. This command cannot be used directly in
a |{pgfpicture}|, you have to put a |\pgftext| around it. The second
command for using shadings, |\pgfshadepath|, on the other hand, can
only be used  inside |{pgfpicture}| environments. It will ``fill'' the
current path with the shading.

A horizontal shading is a horizontal bar of a certain height whose
color changes smoothly. You must at least specify the colors at the
left and at the right end of the bar, but you can also add color
specifications for points in between. For example, suppose you
which to create a bar that is red at the left end, green in the
middle, and blue at the end. Suppose you would like the bar to be 4cm
long. This could be specified as follows:
\begin{codeexample}[code only]
rgb(0cm)=(1,0,0); rgb(2cm)=(0,1,0); rgb(4cm)=(0,0,1)
\end{codeexample}
This line means that at 0cm (the left end) of the bar, the color
should be red, which has red-green-blue (rgb) components (1,0,0). At
2cm, the bar should be green, and at 4cm it should be blue.
Instead of |rgb|, you can currently also specify |gray| as
color model, in which case only one value is needed, or |color|,
in which case you must provide the name of a color in parentheses. In
a color specification the individual specifications must 
be separated using a semicolon, which may be followed by a whitespace
(like a space or a newline). Individual specifications must be given
in increasing order. 


\subsection{Declaring Shadings}

\subsubsection{Horizontal and Vertical Shadings}

\begin{command}{\pgfdeclarehorizontalshading\oarg{color list}\marg{shading
      name}\marg{shading height}\marg{color specification}}
  Declares a horizontal shading named \meta{shading name} of the specified
  \meta{height} with the specified colors. The length of the bar is
  deduced automatically from the maximum dimension in the specification.

\begin{codeexample}[]
\pgfdeclarehorizontalshading{myshadingA}
  {1cm}{rgb(0cm)=(1,0,0); color(2cm)=(green); color(4cm)=(blue)}
\pgfuseshading{myshadingA}
\end{codeexample}

  The effect of the \meta{color list}, which is a
  comma-separated list of colors, is the following: Normally, when
  this list is empty, once a shading has been declared, it becomes
  ``frozen.'' This means that even if you change a color that was used
  in the declaration of the shading later on, the shading will not
  change. By specifying a \meta{color list} you can specify
  that the shading should be recalculated whenever one of the colors
  listed in the list changes (this includes effects like color
  mixins). Thus, when you specify a \meta{color list},
  whenever the shading is used, \pgfname\ first converts the colors in the
  list to \textsc{rgb} triples using the current values of the
  colors and taking any mixins and blends into account. If the
  resulting \textsc{rgb} triples have not yet been   used, a new
  shading is internally created and used. Note that if the 
  option \meta{color list} is used, then no shading is created until
  the first use of |\pgfuseshading|. In particular, the colors
  mentioned in the shading need not be defined when the declaration is
  given.

  When a shading is recalculated because of a change in the
  colors mentioned in \meta{color list}, the complete shading
  is recalculated. Thus even colors not mentioned in the list will be
  used with their current values, not with the values they had upon
  declaration.
  
\begin{codeexample}[]
\pgfdeclarehorizontalshading[mycolor]{myshadingB}
  {1cm}{rgb(0cm)=(1,0,0); color(2cm)=(mycolor)}
\colorlet{mycolor}{green}
\pgfuseshading{myshadingB}
\colorlet{mycolor}{blue}
\pgfuseshading{myshadingB}
\end{codeexample}
\end{command}


\begin{command}{\pgfdeclareverticalshading\oarg{color list}\marg{shading
      name}\marg{shading width}\marg{color specification}}
   Declares a vertical shading named \meta{shading name} of the
   specified \meta{width}. The height of the bar is deduced
   automatically. The effect of \meta{color list} is the same as for
   horizontal shadings.

\begin{codeexample}[]
\pgfdeclareverticalshading{myshadingC}
  {4cm}{rgb(0cm)=(1,0,0); rgb(1.5cm)=(0,1,0); rgb(2cm)=(0,0,1)}
\pgfuseshading{myshadingC}
\end{codeexample}
\end{command}


\subsubsection{Radial Shadings}

\begin{command}{\pgfdeclareradialshading\oarg{color list}\marg{shading
      name}\marg{center point}\marg{color specification}}
  Declares an radial shading. A radial shading is a circle whose inner
  color changes as specified by the color specification. Assuming that
  the center of the shading is at the origin, the color of the center
  will be the color specified for 0cm and the color of the border of
  the circle will be the color for the maximum dimension given in
  the \meta{color specified}. This maximum will also be the radius of
  the circle. If the \meta{center point} is not at the 
  origin, the whole shading inside the circle (whose size remains
  exactly the same) will be distorted such that the given center now
  has the color specified for 0cm. The effect of \meta{color list} is
  the same as for horizontal shadings. 

\begin{codeexample}[]  
\pgfdeclareradialshading{sphere}{\pgfpoint{0.5cm}{0.5cm}}%
  {rgb(0cm)=(0.9,0,0);
   rgb(0.7cm)=(0.7,0,0);
   rgb(1cm)=(0.5,0,0);
   rgb(1.05cm)=(1,1,1)}
\pgfuseshading{sphere}
\end{codeexample}
\end{command}


\subsubsection{General (Functional) Shadings}

\begin{command}{\pgfdeclarefunctionalshading\oarg{color list}\marg{shading
      name}\marg{lower left corner}\marg{upper right corner}\\
    \marg{init code}\marg{type 4 function}}
  \emph{Warning: These shadings are the least portable of all and they
  put the heaviest burden of the renderer. They are slow and,
  possibly, will not print correctly!}

  This command creates a \emph{functional shading}. For such a
  shading, the color of each point is calculated by calling a function
  that gets the coordinates of the point as input and yields the
  color as an output. Note that the function is evaluated by the 
  \emph{renderer}, not by \pgfname\ or \TeX or someone else at
  compile-time. This means that the evaluation of this function has to
  be done \emph{extremely quickly} and the funciton should be
  \emph{very simple}. For this reason, only a very restricted set of
  operations are possible in the function and functions should be
  kept small. Any errors in the function will only be noticed by the
  renderer.

  The syntax for specifying functions is the following: You use a
  simplified form of a subset of the PostScript language. This subset
  will be understood by the PDF-renderer (yes, PDF-renderers do
  have a basic understanding of PostScript) and also by PostScript
  renders. This subset is detailed in Seciton 3.9.4 of the
  PDF-specification (version 1.7). In essence, the specificaiton
  states that these functions may contain ``expressions involving
  integers, real numbers, and boolean values only. There are no
  composite data structures such as strings or arrays, no procedures,
  and no variables or names.'' The allowed operators are (exactly) the
  following: \texttt{abs}, \texttt{add}, \texttt{atan},
  \texttt{ceiling}, \texttt{cos}, \texttt{cvi}, \texttt{cvr},
  \texttt{div}, \texttt{exp}, \texttt{floor}, \texttt{idiv},
  \texttt{ln}, \texttt{log}, \texttt{mod}, \texttt{mul}, \texttt{neg},
  \texttt{round}, \texttt{sin}, \texttt{sqrt}, \texttt{sub},
  \texttt{truncate}, \texttt{and}, \texttt{bitshift}, \texttt{eq},
  \texttt{false}, \texttt{ge}, \texttt{gt}, \texttt{le}, \texttt{lt},
  \texttt{ne}, \texttt{not}, \texttt{or}, \texttt{true}, \texttt{xor},
  \texttt{if}, \texttt{ifelse}, \texttt{copy}, \texttt{dup},
  \texttt{exch}, \texttt{index}, \texttt{pop}.

  When the function is evaluated, the top two stack elements are the
  coordinates of the point for which the color should be computed. The
  coordinates are dimensionless and given in big points, so for the
  coordinate $(50bp, 72.27pt)$ the top two stack elements would be
  \texttt{50.0} and \texttt{72.0}. Ohterwise, the (virtual) stack is
  empty (or should be treated as if it were empty). The function
  should then replace these two values by three values, representing
  the red, green, and blue color of the point. The numbers should be
  real values, not integers since Apple's PDF renderer is broken in
  this regard (use cvr at the end if necessary).

  Conceptually, the function will be evaluated once for each point of
  the rectangle \meta{lower left corner} to \meta{upper right corner},
  which should be a \pgfname-point expression like
  |\pgfpoint{100bp}{100bp}|. A renderer may choose to evaluate the
  function at less points, but, in principle, the function will be
  evaluated for each pixel independently. 

  Because of the rather difficult PostScript syntax, use this macro
  only \emph{if you know what you are doing} (or if you are
  advanterous, of course). 

  As for other shadings, the optional \meta{color list} is used to
  determine whether a shading needs to be recalculated when a color
  has changed.

  The \meta{init code} is executed each time a shading is
  (re)calculated. Typically, it will contain code to extract
  coordinates from colors (see below).

  Inside the PostScript function \meta{type 4 function} you cannot use
  colors directly. Rather, you must push the color components on the
  stack. For this, it is useful to call |\pgfshadecolorrgb| in the
  \meta{init code}. The macro takes a color name as input and stores
  the color's red/green/blue components real numbers between 0.0 and
  1.0 separated by spaces (which is exactly what you need if you want
  to push it on a stack) in a macro. You can then use this macro in
  the argument \meta{type 4 function}.

\begin{codeexample}[]
\pgfdeclarefunctionalshading{twospots}
    {\pgfpointorigin}{\pgfpoint{4cm}{4cm}}{}{
  % Save coordinates for later
  2 copy
  % Compute distance from (40bp,45bp), with x doubled
  45 sub dup mul exch
  40 sub dup mul 0.5 mul add sqrt
  % expontial decay
  dup mul neg 1.0005 exch exp 1.0 exch sub
  % Compute distance form (70bp,70bp) from stored coordiante, scaled
  3 1 roll
  70 sub dup mul .5 mul exch
  70 sub dup mul add sqrt
  % Decay
  dup mul neg 1.002 exch exp 1.0 exch sub
  % red component
  1.0 3 1 roll
}
\pgfuseshading{twospots}
\end{codeexample}

\begin{codeexample}[]
\pgfdeclarefunctionalshading[mycol]{sweep}{\pgfpoint{-1cm}{-1cm}}
{\pgfpoint{1cm}{1cm}}{\pgfshadecolortorgb{mycol}{\myrgb}}{
  2 copy        % whirl
  atan
  3 1 roll
  dup mul exch
  dup mul add sqrt
  30 mul
  add
  sin
  1 add 2 div  
  dup
  \myrgb        % push mycol
  5 4 roll      % multiply all components by calculated value
  mul
  3 1 roll
  3 index
  mul
  3 1 roll
  4 3 roll
  mul
  3 1 roll
}
\colorlet{mycol}{white}%
\pgfuseshading{sweep}%
\colorlet{mycol}{red}%
\pgfuseshading{sweep}
\end{codeexample}
\end{command}


\subsection{Using Shadings}
\label{section-shading-a-path}

\begin{command}{\pgfuseshading\marg{shading name}}
  Inserts a previously declared shading into the text. If you wish to
  use it in a |pgfpicture| environment, you should put a |\pgfbox|
  around it.
  
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfdeclareverticalshading{myshadingD}
    {20pt}{color(0pt)=(red); color(20pt)=(blue)}
  \pgftext[at=\pgfpoint{1cm}{0cm}]  {\pgfuseshading{myshadingD}}
  \pgftext[at=\pgfpoint{2cm}{0.5cm}]{\pgfuseshading{myshadingD}}
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfshadepath\marg{shading name}\marg{angle}}
  This command must be used inside a |{pgfpicture}| environment. The
  effect is a bit complex, so let us go over it step by step.

  First, \pgfname\ will setup a local scope.

  Second, it uses the current path to clip everything inside this
  scope. However, the current path is once more available after the
  scope, so it can be used, for example, to stroke it.

  Now, the \meta{shading name} should be a shading whose width and
  height are 100\,bp, that is, 100 big points. \pgfname\ has a look at
  the bounding box of the current path. This bounding box is computed
  automatically when a path is computed; however, it can sometimes be
  (quite a bit) too large, especially when complicated curves are
  involved. 

  Inside the scope, the low-level transformation matrix is modified.
  The center of the shading is translated (moved) such that it lies on
  the center of the bounding box of the path. The low-level coordinate
  system is also scaled such that the shading ``covers'' the shading (the 
  details are a bit more complex, see below). Then, the coordinate
  system is rotated by \meta{angle}. Finally, if the macro 
  |\pgfsetadditionalshadetransform| has been used, an additional
  transformation is applied. 

  After everything has been set up, the shading is inserted. Due to
  the transformations and clippings, the effect will be that  the
  shading seems to ``fill'' the path.

  If both the path and the shadings were always rectangles and if
  rotation were never involved, it would be easy to scale shadings
  such they always cover the path. However, when a vertical shading is
  rotated, it must obviously be ``magnified'' so that it
  still covers the path. Things get worse when the path is not a
  rectangle itself.

  For these reasons, things work slightly differently ``in reality.''
  The shading is scaled and translated such that the
  the point $(50\mathrm{bp},50\mathrm{bp})$, which is the middle of
  the shading, is at the middle of the path and such that the the
  point $(25\mathrm{bp},25\mathrm{bp})$ is at the lower left corner of
  the path and that  $(75\mathrm{bp},75\mathrm{bp})$  is at upper
  right corner.

  In other words, only the center quarter of the shading will actually
  ``survive the clipping'' if the path is a rectangle. If the path is
  not a rectangle, but, say, a circle, even less is seen of the
  shading. Here is an example that demonstrates this effect:

\begin{codeexample}[]
\pgfdeclareverticalshading{myshadingE}{100bp}    
 {color(0bp)=(red); color(25bp)=(green);  color(75bp)=(blue);  color(100bp)=(black)}
\pgfuseshading{myshadingE} 
\hskip 1cm
\begin{pgfpicture}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{2cm}{1cm}}
  \pgfshadepath{myshadingE}{0}
  \pgfusepath{stroke}
  \pgfpathrectangle{\pgfpoint{3cm}{0cm}}{\pgfpoint{1cm}{2cm}}
  \pgfshadepath{myshadingE}{0}
  \pgfusepath{stroke}
  \pgfpathrectangle{\pgfpoint{5cm}{0cm}}{\pgfpoint{2cm}{2cm}}
  \pgfshadepath{myshadingE}{45}
  \pgfusepath{stroke}
  \pgfpathcircle{\pgfpoint{9cm}{1cm}}{1cm}
  \pgfshadepath{myshadingE}{45}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}

  As can be seen above in the last case, the ``hidden'' part of the
  shading actually \emph{can} become visible if the shading is
  rotated. The reason is that it is scaled as if no rotation took
  place, then the rotation is done.

  The following graphics show which part of the shading are actually
  shown: 

\begin{codeexample}[]
\pgfdeclareverticalshading{myshadingF}{100bp}    
 {color(0bp)=(red); color(25bp)=(green);  color(75bp)=(blue);  color(100bp)=(black)}
\begin{tikzpicture}
  \draw (50bp,50bp) node {\pgfuseshading{myshadingF}};
  \draw[white,thick] (25bp,25bp) rectangle (75bp,75bp);
  \draw (50bp,0bp) node[below] {first two applications};

  \begin{scope}[xshift=5cm]
    \draw (50bp,50bp) node{\pgfuseshading{myshadingF}};
    \draw[rotate around={45:(50bp,50bp)},white,thick] (25bp,25bp) rectangle (75bp,75bp);
    \draw (50bp,0bp) node[below] {third application};
  \end{scope}

  \begin{scope}[xshift=10cm]
    \draw (50bp,50bp) node{\pgfuseshading{myshadingF}};
    \draw[white,thick] (50bp,50bp) circle (25bp);
    \draw (50bp,0bp) node[below] {fourth application};
  \end{scope}
\end{tikzpicture}
\end{codeexample}
  
  An advantage of this approach is that when you rotate a radial
  shading, no distortion is introduced:

\begin{codeexample}[]
\pgfdeclareradialshading{ballshading}{\pgfpoint{-10bp}{10bp}}
 {color(0bp)=(red!15!white); color(9bp)=(red!75!white);
 color(18bp)=(red!70!black); color(25bp)=(red!50!black); color(50bp)=(black)}
\pgfuseshading{ballshading}
\hskip 1cm
\begin{pgfpicture}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{1cm}{1cm}}
  \pgfshadepath{ballshading}{0}
  \pgfusepath{}
  \pgfpathcircle{\pgfpoint{3cm}{0cm}}{1cm}
  \pgfshadepath{ballshading}{0}
  \pgfusepath{}
  \pgfpathcircle{\pgfpoint{6cm}{0cm}}{1cm}
  \pgfshadepath{ballshading}{45}
  \pgfusepath{}
\end{pgfpicture}
\end{codeexample}

  If you specify a rotation of $90^\circ$
  and if the path is not a square, but an elongated rectangle,  the
  ``desired'' effect results: The shading will exactly vary between
  the colors at the 25bp and 75bp boundaries. Here is an example:
  
\begin{codeexample}[]
\pgfdeclareverticalshading{myshadingG}{100bp}    
 {color(0bp)=(red); color(25bp)=(green);  color(75bp)=(blue);  color(100bp)=(black)}
\begin{pgfpicture}
  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{2cm}{1cm}}
  \pgfshadepath{myshadingG}{0}
  \pgfusepath{stroke}
  \pgfpathrectangle{\pgfpoint{3cm}{0cm}}{\pgfpoint{2cm}{1cm}}
  \pgfshadepath{myshadingG}{90}
  \pgfusepath{stroke}
  \pgfpathrectangle{\pgfpoint{6cm}{0cm}}{\pgfpoint{2cm}{1cm}}
  \pgfshadepath{myshadingG}{45}
  \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}


  As a final example, let us define a ``rainbow spectrum'' shading for
  use with \tikzname.
\begin{codeexample}[]
\pgfdeclareverticalshading{rainbow}{100bp}
 {color(0bp)=(red); color(25bp)=(red); color(35bp)=(yellow);
  color(45bp)=(green); color(55bp)=(cyan); color(65bp)=(blue);
  color(75bp)=(violet); color(100bp)=(violet)}
\begin{tikzpicture}[shading=rainbow]
  \shade (0,0) rectangle node[white] {\textsc{pride}} (2,1);
  \shade[shading angle=90] (3,0) rectangle +(1,2);
\end{tikzpicture}
\end{codeexample}

  Note that rainbow shadings are \emph{way} to colorful in almost all
  applications. 
\end{command}

\begin{command}{\pgfsetadditionalshadetransform\marg{transformation}}
    This command allows you to specify an additional transformation
    that should be applied to shadings when the |\pgfshadepath|
    command is used. The \meta{transformation} should be
    transformation code like |\pgftransformrotate{20}|.  
\end{command}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-transformations.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Coordinate and Canvas Transformations}

\subsection{Overview}

\pgfname\ offers two different ways of scaling, shifting, and rotating
(these operations are generally known as \emph{transformations})
graphics: You can apply \emph{coordinate transformations} to all
coordinates and you can apply \emph{canvas transformations} to the
canvas on which you draw. (The names ``coordinate'' and ``canvas''
transformations are not standard, I introduce them only for the
purposes of this manual.) 

The difference is the following:

\begin{itemize}
\item
  As the name ``coordinate transformation'' suggests, coordinate
  transformations apply only to coordinates. For example, when you
  specify a coordinate like |\pgfpoint{1cm}{2cm}| and you wish to
  ``use'' this coordinate---for example as an argument to a
  |\pgfpathmoveto| command---then the coordinate transformation matrix
  is applied to the coordinate, resulting in a new
  coordinate. Continuing the example, if the current coordinate
  transformation is ``scale by a factor of two,'' the coordinate
  |\pgfpoint{1cm}{2cm}| actually designates the point
  $(2\mathrm{cm},4\mathrm{cm})$. 

  Note that coordinate transformations apply \emph{only} to
  coordinates. They do not apply to, say, line width or shadings or
  text.
\item
  The effect of a ``canvas transformation'' like ``scale by a factor
  of two'' can be imagined as follows: You first draw your picture on
  a ``rubber canvas'' normally. Then, once you are done, the whole
  canvas is transformed, in this case stretched by a factor of
  two. In the resulting image \emph{everything} will be larger: Text,
  lines, coordinates, and shadings.
\end{itemize}

In many cases, it is preferable that you use coordinate
transformations and not canvas transformations. When canvas
transformations are used, \pgfname\ looses track of the coordinates of
nodes and shapes. Also, canvas transformations often cause undesirable
effects like changing text size. For these reasons, \pgfname\ makes it
easy to setup the coordinate transformation, but a bit harder to
change the canvas transformation.


\subsection{Coordinate Transformations}

\subsubsection{How PGF Keeps Track of the Coordinate Transformation
  Matrix}

\pgfname\ has an internal coordinate transformation matrix. This
matrix is applied to coordinates ``in certain situations.'' This means
that the matrix is not always applied to every coordinate ``no matter
what.'' Rather, \pgfname\ tries to be reasonably smart at when and how
this matrix should be applied. The most prominent examples are the
path construction commands, which apply the coordinate transformation
matrix to their inputs.

The coordinate transformation matrix consists of four numbers $a$,
$b$, $c$, and $d$, and two dimensions $s$ and $t$. When the coordinate
transformation matrix is applied to a coordinate $(x,y)$ the new
coordinate $(ax+by+s,cx+dy+t)$ results. For more details on how
transformation matrices work in general, please see, for example, the
\textsc{pdf} or PostScript reference or a textbook on computer
graphics.

The coordinate transformation matrix is equal to the identity matrix
at the beginning. More precisely, $a=1$, $b=0$, $c=0$, $d=1$,
$s=0\mathrm{pt}$, and $t=0\mathrm{pt}$.

The different coordinate transformation commands will modify the
matrix by concatenating it with another transformation matrix. This
way the effect of applying several transformation commands will
\emph{accumulate}.

The coordinate transformation matrix is local to the current \TeX\
group (unlike the canvas transformation matrix, which is local to the
current |{pgfscope}|). Thus, the effect of adding a coordinate
transformation to the coordinate transformation matrix will last only
till the end of the current \TeX\ group.




\subsubsection{Commands for Relative Coordinate Transformations}

The following commands add a basic coordinate transformation to the
current coordinate transformation matrix. For all commands, the
transformation is applied \emph{in addition} to any previous
coordinate transformations.

\begin{command}{\pgftransformshift\marg{point}}
  Shifts coordinates by \meta{point}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformshift{\pgfpoint{1cm}{1cm}}
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgftransformxshift\marg{dimensions}}
  Shifts coordinates by \meta{dimension} along the $x$-axis.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformxshift{.5cm}
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgftransformyshift\marg{dimensions}}
  Like |\pgftransformxshift|, only for the $y$-axis.
\end{command}

\begin{command}{\pgftransformscale\marg{factor}}
  Scales coordinates by \meta{factor}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformscale{.75}
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgftransformxscale\marg{factor}}
  Scales coordinates by \meta{factor} in the $x$-direction.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformxscale{.75}
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgftransformyscale\marg{factor}}
  Like |\pgftransformxscale|, only for the $y$-axis.
\end{command}


\begin{command}{\pgftransformxslant\marg{factor}}
  Slants coordinates by \meta{factor} in the $x$-direction. Here, a
  factor of |1| means $45^\circ$.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformxslant{.5}
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgftransformyslant\marg{factor}}
  Slants coordinates by \meta{factor} in the $y$-direction.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformyslant{-1}
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}

  

\begin{command}{\pgftransformrotate\marg{degrees}}
  Rotates coordinates counterclockwise by \meta{degrees}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformrotate{30}
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}

  

\begin{command}{\pgftransformtriangle\marg{a}\marg{b}\marg{c}}
  This command transforms the coordinate system in such a way that the
  triangle given by the points \meta{a}, \meta{b} and \meta{c} lies at
  the coordinates $(0,0)$, $(1\mathrm{pt},0\mathrm{pt})$ and
  $(0\mathrm{pt},1\mathrm{pt})$. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgftransformtriangle
  {\pgfpoint{1cm}{0cm}}
  {\pgfpoint{0cm}{2cm}}
  {\pgfpoint{3cm}{1cm}}
  
  \draw (0,0) -- (1pt,0pt) -- (0pt,1pt) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{command}

  
\begin{command}{\pgftransformcm\marg{a}\marg{b}\marg{c}\marg{d}\marg{point}}
  Applies the transformation matrix given by $a$, $b$, $c$, and $d$
  and the shift \meta{point} to coordinates (in addition to any
  previous transformations already in force).
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformcm{1}{1}{0}{1}{\pgfpoint{.25cm}{.25cm}}
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}

  
\begin{command}{\pgftransformarrow\marg{start}\marg{end}}
  Shift coordinates to the end of the line going from \meta{start} 
  to \meta{end} with the correct rotation. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (3,1);
  \pgftransformarrow{\pgfpointorigin}{\pgfpoint{3cm}{1cm}}
  \pgftext{tip}
\end{tikzpicture}
\end{codeexample}
\end{command}

  
\begin{command}{\pgftransformlineattime\marg{time}\marg{start}\marg{end}}
  Shifts coordinates by a specific point on a line at a specific
  time. The point by which the coordinate is shifted is calculated by
  calling |\pgfpointlineattime|, see
  Section~\ref{section-pointsattime}.

  In addition to shifting the coordinate, a rotation \emph{may} also
  be applied. Whether this is the case depends on whether the \TeX\ if
  |\ifpgfslopedattime| is set to true or not.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1);
  \pgftransformlineattime{.25}{\pgfpointorigin}{\pgfpoint{2cm}{1cm}}
  \pgftext{Hi!}
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (2,1);
  \pgfslopedattimetrue
  \pgftransformlineattime{.25}{\pgfpointorigin}{\pgfpoint{2cm}{1cm}}
  \pgftext{Hi!}
\end{tikzpicture}
\end{codeexample}
  If |\ifpgfslopedattime| is true, another \TeX\ |\if| is important:
  |\ifpgfallowupsidedowattime|. If this is false, \pgfname\ will
  ensure that the rotation is done in such a way that text is never
  ``upside down.''

  There is another \TeX\ if that influences this command. If you set
  |\ifpgfresetnontranslationattime| to true, then, between
  shifting the coordinate and (possibly) rotating/sloping the
  coordinate, the command |\pgftransformresetnontranslations| is
  called. See the description of this command for details.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgftransformscale{1.5}
  \draw      (0,0) -- (2,1);
  \pgfslopedattimetrue
  \pgfresetnontranslationattimefalse
  \pgftransformlineattime{.25}{\pgfpointorigin}{\pgfpoint{2cm}{1cm}}
  \pgftext{Hi!}
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgftransformscale{1.5}
  \draw      (0,0) -- (2,1);
  \pgfslopedattimetrue
  \pgfresetnontranslationattimetrue
  \pgftransformlineattime{.25}{\pgfpointorigin}{\pgfpoint{2cm}{1cm}}
  \pgftext{Hi!}
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgftransformcurveattime\marg{time}\marg{start}\marg{first
      support}\marg{second support}\marg{end}}
  Shifts coordinates by a specific point on a curve at a specific
  time, see  Section~\ref{section-pointsattime} once more.

  As for the line-at-time transformation command, |\ifpgfslopedattime|
  decides whether an additional rotation should be applied. Again, the
  value of |\ifpgfallowupsidedowattime| is also considered. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) .. controls (0,2) and (1,2) .. (2,1);
  \pgftransformcurveattime{.25}{\pgfpointorigin}
    {\pgfpoint{0cm}{2cm}}{\pgfpoint{1cm}{2cm}}{\pgfpoint{2cm}{1cm}}
  \pgftext{Hi!}
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) .. controls (0,2) and (1,2) .. (2,1);
  \pgfslopedattimetrue
  \pgftransformcurveattime{.25}{\pgfpointorigin}
    {\pgfpoint{0cm}{2cm}}{\pgfpoint{1cm}{2cm}}{\pgfpoint{2cm}{1cm}}
  \pgftext{Hi!}
\end{tikzpicture}
\end{codeexample}
  The value of |\ifpgfresetnontranslationsattime| is also taken into account.
\end{command}


{
  \let\ifpgfslopedattime=\relax
  \begin{textoken}{\ifpgfslopedattime}
    Decides whether the ``at time'' transformation commands also
    rotate coordinates or not.
  \end{textoken}
}
{
  \let\ifpgfallowupsidedowattime=\relax
  \begin{textoken}{\ifpgfallowupsidedowattime}
    Decides whether the ``at time'' transformation commands should
    allow the rotation be down in such a way that ``upside-down text''
    can result.
  \end{textoken}
}
{
  \let\ifpgfresetnontranslationsattime=\relax
  \begin{textoken}{\ifpgfresetnontranslationsattime}
    Decides whether the ``at time'' transformation commands should
    reset the non-translations between shifting and rotating.
  \end{textoken}
}


\subsubsection{Commands for Absolute Coordinate Transformations}

The coordinate transformation commands introduced up to now are always
applied in addition to any previous transformations. In contrast, the
commands presented in the following can be used to change the
transformation matrix ``absolutely.'' Note that this is, in general,
dangerous and will often produce unexpected effects. You should use
these commands only if you really know what you are doing.

\begin{command}{\pgftransformreset}
  Resets the coordinate transformation matrix to the identity
  matrix. Thus, once this command is given no transformations are
  applied till the end of the scope.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgftransformrotate{30}
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransformreset
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgftransformresetnontranslations}
  This command sets the $a$, $b$, $c$, and $d$ part of the coordinate
  transformation matrix to $a=1$, $b=0$, $c=0$, and $d=1$. However,
  the current shifting of the matrix is not modified.

  The effect of this command is that any rotation/scaling/slanting is
  undone in the current \TeX\ group, but the origin is not ``moved
  back.''

  This command is mostly useful directly before a |\pgftext| command
  to ensure that the text is not scaled or rotated.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgftransformscale{2}
  \pgftransformrotate{30}
  \pgftransformxshift{1cm}
  {\color{red}\pgftext{rotated}}
  \pgftransformresetnontranslations
  \pgftext{shifted only}
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgftransforminvert}
  Replaces the coordinate transformation matrix by a coordinate
  transformation matrix that ``exactly undoes the original
  transformation.'' For example, if the original transformation was
  ``scale by 2 and then shift right by 1cm'' the new one is ``shift
  left by 1cm and then scale by $1/2$.''

  This command will produce an error if the determinant of
  the matrix is too small, that is, if the matrix is near-singular.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgftransformrotate{30}
  \draw      (0,0) -- (2,1) -- (1,0);
  \pgftransforminvert
  \draw[red] (0,0) -- (2,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{command}

\subsubsection{Saving and Restoring the Coordinate Transformation
  Matrix}

There are two commands for saving and restoring coordinate
transformation matrices.

\begin{command}{\pgfgettransform\marg{macro}}
  This command will (locally) define \meta{macro} to a representation
  of the current coordinate transformation matrix. This matrix can
  later on be reinstalled using |\pgfsettransform|.
\end{command}


\begin{command}{\pgfsettransform\marg{macro}}
  Reinstalls a coordinate transformation matrix that was previously
  saved using |\pgfgettransform|.
\end{command}



\subsection{Canvas Transformations}

The canvas transformation matrix is not managed by \pgfname, but by
the output format like \pdf\ or PostScript. All the \pgfname\ does is
to call appropriate low-level |\pgfsys@| commands to change the canvas
transformation matrix.

Unlike coordinate transformations, canvas transformations apply to
``everything,'' including images, text, shadings, line thickness, and
so on. The idea is that a canvas transformation really stretches and
deforms the canvas after the graphic is finished.

Unlike coordinate transformations, canvas transformations are local to
the current |{pgfscope}|, not to the current \TeX\ group. This is due
to the fact that they are managed by the backend driver, not by \TeX\
or \pgfname.

Unlike the coordinate transformation matrix, it is not possible to
``reset'' the canvas transformation matrix. The only way to change it
is to concatenate it with another canvas transformation matrix or to
end the current |{pgfscope}|.

Unlike coordinate transformations, \pgfname\ does not ``keep track''
of canvas transformations. In particular, it will not be able to
correctly save the coordinates of shapes or nodes when a canvas
transformation is used.

\pgfname\ does not offer a whole set of special commands for modifying
the canvas transformation matrix. Instead, different commands allow
you to concatenate the canvas transformation matrix with a coordinate
transformation matrix (and there are numerous commands for specifying
a coordinate transformation, see the previous section).

\begin{command}{\pgflowlevelsynccm}
  This command concatenates the canvas transformation matrix with the
  current coordinate transformation matrix. Afterward, the coordinate
  transformation matrix is reset.

  The effect of this command is to ``synchronize'' the coordinate
  transformation matrix and the canvas transformation matrix. All
  transformations that were previously applied by the coordinate
  transformations matrix are now applied by the canvas transformation
  matrix.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfsetlinewidth{1pt}
  \pgftransformscale{5}
  \draw      (0,0) -- (0.4,.2);
  \pgftransformxshift{0.2cm}
  \pgflowlevelsynccm
  \draw[red] (0,0) -- (0.4,.2);
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgflowlevel\marg{transformation code}}
  This command concatenates the canvas transformation matrix with the
  coordinate transformation specified by \meta{transformation code}.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfsetlinewidth{1pt}
  \pgflowlevel{\pgftransformscale{5}}
  \draw      (0,0) -- (0.4,.2);
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgflowlevelobj\marg{transformation code}\marg{code}}
  This command creates a local |{pgfscope}|. Inside this scope,
  |\pgflowlevel| is first called with the argument
  \meta{transformation code}, then the \meta{code} is inserted. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfsetlinewidth{1pt}
  \pgflowlevelobj{\pgftransformscale{5}}    {\draw (0,0) -- (0.4,.2);}
  \pgflowlevelobj{\pgftransformxshift{-1cm}}{\draw (0,0) -- (0.4,.2);}
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{environment}{{pgflowlevelscope}\marg{transformation code}}
  This environment first surrounds the \meta{environment contents} by
  a |{pgfscope}|. Then it calls |\pgflowlevel| with the argument
  \meta{transformation code}.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \pgfsetlinewidth{1pt}
  \begin{pgflowlevelscope}{\pgftransformscale{5}}
    \draw (0,0) -- (0.4,.2);
  \end{pgflowlevelscope}
  \begin{pgflowlevelscope}{\pgftransformxshift{-1cm}}
    \draw (0,0) -- (0.4,.2);
  \end{pgflowlevelscope}
\end{tikzpicture}
\end{codeexample}
\end{environment}


\begin{plainenvironment}{{pgflowlevelscope}\marg{transformation code}}
  Plain \TeX\ version of the environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgflowlevelscope}\marg{transformation code}}
  Con\TeX t version of the environment.
\end{contextenvironment}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-base-transparency.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Transparency}

\label{section-transparency}


For an introduction to the notion of transparency, fadings, and
transparency groups, please consult Section~\ref{section-tikz-transparency}. 


\subsection{Specifying a Uniform Opacity}

Specifying a stroke and/or fill opacity is quite easy.

\begin{command}{\pgfsetstrokeopacity\marg{value}}
  Sets the opacity of stroking operations. The \meta{value} should be
  a number between |0| and |1|, where |1| means ``fully opaque'' and
  |0| means ``fully transparent.'' A value like |0.5| will cause paths
  to be stroked in a semitransparent way.
  
\begin{codeexample}[]
\begin{pgfpicture}
  \pgfsetlinewidth{5mm}
  \color{red}
  \pgfpathcircle{\pgfpoint{0cm}{0cm}}{10mm} \pgfusepath{stroke}
  \color{black}
  \pgfsetstrokeopacity{0.5}
  \pgfpathcircle{\pgfpoint{1cm}{0cm}}{10mm} \pgfusepath{stroke}
\end{pgfpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgfsetfillopacity\marg{value}}
  Sets the opacity of filling operations. As for stroking, the
  \meta{value} should be a number between |0| and~|1|.

  The ``filling transparency'' will also be used for text and images.  
  
\begin{codeexample}[]
\begin{tikzpicture}
  \pgfsetfillopacity{0.5}
  \fill[red]   (90:1cm)  circle (11mm);
  \fill[green] (210:1cm) circle (11mm);
  \fill[blue]  (-30:1cm) circle (11mm);
\end{tikzpicture}
\end{codeexample}
\end{command}

Note the following effect: If you setup a certain opacity for stroking
or filling and you stroke or fill the same area twice, the effect
accumulates:

\begin{codeexample}[]
\begin{tikzpicture}
  \pgfsetfillopacity{0.5}
  \fill[red] (0,0) circle (1);
  \fill[red] (1,0) circle (1);
\end{tikzpicture}
\end{codeexample}

Often, this is exactly what you intend, but not always. You can use
transparency groups, see the end of this section, to change this.


\subsection{Specifying a Fading}

The method used by \pgfname\ for specifying fadings is quite
general: You ``paint'' the fading using any of the standard graphics
commands. In more detail: You create a normal picture, which may even
contain text, image, and shadings. Then, you create a fading based on
this picture. For this, the \emph{luminosity} of each pixel of the
picture is analysed (the brighter the pixel, the higher the luminosity
-- a black pixel has luminosity $0$, a white pixel has luminosity $1$,
a gray pixel has some intermediate value as does a red pixel). Then,
when the fading is used, the luminosity of the pixel determines the
opacity of the fading at that position. Positions in the fading where
the picture was black will be completely transparent, positions where
the picture was white will be completely opaque. Positions that have
not been painted at all in the picture are always completely
transparent.


\begin{command}{\pgfdeclarefading\marg{name}\marg{contents}}
  This command declare a fading named \meta{name} for later use. The
  ``picture'' on which the fading is based is given by the
  \meta{contents}. This \meta{contents} is normally typeset in a \TeX\
  box. The resulting box is then used as the ``picture.'' In
  particular, inside the \meta{contents} you must explicitly open a
  |{pgfpicture}| environment if you wish to use \pgfname\ commands.

  Let's start with an easy example. Our first fading picture is just
  some text:
\begin{codeexample}[]
\pgfdeclarefading{fading1}{\color{white}Ti\emph{k}Z}    
\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (2,2);
  \fill [black!30] (0,0) arc (180:0:1);
  \pgfsetfading{fading1}{\pgftransformshift{\pgfpoint{1cm}{1cm}}}
  \fill [red] (0,0) rectangle (2,2);
\end{tikzpicture}
\end{codeexample}
  What's happening here? The ``fading picture'' is mostly transparent,
  except for the pixels that are part of the word Ti\emph{k}Z. Now,
  these pixels are \emph{white} and, thus, have a high
  luminosity. This in turn means that these pixels of the fading will
  be highly opaque. For this reason, only those pixels of the big red
  rectangle ``shine through'' that are at the positions of these
  opaque pixels.

  It is somewhat counter-intuitive that the white pixels in a fading
  picture are opaque in a fading. For this reason, the color
  |pgftransparent| is defined to be the same as |black|. This allows
  one to write |pgftransparent| for completely transparent parts of a
  fading picture and |pgftransparent!0| for the opaque parts and
  things liek |pgftransparent!20| for parts that are 20\%
  transparent.

  Furthermore, the color |pgftransparent!0| (which is the same as
  white and which corresponds to completely opaque) is installed at
  the beginning of a fading picture. Thus, in the above example the
  |\color{white}| was not really necessary.

  Next, let us create a fading that gets more and more transparent as
  we go from left to right. For this, we put a shading inside the
  fading picture that has the color |pgftransparent!0| at the
  left-hand side and the color |pgftransparent!100| at the right-hand
  side. 
\begin{codeexample}[]
\pgfdeclarefading{fading2}
{\tikz \shade[left color=pgftransparent!0,
              right color=pgftransparent!100] (0,0) rectangle (2,2);}    
\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (2,2);
  \fill [black!30] (0,0) arc (180:0:1);
  \pgfsetfading{fading2}{\pgftransformshift{\pgfpoint{1cm}{1cm}}}
  \fill [red] (0,0) rectangle (2,2);
\end{tikzpicture}
\end{codeexample}

  In our final example, we create a fading that is based on a radial
  shading.
\begin{codeexample}[]
\pgfdeclareradialshading{myshading}{\pgfpointorigin}
{
  color(0mm)=(pgftransparent!0);
  color(5mm)=(pgftransparent!0);
  color(8mm)=(pgftransparent!100);
  color(15mm)=(pgftransparent!100)
}
\pgfdeclarefading{fading3}{\pgfuseshading{myshading}}
\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (2,2);
  \fill [black!30] (0,0) arc (180:0:1);
  \pgfsetfading{fading3}{\pgftransformshift{\pgfpoint{1cm}{1cm}}}
  \fill [red] (0,0) rectangle (2,2);
\end{tikzpicture}
\end{codeexample}
\end{command}

After having declared a fading, we can use it. As for shadings, there
are two different commands for using fadings:

\begin{command}{\pgfsetfading\marg{name}\marg{transformations}}
  This command sets the graphic state parameter ``fading'' to a
  previously defined fading \meta{name}. This graphic state works like
  other graphic states, that is, is persists till the end of the
  current scope or until a different transparency setting is chosen.

  When the fading is installed, it will be centered on the origin with
  its natural size. Anything outside the fading pictures's original
  bounding box will be transparent and, thus, the fading effectively
  clips against this bounding box.

  The \meta{transformations} are applied to the fading before it is
  used. They contain normal \pgfname\ transformation commands like
  |\pgftransformshift|. You can also scale the fading using this
  command. Note, however, that the transformation needs to be inverted
  internally, which may result in inaccuracies and the following
  graphics may be slightly distorted if you use a strong
  \meta{transformation}.
\begin{codeexample}[]
\pgfdeclarefading{fading2}
{\tikz \shade[left color=pgftransparent!0,
              right color=pgftransparent!100] (0,0) rectangle (2,2);}    
\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (2,2);
  \fill [black!30] (0,0) arc (180:0:1);
  \pgfsetfading{fading2}{}
  \fill [red] (0,0) rectangle (2,2);
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (2,2);
  \fill [black!30] (0,0) arc (180:0:1);
  \pgfsetfading{fading2}{\pgftransformshift{\pgfpoint{1cm}{1cm}}
                         \pgftransformrotate{20}}
  \fill [red] (0,0) rectangle (2,2);
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfsetfadingforcurrentpath\marg{name}\marg{transformations}}
  This command works like |\pgfsetfading|, but the fading is scaled
  are transformed according to the following rules:
  \begin{enumerate}
  \item
    If the current path is empty, the command has the same effect as
    |\pgfsetfading|. 
  \item
    Otherwise it is assumed that the fading has a size of 100bp times
    100bp. 
  \item
    The fading is resized and shiften (using appropriate
    transformations) such that the position
    $(25\mathrm{bp},25\mathrm{bp})$ lies at the lower-left corner of
    the current path and the position $(75\mathrm{bp},75\mathrm{bp})$
    lies at the upper-right corner of the current path.
  \end{enumerate}
  Note that these rules are the same as the ones used in
  |\pgfshadepath| for shadings. After these transformations, the
  \meta{transformations} are executed (typically a rotation).
\begin{codeexample}[]
\pgfdeclarehorizontalshading{shading}{100bp}
{ color(0pt)=(transparent!0);    color(25bp)=(transparent!0);
  color(75bp)=(transparent!100); color(100bp)=(transparent!100)}

\pgfdeclarefading{fading}{\pgfuseshading{shading}}

\begin{tikzpicture}
  \fill [black!20] (0,0) rectangle (2,2);
  \fill [black!30] (0,0) arc (180:0:1);

  \pgfpathrectangle{\pgfpointorigin}{\pgfpoint{2cm}{1cm}}
  \pgfsetfadingforcurrentpath{fading}{}
  \pgfusepath{discard}
  
  \fill [red] (0,0) rectangle (2,1);

  \pgfpathrectangle{\pgfpoint{0cm}{1cm}}{\pgfpoint{2cm}{1cm}}
  \pgfsetfadingforcurrentpath{fading}{\pgftransformrotate{90}}
  \pgfusepath{discard}

  \fill [red] (0,1) rectangle (2,2);
\end{tikzpicture}
\end{codeexample}

\end{command}

\subsection{Transparency Groups}

Transparency groups are declared using the following commands.

\begin{environment}{{pgftransparencygroup}}
  This environment should only be used inside a |{pgfpicture}|. It has
  the following effect:
  \begin{enumerate}
  \item The \meta{environment contents} is stroked/filled
    ``ignoring any outside transparency.'' This means, all previous
    transparency settings are ignored (you can still set transparency
    inside the group, but never mind). This means that if in the
    \meta{environment contents} you stroke a pixel three times in
    black, it is just black. Stroking it white afterwards yields a
    white pixel, and so on.
  \item When the group is finished, it is painted as a whole. The 
    \emph{fill} transparency settings are now applied to the resulting
    picutre. For instance, the pixel that has been painted three times
    in black and once in white is just white at the end, so this white
    color will be blended with whatever is ``behind'' the group on the
    page.
  \end{enumerate}

  Note that, depending on the driver, \pgfname\ may have to guess the
  size of the contents of the transparency group (because such a group
  is put in an XForm in \textsc{pdf} and a bounding box must be
  supplied). \pgfname\ will use normally use the size of the picture's
  bounding box at the end of the transparency group plus a safety
  margin of 1cm. Under normal circumstances, this will work nicely
  since the picture's bounding box contains everything
  anyway. However, if you have switched off the picture size tracking
  or if you are using canvas transformations, you may have to make
  sure that the bounding box is big enough. The trick is to locallly
  create a picture that is ``large enough'' and then insert this
  picture into the main picture while ignoring the size. The following
  example shows how this is done:

  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (2,2);

  % Stuff outside the picture, but still in a transparency group.
  \node [left,overlay] at (0,1) {
    \begin{tikzpicture}
      \pgfsetfillopacity{0.5}
      \pgftransparencygroup
      \node at (2,0) [forbidden sign,line width=2ex,draw=red,fill=white]
        {Smoking};
      \endpgftransparencygroup
    \end{tikzpicture}  
  };
\end{tikzpicture}
\end{codeexample}


\begin{plainenvironment}{{pgftransparencygroup}}
  Plain \TeX\ version of the |{pgftransparencygroup}| environment.
\end{plainenvironment}

\begin{contextenvironment}{{pgftransparencygroup}}
  This is the Con\TeX t version of the environment.
\end{contextenvironment}

\end{environment}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-drivers.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Input and Output Formats}
\label{section-formats}


\TeX\ was designed to be a flexible system. This is true both for the
\emph{input} for \TeX\ as well as for the \emph{output}. The present
section explains which input formats there are and how they are
supported by \pgfname. It also explains which different output formats
can be produced.



\subsection{Supported Input Formats}

\TeX\ does not prescribe exactly how your input should be
formatted. While it is \emph{customary} that, say, an opening brace
starts a scope in \TeX, this is by no means necessary. Likewise, it is
\emph{customary} that environments start with |\begin|, but \TeX\
could not really care less about the exact command name.

Even though \TeX\ can be reconfigured, users can not. For this reason,
certain \emph{input formats} specify a set of commands and conventions
how input for \TeX\ should be formatted. There are currently three
``major'' formats: Donald Knuth's original |plain| \TeX\ format,
Leslie Lamport's popular \LaTeX\ format, and Hans Hangen's Con\TeX t
format.


\subsubsection{Using the  \LaTeX\ Format}

Using \pgfname\ and \tikzname\ with the \LaTeX\ format is easy: You
say |\usepackage{pgf}| or |\usepackage{tikz}|. Usually, that is all
you need to do, all configuration will be done automatically and
(hopefully) correctly.

The style files used for the \LaTeX\ format reside in the subdirectory
|latex/pgf/| of the \pgfname-system. Mainly, what these files do is to
include files in the directory |generic/pgf|. For example, here is the
content of the file |latex/pgf/frontends/tikz.sty|:

\begin{codeexample}[code only]
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\RequirePackage{pgf,pgffor}

\input{tikz.code.tex}

\endinput
\end{codeexample}

The files in the |generic/pgf| directory do the actual work.



\subsubsection{Using the Plain \TeX\ Format}

When using the plain \TeX\ format, you say |\input{pgf.tex}| or
|\input{tikz.tex}|. Then, instead of  |\begin{pgfpicture}| and
  |\end{pgfpicture}| you use  |\pgfpicture| and |\endpgfpicture|. 

Unlike for the \LaTeX\ format, \pgfname\ is not as good at discerning
the appropriate configuration for the plain \TeX\ format. In
particular, it can only automatically determine the correct output
format if you use |pdftex| or |tex| plus |dvips|. For all other output
formats you need to set the macro |\pgfsysdriver| to the correct
value. See the description of using output formats later on. 

\pgfname\ was originally written for use with \LaTeX\ and this shows
in a number of places. Nevertheless, the plain \TeX\ support is
reasonably good.

Like the \LaTeX\ style files, the plain \TeX\ files like |tikz.tex|
also just include the correct |tikz.code.tex| file.



\subsubsection{Using the Con\TeX t Format}

When using the Con\TeX t format, you say |\usemodule[pgf]| or
|\usemodule[tikz]|. As for the plain \TeX\ format you also have
to replace the start- and end-of-environment tags as follows: Instead
of  |\begin{pgfpicture}| and |\end{pgfpicture}| you use
|\startpgfpicture| and |\stoppgfpicture|; similarly, instead of
|\begin{tikzpicture}| and |\end{tikzpicture}| you use must now use
|\starttikzpicture| and |\stoptikzpicture|; and so on for other
environments. 

The Con\TeX t support is very similar to the plain \TeX\ support, so
the same restrictions apply: You may have to set the output
format directly and graphics inclusion may be a problem.

In addition to |pgf| and |tikz| there also exist modules like
|pgfcore| or |pgfmodulematrix|. To
use them, you may need to include the module |pgfmod| first (the
modules |pgf| and |tikz| both include |pgfmod| for you, so typically
you can skip this). This special module is necessary since Con\TeX t
satanically restricts the length of module names to 6 characters
and \pgfname's long names are mapped
to cryptic 6-letter-names for you by the module |pgfmod|.





\subsection{Supported Output Formats}
\label{section-drivers}

An output format is a format in which \TeX\ outputs the text it has
typeset. Producing the output is (conceptually) a two-stage process:
\begin{enumerate}
\item
  \TeX\ typesets your text and graphics. The result of this
  typesetting is mainly a long list of letter--coordinate pairs, plus 
  (possibly) some ``special'' commands. This long list of pairs
  is written to something called a |.dvi|-file.
\item
  Some other program reads this |.dvi|-file and translates the
  letter--coordinate pairs into, say, PostScript commands for placing
  the given letter at the given coordinate.
\end{enumerate}

The classical example of this process is the combination of |latex|
and |dvips|. The |latex| program (which is just the |tex| program
called with the \LaTeX-macros preinstalled) produces a |.dvi|-file as
its output. The |dvips| program takes this output and produces a
|.ps|-file (a PostScript) file. Possibly, this file is further
converted using, say, |ps2pdf|, whose name is supposed to mean
``PostScript to PDF.'' Another example of programs using this
process is the combination of |tex| and |dvipdfm|. The |dvipdfm|
program takes a |.dvi|-file as 
input and translates the letter--coordinate pairs therein into
\pdf-commands, resulting in a |.pdf| file directly. Finally, the
|tex4ht| is also a program that takes a |.dvi|-file and produces an
output, this time it is a |.html| file. The programs |pdftex| and
|pdflatex| are special: They directly produce a |.pdf|-file without
the intermediate |.dvi|-stage. However, from the programmer's point of
view they behave exactly as if there where an intermediate stage.

Normally, \TeX\ only produces letter--coordinate pairs as its
``output.'' This obviously makes is difficult to draw, say, a
curve. For this, ``special'' commands can be used. Unfortunately,
these special commands are not the same for the different programs
that process the |.dvi|-file. Indeed, every program that takes a
|.dvi|-file as input has a totally different syntax for the special
commands.

One of the main jobs of \pgfname\ is to ``abstract way'' the
difference in the syntax of the different programs. However, this
means that support for each program has to be ``programmed,'' which is
a time-consuming and complicated process. 


\subsubsection{Selecting the Backend Driver}

When \TeX\ typesets your document, it does not know which program
you are going to use to transform the |.dvi|-file. If your |.dvi|-file
does not contain any special commands, this would be fine; but these
days almost all |.dvi|-files contain lots of special commands. It is
thus necessary to tell \TeX\ which program you are going to use later
on.

Unfortunately, there is no ``standard'' way of telling this to
\TeX. For the \LaTeX\ format a sophisticated mechanism exists inside
the |graphics| package and \pgfname\ plugs into this mechanism. For
other formats and when this plugging does not work as expected, it is
necessary to tell \pgfname\ directly which program you are going to
use. This is done by redefining the macro |\pgfsysdriver| to an
appropriate value \emph{before} you load |pgf|. If you are going to
use the |dvips| program, you set this macro to the value
|pgfsys-dvips.def|; if you use |pdftex| or |pdflatex|, you set it to
|pgfsys-pdftex.def|; and so on. In the following, details of the
support of the different programs are discussed.


\subsubsection{Producing PDF Output}

\pgfname\ supports three programs that produce \pdf\ output (\pdf\ means
``portable document format'' and was invented by the Adobe company):
|dvipdfm|, |pdftex|, and |vtex|. The |pdflatex| program is the same as the
|pdftex| program: it uses a different input format, but the output is
exactly the same.

\begin{filedescription}{pgfsys-pdftex.def}
  This is the driver file for use with pdf\TeX, that is, with the
  |pdftex| or |pdflatex| command. It includes
  |pgfsys-common-pdf.def|.

  This driver has the ``complete'' functionality. This means,
  everything \pgfname\ ``can do at all'' is implemented in this
  driver. 
\end{filedescription}

\begin{filedescription}{pgfsys-dvipdfm.def}
  This is a driver file for use with (|la|)|tex| followed by |dvipdfm|. It
  includes |pgfsys-common-pdf.def|.

  This driver supports most of \pgfname's features, but there are some
  restrictions:
  \begin{enumerate}
  \item
    In \LaTeX\ mode it uses |graphicx| for the graphics
    inclusion and does not support masking.
  \item
    In plain \TeX\ mode it does not support image inclusion.
  \item
    For remembering of pictures (inter-picture connections) you need
    to use a recent version of |pdftex| running in DVI-mode.
  \item
    Patterns are not (cannot) be supported.
  \item
    Functional shadings are not (cannot) be supported.
  \end{enumerate}
\end{filedescription}

\begin{filedescription}{pgfsys-xetex.def}
  This is a driver file for use with |xe|(|la|)|tex| followed by
  |xdvipdfmx|. This driver supports the same operations as the dvipdfm
  driver,  except that remembering of pictures (inter-picture
  connections)   always works.
\end{filedescription}

\begin{filedescription}{pgfsys-vtex.def}
  This is the driver file for use with the commercial \textsc{vtex}
  program. Even though it produces  \textsc{pdf} output, it
  includes |pgfsys-common-postscript.def|. Note that the
  \textsc{vtex} program can produce \emph{both} Postscript and
  \textsc{pdf} output, depending on the command line
  parameters. However, whether you produce Postscript or
  \textsc{pdf} output does not change anything with respect to the
  driver. 

  This driver supports most of \pgfname's features, except for
  the following restrictions:
  \begin{enumerate}
  \item
    In \LaTeX\ mode it uses |graphicx| for the graphics
    inclusion and does not support masking.
  \item
    In plain \TeX\ mode it does not support image inclusion.
  \item
    Shading is fully implemented, but yields the same quality as the
    implementation for |dvips|.
  \item
    Opacity is not supported.
  \item
    Remembering of pictures (inter-picture connections) is not
    supported. 
  \end{enumerate}
\end{filedescription}

It is also possible to produce a |.pdf|-file by first producing a
PostScript file (see below) and then using a PostScript-to-\pdf\
conversion program like |ps2pdf| or the Acrobat Distiller.


\subsubsection{Producing PostScript Output}

\begin{filedescription}{pgfsys-dvips.def}
  This is a driver file for use with (|la|)|tex| followed by
  |dvips|. It includes |pgfsys-common-postscript.def|.

  This driver also supports most of \pgfname's features, except for
  the following restrictions:
  \begin{enumerate}
  \item
    In \LaTeX\ mode it uses |graphicx| for the graphics
    inclusion and does not support masking.
  \item
    In plain \TeX\ mode it does not support image inclusion.
  \item
    Shading is fully implemented, but the results will not be 
    as good as with a driver producing |.pdf| as output. 
  \item
    Opacity works only in conjunction with newer versions of
    GhostScript. 
  \item
    For remembering of pictures (inter-picture connections) you need
    to use a recent version of |pdftex| running in DVI-mode.
  \end{enumerate}
\end{filedescription}

\begin{filedescription}{pgfsys-textures.def}
  This is a driver file for use with the \textsc{textures} program. It
  includes |pgfsys-common-postscript.def|. 

  This driver has exactly the same restrictions as the driver for
  |dvips|. 
\end{filedescription}

You can also use the |vtex| program together with |pgfsys-vtex.def| to
produce Postscript output.



\subsubsection{Producing HTML / SVG Output}

The |tex4ht| program converts |.dvi|-files to |.html|-files. While the
\textsc{html}-format cannot be used to draw graphics, the
\textsc{svg}-format can. Using the following driver, you can ask
\pgfname\ to produce an \textsc{svg}-picture for each \pgfname\
graphic in your text.

\begin{filedescription}{pgfsys-tex4ht.def}
  This is a driver file for use with the |tex4ht| program. It includes
  |pgfsys-common-svg.def|.

  When using this driver you should be aware of the following
  restrictions: 
  \begin{enumerate}
  \item
    In \LaTeX\ mode it uses |graphicx| for the graphics
    inclusion.    
  \item
    In plain \TeX\ mode it does not support image inclusion.
  \item
    Remembering of pictures (inter-picture connections) is not
    supported. 
  \item
    Text inside |pgfpicture|s is not supported very well. The reason
    is that the \textsc{svg} specification currently does not support
    text very well and it is also not possible to correctly ``escape
    back'' to \textsc{html}. All these problems will hopefully
    disappear in the future, but currently only two kinds of text work
    reasonably well: First, plain text without math mode, special
    characters or anything else special. Second, \emph{very} simple
    mathematical text that contains subscripts or superscripts. Even
    then, variables are not correctly set in italics and, in general,
    text simple does not look very nice.
  \item
    If you use text that contains anything special, even something as
    simple as |$\alpha$|, this may corrupt the graphic since |text4ht|
    does not always produce valid \textsc{xml} code. So, once more,
    \emph{stick to very simple node text inside graphics.} Sorry.
  \item
    Unlike for other output formats, the bounding box of a picture
    ``really crops'' the picture.
  \item
    Matrices do not work.
  \item
    Functional shadings are not supported.
  \end{enumerate}

  The driver basically works as follows: When a |{pgfpicture}| is
  started, appropriate |\special| commands are used to directed the
  output of |tex4ht| to a new file called |\jobname-xxx.svg|, where
  |xxx| is a number that is increased for each graphic. Then, till the
  end of the picture, each (system layer) graphic command creates a
  special that inserts appropriate \textsc{svg} literal text into the
  output file. The exact details are a bit complicated since the
  imaging model and the processing model of PostScript/\pdf\ and
  \textsc{svg} are not quite the same; but they are ``close enough''
  for \pgfname's purposes.
\end{filedescription}


\subsubsection{Producing Perfectly Portable DVI Output}

\begin{filedescription}{pgfsys-dvi.def}
  This is a driver file that can be used with any output driver,
  except for |tex4ht|.

  The driver will produce perfectly portable |.dvi| files by composing
  all pictures entirely of black rectangles, the basic and only graphic
  shape supported by the \TeX\ core. Even straight, but slanted lines
  are tricky to get right in this model (they need to be composed of
  lots of little squares).

  Naturally, \emph{very little} is possible with this driver. In fact,
  so little is possible that it is easier to list what is possible:
  \begin{itemize}
  \item Text boxes can be placed in the normal way.
  \item Lines and curves can be drawn (stroked). If they are not
    horizontal or vertical, they are composed of hundred of small
    rectangles.
  \item Lines of different width are supported.
  \item Transformations are supported.
  \end{itemize}
  Note that, say, even filling is not supported! (Let alone color or
  anything fancy.)

  This driver has only one real application: It might be useful when
  you only need horizontal or vertical lines in a picture. Then, the
  results are quite satisfactory.
\end{filedescription}


==> pgfmanual-en-guidelines.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Guidelines on Graphics}

The present section is not about \pgfname\ or \tikzname, but about
general guidelines and principles concerning the creation of
graphics for scientific presentations, papers, and books.

The guidelines in this section come from different sources. Many of
them are just what I would like to claim is ``common sense,'' some
reflect my personal experience (though, hopefully, not my personal
preferences), some come from books (the bibliography is still missing,
sorry) on graphic design and typography. 
The most influential source  are the brilliant books
by Edward Tufte. While I do not agree with everything written in these
books, many of Tufte's arguments are so convincing that I decided to
repeat them in the following guidelines. 

The first thing you should ask yourself when someone presents a bunch of
guidelines is: Should I really follow these guidelines? This is an
important questions, because there are good reasons not to follow
general guidelines.  The person who setup the guidelines may have had other
objectives than you do. For example, a guideline might say ``use the
color red for emphasis.'' While this guideline makes perfect sense
for, say, a presentation using a projector, red ``color'' has the
\emph{opposite} effect of ``emphasis'' when printed using a
black-and-white printer. Guidelines were almost always setup to
address a specific situation. If you are not in this situation,
following a guideline can do more harm than good.

The second thing you should be aware of is the basic rule of
typography is: ``Every rule can be broken, as long as you are
\emph{aware}  that you are breaking a rule.'' This rule also applies
to graphics. Phrased differently, the basic rule states: ``The only
mistakes in typography are things done is ignorance.''  When you are
aware of a rule and when you decide that breaking the rule has a
desirable effect, break the rule.


\subsection{Planning the Time Needed for the Creation of Graphics}

When you create a paper with numerous graphics, the time needed to
create these graphics becomes an important factor. How much time
should you calculate for the creation of graphics?

As a general rule, assume that a graphic will need as much time to
create as would a text of the same length. For example, when I
write a paper, I need about one hour per page for
the first draft. Later, I need between two and four hours per page
for revisions. Thus, I expect to need about half an hour for the
creation of \emph{a first draft} of a half page graphic. Later on, I
expect another one to two hours before the final graphic is finished.

In many publications, even in good journals, the authors and editors
have obviously  invested a lot of time on the text, but seem to 
have spend about five minutes to create all of the
graphics. Graphics often seem to have been added as an
``afterthought'' or look like a screen shot of whatever the authors's
statistical software shows them. As will be argued later on, the
graphics that programs like \textsc{gnuplot} produce by default are of
poor quality.

Creating informative graphics that help the reader and that fit
together with the main text is a difficult, lengthy process. 
\begin{itemize}
\item
  Treat graphics as first-class citizens of your papers. They deserve
  as much time and energy as the text does.
  Indeed, the creation of graphics might deserve \emph{even more} time
  than the writing of the main text since more attention will  be paid
  to the graphics and they will be looked at first. 
\item
  Plan as much time for the creation and revision of a graphic as you
  would plan for text of the same size.
\item
  Difficult graphics with a high information density may require even
  more time.
\item
  Very simple graphics will require less time, but most likely you do
  not want to have ``very simple graphics'' in your paper, anyway;
  just as you would not like to have a ``very simple text'' of the
  same size.  
\end{itemize}


\subsection{Workflow for Creating a Graphic}

When you write a (scientific) paper, you will most likely follow the
following pattern: You have some results/ideas that you would
like to report about. The creation of the paper will typically start
with compiling a rough outline. Then, the different sections are
filled with text to create a first draft. This draft is then revised
repeatedly until, often after substantial revision, a final paper
results. In a good journal paper there is typically not be a single 
sentence that has survived unmodified from the first draft.

Creating a graphics follows the same pattern:
\begin{itemize}
\item
  Decide on what the graphic should communicate. Make this a conscious
  decision, that is, determine ``What is the graphic supposed to tell
  the reader?''
\item
  Create an ``outline,'' that is, the rough overall ``shape'' of the
  graphic, containing the most crucial elements. Often, it is
  useful to do this using pencil and paper.
\item
  Fill out the finer details of the graphic to create a first
  draft.
\item
  Revise the graphic repeatedly along with the rest of the paper.
\end{itemize}




\subsection{Linking Graphics With the Main Text}

Graphics can be placed at different places in a text. Either, they can
be inlined, meaning they are somewhere ``in the middle of the text''
or they can be placed in standalone ``figures.'' Since printers (the
people) like to have their pages ``filled,'' (both for aesthetic and
economic reasons) standalone figures may traditionally be placed on
pages in the document far removed from the main text that refers to
them. \LaTeX\ and \TeX\ tend to encourage this ``drifting away'' of
graphics for technical reasons. 

When a graphic is inlined, it will more or less automatically be
linked with the main text in the sense that the labels of the graphic
will be implicitly explained by the surrounding text. Also, the main
text will typically make it clear what the graphic is about and what
is shown.

Quite differently, a standalone figure will often be viewed at a time
when the main text that this graphic belongs to either has not yet
been read or has been read some time ago. For this reason, you should
follow the following guidelines when creating standalone figures:
\begin{itemize}
\item
  Standalone figures should have a caption than should make them
  ``understandable by themselves.''

  For example, suppose a graphic shows an example of the different
  stages of a quicksort algorithm. Then the figure's caption should,
  at the very least, inform the reader that ``The figure shows the
  different stages of the quicksort algorithm introduced on page
  xyz.'' and not just ``Quicksort algorithm.''
\item
  A good caption adds as much context information as possible. For
  example, you could say: ``The figure shows the different stages of
  the quicksort algorithm introduced on page xyz. In the first line,
  the pivot element 5 is chosen. This causes\dots'' While this
  information can also be given in the main text, putting it in the
  caption will ensure that the context is kept. Do not feel afraid of
  a 5-line caption. (Your editor may hate you for this. Consider
  hating them back.)
\item
  Reference the graphic in your main text as in ``For an example of
  quicksort `in action,' see Figure~2.1 on page xyz.''
\item
  Most books on style and typography recommend that you do not use
  abbreviations as in ``Fig.~2.1'' but write ``Figure 2.1.''

  The main argument against abbreviations is that ``a period is too
  valuable to waste it on an abbreviation.'' The idea is that a period
  will make the reader assume that the sentence ends after ``Fig'' and
  it takes a ``conscious backtracking'' to realize that the sentence
  did not end after all.

  The argument in favor of abbreviations is that they save space.
  
  Personally, I am not really convinced by either argument. On the one
  hand, I have not yet seen any hard evidence that abbreviations slow 
  readers down. On the other hand,  abbreviating all ``Figure'' by
  ``Fig.''\ is most unlikely to save even a single line in  most
  documents. I avoid abbreviations.
\end{itemize}



\subsection{Consistency Between Graphics and Text}

Perhaps the most common ``mistake'' people do when creating graphics
(remember that a ``mistake'' in design is always just ``ignorance'')
is to have a mismatch between the way their graphics look and the way 
their text looks.

It is quite common that authors use several different programs for
creating the graphics of a paper. An author might produce some plots
using \textsc{gnuplot}, a diagram using \textsc{xfig}, and include an
|.eps| graphic a coauthor contributed using some unknown program. All
these graphics will, most likely, use different line widths, different
fonts, and have different sizes. In addition, authors often use
options like |[height=5cm]| when including graphics to scale them to
some ``nice size.''

If the same approach were taken to writing the main text, every
section would be written in a different font at a different size. In
some sections all theorems would be underlined, in another they would
be printed all in uppercase letters, and in another in red. In
addition, the margins would be different on each page.
Readers and editors would not tolerate a text if it were written in
this fashion, but with graphics they often have to.

To create consistency between graphics and text, stick to the
following guidelines:
\begin{itemize}
\item
  Do not scale graphics.

  This means that when generating graphics using an external program,
  create them ``at the right size.''
\item
  Use the same font(s) both in graphics and the body text.
\item
  Use the same line width in text and graphics.

  The  ``line width'' for normal text is the width of the stem of
  letters like T{}. For \TeX, this is usually
  $0.4\,\mathrm{pt}$. However, some journals will not accept graphics
  with a normal line width below $0.5\,\mathrm{pt}$.
\item
  When using colors, use a consistent color coding in the text and in  
  graphics. For example, if red is supposed to alert the reader to
  something in the main text, use red also in graphics for important
  parts of the graphic. If blue is used for structural elements like 
  headlines and section titles, use blue also for structural elements
  of your graphic.

  However, graphics may also use a logical intrinsic color
  coding. For example, no matter what colors you normally use, readers
  will generally assume, say, that the color green as ``positive, go,
  ok'' and red as ``alert, warning, action.''
\end{itemize}

Creating consistency when using different graphic programs is almost
impossible. For this reason, you should consider sticking to a single
graphics program.


\subsection{Labels in Graphics}

Almost all graphics will contain labels, that is, pieces of text that
explain parts of the graphics. When placing labels, stick to the
following guidelines:

\begin{itemize}
\item
  Follow the rule of consistency when placing labels. You should do
  so in two ways: First, be consistent with the main text, that is,
  use the same font as the main text also for labels. Second, be
  consistent between labels, that is, if you format some labels in
  some particular way, format all labels in this way.
\item
  In addition to using the same fonts in text and graphics, you should
  also use the same notation. For example, if you write $1/2$ in your
  main text, also use ``$1/2$'' as labels in graphics, not
  ``0.5''. A $\pi$ is a ``$\pi$'' and not ``$3.141$''. Finally,
  $\mathrm e^{-\mathrm i \pi}$ is ``$\mathrm e^{-\mathrm i \pi}$'',
  not ``$-1$'', let alone ``-1''. 
\item
  Labels should be legible. They should not only have a reasonably
  large size, they also should not be obscured by lines or other
  text. This also applies to of lines and text \emph{behind} the
  labels.
\item
  Labels should be ``in  place.'' Whenever there is enough space,
  labels should be placed next to the thing they label. Only if
  necessary, add a (subdued) line from the label to the labeled
  object. Try to avoid labels that only reference explanations in
  external legends. Reader have to jump back and forth between the
  explanation and the object that is described. 
\item
  Consider subduing ``unimportant'' labels using, for example, a gray
  color. This will keep the focus on the actual graphic.
\end{itemize}



\subsection{Plots and Charts}

One of the most frequent kind of graphics, especially in scientific
papers, are \emph{plots}. They come in a large variety, including
simple line plots, parametric plots, three dimensional plots, pie
charts, and many more.

Unfortunately, plots are notoriously hard to get right. Partly, the
default settings of programs like \textsc{gnuplot} or Excel are to
blame for this since these programs make it very convenient to create
bad plots.

The first question you should ask yourself when creating a plot is,
Are there enough data points to merit a plot? If the answer is ``not
really,'' use a table. 

A typical situation where a plot is unnecessary is when people present
a few numbers in a bar diagram. Here is a real-life example: At the
end of a seminar a lecturer asked the participants for feedback. Of
the 50 participants, 30 returned the feedback form. According to the
feedback, three participants considered the seminar ``very good,''
nine considered it  ``good,'' ten ``ok,'' eight ``bad,'' and no one thought 
that the seminar was ``very bad.''

A simple way of summing up this information is the following table:

\medskip
\begin{tabular}{lp{3.75cm}r}
  \emph{Rating given} & \raggedright\emph{Participants (out of 50) who gave this rating} &
  \emph{Percentage} \\[1.75em]
  ``very good'' & \hfil\hphantom{0}3\hfil & \hphantom{0}6\% \\
  ``good'' & \hfil\hphantom{0}9\hfil & 18\% \\
  ``ok'' & \hfil10\hfil & 20\% \\
  ``bad'' & \hfil\hphantom{0}8\hfil & 16\% \\
  ``very bad'' & \hfil\hphantom{0}0\hfil & \hphantom{0}0\% \\[2mm]
  none & \hfil20\hfil & 40\% \\
\end{tabular}

\bigskip
What the lecturer did was to visualize the data using a 3D bar
diagram. It looked like this (except that in reality the numbers
where typeset using some extremely low-resolution bitmap font and
were near-unreadable):

\bigskip
\par
\begin{tikzpicture}[y=0.03cm,z=3mm]
  \foreach \y in {0,20,40,60,80,100}
    \draw[dashed] (0,\y,0) node[left] {\y} -- (0,\y,1)  -- (6,\y,1);

  \draw (0,0,0) -- (0,100,0)  (0,0,1) -- (0,100,1);
  \draw (0,0,0) -- (6,0,0);

  \foreach \x/\xtext/\height in {1/very good/10,2/good/30,3/ok/33,4/bad/27,5/very bad/0}
  {
    \draw (\x,0) node[rotate=90,anchor=east] {\xtext};

    \begin{scope}[xshift=\x cm]
      
    \filldraw[fill=blue!50] (-.3,0,0) rectangle (.3,\height,0);
    \filldraw[fill=blue!30] (.3,0,0) -- (.3,0,1) -- (.3,\height,1) -- (.3,\height,0) --cycle;
    \filldraw[fill=blue!20] (-.3,\height,0) -- (.3,\height,0) --
    (.3,\height,1) -- (-.3,\height,1) --cycle;
    \end{scope}
  }
\end{tikzpicture}
\bigskip

Both the table and the ``plot'' have about the same size. If your first
thought is ``the graphic looks nicer than the table,'' try to answer
the following questions based on the information in the table or in
the graphic: 
\begin{enumerate}
\item
  How many participants where there?
\item
  How many participants returned the feedback form?
\item
  What percentage of the participants returned the feedback form?
\item
  How many participants checked ``very good''?
\item
  What percentage out of all participants checked ``very good''?
\item
  Did more than a quarter of the participants check ``bad'' or ``very bad''?
\item
  What percentage of the participants that returned the form checked ``very good''?
\end{enumerate}

Sadly, the graphic does not allow us to answer \emph{a single one of these
  questions}. The table answers all of them directly, except for the last
one. In essence, the information density of the graphic is very
nearly zero. The table has a much higher information density; despite
the fact that it uses quite a lot of white space to present a few numbers.
Here is the list of things that went wrong with the 3D-bar diagram:
\begin{itemize}
\item
  The whole graphic is dominated by irritating background lines.
\item
  It is not clear what the numbers at the left mean; presumably
  percentages, but it might also be the absolute number of
  participants.
\item
  The labels at the bottom are rotated, making them hard to read.

  (In the real presentation that I saw, the text was rendered at a very 
  low resolution with about 10 by 6 pixels per letter with wrong
  kerning, making the rotated text almost impossible to read.)
\item
  The third dimension adds complexity to the graphic without adding
  information.
\item
  The three dimensional setup makes it much harder to gauge the height
  of the bars correctly. Consider the ``bad'' bar. It the number this
  bar stands for more than 20 or less? While the front of the bar is
  below the 20 line, the back of the bar (which counts) is above.
\item
  It is impossible to tell which  numbers are represented by the
  bars. Thus, the bars needlessly hide the information these bars are
  all about.
\item
  What do the bar heights add up to? Is it 100\% or 60\%?
\item
  Does the bar for ``very bad'' represent 0 or~1?
\item
  Why are the bars blue?
\end{itemize}

You might argue that in the example the exact numbers are not
important for the graphic. The important things is the ``message,''
which is that there are more ``very good'' and ``good'' ratings than
``bad'' and ``very bad.'' However, to convey this message either use a
sentence that says so or use a graphic that conveys this message more
clearly:  

\medskip
\par
\begin{tikzpicture}
  \colorlet{good}{green!75!black}
  \colorlet{bad}{red}
  \colorlet{neutral}{black!60}
  \colorlet{none}{white}

  \node[text centered,text width=3cm]{Ratings given by 50~participants};

  \begin{scope}[line width=4mm,rotate=270]
    \draw[good]          (-123:2cm) arc (-123:-101:2cm);
    \draw[good!60!white] (-36:2cm) arc (-36:-101:2cm);
    \draw[neutral]       (-36:2cm) arc (-36:36:2cm);
    \draw[bad!60!white]  (36:2cm)  arc (36:93:2cm);

    \newcount\mycount
    \foreach \angle in {0,72,...,3599}
    {
      \mycount=\angle\relax
      \divide\mycount by 10\relax
      \draw[black!15,thick] (\the\mycount:18mm) -- (\the\mycount:22mm);
    }
    
    \draw (0:2.2cm) node[below] {``ok'': 10 (20\%)};
    \draw (165:2.2cm) node[above] {none: 20 (40\%)};
    \draw (-111:2.2cm) node[left] {``very good'': 3 (6\%)};
    \draw (-68:2.2cm) node[left] {``good'': 9 (18\%)};
    \draw (65:2.2cm) node[right] {``bad'': 8 (16\%)};
    \draw (93:2.2cm) node[right] {``very bad'': 0 (0\%)};
  \end{scope}  
  \draw[gray] (0,0) circle (2.2cm) circle (1.8cm);
\end{tikzpicture}

\bigskip
The above graphic has about the same information density as the table
(about the same size and the same numbers are shown). In addition, one
can directly ``see'' that there are more good or very good ratings
than bad ones. One can also ``see'' that the number of people who gave
no rating at all is not negligible, which is quite common for feedback
forms. 

Charts are not always a good idea. Let us look at an example
that I redrew from a pie chart in \emph{Die Zeit}, June 4th, 2005:

\bigskip
\par
\begin{tikzpicture}
  \begin{scope}[xscale=3.2,yscale=1.2]

    \sffamily
    \coordinate (right border) at (2.0cm,-1.7cm);
    \coordinate (left border)  at (-2.5cm,2.1cm);

    \fill[black!25] ([xshift=-2mm,yshift=1.1cm]left border) rectangle ([xshift=2mm,yshift=-.3cm]right border);

    \node[below right,text width=10cm,inner sep=0pt] at ([yshift=.9cm,xshift=-1mm]left border)
    { {\color{black!75} \Large Kohle ist am wichtigsten}\\
      Energiemix bei der deutschen Stromerzeugung 2004};

    \filldraw[draw=gray,fill=white] ([xshift=-1mm]left border) node[below right,black]
      {\footnotesize Gesamte Netto-Stromerzeugung in Prozent, in
        Milliarden Kilowattstunden (Mrd.\ kWh)}
      rectangle ([xshift=1mm]right border);
    
    % The 3D stuff
    \pgfdeclarehorizontalshading{zeit}{100bp}
    {color(0pt)=(black);
      color(25bp)=(black);
      color(37bp)=(white);
      color(50bp)=(black);
      color(62bp)=(white);
      color(75bp)=(black);
      color(100bp)=(black)}

    \shadedraw[very thin,shading=zeit,yshift=-1.5mm] (0,0) circle (1cm);

    \fill[green!20!gray]   (0,0) -- (90:1cm) arc (90:-5:1cm);
    \fill[white!20!gray]   (0,0) -- (-5:1cm) arc (-5:-105:1cm);
    \fill[orange!20!gray]  (0,0) -- (-105:1cm) arc (-105:-180:1cm);
    \fill[orange!60!white] (0,0) -- (180:1cm) arc (180:150:1cm);
    \fill[black!75!white]  (0,0) -- (150:1cm) arc (150:145:1cm);
    \fill[blue!90!white]   (0,0) -- (145:1cm) arc (145:135:1cm);
    \fill[blue!50!white]   (0,0) -- (135:1cm) arc (135:92:1cm);
    \fill[yellow!50!black] (0,0) -- (92:1cm) arc (92:90:1cm);

    \begin{scope}[very thin]
      \draw (0,0) -- (90:1cm);
      \draw (0,0) -- (-5:1cm);
      \draw (0,0) -- (-105:1cm);
      \draw (0,0) -- (-180:1cm);
      \draw (0,0) -- (150:1cm);
      \draw (0,0) -- (145:1cm);
      \draw (0,0) -- (135:1cm);
      \draw (0,0) -- (92:1cm);
      
      \draw(0,0) circle (1cm);
    \end{scope}

    \node (Regenerative)   at (115:.75cm)  {\bfseries 9,4\%};
    \node (Kernenergie)    at (30:.5cm)   {\bfseries 27,8\%};
    \node (Braunkohle)     at (-45:.6cm)  {\bfseries 25,6\%};
    \node (Steinkohle)     at (-135:.6cm) {\bfseries 22,3\%};
    \node (Erdgas)         at (168:.75cm) {\bfseries 10,4\%};
    \coordinate (Mineral)  at (147:.9cm);
    \coordinate (Sonstige) at (140:.9cm);

    \small
    \draw (Regenerative.north) |- ([yshift=.25cm]Regenerative.north -| right border) coordinate (Regenerative label);
    \draw (91:.9cm) |- (Regenerative label);
    \node[above left] at (Regenerative label) {Regenerative\
      {\footnotesize (53,7 kWh)/davon} Wind \textbf{4,4\%}  \footnotesize (25,0 kWh)};

    \draw (Kernenergie.base east) -- (Kernenergie.base east -| right border) coordinate (Kernenergie label);
    \node[above left] at (Kernenergie label) {Kernenergie};
    \node[below left] at (Kernenergie label) {\footnotesize (158,4 kWh)};

    \draw (Braunkohle.south) |- ([yshift=-.75cm]Braunkohle.south -| right border) coordinate (Braunkohle label);
    \node[above left] at (Braunkohle label) {Braunkohle\ \ \footnotesize (146,0 kWh)};

    \draw (Steinkohle.south) |- ([yshift=-.75cm]Steinkohle.south -| left border) coordinate (Steinkohle label);
    \node[above right] at (Steinkohle label) {Steinkohle\ \ \footnotesize (127,1 kWh)};

    \draw (Erdgas.base west) -- (Erdgas.base west -| left border) coordinate (Erdgas label);
    \node[above right] at (Erdgas label) {Erdgas\ \ \footnotesize (59,2 kWh)};

    \draw (Mineral) -- (Mineral -| left border) coordinate (Mineral label);
    \node[above right] at (Mineral label) {Mineral\"olprodukte\ \
      \footnotesize (9,2 kWh) \  \ \normalsize\textbf{1,6\%}};

    \draw (Sonstige) |- (Regenerative label -| left border) coordinate (Sonstige label);
    \node[above right] at (Sonstige label) {Sonstige\ \
      \footnotesize (16,5 kWh) \hskip1.5cm\
      \normalsize\textbf{2,9\%}};
  \end{scope}    
\end{tikzpicture}

This graphic has been redrawn in \tikzname, but the original looks
almost exactly the same.

At first sight, the graphic looks  ``nice and informative,'' but there
are a lot of things that went wrong:

\begin{itemize}
\item
  The chart is three dimensional. However, the shadings add
  nothing ``information-wise,'' at best, they distract.
\item
  In a 3D-pie-chart the relative sizes are very strongly
  distorted. For example, the area taken up by the gray color of ``Braunkohle''
  is larger than the area taken up by the green color of
  ``Kernenergie'' \emph{despite the fact that the percentage of
    Braunkohle is less than the percentage of Kernenergie}.
\item
  The 3D-distortion gets worse for small areas. The area of
  ``Regenerative'' somewhat larger  than the area of ``Erdgas.''  
  The area of ``Wind'' is slightly smaller than the area of
  ``Mineral\"olprodukte'' \emph{although the percentage of Wind is
    nearly three times larger than the percentage of
    Mineral\"olprodukte.}

  In the last case, the different sizes are only partly due to
  distortion. The designer(s) of the original graphic have also made
  the ``Wind'' slice too small, even taking distortion into
  account. (Just compare the size of ``Wind'' to ``Regenerative'' in
  general.) 
\item
  According to its caption, this chart is supposed to inform us that
  coal was the most important energy source in Germany in
  2004. Ignoring the strong distortions caused by the superfluous and
  misleading 3D-setup, it takes quite a while for this message to get
  across. 

  Coal as an energy source is split up into two slices: one for
  ``Steinkohle'' and one for ``Braunkohle'' (two different kinds of
  coal). When you add them up, you see that the whole lower half of
  the pie chart is taken up by coal.

  The two areas for the different kinds of coal are not visually
  linked at all. Rather, two different colors are used, the labels are
  on different sides of the graphic. By comparison, ``Regenerative''
  and ``Wind'' are very closely linked.
\item
  The color coding of the graphic follows no logical pattern at
  all. Why is nuclear energy green? Regenerative energy is light blue,
  ``other sources'' are blue. It seems more like a joke that the area
  for ``Braunkohle'' (which literally translates to ``brown coal'') is
  stone gray, while the area for ``Steinkohle'' (which literally
  translates to ``stone coal'') is brown.
\item
  The area with the lightest color is used for ``Erdgas.'' This area
  stands out most because of the brighter color. However, for this
  chart ``Erdgas'' is not really important at all.
\end{itemize}
Edward Tufte calls graphics like the above ``chart junk.'' (I am happy
to announce, however, that \emph{Die Zeit} has stopped using 3D pie
charts and their information graphics have got somewhat better.)

Here are a few recommendations that may help you avoid producing chart junk:
\begin{itemize}
\item
  Do not use 3D pie charts. They are \emph{evil}.
\item
  Consider using a table instead of a pie chart.
\item
  Due not apply colors randomly; use them to direct the readers's 
  focus and to group things.
\item
  Do not use background patterns, like a crosshatch or diagonal
  lines, instead of colors. They distract. Background patterns in
  information graphics are \emph{evil}.
\end{itemize}



\subsection{Attention and Distraction}

Pick up your favorite fiction novel and have a look at a typical
page. You will notice that the page is very uniform. Nothing is there
to distract the reader while reading; no large headlines, no bold
text, no large white areas. Indeed, even when the author does wish to
emphasize something, this is done using italic letters. Such letters
blend nicely with the main text---at a distance you will not be able to
tell whether a page contains italic letters, but you would notice a
single bold word immediately. The reason novels are typeset this way
is the following paradigm: Avoid distractions.

Good typography (like good organization) is something you do
\emph{not} notice. The job of typography is to make reading the text,
that is, ``absorbing'' its information content, as effortless as
possible. For a novel, readers absorb the content by reading the text
line-by-line, as if they were listening to someone telling the
story. In this situation anything on the page that distracts the eye
from  going quickly and evenly from line to line will make the text
harder to read.

Now, pick up your favorite weekly magazine or newspaper and have a
look at a typical 
page. You will notice that there is quite a lot ``going on'' on the
page. Fonts are used at different sizes and in different arrangements,
the text is organized in narrow columns, typically interleaved with
pictures. The reason magazines are typeset in this way is another
paradigm: Steer attention.

Readers will not read a magazine like a novel. Instead of reading a
magazine line-by-line, we use headlines and short abstracts to check
whether we want to read a certain article or not. The job of
typography is to steer our attention to these abstracts and headlines,
first. Once we have decided that we want to read an article, however,
we no longer tolerate distractions, which is why the main text of
articles is typeset exactly the same way as a novel.

The two principles ``avoid distractions'' and ``steer attention'' also
apply to graphics. When you design a graphic, you should eliminate
everything that will ``distract the eye.'' At the same time, you
should try to actively help the reader ``through the graphic'' by
using fonts/colors/line widths to highlight different parts.

Here is a non-exhaustive list of things that can distract readers:
\begin{itemize}
\item
  Strong contrasts will always be registered first by the eye. For
  example, consider the following two grids:

  \medskip\par
  \begin{tikzpicture}[x=40pt,y=40pt]
    \draw[step=10pt,gray] (0,0) grid +(1,1);
    \draw[step=2pt]      (2,0) grid +(1,1);
  \end{tikzpicture}

  \medskip
  Even though the left grid comes first in English reading order,
  the right one is much more likely to be seen first: The
  white-to-black contrast is higher than the gray-to-white
  contrast. In addition, there are more ``places'' adding to the
  overall contrast in the right grid.

  Things like grids and, more generally, help lines usually should not
  grab the attention of the readers and, hence, should be typeset with
  a low contrast to the background. Also, a loosely-spaced grid is
  less distracting than a very closely-spaced grid.
\item
  Dashed lines create many points at which there is black-to-white
  contrast. Dashed or dotted lines can be very distracting and, hence,
  should be avoided in general.

  Do not use different dashing patterns to differentiate curves in
  plots. You loose data points this way and the eye is not
  particularly good at ``grouping things according to a dashing
  pattern.'' The eye is \emph{much} better at grouping things
  according to colors.
\item
  Background patterns filling an area using  diagonal lines or
  horizontal and vertical lines or just dots are almost always
  distracting and, usually, serve no real purpose.
\item
  Background images and shadings distract and only seldom add
  anything of importance to a graphic.
\item
  Cute little cliparts can easily draw attention away from the
  data.
\end{itemize}



==> pgfmanual-en-installation.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Installation}

There are different ways of installing \pgfname, depending
on your system and needs, and you may need to install other
packages as well as, see below. Before installing, you may wish to
review the licenses under which the package is
distributed, see Section~\ref{section-license}. 

Typically, the package will already be installed on your
system. Naturally, in this case you do not need to worry about the
installation process at all and you can skip the rest of this
section. 


\subsection{Package and Driver Versions}

This documentation is part of version \pgfversion\ of the \pgfname\
package. In order to run \pgfname, you need a reasonably recent 
\TeX\ installation. When using \LaTeX, you need the following packages
installed (newer versions should also work):
\begin{itemize}
\item
  |xcolor| version \xcolorversion.
\end{itemize}
With plain \TeX, |xcolor| is not needed, but you obviously do not
get its (full) functionality. 

Currently, \pgfname\ supports the following backend drivers:
\begin{itemize}
\item
  |pdftex| version 0.14 or higher. Earlier versions do not work.
\item
  |dvips| version 5.94a or higher. Earlier versions may also work.

  For inter-picture connections, you need process pictures using
  |pdftex| version 1.40 or higher running in DVI mode.
\item
  |dvipdfm| version 0.13.2c or higher. Earlier versions may also work.

  For inter-picture connections, you need process pictures using
  |pdftex| version 1.40 or higher running in DVI mode.
\item
  |tex4ht| version 2003-05-05 or higher. Earlier versions may also work.
\item
  |vtex| version 8.46a or higher. Earlier versions may also work.
\item
  |textures| version 2.1 or higher. Earlier versions may also work.
\item
  |xetex| version 0.996 or higher. Earlier versions may also work.
\end{itemize}

Currently, \pgfname\ supports the following formats:
\begin{itemize}
\item
  |latex| with complete functionality.
\item
  |plain| with complete functionality, except for graphics inclusion,
  which works only for pdf\TeX.
\item
  |context| with complete functionality, except for graphics inclusion,
  which works only for pdf\TeX.
\end{itemize}

For more details, see Section~\ref{section-formats}.



\subsection{Installing Prebundled Packages}

I do not create or manage prebundled packages of \pgfname, but,
fortunately, nice other people do. I cannot give detailed instructions
on how to install these packages, since I do not manage them, but I
\emph{can} tell you were to find them. If you have a problem with
installing, you might wish to have a look at the Debian page or the
Mik\TeX\ page first.


\subsubsection{Debian}

The command ``|aptitude install pgf|'' should do the trick. Sit back
and relax. In detail, the following packages are installed:  
\begin{verbatim}
http://packages.debian.org/pgf
http://packages.debian.org/latex-xcolor
\end{verbatim}


\subsubsection{MiKTeX}

For MiK\TeX, use the update wizard to install the (latest versions of
the) packages called |pgf| and |xcolor|. 




\subsection{Installation in a texmf Tree}

For a permanent installation, you place the files of the
the \textsc{pgf} package in an appropriate |texmf| tree. 

When you ask \TeX\ to use a certain class or package, it usually looks
for the necessary files in so-called |texmf| trees. These trees
are simply huge directories that contain these files. By default,
\TeX\ looks for files in three different |texmf| trees:
\begin{itemize}
\item
  The root |texmf| tree, which is usually located at
  |/usr/share/texmf/| or |c:\texmf\| or somewhere similar.
\item
  The local  |texmf| tree, which is usually located at
  |/usr/local/share/texmf/| or |c:\localtexmf\| or somewhere similar.
\item
  Your personal  |texmf| tree, which is usually located in your home
  directory at |~/texmf/| or |~/Library/texmf/|.   
\end{itemize}

You should install the packages either in the local tree or in
your personal tree, depending on whether you have write access to the
local tree. Installation in the root tree can cause problems, since an
update of the whole \TeX\ installation will replace this whole tree.


\subsubsection{Installation that Keeps Everything Together}

Once you have located the right texmf tree, you must decide whether
you want to install \pgfname\ in such a way that ``all its files are
kept in one place'' or whether you want to be
``\textsc{tds}-compliant,'' where \textsc{tds} means ``\TeX\ directory
structure.''

If you want to keep ``everything in one place,'' inside the |texmf|
tree that you have chosen create a sub-sub-directory called
|texmf/tex/generic/pgf| or
|texmf/tex/generic/pgf-|\texttt{\pgfversion}, if you prefer. Then
place all files of the |pgf| package in this directory. Finally,
rebuild \TeX's filename database. This is done by running the command
|texhash| or |mktexlsr| (they are the same). In Mik\TeX, there is a
menu option to do this. 


\subsubsection{Installation that is TDS-Compliant}

While the above installation process is the most ``natural'' one and
although I would like to recommend it since it makes updating and
managing the \pgfname\ package easy, it is not
\textsc{tds}-compliant. If you want to be \textsc{tds}-compliant,
proceed as follows: (If you do not know what \textsc{tds}-compliant
means, you probably do not want to be \textsc{tds}-compliant.)

The |.tar| file of the |pgf| package contains the following files and
directories at its root: |README|, |doc|,  |generic|, |plain|, and
|latex|. You should ``merge'' each of the four directories with the
following directories |texmf/doc|, |texmf/tex/generic|,
|texmf/tex/plain|, and |texmf/tex/latex|. For example, in the |.tar|
file the |doc| directory contains just the directory |pgf|, and this
directory has to be moved to |texmf/doc/pgf|. The root |README| file
can be ignored since it is reproduced in |doc/pgf/README|.

You may also consider keeping everything in one place and using
symbolic links to point from the \textsc{tds}-compliant directories to
the central installation.

\vskip1em
For a more detailed explanation of the standard installation process
of packages, you might wish to consult
\href{http://www.ctan.org/installationadvice/}{|http://www.ctan.org/installationadvice/|}.
However, note that the \pgfname\ package does not come with a
|.ins| file (simply skip that part).


\subsection{Updating the Installation}

To update your installation from a previous version, all you need to
do is to replace everything in the directory |texmf/tex/generic/pgf|
with the files of the new version (or in all the directories where
|pgf| was installed, if you chose a \textsc{tds}-compliant
installation). The easiest way to do this is to first delete the old
version and then proceed as described above. Sometimes, there are
changes in the syntax of certain command from version to version. If
things no longer work that used to work, you may wish to have a look
at the release notes and at the change log. 



==> pgfmanual-en-introduction.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Introduction}

The \pgfname\ package, where ``\pgfname'' is supposed to mean ``portable
graphics format'' (or ``pretty, good, functional'' if you
prefer\dots), is a package for creating graphics in an ``inline''  
manner. It defines a number of \TeX\ commands that draw
graphics. For example, the code |\tikz \draw (0pt,0pt) -- (20pt,6pt);|
yields the line \tikz \draw (0pt,0pt) -- (20pt,6pt); and the code
|\tikz \fill[orange] (1ex,1ex) circle (1ex);| yields \tikz
\fill[orange] (1ex,1ex) circle (1ex);.

In a sense, when you use \pgfname\ you ``program'' your graphics, just
as you ``program'' your document when you use \TeX.  You get all  
the advantages of the ``\TeX-approach to typesetting'' for your 
graphics: quick creation of simple graphics, precise positioning, the
use of macros, often superior typography. You also inherit all the
disadvantages: steep learning curve, no \textsc{wysiwyg}, small
changes require a long recompilation time, and the code does not
really ``show'' how things will look like. 



\subsection{Structure of the System}

The \pgfname\ system consists of different layers:

\begin{description}
\item[System layer:] This layer provides a complete abstraction of what is
  going on ``in the driver.'' The driver is a program like |dvips| or
  |dvipdfm| that takes a |.dvi| file as input and generates a |.ps| or
  a |.pdf| file. (The |pdftex| program also counts as a driver, even
  though it does not take a |.dvi| file as input. Never mind.) Each
  driver has its own syntax for the generation of graphics, causing
  headaches to everyone who wants to create graphics in a portable
  way. \pgfname's system layer ``abstracts away'' these
  differences. For example, the system command
  |\pgfsys@lineto{10pt}{10pt}| extends the current path  to the coordinate
  $(10\mathrm{pt},10\mathrm{pt})$ of the current
  |{pgfpicture}|. Depending on whether |dvips|, 
  |dvipdfm|, or |pdftex| is used to process the document, the system
  command will be converted to different |\special| commands.
  The system layer is as ``minimalistic'' as possible since each
  additional command makes it more work to port \pgfname\ to a new
  driver.

  As a user, you will not use the system layer directly.
\item[Basic layer:]
  The basic layer provides a set of basic commands that allow
  you to produce complex graphics in a much easier manner than by using
  the system layer directly. For example,  the system layer provides
  no commands for creating circles since circles can be composed from
  the more basic Bézier curves (well, almost). However, as a user you
  will want to have a simple command to create circles
  (at least I do) instead of having to write down half a page of
  Bézier  curve  support coordinates. Thus, the basic layer provides a
  command |\pgfpathcircle| that generates the necessary curve
  coordinates for you.

  The basic layer is consists of a \emph{core}, which consists of
  several interdependent packages that can only be loaded \emph{en
    bloc,} and additional \emph{modules} that extend the core by more
  special-purpose commands like node management or a plotting
  interface. For instance, the \textsc{beamer} package uses only the
  core and not, say, the |shapes| modules.
\item[Frontend layer:]
  A frontend (of which there can be several) is a set of commands
  or a special syntax that makes using the basic layer easier. A
  problem with directly using the basic layer is that code written for
  this layer is often too ``verbose.'' For example, to draw a simple
  triangle, you may need as many as five commands when using the basic
  layer: One for beginning a path at the first corner of the triangle,
  one for extending the path to the second corner, one for going to
  the third, one for closing the path, and one for actually painting
  the triangle (as opposed to filling it). With the |tikz| frontend
  all this boils down to a single simple \textsc{metafont}-like
  command: 
\begin{verbatim}
\draw (0,0) -- (1,0) -- (1,1) -- cycle;
\end{verbatim}

  There are different frontends:
  \begin{itemize}
  \item
    The \tikzname\ frontend is the ``natural'' frontend for \pgfname. It gives
    you access to all features of \pgfname, but it is intended to be
    easy to use. The syntax is a mixture of \textsc{metafont} and
    \textsc{pstricks} and some ideas of myself. This frontend is
    \emph{neither} a complete \textsc{metafont} compatibility layer nor
    a \textsc{pstricks} compatibility layer and it is not intended to
    become either. 
  \item
    The |pgfpict2e| frontend reimplements the standard \LaTeX\
    |{picture}|  environment and commands like |\line| or |\vector|
    using the \pgfname\ basic layer. This layer is not really ``necessary''
    since the |pict2e.sty| package does at least as good a job at
    reimplementing the |{picture}| environment. Rather, the idea
    behind this package is to have a simple demonstration of how a
    frontend can be implemented.
  \end{itemize}

  It would be possible to implement a |pgftricks| frontend that maps
  \textsc{pstricks} commands to \pgfname\ commands. However, I have not
  done this and even if fully implemented, many things that work in
  \pstricks\ will not work, namely whenever some \pstricks\ command
  relies too heavily on PostScript trickery. Nevertheless, such a
  package might be useful in some situations.
\end{description}

As a user of \pgfname\ you will use the commands of a
frontend plus perhaps some commands of the basic layer. For this
reason, this manual explains the frontends first, then the basic
layer, and finally the system layer.



\subsection{Comparison with Other Graphics Packages}

\pgfname\ is not the only graphics package for \TeX. In the following,
I try to give a reasonably fair comparison of the \pgfname-system and
other packages.
\begin{enumerate}
\item
  The standard \LaTeX\ |{picture}| environment allows you to create
  simple graphics, but little more. This is certainly not
  due to a lack of knowledge or imagination on the part of
  \LaTeX's designer(s). Rather, this is the price paid for the
  |{picture}| environment's portability: It works together with all
  backend drivers.
\item
  The |pstricks| package is certainly powerful enough to create
  any conceivable kind of graphic, but it is not portable at all. Most
  importantly, it does not work with |pdftex| nor with any other
  driver that produces anything but PostScript code.

  Compared to \pgfname, |pstricks| has a broader support base. There
  are many nice extra packages for special purpose situations that have
  been contributed by users over the last decade.

  The \tikzname\ syntax is more consistent than the |pstricks| syntax
  as \tikzname\ was developed ``in a more centralized manner'' and
  also ``with the shortcomings on |pstricks| in mind.''

  Note that a number of neat tricks that |pstricks| can do are
  impossible in \pgfname. In particular, |pstricks| has access to the
  powerful PostScript programming language, which allows trickery
  such as inline function plotting.
\item
  The |xypic| package is an older package for creating
  graphics. However, it is more difficult to use and to learn because
  the syntax and the documentation are a bit cryptic. 
\item
  The |dratex| package is a small graphic package for creating a
  graphics. Compared to the other package, including \pgfname, it is
  very small, which may or may not be an advantage. 
\item
  The |metapost| program is a very powerful alternative to
  \pgfname. However, it is an external program, which entails a
  bunch of problems. The time needed both to create a small graphic 
  and also to compile it is much greater than in \pgfname.
  The main problem with |metapost|, however, is the inclusion of
  labels. This is \emph{much} easier to achieve using \pgfname.
\item
  The |xfig| program is an important alternative to \tikzname\ for
  users who do not wish to ``program'' their graphics as is necessary
  with \tikzname\ and the other packages above. Their is a conversion
  program that will convert |xfig| graphics to both \tikzname\ and
  for \pgfname, but it is still under construction.
\end{enumerate}




\subsection{Utility Packages}

The \pgfname\ package comes along with a numer of utility package that
are not really about creating graphics and which can be used
independently of \pgfname. However, they are bundled with \pgfname,
partly out of convenience, partly because their functionality is
closely intertwined with \pgfname. These utility packages are: 
\begin{enumerate}
\item The |pgfkeys| package defines a powerful key management
  facility. It can be used completely independently of \pgfname.
\item The |pgffor| package defines a useful |\foreach| statement.
\item The |pgfcalendar| package defines macros for creating
  calendars. Typically, these calendars will be rendered using
  \pgfname's graphic engine, but you can use |pgfcalendar| also
  typeset calendars using normal text. The package also defines
  commands for ``working'' with dates.
\item The |pgfpages| package is used to assemble several pages into a
  single page. It provides commands for assembling several
  ``virtual pages'' into a single ``physical page.'' The idea is that
  whenever \TeX\ has a page ready for ``shipout,'' |pgfpages| interrupts
  this shipout and instead stores the page to be shipped out in a
  special box. When enough ``virtual pages'' have been accumulated in
  this way, they are scaled down and arranged on a ``physical page,''
  which then \emph{really} shipped out. This mechanism allows you to
  create ``two page on one page'' versions of a document directly inside
  \LaTeX\ without the use of any external programs. However,
  |pgfpages| can do quite a lot more than that. You can use it to put
  logos and watermark on pages, print up to 16 pages on one page, add
  borders to pages, and more. 
\end{enumerate}



\subsection{How to Read This Manual}

This manual describes both the design of the \pgfname\ system and
its usage. The organization is  very roughly according to
``user-friendliness.'' The commands and subpackages that are easiest
and most frequently used are described first, more low-level and
esoteric features are discussed later.

If you have not yet installed \pgfname, please read the installation
first. Second, it might be a good idea to read the tutorial. Finally,
you might wish to skim through the description of \tikzname. Typically, 
you will not need to read the sections on the basic layer. You will
only need to read the part on the system layer if you intend to write
your own frontend or if you wish to port \pgfname\ to a new driver.

The ``public'' commands and environments provided by the |pgf| package
are described throughout the text. In each such description, the
described command, environment or option is printed in red. Text shown
in green is optional and can be left out.


\subsection{Authors and Acknowledgements}
\label{section-authors}

The bulk of the \pgfname\ system and its documentation was written by
Till Tantau. The \pgfname\ mathematical engine, many shapes, and the
decoration engine were written and documented by Mark
Wibrow. Additionally, numerous people have contributed to the
\pgfname\ system by writing emails, spotting bugs, or sending
libraries. Many thanks to all these people, who are too numerous to
name them all! 



\subsection{Getting Help}

When you need help with \pgfname\ and \tikzname, please do the
following:

\begin{enumerate}
\item
  Read the manual, at least the part that has to do with your problem.
\item
  If that does not solve the problem, try having a look at the
  sourceforge development page for \pgfname\ and \tikzname\ (see the
  title of this document). Perhaps someone has already reported a
  similar problem and someone has found a solution.
\item
  On the website you will find numerous forums for getting
  help. There, you can write to help forums, file bug reports, join
  mailing lists, and so on.
\item
  Before you file a bug report, especially a bug report concerning the
  installation, make sure that this is really a bug. In particular,
  have a look at the |.log| file that results when you \TeX\ your
  files. This |.log| file should show that all the right files are
  loaded from the right directories. Nearly all installation problems
  can be resolved by looking at the |.log| file.
\item
  \emph{As a last resort} you can try to email me (Till Tantau) or, if
  the problem concerns the mathematical engine, Mark Wibrow. I do
  not mind getting emails, I simply get way too many of them. Because
  of this, I cannot guarantee that your emails will be answered timely
  or even at all. Your chances that your problem will be fixed are
  somewhat higher if you mail to the \pgfname\ mailing list
  (naturally, I read this list and answer questions when I have the
  time).
\item
  Please, do not phone me in my office (unless, of course, you attend
  one of my lectures).
\end{enumerate}



==> pgfmanual-en-library-3d.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Three Dimensional Drawing Library}

\begin{tikzlibrary}{3d}
  This packages, which is still under construction, provides some
  styles and options for drawing three dimensional shapes.

  \textbf{This package is not officially released and commands may
    change or disappear without backward compatibility support.}
\end{tikzlibrary}

This package is not yet documented. Here is, at least, an example of
where this whole thing is supposed to head.

\begin{codeexample}[]
\begin{tikzpicture}[z={(10:10mm)},x={(-45:5mm)}]  
  \def\wave{
    \draw[fill,thick,fill opacity=.2]
     (0,0) sin (1,1) cos (2,0) sin (3,-1) cos (4,0) 
           sin (5,1) cos (6,0) sin (7,-1) cos (8,0)
           sin (9,1) cos (10,0)sin (11,-1)cos (12,0);
    \foreach \shift in {0,4,8}
    {
      \begin{scope}[xshift=\shift cm,thin]
        \draw (.5,0)  -- (0.5,0 |- 45:1cm);
        \draw (1,0)   -- (1,1);
        \draw (1.5,0) -- (1.5,0 |- 45:1cm);
        \draw (2.5,0) -- (2.5,0 |- -45:1cm);
        \draw (3,0)   -- (3,-1);
        \draw (3.5,0) -- (3.5,0 |- -45:1cm);
      \end{scope}
    }
  }
  \begin{scope}[canvas is zy plane at x=0,fill=blue]
    \wave
    \node at (6,-1.5) [transform shape] {magnetic field};
  \end{scope}
  \begin{scope}[canvas is zx plane at y=0,fill=red]
    \draw[help lines] (0,-2) grid (12,2);
    \wave
    \node at (6,1.5) [rotate=180,xscale=-1,transform shape] {electric field};
  \end{scope}
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \begin{scope}[canvas is zy plane at x=0]
    \draw (0,0) circle (1cm);
    \draw (-1,0) -- (1,0) (0,-1) -- (0,1);
  \end{scope}

  \begin{scope}[canvas is zx plane at y=0]
    \draw (0,0) circle (1cm);
    \draw (-1,0) -- (1,0) (0,-1) -- (0,1);
  \end{scope}

  \begin{scope}[canvas is xy plane at z=0]
    \draw (0,0) circle (1cm);
    \draw (-1,0) -- (1,0) (0,-1) -- (0,1);
  \end{scope}
\end{tikzpicture}
\end{codeexample}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-arrows.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Arrow Tip Library}
\label{section-library-arrows}

\begin{pgflibrary}{arrows}
  The package defines additional arrow tips, which are described
  below. See page~\pageref{standard-arrows} for the arrows tips that
  are defined by default. Note that neither the standard packages nor
  this package defines an arrow name containing |>| or |<|. These are
  left for the user to defined as he or she sees fit.
\end{pgflibrary}

\subsection{Triangular Arrow Tips}

\begin{tabular}{ll}
  \symarrow{latex'} \\
  \symarrow{latex' reversed}  \\
  \symarrow{stealth'} \\
  \symarrow{stealth' reversed}\\
  \symarrow{triangle 90} \\
  \symarrow{triangle 90 reversed}   \\
  \symarrow{triangle 60} \\
  \symarrow{triangle 60 reversed}   \\
  \symarrow{triangle 45} \\
  \symarrow{triangle 45 reversed}   \\
  \symarrow{open triangle 90} \\
  \symarrow{open triangle 90 reversed}   \\
  \symarrow{open triangle 60} \\
  \symarrow{open triangle 60 reversed}   \\
  \symarrow{open triangle 45} \\
  \symarrow{open triangle 45 reversed}   \\
\end{tabular}

\subsection{Barbed Arrow Tips}

\begin{tabular}{ll}
  \symarrow{angle 90} \\
  \symarrow{angle 90 reversed}   \\
  \symarrow{angle 60} \\
  \symarrow{angle 60 reversed}   \\
  \symarrow{angle 45} \\
  \symarrow{angle 45 reversed}   \\
  \symarrow{hooks} \\
  \symarrow{hooks reversed} \\
\end{tabular}


\subsection{Bracket-Like Arrow Tips}

\begin{tabular}{ll}
  \sarrow{[}{]} \\
  \sarrow{]}{[} \\
  \sarrow{(}{)} \\
  \sarrow{)}{(}
\end{tabular}

\subsection{Circle and Diamond Arrow Tips}


\begin{tabular}{ll}
  \symarrow{o} \\
  \symarrow{*} \\
  \symarrow{diamond} \\
  \symarrow{open diamond}   \\
\end{tabular}



\subsection{Serif-Like Arrow Tips}

\begin{tabular}{ll}
  \symarrow{serif cm}
\end{tabular}


\subsection{Partial Arrow Tips}

\begin{tabular}{ll}
  \symarrow{left to} \\
  \symarrow{left to reversed} \\
  \symarrow{right to} \\
  \symarrow{right to reversed} \\
  \symarrow{left hook} \\
  \symarrow{left hook reversed} \\
  \symarrow{right hook} \\
  \symarrow{right hook reversed}
\end{tabular}



\subsection{Line Caps}

\begin{tabular}{ll}
  \carrow{round cap} \\
  \carrow{butt cap} \\
  \carrow{triangle 90 cap} \\
  \carrow{triangle 90 cap reversed} \\
  \carrow{fast cap} \\
  \carrow{fast cap reversed} \\
\end{tabular}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-automata.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Automata Drawing Library}

\begin{tikzlibrary}{automata}
  This packages provides shapes and styles for drawing finite state
  automata and Turing machines. 
\end{tikzlibrary}


\subsection{Drawing Automata}

The automata drawing library is intended to make it easy to draw
finite automata and Turing machines. It does not cover every
situation imaginable, but most finite automata and Turing machines
found in text books can be drawn in a nice and convenient fashion
using this library. 

To draw an automaton, proceed as follows:
\begin{enumerate}
\item For each state of the automaton, there should be one node with
  the option |state|.
\item To place the states, you can either use absolute positions or
  relative positions, using options like |above| or |right|.
\item Give a unique name to each state node.
\item Accepting and initial states are indicated by adding the
  options |accepting| and |initial|, respectively, to the state
  nodes.
\item Once the states are fixed, the edges can be added. For this, the
  |edge| operation is most useful. It is, however, also possible to
  add edges after each node has been placed.
\item For loops, use the |edge [loop]| operation.
\end{enumerate}

Let us now see how this works for a real example. Let us consider a
nondeterminsitic four state automaton that checks whether an contains
the sequence $0^*1$ or the sequence $1^*0$. 
\begin{codeexample}[]
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,auto]
  \draw[help lines] (0,0) grid (3,2);

  \node[state,initial]  (q_0)                      {$q_0$};
  \node[state]          (q_1) [above right=of q_0] {$q_1$};
  \node[state]          (q_2) [below right=of q_0] {$q_2$};
  \node[state,accepting](q_3) [below right=of q_1] {$q_3$};

  \path[->] (q_0) edge              node        {0} (q_1)
                  edge              node [swap] {1} (q_2)
            (q_1) edge              node        {1} (q_3)
                  edge [loop above] node        {0} ()
            (q_2) edge              node [swap] {0} (q_3)
                  edge [loop below] node        {1} ();
\end{tikzpicture}
\end{codeexample}


\subsection{States With and Without Output}

The |state| style actually just ``selects'' a default underlying
style. Thus, you can define multiple new complicated state style and
then simply set the |state| style to your given style to get the
desired kind of styles.

By default, the following state styles are defined:
\begin{stylekey}{/tikz/state without output}
  This node style causes nodes to be drawn circles. Also, this style
  calls |every state|.
\end{stylekey}

\begin{stylekey}{/tikz/state with output}
  This node style causes nodes to be drawn as split circles, that is,
  using the |circle split| shape. In the upper part of the shape you
  have the name of the style, in the lower part the output is
  placed. To specify the output, use the command |\nodepart{lower}|
  inside the node. This style also calls |every state|.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \node[state without output] {$q_0$};
  
  \node[state with output] at (2,0) {$q_1$ \nodepart{lower} $00$};
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/state (initially state without output)}
  You should redefine it to something else, if you wish to use states
  of a different nature.
\begin{codeexample}[]
\begin{tikzpicture}[state/.style=state with output]
  \node[state]          {$q_0$ \nodepart{lower} $11$};
  \node[state] at (2,0) {$q_1$ \nodepart{lower} $00$};
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/every state (initially \normalfont empyt)}
  This style is used by |state with output| and also by
  |state without output|. By default, it does nothing, but you can use
  it to make your state look more fancy:
\begin{codeexample}[]
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,>=stealth',
    every state/.style={draw=blue!50,very thick,fill=blue!20}]

  \node[state,initial]  (q_0)                      {$q_0$};
  \node[state]          (q_1) [above right=of q_0] {$q_1$};
  \node[state]          (q_2) [below right=of q_0] {$q_2$};

  \path[->] (q_0) edge              node [above left]  {0} (q_1)
                  edge              node [below left]  {1} (q_2)
            (q_1) edge [loop above] node               {0} ()
            (q_2) edge [loop below] node               {1} ();
\end{tikzpicture}
\end{codeexample}
\end{stylekey}


\subsection{Initial and Accepting States}

The styles |initial| and |accepting| are similar to the |state| style
as they also just select an ``underlying'' style, which installs the
actual settings for initial and accepting states.

Let us start with the initial states.
\begin{stylekey}{/tikz/initial (initially initial by arrow)}
  This style is used to draw initial states.
\end{stylekey}
\begin{stylekey}{/tikz/initial by arrow}
  This style causes an arrow and, possibly, some text to be added to
  the node. The arrow points from the text to the node. The node text
  and the direction and the distance can be set using the following
  key:
  \begin{key}{/tikz/initial text=\meta{text} (initially start)}
    This key sets the text to be used. Use an empty text to suppress
    all text.
  \end{key}
  \begin{key}{/tikz/initial where=\meta{direction} (initially left)}
    Set the place where the text should be shown. Allowed values are
    |above|, |below|, |left|, and |right|.
  \end{key}
  \begin{key}{/tikz/intial distance=\meta{distance} (initially 3ex)}
    Sets the length of the arrow leading from the text to the state
    node.
  \end{key}
  \begin{stylekey}{/tikz/every initial by arrow (initially \normalfont empty)}
    This style is executed at the beginning of every path that contains
    the arrow and the text. You can use it to, say, make the text red or
    whatever.
  \end{stylekey}
\begin{codeexample}[]
\begin{tikzpicture}[every initial by arrow/.style={text=red,->>}]
  \node[state,initial,initial distance=2cm] {$q_0$};
\end{tikzpicture}
\end{codeexample}
  %<<
\end{stylekey}
\begin{stylekey}{/tikz/initial above}
  This is a shorthand for |initial by arrow,initial where=above|.
\end{stylekey}
\begin{stylekey}{/tikz/initial below}
  Works similarly to the previous option.
\end{stylekey}
\begin{stylekey}{/tikz/initial left}
  Works similarly to the previous option.
\end{stylekey}
\begin{stylekey}{/tikz/initial right}
  Works similarly to the previous option.
\end{stylekey}

\begin{stylekey}{/tikz/initial by diamond}
  This style uses a diamond to indicate an initial node. 
\end{stylekey}

For the accepting states, the sitation is similar: There is also an
|accepting| style that selects the way accepting states are
rendered. There are now two options: First,
|accepting by arrow|, which works the same way as |initial by arrow|,
only with the direction of arrow reversed, and |accepting by double|,
where accepting states get a double line around them.

\begin{stylekey}{/tikz/accepting (initially accepting by double)}
  This style is used to draw accepting states.  You can replace
  this by the style |accepting by arrow| to get accepting states with
  an arrow leaving them.
\end{stylekey}

\begin{stylekey}{/tikz/accepting by double}
  This style causes a double line to be drawn arond a state.
\end{stylekey}

\begin{stylekey}{/tikz/accepting by arrow}
  This style causes an arrow and, possibly, some text to be added to
  the node. The arrow points to the text from the node.

  The same options as for initial states can be used, only with
  |initial| replaced by |accepting|:
  \begin{key}{/tikz/accepting text=\meta{text} (initially \normalfont empty)}
    This key sets the text to be used.
  \end{key}
  \begin{key}{/tikz/accepting where=\meta{direction} (initially right)}
    Set the place where the text should be shown. Allowed values are
    |above|, |below|, |left|, and |right|.
  \end{key}
  \begin{key}{/tikz/intial distance=\meta{distance} (initially 3ex)}
    Sets the length of the arrow leading from the text to the state
    node.
  \end{key}
  \begin{stylekey}{/tikz/every accepting by arrow (initially \normalfont empty)}
    Executed at the beginning of every path that contains
    the arrow and the text.
  \end{stylekey}  
\begin{codeexample}[]
\begin{tikzpicture}
  [shorten >=1pt,node distance=2cm,on grid,>=stealth',initial text=,
   every state/.style={draw=blue!50,very thick,fill=blue!20},
   accepting/.style=accepting by arrow]

  \node[state,initial]  (q_0)                      {$q_0$};
  \node[state]          (q_1) [above right=of q_0] {$q_1$};
  \node[state]          (q_2) [below right=of q_0] {$q_2$};
  \node[state,accepting](q_3) [below right=of q_1] {$q_3$};

  \path[->] (q_0) edge              node [above left]  {0} (q_1)
                  edge              node [below left]  {1} (q_2)
            (q_1) edge              node [above right] {1} (q_3)
                  edge [loop above] node               {0} ()
            (q_2) edge              node [below right] {0} (q_3)
                  edge [loop below] node               {1} ();
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/accepting above}
  This is a shorthand for |accepting by arrow,accepting where=above|.
\end{stylekey}
\begin{stylekey}{/tikz/accepting below}
  Works similarly to the previous option.
\end{stylekey}
\begin{stylekey}{/tikz/accepting left}
  Works similarly to the previous option.
\end{stylekey}
\begin{stylekey}{/tikz/accepting right}
  Works similarly to the previous option.
\end{stylekey}



\subsection{Examples}

In the following example, we once more typeset the automaton presented
in the previous sections. This time, we use the following rule for
accepting/initial state: Initial states are red, accepting states are
green, and normal states are orange. Then, we must find a path from a
red state to a green state. 

\begin{codeexample}[]
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid,>=stealth',thick,
    every state/.style={fill,draw=none,orange,text=white,circular drop shadow},
    accepting/.style  ={green!50!black,text=white},
    initial/.style    ={red,text=white}]

  \node[state,initial]  (q_0)                      {$q_0$};
  \node[state]          (q_1) [above right=of q_0] {$q_1$};
  \node[state]          (q_2) [below right=of q_0] {$q_2$};
  \node[state,accepting](q_3) [below right=of q_1] {$q_3$};

  \path[->] (q_0) edge              node [above left]  {0} (q_1)
                  edge              node [below left]  {1} (q_2)
            (q_1) edge              node [above right] {1} (q_3)
                  edge [loop above] node               {0} ()
            (q_2) edge              node [below right] {0} (q_3)
                  edge [loop below] node               {1} ();
\end{tikzpicture}
\end{codeexample}

The next example is the current candidate for the five-state busiest
beaver:

\begin{codeexample}[]
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,%
                    auto,node distance=2cm,on grid,semithick,
                    inner sep=2pt,bend angle=45]
  \node[initial,state] (A)                    {$q_a$};
  \node[state]         (B) [above right=of A] {$q_b$};
  \node[state]         (D) [below right=of A] {$q_d$};
  \node[state]         (C) [below right=of B] {$q_c$};
  \node[state]         (E) [below=of D]       {$q_e$};

  \path [every node/.style={font=\footnotesize}]
        (A) edge              node {0,1,L} (B)
            edge              node {1,1,R} (C)
        (B) edge [loop above] node {1,1,L} (B)  
            edge              node {0,1,L} (C)
        (C) edge              node {0,1,L} (D)
            edge [bend left]  node {1,0,R} (E)    
        (D) edge [loop below] node {1,1,R} (D)
            edge              node {0,1,R} (A)
        (E) edge [bend left]  node {1,0,R} (A);
\end{tikzpicture}
\end{codeexample}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-backgrounds.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.



\section{Background Library}

\label{section-tikz-backgrounds}

\begin{tikzlibrary}{backgrounds}
  This library defines ``backgrounds'' for pictures. This does not
  refer to background pictures, but rather to frames drawn around and
  behind pictures. For example, this package allows you to just add
  the |framed| option to a picture to get a rectangular box around
  your picture or |gridded| to put a grid behind your picture.
\end{tikzlibrary}

When this package is loaded, the following styles become available:
\begin{stylekey}{/tikz/show background rectangle}
  This style causes a rectangle to be drawn behind your graphic. This
  style option must be given to the |{tikzpicture}| environment or to
  the |\tikz| command.
\begin{codeexample}[]
\begin{tikzpicture}[show background rectangle]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
  The size of the background rectangle is determined as follows:
  We start with the bounding box of the picture. Then, a certain
  separator distance is added on the sides. This distance can be
  different for the $x$- and $y$-directions and can be set using the
  following options:
  \begin{key}{/tikz/inner frame xsep=\meta{dimension} (initially 1ex)}
    Sets the additional horizontal separator distance for the
    background rectangle.    
  \end{key}
  \begin{key}{/tikz/inner frame ysep=\meta{dimension} (initially 1ex)}
    Same for the vertical separator distance.
  \end{key}  
  \begin{key}{/tikz/inner frame sep=\meta{dimension}}
    Sets the horizontal and vertical separator distances
    simultaneously. 
  \end{key}
  The following two styles make setting the inner separator a bit
  easier to remember:
  \begin{stylekey}{/tikz/tight background}
    Sets the inner frame separator to 0pt. The background rectangle
    will have the size of the bounding box. 
  \end{stylekey}
  \begin{stylekey}{/tikz/loose background}
    Sets the inner frame separator to 2ex.
  \end{stylekey}  

  You can influence how the background rectangle is rendered by setting
  the following style:
  \begin{stylekey}{/tikz/background rectangle (initially draw)}
    This style dictates how the background rectangle is drawn or
    filled. The default setting causes the path of the background
    rectangle to be drawn in the usual 
    way. Setting this style to, say, |fill=blue!20| causes a light
    blue background to be added to the picture. You can also use more
    fancy settings as shown in the following example:
\begin{codeexample}[]
\begin{tikzpicture}
  [background rectangle/.style=
     {double,ultra thick,draw=red,top color=blue,rounded corners},  
   show background rectangle]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
    Naturally, no one in their right mind would use the above, but
    here is a nice background: 
\begin{codeexample}[]
\begin{tikzpicture}
  [background rectangle/.style=
     {draw=blue!50,fill=blue!20,rounded corners=1ex},
   show background rectangle]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
\end{stylekey}

\begin{stylekey}{/tikz/framed}
  This is a shorthand for |show background rectangle|.
\end{stylekey}

\begin{stylekey}{/tikz/show background grid}
  This style behaves similarly to the |show background rectangle|
  style, but it will not use a rectangle path, but a grid. The lower
  left and upper right corner of the grid is computed in the same way
  as for the background rectangle:
\begin{codeexample}[]
\begin{tikzpicture}[show background grid]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
  You can influence the background grid by setting
  the following style:
  \begin{stylekey}{/tikz/background grid (initially draw,help lines)}
    This style dictates how the background grid path is drawn. 
\begin{codeexample}[]
\begin{tikzpicture}
  [background grid/.style={thick,draw=red,step=.5cm},
   show background grid]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
  This option can be combined with the |framed| option (use the
  |framed| option first):
\begin{codeexample}[]
\tikzset{background grid/.style={thick,draw=red,step=.5cm},
         background rectangle/.style={rounded corners,fill=yellow}}
\begin{tikzpicture}[framed,gridded]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/gridded}
  This is a shorthand for |show background grid|.
\end{stylekey}

\begin{stylekey}{/tikz/show background top}
  This style causes a single line to be drawn at the top of the
  background rectangle. Normally, the line coincides exactly with the
  top line of the background rectangle:
\begin{codeexample}[]
\begin{tikzpicture}[
    background rectangle/.style={fill=yellow},
    framed,show background top]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
  The following option allows you to lengthen (or shorten) the line:
  \begin{key}{/tikz/outer frame xsep=\meta{dimension} (initially 0pt)}
    The \meta{dimension} is added at the left and right side of the
    line. 
\begin{codeexample}[]
\begin{tikzpicture}
  [background rectangle/.style={fill=yellow},
   framed,
   show background top,
   outer frame xsep=1ex]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  \begin{key}{/tikz/outer frame ysep=\meta{dimension} (initially 0pt)}
    This option does not apply to the top line, but to the left and
    right lines, see below.
  \end{key}
  \begin{key}{/tikz/outer frame sep=\meta{dimension}}
    Sets both the $x$- and $y$-separation.
  \end{key}
\begin{codeexample}[]
\begin{tikzpicture}
  [background rectangle={fill=blue!20},
   outer frame sep=1ex,%
   show background top,%
   show background bottom,%
   show background left,%
   show background right]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
  You can influence how the line is drawn grid by setting
  the following style:
  \begin{stylekey}{/tikz/background top (initially draw)}
\begin{codeexample}[]
\tikzset{background rectangle/.style={fill=blue!20},
         background top/.style={draw=blue!50,line width=1ex}}
\begin{tikzpicture}[framed,show background top]
  \draw (0,0) ellipse (10mm and 5mm);
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
\end{stylekey}

\begin{stylekey}{/tikz/show background bottom}
  Works like the style for the top line.
\end{stylekey}
\begin{stylekey}{/tikz/show background left}
  Works similarly.
\end{stylekey}
\begin{stylekey}{/tikz/show background right}
  Works similarly.
\end{stylekey}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-calendar.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Calendar Library}

\label{section-calender}

\begin{tikzlibrary}{calendar}
  The library defines the |\calendar| command, which can be used to
  typeset calendars. The command relies on the |\pgfcalendar| command
  from the |pgfcalendar| package, which is loaded automatically.

  The |\calendar| command is quite configurable, allowing you to
  produce all kinds of different calendars.
\end{tikzlibrary}


\subsection{Calendar Command}

The core command for creating calendars in \tikzname\ is the
|\calendar| command. It is available only inside |{tikzpicture}|
environments (similar to, say, the |\draw| command). 

\begin{command}{\calendar \meta{calendar specification}|;|}
  The syntax for this command is similar to commands like |\node| or
  |\matrix|. However, it has its complete own parser and only those
  commands described in the following will be recognized, nothing
  else. Note, furthermore, that a \meta{calendar specification} is not
  a path specification, indeed, no path is created for the calendar.

  \medskip
  \textbf{The specification syntax.}
  The \meta{calendar specification} must be a sequence of
  elements, each of which has one of the following structures:
  \begin{itemize}
  \item |[|\meta{options}|]|

    You provide \meta{options} in square brackets as
    in |[red,draw=none]|. These \meta{options} can be any \tikzname\ 
    option and they apply to the whole calendar. You can provide this
    element multiple times, the effect accumulates.
  \item |(|\meta{name}|)|

    This has the same effect as saying |[name=|\meta{name}|]|. The
    effect of providing a \meta{name} is explained later. Note
    alreadys that \emph{a calendar is not a node} and the \meta{name}
    is \emph{not the name of a node}.
  \item |at (|\meta{coordinate}|)|

    This has the same effect as saying |[at=(|\meta{coordinate}|)]|.
  \item |if (|\meta{date condition}|)| \meta{options or
      commands}\opt{|else|\meta{else options or commands}}

    The effect of such an |if| is explained later.
  \end{itemize}

  At the beginning of every calendar, the following style is used:
  \begin{stylekey}{/tikz/every calendar (initially \normalfont empty)}
    This style is used with every calendar.
  \end{stylekey}
  
  \medskip
  \textbf{The date range.}
  The overall effect of the |\calendar| command is to execute code for
  each day of a range of dates. This range of dates is set using the
  following option:
  \begin{key}{/tikz/dates=\meta{start date}| to |\meta{end date}}
    This
    option specifies the date range. Both the start and end date are
    specified as described on page~\pageref{calendar-date-format}. In
    short: You can provide ISO-format type dates like |2006-01-02|, you
    can replace the day of month by |last| to refer to the last day of a
    month (so |2006-02-last| is the same as |2006-02-28|), and you can
    add a plus sign followed by a number to specify an offset (so
    |2006-01-01+-1| is the same as |2005-12-31|).
  \end{key}
  It will be useful to fix two pieces of terminology for the following
  descriptions: The |\calendar| command iterates over the dates in the
  range. The \emph{current date} refers to the current date the
  command is processing as it iterates over the dates. For each
  current date code is executed, which will be called the
  \emph{current date code}. The current date code consists of
  different parts, to be detailed later.
  
  The central part of the current date code is the execution of the
  code |\tikzdaycode|. By default, this code simply produces a node
  whose text is set to the day of month. This means that unless further
  action is taken, all days of a calendar will be put on top of each
  other! To avoid this, you must modify the current date code to shift
  days around appropriately. Predefined arrangements like 
  |day list downward| or |week list| do this for you, but you can
  define arrangements yourself. Since defining an arrangement is a bit
  tricky, it is explained only later on. For the time being, let us
  use a predefined arrangement to produce our first calendar:

\begin{codeexample}[]
\tikz \calendar[dates=2000-01-01 to 2000-01-31,week list];  
\end{codeexample}

  \medskip
  \textbf{Changing the spacing.}
  In the above calendar, the spacing between the days is determined by
  the numerous options. Most arrangement do not use all of these
  options, but only those that apply naturally.
  \begin{key}{/tikz/day xshift=\meta{dimension} (initially 3.5ex)}
    Specifies the
    horizontal shift between days. This is not the gap between days,
    but the shift between the anchors of their nodes.
\begin{codeexample}[]
\tikz \calendar[dates=2000-01-01 to 2000-01-31,week list,day xshift=3ex];  
\end{codeexample}
  \end{key}
  \begin{key}{/tikz/day yshift=\meta{dimension} (initially 3ex)}
    Specifies the
    vertical shift between days. Again, this is the shift between the
    anchors of their nodes.
\begin{codeexample}[]
\tikz \calendar[dates=2000-01-01 to 2000-01-31,week list,day yshift=2ex];  
\end{codeexample}
  \end{key}
  \begin{key}{/tikz/month xshift=\meta{dimension}}
    Specifies an additional  horizontal shift between different
    months.
  \end{key}
  \begin{key}{/tikz/month yshift=\meta{dimension}}
    Specifies an
    additional  vertical shift between different months. 
\begin{codeexample}[]
\tikz \calendar[dates=2000-01-01 to 2000-02-last,week list,
                month yshift=0pt];  
\end{codeexample}
\begin{codeexample}[]
\tikz \calendar[dates=2000-01-01 to 2000-02-last,week list,
                month yshift=1cm];  
\end{codeexample}
  \end{key}

  \medskip
  \textbf{Changing the position of the calendar.}
  The calendar is placed in such a way that, normally, the anchor of
  the first day label is at the origin. This can be changed by using
  the |at| option. When you say |at={(1,1)}|, this anchor of the first
  day will lie at coordinate $(1,1)$.

  In general, arrangements will not always place the anchor of the
  first day at the origin. Sometimes, additional spacing rules get in
  the way. There are different ways of addressing this problem: First,
  you can just ignore it. Since calendars are often placed in their own
  |{tikzpicture}| and since their size if computed automatically, the
  exact position of the origin often does not matter at all. Second,
  you can put the calendar inside a node as in
  |...node {\tikz \calendar...}|. This allows you to position the node
  in the normal ways using the node's anchors. Third, you can be very
  clever and use a single-cell matrix. The advantage is that a matrix
  allows you to provide any anchor of any node inside the matrix as an
  anchor for the whole matrix. For example, the following calendar is
  placed in such a way the center of 2000-01-20 lies on the position
  $(2,2)$:
\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[help lines] (0,0) grid (3,2);
  \matrix [anchor=cal-2000-01-20.center] at (2,2)
  { \calendar(cal)[dates=2000-01-01 to 2000-01-31,week list]; \\};
\end{tikzpicture}
\end{codeexample}
  Unfortunately, the matrix-base positions, which is the cleanest way,
  isnot as portable as the other approaches (it currently does not
  work with the \textsc{svg} backend for instance). 

  \medskip
  \textbf{Changing the appearance of days.}
  As mentioned before, each day in the above calendar is produced by
  an execution of the |\tikzdaycode|. Each time this code is executed,
  the coordinate system will have been setup appropriately to place
  the day of the month correctly. You can change both the code and its
  appearance using the following options.
  \begin{key}{/tikz/day code=\meta{code} (initially \normalfont see below)}
    This option allows you to change the code that is executed for
    each day. The default is to create a node with an appropriate
    name, but you can change this:
\begin{codeexample}[]
\tikz \calendar[dates=2000-01-01 to 2000-01-31,week list,
                day code={\fill[blue] (0,0) circle (2pt);}];  
\end{codeexample}
    The default code is the following:
\begin{codeexample}[code only]
\node[name=\pgfcalendarsuggestedname,every day]{\tikzdaytext};
\end{codeexample}
    The first part causes the day nodes to be accessible via the
    following names: If \meta{name} is the name given to the calendar
    via a |name=| option or via the specification element
    |(|\meta{name}|)|, then |\pgfcalendarsuggestedname| will expand to
    \meta{name}|-|\meta{date}, where \meta{date} is the date of the
    day that is currently being processed in ISO format .

    For example, if January 1, 2006 is being processed and the
    calendar has been named |mycal|, then the node containg the |1|
    for this date will be names |mycal-2006-01-01|. You can later
    reference this node.
\begin{codeexample}[]
\begin{tikzpicture}
  \calendar (mycal) [dates=2000-01-01 to 2000-01-31,week list];

  \draw[red] (mycal-2000-01-20) circle (4pt);
\end{tikzpicture}
\end{codeexample}
  \end{key}

  \begin{key}{/tikz/day text=\meta{text}}
    This option changes the setting of the |\tikzdaytext|. By default,
    this macro simply yields the current day of month, but you can
    change it arbitrarily. Here is a silly example:
\begin{codeexample}[]
\tikz \calendar[dates=2000-01-01 to 2000-01-31,week list,
                day text=x];  
\end{codeexample}
    More useful examples are based on using the |\%| command. This
    command is redefined inside a |\pgfcalendar| to mean the same as
    |\pgfcalendarshorthand|. (The original meaning of |\%| is lost
    inside the calendar, you need to save if before the calendar if
    you really need it.)

    The |\%| inserts the current day/month/year/day of week in a
    certain format into the text. The first letter following the |\%|
    selects the type (permisslbe values are |d|, |m|, |y|, |w|), the
    second letter specifies how the value should be displayed (|-|
    means numerically, |=| means numerically with leading
    space, |0| means numerically with leading zeros, |t| means
    textual, and |.| means textual, abbreviated). For example |\%d0|
    gives the day with a leading zero (for more details see
    the description of |\pgfcalendarshorthand| on
    page~\pageref{pgfcalendarshorthand}).

    Let us redefine the |day text| so that it yields the day with a
    leading zero:
\begin{codeexample}[leave comments]
\tikz \calendar[dates=2000-01-01 to 2000-01-31,week list,
                day text=\%d0];  
\end{codeexample}
  \end{key}

  \begin{stylekey}{/tikz/every day (initially anchor=base east)}
    This style is executed by the default node code for each day.
    The |every day| style is useful for changing the way days
    look. For example, let us make all days red:
\begin{codeexample}[leave comments]
\tikz[every day/.style=red]
  \calendar[dates=2000-01-01 to 2000-01-31,week list];
\end{codeexample}
  \end{stylekey}


  \medskip
  \textbf{Changing the appearance of month and year labels.}
  In addition to the days of a calendar, labels for the months and
  even years (for really long calendars) can be added. These labels
  are only added once per month or year and this is not done by
  default. Rather, special styles starting with |month label|
  place these labels and make them visible:
\begin{codeexample}[]
\tikz \calendar[dates=2000-01-01 to 2000-02-last,week list,
                month label above centered];
\end{codeexample}

  The following options change the appearance of the month and year
  label:
  \begin{key}{/tikz/month code=\meta{code} (initially \normalfont see below)}
    This option allows you to specify what the macro |\tikzmonthcode|
    should expand to.

    By default, the |\tikzmonthcode| it is set to
\begin{codeexample}[code only]
\node[every month]{\tikzmonthtext};
\end{codeexample}
    Note that this node is not named by default.
  \end{key}

  \begin{key}{/tikz/month text=\meta{text}}
    This option allows you to change the macro |\tikzmonthtext|. By
    default, the month text is a long textual presentation of the
    current month being typeset. 
\begin{codeexample}[leave comments]
\tikz \calendar[dates=2000-01-01 to 2000-01-31,week list,
                month label above centered,  
                month text=\textcolor{red}{\%mt} \%y-];
\end{codeexample}
  \end{key}

  \begin{stylekey}{/tikz/every month (initially \normalfont empty)}
    This style can be used to change the
    appearance of month labels.
  \end{stylekey}

  \begin{key}{/tikz/year code=\meta{code}}
    Works like |month code|, only for years.
  \end{key}

  \begin{key}{/tikz/year text=\meta{text}}
    Works like |month text|, only for years.
  \end{key}


  \begin{key}{/tikz/every year}
    Works like |every month|, only for years.
  \end{key}
  
  \medskip
  \textbf{Date ifs.}
  Much of the power of the |\calendar| command comes from the use of
  conditionals. There are two equivalent way of specifying such a
  conditional. First, you can add the text
  |if (|\meta{conditions}|) |\meta{code or options} to your
  \meta{calendar specification}, possibly followed by |else|\meta{else
    code or options}. You can have multiple such conditionals (but
  you cannot nest them in this simple manner). The second way is to
  use the following option:
  \begin{key}{/tikz/if=|(|\meta{coditions}|)|\meta{code or
        options}\opt{|else|\meta{else code or options}}}
    This option has
    the same effect as giving a corresponding if in the \meta{calendar
      specification}.  The option is mostly useful for use in the
    |every calendar| style, where you cannot provide if conditionals
    otherwise. 
  \end{key}
  Now, regardless of how you specify a conditional, it has the
  following effect (individually and independently for each date in
  the calendar):
  \begin{enumerate}
  \item It is checked whether the current date is one of the
    possibilities listed in \meta{coditions}. An example of such a
    condition is |Sunday|. Thus, when you write
    |if (Saturday,Sunday) {foo}|,  then |foo| will be executed for
    every day in the calendar that is a Saturday \emph{or} a Sunday.

    The command |\ifdate| and, thereby, |\pgfcalendarifdate| are used
    to evaluate the \meta{conditions}, see
    page~\pageref{pgfcalendarifdate} for a complete list of possible
    tests. The most useful tests are: Tests like |Monday| and so on,
    |workday| for the days Monday to Friday, |weekend| for Saturday
    and Sunday, |equals| for testing whether the current date equals a
    given date, |at least| and  |at least| for comparing the current
    date with a given date.
  \item If the date passes the check, the \meta{code or options} is
    evaluated in a manner to be described in a moment; if the date
    fails, the \meta{else code or options} is evaluated, if present.

    The \meta{code or options} can either be some code. This is
    indicated by surrounding the code with curly braces. It can also
    be a list of \tikzname\ options. This is indicated by surrounding
    the options with square brackets. For example in the date test
    |if (Sunday) {\draw...} else {\fill...}| there are two pieces of
    code involved. By comparison, |if (Sunday) [red] else [green]|
    involves two options.

    If \meta{code or options} is code, it is simply executed (for the
    current day). If it is a list of options, these options are passed
    to a scope surrounding the current date.
  \end{enumerate}
  Let us now have a look at some examples. First, we use a conditional
  to make all Sundays red.
\begin{codeexample}[]
\tikz
  \calendar
    [dates=2000-01-01 to 2000-01-31,week list]
    if (Sunday) [red];
\end{codeexample}
  Next, let us do something on a specific date:
\begin{codeexample}[]
\tikz
  \calendar
    [dates=2000-01-01 to 2000-01-31,week list]
    if (Sunday)            [red]
    if (equals=2000-01-20) {\draw (0,0) circle (8pt);};
\end{codeexample}
  You might wonder why the circle seems to be ``off'' the
  date. Actually, it is centered on the date, it is just that the date
  label uses the |base east| anchor, which shifts the label up and
  right. To overcome this problem we can change the anchor:
\begin{codeexample}[]
\tikz [every day/.style={anchor=mid}]
  \calendar
    [dates=2000-01-01 to 2000-01-31,week list]
    if (Sunday)            [red]
    if (equals=2000-01-20) {\draw (0,0) circle (8pt);};
\end{codeexample}
  However, the single day dates are now no longer aligned
  correctly. For this, we can change the day text to |\%d=|,
  which adds a space at the beginning of single day
  text.
  
  In the following, more technical information is covered. Most
  readers may wish to skip it.

  \medskip
  \textbf{The current date code.}
  As mentioned earlier, for each date in the calendar the current date
  code is executed. It is the job of this code to shift around date
  nodes, to render the date nodes, to draw the month labels and to do
  all other stuff that is necessary to draw a calendar.

  The current daet code consists of the following parts, in this order:
  \begin{enumerate}
  \item The before-scope code.
  \item A scope is opened.
  \item The at-begin-scope code.
  \item All date-ifs from the \meta{calendar specification} are
    executed.
  \item The at-end-scope code.
  \item The scope is closed.
  \item The after-scope code.
  \end{enumerate}
  All of the codes mentioned above can be changed using appropriate
  options, see below. In case you wonder why so many are needed, the
  reason is that the current date code as a whole is not
  surrounded by a scope or \TeX\ group. This means that code executed
  in the before-scope code and in the after-scope code has an effect
  on all following days. For example, if the after-scope code modifies
  the transformation matrix by shifting everything downward, all
  following days will be shifted downward. If each day does this, you
  get a list of days, one below the other.

  However, you do not always want code to have an effect on everything
  that follows. For instance, if a day has the date-if
  |if (Sunday) [red]|, we only want this Sunday to red, not all
  following days also. Similarly, sometimes it is easier to compute
  the position of a day relative to a fixed origin and we do not want
  any modifications of the transformation matrix to have an effect
  outside the scope.

  By cleverly adjusting the different codes, all sorts of different
  day arrangements are possible.

  \begin{key}{/tikz/execute before day scope=\meta{code}}
    The \meta{code} is executed before everything else for each
    date. Multiple 
    calls of this option have an accumulative effect. Thus, if you use
    this option twice, the code from the first use is used first for
    each day, followed by the code given the second time.
  \end{key}
  \begin{key}{/tikz/execute at begin day scope=\meta{code}}
    This code is execute before everything else inside the scope of
    the current date. Again, the effect is accumulative.
  \end{key}
  \begin{key}{/tikz/execute at end day scope=\meta{code}}
    This code is executed just before the day scope is
    closed. The effect is also accumulative, however, in reverse
    order. This is useful to pair, say, |\scope| and |\endscope|
    commands in at-begin- and at-end-code.
  \end{key}
  \begin{key}{/tikz/execute after day scope=\meta{code}}
    This is executed at the very end of the current date, outside the 
    scope. The accumulation is also in reverse.
  \end{key}    
\end{command}


In the rest of the following subsections we have a look at how the
different scope codes can be used to create different calendar
arrangements. 


\subsubsection{Creating a Simple List of Days}

We start with a list the days of the calendar, one day below the
other. For this, we simply shift the coordinate system downward at the
end of the code for each day. This shift must be \emph{outside} the
day scope as we want day shifts to accumulate. Thus, we use the
following code: 
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-01 to 2000-01-08,
             execute after day scope=
               {\pgftransformyshift{-1em}}];
\end{codeexample}
Clearly, we can use this approach to create day lists going up,
down, right, left, or even diagonally.


\subsubsection{Adding a Month Label}

We now want to add a month label to the left of the beginning of each
month. The idea is to do two things:
\begin{enumerate}
\item We add code that is executed only on the first of each month.
\item The code is executed before the actual day is rendered. This
  ensures that options applying to the days do not affect the month
  rendering.
\end{enumerate}
We have two options where we should add the month code: Either we add
it at the beginning of the day scope or before. Either will work fine,
but it might be safer to put the code inside the scope to ensure that
settings to not inadventerdly ``leak outside.''
\begin{codeexample}[]
\tikz
  \calendar
    [dates=2000-01-01 to 2000-01-08,
     execute after day scope={\pgftransformyshift{-1em}},
     execute at begin day scope=
       {\ifdate{day of month=1}{\tikzmonthcode}{}},
     every month/.append style={anchor=base east,xshift=-2em}];
\end{codeexample}

In the above code we used the |\ifdate|\marg{condition}\marg{then
  code}\marg{else code} command, which is described on
page~\pageref{ifdate} in detail and which has much the same effect as
|if (|\meta{condition}|)|\marg{then code}| else |\marg{else code}, but
works in normal code.


\subsubsection{Creating a Week List Arrangement}

Let us now address a more complicated arrangement: A week list. In
this arrangement there is line for each week. The horizontal placement
of the days is thus that all Mondays lie below each other, likewise
for all Tuesdays, and so on.

In order to typeset this arrangement, we can use the following
approach: The origin of the coordinate system rests at the anchor for
the Monday of each week. That means that at the end of each week the
origin is moved downward one line. On all other days, the origin at
the end of the day code is the same as at the beginning. To position
each day correctly, we use code inside and at the beginning of the day
scope to horizontally shift the day according to its day of week. 
\begin{codeexample}[]
\tikz
  \calendar
    [dates=2000-01-01 to 2000-01-20,
     % each day is shifted right according to the day of week
     execute at begin day scope=
       {\pgftransformxshift{\pgfcalendarcurrentweekday em}},
     % after each week, the origin is shifted downward:
     execute after day scope=
       {\ifdate{Sunday}{\pgftransformyshift{-1em}}{}}];
\end{codeexample}


\subsubsection{Creating a Month List Arrangement}

For another example, let us create an arrangment that contains one
line for each month. This is easy enough to do as for weeks, unless we
add the following requirement: Again, we want all days in a column to
have the same day of week. Since months start on different days of
week, this means that each row has to have an individual offset.

One possible way is to use the following approach: After each month
(or at the beginning of each month) we advance the vertical position
of the offset by one line. For horizontal placement, inside the day
scope we locally shift the day by its day of month. Furthermore, we
must additionally shift the day to ensure that the first day of the
month lies on the correct day of week column. For this, we remember
this day of week the first time we see it.
\begin{codeexample}[]
\newcount\mycount
\tikz
  \calendar
    [dates=2000-01-01 to 2000-02-last,
     execute before day scope=
     {
       \ifdate{day of month=1} {
         % Remember the weekday of first day of month
         \mycount=\pgfcalendarcurrentweekday
         % Shift downward
         \pgftransformyshift{-1em}
       }{}
     },
     execute at begin day scope=
     {
       % each day is shifted right according to the day of month
       \pgftransformxshift{\pgfcalendarcurrentday em}
       % and additionally according to the weekday of the first
       \pgftransformxshift{\the\mycount em}
     }];
\end{codeexample}


\subsection{Arrangements}

An \emph{arrangement} specifies how the days of calendar are arranged
on the page. The calendar library defines a number of predefined
arrangements.

We start with arrangements in which the days are listed in a long
line. 

\begin{stylekey}{/tikz/day list downward}
  This style causes the days of a month to be typeset one below the
  other. The shift between days is given by |day yshift|. Between
  month an additional shift of |month yshift| is added.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-28 to 2000-02-03,
             day list downward,month yshift=1em];
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/day list upward}
  works as above, only the list grows upward instead of downward.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-28 to 2000-02-03,
             day list upward,month yshift=1em];
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/day list right}
  This style also works as before, but the list of days grows to the
  right. Instead of |day yshift| and |month yshift|, the values of
  |day xshift| and |month xshift| are used.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-28 to 2000-02-03,
             day list right,month xshift=1em];
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/day list left}
  As above, but the list grows left.
\end{stylekey}

The next arrangement lists days weekwise.

\begin{stylekey}{/tikz/week list}
  This style creates one row for each week in the range. The value
  of |day xshift| is used for the distance between days in each week
  row, the value of |day yshift| is used for the distance between
  rows. In both cases, ``distance''  refers to the distance between
  the anchors of the nodes of the days (or, more generally, the
  distance between the origins of the little pictures created for each
  day).

  The days inside each week are shifted such that Monday is always
  at the first position (to change this, you need to copy and then
  modify the code appropriately). If the date range does not start on
  a Monday, the first line will not start in the first column, but
  rather in the column appropriate for the first date in the range.

  At the beginning of each month (except for the first month in the
  range) an additional vertical space of |month yshift| is added. If
  this is set to |0pt| you get a continuous list of days.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-01 to 2000-02-last,week list];
\end{codeexample}
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-01 to 2000-02-last,week list,
             month yshift=0pt];
\end{codeexample}
\end{stylekey}

The following arrangement gives a very compact view of a whole year.
\begin{stylekey}{/tikz/month list}
  In this arrangement there is a row for each month. As for the
  |week list|, the |day xshift| is used for the horizontal distance.
  For the vertical shft, |month yshift| is used.

  In each row, all days of the month are listed alongside each
  other. However, it is once more ensured that days in each column lie
  on the same day of week. Thus, the very first column contains only
  Mondays. If a month does not start with a Monday, its days are
  shifted to the right such that the days lie on the correct columns. 
\begin{codeexample}[]
\sffamily\scriptsize    
\tikz
  \calendar [dates=2000-01-01 to 2000-12-31,
             month list,month label left,month yshift=1.25em]
            if (Sunday) [black!50];
\end{codeexample}
\end{stylekey}

\subsection{Month Labels}

For many calendars you may wish to add a labels to each month. We have
already covered how month nodes are created and rendered in the
description of the |\calendar| command: use |month text|,
|every month|, and also |month code| (if necessary) to change the
appearance of the month labels.

What we have not yet covered is where these labels are placed. By
default, they are not placed at all as there is no good ``default
position'' for them. Instead, you can use one of the following options
to specify a position for the labels:
\begin{stylekey}{/tikz/month label left}
  Places the month label to the left of the first day of the
  month. (For |week list| and |month list| where a month does not
  start on a Monday, the position is chosen ``as if'' the month had
  started on a Monday --  which is usually exactly what you want.)
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-28 to 2000-02-03,
             day list downward,month yshift=1em,
             month label left];
\end{codeexample}
\end{stylekey}
\begin{stylekey}{/tikz/month label left vertical}
  This style works like the above style, only the label is rotated
  counterclockwise by 90 degrees.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-28 to 2000-02-03,
             day list downward,month yshift=1em,
             month label left vertical];
\end{codeexample}
\end{stylekey}
\begin{stylekey}{/tikz/month label right}
  This style places the month label to the right of the row in which
  the first day of the month lies. This means that for a day list the
  label is to the right of the first day, for a week list it is to the
  right of the first week, and for a month list it is to the right of
  the whole month.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-28 to 2000-02-03,
             day list downward,month yshift=1em,
             month label right];
\end{codeexample}
\end{stylekey}
\begin{stylekey}{/tikz/month label right vertical}
  Works as above, only the label is rotated clockwise by 90 degrees.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-28 to 2000-02-03,
             day list downward,month yshift=1em,
             month label right vertical];
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/month label above left}
  This style places the month label above of the row of the first day,
  flushed left to the leftmost column. The amount by which the label
  is raised is fixed to |1.25em|; use the |yshift| option with the
  month node to modify this.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-28 to 2000-02-03,
             day list right,month xshift=1em,
             month label above left];
\end{codeexample}
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-20 to 2000-02-10,
             week list,month label above left];
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/month label above centered}
  works as above, only the label is centered above the row containing
  the first day.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-02-01 to 2000-02-last,
             day list right,month label above centered];
\end{codeexample}
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-20 to 2000-02-10,
             week list,month label above centered];
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/month label above right}
  works as above, but flushed right
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-01-20 to 2000-02-10,
             week list,month label above right];
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/month label below left}
  Works like |month label above left|, only the label is placed below
  the row. This placement is not really useful with the |week list|
  arrangement, but rather with the |day list right| or |month list|
  arrangement.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-02-01 to 2000-02-last,
             day list right,month label below left];
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/month label below centered}
  Works like |month label above centered|, only below.
\begin{codeexample}[]
\tikz
  \calendar [dates=2000-02-01 to 2000-02-last,
             day list right,month label below centered];
\end{codeexample}
\end{stylekey}



\subsection{Examples}

In the following, some example calendars are shown that come either
from real applications or are just nice to look at.

Let us start with a year-2100-countdown, in which we cross out dates
as we approach the big celebration. For
this, we set the shape to |strike out| for these dates.

\begin{codeexample}[leave comments]
\begin{tikzpicture}
  \calendar
  [
    dates=2099-12-01 to 2100-01-last,
    week list,inner sep=2pt,month label above centered,
    month text=\%mt \%y0
  ]
  if (at most=2099-12-29) [nodes={strike out,draw}]
  if (weekend)            [black!50,nodes={draw=none}]
  ;
\end{tikzpicture}
\end{codeexample}

The next calendar shows a deadline, which is 10 days in the future
from the current date. The last three days before the deadline are in
red, because we really should be done by then. All days on which we
can no longer work on the project are crossed out.

\begin{codeexample}[leave comments]
\begin{tikzpicture}
  \calendar
  [
    dates=\year-\month-\day+-25 to \year-\month-\day+25,
    week list,inner sep=2pt,month label above centered,
    month text=\textit{\%mt \%y0}
  ]
  if (at least=\year-\month-\day) {}
    else [nodes={strike out,draw}]
  if (at most=\year-\month-\day+7)
    [green!50!black]
  if (between=\year-\month-\day+8 and \year-\month-\day+10)
    [red]
  if (Sunday)
    [gray,nodes={draw=none}]
  ;
\end{tikzpicture}
\end{codeexample}

The following example is a futuristic calendar that is all about circles:

\begin{codeexample}[]
\sffamily

\colorlet{winter}{blue}  
\colorlet{spring}{green!60!black}  
\colorlet{summer}{orange}  
\colorlet{fall}{red}  

% A counter, since TikZ is not clever enough (yet) to handle
% arbitrary angle systems.
\newcount\mycount

\begin{tikzpicture}
  [transform shape,
   every day/.style={anchor=mid,font=\fontsize{6}{6}\selectfont}]
  \node{\normalsize\the\year};
  \foreach \month/\monthcolor in
    {1/winter,2/winter,3/spring,4/spring,5/spring,6/summer,
     7/summer,8/summer,9/fall,10/fall,11/fall,12/winter}
  {
    % Computer angle:
    \mycount=\month
    \advance\mycount by -1
    \multiply\mycount by 30
    \advance\mycount by -90

    % The actual calendar
    \calendar at (\the\mycount:6.4cm)
    [
      dates=\the\year-\month-01 to \the\year-\month-last,
    ]
    if (day of month=1) {\color{\monthcolor}\tikzmonthcode}
    if (Sunday) [red]
    if (all) 
    {
      % Again, compute angle
      \mycount=1
      \advance\mycount by -\pgfcalendarcurrentday
      \multiply\mycount by 11
      \advance\mycount by 90
      \pgftransformshift{\pgfpointpolar{\mycount}{1.4cm}}
    };
  }
\end{tikzpicture}
\end{codeexample}

Next, lets us have a whole year in a tight column:
\begin{codeexample}[leave comments]
\begin{tikzpicture}
  \small\sffamily
  \colorlet{darkgreen}{green!50!black}
  \calendar[dates=\year-01-01 to \year-12-31,week list,
            month label left,month yshift=0pt,
            month text=\textcolor{darkgreen}{\%m0}]
           if (Sunday) [black!50];
\end{tikzpicture}
\end{codeexample}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-chains.tex <==
% Copyright 2008 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Chains}

\label{section-chains}

\begin{tikzlibrary}{chains}
  This library defines options for creating chains.
\end{tikzlibrary}


\subsection{Overview}

\emph{Chains} are sequences of nodes that are -- typically -- arranged
in an o row or a column and that are -- typically -- connected by
edges. More generally, they can be used to position nodes of a
branching network in a systematic manner. For the positioning of nodes
in rows and columns you can also use matrices, see 
Section~\ref{section-matrices}, but chains can also be used 
to describe the connections between nodes that have already been
connected using, say, matrices. Thus, it often makes sense to use
matrices for the positioning of elements and chains to describe the
connections. 



\subsection{Starting and Continuing a Chain}

Typically, you construct one chain at a time, but it is
permissible to have construct multiple chains simultaneously. In this
case, the chains must be named differently and you must specify for
each node which chain it belongs to.

The first step toward creating a chain is to use the |start chain|
option.

\begin{key}{/tikz/start chain=\opt{\meta{chain name}}\opt{\meta{direction}}}
  This key should, but need not, be given as an option to a scope
  enclosing all nodes of the chain. Typically, this will be a |scope|
  or the whole |tikzpicture|, but it might just be a path on which all
  nodes of the chain are found.
  If no \meta{chain name} is given, the default value |chain| will be
  used instead.

  The key starts a chain named \meta{chain name} and makes it
  \emph{active}, which means that is currently being constructed. The
  |start chain| can be issued only once to activate a chain, inside a
  scope in which a chain is active you cannot use this option once
  more (for the same chain name). The chain stops being active at the
  end of the scope in which the |start chain| command was given.

  Although chains are only locally active (that is, active inside the
  scope the |start chain| command was issued), the information
  concerning the chains is stored globally and it is possible
  to \emph{continue} a chain after a scope has ended. For this, the
  |continue chain| option can be used, which allows you to reactivate
  an existing chain in another scope.

  The \meta{direction} is used to determine the placement rule for
  nodes on the chain. If it is omitted, the current value of the
  following key is used:
  \begin{key}{/tikz/chain default direction=\meta{direction}
      (initially going right)}
    This \meta{direction} is used in a |chain| option, if no other
    \meta{direction} is specified.
  \end{key}

  The \meta{direction} can have two different forms:
  \declare{|going |\meta{options}} or
  \declare{|placed |\meta{options}}. The effect of these rules will be
  explained in the description of the |on chain| option. Right now,
  just remember that the \meta{direction} you provide with the |chain|
  option applies to the whole chain.
  
  Other than this, this key has no further effect. In particular, to
  place nodes on the chain, you must use the |on chain| option,
  described next.
\begin{codeexample}[]
\begin{tikzpicture}[start chain]
  % The chain is called just "chain"
  \node [on chain] {A};
  \node [on chain] {B};
  \node [on chain] {C};
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  % Same as above, using the scope shorthand
  { [start chain]
    \node [on chain] {A};
    \node [on chain] {B};
    \node [on chain] {C};
  }
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[start chain=1 going right,
                    start chain=2 going below,
                    node distance=5mm,
                    every node/.style=draw]
  \node [on chain=1] {A};
  \node [on chain=1] {B};
  \node [on chain=1] {C};

  \node [on chain=2] at (0.5,-.5) {0};
  \node [on chain=2] {1};
  \node [on chain=2] {2};
  
  \node [on chain=1] {D}; 
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/continue chain=\opt{\meta{chain name}}\opt{\meta{direction}}}
  This option allows you to (re)activate an existing chain and to
  possibly change the default direction. If the |chain name| is
  missing, the name of the innermost activated chain is used. If no
  chain is activated, |chain| is used.

  Let us have a look at the two different applications of this
  option. The first is to change the direction of a chain as it is
  begin constructed. For this, just give this option somewhere inside
  the scope of the chain.
\begin{codeexample}[]
\begin{tikzpicture}[start chain=going right,node distance=5mm]
  \node [draw,on chain] {Hello};
  \node [draw,on chain] {World};
  \node [draw,continue chain=going below,on chain] {,};
  \node [draw,on chain] {this};
  \node [draw,on chain] {is};
\end{tikzpicture}
\end{codeexample}

  The second application is to reactivate a chain after it ``has
  already been closed down.''

\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm,
                    every node/.style=draw]
  { [start chain=1]
    \node [on chain] {A};
    \node [on chain] {B};
    \node [on chain] {C};
  }

  { [start chain=2 going below]
    \node [on chain=2] at (0.5,-.5) {0};
    \node [on chain=2] {1};
    \node [on chain=2] {2};
  }

  { [continue chain=1]
    \node [on chain] {D};
  }
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsection{Nodes on a Chain}

\begin{key}{/tikz/on chain=\opt{\meta{chain name}}\opt{\meta{direction}}}
  This key should be given as an option to a node. When the option is
  used, the \meta{chain name} must be the name of a chain that has
  been started using the |start chain| option. If \meta{chain name} is
  the empty string, the current value of the innermost activated chain
  is used. If this option is used several times for a node, only the
  last invocation ``wins.'' (To place a node on several chains, use
  the |\chainin| command repeatedly.)

  The \meta{direction} part is optional. If present it sets the
  direction used for this node, otherwise the \meta{direction}
  that was given to the original |start chain| option is used (or of
  the last |continue chain| option, which allows you to change this
  default). 

  The effects of this option are the following:
  \begin{enumerate}
  \item An internal counter (there is one, local, counter
    for each chain) is increased. This counter reflects the current
    number of the node in the chain, where the first node is node 1,
    the second is node 2, and so on.

    This value of this internal counter is globally stored in the
    macro \declare{|\tikzchaincount|}.
  \item If the node does not yet have a name, (having been given using
    the |name| option or the name-syntax), the name of the node is set to
    \meta{chain name}|-|\meta{value of the internal chain
      counter}. For instance, if the chain is called |nums|, the first
    node would be named |nums-1|, the second |nums-2|, and so on. For
    the default chain name |chain|, the first node is named |chain-1|,
    the second |chain-2|, and so on.
  \item Independently of whether the name has been provided
    automatically or via the |name| option, the name of the node is
    globally stored in the macro \declare{|\tikzchaincurrent|}.
  \item Except for the first node, the macro
    \declare{|\tikzchainprevious|} is now globally set to the name of
    the node of the previous node on the chain. For the first node of
    the chain, this macro is globally set to the empty string.
  \item Except possibly for the first node of the chain, the placement
    rule is now executed. The placement rule is just a \tikzname\ option
    that is applied automatically to each node on the chain. Depending
    on the form of the \meta{direction} parameter (either the locally
    given one or the one given to the |start chain| option), different
    things happen.

    First, it makes a difference whether the \meta{direction} starts
    with |going| or with |placed|. The difference is that in the first
    case, the placement rule is not applied to the first node of the
    chain, while in the second case the placement rule is applied also
    to this first node. The idea is that a |going|-direciton indicates
    that we are ``going somewhere relative to the previous node''
    whereas a |placed| indicates that we are ``placing nodes according
    to their number.''

    Independently of which form is used, the \meta{text} inside
    \meta{direction} that follows |going| or |placed| (separated by a
    compulsory space) can have two different effects:
    \begin{enumerate}
    \item If it contains an equal sign, then this \meta{text} is used
      as the placement rule, that is, it is simply executed.  
    \item If it does not contain an equal sign, then
      \meta{text}|=of \tikzchainprevious| is used as the placement
      rule. 
    \end{enumerate}

    Note that in the first case, inside the \meta{text} you have
    access to |\tikzchainprevious| and |\tikzchaincount| for doing
    your positioning calculations.
\begin{codeexample}[]
\begin{tikzpicture}[start chain=circle placed {at=(\tikzchaincount*30:1.5)}]
  \foreach \i in {1,...,10}
    \node [on chain] {\i};
  
  \draw (circle-1) -- (circle-10);
\end{tikzpicture}
\end{codeexample}
  \item
    The following style is executed:
    \begin{stylekey}{/tikz/every on chain}
      This key is executed for every node of a chain, including the
      first one. 
    \end{stylekey}
  \end{enumerate}

  Recall that the standard replacement rule has a form like
  |right=of (\tikzchainprevious)|. This means that each 
  new node is placed to the right of the previous one, spaced by the
  current value of |node distance|.
\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm]
  \node [draw,on chain] {};
  \node [draw,on chain] {Hallo};
  \node [draw,on chain] {Welt};
\end{tikzpicture}
\end{codeexample}

  The optional \meta{direction} allows us to temporarily change the
  direction in the middle of a chain:
\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm]
  \node [draw,on chain] {Hello};
  \node [draw,on chain] {World};
  \node [draw,on chain=going below] {,};
  \node [draw,on chain] {this};
  \node [draw,on chain] {is};
\end{tikzpicture}
\end{codeexample}

  You can also use more complicated computations in the \meta{direction}:
\begin{codeexample}[]
\begin{tikzpicture}[start chain=going {at=(\tikzchainprevious),shift=(30:1)}]
  \draw [help lines] (0,0) grid (3,2);
  \node [draw,on chain] {1};
  \node [draw,on chain] {Hello};
  \node [draw,on chain] {World};
  \node [draw,on chain] {.};
\end{tikzpicture}
\end{codeexample}
\end{key}

For each chain, two special ``pseudo nodes'' are created.

\begin{predefinednode}{\meta{chain name}-begin}
  This node is the same as the first node on the chain. It is only
  defined after a first node has been defined.
\end{predefinednode}

\begin{predefinednode}{\meta{chain name}-end}
  This node is the same as the (currently) last node on the chain. As
  the chain is extended, this node changes.
\end{predefinednode}

The |on chain| option can also be used, in conjunction with
|late options|, to add an already existing node to a chain. The
following command, which is only defined inside scopes where a
|start chain| option is present, simplifies this process.

\begin{command}{\chainin |(|\meta{existing name}|)| \opt{\oarg{options}}}
  This command makes it easy to add a node to chain that has already
  been constructed. This node may even be part of a another chain.

  When you say |\chainin (some node);|, the node |some node| must
  already exist. It will then be made part of the current chain. This
  does not mean that the node can be changed (it is already
  constructed, after all), but the |join| option can be used to join
  |some node| to the previous last node on the chain and subsequent
  nodes will be placed relative to |some node|.

  It is permissible to give the |on chain| option inside the
  \meta{options} in order to specify on which chain the node should be
  put. 
  
  This command is just a shortcut for
\begin{quote}
|\path (|\meta{existing name}|) [late options={on chain,every chain in,|\meta{options}|}]|
\end{quote}
  In particular, it is possible to continue to path after a |\chainin|
  command, though that does not seem very useful.
  
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm,
                    every node/.style=draw,every join/.style=->]
  \draw [help lines] (0,0) grid (3,2);

  \node[red] (existing) at (0,2) {existing};

  { [start chain]
    \node [draw,on chain,join] {Hello};
    \node [draw,on chain,join] {World};
    \chainin (existing) [join];
    \node [draw,on chain,join] {this};
    \node [draw,on chain,join] {is};
  } 
\end{tikzpicture}
\end{codeexample}

  Here is an example where nodes are positioned using a matrix and
  then connected using a chain
{\catcode`\|=12  
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style=draw]
  \matrix [matrix of nodes,column sep=5mm,row sep=5mm]
  {
    |(a)|           World & |(b) [circle]|             peace \\
    |(c)|           be    & |(d) [isosceles triangle]| would \\
    |(e) [ellipse]| great & |(f)|                      ! \\
  };
  
  { [start chain,every on chain/.style={join=by ->}]
    \chainin (a);
    \chainin (b);
    \chainin (d);
    \chainin (c);
    \chainin (e);
    \chainin (f);
  } 
\end{tikzpicture}
\end{codeexample}
}
\end{command}



\subsection{Joining Nodes on a Chain}

\begin{key}{/tikz/join=\opt{|with |\meta{with} }\opt{|by |\meta{options}}}
  When this key is given to any node on a chain (except possibly for
  the first node), an |edge| command is added after the node. The
  |with| part specifies which node should be used for the start point
  of the edge; if the |with| part is omitted, the |\tikzchainprevious|
  is used. This |edge| command gets the \meta{options} as parameter
  and the current node as its target. If there is no
  previous node and no |with| is given, no |edge| command gets
  executed.  
  \begin{stylekey}{/tikz/every join}
    This style is executed each time this command is used.
  \end{stylekey}

  Note that is makes sense to call this option several times for a
  node, in order to connect it to several nodes. This is especially
  useful for joining in branches, see the next section.
\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm,
                    every join/.style={->,red}]
  \node [draw,on chain,join] {};
  \node [draw,on chain,join] {Hallo};
  \node [draw,on chain,join] {Welt};
  \node [draw,on chain=going below,
         join,join=with chain-1 by {blue,<-}] {foo};
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsection{Branches}

A \emph{branch} is a chain that (typically only temporarily) extends
an existing chain. The idea is the following: Suppose we are
constructing a chain and at some node |x| there is a fork. In this
case, one (or even more) branches starts at this fork. For each branch
a chain is created, but the first node on this chain should
be~|x|. For this, it is useful to use |\chainin| on the node |x| to
make it part of the different branch chains and to name the branch
chains in some way that reflects the name of the main chain.

The |start branch| option provides a shorthand for doing exactly what
was just described.

\begin{key}{/tikz/start branch=\meta{branch name}\opt{\meta{direction}}}
  This key is used in the same manner as the |start chain| command,
  however, the effect is slightly different:
  \begin{itemize}
  \item This option may only be used if some chain is already active
    and there is a (last) node on this chain. Let us call this node
    the \meta{fork node}.
  \item The chain is not just called \meta{branch name}, but
    \meta{current chain}|/|\meta{branch name}. For instance, if the
    \meta{fork node} is part of the chain called |trunk| and the
    \meta{branch name} is set to |left|, the complete chain name of
    the branch is |trunk/left|. The \meta{branch name} must be given,
    there is no default value.
  \item The \meta{fork node} is automatically ``chained into'' the
    branch chain as its first node. Thus, for the first node on the
    branch that you provide, the |join| option will cause it to be
    connected to the fork node.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[every on chain/.style=join,every join/.style=->,
                    node distance=2mm and 1cm]
  { [start chain=trunk]
    \node [on chain] {A};
    \node [on chain] {B};

    { [start branch=numbers going below]
      \node [on chain] {1};
      \node [on chain] {2};
      \node [on chain] {3};
    }
    { [start branch=greek going above]
      \node [on chain] {$\alpha$};
      \node [on chain] {$\beta$};
      \node [on chain] {$\gamma$};
    }
    
    \node [on chain,join=with trunk/numbers-end,join=with trunk/greek-end] {C};
    { [start branch=symbols going below]
      \node [on chain] {$\star$};
      \node [on chain] {$\circ$};
      \node [on chain] {$\int$};
    }
  }
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/continue branch=\meta{branch name}\opt{\meta{direction}}}
  This option works like the |continue chain| option, only 
  \meta{current chain}|/|\meta{branch name} is used as the chain name,
  rather than just \meta{branch name}.
\begin{codeexample}[]
\begin{tikzpicture}[every on chain/.style=join,every join/.style=->,
                    node distance=2mm and 1cm]
  { [start chain=trunk]
    \node [on chain] {A};
    \node [on chain] {B};
    { [start branch=numbers going below] } % just a declaration,
    { [start branch=greek   going above] } % we will come back later
    \node [on chain] {C};

    % Now come the branches...
    { [continue branch=numbers]
      \node [on chain] {1};
      \node [on chain] {2};
    }
    { [continue branch=greek]
      \node [on chain] {$\alpha$};
      \node [on chain] {$\beta$};
    }
  }
\end{tikzpicture}
\end{codeexample}
\end{key}


==> pgfmanual-en-library-decorations.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Decoration Library}
\label{section-library-decorations}



\subsection{Overview and Common Options}

The decoration libraries define a number of (more or less useful)
decorations that can be applied to paths. The usage of decorations is
not covered in the present section, please consult 
Sections~\ref{section-tikz-decorations}, which explains how
decorations are used in \tikzname, and
\ref{section-base-decorations}, which  explains how new
decorations can be defined. 

The decorations are influenced by a number of parameters that can be
set using the |decoration| option. These parameters are
typically shared between different decorations. In the following, the
general options are documented (they are defined directly in the
|decoration| module), special-purpose keys are documented
with the decoration that uses it.

Since you are encouraged to use these keys to make your own
decorations configurable, it is indicated for each key where the value
is stored (so that you can access it). Note that some values are
stored in \TeX\ dimension registers while others are stored in macros.

\begin{key}{/pgf/decoration/amplitude=\meta{dimension} (initially 2.5pt)}
  This key determines the ``desired height'' (or amplitude) of 
  decorations for which this makes sense. For instance, the initial
  value of |2.5pt| means that deforming decorations should deform a
  path by up to 2.5pt away from the original path.

  This key set the \TeX-dimension |\pgfdecorationsegmentamplitude|. 
\end{key}

\begin{key}{/pgf/decoration/meta-amplitude=\meta{dimension} (initially 2.5pt)}
  This key determines the amplitude for a meta-decoration. 

  The key set the \TeX-macro (!) |\pgfmetadecorationsegmentamplitude|.
\end{key}

\begin{key}{/pgf/decoration/segment length=\meta{dimension} (initially 10pt)}
  Many decorations are made up of small segments. This key determines
  the desired length of such segments. 

  This key set the \TeX-dimension |\pgfdecorationsegmentlength|. 
\end{key}

\begin{key}{/pgf/decoration/meta-segment length=\meta{dimension} (initially 1cm)}
  This determined the length of the meta-segments from which a
  meta-decoration is made up.

  This key set the \TeX-macro (!) |\pgfmetadecorationsegmentlength|. 
\end{key}

\begin{key}{/pgf/decoration/angle=\meta{degree} (initially 45)}
  The way some decorations look like depends on a configurable angle. For
  instance, a |wave| decoration consists of arcs and the opening angle
  of these arcs is given by the |angle|.

  This key set the \TeX-macro |\pgfdecorationsegmentangle|. 
\end{key}

\begin{key}{/pgf/decoration/aspect=\meta{factor} (initially 0.5)}
  For some decorations there is a natural aspect ratio. For instance,
  for a |brace| decoration the aspect ratio determines where the brace
  point will be.

  This key set the \TeX-macro |\pgfdecorationsegmentaspect|. 
\end{key}

\begin{key}{/pgf/decoration/start radius=\meta{dimension} (initially 2.5pt)}
  For some decorations there is a natural start radius (of some circle, presumably).

  This key stores the value directly inside the key.
\end{key}

\begin{key}{/pgf/decoration/end radius=\meta{dimension} (initially 2.5pt)}
  For some decorations there is a natural radius (of some circle, presumably).

  This key stores the value directly inside the key.
\end{key}

\begin{stylekey}{/pgf/decoration/radius=\meta{dimension}}
  Sets the start and end radius simultaneously.
\end{stylekey}


\begin{key}{/pgf/decoration/path has corners=\meta{boolean} (initially false)}
  This is a hint to the decoration code as to whether the path has
  corners or not. If a path has a sharp corner, setting this option to
  |true| may result in better rendering of the decoration because the
  joins of input segements are approached ``more carefully'' than
  when this key is set to false. However, if the path is, say, a
  smooth circle, setting this key to |true| will usually look
  worse. Most decorations ignore this key, anyway. Internally, it sets
  the \TeX-if |\ifpgfdecoratepathhascorners|.
\end{key}


\subsection{Path Morphing Decorations}

\begin{pgflibrary}{decorations.pathmorphing}
  A \emph{path morphing decorations} ``morphs'' or ``deforms'' the
  to-be-decorated path. This means that what used to be a straight
  line might afterwards be a snaking curve and have bumps. However, a
  line is still and a line and path deforming decorations do not
  change the number of subpaths. For instance, if the path used to
  consist of two circles and an open arc, the path will after the
  decoration process still consist of two closed subpath and one open
  subpath. 
\end{pgflibrary}


\subsubsection{Decorations Producing Straight Line Paths}

The following deformations use only straight lines in order to morph
the paths.

\begin{decoration}{lineto}
  This decoration replaces the path by straight lines. For each curve,
  the path simply goes directly from the start point to the end point.
  In the following example, the arc actually consist of two
  subcurves.

  This decoration is actually always defined when the decoration
  module is loaded, but it is documented here for consistency.
\begin{codeexample}[]
\begin{tikzpicture}[decoration=lineto]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{straight zigzag}
  This (meta-)decoration decorates the path by alternating between 
  |curveto| and |zigzag| decorations. It always finishes
  with the |curveto| decoration. The following parameters influence
  the decoration:
  \begin{itemize}
  \item |amplitude|
    determines how much the zig-zag lines raises above and falls below
    a straight line to the target point.
  \item |segment length|
    determines the length of a complete ``up-down'' cycle.
  \item	|meta-segment length|
    determines the length of the |curveto| and the |zigzag| decorations.
  \end{itemize}

\begin{codeexample}[]
\begin{tikzpicture}[decoration={straight zigzag,meta-segment length=1.1cm}]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{random steps}
  This decoration consists of straight line segments. The line segments
  head towards the target, but each step is randomly shifted a little
  bit. The following parameters influence the decorations:
  \begin{itemize}
  \item |segment length|
    determines the basic length of each step.
  \item |amplitude|
    The end of each step is perturbed both in $x$- and in
    $y$-direction by two values drawn uniformly from the interval
    $[-d,d]$, where $d$ is the value of |amplitude|.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}
    [decoration={random steps,segment length=2mm}]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{saw}
  This decoration looks like the blade of a saw. The following parameters
  influence the decoration:
  \begin{itemize}
  \item |amplitude|
    determines how much each spike raises above the straight line.
  \item |segment length|
    determines the length each spike.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=saw]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{zigzag}
  This decoration looks like a zig-zag line. The following parameters
  influence the decoration:
  \begin{itemize}
  \item |amplitude|
    determines how much the zig-zag lines raises above and falls below
    a straight line to the target point.
  \item |segment length|
    determines the length of a complete ``up-down'' cycle.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=zigzag]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}



\subsubsection{Decorations Producing Curved Line Paths}

\begin{decoration}{bent}
  This decoration adds a slightly bent line from the start to the
  target. The amplitude of the bent is given |amplitude|
  (an amplitude of zero gives a straight line). 
  \begin{itemize}
  \item |amplitude|
    determines the amplitude of the bent.
  \item |aspect|
    determines how tight the bent is. A good value is around |0.3|. 
  \end{itemize}
  Note that this decoration makes only little sense for curves. You
  should apply it only to straight lines.
\begin{codeexample}[]
\begin{tikzpicture}[decoration=bent]
  \draw [help lines] grid (3,2);
  \draw [decorate] (0,0) -- (3,1) -- (1.5,2) -- (0,1);
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}[decoration={bent,aspect=.3}]
  \draw [decorate,fill=examplefill] (0,0) rectangle (3.5,2);
  \node[circle,draw] (A) at (.5,.5) {A};
  \node[circle,draw] (B) at (3,1.5) {B};
  \draw[->,decorate] (A) -- (B);
  \draw[->,decorate] (B) -- (A);
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{bumps}
  This decoration replaces the path by little half ellipses. The
  following parameters influence itL
  \begin{itemize}
  \item |amplitude|
    determines the height of the half ellipse.
  \item |segment length|
    determines the width of the half ellipse.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=bumps]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{coil}
  This decoration replaces the path by a coiled line. To understand how this works,
  imagine a three-dimensional spring. The spring's axis points along
  the path toward the target. Then, we ``view'' the spring from a
  certain angle. If we look ``straight from the side'' we will see a
  perfect sine curve, if we look ``more from the front'' we will see a
  coil. The following parameters influence the decoration:  
  \begin{itemize}
  \item |amplitude|
    determines how much the coil rises above the path and falls below
    it. Thus, this is the radius of the coil.
  \item |segment length|
    determines the distance between two consecutive ``curls.'' Thus,
    when the spring is see ``from the side'' this will be the wave
    length of the sine curve. 
  \item |aspect|
    determines the ``viewing direction.'' A value of |0| means
    ``looking from the side'' and a value of |0.5|, which is the
    default, means ``look more from the front.'' 
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=coil]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
    [decoration={coil,aspect=0.3,segment length=3mm,amplitude=3mm}]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}



\begin{decoration}{curveto}
  This decoration simply yields a line following the original
  path. This means that (ideally) it does not change the path and
  follows any curves in the path (hence the name). In
  reality, due to the internals of how decorations are implemented,
  this decoration actually replaces the path by numerous small
  straight lines.

  This decoration is mostly useful in conjunction with
  meta-decorations. It is also actually defined in the decoration
  module and is always available.

\begin{codeexample}[]
\begin{tikzpicture}[decoration=curveto]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}



\begin{decoration}{snake}
  This decoration replaces the path by a line that looks like a snake
  seen from above. More precisely, the snake is a sine wave with a
  ``softened'' start and ending. The following parameters influence
  the snake: 
  \begin{itemize}
  \item |amplitude|
    determines the sine wave's amplitude.
  \item |segment length|
    determines the sine wave's wave length.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=snake]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill]
    (0,0) -- (3,1) arc (0:180:1.5 and 1) -- cycle;
\end{tikzpicture}
\end{codeexample}
\end{decoration}



  
\subsection{Path Replacing Decorations}

\begin{pgflibrary}{decorations.pathreplacing}
  This library defines decorations that replace the to-be-decorated
  path by another path. Unlike morphing decorations, the replaced path
  might be quite different, for instance a straight line might be
  replaced by a set of circles. Note that filling a path that has been
  replaced using one of the decorations in this library typically does
  not fill the original area but, rather, the smaller area of the
  newly-created path segments.
\end{pgflibrary}

\begin{decoration}{border}
  This decoration adds straight lines the path that are at a specific
  angle to the line toward the target. The idea is to add these little
  lines to indicate the ``border'' or an area. The following
  parameters influence the decoration:  
  \begin{itemize}
  \item |segment length|
    determines the distance between consecutive ticks.
  \item |amplitude|
    determines the length of the ticks.
  \item |angle|
    determines the angle between the ticks and the line of the path. 
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=border]
  \draw [help lines] grid (3,2);
  \draw [postaction={decorate,draw,red}]
        (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{brace}
  This decoration replaces a straight line path by a long brace. The
  left and right end of the brace will be exactly on the start and
  endpoint of the decoration. The decoration really only makes sense
  for paths that are a straight line.
  \begin{itemize}
  \item |amplitude|
    determines how much the brace rises above the path.
  \item |aspect|
    determines the fraction of the total length where the ``middle
    part'' of the brace will be.  
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=brace]
  \draw [help lines] grid (3,2);
  \draw [decorate] (0,0) -- (3,1);
\end{tikzpicture}
\end{codeexample}
\end{decoration}



\begin{decoration}{expanding waves}
  This decoration adds arcs to the path that get bigger along the line
  towards the target. The following parameters influence the decoration:
  \begin{itemize}
  \item |segment length|
    determines the distance between consecutive arcs.
  \item |angle|
    determines the opening angle below and above the path. Thus, the
    total opening angle is twice this angle.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration={expanding waves,angle=5}]
  \draw [help lines] grid (3,2);
  \draw [decorate] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{ticks}
  This decoration replaces the path by straight lines that are
  orthogonal to the path. The following parameters influence the
  decoration:  
  \begin{itemize}
  \item |segment length|
    determines the distance between consecutive ticks.
  \item |amplitude|
    determines half the length of the ticks.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=ticks]
  \draw [help lines] grid (3,2);
  \draw [decorate] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}
\end{decoration}



\begin{decoration}{waves}
  This decoration replaces the path by arcs that have a constant
  size. The following parameters influence the decoration: 
  \begin{itemize}
  \item |segment length|
    determines the distance between consecutive arcs.
  \item |angle|
    determines the opening angle below and above the path. Thus, the
    total opening angle is twice this angle.
  \item |radius|
    determines the radius of each arc.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration={waves,radius=4mm}]
  \draw [help lines] grid (3,2);
  \draw [decorate] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}
\end{decoration}




\subsection{Decorations with Shapes}

\begin{pgflibrary}{decorations.shapes}
  This library defines decorations that use shapes or shape-like
  drawings to decorate a path. The following options are common
  options used by the decorations in this library:
  
  \begin{key}{/pgf/decoration/shape width=\meta{dimension}  (initially 2.5pt)}
    The desired width of the shapes. For decorations that support
    varying shape sizes, this key sets both the start and end width
    (which can be overwritten using options like |shape start width|).
  \end{key}

  \begin{key}{/pgf/decoration/shape height=\meta{dimension} (initially 2.5pt)}
    Works like the previous key, only for the height.
  \end{key}

  \begin{key}{/pgf/decoration/shape size=\meta{dimension}}
    Sets the desired width and height simultaneously.
  \end{key}

  For the exact places and macros where these keys store the values,
  please consult the beginning of the code of the library.
\end{pgflibrary}



\begin{decoration}{crosses}
  This decoration replaces the path by (diagonal) crosses. The
  following parameters influence the decoration:  
  \begin{itemize}
  \item |segment length|
    determines the distance between (the centers of) consecutive crosses.
  \item |shape height|
    determines the height of each cross.
  \item |shape width|
    determines the width of each cross.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=crosses]
  \draw [help lines] grid (3,2);
  \draw [decorate] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}
\end{decoration}

\begin{decoration}{triangles}
  This decoration replaces the path by triangles that point along the
  path. The following parameters influence the decoration: 
  \begin{itemize}
  \item |segment length|
    determines the distance between consecutive triangles.
  \item |shape height|
    determines height of the triangle side that is orthogonal
    to the path.
  \item |shape width|
    determines the width of the triangle.
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[decoration=triangles]
  \draw [help lines] grid (3,2);
  \draw [decorate,fill=examplefill] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}
\end{decoration}



\begin{decoration}{shape backgrounds}
  This is a general decoration that replaces the to-be-decorated path by repeated
  copies of the background path of an arbitrary shape that has
  previously defined using the |\pgfdeclareshape| command (that is,
  you can use any shape in the shape libraries). Please note that the
  background path of the shapes is used, but \emph{no nodes are
    created}. You cannot have text inside the shapes of this path, you
  cannot name them, or refer to them. 

\begin{codeexample}[]
\begin{tikzpicture}[decoration={shape backgrounds,shape=star,shape size=5pt}]
  \draw [help lines] grid (3,2);
  \draw [decorate] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\tikzset{paint/.style={ draw=#1!50!black, fill=#1!50 },
         decorate with/.style=
           {decorate,decoration={shape backgrounds,shape=#1,shape size=2mm}}}
\begin{tikzpicture}
  \draw [decorate with=dart,      paint=red]    (0,1.5) -- (3,1.5);
  \draw [decorate with=diamond,   paint=green]  (0,1)   -- (3,1);
  \draw [decorate with=rectangle, paint=blue]   (0,0.5) -- (3,0.5);
  \draw [decorate with=circle,    paint=yellow] (0,0)   -- (3,0);
\end{tikzpicture}
\end{codeexample}

  All shapes are positioned by the anchor that is specified via the
  |anchor| decoration option:

  \begin{key}{/pgf/decoration/anchor=\meta{anchor} (initially center)}
    The anchor used to position the shapes backgrounds.
  \end{key}

  A shape background path is added at the start point of the path and,
  if the distance between the shapes is appropriate, at the end point
  of the path. 
	
\begin{codeexample}[]
\begin{tikzpicture}[decoration={
      shape backgrounds,shape=regular polygon,shape size=4mm}]
  \draw [help lines] grid (3,2);
  \draw [thick] (0,0) -- (2,2) (1,0) -- (3,0);
  \draw [red, decorate, decoration={shape sep=.5cm}]  (1,0) -- (3,0);
  \draw [blue, decorate, decoration={shape sep=.5cm}] (0,0) -- (2,2);
\end{tikzpicture}
\end{codeexample}

  Keys for cusomizing specific shapes can be specified (e.g., 
  |star points|, |cloud puffs|, |kite angles|, and so on). The size of
  the shape is ``enforced'' using transformations. This means that the
  shape is typeset with an empty text box and some default size
  values, resulting in an initial shape. This shape is then rescaled
  using coordinate transformations so that it has the desired size
  (which may vary as we travel along the to-be-decorated path). This
  means that settings involving angles and distances may not appear
  entirely accurate. More general options such as |inner sep| and
  |minimum size| will be ignored,  but transformations can be applied
  to each segment as described below.
  
\begin{codeexample}[]
\tikzset{
  paint/.style={draw=#1!50!black, fill=#1!50},
  my star/.style={decorate,decoration={shape backgrounds,shape=star},
                  star points=#1}
}
\begin{tikzpicture}[decoration={shape sep=.5cm, shape size=.5cm}]
  \draw [my star=9, paint=red]                            (0,1.5) -- (3,1.5);
  \draw [my star=5, paint=blue]                           (0,.75) -- (3,.75);
  \draw [my star=5, paint=yellow, shape border rotate=30] (0,0) -- (3,0);
\end{tikzpicture}
\end{codeexample}

  There are various keys to control the drawing of the shape
  decoration. 
  
  \begin{key}{/pgf/decoration/shape=\meta{shape name} (initially circle)}
    The shape whose background path is used.
  \end{key}
  
  \begin{key}{/pgf/decorations/shape sep=\meta{spacing} (initially {.25cm, between centers})}
    Set the spacing between the shapes on the decorationd path. This can be
    just a distance on its own, but the additional keywords 
    |between centers|, and |between borders| (which must be preceded by a 
    comma), specify that the distance	is between the center anchors of 
    the shapes or between the edges of the \emph{boundaries} of
    the shape borders.
	
\begin{codeexample}[]
\begin{tikzpicture}[
    decoration={shape backgrounds,shape size=.5cm,shape=signal},
    signal from=west, signal to=east,
    paint/.style={decorate, draw=#1!50!black, fill=#1!50}]
  \draw [help lines] grid (3,2);
  \draw [paint=red, decoration={shape sep=.5cm}]
    (0,2) -- (3,2);
  \draw [paint=green, decoration={shape sep={1cm, between center}}]
    (0,1) -- (3,1);
  \draw [paint=blue, decoration={shape sep={1cm, between borders}}]
    (0,0) -- (3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  
  \begin{key}{/pgf/decoration/shape evenly spread=\meta{number}}
    This key overides the |shape sep| key and forces the decoration to
    fit \meta{number} shapes evenly across the path. 
    If \meta{number} is less than |1|, then no shapes will be used. 
    If \meta{number} equals |1|, then one shape is put in the middle 
    of the path. 
    The additional keywords |by centers| (the default, if no keyword is
    specified) and |by borders| can be used (both preceded by a comma), 
    to specify how the distance between shapes is determined. These
    keywords will only have a noticable effect if the shapes sizes
    differ over time.
    
\begin{codeexample}[]
\tikzset{
  paint/.style={draw=#1!50!black, fill=#1!50},
  spreading/.style={
    decorate,decoration={shape backgrounds, shape=rectangle,
    shape start size=4mm,shape end size=1mm,shape evenly spread={#1}}}
}
\begin{tikzpicture}
  \fill [paint=green,spreading={5, by borders},
         decoration={shape scaled}]            (0,2)   -- (3,2);
  \fill [paint=blue,spreading={5, by centers},
         decoration={shape scaled}]            (0,1.5) -- (3,1.5);   
  \fill [paint=red,    spreading=5]            (0,1)   -- (3,1);
  \fill [paint=orange, spreading=4]            (0,.5)  -- (3,.5);
  \fill [paint=gray,    spreading=1]            (0,0)   -- (3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}

  \begin{key}{/pgf/decoration/shape sloped=\opt{\meta{boolean}} (initially true)}
    By default, shapes are rotated to the slope of the decorationd path. If 
    \meta{boolean} is the value |false|, then this rotation is turned 
    off. Internally this sets the \TeX-if |\ifpgfshapedecorationsloped|
    appropriately.

\begin{codeexample}[]
\tikzset{
  paint/.style={draw=#1!50!black, fill=#1!50}
}
\begin{tikzpicture}[decoration={
    shape width=.65cm, shape height=.45cm,
    shape=isosceles triangle, shape sep=.75cm,
    shape backgrounds}]    
  \draw [help lines] grid (3,2);
  \draw [paint=red,decorate] (0,0) -- (2,2);
  \draw [paint=blue,decorate,decoration={shape sloped=false}]
                             (1,0) -- (3,2);
\end{tikzpicture}
\end{codeexample}
  \end{key}%

  It is possible to scale the width and height of the shapes across the
  length of the decorationd path. The shapes are scaled between the starting
  size and the ending size. The following keys customize the way the
  decoration shapes are scaled:
	
  \begin{key}{/pgf/decoration/shape scaled=\meta{boolean} (initially false)}
\begin{codeexample}[]
\tikzset{
  bigger/.style={decoration={shape start size=.125cm, shape end size=.5cm}},
  smaller/.style={decoration={shape start size=.5cm, shape end size=.125cm}},
  decoration={shape backgrounds,
              shape sep={.25cm, between borders},shape scaled}
}
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \fill [decorate, bigger, red!50]   (0,1) -- (3,2);
  \fill [decorate, smaller, blue!50] (0,0) -- (3,1);
\end{tikzpicture}
\end{codeexample}

    If this key is set to false (which is the default), then only the
    start width and height are used. Note that the keys |shape width|
    and |shape height| set the start and end height simultaneously.
  \end{key}

  \begin{key}{/pgf/decoration/shape start width=\meta{length} (initially 2.5pt)}
    The starting width of the shape.
  \end{key}%

  \begin{key}{/pgf/decoration/shape start height=\meta{length} (initially 2.5pt)}
    The starting height of the shape.
  \end{key}%
  
  \begin{stylekey}{/pgf/decoration/shape start size=\meta{length}}
    Set both the the start height and start width simultaneously.
  \end{stylekey}%

  \begin{key}{/pgf/decoration/shape end width=\meta{length} (initially 2.5pt)}
    The recommended ending width of the shape. Note, that this is the
    width that a shape will take only if it is drawn exactly at the end
    of the path.


\begin{codeexample}[]    
\tikzset{
  bigger/.style={decoration={shape start size=.25cm, shape end size=1cm}},
  smaller/.style={decoration={shape start size=1cm, shape end size=.25cm}},
  decoration={shape backgrounds,
              shape sep={.25cm, between borders},shape scaled}
}
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \fill [decorate,bigger,
         decoration={shape sep={.25cm, between borders}}, blue!50] 
    (0,1.5) -- (3,1.5);
  \fill [decorate,smaller,
         decoration={shape sep={1cm, between centers}},   red!50]  
    (0,.5)  -- (3,.5);
  \draw [gray, dotted] (0,1.625) -- (3,2)    (0,1.375) -- (3,1) 
                       (0,1)     -- (3,.625) (0,0)     -- (3,.375); 
\end{tikzpicture}
\end{codeexample}
  \end{key}%

  \begin{key}{/pgf/decoration/shape end height=\meta{length}}
    The recommended ending height of the shape.
  \end{key}%

  \begin{stylekey}{/pgf/decoration/shape end size=\meta{length}}
    Set both the the end height and end width simultaneously.
  \end{stylekey}
\end{decoration}





\subsection{Text Decorations}

\begin{pgflibrary}{decorations.text}
  The decoration in this library decorates the path with some
  text. This can be used to draw text that follows a curve.  
\end{pgflibrary}

\begin{decoration}{text along path}
  This decoration decorates the path with text. This drawing of the
  text is a ``side effect'' of the decoration. The to-be-decorated
  path is only used to determine where the characters should be put
  and it is thrown away after the decoration is done. This is why in
  the following example no line is shown.
	
\begin{codeexample}[]
\catcode`\|12
\begin{tikzpicture}[decoration={text along path,
    text={Some long text along a ridiculously long curve that}}] 
  \draw [help lines] grid (3,2);
  \draw [decorate] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}

  \pgfname{} ``does its best'' to typeset the text, however you
  should note the following points:
  \begin{itemize}
  \item
    Each character in the text is typeset in a separate |\hbox|. This
    means that if you want fancy things like kerning or ligatures you
    will have to manually annotate the characters in the decoration 
    text within a group, for example, |W{\kern-1ptA}TER|. 
  \item
    Each character is positioned using the center of its baseline. To
    move the text vertcally (relative to the path), the additional
    transform key should be used.
  \item
    No attempt is made to ensure characters do not overlap when
    the angle between segments is considerably less than 180\textdegree{}
    (this is tricky to do in \TeX{} without a huge processing
    overhead). In general this should not be too much of a problem, 
    but, once again, kerning can be used in most cases to overcome 
    any undesirable effects.
  \item			
    It is only possible to typeset text in math mode under considerable
    restrictions. Math mode is entered and exited using any character	
    of category code 3 (e.g., in plain \TeX{} this is |$|). %$
    Math subscripts and superscripts need to be	contained within braces 
    (e.g., |{^y_i}|) as do commands like |\times| or |\cdot|. 
    However, even modestly complex mathematical	typesetting is unlikely 
    to be sucessful along a path (or even desirable).
  \item
    Some inaccuracies in positioning may be particularly apparent
    at input segment boundaries. This can (unfortunately) only be solved 
    on case by case basis by individually kerning the offending 
    characters within a group.
  \end{itemize}
  
  The following keys are used by the |text| decoration:
  \begin{key}{/pgf/decoration/text=\meta{text}
      (initially \normalfont empty)}
    Set the text to typeset along the curve. 
    Consecutive spaces are ignored, so |\ | (or |\space| in \LaTeX) 
    should be used to insert multiple spaces.	It is possible to
    format the text using normal formating commands, such as |\it|, |\bf|
    and |\color|, within customisable delimiters. Initially these
    delimiters are both {\tt\char`\|} (however, care will be needed 
    regarding	the category codes of delimiters --- see below). 

{\catcode`\|12
\begin{codeexample}[]
\catcode`\|12
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \path [decorate,decoration={text along path,
           text={a big |\color{green}|green|| juicy apple.}}] 
    (0,0) .. controls (0,2) and (3,0) .. (3,2);
\end{tikzpicture}
\end{codeexample}
}
    By following the first delimiter
    with |+|, the formatting commands are added to any exisiting 
    formatting.

{\catcode`\|12
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \path [decorate,decoration={text along path,
           text={a |\large|big |+\bf\color{red}|red|| juicy apple.}}] 
    (0,0) .. controls (0,2) and (3,0) .. (3,2);
\end{tikzpicture}
\end{codeexample}
}
	
    Internally, the text is stored in the macro |\pgfdecorationtext|. 
    Any characters that have not been typeset when the end of the 
    path has been reached will be stored in |\pgfdecorationrestoftext|.
    
  \end{key}

{\catcode`\|12
  \begin{key}{/pgf/decoration/text format delimiters=\marg{before}\marg{after} (initially \char`\{|\char`\}\char`\{\char`\})}

    \catcode`\|13
	
    Set the characters that the text decoration will use to parse 
    formatting commands. 
    If \meta{after} is empty, then \meta{before} will be used for both
    delimiters.
    In general you should stick to characters	whose category codes are 
    |11| or |12|.
    As |+| is used to indicate that the specifed format commands 
    are added	to any exisiting ones, you should avoid using |+| as
    a delimiter. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \path [decorate, decoration={text along path,text format delimiters={[}{]}, 
           text={A big [\color{red}]red[] and [\color{green}]green[] apple.}}] 
    (0,0) .. controls (0,2) and (3,0) .. (3,2);
\end{tikzpicture}
\end{codeexample}
  \end{key}
}

  \begin{key}{/pgf/decoration/text color=\meta{color}  (initially black)}
    The color of the text.
  \end{key}
\end{decoration}




\subsection{Mark Decorations: Adding Arrow Tips and Nodes on a Path}

\begin{pgflibrary}{decorations.markings}
  Markings are arbitrary ``marks'' that can be put on a path. Marks
  can be arrow tips or nodes or even whole pictures. 
\end{pgflibrary}

\begin{decoration}{markings}
  A \emph{marking} can be thought of a ``little picture'' or a more
  precisely of ``some scope contents'' that is placed ``on'' a path at
  a certain position. Suppose the marking should be a simple cross. We
  can produce this with the following code:
\begin{codeexample}[code only]
\draw (-2pt,-2pt) -- (2pt,2pt);
\draw (2pt,-2pt) -- (-2pt,2pt);
\end{codeexample}
  If we use this code as a marking at position |2cm| on a path, then
  the following happens: \pgfname\ determines the position on the path
  that is 2cm along the path. Then is translates the coordiante system
  to this position and rotates it such that the positive $x$-axis is
  tangent to the path. Then a protective scope is created, inside
  which the above code is executed -- resulting in a little cross on
  the path.

  The |markings| decoration allows you to place one or more such
  markings on a path. The decoration destroys the input path, which
  means that it uses the path for determining positions on the path,
  but after the decoration is done this path is gone. You typically
  need to use a |postaction| to add markings.

  Let us start with the above example in real code:
\begin{codeexample}[]
\begin{tikzpicture}[decoration={
    markings,% switch on markings
    mark=% actually add a mark
      at position 2cm
      with
      {
        \draw (-2pt,-2pt) -- (2pt,2pt);
        \draw (2pt,-2pt) -- (-2pt,2pt);
      }
    }
    ]
  \draw [help lines] grid (3,2);
  \draw [postaction={decorate}] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}  

  The |mark| decoration option is used to specify a marking. It has
  the following syntax:
  \begin{key}{/pgf/decoration/mark=|at position|
      \meta{pos}| with |\meta{code}}
    The options specifies that when a |marking| decoration is applied,
    there should be a marking at position \meta{pos} on the path whose
    code is given by \meta{code}.

    The \meta{pos} can have four different forms:
    \begin{enumerate}
    \item It can be a non-negative dimension like |0pt| or |2cm| or
      |5cm/2|. In this case, it refers to the position along the path
      that is this far removed from the start.
    \item It can be a negative dimesion like |-1cm-2pt| or |-1sp|. In
      this case, the position is taken from the end of the path. Thus,
      |-1cm| is the position that is $-1$cm removed from the end of
      the path.
    \item It can be a dimensionless non-negative number like |1/2| or
      |0.333+2*0.1|. In this case, the \meta{pos} is interpreted as a
      factor of the total path lenght. Thus, a \meta{pos} or |0.5|
      refers to the middle of the path, |0.1| is near the start, and
      so on.
    \item It can be a dimensionless negative number like |-0.1|. Then,
      again, the fraction of the path length counts ``from the end.''
    \end{enumerate}

    The \meta{pos} determines a position on the path. When the marking
    is applied, the (high level) coordinate system will have been
    transformed so that the origin lies at this position and the
    positive $x$-axis points along the path. For this coordinate
    system, the \meta{code} is executed. It can contains all sorts of
    graphic drawing commands, including (even named) nodes.

    If the position position lies past the end of the path (for
    instance if \meta{pos} is set to |1.2|), the marking will not be
    drawn.

    It is possible to give the |mark| option several times, which
    causes several markings to be applied. In this case, however, it
    is necessary that the positions on the path are in increasing
    order. That is, it is not allowed (and will result in chaos) to
    have a marking that lies earlier on the path to follow a marking
    that is later on the path.

\begin{codeexample}[]
\begin{tikzpicture}[decoration={
    markings,% switch on markings
    mark=at position 1cm  with \node[red]{1cm};,
    mark=at position .5   with \node[green]{mid};,
    mark=at position -1cm with {\node[blue,transform shape]{1cm from end};}}
    ]
  \draw [help lines] grid (3,2);
  \draw [postaction={decorate}] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}  

  Here is an example that shows how markings can be used to place text
  on plots:
\begin{codeexample}[]
\begin{tikzpicture}[domain=0:4,label/.style={postaction={
      decorate,
      decoration={
        markings,
        mark=at position .75 with \node #1;}}}]
  \draw[very thin,color=gray] (-0.1,-1.1) grid (3.9,3.9);
  
  \draw[->] (-0.2,0) -- (4.2,0) node[right] {$x$};
  \draw[->] (0,-1.2) -- (0,4.2) node[above] {$f(x)$};
  
  \draw[red,label={[above left]{$f(x)=x$}}]                       plot (\x,\x);
  \draw[blue,label={[below left]{$f(x)=\sin x$}}]                 plot (\x,{sin(\x r)});
  \draw[orange,label={[right]{$f(x)= \frac{1}{20} \mathrm e^x$}}] plot (\x,{0.05*exp(\x)});
\end{tikzpicture}
\end{codeexample}

    Frequent markings that are hard to create correctly are arrow
    tips. For them, inside the \meta{code} two special commands can be
    useful, which are only defined in this code:
    \begin{command}{\arrow\opt{\oarg{options}}\marg{arrow end tip}}
      This command simply draws the \meta{arrow end tip} at the origin,
      pointing right. This is exactly what you need when you want to
      draw an arrow tip as a marking.

      The \meta{options} can only be given when \tikzname\ is used. In
      this case, they are executed in a scope that contains the arrow
      tip. 
\begin{codeexample}[]
\begin{tikzpicture}[decoration={
    markings,% switch on markings
    mark=at position 1cm  with {\node[red]{1cm};},
    mark=at position .75  with {\arrow[blue,line width=2mm]{>}},
    mark=at position -1cm with {\arrowreversed[black]{stealth};}}
    ]
  \draw [help lines] grid (3,2);
  \draw [postaction={decorate}] (0,0) -- (3,1) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}  
   \end{command}
    \begin{command}{\arrowreversed\opt{\oarg{options}}\marg{arrow end tip}}
      As above, only the arrow end tip is flipped and points in the
      other direction. 
    \end{command}
  \end{key}

  \begin{key}{/pgf/decoration/reset marks}
    Since |mark| options accumulate, there needs to be a way to
    ``reset'' things, so that any |mark| options set in an enclosing
    scope do not interfere. This option does exactly this. Note that
    when the \meta{code} of a marking is executed, the markings are
    automatically reset.
  \end{key}
\end{decoration}




\subsection{Fractal Decorations}

\begin{pgflibrary}{decorations.fractals}
  The decorations of this library can be used to create fractal
  lines. To use them, you typically have to apply the decoration
  repeatedly to an originally straight path.
\end{pgflibrary}


\begin{decoration}{Koch curve type 1}
  This decoration replaces a straight line by a ``rectangular bump.''
  By repeatedly applying this replacement, different levels of the
  Koch curve fractal can be created. Its Hausdorff dimension is $\log
  5/\log 3$.
\begin{codeexample}[]
\begin{tikzpicture}[decoration=Koch curve type 1]
  \draw decorate{ (0,0) -- (3,0) };
  \draw decorate{ decorate{ (0,-1.5) -- (3,-1.5) }};
  \draw decorate{ decorate{ decorate{ (0,-3) -- (3,-3) }}};
\end{tikzpicture}
\end{codeexample}
\end{decoration}


\begin{decoration}{Koch curve type 2}
  This decoration replaces a straight line by a ``rectangular sine.''
  Its Hausdorff dimension is $3/2$.
\begin{codeexample}[]
\begin{tikzpicture}[decoration=Koch curve type 2]
  \draw decorate{ (0,0) -- (3,0) };
  \draw decorate{ decorate{ (0,-2) -- (3,-2) }};
  \draw decorate{ decorate{ decorate{ (0,-4) -- (3,-4) }}};
\end{tikzpicture}
\end{codeexample}
\end{decoration}

\begin{decoration}{Koch snowflake}
  This decoration replaces a straight line by a ``line with a spike.''
  Koch's snowflake's Hausdorff dimension is $\log 4/\log 3$.
\begin{codeexample}[]
\begin{tikzpicture}[decoration=Koch snowflake]
  \draw decorate{ (0,0) -- (3,0) };
  \draw decorate{ decorate{ (0,-1) -- (3,-1) }};
  \draw decorate{ decorate{ decorate{ (0,-2) -- (3,-2) }}};
  \draw decorate{ decorate{ decorate{ decorate{ (0,-3) -- (3,-3) }}}};
\end{tikzpicture}
\end{codeexample}
\end{decoration}

\begin{decoration}{Cantor set}
  This decoration replaces a straight line by a ``line with a whole in
  the middle.'' The Hausdorff dimension of the Cantor set is $\log
  2/\log 3$. 
\begin{codeexample}[]
\begin{tikzpicture}[decoration=Cantor set,very thick]
  \draw decorate{ (0,0) -- (3,0) };
  \draw decorate{ decorate{ (0,-.5) -- (3,-.5) }};
  \draw decorate{ decorate{ decorate{ (0,-1) -- (3,-1) }}};
  \draw decorate{ decorate{ decorate{ decorate{ (0,-1.5) -- (3,-1.5) }}}};
\end{tikzpicture}
\end{codeexample}
\end{decoration}




\subsection{Footprint Decorations}


\begin{pgflibrary}{decorations.footprints}
  The decorations of this library can be used to decorate a path with
  little footprints, as if someone had ``walked'' along the path.
\end{pgflibrary}


\begin{decoration}{footprints}
  The footprint decoration adds little footprints around the
  path. They start with the left foot.
\begin{codeexample}[]
\begin{tikzpicture}[decoration={footprints,foot length=5pt,stride length=10pt}]
  \draw [help lines] grid (3,3);
  \fill [decorate] (0,0) -- (3,2) arc (0:180:1.5 and 1);
\end{tikzpicture}
\end{codeexample}
  You can influence the way this decoration looks using the following
  options:
  \begin{key}{/pgf/decoration/foot length (initially 10pt)}
    The length or size of the footprint itself. A larger value makes
    the footprint larger, but does not change the stride length.
\begin{codeexample}[]
\begin{tikzpicture}[decoration={footprints,foot length=20pt}]
  \fill [decorate] (0,0) -- (3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/decoration/stride length (initially 30pt)}
    The length of strides. This is the distance between the beginnings
    of left footprints along the path.
\begin{codeexample}[]
\begin{tikzpicture}[decoration={footprints,stride length=50pt}]
  \fill [decorate] (0,0) -- (3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/decoration/foot sep (initially 4pt)}
    The separation in the middle between the footprints. The
    footprints are moved away from the path by half this amount.
\begin{codeexample}[]
\begin{tikzpicture}[decoration={footprints,foot sep=10pt}]
  \fill [decorate] (0,0) -- (3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/decoration/foot angle (initially 10)}
    Footprints are rotate by this much.
\begin{codeexample}[]
\begin{tikzpicture}[decoration={footprints,foot angle=60}]
  \fill [decorate] (0,0) -- (3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  \begin{key}{/pgf/decoration/foot of (initially human)}
    The species whose footprints are shown. Possible values are:

    \def\render#1{
      \texttt{#1} &
      \tikz [baseline,decoration={footprints,foot of=#1}]
        \fill [decorate] (0,0) -- (6,0); \\[3em]
    }
    \begin{tabular}{ll}
      \emph{Species} & \emph{Result} \\[1em]
      \render{gnome}
      \render{human}
      \render{bird}
      \render{felis silvestris}
    \end{tabular}
  \end{key}
\end{decoration}



\endinput





==> pgfmanual-en-library-edges.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{To Path Library}

\label{library-to-paths}

\begin{tikzlibrary}{topaths}
  This library provides predefined to paths for use with the |to|
  path operation. After loading this package, you can say for instance
  |to [loop]| to add a loop to a node.

  This library is loaded automatically by \tikzname, so you do not
  need to load it yourself.
\end{tikzlibrary}


\subsection{Straight Lines}

The following style installs a to path that is simply a straight line
from the start coordinate to the target coordinate.

\begin{key}{/tikz/line to}
  Causes a straight line to be added to the path upon a |to| or an
  |edge| operation.
\begin{codeexample}[]
\tikz {\draw (0,0) to[line to] (1,0);}
\end{codeexample}
\end{key}


\subsection{Curves}

The |curve to| style causes the to path to be set to a curve. The
exact way this curve looks can be influenced via a number of options.

\begin{key}{/tikz/curve to}
  Specifies that the |to path| should be a curve. This curve will
  leave the start coordinate at a certain angle, which can be
  specified using the |out| option. It reaches the target coordinate
  also at a certain angle, which is specified using the |in|
  option. The control points of the curve are at a certain distance
  that is computed in different ways, depending on which options are
  set.

  All of the following options implictly cause the |curve to| style to
  be installed.

  \begin{key}{/tikz/out=\meta{angle}}
    The angle at which the curve leaves the start coordinate. If the
    start coordinate is a node, the start coordinate is the point on the
    border of the node at the given \meta{angle}. The control point
    will, thus, lie at a certain distance in the direction \meta{angle}
    from the start coordinate.
\begin{codeexample}[]
\begin{tikzpicture}[out=45,in=135]
  \draw (0,0) to (1,0)
        (0,0) to (2,0)
        (0,0) to (3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  \begin{key}{/tikz/in=\meta{angle}}
    The angle at which the curve reaches the target coordinate.
  \end{key}

  \begin{key}{/tikz/relative=\meta{true or false} (default true)}
    This option tells \tikzname\ whether the |in| and |out| angles
    should be considered absolute or relative. Absolute means that an
    |out| angle of 30$^\circ$ means that the curve leaves the start
    coordinate at an angle of 30$^\circ$ relative to the paper (unless,
    of course, further transformations have been installed). A
    \emph{relative} angle is, by comparison, measured relative to a
    straight line from the start coordinate to the target
    coordinate. Thus, a relative angle of 30$^\circ$ means that the
    curve will bend to the left from the line going straight from the
    start to the target. For the target, the relative coordinate is
    measured in the same manner, namely relative to the line going from
    the start to the target. Thus, an angle of 150$^\circ$ means that
    the curve will reach target coming slightly from the left.

\begin{codeexample}[]
\begin{tikzpicture}[out=45,in=135,relative]
  \draw (0,0) to (1,0)
              to (2,1)
              to (2,2);
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[out=90,in=90,relative]
  \node [circle,draw] (a) at (0,0) {a};
  \node [circle,draw] (b) at (1,1) {b};
  \node [circle,draw] (c) at (2,2) {c};

  \path (a) edge (b)
            edge (c);
\end{tikzpicture}
\end{codeexample}
  \end{key}

  \begin{key}{/tikz/bend left=\meta{angle} (default \normalfont last value)}
    This option sets |out=|\meta{angle}|,in=|$180-\meta{angle}$|,relative|. If no
    \meta{angle} is given, the last given |bend left| or |bend right|
    angle is used.  
  
\begin{codeexample}[]
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,on grid]
  \node[state,initial]  (q_0)                {$q_0$};
  \node[state]          (q_1) [right=of q_0] {$q_1$};
  \node[state,accepting](q_2) [right=of q_1] {$q_2$};

  \path[->] (q_0) edge              node [above]  {0} (q_1)
                  edge [loop above] node          {1} ()
                  edge [bend left]  node [above]  {1} (q_2)
                  edge [bend right] node [below]  {0} (q_2)
            (q_1) edge              node [above]  {1} (q_2);
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \angle in {0,45,...,315}
    \node[rectangle,draw=black!50] (\angle) at (\angle:2) {\angle};

  \foreach \from/\to in {0/45,45/90,90/135,135/180,
                         180/225,225/270,270/315,315/0}
    \path (\from) edge [->,bend right=22,looseness=0.8] (\to)
                  edge [<-,bend left=22,looseness=0.8] (\to);
\end{tikzpicture}
\end{codeexample}
  \end{key}

  \begin{key}{/tikz/bend right=\meta{angle} (default \normalfont last  value)}
    Works like the |bend left| option, only the bend is to the other side.
  \end{key}

  \begin{key}{/tikz/bend angle=\meta{angle}}
    Sets the angle to be used by the |bend left| or |bend right|, but
    without actually selecting the |curve to| or the |relative|
    option. This is useful for globally specifying a |bend angle| for a
    whole picture.
  \end{key}

  \begin{key}{/tikz/looseness=\meta{number} (initially 1)}
    This number specifies how ``loose'' the curve will be. In detail,
    the following happens: \tikzname\ computes the distance between the
    start and the target coordinate (if the start and/or target
    coordinate are nodes, the distance is computed between the points on
    their border). This distance is then multiplied by a fixed factor
    and also by the factor \meta{number}. The resulting distance, let us
    call it $d$, is then used as the distance of the control points from
    the start and target coordinates.

    The fixed factor has been chosen in such a way that if \meta{number}
    is |1|, if the |in| and |out| angles differ by
    90$\circ$, then a quarter circle results:
  \begin{codeexample}[]
\tikz \draw (0,0) to [out=0,in=-90]               (1,1);
\tikz \draw (0,0) to [out=0,in=-90,looseness=0.5] (1,1);
  \end{codeexample}
  \end{key}

  \begin{key}{/tikz/out looseness=\meta{number}}
    specifies the looseness factor for the out distance only.
  \end{key}

  \begin{key}{/tikz/in looseness=\meta{number}}
    specifies the looseness factor for the in distance only.
  \end{key}
  \begin{key}{/tikz/min distance=\meta{distance}}
    If the computed distance for the start and target coordinates are
    below \meta{distance}, then \meta{distance} is used instead.
  \end{key}
  \begin{key}{/tikz/max distance=\meta{distance}}
    If the computed distance for the start and target coordinates are
    above \meta{distance}, then \meta{distance} is used instead.
  \end{key}
  \begin{key}{/tikz/out min distance=\meta{distance}}
    The mininimum distance set only for the start coordinate.
  \end{key}
  \begin{key}{/tikz/out max distance=\meta{distance}}
    The maximum distance set only for the start coordinate.
  \end{key}
  \begin{key}{/tikz/in min distance=\meta{distance}}
    The min distance set only for the target coordinate.
  \end{key}
  \begin{key}{/tikz/in max distance=\meta{distance}}
    The max distance set only for the target coordinate.
  \end{key}
  \begin{key}{/tikz/distance=\meta{distance}}
    Set the min and max distance to the same value \meta{distance}. Note
    that this causes any computed distance $d$ to be ignored and
    \meta{distance} to be used instead.
\begin{codeexample}[]
\begin{tikzpicture}[out=45,in=135,distance=1cm]
  \draw (0,0) to (1,0)
        (0,0) to (2,0)
        (0,0) to (3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  \begin{key}{/tikz/out distance=\meta{distance}}
    Sets the min and max out distance.
  \end{key}
  \begin{key}{/tikz/in distance=\meta{distance}}
    Sets the min and max in distance.
  \end{key}
  \begin{key}{/tikz/out control=\meta{coordinate}}
    This option causes the \meta{coordinate} to be used as the start
    control point. All computations of $d$ are ignored. You can use a
    coordinate like |+(1,0)| to specify a point relative to the start
    coordinate.
  \end{key}
  \begin{key}{/tikz/in control=\meta{coordinate}}
    This option causes the \meta{coordinate} to be used as the target
    control point.
  \end{key}
  \begin{key}{/tikz/controls=\meta{coordinate}| and |\meta{coordinate}}
    This option causes the \meta{coordinate}s to be used as control
    points. 
\begin{codeexample}[]
\tikz \draw (0,0) to [controls=+(90:1) and +(90:1)] (3,0);
\end{codeexample}
  \end{key}
\end{key}


\subsection{Loops}

\begin{key}{/tikz/loop}
  This key is similar to the |curve to| key, but differs in the
  following ways: First, the actual target coordinate is ignored and the
  start coordiante is used as the target coordinate. Thus, it is
  allowed not to provide any target coordinate, which can be useful
  with unnamed nodes. Second, the |looseness| is set to |8| and the
  |min distance| to |5mm|. These settings result in rather nice loops
  when the opening angle (difference between |in| and |out|) is
  30$^\circ$.
\begin{codeexample}[]
\begin{tikzpicture}
  \node [circle,draw] {a} edge [in=30,out=60,loop] ();    
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{stylekey}{/tikz/loop above}
  Sets the |loop| style and sets in and out angles such that
  loop is above the node. Furthermore, the |above| option is set,
  which causes a node label to be placed at the correct position. 
\begin{codeexample}[]
\begin{tikzpicture}
  \node [circle,draw] {a} edge [loop above] node {x} ();    
\end{tikzpicture}
\end{codeexample}
\end{stylekey}
\begin{stylekey}{/tikz/loop below} Works like the previous option. \end{stylekey}
\begin{stylekey}{/tikz/loop left} Works like the previous option. \end{stylekey}
\begin{stylekey}{/tikz/loop right} Works like the previous option. \end{stylekey}
\begin{stylekey}{/tikz/every loop (initially {->,shorten >=1pt})}
  This style is installed at the beginning of
  every loop.
\begin{codeexample}[]
\begin{tikzpicture}[every loop/.style={}]
  \draw (0,0) to [loop above] () to [loop right] ()
              to [loop below] () to [loop left]  ();
\end{tikzpicture}
\end{codeexample}
\end{stylekey}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-er.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Entity-Relationship Diagram Drawing Library}

\begin{tikzlibrary}{er}
  This packages provides styles for drawing entity-relationship
  diagrams. 
\end{tikzlibrary}

This library is intended to help you in creating E/R-diagrams. It defines
only very little new styles, but using these style |entity| instead of
saying |rectangle,draw| makes the code more expressive.


\subsection{Entities}

The package defines a simple style for drawing entities:

\begin{stylekey}{/tikz/entity}
  This style is to be used with nodes that represent entity types. It
  causes the node's shape to be set to a rectangle that is drawn and
  whose minimum size and width are set to sensible values.

  Note that this style is called |entity| despite the fact that it is
  to be used for nodes representing entity \emph{types} (the
  difference between an entity and an entity type is the same as the
  difference between an object and a class in object-oriented
  programming). If this bothers you, feel free to define a style
  |entity type| instead.
\begin{codeexample}[]
\begin{tikzpicture}
  \node[entity] (sheep)                   {Sheep};
  \node[entity] (genome) [right=of sheep] {Genome};
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/every entity}
  This stype is envoked by the style |entity|. To change the
  appearance of entities, you can change this style.
\begin{codeexample}[]
\begin{tikzpicture}
  [every entity/.style={draw=blue!50,fill=blue!20,thick}]
  \node[entity] (sheep)                   {Sheep};
  \node[entity] (genome) [right=of sheep] {Genome};
\end{tikzpicture}
\end{codeexample}
\end{stylekey}



\subsection{Relationships}

Relationships are drawn using styles that are very similar to the
styles for entities.

\begin{stylekey}{/tikz/relationship}
  This style works like |entity|, only it is to be used for
  relationships. Again, |relationship|s are actually relationship types. 
\begin{codeexample}[]
\begin{tikzpicture}
  \node[entity] (sheep)  at (0,0)   {Sheep};
  \node[entity] (genome) at (2,0)   {Genome};
  \node[relationship]    at (1,1.5) {has}
    edge (sheep) 
    edge (genome);
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/every relationship}
  Works like |every entity|.
\begin{codeexample}[]
\begin{tikzpicture}
  [every entity/.style={fill=blue!20,draw=blue,thick},
   every relationship/.style={fill=orange!20,draw=orange,thick,aspect=1.5}]
  \node[entity] (sheep)  at (0,0)   {Sheep};
  \node[entity] (genome) at (2,0)   {Genome};
  \node[relationship]    at (1,1.5) {has}
    edge (sheep) 
    edge (genome);
\end{tikzpicture}
\end{codeexample}
\end{stylekey}



\subsection{Attributes}

\begin{stylekey}{/tikz/attribute}
  This style is used to indicate that a node is an attribute. To
  connect an attribute to its entity, you can use, for example, the
  |child| command or the |pin| option. 
\begin{codeexample}[]
\begin{tikzpicture}
  \node[entity] (sheep)  {Sheep}
    child {node[attribute] {name}}
    child {node[attribute] {color}};
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}[every pin edge/.style=draw]    
  \node[entity,pin={[attribute]60:name},pin={[attribute]120:color}] {Sheep};
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/key attribute}
  This style is intended for key attributes. By default, the will
  cause the attribute to be typeset in italics. Typcially, underlining
  is used instead, but that looks ugly and it is difficult to
  implement in \TeX.
\end{stylekey}


\begin{stylekey}{/tikz/every attribute}
  This style is used with every (key) attribute.
\begin{codeexample}[]
\begin{tikzpicture}
  [text depth=1pt,
   every attribute/.style={fill=black!20,draw=black},
   every entity/.style={fill=blue!20,draw=blue,thick},
   every relationship/.style={fill=orange!20,draw=orange,thick,aspect=1.5}]

  \node[entity] (sheep)  at (0,0)   {Sheep}
    child {node  [key attribute] {name}};
  \node[entity] (genome) at (2,0)   {Genome};
  \node[relationship]    at (1,1.5) {has}
    edge (sheep) 
    edge (genome);
\end{tikzpicture}
\end{codeexample}
\end{stylekey}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-fadings.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Fading Library}
\label{section-library-fadings}

\begin{pgflibrary}{fadings}
  The package defines a number of fadings, see
  Section~\ref{section-tikz-transparency} for an introduction.  The
  \tikzname\ version defines special \tikzname\ commands for creating
  fadings. These commands are explained in
  Section~\ref{section-tikz-transparency}.   
\end{pgflibrary}

\newcommand\fadingindex[1]{%
  \index{#1@\protect\texttt{#1} fading}%
  \index{Fadings!#1@\protect\texttt{#1}}%
  \texttt{#1}& 
  \begin{tikzpicture}[baseline=5mm-.5ex]
    \fill [black!20] (0,0) rectangle (1,1);
    \path [pattern=checkerboard,pattern color=black!30] (0,0) rectangle (1,1);

    \fill [path fading=#1,blue] (0,0) rectangle (1,1);
  \end{tikzpicture} \\[4.5mm]
}

\noindent
\begin{tabular}{ll}
  \emph{Fading name} & \emph{Example (solid blue faded on checkerboard)} \\[1mm]
  \fadingindex{west}  
  \fadingindex{east}  
  \fadingindex{north}  
  \fadingindex{south} 
  \fadingindex{circle with fuzzy edge 10 percent} 
  \fadingindex{circle with fuzzy edge 15 percent} 
  \fadingindex{circle with fuzzy edge 20 percent} 
  \fadingindex{fuzzy ring 15 percent} 
\end{tabular}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-fit.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Fitting Library}
\label{section-library-fit}

\begin{tikzlibrary}{fit}
  The library defines (currently only one) option for fitting a node
  so that it contains a set of coordinates.
\end{tikzlibrary}

When you load this library, the following option becomes available:

\begin{key}{/tikz/fit=\meta{coordinates or nodes}}
  This option must be given to a |node| path command. The
  \meta{coordinates or nodes} should be a sequence of \tikzname\
  coordinates or node names,  one directly after the other without
  commas (like with the |plot coordinates| path operation). Examples
  as |(1,0) (2,2)| or |(a) (1,0) (b)|, where |a| and |b| are nodes.

  For this sequence of coordinates, a minimal bounding box is computed
  that encompasses all the listed \meta{coordinates or nodes}. For
  coordinates in the list, the bounding box is guaranteed to contain
  this coordinate, for nodes it is guaranteed to contain the |east|,
  |west|, |north| and |south| anchors of the node. In principle (the
  details will be explained in a moment), things are now setup such
  that the text box of the node will be exactly this bounding box.

  Here is an example: We fit several points in a rectangular node. By
  setting the |inner sep| to zero, we see exactly the text box of the
  node. Then we fit these points again in circular node. Note how
  the circle encompasses exactly the same bounding box.
\begin{codeexample}[]
\begin{tikzpicture}[inner sep=0pt,thick,
                    dot/.style={fill=blue,circle,minimum size=3pt}]
  \draw[help lines] (0,0) grid (3,2);
  \node[dot] (a) at (1,1) {};
  \node[dot] (b) at (2,2) {};
  \node[dot] (c) at (1,2) {};
  \node[dot] (d) at (1.25,0.25) {};
  \node[dot] (e) at (1.75,1.5) {};

  \node[draw=red,   fit=(a) (b) (c) (d) (e)] {box};
  \node[draw,circle,fit=(a) (b) (c) (d) (e)] {};
\end{tikzpicture}  
\end{codeexample}

  Every time the |fit| option is used, the following style is also
  applied to the node:
  \begin{stylekey}{/tikz/every fit (initially \normalfont empty)}
    Set this style to change the appearance of a node that uses the
    |fit| option.
  \end{stylekey}

  The exact effects of the |fit| option are the following:
  \begin{enumerate}
  \item A minimal bounding box containg all coordinates is
    computed. Note that if a coordinate like |(a)| is used that
    contain a node name, this has the same effect as explicitly
    providing the |(a.north)| and |(a.south)| and |(a.west)| and
    |(a.east)|. If you wish to refer only to the center of the |a|
    node, use  |(a.center)| instead.
  \item The |text width| option is set to the width of this bounding box.
  \item The |text centered| option is set.
  \item The |anchor| is set to |center|.
  \item The |at| position of the node is set to the center of the
    computed bounding box.
  \item After the node has been typeset, its height and depth are
    adjusted such that they add up to the height of the computed
    bounding box and such that the text of the node is vertically
    centered inside the box.
  \end{enumerate}
  The above means that, generally speaking, if the node contains text
  like |box| in the above example, it will be centered inside the
  box. It will be difficult to put the text elsewhere, in particular,
  changing the |anchor| of the node will not have the desired
  effect. Instead, what you should do is to create a node with the
  |fit| option that does not contain any text, give it a name, and
  then use normal nodes to add text at the desired
  positions. Alternatively, consider using the |label| or |pin|
  options. 

  Suppose, for instance, that in the above example we want the word
  ``box'' to appear inside the box, but at its top. This can be
  achieved as follows: 
\begin{codeexample}[]
\begin{tikzpicture}[inner sep=0pt,thick,
                    dot/.style={fill=blue,circle,minimum size=3pt}]
  \draw[help lines] (0,0) grid (3,2);
  \node[dot] (a) at (1,1) {};
  \node[dot] (b) at (2,2) {};
  \node[dot] (c) at (1,2) {};
  \node[dot] (d) at (1.25,0.25) {};
  \node[dot] (e) at (1.75,1.5) {};

  \node[draw=red,fit=(a) (b) (c) (d) (e)] (fit) {};
  \node[below] at (fit.north) {box};
\end{tikzpicture}  
\end{codeexample}

  Here is a real-life example that uses fitting:

\begin{codeexample}[]
\begin{tikzpicture}
  [vertex/.style={minimum size=2pt,fill,draw,circle},
   open/.style={fill=none},
   sibling distance=1.5cm,level distance=.75cm,
   every fit/.style={ellipse,draw,inner sep=-2pt},
   leaf/.style={label={[name=#1]below:$#1$}},auto]

  \node [vertex] (root) {}
  child { node [vertex,open] {}
    child { node [vertex,open] {}
      child { node [vertex] (b's parent) {}
        child { node [vertex] {}
          child { node [vertex,leaf=d] {} }
          child { node [vertex,leaf=e] {} } }
        child { node [vertex,leaf=b] {} } }
      child { node [vertex,leaf=a] {} } }
    child { node [coordinate] {}
      child[missing] 
      child { node [vertex] (f's parent) {}
        child { node [vertex,leaf=c] {} }
        child { node [vertex,leaf=f] {} } } }
    edge from parent node {$\rho$} };
  
  \node [fit=(d) (e) (b) (b's parent),label=above left:$F^{(b,R)}$] {};
  \node [fit=(c) (f) (f's parent),label=above right:$F^{(c,R)}$]    {};
\end{tikzpicture}
\end{codeexample}


\end{key}



==> pgfmanual-en-library-folding.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Paper Folding Diagrams Library}

\label{section-calender-folding}

\begin{tikzlibrary}{folding}
  This library defines commands for creating paper folding
  diagrams. Currently, it just contains a single command for creating
  a single diagram, but that one is really useful for creating
  calendars for your (real) desktop.
\end{tikzlibrary}

\begin{command}{\tikzfoldingdodecahedron|[|\meta{options}|];|}
  This command draws a folding diagram for a dodecahedron. The syntax
  is intended to remind of the |\path| command, but (currently) you
  must specify the \meta{options} and nothing else may be specified
  between the command name and the closing semicolon.

  The following keys may be used in the \meta{options}:
  \begin{key}{/tikz/folding line length=\meta{dimension}}
    Sets the length of the base line for folding. For the dodecahedron
    this is the length of all the sides of the pentagons.
  \end{key}
  \begin{key}{/tikz/face 1=\meta{code}}
    The \meta{code} is executed for the first face of the
    dodecahedron. When it is executed, the coordinate system will have
    been shifted and rotated such that it lies at the middle of the
    first face of the dodecahedron.
  \end{key}
  \begin{key}{/tikz/face 2=\meta{code}}
    Same as |face 1|, but for the second face.
  \end{key}
  \begin{key}{/tikz/face 3=\meta{code}}
    Same as |face 1|, but for the third face.
  \end{key}
  There are further similar options, ending with the following:
  \begin{key}{/tikz/face 12=\meta{code}}
    Same as |face 1|, but for the last face.
  \end{key}

  Here is a simple example:
\begin{codeexample}[]
\begin{tikzpicture}[transform shape]
  \tikzfoldingdodecahedron
  [folding line length=6mm,
  face 1={ \node[red] {1};},
  face 2={ \node      {2};},
  face 3={ \node      {3};},
  face 4={ \node      {4};},
  face 5={ \node      {5};},
  face 6={ \node      {6};},
  face 7={ \node      {7};},
  face 8={ \node      {8};},
  face 9={ \node      {9};},
  face 10={\node      {10};},
  face 11={\node      {11};},
  face 12={\node      {12};}];
\end{tikzpicture}
\end{codeexample}

  The appearance of the cut and folding lines can be influenced using
  the following styles:
  \begin{stylekey}{/tikz/every cut (initially \normalfont empty)}
    Executed for every line that should be cut using scissors.
  \end{stylekey}
  \begin{stylekey}{/tikz/every fold (initially help lines)}
    Executed for every line that should be
    folded.
\begin{codeexample}[]
\begin{tikzpicture}[every cut/.style=red,every fold/.style=dotted]
  \tikzfoldingdodecahedron[folding line length=6mm];
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
\end{command}

Here is a big example that produces a diagram for a calendar:

\begin{codeexample}[leave comments]
\sffamily\scriptsize
\begin{tikzpicture}
  [transform shape,
   every calendar/.style=
   {
     at={(-8ex,4ex)},
     week list,
     month label above centered,
     month text=\bfseries\textcolor{red}{\%mt} \%y0,
     if={(Sunday) [black!50]}
   }]
  \tikzfoldingdodecahedron
  [
    folding line length=2.5cm,
    face 1={ \calendar [dates=\the\year-01-01 to \the\year-01-last];},
    face 2={ \calendar [dates=\the\year-02-01 to \the\year-02-last];},
    face 3={ \calendar [dates=\the\year-03-01 to \the\year-03-last];},
    face 4={ \calendar [dates=\the\year-04-01 to \the\year-04-last];},
    face 5={ \calendar [dates=\the\year-05-01 to \the\year-05-last];},
    face 6={ \calendar [dates=\the\year-06-01 to \the\year-06-last];},
    face 7={ \calendar [dates=\the\year-07-01 to \the\year-07-last];},
    face 8={ \calendar [dates=\the\year-08-01 to \the\year-08-last];},
    face 9={ \calendar [dates=\the\year-09-01 to \the\year-09-last];},
    face 10={\calendar [dates=\the\year-10-01 to \the\year-10-last];},
    face 11={\calendar [dates=\the\year-11-01 to \the\year-11-last];},
    face 12={\calendar [dates=\the\year-12-01 to \the\year-12-last];}
  ];
\end{tikzpicture}
\end{codeexample}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-matrices.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Matrix Library}

\begin{tikzlibrary}{matrix}
  This library packages defines additional styles and options for
  creating matrices.
\end{tikzlibrary}


\subsection{Matrices of Nodes}

A \emph{matrix of nodes} is a \tikzname\ matrix in which each cell
contains a node. In this case it is bothersome having to write
|\node{| at the beginning of each cell and |};| at the end of each
cell. The following key simplifies typesetting such matrices.

\begin{key}{/tikz/matrix of nodes}
  Conceptually, this key adds |\node{| at the beginning and |};| at
  the end of each cell and sets the |anchor| of the node to
  |base|. Furthermore, it adds  the option |name| option to each node,
  where the name is set to  \meta{matrix name}|-|\meta{row
    number}|-|\meta{column number}. For  example, if the matrix has
  the name |my matrix|, then the node in  the upper left cell will get
  the name |my matrix-1-1|. 
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix (magic) [matrix of nodes]
  {
    8 & 1 & 6 \\
    3 & 5 & 7 \\
    4 & 9 & 2 \\
  };

  \draw[thick,red,->] (magic-1-1) |- (magic-2-3);
\end{tikzpicture}
\end{codeexample}

  You may wish to add options to certain nodes in the matrix. This can
  be achieved in three ways.
  \begin{enumerate}
  \item You can modify, say, the
    |row 2 column 5| style to pass special options to this particular
    cell.

\begin{codeexample}[]
\begin{tikzpicture}[row 2 column 3/.style=red]
  \matrix [matrix of nodes]
  {
    8 & 1 & 6 \\
    3 & 5 & 7 \\
    4 & 9 & 2 \\
  };
\end{tikzpicture}
\end{codeexample}
    
  \item At the beginning of a cell, you can use a special syntax. If a
    cell starts with a vertical bar, then everything between this bar
    and the next bar is passed on to the |node| command.
{\catcode`\|=12
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of nodes]
  {
    8 & 1 &         6 \\
    3 & 5 & |[red]| 7 \\
    4 & 9 &         2 \\
  };
\end{tikzpicture}
\end{codeexample}
}
  You can also use an option like \verb!|[red] (seven)|! to give a
  different name to the node.

  Note that the |&| character also takes an optional argument, which
  is an extra column skip.
{\catcode`\|=12  
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of nodes]
  {
    8 &[1cm] 1 &[3mm] |[red]| 6 \\
    3 &      5 &      |[red]| 7 \\
    4 &      9 &              2 \\
  };
\end{tikzpicture}
\end{codeexample}
}
  \item If your cell starts with a |\path| command or any command that
    expands to |\path|, which includes |\draw|, |\node|, |\fill| and
    others, the |\node{| startup code and the |};| code are
    suppressed. This means that for this particular cell you can
    provide a totally different contents.

\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of nodes]
  {
    8 & 1 & 6 \\
    3 & 5 & \node[red]{7}; \draw(0,0) circle(10pt);\\
    4 & 9 & 2 \\
  };
\end{tikzpicture}
\end{codeexample}
  \end{enumerate}
\end{key}

\begin{key}{/tikz/matrix of math nodes}
  This style is almost the same as the previous style, only |$| is %$
  added at the beginning and at the end of each node, so math mode
  will be switched on in all nodes.
{\catcode`\|=12
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of math nodes]
  {
    a_8 & a_1 &         a_6 \\
    a_3 & a_5 & |[red]| a_7 \\
    a_4 & a_9 &         a_2 \\
  };
\end{tikzpicture}
\end{codeexample}
}
\end{key}

\begin{key}{/tikz/nodes in empty cells=\meta{true or false} (default true)}
  When set to |true|, a node (with an empty contents) is put in empty
  cells. Normally, empty cells are just, well, empty. The style can be
  used together with both a |matrix of nodes| and a
  |matrix of math nodes|.
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of math nodes,nodes={circle,draw}]
  {
    a_8 &     & a_6 \\
    a_3 &     & a_7 \\
    a_4 & a_9 &     \\
  };
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of math nodes,nodes={circle,draw},nodes in empty cells]
  {
    a_8 &     & a_6 \\
    a_3 &     & a_7 \\
    a_4 & a_9 &     \\
  };
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsection{End-of-Lines and End-of-Row Characters in Matrices of Nodes}

Special care must be taken about the usage of the |\\| command inside
a matrix of nodes. The reason is that this character is overloaded in
\TeX: On the one hand, it is used to denote the end of a line in
normal text; on the other hand it is used to denote the end of a row
in a matrix. Now, if a matrix contains node which in turn may have
multiple lines, it is unclear which meaning of |\\| should be used.

This problem arises only when you use the |text width| option of
nodes. Suppose you write a line like
\begin{codeexample}[code only]
\matrix [text width=5cm,matrix of nodes]
{
  first row & upper line \\ lower line \\
  second row & hmm \\
};
\end{codeexample}
This leaves \TeX\ trying to riddle out how many rows this matrix
should have. Do you want two rows with the upper right cell containing
a two-line text. Or did you mean a three row matrix with the second
row having only one cell?

Since \TeX\ is not clairvoyant, the following rules are used:
\begin{enumerate}
\item Inside a matrix, the |\\| command, by default, signals the end
  of the row, not the end of a line in a cell.
\item However, there is an exception to this rule: If a cell
  starts with a \TeX-group (this is, with |{|), % }
  then inside this first group the |\\| command retains the meaning of
  ``end of line'' character. Note that this special rule works only
  for the first group in a cell and this group must be at the
  beginning. 
\end{enumerate}

The net effect of these rules is the following: Normally, |\\| is an
end-of-row indicator; if you want to use it as an end-of-line
indicator in a cell, just put the whole cell in curly braces. The
following example illustrates the difference:
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of nodes,nodes={text width=16mm,draw}]
  {
    row 1 & upper line \\ lower line \\
    row 2 & hmm \\
  };
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of nodes,nodes={text width=16mm,draw}]
  {
    row 1 & {upper line \\ lower line} \\
    row 2 & hmm \\
  };
\end{tikzpicture}
\end{codeexample}

Note that this system is not fool-proof. If you write things like
|a&b{c\\d}\\| in a matrix of nodes, an error will result (because the
second cell did not start with a brace, so |\\| retained its normal
meaning and, thus, the second cell contained the text |b{c|, which is
not balanced with respect to the number of braces).

\subsection{Delimiters}

Delimiters are parantheses or braces to the left and right of a
formula or a matrix. The matrix library offers options for adding such
delimiters to a matrix. However, delimiters can actually be added to
any node that has the standard anchors |north|, |south|, |north west|
and so on. In particular, you can add delimiters to any |rectangle|
box. They are implemented by ``measuring the height'' of the node and
then adding a delimiter of the correct size to the left or right using
some after node magic.

\begin{key}{/tikz/left delimiter=\meta{delimiter}}
  This option can be given to a any node that has the standard anchors
  |north|, |south| and so on. The \meta{delimiter} can be any
  delimiter that is acceptable to \TeX's |\left| command.
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of math nodes,left delimiter=(,right delimiter=\}]
  {
    a_8 & a_1 & a_6 \\
    a_3 & a_5 & a_7 \\
    a_4 & a_9 & a_2 \\
  };
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \node [fill=red!20,left delimiter=(,right delimiter=\}]
    {$\displaystyle\int_0^1 x\,dx$};
\end{tikzpicture}
\end{codeexample}

  \begin{stylekey}{/tikz/every delimiter (initially \normalfont empyt)}
    This style is executed for every delimiter. You can use it to shift
    or color delimiters or do whatever.
  \end{stylekey}

  \begin{stylekey}{/tikz/every left delimiter (initially \normalfont empty)}
    This style is additionally executed for every left delimiter.
\begin{codeexample}[]
\begin{tikzpicture}
  [every left delimiter/.style={red,xshift=1ex},
   every right delimiter/.style={xshift=-1ex}]
  \matrix [matrix of math nodes,left delimiter=(,right delimiter=\}]
  {
    a_8 & a_1 & a_6 \\
    a_3 & a_5 & a_7 \\
    a_4 & a_9 & a_2 \\
  };
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
\end{key}

\begin{key}{/tikz/right delimiter=\meta{delimiter}}
  Works as above.
  \begin{stylekey}{/tikz/every right delimiter (initially \normalfont empty)}
    Works as above.
  \end{stylekey}
\end{key}


\begin{key}{/tikz/above delimiter=\meta{delimiter}}
  This option allows you to add a delimiter above the node. It is
  implementing by rotating a left delimiter.
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix of math nodes,%
           left delimiter=\|,right delimiter=\rmoustache,%
           above delimiter=(,below delimiter=\}]
  {
    a_8 & a_1 & a_6 \\
    a_3 & a_5 & a_7 \\
    a_4 & a_9 & a_2 \\
  };
\end{tikzpicture}
\end{codeexample}

  \begin{stylekey}{/tikz/every above delimiter (initially \normalfont empty)}
    Works as above.
  \end{stylekey}
\end{key}

\begin{key}{/tikz/below delimiter=\meta{delimiter}}
  Works as above.
  \begin{stylekey}{/tikz/every below delimiter (initially \normalfont empty)}
    Works as above.
  \end{stylekey}
\end{key}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-mindmaps.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Mindmap Drawing Library}

\begin{tikzlibrary}{mindmap}
  This packages provides styles for drawing mindmap diagrams.
\end{tikzlibrary}

\subsection{Overview}

This library is intended to make the creation of mindmaps or concept
maps easier. A \emph{mindmap} is a graphical representation of a
concept together 
with related concepts and annotations. Mindmaps are, essentially,
trees, possibly with a few extra edges added, but they are usually
drawn in a special way: The root concept is placed in the middle of
the page and is drawn as a huge circle, ellipse, or cloud. The related
concepts then ``leave'' this root concept via branch-like tendrils.

The mindmap library of \tikzname\ produces mindmaps that look a bit
different from the standard mindmaps: While the big root concept is
still a circle, related concepts are also depicted as (smaller)
circles. The related concepts are linked to the root concept via
organic-looking connections. The overall effect is visually rather
pleasing, but readers may not immediately think of a mindmap when they
see a picture created with this library.

Although it is not strictly necessary, you will usually create
mindmaps using \tikzname's tree mechanism and some of the styles and
macros of the package work best when used inside trees. However, it is
still possible and sometimes necessary to treat parts of a mindmap as
a graph with arbitrary edges and this is also possible.


\subsection{The Mindmap Style}

Every mindmap should be put in a scope or a picture where the
|mindmap| style is used. This style installs some internal settings.

\begin{stylekey}{/tikz/mindmap}
  Use this style with all pictures or at least scopes that contain a
  mindmap. It installs a whole bunch of settings that are useful for
  drawing mindmaps. 
\begin{codeexample}[]
\tikz[mindmap,concept color=red!50]
  \node [concept] {Root concept}
    child[grow=right] {node[concept] {Child concept}};
\end{codeexample}
  The sizes of concepts are predefined in such a way that a
  medium-size mindmap will fit on an A4 page (more or less).  
  \begin{stylekey}{/tikz/every mindmap}
    This style is included by the |mindmap| style. Change this style to
    add special settings to your mindmaps.
\begin{codeexample}[]
\tikz[large mindmap,concept color=red!50]
  \node [concept] {Root concept}
    child[grow=right] {node[concept] {Child concept}};
\end{codeexample}
  \end{stylekey}
\end{stylekey}

\begin{stylekey}{/tikz/large mindmap}
  This style includes the |mindmap| style, but additionally changes
  the default size of concepts and of distances so that a medium-sized
  mindmap will fit on an A3 page (A3 pages are twice as large as A4
  pages).
\end{stylekey}
\begin{stylekey}{/tikz/huge mindmap}
  This style causes conepts to be even bigger and it is best used with
  A2 paper and above.
\end{stylekey}


\subsection{Concepts Nodes}

The basic entities of mindmaps are called \emph{concepts} in
\tikzname. A concept is a node of style |concept| and it must be
circular for some of the connection macros to work.


\subsubsection{Isolated Concepts}

The following styles influence how isolated concepts are rendered:

\begin{stylekey}{/tikz/concept}
  This style should be used with all nodes that are concepts, although
  some styles like |extra concept| install this style automatically.

  Bascially, this style makes the concept node circular and installs a
  uniform color called |concept color|, see below. Additionally, the
  style |every concept| is called.
\begin{codeexample}[]
\tikz[mindmap,concept color=red!50] \node [concept] {Some concept};
\end{codeexample}

  \begin{stylekey}{/tikz/every concept}
    In order to change the appearance of concept nodes, you should
    change this style. Note, however, that the color of a concept should
    be uniform for some of the connection bar stuff to work, so you
    should not change the color or the draw/fill state of concepts using
    this option. It is mostly useful for changing the text color and
    font.
  \end{stylekey}

  \begin{key}{/tikz/concept color=\meta{color}}
    This option tells \tikzname\ which color should be used for filling
    and stroking concepts. The difference between this option and just
    setting |every concept| to the desired color is that this option
    allows \tikzname\ to keep track of the colors used for
    concepts. This is important when you \emph{change} the color between
    two connected concepts. In this case, \tikzname\ can automatically
    create a shading that provides a smooth transition between the old
    and the new concept color; we will come back to this in the next
    section.
  \end{key}
\end{stylekey}

\begin{stylekey}{/tikz/extra concept}
  This style is intended for concepts that are not part of the
  ``mindmap tree,'' but stand beside it. Typically, they will have a
  subdued color are be smaller. In order to have these concepts appear
  in a uniform way and in order to indicate in the code that these
  concepts are extra, you can use this style.
\begin{codeexample}[]
\begin{tikzpicture}[mindmap,concept color=blue!80]
  \node [concept]                 {Root concept};
  \node [extra concept] at (10,0) {extra concept};
\end{tikzpicture}
\end{codeexample}
  \begin{stylekey}{/tikz/every extra concept}
    Change this style to change the appearance of extra concepts.
  \end{stylekey}
\end{stylekey}


\subsubsection{Concepts in Trees}

As pointed out earlier, \tikzname\ assumes that your mindmap is build
using the |child| facilities of \tikzname. There are numerous options
that influence how concepts are rendered at the different levels of a
tree. 

\begin{stylekey}{/tikz/root concept}
  This style is used for the roots of mindmap trees. By adding
  something to this, you can change how the root of a mindmap will be
  rendered.
\begin{codeexample}[]
\tikz
  [root concept/.append style={concept color=blue!80,minimum size=3.5cm},
   mindmap]
  \node [concept] {Root concept};
\end{codeexample}

  Note that styles like |large mindmap| redefine these styles, so you
  should add something to this style only inside the picture.
\end{stylekey}

\begin{stylekey}{/tikz/level 1 concept}
  The |mindmap| style adds this style to the |level 1| style. This
  means that the first level children of a mindmap tree will use this
  style. 
\begin{codeexample}[]
\tikz
  [root concept/.append style={concept color=blue!80},
   level 1 concept/.append style={concept color=red!50},
   mindmap]
  \node [concept] {Root concept}
    child[grow=30] {node[concept] {child}}
    child[grow=0 ] {node[concept] {child}};
\end{codeexample}
\end{stylekey}
\begin{stylekey}{/tikz/level 2 concept}
  Works like |level 1 concept|, only for second level children.
\end{stylekey}
\begin{stylekey}{/tikz/level 3 concept}
  Works like |level 1 concept|.
\end{stylekey}
\begin{stylekey}{/tikz/level 4 concept}
  Works like |level 1 concept|. Note that there are not fifth and
  higher level styles, you need to modify |level 5| directly in such
  cases. 
\end{stylekey}  

\begin{key}{/tikz/concept color=\meta{color}}
  We saw already that this option is used to change the color of
  concepts. We now have a look at its effect when used on child nodes
  of a concept. Normally, this option simply changes the color of the
  children. However, when the option is given as an option to the
  |child| operation (and not to the |node| operation and also not as
  an option to all children via the |level 1| style), \tikzname\ will
  smoothly change the concept color from the parent's color to the
  color of the child concept. 

  Here is an example:
\begin{codeexample}[]
\tikz[mindmap,concept color=blue!80]
  \node [concept] {Root concept}
    child[concept color=red,grow=30] {node[concept] {Child concept}}
    child[concept color=orange,grow=0]  {node[concept] {Child concept}};
\end{codeexample}

  In order to have all children of a certain level have a different
  concept color, a tiny bit of magic is needed:
\begin{codeexample}[]
\tikz[mindmap,text=white,
      root concept/.style={concept color=blue},
      level 1 concept/.append style=
        {every child/.style={concept color=blue!50}}]
  \node [concept] {Root concept}
    child[grow=30] {node[concept] {child}}
    child[grow=0 ] {node[concept] {child}};
\end{codeexample}
\end{key}

\subsection{Connecting Concepts}

\subsubsection{Simple Connections}

The easiest way to connect two concepts is to draw a line between
them. In order to give such lines a consistent appearance, it is
recommendable to use the following style when drawing such lines:

\begin{stylekey}{/tikz/concept connection}
  This style can be used for lines between two concepts. Feel free to
  redefine this style.
\end{stylekey}

A problem arises when you need to connect concepts after the main
mindmap has been drawn. In this case you will want the connection
lines to lie \emph{behind} the main mindmap. However, you can draw the
lines only after the coordinates of the concepts have been
determined. In this case you should place the connecting lines on a
background layer as in the following example:

\begin{codeexample}[]
\begin{tikzpicture}
  [root concept/.append style={concept color=blue!20,minimum size=2cm},
   level 1 concept/.append style={sibling angle=45},
   mindmap]
  \node [concept] {Root concept}
    [clockwise from=45]
    child { node[concept] (c1) {child}}
    child { node[concept] (c2) {child}}
    child { node[concept] (c3) {child}};
  \begin{pgfonlayer}{background}
    \draw [concept connection]  (c1) edge (c2)
                                     edge (c3)
                                (c2) edge (c3);
  \end{pgfonlayer}
\end{tikzpicture}
\end{codeexample}


\subsubsection{The Circle Connection Bar Decoration}

Instead of a simple line between two concepts, you can also add a bar
between the two nodes that has slightly organic ends. These bars are
also used by default as the edges from parents in the mindmap tree.

For the drawing of the bars a special decoration is used, which is defined
in the mindmap library:

\begin{decoration}{circle connection bar}
  This decoration can be used to connect two circles. The start of the
  to-be-decorated path should lie on the border of the first circle,
  the end should lie on the border of the second circle. The following
  two decoration keys should be initialized with the sizes of the circles:
  \begin{itemize}
  \item |start radius|
  \item |end radius|
  \end{itemize}
  Furthermore, the following two decoration keys influence the decoration:
  \begin{itemize}
  \item |amplitude|
  \item |angle|
  \end{itemize}
  The decoration turns a straight line into a path that starts on the border of the
  first circle at the specified angle relative to the line connecting
  the centers of the circles. The path then changes into a rectangle
  whose thickness is given by the amplitude. Finally, the path ends
  with the same angles on the second circle. 

  Here is an example that should make this clearer:
\begin{codeexample}[]
\begin{tikzpicture}
    [decoration={start radius=1cm,end radius=.5cm,amplitude=2mm,angle=30}]
  \fill[blue!20] (0,0) circle   (1cm);
  \fill[red!20]  (2.5,0) circle (.5cm);

  \filldraw [draw=red,fill=black,
             decorate,decoration=circle connection bar] (1,0) -- (2,0);
\end{tikzpicture}
\end{codeexample}

  As can be seen, the decorated path consists of three parts and is not really
  useful for drawing. However, if you fill the decorated path only, and if you
  use the same color as for the circles, the result is better.
\begin{codeexample}[]
\begin{tikzpicture}
  [blue!50,decoration={start radius=1cm,
                       end radius=.5cm,amplitude=2mm,angle=30}]
  \fill (0,0) circle   (1cm);
  \fill  (2.5,0) circle (.5cm);

  \fill [decorate,decoration=circle connection bar] (1,0) -- (2,0);
\end{tikzpicture}
\end{codeexample}

  In the above example you may notice the small white line between the
  circles and the decorated path. This is due to rounding
  errors. Unfortunately, for larger distances, there errors can
  accumulate quite strongly, especially since \tikzname\ and \TeX\ are
  not very good at computing square roots. For this reason, it is a
  good idea to make the circles slightly larger to cover up such
  problems. When using nodes of shape |circle|, you can just add the
  |draw| option with a |line width| or one or two points (for very
  large distances you may need line width up to 4pt). 
\begin{codeexample}[]
\begin{tikzpicture}
  [blue!50,decoration={start radius=1cm,
                       end radius=.5cm,amplitude=2mm,angle=30}]
  \fill (0,0) circle   (1cm+1pt);
  \fill  (2.4,0) circle (.5cm+1pt);

  \fill [decorate,decoration=circle connection bar] (1,0) -- (1.9,0);
\end{tikzpicture}
\end{codeexample}

  Note the slightly strange |outer sep=0pt|. This is needed so that
  the decorated path lies on the border of the filled circle, not on the
  border of the stroked circle (which is slightly larger and this
  slightly larger size is exactly what we wish to use to cover up the
  rounding errors).
\end{decoration}



\subsubsection{The Circle Connection Bar To-Path}

The |circle connection bar| decoration is a bit complicated to
use. Especially specifying the radii is quite bothersome (the
amplitude and the angle can be set once and for all). For this reason,
the mindmap library defines a special to-path, that performs the
necessary computations for you.

\begin{stylekey}{/tikz/circle connection bar}
  This style installs a rather involved to-path. Unlike normal
  to-paths, this path requires that the start and the target of the
  to-path are named nodes of shape |circle| -- if this is not the case,
  this path will produce errors.

  Assuming that the start and the target are circles, the to-path will
  first compute the radii of these circles (by measuring the distance
  from the |center| anchor to some anchor on the border) and will set
  the |start circle| keys accordingly. Next, the |fill| option
  is set to the |concept color| while |draw=none| is set. The decoration is
  set to |circle conncetion bar|. Finally, the following style is
  included:
  \begin{stylekey}{/tikz/every circle connection bar}
    Redefine this sytle to change the appearance of circle connection
    bar to-paths.      
  \end{stylekey}
\begin{codeexample}[]
\begin{tikzpicture}[concept color=blue!50,blue!50,outer sep=0pt]
  \node (n1) at (0,0)   [circle,minimum size=2cm,fill,draw,thick] {};
  \node (n2) at (2.5,0) [circle,minimum size=1cm,fill,draw,thick] {};

  \path (n1) to[circle connection bar] (n2);
\end{tikzpicture}
\end{codeexample}
  Note that it is not a good idea to have more than one |to| operation
  together this the option |circle connection bar| in a single
  |\path|. Use the |edge| operation, instead, for creating multiple
  connections and this operation creates a new scope for each edge.
\end{stylekey}

In a mindmap we sometimes want colors to change from one concept color
to another. Then, the connection bar should, ideally, consist of a
smooth transition between these two colors. Getting this right using
shadings is a bit tricky if you try this ``by hand,'' so the  mindmap
library provides a special option for facilitating this procedure.

\begin{key}{/tikz/circle connection bar switch color=|from (|\meta{first
    color}|) to (|\meta{second color}|)|}
  This style works similarly to the |circle connection bar|. The only
  difference is that instead of filling the path with a single color a
  shading is used.
\begin{codeexample}[]
\begin{tikzpicture}[outer sep=0pt]
  \node (n1) at (0,0)    [circle,minimum size=2cm,fill,draw,thick,red] {};
  \node (n2) at (30:2.5) [circle,minimum size=1cm,fill,draw,thick,blue] {};

  \path (n1) to[circle connection bar switch color=from (red) to (blue)] (n2);
\end{tikzpicture}  
\end{codeexample}
\end{key}


\subsubsection{Tree Edges}

Most of the time, concepts in a mindmap are connected automatically
when the mindmap is build as a tree. The reason is that the |mindmap|
installs a |circle connection bar| path as the edge from parent
path. Also, the |mindmap| option takes care of things like setting the
correct |draw| and |outer sep| settings and some other stuff.

In detail, the |mindmap| option sets the |edge from parent path| to a
path that uses the to-path |circle connection bar| to connect the parent node
and the child node. The |concept color| option (locally) changes this
by using |circle connection bar switch color| instead with the
from-color set to the old (parent's) concept color and the to-color
set to the new (child's) concept color. This menas that when you
provide the |concept color| option to a |child| command, the color
will change from the parent's concept color to the specified color.

Here is an example of a tree build in this way:

\begin{codeexample}[]
\begin{tikzpicture}
  \path[mindmap,concept color=black,text=white]
    node[concept] {Computer Science}
    [clockwise from=0]
    child[concept color=green!50!black] {
      node[concept] {practical}
      [clockwise from=90]
      child { node[concept] {algorithms} }
      child { node[concept] {data structures} }
      child { node[concept] {pro\-gramming languages} }
      child { node[concept] {software engineer\-ing} }
    }  
    child[concept color=blue] {
      node[concept] {applied}
      [clockwise from=-30]
      child { node[concept] {databases} }
      child { node[concept] {WWW} }
    }
    child[concept color=red] { node[concept] {technical} }
    child[concept color=orange] { node[concept] {theoretical} };
\end{tikzpicture}
\end{codeexample}



\subsection{Adding Annotations}

An \emph{annotation} is some text outside a mindmap that, unlike an
extra concept, simply explains something in the mindmap. The following
style is mainly intended to help readers of the code see that a node
in an annotation node.

\begin{stylekey}{/tikz/annotation}
  This style indicates that a node is an annotation node. It includes
  the style |every annotation|, which allows you to change this style
  in a convenient fashion.
\begin{codeexample}[]

\begin{tikzpicture}
  [mindmap,concept color=blue!80,
  every annotation/.style={fill=red!20}]
  \node [concept] (root)  {Root concept};

  \node [annotation,right] at (root.east)
  {The root concept is, in general, the most important concept.};
\end{tikzpicture}
\end{codeexample}
  \begin{stylekey}{/tikz/every annotation}
    This style is included by |annotation|.
  \end{stylekey}
\end{stylekey}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-patterns.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Pattern Library}
\label{section-library-patterns}

\begin{pgflibrary}{patterns}
  The package defines patterns for filling areas.
\end{pgflibrary}


\newcommand\patternindex[1]{%
  \index{#1@\protect\texttt{#1} pattern}%
  \index{Patterns!#1@\protect\texttt{#1}}%
  \texttt{#1}& 
  \begin{tikzpicture}[baseline=.5ex]

    % Background
    \pattern [path fading=west,pattern=checkerboard light gray]
      (0,0) rectangle (5cm,2em);
    
    \pattern [pattern=#1,pattern color=black] (0,0) rectangle +(1.5cm,2em);
    \pattern [pattern=#1,pattern color=blue] (1.75,0) rectangle +(1.5cm,2em);
    \pattern [pattern=#1,pattern color=red] (3.5,0) rectangle +(1.5cm,2em);
  \end{tikzpicture} \\[1ex]
}

\newcommand\patternindexinherentlycolored[1]{%
  \index{#1@\protect\texttt{#1} pattern}%
  \index{Patterns!#1@\protect\texttt{#1}}%
  \texttt{#1}& 
  \begin{tikzpicture}[baseline=.5ex]

    % Background
    \pattern [path fading=west,pattern=checkerboard light gray]
      (0,0) rectangle (5cm,2em);
    
    \pattern [pattern=#1,pattern color=blue] (0,0) rectangle +(5cm,2em);
  \end{tikzpicture} \\[1ex]
}

\subsection{Form-Only Patterns}

\begin{tabular}{ll}
  \emph{Pattern name} & \emph{Example (pattern in black, blue, and red
    on faded checkerboard)} \\ 
  \patternindex{horizontal lines} 
  \patternindex{vertical lines} 
  \patternindex{north east lines} 
  \patternindex{north west lines} 
  \patternindex{grid} 
  \patternindex{crosshatch} 
  \patternindex{dots} 
  \patternindex{crosshatch dots} 
  \patternindex{fivepointed stars} 
  \patternindex{sixpointed stars} 
  \patternindex{bricks}
  \patternindex{checkerboard}
\end{tabular}
  
\subsection{Inherently Colored Patterns}


\begin{tabular}{ll}
  \emph{Pattern name} & \emph{Example} \\
  \patternindexinherentlycolored{checkerboard light gray} 
  \patternindexinherentlycolored{horizontal lines light gray} 
  \patternindexinherentlycolored{horizontal lines gray} 
  \patternindexinherentlycolored{horizontal lines dark gray} 
  \patternindexinherentlycolored{horizontal lines light blue} 
  \patternindexinherentlycolored{horizontal lines dark blue} 
  \patternindexinherentlycolored{crosshatch dots gray} 
  \patternindexinherentlycolored{crosshatch dots light steel blue} 
\end{tabular}
  

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-petri.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Petri-Net Drawing Library}

\begin{tikzlibrary}{petri}
  This packages provides shapes and styles for drawing Petri nets. 
\end{tikzlibrary}



\subsection{Places}

The package defines a style for drawing places of Petri nets. 

\begin{stylekey}{/tikz/place}
  This style indicates that a node is a place of a Petri net. Usually,
  the text of the node should be empty since places do not contain any
  text. You should use the |label| option to add text outside the node
  like its name or its capacity. You should use the |tokens| options,
  explained in Section~\ref{section-tokens}, to add tokens inside the
  place.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \node[place,label=above:$p_1$,tokens=2]        (p1) {};
  \node[place,label=below:$p_2\ge1$,right=of p1] (p2) {};
\end{tikzpicture}
\end{codeexample}
  
  \begin{stylekey}{/tikz/every place}
    This stype is envoked by the style |place|. To change the
    appearance of places, you can change this style.
\begin{codeexample}[]
\begin{tikzpicture}
  [every place/.style={draw=blue,fill=blue!20,thick,minimum size=9mm}]
  \node[place,tokens=7,label=above:$p_1$]  (p1) {};
  \node[place,structured tokens={3,2,9},
        label=below:$p_2\ge1$,right=of p1] (p2) {};
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
\end{stylekey}




\subsection{Transitions}

Transitions are also nodes. They should be drawn using the following
style: 

\begin{stylekey}{/tikz/transition}
  This style indicates that a node is a transition. As for places, the
  text of a transition should be empty and the |label| option should
  be used for adding labels.

  To connect a transition to places, you can use the |edge| command as
  in the following example:
  
\begin{codeexample}[]
\begin{tikzpicture}
  \node[place,tokens=2,label=above:$p_1$]        (p1) {};
  \node[place,label=above:$p_2\ge1$,right=of p1] (p2) {};

  \node[transition,below right=of p1,label=below:$t_1$] {}
    edge[pre]                 (p1)
    edge[post] node[auto] {2} (p2);
\end{tikzpicture}
\end{codeexample}
  
  \begin{stylekey}{/tikz/every transition}
    This style is envoked by the style |transition|.
  \end{stylekey}

  \begin{stylekey}{/tikz/pre}
    This style can be used with paths leading \emph{from} a transition
    \emph{to} a place to indicate that the place is in the pre-set of
    the transition. By default, this style is |<-,shorten <=1pt|, but
    feel free to redefine it.
  \end{stylekey}

  \begin{stylekey}{/tikz/post}
    This style is also used with paths leading \emph{from} a transition
    \emph{to} a place, but this time the place is in the post-set of
    the transition. Again, feel free to redefine it.
  \end{stylekey}

  \begin{stylekey}{/tikz/pre and post}
    This style is to be used to indicate that a place is both in the
    pre- and post-set of a transition.
  \end{stylekey}
\end{stylekey}


\subsection{Tokens}
\label{section-tokens}

Interestingly, the most complicated aspect of drawing Petri nets in
\tikzname\ turns out to be the placement of tokens.

Let us start with a single token. They are also nodes and there is a
simple style for typesetting them.

\begin{stylekey}{/tikz/token}
  This style indicates that a node is a token. By default, this causes
  the node to be a small black circle. Unlike places and transitions,
  it \emph{does} make sense to provide text for the token node. Such
  text will be typeset in a tiny font and in white on black
  (naturally, you can easily change this by setting the style
  |every token|).
    
\begin{codeexample}[]
\begin{tikzpicture}
  \node[place,label=above:$p_1$]             (p1) {};
  \node[token] at (p1) {};

  \node[place,label=above:$p_2$,right=of p1] (p2) {};
  \node[token] at (p2) {$y$};
\end{tikzpicture}
\end{codeexample}
  \begin{stylekey}{/tikz/every token}
    Change this style to chagne the appearance of tokens.
  \end{stylekey}
\end{stylekey}

In the above example, it is bothersome that we need an extra command
for the token node. Worse, when we have \emph{two} tokens on a node,
it is difficult to place both nodes inside the node without overlap.

The Petri net library offers a solution to this problem: The
|children are tokens| style.


\begin{stylekey}{/tikz/children are tokens}
  The idea behind this style is to use trees mechanism for placing
  tokens. Every token lying on a place is treated as a child of the
  node. Normally this would have the effect that the tokens are placed
  below the place and they would be connected to the place by an
  edge. The |children are tokens| style, however, redefines the growth
  function of trees such that it places the children next to each
  other inside (or, rather, on top) of the place node. Additionally,
  the edge from the parent node is not drawn.
\begin{codeexample}[]
\begin{tikzpicture}
  \node[place,label=above:$p_1$] {}
  [children are tokens]
  child {node [token] {1}}
  child {node [token] {2}}
  child {node [token] {3}};
\end{tikzpicture}
\end{codeexample}

  In detail, what happens is the following: Tree growth functions tell
  \tikzname\ where it should place the children of nodes. These
  functions get passed the number of children that a node has an the
  number of the child that should be placed. The special tree growth
  function for tokens has a special mapping for each possible number
  of children up to nine children. This mapping decides for each child
  where it should be placed on top of the place. For example, a single
  child is placed directly on top of the place. Two children are
  placed next to each other, separated by the |token distance|. Three
  children are placed in a triangle whose side lengths are
  |token distance|; and so on up to nine tokens. If you wish to place
  more than nice tokens on a place, you will have to write your own
  placement code.
\begin{codeexample}[]
\begin{tikzpicture}
  \node[place,label=above:$p_2$] {}
  [children are tokens]
  child {node [token] {1}}
  child {node [token,fill=red] {2}}
  child {node [token,fill=red] {2}}
  child {node [token] {1}};
\end{tikzpicture}
\end{codeexample}

  \begin{key}{/tikz/token distance=\meta{distance}}
  This specifies the distance between the centers of the tokens in the
  arrangements of the option |children are tokens|.
\begin{codeexample}[]
\begin{tikzpicture}
  \node[place,label=above:$p_3$] {}
  [children are tokens,token distance=1.1ex]
  child {node [token] {}}
  child {node [token,red] {}}
  child {node [token,blue] {}}
  child {node [token] {}};
\end{tikzpicture}
\end{codeexample}
  \end{key}
\end{stylekey}

The |children are tokens| options gives you a lot of flexibility, but
it is a bit cumbersome to use. For this reason there are some options
that help in standard situations. They all use |children are tokens|
internally, so any change to, say, the |every tokens| style will
affect how these options depict tokens.

\begin{key}{/tikz/tokens=\meta{number}}
  This option is given to a |place| node, not to a |token| node. The
  effect of this option is to add \meta{number} many child nodes to
  the place, each having the style |token|. Thus, the following two
  pieces of codes have the same effect:
\begin{codeexample}[]
\tikz
  \node[place] {}
  [children are tokens]
  child {node [token] {}}
  child {node [token] {}}
  child {node [token] {}};
\tikz
  \node[place,tokens=3] {};
\end{codeexample}
  It is legal to say |tokens=0|, no tokens are drawn in this
  case. This option does not handle ten or more tokens correctly. If
  you need this many tokens, you will have to program your own code.
\begin{codeexample}[]
\begin{tikzpicture}[every place/.style={minimum size=9mm}]

  \foreach \x/\y/\tokennumber in {0/2/1,1/2/2,2/2/3,
                                  0/1/4,1/1/5,2/1/6,
                                  0/0/7,1/0/8,2/0/9}
    \node [place,tokens=\tokennumber] at (\x,\y) {};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/colored tokens=\meta{color list}}
  This option, which must also be given when a place node is being
  created, gets a list of colors as parameter. It will then add as
  many tokens to the place are in this list, each colored with the
  corresponding color in the list.
\begin{codeexample}[]
\tikz  \node[place,colored tokens={black,black,red,blue}] {};
\end{codeexample}
\end{key}
\begin{key}{/tikz/structured tokens=\meta{token texts}}
  This option, which must again be passed to a place, gets a list
  texts for tokens. For each text, another token will be added to the place.
\begin{codeexample}[]
\tikz  \node[place,structured tokens={$x$,$y$,$z$}] {};
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}[every place/.style={minimum size=9mm}]

  \foreach \x/\y/\tokennumber in {0/2/1,1/2/2,2/2/3,
                                  0/1/4,1/1/5,2/1/6,
                                  0/0/7,1/0/8,2/0/9}
    \node [place,structured tokens={1,...,\tokennumber}] at (\x,\y) {};
\end{tikzpicture}
\end{codeexample}
  If you use lots of structured tokens, consider redefining the
  |every token| style so that the tokens are larger.
\end{key}


\subsection{Examples}


\begin{codeexample}[]
\begin{tikzpicture}[yscale=-1.6,xscale=1.5,thick,
  every transition/.style={draw=red,fill=red!20,minimum size=3mm},
  every place/.style={draw=blue,fill=blue!20,minimum size=6mm}]

  \foreach \i in {1,...,6} {
    \node[place,label=left:$p_\i$] (p\i) at (0,\i) {}; 
    \node[place,label=right:$q_\i$] (q\i) at (8,\i) {};
  }
  \foreach \name/\var/\vala/\valb/\height/\x in
      {m1/m_1/f/t/2.25/3,m2/m_2/f/t/2.25/5,h/\mathit{hold}/1/2/4.5/4} {
    \node[place,label=above:{$\var = \vala$}] (\name\vala) at (\x,\height) {};
    \node[place,yshift=-8mm,label=below:{$\var = \valb$}] (\name\valb) at (\x,\height) {};
  }
  \node[token] at (p1) {};   \node[token] at (q1) {};
  \node[token] at (m1f) {};  \node[token] at (m2f) {};
  \node[token] at (h1) {};

  \node[transition] at (1.5,1.5) {}  edge [pre] (p1)  edge [post] (p2);
  \node[transition] at (1.5,2.5) {}  edge[pre] (p2)   edge[pre] (m1f)
                                     edge[post] (p3)  edge[post] (m1t);
  \node[transition] at (1.5,3.3) {}  edge [pre] (p3)  edge [post] (p4)
                                     edge [pre and post] (h1);
  \node[transition] at (1.5,3.7) {}  edge [pre] (p3)  edge [pre] (h2)
                                     edge [post] (p4) edge [post] (h1.west);
  \node[transition] at (1.5,4.3) {}  edge [pre] (p4)  edge [post] (p5)
                                     edge [pre and post] (m2f);
  \node[transition] at (1.5,4.7) {}  edge [pre] (p4)  edge [post] (p5)
                                     edge [pre and post] (h2);
  \node[transition] at (1.5,5.5) {}  edge [pre] (p5)  edge [pre] (m1t)
                                     edge [post] (p6) edge [post] (m1f);
  \node[transition] at (1.5,6.5) {}  edge [pre] (p6)  edge [post] (p1.south east);
  \node[transition] at (6.5,1.5) {}  edge [pre] (q1)  edge [post] (q2);
  \node[transition] at (6.5,2.5) {}  edge [pre] (q2)  edge [pre] (m2f)
                                     edge [post] (q3) edge [post] (m2t);
  \node[transition] at (6.5,3.3) {}  edge [pre] (q3)  edge [post] (q4)
                                     edge [pre and post] (h2);
  \node[transition] at (6.5,3.7) {}  edge [pre] (q3)  edge [pre] (h1)
                                     edge [post] (q4) edge [post] (h2.east);
  \node[transition] at (6.5,4.3) {}  edge [pre] (q4)  edge [post] (q5)
                                     edge [pre and post] (m1f);
  \node[transition] at (6.5,4.7) {}  edge [pre] (q4)  edge [post] (q5)
                                     edge [pre and post] (h1);
  \node[transition] at (6.5,5.5) {}  edge [pre] (q5)  edge [pre] (m2t)
                                     edge [post] (q6) edge [post] (m2f);
  \node[transition] at (6.5,6.5) {}  edge [pre] (q6)  edge [post] (q1.south west);
\end{tikzpicture}  
\end{codeexample}

Here is the same net once more, but with these styles changes:
\begin{codeexample}[code only]
\begin{tikzpicture}[yscale=-1.1,thin,>=stealth,
  every transition/.style={fill,minimum width=1mm,minimum height=3.5mm},
  every place/.style={draw,thick,minimum size=6mm}]
\end{codeexample}

\begin{tikzpicture}[yscale=-1.1,thin,>=stealth,
  every transition/.style={fill,minimum width=1mm,minimum height=3.5mm},
  every place/.style={draw,thick,minimum size=6mm}]

  \foreach \i in {1,...,6} {
    \node[place,label=left:$p_\i$] (p\i) at (0,\i) {}; 
    \node[place,label=right:$q_\i$] (q\i) at (8,\i) {};
  }
  \foreach \name/\var/\vala/\valb/\height/\x in
      {m1/m_1/f/t/2.25/3,m2/m_2/f/t/2.25/5,h/\mathit{hold}/1/2/4.5/4} {
    \node[place,label=above:{$\var = \vala$}] (\name\vala) at (\x,\height) {};
    \node[place,yshift=-8mm,label=below:{$\var = \valb$}] (\name\valb) at (\x,\height) {};
  }
  \node[token] at (p1) {};   \node[token] at (q1) {};
  \node[token] at (m1f) {};  \node[token] at (m2f) {};
  \node[token] at (h1) {};

  \node[transition] at (1.5,1.5) {}  edge [pre] (p1)  edge [post] (p2);
  \node[transition] at (1.5,2.5) {}  edge[pre] (p2)   edge[pre] (m1f)
                                     edge[post] (p3)  edge[post] (m1t);
  \node[transition] at (1.5,3.3) {}  edge [pre] (p3)  edge [post] (p4)
                                     edge [pre and post] (h1);
  \node[transition] at (1.5,3.7) {}  edge [pre] (p3)  edge [pre] (h2)
                                     edge [post] (p4) edge [post] (h1.west);
  \node[transition] at (1.5,4.3) {}  edge [pre] (p4)  edge [post] (p5)
                                     edge [pre and post] (m2f);
  \node[transition] at (1.5,4.7) {}  edge [pre] (p4)  edge [post] (p5)
                                     edge [pre and post] (h2);
  \node[transition] at (1.5,5.5) {}  edge [pre] (p5)  edge [pre] (m1t)
                                     edge [post] (p6) edge [post] (m1f);
  \node[transition] at (1.5,6.5) {}  edge [pre] (p6)  edge [post] (p1.south east);
  \node[transition] at (6.5,1.5) {}  edge [pre] (q1)  edge [post] (q2);
  \node[transition] at (6.5,2.5) {}  edge [pre] (q2)  edge [pre] (m2f)
                                     edge [post] (q3) edge [post] (m2t);
  \node[transition] at (6.5,3.3) {}  edge [pre] (q3)  edge [post] (q4)
                                     edge [pre and post] (h2);
  \node[transition] at (6.5,3.7) {}  edge [pre] (q3)  edge [pre] (h1)
                                     edge [post] (q4) edge [post] (h2.east);
  \node[transition] at (6.5,4.3) {}  edge [pre] (q4)  edge [post] (q5)
                                     edge [pre and post] (m1f);
  \node[transition] at (6.5,4.7) {}  edge [pre] (q4)  edge [post] (q5)
                                     edge [pre and post] (h1);
  \node[transition] at (6.5,5.5) {}  edge [pre] (q5)  edge [pre] (m2t)
                                     edge [post] (q6) edge [post] (m2f);
  \node[transition] at (6.5,6.5) {}  edge [pre] (q6)  edge [post] (q1.south west);
\end{tikzpicture}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-plot-handlers.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Plot Handler Library}
\label{section-library-plothandlers}

\begin{pgflibrary}{plothandlers}
  This library packages defines additional plot handlers, see
  Section~\ref{section-plot-handlers} for an introduction to plot
  handlers. The additional handlers are described in the following.

  This library is loaded automatically by \tikzname.
\end{pgflibrary}


\subsection{Curve Plot Handlers}
  
\begin{command}{\pgfplothandlercurveto}
  This handler will issue a |\pgfpathcurveto| command for each point of
  the plot, \emph{except} possibly for the first. As for the line-to
  handler, what happens with the first point can be specified using
  |\pgfsetmovetofirstplotpoint| or |\pgfsetlinetofirstplotpoint|.

  Obviously, the |\pgfpathcurveto| command needs, in addition to the
  points on the path, some control points. These are generated
  automatically using a somewhat ``dumb'' algorithm: Suppose you have
  three points $x$, $y$, and $z$ on the curve such that $y$ is between
  $x$ and $z$:
\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlercurveto
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}

  In order to determine the control points of the curve at the point
  $y$, the handler computes the vector $z-x$ and scales it by the
  tension factor (see below). Let us call the resulting vector
  $s$. Then $y+s$ and $y-s$ will be the control points around $y$. The
  first control point at the beginning of the curve will be the
  beginning itself, once more; likewise the last control point is the
  end itself.
\end{command}

\begin{command}{\pgfsetplottension\marg{value}}
  Sets the factor used by the curve plot handlers to determine the
  distance of the control points from the points they control. The
  higher the curvature of the curve points, the higher this value
  should be. A value of $1$ will cause four points at quarter
  positions of a circle to be connected using a circle. The default is
  $0.5$. 

\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfsetplottension{0.75}
  \pgfplothandlercurveto
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgfplothandlerclosedcurve}
  This handler works like the curve-to plot handler, only it will
  add a new part to the current path that is a closed curve through
  the plot points.
\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlerclosedcurve
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}


\subsection{Comb Plot Handlers}

There are three ``comb'' plot handlers. There name stems from the fact
that the plots they produce look like ``combs'' (more or less).

\begin{command}{\pgfplothandlerxcomb}
  This handler converts each point in the plot stream into a line from
  the $y$-axis to the point's coordinate, resulting in a ``horizontal
  comb.''

  
\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlerxcomb
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgfplothandlerycomb}
  This handler converts each point in the plot stream into a line from
  the $x$-axis to the point's coordinate, resulting in a ``vertical
  comb.''
  
  This handler is useful for creating ``bar diagrams.''
\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlerycomb
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfplothandlerpolarcomb}
  This handler converts each point in the plot stream into a line from
  the origin to the point's coordinate.
  
\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlerpolarcomb
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}

\subsection{Mark Plot Handler}

\label{section-plot-marks}

\begin{command}{\pgfplothandlermark\marg{mark code}}
  This command will execute the \meta{mark code} for some points of the
  plot, but each time the coordinate transformation matrix will be
  setup such that the origin is at the position of the point to be
  plotted. This way, if the \meta{mark code} draws a little circle
  around the origin, little circles will be drawn at some point of the
  plot.

  By default, a mark is drawn at all points of the plot. However, two
  parameters $r$ and $p$ influence this. First, only every $r$th mark
  is drawn. Second, the first mark drawn is the $p$th. These
  parameters can be influenced using the commands below.
  
\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlermark{\pgfpathcircle{\pgfpointorigin}{4pt}\pgfusepath{stroke}}
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}

  Typically, the \meta{code} will be |\pgfuseplotmark{|\meta{plot mark
      name}|}|, where \meta{plot mark name} is the name of a
  predefined plot mark.
\end{command}

\begin{command}{\pgfsetplotmarkrepeat\marg{repeat}}
  Sets the $r$ parameter to \meta{repeat}, that is, only every $r$th
  mark will be drawn.
\end{command}

\begin{command}{\pgfsetplotmarkphase\marg{phase}}
  Sets the $p$ parameter to \meta{phase}, that is, the first mark to
  be drawn is the $p$th, followed by the $(p+r)$th, then the
  $(p+2r)$th, and so on.
\end{command}

\begin{command}{\pgfplothandlermarklisted\marg{mark code}\marg{index list}}
  This command works similar to the previous one. However, marks will
  only be placed at those indices in the given \meta{index list}. The
  syntax for the list is the same as for the |\foreach| statement. For
  example, if you provide the list |1,3,...,25|, a mark will be placed
  only at every second point. Similarly, |1,2,4,8,16,32| yields marks
  only at those points that are powers of two.
  
\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlermarklisted
    {\pgfpathcircle{\pgfpointorigin}{4pt}\pgfusepath{stroke}}
    {1,3}
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfuseplotmark\marg{plot mark name}}
  Draws the given \meta{plot mark name} at the origin. The \meta{plot
    mark name} must previously have been declared using
  |\pgfdeclareplotmark|. 

\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlermark{\pgfuseplotmark{pentagon}}
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfdeclareplotmark\marg{plot mark name}\marg{code}}
  Declares a plot mark for later used with the |\pgfuseplotmark|
  command.

\begin{codeexample}[]
\pgfdeclareplotmark{my plot mark}
  {\pgfpathcircle{\pgfpoint{0cm}{1ex}}{1ex}\pgfusepathqstroke}  
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfplothandlermark{\pgfuseplotmark{my plot mark}}
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgfsetplotmarksize\marg{dimension}}
  This command sets the \TeX\ dimension |\pgfplotmarksize| to
  \meta{dimension}. This dimension is a ``recommendation'' for plot
  mark code at which size the plot mark should be drawn; plot mark
  code may choose to ignore this \meta{dimension} altogether. For
  circles, \meta{dimension} should  be the radius, for other shapes it
  should be about half the width/height.

  The predefined plot marks all take this dimension into account.

\begin{codeexample}[]
\begin{tikzpicture}    
  \draw[gray] (0,0) node {x} (1,1) node {y} (2,.5) node {z};
  \pgfsetplotmarksize{1ex}
  \pgfplothandlermark{\pgfuseplotmark{*}}
  \pgfplotstreamstart
  \pgfplotstreampoint{\pgfpoint{0cm}{0cm}}
  \pgfplotstreampoint{\pgfpoint{1cm}{1cm}}
  \pgfplotstreampoint{\pgfpoint{2cm}{0.5cm}}
  \pgfplotstreamend
  \pgfusepath{stroke}
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{textoken}{\pgfplotmarksize}
  A \TeX\ dimension that is a ``recommendation'' for the size of plot
  marks.
\end{textoken}

The following plot marks are predefined (the filling color has been
set to yellow):

\medskip
\begin{tabular}{lc}
  \plotmarkentry{*}
  \plotmarkentry{x}
  \plotmarkentry{+}
\end{tabular}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-plot-marks.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Plot Mark Library}

\begin{pgflibrary}{plotmarks}
  This library defines a number of plot marks.
\end{pgflibrary}

This library defines the following plot marks in
addition to |*|, |x|, and |+| (the filling color has been set to a
dark yellow):

{
\catcode`\|=12
\medskip
\begin{tabular}{lc}
  \plotmarkentry{-}
  \index{*vbar@\protect\texttt{\protect\myvbar} plot mark}%
  \index{Plot marks!*vbar@\protect\texttt{\protect\myvbar}}
  \texttt{\char`\\pgfuseplotmark\char`\{\declare{|}\char`\}} &
  \tikz\draw[color=black!25] plot[mark=|,mark options={fill=yellow,draw=black}]
  coordinates {(0,0) (.5,0.2) (1,0) (1.5,0.2)};\\
  \plotmarkentry{o}
  \plotmarkentry{asterisk}
  \plotmarkentry{star}
  \plotmarkentry{oplus}
  \plotmarkentry{oplus*}
  \plotmarkentry{otimes}
  \plotmarkentry{otimes*}
  \plotmarkentry{square}
  \plotmarkentry{square*}
  \plotmarkentry{triangle}
  \plotmarkentry{triangle*}
  \plotmarkentry{diamond}
  \plotmarkentry{diamond*}
  \plotmarkentry{pentagon}
  \plotmarkentry{pentagon*}
\end{tabular}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-shadows.tex <==
% Copyright 2007 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Shadow Library}
\label{section-libs-shadows}

\begin{pgflibrary}{shadows}
  This library defines styles that help adding a (partly) transparent
  shadow to a path or node.
\end{pgflibrary}


\subsection{Overview}

A \emph{shadow} is usually a black or gray area that is drawn behind a
path or a node, thereby adding visual depth to a picture. The shadows
library defines options that make it easy to add shadows to
paths. Internally, these options are based on using the |preaction|
option to use a path twice: Once for drawing the shadow (slightly
shifted) and once for actually using the path.

Note that you can only add shadows to \emph{paths}, not to whole
scopes.

In addition to the general |shadow| option, there exist special
options like |circular shadow|. These can only (sensibly) be used with
a special kind of path (for |circular shadow|, a circle) and, thus,
there are not as general. The advantage is, however, that they are
more visually pleasing since these shadows blend smoothly with the
background. Note that these special shadows use fadings, which few
printers will support.


\subsection{The General Shadow Option}

The shadows are internally created by using a single option called
|general shadow|. The different options like |drop shadow| or
|copy shadow| only differ in the commands that they preset.

You will not need to use this option directly under normal
circumstances.


\begin{key}{/tikz/general shadow=\meta{shadow options} (default \normalfont empty)}
  This option should be given to a |\path| or a |node|. It has the
  following effect: Before the path is used normally, it is used once
  with the \meta{shadow options} in force. Furthermore, when the path
  is ``preused'' in this way, it is shifted and scaled a little bit.

  In detail, the following happens: A |preaction| is used to
  paint the path in a special manner before it is actually
  painted. This ``special'' manner is as follows: The options in
  \meta{shadow options} are used for painting this path. Typically,
  the \meta{shadow options} will contain options like |fill=black| to
  create, say, a black shadow. Furthermore, after the \meta{shadow
    options} have been setup, the following extra canvas
  transformations are applied to the path: It is scaled by
  |shadow scale| (with the origin of scaling at the path's center) and
  it is shifted by |shadow xshift| and |shadow yshift|. 

  Note that since scaling and shifting is done using canvas
  transformations, shadows are not taken into account when the
  picture's bounding box is computed.
\begin{codeexample}[]
\tikz [even odd rule]
  \draw [general shadow={fill=red}] (0,0) circle (.5) (0.5,0) circle (.5);  
\end{codeexample}
  
  \begin{key}{/tikz/shadow scale=\meta{factor} (initially 1)}
    Shadows are scaled by this amount.
\begin{codeexample}[]
\tikz [even odd rule]
  \draw [general shadow={fill=red,shadow scale=1.25}]
    (0,0) circle (.5) (0.5,0) circle (.5);  
\end{codeexample}
  \end{key}
  \begin{key}{/tikz/shadow xshift=\meta{factor} (initially 0pt)}
    Shadows are shifted horizontally by this amount.
\begin{codeexample}[]
\tikz [even odd rule]
  \draw [general shadow={fill=red,shadow xshift=-5pt}]
    (0,0) circle (.5) (0.5,0) circle (.5);  
\end{codeexample}
  \end{key}
  \begin{key}{/tikz/shadow yshift=\meta{factor} (initially 0pt)}
    Shadows are shifted vertically by this amount.
  \end{key}
\end{key}



\subsection{Shadows for Arbitrary Paths and Shapes}

\subsubsection{Drop Shadows}

\begin{key}{/tikz/drop shadow=\meta{shadow options} (default \normalfont empty)}
  This option adds a drop shadow to a path or node. |\path| or a
  |node|. It uses the |general shadow| and passes the \meta{shadow
    options} to it plus, before them, the following extra options:
\begin{codeexample}[code only]
  shadow scale=1, shadow xshift=.5ex, shadow yshift=-.5ex,
  opacity=.5, fill=black!50, every shadow
\end{codeexample}

\begin{codeexample}[]
\tikz [even odd rule]
  \filldraw [drop shadow,fill=white] (0,0) circle (.5) (0.5,0) circle (.5);  
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \i in {1,...,4}
    \node[starburst,drop shadow,fill=white,draw] at (0,\i) {Burst \i};
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);
  \filldraw [drop shadow={opacity=0.25},fill=white]
    (1,.5) circle (.5) (1.5,.5) circle (.5);  

  \filldraw [drop shadow={opacity=1},fill=white]
    (1,2)  circle (.5) (1.5,2)  circle (.5);  
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{stylekey}{/tikz/every shadow (initially \normalfont empty)}
  This style is executed in addition to any \meta{shadow options} for
  each shadow. Use this style to reconfigure the way shadows are
  drawn.
\begin{codeexample}[]
\begin{tikzpicture}[every shadow/.style={opacity=.8,fill=blue!50!black}]    
  \filldraw [drop shadow,fill=white] (0,0) circle (.5) (0.5,0) circle (.5);  
\end{tikzpicture}
\end{codeexample}
\end{stylekey}



\subsubsection{Copy Shadows}

A \emph{copy shadow} is not really a shadow. Rather, it looks like
another copy of the path drawn behind the path and a little bit
offset. This creates the visual impression of having multiple copies
of the path/object present.

\begin{key}{/tikz/copy shadow=\meta{shadow options} (default \normalfont empty)}
  This shadow installs the following default options:
\begin{codeexample}[code only]
  shadow scale=1, shadow xshift=.5ex, shadow yshift=-.5ex, every shadow
\end{codeexample}
  Furthermore, the options |fill=|\meta{fill color} and
  |draw=|\meta{draw color} are also set, where the \meta{fill color}
  and \meta{draw color} are the fill and draw colors used for the main 
  path. 
\begin{codeexample}[]
\begin{tikzpicture}
  \node [copy shadow,fill=blue!20,draw=blue,thick] {Hello World!};

  \node at (0,-1) [copy shadow={shadow xshift=1ex,shadow yshift=1ex},
                   fill=blue!20,draw=blue,thick]
    {Hello World!};

  \node at (0,-2) [copy shadow={opacity=.5},tape,
                   fill=blue!20,draw=blue,thick]
    {Hello World!};

  % We have to repeat the left color since shadings are not
  % automatically applied to shadows
  \node at (0,-3) [copy shadow={left color=blue!50},
                   left color=blue!50,draw=blue,thick]
    {Hello World!};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/double copy shadow=\meta{shadow options} (default \normalfont empty)}
  This shadow works like a |copy shadow|, only the shadow is added
  twice, the first time with the double |xshift| and |yshift|.
\begin{codeexample}[]
\begin{tikzpicture}
  \node [double copy shadow,fill=blue!20,draw=blue,thick] {Hello World!};

  \node at (0,-1) [double copy shadow={shadow xshift=1ex,shadow yshift=1ex},
                   fill=blue!20,draw=blue,thick]
    {Hello World!};

  \node at (0,-2) [double copy shadow={opacity=.5},tape,
                   fill=blue!20,draw=blue,thick]
    {Hello World!};

  \node at (0,-3) [double copy shadow={left color=blue!50},
                   left color=blue!50,draw=blue,thick]
    {Hello World!};
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsection{Shadows for Special Paths and Nodes}

The shadows in this section should normally be added only to paths
that have a special shape. They will look strange with other shapes.

\begin{key}{/tikz/circular drop shadow=\meta{shadow options}}
  This shadow works like a drop shadow, only it adds a circular
  fading to the shadow. This means that the shadow will fade out at
  the border. The following options are preset for this shadow:
\begin{codeexample}[code only]
  shadow scale=1.1, shadow xshift=.3ex, shadow yshift=-.3ex,
  fill=black, path fading={circle with fuzzy edge 15 percent},
  every shadow,
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \i in {1,...,8}
    \node[circle,circular drop shadow,draw=blue,fill=blue!20,thick]
      at (\i*45:1) {Circle \i};
\end{tikzpicture}
\end{codeexample}
\end{key}


\begin{key}{/tikz/circular glow=\meta{shadow options}}
  This shadow works much like the |circular shadow|, only it is not
  shifted. This creates a visual effect of a ``glow'' behind the
  circle.  The following options are preset for this shadow:
\begin{codeexample}[code only]
  shadow scale=1.25, shadow xshift=0pt, shadow yshift=0pt,
  fill=black, path fading={circle with fuzzy edge 15 percent},
  every shadow,
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \i in {1,...,8}
  \node[circle,circular glow,fill=red!20,draw=red,thick]
    at (\i*45:1) {Circle \i};
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \i in {1,...,8}
  \node[circle,circular glow={fill=white},fill=red!20,draw=red,thick]
    at (\i*45:1) {Circle \i};
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \i in {1,...,8}
  \node[circle,circular glow={fill=green},fill=black,text=green!50!black]
    at (\i*45:1) {Circle \i};
\end{tikzpicture}
\end{codeexample}
  An especially interesting effect can be achieved by only using the
  glow and not filling the path:
\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \i in {1,...,8}
  \node[circle,circular glow={fill=red!\i0}]
    at (\i*45:1) {Circle \i};
\end{tikzpicture}
\end{codeexample}
\end{key}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-shapes.tex <==
% Copyright 2007 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Shape Library}
\label{section-libs-shapes}


\subsection{Overview}

In addition to the standard shapes |rectangle|, |circle| and
|coordinate|, there exist a number of additional shapes defined in
different shape libraries. Most of these shapes have been 
contributed by Mark Wibrow. In the present section, these shapes are
described. Note that the library |shapes| is provided for
compatibility only. Please include sublibraries like
|shapes.geometric| or |shapes.misc| directly.

The appearance of shapes is influenced by numerous parameters like
|minimum height| or |inner xsep|. These general parameters are documented in
Section~\ref{section-shape-common-options} 


\subsection{Predefined Shapes}
\label{section-predefined-shapes}

The three shapes |rectangle|, |circle|, and |coordiante| are always
defined and no library needs to be loaded for them. While the
|coordinate| shape defines only the |center| anchor, the other two
shapes define a standard set of anchors.

\begin{shape}{circle}
  This shape draws a tightly fitting circle around the text. The
  following figure shows the anchors this shape defines; the anchors
  |10| and |130| are example of border anchors. 
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=circle,shape example] {Circle\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {north west/above left, north/above, north east/above right, 
     west/left, center/above, east/right, 
     mid west/right, mid/above, mid east/left, 
     base west/left, base/below, base east/right, 
     south west/below left, south/below, south east/below right, 
     text/left, 10/right, 130/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}

\begin{shape}{rectangle}
  This shape, which is the standard, is a rectangle around the
  text. The inner   and outer separations (see
  Section~\ref{section-shape-seps}) influence the white space around
  the text. The following figure shows the anchors this
  shape defines; the anchors |10| and |130| are example of border anchors.
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=rectangle,shape example] {Rectangle\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {north west/above left, north/above, north east/above right, 
     west/left, center/above, east/right, 
     mid west/right, mid/above, mid east/left, 
     base west/left, base/below, base east/right, 
     south west/below left, south/below, south east/below right, 
     text/left, 10/right, 130/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}



\subsection{Geometric Shapes}

\begin{pgflibrary}{shapes.geometric}
  This library defines different shapes that correspond to basic
  geometric objects like ellipses or polygons.
\end{pgflibrary}


\begin{shape}{diamond}
  This shape is a diamond tightly fitting the text box. The ratio
  between width and height is 1 by default, but can be changed by
  setting the shape aspect ratio using the following \pgfname{}
  key (to use this key in \tikzname{} simply remove the 
  \declare{|/pgf/|} path). 

  \begin{key}{/pgf/aspect=\meta{value} (initially 1.0)}
    The aspect is a recommendation for the quotient of the width and 
    the height of a shape. This key calls the macro
    |\pgfsetshapeaspect|.
  \end{key}
  
  The following figure shows the anchors this
  shape defines; the anchors |10| and |130| are example of border
  anchors.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=diamond,shape example] {Diamond\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {north west/above left, north/above, north east/above right, 
     west/left, center/above, east/right, 
     mid/above, 
     base/below,  
     south west/below left, south/below, south east/below right, 
     text/left, 10/right, 130/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}

\begin{shape}{ellipse}
  This shape is an ellipse tightly fitting the text box, if no inner
  separation is given. The following figure shows the anchors this
  shape defines; the anchors |10| and |130| are example of border anchors.
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=ellipse,shape example] {Ellipse\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {north west/above left, north/above, north east/above right, 
     west/left, center/above, east/right, 
     mid west/right, mid/above, mid east/left, 
     base west/left, base/below, base east/right, 
     south west/below left, south/below, south east/below right, 
     text/left, 10/right, 130/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}





\begin{shape}{trapezium}
  This shape is a trapezium, that is, a quadrilateral with a single
  pair of parallel lines (this can sometimes be known as a trapezoid).
  The trapezium shape supports the rotation of the shape border, as 
  described in Section~\ref{section-rotating-shape-borders}. 
  
  The lower internal angles at the lower corners of the trapezium can 
  be specified independently, and the resulting extensions are in 
  addition to the natural dimensions of the node contents (which
  includes any |inner sep|.
	
\begin{codeexample}[]
\begin{tikzpicture}
   \tikzstyle{every node}=[trapezium, draw]
   \node at (0,2) {A};
   \node[trapezium left angle=75, trapezium right angle=45pt]
         at (0,1) {B};
   \node[trapezium left angle=120, trapezium right angle=60pt]
         at (0,0) {C};
\end{tikzpicture}
\end{codeexample}

         
  The \pgfname{} keys to set the lower internal angles of the trapezium 
  are shown below. 
  To use these keys in \tikzname, simply remove the \declare{|/pgf/|} path.
	
  \begin{key}{/pgf/trapezium left angle=\meta{angle} (initially 60)}
    Set the lower internal angle of the left side. 
  \end{key}
   
  \begin{key}{/pgf/trapezium right angle=\meta{angle} (initially 60)}
    Set the lower internal angle of the right side. 
  \end{key}
  
  \begin{stylekey}{/pgf/trapezium angle=\meta{angle}}
    This key stores no value itself, but sets the value of the
    previous two keys to \meta{angle}. 
  \end{stylekey}
     
  Regardless of the rotation of the shape border, the width
  and height of the trapezium are as follows:

\begin{codeexample}[]
\begin{tikzpicture}[>=stealth, every node/.style={text=black}, 
    shape border uses incircle, shape border rotate=60]
  \node [trapezium, fill=gray!25, minimum width=2cm] (t) {};
  \draw [red, <->] (t.bottom left corner) -- (t.bottom right corner) 
    node [midway, below right] {width};
  \draw [red, <->] (t.top side) -- (t.bottom side) 
    node [at start, above] {height};
\end{tikzpicture}
\end{codeexample}

  \begin{key}{/pgf/trapezium stretches=\meta{boolean} (default true)}
    This key controls whether \pgfname{} allows the width and the height
    of the trapezium to be enlarged independently, 
    when considering any minimum size specification. This is initially 
    |false|,  ensuring that the shape ``looks the same but bigger'' when 
    enlarged.
  
\begin{codeexample}[]
\tikzset{my node/.style={trapezium, fill=#1!20, draw=#1!75, text=black}}
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \node [my node=red]                                      {A};
  \node [my node=green, minimum height=1.5cm] at (1, 1.25) {B};
  \node [my node=blue,  minimum width=1.5cm]  at (2, 0)    {C};
\end{tikzpicture}
\end{codeexample} 

    By setting \meta{boolean} to |true|, the trapezium can be stretched
    horizontally or vertically.
  
\begin{codeexample}[]
\tikzset{my node/.style={trapezium, fill=#1!20, draw=#1!75, text=black}}
\begin{tikzpicture}
\tikzset{trapezium stretches=true}
  \draw [help lines] grid (3,2);
  \node [my node=red]                                      {A};
  \node [my node=green, minimum height=1.5cm] at (1, 1.25) {B};
  \node [my node=blue,  minimum width=1.5cm]  at (2, 0)    {C};
\end{tikzpicture}
\end{codeexample}
\end{key}

  \begin{key}{/pgf/trapezium stretches body=\meta{boolean} (default true)}
    This is similar to the |trapezium stretches| key execept that
    when \meta{boolean} is |true|, \pgfname{} enlarges only the body 
    of the trapezium when applying minimum width.
  
\begin{codeexample}[]
\tikzset{my node/.style={trapezium, fill=#1!20, draw=#1!75, text=black}}
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \node [my node=red]                      at (1.5,.25)  {A};
  \node [my node=green, minimum width=3cm, trapezium stretches] 
    at (1.5,1)    {B};
  \node [my node=blue,  minimum width=3cm, trapezium stretches body] 
    at (1.5,1.75) {C};
\end{tikzpicture}
\end{codeexample}
  \end{key}

  The anchors for the trapezium are shown below. The anchor |160| is an
  example of a border anchor.

\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=trapezium, shape example, inner sep=1cm] 
    {Trapezium\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {bottom left corner/below, top right corner/right, 
     top left corner/left,     bottom right corner/below,
     bottom side/below,        left side/left, 
     right side/right,         top side/above,
     center/above,   text/below,      mid/right,       base/below, 
     mid west/right, base west/below, mid east/left,   base east/below, 
     west/above,     east/above,      north/below,     south/above,
     north west/above, north east/above, 
     south west/below, south east/below, 160/above}    
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}  
\end{shape}


\begin{shape}{semicircle}
  This shape is a semicircle, which tightly fits the node contents.
  This shape supports the rotation of the shape border, as described in 
  Section~\ref{section-rotating-shape-borders}.
  The anchors for the |semicircle| shape are shown below. 
  Anchor |30| is an example of a border anchor.
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=semicircle,shape border rotate=0,shape example, inner sep=1cm] 
  	{Semicircle\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {apex/above,      arc start/below, arc end/below,  chord center/below,
     center/above,    base/below,      mid/right,      text/left,
     base west/below, base east/below, mid west/left, mid east/right, 
     north/below,     south/above,     east/above,     west/above,
     north west/above left, north east/above right,
     south west/below,      south east/below, 30/right}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}





\begin{shape}{regular polygon}
  This shape is a regular polygon, which, by default, is drawn so that 
  a side (rather than a corner) is always at the bottom. 
  This shape supports the rotation as described in 
  Section~\ref{section-rotating-shape-borders}, but the border of the 
  polygon is \emph{always} constructed using the incircle, whose
  radius is calculated to tightly fit the node contents (including
  any |inner sep|).
  
\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \a in {3,...,7}{
    \draw[red, dashed] (\a*2,0)  circle(0.5cm);
    \node[regular polygon, regular polygon sides=\a, draw,
     inner sep=0.3535cm] at (\a*2,0) {};
   }  
\end{tikzpicture}
\end{codeexample}	
	
  If the node is enlarged to any specified minimum size, 
  this is interpreted as the diameter of the the 
  circumcircle, that is, the circle that passes through all the 
  corners of the polygon border.

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \a in {3,...,7}{
    \draw[blue, dashed] (\a*2,0)  circle(0.5cm);
    \node[regular polygon, regular polygon sides=\a, minimum size=1cm, draw] at (\a*2,0) {};
   }  
\end{tikzpicture}
\end{codeexample}	

  There is a \pgfname{} key to set the number of sides for the regular
  polygon.
  To use this key in \tikzname, simply remove the \declare{|/pgf/|} path.
	
  \begin{key}{/pgf/regular polygon sides=\meta{integer} (initially 5)}
  \end{key}
  
  The anchors for a regular polygon shape are shown below.  
  The anchor |75| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=regular polygon, shape example, inner sep=.5cm] 
    {Regular Polygon\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {corner 1/above, corner 2/above, corner 3/left, corner 4/right, corner 5/above, 
     side 1/above,   side 2/left,    side 3/below,  side 4/right,   side 5/above,  
     center/above, text/left,  mid/right,   base/below, 75/above,
     west/above,   east/above, north/below, south/above,
     north east/below, south east/above, north west/below, south west/above}
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}

\begin{shape}{star}
  This shape is a star, which by default (minus any transformations) is
  drawn with the first point pointing upwards.  
  This shape supports the rotation as described in 
  Section~\ref{section-rotating-shape-borders}, but the border of the 
  star is \emph{always} constructed using the incircle.
  
  A star should be thought of as having an set of ``inner points'' and
  and ``outer points''. 
  The inner points of the border are based on the radius of the circle
  which tightly fits the node contents, and the outer points are based
  on the circumcircle, the circle that passes through every outer
  point.
  Any specified minimum size, width or height, is interpreted as the 
  diameter of the circumcircle.
 
\begin{codeexample}[]
\begin{tikzpicture}
   \draw [help lines]   (0,0) grid (2,2);
   \draw [blue, dashed]  (1,1) circle(1cm);
   \draw [red, dashed] (1,1) circle(.5cm);
   \node [star, star point height=.5cm, minimum size=2cm, draw] 
       at (1,1) {S};
\end{tikzpicture}
\end{codeexample} 
  
  The \pgfname{} keys to set the number of star points, and the height
  of the star points, are shown below. To use these keys in \tikzname,
  simply remove the \declare{|/pgf/|} path.
  
  \begin{key}{/pgf/star points=\meta{integer} (initially 5)}
    Sets the number of points for the star.
  \end{key}
  
  \begin{key}{/pgf/star point height=\meta{distance} (initially .5cm)}
    Sets the height of the star points. This is the distance between the
    inner point and outer point radii. If the star is enlarged to some
    specified minimum size, the inner radius is increased to maintain
    the point height.	
  \end{key}
  
  \begin{key}{/pgf/star point ratio=\meta{number} (initially 1.5)}
    Sets the ratio between the inner point and outer point radii.		
    If the star is enlarged to some specified minimum size, the
    inner radius is increased to maintain the ratio.	
  \end{key}

	The inner and outer points form the principle anchors for the star,
   as shown below (anchor |75| is an example of a border anchor).
  
  \begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=star, star points=5, star point ratio=1.65, shape example, inner sep=1.5cm] 
    {Star\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
     {inner point 1/above, inner point 2/above, inner point 3/below, inner point 4/right, 
      inner point 5/above, outer point 1/above, outer point 2/above, outer point 3/left,  
      outer point 4/right, outer point 5/above,
      center/above, text/left,  mid/right,   base/below, 75/above,
     	west/above,   east/above, north/below, south/above,
     	north east/below, south east/above, north west/below, south west/above}
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}





\begin{shape}{isosceles triangle}
  This shape is an isosceles triangle, which supports the rotation of 
  the shape border, as described in 
  Section~\ref{section-rotating-shape-borders}. The angle of rotation
  determines the direction in which the apex of the triangle points
  (provided no other transformations are applied). However, regardless
  of the rotation of the shape border, the width and height are 
  always considered as follows:
	
\begin{codeexample}[]
\begin{tikzpicture}[>=stealth, every node/.style={text=black},
    shape border uses incircle, shape border rotate=-30]
  \node [isosceles triangle, fill=gray!25, minimum width=1.5cm] (t) {};
  \draw [red, <->] (t.left corner) -- (t.right corner)
    node [midway, above left] {width};
  \draw [red, <->] (t.apex) -- (t.lower side)
    node [midway, above right] {height};
\end{tikzpicture}
\end{codeexample}

	There are \pgfname{} keys to customise this shape. 
	To use these keys in \tikzname, simply remove the \declare{|/pgf/|} 
	path.
    
  \begin{key}{/pgf/isosceles triangle apex angle=\meta{angle} (initially 45)}
    Sets the angle of the apex of the isosceles triangle. 
  \end{key}

\begin{key}{/pgf/isosceles triangle stretches=\meta{boolean} (default true)}
  
	By default \meta{boolean} is |false|. This means, that when applying
	any minimum width or minimum height requirements, increasing the 
	height will increase the width (and	vice versa), in order to keep the
	apex angle the same.
   
\begin{codeexample}[]
\begin{tikzpicture}[paint/.style={draw=#1!75, fill=#1!20}]
  \tikzset{every node/.style={isosceles triangle, draw, inner sep=0pt, 
    anchor=left corner, shape border rotate=90}}
  \draw[help lines] grid(4,2);
  \foreach \a/\c in {1.5/blue, 1/green, 0.5/red}{
    \node[paint=\c, minimum height=\a cm] at (0,0) {};
    \node[paint=\c, minimum width=\a cm] at (2,0) {};
  }
\end{tikzpicture}
\end{codeexample}	

	However, by setting \meta{boolean} to |true|, minimum width and 
	height can be applied	independently.
	
\begin{codeexample}[]
\begin{tikzpicture}[paint/.style={draw=#1!75, fill=#1!20}]
  \tikzset{every node/.style={isosceles triangle, draw, inner sep=0pt, 
     anchor=south, shape border rotate=90, isosceles triangle stretches}}
  \draw[help lines] grid(4,2);
  \foreach \a/\c in {1.5/blue, 1/green, 0.5/red}{
    \node[paint=\c, minimum height=\a cm, minimum width=1.5cm] at (0.75,0) {};
    \node[paint=\c, minimum width=\a cm, minimum height=1.5cm] at (3,0)    {};
  }
\end{tikzpicture}
\end{codeexample}	
\end{key}
	
   The anchors for the |isosceles triangle| are shown below 
   (anchor |150| is an	example of a border anchor). Note that,
   somewhat confusingly, the anchor names such as |left side| and
   |right corner| are named as if the triangle is rotated to 
   90 degrees. Note also that the |center| anchor
   does not	necessarily correspond to any kind of geometric center.
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=isosceles triangle, shape example, inner xsep=1cm]
    {Isosceles Triangle\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {apex/above,      left corner/right, right corner/right,
     left side/above, right side/below,  lower side/right,    
     center/above,    text/right,        150/above,
     mid/right,       mid west/above,    mid east/right,
     base/below,      base west/below,   base east/below,
     west/above, east/below, north/below, south/above,
     north west/below, north east/below, 
     south west/above, south east/above}  
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample} 
\end{shape}






\par\leavevmode
\begin{shape}{kite}

	This shape is a kite, which supports the rotation of the shape border, 
	as described in Section~\ref{section-rotating-shape-borders}. 
	There are \pgfname{} keys to specify the upper and lower vertex angles
	of the kite. 
	To use these keys in \tikzname, simply remove the \declare{|/pgf/|} 
	path.
	
	\begin{key}{/pgf/kite upper vertex angle=\meta{angle} (initially 120)}
	Set the upper internal angle of the kite.
	\end{key}
	
	\begin{key}{/pgf/kite lower vertex angle=\meta{angle} (initially 60)}
	Set the lower internal angle of the kite.
	\end{key}
	
	\begin{key}{/pgf/kite vertex angles=\meta{angle specification}}
		This key sets the keys for both the upper and lower vertex angles
		(it stores no value itself).
	   \meta{angle specification} can be pair of angles in the form
	   \meta{upper angle} |and| \meta{lower angle}, or a single angle.
	   In this latter case, both the upper and lower vertex angles will 
	   be the same.
	\end{key}%
    
\begin{codeexample}[]
\begin{tikzpicture}
  \tikzstyle{every node}=[kite, draw]
  \node[kite upper vertex angle=135, kite lower vertex angle=70] at (0,0) {A};
  \node[kite vertex angles=90 and 45] at (1,0) {B};
  \node[kite vertex angles=60]        at (2,0) {C};
\end{tikzpicture}
\end{codeexample}


	The anchors for the |kite| are shown below. Anchor |110| is an 
	example of a border anchor.
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=kite, shape example, inner sep=1.5cm] 
    {Kite\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {upper vertex/above, left vertex/above,    lower vertex/below, 
     right vertex/above, upper left side/above, upper right side/above,
     lower left side/below, lower right side/below,
     center/above,   text/left,       mid/right,        base/below, 
     mid west/left,  base west/below, mid east/right,   base east/below,
     west/above,     east/above,      north/below,     south/above,
     north west/left, north east/right, 
     south west/above, south east/above, 110/above}  
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}


\begin{shape}{dart}


	This shape is a dart (which can also be known as an arrowhead or
	concave kite). This shape supports the rotation of the shape border, 
	as described in Section~\ref{section-rotating-shape-borders}. 
	The angle of the border rotation determines the direction in which 
	the dart points (unless other transformations have been applied).
	
	There are \pgfname{} keys to set the 
	angle for the `tip' of the dart and the angle between the `tails'
	of the dart. 
	To use these keys in \tikzname, simply remove the \declare{|/pgf/|} 
	path.

\begin{codeexample}[]
\begin{tikzpicture}
   \node[dart, draw, gray, shape border uses incircle, shape border rotate=45] 
       (d) {dart};
   \draw [<->] (d.tip)++(202.5:.5cm) arc(202.5:247.5:.5cm);
   \node [left=.5cm] at (d.tip) {tip angle};
   \draw [<->] (d.tail center)++(157.5:.5cm) arc(157.5:292.5:.5cm);
   \node [right] at (d.tail center) {tail angle};
\end{tikzpicture}
\end{codeexample}

	\begin{key}{/pgf/dart tip angle=\meta{angle} (initially 45)}
		Set the angle at the tip of the dart.
	\end{key}
	
	\begin{key}{/pgf/dart tail angle=\meta{angle} (initially 135)}
		Set the angle between the tails of the dart.
	\end{key}
		
	The anchors for the |dart| shape are shown below (note that the 
	shape is rotated 90 degrees anti-clockwise). Anchor |110| is an 
	example of a border anchor.
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=dart, shape border rotate=90, shape example, inner sep=1.25cm] 
    {Dart\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {tip/above,       tail center/below, right tail/below, 
     left tail/below, right tail/below,  left side/left,   right side/right,
     center/above,    text/left,         mid/right,        base/below, 
     mid west/left,   base west/below,   mid east/right,   base east/below,
     west/above,      east/above,        north/below,      south/above,
     north west/left, north east/right,  south west/above, south east/above,
     110/above}    
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}




\begin{shape}{circular sector}

	This shape is a circular sector (which can also be known as a
	wedge).
	This shape supports the rotation of the shape border, 
	as described in Section~\ref{section-rotating-shape-borders}. 
	The angle of the border rotation determines the direction in which 
	the `apex' of the sector points (unless other transformations have 
	been applied).
	
\begin{codeexample}[]
\begin{tikzpicture}
	\tikzstyle{every node}=[circular sector, shape border uses incircle, draw];
   \node at (0,0) {A};
   \node [shape border rotate=30] at (1.5,0) {A};
\end{tikzpicture}
\end{codeexample}

	There is a \pgfname{} key to set the central angle of the sector, 
	which is expected to be less than 180 degrees. 
	To use this key in \tikzname,	simply remove the \declare{|/pgf/|} 
	path.
	
	\begin{key}{/pgf/circular sector angle=\meta{angle} (initially 60)}
		Set the central angle of the sector. 
	\end{key}
	
	The anchors for the circular sector shape are shown below.
	Anchor |30| is an example of a border anchor.
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=circular sector,  style=shape example, inner sep=1cm] 
  	{Circular Sector\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
   {sector center/above, arc start/below, arc end/below, arc center/below,
    center/above,        base/below,      mid/right,     text/below,
    north/below,         south/above,     east/below,    west/above,
    north west/above left, north east/above right,
    south west/below,      south east/below, 30/right}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}




\begin{shape}{cylinder}
	This shape is a 2-dimensional representation of a cylinder, which 
	supports the rotation of the shape border as described in
	Section~\ref{section-rotating-shape-borders}.

\begin{codeexample}[]
\begin{tikzpicture}
  \node[cylinder, draw, shape aspect=.5] {ABC};
\end{tikzpicture}
\end{codeexample}
		
	Regardless the rotation of the shape border, the height is always the
	distance between the curved ends, and the width is always the	
	distance between the straight sides. 

\begin{codeexample}[]
\begin{tikzpicture}[>=stealth]
  \node [cylinder, gray!50, rotate=30, draw, 
    minimum height=2cm, minimum width=1cm] (c) {Cylinder};
  \draw[red, <->] (c.top)   -- (c.bottom) 
    node [at end, below, black]   {height};
  \draw[red, <->] (c.north) -- (c.south) 
    node [at start, above, black] {width};
\end{tikzpicture}
\end{codeexample}

	Enlarging the shape to some minimum height will stretch only the body
	of the cylinder. By contrast, enlarging the shape to some minimum 
	width will stretch the curved ends.
	
\begin{codeexample}[]
\begin{tikzpicture}[>=stealth, shape aspect=.5]
  \tikzset{every node/.style={cylinder, shape border rotate=90, draw}}
  \node [minimum height=1.5cm]            {A};  
  \node [minimum width=1.5cm]  at (1.5,0) {B};  
\end{tikzpicture}
\end{codeexample}

  There are various keys to customize this shape (to use \pgfname{}
  keys in \tikzname{}, simply remove the \declare{|/pgf/|} path).
  
\begin{key}{/pgf/aspect=\meta{value} (initially 1.0)}
  The aspect is a recommendation for the quotient of the radii of
  the cylinder end. This may be ignored if the shape is enlarged
  to some minimum width.

\begin{codeexample}[]
\begin{tikzpicture}[>=stealth]
  \tikzset{every node/.style={cylinder, shape border rotate=90, draw}}
  \node [aspect=1.0]           {A};  
  \node [aspect=0.5]  at (1,0) {B};  
  \node [aspect=0.25] at (2,0) {C};  
\end{tikzpicture}
\end{codeexample}

\end{key}

\begin{key}{/pgf/cylinder uses custom fill=\meta{boolean} (default true)}
	This enables the use of a custom fill for the body and the end of 
	the cylinder. The background path for the shape should not be 
	filled (e.g., in \tikzname{}, the |fill| option for the node must 
	be implicity or explicitly set to |none|).
  Internally, this key sets the \TeX-if 
  |\ifpgfcylinderusescustomfill| appropriately.
\end{key}

\begin{codeexample}[]
\begin{tikzpicture}[>=stealth, aspect=0.5]
  \node [cylinder, cylinder uses custom fill, cylinder end fill=red!50,
         cylinder body fill=red!25] {Cylinder};  
\end{tikzpicture}
\end{codeexample}

\begin{key}{/pgf/cylinder end fill=\meta{color} (initially white)}
	Set the color for the end of the cylinder.
\end{key}
\begin{key}{/pgf/cylinder body fill=\meta{color} (initially white)}
	Set the color for the body of the cylinder.
\end{key}


  The anchors this shape are shown below (anchor |160| is an
	example of a border anchor). Note the the cylinder shape does not 
	distinguish between |outer xsep| and |outer ysep|. Only the larger 
	of the two values is used for the shape. Note also the difference 
	between the |center| and |shape center| anchors: |center| is the
	center of the cylinder body and also the center of rotation. 
	The |shape center| is the center of the shape which includes the 
	2-dimensional representation of the cylinder top.	
	 

\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=cylinder, shape example, aspect=.5, inner xsep=3cm,
        inner ysep=1cm] {Cylinder\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {before top/above,    top/above,       after top/below,
     before bottom/below, bottom/above,    after bottom/above,
     mid/right,           mid west/right,  mid east/left,  
     base/below,          base west/below, base east/below,
     center/above,        text/above,      shape center/right, 
     west/right, east/left, north/above, south/below,
     north west/below, north east/above, 
     south west/above, south east/below, 160/above}    
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}  


\end{shape}






\subsection{Symbol Shapes}

\begin{pgflibrary}{shapes.symbols}
  This library defines shapes that can be used for drawing symbols
  like a forbidden sign or a cloud.
\end{pgflibrary}



\begin{shape}{forbidden sign}
  This shape places the node inside a circle with a diagonal from the
  lower left to the upper right added. The circle is part of the
  background, the diagonal line part of the foreground path; thus, the
  diagonal line is on top of the text.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \node [forbidden sign,line width=1ex,draw=red,fill=white] {Smoking};
\end{tikzpicture}
\end{codeexample}

  The shape inherits all anchors from the |circle| shape, see also the
  following figure:
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=forbidden sign,shape example] {Forbidden\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {north west/above left, north/above, north east/above right, 
     west/left, center/above, east/right, 
     mid west/right, mid/above, mid east/left, 
     base west/left, base/below, base east/right, 
     south west/below left, south/below, south east/below right, 
     text/left, 10/right, 130/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}


\begin{shape}{cloud}

	This shape is a cloud, drawn to tightly fit the node contents 
	(strictly speaking, using an ellipse which tightly fits the node
	contents -- including any |inner sep|). 
	
\begin{codeexample}[]
\begin{tikzpicture}
  \node[cloud, draw, fill=gray!20, aspect=2] {ABC};
  \node[cloud, draw, fill=gray!20] at (1.5,0) {D};
\end{tikzpicture}
\end{codeexample}

	A cloud should be thought of as having a number of ``puffs'', which
	are the individual arcs drawn around the border. There are \pgfname{}
	keys to specify how the cloud is drawn (to use these keys in 
	\tikzname{}, simply remove the \declare{|/pgf/|} path).
	
	\begin{key}{/pgf/cloud puffs=\meta{integer} (initially 10)}
	  Set the number of puffs for the cloud.
	\end{key}
	
	\begin{key}{/pgf/cloud puff arc=\meta{angle} (initially 135)}
	  Set the length of the puff arc (in degrees). A shorter arc can 
	  produce better looking joins between puffs for larger line widths.
	\end{key}
	
	Like the diamond shape, the cloud shape also uses the 
	\declare{|aspect|} key, to determine the ratio of the width and the 
	height of the cloud. However there may be cirumstances where it may
	be undesirable to continually specify the |aspect| for the cloud.
	Therefore, the following key is implemented:
	
	\begin{key}{/pgf/cloud ignores aspect=\meta{boolean} (default true)}
		Instruct \pgfname{} to ignore the |aspect| key. Internally, the
		\TeX-if |\ifpgfcloudignoresaspect| is set appropriately. The initial
		value is |false|.

\begin{codeexample}[]
\begin{tikzpicture}[aspect=1, every node/.style={cloud, cloud puffs=11, draw}]
  \node [fill=gray!20]                                {rain};
  \node [cloud ignores aspect, fill=white] at (1.5,0) {snow};
\end{tikzpicture}
\end{codeexample}	
	
	\end{key}
	
	
	Any minimum size requirements are applied to the ``circum-ellipse'',
	which is the ellipse which passes through all the midpoints of the
	puff arcs. These requirements are considered \emph{after} any 
	aspect specification is applied.
	
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \draw [blue, dashed] (1.5, 1) ellipse (1.5cm and 1cm);
  \node [cloud, cloud puffs=9, draw, minimum width=3cm, minimum height=2cm] 
    at (1.5, 1) {};
\end{tikzpicture}
\end{codeexample}
	
  The anchors for the cloud shape are shown below for a cloud with
  eleven puffs. Anchor 70 is an example of a border anchor. 
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=cloud, style=shape example, cloud puffs=11, aspect=1.5,
       cloud puff arc=120,inner ysep=1cm] {Cloud\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
   {puff 1/above, puff 2/above,  puff 3/above,  puff 4/below, 
    puff 5/left,  puff 6/below,  puff 7/below,  puff 8/right,
    puff 9/below, puff 10/above, puff 11/above, 70/right,
    center/above, base/below,    mid/right,     text/left, 
    north/below,  south/below,   east/above,    west/above,
    north west/left,             north east/right, 
    south west/below,            south east/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape} 






\begin{shape}{starburst}

	This shape is a randomly generated eliptical star,
	which supports the rotating of the shape border as described in 
	Section~\ref{section-rotating-shape-borders}. 
\begin{codeexample}[]
\begin{tikzpicture}
  \node[starburst, fill=yellow, draw=red, line width=2pt] {\bf BANG!};
\end{tikzpicture}
\end{codeexample}	
	Like the |star| shape, the starburst should be thought of as having a set
	of inner points and outer points. The inner points lie on the ellipse
	which tightly fits the node contents (including any |inner sep|).
	
	Using a specified `starburst point height' value, the outer points
	are generated randomly between this value and one quarter of this 
	value. For a given starburst shape the angle between each point is 
	fixed, and is determined by the number of points specified for
	the starburst.
	
	It is important to note that, whilst the maximum possible point 
	height is used to calculate minimum width or height requirements, 
	the outer points are randomly generated, so there is (unfortunately) 
	no guarantee that any such requirements will be fully met. 
	
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] grid(3,2);
  \node[starburst, draw, minimum width=3cm, minimum height=2cm] 
    at (1.5, 1) {\bf BOOM!};
\end{tikzpicture}
\end{codeexample}

	There are \pgfname{} keys to control the drawing of the starburst
	shape. To use these keys in \tikzname,	simply remove the 
	\declare{|/pgf/|}	path.

	\begin{key}{/pgf/starburst points=\meta{integer} (initially 17)}
		Set the number of points for the starburst.
	\end{key}
	\begin{key}{/pgf/starburst point height=\meta{length} (initially .5cm)}
      Set the \emph{maximum} distance between the inner point radius  
      and the outer point radius.
	\end{key}
	
	\begin{key}{/pgf/random starburst=\meta{integer} (initially 100)}
      Set the seed for the random number generator for creating the
      starburst.  The maximum value for \meta{integer} is |16383|.
      If \meta{integer}|=0|, the random number generator will not be 
      used, and the maximum point height will be used for all outer 
      points. If \meta{integer} is omitted, a seed will be randomly
      chosen.
	\end{key}
	
	The basic anchors for a nine point |starburst| shape are shown below. 
	Anchor |80| is an example of a border anchor.
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=starburst, starburst points=9, starburst point height=3.5cm, 
        style=shape example,inner sep=1cm] 
    {Starburst\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {outer point 1/above, outer point 2/above, outer point 3/right,
     outer point 4/above, outer point 5/below, outer point 6/above,
     outer point 7/left,  outer point 8/above, outer point 9/above,
     inner point 1/below, inner point 2/above, inner point 3/left,
     inner point 4/above, inner point 5/above, inner point 6/above,
     inner point 7/below, inner point 8/above, inner point 9/below,
     center/above, text/left,   mid/right, base/below, 80/above,
     north/below,  south/below, east/left, west/right,
     north east/below, south west/below, south east/below, north west/below}
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}

\begin{shape}{signal}

	This shape is a ``signal'' or sign shape, that is, a rectangle, with
	optionally pointed sides. A signal can point ``to'' somewhere, with 
	outward points in that direction. It can also be ``from'' 
	somewhere, with inward points from that direction. The resulting 
	points extend the node contents (which include the |inner sep|).
	
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={signal, draw,  text=white}]
  \node[fill=green!65!black, signal to=east] at (0,1) {To East};
  \node[fill=red!65!black, signal from=east] at (0,0) {From East};
\end{tikzpicture}
\end{codeexample}

	There are \pgfname{} keys for drawing the signal shape (to use these
	keys in \tikzname{}, simply remove the \declare{|/pgf/|} path):
	
	\begin{key}{/pgf/signal pointer angle=\meta{angle} (initially 90)} 
		Set the angle for the pointed sides of the shape. This angle is
		maintained when enforcing any minimum size requirements, so
		any adjustment to the width will affect the height, and vice versa.
	\end{key}
	
	\begin{key}{/pgf/signal from=\meta{direction}\space\opt{and \meta{opposite direction}} (initially nowhere)} 
		Set which sides take an inward pointer (i.e., that points towards the
		center of the shape). The possible values for \meta{direction} and 
		\meta{opposide direction} are the compass point directions |north|,
		|south|, |east| and |west| (or |above|, |below|, |right| and |left|).
		An additional keyword |nowhere| can be used to reset the sides so 
		they have no pointers. When used with |signal from| key, this only 
		resets inward pointers;	used with the |signal to| key, it only 
		resets outward pointers. 
		
	\end{key}
	
	\begin{key}{/pgf/signal to=\meta{direction}\space\opt{and \meta{opposite direction}} (initially east)} 
		Set which sides take an outward pointer (i.e., that points away from 
		the	the shape). 
	\end{key}
	
	Note that \pgfname{} will ignore any instruction to use directions
	that are not opposites (so using the value |east and north|, will
	result in only |north| being assigned a pointer). This is also 
	the case if non-opposite values are used in the |signal to| and
	|signal from| keys at the same time. So, for example, it is not 
	possible for a signal to have an outward point to the left, and also
	have an inward point from below.
	
	The anchors for the signal shape are shown below. Anchor |70| is an
	example of a border anchor.

\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=signal, signal from=west, shape example, inner sep=2cm] 
    {Signal\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {text/left,   center/above,    70/above,
     base/below,  base east/below, base west/below,
     mid/right,   mid east/above left,  mid west/above left, 
     north/above,      south/below, 
     east/above,       west/above,        
     north west/above, north east/above, 
     south west/below, south east/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}





\begin{shape}{tape}
	This shape is a rectangle with optional, ``bendy'' top and bottom
	sides, which tightly fits the node contents (including the 
	|inner sep|).
	
\begin{codeexample}[]
\begin{tikzpicture}
  \node[tape, draw]{ABCD};
  \node[tape, draw, tape bend top=none] at (1.5, 0) {EFGH};
\end{tikzpicture}
\end{codeexample}

  There are \pgfname{} keys to specify which sides bend and how high
  the bends are (to use these keys in \tikzname{}, simply remove the
  \declare{|/pgf/|} path):
  
  \begin{key}{/pgf/tape bend top=\meta{bend style} (initially in and out)}
  	Specify how the top side bends. The \meta{bend style} is either
  	|in and out|, |out and in| or |none| (i.e., a straight line). 
  	The bending sides are drawn in a 
  	clockwise direction, and using the bend style |in and out| will mean 
  	the side will first	bend inwards and then bend outwards. 
  	The opposite holds true for	|out and in|. 
  	
\begin{codeexample}[]
\begin{tikzpicture}[-stealth]
  \node[tape, draw, gray, minimum width=2cm](t){Tape};
  \draw [blue]([yshift=5pt] t.north west) -- ([yshift=5pt]t.north east) 
         node[midway, above, black]{in and out};
  \draw [blue]([yshift=-5pt]t.south east) -- ([yshift=-5pt]t.south west) 
         node[sloped, allow upside down, midway, above, black]{in and out};
\end{tikzpicture}
\end{codeexample}  

    This might take a bit of getting used to, but just remember that 
    when you want the bendy sides to be parallel, the sides take the 
    same bend style. It is possible for the top and bottom sides to 
    take opposite bend styles, but the author of this shape cannot 
    think of a single use for such a combination.
    
\begin{codeexample}[]
\begin{tikzpicture}
  \tikzstyle{every node}=[tape, draw]
  \node [tape bend top=out and in, tape bend bottom=out and in] {Parallel};
  \node at (2,0) [tape bend bottom=out and in]                  {Why?};
\end{tikzpicture}
\end{codeexample} 

	\end{key}
	
	\begin{key}{/pgf/tape bend bottom=\meta{bend style} (initially in and out)}
		Specify how the bottom side bends.
	\end{key}%
	
	\begin{key}{/pgf/tape bend height=\meta{length} (initially 5pt)}
		Set the total height for a side with a bend.
		
\begin{codeexample}[]
\begin{tikzpicture}[>=stealth]
  \draw [help lines] grid(3,2);
  \node [tape, fill, minimum size=2cm, red!50, tape bend top=none,
         tape bend height=1cm] at (1.5,1.5) (t) {};
  \draw [|<->|, blue] (1.5,0) -- (1.5,1) 
         node [at end, above, black]{tape bend height};
\end{tikzpicture}
\end{codeexample} 
 
	\end{key}
	
	The anchors for the tape shape are shown below. Anchor |60| is an
	example of a border anchor. Note that border anchors will snap to
	the center of convex curves (i.e. when bending in). 
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=tape, tape bend height=1cm, shape example, inner xsep=3cm] 
    {Tape\vrule width1pt height2cm};
   \foreach \anchor/\placement in
    {text/left,  center/above,    60/above, 
     base/below, base east/below, base west/below,
     mid/right,  mid east/left,   mid west/right,  
     north/above, south/below,  east/above, west/above,        
     north west/above, north east/above, 
     south west/below, south east/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}%



\subsection{Arrow Shapes}

\begin{pgflibrary}{shapes.arrows}
  This library defines arrow shapes. Note that an arrow shape is
  something quite different from a (normal) arrow tip: It is a shape
  that just ``happens'' to ``look like'' an arrow. In particular, you
  cannot use these shapes as arrow tips.
\end{pgflibrary}

\begin{shape}{single arrow}
	This shape is an arrow, which tightly fits the note contents 
	(including any |inner sep|). 
	This shape supports the rotation of the shape border, as 
	described in Section~\ref{section-rotating-shape-borders}. 
	The angle of rotation determines which direction the arrow
	points (provided no other rotational transformations are applied).
	
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={single arrow, draw},
    rotate border/.style={shape border uses incircle, shape border rotate=#1}]
  \node {right};
  \node at (2,0) [shape border rotate=90]{up};
  \node at (1,1) [rotate border=37, inner sep=0pt]{$37^\circ$};
\end{tikzpicture}
\end{codeexample}

	Regardless of the rotation of the arrow border, the width is 
  measured between the back ends of the arrow head, and the 
  height is measured from the arrow tip to the end of the arrow 
  tail.

\begin{codeexample}[]
\begin{tikzpicture}[>=stealth, 
    rotate border/.style={shape border uses incircle, shape border rotate=#1}]
  \node[rotate border=-30, fill=gray!25, minimum height=3cm, single arrow, 
    single arrow head extend=.5cm, single arrow head indent=.25cm] (arrow) {};
  \draw[red, <->] (arrow.before tip) -- (arrow.after tip)
    node [near end, left, black] {width};
  \draw[red, <->] (arrow.tip) -- (arrow.tail)
    node [near end, below left, black] {height};
\end{tikzpicture}
\end{codeexample}

	There are \pgfname{} keys that can be used to customize this shape (to
	use these keys in \tikzname{}, simply remove the \declare{|/pgf/|}
	path).
	
\begin{key}{/pgf/single arrow tip angle=\meta{angle} (initially 90)}
  Set the angle for the arrow tip. Enlarging the arrow to some
  minimum width may increase the the height of the shape to maintain
  this angle.
\end{key}

\begin{key}{/pgf/single arrow head extend=\meta{length} (initially .5cm)}
  This sets the distance between the tail of the arrow and the outer
  end of the arrow head. This may change if the shape is enlarged to
  some minimum width.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \node[single arrow, draw, single arrow head extend=.5cm, gray!50, rotate=60] 
     (a) {Arrow};
  \draw[red, |<->|] (a.before tip) -- (a.before head) 
    node [midway, below, sloped, black] {head extend};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/single arrow head indent=\meta{length} (initially 0cm)}
  This moves the point where the arrow head joins the shaft of the
  arrow \emph{towards} the arrow tip, by \meta{length}.
  
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={single arrow, draw=none, rotate=60}]
  \node [fill=red!50]                                           {arrow 1};
  \node [fill=blue!50, single arrow head indent=1ex] at (1.5,0) {arrow 2};
\end{tikzpicture}
\end{codeexample}
\end{key}

  The anchors for this shape are shown below (anchor |20| is an 
  example of a border anchor).
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=single arrow, shape example, single arrow head extend=1.5cm] 
    {Single Arrow\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {text/above,      center/above, 20/above,
     mid west/left,   mid/above,    mid east/above left,
     base west/below, base/below,   base east/below,
     tip/above, before tip/above, after tip/below, before head/above, 
     after head/below, after tail/above, before tail/below, tail/right,   
     north/above, south/below, east/below, west/above,
     north west/above, north east/below, south west/below, south east/above}    
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}





\begin{shape}{double arrow}
  This shape is a double arrow, which tightly fits the note contents 
	(including any |inner sep|), and supports the rotation of the shape
	 border, as described in Section~\ref{section-rotating-shape-borders}. 
	 
	
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={double arrow, draw}]
  \node [double arrow, draw] {Left or Right};
\end{tikzpicture}
\end{codeexample}

  The double arrow behaves exactly like the single arrow, so you
  need to remember that the width is \emph{always} the distance
  between the back ends of the arrow heads, and the height
  is \emph{always} the the tip-to-tip distance.
  
\begin{codeexample}[]
\begin{tikzpicture}[>=stealth, 
    rotate border/.style={shape border uses incircle, shape border rotate=#1}]
  \node[rotate border=210, fill=gray!25, minimum height=3cm, double arrow, 
    double arrow head extend=.5cm, double arrow head indent=.25cm] (arrow) {};
  \draw[red, <->] (arrow.before tip 1) -- (arrow.after tip 1)
    node [near start, right, black] {width};
  \draw[red, <->] (arrow.tip 1) -- (arrow.tip 2)
    node [near end, above left, black] {height};
\end{tikzpicture}
\end{codeexample}

  The \pgfname{} keys that can be used to customize the double arrow 
  behave similarly to the keys for the single arrow (to
	use these keys in \tikzname{}, simply remove the \declare{|/pgf/|}
	path).
  
\begin{key}{/pgf/double arrow tip angle=\meta{angle} (initially 90)}
  Set the angle for the arrow tip. Enlarging the arrow to some
  minimum width may increase the the height of the shape to maintain
  this angle.
\end{key}

\begin{key}{/pgf/double arrow head extend=\meta{length} (initially .5cm)}
  This sets the distance between the shaft of the arrow and the outer
  end of the arrow heads. This may change if the shape is enlarged to
  some minimum width.
\end{key}

\begin{key}{/pgf/double arrow head indent=\meta{length} (initially 0cm)}
  This moves the point where the arrow heads join the shaft of the
  arrow \emph{towards} the arrow tips, by \meta{length}.
  \begin{codeexample}[]
\begin{tikzpicture}[every node/.style={double arrow, draw=none, rotate=-60}]
  \node [fill=red!50]                                           {arrow 1};
  \node [fill=blue!50, double arrow head indent=1ex] at (1.5,0) {arrow 2};
\end{tikzpicture}
\end{codeexample}
\end{key}


  The anchors for this shape are shown below (anchor |20| is an 
  example of a border anchor).
  
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=double arrow, double arrow head extend=1.5cm, shape example, inner xsep=2cm] 
    {Double Arrow\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {text/above, center/above, 20/above,
     mid west/above right, mid/above, mid east/above left,
     base west/below, base/below, base east/below,
     before head 1/above, before tip 1/above, tip 1/above, after tip 1/below, after head 1/below,
     before head 2/above, before tip 2/below, tip 2/above, after tip 2/above, after head 2/below,
     north/above, south/below, east/below, west/below,
     north west/below, north east/below, south west/above, south east/above}    
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}




\begin{shape}{arrow box}
This shape is a rectangle with optional arrows which extend from the
four sides.

\begin{codeexample}[]
\begin{tikzpicture}
  \node[arrow box, draw] {A};
  \node[arrow box, draw, arrow box arrows={north:.5cm, west:0.75cm}] 
    at (2,0) {B};
\end{tikzpicture}
\end{codeexample}

Any minimum size requirements are applied to the main rectangle
\emph{only}. This does not pose too many problems if you wish to
accommodate the length of the arrows, as it is possible to specify 
the length of each arrow independently, from either the border of the
rectangle (the default) or the center of the rectangle.

\begin{codeexample}[]
\begin{tikzpicture}
	\tikzset{box/.style={arrow box, fill=#1}}
	\draw [help lines] grid(3,2);
  \node[box=blue!50, arrow box arrows={east:2cm}]             at (1,1.5){One};
  \node[box=red!50,  arrow box arrows={east:2cm from center}] at (1,0.5){Two};
\end{tikzpicture}
\end{codeexample}

There are various \pgfname{} keys for drawing this shape (to use these
keys in \tikzname, simply remove the \declare{/pgf/} path).

\begin{key}{/pgf/arrow box tip angle=\meta{angle} (initially 90)}
  Set the angle at the arrow tip for all four arrows. 
\end{key}

\begin{key}{/pgf/arrow box head extend=\meta{length} (initially .125cm)}
  Set the the distance the arrow head extends away from the the shaft
  of the arrow. This applies to all arrows.
\end{key}

\begin{key}{/pgf/arrow box head indent=\meta{length} (initially 0cm)}
  Move the point where the arrow head joins the shaft of the arrow
  \emph{towards} the arrow tip. This applies to all arrows.
\end{key}

\begin{key}{/pgf/arrow box shaft width=\meta{length} (initially .125cm)}
  Set the width of the shaft of all arrows.
\end{key}

\begin{key}{/pgf/arrow box north arrow=\meta{distance} (initially .5cm)}
  Set distance the north arrow extends from the node. By default this
  is from the border of the shape, but by using the additional keyword
  |from center|, the distance will be measured from the center of the
  shape. If \meta{distance} is |0pt| or a negative distance, the arrow
  will not be drawn.
\end{key}

\begin{key}{/pgf/arrow box south arrow=\meta{distance} (initially .5cm)}
	Set distance the south arrow extends from the node.
\end{key}

\begin{key}{/pgf/arrow box east arrow=\meta{distance} (initially .5cm)}
	Set distance the east arrow extends from the node.
\end{key}

\begin{key}{/pgf/arrow box west arrow=\meta{distance} (initially .5cm)}
	Set distance the west arrow extends from the node.
\end{key}

\begin{key}{/pgf/arrow box arrows={\ttfamily\char`\{}\meta{list}{\ttfamily\char`\}}}
  Set the distance that all arrows extend from the node. The 
  specification in \meta{list} consists of the four compass points
  |north|, |south|, |east| or |west|, separated by commas (so the list
  must be contained within braces). 
  The distances can be specified after each side separated by a colon 
  (e.g., |north:1cm|, or |west:5cm from center|). 
  If an item specifies no distance, the most recently specifed 
  distance will be used (at the start of the list this is |0cm|,
  so the first item in the list should specify a distance). 
  Any sides not specified will not be drawn with an arrow.
\end{key}

The anchors for this shape are shown below (unfortunately due to its
size, this example must be rotated). Anchor |75| is an example of a
border anchor.
If a side is drawn without an arrow, the anchors for that arrow should 
be considered unavailable. They are (unavoidably) defined, but default 
to the center of the appropriate side.

\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[shape=arrow box, shape example, inner xsep=1cm, inner ysep=1.5cm, arrow box shaft width=2cm,
    arrow box arrows={north:3.5cm from border, south, east:5cm from border, west}, 
    arrow box head extend=0.75cm, rotate=-90](s) {Arrow Box\vrule width1pt height2cm};
  \foreach \anchor/\placement in
   {center/above, text/above, mid/right, base/below, 75/above,
    mid east/right, mid west/left, base east/right, base west/left,
    north/below, south/below, east/below, west/below,
    north east/above, south east/above, south west/below, north west/below,
    north arrow tip/above,south arrow tip/above, east arrow tip/above, west arrow tip/above,
    before north arrow/above, before north arrow head/below left, before north arrow tip/above left, 
    after north arrow tip/above right, after north arrow head/below right, after north arrow/below,
    before south arrow/below, before south arrow head/above right, before south arrow tip/below right, 
    after south arrow tip/below left, after south arrow head/above left, after south arrow/above,
    before east arrow/above, before east arrow head/above right, before east arrow tip/above, 
    after east arrow tip/below, after east arrow head/below right, after east arrow/below, 
    before west arrow/below, before west arrow head/below left, before west arrow tip/below, 
    after west arrow tip/above, after west arrow head/above left, after west arrow/below}
      \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
        node[\placement, rotate=-90] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}



\subsection{Shapes with Multiple Text Parts}

\begin{pgflibrary}{shapes.multipart}
  This library defines general-purpose shapes that are composed of
  multiple (text) parts. 
\end{pgflibrary}


\begin{shape}{circle split}
  This shape is a multi-part shape consisting of a circle with a line
  in the middle. The upper part is the main part (the |text| part),
  the lower part is the |lower| part.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \node [circle split,draw,double,fill=red!20]
  {
    $q_1$
    \nodepart{lower}
    $00$
  };
\end{tikzpicture}
\end{codeexample}

  The shape inherits all anchors from the |circle| shape and defines
  the |lower| anchor in addition. See also the
  following figure:
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=circle split,shape example] {text\nodepart{lower}lower};
  \foreach \anchor/\placement in
    {north west/above left, north/above, north east/above right, 
     west/left, center/below, east/right, 
     mid west/right, mid/above, mid east/left, 
     base west/left, base/below, base east/right, 
     south west/below left, south/below, south east/below right, 
     text/left, lower/left, 130/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}


\begin{shape}{ellipse split}
	This shape is a multi-part shape consisting of an ellipse with a line
  in the middle. The upper part is the main part (the |text| part),
  the lower part is the |lower| part.  
  The anchors for this shape are shown below. Anchor |60| is a border anchor.
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=ellipse split,shape example] {text\nodepart{lower}lower};
  \foreach \anchor/\placement in
    {center/below, text/left, lower/left, 60/above right,
     mid/above, mid east/above, mid west/above,
     base/right, base east/left, base west/right,
     north/above, south/below, east/below, west/below,
     north east/above, south east/below, south west/below, north west/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}


\begin{shape}{rectangle split}
  This shape is a rectangle which can optionally be split into 
  two, three or four node parts, or even used with a single node 
  part. 

\begin{codeexample}[]
\begin{tikzpicture}[every text node part/.style={text centered}]
  \node[rectangle split, rectangle split parts=3, draw, text width=2.75cm] 
    {Student
     \nodepart{second}
       age:int \\
       name:String
     \nodepart{third}
       getAge():int \\
       getName():String};
\end{tikzpicture}
\end{codeexample} 

  
  The contents of node parts which are not used are ignored. 
  Which node parts are used in each case is shown below:

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \a/\x/\y in {1/0/0, 2/1.5/0, 3/0/-1.5, 4/1.5/-1.5}
  \node[rectangle split, rectangle split parts=\a, draw, anchor=north] 
    at (\x,\y){
      text
    \nodepart{second}
      second
    \nodepart{third}
      third
    \nodepart{fourth}
      fourth};
\end{tikzpicture}
\end{codeexample} 

  There are several \pgfname{} keys to specify how the shape is
  drawn. To use these keys in \tikzname, simply remove the 
  \declare{|/pgf/|} path:
  
  \begin{key}{/pgf/rectangle split parts=\meta{number} (initially 4)}
    Split the rectangle into \meta{number} parts, 
    which should be in the range |1| to |4|.
  \end{key}
  
  \begin{key}{/pgf/rectangle split empty part height=\meta{length} (initially 1ex)}
    Set the default height for a node part box if it is empty.
  \end{key}
  
  \begin{key}{/pgf/rectangle split part align={\ttfamily\char`\{}\meta{list}{\ttfamily\char`\}} (initially center)}
  	Set the alignment of the boxes inside the node parts.
  	There should be a maximum of four entries in \meta{list}, 
  	separated by commas (so if there is more than one entry in 
  	\meta{list} it must be surrounded by braces).
  	Each entry is one of |left|,
    |right|, or |center|. If \meta{list} has less entries than 
    node parts then the remaining node parts are aligned according to 
    the last entry in the list.    
    Note that this only aligns the boxes in each part and \emph{does not} 
    affect the alignment of the contents of the boxes.
    
\begin{codeexample}[]
\def\v#1{\vrule width#1ex height2ex}
\def\x{\v2 \nodepart{second} \v5 \nodepart{third} \v2 \nodepart{fourth} \v2}
\begin{tikzpicture}[every node/.style={rectangle split, draw, text=blue!40}]
  \node[rectangle split part align={center, left, right}] at (0,0)    {\x};
  \node[rectangle split part align={center, left}]        at (1.25,0) {\x};
  \node[rectangle split part align={center}]              at (2.5,0)  {\x};
\end{tikzpicture}
\end{codeexample}
  \end{key}
   
  \begin{key}{/pgf/rectangle split draw splits=\meta{boolean} (initially true)}
  	Set whether the line or lines between node parts will be drawn.
  	Internally, this sets the \TeX-if |\ifpgfrectanglesplitdrawsplits| 
  	appropriately.
  \end{key}
  
  \begin{key}{/pgf/rectangle split use custom fill=\meta{boolean} (initially false)}
    This enables the use of a custom fill for each of the node
    parts (including the area covered by the |inner sep|). The 
    background path for the shape should not be filled (e.g., in
    \tikzname{}, the |fill|
    option for the node must be implicity or explicitly set to |none|).
    Internally, this key sets the \TeX-if 
    |\ifpgfrectanglesplitusecustomfill| appropriately.
  \end{key}
  
  \begin{key}{/pgf/rectangle split part fill={\ttfamily\char`\{}\meta{list}{\ttfamily\char`\}} (initially white)}
  	Set the custom fill color for each node part shape. 
  	There should be a maximum of four entries in \meta{list} (one 
  	for each node part), separated by commas (so if there is more than 
  	one entry in \meta{list} it must be surrounded by braces).
  	If \meta{list}  has less entries than node
    parts then the remaining node parts use the color from
    the last entry in the list. This key will automatically set
    |/pgf/rectangle split use custom fill|.
    
\begin{codeexample}[]
\begin{tikzpicture}
  \tikzset{every node/.style={rectangle split, draw, minimum width=.5cm}}
  \node[rectangle split part fill={red!50, green!50, blue!50, yellow!50}]  {};
  \node[rectangle split part fill={red!50, green!50, blue!50}] at (0.75,0) {};
  \node[rectangle split part fill={red!50, green!50}]          at (1.5,0)  {};
  \node[rectangle split part fill={red!50}]                    at (2.25,0) {};
\end{tikzpicture}
\end{codeexample}

	\end{key}
	
  The anchors for the |rectangle split| shape, are
  shown below (anchor |70| is an example of a border angle). When a 
  node part is missing (i.e., when the number of parts is less than 
  |4|), the anchors prefixed with name of that node part should be 
  considered unavailable. They are (unavoidably) defined, but default 
  to other anchor positions.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=rectangle split, rectangle split parts=4, shape example] 
    {\nodepart{text}Text\nodepart{second}Second
		\nodepart{third}Third\nodepart{fourth}fourth};
  \foreach \anchor/\placement in
    {text/left,   text east/above,   text west/above, 
     second/left, second east/above, second west/above,    
     third/left,  third east/below,  third west/below,
     fourth/left, fourth east/below, fourth west/below,
     text split/left,   text split east/above,   text split west/above,
     second split/left, second split east/above, second split west/above,    
     third split/left,  third split east/below,  third split west/below, 
     north/above,  south/below,  east/below,  west/below,  
     center/above, 70/above,     mid/above,   base/below,
     north west/above, north east/above, south west/below, south east/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}





\subsection{Callout Shapes}

\begin{pgflibrary}{shapes.callout}
  Producing basic callouts can be done quite easily in \pgfname{} and 
	\tikzname{} by creating a node and then subsequently drawing a path
	from the border of the node to the required point. This library
	provides more fancy, `balloon'-style callouts.
    
\end{pgflibrary}

Callouts consist of a 
main shape, and a pointer (which is part of the shape) which points
to something in (or outside) the picture. The position on the border
of the main shape to which the pointer is connected is determined
automatically. However, the pointer is ignored when calculating the 
minimum size of the shape, and also when positioning anchors.

\begin{codeexample}[]
\begin{tikzpicture}[remember picture]
  \node[ellipse callout, draw] (hallo) {Hallo!};
\end{tikzpicture}
\end{codeexample}

There are two kinds of pointer:	the ``relative'' pointer and the 
``absolute'' pointer.	The relative pointer calculates the angle of a
specified coordinate relative to the center of the main shape, locates 
the point on the border to which this angle corresponds, and then adds 
the coordinate to this point. This seemingly over-complex approach 
means than you do not have to guess the size of the main shape: the 
relative pointer will always be outside. 
The absolute pointer, on the 
other hand, is much simpler: it points to the specified coordinate
absolutely (and can even point to named coordinates in different 
pictures).


\begin{codeexample}[]
\begin{tikzpicture}[remember picture, note/.style={rectangle callout, fill=#1}]
  \draw [help lines] grid(3,2);
  \node [note=red!50,  callout relative pointer={(0,1)}] at (3,1) {Relative};
  \node [note=blue!50, callout absolute pointer={(0,1)}] at (1,0) {Absolute};
  \node [note=green!50, opacity=.5, overlay, 
         callout absolute pointer={(hallo.south)}]       at (1,2) {Outside};
\end{tikzpicture}
\end{codeexample}


The following keys are common to all callouts. Please remember
that the |callout| |relative| |pointer|, and |callout| |absolute|
|pointer| keys take a different format for their value depending 
on whether they are being used in \pgfname{} or \tikzname{}.
  
  
\begin{key}{/pgf/callout relative pointer=\meta{coordinate} (initially {\ttfamily\char`\\pgfpointpolar\char`\{315\char`\}\char`\{.5cm\char`\}})}
  
  Set the vector of the callout pointer `relative' to the callout 
  shape. 
  
\end{key}

\begin{key}{/pgf/callout absolute pointer=\meta{coordinate}}
  
  Set the vector of the callout pointer absolutely within the picture.
  
\end{key}



\begin{key}{/tikz/callout relative pointer=\meta{coordinate} (initially {(315:.5cm)})}
	The \tikzname{} version of the |callout relative pointer| key. Here,
	\meta{coordinate} can be specified using the \tikzname{} format for
	coordinates.
\end{key}

\begin{key}{/tikz/callout absolute pointer=\meta{coordinate}}
	The \tikzname{} version of the |callout absolute pointer| key. Here,
	\meta{coordinate} can be specified using the \tikzname{} format for
	coordinates.
\end{key}

	It is also possible to shorten the pointer by some distance, using 
	the following key:
	
\begin{key}{/pgf/callout pointer shorten=\meta{distance} (initially 0cm)}
	Move the callout pointer towards the center of the callouts main 
	shape by \meta{distance}. 
	
\begin{codeexample}[]
\begin{tikzpicture}
	\tikzset{callout/.style={ellipse callout, callout pointer arc=30,
	  callout absolute pointer={#1}}}
  \draw (0,0) grid (3,2);
  \node[callout={(3,1.5)}, fill=red!50] at (0,1.5) {A};
  \node[callout={(3,.5)},  fill=green!50, callout pointer shorten=1cm]          
    at (0,.5)  {B};
\end{tikzpicture} 
\end{codeexample}
\end{key}
	
  
\begin{shape}{rectangle callout}%
	
  This shape is a callout whose main shape is a rectangle, which 
  tightly fits the node contents (including any |inner sep|).
  It  supports the keys described above and also the following 
  key:
  
  
\begin{key}{/pgf/callout pointer width=\meta{length} (initially .25cm)} 
  Set the width of the pointer at the border of the rectangle.
\end{key}
		
	The anchors for this shape are shown below (anchor |60| is an
	example of a border anchor). The pointer direction is ignored when 
	placing anchors. 
	Additionally, when using an absolute pointer, the |pointer| 
	anchor should not be used to used to position the shape as it is 
	calculated whilst the shape is being drawn.
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=rectangle callout, callout relative pointer={(1.25cm,-1cm)}, 
     callout pointer width=2cm, shape example, inner xsep=2cm, inner ysep=1cm] 
  	{Rectangle Callout\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {center/above, text/below,      60/above,
     mid/right,    mid west/left,  mid east/right, 
     base/below,   base west/below, base east/below, 
     north/above,  south/below, east/above, west/above,
     north west/above, north east/above,     
     south west/below, south east/below,
     pointer/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}%


\begin{shape}{ellipse callout}%
	
  This shape is a callout whose main shape is a ellipse, which 
  tightly fits the node contents (including any |inner sep|).
  It uses the |absolute callout pointer|, 
	|relative callout pointer| and |callout pointer shorten| keys, and
	also the following key:
  
  
\begin{key}{/pgf/callout pointer arc=\meta{angle} (initially 15)} 
  Set the width of pointer at the border of the ellipse according
  to an arc of length \meta{angle}.
\end{key}
	
	
	The anchors for this shape are shown below (anchor |60| is an
	example of a border anchor). The pointer direction is ignored 
	when placing anchors and the |pointer| anchor can only be
	used to position the shape when the relative anchor is 
	specified.
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=ellipse callout, callout relative pointer={(1.25cm,-1cm)}, 
    callout pointer width=2cm, shape example, inner xsep=1cm, inner ysep=.5cm] 
  	{Ellipse Callout\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {center/above, text/below,      60/above,
     mid/above,    mid west/right,  mid east/left, 
     base/below,   base west/below, base east/below, 
     north/above,  south/below, east/above, west/above,
     north west/above left,    north east/above right,     
     south west/below left,    south east/below right,
     pointer/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}


\begin{shape}{cloud callout}
This shape is a callout whose main shape is a cloud which fits the 
node contents. The pointer is segmented, consisting of a series of 
shrinking ellipses. This callout requires the symbol shape library 
(for the cloud shape). If this library is not loaded an error will 
result.

\begin{codeexample}[]
\begin{tikzpicture}
  \node[cloud callout, cloud puffs=15, aspect=2.5, cloud puff arc=120, 
    shading=ball,text=white] {\bf Imagine...};
\end{tikzpicture}
\end{codeexample}

The |cloud callout| supports the |absolute callout pointer|,
|relative callout pointer| and |callout pointer shorten| keys, as 
described above.
The main shape can be modified using the same keys as the |cloud| 
shape. The following keys are also supported:

\begin{key}{/pgf/callout pointer start size=\meta{value} (initially .2 of callout)}
	Set the size of the first segment in the pointer (i.e., the segment
	nearest the main cloud shape). There are three possible forms for
	\meta{value}:
	\begin{itemize}
		\item
			A single dimension (e.g., |5pt|), in which case the first ellipse 
			will have equal diameters of 5pt.
		\item
			Two dimensions (e.g., |10pt and 2.5pt|), which sets the $x$ and 
			$y$ diameters of the first ellipse.
		\item
			A decimal fraction (e.g., |.2 of callout|), in which case
			the $x$ and $y$ diameters of the first ellipse will be set as 
			fractions of the width and height of the main shape. The keyword
			|of callout| cannot be omitted.	
	\end{itemize}
\end{key}

\begin{key}{/pgf/callout pointer end size=\meta{value} (initially .1 of callout)}
	Set the size of the last ellipse in the pointer.
\end{key}

\begin{key}{/pgf/callout pointer segments=\meta{number} (initially 2)}
	Set the number of segments in the pointer. Note that \pgfname{} will 
	happily	overlap segments if too many are specified. 
\end{key}

The anchors for this shape are shown below (anchor |70| is an example 
of a border anchor). The pointer direction is ignored when placing 
anchors and the pointer anchor can only be used to position the
shape when the relative anchor is specified. Note that the center
of the last segment is drawn at the |pointer| anchor.

\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s, shape=cloud callout, style=shape example, cloud puffs=11, aspect=1.5,
    cloud puff arc=120,inner xsep=.5cm, callout pointer start size=.25 of callout,
    callout pointer end size=.15 of callout, callout relative pointer={(315:4cm)},
    callout pointer segments=2] {Cloud Callout\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {puff 1/above, puff 2/above, puff 3/above, puff 4/below,
     puff 5/left, puff 6/below, puff 7/below, puff 8/right,
     puff 9/below, puff 10/above, puff 11/above, 70/right,
     center/above, base/below, mid/right, text/left,
     north/below, south/below, east/above, west/above,
     north west/left, north east/right,
     south west/below, south east/below,pointer/above}
  \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
    node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}%
\end{shape}




\subsection{Logic Gate Shapes}

\subsubsection{Overview}
	\pgfname{} provides two libraries of logic gates, one providing
	``American'' style gates and the other, providing ``rectangular'' 
	logic gates.	
	Each library suffixes the gate names with an identifer:
	|US| for the American style gates, and |IEC| for the rectangular
	gates (additionally, two shapes in the |US| library use the
	suffix |CDH|). Keys which are specific
	to a particular library	also contain this identifier (e.g., 
	|/pgf/and gate IEC symbol|).
	However, as described below, a \tikzname{} key is provided which
	sets up several styles allowing the identifier to be omitted,
	for example, |and gate| can become a synonym for |shape=and gate US|.
	
	Multiple inputs can be specified for a logic gate (provided they
  support multiple inputs: a not gate --- also known as an inverter ---
  does not). However, there is an upper limit for the number of inputs 
  which has been set at 1024, which should be \emph{way} 
  more than would ever be needed.
    
  There are some \pgfname{} keys which are common to both 
  libraries, which have no library identifier contained in them:
  
  
  \begin{key}{/pgf/logic gate inputs=\meta{input list} (initially \char`\{normal,normal\char`\})}
  Specify the inputs for for the logic gate. The keyword |inverted|
  indicates an inverted input which will mean \pgfname{} will draw a
  circle attached to the main shape of the logic gate. Any keyword
  that is not |inverted| will be treated as a ``normal'' or 
  ``non-inverted'' input (however, for readability, you may wish to 
  use |normal| or |non-inverted|), and \pgfname{} will not draw the 
  circle.  
  In both cases the anchors for the inputs will be set 
  up appropriately, numbered from top to bottom |input 1|, |input 2|,
  \ldots and so on. If the gate only supports one input the anchor
  is simply called |input| with no numerical index.
  
\begin{codeexample}[]
\begin{tikzpicture}[minimum height=0.75cm]
  \node[and gate IEC, draw, logic gate inputs={inverted, normal, inverted}] 
  (A) {};
  \foreach \a in {1,...,3}
    \draw (A.input \a -| -1,0) -- (A.input \a);
  \draw (A.output) -- ([xshift=0.5cm]A.output);
\end{tikzpicture}
\end{codeexample} 
  
  For multiple inputs it may be somewhat unweildy to specify a long
  list, thus, the following ``shorthand'' is permitted (this is an  
  extension of ideas due to Juergen Werber and Christoph Bartoschek):
  Using |i| for inverted and |n| for normal inputs, \meta{input list}
  can be specfied \emph{without the commas}. So, for example,
  |ini| is equivalent to |inverted, normal, inverted|.
  
\begin{codeexample}[]
\begin{tikzpicture}[minimum height=0.75cm]
  \node[or gate US, draw,logic gate inputs=inini] (A) {};
  \foreach \a in {1,...,5}
    \draw (A.input \a -| -1,0) -- (A.input \a);
  \draw (A.output) -- ([xshift=0.5cm]A.output);
\end{tikzpicture}
\end{codeexample} 
 
\end{key}


The height of the gate may be increased to accommodate the number 
of inputs. In fact, it depends on three variables:
$n$, the number of inputs, $r$, the radius of the circle used
to indicate an inverted input and $s$, the distance between
the centers of the inputs.
The default height is then calculated according to the expression 
$(n+1)\times\max(2r,s)$. This then may
be increased to accommodate the node contents or any
minimum size specifications.

The radius of the inverted input circle and the distance between the 
centers of the inputs can be customised using the following keys:

\begin{key}{/pgf/logic gate inverted radius=\meta{length} (initially 2pt)}
  Set the radius of the circle that is used to indicate inverted
  inputs. This is also the radius of the circle used for the inverted
  output of the |nand|, |nor|, |xnor| and |not| gates. 
    
\begin{codeexample}[]
\begin{tikzpicture}[minimum height=0.75cm]
  \tikzset{every node/.style={shape=nand gate CDH, draw, logic gate inputs=ii}}
  \node[logic gate inverted radius=2pt] {A};
  \node[logic gate inverted radius=4pt] at (0,-1) {B};
\end{tikzpicture}
\end{codeexample} 
\end{key}

\begin{key}{/pgf/logic gate input sep=\meta{length} (initially .125cm)}
  Set the distance between the \emph{centers} of the inputs to the
  logic gate. 
  
\begin{codeexample}[]
\begin{tikzpicture}[minimum size=0.75cm]
  \draw [help lines] grid (3,2);
  \tikzset{every node/.style={shape=and gate IEC, draw, logic gate inputs=ini}}
  \node[logic gate input sep=0.33333cm] at (1,1)(A) {A};
  \node[logic gate input sep=0.5cm]     at (3,1) (B) {B};
  \foreach \a in {1,...,3}
    \draw (A.input \a -| 0,0) -- (A.input \a)
          (B.input \a -| 2,0) -- (B.input \a);
\end{tikzpicture}
\end{codeexample} 
\end{key}


\subsubsection{US Logic Gates}

\begin{pgflibrary}{shapes.gates.logic.US}
 This library provides ``American'' logic gate shapes whose names are 
  suffixed with the identifier |US|. Additionally,
  alternative |and| and |nand| gates are provided which are based on the 
  logic symbols used in A. Croft, R. Davidson, and M. Hargreaves (1992), 
  \emph{Engineering Mathematics}, Addison-Wesley, 82--95. These two 
  shapes are suffixed with |CDH|. 
\end{pgflibrary}

  To use the shapes in \tikzname{} without their suffixes, the 
  following keys are provided:
  
\begin{key}{/tikz/use US style logic gates}
	This allows the the shapes suffixed with |US| to be used without
	the suffix. So, for example, |and gate| becomes a synonym for
	|shape=and gate US|.
\begin{codeexample}[]
\tikz\node[draw, and gate US, red]{and};
\space
\tikz[use US style logic gates,blue]\node[draw, and gate]{and};
\end{codeexample}
\end{key}

\begin{key}{/tikz/use CDH style logic gates}
	This key again allows the the shapes suffixed with |US| to be used 
	without	the |US| suffix. However, |and gate| becomes a synonym for
	|shape=and gate CDH| and |nand gate| becomes a synonym for
	|shape=nand gate CDH|, providing alternative symbols for these
	gates.
	
\begin{codeexample}[]
\begin{tikzpicture}[minimum height=1cm]
  \node[draw, and gate US, red]  at  (0,1.5) {and};
  \node[draw, nand gate US, red] at (2,1.5) {nand};
  \tikzset{use CDH style logic gates}
  \node[draw, and gate, blue]  at (0,0) {and};
  \node[draw, nand gate, blue] at (2,0) {nand};
\end{tikzpicture}
\end{codeexample}
\end{key}



As described above, \pgfname{} will increase the size of the 
logic gate to accommodate the number of inputs, and the size
of the inverted radius and the separation between the inputs.
However with all shapes in this library, any increase in size 
(including any minimum size requirements) will be applied so that 
the default aspect ratio is unaltered. This means that changing
the height will change the width and vice versa. 

The ``compass point'' anchors apply to the main part of the shape
and do not include any inverted inputs or outputs. This library
provides an additonal feature to facilitate the relative positioning
of logic gates:

\begin{key}{/pgf/logic gate anchors use bounding box=\meta{boolean} (initially false)}
When set to |true| this key will ensure that the 
compass point anchors use the bounding rectangle of the
main shape, which, ignore any inverted inputs or outputs, but
includes any |outer sep|. 
This \emph{only} affects the compass point anchors
and is not set on a shape by shape basis: whether the bounding
box is used is determined by value of this key when the anchor
is accessed.

\begin{codeexample}[]
\begin{tikzpicture}[minimum height=1.5cm]
  \node[xnor gate US, draw, gray!50,line width=2pt] (A) {};
  \foreach \x/\y/\z in {false/blue/1pt, true/red/2pt}
    \foreach \a in {north, south, east, west, north east, 
      south east, north west, south west}
      \draw[logic gate anchors use bounding box=\x, color=\y]	
        (A.\a) circle(\z);
\end{tikzpicture}
\end{codeexample} 



\end{key}




\begin{shape}{and gate US}
  This shape is an and gate which supports two or more inputs. If
	less than two inputs are specified an error will result. 
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=and gate US,shape example, inner sep=0cm,
    logic gate inverted radius=.5cm] {And Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/right, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/above, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}

\begin{shape}{nand gate US}
  This shape is a nand gate, which supports two or more inputs. If
	less than two inputs are specified an error will result. 
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
 
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=nand gate US,shape example, inner sep=0cm,
  logic gate inverted radius=.5cm] {Nand Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/above, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}

\begin{shape}{or gate US}

	This shape is an or gate, which supports two or more inputs. If
	less than two inputs are specified an error will result. 
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=or gate US,shape example, inner sep=0cm,
  logic gate inverted radius=.5cm] {Or Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/left, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}

\begin{shape}{nor gate US}
	This shape is a nor gate, which supports two or more inputs. If
	less than two inputs are specified an error will result. 
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.

\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=nor gate US,shape example, inner sep=0cm,
  logic gate inverted radius=.5cm] {Nor Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/left, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}

\begin{shape}{xor gate US}
  This shape is an xor gate, which supports only two inputs. If
  less than two inputs are specified an error will result. If more
  than two inputs are specified, the extra inputs are ignored.
  The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=xor gate US,shape example, inner sep=0cm,
    logic gate inverted radius=.5cm] {Xor Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/above, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}

\begin{shape}{xnor gate US}

	This shape is an xnor gate, which supports only two inputs. If
	less than two inputs are specified an error will result. If more
	than two inputs are specified, the extra inputs are ignored.
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=xnor gate US,shape example, inner sep=0cm,
  logic gate inverted radius=.5cm] {Xnor Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/above, input 1/above, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}


\end{shape}

\begin{shape}{not gate US}
	This shape is a not gate, which supports only one input. If
	no inputs are specified an error will result. If more
	than one input is specified, the extra inputs are ignored.
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=not gate US,shape example, inner sep=1.5cm,
  logic gate inverted radius=.5cm] 
  {Not Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/below,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}

\begin{shape}{buffer gate US}
	This shape is a not gate, which supports only one input. If
	no inputs are specified an error will result. If more
	than one input is specified, the extra inputs are ignored.
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=buffer gate US,shape example, inner sep=1.5cm,
  logic gate inverted radius=.5cm] 
  {Buffer Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/below,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}





\begin{shape}{and gate CDH}
  This shape is the alternative and gate. It supports two or more inputs.
  If less than two inputs are specified an error will result. 
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=and gate CDH,shape example, inner sep=0cm,
    logic gate inverted radius=.5cm] {And Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/above, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}

\begin{shape}{nand gate CDH}
  This shape is the alternative nand gate. It supports two or more inputs.
  If less than two inputs are specified an error will result. 
	The anchors for this gate with two
  non-inverted inputs (using the normal compass point anchors) are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=nand gate CDH,shape example, inner xsep=0cm,
    logic gate inverted radius=.5cm] {Nand Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/above, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}





\subsubsection{IEC Logic Gates}

\begin{pgflibrary}{shapes.gates.logic.IEC}
  This library provides rectangular logic gate shapes. These shapes
  are suffixed with |IEC| as they are based on gates recommended by
  the International Electrotechincal Commission.
\end{pgflibrary}

  In order to use these shapes in \tikzname{} without the |IEC|
  suffix, the following key is provided:
  
\begin{key}{/tikz/use IEC style logic gates}
	This allows the the shapes suffixed with |IEC| to be used without
	the suffix. So, for example, |and gate| becomes a synonym for
	|shape=and gate IEC|. In addtion the |IEC| specific keys can be
	used without |IEC|, so |and gate symbol| can be
	used for |and gate IEC symbol|.
\end{key}

  By default each gate is drawn with a symbol, $\char`\&$ for |and| and 
  |nand| gates, $\geq1$ for |or| and |nor| gates, $1$ for |not| and 
  |buffer| gates, and $=1$ for |xor| and |xnor| gates. These symbols 
  are drawn automatically (internally they are drawn using the 
  ``foreground'' path), and are not strictly speaking part of the node
  contents. However, the gate is enlarged to make sure the symbols are 
  within the border of the node.
  It is possible to change
  the symbols and their position within the node using the following
  keys:
  
\begin{key}{/pgf/and gate IEC symbol=\meta{text} (initially \char`\\char\char`\`\char`\\\char`\&)}
  Set the symbol for the |and gate|. Note that if the node is filled,
  this color will be used for the symbol, making it invisible, so
  it will be necessary set \meta{text} to something like
  |\color{black}\char`\&|. Alternatively, the 
  |logic gate IEC symbol color| key can be used to set the color
  of all symbols simultaneously.
  
  In \tikzname, when the |use IEC style logic gates| key has been 
  used, this key can be replaced by |and gate symbol|.
\end{key}

\begin{key}{/pgf/nand gate IEC symbol=\meta{text} (initially \char`\\char\char`\`\char`\\\char`\&)}
  Set the symbol for the |nand gate|.  
  In \tikzname, when the |use IEC style logic gates| key has been 
  used, this key can be replaced by |nand gate symbol|.
\end{key}

\begin{key}{/pgf/or gate IEC symbol=\meta{text} (initially \char`\$\char`\\geq1\char`\$)}
  Set the symbol for the |or gate|.  
  In \tikzname, when the |use IEC style logic gates| key has been 
  used, this key can be replaced by |or gate symbol|.
\end{key}

\begin{key}{/pgf/nor gate IEC symbol=\meta{text} (initially \char`\$\char`\\geq1\char`\$)}
  Set the symbol for the |nor gate|.  
  In \tikzname, when the |use IEC style logic gates| key has been 
  used, this key can be replaced by |nor gate symbol|.
\end{key}

\begin{key}{/pgf/xor gate IEC symbol=\meta{text} (initially \char`\{\char`\$=1\char`\$\char`\})}
  Set the symbol for the |xor gate|. Note the necessity for braces,
  as the symbol contains |=|.
  In \tikzname, when the |use IEC style logic gates| key has been 
  used, this key can be replaced by |or gate symbol|.
\end{key}

\begin{key}{/pgf/xnor gate IEC symbol=\meta{text} (initially  \char`\{\char`\$=1\char`\$\char`\})}
  Set the symbol for the |xnor gate|.  
  In \tikzname, when the |use IEC style logic gates| key has been 
  used, this key can be replaced by |xnor gate symbol|.
\end{key}

\begin{key}{/pgf/not gate IEC symbol=\meta{text} (initially 1)}
  Set the symbol for the |not gate|.  
  In \tikzname, when the |use IEC style logic gates| key has been 
  used, this key can be replaced by |not gate symbol|.
\end{key}

\begin{key}{/pgf/buffer gate IEC symbol=\meta{text} (initially 1)}
  Set the symbol for the |buffer gate|.  
  In \tikzname, when the |use IEC style logic gates| key has been 
  used, this key can be replaced by |buffer gate symbol|.
\end{key}

\begin{key}{/pgf/logic gate IEC symbol align=\meta{align} (initially top)}
  Set the alignment of the logic gate symbol (in \tikzname, when the 
  |use IEC style logic gates| key has been used, |IEC| can be omitted.
  The specification in \meta{align} is a comma separated list from
  |top|, |bottom|, |left| or |right|. The distance between the border
  of the node and the outer edge of the symbol is determined by the values 
  of the |inner xsep| and |inner ysep|.
  
\begin{codeexample}[]
\begin{tikzpicture}[minimum size=1cm, use IEC style logic gates]
	\tikzset{every node/.style={nor gate, draw}}
  \node (A) at (0,1.5) {};
  \node [logic gate symbol align={bottom, right}] (B) at (0,0) {}; 
  \foreach \g in {A, B}{
    \foreach \i in {1,2}
      \draw ([xshift=-0.5cm]\g.input \i) -- (\g.input \i);
    \draw (\g.output) -- ([xshift=0.5cm]\g.output);
  }
\end{tikzpicture}
\end{codeexample} 

\end{key}


\begin{key}{/pgf/logic gate IEC symbol color=\meta{color}}
  This key sets the color for all symbols simultaneously. This color
  can be overridden on a case by case basis by specifying a color
  when seting the symbol text.
\end{key}


\begin{shape}{and gate IEC}
  This shape is an and gate. It supports two or more inputs.
  If less than two inputs are specified an error will result. 
	The anchors for this gate with two
  non-inverted inputs are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=and gate IEC ,shape example, inner xsep=1cm, inner ysep=1cm,
    minimum height=6cm, and gate IEC symbol=\color{black!30}\char`\&] 
  {And Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/above, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}


\begin{shape}{nand gate IEC}
  This shape is a nand gate. It supports two or more inputs.
  If less than two inputs are specified an error will result. 
	The anchors for this gate with two
  non-inverted inputs are
  shown below. Anchor |30| is an example of a border anchor.
  
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=nand gate IEC ,shape example, inner xsep=1cm, inner ysep=1cm,
    minimum height=6cm, nand gate IEC symbol=\color{black!30}\char`\&,
    logic gate inverted radius=0.65cm] 
  {Nand Gate\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {center/above, text/above, 30/above right,
     mid/right, mid east/left, mid west/above,
     base/below, base east/below, base west/left,
     north/above, south/below, east/above, west/above,
     north east/above, south east/below, south west/below, north west/above,
     output/right, input 1/above, input 2/below}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}

\begin{shape}{or gate IEC}
  This shape is an or gate. It supports two or more inputs.
  If less than two inputs are specified an error will result. 
	See the |and gate IEC| shape for the anchors.
	
\begin{codeexample}[]
\begin{tikzpicture}[minimum width=.875cm, minimum height=1cm]
  \node[or gate IEC, draw, logic gate inputs=in] (A) {};
  \draw (A.input 1 -| -1,0) -- (A.input 1) (A.input 2 -| -1,0) -- (A.input 2)
        (A.output) -- ([xshift=0.5cm]A.output);
\end{tikzpicture}
\end{codeexample} 

\end{shape}


\begin{shape}{nor gate IEC}
  This shape is an nor gate. It supports two or more inputs.
  If less than two inputs are specified an error will result. 
	See the |nand gate IEC| shape for the anchors.
	
\begin{codeexample}[]
\begin{tikzpicture}[minimum width=.875cm, minimum height=1cm]
  \node[nor gate IEC, draw, logic gate inputs=in] (A) {};
  \draw (A.input 1 -| -1,0) -- (A.input 1) (A.input 2 -| -1,0) -- (A.input 2)
        (A.output) -- ([xshift=0.5cm]A.output);
\end{tikzpicture}
\end{codeexample}

\end{shape}

\begin{shape}{xor gate IEC}
  This shape is an xor gate. It supports only two inputs.
   If less than two inputs are specified an error will result.
  Any extra inputs are ignored.  
		See the |and gate IEC| shape for the anchors.
	
\begin{codeexample}[]
\begin{tikzpicture}[minimum width=.875cm, minimum height=1cm]
  \node[xor gate IEC, draw, logic gate inputs=in] (A) {};
  \draw (A.input 1 -| -1,0) -- (A.input 1) (A.input 2 -| -1,0) -- (A.input 2)
        (A.output) -- ([xshift=0.5cm]A.output);
\end{tikzpicture}
\end{codeexample}

\end{shape}


\begin{shape}{xnor gate IEC}
  This shape is an xnor gate. It supports only two inputs.
  If less than two inputs are specified an error will result.
  Any extra inputs are ignored.  
	See the |nand gate IEC| shape for the anchors.
	
\begin{codeexample}[]
\begin{tikzpicture}[minimum width=.875cm, minimum height=1cm]
  \node[xnor gate IEC, draw, logic gate inputs=in] (A) {};
  \draw (A.input 1 -| -1,0) -- (A.input 1) (A.input 2 -| -1,0) -- (A.input 2)
        (A.output) -- ([xshift=0.5cm]A.output);
\end{tikzpicture}
\end{codeexample}

\end{shape}

\begin{shape}{buffer gate IEC}
   This shape is a buffer gate. It supports only one input.
  If less than one input is specified an error will result.
  Any extra inputs are ignored. 
	See the |and gate IEC| shape for the anchors.

\begin{codeexample}[]
\begin{tikzpicture}[minimum width=.875cm, minimum height=1cm]
  \node[buffer gate IEC, draw] (A) {};
  \draw (A.input -| -1,0) -- (A.input) (A.output) -- ([xshift=0.5cm]A.output);
\end{tikzpicture}
\end{codeexample}

\end{shape}


\begin{shape}{not gate IEC}
  This shape is a not gate. It supports only one input.
  If less than one input is specified an error will result.
  Any extra inputs are ignored. 
  See the |nand gate IEC| shape for the anchors.

\begin{codeexample}[]
\begin{tikzpicture}[minimum width=.875cm, minimum height=1cm]
  \node[not gate IEC, draw] (A) {};
  \draw (A.input -| -1,0) -- (A.input) (A.output) -- ([xshift=0.5cm]A.output);
\end{tikzpicture}
\end{codeexample}


\end{shape}






\subsection{Miscellaneous Shapes}

\begin{pgflibrary}{shapes.misc}
  This library defines general-purpose shapes that do not fit in the
  previous categories.
\end{pgflibrary}

\begin{shape}{cross out}
  This shape ``crosses out'' the node. Its foreground path are simply
  two diagonal lines that between the corners of the node's bounding
  box. Here is an example:  
\begin{codeexample}[]
\begin{tikzpicture} 
  \draw [help lines] (0,0) grid (3,2); 
  \node [cross out,draw=red] at (1.5,1) {cross out}; 
\end{tikzpicture}
\end{codeexample}

  A useful application is inside text as in the following example:
\begin{codeexample}[]
Cross \tikz[baseline] \node [cross out,draw,anchor=text] {me}; out!  
\end{codeexample}

  This shape inherits all anchors from the |rectangle| shape, see also
  the following figure:
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=cross out,shape example] {cross out\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {north west/above left, north/above, north east/above right, 
     west/left, center/above, east/right, 
     mid west/right, mid/above, mid east/left, 
     base west/left, base/below, base east/right, 
     south west/below left, south/below, south east/below right, 
     text/left, 10/right, 130/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}


\begin{shape}{cross out}
  This shape ``crosses out'' the node. Its foreground path are simply
  two diagonal lines that between the corners of the node's bounding
  box. Here is an example:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \node [cross out,draw=red] at (1.5,1) {cross out};
\end{tikzpicture}
\end{codeexample}

  A useful application is inside text as in the following example:
\begin{codeexample}[]
Cross \tikz[baseline] \node [cross out,draw,anchor=text] {me}; out!  
\end{codeexample}

  This shape inherits all anchors from the |rectangle| shape, see also
  the following figure:
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=cross out,shape example] {cross out\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {north west/above left, north/above, north east/above right, 
     west/left, center/above, east/right, 
     mid west/right, mid/above, mid east/left, 
     base west/left, base/below, base east/right, 
     south west/below left, south/below, south east/below right, 
     text/left, 10/right, 130/above}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}
\end{shape}

\begin{shape}{strike out}
  This shape is idential to the |cross out| shape, only its foreground
  path consists of a single line from the lower left to the upper
  right.
  
\begin{codeexample}[]
Strike \tikz[baseline] \node [strike out,draw,anchor=text] {me}; out!  
\end{codeexample}

  See the |cross out| shape for the anchors.
\end{shape}




\begin{shape}{rounded rectangle}
	This shape is a rectangle which can be optionally round sides.

\begin{codeexample}[]
\begin{tikzpicture}
  \node[rounded rectangle, draw, fill=red!20]{Hallo};
\end{tikzpicture}
\end{codeexample}

	There are keys to specify how the sides are rounded (to use
	these keys in \tikzname, simply remove the \declare{|/pgf/|} path).


\begin{key}{/pgf/rounded rectangle arc length=\meta{angle} (initially 180)}

	Set the length of the arcs for the rounded ends. Recommended values 
	for	\meta{angle} are between |90| and |180|. 
	
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix[row sep=5pt, every node/.style={draw, rounded rectangle}]{
    \node[rounded rectangle arc length=180] {180}; \\
    \node[rounded rectangle arc length=120] {120}; \\
    \node[rounded rectangle arc length=90]  {90};  \\};
\end{tikzpicture} 
\end{codeexample}

\end{key}

\begin{key}{/pgf/rounded rectangle west arc=\meta{arc type} (initially convex)}
	Set the style of the rounding for the left side. The permitted values
	for \meta{arc type} are |concave|, |convex|, or |none|.

\begin{codeexample}[]
\begin{tikzpicture}
  \matrix[row sep=5pt, every node/.style={draw, rounded rectangle}]{
  	\node[rounded rectangle west arc=concave] {Concave}; \\
  	\node[rounded rectangle west arc=convex]  {Convex};  \\
  	\node[rounded rectangle left arc=none]    {None};    \\};
\end{tikzpicture} 
\end{codeexample}
\end{key}

\begin{stylekey}{/pgf/rounded rectangle left arc=\meta{arc type}}
	Alternative key for specifying the west arc.
\end{stylekey}

\begin{key}{/pgf/rounded rectangle east arc=\meta{arc type} (initially convex)}
	Set the style of the rounding for the east side.
\end{key}

\begin{stylekey}{/pgf/rounded rectangle right arc=\meta{arc type}}
	Alternative key for specifying the east arc.
\end{stylekey}

	The anchors for this shape are shown below (anchor |10| is an example
	of a border angle). Note that if only one side is rounded, the 
	|center| anchor will not be the precise center of the shape.
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=rounded rectangle, shape example, inner xsep=1.5cm, inner ysep=1cm] 
  	{Rounded Rectangle\vrule width 1pt height 2cm};
  \foreach \anchor/\placement in
    {center/above, text/below,      10/above,
     mid/above,    mid west/right,  mid east/left, 
     base/below,   base west/below, base east/below, 
     north/above,  south/below, east/above, west/above, 
     north west/above left,    north east/above right,     
     south west/below left,    south east/below right}
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}


\begin{shape}{chamfered rectangle}

	This shape is a rectangle with optionally chamfered corners.
	
\begin{codeexample}[]
\begin{tikzpicture}
  \node[chamfered rectangle, white, fill=red, double=red, draw, very thick]
    {\bf STOP!};
\end{tikzpicture}
\end{codeexample}

	There are \pgfname{} keys to specify how this shape is drawn (to use
	these keys in \tikzname{} simply remove the \declare{|/pgf/|} path).

\begin{key}{/pgf/chamfered rectangle angle=\meta{angle} (initially 45)}
	Set the angle \emph{from the vertical} for the chamfer.
	
\begin{codeexample}[]
\begin{tikzpicture}
  \tikzset{every node/.style={chamfered rectangle, draw}}
  \node[chamfered rectangle angle=30] {abc};
  \node[chamfered rectangle angle=60] at (1.5,0) {123};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/chamfered rectangle xsep=\meta{length} (initially .666ex)}
	Set the distance that the chamfer extends horizontally beyond the node 
	contents (which includes the |inner sep|). 
	If \meta{length} is large, such
	that the top and bottom chamfered edges would cross, then 
	\meta{length} is ignored and the chamfered edges are drawn so that
	they meet in the middle.

\begin{codeexample}[]
\begin{tikzpicture}
  \tikzset{every node/.style={chamfered rectangle, draw}}
  \node[chamfered rectangle xsep=2pt] {def};
  \node[chamfered rectangle xsep=2cm] at (1.5,0) {456};
\end{tikzpicture}
\end{codeexample}
	
\end{key}

\begin{key}{/pgf/chamfered rectangle ysep=\meta{length} (initially .666ex)}
	Set the distance that the chamfer extends vertically beyond the node 
	contents. 
	If \meta{length} is large, such that the left and right chamfered 
	edges would cross, then \meta{length} is ignored and the chamfered 
	edges are drawn so that	they meet in the middle.
\end{key}

\begin{key}{/pgf/chamfered rectangle sep=\meta{length} (initially .666ex)}
	Set both the |xsep| and |ysep| simultaneously.
\end{key}

\begin{key}{/pgf/chamfered rectangle corners=\meta{list} (initially chamfer all)}
	Specify which corners are chamfered. The corners are identified by 
	their ``compass point'' directions (i.e. |north east|, |north west|,
	|south west|, and |south east|), and must be separated by commas (so
	if there is more than one corner in the list, it must be surrounded
	by braces). Any corners not mentioned in 
	\meta{list} are automatically not chamfered. Two additional values
	|chamfer all| and |chamfer none|, are also permitted.

\begin{codeexample}[]
\begin{tikzpicture}
  \tikzset{every node/.style={chamfered rectangle, draw}}
  \node[chamfered rectangle corners=north west] {ghi};
  \node[chamfered rectangle corners={north east, south east}] at (1.5,0) {789};
\end{tikzpicture}
\end{codeexample}
\end{key}


	The anchors for this shape are shown below (anchor |60| is an example
	of a border angle.
	
\begin{codeexample}[]
\Huge
\begin{tikzpicture}
  \node[name=s,shape=chamfered rectangle, chamfered rectangle sep=1cm,
        shape example, inner ysep=1cm, inner xsep=.75cm] 
    {Chamfered Rectangle\vrule width1pt height2cm};
  \foreach \anchor/\placement in
    {text/right, center/above,    70/above, 
     base/below, base east/left, base west/right,
     mid/right,  mid east/above,   mid west/above,  
     north/above, south/below, east/above, west/above,
     before north east/above, north east/above, after north east/above,
     before north west/above, north west/above, after north west/above,
     before south west/below, south west/below, after south west/below,
     before south east/below, south east/below, after south east/below}     
     \draw[shift=(s.\anchor)] plot[mark=x] coordinates{(0,0)}
       node[\placement] {\scriptsize\texttt{(s.\anchor)}};
\end{tikzpicture}
\end{codeexample}

\end{shape}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-through.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Through Library}

\label{section-through-library}


\begin{tikzlibrary}{through}
  This library defines keys for creating shapes that go through given
  points. 
\end{tikzlibrary}


\begin{key}{/tikz/circle through=\meta{coordinate}}

  When this key is given as an option to a node, the following
  happens:
  \begin{enumerate}
  \item The |inner sep| and the |outer sep| are set to zero.
  \item The shape is set to |circle|.
  \item The |minimum size| is set such that the circle around the
    center of the node (which is specified using |at|), goes through
    \meta{coordinate}. 
  \end{enumerate}
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \node (a) at (2,1.5) {$a$};
  \node [draw] at (1,1) [circle through={(a)}] {$c$};
\end{tikzpicture}
\end{codeexample}
\end{key}

  

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-library-trees.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Tree Library}

\label{section-tree-library}


\begin{tikzlibrary}{trees}
  This packages defines styles to be used when drawing trees. 
\end{tikzlibrary}

\subsection{Growth Functions}

The package |pgflibrarytikztrees| defines two new growth
functions. They are installed using the following options:

\begin{key}{/tikz/grow via three points=|one child at (|\meta{x}%
  |) and two children at (|\meta{y}|) and (|\meta{z}|)|}
  This option installs a growth function that works as follows: If a
  parent node has just one child, this child is placed at \meta{x}. If
  the parent node has two children, these are placed at \meta{y} and
  \meta{z}. If the parent node has more than two children, the
  children are placed at points that are linearly extrapolated from
  the three points \meta{x}, \meta{y}, and \meta{z}. In detail, the
  position is $x + \frac{n-1}{2}(y-x) + (c-1)(z-y)$, where $n$ is the
  number of children and $c$ is the number of the current child
  (starting with~$1$).

  The net effect of all this is that if you have a certain ``linear
  arrangement'' in mind and use this option to specify the placement
  of a single child and of two children, then any number of children
  will be placed correctly.

  Here are some arrangements based on this growth function. We start
  with a simple ``above'' arrangement:
\begin{codeexample}[]
\begin{tikzpicture}[grow via three points={%
    one child at (0,1) and two children at (-.5,1) and (.5,1)}]
  \node at (0,0) {one} child;
  \node at (0,-1.5) {two} child child;
  \node at (0,-3) {three} child child child;
  \node at (0,-4.5) {four} child child child child;
\end{tikzpicture}
\end{codeexample}    

  The next arrangement places children above, but ``grows only to the
  right.'' 
\begin{codeexample}[]
\begin{tikzpicture}[grow via three points={%
    one child at (0,1) and two children at (0,1) and (1,1)}]
  \node at (0,0) {one} child;
  \node at (0,-1.5) {two} child child;
  \node at (0,-3) {three} child child child;
  \node at (0,-4.5) {four} child child child child;
\end{tikzpicture}
\end{codeexample}    

  In the final arrangement, the children are placed along a line going
  down and right.
\begin{codeexample}[]
\begin{tikzpicture}[grow via three points={%
    one child at (-1,-.5) and two children at (-1,-.5) and (0,-.75)}]
  \node at (0,0) {one} child;
  \node at (0,-1.5) {two} child child;
  \node at (0,-3) {three} child child child;
  \node at (0,-4.5) {four} child child child child;
\end{tikzpicture}
\end{codeexample}

  These examples should make it clear how you can create new styles to
  arrange your children along a line.
\end{key}

\begin{key}{/tikz/grow cyclic}
  This style causes the children to be arranged ``on a circle.'' For
  this, the children are placed at distance |\tikzleveldistance| from
  the parent node, but not on a straight line, but points on a
  circle. Instead of a sibling distance, there is a |sibling angle|
  that denotes the angle between two given children.
  \begin{key}{/tikz/sibling angle=\meta{angle}}
    Sets the angle between siblings in the |grow cyclic| style.
  \end{key}
  Note that this function will rotate the coordinate system of the
  children to ensure that the grandchildren will grow in the right
  direction.
\begin{codeexample}[]
\begin{tikzpicture}
  [grow cyclic,
   level 1/.style={level distance=8mm,sibling angle=60},
   level 2/.style={level distance=4mm,sibling angle=45},
   level 3/.style={level distance=2mm,sibling angle=30}]
  \coordinate [rotate=-90] % going down
    child foreach \x in {1,2,3}
      {child foreach \x in {1,2,3}
        {child foreach \x in {1,2,3}}};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/clockwise from=\meta{angle}}
  This option also cuases children to be arranged on a
  circle. However, the rule for placing children is simpler than with
  the |grow cyclic| style: The first child is placed at
  \meta{angle} at a distance of |\tikzleveldistance|. The second child
  is placed at the same distance from the parent, but at angle
  \meta{angle}${}-{}$|\tikzsiblingangle|. The third child is displaced
  by another |\tikzsiblingangle| in a clockwise fashion, and so on. 

  Note that this function will not rotate the coordinate system.
\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
  [clockwise from=30,sibling angle=30]
  child {node {$30$}}
  child {node {$0$}}
  child {node {$-30$}}
  child {node {$-60$}};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/counterclockwise from=\meta{angle}}
  Works the same way as |clockwise from|, but sibling angles are added
  instead of subtracted.
\end{key}

\subsection{Edges From Parent}

The following styles can be used to modify how the edges from parents
are drawn:

\begin{stylekey}{/tikz/edge from parent fork down}
  This style will draw a line from the parent downwards (for half the
  level distance) and then on to the child using only horizontal and
  vertical lines. 
\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
    [edge from parent fork down]
    child {node {left}}
    child {node {right}
      child[child anchor=north east] {node {child}}
      child {node {child}}
    };
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/edge from parent fork right}
  This style behaves similarly, only it will first draw its edge to
  the right.
\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
    [edge from parent fork right,grow=right]
    child {node {left}}
    child {node {right}
      child {node {child}}
      child {node {child}}
    };
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/edge from parent fork left}
  Behaves similary to the previous styles.
\end{stylekey}

\begin{stylekey}{/tikz/edge from parent fork up}
  Behaves similary to the previous styles.
\end{stylekey}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-macros.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% $Header: /cvsroot/pgf/pgf/doc/generic/pgf/macros/pgfmanual-en-macros.tex,v 1.28 2008/02/20 11:00:42 tantau Exp $


\providecommand\href[2]{\texttt{#1}}


\colorlet{examplefill}{yellow!80!black}
\definecolor{graphicbackground}{rgb}{0.96,0.96,0.8}
\definecolor{codebackground}{rgb}{0.8,0.8,1}

\newenvironment{pgfmanualentry}{\list{}{\leftmargin=2em\itemindent-\leftmargin\def\makelabel##1{\hss##1}}}{\endlist}
\newcommand\pgfmanualentryheadline[1]{\itemsep=0pt\parskip=0pt\item\strut{#1}\par\topsep=0pt}
\newcommand\pgfmanualbody{\parskip3pt}



\newenvironment{pgflayout}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{\texttt{\string\pgfpagesuselayout\char`\{\declare{#1}\char`\}}\oarg{options}}
    \index{#1@\protect\texttt{#1} layout}%
    \index{Page layouts!#1@\protect\texttt{#1}}%
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}


\newenvironment{command}[1]{
  \begin{pgfmanualentry}
    \extractcommand#1\@@
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

%% MW: START MATH MACROS
\def\mvar#1{{\rmfamily\textit{#1}}}

\makeatletter

\def\extractmathfunctionname#1{\extractmathfunctionname@#1(,)\tmpa\tmpb}
\def\extractmathfunctionname@#1(#2)#3\tmpb{\def\mathname{#1}}

\def\extractmathoperatorname{\begingroup\def\mvar##1{}\def\ {}\extractmathoperatorname@}
\def\extractmathoperatorname@#1{\xdef\mathname{#1}\endgroup}

\makeatother
	
\def\vskipspecial#1{\vskip#1\vskip0em}

\newenvironment{math-function}[1]{
	\begin{pgfmanualentry}
		\extractmathfunctionname{#1}
		\pgfmanualentryheadline{\texttt{#1}}%
		\index{\mathname @\protect\texttt{\mathname} math function}%
		\index{Math functions!\mathname @\protect\texttt{\mathname}}
		\pgfmanualbody
}
{
	\end{pgfmanualentry}\vskipspecial{-3em}
}

\newenvironment{math-operator}[1]{	
	\begin{pgfmanualentry}
		\extractmathoperatorname{#1}
		\pgfmanualentryheadline{\texttt{#1}}%
		\index{\mathname @\protect\texttt{\mathname} math operator}%
		\index{Math operators!\mathname @\protect\texttt{\mathname}}
    	\pgfmanualbody
}
{%
	\end{pgfmanualentry}\vskipspecial{-3em}
}

\newenvironment{math-constant}[1]{
	\begin{pgfmanualentry}
		\pgfmanualentryheadline{\texttt{#1}}%
		\index{#1@\protect\texttt{#1} math constant}%
		\index{Math constants!#1@\protect\texttt{#1}}
		\pgfmanualbody
}
{
	\end{pgfmanualentry}\vskipspecial{-3em}
}
\def\calcname{\textsc{calc}}
%% MW: END MATH MACROS


\def\extractcommand#1#2\@@{%
  \pgfmanualentryheadline{\declare{\texttt{\string#1}}#2}%
  \removeats{#1}%
  \index{\strippedat @\protect\myprintocmmand{\strippedat}}}


\renewenvironment{environment}[1]{
  \begin{pgfmanualentry}
    \extractenvironement#1\@@
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\def\extractenvironement#1#2\@@{%
  \pgfmanualentryheadline{{\ttfamily\char`\\begin\char`\{\declare{#1}\char`\}}#2}%
  \pgfmanualentryheadline{{\ttfamily\ \ }\meta{environment contents}}%
  \pgfmanualentryheadline{{\ttfamily\char`\\end\char`\{\declare{#1}\char`\}}}%
  \index{#1@\protect\texttt{#1} environment}%
  \index{Environments!#1@\protect\texttt{#1}}}


\newenvironment{plainenvironment}[1]{
  \begin{pgfmanualentry}
    \extractplainenvironement#1\@@
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\def\extractplainenvironement#1#2\@@{%
  \pgfmanualentryheadline{{\ttfamily\declare{\char`\\#1}}#2}%
  \pgfmanualentryheadline{{\ttfamily\ \ }\meta{environment contents}}%
  \pgfmanualentryheadline{{\ttfamily\declare{\char`\\end#1}}}%
  \index{#1@\protect\texttt{#1} environment}%
  \index{Environments!#1@\protect\texttt{#1}}}


\newenvironment{contextenvironment}[1]{
  \begin{pgfmanualentry}
    \extractcontextenvironement#1\@@
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\def\extractcontextenvironement#1#2\@@{%
  \pgfmanualentryheadline{{\ttfamily\declare{\char`\\start#1}}#2}%
  \pgfmanualentryheadline{{\ttfamily\ \ }\meta{environment contents}}%
  \pgfmanualentryheadline{{\ttfamily\declare{\char`\\stop#1}}}%
  \index{#1@\protect\texttt{#1} environment}%
  \index{Environments!#1@\protect\texttt{#1}}}


\newenvironment{shape}[1]{
  \begin{pgfmanualentry}
  	\pgfmanualentryheadline{Shape {\ttfamily\declare{#1}}}%
    \index{#1@\protect\texttt{#1} shape}%
    \index{Shapes!#1@\protect\texttt{#1}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}


\newenvironment{handler}[1]{
  \begin{pgfmanualentry}
    \extracthandler#1\@nil%
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\def\gobble#1{}
\def\extracthandler#1#2\@nil{%
  \pgfmanualentryheadline{Key handler \meta{key}{\ttfamily/\declare{#1}}#2}%
  \index{\gobble#1@\protect\texttt{#1} handler}%
  \index{Key handlers!#1@\protect\texttt{#1}}
}


\makeatletter


\newenvironment{stylekey}[1]{
  \begin{pgfmanualentry}
    \def\extrakeytext{style, }
    \extractkey#1\@nil%
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}


\newenvironment{key}[1]{
  \begin{pgfmanualentry}
    \def\extrakeytext{}
    %\def\altpath{\emph{\color{gray}or}}%
    \extractkey#1\@nil%
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\def\extractkey#1\@nil{%
  \pgfutil@in@={#1}%
  \ifpgfutil@in@%
    \extractkeyequal#1\@nil
  \else%
    \pgfutil@in@{(initial}{#1}%
    \ifpgfutil@in@%
      \extractequalinitial#1\@nil%
    \else
      \pgfmanualentryheadline{{\ttfamily\declare{#1}}\hfill(\extrakeytext no value)}%
      \def\mykey{#1}%
      \def\mypath{}%
      \def\myname{}%
      \firsttimetrue%
      \decompose#1/\nil%
    \fi
  \fi%
}

\def\extractkeyequal#1=#2\@nil{%
  \pgfutil@in@{(default}{#2}%
  \ifpgfutil@in@%
    \extractdefault{#1}#2\@nil%
  \else%
    \pgfutil@in@{(initial}{#2}%
    \ifpgfutil@in@%
      \extractinitial{#1}#2\@nil%
    \else
      \pgfmanualentryheadline{{\ttfamily\declare{#1}=}#2\hfill(\extrakeytext no default)}%
    \fi%
  \fi%
  \def\mykey{#1}%
  \def\mypath{}%
  \def\myname{}%
  \firsttimetrue%
  \decompose#1/\nil%
}

\def\extractdefault#1#2(default #3)\@nil{%
  \pgfmanualentryheadline{{\ttfamily\declare{#1}\opt{=}}\opt{#2}\hfill (\extrakeytext default {\ttfamily#3})}%
}

\def\extractinitial#1#2(initially #3)\@nil{%
  \pgfmanualentryheadline{{\ttfamily\declare{#1}=}#2\hfill (\extrakeytext no default, initially {\ttfamily#3})}%
}

\def\extractequalinitial#1 (initially #2)\@nil{%
  \pgfmanualentryheadline{{\ttfamily\declare{#1}}\hfill (\extrakeytext initially {\ttfamily#2})}%
  \def\mykey{#1}%
  \def\mypath{}%
  \def\myname{}%
  \firsttimetrue%
  \decompose#1/\nil%
}

\def\keyalias#1{\vspace{-3pt}\item{\small alias {\ttfamily/#1/\myname}}\vspace{-2pt}\par}

\newif\iffirsttime

\makeatother

\def\decompose/#1/#2\nil{%
  \def\test{#2}%
  \ifx\test\empty%
    % aha.
    \index{#1@\protect\texttt{#1} key}%
    \index{\mypath#1@\protect\texttt{#1}}%
    \def\myname{#1}%
  \else%
    \iffirsttime
      \def\mypath{#1@\protect\texttt{/#1/}!}%
      \firsttimefalse
    \else
      \expandafter\def\expandafter\mypath\expandafter{\mypath#1@\protect\texttt{#1/}!}%
    \fi
    \def\firsttime{}
    \decompose/#2\nil%
  \fi%
}


\newenvironment{predefinednode}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{Predefined node {\ttfamily\declare{#1}}}%
    \index{#1@\protect\texttt{#1} node}%
    \index{Predefined node!#1@\protect\texttt{#1}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\newenvironment{coordinatesystem}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{Coordinate system {\ttfamily\declare{#1}}}%
    \index{#1@\protect\texttt{#1} coordinate system}%
    \index{Coordinate systems!#1@\protect\texttt{#1}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\newenvironment{snake}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{Snake {\ttfamily\declare{#1}}}%
    \index{#1@\protect\texttt{#1} snake}%
    \index{Snakes!#1@\protect\texttt{#1}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\newenvironment{decoration}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{Decoration {\ttfamily\declare{#1}}}%
    \index{#1@\protect\texttt{#1} decoration}%
    \index{Decorations!#1@\protect\texttt{#1}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}


\def\pgfmanualbar{\char`\|}
\makeatletter
\newenvironment{pathoperation}[3][]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{\textcolor{gray}{{\ttfamily\char`\\path}\
        \ \dots}
      \declare{\texttt{#2}}#3\ \textcolor{gray}{\dots\texttt{;}}}%
    \def\pgfmanualtest{#1}%
    \ifx\pgfmanualtest\@empty%
      \index{#2@\protect\texttt{#2} path operation}%
      \index{Path operations!#2@\protect\texttt{#2}}%
    \fi%
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}
\makeatother

\def\extractcommand#1#2\@@{%
  \pgfmanualentryheadline{\declare{\texttt{\string#1}}#2}%
  \removeats{#1}%
  \index{\strippedat @\protect\myprintocmmand{\strippedat}}}

\def\doublebs{\texttt{\char`\\\char`\\}}


\newenvironment{package}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{{\ttfamily\char`\\usepackage\char`\{\declare{#1}\char`\}\space\space \char`\%\space\space  \LaTeX}}
    \index{#1@\protect\texttt{#1} package}%
    \index{Packages and files!#1@\protect\texttt{#1}}%
    \pgfmanualentryheadline{{\ttfamily\char`\\input \declare{#1}.tex\space\space\space \char`\%\space\space  plain \TeX}}
    \pgfmanualentryheadline{{\ttfamily\char`\\usemodule[\declare{#1}]\space\space \char`\%\space\space  Con\TeX t}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}


\newenvironment{pgfmodule}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{{\ttfamily\char`\\usepgfmodule\char`\{\declare{#1}\char`\}\space\space\space
        \char`\%\space\space  \LaTeX\space and plain \TeX\space and pure pgf}}
    \index{#1@\protect\texttt{#1} module}%
    \index{Modules!#1@\protect\texttt{#1}}%
    \pgfmanualentryheadline{{\ttfamily\char`\\usepgfmodule[\declare{#1}]\space\space \char`\%\space\space  Con\TeX t\space and pure pgf}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\newenvironment{pgflibrary}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{{\ttfamily\char`\\usepgflibrary\char`\{\declare{#1}\char`\}\space\space\space
        \char`\%\space\space  \LaTeX\space and plain \TeX\space and pure pgf}}
    \index{#1@\protect\texttt{#1} library}%
    \index{Libraries!#1@\protect\texttt{#1}}%
    \pgfmanualentryheadline{{\ttfamily\char`\\usepgflibrary[\declare{#1}]\space\space \char`\%\space\space  Con\TeX t\space and pure pgf}}
    \pgfmanualentryheadline{{\ttfamily\char`\\usetikzlibrary\char`\{\declare{#1}\char`\}\space\space
        \char`\%\space\space  \LaTeX\space and plain \TeX\space when using \tikzname}}
    \pgfmanualentryheadline{{\ttfamily\char`\\usetikzlibrary[\declare{#1}]\space
        \char`\%\space\space  Con\TeX t\space when using \tikzname}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}

\newenvironment{tikzlibrary}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{{\ttfamily\char`\\usetikzlibrary\char`\{\declare{#1}\char`\}\space\space \char`\%\space\space  \LaTeX\space and plain \TeX}}
    \index{#1@\protect\texttt{#1} library}%
    \index{Libraries!#1@\protect\texttt{#1}}%
    \pgfmanualentryheadline{{\ttfamily\char`\\usetikzlibrary[\declare{#1}]\space \char`\%\space\space Con\TeX t}}
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}



\newenvironment{filedescription}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{File {\ttfamily\declare{#1}}}%
    \index{#1@\protect\texttt{#1} file}%
    \index{Packages and files!#1@\protect\texttt{#1}}%
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}


\newenvironment{packageoption}[1]{
  \begin{pgfmanualentry}
    \pgfmanualentryheadline{{\ttfamily\char`\\usepackage[\declare{#1}]\char`\{pgf\char`\}}}
    \index{#1@\protect\texttt{#1} package option}%
    \index{Package options for \textsc{pgf}!#1@\protect\texttt{#1}}%
    \pgfmanualbody
}
{
  \end{pgfmanualentry}
}



\newcommand\opt[1]{{\color{black!50!green}#1}}
\newcommand\ooarg[1]{{\ttfamily[}\meta{#1}{\ttfamily]}}

\def\opt{\afterassignment\pgfmanualopt\let\next=}
\def\pgfmanualopt{\ifx\next\bgroup\bgroup\color{black!50!green}\else{\color{black!50!green}\next}\fi}



\def\beamer{\textsc{beamer}}
\def\pdf{\textsc{pdf}}
\def\pgfname{\textsc{pgf}}
\def\tikzname{Ti\emph{k}Z}
\def\pstricks{\textsc{pstricks}}
\def\prosper{\textsc{prosper}}
\def\seminar{\textsc{seminar}}
\def\texpower{\textsc{texpower}}
\def\foils{\textsc{foils}}

{
  \makeatletter
  \global\let\myempty=\@empty
  \global\let\mygobble=\@gobble
  \catcode`\@=12
  \gdef\getridofats#1@#2\relax{%
    \def\getridtest{#2}%
    \ifx\getridtest\myempty%
      \expandafter\def\expandafter\strippedat\expandafter{\strippedat#1}
    \else%
      \expandafter\def\expandafter\strippedat\expandafter{\strippedat#1\protect\printanat}
      \getridofats#2\relax%
    \fi%
  }

  \gdef\removeats#1{%
    \let\strippedat\myempty%
    \edef\strippedtext{\stripcommand#1}%
    \expandafter\getridofats\strippedtext @\relax%
  }
  
  \gdef\stripcommand#1{\expandafter\mygobble\string#1}
}

\def\printanat{\char`\@}

\def\declare{\afterassignment\pgfmanualdeclare\let\next=}
\def\pgfmanualdeclare{\ifx\next\bgroup\bgroup\color{red!75!black}\else{\color{red!75!black}\next}\fi}


\let\textoken=\command
\let\endtextoken=\endcommand

\def\myprintocmmand#1{\texttt{\char`\\#1}}

\def\example{\par\smallskip\noindent\textit{Example: }}
\def\themeauthor{\par\smallskip\noindent\textit{Theme author: }}


\def\indexoption#1{%
  \index{#1@\protect\texttt{#1} option}%
  \index{Graphic options and styles!#1@\protect\texttt{#1}}%
}

\def\itemcalendaroption#1{\item \declare{\texttt{#1}}%
  \index{#1@\protect\texttt{#1} date test}%
  \index{Date tests!#1@\protect\texttt{#1}}%
}



\def\class#1{\list{}{\leftmargin=2em\itemindent-\leftmargin\def\makelabel##1{\hss##1}}%
\extractclass#1@\par\topsep=0pt}
\def\endclass{\endlist}
\def\extractclass#1#2@{%
\item{{{\ttfamily\char`\\documentclass}#2{\ttfamily\char`\{\declare{#1}\char`\}}}}%
  \index{#1@\protect\texttt{#1} class}%
  \index{Classes!#1@\protect\texttt{#1}}}

\def\partname{Part}

\makeatletter
\def\index@prologue{\section*{Index}\addcontentsline{toc}{section}{Index}
  This index only contains automatically generated entries. A good
  index should also contain carefully selected keywords. This index is
  not a good index.
  \bigskip
}
\c@IndexColumns=2
  \def\theindex{\@restonecoltrue
    \columnseprule \z@  \columnsep 29\p@
    \twocolumn[\index@prologue]%
       \parindent -30pt
       \columnsep 15pt
       \parskip 0pt plus 1pt
       \leftskip 30pt
       \rightskip 0pt plus 2cm
       \small
       \def\@idxitem{\par}%
    \let\item\@idxitem \ignorespaces}
  \def\endtheindex{\onecolumn}
\def\noindexing{\let\index=\@gobble}



\newcommand\symarrow[1]{
  \index{#1@\protect\texttt{#1} arrow tip}%
  \index{Arrow tips!#1@\protect\texttt{#1}}
  \texttt{#1}& yields thick  
  \begin{tikzpicture}[arrows={#1-#1},thick,baseline]
    \useasboundingbox (0pt,-0.5ex) rectangle (1cm,2ex);
    \draw (0pt,.5ex) -- (1cm,.5ex);
  \end{tikzpicture} and thin
  \begin{tikzpicture}[arrows={#1-#1},thin,baseline]
    \useasboundingbox (0pt,-0.5ex) rectangle (1cm,2ex);
    \draw (0pt,.5ex) -- (1cm,.5ex);
  \end{tikzpicture}
}

\newcommand\sarrow[2]{
  \index{#1@\protect\texttt{#1} arrow tip}%
  \index{Arrow tips!#1@\protect\texttt{#1}}
  \index{#2@\protect\texttt{#2} arrow tip}%
  \index{Arrow tips!#2@\protect\texttt{#2}}
  \texttt{#1-#2}& yields thick  
  \begin{tikzpicture}[arrows={#1-#2},thick,baseline]
    \useasboundingbox (0pt,-0.5ex) rectangle (1cm,2ex);
    \draw (0pt,.5ex) -- (1cm,.5ex);
  \end{tikzpicture} and thin
  \begin{tikzpicture}[arrows={#1-#2},thin,baseline]
    \useasboundingbox (0pt,-0.5ex) rectangle (1cm,2ex);
    \draw (0pt,.5ex) -- (1cm,.5ex);
  \end{tikzpicture}
}

\newcommand\carrow[1]{
  \index{#1@\protect\texttt{#1} arrow tip}%
  \index{Arrow tips!#1@\protect\texttt{#1}}
  \texttt{#1}& yields for line width 1ex
  \begin{tikzpicture}[arrows={#1-#1},line width=1ex,baseline]
    \useasboundingbox (0pt,-0.5ex) rectangle (1.5cm,2ex);
    \draw (0pt,.5ex) -- (1.5cm,.5ex);
  \end{tikzpicture}
}
\def\myvbar{\char`\|}
\newcommand\plotmarkentry[1]{%
  \index{#1@\protect\texttt{#1} plot mark}%
  \index{Plot marks!#1@\protect\texttt{#1}}
  \texttt{\char`\\pgfuseplotmark\char`\{\declare{#1}\char`\}} &
  \tikz\draw[color=black!25] plot[mark=#1,mark options={fill=examplefill,draw=black}] coordinates{(0,0) (.5,0.2) (1,0) (1.5,0.2)};\\
}
\newcommand\plotmarkentrytikz[1]{%
  \index{#1@\protect\texttt{#1} plot mark}%
  \index{Plot marks!#1@\protect\texttt{#1}}
  \texttt{mark=\declare{#1}} & \tikz\draw[color=black!25]
  plot[mark=#1,mark options={fill=examplefill,draw=black}] 
    coordinates {(0,0) (.5,0.2) (1,0) (1.5,0.2)};\\
}



\ifx\scantokens\@undefined
  \PackageError{pgfmanual-macros}{You need to use extended latex
    (elatex) or (pdfelatex) to process this document}{}
\fi

\begingroup
\catcode`|=0
\catcode`[= 1
\catcode`]=2
\catcode`\{=12
\catcode `\}=12
\catcode`\\=12 |gdef|find@example#1\end{codeexample}[|endofcodeexample[#1]]
|endgroup

\begingroup
\catcode`\^=7
\catcode`\^^M=13
\catcode`\ =13%
\gdef\returntospace{\catcode`\ =13\def {\space}\catcode`\^^M=13\def^^M{}}%
\endgroup

\begingroup
\catcode`\%=13
\catcode`\^^M=13
\gdef\commenthandler{\catcode`\%=13\def%{\@gobble@till@return}}
\gdef\@gobble@till@return#1^^M{}
\gdef\@gobble@till@return@ignore#1^^M{\ignorespaces}
\gdef\typesetcomment{\catcode`\%=13\def%{\@typeset@till@return}}
\gdef\@typeset@till@return#1^^M{{\def%{\char`\%}\textsl{\char`\%#1}}\par}
\endgroup

\define@key{codeexample}{width}{\setlength\codeexamplewidth{#1}}
\define@key{codeexample}{graphic}{\colorlet{graphicbackground}{#1}}
\define@key{codeexample}{code}{\colorlet{codebackground}{#1}}
\define@key{codeexample}{execute code}{\csname code@execute#1\endcsname}
\define@key{codeexample}{code only}[]{\code@executefalse}
\define@key{codeexample}{pre}{\def\code@pre{#1}}
\define@key{codeexample}{post}{\def\code@post{#1}}
\define@key{codeexample}{vbox}[]{\def\code@pre{\vbox\bgroup\setlength{\hsize}{\linewidth-6pt}}\def\code@post{\egroup}}
\define@key{codeexample}{ignorespaces}[]{\let\@gobble@till@return=\@gobble@till@return@ignore}
\define@key{codeexample}{leave comments}[]{\def\code@catcode@hook{\catcode`\%=12}\let\commenthandler=\relax\let\typesetcomment=\relax}

\def\code@pre{}
\def\code@post{}
\def\code@catcode@hook{}

\newdimen\codeexamplewidth
\newif\ifcode@execute
\newbox\codeexamplebox
\def\codeexample[#1]{%
  \begingroup%
  \code@executetrue
  \setlength\codeexamplewidth{4cm+7pt}
  \setkeys{codeexample}{#1}%
  \parindent0pt
  \begingroup%
  \par%
  \medskip%
  \let\do\@makeother%
  \dospecials%
  \obeylines%
  \@vobeyspaces%
  \catcode`\%=13%
  \catcode`\^^M=13%
  \code@catcode@hook%
  \relax%
  \find@example}
\def\endofcodeexample#1{%
  \endgroup%
  \ifcode@execute%
    \setbox\codeexamplebox=\hbox{%
      {%
        {%
          \returntospace%
          \commenthandler%
          \xdef\code@temp{#1}% removes returns and comments
        }%
        \colorbox{graphicbackground}{\color{black}\ignorespaces%
          \code@pre\expandafter\scantokens\expandafter{\code@temp\ignorespaces}\code@post\ignorespaces}%
      }%
    }%
    \ifdim\wd\codeexamplebox>\codeexamplewidth%
      \def\code@start{\par}%
      \def\code@flushstart{}\def\code@flushend{}%
      \def\code@mid{\parskip2pt\par\noindent}%
      \def\code@width{\linewidth-6pt}%
      \def\code@end{}%
    \else%
      \def\code@start{%
        \linewidth=\textwidth%
        \parshape \@ne 0pt \linewidth
        \leavevmode%
        \hbox\bgroup}%
      \def\code@flushstart{\hfill}%
      \def\code@flushend{\hbox{}}%
      \def\code@mid{\hskip6pt}%
      \def\code@width{\linewidth-12pt-\codeexamplewidth}%
      \def\code@end{\egroup}%
    \fi%
    \code@start%
    \noindent%
    \begin{minipage}[t]{\codeexamplewidth}\raggedright
      \hrule width0pt%
      \footnotesize\vskip-1em%
      \code@flushstart\box\codeexamplebox\code@flushend%
      \vskip-1ex
      \leavevmode%
    \end{minipage}%
  \else%
    \def\code@mid{\par}
    \def\code@width{\linewidth-6pt}
    \def\code@end{}
  \fi%
  \code@mid%  
  \colorbox{codebackground}{%
    \begin{minipage}[t]{\code@width}%
      {%
        \let\do\@makeother
        \dospecials
        \frenchspacing\@vobeyspaces
        \normalfont\ttfamily\footnotesize
        \typesetcomment%
        \@tempswafalse
        \def\par{%
          \if@tempswa
          \leavevmode \null \@@par\penalty\interlinepenalty
          \else
          \@tempswatrue
          \ifhmode\@@par\penalty\interlinepenalty\fi
          \fi}%
        \obeylines
        \everypar \expandafter{\the\everypar \unpenalty}%
        #1}
    \end{minipage}}%
  \code@end%
  \par%
  \medskip
  \end{codeexample}
}

\def\endcodeexample{\endgroup}


\makeatother


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "beameruserguide"
%%% End: 


==> pgfmanual-en-main.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% pgf version is defined in \pgfversion in file
% generic/pgf/utilities/pgfrcs.code.tex 

\def\xcolorversion{2.00}

\usepackage[version=latest]{pgf}

\usepackage{xkeyval,calc,listings,tikz}

% We need lots of libraries...
\usetikzlibrary{%
  arrows,%
  calc,%
  fit,%
  patterns,%
  plotmarks,%
  shapes.geometric,%
  shapes.misc,%
  shapes.symbols,%
  shapes.arrows,%
  shapes.callouts,%
  shapes.multipart,%
  shapes.gates.logic.US,%
  shapes.gates.logic.IEC,%
  er,%
  automata,%
  backgrounds,%
  chains,%
  topaths,%
  trees,%
  petri,%
  mindmap,%
  matrix,%
  calendar,%
  folding,%
  fadings,%
  through,%
  positioning,%
  scopes,%
  decorations.fractals,%
  decorations.shapes,%
  decorations.text,%
  decorations.pathmorphing,%
  decorations.pathreplacing,%
  decorations.footprints,%
  decorations.markings,%
  shadows}

\usepackage[a4paper,left=2.25cm,right=2.25cm,top=2.5cm,bottom=2.5cm,nohead]{geometry}
\usepackage{amsmath,amssymb}
\usepackage{xxcolor}
\usepackage{pifont}
\usepackage{makeidx}
\usepackage[latin1]{inputenc}
\usepackage{amsmath}

\input{../../macros/pgfmanual-en-macros}

\makeindex

\makeatletter
\renewcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.8em}}
\renewcommand*\l@subsubsection{\@dottedtocline{3}{4.3em}{3.2em}}
\makeatother

%\includeonly{}

% Global styles:
\tikzset{
  every plot/.style={prefix=plots/pgf-},
  shape example/.style={
    color=black!30,
    draw,
    fill=yellow!30,
    line width=.5cm,
    inner xsep=2.5cm,
    inner ysep=0.5cm}
}

\index{Options for graphics|see{Graphic options and styles}}
\index{Styles for graphics|see{Graphic options and styles}}
\index{Options for packages|see{Package options}}
\index{Handlers for keys|see{Key handlers}}
\index{File|see{Packages and files}}
\index{Layout|see{Page layout}}
\index{Node|see{Predefined node}}

\begin{document}

%\include{pgfmanual-en-base-decorations}
%\end{document}



% The titlepage

{
  \parindent0pt
  \null
  \colorlet{mintgreen}{green!50!black!50}
  
  \thispagestyle{empty}
  \vskip3cm
  \vfill
  \hfil
  \begin{tikzpicture}[overlay]
    \coordinate (front) at (0,0);
    \coordinate (horizon) at (0,.31\paperheight);
    \coordinate (bottom) at (0,-.6\paperheight);
    \coordinate (sky) at (0,.57\paperheight);
    \coordinate (left) at (-.51\paperwidth,0);
    \coordinate (right) at (.51\paperwidth,0);
    
    \shade [bottom color=blue!30!black!10,top color=blue!30!black!50]
      ([yshift=-5mm]horizon -|  left) rectangle (sky -| right);
    \shade [bottom color=black!70!green!25,top color=black!70!green!10]
      (front -| left) -- (horizon -| left)
      decorate [decoration=random steps] { -- (horizon -| right) }
      -- (front -| right) -- cycle;
    \shade [top color=black!70!green!25,bottom color=black!25]
      ([yshift=-5mm-1pt]front -| left) rectangle ([yshift=1pt]front -| right);
    \fill [black!25] (bottom -| left) rectangle ([yshift=-5mm]front -| right);

    \def\nodeshadowed[#1]#2;{\node[scale=2,above,#1]{#2};\node[scale=2,above,#1,yscale=-1,scope fading=south,opacity=0.4]{#2};}

    \nodeshadowed [at={(-5,5  )},yslant=0.05] {\Huge Ti\textcolor{orange}{\emph{k}}Z};
    \nodeshadowed [at={( 0,5.3)}] {\huge \textcolor{mintgreen}{\&}};
    \nodeshadowed [at={( 5,5  )},yslant=-0.05] {\Huge \textsc{PGF}};
    \nodeshadowed [at={( 0,2  )}] {Manual for Version \pgftypesetversion};

    \foreach \i in {0.5,0.6,...,2}
      \fill [white,decoration=Koch snowflake,opacity=.9]
            [shift=(horizon),shift={(rand*11,rnd*7)},scale=\i]
            [double copy shadow={opacity=0.2,shadow xshift=0pt,shadow
              yshift=3*\i pt,fill=white,draw=none}]
        decorate { 
          decorate { 
            decorate {
              (0,0) -- ++(60:1) -- ++(-60:1) -- cycle
            }
          }
        };

  \node (left text) [text width=.5\paperwidth-2cm,below right,at={(-.5\paperwidth+1cm,-1.5cm)}]
  {
    \fontfamily{pcr}
    \def\textbraceleft{\char`\{}
    \def\textbraceright{\char`\}}
    \def\textbackslash{\char`\\}
    \begin{lstlisting}[basicstyle=\scriptsize\color{black},
                       keywordstyle=\bfseries\color{white},
                       identifierstyle=\bfseries\color{black},
                       keywords={tikzpicture,shade,fill,draw,path,node},
                       literate={-}{{-}}1]
\begin{tikzpicture}
  \coordinate (front) at (0,0);
  \coordinate (horizon) at (0,.31\paperheight);
  \coordinate (bottom) at (0,-.6\paperheight);
  \coordinate (sky) at (0,.57\paperheight);
  \coordinate (left) at (-.51\paperwidth,0);
  \coordinate (right) at (.51\paperwidth,0);
    
  \shade [bottom color=white,
          top color=blue!30!black!50]
              ([yshift=-5mm]horizon -|  left)
    rectangle (sky -| right);
  
  \shade [bottom color=black!70!green!25,
          top color=black!70!green!10]
    (front -| left) -- (horizon -| left)
    decorate [decoration=random steps] {
      -- (horizon -| right)  }
    -- (front -| right) -- cycle;
    
  \shade [top color=black!70!green!25,
         bottom color=black!25]
              ([yshift=-5mm-1pt]front -| left)
    rectangle ([yshift=1pt]front -| right);

  \fill [black!25]
              (bottom -| left)
    rectangle ([yshift=-5mm]front -| right);
 
  \def\nodeshadowed[#1]#2;{
    \node[scale=2,above,#1]{#2};
    \node[scale=2,above,#1,yscale=-1,
          scope fading=south,opacity=0.4]{#2};
  }
\end{lstlisting}
};

  \node (right text) [text width=.5\paperwidth-2cm,below right,at={(1cm,-1.5cm)}]
  {
    \fontfamily{pcr}
    \def\textbraceleft{\char`\{}
    \def\textbraceright{\char`\}}
    \def\textbackslash{\char`\\}
    \begin{lstlisting}[basicstyle=\scriptsize\color{black},
                       keywordstyle=\bfseries\color{white},
                       identifierstyle=\bfseries\color{black},
                       keywords={tikzpicture,shade,fill,draw,path,node},
                       literate={-}{{-}}1]
  \nodeshadowed [at={(-5,8  )},yslant=0.05]
    {\Huge Ti\textcolor{orange}{\emph{k}}Z};
  \nodeshadowed [at={( 0,8.3)}]
    {\huge \textcolor{green!50!black!50}{\&}};
  \nodeshadowed [at={( 5,8  )},yslant=-0.05]
    {\Huge \textsc{PGF}};
  \nodeshadowed [at={( 0,5  )}]
    {Manual for Version \pgftypesetversion};

  \foreach \i in {0.5,0.6,...,2}
    \fill
      [white,opacity=\i/2,
       decoration=Koch snowflake,
       shift=(horizon),shift={(rand*11,rnd*7)},
       scale=\i,double copy shadow={
         opacity=0.2,shadow xshift=0pt,
         shadow yshift=3*\i pt,
         fill=white,draw=none}]
      decorate {
        decorate { 
          decorate { 
            (0,0)- ++(60:1) -- ++(-60:1) -- cycle
          } } };

   \node (left text) ...
   \node (right text) ...

   \fill [decorate,
          decoration={footprints,foot of=gnome},
          opacity=.5,brown] (left text.south)
     to [out=-45,in=135]    (right text.north);
   \fill [decorate,
     decoration={footprints,foot of=felis silvestris,
       foot length=5pt,stride length=15pt,foot angle=0},
     opacity=.5,green!50!black] (left text.south)
    to [out=20,in=180] (right text.north west);
\end{tikzpicture}
  \end{lstlisting}
  };

  \fill [decorate,decoration=footprints,
         decoration={footprints,foot of=gnome},
         opacity=.5,brown] (left text.south)
    to [out=-45,in=135]    (right text.north);
  \fill [decorate,decoration={footprints,foot length=5pt,foot of=felis
    silvestris,stride  length=15pt,foot angle=0},
     opacity=.5,green!50!black] (left text.south)
    to [out=20,in=180] (right text.north west);
\end{tikzpicture}
\vfill
\vbox{}
\clearpage
}

{
  \vbox{}
  \vskip0pt plus 1fill
  Für meinen Vater, damit er noch viele schöne \TeX-Graphiken
  erschaffen kann.
  \vskip1em
  \hfill\emph{Till}
  \vskip0pt plus 3fill

  \parindent=0pt
  Copyright 2007 by Till Tantau

  \medskip  
  Permission is granted to copy, distribute and/or modify \emph{the documentation}
  under the terms of the \textsc{gnu} Free Documentation License, Version 1.2
  or any later version published by the Free Software Foundation;
  with no Invariant Sections, no Front-Cover Texts, and no Back-Cover Texts.
  A copy of the license is included in the section entitled \textsc{gnu}
  Free Documentation License.

  \medskip  
  Permission is granted to copy, distribute and/or modify \emph{the
    code of the package} under the terms of the \textsc{gnu} Public License, Version 2
  or any later version published by the Free Software Foundation.
  A copy of the license is included in the section entitled \textsc{gnu}
  Public License.

  \medskip  
  Permission is also granted to distribute and/or modify \emph{both
    the documentation and the code} under the conditions of the LaTeX
  Project Public License, either version 1.3 of this license or (at
  your option) any later version. A copy of the license is included in
  the section entitled \LaTeX\ Project Public License. 

  \vbox{}
  \clearpage
}


\title{\bfseries The \tikzname\ and {\Large PGF} Packages\\
  \large Manual for version \pgfversion\\[1mm]
\large\href{http://sourceforge.net/projects/pgf}{\texttt{http://sourceforge.net/projects/pgf}}}
\author{Till Tantau\footnote{Editor of this documentation. Parts of
    this documentation have been written by other authors as indicated
    in these parts or chapters and in Section~\ref{section-authors}.}\\
  \normalsize Institut f\"ur Theoretische Informatik\\[-1mm]
  \normalsize Universit\"at zu L\"ubeck}

\maketitle

\tableofcontents

\clearpage


\include{pgfmanual-en-introduction}


\part{Tutorials and Guidelines}

{\Large \emph{by Till Tantau}}

\bigskip
\noindent
To help you get started with \tikzname, instead of a long installation
and configuration section, this manual starts with tutorials. They
explain all the basic and some of the more advanced features of the
system, without going into all the details. This part also contains
some guidelines on how you should proceed when creating graphics using
\tikzname. 

\vskip3cm

\begin{codeexample}[graphic=white,width=0pt]
\tikz \draw[thick,rounded corners=8pt]
  (0,0) -- (0,2) -- (1,3.25) -- (2,2) -- (2,0) -- (0,2) -- (2,2) -- (0,0) -- (2,0);
\end{codeexample}

\include{pgfmanual-en-tutorial}
\include{pgfmanual-en-tutorial-nodes}
\include{pgfmanual-en-tutorial-Euclid}
\include{pgfmanual-en-tutorial-chains}
\include{pgfmanual-en-guidelines}



\part{Installation and Configuration}

{\Large \emph{by Till Tantau}}


\bigskip
\noindent
This part explains how the system is installed. Typically, someone has
already done so for your system, so this part can be skipped; but if
this is not the case and you are the poor fellow who has to do the
installation, read the present part. 


\vskip1cm

\begin{codeexample}[graphic=white]
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm,on grid,semithick,
                    every state/.style={fill=red,draw=none,circular drop shadow,text=white}]

  \node[initial,state] (A)                    {$q_a$};
  \node[state]         (B) [above right=of A] {$q_b$};
  \node[state]         (D) [below right=of A] {$q_d$};
  \node[state]         (C) [below right=of B] {$q_c$};
  \node[state]         (E) [below=of D]       {$q_e$};

  \path (A) edge              node {0,1,L} (B)
            edge              node {1,1,R} (C)
        (B) edge [loop above] node {1,1,L} (B)  
            edge              node {0,1,L} (C)
        (C) edge              node {0,1,L} (D)
            edge [bend left]  node {1,0,R} (E)    
        (D) edge [loop below] node {1,1,R} (D)
            edge              node {0,1,R} (A)
        (E) edge [bend left]  node {1,0,R} (A);

   \node [right=1cm,text width=8cm] at (C)
   {
     The current candidate for the busy beaver for five states. It is
     presumed that this Turing machine writes a maximum number of
     $1$'s before halting among all Turing machines with five states
     and the tape alphabet $\{0, 1\}$. Proving this conjecture is an
     open research problem.
   };
\end{tikzpicture}
\end{codeexample}

\include{pgfmanual-en-installation}
\include{pgfmanual-en-license}
\include{pgfmanual-en-drivers}


\part{Ti\emph{k}Z ist \emph{kein} Zeichenprogramm}
\label{part-tikz}

{\Large \emph{by Till Tantau}}


\bigskip
\noindent
\vskip3cm
\begin{codeexample}[graphic=white]
\begin{tikzpicture}
  \draw[fill=yellow] (0,0) -- (60:.75cm) arc (60:180:.75cm);
  \draw(120:0.4cm) node {$\alpha$};

  \draw[fill=green!30] (0,0) -- (right:.75cm) arc (0:60:.75cm);
  \draw(30:0.5cm) node {$\beta$};

  \begin{scope}[shift={(60:2cm)}]
    \draw[fill=green!30] (0,0) -- (180:.75cm) arc (180:240:.75cm);
    \draw (30:-0.5cm) node {$\gamma$};

    \draw[fill=yellow] (0,0) -- (240:.75cm) arc (240:360:.75cm);
    \draw (-60:0.4cm) node {$\delta$};
  \end{scope}

  \begin{scope}[thick]
    \draw  (60:-1cm) node[fill=white] {$E$} -- (60:3cm) node[fill=white] {$F$};
    \draw[red]                   (-2,0) node[left] {$A$} -- (3,0) node[right]{$B$};
    \draw[blue,shift={(60:2cm)}] (-3,0) node[left] {$C$} -- (2,0) node[right]{$D$};
  
    \draw[shift={(60:1cm)},xshift=4cm]
    node [right,text width=6cm,rounded corners,fill=red!20,inner sep=1ex]
    {
      When we assume that $\color{red}AB$ and $\color{blue}CD$ are
      parallel, i.\,e., ${\color{red}AB} \mathbin{\|} \color{blue}CD$,
      then $\alpha = \delta$ and $\beta = \gamma$.
    };
  \end{scope}
\end{tikzpicture}
\end{codeexample}



\include{pgfmanual-en-tikz-design}
\include{pgfmanual-en-tikz-scopes}
\include{pgfmanual-en-tikz-coordinates}
\include{pgfmanual-en-tikz-paths}
\include{pgfmanual-en-tikz-actions}
\include{pgfmanual-en-tikz-shapes}
\include{pgfmanual-en-tikz-matrices}
\include{pgfmanual-en-tikz-trees}
\include{pgfmanual-en-tikz-plots}
\include{pgfmanual-en-tikz-transparency}
\include{pgfmanual-en-tikz-decorations}
\include{pgfmanual-en-tikz-transformations}



\part{Libraries}
\label{part-libraries}

{\Large \emph{by Till Tantau}}


\bigskip
\noindent
In this part the library packages are documented. They
provide additional predefined graphic objects like new arrow heads or
new plot marks, but also sometimes extensions of the basic \pgfname\
or \tikzname\ system. The libraries are not loaded by default since
many users will not need them.  

\medskip
\noindent
\begin{codeexample}[graphic=white]
\tikzset{
  ld/.style={level distance=#1},lw/.style={line width=#1},  
  level 1/.style={ld=4.5mm, trunk,          lw=1ex ,sibling angle=60},
  level 2/.style={ld=3.5mm, trunk!80!leaf a,lw=.8ex,sibling angle=56},
  level 3/.style={ld=2.75mm,trunk!60!leaf a,lw=.6ex,sibling angle=52},
  level 4/.style={ld=2mm,   trunk!40!leaf a,lw=.4ex,sibling angle=48},
  level 5/.style={ld=1mm,   trunk!20!leaf a,lw=.3ex,sibling angle=44},
  level 6/.style={ld=1.75mm,leaf a,         lw=.2ex,sibling angle=40},
}
\pgfarrowsdeclare{leaf}{leaf}
  {\pgfarrowsleftextend{-2pt} \pgfarrowsrightextend{1pt}}
{
  \pgfpathmoveto{\pgfpoint{-2pt}{0pt}}
  \pgfpatharc{150}{30}{1.8pt}
  \pgfpatharc{-30}{-150}{1.8pt}    
  \pgfusepathqfill
}

\newcommand{\logo}[5]
{
  \colorlet{border}{#1}
  \colorlet{trunk}{#2}
  \colorlet{leaf a}{#3}
  \colorlet{leaf b}{#4}
  \begin{tikzpicture}
    \scriptsize\scshape
    \draw[border,line width=1ex,yshift=.3cm,
          yscale=1.45,xscale=1.05,looseness=1.42]
      (1,0) to [out=90, in=0]    (0,1)  to [out=180,in=90]  (-1,0)
            to [out=-90,in=-180] (0,-1) to [out=0,  in=-90] (1,0) -- cycle;

    \coordinate (root) [grow cyclic,rotate=90]
    child {
      child [line cap=round] foreach \a in {0,1} {
        child foreach \b in {0,1} {
          child foreach \c in {0,1} {
            child foreach \d in {0,1} {
              child foreach \leafcolor in {leaf a,leaf b}
                { edge from parent [color=\leafcolor,-#5] }
        } } }
      } edge from parent [shorten >=-1pt,serif cm-,line cap=butt]
    };

    \node [text centered,text width=2cm,below] at (0pt,-.5ex)
    { \textcolor{border}{T}heoretical \\ \textcolor{border}{C}omputer \\
      \textcolor{border}{S}cience };
  \end{tikzpicture}
}
\begin{minipage}{3cm}
  \logo{green!80!black}{green!25!black}{green}{green!80}{leaf}\\
  \logo{green!50!black}{black}{green!80!black}{red!80!green}{leaf}\\
  \logo{red!75!black}{red!25!black}{red!75!black}{orange}{leaf}\\
  \logo{black!50}{black}{black!50}{black!25}{}
\end{minipage}
\end{codeexample}

\include{pgfmanual-en-library-arrows}
\include{pgfmanual-en-library-automata}
\include{pgfmanual-en-library-backgrounds}
\include{pgfmanual-en-library-calendar}
\include{pgfmanual-en-library-chains}
\include{pgfmanual-en-library-decorations}
\include{pgfmanual-en-library-er}
\include{pgfmanual-en-library-fadings}
\include{pgfmanual-en-library-fit}
\include{pgfmanual-en-library-matrices}
\include{pgfmanual-en-library-mindmaps}
\include{pgfmanual-en-library-folding}
\include{pgfmanual-en-library-patterns}
\include{pgfmanual-en-library-petri}
\include{pgfmanual-en-library-plot-handlers}
\include{pgfmanual-en-library-plot-marks}
\include{pgfmanual-en-library-shadows}
\include{pgfmanual-en-library-shapes}
%\include{pgfmanual-en-library-3d}
\include{pgfmanual-en-library-edges}
\include{pgfmanual-en-library-through}
\include{pgfmanual-en-library-trees}




\part{Utilities}
\label{part-utilities}

{\Large \emph{by Till Tantau}}


\bigskip
\noindent
The utility packages are not directly involved in creating graphics,
but you may find them useful nonetheless. All of them either directly
depend on \pgfname\ or they are designed to work well together with
\pgfname\ even though they can be used in a stand-alone way.

\vskip2cm
\medskip
\noindent
\begin{codeexample}[graphic=white]
\begin{tikzpicture}[scale=2]
  \shade[top color=blue,bottom color=gray!50] (0,0) parabola (1.5,2.25) |- (0,0);
  \draw (1.05cm,2pt) node[above] {$\displaystyle\int_0^{3/2} \!\!x^2\mathrm{d}x$};
  
  \draw[help lines] (0,0) grid (3.9,3.9)
       [step=0.25cm]      (1,2) grid +(1,1);

  \draw[->] (-0.2,0) -- (4,0) node[right] {$x$};
  \draw[->] (0,-0.2) -- (0,4) node[above] {$f(x)$};

  \foreach \x/\xtext in {1/1, 1.5/1\frac{1}{2}, 2/2, 3/3}
    \draw[shift={(\x,0)}] (0pt,2pt) -- (0pt,-2pt) node[below] {$\xtext$};

  \foreach \y/\ytext in {1/1, 2/2, 2.25/2\frac{1}{4}, 3/3}
    \draw[shift={(0,\y)}] (2pt,0pt) -- (-2pt,0pt) node[left] {$\ytext$};
    
  \draw (-.5,.25) parabola bend (0,0) (2,4) node[below right] {$x^2$};
\end{tikzpicture}
\end{codeexample}

\include{pgfmanual-en-pgfkeys}
\include{pgfmanual-en-pgffor}
\include{pgfmanual-en-pgfcalendar}
\include{pgfmanual-en-pages}
\include{pgfmanual-en-xxcolor}


\part{Mathematical Engine}

{\Large \emph{by Mark Wibrow and Till Tantau}}


\bigskip
\noindent
\pgfname\ comes with its own mathematical engine. The job of this
engine is to support mathematical operations like addition,
subtraction, multiplication and division, using both integers and 
non-integers, but also functions such as square-roots, sine, cosine,
and generate pseudo-random numbers.

Mostly, you will use the mathematical facilities of \pgfname\
indirectly, namely when you write a coordinate like |(5cm*3,6cm/4)|,
but the mathematical engine can also be used independently of
\pgfname\ and \tikzname. 

\vskip1cm
\begin{codeexample}[graphic=white]
\pgfmathsetseed{1}
\foreach \col in {black,red,green,blue}
{
  \begin{tikzpicture}[x=10pt,y=10pt,ultra thick,baseline,line cap=round]
    \coordinate (current point) at (0,0);
    \coordinate (old velocity) at (0,0);
    \coordinate (new velocity) at (rand,rand);
    
    \foreach \i in {0,1,...,100}
    {
      \draw[\col!\i] (current point)
      .. controls ++([scale=-1]old velocity) and
                  ++(new velocity) .. ++(rand,rand)
         coordinate (current point);
      \coordinate (old velocity) at (new velocity);
      \coordinate (new velocity) at (rand,rand);
    }
  \end{tikzpicture}
}
\end{codeexample}

\include{pgfmanual-en-math-design}
\include{pgfmanual-en-math-parsing}
\include{pgfmanual-en-math-commands}
\include{pgfmanual-en-math-algorithms}


\part{The Basic Layer}

{\Large \emph{by Till Tantau}}


\bigskip
\noindent
\vskip1cm
\begin{codeexample}[graphic=white]
\begin{tikzpicture}
  \draw[gray,very thin] (-1.9,-1.9) grid (2.9,3.9)
          [step=0.25cm] (-1,-1) grid (1,1);
  \draw[blue] (1,-2.1) -- (1,4.1); % asymptote
                
  \draw[->] (-2,0) -- (3,0) node[right] {$x(t)$};
  \draw[->] (0,-2) -- (0,4) node[above] {$y(t)$};

  \foreach \pos in {-1,2}
    \draw[shift={(\pos,0)}] (0pt,2pt) -- (0pt,-2pt) node[below] {$\pos$};

  \foreach \pos in {-1,1,2,3}
    \draw[shift={(0,\pos)}] (2pt,0pt) -- (-2pt,0pt) node[left] {$\pos$};

  \fill (0,0) circle (0.064cm);
  \draw[thick,parametric,domain=0.4:1.5,samples=200]
    % The plot is reparameterised such that there are more samples
    % near the center.
    plot[id=asymptotic-example] function{(t*t*t)*sin(1/(t*t*t)),(t*t*t)*cos(1/(t*t*t))}
    node[right] {$\bigl(x(t),y(t)\bigr) = (t\sin \frac{1}{t}, t\cos \frac{1}{t})$};

  \fill[red] (0.63662,0) circle (2pt)
    node [below right,fill=white,yshift=-4pt] {$(\frac{2}{\pi},0)$};
\end{tikzpicture}
\end{codeexample}


\include{pgfmanual-en-base-design}
\include{pgfmanual-en-base-scopes}
\include{pgfmanual-en-base-points}
\include{pgfmanual-en-base-paths}
\include{pgfmanual-en-base-decorations}
\include{pgfmanual-en-base-actions}
\include{pgfmanual-en-base-arrows}
\include{pgfmanual-en-base-nodes}
\include{pgfmanual-en-base-matrices}
\include{pgfmanual-en-base-transformations}
\include{pgfmanual-en-base-patterns}
%\include{pgfmanual-en-base-images}
\include{pgfmanual-en-base-external}
\include{pgfmanual-en-base-plots}
\include{pgfmanual-en-base-layers}
\include{pgfmanual-en-base-shadings}
\include{pgfmanual-en-base-transparency}
\include{pgfmanual-en-base-quick}




\part{The System Layer}
\label{part-system}

{\Large \emph{by Till Tantau}}


\bigskip
\noindent
This part describes the low-level interface of \pgfname, called the
\emph{system layer}. This interface provides a complete abstraction of
the internals of the underlying drivers. 

Unless you intend to port \pgfname\ to another driver or unless you intend
to write your own optimized frontend, you need not read this part.

In the following it is assumed that you are familiar with the basic
workings of the |graphics| package and that you know what
\TeX-drivers are and how they work.

\vskip1cm
\begin{codeexample}[graphic=white]
\begin{tikzpicture}
  [shorten >=1pt,->,
   vertex/.style={circle,fill=black!25,minimum size=17pt,inner sep=0pt}]
  
  \foreach \name/\x in {s/1, 2/2, 3/3, 4/4, 15/11, 16/12, 17/13, 18/14, 19/15, t/16}
    \node[vertex] (G-\name) at (\x,0) {$\name$};

  \foreach \name/\angle/\text in {P-1/234/5, P-2/162/6, P-3/90/7, P-4/18/8, P-5/-54/9}
    \node[vertex,xshift=6cm,yshift=.5cm] (\name) at (\angle:1cm) {$\text$};
  
  \foreach \name/\angle/\text in {Q-1/234/10, Q-2/162/11, Q-3/90/12, Q-4/18/13, Q-5/-54/14}
    \node[vertex,xshift=9cm,yshift=.5cm] (\name) at (\angle:1cm) {$\text$};

  \foreach \from/\to in {s/2,2/3,3/4,3/4,15/16,16/17,17/18,18/19,19/t}
    \draw (G-\from) -- (G-\to);  

  \foreach \from/\to in {1/2,2/3,3/4,4/5,5/1,1/3,2/4,3/5,4/1,5/2}
    { \draw (P-\from) -- (P-\to); \draw (Q-\from) -- (Q-\to); }

  \draw (G-3) .. controls +(-30:2cm) and +(-150:1cm) .. (Q-1);
  \draw (Q-5) -- (G-15);
\end{tikzpicture}
\end{codeexample}

\include{pgfmanual-en-pgfsys-overview}
\include{pgfmanual-en-pgfsys-commands}
\include{pgfmanual-en-pgfsys-paths}
\include{pgfmanual-en-pgfsys-protocol}



\part{References and Index}

\vskip1cm
\begin{codeexample}[graphic=white]
\begin{tikzpicture}
  \draw[line width=0.3cm,color=red!30,line cap=round,line join=round] (0,0)--(2,0)--(2,5);
  \draw[help lines] (-2.5,-2.5) grid (5.5,7.5);
  \draw[very thick] (1,-1)--(-1,-1)--(-1,1)--(0,1)--(0,0)--
    (1,0)--(1,-1)--(3,-1)--(3,2)--(2,2)--(2,3)--(3,3)--
    (3,5)--(1,5)--(1,4)--(0,4)--(0,6)--(1,6)--(1,5)
    (3,3)--(4,3)--(4,5)--(3,5)--(3,6)
    (3,-1)--(4,-1);
  \draw[below left] (0,0) node(s){$s$};
  \draw[below left] (2,5) node(t){$t$};
  \fill (0,0) circle (0.06cm) (2,5) circle (0.06cm);
  \draw[->,rounded corners=0.2cm,shorten >=2pt]
    (1.5,0.5)-- ++(0,-1)-- ++(1,0)-- ++(0,2)-- ++(-1,0)-- ++(0,2)-- ++(1,0)--
    ++(0,1)-- ++(-1,0)-- ++(0,-1)-- ++(-2,0)-- ++(0,3)-- ++(2,0)-- ++(0,-1)--
    ++(1,0)-- ++(0,1)-- ++(1,0)-- ++(0,-1)-- ++(1,0)-- ++(0,-3)-- ++(-2,0)--
    ++(1,0)-- ++(0,-3)-- ++(1,0)-- ++(0,-1)-- ++(-6,0)-- ++(0,3)-- ++(2,0)--
    ++(0,-1)-- ++(1,0);
\end{tikzpicture}
\end{codeexample}

\printindex

\end{document}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/texmf/tex/generic/pgf/doc/pgf/version-for-pdftex/en/pgfmanual"
%%% End: 


==> pgfmanual-en-math-algorithms.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section[Reimplementing the Computations of the Mathematical Engine]
  {Reimplementing the Computations of the\\ Mathematical Engine}

\label{pgfmath-reimplement}

Perhaps you are not satisfied with the Maclaurin series for
$e^x$. Perhaps you have a fantastically more accurate
and efficient way of calculating the sine or cosine of angles. Perhaps
 you would like the library to interface with a package such as |fp| 
 for fixed-point arithmetic (but you may find that exclusively
 using |fp| can cause a significant increase in compile time for
 documents involving many hundreds of calculations).
In these cases you will want to replace the current implementations of
the computations done by the mathematical engine by your own code. 

The mathematical engine was designed with such a replacement in
mind. For this reason, the operations and functions like |\pgfmathadd|
are implemented in the following manner: 

\begin{itemize}
\item |\pgfmath|\meta{function name} 

  This macro is the ``public'' interface for the function
  \meta{function name}. All arguments passed to this macro are 
  evaluated using |\pgfmathparse| and then passed on to the following
  function:
  
\item |\pgfmath|\meta{function name}|@|
  
  This macro is the ``non-public'' implementation of the functions 
  algorithm (but note that, for speed, the parser calls this macro 
  rather than the ``public'' one). Arguments passed to this macro 
  are expected to be numbers \emph{without units}. This is the macro 
  which should be rewritten with your prize-winning new algorithm.

  Note, furthermore, that if the function takes more than one
  argument, the second argument should not involve the dimensions
  |\pgfmath@x| nor |\pgfmath@xa| nor |\pgf@x| nor |\pgf@xa| since
  these may be set to the value of the first argument when the
  second argument is parsed.
\end{itemize}

The effect of |\pgfmath|\meta{function name}|@| should be to set the
macro |\pgfmathresult| to the correct value (namely to the result of
the computation without units). Furthermore, the function should have
no other side effects, that is, it should not change any global
values. One way to achieve this is to use the following code:

\begin{codeexample}[code only]
\def\pgfmath...@#1#2...{%
   \begingroup%
      ... code for algorithm ...
      \pgfmath@returnone\pgfmath@x%
   \endgroup%
}
\end{codeexample}


The macro |\pgfmath@returnone|\meta{code} must be directly followed by an
|\endgroup| and will save result of the algorithm, by defining
|\pgfmathresult| as the  expansion of \meta{code} \emph{without units}
outside the group. The \meta{code} should expand to a dimension
register or to a dimension. By performing the algorithm within a
\TeX{} group, \pgfname{} registers such as |\pgf@x|, |\pgf@y| and 
|\c@pgf@counta|, |\c@pgfcountb|, and so forth, can be used at will.

\pgfname{} uses the last known definition of a function within the
prevailing scope, so it is possible for a function to be redefined 
or |\let| to an alternative definition locally.
You should also remember that any |.sty| or |.tex| file contatining any
re-implementions should be loaded \emph{after} \pgfname-Math.

==> pgfmanual-en-math-commands.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Evaluating Mathematical Operations}

\label{pgfmath-commands}

Instead of parsing and evaluating complex expressions, you can also
use the mathematical engine to evaluate a single mathematical
operation. The macros used for these computations are described in the
following. 


\subsection{Basic Operations and Functions}

\label{pgfmath-operations}

\begin{command}{\pgfmathadd\marg{x}\marg{y}}  
	Defines |\pgfmathresult| as $\meta{x}+\meta{y}$.
\end{command}

\begin{command}{\pgfmathsubtract\marg{x}\marg{y}}      
	Defines |\pgfmathresult| as $\meta{x}-\meta{y}$.                                       
\end{command}

\begin{command}{\pgfmathmultiply\marg{x}\marg{y}}      
	Defines |\pgfmathresult| as $\meta{x}\times\meta{y}$.                                
\end{command}

\begin{command}{\pgfmathdivide\marg{x}\marg{y}}        
	Defines |\pgfmathresult| as $\meta{x}\div\meta{y}$. An error will
	result if \meta{y} is	|0|, or if the result of the division is
	too big for the mathematical engine.
	Please remember	when using this command that accurate (and reasonably 
	quick) division of non-integers is particularly tricky in \TeX{}. 	
	There are three different forms of division used in this command:
	\begin{itemize}
		\item 
		If \meta{y} is an integer then the native |\divide| operation of 
		\TeX{} is used.
		\item
		If \vrule\meta{y}\vrule$<1$, then |\pgfmathreciprocal| is employed.
		\item
		For all other values of \meta{y} an optimised long division 
		algorithm is used. In theory this should be accurate
		to any finite precision, but in practice it is constrained by the
		limits of \TeX{}'s native mathematics.
	\end{itemize}
	                             
\end{command}

\begin{command}{\pgfmathreciprocal\marg{x}}         
	Defines |\pgfmathresult| as $1\div\meta{x}$.                            
\end{command}

\begin{command}{\pgfmathgreaterthan\marg{x}\marg{y}}   
	Defines |\pgfmathresult| as 1.0 if \meta{x} $>$ \meta{y}, but 0.0 otherwise.                 
\end{command}

\begin{command}{\pgfmathlessthan\marg{x}\marg{y}} 
	Defines |\pgfmathresult| as 1.0 if \meta{x} $<$ \meta{y}, but 0.0 otherwise.             
\end{command}
	
\begin{command}{\pgfmathequalto\marg{x}\marg{y}}       
	Defines |\pgfmathresult| 1.0 if \meta{x} $=$ \meta{y}, but 0.0 otherwise.                    
\end{command}

\begin{command}{\pgfmathround\marg{x}}              
	Defines |\pgfmathresult| as $\left\lfloor\textrm{\meta{x}}\right\rceil$.	
	This uses asymmetric	half-up rounding.                          
\end{command}

\begin{command}{\pgfmathfloor\marg{x}}              
	Defines |\pgfmathresult| as $\left\lfloor\textrm{\meta{x}}\right\rfloor$.
\end{command}

\begin{command}{\pgfmathceil\marg{x}}               
	Defines |\pgfmathresult| as $\left\lceil\textrm{\meta{x}}\right\rceil$.                           
\end{command}
	
\begin{command}{\pgfmathpow\marg{x}\marg{y}}         
	Defines |\pgfmathresult| as $\meta{x}^{\meta{y}}$.  For greatest 
	accuracy \mvar{y} should be an integer. If \mvar{y} is not an integer 
	the actual calculation will be an approximation of $e^{y\ln(x)}$.
\end{command}

\begin{command}{\pgfmathmod\marg{x}\marg{y}}           
	Defines |\pgfmathresult| as \meta{x} modulo \meta{y}.                       
\end{command}

\begin{command}{\pgfmathmax\marg{x}\marg{y}}           
	Defines |\pgfmathresult| as the maximum of \meta{x} or \meta{y}.                       
\end{command}

\begin{command}{\pgfmathmin\marg{x}\marg{y}}           
	Defines |\pgfmathresult| as the minimum \meta{x} or \meta{y}.                       
\end{command}
	
\begin{command}{\pgfmathabs\marg{x}}                
	Defines |\pgfmathresult| as  absolute value of \meta{x}.                                 
\end{command}
	
\begin{command}{\pgfmathexp\marg{x}}                
	Defines |\pgfmathresult| as $e^{\meta{x}}$. Here, \meta{x} can be a 
	non-integer. The algorithm	uses a Maclaurin series.               
\end{command}

\begin{command}{\pgfmathln\marg{x}}                
	Defines |\pgfmathresult| as $\ln{\meta{x}}$. This uses an algorithm
	due to Rouben Rostamian, and coefficients suggested by
	Alain Matthes.             
\end{command}
	
\begin{command}{\pgfmathsqrt\marg{x}} 
	Defines |\pgfmathresult| as $\sqrt{\meta{x}}$. 
\end{command}
	
\begin{command}{\pgfmathveclen\marg{x}\marg{y}}        
	Defines |\pgfmathresult| as $\sqrt{\meta{x}^2+\meta{y}^2}$. This uses
	a polynomial approximation, based on ideas due to Rouben Rostamian.                                    
\end{command}

\subsection{Trignometric Functions}

\label{pgfmath-trigonmetry}

\begin{command}{\pgfmathpi}
  	Defines |\pgfmathresult| as $3.14159$.
\end{command}
   
\begin{command}{\pgfmathdeg{\marg{x}}} 
	Defines |\pgfmathresult| as \meta{x} (given in radians) converted to 
	degrees. 
\end{command}

\begin{command}{\pgfmathrad{\marg{x}}} 
	Defines |\pgfmathresult| as \meta{x} (given in degrees) converted to 
	radians. 
\end{command}

\begin{command}{\pgfmathsin{\marg{x}}}  
	Defines |\pgfmathresult| as the sine of \meta{x}.  
\end{command}

\begin{command}{\pgfmathcos{\marg{x}}}
	Defines |\pgfmathresult| as the cosine of \meta{x}.
\end{command}

\begin{command}{\pgfmathtan{\marg{x}}}  
	Defines |\pgfmathresult| as the tangant of \meta{x}.  
\end{command}

\begin{command}{\pgfmathsec{\marg{x}}}
	Defines |\pgfmathresult| as the secant of \meta{x}.
\end{command}

\begin{command}{\pgfmathcosec{\marg{x}}}  
	Defines |\pgfmathresult| as the cosecant of \meta{x}.  
\end{command}

\begin{command}{\pgfmathcot{\marg{x}}}  
	Defines |\pgfmathresult| as the cotangant of \meta{x}.  
\end{command}

\begin{command}{\pgfmathasin{\marg{x}}}
	Defines |\pgfmathresult| as the arcsine of \meta{x}. 
	The result will be in the range $\pm90^\circ$.
\end{command}

\begin{command}{\pgfmathacos{\marg{x}}}
	Defines |\pgfmathresult| as the arccosine of \meta{x}.
	The result will be in the range $\pm90^\circ$.
\end{command}

\begin{command}{\pgfmathatan{\marg{x}}}
 	Defines |\pgfmathresult| as the arctangent of \meta{x}.
\end{command}



\subsection{Pseudo-Random Numbers}

\label{pgfmath-random}


\begin{command}{\pgfmathgeneratepseudorandomnumber}
	Defines |\pgfmathresult| as a pseudo-random integer between 1 and 
	$2^{31}-1$. This uses a linear congruency generator, based on ideas
	due to Erich Janka.
\end{command}

\begin{command}{\pgfmathrnd}
	Defines |\pgfmathresult| as a pseudo-random number between |0| and |1|.
\end{command}

\begin{command}{\pgfmathrand}
	Defines |\pgfmathresult| as a pseudo-random number between |-1| and |1|.
\end{command}

\begin{command}{\pgfmathrandominteger\marg{macro}\marg{maximum}\marg{minimum}}
	This defines \meta{macro} as a pseudo-randomly generated integer from 
	the range \meta{maximum} to \meta{minimum} (inclusive).
	
\begin{codeexample}[]
\begin{pgfpicture}
   \foreach \x in {1,...,50}{
      \pgfmathrandominteger{\a}{1}{50}
      \pgfmathrandominteger{\b}{1}{50}
      \pgfpathcircle{\pgfpoint{+\a pt}{+\b pt}}{+2pt}
      \color{blue!40!white}
      \pgfsetstrokecolor{blue!80!black}
      \pgfusepath{stroke, fill}
   }	  
\end{pgfpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfmathdeclarerandomlist\marg{list name}\{\marg{item-1}\marg{item 2}...\}}
	This creates a list of items with the name \meta{list name}.
\end{command}

\begin{command}{\pgfmathrandomitem\marg{macro}\marg{list name}}
	Select an item from a random list \meta{list name}. The
	selected item is placed in \meta{macro}.
\end{command}

\begin{codeexample}[]
\begin{pgfpicture}
   \pgfmathdeclarerandomlist{color}{{red}{blue}{green}{yellow}{white}}
   \foreach \a in {1,...,50}{
      \pgfmathrandominteger{\x}{1}{85}
      \pgfmathrandominteger{\y}{1}{85}
      \pgfmathrandominteger{\r}{5}{10}
      \pgfmathrandomitem{\c}{color}
      \pgfpathcircle{\pgfpoint{+\x pt}{+\y pt}}{+\r pt}
      \color{\c!40!white}
      \pgfsetstrokecolor{\c!80!black}
      \pgfusepath{stroke, fill}
   }	  
\end{pgfpicture}
\end{codeexample}

\begin{command}{\pgfmathsetseed\marg{integer}}
  Explicitly set seed for the pseudo-random number generator. By
  default it is set to the value of |\time|$\times$|\year|.
\end{command}


      
\subsection{Conversion Between Bases}
	
\label{pgfmath-bases}

\pgfname{} provides limited support for conversion between 
\emph{representations} of numbers. Currently the numbers must be
positive integers in the range $0$ to $2^{31}-1$, and the bases in the
range $2$ to $36$. All digits representing numbers greater than 9 (in
base ten), are alphabetic, but may be upper or lower case. 

\begin{command}{\pgfmathbasetodec\marg{macro}\marg{number}\marg{base}}
	Defines \meta{macro} as the result of converting \meta{number} from
	base \meta{base} to base 10. Alphabetic digits can be upper or lower
	case.

\medskip{\def\medskip{}

\begin{codeexample}[]
\pgfmathbasetodec\mynumber{107f}{16} \mynumber
\end{codeexample}


\begin{codeexample}[]
\pgfmathbasetodec\mynumber{33FC}{20} \mynumber
\end{codeexample}

}\medskip

\end{command}

\begin{command}{\pgfmathdectobase\marg{macro}\marg{number}\marg{base}}
	Defines \meta{macro} as the result of converting \meta{number} from
	base 10 to base \meta{base}. Any resulting alphabetic digits are in
	\emph{lower case}.
	
\begin{codeexample}[]
\pgfmathdectobase\mynumber{65535}{16} \mynumber
\end{codeexample}

\end{command}

\begin{command}{\pgfmathdectoBase\marg{macro}\marg{number}\marg{base}}
	Defines \meta{macro} as the result of converting \meta{number} from
	base 10 to base \meta{base}. Any resulting alphabetic digits are in
	\emph{upper case}.
	
\begin{codeexample}[]
\pgfmathdectoBase\mynumber{65535}{16} \mynumber
\end{codeexample}

\end{command}

\begin{command}{\pgfmathbasetobase\marg{macro}\marg{number}\marg{base-1}\marg{base-2}}
	Defines \meta{macro} as the result of converting \meta{number} from
	base \meta{base-1} to base \meta{base-2}. Alphabetic digits in 
	\meta{number} can be upper or lower case, but any resulting 
	alphabetic digits are in \emph{lower case}.
	
\begin{codeexample}[]
\pgfmathbasetobase\mynumber{11011011}{2}{16} \mynumber
\end{codeexample}

\end{command}

\begin{command}{\pgfmathbasetoBase\marg{macro}\marg{number}\marg{base-1}\marg{base-2}}
	Defines \meta{macro} as the result of converting \meta{number} from
	base \meta{base-1} to base \meta{base-2}. Alphabetic digits in 
	\meta{number} can be upper or lower case, but any resulting 
	alphabetic digits are in \emph{upper case}.
	
\begin{codeexample}[]
\pgfmathbasetoBase\mynumber{121212}{3}{12} \mynumber
\end{codeexample}

\end{command}


\begin{command}{\pgfmathsetbasenumberlength\marg{integer}}
	Set the number of digits in the result of a base conversion to 
	\meta{integer}. If the result of a conversion has less digits
	than this number it is prefixed with zeros.

\begin{codeexample}[]
\pgfmathsetbasenumberlength{8}
\pgfmathdectobase\mynumber{15}{2} \mynumber
\end{codeexample}

\end{command}

==> pgfmanual-en-math-design.tex <==
% Copyright 2007 by Mark Wibrow and Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.



\section{Design Principles}

\pgfname{} needs to perform many computations while typesetting a
picture. For this, \pgfname\ relies on a mathematical engine, which
can also be used independently of \pgfname, but which is distributed
as part of the \pgfname\ package nevertheless. Basically, the engine
provides a parsing mechanism similar to the \calcname{} package so
that expressions like |2*3cm+5cm| can be parsed; but the \pgfname\
engine is more powerful and can be extended and enhanced. 

\pgfname{} provides enhanced functionality, which permits the parsing
of mathematical operations involving integers and non-integers 
with or without units. Furthermore, various functions, including
trigonometric functions and random number generators can also be 
parsed (see Section~\ref{pgfmath-parsing}). 
The \calcname{} macros |\setlength| and friends have \pgfname{} versions 
which can parse these operations and functions 
(see Section~\ref{pgfmath-registers}). Additionally, each operation
and function has an independent \pgfname{} command associated with it
(see Section~\ref{pgfmath-commands}), and can be 
accessed outside the parser.

The mathematical engine of \pgfname\ is implicitly used whenever you
specify a number or dimension in a higher-level macro. For instance,
you can write |\pgfpoint{2cm+4cm/2}{3cm*sin(30)}| or
suchlike. However, the mathematical engine can also be used
independently of the \pgfname\ core, that is, you can also just load
it to get access to a mathematical parser.


\subsection{Loading the Mathematical Engine}

The mathematical engine of \pgfname\ is loaded automatically by
\pgfname, but if you wish to use the mathematical engine but you do
not need \pgfname\ itself, you can load the following package:

\begin{package}{pgfmath}
  This command will load the mathematical engine of \pgfname, but not
  \pgfname\ itself. It defines commands like |\pgfmathparse|.
\end{package}


\subsection{Layers of the Mathematical Engine}

Like \pgfname\ itself, the mathematical engine is also structured into
different layers:

\begin{enumerate}
\item The top layer, which you will typically use directly, provides
  the command |\pgfmathparse|. This command parses a mathematical
  expression and evaluates it.

  Additionally, the top layer also defines some additional functions
  similar to the macros of the |calc| package for setting dimensions
  and counters. These macros are just wrappers around the
  |\pgfmathparse| macro.
\item The calculation layer provides macros for performing one
  specific computation like computing a reciprocal or a
  multiplication. The parser uses these macros for the actual
  computation.
\item The implementation layer provides the actual implementations of
  the computations. These can be changed (and possibly be made more
  efficient) without affecting the higher layers.
\end{enumerate}



\subsection{Efficiency and Accuracy of the Mathematical Engine}

Currently, the mathematical algorithms are all implemented in \TeX.
This poses some intriguing programming challenges as \TeX{} is a
language for typesetting, rather than general mathematics,
and as with any programming language, there is a trade-off between 
accuracy and efficiency. 
If you find the level of accuracy insufficient for you
purposes, you will have to replace the algorithms in the
implementation layer.

All the fancy mathematical ``bells-and-whistles'' that the parser 
provides, come with an additional processing cost, and in some
instances, such as simply setting a length to |1cm|, with no other
operations involved, the additional processing time is undesirable. 
To overcome this, the following feature is implemented: when no
mathematical operations are required, an expression
can be preceded by |+|. This will bypass the parsing process and the 
assignment will be orders of magnitude faster. This feature 
\emph{only} works with the macros for setting registers described in
Section~\ref{pgfmath-registers}.

\begin{codeexample}[code only]
\pgfmathsetlength\mydimen{1cm}  % parsed     : slower.
\pgfmathsetlength\mydimen{+1cm} % not parsed : much faster.
\end{codeexample}



==> pgfmanual-en-math-parsing.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%

\section{Evaluating Mathematical Expressions}

The easiest way of using \pgfname's mathematical engine is to provide
a mathematical expression given in the usual infix notation (such as
|1cm+4*2cm/5.5| or |2*3+3*sin(30)|). This expression can be parsed by
the mathematical engine and the result be placed in a dimension
register, a counter, or a macro. Supported are infix mathematical
operations involving integers and non-integers, with or without
units.

It should be noted that all 
calculations must not exceed $\pm16383.99999$ at \emph{any} point, 
because the underlying algorithms rely on \TeX{} dimensions. This
means that many of the underlying algorithms are necessarily
approximate. It also means that some of the algorithms are not very
fast. \TeX{} is, after all, a typesetting language and not ideally
suited to relatively advanced mathematical operations. However, it is
possible to change the algorithms as described in
Section~\ref{pgfmath-reimplement}. 

In the present section, the high-level macros for parsing an
expression are explained first, then the syntax for expression is
explained.


\subsection{Commands for Parsing Expressions}

\label{pgfmath-registers}

\label{pgfmath-parsing}

The basic command for invoking the parser of \pgfname's mathematical
engine is the following:

\begin{command}{\pgfmathparse\marg{expression}}
  This macro parses \meta{expression} and returns the result without
  units in  the macro |\pgfmathresult|.

  \example |\pgfmathparse{2pt+3.5pt}| will set |\pgfmathresult| to the
  text |5.5|.

  In the following, the special properties of this command are
  explained. The exact syntax of mathematical expressions is explained
  in Section~\ref{pgfmath-syntax}.

  \begin{itemize}
  \item
    The result stored in the macro |\pgfmathresult| is a decimal
    \emph{without units}. This is true regardless of whether the
    \meta{expression} contains any unit specification. But, any units
    specified will be converted to points first.
\begin{codeexample}[]
\pgfmathparse{2pt+3.4pt} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{2cm+3.4cm} \pgfmathresult
\end{codeexample}

  \item If no units are specified \emph{at any point} in the 
    expression, the result will be multiplied by the value in 
    |\pgfmathresultunitscale|, which can be a number or a dimension 
    (which will be converted to points). By default it is set to 1, 
    but can be changed with |\pgfmathsetresultunitscale|. Note that 
    the result will still be a number \emph{without} units.

\begin{codeexample}[]
\pgfmathparse{2pt+3.4pt} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathsetresultunitscale{1cm}
\pgfmathparse{2+3.4} \pgfmathresult
\end{codeexample}

    \pgfmathsetresultunitscale{1pt}
    
  \item You can check whether an expression contained a unit using 
    the \TeX-if |\||ifpgfmathunitsdeclared|. After a call
    of |\pgfmathparse| this if will be true exactly if some unit was
    encountered in the expression.
    
  \item The parser handles numbers with or without units regardless
    of the operation.

\begin{codeexample}[]
\pgfmathparse{54pt/3cm*2.1} \pgfmathresult
\end{codeexample}

  \item the parser can cope with \TeX{} registers, including those 
    preceded by |\the|.

    \makeatletter

\begin{codeexample}[]
\pgf@x=12.34pt
\c@pgf@counta=5
\pgfmathparse{\pgf@x+\c@pgf@counta*6} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgf@x=56.78pt
\pgfmathparse{\pgf@x+\the\pgf@x} \pgfmathresult
\end{codeexample}

  \item \TeX{} dimension registers can be multiplied without the |*| 
    operator by preceding them with a number (\emph{not} a function),
     or a count register.
	 
\begin{codeexample}[]
\c@pgf@counta=-4
\pgf@x=10pt
\pgfmathparse{.5\pgf@x-\c@pgf@counta\pgf@x} \pgfmathresult
\end{codeexample}

  \item Parenthesis can be used to group operations.

\begin{codeexample}[]
\pgfmathparse{(4pt+0.5)*3} \pgfmathresult
\end{codeexample}

  \item functions are recognized, so it is possible to parse
    |sin(.5*pi r)*60|, which means ``the sine of $0.5$ times $\pi$ 
    radians, multiplied by 60''. The argument of most functions can
    be any expression.

\begin{codeexample}[]
\pgfmathparse{sin(pi/2 r)*60} \pgfmathresult
\end{codeexample}

  \item Scientific notation in the form |1.234e+4| is recognised (but
  the restriction on the range of values still applies). The exponent
  symbol can be upper or lower case (i.e., |E| or |e|). 
  
\begin{codeexample}[]
\pgfmathparse{1.234567891e-2} \pgfmathresult
\end{codeexample}
\begin{codeexample}[]
\pgfmathparse{1.234567891e4} \pgfmathresult
\end{codeexample}
  \end{itemize}
\end{command}

\begin{command}{\pgfmathqparse\marg{expression}}
  This macro is similar to |\pgfmathparse|: it parses 
  \meta{expression} and returns the result in the macro 
  |\pgfmathresult|. It differs in two respects. Firstly, 
  |\pgfmathqparse| does not parse functions or scientific
  notation. 
  Secondly, numbers in \meta{expression} \emph{must}
  specify a \TeX{} unit (except in such instances as |0.5\pgf@x|), 
  which greatly simplifies the problem of parsing 
  of non-integers. As a result of these restrictions |\pgfmathqparse| 
  is about twice as fast as |\pgfmathparse|. Note that the result 
  will still be a number \emph{without} units.	
\end{command}

\begin{command}{\pgfmathsetresultunitscale\marg{number or dimension}}
  Sets the value in |\pgfmathresultunitscale|, which scales the result
  of an expression parsed with |\pgfmathparse|, if that expression
  contains no units \emph{at any point}. The argument can be an integer,
  non-integer or a dimension, but the result will still be a number 
  \emph{without} units. Note, that this will affect |\pgfmathsetlength| 
  and friends, but not if the expression starts with |+| (which
  switches parsing off). By default the value in
  |\pgfmathresultunitscale| is 1. 
\end{command}

Instead of the |\pgfmathparse| macro you can also wrapper commands,
whose usage is very similar to their cousins in the \calcname{} 
package. The only difference is that the expressions can be any
expression that is handled by |\pgfmathparse|.

For all of the following commands, if \meta{expression} starts with
|+|, no parsing is done and a simple assignment or increment is done
using normal \TeX\ assignments or increments. This will be orders of
magnitude faster than calling the parser. 

\begin{command}{\pgfmathsetlength\marg{dimension register}\marg{expression}}
  Sets the length of the \TeX{} \meta{dimension register}, to the value
  (in points) specified by \meta{expression}. The \meta{expression}
  will be parsed using |\pgfmathparse|.
\end{command}

\begin{command}{\pgfmathaddtolength\marg{dimension register}\marg{expression}}
  Adds the value (in points) of \meta{expression} to the \TeX{} 
  \meta{dimension register}. 
\end{command}

\begin{command}{\pgfmathsetcount\marg{count register}\marg{expression}}
  Sets the value of the \TeX{} \meta{count register}, to the 
  \emph{truncated} value specified by \meta{expression}. 
\end{command}

\begin{command}{\pgfmathaddtocount\marg{count register}\marg{expression}}
  Adds the \emph{truncated} value  of \meta{expression} to the \TeX{} 
  \meta{count register}.
\end{command}

\begin{command}{\pgfmathsetcounter\marg{counter}\marg{expression}}
  Sets the value of the \LaTeX{} \meta{counter}, to the \emph{truncated} 
  value specified by \meta{expression}. 
\end{command}

\begin{command}{\pgfmathaddtocounter\marg{counter}\marg{expression}}
  Adds the \emph{truncated} value  of \meta{expression} to 
  \meta{counter}.
\end{command}

% \begin{command}{\pgfmathnewcounter\marg{counter}}
%   This is simply a version of the \LaTeX{} macro |\newcounter|, 
%   implemented to maintain consistency (consistency is good,
%   inconsistency is evil). Considering |\pgfmathnewcounter{foo}|, this
%   creates a new count register |\c@foo|, and a macro |\thefoo|, which
%   returns the value in |\c@foo|.
% \end{command}

\begin{command}{\pgfmathsetmacro\marg{macro}\marg{expression}}
  Defines \meta{macro} as the  value of \meta{expression}. The result
  is a decimal \emph{without} units.
\end{command}

\begin{command}{\pgfmathsetlengthmacro\marg{macro}\marg{expression}}
  Defines \meta{macro} as the value of \meta{expression} 
  \LaTeX{}\emph{in points}.
\end{command}

\begin{command}{\pgfmathtruncatemacro\marg{macro}\marg{expression}}
  Defines \meta{macro} as the truncated value of \meta{expression}.
\end{command}



\subsection{Syntax for mathematical expressions}

\label{pgfmath-syntax}

The syntax for the expressions recognized by |\pgfmathparse| and
friends is straightfoward, and the following operations and 
functions are currently recognized:

\begin{math-operator}{\mvar{x}\ +\ \mvar{y}}
	Adds \mvar{y} to \mvar{x}.
	
\begin{codeexample}[]
\pgfmathparse{4+2pt} \pgfmathresult
\end{codeexample}
\end{math-operator}

\begin{math-operator}{\mvar{x}\ -\ \mvar{y}}
	Subtracts \mvar{y} from  \mvar{x}.
	
\begin{codeexample}[]
\pgfmathparse{155.35-4cm} \pgfmathresult
\end{codeexample}
\end{math-operator}
\begin{math-operator}{\mvar{x}\ *\ \mvar{y}}
	Multiplies \mvar{x} by  \mvar{y}.
	
\begin{codeexample}[]
\pgfmathparse{3.9pt*4.56} \pgfmathresult
\end{codeexample}

\end{math-operator}
\begin{math-operator}{\mvar{x}\ /\ \mvar{y}}
	Divides \mvar{x} by  \mvar{y}.
	
\begin{codeexample}[]
\pgfmathparse{-31.6pt/17} \pgfmathresult
\end{codeexample}

\end{math-operator}
\begin{math-operator}{\mvar{x}\ {\char94}\ \mvar{y}} 

Raises \mvar{x} to the power \mvar{y}. For greatest accuracy \mvar{y}
should be an integer. If \mvar{y} is not an integer the actual
calculation will be an approximation of $e^{y\ln(x)}$.

{
\catcode`\^=7

\begin{codeexample}[]
\pgfmathparse{2.3^4} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{2^-4} \pgfmathresult
\end{codeexample}
}
\end{math-operator}

\begin{math-operator}{\mvar{x}\ ==\ \mvar{y}} 

	This evaluates to |1| if \mvar{x} equals \mvar{y}, or |0| if \mvar{x}
	does not equal \mvar{y}. 
	Note that equalities (and inequalities) are evaluated left to right, 
	and are only evaluated when another equality (or inequality) operator 
	is scanned, or the end of the current group or parse is reached. So 
	|5+4==3+2==9| results in |0| because |5+4| does not equal |3+2|, 
	resulting in zero, and the second equality is therefore evaluating 
	|0==9|.

\begin{codeexample}[]
\pgfmathparse{3*5==15} \pgfmathresult
\end{codeexample}

\end{math-operator}


\begin{math-operator}{\mvar{x}\ >\ \mvar{y}} 

	This evaluates to |1| if \mvar{x} is greater than \mvar{y}, or |0| if 
	\mvar{x} is smaller or equal to \mvar{y}.
	
\begin{codeexample}[]
\pgfmathparse{17>4.2*1.97+4} \pgfmathresult
\end{codeexample}

\end{math-operator}

\begin{math-operator}{\mvar{x}\ <\ \mvar{y}}

	This evaluates to |1| if \mvar{x} is smaller than \mvar{y}, or |0| if
	\mvar{x} is greater or equal to \mvar{y}.
	
\begin{codeexample}[]
\pgfmathparse{2<-5.2/-3.6-2} \pgfmathresult
\end{codeexample}

\end{math-operator}

\begin{math-function}{mod(\mvar{x},\mvar{y})}
	This evaluates \mvar{x} modulo \mvar{y} (using truncated division).
	This function cannot be nested inside itself or the functions |max|, 
	|min| or |pow|.

\begin{codeexample}[]
\pgfmathparse{mod(20,6)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{max(\mvar{x},\mvar{y})}
	This evaluates to the maximum of \mvar{x} or \mvar{y}. This function 
	cannot be nested inside itself or the functions |min|, |mod| or 
	|pow|.

\begin{codeexample}[]
\pgfmathparse{max(17,23)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{min(\mvar{x},\mvar{y})}
	This evaluates to the minimum of \mvar{x} or \mvar{y}. This function 
	cannot be nested inside itself or the functions |max|, |mod| or 
	|pow|.

\begin{codeexample}[]
\pgfmathparse{min(17,23)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{abs(\mvar{x})} 

	Evaluates the absolute value of $x$.
	
\begin{codeexample}[]
\pgfmathparse{abs(-5)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{-abs(4*-3)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{round(\mvar{x})}

	Rounds \mvar{x} to the nearest integer. It uses ``asymmetric half-up'' 
	rounding. So |1.5| is rounded to |2|, but |-1.5| is rounded to |-2| 
	(\emph{not} |0|).

\begin{codeexample}[]
\pgfmathparse{round(32.5/17)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{round(398/12)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{floor(\mvar{x})}

	Rounds \mvar{x} down to the nearest integer. 
	
\begin{codeexample}[]
\pgfmathparse{floor(32.5/17)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{floor(398/12)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{ceil(\mvar{x})}

	Rounds \mvar{x} up to the nearest integer. 

\begin{codeexample}[]
\pgfmathparse{ceil(32.5/17)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{ceil(398/12)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{exp(\mvar{x})}
{
\catcode`\^=7

	Maclaurin series for $e^x$. 
}	
\begin{codeexample}[]
\pgfmathparse{exp(1)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{exp(2.34)} \pgfmathresult
\end{codeexample}

\end{math-function}


\begin{math-function}{ln(\mvar{x})}
{
\catcode`\^=7

	An approximation for for $\ln(\textrm{\mvar{x}})$. 
}	
\begin{codeexample}[]
\pgfmathparse{ln(10)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{ln(exp(5))} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{pow(\mvar{x},\mvar{y})}

 Raises \mvar{x} to the power \mvar{y}. 

\begin{codeexample}[]
\pgfmathparse{pow(2,7)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{sqrt(\mvar{x})}

 Calculates $\sqrt{\textrm{\mvar{x}}}$.

\begin{codeexample}[]
\pgfmathparse{sqrt(10)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{sqrt(8765.432)}  \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{veclen(\mvar{x},\mvar{y})}

 Calculates $\sqrt{\left(\textrm{\mvar{x}}^2+\textrm{\mvar{y}}^2\right)}$.

\begin{codeexample}[]
\pgfmathparse{veclen(12,5)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-constant}{pi}

	The constant $\pi=3.14159$.
	
\begin{codeexample}[]
\pgfmathparse{pi} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{pi r} \pgfmathresult
\end{codeexample}

\end{math-constant}

\begin{math-operator}{\mvar{x}\ r}

	This converts \mvar{x} from radians to degrees. Note that |r| will 
	evaluate any preceding series of multiplication or division 
	\emph{before} conversion, but not other operations. So |3*4/6r| 
	converts 2 radians to degrees, but |3-4+6r|, converts 6 radians to
	degrees and adds the result to |-1|.

\begin{codeexample}[]
\pgfmathparse{2*pi r-pi r} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{2*pi/8 r} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{sin(3*pi/2r)*60} \pgfmathresult
\end{codeexample}

\end{math-operator}

\begin{math-function}{rad(\mvar{x})}

	Convert \mvar{x} to radians. \mvar{x} is assumed to be in degrees.
	
\begin{codeexample}[]
\pgfmathparse{rad(90)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{deg(\mvar{x})}

	Convert \mvar{x} to degrees. \mvar{x} is assumed to be in radians.
	
\begin{codeexample}[]
\pgfmathparse{deg(3*pi/2)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{sin(\mvar{x})}

	Sine of \mvar{x}. By employing the |r| operator, \mvar{x} can be in 
	radians.
	
\begin{codeexample}[]
\pgfmathparse{sin(60)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{sin(pi/3 r)}
\end{codeexample}

\end{math-function}

\begin{math-function}{cos(\mvar{x})}

	Cosine of \mvar{x}. By employing the |r| operator, \mvar{x} can be in 
	radians.

\begin{codeexample}[]
\pgfmathparse{cos(60)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{cos(pi/3 r)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{tan(\mvar{x})}

	Tangent of \mvar{x}. By employing the |r| operator, \mvar{x} can be in 
	radians.
	
\begin{codeexample}[]
\pgfmathparse{tan(45)} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{tan(2*pi/8 r)} \pgfmathresult
\end{codeexample}

\end{math-function}


\begin{math-function}{sec(\mvar{x})}

	Secant of \mvar{x}. By employing the |r| operator, \mvar{x} can be in 
	radians.

\begin{codeexample}[]
\pgfmathparse{sec(45)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{cosec(\mvar{x})}

	Cosecant of \mvar{x}. By employing the |r| operator, \mvar{x} can be in 
	radians.
	
\begin{codeexample}[]
\pgfmathparse{cosec(30)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{cot(\mvar{x})}

	Cotangent of \mvar{x}. By employing the |r| operator, \mvar{x} can be in 
	radians.
	
\begin{codeexample}[]
\pgfmathparse{cot(15)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{asin(\mvar{x})}

	Arcsine of \mvar{x}. The result is in degrees and in the range $\pm90^\circ$.

\begin{codeexample}[]
\pgfmathparse{asin(0.7071)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{acos(\mvar{x})}

	Arccosine of \mvar{x} in degrees. The result is in the range $\pm90^\circ$.


\begin{codeexample}[]
\pgfmathparse{acos(0.5)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{atan(\mvar{x})}

	Arctangent of $x$ in degrees. 

\begin{codeexample}[]
\pgfmathparse{atan(1)} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{rnd}

	Generates a pseudo-random number between 0 and 1.

\begin{codeexample}[]
\pgfmathparse{rnd} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{2*rnd} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{-rnd+5} \pgfmathresult
\end{codeexample}

\end{math-function}

\begin{math-function}{rand}

	Generates a pseudo-random number between -1 and 1.

\begin{codeexample}[]
\pgfmathparse{rand} \pgfmathresult
\end{codeexample}

\begin{codeexample}[]
\pgfmathparse{rand*15} \pgfmathresult
\end{codeexample} 

\end{math-function}


==> pgfmanual-en-pgfcalendar.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Date and Calendar Utility Macros}
\label{section-calendar}

This section describes the package |pgfcalendar|.

\begin{package}{pgfcalendar}
  This package can be used independently of \pgfname. It has two
  purposes:
  \begin{enumerate}
  \item It provides functions for working with dates. Most noticably,
    it can convert a date in ISO-standard format (like 1975-12-26) to
    a so-called Julian day number, which is defined in Wikipedia as
    follows:  ``The Julian day or Julian day number is the
    (integer) number of days that have elapsed since the initial epoch
    at noon Universal Time (UT) Monday, January 1, 4713 BC in the
    proleptic Julian calendar.'' The package also provides a function
    for converting a Julian day number to an ISO-format date.

    Julian day numbers make it very easy to work with days. For
    example, the date ten days in the future of 2008-02-20 can
    be computed by converting this date to a Julian day number, adding
    10, and then converting it back. Also, the day of week of a given
    date can be computed by taking the Julian day number modulo~7.
  \item It provides a macro for typesetting a calendar. This macro
    is highly configurable and flexible (for example, it can produce
    both plain text calendars and also complicated \tikzname-based
    calendars), but most users will not use the macro directly. It is
    the job of a frontend to provide useful configruations for
    typesetting calendars based on this command.
  \end{enumerate}
\end{package}


\subsection{Handling Dates}

\subsubsection{Conversions Between Date Types}

\begin{command}{\pgfcalendardatetojulian\marg{date}\marg{counter}}
  This macro converts a date in a format to be described in a moment
  to the Julian day number in the Gregorian calendar. The \meta{date}
  should expand to a string of the following form:
  \begin{enumerate}\label{calendar-date-format}
  \item It should start with a number representing the year. Use
    |\year| for the current year, that is, the year the file is being
    typeset.
  \item The year must be followed by a hyphen.
  \item Next should come a number representing the month. Use |\month|
    for the current month. You can, but need not, use leading
    zeros. For example, |02| represents February, just like |2|.
  \item The month must also be followed by a hyphen.
  \item Next you must either provide a day of month (again, a number
    and, again, |\day| yields the current day of month) or the keyword
    |last|. This keyword refers to the last day of the month, which is
    automatically computed (and which is a bit tricky to compute,
    especially for February).
  \item Optionally, you can next provide a plus sign followed by
    positive or negative number. This number of days will be added to
    the computed date.
  \end{enumerate}

  Here are some examples:
  \begin{itemize}
  \item |2006-01-01| refers to the first day of 2006.
  \item |2006-02-last| refers to February 28, 2006.
  \item |\year-\month-\day| refers to today.
  \item |2006-01-01+2| refser to January 3, 2006.
  \item |\year-\month-\day+1| refers to tomorrow.
  \item |\year-\month-\day+-1| refers to yesterday.
  \end{itemize}
  
  The conversion method is taken from the English Wikipedia entry on
  Julian days. 

  \newcount\mycount
  \example |\pgfcalendardatetojulian{2007-01-14}{\mycount}| sets
  |\mycount| to
  \pgfcalendardatetojulian{2007-01-14}{\mycount}\the\mycount.

  
\end{command}

\begin{command}{\pgfcalendarjuliantodate\marg{Julian day}\marg{year
      macro}\marg{month macro}\marg{day macro}}
  This command converts a Julian day number to an ISO-date. The
  \meta{Julian day} must be a number or \TeX\ counter, the \meta{year macro},
  \meta{month macro} and \meta{day macro} must be \TeX\ macro
  names. They will be set to numbers representing the year, month, and
  day of the given Julian day in the Gregorian calendar.

  The \meta{year macro} will be assigned the year without leading
  zeros. Note that this macro will produce year 0 (as opposed to other
  calendars, where year 0 does not exist). However, if you really need
  calendars for before the year 1, it is expected that you know what
  you are doing anyway.

  The \meta{month macro} gets assigned a two-digit number representing
  the month (with a leading zero, if necessary). Thus, the macro is
  set to |01| for January.

  The \meta{day macro} gets assigned a two-digit number representing
  the day of the month (again with a possible leading zero).

  To convert a Julian day number to an ISO-date you use code like the
  following:
\begin{verbatim}
\pgfcalendardatetojulian{2454115}{\myyear}{\mymonth}{\myday}
\edef\isodate{\myyear-\mymonth-\myday}
\end{verbatim}
  The above code sets |\isodate| to
  \pgfcalendarjuliantodate{2454115}{\myyear}{\mymonth}{\myday}%
  \edef\isodate{\myyear-\mymonth-\myday}\texttt{\isodate}.
\end{command}


\begin{command}{\pgfcalendarjuliantoweekday\marg{Julian day}\marg{week day counter}}
  This command converts a Julian day to a week day by computing the
  day modulo 7. The \meta{week day counter} must be a \TeX\
  counter. It will be set to 0 for a Monday, to 1 for a Tuesday, and
  so on.

  \example |\pgfcalendarjuliantoweekday{2454115}{\mycount}| sets
  |\mycount| to
  \pgfcalendarjuliantoweekday{2454115}{\mycount}\the\mycount. 
\end{command}


\subsubsection{Checking Dates}


\begin{command}{\pgfcalendarifdate\marg{date}\marg{tests}\marg{code}\marg{else code}}
  \label{pgfcalendarifdate}
  This command is used to execute code based on properties of
  \meta{date}. The \meta{date} must be a date in ISO-format. For
  this date, the \meta{tests} are checked (to be detailed later)
  and if one of the tests applied, the \meta{code} is
  executed. If none of the tests applies, the \meta{else code} is
  executed.

  \example |\pgfcalendarifdate{2007-02-07}{Wednesday}{Is a Wednesday}{Is not a Wednesday}|
  yields \texttt{\pgfcalendarifdate{2007-02-07}{Wednesday}{Is a
      Wednesday}{Is not a Wednesday}}.

  The \meta{tests} is a comma-separated list of key-value
  pairs. The following are defined by default:
  \begin{itemize}
  \itemcalendaroption{all} This test is passed by all dates.
  \itemcalendaroption{Monday} This test is passed by all dates that
  are Mondays.
  \itemcalendaroption{Tuesday} as above.
  \itemcalendaroption{Wednesday} as above.
  \itemcalendaroption{Thursday} as above.
  \itemcalendaroption{Friday} as above.
  \itemcalendaroption{Saturday} as above.
  \itemcalendaroption{Sunday} as above.
  \itemcalendaroption{workday} Passed by Mondays, Tuesdays,
  Wednesdays, Thursdays, and Fridays.
  \itemcalendaroption{weekend} Passed Saturdays and Sundays. 
  \itemcalendaroption{equals}|=|\meta{reference} The \meta{reference}
  can be in one of two forms: Either, it is a full ISO format date
  like |2007-01-01| or the year may be missing as in |12-31|. In the
  first case, the test is passed if \meta{date} is the same as
  \meta{reference}. In the second case, the test is passed if the
  month and day part of \meta{date} is the same as \meta{reference}.

  For example, the test |equals=2007-01-10| will only be passed by this
  particular date. The test |equals=05-01| will be passed by every first
  of May on any year.
  \itemcalendaroption{at least}|=|\meta{reference} This test works
  similarly to the |equals| test, only it is checked whether
  \meta{date} is equal to \meta{reference} or to any later
  date. Again, the \meta{reference} can be a full date like
  |2007-01-01| or a short version like |07-01|. For example,
  |at least=07-01| is true for every day in the second half of any
  year.
  \itemcalendaroption{at most}|=|\meta{reference} as above.
  \itemcalendaroption{between}|=|\meta{start reference}| and |\meta{end
    refernce} This test checks whether the current date lies between
  the two given reference dates. Both full and short version may be
  given.

  For example |between=2007-01-01 and 2007-02-28| is true for the days
  in January and February of 2007.

  For another example, |between=05-01 and 05-07| is true for the
  days of the first week of May of any year.
  \itemcalendaroption{day of month}|=|\meta{number} Passed by the day
  of month of the \meta{date} is \meta{number}. For example, the test
  |day of month=1| is passed by every first of every month.
  \itemcalendaroption{end of month}\opt{|=|\meta{number}} Passed by
  the day of month of the \meta{date} that is \meta{number} from the
  end of the month. For example, the test |end of month=1| is passed
  by the last day of every month, the test |end of month=2| is passed
  by the second last day of every month. If \meta{number} is omitted,
  it is assumed to be |1|.
  \end{itemize}

  In addition to the above checks, you can also define new checks. To
  do so, you must add a new key to the key-value group |pgfcalendar|
  using |\define@key|. The job of the code of this new key is to
  possibly set the \TeX-if |\ifpgfcalendarmatches| to true (if it is
  already true, no action should be taken) to indicate that the
  \meta{date} passes the test setup by this new key.

  In order to perform the test, the key code needs to know the date
  that should be checked. The date is available through a macro, but a
  whole bunch of additional information about this date is also
  available through the following macros:
  \begin{itemize}
  \item |\pgfcalendarifdatejulian|
    is the Julian day number of the \meta{date} to be checked.
  \item |\pgfcalendarifdateweekday|
    is the weekday of the \meta{date} to be checked.
  \item |\pgfcalendarifdateyear|
    is the year of the \meta{date} to be checked.
  \item |\pgfcalendarifdatemonth|
    is the month of the \meta{date} to be checked.
  \item |\pgfcalendarifdateday|
    is the day of month of the \meta{date} to be checked.
  \end{itemize}

  For example, let us define a new key that checks whether the
  \meta{date} is a Workers day (first of May). This can be done as
  follows:
\begin{verbatim}
\define@key{pgfcalendar}{workers day}[]
{
  \ifnum\pgfcalendarifdatemonth=5\relax
    \ifnum\pgfcalendarifdateday=1\relax
      \pgfcalendarmatchestrue
    \fi
  \fi
}
\end{verbatim}
\end{command}


\subsubsection{Typesetting Dates}




\begin{command}{\pgfcalendarweekdayname\marg{week day number}}
  This command expands to a textual representation of the day of week,
  given by the \meta{week day number}. Thus,
  |\pgfcalendarweekdayname{0}| expands to |Monday| if the current
  language is English and to |Montag| if the current language is
  German, and so on. See Section~\ref{section-calendar-locale} for
  more details on translations.

  \example |\pgfcalendarweekdayname{2}| yields
  \texttt{\pgfcalendarweekdayname{2}}. 
\end{command}


\begin{command}{\pgfcalendarweekdayshortname\marg{week day number}}
  This command works similiarly to the previous command, only an
  abbreviated version of the week day is produced.

  \example |\pgfcalendarweekdayshortname{2}| yields
  \texttt{\pgfcalendarweekdayshortname{2}}. 
\end{command}


\begin{command}{\pgfcalendarmonthname\marg{month number}}
  This command expands to a textual representation of the month, which
  is given by the \meta{month number}.

  \example |\pgfcalendarmonthname{12}| yields
  \texttt{\pgfcalendarmonthname{12}}. 
\end{command}


\begin{command}{\pgfcalendarmonthshortname\marg{month number}}
  As above, only an abbreviated version is produced.

  \example |\pgfcalendarmonthshortname{12}| yields
  \texttt{\pgfcalendarmonthshortname{12}}.   
\end{command}



\subsubsection{Localization}

\label{section-calendar-locale}
All textual representations of week days or months (like ``Monday'' or
``February'') are wrapped with |\translate| commands from the
|translator| package (it this package is not loaded, no translation
takes place). Furthermore, the |pgfcalendar| package will try to load
the |translator-months-dictionary|, if the |translator| package is
loaded.

The net effect of all this is that all dates will be translated to the
current language setup in the |translator| package. See the
documentation of this package for more details.



\subsection{Typesetting Calendars}

\begin{command}{\pgfcalendar\marg{prefix}\marg{start date}\marg{end
      date}\marg{rendering code}}
  This command can be used to typeset a calendar. It is a very general
  command, the actual work has to be done by giving clever
  implementations of \meta{rendering code}. Note that this macro need
  \emph{not} be called inside a |{pgfpicture}| environment (even
  though it typically will be) and you can use it to typeset calendars
  in normal \TeX\ or using packages other than \pgfname.

  \medskip
  \textbf{Basic typesetting process.}
  A calendar is typeset as follows: The \meta{start date} and
  \meta{end date} specify a range of dates. For each date in this 
  range the \meta{rendering code} is executed with certain macros
  setup to yield information about the \emph{current date}
  (the current date in the enumeration of dates of the
  range). Typically, the \meta{rendering code} places nodes inside a
  picture, but it can do other things as well. Note that it is also
  the job of the \meta{rendering code} to position the calendar
  correctly. 

  The different calls of the \meta{rending code} are not
  surrounded by \TeX\ groups (though you can do so yourself, of
  course). This means that settings can accumulate between different
  calls, which is often desirable and useful.

  \medskip
  \textbf{Information about the current date.}
  Inside the \meta{rendering code}, different macros can be access:

  \begin{itemize}
  \item |\pgfcalendarprefix|
    The \meta{prefix} parameter. This prefix is recomended for nodes
    inside the calendar, but you have to use it yourself explicitly.
  \item |\pgfcalendarbeginiso|
    The \meta{start date} of range being typeset in ISO format (like 2006-01-10).
  \item |\pgfcalendarbeginjulian|
    Julian day number of \meta{start date}.
  \item |\pgfcalendarendiso|
    The \meta{end date} of range being typeset in ISO format.
  \item |\pgfcalendarendjulian|
    Julian day number of \meta{end date}.
  \item |\pgfcalendarcurrentjulian| This \TeX\ count holds the 
    Julian day number of day currently begin rendered.
  \item |\pgfcalendarcurrentweekday| The weekday
    (a number with zero representing Monday) of the current date.
  \item |\pgfcalendarcurrentyear| The year of the current date.
  \item |\pgfcalendarcurrentmonth| The month of the current date
    (always two digits with a leading zero, if necessary).
  \item |\pgfcalendarcurrentday| The day of month of the current date
    (alwyas two digits).
  \end{itemize}

  \medskip
  {\bfseries The |\ifdate| command.}
  Inside the |\pgfcalendar| the macro |\ifdate| is available
  locally:
  \begin{command}{\ifdate\marg{tests}\marg{code}\marg{else code}}
    \label{ifdate}%
    This command has the same effect as calling |\pgfcalendarifdate|
    for the current date.
  \end{command}

  \medskip
  \textbf{Examples.}
  In a first example, let us create a very simple calendar: It just
  lists the dates in a certain range.
\begin{codeexample}[vbox,ignorespaces]
\pgfcalendar{cal}{2007-01-20}{2007-02-10}{\pgfcalendarcurrentday\ }    
\end{codeexample}
  Let us now make this a little more interesting: Let us add a line
  break after each Sunday.
\begin{codeexample}[vbox,ignorespaces]
\pgfcalendar{cal}{2007-01-20}{2007-02-10}
{
  \pgfcalendarcurrentday\
  \ifdate{Sunday}{\par}{}
}    
\end{codeexample}
  We now want to have all Mondays to be aligned on a column. For this,
  different approaches work. Here is one based positioning each day
  horizontally using a skip.
\begin{codeexample}[vbox,ignorespaces]
\pgfcalendar{cal}{2007-01-20}{2007-02-10}
{%
  \leavevmode%
  \hbox to0pt{\hskip\pgfcalendarcurrentweekday cm\pgfcalendarcurrentday\hss}%
  \ifdate{Sunday}{\par}{}%
}    
\end{codeexample}
  Let us now typeset two complete months.
\begin{codeexample}[vbox,ignorespaces]
\pgfcalendar{cal}{2007-01-01}{2007-02-28}{%
  \ifdate{day of month=1}{
    \par\bigskip\hbox to7.5cm{\itshape\hss\pgfcalendarshorthand mt\hss}\par
  }{}%
  \leavevmode%
  {%
    \ifdate{weekend}{\color{black!50}}{\color{black}}%
    \hbox to0pt{%
      \hskip\pgfcalendarcurrentweekday cm%
      \hbox to1cm{\hss\pgfcalendarshorthand d-}\hss%
    }%
  }%
  \ifdate{Sunday}{\par}{}%
}    
\end{codeexample}
  For our final example, we use a |{tikzpicture}|. 
\begin{codeexample}[vbox,ignorespaces]
\begin{tikzpicture}    
  \pgfcalendar{cal}{2007-01-20}{2007-02-10}{%
    \ifdate{workday}
      {\tikzset{filling/.style={fill=blue!20}}}
      {\tikzset{filling/.style={fill=red!20}}}
    \node (\pgfcalendarsuggestedname) at (\pgfcalendarcurrentweekday,0)
      [anchor=base,circle,filling] {\pgfcalendarcurrentday};
    \ifdate{Sunday}{\pgftransformyshift{-3em}}{}%
  }
  \draw (cal-2007-01-21) -- (cal-2007-02-03);
\end{tikzpicture}
\end{codeexample}
\end{command}


\begin{command}{\pgfcalendarshorthand\marg{kind}\marg{representation}}
  \label{pgfcalendarshorthand}
  This command can be used inside a |\pgfcalendar|, where it will
  expand to a representation of the current day, month, year or day of
  week, depending on whether \meta{kind} is |d|, |m|, |y| or |w|. The
  \meta{representation} can be one of the following: |-|, |=|, |0|,
  |.|, and |t|. They have the following meanings:
  \begin{itemize}
  \item The minus sign selects the shortest numerical representation
    possible (no leading zeros).
  \item The equal sign also selects the shortest numerical
    representation, but a space is added to single digit days and
    months (thereby ensuring that they have the same length as other
    days).
  \item The zero digit selects a two-digit numerical representation
    for days and months. For years it is allowed, but has no effect.
  \item The letter |t| selects a textual representation.
  \item The dot selects an abbreviated textual representation.
  \end{itemize}
  Normally, you should say |\let\%=\pgfcalendarshorthand| locally, so
  that you can write |\%wt| instead of the much more cumbersome
  |\pgfcalendarshorthand{w}{t}|. 

\begin{codeexample}[leave comments]
\let\%=\pgfcalendarshorthand
\pgfcalendar{cal}{2007-01-20}{2007-01-20}
{ ISO form: \%y0-\%m0-\%d0, long form: \%wt, \%mt \%d-, \%y0}    
\end{codeexample}
\end{command}


\begin{command}{\pgfcalendarsuggestedname}
  This macro expands to a suggested name for nodes representing days
  in a calendar. If the \meta{prefix} is empty, it expands to the
  empty string, otherwise it expands to the \meta{prefix} of the
  calendar, followed by a hyphen, followed by the ISO format version
  of the date. Thus, when the date |2007-01-01| is typeset in a
  calendar for the prefix |mycal|, the macro expands to
  |mycal-2007-01-01|. 
\end{command}




==> pgfmanual-en-pgffor.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Repeating Things: The Foreach Statement}
\label{section-foreach}

This section describes the package |pgffor|, which is loaded
automatically by \tikzname, but not by \pgfname:

\begin{package}{pgffor}
  This package can be used independently of \pgfname, but works
  particularly well together with \pgfname\ and \tikzname. It defines
  two new commands: |\foreach| and |\breakforeach|.
\end{package}

\begin{command}{\foreach| |\meta{variables}| in |\meta{list}
    \meta{commands}}
  The syntax of this command is a bit complicated, so let us go
  through it step-by-step.

  In the easiest case, \meta{variables} is a single \TeX-command like
  |\x| or |\point|. (If you want to have some fun, you can also use
  active characters. If you do not know what active characters are,
  you are blessed.)

  Still in the easiest case, \meta{list} is either a comma-separated
  list of values surrounded by curly braces or it is the name of a
  macro that contain such a list of values. Anything can be used as a
  value, but numbers are most likely.

  Finally, in the easiest case, \meta{commands} is some \TeX-text in
  curly braces.

  With all these assumptions, the |\foreach| statement will execute
  the \meta{commands} repeatedly, once for every element of the
  \meta{list}. Each time the \meta{commands} are executed, the
  \meta{variable} will be set to the current value of the list
  item.

\begin{codeexample}[]
\foreach \x in {1,2,3,0} {[\x]}
\end{codeexample}

\begin{codeexample}[]
\def\mylist{1,2,3,0}
\foreach \x in \mylist {[\x]}
\end{codeexample}

  Note that in each execution of \meta{commands} the
  \meta{commands} are put in a \TeX\ group. This means that
  \emph{local changes to counters inside \meta{commands} do not
    persist till the next iteration}. For instance, if you add 1 to a
  counter inside \meta{commands} locally, then in the next iteration
  the counter will have the same value it had at the beginning of the
  first iteration. You have to add |\global| if you wish changes to
  persist from iteration to iteration.

  \medskip
  \textbf{Syntax for the commands.}
  Let us move on to a more complicated setting. The first
  complication occurs when the \meta{commands} are not some text in
  curly braces. If the |\foreach| statement does not encounter an
  opening brace, it will instead scan everything up to the next
  semicolon and use this as \meta{commands}. This is most useful in
  situations like the following:

\begin{codeexample}[]
\tikz
  \foreach \x in {0,1,2,3}
    \draw (\x,0) circle (0.2cm);
\end{codeexample}

  However, the ``reading till the next semicolon'' is not the whole
  truth. There is another rule: If a |\foreach| statement is directly
  followed by another |\foreach| statement, this second foreach
  statement is collected as \meta{commands}. This allows you to write
  the following:

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \x in {0,1,2,3}
    \foreach \y in {0,1,2,3}
      {
        \draw (\x,\y) circle (0.2cm);
        \fill (\x,\y) circle (0.1cm);
      }
\end{tikzpicture}
\end{codeexample}

  \medskip
  \textbf{The dots notation.}
  The second complication concerns the \meta{list}. If this
  \meta{list} contains the list item ``|...|'', this list item is replaced
  by the ``missing values.'' More precisely, the following happens:

  Normally, when a list item |...| is encountered, there should
  already have been \emph{two} list items before it, which where
  numbers. Examples of \emph{numbers} are |1|, |-10|, or
  |-0.24|. Let us call these numbers $x$ and $y$ and let $d := y-x$ be
  their difference. Next, there should also be one number following
  the three dots, let us call this number~$z$.

  In this situation, the part of the list reading
  ``$x$|,|$y$|,...,|$z$'' is replaced by ``$x$, $x+d$, $x+2d$, $x+3d$,
  \dots, $x+md$,'' where the last dots are semantic dots, not
  syntactic dots. The value $m$ is the largest number such that $x +
  md \le z$ if $d$ is positive or such that $x+md \ge z$ if $d$ is
  negative. 

  Perhaps it is best to explain this by some examples:  The following
  \meta{list} have the same effects:

  |\foreach \x in {1,2,...,6} {\x, }| yields \foreach \x in {1,2,...,6} {\x, }

  |\foreach \x in {1,2,3,...,6} {\x, }| yields \foreach \x in {1,2,3,...,6} {\x, }

  |\foreach \x in {1,3,...,11} {\x, }| yields \foreach \x in {1,3,...,11} {\x, }

  |\foreach \x in {1,3,...,10} {\x, }| yields \foreach \x in {1,3,...,10} {\x, }

  |\foreach \x in {0,0.1,...,0.5} {\x, }| yields \foreach \x in {0,0.1,...,0.5} {\x, }

  |\foreach \x in {a,b,9,8,...,1,2,2.125,...,2.5} {\x, }| yields \foreach \x in {a,b,9,8,...,1,2,2.125,...,2.5} {\x, }

  As can be seen, for fractional steps that are not multiples of
  $2^{-n}$ for some small $n$, rounding errors can occur pretty
  easily. Thus, in the second last case, |0.5| should probably be
  replaced by |0.501| for robustness.
  
  There is yet another special case for the |...| statement: If the
  |...| is used right after the first item in the list, that is, if
  there is an $x$, but no $y$, the difference $d$ obviously cannot be
  computed and is set to $1$ if the number $z$ following the dots is
  larger than $x$ and is set to $-1$ if $z$ is smaller:

  |\foreach \x in {1,...,6} {\x, }| yields \foreach \x in {1,...,6} {\x, }

  |\foreach \x in {9,...,3.5} {\x, }| yields \foreach \x in {9,...,3.5} {\x, }

  \medskip
  \textbf{Special handling of pairs.}
  Different list items are separated by commas. However, this causes a
  problem when the list items contain commas themselves as pairs like
  |(0,1)| do. In this case, you should put the items containing commas
  in braces as in |{(0,1)}|. However, since pairs are such a natural
  and useful case, they get a special treatment by the |\foreach|
  statement. When a list item starts with a |(| everything up to the
  next |)| is made part of the item. Thus, we can write things like
  the following:

\begin{codeexample}[]
\tikz
  \foreach \position in {(0,0), (1,1), (2,0), (3,1)}
    \draw \position rectangle +(.25,.5);
\end{codeexample}
  
  \medskip
  \textbf{Using the foreach-statement inside paths.}
  \tikzname\ allows you to use a |\foreach| statement inside a path
  construction. In such a case, the \meta{commands} must be path
  construction commands. Here are two examples:

\begin{codeexample}[]
\tikz
  \draw (0,0)
    \foreach \x in {1,...,3}
      { -- (\x,1) -- (\x,0) }
    ;
\end{codeexample}

\begin{codeexample}[]
\tikz \draw \foreach \p in {1,...,3} {(\p,1)--(\p,3) (1,\p)--(3,\p)};
\end{codeexample}
    
  \medskip
  \textbf{Multiple variables.}
  You will often wish to iterate over two variables at the same
  time. Since you can nest |\foreach| loops, this is normally
  straight-forward. However, you sometimes wish variables to
  iterate ``simultaneously.'' For example, we might be given a list of
  edges that connect two coordinates and might wish to iterate over
  these edges. While doing so, we would like the source and target of
  the edges to be set to two different variables.

  To achieve this, you can use the following syntax: The
  \meta{variables} may not only be a single \TeX-variable. Instead, it
  can also be a list of variables separated by slashes (|/|). In this
  case the list items can also be lists of values separated by
  slashes.

  Assuming that the \meta{variables} and the list items are lists of
  values, each time the \meta{commands} are executed, each of the
  variables in \meta{variables} is set to one part of the list making
  up the current list item. Here is an example to clarify this:

  \example |\foreach \x / \y in {1/2,a/b} {``\x\ and \y''}| yields
  \foreach \x / \y in {1/2,a/b} {``\x\ and \y''}.

  If some entry in the \meta{list} does not have ``enough'' slashes,
  the last entry will be repeated. Here is an example:
\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \x/\xtext in {0,...,3,2.72 / e}
    \draw (\x,0) node{$\xtext$};
\end{tikzpicture}
\end{codeexample}
  
  Here are more useful examples:
\begin{codeexample}[]
\begin{tikzpicture}
  % Define some coordinates:
  \path[nodes={circle,fill=examplefill,draw}]
    (0,0)    node(a) {a}
    (2,0.55) node(b) {b}
    (1,1.5)  node(c) {c}
    (2,1.75) node(d) {d};

  % Draw some connections:
  \foreach \source/\target in {a/b, b/c, c/a, c/d}
    \draw (\source) .. controls +(.75cm,0pt) and +(-.75cm,0pt)..(\target);  
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  % Let's draw circles at interesting points:
  \foreach \x / \y / \diameter in {0 / 0 / 2mm, 1 / 1 / 3mm, 2 / 0 / 1mm}
    \draw (\x,\y) circle (\diameter);
    
  % Same effect
  \foreach \center/\diameter in {{(0,0)/2mm}, {(1,1)/3mm}, {(2,0)/1mm}}
    \draw[yshift=2.5cm] \center circle (\diameter);
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[line cap=round,line width=3pt]
  \filldraw [fill=examplefill] (0,0) circle (2cm);

  \foreach \angle / \label in
    {0/3, 30/2, 60/1, 90/12, 120/11, 150/10, 180/9,
     210/8, 240/7, 270/6, 300/5, 330/4}
  {
    \draw[line width=1pt] (\angle:1.8cm) -- (\angle:2cm);
    \draw (\angle:1.4cm) node{\textsf{\label}};
  }
  
  \foreach \angle in {0,90,180,270}
    \draw[line width=2pt] (\angle:1.6cm) -- (\angle:2cm);

  \draw (0,0) -- (120:0.8cm); % hour
  \draw (0,0) -- (90:1cm);    % minute
\end{tikzpicture}%
\end{codeexample}

\begin{codeexample}[]
\tikz[shading=ball]
  \foreach \x / \cola in {0/red,1/green,2/blue,3/yellow}
    \foreach \y / \colb in {0/red,1/green,2/blue,3/yellow}
      \shade[ball color=\cola!50!\colb] (\x,\y) circle (0.4cm);
\end{codeexample}
\end{command}


\begin{command}{\breakforeach}
  If this command is given inside a |\foreach| command, no further
  executions of the \meta{commands} will occur. However, the current
  execution of the \meta{commands} is continued normally, so it is
  probably best to use this command only at the end of a |\foreach|
  command. 

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \x in {1,...,4}
    \foreach \y in {1,...,4}
    {
      \fill[red!50] (\x,\y) ellipse (3pt and 6pt);

      \ifnum \x<\y
        \breakforeach
      \fi
    }      
\end{tikzpicture}
\end{codeexample}
  
\end{command}




==> pgfmanual-en-pgfkeys.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Key Management}
\label{section-keys}

This section describes the package |pgfkeys|. It is loaded
automatically by both \pgfname\ and \tikzname.

\begin{package}{pgfkeys}
  This package can be used independently of \pgfname. Note that no
  other package of \pgfname\ needs to be loaded (so neither the
  emulation layer nor the system layer is needed). The Con\TeX t
  abbreviation is |pgfkey| if |pgfmod| is not loaded.
\end{package}



\subsection{Introduction}

\subsubsection{Comparison to Other Packages}

The |pgfkeys| package defines a key--value management system that is in
some sense similar to the more light-weight |keyval| system and the
improved |xkeyval| system. However, |pgfkeys| uses a slightly
different philosophy than these systems and it will coexist peacefully
with both of them.

The main differences between |pgfkeys| and |xkeyval| are the
following:

\begin{itemize}
\item |pgfkeys| organizes keys in a tree, while |keyval| and |xkeyval|
  use families. In |pgfkeys| the families correspond to the root
  entries of the key tree.
\item For efficiency reasons, |pgfkeys| does not directly support
  setting keys drawn from multiple families as |xkeyval| does. This
  can be emulated if necessary, but it will be slower than |xkeyval|'s
  native support.
\item |pgfkeys| has no save-stack impact (you will have to read the
  \TeX Book very carefully to appreciate this).
\item |pgfkeys| is slightly slower than |keyval|, but not much.
\item |pgfkeys| supports styles. This means that keys can just stand
  for other keys (which can stand for other keys in turn or which can
  also just execute some code). \tikzname\ uses this mechanism heavily.
\item |pgfkeys| supports multi-argument key code. This can, however,
  be emulated in |keyval|.
\item |pgfkeys| supports handlers. These are call-backs that are
  called when a key is not known. They are very flexible, in fact even
  defining keys in different ways is handled by, well, handlers.
\end{itemize}


\subsubsection{Quick Guide to Using the Key Mechanism}

The following quick guide to \pgfname's key mechanism only treats the
most commonly used features. For an in-depth discussion of what is
going on, please consult the remainder of this section.

Keys are organized in a large tree that is reminiscent of the Unix
file tree. A typical key might be, say, |/tikz/coordinate system/x|
or just |/x|. Again as in Unix, when you specify keys you can provide
the complete path of the key, but you usually just provide the name of
the key (corresponding to the file name without any path) and the path
is added automatically.

Typically (but not necessarily) some code is associated with a key. To
execute this code, you use the |\pgfkeys| command. This command takes
a list of so-called key--value pairs. Each pair is of the form
\meta{key}|=|\meta{value}. For each pair the |\pgfkeys| command will
execute the code stored for the \meta{key} with its parameter set to
\meta{value}.

Here is a typical example of how the |\pgfkeys| command is used:
\begin{codeexample}[code only]
\pgfkeys{/my key=hallo,/your keys/main key=something\strange,
         key name without path=something else}
\end{codeexample}

Now, to set the code that is stored in a key you do not need to learn
a new command. Rather, the |\pgfkeys| command can also be used to set
the code of a key. This is done using so-called \emph{handlers}. They
look like keys whose names look like ``hidden files in Unix'' since
they start with a dot. The handler for setting the code of a key is
appropriately called |.code| and it is used as follows:
\begin{codeexample}[]
\pgfkeys{/my key/.code=The value is '#1'.}
\pgfkeys{/my key=hi!}
\end{codeexample}
As you can see, in the first line we defined the code for the key
|/my key|. In the second line we executed this code with the parameter
set to |hi!|.

There are numerous handlers for defining a key. For instance, we can
also define a key whose value actually consists of more than one
parameter. 
\begin{codeexample}[]
\pgfkeys{/my key/.code 2 args=The values are '#1' and '#2'.}
\pgfkeys{/my key={a1}{a2}}
\end{codeexample}

We often want to have keys where the code is called with some default
value if the user does not provide a value. Not surprisingly, this is
also done using a handler, this time called |.default|.
\begin{codeexample}[]
\pgfkeys{/my key/.code=(#1)}
\pgfkeys{/my key/.default=hello}
\pgfkeys{/my key=hallo,/my key}
\end{codeexample}

The other way round, it is also possible to specify that a value
\emph{must} be specified, using a handler called
|.value required|. Finally, you can also require that no value
\emph{may} be specified using |.value forbidden|.

All keys for a package like, say, \tikzname\ start with the path
|/tikz|. We obviously do not like to write this path down every
time we use a key (so we do not have to write things like
|\draw[/tikz/line width=1cm]|). What we need is to somehow ``change
the default path to a specific location.'' This is done using the
handler |.cd| (for ``change directory''). Once this handler has been
used on a key, all subsequent keys {\itshape in the current call of
  |\pgfkeys| only} are automatically prefixed with this path, if
necessary.

Here is an example:
\begin{codeexample}[code only]
\pgfkeys{/tikz/.cd,line width=1cm,line cap=round}
\end{codeexample}
This makes it easy to define commands like |\tikzset|, which could be
defined as follows (the actual definition is a bit faster, but the
effect is the same):
\begin{codeexample}[code only]
\def\tikzset#1{\pgfkeys{/tikz/.cd,#1}}
\end{codeexample}

When a key is handled, instead of executing some code, the key can
also cause further keys to be executed. Such keys will be called
\emph{styles}. A style is, in essence, just a key list that should be
executed whenever the style is executed. Here is an example:
\begin{codeexample}[]
\pgfkeys{/a/.code=(a:#1)}
\pgfkeys{/b/.code=(b:#1)}
\pgfkeys{/my style/.style={/a=foo,/b=bar,/a=#1}}
\pgfkeys{/my style=wow}
\end{codeexample}
As the above example shows, style can also be parametrized, just like
the normal code keys.

As a typical use of styles, suppose we wish to setup the key |/tikz|
so that it will change the default path to |/tikz|. This can be
achieved as follows:
\begin{codeexample}[code only]
\pgfkeys{/tikz/.style=/tikz/.cd}
\pgfkeys{tikz,line width=1cm,draw=red}
\end{codeexample}

Note that when |\pgfkeys| is executed, the default path is set
to~|/|. This means that the first |tikz| will be completed to
|/tikz|. Then |/tikz| is a style and, thus, replaced by |/tikz/.cd|,
which changes the default path to |/tikz|. Thus, the |line width| is
correctly prefixed with |/tikz|.

\subsection{The Key Tree}

The |pgfkeys| package organizes keys in a so-called \emph{key
  tree}. This tree will be familiar to anyone who has used a Unix
operating system: A key is addressed by a path, which consists of
different parts separated by slashes. A typical key might be
|/tikz/line width| or just |/tikz| or something more complicated like
|/tikz/cs/x/.store in|.

Let us fix some further terminology: Given a key like |/a/b/c|, we
call the part leading up the last slash (|/a/b|) the \emph{path} of
the key. We call everything after the last slash (|c|) the \emph{name}
of the key (in a file system this would be the file name). 

We do not always wish to specify keys completely. Instead, we usually
specify only part of a key (typically only the name) and the
\emph{default path} is then added to the key at the front. So, when
the default path is |/tikz| and you 
refer to the (partial) key |line width|, the actual key that is used
is |/tikz/line width|. There is a simple rule for deciding whether a
key is a partial key or a full key: If it starts with a slash, then it
is a full key and it is not modified; if it does not start with
a slash, then the default path is automatically prefixed.

Note that the default path is not the same as a search path. In
particular, the default path is just a single path. When a partial key
is given, only this single default path is prefixed; |pgfkeys| does
not try to lookup the key in different parts of a search path. It is,
however, possible to emulate search paths, but a much more
complicated mechanism must be used.

When you set keys (to be explained in a moment), you can freely mix
partial and full keys and you can change the default path. This makes
it possible to temporarily use keys from another part of the key tree
(this turns out to be a very useful feature).

Each key (may) store some \emph{tokens} and there exist commands,
described below, for setting, getting, and changing the tokens stored
in a key. However, you will only very seldom use these commands
directly. Rather, the standard way of using keys is the |\pgfkeys|
command or some command that uses it internally like, say,
|\tikzset|. So, you may wish to skip the following commands and
continue with the next subsection.

\begin{command}{\pgfkeyssetvalue\marg{full key}\marg{token text}}
  Stores the \meta{token text} in the \meta{full key}. The \meta{full key}
  may not be a partial key, so no default-path-adding is done. The
  \meta{token text} can be arbitrary tokens and may even contain things
  like |#| or unbalanced \TeX-ifs.
\begin{codeexample}[]
\pgfkeyssetvalue{/my family/my key}{Hello, world!}
\pgfkeysvalueof{/my family/my key}  
\end{codeexample}

  The setting of a key is always local to the current \TeX\ group.
\end{command}

\begin{command}{\pgfkeyslet\marg{full key}\marg{macro}}
  Performs a |\let| statement so the the \meta{full key} pionts to the
  contents of \meta{macro}.
\begin{codeexample}[]
\def\helloworld{Hello, world!}
\pgfkeyslet{/my family/my key}{\helloworld}
\pgfkeysvalueof{/my family/my key}  
\end{codeexample}
  You should never let a key be equal to |\relax|. Such a key may or
  may not be indistinguishable from an undefined key.
\end{command}

\begin{command}{\pgfkeysgetvalue\marg{full key}\marg{macro}}
  Retrieves the tokens stored in the \meta{full key} and lets
  \meta{macro} be equal to these tokens. If the key has
  not been set, the \meta{macro} will be equal to |\relax|. 
\begin{codeexample}[]
\pgfkeyssetvalue{/my family/my key}{Hello, world!}
\pgfkeysgetvalue{/my family/my key}{\helloworld}
\helloworld
\end{codeexample}
\end{command}

\begin{command}{\pgfkeysvalueof\marg{full key}}
  Inserts the value stored in \meta{full key} at the current position
  into the text.

\begin{codeexample}[]
\pgfkeyssetvalue{/my family/my key}{Hello, world!}
\pgfkeysvalueof{/my family/my key}
\end{codeexample}
\end{command}


\begin{command}{\pgfkeysifdefined\marg{full key}\marg{if}\marg{else}}
  Checks whether this key was previously set using either
  |\pgfkeyssetvalue| or |\pgfkeyslet|. If so, the code in \meta{if} is
  executed, otherwise the code in \meta{else}.

  This command will use e\TeX's |\ifcsname| command, if available, for
  efficiency. This means, however, that it may behave differently for
  \TeX\ and for e\TeX\ when you set keys to |\relax|. For this reason
  you should not do so. 
\begin{codeexample}[]
\pgfkeyssetvalue{/my family/my key}{Hello, world!}
\pgfkeysifdefined{/my family/my key}{yes}{no}
\end{codeexample}
\end{command}


\subsection{Setting Keys}

Settings keys is done using a powerful command called |\pgfkeys|. This
command takes a list of so-called \emph{key--value pairs}. These are
pairs of the form \meta{key}|=|\meta{value}. The principle idea is the
following: For each pair in the list, some \emph{action} is
taken. This action can be one of the following:

\begin{enumerate}
\item A command is executed whose argument(s) are \meta{value}. This
  command is stored in a special subkey of \meta{key}.
\item The \meta{value} is stored in the \meta{key} itself.
\item If the key's name (the part after the last slahs) is a known
  \emph{handler}, then this handler will take care of the key.
\item If the key is totally unknown, one of several possible
  \emph{unknown key handlers} is called. 
\end{enumerate}

Addtionally, if the \meta{value} is missing, a default value may or
may not be substituted. Before we plunge into all the details,
let us have a quick look at the command itself.

\begin{command}{\pgfkeys\marg{key list}}
  The \meta{key list} should be a list of key--value pairs, separated
  by commas. A key--value pair can have the following two forms:
  \meta{key}|=|\meta{value} or just \meta{key}. Any spaces around the
  \meta{key} or around the \meta{value} are removed. It is permissible
  to surround both the \meta{key} or the \meta{value} in curly braces,
  which are also removed. Especially putting the \meta{value} in curly
  braces needs to be done quite often, namely whenever the \meta{value}
  contains an equal-sign or a comma.

  The key--value pairs in the list are handled in the order they
  appear. How this handling is done, exactly, is described in the rest
  of this section.

  If a \meta{key} is a partial key, the current value of the default
  path is prefixed to the \meta{key} and this ``upgraded'' key is
  then used. The default path is just the root path |/| when the first
  key is handled, but it may change later on. At the end of the
  command, the default path is reset to the value it had before this
  command was executed. 
  
  Calls of this command may be nested. Thus, it is permissible to call
  |\pgfkeys| inside the code that is executed for a key. Since the
  default path is restored after a call of |\pgfkeys|, the default
  path will not change when you call |\pgfkeys| while executing code
  for a key (which is exactly what you want).
\end{command}

\begin{command}{\pgfqkeys\marg{default path}\marg{key list}}
  This command has the same effect as |\pgfkeys{|\meta{default
      path}|/.cd,|\meta{key list}|}|, it is only marginally
  quicker. This command should not be used in user code, but rather in
  commands like |\tikzset| or |\pgfset| that get called very often.   
\end{command}

\begin{command}{\pgfkeysalso\marg{key list}}
  This command has execatly the same effect as |\pgfkeys|, only the
  default path is not modified before or after the keys are being
  set. This command is mainly intended to be called by the code that
  is being processed for a key.
\end{command}

\begin{command}{\pgfqkeysalso\marg{default path}\marg{key list}}
  This command has the same effect as |\pgfkeysalso{|\meta{default
      path}|/.cd,|\meta{key list}|}|, it is only quicker. Changing the
  default path inside a |\pgfkeyalso| is dangerous, so use with
  care. A rather safe place to call this command is at the beginning
  of a \TeX\ group.
\end{command}


\subsubsection{Default Arguments}

The arguments of the |\pgfkeys| command can either be of the form
\meta{key}|=|\meta{value} or of the form \meta{key} with the
value-part missing. In the second case, the |\pgfkeys| will try to
provide a \emph{default value} for the \meta{value}. If such a default
value is defined, it will be used as if you had written
\meta{key}|=|\meta{default value}.

In the following, the details of how default values are determined is
described; however, you should normally use the handlers |.default|
and |.value required| as described in
Section~\ref{section-default-handlers} and you can may wish to skip
the following details.

When |\pgfkeys| encounters a \meta{key} without an equal-sign, the
following happens:
\begin{enumerate}
\item The input is replaced by \meta{key}|=\pgfkeysnovalue|. In
  particular, the commands |\pgfkeys{my key}| and
  |\pgfkeys{my key=\pgfkeysnovalue}| have exactly the same effect and
  you can ``simulate'' a missing value by providing the value
  |\pgfkeysnovalue|, which is sometimes useful. 
\item If the \meta{value} is |\pgfkeysnovalue|, then it is checked
  whether the subkey \meta{key}|/.@def| exists. For instance, if you
  write |\pgfkeys{/my key}|, then it is checked whether the key
  |/my key/.@def| exists.
\item If the key \meta{key}|/.@def| exists, then the tokens stored in
  this key are used as \meta{value}.
\item If the key does not exist, then |\pgfkeysnovalue| is used as the
  \meta{value}.
\item At the end, if the \meta{value} is now equal to
  |\pgfkeysvaluerequired|, then the code  (or something fairly equivalent)
  |\pgfkeys{/errors/value required=|\meta{key}|{}}|
  is executed. Thus, by changing this key you can change the error
  message that is printed or you can handle the missing value in some
  other way.
\end{enumerate}



\subsubsection{Keys That Execute Commands}
\label{section-key-code}

After the transformation process described in the previous subsection,
we arrive at a key of the form \meta{key}=\meta{value}, where
\meta{key} is a full key. Different things can now happen, but always
the macro |\pgfkeyscurrentkey| will have been setup to expand to the
text of the \meta{key} that is currently being processed.

The first things that is tested is whether the key \meta{key}|/.@cmd|
exists. If this is the case, then it is assumed that this key stores
the code of a macro and this macro is executed. The argument of this
macro is \meta{value} directly followed by |\pgfeov|, which stands for
``end of value.'' The \meta{value} is not surrounded by braces. After
this code has been executed, |\pgfkeys| continues with the next key in
the \meta{key list}.

It may seem quite peculiar that the macro stored in the key
\meta{key}|/.@cmd| is not simply executed with the argument
|{|\meta{value}|}|. However, the approach taken in the |pgfkeys|
packages allows for more flexibility. For instance, assume that you
have a key that expects a \meta{value} of the form
``\meta{text}|+|\meta{more text}'' and wishes to store \meta{text} and
\meta{more text} in two different macros. This can be achieved as
follows:
\begin{codeexample}[]
\def\mystore#1+#2\pgfeov{\def\a{#1}\def\b{#2}}
\pgfkeyslet{/my key/.@cmd}{\mystore}
\pgfkeys{/my key=hello+world}

|\a| is \a, |\b| is \b.
\end{codeexample}

Naturally, defining the code to be stored in a key in the above manner
is too awkward. The following commands simplify things a bit, but the
usual manner of setting up code for a key is to use one of the
handlers described in Section~\ref{section-code-handlers}.

\begin{command}{\pgfkeysdef\marg{key}\marg{code}}
  This command temporarily defines a \TeX-macro with the argument list
  |#1\pgfeov| and then lets \meta{key}|/.@cmd| be equal to this
  macro. The net effect of all this is that you have then setup code
  for the key \meta{key} so that when you write
  |\pgfkeys{|\meta{key}|=|\meta{value}|}|, then the \meta{code} is
  executed with all occurrences of |#1| in \meta{code} being replaced
  by \meta{value}. (This behaviour is quite similar to the
  |\define@key| command of |keyval| and |xkeyval|).

\begin{codeexample}[]
\pgfkeysdef{/my key}{#1, #1.}
\pgfkeys{/my key=hello}
\end{codeexample}
\end{command}

\begin{command}{\pgfkeysedef\marg{key}\marg{code}}
  This command works like |\pgfkeysdef|, but it uses |\edef| rather
  than |\def| when defining the key macro. If you do not know the
  difference between the two, then you will not need this command;
  and if you know the difference, then you will know when you need this
  command.
\end{command}

\begin{command}{\pgfkeysdeargs\marg{key}\marg{argument pattern}\marg{code}}
  This command works like |\pgfkeysdef|, but it allows you to provide
  an arbitrary \meta{argument pattern} rather than just the simple
  single argument of |\pgfkeysdef|. 

\begin{codeexample}[]
\pgfkeysdefargs{/my key}{#1+#2}{\def\a{#1}\def\b{#2}}
\pgfkeys{/my key=hello+world}

|\a| is \a, |\b| is \b.
\end{codeexample}
\end{command}

\begin{command}{\pgfkeysedefargs\marg{key}\marg{argument pattern}\marg{code}}
  The |\edef| version of |\pgfkeysdefargs|.
\end{command}


\subsubsection{Keys That Store Values}

Let us continue with what happens when |\pgfkeys| processes the
current key and  the subkey \meta{key}|/.@cmd| is not defined. Then
it is checked whether the \meta{key} itself exists (has been
previously assigned a value using, for instance,
|\pgfkeyssetvalue|). In this case, the tokens stored in \meta{key} are
replaced by \meta{value} and |\pgfkeys| proceeds with the next key in
the \meta{key list}. 


\subsubsection{Keys That Are Handled}
\label{section-key-handlers}

If neither the \meta{key} itself nor the subkey \meta{key}|/.@cmd| are
defined, then the \meta{key} cannot be processed ``all by itself.''
Rather, a \meta{handler} is needed for this key. Most of the power of
|pgfkeys| comes from the proper use of such handlers.

Recall that the \meta{key} is always a full key (if it was not
originally, it has already been upgraded at this point to a full
key). It decomposed into  two parts:

\begin{enumerate}
\item The \meta{path} of \meta{key} (everything
  before the last slash) is stored in the macro |\pgfkeyscurrentpath|.
\item The \meta{name} of \meta{key} (everything
  after the last slash) is stored in the macro |\pgfkeyscurrentname|.

  It is recommended (but not necessary) that the name of a handler
  starts with a dot (but not with |.@|), so that they are easy to
  detect for the reader.  
\end{enumerate}

(For efficiency reasons, these two macros are only setup at this point;
so when code is executed for a key in the ``usual'' manner then these
macros are not setup.)

The |\pgfkeys| command now checks whether the key
|/handlers/|\meta{name}|/.@cmd| exists. If so, it should store a command
and this command is executed exactly in the same manner as described
in Section~\ref{section-key-code}.
Thus, this code gets the \meta{value} that was originally intended for
\meta{key} as its argument, followed by |\pgfeov|.
It is the job of the handlers to so something useful with the
\meta{value}.

For an example, let us write a handler that will output the value
stored in a key to the log file. We call this handler
|.print to log|. The idea is that when someone tries to use the key
|/my key/.print to log|, then this key will not be defined and the
handler gets executed. The handler will then have access to the
path-part of the key, which is |/my key|, via the macro
|\pgfkeyscurrentpath|. It can then lookup which value is stored in
this key and print it.

\begin{codeexample}[code only]
\pgfkeysdef{/handlers/.print to log}
{%
  \pgfkeysgetvalue{\pgfkeyscurrentpath}{\temp}
  \writetolog{\temp}
}
\pgfkeyssetvalue{/my key}{Hi!}
...
\pgfkeys{/my key/.print to log}
\end{codeexample}
The above code will print |Hi!| in the log, provided the macro
|\writetolog| is setup appropriately.

For a more interesting handler, let us program a handler that will
setup a key so that when the key is used some code is executed. This
code is given as \meta{value}. All the handler must do is to call
|\pgfkeysdef| for the path of the key (which misses the handler's
name) and assign the parameter value to it.
\begin{codeexample}[]
\pgfkeysdef{/handlers/.my code}{\pgfkeysdef{\pgfkeyscurrentpath}{#1}}
\pgfkeys{/my key/.my code=(#1)}
\pgfkeys{/my key=hallo}
\end{codeexample}


\subsubsection{Keys That Are Unknown}

For some keys, neither the key is defined nor its |.@cmd| subkey nor
is a handler defined for this key. In this case, it is checked whether
the key \meta{current path}|/.unknown/.@cmd| exists. Thus, when you try to
use the key |/tikz/strange|, then it is checked whether
|/tikz/.unknown/.@cmd| exists. If this key exists (which it does), it is
executed. This code can then try to make sense of the key. For
instance, the handler for \tikzname\ will try to interpret the key's
name as a color or as an arrow specification or as a \pgfname\
option.

You can setup unknown key handlers for your own keys by simply setting
the code of the key \meta{my path prefix}|/.unknown|. This also allows
you to setup ``search paths.'' The idea is that you would like keys to
be searched not only in a single default path, but in
several. Suppose, for instance, that you would like keys to be
searched 
for in |/a|, |/b|, and |/b/c|. We setup a key |/my search path| for
this:
\begin{codeexample}[code only]
\pgfkeys{/my search path/.unknown/.code=
  {%
    \let\searchname=\pgfkeyscurrentname%
    \pgfkeysalso{%
      /a/\searchname/.try=#1,
      /b/\searchname/.retry=#1,
      /b/c/\searchname/.retry=#1%
    }%
  }%
}
\pgfkeys{/my search path/.cd,foo,bar}
\end{codeexample}
In the above code, |foo| and |bar| will be searched for in the three
directories  |/a|, |/b|, and |/b/c|. 

If the key \meta{current path}|/.unknown/.@cmd| does not exist, the
handler |/handlers/.unknown| is invoked instead, which is always
defined and which prints an error message by default.

\subsection{Key Handlers}

We now describe which key handlers are defined by default. You can
also define new ones as described in Section~\ref{section-key-handlers}.


\subsubsection{Handlers for Path Management}

\begin{handler}{{.cd}}
  This handler causes the default path to be set to \meta{key}. Note that
  the default path is reset at the beginning of each call to
  |\pgfkeys| to be equal to~|/|.

  \example |\pgfkeys{/tikz/.cd,...}|
\end{handler}

\begin{handler}{{.is family}}
  This handler sets up things such that when \meta{key} is executed, then
  the current path is set to \meta{key}. A typical use is the following:
\begin{codeexample}[code only]
\pgfkeys{/tikz/.is family}
\pgfkeys{tikz,line width=1cm}  
\end{codeexample}
  The effect of this handler is the same as if you had written
  \meta{key}|/.style=|\meta{key}|/.cd|, only the code produced by the
  |.is family| handler is quicker.
\end{handler}


\subsubsection{Setting Defaults}
\label{section-default-handlers}

\begin{handler}{{.default}|=|\meta{value}}
  Sets the default value of \meta{key} to \meta{value}. This means
  that whenever no value is provided in a call to |\pgfkeys|, then
  this \meta{value} will be used instead.

  \example |\pgfkeys{/width/.default=1cm}|
\end{handler}

\begin{handler}{{.value required}}
  This handler causes the error message key |/erros/value required| to
  be issued whenever the \meta{key} is used without a value.

  \example |\pgfkeys{/width/.value required}|
\end{handler}

\begin{handler}{{.value forbidden}}
  This handler causes the error message key |/erros/value forbidden|
  to be issued whenever the \meta{key} is used with a value.

  This handler works be adding code to the code of the key. This means
  that you have to define the key first before you can use this
  handler. 
\begin{codeexample}[code only]
\pgfkeys{/my key/.code=I do not want an argument!}
\pgfkeys{/my key/.value forbidden}

\pgfkeys{/my key}     % Ok
\pgfkeys{/my key=foo} % Error
\end{codeexample}
\end{handler}


\subsubsection{Defining Key Codes}
\label{section-code-handlers}

A number of handlers exist for defining the code of keys.

\begin{handler}{{.code}|=|\meta{code}}
  This handler executes |\pgfkeysdef| with the parameters \meta{key}
  and \meta{code}. This means that, afterwards, whenever the
  \meta{key} is used, the \meta{code} gets executed. More precisely,
  when \meta{key}|=|\meta{value} is encountered in a key list,
  \meta{code} is executed with any occurrence of |#1| replaced by
  \meta{value}. As always, if no \meta{value} is given, the default
  value is used, if defined, or the special value |\pgfkeysnovalue|.

  It is permissible that \meta{code} calls the command |\pgfkeys|. It
  is also permissible the \meta{code} calls the command
  |\pgfkeysalso|, which is useful for styles, see below.

\begin{codeexample}[code only]
\pgfkeys{/par indent/.code={\parindent=#1},/par indent/.default=2em}
\pgfkeys{/par indent=1cm}
...
\pgfkeys{/par indent}
\end{codeexample}
\end{handler}

\begin{handler}{{.ecode}|=|\meta{code}}
  This handler works like |.code|, only the command |\pgfkeysedef| is
  used. 
\end{handler}


\begin{handler}{{.code 2 args}|=|\meta{code}}
  This handler works like |.code|, only two arguments rather than one
  are expected when the \meta{code} is executed. This means that when
  \meta{key}|=|\meta{value} is encountered in a key list, the
  \meta{value} should consist of two arguments. For instance,
  \meta{value} could be |{first}{second}|. Then \meta{code} is
  executed with any occurrence of |#1| replaced |first| and any
  occurrence of |#2| replaced by |second|.

  Because of the special way the \meta{value} is parsed, if you set
  \meta{value} to, for instance, |first| (without any braces), then
  |#1| will be set to |f| and |#2| will be set to |irst|. 

\begin{codeexample}[code only]
\pgfkeys{/page size/.code 2 args={\paperheight=#2\paperwidth=#1}}
\pgfkeys{/page size={30cm}{20cm}}
\end{codeexample}
\end{handler}

\begin{handler}{{.ecode 2 args}|=|\meta{code}}
  This handler works like |.code 2 args|, only an |\edef| is used
  rather than a |\def| to define the macro.
\end{handler}



\begin{handler}{{.code args}|=|\marg{argument pattern}\marg{code}}
  This handler also works like |.code|, but you can now specify an
  arbitrary \meta{argument pattern}. Such a pattern is a usual \TeX\
  macro pattern. For instance, suppose \meta{argument pattern} is
  |(#1/#2)| and \meta{key}|=|\meta{value} is encountered in a
  key list with \meta{value} being |(first/second)|. Then \meta{code}
  is executed with any occurrence of |#1| replaced |first| and any
  occurrence of |#2| replaced by |second|. So, the actual \meta{value}
  is matched against the \meta{argument pattern} in the standard \TeX\
  way. 

\begin{codeexample}[code only]
\pgfkeys{/page size/.code args={#1 and #2}{\paperheight=#2\paperwidth=#1}}
\pgfkeys{/page size=30cm and 20cm}
\end{codeexample}
\end{handler}

\begin{handler}{{.ecode args}|=|\marg{argument pattern}\marg{code}}
  This handler works like |.code args|, only an |\edef| is used
  rather than a |\def| to define the macro.
\end{handler}


There are also handlers for modifying existing keys.

\begin{handler}{{.add code}|=|\marg{prefix code}\marg{append code}}
  This handler adds code to an existing key. The \meta{prefix code} is
  added to the code stored in \meta{key}|/.@cmd| at the beginning, the
  \meta{append code} is added to this code at the end. Either can be
  empty. The argument list of \meta{code} cannot be changed using this
  handler. Note that both \meta{prefix code} and \meta{append code}
  may contain parameters like |#2|. 
  
\begin{codeexample}[code only]
\pgfkeys{/par indent/.code={\parindent=#1}}
\newdimen\myparindent  
\pgfkeys{/par indent/.add code={}{\myparindent=#1}}
...
\pgfkeys{/par indent=1cm} % This will set both \parindent and
                          % \myparindent to 1cm
\end{codeexample}
\end{handler}

\begin{handler}{{.prefix code}|=|\meta{prefix code}}
  This handler is a shortcut for \meta{key}|/.add code={|\meta{prefix
      code}|}{}|. That is, this handler adds the \meta{prefix code} at
  the beginning of the code stored in \meta{key}|/.@cmd|.
\end{handler}

\begin{handler}{{.append code}|=|\meta{append code}}
  This handler is a shortcut for \meta{key}|/.add code={}{|\meta{append
      code}|}{}|.
\end{handler}


\subsubsection{Defining Styles}

The following handlers allow you to define \emph{styles}. A style is a
key list that is processed whenever the style is given as a key in a
key list. Thus, a style ``stands for'' a certain key value
list. Styles can be parametrized just like normal code.

\begin{handler}{{.style}|=|\meta{key list}}
  This handler set things up so that whenever \meta{key}|=|\meta{value} is
  encountered in a key list, then the \meta{key list}, with every
  occurrence of |#1| replaced by \meta{value}, is processed
  instead. As always, if no \meta{value} is given, the default
  value is used, if defined, or the special value |\pgfkeysnovalue|.

  You can achieve the same effect by writing
  \meta{key}|/.code=\pgfkeysalso{|\meta{key list}|}|. This means, in
  particular, that the code of a key could also first execute some
  normal code and only then process some further keys. 

\begin{codeexample}[code only]
\pgfkeys{/par indent/.code={\parindent=#1}}
\pgfkeys{/no indent/.style={/par indent=0pt}}
\pgfkeys{/normal indent/.style={/par indent=2em}}
\pgfkeys{/no indent}
...
\pgfkeys{/normal indent}
\end{codeexample}
  The following example shows a parametrized style ``in action''.
\begin{codeexample}[]
\begin{tikzpicture}[outline/.style={draw=#1,fill=#1!20}]
  \node [outline=red]            {red box};
  \node [outline=blue] at (0,-1) {blue box};
\end{tikzpicture}
\end{codeexample}
\end{handler}

\begin{handler}{{.estyle}|=|\meta{key list}}
  This handler works like |.style|, only the \meta{code} is set using
  |\edef| rather than |\def|. Thus, all macros in the \meta{code} are
  expanded prior to saving the style.
\end{handler}

For styles the corresponding handlers as for normal code exist:

\begin{handler}{{.style 2 args}|=|\meta{key list}}
  This handler works like |.code 2 args|, only for styles. Thus, the
  \meta{key list} may contain occurrences of both |#1| and |#2| and
  when the style is used, two parameters must be given as
  \meta{value}. 
\begin{codeexample}[code only]
\pgfkeys{/paper height/.code={\paperheight=#1},/paper width/.code={\paperwidth=#1}}
\pgfkeys{/page size/.style 2 args={/paper height=#1,/paper width=#2}}
\pgfkeys{/page size={30cm}{20cm}}
\end{codeexample}
\end{handler}

\begin{handler}{{.estyle 2 args}|=|\meta{key list}}
  This handler works like |.style 2 args|, only an |\edef| is used
  rather than a |\def| to define the macro.
\end{handler}

\begin{handler}{{.style args}|=|\marg{argument pattern}\marg{key list}}
  This handler works like |.code args|, only for styles.
\end{handler}

\begin{handler}{{.estyle args}|=|\marg{argument pattern}\marg{code}}
  This handler works like |.ecode args|, only for styles.
\end{handler}

\begin{handler}{{.add style}|=|\marg{prefix key list}\marg{append key list}}
  This handler works like |.add code|, only for styles. However, it is
  permissible to add styles to keys that have previously been set
  using  |.code|. (It is also permissible to add normal \meta{code} to
  a key that has previously been set using |.style|). When you add a
  style to a key that was previously set using |.code|, the following
  happens: When \meta{key} is processed, the \meta{prefix key list}
  will be processed first, then the \meta{code} that was previously
  stored in \meta{key}|/.@cmd|, and then the keys in \meta{append key
    list} are processed.
\begin{codeexample}[code only]
\pgfkeys{/par indent/.code={\parindent=#1}}
\pgfkeys{/par indent/.add style={}{/my key=#1}}
...
\pgfkeys{/par indent=1cm} % This will set \parindent and
                          % then execute /my key=#1
\end{codeexample}
\end{handler}

\begin{handler}{{.prefix style}|=|\meta{prefix key list}}
  Works like |.add style|, but only for the prefix key list.
\end{handler}

\begin{handler}{{.append style}|=|\meta{append key list}}
  Works like |.add style|, but only for the append key list.
\end{handler}


\subsubsection{Defining Value-, Macro-, If- and Choice-Keys}

For some keys, the code that should be executed for them is rather
``specialized.'' For instance, it happens often that the code for a
key just sets a certain \TeX-if to true or false. For these case
predefine handlers make it easier to install the necessary code.

However, we start with some handlers that are used to manage the value
that is directly stored in a key.

\begin{handler}{{.initial}|=|\meta{value}}
  This handler sets the value of \meta{key} to \meta{value}. Note that
  no subkeys are involved. After this handler has been used, by the
  rules governing keys, you can subsequently change the value of the
  \meta{key} by just writing \meta{key}|=|\meta{value}. Thus, this
  handler is used to set the initial value of key.

\begin{codeexample}[code only]
\pgfkeys{/my key/.initial=red}
% "/my key" now stores the value "red"
\pgfkeys{/my key=blue}
% "/my key" now stores the value "blue"
\end{codeexample}

  Note that in the after the example, writing |\pgfkeys{/my key}| will not
  have the effect you might expect (namely that |blue| is inserted
  into the main text). Rather, |/my key| will be promoted to
  |/my key=\pgfkeysnovalue| and, thus, |\pgfkeysnovalue| will be
  stored in |/my key|.

  To retrieve the value stored in a key, the handler |.get| is used.
\end{handler}

\begin{handler}{{.get}|=|\meta{macro}}
  Executes a |\let| command so that \meta{macro} contains the contents
  stored in \meta{key}.  

\begin{codeexample}[]
\pgfkeys{/my key/.initial=red}
\pgfkeys{/my key=blue}
\pgfkeys{/my key/.get=\mymacro}
\mymacro
\end{codeexample}
\end{handler}

\begin{handler}{{.add}|=|\marg{prefix value}\marg{append value}}
  Adds the \meta{prefix value} and the beginning and the \meta{append
    value} at the end of the value stored in \meta{key}.
\end{handler}

The next handler is useful for the common situation where
\meta{key}|=|\meta{value} should cause the \meta{value} to be stored
in some macro. Note that, typically, you could just as well store the
value in the key itself.

\begin{handler}{{.store in}|=|\meta{macro}}
  This handler has the following effect: When you write
  \meta{key}|=|\meta{value}, the code
  |\def|\meta{macro}|{|\meta{value}|}| is executed. Thus, the given
  value is ``stored'' in the \meta{macro}.  
\begin{codeexample}[]
\pgfkeys{/text/.store in=\mytext}
\def\a{world} 
\pgfkeys{/text=Hello \a!}
\def\a{Gruffalo}
\mytext
\end{codeexample}
\end{handler}

\begin{handler}{{.estore in}|=|\meta{macro}}
  This handler is similar to |.store in|, only the code 
  |\edef|\meta{macro}|{|\meta{value}|}| is used. Thus, the
  macro-expanded version of \meta{value} is stored in the
  \meta{macro}. 
\begin{codeexample}[]
\pgfkeys{/text/.estore in=\mytext}
\def\a{world} 
\pgfkeys{/text=Hello \a!}
\def\a{Gruffalo}
\mytext
\end{codeexample}
\end{handler}

In another common situation a key is used to set a \TeX-if to true or
false. 

\begin{handler}{{.is if}|=|\meta{\TeX-if name}}
  This handler has the following effect: When you write
  \meta{key}|=|\meta{value}, it is first checked that \meta{value} is
  |true| or |false| (the default is |true| if no \meta{value} is
  given). If this is not the case, the error key
  |/errors/boolean expected| is executed. Otherwise, 
  the code |\|\meta{\TeX-if name}\meta{value} is executed, which sets
  the \TeX-if accordingly.
\begin{codeexample}[]
\newif\iftheworldisflat    
\pgfkeys{/flat world/.is if=theworldisflat}
\pgfkeys{/flat world=false}
\iftheworldisflat
  Flat
\else
  Round?
\fi
\end{codeexample}
\end{handler}

The next handler deals with the problem when a
\meta{key}|=|\meta{value} makes sense only for a small set of possible
\meta{value}s. For instance, the line cap can only be |rounded| or
|rect| or |butt|, but nothing else. For this situation the following
handler is useful.

\begin{handler}{{.is choice}}
  This handler set things up so that writing \meta{key}|=|\meta{value}
  will cause the subkey \meta{key}|/|\meta{value} to be executed. So,
  each of the different possible choices should be given by a subkey
  of \meta{key}.
\begin{codeexample}[code only]
\pgfkeys{/line cap/.is choice}
\pgfkeys{/line cap/round/.style={\pgfsetbuttcap}}
\pgfkeys{/line cap/butt/.style={\pgfsetroundcap}}
\pgfkeys{/line cap/rect/.style={\pgfsetrectcap}}
\pgfkeys{/line cap/rectangle/.style={/line cap=rect}}
...
\draw [/line cap=butt] ...
\end{codeexample}
  If the subkey \meta{key}|/|\meta{value} does not exist, the error
  key |/errors/unknown choice value| is executed.
\end{handler}


\subsubsection{Expanding Values}

When you write \meta{key}|=|\meta{value}, you usually wish to use the
\meta{value} ``as is.'' Indeed, great care is taken to ensure that you
can even use things like |#1| or unbalanced \TeX-ifs inside
\meta{value}. However, sometimes you want the \meta{value} to be
expanded before it is used. For instance, \meta{value} might be a
macro name like |\mymacro| and you do not want |\mymacro| to be used
as the macro, but rather the \emph{contents} of |\mymacro|. Thus,
instead of using \meta{value} you wish to use whatever \meta{value}
expands to. Instead of using some fancy |\expandafter| hackery, you
can use the following handlers:

\begin{handler}{{.expand once}|=|\meta{value}}
  This handler expands \meta{value} once (more precisely, it executes
  an |\expandafter| command on the first token of \meta{value}) and
  then process the resulting \meta{result} as if you had written
  \meta{key}|=|\meta{result}. Note that if \meta{key} contains a
  handler itself, this handler will be called normally.
\begin{codeexample}[]
\def\a{bottom}
\def\b{\a}
\def\c{\b}

\pgfkeys{/key1/.initial=\c}
\pgfkeys{/key2/.initial/.expand once=\c}
\pgfkeys{/key3/.initial/.expand twice=\c}
\pgfkeys{/key4/.initial/.expanded=\c}

\def\a{{\ttfamily\string\a}}
\def\b{{\ttfamily\string\b}}
\def\c{{\ttfamily\string\c}}

\begin{tabular}{ll}
Key 1:& \pgfkeys{/key1} \\
Key 2:& \pgfkeys{/key2} \\
Key 3:& \pgfkeys{/key3} \\
Key 4:& \pgfkeys{/key4}
\end{tabular}
\end{codeexample}
\end{handler}

\begin{handler}{{.expand twice}|=|\meta{value}}
  This handler works like saying \meta{key}|/.expand once/.expand once=|\meta{value}.
\end{handler}

\begin{handler}{{.expanded}|=|\meta{value}}
  This handler will completely expand \meta{value} (using |\edef|)
  before processing \meta{key}|=|\meta{result}.
\end{handler}


\subsubsection{Handlers for Testing Keys}

\begin{handler}{{.try}|=|\meta{value}}
  This handler causes the same things to be done as if
  \meta{key}|=|\meta{value} had been written instead. However, if
  neither \meta{key}|/.@cmd| nor the key itself is defined, no
  handlers will be called. Instead, 
  the execution of the key just stops. Thus, this handler will ``try''
  to use the key, but no further action is taken when the key is not
  defined.

  The \TeX-if |\||ifpgfkeyssuccess| will be set according to whether
  the \meta{key} was successfully executed or not. 
\begin{codeexample}[]
\pgfkeys{/a/.code=(a:#1)}
\pgfkeys{/b/.code=(b:#1)}
\pgfkeys{/x/.try=hmm,/a/.try=hallo,/b/.try=welt}
\end{codeexample}
\end{handler}

\begin{handler}{{.retry}|=|\meta{value}}
  This handler works just like |.try|, only it will not do anything if
  |\||ifpgfkeyssuccess| is false. Thus, this handler will only retry
  to set a key if ``the last attempt failed''. 
\begin{codeexample}[]
\pgfkeys{/a/.code=(a:#1)}
\pgfkeys{/b/.code=(b:#1)}
\pgfkeys{/x/.try=hmm,/a/.retry=hallo,/b/.retry=welt}
\end{codeexample}
\end{handler}


\subsubsection{Handlers for Key Inspection}

\begin{handler}{{.show value}}
  This handler executes a |\show| command on the value stored in
  \meta{key}. This is useful mostly for debugging.

  \example |\pgfkeys{/my/obscure key/.show value}|
\end{handler}

\begin{handler}{{.show code}}
  This handler executes a |\show| command on the code stored in
  \meta{key}|/.@cmd|. This is useful mostly for debugging.

  \example |\pgfkeys{/my/obscure key/.show code}|
\end{handler}

The following key is not a handler, but it also commonly used for
inspecting things:
\begin{key}{/utils/exec=\meta{code}}
  This key will simply execute the given \meta{code}. 

  \example |\pgfkeys{some key=some value,/utils/exec=\show\hallo,obscure key=obscure}|
\end{key}


\subsection{Error Keys}

In certain situations errors can occur, like using an undefined
key. In these situations error keys are executed. They should store a
macro that gets two arguments: The first is the offending key
(possibly only after macro expansion), the second is the value that
was passed as a parameter (also possibly only after macro expansion).

Currently, error keys are simply executed. In the future it might be a
good idea to have different subkeys that are executed depending on the
language currently set so that users get a localized error message.

\begin{key}{/errors/value required=\marg{offending key}\marg{value}}
  This key is executed whenever an \meta{offending key} is used
  without a value when a value is actually required. 
\end{key}

\begin{key}{/errors/value forbidden=\marg{offending key}\marg{value}}
  This key is executed whenever a key is used with a value when a
  value is actually forbidden.
\end{key}

\begin{key}{/errors/boolean expected=\marg{offending key}\marg{value}}
  This key is executed whenever a key setup using |.is if| gets called
  with a \meta{value} other than |true| or |false|.
\end{key}

\begin{key}{/errors/unknown choice value=\marg{offending key}\marg{value}}
  This key is executed whenever a choice is used as a \meta{value} for
  a key setup using the |.is choice| handler that is not defined.
\end{key}

\begin{key}{/errors/unknown key=\marg{offending key}\marg{value}}
  This key is executed whenever a key is unknown and no specific
  |.unknown| handler is found.
\end{key}


==> pgfmanual-en-pgfsys-commands.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Commands of the System Layer}

\makeatletter

\subsection{Beginning and Ending a Stream of System Commands}

A ``user'' of the \pgfname\ system layer (like the basic layer or a
frontend) will interface with the system layer by calling a stream of
commands starting with |\pgfsys@|. From the system layer's point of
view, these commands form a long stream. Between calls to the system
layer, control goes back to the user.

The driver files implement system layer commands by inserting
|\special| commands that implement the desired operation. For example,
|\pgfsys@stroke| will be mapped to |\special{pdf: S}| by the driver
file for |pdftex|.

For many drivers, when such a stream of specials starts, it is
necessary to install an appropriate transformation and perhaps perform
some more bureaucratic tasks. For this reason, every stream will start
with a |\pgfsys@beginpicture| and will end with a corresponding ending
command.

\begin{command}{\pgfsys@beginpicture}
  Called at the beginning of a |{pgfpicture}|. This command should
  ``setup things.''

  Most drivers will need to implement this command.
\end{command}

\begin{command}{\pgfsys@endpicture}
  Called at the end of a pgfpicture. 

  Most drivers will need to implement this command.
\end{command}

\begin{command}{\pgfsys@typesetpicturebox\marg{box}}
  Called \emph{after} a |{pgfpicture}| has been typeset. The picture
  will have been put in box \meta{box}. This command should insert the
  box into the normal text. The box \meta{box} will still be a ``raw''
  box that contains only the |\special|'s that make up the description
  of the picture. The  job of this command is to resize and shift
  \meta{box} according to the  baseline shift and the size of the
  box. 

  This command has a default implementation and need not be
  implemented by a driver file.
\end{command}

\begin{command}{\pgfsys@beginpurepicture}
  This version of the |\pgfsys@beginpicture| picture command can be
  used for pictures that are guaranteed not to contain any escaped
  boxes (see below). In this case, a driver might provide a more
  compact version of the command. 
  
  This command has a default implementation and need not be
  implemented by a driver file.
\end{command}

\begin{command}{\pgfsys@endpurepicture}
  Called at the end of a ``pure'' |{pgfpicture}|.
  
  This command has a default implementation and need not be
  implemented by a driver file.
\end{command}

Inside a stream it is sometimes necessary to ``escape'' back into
normal typesetting mode; for example to insert some normal text, but
with all of the current transformations and clippings being in
force. For this escaping, the following command is used:

\begin{command}{\pgfsys@hbox\marg{box number}}
  Called to insert a (horizontal) TeX box inside a
  |{pgfpicture}|.
  
  Most drivers will need to (re-)implement this command.
\end{command}

\begin{command}{\pgfsys@hboxsynced\marg{box number}}
  Called to insert a (horizontal) TeX box inside a
  |{pgfpicture}|, but with the current coordiante transformation
  matrix synced with the canvas transformation matrix. 

  This command should do the same as if you used
  |\pgflowlevelsynccm| followed by |\pgfsys@hbox|. However, the default
  implementation of this command will use a ``TeX-translation'' for
  the translation part of the transformation matrix. This will ensure
  that hyperlinks ``survive'' at least translations. On the other
  hand, a driver may choose to revert to a simpler
  implementation. This is done, for example, for the \textsc{svg}
  implementation, where a \TeX-translation makes no sense.
\end{command}



\subsection{Path Construction System Commands}

\begin{command}{\pgfsys@moveto\marg{x}\marg{y}}
  This command is used to start a path at a specific point
  $(x,y)$ or to move the current point of the current path to  $(x,y)$
  without drawing anything upon stroking (the current path is
  ``interrupted'').

  Both \meta{x} and \meta{y} are given as \TeX\ dimensions. It is the
  driver's job to transform these to the coordinate system of the
  backend. Typically, this means converting the \TeX\ dimension into a
  dimensionless multiple of $\frac{1}{72}\mathrm{in}$. The function
  |\pgf@sys@bp| helps with this conversion.

  \example Draw a line from $(10\mathrm{pt},10\mathrm{pt})$ to the
  origin of the picture. 
\begin{codeexample}[code only]
\pgfsys@moveto{10pt}{10pt}
\pgfsys@lineto{0pt}{0pt}
\pgfsys@stroke
\end{codeexample}

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\begin{command}{\pgfsys@lineto\marg{x}\marg{y}}
  Continue the current path to $(x,y)$ with
  a straight line.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\begin{command}{\pgfsys@curveto\marg{$x_1$}\marg{$y_1$}\marg{$x_2$}\marg{$y_2$}\marg{$x_3$}\marg{$y_3$}}
  Continue the current path to $(x_3,y_3)$
  with a Bézier curve that has the two control points  $(x_1,y_1)$ and  $(x_2,y_2)$.

  \example Draw a good approximation of a quarter circle:
\begin{codeexample}[code only]
\pgfsys@moveto{10pt}{0pt}
\pgfsys@curveto{10pt}{5.55pt}{5.55pt}{10pt}{0pt}{10pt}
\pgfsys@stroke
\end{codeexample}

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\begin{command}{\pgfsys@rect\marg{x}\marg{y}\marg{width}\marg{height}}
  Append a rectangle to the current path whose lower left corner is
  at $(x,y)$ and whose width and height in
  big points are  given by \meta{width} and \meta{height}.

  This command can be ``mapped back'' to |\pgfsys@moveto| and
  |\pgfsys@lineto| commands, but it is included since \pdf\ has a
  special, quick version of this command. 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\begin{command}{\pgfsys@closepath}
  Close the current path. This results in joining the current point of
  the path with the point specified by the last |\pgfsys@moveto|
  operation. Typically, this is preferable over using |\pgfsys@lineto|
  to the last point specified by a |\pgfsys@moveto|, since the line
  starting at this point and the line ending at this point will be
  smoothly joined by |\pgfsys@closepath|.

  \example Consider
\begin{codeexample}[code only]
\pgfsys@moveto{0pt}{0pt}
\pgfsys@lineto{10bp}{10bp}
\pgfsys@lineto{0bp}{10bp}
\pgfsys@closepath
\pgfsys@stroke
\end{codeexample}
  and
\begin{codeexample}[code only]
\pgfsys@moveto{0bp}{0bp}
\pgfsys@lineto{10bp}{10bp}
\pgfsys@lineto{0bp}{10bp}
\pgfsys@lineto{0bp}{0bp}
\pgfsys@stroke
\end{codeexample}
  
  The difference between the above will be that in the second triangle
  the corner at the origin will be wrong; it will just be the overlay
  of two lines going in different directions, not a sharp pointed
  corner.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}




\subsection{Canvas Transformation System Commands}

\begin{command}{\pgfsys@transformcm\marg{a}\marg{b}\marg{c}\marg{d}\marg{e}\marg{f}}
  Perform a concatenation of the canvas transformation matrix with the
  matrix given by the values \meta{a} to \meta{f}, see the \pdf\ or
  PostScript manual for details. The values \meta{a} to \meta{d} are
  dimensionless factors, \meta{e} and \meta{f} are \TeX\ dimensions 

  \example |\pgfsys@transformcm{1}{0}{0}{1}{1cm}{1cm}|.

  This command is protocoled, see Section~\ref{section-protocols}.  
\end{command}


\begin{command}{\pgfsys@transformshift\marg{x displacement}\marg{y displacement}}
  This command will change the origin of the canvas to $(x,y)$.

  This command has a default implementation and need not be
  implemented by a driver file.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@transformxyscale\marg{x scale}\marg{y scale}}
  This command will scale the canvas (and  everything that is drawn)
  by a factor of \meta{x scale} in the $x$-direction and \meta{y
    scale} in the  $y$-direction. Note that this applies to
  everything, including  lines. So a scaled line will have a different
  width and may even have a different width when going along the
  $x$-axis and when going along the $y$-axis, if the scaling is
  different in these directions. Usually, you do not want this.

  This command has a default implementation and need not be
  implemented by a driver file.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\subsection{Stroking, Filling, and Clipping System Commands}

\begin{command}{\pgfsys@stroke}
  Stroke the current path (as if it were drawn with a pen). A number
  of graphic state parameters influence this, which can be
  set using appropriate system commands described later.

  \begin{description}
  \item[Line width]
    The ``thickness'' of the line. A width of 0 is the thinnest width
    renderable on the device. On a high-resolution printer this may
    become invisible and should be avoided. A good choice is 0.4pt,
    which is the default.

  \item[Stroke color]
    This special color is used for stroking. If it is not set, the
    current color is used.
 
  \item[Cap]
    The cap describes how the endings of lines are drawn. A round cap
    adds a little half circle to these endings. A butt cap ends the
    lines exactly at the end (or start) point without anything
    added. A rectangular cap ends the lines like the butt cap, but the
    lines protrude over the endpoint by the line thickness. (See also
    the \pdf\ manual.) If the path has been closed, no cap
    is drawn.
 
  \item[Join]
    This describes how a bend (a join) in a path is rendered. A round
    join draws bends using small arcs. A bevel join just draws the two
    lines and then fills the join minimally so that it becomes
    convex. A miter join extends the lines so that they form a single
    sharp corner, but only up to a certain miter limit. (See the \pdf\
    manual once more.)
 
  \item[Dash]
    The line may be dashed according to a dashing pattern.
 
  \item[Clipping area]
    If a clipping area is established, only those parts of the path
    that are inside the clipping area will be drawn.
  \end{description}
  
  In addition to stroking a path, the path may also be used for
  clipping after it has been stroked. This will happen if the
  |\pgfsys@clipnext| is used prior to this command, see there for
  details.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\begin{command}{\pgfsys@closestroke}
  This command should have the same effect as first closing the path
  and then stroking it.

  This command has a default implementation and need not be
  implemented by a driver file.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\begin{command}{\pgfsys@fill}
  This command fills the area surrounded by the current path. If the
  path has not yet been closed, it is closed prior to filling. The
  path itself is not stroked. For self-intersecting paths or paths
  consisting of multiple parts, the nonzero winding number rule is
  used to determine whether a point is inside or outside the
  path, except if |\ifpgfsys@eorule| holds -- in which case the
  even-odd rule should be used. (See the \pdf\ or PostScript manual
  for details.)  
 
  The following graphic state parameters influence the filling:
 
  \begin{description}
  \item[Interior rule]
    If |\ifpgfsys@eorule| is set, the even-odd rule is used, otherwise
    the non-zero winding number rule.
 
  \item[Fill color]
    If the fill color is not especially set, the current color is
    used. 
 
  \item[Clipping area]
    If a clipping area is established, only those parts of the filling
    area that are inside the clipping area will be drawn.
  \end{description}

  In addition to filling the path, the path will also be used for
  clipping if |\pgfsys@clipnext| is used prior to this command.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@fillstroke}
  First, the path is filled, then the path is stroked. If the fill and
  stroke colors are the same (or if they are not specified and the
  current color is used), this yields almost the same as a
  |\pgfsys@fill|. However, due to the line thickness of the stroked
  path, the fill-stroked area will be slightly larger.

  In addition to stroking and filling the path, the path will also be
  used for clipping if |\pgfsys@clipnext| is used prior to this command.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\begin{command}{\pgfsys@discardpath}
 Normally, this command should ``throw away'' the current path.
 However, after |\pgfsys@clipnext| has been called, the current path
 should subsequently be used for clipping. See |\pgfsys@clipnext| for 
 details. 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\begin{command}{\pgfsys@clipnext}
  This command should be issued after a path has been constructed, but
  before it has been stroked and/or filled or discarded. When the
  command is used, the next stroking/filling/discarding command will
  first be executed normally. Then, afterwards, the just-used path
  will be used for subsequent clipping. If there has already been a
  clipping region, this region is intersected with the new clipping
  path (the clipping cannot get bigger). The nonzero winding number
  rule is used to determine whether a point is inside or outside the
  clipping area or the even-odd rule, depending on whether
  |\ifpgfsys@eorule| holds.
\end{command}




\subsection{Graphic State Option System Commands}

\begin{command}{\pgfsys@setlinewidth\marg{width}}
  Sets the width of lines, when stroked, to \meta{width}, which must
  be a \TeX\ dimension.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@buttcap}
  Sets the cap to a butt cap. See |\pgfsys@stroke|.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@roundcap}
  Sets the cap to a round cap. See |\pgfsys@stroke|.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@rectcap}
  Sets the cap to a rectangular cap. See |\pgfsys@stroke|.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@miterjoin}
  Sets the join to a miter join. See |\pgfsys@stroke|.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@setmiterlimit\marg{factor}}
  Sets the miter limit of lines to \meta{factor}. See
  the \pdf\ or PostScript for details on what the miter limit is.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@roundjoin}
  Sets the join to a round join. See |\pgfsys@stroke|.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@beveljoin}
  Sets the join to a bevel join. See |\pgfsys@stroke|.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@setdash\marg{pattern}\marg{phase}}
  Sets the dashing patter. \meta{pattern} should be a list of \TeX\
  dimensions lengths separated by commas. \meta{phase} should be a
  single dimension.

  \example |\pgfsys@setdash{3pt,3pt}{0pt}|
 
  The list of values in \meta{pattern} is used to determine the
  lengths of the ``on'' phases of the dashing and of the ``off''
  phases. For example, if \meta{pattern} is |3bp,4bp|, then the dashing
  pattern is ``3bp on followed by 4bp off, followed by 3bp on,
  followed by 4bp off, and so on.'' A pattern of |.5pt,4pt,3pt,1.5pt| means
  ``.5pt on, 4pt off, 3pt on, 1.5pt off, .5pt on, \dots'' If the
  number of entries is odd, the last one is used twice, so |3pt| means
  ``3pt on, 3pt off, 3pt on, 3pt off, \dots'' An empty list 
  means  ``always on.''
 
  The second argument determines the ``phase'' of the pattern. For
  example, for a pattern of |3bp,4bp| and a phase of |1bp|, the pattern
  would start: ``2bp on, 4bp off, 3bp on, 4bp off, 3bp on, 4bp off,
  \dots''

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

{\let\ifpgfsys@eorule=\relax
\begin{command}{\ifpgfsys@eorule}
  Determines whether the even odd rule is used for filling and
  clipping or not.
\end{command}
}


\subsection{Color System Commands}

The \pgfname\ system layer provides a number of system commands for
setting colors. These command coexist with commands from the |color|
and |xcolor| package, which perform similar functions. However, the
|color| package does not support having two different colors for
stroking and filling, which is a useful feature that is supported by
\pgfname. For this reason, the \pgfname\ system layer offers commands for
setting these colors separatedly. Also, plain \TeX\ profits from the
fact that \pgfname\ can set colors.

For \pdf, implementing these color commands is easy since \pdf\ 
supports different stroking and filling colors directly. For
PostScript, a more complicated approach is needed in which the colors
need to be stored in special PostScript variables that are set
whenever a stroking or a filling operation is done.

\begin{command}{\pgfsys@color@rgb\marg{red}\marg{green}\marg{blue}}
  Sets the color used for stroking and filling operations to the given 
  red/green/blue tuple (numbers between 0 and 1).

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@rgb@stroke\marg{red}\marg{green}\marg{blue}}
  Sets the color used for stroking operations to the given
  red/green/blue tuple (numbers between 0 and 1). 

  \example Make stroked text dark red: |\pgfsys@color@rgb@stroke{0.5}{0}{0}|

  The special stroking color is only used if the stroking color has
  been set since the last |\color| or |\pgfsys@color@xxx|
  command. Thus, each |\color| command will reset both the stroking
  and filling colors by calling |\pgfsys@color@reset|. 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@rgb@fill\marg{red}\marg{green}\marg{blue}}
  Sets the color used for filling operations to the given
  red/green/blue tuple (numbers between 0 and 1). This color may be
  different from the stroking color.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@cmyk\marg{cyan}\marg{magenta}\marg{yellow}\marg{black}}
  Sets the color used for stroking and filling operations to the given
  cymk tuple (numbers between 0 and 1). 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@cmyk@stroke\marg{cyan}\marg{magenta}\marg{yellow}\marg{black}}
  Sets the color used for stroking operations to the given cymk tuple
  (numbers between 0 and 1). 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@cmyk@fill\marg{cyan}\marg{magenta}\marg{yellow}\marg{black}}
  Sets the color used for filling operations to the given cymk tuple
  (numbers between 0 and 1). 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@cmy\marg{cyan}\marg{magenta}\marg{yellow}}
  Sets the color used for stroking and filling operations to the given
  cym tuple (numbers between 0 and 1). 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@cmy@stroke\marg{cyan}\marg{magenta}\marg{yellow}}
  Sets the color used for stroking operations to the given cym tuple
  (numbers between 0 and 1). 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@cmy@fill\marg{cyan}\marg{magenta}\marg{yellow}}
  Sets the color used for filling operations to the given cym tuple
  (numbers between 0 and 1). 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@gray\marg{black}}
  Sets the color used for stroking and filling operations to the given
  black value, where 0 means black and 1 means white.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@gray@stroke\marg{black}}
  Sets the color used for stroking operations to the given black value,
  where 0 means black and 1 means white.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@gray@fill\marg{black}}
  Sets the color used for filling operations to the given black value,
  where 0 means black and 1 means white.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@color@reset}
  This command will be called when the |\color| command is used. It
  should purge any internal settings of stroking and filling
  color. After this call, till the next use of a command like
  |\pgfsys@color@rgb@fill|, the current color installed by the
  |\color| command should be used.

  If the \TeX-if |\pgfsys@color@reset@inorder| is set to true, this
  command may ``assume'' that any call to a color command that sets
  the fill or stroke color came ``before'' the call to this command
  and may try to optimize the output accordingly.

  An example of an incorrect ``out of order'' call would be using
  |\pgfsys@color@reset| at the beginning of a box that is constructed
  using |\setbox|. Then, when the box is constructed, no special fill
  or stroke color might be in force. However, when the box is later on
  inserted at some point, a special fill color might already have been
  set. In this case, this command is not guaranteed to reset the color
  correctly. 
\end{command}

\begin{command}{\pgfsys@color@reset@inordertrue}
  Sets the optimized ``in order'' version of the color resetting. This
  is the default.
\end{command}

\begin{command}{\pgfsys@color@reset@inorderfalse}
  Switches off the optimized color resetting. 
\end{command}

\begin{command}{\pgfsys@color@unstacked\marg{\LaTeX\ color}}
  This slightly obscure command causes the color stack to be
  tricked. When called, this command should set the current color to
  \meta{\LaTeX\ color} without causing any change in the color stack.

  \example |\pgfsys@color@unstacked{red}|
\end{command}




\subsection{Pattern System Commands}


\begin{command}{\pgfsys@declarepattern
    \marg{name}\marg{$x_1$}\marg{$y_1$}\marg{$x_2$}\marg{$y_2$}
    \marg{$x$ step}\marg{$y$ step}\marg{code}\marg{flag}}
  This command declares a new colored or uncolored pattern, depending
  on whether \meta{flag} is |0|, which means uncolored, or |1|, which
  means colored. Uncolored patterns have no inherent color, the color
  is provided when they are set. Colored patters have an inherent
  color.

  The \meta{name} is a name for later use when the pattern is to be
  shown. The pairs $(x_1,y_1)$ and $(x_2,y_2)$ must describe a
  bounding box of the pattern \meta{code}.

  The tiling step of the pattern is given by \meta{$x$ step} and
  \meta{$y$ step}.

  \example
\begin{codeexample}[code only]
\pgfsys@declarepattern{hori}{-.5pt}{0pt}{.5pt}{3pt}{3pt}{3pt}
{\pgfsys@moveto{0pt}{0pt}\pgfsys@lineto{0pt}{3pt}\pgfsys@stroke}
{0}
\end{codeexample}
\end{command}

\begin{command}{\pgfsys@setpatternuncolored\marg{name}\marg{red}\marg{green}\marg{blue}}
  Sets the fill color to the pattern named \meta{name}. This pattern
  must previously have been declared with \meta{flag} set to |0|. The
  color of the pattern is given in the parameters \meta{red},
  \meta{green}, and \meta{blue} in the usual way.

  The fill color ``pattern''  will persist till the next color command
  that modifies the fill color.
\end{command}

\begin{command}{\pgfsys@setpatterncolored\marg{name}}
  Sets the fill color to the pattern named \meta{name}. This pattern 
  must have been declared with the |1| flag.
\end{command}



\subsection{Scoping System Commands}

The scoping commands are used to keep changes of the graphics state
local.

\begin{command}{\pgfsys@beginscope}
  Saves the current graphic state on a graphic state stack. All
  changes to the graphic state parameters mentioned for |\pgfsys@stroke|
  and |\pgfsys@fill| will be local to the current graphic state and 
  the old values will be restored after |\pgfsys@endscope| is used.
 
  \emph{Warning:} \pdf\ and PostScript differ with respect to the
  question of whether the current path is part of the graphic state or
  not. For this reason, you should never use this command unless the
  path is currently empty. For example, it might be a good idea to use 
  |\pgfsys@discardpath| prior to calling this command. 

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}

\begin{command}{\pgfsys@endscope}
  Restores the last saved graphic state.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}







\subsection{Image System Commands}

The system layer provides some commands for image inclusion.

\begin{command}{\pgfsys@imagesuffixlist}
  This macro should expand to a list of suffixes, separated by `:',
  that will be tried when searching for an image.

  \example |\def\pgfsys@imagesuffixlist{eps:epsi:ps}|
\end{command}


\begin{command}{\pgfsys@defineimage}
  Called, when an image should be defined. 
 
  This command does not take any parameters. Instead, certain macros
  will be preinstalled with appropriate values when this command is
  invoked. These are:
 
  \begin{itemize}
  \item\declare{|\pgf@filename|}
    File name of the image to be defined.

  \item\declare{|\pgf@imagewidth|}
    Will be set to the desired (scaled) width of the image.

  \item\declare{|\pgf@imageheight|}
    Will be set to the desired (scaled) height of the image.
 
    If this macro and also the height macro are empty, the image
    should have its ``natural'' size.
 
    If exactly only of them is specified, the undefined value the
    image is scaled so that the aspect ratio is kept.
 
    If both are set, the image is scaled in both directions
    independently, possibly changing the aspect ratio.
  \end{itemize}
 
  The following macros presumable mostly make sense for drivers that
  can handle \pdf: 

  \begin{itemize}
  \item \declare{|\pgf@imagepage|}
    The desired page number to be extracted from a multi-page
    ``image.''

  \item\declare{|\pgf@imagemask|}
    If set, it will be set to |/SMask x 0 R| where |x| is the \pdf\ 
    object number of a soft mask to be applied to the image.

  \item\declare{|\pgf@imageinterpolate|}
    If set, it will be set to |/Interpolate true| or
    |/Interpolate false|, indicating whether the image should be
    interpolated in \pdf. 
  \end{itemize}
 
  The command should now setup the macro |\pgf@image| such that calling
  this macro will result in typesetting the image. Thus, |\pgf@image| is
  the ``return value'' of the command.

  This command has a default implementation and need not be
  implemented by a driver file.
\end{command}



\subsection{Shading System Commands}


\begin{command}{\pgfsys@horishading\marg{name}\marg{height}\marg{specification}}
  Declares a horizontal shading for later use. The effect of this
  command should be the definition of a macro called |\@pgfshading|\meta{name}|!|
  (or |\csname @pdfshading|\meta{name}|!\endcsname|, to be
  precise). When invoked, this new macro should insert a shading at
  the current position. 
 
  \meta{name} is the name of the shading, which is also used in the
  output macro name. \meta{height} is the height of the shading and
  must be given as a TeX dimension like |2cm| or
  |10pt|. \meta{specification} is a shading color 
  specification as specified in Section~\ref{section-shadings}. The
  shading specification implicitly fixes the width of the shading. 
 
  When |\@pgfshading|\meta{name}|!| is invoked, it should insert a box
  of height \meta{height} and the width implicit in the shading
  declaration. 
\end{command}


\begin{command}{\pgfsys@vertshading\marg{name}\marg{width}\marg{specification}}
  Like the horizontal version, only for vertical shadings. This time,
  the height of the shading is implicit in \meta{specification} and
  the width is given as \meta{width}.
\end{command}

\begin{command}{\pgfsys@radialshading\marg{name}\marg{starting point}\marg{specification}}
  Declares a radial shading. Like the previous macros, this command
  should setup the macro |\@pgfshading|\meta{name}|!|, which upon
  invocation should insert a radial shading whose size is implicit in
  \meta{specification}.

  The parameter \meta{starting point} is a \pgfname\ point
  specifying the inner starting point of the shading.
\end{command}


\begin{command}{\pgfsys@radialshading\marg{name}\marg{lower left
      corner}\meta{upper right corner}\marg{type 4 function}}
 Declares a shading using a PostScript-like function that provides a
 color for each point. Like the previous macros, this command
 should setup the macro |\@pgfshading|\meta{name}|!| so that it will
 produce a box containing the desired shading.

 Parameter \meta{name} is the name of the shading. Parameter
 \meta{type 4 function} is a
 Postscript-like function (type 4 function of the PDF specification)
 as described in Section 3.9.4 of the PDF Specification version 1.7.
 Parameters \meta{lower left corner} and \meta{upper right corner} are
 \pgfname\ points that specifies the lower left and upper right
 corners of the shading.

 When \meta{type 4 function} is evaluated, the coordinate of the current
 point will be on the (virtual) PostScript stack in bp units. After
 the function has been evaluated, the stack should consist of three
 numbers (not integers! -- the Apple PDF renderer is broken in this
 regard, so add cvr's at the end if needed) that represent the red,
 green, and blue components of the color.

 A buggy function will result is \emph{totally unpredictable chaos} during
 rendering. 
\end{command}



\subsection{Transparency System Commands}

\begin{command}{\pgfsys@stroke@opacity\marg{value}}
  Sets the opacity of stroking operations.
\end{command}

\begin{command}{\pgfsys@fill@opacity\marg{value}}
  Sets the opacity of filling operations.
\end{command}

\begin{command}{\pgfsys@transparencygroupfrombox\marg{box}}
  This takes a TeX box and converts it into a transparency
  group. This means that any transparency settings apply to the box as
  a whole. For instance, if a box contains two overlapping black
  circles and you draw the box and, thus, the two cirlces normally
  with 50\% transparency, then the overlap will be darker than the
  rest. By comparison, if the circles are part of a transparency
  group, the overlap will get the same color as the rest.
\end{command}

\begin{command}{\pgfsys@fadingfrombox\marg{name}\marg{box}}
  Declares the fading \meta{name}. The \meta{box} is a \TeX-box. Its
  contents luminosity determines the opacity of the resulting
  fading. This means that the lighter a pixel inside the box, the more
  opaque the fading will be at this position.
\end{command}

\begin{command}{\pgfsys@usefading\meta{name}\marg{a}\marg{b}\marg{c}\marg{d}\marg{e}\marg{f}}
  Installs a previously declared fading \meta{name} in the current
  graphics state. Afterwards, all drawings will be masked by the
  fading. The fading should be centered on the origin and have its
  original size, except that the parameters \meta{a} to \meta{f}
  specify a transformation matrix that should be applied additionally
  to the fading before it is installed. The transformtion should not
  apply to the following graphics, however.
\end{command}


\begin{command}{\pgfsys@definemask}
  This command declares a fading (known as a soft mask in this
  context) based on an image and for usage with images. It
  works similar to |\pgfsys@defineimage|: Certain macros are set when
  the command is called. The result should be to set the macro
  |\pgf@mask| to a pdf object count that can subsequently be used as a
  transparency mask. The following macros will be set when this command is
  invoked: 
 
  \begin{itemize}
  \item \declare{|\pgf@filename|}
    File name of the mask to be defined.

  \item \declare{|\pgf@maskmatte|}
    The so-called matte of the mask (see the \pdf\ documentation for
    details). The matte is a color specification consisting of 1, 3 or
    4 numbers between 0 and 1. The number of numbers depends on the
    number of color channels in the image (not in the mask!). It will
    be assumed that the image has been preblended with this color.
  \end{itemize}
\end{command}




\subsection{Reusable Objects System Commands}

\begin{command}{\pgfsys@invoke\marg{literals}}
  This command gets protocoled literals and should insert them into
  the |.pdf| or |.dvi| file using an appropriate |\special|.
\end{command}

\begin{command}{\pgfsys@defobject\marg{name}\marg{lower
      left}\marg{upper right}\marg{code}}
  Declares an object for later use. The idea is that the object can be
  precached in some way and then be rendered more quickly when used
  several times. For example, an arrow head might be defined and
  prerendered in this way.
 
  The parameter \meta{name} is the name for later use. \meta{lower
  left} and \meta{upper right} are \pgfname\ points specifying a bounding
  box for the object. \meta{code} is the code for the object. The code
  should not be too fancy.

  This command has a default implementation and need not be
  implemented by a driver file.
\end{command}

\begin{command}{\pgfsys@useobject\marg{name}\marg{extra code}}
  Renders a previously declared object. The first parameter is the
  name of the the object. The second parameter is extra code that
  should be executed right \emph{before} the object is
  rendered. Typically, this will be some transformation code.

  This command has a default implementation and need not be
  implemented by a driver file.
\end{command}


\subsection{Invisibility System Commands}

All drawing or stroking or text rendering between calls of the
following commands should be suppressed. A similar effect can be
achieved by clipping against an empty region, but the following
commands do not open a graphics scope and can be opened and closed
``orthogonally'' to other scopes.

\begin{command}{\pgfsys@begininvisible}
  Between this command and the closing |\pgfsys@endinvisible| all
  output should be suppressed. Nothing should be drawn at all, which
  includes all paths, images and shadings. However, no groups (neither
  \TeX\ groups nor graphic state groups) should be opened by this
  command. 

  This command has a default implementation and need not be
  implemented by a driver file.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}
  
\begin{command}{\pgfsys@endinvisible}
  Ends the invisibility section, unless invisibility blocks have been
  nested. In this case, only the ``last'' one restores visibility.

  This command has a default implementation and need not be
  implemented by a driver file.

  This command is protocoled, see Section~\ref{section-protocols}.
\end{command}


\subsection{Position Tracking Commands}

The following commands are used to determine the position of text on a
page. This is a rather complicated process in general since at the
moment when the text is read by \TeX\ the final position cannot be
determined, yet. For example, the text might be put in a box which is
later put in the headline or perhaps in the footline or perhaps even
on a different page.

For these reasons, position tracking is typically a two-stage
process. In a first stage you indicate that a certain position is of
interest by \emph{marking} it. This will (depending on the details of
the backend driver) cause page coordinates or this position to be
written to a |.aux| file when the page is shipped. Possibly, the
position might also be determined at an even later stage. Then, on a
second run of \TeX, the position is read from the |.aux| file and can
be used.

\begin{command}{\pgfsys@markposition\marg{name}}
  Marks a position on the page. This command should be given while
  normal typesetting is done such as in
\begin{codeexample}[code only]
The value of $x$ is \pgfsys@markposition{here}important.
\end{codeexample}
  It causes the position |here| to be saved when the page is shipped
  out.
\end{command}

\begin{command}{\pgfsys@getposition\marg{name}\marg{macro}}
  This command retrieves a position that has been marked on an earlier
  run of \TeX\ on the current file. The \meta{macro} must be a macro
  name such as |\mymarco|. It will redefined such that it is
  \begin{itemize}
  \item either just |\relax| or
  \item a |\pgfpoint...| command.
  \end{itemize}
  The first case will happen when the position has not been marked at
  all or when the file is typeset for the first time, when the
  coordinates are not yet available.

  In the second case, executing \meta{macro} yields the position on
  the page that is to be interpreted as follows: A coordinate like
  |\pgfpoint{2cm}{3cm}| means ``2cm to the right and 3cm up from the
  origin of the page.'' The position of the origin of the page is not
  guaranteed to be at the lower left corner, it is only guaranteed
  that all pictures on a page use the same origin.

  To determine the lower left corner of a page, you can call
  |\pgfsys@getposition| with \meta{name} set to the special name
  |pgfpageorigin|. By shifting all positions by the amount returned by
  this call you can position things absolutely on a page.

  \example Referencing a point or the page:
\begin{codeexample}[code only]
The value of $x$ is \pgfsys@markposition{here}important.

Lots of text.

\hbox{\pgfsys@markposition{myorigin}%
\begin{pgfpicture}
  % Switch of size protocol
  \pgfpathmoveto{\pgfpointorigin}
  \pgfusepath{use as bounding box}

  \pgfsys@getposition{here}{\hereposition}
  \pgfsys@getposition{myorigin}{\thispictureposition}

  \pgftransformshift{\pgfpointscale{-1}{\thispictureposition}}
  \pgftransformshift{\hereposition}

  \pgfpathcircle{\pgfpointorigin}{1cm}
  \pgfusepath{draw}
\end{pgfpicture}}
\end{codeexample}
\end{command}


\subsection{Internal Conversion Commands}

The system commands take \TeX\ dimensions as input, but the dimensions
that have to be inserted into \pdf\ and PostScript files need to be
dimensionless values that are interpreted as multiples of
$\frac{1}{72}\mathrm{in}$. For example, the \TeX\ dimension $2bp$
should be inserted as |2| into a \pdf\ file and the \TeX\ dimension
$10\mathrm{pt}$ as |9.9626401|. To make this conversion easier, the following
command may be useful:

\begin{command}{\pgf@sys@bp\marg{dimension}}
  Inserts how many multiples of $\frac{1}{72}\mathrm{in}$ the
  \meta{dimension} is into the current protocol stream (buffered).

  \example |\pgf@sys@bp{\pgf@x}| or |\pgf@sys@bp{1cm}|.
\end{command}

Note that this command is \emph{not} a system command that can/needs
to be overwritten by a driver. 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-pgfsys-overview.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.



\section{Design of the System Layer}

\makeatletter


\subsection{Driver Files}
\label{section-pgfsys}

The \pgfname\ system layer mainly consists of a large number of
commands starting with |\pgfsys@|. These commands will be called
\emph{system commands} in the following. The higher layers
``interface'' with the system layer by calling these commands. The
higher layers should never use |\special| commands directly or even
check whether |\pdfoutput| is defined. Instead, all drawing requests
should be ``channeled'' through the system commands. 

The system layer is loaded and setup by the following package:

\begin{package}{pgfsys}
  This file provides ``default implementations'' of all system
  commands, but most simply produce a warning that they are not
  implemented. The actual implementations of the system commands for a
  particular driver like, say, |pdftex| reside in files called
  |pgfsys-xxxx.sty|, where |xxxx| is the driver name. These will be
  called \emph{driver files} in the following.

  When |pgfsys.sty| is loaded, it will try to determine which driver
  is used by loading |pgf.cfg|. This file should setup the macro
  |\pgfsysdriver| appropriately. The, |pgfsys.sty| will input the
  appropriate |pgfsys-|\meta{drivername}|.sty|. 
\end{package}

\begin{command}{\pgfsysdriver}
  This macro should expand to the name of the driver to be used by
  |pgfsys|. The default from |pgf.cfg| is |pgfsys-\Gin@driver|. This
  is very likely to be correct if you are using \LaTeX. For plain
  \TeX, the macro will be set to |pgfsys-pdftex.def| if |pdftex| is
  used and to |pgfsys-dvips.def| otherwise.
\end{command}

\begin{filedescription}{pgf.cfg}
  This file should setup the command |\pgfsysdriver| correctly. If
  |\pgfsysdriver| is already set to some value, the driver normally
  should not change it. Otherwise, it should make a ``good guess'' at
  which driver will be appropriate.
\end{filedescription}


The currently supported backend drivers are discussed in
Section~\ref{section-drivers}. 


\subsection{Common Definition Files}

Some drivers share many |\pgfsys@| commands. For the reason, files
defining these ``common'' commands are available. These files are
\emph{not} usable alone.

\begin{filedescription}{pgfsys-common-postscript}
  This file defines some |\pgfsys@| commands so that they produce
  appropriate PostScript code.
\end{filedescription}

\begin{filedescription}{pgfsys-common-pdf}
  This file defines some |\pgfsys@| commands so that they produce
  appropriate \textsc{pdf} code.
\end{filedescription}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-pgfsys-paths.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.



\section{The Soft Path Subsystem}

\label{section-soft-paths}

\makeatletter


This section describes a set of commands for creating \emph{soft
  paths} as opposed to the commands of the previous section, which
created \emph{hard paths}. A soft path is a path that can still be
``changed'' or ``molded.'' Once you (or the \pgfname\ system) is
satisfied with a soft path, it is turned into a hard path, which can
be inserted into the resulting |.pdf| or |.ps| file.

Note that the commands described in this section are ``high-level'' in
the sense that they are not implemented in driver files, but rather
directly by the \pgfname-system layer. For this reason, the commands for
creating soft paths do not start with |\pgfsys@|, but rather with
|\pgfsyssoftpath@|. On the other hand, as a user you will never use
these commands directly, so they are described as part of the
low-level interface. 



\subsection{Path Creation Process}

When the user writes a command like |\draw (0bp,0bp) -- (10bp,0bp);|
quite a lot happens behind the scenes:
\begin{enumerate}
\item
  The frontend command is translated by \tikzname\ into commands
  of the basic layer. In essence, the command is translated to
  something like
\begin{codeexample}[code only]
\pgfpathmoveto{\pgfpoint{0bp}{0bp}}
\pgfpathlineto{\pgfpoint{10bp}{0bp}}
\pgfusepath{stroke}
\end{codeexample}
\item
  The |\pgfpathxxxx| command do \emph{not} directly call ``hard''
  commands like |\pgfsys@xxxx|. Instead, the command |\pgfpathmoveto|
  invokes a special command called |\pgfsyssoftpath@moveto| and
  |\pgfpathlineto| invokes |\pgfsyssoftpath@lineto|. 

  The |\pgfsyssoftpath@xxxx| commands, which are described below,
  construct a soft path. Each time such a command is used, special
  tokens are added to the end of an internal macro that stores the
  soft path currently being constructed. 
\item
  When the |\pgfusepath| is encountered, the soft path stored in
  the internal macro is ``invoked.'' Only now does a special macro
  iterate over the soft path. For each line-to or move-to
  operation on this path it calls an appropriate |\pgfsys@moveto| or
  |\pgfsys@lineto| in order to, finally, create the desired hard path,
  namely, the string of literals in the |.pdf| or |.ps| file.
\item
  After the path has been invoked, |\pgfsys@stroke| is called to
  insert the literal for stroking the path.
\end{enumerate}

Why such a complicated process? Why not have |\pgfpathlineto| directly
call |\pgfsys@lineto| and be done with it? There are two reasons:
\begin{enumerate}
\item
  The \pdf\ specification requires that a path is not interrupted by
  any non-path-construction commands. Thus, the following code will
  result in a corrupted |.pdf|:
\begin{codeexample}[code only]
\pgfsys@moveto{0}{0}
\pgfsys@setlinewidth{1}
\pgfsys@lineto{10}{0}
\pgfsys@stroke
\end{codeexample}
  Such corrupt code is \emph{tolerated} by most viewers, but not
  always. It is much better to create only (reasonably) legal code.
\item
  A soft path can still be changed, while a hard path is fixed. For
  example, one can still change the starting and end points of a soft
  path or do optimizations on it. Such transformations are not possible
  on hard paths.
\end{enumerate}


\subsection{Starting and Ending a Soft Path}

No special action must be taken in order to start the creation of a
soft path. Rather, each time a command like |\pgfsyssoftpath@lineto|
is called, a special token is added to the (global) current soft path
being constructed.

However, you can access and change the current soft path. In this way,
it is possible to store a soft path, to manipulate it, or to invoke
it.

\begin{command}{\pgfsyssoftpath@getcurrentpath\marg{macro name}}
  This command will store the current soft path in \meta{macro name}.
\end{command}

\begin{command}{\pgfsyssoftpath@setcurrentpath\marg{macro name}}
  This command will set the current soft path to be the path stored in
  \meta{macro name}. This macro should store a path that has
  previously been extracted using the |\pgfsyssoftpath@getcurrentpath|
  command and has possibly been modified subsequently.
\end{command}

\begin{command}{\pgfsyssoftpath@invokecurrentpath}
  This command will turn the current soft path in a ``hard'' path. To
  do so, it iterates over the soft path and calls an appropriate
  |\pgfsys@xxxx| command for each element of the path. Note that the
  current soft path is \emph{not changed} by this command. Thus, in
  order to start a new soft path after the old one has been invoked
  and is no longer needed, you need to set the current soft path to be
  empty. This may seems strange, but it is often useful to immediately
  use the last soft path again.
\end{command}

\begin{command}{\pgfsyssoftpath@flushcurrentpath}
  This command will invoke the current soft path and then set it to be
  empty. 
\end{command}



\subsection{Soft Path Creation Commands}

\begin{command}{\pgfsyssoftpath@moveto\marg{x}\marg{y}}
  This command appends a ``move-to'' segment to the current soft
  path. The coordinates \meta{x} and \meta{y} are given as normal
  \TeX\ dimensions.

  \example One way to draw a line:
\begin{codeexample}[code only]
\pgfsyssoftpath@moveto{0pt}{0pt}
\pgfsyssoftpath@lineto{10pt}{10pt}
\pgfsyssoftpath@flushcurrentpath
\pgfsys@stroke
\end{codeexample}
\end{command}

\begin{command}{\pgfsyssoftpath@lineto\marg{x}\marg{y}}
  Appends a ``line-to'' segment to the current soft path. 
\end{command}

\begin{command}{\pgfsyssoftpath@curveto\marg{a}\marg{b}\marg{c}\marg{d}\marg{x}\marg{y}}
  Appends a ``curve-to'' segment to the current soft path with controls
  $(a,b)$ and $(c,d)$.
\end{command}

\begin{command}{\pgfsyssoftpath@rect\marg{lower left x}\marg{lower left y}\marg{width}\marg{height}}
  Appends a rectangle segment to the current soft path. 
\end{command}

\begin{command}{\pgfsyssoftpath@closepath}
  Appends a ``close-path'' segment to the current soft path. 
\end{command}




\subsection{The Soft Path Data Structure}

A soft path is stored in a standardized way, which makes it possible to
modify it before it becomes ``hard.'' Basically, a soft path is a long
sequence of triples. Each triple starts with a \emph{token} that
identifies what is going on. This token is followed by two dimensions in
braces. For example, the following is a soft path that means ``the
path starts at $(0\mathrm{bp}, 0\mathrm{bp})$ and then
continues in a straight line to $(10\mathrm{bp},
0\mathrm{bp})$.''

\begin{codeexample}[code only]
\pgfsyssoftpath@movetotoken{0bp}{0bp}\pgfsyssoftpath@linetotoken{10bp}{0bp}
\end{codeexample}

A curve-to is hard to express in this way since we need six numbers to
express it, not two. For this reasons, a curve-to is expressed using
three triples as follows: The command
\begin{codeexample}[code only]
\pgfsyssoftpath@curveto{1bp}{2bp}{3bp}{4bp}{5bp}{6bp}
\end{codeexample}
\noindent
results in the following three triples:
\begin{codeexample}[code only]
\pgfsyssoftpath@curvetosupportatoken{1bp}{2bp}
\pgfsyssoftpath@curvetosupportbtoken{3bp}{4bp}
\pgfsyssoftpath@curvetotoken{5bp}{6bp}
\end{codeexample}

These three triples must always ``remain together.'' Thus, a lonely
|supportbtoken| is forbidden.

In details, the following tokens exist:
\begin{itemize}
\item
  \declare{|\pgfsyssoftpath@movetotoken|} indicates a move-to
  operation. The two following numbers indicate the position to which
  the current point should be moved.
\item
  \declare{|\pgfsyssoftpath@linetotoken|} indicates a line-to
  operation. 
\item
  \declare{|\pgfsyssoftpath@curvetosupportatoken|} indicates the first
  control point of a curve-to operation. The triple must be followed
  by a |\pgfsyssoftpath@curvetosupportbtoken|.
\item
  \declare{|\pgfsyssoftpath@curvetosupportbtoken|} indicates the second
  control point of a curve-to operation. The triple must be followed
  by a |\pgfsyssoftpath@curvetotoken|.
\item
  \declare{|\pgfsyssoftpath@curvetotoken|} indicates the target
  of a curve-to operation.
\item
  \declare{|\pgfsyssoftpath@rectcornertoken|} indicates the corner of
  a rectangle on the soft path. The triple must be followed
  by a |\pgfsyssoftpath@rectsizetoken|.
\item
  \declare{|\pgfsyssoftpath@rectsizetoken|} indicates the size of
  a rectangle on the soft path.
\item
  \declare{|\pgfsyssoftpath@closepath|} indicates that the subpath
  begun with the last move-to operation should be closed. The parameter
  numbers are currently not important, but if set to anything
  different from |{0pt}{0pt}|, they should be set to the coordinate of
  the original move-to operation to which the path ``returns'' now.
\end{itemize}






==> pgfmanual-en-pgfsys-protocol.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{The Protocol Subsystem}

\label{section-protocols}

\makeatletter

This section describes commands for \emph{protocolling} literal text
created by \pgfname. The idea is that some literal text, like the string
of commands used to draw an arrow head, will be used over and over
again in a picture. It is then much more efficient to compute the
necessary literal text just once and to quickly insert it ``in a
single sweep.''

When protocolling is ``switched on,'' there is a ``current protocol''
to which literal text gets appended. Once all commands that needed to
be protocoled have been issued, the protocol can be obtained and
stored using |\pgfsysprotocol@getcurrentprotocol|. At any point, the
current protocol can be changed using a corresponding setting
command. Finally, |\pgfsysprotocol@invokecurrentprotocol| is used to
insert the protocoled commands into the |.pdf| or |.dvi| file.

Only those |\pgfsys@| commands can be protocolled that use the
command |\pgfsysprotocol@literal| interally. For example, the
definition of |\pgfsys@moveto| in |pgfsys-common-pdf.def| is
\begin{codeexample}[code only]
\def\pgfsys@moveto#1#2{\pgfsysprotocol@literal{#1 #2 m}}
\end{codeexample}
All ``normal'' system-level commands can be protocolled. However,
commands for creating or invoking shadings, images, or whole pictures
require special |\special|'s and cannot be protocolled.

\begin{command}{\pgfsysprotocol@literalbuffered\marg{literal text}}
  Adds the \meta{literal text} to the current protocol, after it has
  been ``|\edef|ed.'' This command will always protocol.
\end{command}

\begin{command}{\pgfsysprotocol@literal\marg{literal text}}
  First calls |\pgfsysprotocol@literalbuffered| on \meta{literal
    text}. Then, if protocolling is currently switched off, the
  \meta{literal text} is passed on to |\pgfsys@invoke|.
\end{command}

\begin{command}{\pgfsysprotocol@bufferedtrue}
  Turns on protocolling. All subsequent calls of
  |\pgfsysprotocol@literal| will append their argument to the current
  protocol. 
\end{command}

\begin{command}{\pgfsysprotocol@bufferedfalse}
  Turns off protocolling. Subsequent calls of
  |\pgfsysprotocol@literal| directly insert their argument into the
  current |.pdf| or |.ps|.

  Note that if the current protocol is not empty when protocolling is
  switched off, the next call to |\pgfsysprotocol@literal| will first
  flush the current protocol, that is, insert it into the file.
\end{command}

\begin{command}{\pgfsysprotocol@getcurrentprotocol\marg{macro name}}
  Stores the current protocol in \meta{macro name} for later use.
\end{command}

\begin{command}{\pgfsysprotocol@setcurrentprotocol\marg{macro name}}
  Sets the current protocol to \meta{macro name}.
\end{command}

\begin{command}{\pgfsysprotocol@invokecurrentprotocol}
  Inserts the text stored in the current protocol into the |.pdf| or
  |.dvi| file. This does \emph{not} change the current protocol.
\end{command}

\begin{command}{\pgfsysprotocol@flushcurrentprotocol}
  First inserts the current protocol, then sets the current protocol
  to the empty string.
\end{command}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-tikz-actions.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Actions on Paths}

\subsection{Overview}

Once a path has been constructed, different things can be done with
it. It can be drawn (or stroked) with a ``pen,'' it can be filled with
a color or shading, it can be used for clipping subsequent drawing, it
can be used to specify the extend of the picture---or  any
combination of these actions at the same time.

To decide what is to be done with a path, two methods can be
used. First, you can use a special-purpose command like |\draw| to
indicate that the path should be drawn. However, commands like |\draw|
and |\fill| are just abbreviations for special cases of the more
general method: Here, the |\path| command is used to specify the
path. Then, options encountered on the path indicate what should be
done with the path.

For example, |\path (0,0) circle (1cm);| means ``This is a path
consisting of a circle around the origin. Do not do anything with it
(throw it away).'' However, if the option |draw| is encountered
anywhere on the path, the circle will be drawn. ``Anywhere'' is any
point on the path where an option can be given, which is everywhere
where a path command like |circle (1cm)| or |rectangle (1,1)| or even
just |(0,0)| would also be allowed. Thus, the following commands all
draw the same circle:
\begin{codeexample}[code only]
\path [draw] (0,0) circle (1cm);
\path (0,0) [draw] circle (1cm);
\path (0,0) circle (1cm) [draw];
\end{codeexample}
Finally, |\draw (0,0) circle (1cm);| also draws a path, because
|\draw| is an abbreviation for |\path [draw]| and thus the command
expands to the first line of the above example.

Similarly, |\fill| is an abbreviation for |\path[fill]| and
|\filldraw| is an abbreviation for the command
|\path[fill,draw]|. Since options accumulate, the following commands
all have the same effect: 
\begin{codeexample}[code only]
\path [draw,fill]   (0,0) circle (1cm);
\path [draw] [fill] (0,0) circle (1cm);
\path [fill] (0,0) circle (1cm) [draw];
\draw [fill] (0,0) circle (1cm);
\fill (0,0) [draw] circle (1cm);
\filldraw (0,0) circle (1cm);
\end{codeexample}

In the following subsection the different actions are explained that
can be performed on a path. The following commands are abbreviations for
certain sets of actions, but for many useful combinations there are no
abbreviations:

\begin{command}{\draw}
  Inside |{tikzpicture}| this is an abbreviation for |\path[draw]|.
\end{command}

\begin{command}{\fill}
  Inside |{tikzpicture}| this is an abbreviation for |\path[fill]|.
\end{command}

\begin{command}{\filldraw}
  Inside |{tikzpicture}| this is an abbreviation for |\path[fill,draw]|.
\end{command}

\begin{command}{\pattern}
  Inside |{tikzpicture}| this is an abbreviation for |\path[pattern]|.
\end{command}

\begin{command}{\shade}
  Inside |{tikzpicture}| this is an abbreviation for |\path[shade]|.
\end{command}

\begin{command}{\shadedraw}
  Inside |{tikzpicture}| this is an abbreviation for |\path[shade,draw]|.
\end{command}

\begin{command}{\clip}
  Inside |{tikzpicture}| this is an abbreviation for |\path[clip]|.
\end{command}

\begin{command}{\useasboundingbox}
  Inside |{tikzpicture}| this is an abbreviation for |\path[use as bounding box]|.
\end{command}



\subsection{Specifying a Color}

The most unspecific option for setting colors is the following:

\begin{key}{/tikz/color=\meta{color name}}
  \indexoption{color option}%
  This option sets the color that is used for fill, drawing, and text
  inside the current scope. Any special settings for filling colors or
  drawing colors are immediately ``overruled'' by this option.

  The \meta{color name} is the name of a previously defined color. For
  \LaTeX\ users, this is just a normal ``\LaTeX-color'' and the
  |xcolor| extensions are allows. Here is an example:

\begin{codeexample}[]
\tikz \fill[color=red!20] (0,0) circle (1ex);
\end{codeexample}

  It is possible to ``leave out'' the |color=| part and you can also
  write:
\begin{codeexample}[]
\tikz \fill[red!20] (0,0) circle (1ex);
\end{codeexample}
  What happens is that every option that \tikzname\ does not know, like
  |red!20|, gets a ``second chance'' as a color name.

  For plain \TeX\ users, it is not so easy to specify colors since
  plain \TeX\ has no ``standardized'' color naming
  mechanism. Because of this, \pgfname\ emulates the |xcolor| package,
  though the emulation is \emph{extremely basic} (more precisely, what
  I could hack together in two hours or so). The emulation allows you
  to do the following:
  \begin{itemize}
  \item Specify a new color using |\definecolor|. Only the two color
    models |gray| and |rgb| are supported.
    \example |\definecolor{orange}{rgb}{1,0.5,0}|
  \item Use |\colorlet| to define a new color based on an old
    one. Here, the |!| mechanism is supported, though only ``once''
    (use multiple |\colorlet| for more fancy colors).
    \example |\colorlet{lightgray}{black!25}|
  \item Use |\color|\marg{color name} to set the color in the current
    \TeX\ group. |\aftergroup|-hackery is used to restore the color
    after the group.
  \end{itemize}
\end{key}

As pointed out above, the |color=| option applies to ``everything''
(except to shadings), which is not always what you want. Because of
this, there are several more specialized color options. For example,
the |draw=| option sets the color used for drawing, but does not
modify the color used for filling. These color options are documented
where the path action they influence is described.


\subsection{Drawing a Path}

You can draw a path using the following option:
\begin{key}{/tikz/draw=\meta{color} (default \normalfont is scope's color setting)}
  Causes the path to be drawn. ``Drawing'' (also known as
  ``stroking'') can be thought of as picking up a pen and moving it
  along the path, thereby leaving ``ink'' on the canvas.

  There are numerous parameters that influence how a line is drawn,
  like the thickness or the dash pattern. These options are explained
  below.

  If the optional \meta{color} argument is given, drawing is done
  using the given \meta{color}. This color can be different from the
  current filling color, which allows you to draw and fill a path with
  different colors. If no \meta{color} argument is given, the last
  usage of the |color=| option is used.

  If the special color name |none| is given, this option causes
  drawing to be ``switched off.'' This is useful if a style has
  previously switched on drawing and you locally wish to undo this
  effect. 

  Although this option is normally used on paths to indicate that the
  path should be drawn, it also makes sense to use the option with a
  |{scope}| or |{tikzpicture}| environment. However, this will
  \emph{not} cause all path to drawn. Instead, this just sets the
  \meta{color} to be used for drawing paths inside the environment.

\begin{codeexample}[]
\begin{tikzpicture}
  \path[draw=red] (0,0) -- (1,1) -- (2,1) circle (10pt);
\end{tikzpicture}
\end{codeexample}
\end{key}


The following subsections list the different options that influence
how a path is drawn. All of these options only have an effect if the
|draw| options is given (directly or indirectly).

\subsubsection{Graphic Parameters: Line Width, Line Cap, and Line Join}

\label{section-cap-joins}

\begin{key}{/tikz/line width=\meta{dimension} (initially 0.4pt)}
  Specifies the line width. Note the space.

\begin{codeexample}[]
  \tikz \draw[line width=5pt] (0,0) -- (1cm,1.5ex);
\end{codeexample}
\end{key}

There are a number of predefined styles that provide more ``natural''
ways of setting the line width. You can also redefine these
styles. 

\begin{stylekey}{/tikz/ultra thin}
  Sets the line width to 0.1pt.
\begin{codeexample}[]
  \tikz \draw[ultra thin] (0,0) -- (1cm,1.5ex);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/very thin}
  Sets the line width to 0.2pt.
\begin{codeexample}[]
  \tikz \draw[very thin] (0,0) -- (1cm,1.5ex);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/thin}
  Sets the line width to 0.4pt.
\begin{codeexample}[]
  \tikz \draw[thin] (0,0) -- (1cm,1.5ex);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/semithick}
  Sets the line width to 0.6pt.
\begin{codeexample}[]
  \tikz \draw[semithick] (0,0) -- (1cm,1.5ex);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/thick}
  Sets the line width to 0.8pt.
\begin{codeexample}[]
  \tikz \draw[thick] (0,0) -- (1cm,1.5ex);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/very thick}
  Sets the line width to 1.2pt.
\begin{codeexample}[]
  \tikz \draw[very thick] (0,0) -- (1cm,1.5ex);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/ultra thick}
  Sets the line width to 1.6pt.
\begin{codeexample}[]
  \tikz \draw[ultra thick] (0,0) -- (1cm,1.5ex);
\end{codeexample}
\end{stylekey}


\begin{key}{/tikz/line cap=\meta{type} (initially butt)}
  Specifies how lines ``end.'' Permissible \meta{type} are |round|,
  |rect|, and |butt|. They have the following effects:

\begin{codeexample}[]
\begin{tikzpicture}
  \begin{scope}[line width=10pt]
    \draw[line cap=rect]  (0,0 ) -- (1,0);
    \draw[line cap=butt]  (0,.5) -- (1,.5);
    \draw[line cap=round] (0,1 ) -- (1,1);
  \end{scope}
  \draw[white,line width=1pt]
    (0,0 ) -- (1,0) (0,.5) -- (1,.5) (0,1 ) -- (1,1);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/line join=\meta{type} (initially miter)}
  Specifies how lines ``join.'' Permissible \meta{type} are |round|,
  |bevel|, and |miter|. They have the following effects:

\begin{codeexample}[]
\begin{tikzpicture}[line width=10pt]
  \draw[line join=round] (0,0) -- ++(.5,1) -- ++(.5,-1);
  \draw[line join=bevel] (1.25,0) -- ++(.5,1) -- ++(.5,-1); 
  \draw[line join=miter] (2.5,0) -- ++(.5,1) -- ++(.5,-1); 
  \useasboundingbox (0,1.5); % make bounding box bigger
\end{tikzpicture}
\end{codeexample}

  \begin{key}{/tikz/miter limit=\meta{factor} (initially 10)}
    When you use the miter join and there is a very sharp corner (a
    small angle), the miter join may protrude very far over the actual
    joining point. In this case, if it were to protrude by 
    more than \meta{factor} times the line width, the miter join is
    replaced by a bevel join. 

\begin{codeexample}[]
\begin{tikzpicture}[line width=5pt]
  \draw                 (0,0) -- ++(5,.5) -- ++(-5,.5);
  \draw[miter limit=25] (6,0) -- ++(5,.5) -- ++(-5,.5);
  \useasboundingbox (14,0); % make bounding box bigger
\end{tikzpicture}
\end{codeexample}
  \end{key}
\end{key}

\subsubsection{Graphic Parameters: Dash Pattern}

\begin{key}{/tikz/dash pattern=\meta{dash pattern}}
  Sets the dashing pattern. The syntax is the same as in
  \textsc{metafont}. For example following pattern
  |on 2pt off 3pt on 4pt off 4pt| means ``draw
  2pt, then leave out 3pt, then draw 4pt once more, then leave out 4pt
  again, repeat''. 

\begin{codeexample}[]
\begin{tikzpicture}[dash pattern=on 2pt off 3pt on 4pt off 4pt]
  \draw (0pt,0pt) -- (3.5cm,0pt);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/dash phase=\meta{dash phase} (initially 0pt)}
  Shifts the start of the dash pattern by \meta{phase}.

\begin{codeexample}[]
\begin{tikzpicture}[dash pattern=on 20pt off 10pt]
  \draw[dash phase=0pt] (0pt,3pt) -- (3.5cm,3pt);
  \draw[dash phase=10pt] (0pt,0pt) -- (3.5cm,0pt);
\end{tikzpicture}
\end{codeexample}
\end{key}

As for the line thickness, some predefined styles allow you to set the
dashing conveniently.

\begin{stylekey}{/tikz/solid}
  Shorthand for setting a solid line as ``dash pattern.'' This is the default.

\begin{codeexample}[]
\tikz \draw[solid] (0pt,0pt) -- (50pt,0pt);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/dotted}
  Shorthand for setting a dotted dash pattern.

\begin{codeexample}[]
\tikz \draw[dotted] (0pt,0pt) -- (50pt,0pt);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/densely dotted}
  Shorthand for setting a densely dotted dash pattern.

\begin{codeexample}[]
\tikz \draw[densely dotted] (0pt,0pt) -- (50pt,0pt);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/loosely dotted}
  Shorthand for setting a loosely dotted dash pattern.

\begin{codeexample}[]
\tikz \draw[loosely dotted] (0pt,0pt) -- (50pt,0pt);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/dashed}
  Shorthand for setting a dashed dash pattern.

\begin{codeexample}[]
\tikz \draw[dashed] (0pt,0pt) -- (50pt,0pt);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/densely dashed}
  Shorthand for setting a densely dashed dash pattern.

\begin{codeexample}[]
\tikz \draw[densely dashed] (0pt,0pt) -- (50pt,0pt);
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/loosely dashed}
  Shorthand for setting a loosely dashed dash pattern.

\begin{codeexample}[]
\tikz \draw[loosely dashed] (0pt,0pt) -- (50pt,0pt);
\end{codeexample}
\end{stylekey}


\subsubsection{Graphic Parameters: Draw Opacity}

When a line is drawn, it will normally ``obscure'' everything behind
it as if you has used perfectly opaque ink. It is also possible to ask
\tikzname\ to use an ink that is a little bit (or a big bit)
transparent using the |draw opacity| option. This is explained in
Section~\ref{section-tikz-transparency} on transparency in more detail.



\subsubsection{Graphic Parameters: Arrow Tips}

When you draw a line, you can add arrow tips at the ends. It is
only possible to add one arrow tip at the start and one at the end. If
the path consists of several segments, only the last segment gets
arrow tips. The behavior for paths that are closed is not specified
and may change in the future.

\begin{key}{/tikz/arrows=\meta{start arrow kind}|-|\meta{end arrow kind}}
  This option sets the start and end arrow tips (an empty value as in |->|
  indicates that no arrow tip should be drawn at the start).%
  \indexoption{arrows}

  \emph{Note: Since the arrow option is so often used, you can leave
    out the text |arrows=|.} What happens is that every option that
  contains a |-| is interpreted as an arrow specification.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[->]        (0,0)   -- (1,0);
  \draw[o-stealth] (0,0.3) -- (1,0.3);
\end{tikzpicture}
\end{codeexample}

  The permissible values are all predefined arrow tips, though
  you can also define new arrow tip kinds as explained in
  Section~\ref{section-arrows}. This is often necessary to obtain
  ``double'' arrow tips and arrow tips that have a fixed size. Since
  |pgflibraryarrows| is loaded by default, all arrow tips described in
  Section~\ref{section-library-arrows} are available.

  One arrow tip kind is special: |>| (and all arrow tip kinds containing the
  arrow tip kind such as |<<| or \verb!>|!). This arrow tip type is not  
  fixed. Rather, you can redefine it using the |>=| option, see
  below. 

  \example You can also combine arrow tip types as in
\begin{codeexample}[]
\begin{tikzpicture}[thick]
  \draw[to reversed-to]   (0,0) .. controls +(.5,0) and +(-.5,-.5) .. +(1.5,1);
  \draw[[-latex reversed] (1,0) .. controls +(.5,0) and +(-.5,-.5) .. +(1.5,1);
  \draw[latex-)]          (2,0) .. controls +(.5,0) and +(-.5,-.5) .. +(1.5,1);
  \useasboundingbox (-.1,-.1) rectangle (3.1,1.1); % make bounding box bigger
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/>=\meta{end arrow kind}}
  This option can be used to redefine the ``standard'' arrow tip |>|. The
  idea is that different people have different ideas what arrow tip kind
  should normally be used. I prefer the arrow tip of \TeX's |\to| command
  (which is used in things like $f\colon A \to B$). Other people will
  prefer \LaTeX's standard arrow tip, which looks like this: \tikz
  \draw[-latex] (0,0) -- (10pt,1ex);. Since the arrow tip kind |>| is
  certainly the most ``natural'' one to use, it is kept free of any
  predefined meaning. Instead, you can change it by saying |>=to| to
  set the ``standard'' arrow tip kind to \TeX's arrow tip, whereas |>=latex|
  will set it to \LaTeX's arrow tip and |>=stealth| will use a
  \textsc{pstricks}-like arrow tip.

  Apart from redefining the arrow tip kind |>| (and |<| for the start),
  this option also redefines the following arrow tip kinds: |>| and |<| as
  the swapped version of \meta{end arrow kind}, |<<| and |>>| as
  doubled versions, |>>| and |<<| as swapped doubled versions, %>>
  and \verb!|<! and \verb!>|! as arrow tips ending with a vertical bar.

\begin{codeexample}[]
\begin{tikzpicture}[scale=2]
  \begin{scope}[>=latex]
    \draw[->]    (0pt,6ex) -- (1cm,6ex);
    \draw[>->>]  (0pt,5ex) -- (1cm,5ex); 
    \draw[|<->|] (0pt,4ex) -- (1cm,4ex);
  \end{scope}
  \begin{scope}[>=diamond]
    \draw[->]    (0pt,2ex) -- (1cm,2ex);
    \draw[>->>]  (0pt,1ex) -- (1cm,1ex);
    \draw[|<->|] (0pt,0ex) -- (1cm,0ex);
  \end{scope} 
\end{tikzpicture}
\end{codeexample} 
% <<
\end{key}

\begin{key}{/tikz/shorten >=\meta{dimension} (initially 0pt)}
  This option will shorten the end of lines by the given
  \meta{dimension}. If you specify an arrow tip, lines are already
  shortened a bit such that the arrow tip touches the specified endpoint
  and does not ``protrude over'' this point. Here is an example:

\begin{codeexample}[]
\begin{tikzpicture}[line width=20pt]
  \useasboundingbox (0,-1.5) rectangle (3.5,1.5);
  \draw[red]        (0,0) -- (3,0);
  \draw[gray,->]    (0,0) -- (3,0);
\end{tikzpicture}
\end{codeexample}

  The |shorten >| option allows you to shorten the end on the line
  \emph{additionally} by the given distance. This option can also be
  useful if you have not specified an arrow tip at all.

\begin{codeexample}[]
\begin{tikzpicture}[line width=20pt]
  \useasboundingbox (0,-1.5) rectangle (3.5,1.5);
  \draw[red]                     (0,0) -- (3,0);
  \draw[-to,shorten >=10pt,gray] (0,0) -- (3,0);
\end{tikzpicture}
\end{codeexample}
\end{key}


\begin{key}{/tikz/shorten <=\meta{dimension}}
  Works like |shorten >|, but for the start.
\end{key}



\subsubsection{Graphic Parameters: Double Lines and Bordered Lines}

\begin{key}{/tikz/double=\meta{core color} (default white)}
  This option causes ``two'' lines to be drawn instead of a single
  one. However, this is not what really happens. In reality, the path
  is drawn twice. First, with the normal drawing color, secondly with
  the \meta{core color}, which is normally |white|. Upon the second
  drawing, the line width is reduced. The net effect is that it
  appears as if two lines had been drawn and this works well even with
  complicated, curved paths:

\begin{codeexample}[]
\tikz \draw[double]
  plot[smooth cycle] coordinates{(0,0) (1,1) (1,0) (0,1)};
\end{codeexample}

  You can also use the doubling option to create an effect in which a
  line seems to have a certain ``border'':

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) -- (1,1);
  \draw[draw=white,double=red,very thick] (0,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/double distance=\meta{dimension} (initially 0.6pt)}
  Sets the distance the ``two'' lines are spaced apart. In reality,
  this is the thickness of the line that is used 
  to draw the path for the second time. The thickness of the
  \emph{first} time the path is drawn is twice the normal line width
  plus the given \meta{dimension}. As a side-effect, this option
  ``selects'' the |double| option.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[very thick,double]              (0,0) arc (180:90:1cm);
  \draw[very thick,double distance=2pt] (1,0) arc (180:90:1cm);
  \draw[thin,double distance=2pt]       (2,0) arc (180:90:1cm);
\end{tikzpicture}
\end{codeexample}
\end{key}


  




\subsection{Filling a Path}
\label{section-rules}
To fill a path, use the following option:
\begin{key}{/tikz/fill=\meta{color} (default \normalfont is scope's color setting)}
  This option causes the path to be filled. All unclosed parts of the
  path are first closed, if necessary. Then, the area enclosed by the
  path is filled with the current filling color, which is either the
  last color set using the general |color=| option or the optional
  color \meta{color}. For self-intersection paths and for paths
  consisting of several closed areas, the ``enclosed area'' is
  somewhat complicated to define and two different definitions exist,
  namely the nonzero winding number rule and the even odd rule, see
  the explanation of these options, below.

  Just as for the |draw| option, setting \meta{color} to |none|
  disables filling locally.

\begin{codeexample}[]
\begin{tikzpicture}
  \fill (0,0) -- (1,1) -- (2,1);
  \fill (4,0) circle (.5cm)  (4.5,0) circle (.5cm);
  \fill[even odd rule] (6,0) circle (.5cm)  (6.5,0) circle (.5cm);
  \fill (8,0) -- (9,1) -- (10,0) circle (.5cm);
\end{tikzpicture}
\end{codeexample}

  If the |fill| option is used together with the |draw| option (either
  because both are given as options or because a |\filldraw| command
  is used), the path is filled \emph{first}, then the path is drawn
  \emph{second}. This is especially useful if different colors are
  selected for drawing and for filling. Even if the same color is
  used, there is a difference between this command and a plain 
  |fill|: A ``filldrawn'' area will be slightly larger than a filled
  area because of the thickness of the ``pen.''

\begin{codeexample}[]
\begin{tikzpicture}[fill=examplefill,line width=5pt]
  \filldraw (0,0) -- (1,1) -- (2,1);
  \filldraw (4,0) circle (.5cm)  (4.5,0) circle (.5cm);
  \filldraw[even odd rule] (6,0) circle (.5cm)  (6.5,0) circle (.5cm);
  \filldraw (8,0) -- (9,1) -- (10,0) circle (.5cm);
\end{tikzpicture}
\end{codeexample}
\end{key}



\subsubsection{Graphic Parameters: Fill Pattern}

\label{section-fill-pattern}
Instead of filling a path with a single solid color, it is also
possible to fill it with a \emph{tiling pattern}. Imagine a small tile
that contains a simple picture like a star. Then these tiles are
(conceptually) repeated infinitely in all directions, but clipped
against the path.

Tiling patterns come in two variants: \emph{inherently 
  colored patterns} and \emph{form-only patterns}. An inherently colored
pattern is, say, a red star with a black border and will always look
like this. A form-only pattern may have a different color each time
it is used, only the form of the pattern will stay the same. As such,
form-only patterhns do not have any colors of their own, but when it
is used the current \emph{pattern color} is used as its color.

Patterns are not overly flexible. In particular, it is not possible to
change the size or orientation of a pattern without declaring a new
pattern. For complicated case, it may be easier to use two nested
|\foreach| statements to simulate a pattern, but patterns are rendered
\emph{much} more quickly than simulated ones.

\begin{key}{/tikz/pattern=\meta{name} (default \normalfont is scope's pattern)}
  This option causes the path to be filled with a pattern. If the
  \meta{name} is given, this pattern is used, otherwise the pattern
  set in the enclosing scope is used. As for the |draw| and |fill|
  options, setting \meta{name} to |none| disables filling locally.

  The pattern works like a fill color. In particular, setting a new
  fill color will fill the path with a solid color once more.

  Strangely, no \meta{name}s are permissible by default. You need to
  load for instance |pgflibrarypatterns|, see
  Section~\ref{section-library-patterns}, to install predefined
  patterns.  
  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[pattern=dots] (0,0) circle (1cm);
  \draw[pattern=fivepointed stars] (0,0) rectangle (3,1);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/pattern color=\meta{color}}
  This option is used to set the color to be used for form-only
  patterns. This option has no effect on inherently colored patterns. 
  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[pattern color=red,pattern=fivepointed stars]  (0,0) circle (1cm);
  \draw[pattern color=blue,pattern=fivepointed stars] (0,0) rectangle (3,1);
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \def\mypath{(0,0) -- +(0,1) arc (180:0:1.5cm) -- +(0,-1)}
  \fill   [red]                                \mypath;
  \pattern[pattern color=white,pattern=bricks] \mypath;
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsubsection{Graphic Parameters: Interior Rules}

The following two options can be used to decide how interior points
should be determined:
\begin{key}{/tikz/nonzero rule}
  If this rule is used (which is the default), the following method is
  used to determine whether a given point is ``inside'' the path: From
  the point, shoot a ray in some direction towards infinity (the
  direction is chosen such that no strange borderline cases
  occur). Then the ray may hit the path. Whenever it hits the path, we
  increase or decrease a counter, which is initially zero. If the ray
  hits the path as the path goes ``from left to right'' (relative to
  the ray), the counter is increased, otherwise it is decreased. Then,
  at the end, we check whether the counter is nonzero (hence the
  name). If so, the point is deemed to lie ``inside,'' otherwise it is
  ``outside.'' Sounds complicated? It is.

\begin{codeexample}[]
\begin{tikzpicture}
  \filldraw[fill=examplefill]
  % Clockwise rectangle
  (0,0) -- (0,1) -- (1,1) -- (1,0) -- cycle
  % Counter-clockwise rectangle
  (0.25,0.25) -- (0.75,0.25) -- (0.75,0.75) -- (0.25,0.75) -- cycle;

  \draw[->] (0,1) -- (.4,1);
  \draw[->] (0.75,0.75) -- (0.3,.75);

  \draw[->] (0.5,0.5) -- +(0,1) node[above] {crossings: $-1+1 = 0$};

  \begin{scope}[yshift=-3cm]
    \filldraw[fill=examplefill]
    % Clockwise rectangle
    (0,0) -- (0,1) -- (1,1) -- (1,0) -- cycle
    % Clockwise rectangle
    (0.25,0.25) -- (0.25,0.75) -- (0.75,0.75) -- (0.75,0.25) -- cycle;

    \draw[->] (0,1) -- (.4,1);
    \draw[->] (0.25,0.75) -- (0.4,.75);
      
    \draw[->] (0.5,0.5) -- +(0,1) node[above] {crossings: $1+1 = 2$};
  \end{scope}
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/even odd rule}
  This option causes a different method to be used for determining the
  inside and outside of paths. While it is less flexible, it turns out
  to be more intuitive.

  With this method, we also shoot rays from the point for which we
  wish to determine whether it is inside or outside the filling
  area. However, this time we only count how often we ``hit'' the path
  and declare the point to be ``inside'' if the number of hits is odd.

  Using the even-odd rule, it is easy to ``drill holes'' into a path.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \filldraw[fill=examplefill,even odd rule]
    (0,0) rectangle (1,1) (0.5,0.5) circle (0.4cm);
  \draw[->] (0.5,0.5) -- +(0,1) [above] node{crossings: $1+1 = 2$};
\end{tikzpicture}
\end{codeexample}
\end{key}



\subsubsection{Graphic Parameters: Fill Opacity}

\label{section-fill-opacity}
Analogously to the |draw opacity|, you can also set the filling
opacity. Please see Section~\ref{section-tikz-transparency} for more
details. 


\subsection{Shading a Path}

You can shade a path using the |shade| option. A shading is like a
filling, only the shading changes its color smoothly from one color to
another.

\begin{key}{/tikz/shade}
  Causes the path to be shaded using the currently selected shading
  (more on this later). If this option is used together with the
  |draw| option, then the path is first shaded, then drawn.

  It is not an error to use this option together with the |fill|
  option, but it makes no sense.

\begin{codeexample}[]
\tikz \shade (0,0) circle (1ex);
\end{codeexample}

\begin{codeexample}[]
\tikz \shadedraw (0,0) circle (1ex);
\end{codeexample}
\end{key}

For some shadings it is not really clear how they can ``fill'' the
path. For example, the |ball| shading normally looks like this: \tikz
\shade[shading=ball] (0,0) circle (0.75ex);. How is this supposed to
shade a rectangle? Or a triangle?

To solve this problem, the predefined shadings like |ball| or |axis|
fill a large rectangle completely in a sensible way. Then, when the
shading is used to ``shade'' a path, what actually happens is that the
path is temporarily used for clipping and then the rectangular shading
is drawn, scaled and shifted such that all parts of the path are
filled.


\subsubsection{Choosing a Shading Type}

The default shading is a smooth transition from gray
to white and from above to bottom. However, other shadings are also
possible, for example a shading that will sweep a color from the
center to the corners outward. To choose the shading, you can use the
|shading=| option, which will also automatically invoke the |shade|
option. Note that this does \emph{not} change the shading color, only
the way the colors sweep. For changing the colors, other options are
needed, which are explained below.

\begin{key}{/tikz/shading=\meta{name}}
  This selects a shading named \meta{name}. The following shadings are
  predefined:
  \begin{itemize}
  \item \declare{|axis|}
    This is the default shading in which the color changes gradually
    between three horizontal lines. The top line is at the top
    (uppermost) point of the path, the middle is in the middle, the
    bottom line is at the bottom of the path.

\begin{codeexample}[]
\tikz \shadedraw [shading=axis] (0,0) rectangle (1,1);
\end{codeexample}

    The default top color is gray, the default bottom color is white,
    the default middle is the ``middle'' of these two.
  \item \declare{|radial|}
    This shading fills the path with a gradual sweep from a certain
    color in the middle to another color at the border. If the path is
    a circle, the outer color will be reached exactly at the
    border. If the shading is not a circle, the outer color will
    continue a bit towards the corners. The default inner color is
    gray, the default outer color is white.

\begin{codeexample}[]
\tikz \shadedraw [shading=radial] (0,0) rectangle (1,1);
\end{codeexample}
  \item \declare{|ball|}
    This shading fills the path with a shading that ``looks like a
    ball.'' The default ``color'' of the ball is blue (for no
    particular reason).

\begin{codeexample}[]
\tikz \shadedraw [shading=ball] (0,0) rectangle (1,1);
\end{codeexample}

\begin{codeexample}[]
\tikz \shadedraw [shading=ball] (0,0) circle (.5cm);
\end{codeexample}
  \end{itemize}

  \begin{key}{/tikz/shading angle=\meta{degrees} (initially 0)}
    This option rotates the shading (not the path!) by the given
    angle. For example, we can turn a top-to-bottom axis shading into a
    left-to-right shading by rotating it by $90^\circ$.

\begin{codeexample}[]
\tikz \shadedraw [shading=axis,shading angle=90] (0,0) rectangle (1,1);
\end{codeexample}
  \end{key}
\end{key}

You can also define new shading types yourself. However, for this, you
need to use the basic layer directly, which is, well, more basic and
harder to use. Details on how to create a shading appropriate for
filling paths are given in Section~\ref{section-shading-a-path}.



\subsubsection{Choosing a Shading Color}

The following options can be used to change the colors used for
shadings. When one of these options is given, the |shade| option is
automatically selected and also the ``right'' shading.

\begin{key}{/tikz/top color=\meta{color}}
  This option prescribes the color to be used at the top in an |axis|
  shading. When this option is given, several things happen:
  \begin{enumerate}
  \item
    The |shade| option is selected.
  \item
    The |shading=axis| option is selected.
  \item
    The middle color of the axis shading is set to the average of the
    given top color \meta{color} and of whatever color is currently
    selected for the bottom.
  \item
    The rotation angle of the shading is set to 0.
  \end{enumerate}

\begin{codeexample}[]
\tikz \draw[top color=red] (0,0) rectangle (2,1);
\end{codeexample}
\end{key}  

\begin{key}{/tikz/bottom color=\meta{color}}
  This option works like |top color|, only for the bottom color.
\end{key}

\begin{key}{/tikz/middle color=\meta{color}}
  This option specifies the color for the middle of an axis
  shading. It also sets the |shade| and |shading=axis| options, but it
  does not change the rotation angle.

  \emph{Note:} Since both |top color| and |bottom color| change the
  middle color, this option should be given \emph{last} if all of
  these options need to be given:

\begin{codeexample}[]
\tikz \draw[top color=white,bottom color=black,middle color=red]
  (0,0) rectangle (2,1);
\end{codeexample}  
\end{key}

\begin{key}{/tikz/left color=\meta{color}}
  This option does exactly the same as |top color|, except that the
  shading angle is set to $90^\circ$.
\end{key}

\begin{key}{/tikz/right color=\meta{color}}
  Works like |left color|.
\end{key}

\begin{key}{/tikz/inner color=\meta{color}}
  This option sets the color used at the center of a |radial|
  shading. When this option is used, the |shade| and |shading=radial|
  options are set.
  
\begin{codeexample}[]
\tikz \draw[inner color=red] (0,0) rectangle (2,1);
\end{codeexample}
\end{key}

\begin{key}{/tikz/outer color=\meta{color}}
  This option sets the color used at the border and outside of a
  |radial| shading.
  
\begin{codeexample}[]
\tikz \draw[outer color=red,inner color=white]
  (0,0) rectangle (2,1);
\end{codeexample}
\end{key}


\begin{key}{/tikz/ball color=\meta{color}}
  This option sets the color used for the ball shading. It sets the
  |shade| and |shading=ball| options. Note that the ball will never
  ``completely'' have the color \meta{color}. At its ``highlight'' spot
  a certain amount of white is mixed in, at the border a certain
  amount of black. Because of this, it also makes sense to say
  |ball color=white| or |ball color=black|

\begin{codeexample}[]
\begin{tikzpicture}
  \shade[ball color=white] (0,0) circle (2ex);
  \shade[ball color=red] (1,0) circle (2ex);
  \shade[ball color=black] (2,0) circle (2ex);
\end{tikzpicture}
\end{codeexample}
\end{key}



\subsection{Establishing a Bounding Box}

\pgfname\ is reasonably good at keeping track of the size of your picture
and reserving just the right amount of space for it in the main
document. However, in some cases you may want to say things like
``do not count this for the picture size'' or ``the picture is
actually a little large.'' For this you can use the option
|use as bounding box| or the command |\useasboundingbox|, which is just
a shorthand for |\path[use as bounding box]|.

\begin{key}{/tikz/use as bounding box}
  Normally, when this option is given on a path, the bounding box of
  the present path is used to determine the size of the picture and
  the size of all \emph{subsequent} paths are
  ignored. However, if there were previous path operations that have
  already established a larger bounding box, it will not be made
  smaller by this operation.

  In a sense, |use as bounding box| has the same effect as clipping
  all subsequent drawing against the current path---without actually
  doing the clipping, only making \pgfname\ treat everything as if it
  were clipped.

  The first application of this option is to have a |{tikzpicture}|
  overlap with the main text:

\begin{codeexample}[]
Left of picture\begin{tikzpicture}
  \draw[use as bounding box] (2,0) rectangle (3,1);
  \draw (1,0) -- (4,.75);
\end{tikzpicture}right of picture.
\end{codeexample}

  In a second application this option can be used to get better
  control over the white space around the picture:
  
\begin{codeexample}[]
Left of picture
\begin{tikzpicture}
  \useasboundingbox (0,0) rectangle (3,1);
  \fill (.75,.25) circle (.5cm);
\end{tikzpicture}
right of picture.
\end{codeexample}

  Note: If this option is used on a path inside a \TeX\ group (scope),
  the effect ``lasts'' only till the end of the scope. Again, this
  behavior is the same as for clipping.
\end{key}

There is a node that allows you to get the size of the current
bounding box. The |current bounding box| node has the |rectangle|
shape and its size is always the size of the current 
bounding box.

Similarly, the |current path bounding box| node has the |rectangle|
hape and the size of the bounding box of the current path.


\begin{codeexample}[]
\begin{tikzpicture}
  \draw[red] (0,0) circle (2pt);
  \draw[red] (2,1) circle (3pt);

  \draw (current bounding box.south west) rectangle
        (current bounding box.north east);

  \draw[red] (3,-1) circle (4pt);

  \draw[thick] (current bounding box.south west) rectangle
               (current bounding box.north east);
\end{tikzpicture}
\end{codeexample}



\subsection{Clipping and Fading (Soft Clipping)}

\emph{Clipping path} means that all painting on the page is restricted
to a certain area. This area need not be rectangular, rather an
arbitrary path can be used to specify this area. The |clip| option,
explained below, is used to specify the region that is to be used for
clipping.

A \emph{fading} (a term that I propose, fadings are commonly known
as soft masks, transparency masks, opacity masks or soft clips) is
similar to clipping, but a fading allows parts of the picture to be
only ``half clipped.'' This means that a fading can specify that newly
painted pixels should be partly transparent. The specification
and handling of fadings is a bit complex and it is detailed in
Section~\ref{section-tikz-transparency}, which is devoted to
transparency in general.

\begin{key}{/tikz/clip}
  This option causes all subsequent drawings to be clipped against the
  current path and the size of subsequent paths will not be important
  for the picture size.  If you clip against a self-intersecting path,
  the even-odd rule or  the nonzero winding number rule is used to
  determine whether a point is inside or outside the clipping region.

  The clipping path is a graphic state parameter, so it will be reset
  at the end of the current scope. Multiple clippings accumulate, that
  is, clipping is always done against the intersection of all clipping
  areas that have been specified inside the current scopes. The only
  way of enlarging the clipping area is to end a |{scope}|.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[clip] (0,0) circle (1cm);
  \fill[red] (1,0) circle (1cm);
\end{tikzpicture}
\end{codeexample}

  It  is usually a \emph{very} good idea to apply the |clip| option only
  to the first path command in a scope. 

  If you ``only wish to clip'' and do not wish to draw anything, you can
  use the |\clip| command, which is a shorthand for |\path[clip]|.

\begin{codeexample}[]
\begin{tikzpicture}
  \clip (0,0) circle (1cm);
  \fill[red] (1,0) circle (1cm);
\end{tikzpicture}
\end{codeexample}

  To keep clipping local, use |{scope}| environments as in the
  following example:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) -- ( 0:1cm);
  \draw (0,0) -- (10:1cm);
  \draw (0,0) -- (20:1cm);
  \draw (0,0) -- (30:1cm);
  \begin{scope}[fill=red]
    \fill[clip] (0.2,0.2) rectangle (0.5,0.5);
    
    \draw (0,0) -- (40:1cm);
    \draw (0,0) -- (50:1cm);
    \draw (0,0) -- (60:1cm);
  \end{scope}
  \draw (0,0) -- (70:1cm);
  \draw (0,0) -- (80:1cm);
  \draw (0,0) -- (90:1cm);
\end{tikzpicture}
\end{codeexample}

  There is a slightly annoying catch: You cannot specify certain graphic
  options for the command used for clipping. For example, in the above
  code we could not have moved the |fill=red| to the |\fill|
  command. The reasons for this have to do with the internals of the
  \pdf\ specification. You do not want to know the details. It is best
  simply not to specify any options for these 
  commands. 
\end{key}



\subsection{Doing Multiple Actions on a Path}

If more than one of the basic actions like drawing, clipping and
filling are requested, they are automatically applied in a sensible
order: First, a path is filled, then drawn, and then clipped (although
it took Apple two mayor revisions of their operating system to get
this right\dots). Sometimes, however, you need finer control over what
is done with a path. For instance, you might wish to first fill a path
with a color, then repaint the path with a pattern and then repaint it
with yet another pattern. In such cases you can use the following two
options:

\begin{key}{/tikz/preactions=\meta{options}}
  This option can be given to a |\path| command (or to derived
  commands like |\draw| which internally call |\path|). Similarly to
  options like |draw|, this option only has an effect when given to a
  |\path| or as part of the options of a |node|; as an option to a
  |{scope}| it has no effect.

  When this option is used on a |\path|, the effect is the following:
  When the path has been completely constructed and is about to be
  used, a scope is created. Inside this scope, the path is used but
  not with the original path options, but with \meta{options}
  instead. Then, the path is used in the usual manner. In other words,
  the path is used twice: Once with \meta{options} in force and then
  again with the normal path options in force.

  Here is an example in which the path consists of a rectangle. The
  main action is to draw this path in red (which is why we see a red
  rectangle). However, the preaction is to draw the path in blue,
  which is why we see a blue rectangle behind the red rectangle.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \draw
    [preaction={draw,line width=4mm,blue}]
    [line width=2mm,red] (0,0) rectangle (2,2);
\end{tikzpicture}
\end{codeexample}

  Note that when the preactions are preformed, then the path is
  already ``finished.'' In particular, applying a coordinate
  transformation to the path has no effect. By comparison, applying a
  canvas transformation does have an effect. Let us use this to add a
  ``shadow'' to a path. For this, we use the preaction to fill the
  path in gray, shifted a bit to the right and down:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw
    [preaction={fill=black,opacity=.5,
                transform canvas={xshift=1mm,yshift=-1mm}}]
    [fill=red] (0,0) rectangle (1,2)
               (1,2) circle (5mm);
\end{tikzpicture}
\end{codeexample}

  Naturally, you would normally create a style |shadow| that contains
  the above code. The shadow library, see
  Section~\ref{section-libs-shadows}, contains predefined shadows of
  this kind.

  It is possible to use the |preaction| option multiple times. In this
  case, for each use of the |preaction| option, the path is used again
  (thus, the \meta{options} do not accumulate in a single usage of the
  path). The path is used in the order of |preaction| options given.

  In the following example, we use one |preaction| to add a shadow and
  another to provide a shading, while the main action is to use a
  pattern. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw [pattern=fivepointed stars]
    [preaction={fill=black,opacity=.5,
                transform canvas={xshift=1mm,yshift=-1mm}}]
    [preaction={top color=blue,bottom color=white}]
               (0,0) rectangle (1,2)
               (1,2) circle (5mm);
\end{tikzpicture}
\end{codeexample}

  A complicated application is shown in the following example, where
  the path is used several times with different fadings and shadings
  to create a special visual effect:
\begin{codeexample}[]
\begin{tikzpicture}
  [
    % Define an interesting style
    button/.style={
      % First preaction: Fuzzy shadow
      preaction={fill=black,path fading=circle with fuzzy edge 20 percent,
                 opacity=.5,transform canvas={xshift=1mm,yshift=-1mm}},
      % Second preaction: Background pattern
      preaction={pattern=#1,
                 path fading=circle with fuzzy edge 15 percent},
      % Third preaction: Make background shiny
      preaction={top color=white,
                 bottom color=black!50,
                 shading angle=45,
                 path fading=circle with fuzzy edge 15 percent,
                 opacity=0.2},
      % Fourth preaction: Make edge especially shiny
      preaction={path fading=fuzzy ring 15 percent,
                 top color=black!5,
                 bottom color=black!80,
                 shading angle=45},
      inner sep=2ex
    },
    button/.default=horizontal lines light blue,
    circle
  ]

  \draw [help lines] (0,0) grid (4,3);

  \node [button] at (2.2,1) {\Huge Big};
  \node [button=crosshatch dots light steel blue,
         text=white] at (1,1.5) {Small};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/postaction=\meta{options}}
  The postactions work in the same way as the preactions, only they
  are applied \emph{after} the main action has been taken. Like
  preactions, multiple |postaction| options may be given to a |\path|
  command, in which case the path is reused several times, each time
  with a different set of options in force.

  If both pre- and postactions are specified, then the preactions are
  taken first, then the main action, and then the post actions.

  In the first example, we use a postaction to draw the path, after it
  has already been drawn:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \draw
    [postaction={draw,line width=2mm,blue}]
    [line width=4mm,red,fill=white] (0,0) rectangle (2,2);
\end{tikzpicture}
\end{codeexample}

  In another example, we use a postaction to ``colorzie'' a path: 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw
    [postaction={path fading=south,fill=white}]
    [postaction={path fading=south,fading angle=45,fill=blue,opacity=.5}]
    [left color=black,right color=red,draw=white,line width=2mm]
               (0,0) rectangle (1,2)
               (1,2) circle (5mm);
\end{tikzpicture}
\end{codeexample}
\end{key}



\subsection{Decorating and Morphing a Path}

Before a path is used, it is possible to first ``decorate'' and/or
``morph'' it. Morphing means that the path is replaced by another path
that slightly varied. Such morphings are a special case
of the more general ``decorations'' described in detail in
Section~\ref{section-tikz-decorations}. For instance, in the following
example the path is drawn twice: Once normally and then in a morphed
(=decorated) manner. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) rectangle (3,2);
  \draw [red, decorate, decoration=zigzag]
        (0,0) rectangle (3,2);
\end{tikzpicture}
\end{codeexample}

Naturally, we could have combined this into a single command using
pre- or postaction. It is also possible to deform shapes:
\begin{codeexample}[]
\begin{tikzpicture}
  \node [circular drop shadow={shadow scale=1.05},minimum size=3.13cm,
         decorate, decoration=zigzag,
         fill=blue!20,draw,thick,circle] {Hello!};
\end{tikzpicture}
\end{codeexample}



==> pgfmanual-en-tikz-coordinates.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Specifying Coordinates}


\subsection{Overview}

A \emph{coordinate} is a position on the canvas on which your picture
is drawn. \tikzname\ uses a special syntax for specifying
coordinates. Coordinates are always put in round brackets. The general
syntax is 
\declare{|(|\opt{|[|\meta{options}|]|}\meta{coordinate  specification}|)|}. 

The \meta{coordinate specification} specified coordinates using one of
many different possible \emph{coordinate systems}. Examples are the
Cartesian coordinate system or polar coordinates or spherical
coordinates. No matter which coordinate system is used, in the end, a
specific point on the canvas is represented by the coordinate.

There are two ways of specifying which coordinate system should be used:
\begin{description}
\item[Explicitly] You can specify the coordinate system explicitly. To
  do so, you give the name of the coordinate system at the beginning,
  followed by |cs:|, which stands for ``coordinate system,'' followed
  by a specification of the coordinate using the key-value
  syntax. Thus, the general syntax for \meta{coordinate specification}
  in the explicit case is |(|\meta{coordinate system}| cs:|\meta{list
    of key-value pairs specific to the coordinate system}|)|.
\item[Implicitly] The explicit specification is often too verbose when
  numerous coordinates should be given. Because of this, for the
  coordinate systems that you are likely to use often a special syntax
  is provided. \tikzname\ will notice when you use a coordinate
  specified in a special syntax and will choose the correct coordinate
  system automatically.
\end{description}

Here is an example in which explicit the coordinate systems are
specified explicitly:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw (canvas cs:x=0cm,y=2mm)
     -- (canvas polar cs:radius=2cm,angle=30);
\end{tikzpicture}
\end{codeexample}
In the next example, the coordinate systems are implicit:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw (0cm,2mm) -- (30:2cm);
\end{tikzpicture}
\end{codeexample}

It is possible to give options that apply only to a single
coordinate, although this makes sense for transformation options
only. To give transformation options for a single coordinate, give
these options at the beginning in brackets:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw      (0,0) -- (1,1);
  \draw[red] (0,0) -- ([xshift=3pt] 1,1);
  \draw      (1,0) -- +(30:2cm);
  \draw[red] (1,0) -- +([shift=(135:5pt)] 30:2cm);
\end{tikzpicture}
\end{codeexample}


\subsection{Coordinate Systems}

\subsubsection{Canvas, XYZ, and Polar Coordinate Systems}

Let us start with the basic coordinate systems.

\begin{coordinatesystem}{canvas}
  The simplest way of specifying a coordinate is to use the |canvas|
  coordinate system. You provide a dimension $d_x$ using the |x=|
  option and another dimension $d_y$ using the |y=| option. The position on
  the canvas is located at the position that is $d_x$ to the right and
  $d_y$ above the origin.

  \begin{key}{/tikz/cs/x=\meta{dimension} (initially 0pt)}
    Distance by which the coordinate
    is to the right of the origin. You can also write things like
    |1cm+2pt| since the mathematical engine is used to evaluate the
    \meta{dimension}.
  \end{key}

  \begin{key}{/tikz/cs/y=\meta{dimension} (initially 0pt)}
    Distance by which the coordinate
    is above the origin.
  \end{key}

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \fill (canvas cs:x=1cm,y=1.5cm)    circle (2pt);
  \fill (canvas cs:x=2cm,y=-5mm+2pt) circle (2pt);
\end{tikzpicture}
\end{codeexample}

  To specify a coordinate in the coordinate system implicitly, you use
  two dimensions that are separated by a comma as in |(0cm,3pt)| or
  |(2cm,\textheight)|. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \fill (1cm,1.5cm)    circle (2pt);
  \fill (2cm,-5mm+2pt) circle (2pt);
\end{tikzpicture}
\end{codeexample}
\end{coordinatesystem}


\begin{coordinatesystem}{xyz}
  The |xyz| coordinate system allows you to specify a point as a
  multiple of three vectors called the $x$-, $y$-, and
  $z$-vectors.  By default, the $x$-vector points 1cm to the right,
  the $y$-vector points 1cm upwards, but this can be changed
  arbitrarily as explained in Section~\ref{section-xyz}. The default
  $z$-vector points to $\bigl(-\frac{1}{\sqrt2}
  \textrm{cm},-\frac{1}{\sqrt2}\textrm{cm}\bigr)$.

  To specify the factors by which the vectors should be multiplied
  before being added, you use the following three options:  
  \begin{key}{/tikz/cs/x=\meta{factor} (initially 0)}
    Factor by which the $x$-vector is multiplied.
  \end{key}
  \begin{key}{/tikz/cs/y=\meta{factor} (initially 0)}
    Works like |x|.
  \end{key}
  \begin{key}{/tikz/cs/z=\meta{factor} (initially 0)}
    Works like |x|.
  \end{key}

\begin{codeexample}[]
\begin{tikzpicture}[->]
  \draw (0,0) -- (xyz cs:x=1);
  \draw (0,0) -- (xyz cs:y=1);
  \draw (0,0) -- (xyz cs:z=1);
\end{tikzpicture}
\end{codeexample}

  This coordinate system can also be selected implicitly. To do so,
  you just provide two or three comma-separated factors (not
  dimensions). 
\begin{codeexample}[]
\begin{tikzpicture}[->]
  \draw (0,0) -- (1,0);
  \draw (0,0) -- (0,1,0);
  \draw (0,0) -- (0,0,1);
\end{tikzpicture}
\end{codeexample}
\end{coordinatesystem}

\emph{Note:} It is possible to use coordinates like |(1,2cm)|, which
are neither |canvas| coordinates nor |xyz| coordinates. The rule is
the following: If a coordinate is of the implicit form
|(|\meta{x}|,|\meta{y}|)|, then \meta{x} and \meta{y} are checked,
independently, whether they have a dimension or whether they are
dimensionless. If both have a dimension, the |canvas| coordinate
system is used. If both lack a dimension, the |xyz| coordinate system
is used. If \meta{x} has a dimension and \meta{y} has not, then the
sum of two coordinate |(|\meta{x}|,0pt)| and |(0,|\meta{y}|)| is
used. If \meta{y} has a dimension and \meta{x} has not, then the sum
of two coordinate |(|\meta{x}|,0)| and |(0pt,|\meta{y}|)| is used.

\emph{Note furthermore:} An expression like |(2+3cm,0)| does
\emph{not} mean the same as |(2cm+3cm,0)|. Instead, if \meta{x} or
\meta{y} internally uses a mixture of dimensions and dimensionless
values, then all dimensionless values are ``upgraded'' to dimensions
by interpreting them as |pt|. So, |2+3cm| is the same dimension as
|2pt+3cm|. 

\begin{coordinatesystem}{canvas polar}
  The |canvas polar| coordinate system allows you to specify
  polar coordinates. You provide an angle using the |angle=| option
  and a radius using the |radius=| option. This yields the point on
  the canvas that is at the given radius distance from the origin at
  the given degree. A degree of zero points to the right, a degree of
  90 upward.
  \begin{key}{/tikz/cs/angle=\meta{degrees}}
    The angle of the coordinate.
    The angle must always be given in degrees and should be between
    $-360$ and $720$.
  \end{key}
  \begin{key}{/tikz/cs/radius=\meta{dimension}}
    The distance from the origin.
  \end{key}
  \begin{key}{/tikz/cs/x radius=\meta{dimension}}
    A polar coordinate is,
    after all, just a point on a circle of the given \meta{radius}. When
    you provide an $x$-radius and also a $y$-radius, you specify an
    ellipse instead of a circle. The |radius| option has the same effect
    as specifying identical |x radius| and |y radius| options.
  \end{key}
  \begin{key}{/tikz/cs/y radius=\meta{dimension}}
    Works like |x radius|.
  \end{key}
\begin{codeexample}[]
\tikz \draw (0,0) -- (canvas polar cs:angle=30,radius=1cm);
\end{codeexample}

  The implicit form for canvas polar coordinates is the following: 
  you specify the angle and the distance, separated by a colon as in
  |(30:1cm)|. 

\begin{codeexample}[]
\tikz \draw    (0cm,0cm) -- (30:1cm) -- (60:1cm) -- (90:1cm)
            -- (120:1cm) -- (150:1cm) -- (180:1cm);
\end{codeexample}

  Two different radii are specified by writing |(30:1cm and 2cm)|.

  For the implicit form, instead of an angle given as a number you can
  also use certain words. For example, |up| is the same as |90|, so
  that you can write |\tikz \draw (0,0) -- (2ex,0pt) -- +(up:1ex);|
  and get \tikz \draw (0,0) -- (2ex,0pt) -- +(up:1ex);. Apart from |up|
  you can use |down|, |left|, |right|, |north|, |south|, |west|, |east|,
  |north east|, |north west|, |south east|, |south west|, all of which
  have their natural meaning.
\end{coordinatesystem}

\begin{coordinatesystem}{xyz polar}
  This coordinate system work similarly to the |canvas polar|
  system. However, the radius and the angle are interpreted in the
  $xy$-coordinate system, not in the canvas system. More detailed,
  consider the circle or ellipse whose half axes are given by the
  current $x$-vector and the current $y$-vector. Then, consider the
  point that lies at a given angle on this ellipse, where an angle of
  zero is the same as the $x$-vector and an angle of 90 is the
  $y$-vector. Finally, multiply the resulting vector by the given
  radius factor. Voilà.
  \begin{key}{/tikz/cs/angle=\meta{degrees}}
    The angle of the coordinate
    interpreted in the ellipse whose axes are the $x$-vector and the
    $y$-vector.
  \end{key}
  \begin{key}{/tikz/cs/radius=\meta{factor}}
    A factor by which the $x$-vector
    and $y$-vector are multiplied prior to forming the ellipse.
  \end{key}
  \begin{key}{/tikz/cs/x radius=\meta{dimension}} A specific factor by
    which only the $x$-vector is multiplied.
  \end{key}
  \begin{key}{/tikz/cs/y radius=\meta{dimension}}
    Works like |x radius|.
  \end{key}
\begin{codeexample}[]
\begin{tikzpicture}[x=1.5cm,y=1cm]
  \draw[help lines] (0cm,0cm) grid (3cm,2cm);

  \draw (0,0) -- (xyz polar cs:angle=0,radius=1);
  \draw (0,0) -- (xyz polar cs:angle=30,radius=1);
  \draw (0,0) -- (xyz polar cs:angle=60,radius=1);
  \draw (0,0) -- (xyz polar cs:angle=90,radius=1);

  \draw (xyz polar cs:angle=0,radius=2)
     -- (xyz polar cs:angle=30,radius=2)
     -- (xyz polar cs:angle=60,radius=2)
     -- (xyz polar cs:angle=90,radius=2);
 \end{tikzpicture}
\end{codeexample}

  The implicit version of this option is the same as the implicit
  version of |canvas polar|, only you do not provide a unit.

\begin{codeexample}[]
\tikz[x={(0cm,1cm)},y={(-1cm,0cm)}]
  \draw  (0,0) -- (30:1) -- (60:1) -- (90:1)
             -- (120:1) -- (150:1) -- (180:1);
\end{codeexample}
\end{coordinatesystem}

\begin{coordinatesystem}{xy polar}
  This is just an alias for |xyz polar|, which some people might
  prefer as there is no z-coordinate involved in the |xyz polar|
  coordinates.   
\end{coordinatesystem}


\subsubsection{Barycentric Systems}
\label{section-barycentric-coordinates}

In the barycentric coordinate system a point is expressed as the
linear combination of multiple vectors. The idea is that you specify
vectors $v_1$, $v_2$, \dots, $v_n$ and numbers $\alpha_1$, $\alpha_2$,
\dots, $\alpha_n$. Then the barycentric coordinate specified by these
vectors and numbers is
\begin{align*}
  \frac{\alpha_1 v_1 + \alpha_2 v_2 + \cdots + \alpha_n v_n}{\alpha_1
    + \alpha_2 + \cdots + \alpha_n}
\end{align*}

The |barycentric cs| allows you to specify such coordinates easily.

\begin{coordinatesystem}{barycentric}
  For this coordinate system, the \meta{coordinate specification}
  should be a comma-separated list of expressions of the form
  \meta{node name}|=|\meta{number}. Note that (currently) the list
  should not contain any spaces before or after the \meta{node name}
  (unlike normal key-value pairs). 

  The specified coordinate is now computed as follows: Each pair
  provides one vector and a number. The vector is the |center| anchor
  of the \meta{node name}. The number is the \meta{number}. Note that
  (currently) you cannot specify a different anchor, so that in order
  to use, say, the |north| anchor of a node you first have to create a
  new coordinate at this north anchor. (Using for instance
  \texttt{\string\coordinate (mynorth) at (mynode.north);}.)

\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate (content)   at (90:3cm);
  \coordinate (structure) at (210:3cm);
  \coordinate (form)      at (-30:3cm);
    
  \node [above]       at (content)   {content oriented};
  \node [below left]  at (structure) {structure oriented};
  \node [below right] at (form)      {form oriented};

  \draw [thick,gray] (content.south) -- (structure.north east) -- (form.north west) -- cycle;

  \small
  \node at (barycentric cs:content=0.5,structure=0.1 ,form=1)    {PostScript};
  \node at (barycentric cs:content=1  ,structure=0   ,form=0.4)  {DVI};
  \node at (barycentric cs:content=0.5,structure=0.5 ,form=1)    {PDF};
  \node at (barycentric cs:content=0  ,structure=0.25,form=1)    {CSS};
  \node at (barycentric cs:content=0.5,structure=1   ,form=0)    {XML};
  \node at (barycentric cs:content=0.5,structure=1   ,form=0.4)  {HTML};
  \node at (barycentric cs:content=1  ,structure=0.2 ,form=0.8)  {\TeX};
  \node at (barycentric cs:content=1  ,structure=0.6 ,form=0.8)  {\LaTeX};
  \node at (barycentric cs:content=0.8,structure=0.8 ,form=1)    {Word};
  \node at (barycentric cs:content=1  ,structure=0.05,form=0.05) {ASCII};
\end{tikzpicture}
\end{codeexample}
\end{coordinatesystem}

\subsubsection{Node Coordinate System}
\label{section-node-coordinates}

In \pgfname\ and in \tikzname\ it is quite easy to define a node that you
wish to reference at a later point. Once you have defined a node,
there are different ways of referencing points of the node. To do so,
you use the following coordinate system:

\begin{coordinatesystem}{node}
  This coordinate system is used to reference a specific point inside
  or on the border of a previously defined node. It can be used in
  different ways, so let us go over them one by one.

  You can use three options to specify which coordinate you mean:
  \begin{key}{/tikz/cs/name=\meta{node name}}
    Specifies the node in which you which to specify a coordinate. The
    \meta{node name} is 
    the name that was previously used to name the node using the
    |name=|\meta{node name} option or the special node name syntax.
  \end{key}
  \begin{key}{/tikz/anchor=\meta{anchor}}
    Specifies an anchor of the node. Here is an example: 
\begin{codeexample}[]
\begin{tikzpicture}
  \node (shape)   at (0,2)  [draw] {|class Shape|};
  \node (rect)    at (-2,0) [draw] {|class Rectangle|};
  \node (circle)  at (2,0)  [draw] {|class Circle|};
  \node (ellipse) at (6,0)  [draw] {|class Ellipse|};

  \draw (node cs:name=circle,anchor=north) |- (0,1);
  \draw (node cs:name=ellipse,anchor=north) |- (0,1);
  \draw[-open triangle 90] (node cs:name=rect,anchor=north)
        |- (0,1) -| (node cs:name=shape,anchor=south);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  \begin{key}{/tikz/cs/angle=\meta{degrees}}
    It is also possible to provide an angle \emph{instead} of an
    anchor. This coordinate refers to a point of the node's
    border where a ray shot from the center
    in the given angle hits the border. Here is an example:
\begin{codeexample}[]
\begin{tikzpicture}
  \node (start) [draw,shape=ellipse] {start};
  \foreach \angle in {-90, -80, ..., 90}
    \draw (node cs:name=start,angle=\angle)
      .. controls +(\angle:1cm) and +(-1,0) .. (2.5,0);
  \end{tikzpicture}
\end{codeexample}
  \end{key}

  It is possible to provide \emph{neither} the |anchor=| option nor
  the |angle=| option. In this case, \tikzname\ will calculate an
  appropriate border position for you. Here is an example: 

\begin{codeexample}[]
\begin{tikzpicture}
  \path (0,0)  node(a) [ellipse,rotate=10,draw] {An ellipse}
        (3,-1) node(b) [circle,draw]            {A circle};
  \draw[thick] (node cs:name=a) -- (node cs:name=b);
\end{tikzpicture}
\end{codeexample}

  \tikzname\ will be reasonably clever at determining the border points that
  you ``mean,'' but, naturally, this may fail in some situations. If
  \tikzname\ fails to determine an appropriate border point, the center will
  be used instead.

  Automatic computation of anchors works only with the line-to operations
  |--|, the vertical/horizontal versions \verb!|-! and \verb!-|!, and
  with the curve-to operation |..|. For other path commands, such as
  |parabola| or |plot|, the center will be used. If this is not desired,
  you should give a named anchor or an angle anchor.
  
  Note that if you use an automatic coordinate for both the start and
  the end of a line-to, as in |--(node cs:name=b)--|, then \emph{two}
  border   coordinates are computed with a move-to between them. This
  is usually   exactly what you want.
  
  If you use relative coordinates together with automatic anchor
  coordinates, the relative coordinates are computed relative to
  the node's center, not relative to the border point. Here is an
  example:

\begin{codeexample}[]
\tikz \draw (0,0) node(x) [draw] {Text}
            rectangle (1,1)
            (node cs:name=x) -- +(1,1);
\end{codeexample}

Similarly, in the following examples both control points are $(1,1)$:

\begin{codeexample}[]
\tikz \draw (0,0) node(x) [draw] {X}
            (2,0) node(y) {Y}
            (node cs:name=x) .. controls +(1,1) and +(-1,1) ..
            (node cs:name=y);
\end{codeexample}

  The implicit way of specifying the node coordinate system is to
  simply use the name of the node in parentheses as in |(a)| or to
  specify a name together with an anchor or an angle separated by a
  dot as in |(a.north)| or |(a.10)|.

  Here is a more complete example:
\begin{codeexample}[]
\begin{tikzpicture}[fill=blue!20]
  \draw[help lines] (-1,-2) grid (6,3);
  \path (0,0)  node(a) [ellipse,rotate=10,draw,fill]    {An ellipse}
        (3,-1) node(b) [circle,draw,fill]               {A circle}
        (2,2)  node(c) [rectangle,rotate=20,draw,fill]  {A rectangle}
        (5,2)  node(d) [rectangle,rotate=-30,draw,fill] {Another rectangle};
  \draw[thick] (a.south) -- (b) -- (c) -- (d);
  \draw[thick,red,->] (a) |- +(1,3) -| (c) |- (b);       
  \draw[thick,blue,<->] (b) .. controls +(right:2cm) and +(down:1cm) .. (d);       
\end{tikzpicture}
\end{codeexample}
\end{coordinatesystem}


           
\subsubsection{Intersection Coordinate Systems}

Often you wish to specify a point that is on the
intersection of two lines or shapes. For this, the following
coordinate system is useful:

\begin{coordinatesystem}{intersection}
  First, you must specify two objects that should be
  intersected. These ``objects'' can either be lines or the shapes of
  nodes. There are two option to specify the first object:
  \begin{key}{/tikz/cs/first line={\ttfamily\char`\{}|(|\meta{first
          coordinate}|)--(|\meta{second coordinate}|)|{\ttfamily\char`\}}}
    Specifies that the first object is a line that goes from
    \meta{first coordinate} to meta{second coordinate}.
  \end{key}
  Note that you have to write |--| between the coordinate, but this
  does not mean that anything is added to the path. This is simply a
  special syntax.
  \begin{key}{/tikz/cs/first node=\meta{node}}
    Specifies that the first object is a previously defined node named
    \meta{node}.
  \end{key}
  
  To specify the second object, you use one of the following keys:
  \begin{key}{/tikz/cs/second line={\ttfamily\char`\{}|(|\meta{first
          coordinate}|)--(|\meta{second coordinate}|)|{\ttfamily\char`\}}}
    As above.
  \end{key}
  \begin{key}{/tikz/cs/second node=\meta{node}}
    Specifies that the second object is a previously defined node
    named \meta{node}.
  \end{key}

  Since it is possible that two objects have multiple intersections,
  you may need to specify which solution you want:
  \begin{key}{/tikz/cs/solution=\meta{number} (initially 1)}
    Specifies which solution should be used. Numbering starts with 1.
  \end{key}
  The coordinate specified in this way is the \meta{number}th
  intersection of the two objects.  If the objects do not intersect,
  an error may occur.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw (0,0) coordinate (A) -- (3,2) coordinate (B)
        (1,2)                -- (3,0);

  \fill[red] (intersection cs:
    first line={(A)--(B)},
    second line={(1,2)--(3,0)}) circle (2pt);
\end{tikzpicture}
\end{codeexample}

  The implicit way of specifying this coordinate system is to write
  \declare{|(intersection |\opt{\meta{number}}| of |\meta{first
      object}%
    | and |\meta{second object}|)|}. Here, \meta{first obejct} either
  has the form \meta{$p_1$}|--|\meta{$p_2$} or it is just a node
  name. Likewise for \meta{second object}. Note that there are \emph{no}
  parentheses around the $p_i$. Thus, you would write
  |(intersection of A--B and 1,2--3,0)|  for the intersection of the
  line through the coordinates |A| and |B| and the line through the
  points $(1,2)$ and $(3,0)$. You would write 
  |(intersection 2 of c_1 and c_2)| for the second
  intersection of the node named |c_1| and the node named
  |c_2|.

  \tikzname\ needs an explicit algorithm for computing the
  intersection of two shapes and such an algorithm is available only
  for few shapes. Currently, the following intersection will be
  computed correctly:
  \begin{itemize}
  \item a line and a line
  \item a |circle| node and a line (in any order)
  \item a |circle| and a |circle|
  \end{itemize}
\begin{codeexample}[]
\begin{tikzpicture}[scale=.25]
  \coordinate [label=-135:$a$] (a) at ($ (0,0)   + (rand,rand) $);
  \coordinate [label=45:$b$]   (b) at ($ (3,2) + (rand,rand) $);

  \coordinate [label=-135:$u$] (u) at (-1,1);
  \coordinate [label=45:$v$]   (v) at (6,0);

  \draw (a) -- (b)
        (u) -- (v);

  \node (c1) at (a) [draw,circle through=(b)] {};
  \node (c2) at (b) [draw,circle through=(a)] {};

  \coordinate [label=135:$c$] (c) at (intersection 2 of c1 and c2);
  \coordinate [label=-45:$d$] (d) at (intersection of u--v and c2);
  \coordinate [label=135:$e$] (e) at (intersection of u--v and a--b);

  \foreach \p in {a,b,c,d,e,u,v}
    \fill [opacity=.5] (\p) circle (8pt);
\end{tikzpicture}
\end{codeexample}
\end{coordinatesystem}

A frequent special case of intersections is the intersection of a
vertical line going through a point $p$ and a horizontal line going
through some other point $q$. For this situation there is another
coordinate system.

\begin{coordinatesystem}{perpendicular}
  This coordinate system works the same way as |intersection|, only
  the lines are specified differently:

  \begin{key}{/tikz/cs/horizontal line through={\ttfamily\char`\{}|(|\meta{coordinate}|)|{\ttfamily\char`\}}}
    Specifies that one line is a horizontal line that goes through the
    given coordinate.
  \end{key}
  \begin{key}{/tikz/cs/vertical line through={\ttfamily\char`\{}|(|\meta{coordinate}|)|{\ttfamily\char`\}}}
    Specifies that the other line is vertical and goes through the
    given coordinate.  
  \end{key}

  The implicit syntax is to write \declare{|(|\meta{p}\verb! |- !\meta{q}|)|} or
  \declare{|(|\meta{q}\verb! -| !\meta{p}|)|}.

  For example, \verb!(2,1 |- 3,4)! and  \verb!(3,4 -| 2,1)! both yield
  the same as \verb!(2,4)! (provided the $xy$-coordinate system has not
  been modified). 

  The most useful application of the syntax is to draw a line up to some
  point on a vertical or horizontal line. Here is an example:

\begin{codeexample}[]
\begin{tikzpicture}
  \path (30:1cm) node(p1) {$p_1$}   (75:1cm) node(p2) {$p_2$};

  \draw (-0.2,0) -- (1.2,0) node(xline)[right] {$q_1$};
  \draw (2,-0.2) -- (2,1.2) node(yline)[above] {$q_2$};

  \draw[->] (p1) -- (p1 |- xline);
  \draw[->] (p2) -- (p2 |- xline);
  \draw[->] (p1) -- (p1 -| yline);
  \draw[->] (p2) -- (p2 -| yline);
\end{tikzpicture}
\end{codeexample}
\end{coordinatesystem}

           
\subsubsection{Tangent Coordinate Systems}

\begin{coordinatesystem}{tangent}
  This coordinate system, which is available only when the \tikzname\
  library |calc| is loaded, allows you to compute the point that lies
  tangent to a shape. In detail, consider a \meta{node} and a
  \meta{point}. Now, draw a straight line from the \meta{point} so
  that it ``touches'' the \meta{node} (more formally, so that it is
  \emph{tangent} to this \meta{node}). The point where the line
  touches the shape is the point referred to by the |tangent|
  coordinate system.

  The following options may be given:
  \begin{key}{/tikz/cs/node=\meta{node}}
    This key specifies the node on whose border the tangent should
    lie. 
  \end{key}
  \begin{key}{/tikz/cs/point=\meta{point}}
    This key speicifes the point through which the tangent should go.
  \end{key}
  \begin{key}{/tikz/cs/solution=\meta{number}}
    Specifies which solution should be used if there are more than one.
  \end{key}

  As for intersection coordinate system, a special algorithm is needed
  in order to compute the tangent for a given shape. Currently,
  tangents can be computed for nodes whose shape is one of the
  following:
  \begin{itemize}
  \item |coordinate|
  \item |circle|
  \end{itemize}

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);

  \coordinate (a) at (3,2);

  \node [circle,draw] (c) at (1,1) [minimum size=40pt] {$c$};
  
  \draw[red] (a)  -- (tangent cs:node=c,point={(a)},solution=1) --
       (c.center) -- (tangent cs:node=c,point={(a)},solution=2) -- cycle;
\end{tikzpicture}
\end{codeexample}

  There is no implicit syntax for this coordinate system.
\end{coordinatesystem}

\subsubsection{Defining New Coordinate Systems}

While the set of coordinate systems that \tikzname\ can parse via
their special syntax is fixed, it is possible and quite easy to define
new explicitly named coordinate systems. For this, the following
commands are used:

\begin{command}{\tikzdeclarecoordinatesystem\marg{name}\marg{code}}
  This command declares a new coordinate system named \meta{name} that
  can later on be used by writing
  |(|\meta{name}| cs:|\meta{arguments}|)|. When \tikzname\ encounters a coordinate
  specified in this way, the \meta{arguments} are passed to
  \meta{code} as argument |#1|.

  It is now the job of \meta{code} to make sense of the
  \meta{arguments}. At the end of \meta{code}, the two \TeX\ dimensions
  |\pgf@x| and |\pgf@y| should be have the $x$- and $y$-canvas
  coordinate of the coordinate.

  It is not necessary, but customary, to parse \meta{arguments} using
  the key-value syntax. However, you can also parse it in any way you
  like.

  In the following example, a coordinate system |cylindrical| is
  defined.
\begin{codeexample}[]
\makeatletter
\define@key{cylindricalkeys}{angle}{\def\myangle{#1}}    
\define@key{cylindricalkeys}{radius}{\def\myradius{#1}}    
\define@key{cylindricalkeys}{z}{\def\myz{#1}}
\tikzdeclarecoordinatesystem{cylindrical}%
{%
  \setkeys{cylindricalkeys}{#1}%
  \pgfpointadd{\pgfpointxyz{0}{0}{\myz}}{\pgfpointpolarxy{\myangle}{\myradius}}
}
\begin{tikzpicture}[z=0.2pt]
  \draw [->] (0,0,0) -- (0,0,350);
  \foreach \num in {0,10,...,350}
    \fill (cylindrical cs:angle=\num,radius=1,z=\num) circle (1pt);
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\tikzaliascoordinatesystem\marg{new name}\marg{old name}}
  Creates an alias of \meta{old name}.  
\end{command}




\subsection{Relative and Incremental Coordinates}


\subsubsection{Specifying Relative Coordinates}

You can prefix coordinates by |++| to make them ``relative.'' A
coordinate such as |++(1cm,0pt)| means ``1cm to the right of the
previous position.'' Relative coordinates are often useful in
``local'' contexts:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0)     -- ++(1,0) -- ++(0,1) -- ++(-1,0) -- cycle;
  \draw (2,0)     -- ++(1,0) -- ++(0,1) -- ++(-1,0) -- cycle;
  \draw (1.5,1.5) -- ++(1,0) -- ++(0,1) -- ++(-1,0) -- cycle;
\end{tikzpicture}
\end{codeexample}

Instead of |++| you can also use a single |+|. This also specifies a
relative coordinate, but it does not ``update'' the current point for
subsequent usages of relative coordinates. Thus, you can use this
notation to specify numerous points, all relative to the same
``initial'' point:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0)     -- +(1,0) -- +(1,1) -- +(0,1) -- cycle;
  \draw (2,0)     -- +(1,0) -- +(1,1) -- +(0,1) -- cycle;
  \draw (1.5,1.5) -- +(1,0) -- +(1,1) -- +(0,1) -- cycle;
\end{tikzpicture}
\end{codeexample}

There is a special situation, where relative coordinates are
interpreted differently. If you use a relative coordinate as a control
point of a Bézier curve, the following rule applies: First, a relative
first control point is taken relative to the beginning of the
curve. Second, a relative second control point is taken relative to
the end of the curve. Third, a relative end point of a curve is taken
relative to the start of the curve.

This special behavior makes it easy to specify that a curve should
``leave or arrives from a certain direction'' at the start or end. In
the following example, the curve ``leaves'' at $30^\circ$ and
``arrives'' at $60^\circ$: 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (1,0) .. controls +(30:1cm) and +(60:1cm) .. (3,-1);
  \draw[gray,->] (1,0) -- +(30:1cm);
  \draw[gray,<-] (3,-1) -- +(60:1cm);
\end{tikzpicture}
\end{codeexample}


\subsubsection{Relative Coordinates and Scopes}
\label{section-scopes-relative}
An interesting question is, how do relative coordinates behave in the
presence of scopes? That is, suppose we use curly braces in a path to
make part of it ``local,'' how does that affect the current position?
On the one hand, the current position certainly changes since the
scope only affects options, not the path itself. On the other hand, it
may be useful to ``temporarily escape'' from the updating of the
current point.

Since both interpretations of how the current point and scopes should
``interact'' are useful, there is a (local!) option that allows you to
decide which you need.

\begin{key}{/tikz/current point is local=\opt{\meta{boolean}} (initially
    false)}
  Normally, the scope path operation has no effect on the current
  point. That is, curly braces on a path have no effect on the current
  position:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw      (0,0) -- ++(1,0)   -- ++(0,1)   -- ++(-1,0);
  \draw[red] (2,0) -- ++(1,0) { -- ++(0,1) } -- ++(-1,0);
\end{tikzpicture}
\end{codeexample}
  If you set this key to |true|, this behaviour changes. In this case,
  at the end of a group created on a path, the last current position
  reverts to whatever value it had at the beginning of the scope. More
  precisely, when \tikzname\ encounters |}| on a path, it checks
  whether at this particular moment the key is set to |true|. If so,
  the current position reverts to the value is had when the matching
  |{| was read.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw      (0,0) -- ++(1,0)   -- ++(0,1)   -- ++(-1,0);
  \draw[red] (2,0) -- ++(1,0)
     { [current point is local] -- ++(0,1) } -- ++(-1,0);
\end{tikzpicture}
\end{codeexample}  
  In the above example, we could also have given the option outside
  the scope, for instance as a parameter to the whole scope.
\end{key}


\subsection{Coordinate Calculations}

\begin{tikzlibrary}{calc}
  You need to load this library in order to use the coordinate
  calculation functions described in the present section.
\end{tikzlibrary}


It is possible to do some basic calculations that involve
coordinates. In essence, you can add and subtract coordinates, scale
them, compute midpoints, and do projections. For instance,
|($(a) + 1/3*(1cm,0)$)| is the coordinate that is $1/3$cm to the right
of the point |a|:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \node (a) at (1,1) {A};
  \fill [red] ($(a) + 1/3*(1cm,0)$) circle (2pt);
\end{tikzpicture}
\end{codeexample}



\subsubsection{The General Syntax}

The general syntax is the following:

\begin{quote}
  \declare{|(|\opt{|[|\meta{options}|]|}|$|\meta{coordinate computation}|$)|}. 
\end{quote}

As you can see, the syntax uses the \TeX\ math symbol |$| to %$
indicate that a ``mathematical computation'' is involved. However, the |$| %$
has no other effect, in particular, no mathematical text is typeset.

The \meta{coordinate computation} has the following structure:
\begin{enumerate}
\item
  It starts with
  \begin{quote}
    \opt{\meta{factor}|*|}\meta{coordinate}\opt{\meta{modifiers}} 
  \end{quote}
\item
  This is optionally followed by |+| or |-| and then another
  \begin{quote}
    \opt{\meta{factor}|*|}\meta{coordinate}\opt{\meta{modifiers}} 
  \end{quote}
\item
  This is once more followed by |+| or |-| and another of the above
  modified coordinate; and so on.
\end{enumerate}

In the following, the syntax of factors and of the different modifiers
is explained in detail.


\subsubsection{The Syntax of Factors}

The \meta{factor}s are optional and detected
by checking whether the \meta{coordinate computation} starts with a
|(|. Also, after each $\pm$ a \meta{factor} is present if, and only
if, the |+| or |-| sign is not directly followed by~|(|.

If a \meta{factor} is present, it is evaluated using the
|\pgfmathparse| macro. This means that you can use pretty complicated
computations inside a factor. A \meta{factor} may even contain opening
parentheses, which creates a complication: How does \tikzname\ know
where a \meta{factor} ends and where a coordinate starts? For
instance, if the beginning of a \meta{coordinate computation} is
|2*(3+4|\dots, it is not clear whether |3+4| is part of a
\meta{coordinate} or part of a \meta{factor}. Because of this, the
following rule is used: Once it has been determined, that a
\meta{factor} is present, in principle, the \meta{factor} contains
everything up to the next occurrence of |*(|. Note that there is no
space between the asterisk and the parenthesis.

It is permissible to put the \meta{factor} is curly braces. This can
be used whenever it is unclear where the \meta{factor} would end. 

Here are some examples of coordinate specifications that consist of
exactly one \meta{factor} and one \meta{coordinate}:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \fill [red] ($2*(1,1)$) circle (2pt);
  \fill [green] (${1+1}*(1,.5)$) circle (2pt);
  \fill [blue] ($cos(0)*sin(90)*(1,1)$) circle (2pt);
  \fill [black] (${3*(4-3)}*(1,0.5)$) circle (2pt);
\end{tikzpicture}
\end{codeexample}



\subsubsection{The Syntax of Partway Modifiers}

A \meta{coordinate} can be followed by different \meta{modifiers}. The
first kind of modifier is the \emph{partway modifier}. The syntax
(which is loosely inspired by Uwe Kern's |xcolor| package) is the
following:
\begin{quote}
  \meta{coordinate}\declare{|!|\meta{number}|!|\opt{\meta{angle}|:|}\meta{second coordinate}}
\end{quote}
One could write for instance
\begin{codeexample}[code only]
(1,2)!.75!(3,4)
\end{codeexample}
The meaning of this is: ``Use the coordinate that is three quarters on
the way from |(1,2)| to |(3,4)|.'' In general, \meta{coordinate
  x}|!|\meta{number}|!|\meta{coordinate y} yields the coordinate
$(1-\meta{number})\meta{coordinate x} + \meta{number} \meta{coordinate
  y}$. Note that this is a bit different from the way the
\meta{number} is interpreted in the |xcolor| package: First, you use a
factor between $0$ and $1$, not a percentage, and, second, as the
\meta{number} approaches $1$, we approach the second coordinate, not
the first. It is permissible to use \meta{numbers} that are smaller
than $0$ or larger than $1$. The \meta{number} is evaluated using the
|\pgfmathparse| command and, thus, it can involve complicated
computations. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \draw (1,0) -- (3,2);
  
  \foreach \i in {0,0.2,0.5,0.9,1}
    \node at ($(1,0)!\i!(3,2)$) {\i};
\end{tikzpicture}
\end{codeexample}

The \meta{second coordinate} may be prefixed by an \meta{angle},
separated with a colon, as in |(1,1)!.5!60:(2,2)|. The general meaning
of \meta{a}|!|\meta{factor}|!|\meta{angle}|:|\meta{b} is ``First,
consider the line from \meta{a} to \meta{b}. Then rotate this line by
\meta{angle} \emph{around the point \meta{a}}. Then the two endpoints
of this line will be \meta{a} and some point \meta{c}. Use this point
\meta{c} for the subsequent computation, namely the partway
computation.''

Here are two examples:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,3);

  \coordinate (a) at (1,0);
  \coordinate (b) at (3,2);

  \draw[->] (a) -- (b);

  \coordinate (c) at ($ (a)!1! 10:(b) $);

  \draw[->,red] (a) -- (c);

  \fill ($ (a)!.5! 10:(b) $) circle (2pt);
\end{tikzpicture}
\end{codeexample}


\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (4,4);

  \foreach \i in {0,0.1,...,2}
    \fill ($(2,2) !\i! \i*180:(3,2)$) circle (2pt);
\end{tikzpicture}
\end{codeexample}


You can repeatedly apply modifiers. That is, after any modifier
you can add another (possibly different) modifier.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \draw (0,0) -- (3,2);
  \draw[red] ($(0,0)!.3!(3,2)$) -- (3,0);
  \fill[red] ($(0,0)!.3!(3,2)!.7!(3,0)$) circle (2pt);
\end{tikzpicture}
\end{codeexample}


\subsubsection{The Syntax of Distance Modifiers}

A \emph{distance modifier} has nearly the same syntax as a partway
modifier, only you use a \meta{dimension} (something like |1cm|)
instead of a \meta{factor} (something like |0.5|):
\begin{quote}
  \meta{coordinate}\declare{|!|\meta{dimension}|!|\opt{\meta{angle}|:|}\meta{second coordinate}}
\end{quote}

When you write \meta{a}|!|\meta{dimension}|!|\meta{b}, this means the
following: Use the point that is distanced \meta{dimension} from
\meta{a} on the straight line from \meta{a} to \meta{b}. Here is an example:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \draw (1,0) -- (3,2);
  
  \foreach \i in {0cm,1cm,15mm}
    \node at ($(1,0)!\i!(3,2)$) {\i};
\end{tikzpicture}
\end{codeexample}

As before, if you use a \meta{angle}, the \meta{second coordinate} is
rotated by this much around the \meta{coordinate} before it is used.

The combination of an \meta{angle} of |90| degrees with a distance can
be used to ``offset'' a point relative to a line. Suppose, for
instance, that you have computed a point |(c)| that lies somewhere on
a line from |(a)| to~|(b)| and you now wish to offset this point by
|1cm| so that the distance from this offset point to the line is
|1cm|. This can be achieved as follows:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \coordinate (a) at (1,0);
  \coordinate (b) at (3,1);

  \draw (a) -- (b);

  \coordinate (c) at ($ (a)!.25!(b) $);
  \coordinate (d) at ($ (c)!1cm!90:(b) $);

  \draw [<->] (c) -- (d) node [sloped,midway,above] {1cm};
\end{tikzpicture}
\end{codeexample}



\subsubsection{The Syntax of Projection Modifiers}

The projection modifier is also similar to the above modifiers: It also
gives a point on a line from the \meta{coordinate} to the \meta{second
  coordinate}. However, the \meta{number} or \meta{dimension} is replaced by a
\meta{projection coordinate}:
\begin{quote}
  \meta{coordinate}\declare{|!|\meta{projection coordinate}|!|\opt{\meta{angle}|:|}\meta{second coordinate}}
\end{quote}

Here is an example:
\begin{codeexample}[code only]
(1,2)!(0,5)!(3,4)
\end{codeexample}

The effect is the following: We project the \meta{projection
  coordinate} orthogonally onto to the line from \meta{coordinate} to
\meta{second coordinate}. This makes it easy to compute projected
points: 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \coordinate (a) at (0,1);
  \coordinate (b) at (3,2);
  \coordinate (c) at (2.5,0);

  \draw (a) -- (b) -- (c) -- cycle;

  \draw[red]    (a) -- ($(b)!(a)!(c)$);
  \draw[orange] (b) -- ($(a)!(b)!(c)$);
  \draw[blue]   (c) -- ($(a)!(c)!(b)$);
\end{tikzpicture}
\end{codeexample}


==> pgfmanual-en-tikz-decorations.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Decorated Paths}

\label{section-tikz-decorations}


\subsection{Overview}

Decorations are a general concept to make (sub)paths ``more
interesting.'' Before we have a look at the details, let us have a
look at some examples:

\begin{codeexample}[]
\begin{tikzpicture}[thick]
  \draw                                                (0,3)   -- (3,3);
  \draw[decorate,decoration=zigzag]                    (0,2.5) -- (3,2.5);
  \draw[decorate,decoration=brace]                     (0,2)   -- (3,2);
  \draw[decorate,decoration=triangles]                 (0,1.5) -- (3,1.5);
  \draw[decorate,decoration={coil,segment length=4pt}] (0,1)   -- (3,1);
  \draw[decorate,decoration={coil,aspect=0}]           (0,.5)  -- (3,.5);
  \draw[decorate,decoration={expanding waves,angle=7}] (0,0)   -- (3,0);
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \node [fill=red!20,draw,decorate,decoration={bumps,mirror},
         minimum height=1cm]
  {Bumpy};
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \filldraw[fill=blue!20]                    (0,3)
  decorate [decoration=saw]             { -- (3,3) }
  decorate [decoration={coil,aspect=0}] { -- (2,1) }
  decorate [decoration=bumps]           { -| (0,3) }; 
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \node [fill=yellow!50,draw,thick, minimum height=2cm, minimum width=3cm,
         decorate, decoration={random steps,segment length=3pt,amplitude=1pt}]
    {Saved from trash};
\end{tikzpicture}
\end{codeexample}

The general idea of decorations is the following: First, you construct
a path using the usual path construction commands. The resulting path
is, in essence, a series of straight and curved lines. Instead of
directly using this path for filling or drawing, you can then specify
that it should form the basis for a decoration. In this case,
depending on which decoration you use, a new path is constructed
``along'' the path you specified. For instance, with the |zigzag|
decoration, the new path is a zigzagging line that goes along the old
path.

Let us have a look at an example: In the first picture, we see a path
that consists of a line, an arc, and a line. In the second picture,
this path has been used as the basis of a decoration.

\begin{codeexample}[]
\tikz \fill
  [fill=blue!20,draw=blue,thick] (0,0) -- (2,1) arc (90:-90:.5) -- cycle;
\end{codeexample}
\begin{codeexample}[]
\tikz \fill [decorate,decoration={zigzag}]
  [fill=blue!20,draw=blue,thick] (0,0) -- (2,1) arc (90:-90:.5) -- cycle;
\end{codeexample}

It is also possible to decorate only a subpath (the exact syntax will
be explained later in this section).
\begin{codeexample}[]
\tikz \fill [decoration={zigzag}]
  [fill=blue!20,draw=blue,thick] (0,0) -- (2,1)
    decorate { arc (90:-90:.5) } -- cycle;
\end{codeexample}

The |zigzag| decoration will be called a \emph{path
  morphing} decoration because it morphs a path into a different, but
topologically equivalent path. Not all decorations are path
morphing; rather there are three kinds of decorations.


\begin{enumerate}
\item The just-mentioned \emph{path morphing} decorations morph the
  path in the sense that what used to be a straight  line might
  afterwards be a squiggly line or might have bumps. However, a line
  is still and a line and path deforming decorations do not change
  the number of subpaths. 

  Examples of such decorations are the |snake| or the |zigzag|
  decoration. Many such decorations are defined in the library
  |decorations.pathmorphing|.
  
\item \emph{Path replacing} decorations completely replace the
  path by a different path that is only ``loosely based'' on the
  original path. For instance, the |crosses| decoration replaces a path
  by a path consisting of a sequence of crosses. Note how in the
  following example filling the path has no effect since the path
  consist only of (numerous) unconnected straight line subpaths:
\begin{codeexample}[]
\tikz \fill [decorate,decoration={crosses}]
  [fill=blue!20,draw=blue,thick] (0,0) -- (2,1) arc (90:-90:.5) -- cycle;
\end{codeexample}

  Examples of path replacing decorations are |crosses| or |ticks| or
  |shape backgrounds|. Such decorations are defined in the library
  |decorations.pathreplacing|, but also in |decorations.shapes|.
  
\item \emph{Path removing} decorations completely remove the
  to-be-decorated path. Thus, they have no effect on the main path
  that is being constructed. Instead, they typically have numerous
  \emph{side  effects}. For instance, they might ``write some text''
  along the (removed) path or they might place nodes along this
  path. Note that for such decorations the path usage command for the
  main path have no influence on how the decoration looks like.

\begin{codeexample}[]
\tikz \fill [decorate,decoration={text along path,
               text=This is a text along a path. Note how the path is lost.}]
  [fill=blue!20,draw=blue,thick] (0,0) -- (2,1) arc (90:-90:.5) -- cycle;
\end{codeexample}
\end{enumerate}

Decorations are defined in different decoration libraries, see
Section~\ref{section-library-decorations} for details. It is also
possible to define your own decorations, see
Section~\ref{section-base-decorations}, but you need to use the
\pgfname\ basic layer and a bit of theory is involved.

Decorations can be used to decorate already decorated paths. In the
following three graphics, we start with a simple path, then decorate
it once, and then decorate the decorated path once more.

\begin{codeexample}[]
\tikz \fill [fill=blue!20,draw=blue,thick]
  (0,0) rectangle (3,2);
\end{codeexample}
\begin{codeexample}[]
\tikz \fill [fill=blue!20,draw=blue,thick]
  decorate[decoration={zigzag,segment length=10mm,amplitude=2.5mm}]
    { (0,0) rectangle (3,2) };
\end{codeexample}
\begin{codeexample}[]
\tikz \fill [fill=blue!20,draw=blue,thick]
  decorate[decoration={crosses,segment length=2mm}] {
    decorate[decoration={zigzag,segment length=10mm,amplitude=2.5mm}] {
      (0,0) rectangle (3,2) 
    }
  };
\end{codeexample}

One final word of warning: Decorations can be pretty slow to
typeset and they can be inaccurate. The reason is that \pgfname\ has
to a \emph{lot} of rather difficult computations in the background and
\TeX\ is not very good at doing math. Decorations are fastest when
applied to straight line segments, but even then they are much slower
than other alternative. For instance, the |ticks| decoration can be
simulated by clever use of a dashing pattern and the dashing pattern
will literally be thousands of times faster to typeset. However, for
most decorations there are no real alternatives.

\begin{tikzlibrary}{decorations}
  In order to use decorations, you first have to load a decoration
  library. This |decoration| library defines the basic options
  described in the following, but it does not define any new
  decorations. This is done by libraries like
  |decorations.text|. Since these more specialized libraries include
  the |decoration| library automatically, you usually do not have to
  bother about it.
\end{tikzlibrary}



\subsection{Decorating a Subpath Using the Decorate Path Command}

The most general way to decorate a (sub)path is the following path
command.

\begin{pathoperation}{decorate}{\opt{\oarg{options}}\marg{subpath}}
  This path operation causes the \meta{subpath} to be
  decorated using the current decoration. Depending on the decoration,
  this may or may not extend the current path.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \draw decorate [decoration={name=zigzag}]
         { (0,0) .. controls (0,2) and (3,0) .. (3,2) |- (0,0) };
\end{tikzpicture}
\end{codeexample}
  The path can include straight lines, curves,
  rectangles, arcs, circles, ellipses, and even already decorated
  paths (that is, you can nest applications of the |decorate| path
  command, see below).

  Due to the limits on the precision in  \TeX, some inaccuraces in
  positioning when crossing input segment boundaries may occasionally be
  found. 

  You can use nodes normally inside the \meta{subpath}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \draw decorate [decoration={name=zigzag}]
    { (0,0) -- (2,2) node (hi) [left,draw=red] {Hi!} arc(90:0:1)};

  \draw [blue] decorate [decoration={crosses}] {(3,0) -- (hi)};
\end{tikzpicture}
\end{codeexample}
  
  The following key is used to select the decoration and also to
  select further ``rendering options'' for the decoration.

  \begin{key}{/pgf/decoration=\meta{decoration options}}
    \keyalias{tikz}
    This option is used to specify which decoration is used and how it
    will look like. Note that his key will \emph{not} cause any
    decorations to be applied, immediately. It takes the |decorate| path
    command or the |decorate| option to actually decorate a path. The
    |decoration| option is only used to specify which decoration should
    be used, in principle. You can also use this option at the
    beginning of a picture or a scope to specify the decoration to be
    used with each invocation of the |decorate| path
    command. Naturally, any local options of the |decorate| path
    command override these ``global'' options.
\begin{codeexample}[]
\begin{tikzpicture}[decoration=zigzag]
  \draw       decorate                      {(0,0) -- (3,2)};
  \draw [red] decorate [decoration=crosses] {(0,2) -- (3,0)};
\end{tikzpicture}
\end{codeexample}
    
    The \meta{decoration options} are special options
    (which have the path prefix |/pgf/decoration/|) that determine the
    properties of the decoration. Which options are appropriate for a
    decoration depend strongly on the decoration, you will have to look
    up the appropriate options in the documentation of the decoration,
    see Section~\ref{section-library-decorations}.
    
    There is one option (available only in \tikzname) that is special:
    \begin{key}{/pgf/decoration/name=\meta{name} (initially none)}
      Use this key to set which decoration is to be used. The
      \meta{name} can both be a decoration or a meta-decoration (you
      need to worry about the difference only if you wish to define
      your own decorations).
      
      If you set \meta{name} to |none|, no decorations are added.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \draw decorate [decoration={name=zigzag}]
         { (0,0) .. controls (0,2) and (3,0) .. (3,2) };
\end{tikzpicture}
\end{codeexample}
      Since this option is used so often, you can also leave out the
      |name=| part. Thus, the above example can be rewritten more
      succinctly: 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] grid (3,2);
  \draw decorate [decoration=zigzag]
         { (0,0) .. controls (0,2) and (3,0) .. (3,2) };
\end{tikzpicture}
\end{codeexample}
      In general, when \meta{decoration options} are parsed, for each
      unknown key it is checked whether that key happens to be a
      (meta-)decoration and, if so, the |name| option is executed for
      this key.
    \end{key}

    Further options allow you to adjust the position of decorations
    relative to the to-be-decorated path. See
    Section~\ref{section-decorations-adjust} below for details.
  \end{key}

  Recall that some decorations actually completely remove the
  to-be-decorated path. In such cases, the construction of the main
  path is resumed after the |decorate| path command ends.
  
\begin{codeexample}[]
\begin{tikzpicture}[decoration={text along path,text=
      around and around and around and around we go}]

  \draw (0,0) -- (1,1) decorate { -- (2,1) } -- (3,0);
\end{tikzpicture}
\end{codeexample}

  It is permissible to nest |decorate| commands. In this case, the
  path resulting from the first decoration process is used as the
  to-be-decorated path for the second decoration process. This is
  especially useful for drawing fractals. The |Koch snowflake|
  decoration replaces a straight line like \tikz\draw (0,0) -- (1,0);
  by \tikz[decoration=Koch snowflake] \draw decorate{(0,0) --
    (1,0)};. Repeatedly applying this transformation to a triangle
  yields a fractal that looks a bit like a snowflake, hence the name. 
\begin{codeexample}[]
\begin{tikzpicture}[decoration=Koch snowflake,draw=blue,fill=blue!20,thick]
  \filldraw (0,0) -- ++(60:1) -- ++(-60:1) -- cycle ;
  \filldraw decorate{ (0,-1) -- ++(60:1) -- ++(-60:1) -- cycle };
  \filldraw decorate{ decorate{ (0,-2.5) -- ++(60:1) -- ++(-60:1) -- cycle }};
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}



\subsection{Decorating a Complete Path}

You may sometimes wish to decorate a path over whose construction you
have no control. For instance, the path of the background of a node is
created without your having a chance to issue a |decorate| path
command. In such cases you can use the following option, which allows
you to decorate a path ``after the fact.''

\begin{key}{/tikz/decorate=\opt{\meta{boolean}} (default true)}
  When this key is set, the whole path is decorated after it has been
  finished. The decoration used for decorating the path is set via the
  |decoration| way, in exactly the same way as for the |decorate| path
  command. Indeed, the following two commands have the same effect:
  \begin{enumerate}
  \item |\path decorate[|\meta{options}|] {|\meta{path}|};|
  \item |\path [decorate,|\meta{options}|] |\meta{path}|;|
  \end{enumerate}
  The main use or the |decorate| option is the you can also use it
  with the nodes. It then causes the background path of the node to be
  decorated. Note that you decorate a background path only once in
  this manner. That is, in contrast to the |decorate| path command you
  cannot apply this option twice (this would just set it to |true|,
  once more).

\begin{codeexample}[]
\begin{tikzpicture}[decoration=zigzag]
  \draw [help lines] (0,0) grid (3,5);
  
  \draw [fill=blue!20,decorate] (1.5,4) circle (1cm);

  \node at (1.5,2.5) [fill=red!20,decorate,ellipse] {Ellipse};

  \node at (1.5,1) [inner sep=6mm,fill=red!20,decorate,ellipse,decoration=
    {text along path,text={This is getting silly}}] {Ellipse};
\end{tikzpicture}
\end{codeexample}

  In the last example, the |text along path| decoration removes the
  path. In such cases it is useful to use a pre- or postaction to
  cause the decoration to be applied only before or after the main
  path has been used. Incidentally, this is another application of the
  |decorate| option that you cannot achieve with the decorate path
  command. 
\begin{codeexample}[]
\begin{tikzpicture}[decoration=zigzag]
  \node at (1.5,1) [inner sep=6mm,fill=red!20,ellipse,
    postaction={decorate,decoration=
    {text along path,text={This is getting silly}}}] {Ellipse};
\end{tikzpicture}
\end{codeexample}
  Here is more useful example, where a postaction is used to add the
  path after the main path has been drawn.
\begin{codeexample}[]
\catcode`\|12
\begin{tikzpicture}
\draw [help lines] grid (3,2);
\fill [draw=red,fill=red!20,
         postaction={decorate,decoration={raise=2pt,text along path,
           text=around and around and around and around we go}}] 
  (0,1) arc (180:-180:1.5cm and 1cm);
\end{tikzpicture}
\end{codeexample} 
\end{key}


\subsection{Adjusting Decorations}

\label{section-decorations-adjust}

\subsubsection{Positioning Decorations Relative to the To-Be-Decorate Path}

The following option, which are only available with \tikzname, allow
you to modify the positioning of decorations relative to the
to-be-decorated path.

\begin{key}{/pgf/decoration/raise=\meta{dimension} (initially 0pt)}
  The segments of the decoration are raised by \meta{dimension}
  relative to the to-be-decorated path. More precisely, the segments
  of the path are offset by this much ``to the left'' of the path as
  we travel along the path. This raising is done after and in addition
  to any transformations set using the |transform| option (see below).

  A negative \meta{dimension} will offset the decoration ``to the
  right'' of the to-be-decorated path.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \draw (0,0) -- (1,1) arc (90:0:2 and 1);
  \draw      decorate [decoration=crosses]
        { (0,0) -- (1,1) arc (90:0:2 and 1) };
  \draw[red] decorate [decoration={crosses,raise=5pt}]
        { (0,0) -- (1,1) arc (90:0:2 and 1) };
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/decoration/mirror=\opt{\meta{boolean}}}
  Causes the segments of the decoration to be mirrored along the
  to-be-decorated path. This is done after and in addition to any
  transformations set using the |transform| and/or |raise| options.
\begin{codeexample}[]
\begin{tikzpicture}
  \node (a)          {A};
  \node (b) at (2,1) {B};
  \draw                                                    (a) -- (b);
  \draw[decorate,decoration=brace]                         (a) -- (b);
  \draw[decorate,decoration={brace,mirror},red]            (a) -- (b);
  \draw[decorate,decoration={brace,mirror,raise=5pt},blue] (a) -- (b);
\end{tikzpicture}
\end{codeexample}
\end{key}


\begin{key}{/pgf/decoration/transform=\meta{transformations}}
  This key allows you to specify general \meta{transformations} to be
  applied to the segments of a decoration. These transformations are
  applied before and independently of |raise| and |mirror|
  transformations. The \meta{transformations} should be normal
  \tikzname\ transformations like |shift| or |rotate|.

  In the following example the |shift only| transformation is used to
  make sure that the crosses are \emph{not} sloped along the path.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \draw (0,0) -- (1,1) arc (90:0:2 and 1);
  \draw[red,very thick] decorate [decoration={
               crosses,transform={shift only},shape size=1.5mm}]
        { (0,0) -- (1,1) arc (90:0:2 and 1) };
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsubsection{Starting and Ending Decorations Early or Late}

You sometimes may wish to ``end'' a decoration a bit early on the
path. For instance, you might wish a |snake| decoration to stop 5mm
before the end of the path and to continue in a straight line. There
are different ways of achieving this effect, but the easiest may be
the |pre| and |post| options, which only have an effect in
\tikzname. Note, however, that they can only be used with decorations,
not with meta-decorations.

\begin{key}{/pgf/decoration/pre=\meta{decoration} (initially lineto)}
  This key sets a decoration that should be used before the main
  decoration starts. The \meta{decoration} will be used for a length
  of |pre length|, which |0pt| by default. Thus, for the |pre| option
  to have any effect, you also need to set the |pre length| option.
\begin{codeexample}[]
\begin{tikzpicture}
\tikz [decoration={zigzag,pre=lineto,pre length=1cm}]
  \draw [decorate] (0,0) -- (2,1) arc (90:0:1);
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
\tikz [decoration={zigzag,pre=moveto,pre length=1cm}]
  \draw [decorate] (0,0) -- (2,1) arc (90:0:1);
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
\tikz [decoration={zigzag,pre=crosses,pre length=1cm}]
  \draw [decorate] (0,0) -- (2,1) arc (90:0:1);
\end{tikzpicture}
\end{codeexample}

  Note that the default |pre| option is |lineto|, not |curveto|. This
  means that the default |pre| decoration will not follow curves (for
  efficiency reasons). Change the |pre| key to |curveto| if you have a
  curved path. 
\begin{codeexample}[]
\begin{tikzpicture}
\tikz [decoration={zigzag,pre length=3cm}]
  \draw [decorate] (0,0) -- (2,1) arc (90:0:1);
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
\tikz [decoration={zigzag,pre=curveto,pre length=3cm}]
  \draw [decorate] (0,0) -- (2,1) arc (90:0:1);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/decoration/pre length=\meta{dimension} (initially 0pt)}
  This key sets the distance along which the pre-decoration should be
  used. If you do not need/wish a pre-decoration, set this key to
  |0pt| (exactly this string, not just to something that evaluated to
  the same things such as |0cm|).
\end{key}

\begin{key}{/pgf/decorations/post=\meta{decoration} (initially
    lineto)}
  Works like |pre|, only for the end of the decoration.  
\end{key}

\begin{key}{/pgf/decorations/post length=\meta{dimension} (initially
    0pt)}
  Works like |pre length|, only for the end of the decoration.  
\end{key}

Here is a typical example that shows how these keys can be used:

\begin{codeexample}[]
\begin{tikzpicture}
  [decoration=snake,
   line around/.style={decoration={pre length=#1,post length=#1}}]

  \draw[->,decorate]                  (0,0)    -- ++(3,0);
  \draw[->,decorate,line around=5pt]  (0,-5mm) -- ++(3,0);
  \draw[->,decorate,line around=1cm]  (0,-1cm) -- ++(3,0);
\end{tikzpicture}
\end{codeexample}



\endinput

==> pgfmanual-en-tikz-design.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Design Principles}

This section describes the design principles behind the \tikzname\
frontend, where \tikzname\ means ``\tikzname\ ist \emph{kein}
Zeichenprogramm.'' To use \tikzname, as a \LaTeX\ user say
|\usepackage{tikz}| somewhere in the preamble, as a plain \TeX\ user
say |\input tikz.tex|. \tikzname's job is to make your life easier by
providing an easy-to-learn and easy-to-use syntax for describing
graphics. 

The commands and syntax of \tikzname\ were influenced by several
sources. The basic command names and the notion of  path operations is
taken from \textsc{metafont}, the option mechanism comes from
\textsc{pstricks}, the notion of styles is reminiscent of
\textsc{svg}. To make it all work together, some compromises were
necessary. I also added some ideas of my own, like coordinate
transformations.  

The following basic design principles underlie \tikzname:
\begin{enumerate}
\item Special syntax for specifying points.
\item Special syntax for path specifications.
\item Actions on paths.
\item Key-value syntax for graphic parameters.
\item Special syntax for nodes.
\item Special syntax for trees.
\item Grouping of graphic parameters.
\item Coordinate transformation system.
\end{enumerate}



\subsection{Special Syntax For Specifying Points}

\tikzname\ provides a special syntax for specifying points and
coordinates. In the simplest case, you provide two \TeX\ dimensions,
separated by commas, in round brackets as in |(1cm,2pt)|.

You can also specify a point in polar coordinates by using a colon
instead of a comma as in |(30:1cm)|, which means ``1cm in a 30
degrees direction.'' 

If you do not provide a unit, as in |(2,1)|, you specify a point in
\pgfname's $xy$-coordinate system. By default, the unit $x$-vector
goes 1cm to the right and the unit $y$-vector goes 1cm upward.

By specifying three numbers as in |(1,1,1)| you specify a point in
\pgfname's $xyz$-coordinate system.

It is also possible to use an anchor of a previously defined shape
as in |(first node.south)|.

You can add two plus signs before a coordinate as in
|++(1cm,0pt)|. This means ``1cm to the right of the last point
used.'' This allows you to easily specify relative movements. For
example, |(1,0) ++(1,0) ++(0,1)| specifies the three coordinates
|(1,0)|, then |(2,0)|, and |(2,1)|.

Finally, instead of two plus signs, you can also add a single
one. This also specifies a point in a relative manner, but it does
not ``change'' the current point used in subsequent relative
commands. For example, |(1,0) +(1,0) +(0,1)| specifies the three
coordinates |(1,0)|, then |(2,0)|, and |(1,1)|.

\subsection{Special Syntax For Path Specifications}

When creating a picture using \tikzname, your main job is the
specification of \emph{paths}. A path is a series of straight or curved
lines, which need not be connected. \tikzname\ makes it easy to
specify paths, partly using the syntax of \textsc{metapost}. For
example, to specify a triangular path you use
\begin{codeexample}[code only]
(5pt,0pt) -- (0pt,0pt) -- (0pt,5pt) -- cycle
\end{codeexample}
and you get \tikz \draw (5pt,0pt) -- (0pt,0pt) -- (0pt,5pt) -- cycle;
when you draw this path.

\subsection{Actions on Paths}

A path is just a series of straight and curved lines, but it is not
yet specified what should happen with it. One can \emph{draw} a
path, \emph{fill} a path, \emph{shade} it, \emph{clip} it, or do any
combination of these. Drawing (also known as \emph{stroking}) can be
thought of as taking a pen of a certain thickness and moving it
along the path, thereby drawing on the canvas. Filling means that
the interior of the path is filled with a uniform color. Obviously,
filling makes sense only for \emph{closed} paths and a path is
automatically closed prior to filling, if necessary.

Given a path as in |\path (0,0) rectangle (2ex,1ex);|, you can draw
it by adding the |draw| option as in
|\path[draw] (0,0) rectangle (2ex,1ex);|, which yields \tikz \path[draw]
(0,0) rectangle (2ex,1ex);. The |\draw| command is just an abbreviation for
|\path[draw]|. To fill a path, use the |fill| option or the |\fill|
command, which is an abbreviation for |\path[fill]|. The
|\filldraw| command is an abbreviation for
|\path[fill,draw]|. Shading is caused by the |shade| option (there
are |\shade| and |\shadedraw| abbreviations) and clipping by the
|clip| option. There is is also a |\clip| command, which does the
same as |\path[clip]|, but not commands like |\drawclip|. Use, say,
|\draw[clip]| or |\path[draw,clip]| instead.

All of these commands can only be used inside |{tikzpicture}|
environments. 

\tikzname\ allows you to use different colors for filling and
stroking.

\subsection{Key-Value Syntax for Graphic Parameters}

Whenever \tikzname\ draws or fills a path, a large number of graphic
parameters influenced the rendering. Examples include the colors
used, the dashing pattern, the clipping area, the line width, and
many others. In \tikzname, all these options are specified as lists
of so called key-value pairs, as in |color=red|, that are
passed as optional parameters to the path drawing and filling
commands. This usage is similar to \textsc{pstricks}. For
example, the following will draw a thick, red triangle;
\begin{codeexample}[]
\tikz \draw[line width=2pt,color=red] (1,0) -- (0,0) -- (1,0) -- cycle; 
\end{codeexample}

\subsection{Special Syntax for Specifying Nodes}
\tikzname\ introduces a special syntax for adding text or, more
generally, nodes to a graphic. When you specify a path, add nodes as
in the following example:
\begin{codeexample}[]
\tikz \draw (1,1) node {text} -- (2,2);
\end{codeexample}
Nodes are inserted at the current position of
the path, but only \emph{after} the path has been rendered. When
special options are given, as in
|\draw (1,1) node[circle,draw] {text};|, the text is not just put 
at the current position. Rather, it is surrounded by a circle and
this circle is ``drawn.'' 

You can add a name to a node for later reference either by using the
option   |name=|\meta{node name} or by stating the node name in
parentheses outside the text as in |node[circle](name){text}|.

Predefined shapes include |rectangle|, |circle|, and |ellipse|, but
it is possible (though a bit challenging) to define new shapes.

\subsection{Special Syntax for Specifying Trees}

In addition to the ``node syntax,'' \tikzname\ also introduces a
special syntax for drawing trees. The syntax is intergrated with the
special node syntax and only few new commands need to be remebered.
In essence, a |node| can be followed by any number of children, each
introduced by the keyword |child|. The children are nodes themselves,
each of which may have children in turn.

\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
    child {node {left}}
    child {node {right}
      child {node {child}}
      child {node {child}}
    };
\end{tikzpicture}
\end{codeexample}

Since trees are made up from nodes, it is possible to use options to
modify the way trees are drawn. Here are two examples of the above tree,
redrawn with different options:

\begin{codeexample}[]
\begin{tikzpicture}
  [edge from parent fork down,
   every node/.style={fill=red!30,rounded corners},
   edge from parent/.style={red,-o,thick,draw}]
  \node {root}
      child {node {left}}
      child {node {right}
        child {node {child}}
        child {node {child}}
      };
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  [parent anchor=east,child anchor=west,grow=east,
   every node/.style={ball color=red,circle,text=white}
   edge from parent/.style={draw,dashed,thick,red}]
  \node {root}
      child {node {left}}
      child {node {right}
        child {node {child}}
        child {node {child}}
      };
\end{tikzpicture}
\end{codeexample}

\subsection{Grouping of Graphic Parameters}

Graphic parameters should often apply to several path drawing or
filling commands. For example, we may wish to draw numerous lines all
with the same line width of 1pt. For this, we put these commands
in a |{scope}| environment that takes the desired graphic options
as an optional parameter. Naturally, the specified graphic
parameters apply only to the drawing and filling commands inside the
environment. Furthermore, nested |{scope}| environments or
individual drawing commands can override the graphic parameters of
outer |{scope}| environments. In the following example, three red
lines, two green lines, and one blue line are drawn:

\begin{codeexample}[]
\begin{tikzpicture}
  \begin{scope}[color=red]
    \draw (0mm,10mm) -- (10mm,10mm);
    \draw (0mm, 8mm) -- (10mm, 8mm);
    \draw (0mm, 6mm) -- (10mm, 6mm);
  \end{scope}
  \begin{scope}[color=green]
    \draw             (0mm, 4mm) -- (10mm, 4mm);
    \draw             (0mm, 2mm) -- (10mm, 2mm);
    \draw[color=blue] (0mm, 0mm) -- (10mm, 0mm);
  \end{scope}
\end{tikzpicture}
\end{codeexample}

The |{tikzpicture}| environment itself also behaves like a
|{scope}| environment, that is, you can specify graphic parameters
using an optional argument. These optional apply to all commands in
the picture.


\subsection{Coordinate Transformation System}

\tikzname\ supports both \pgfname's \emph{coordinate} transformation
system to perform transformations as well as \emph{canvas}
transformations, a more low-level transformation system. (For 
details on the difference between coordinate transformations and
canvas transformations see Section~\ref{section-design-transformations}.) 

The syntax is setup in such a way that is harder to use canvas
transformations than coordinate transformations. There are two reasons
for this: First, the canvas transformation must be used with great
care and often results in ``bad'' graphics with changing line width
and text in wrong sizes. Second, \pgfname\ looses track of where nodes
and shapes are positioned when canvas transformations are used.
So, in almost all circumstances, you should use coordinate
transformations rather than canvas transformations.


==> pgfmanual-en-tikz-matrices.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Matrices and Alignment}

\label{section-matrices}

\subsection{Overview}

When creating pictures, one often faces the problem of correctly
aligning parts of the picture. For example, you might wish that the
base lines of certain nodes should be on the same line and some
further nodes should be below these nodes with, say, their centers on
a vertical lines. There are different ways of solving such
problems. For example, by making clever use of anchors, nearly all
such alignment problems can be solved. However, this often leads to
complicated code. An often simpler way is to use \emph{matrices},
the use of which is explaied in the current section.

A \tikzname\ matrix is similar to \LaTeX's |{tabular}| or
|{array}| environment, only instead of text each cell contains a
little picture or a node. The sizes of the cells are automatically
adjusted such that they are large enough to contain all the cell
contents.

Matrices are a powerful tool and they need to handled with some care.
For impatient readers who skip the rest of this section: you
\emph{must} end \emph{every} row with |\\|. In particular, the last
row \emph{must} be ended with |\\|.

Many of the ideas implemented in \tikzname's matrix support are due to
Mark Wibrow -- many thanks to Mark at this point!



\subsection{Matrices are Nodes}

Matrices are special in many ways, but for most purposes matrices are
treated like nodes. This means, that you use the |node| path command
to create a matrix and you only use a special option, namely the
|matrix| option, to signal that the node will contain a
matrix. Instead of the usual \TeX-box that makes up the |text| part of
the node's shape, the matrix is used. Thus, in particular, a matrix
can have a shape, this shape can be drawn or filled, it can be used in
a tree, and so on. Also, you can refer to the different anchors of a
matrix. 

\begin{key}{/tikz/matrix=\meta{true or false} (default true)}
  This option can be passed to a |node| path command. It signals that
  the node will contain a matrix.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (4,2);
  \node [matrix,fill=red!20,draw=blue,very thick] (my matrix) at (2,1)
  {
    \draw (0,0)   circle (4mm); & \node[rotate=10] {Hello};        \\
    \draw (0.2,0) circle (2mm); & \fill[red]   (0,0) circle (3mm); \\
  };

  \draw [very thick,->] (0,0) |- (my matrix.west);
\end{tikzpicture}
\end{codeexample}
  The exact syntax of the matrix is explained in the course of this
  section.
  \begin{stylekey}{/tikz/every matrix (initially \normalfont empty)}
    This style is used in every matrix.
  \end{stylekey}
\end{key}

Even more so than nodes, matrices will often be the only object on a
path. Because of this, there is a special abbreviation for creating matrices:

\begin{command}{\matrix}
  Inside |{tikzpicture}| this is an abbreviation for |\path node[matrix]|.
\end{command}

Even though matrices are nodes, some options do not have the same
effect as for normal nodes:
\begin{enumerate}
\item Rotations and scaling have no effect on a matrix as a whole
  (however, you can still transform the contents of the cells
  normally). Before the matrix is typeset, the rotational and scaling
  part of the transformation matrix is reset.
\item For multi-part shapes you can only set the |text| part of the
  node. 
\item All options starting with |text| such as |text width| have no
  effect.
\end{enumerate}



\subsection{Cell Pictures}

A matrix consists of rows of \emph{cells}. Each row (including the
last one!) is ended by the command |\\|. The character |&| is used
to separate cells. Inside each cell, you must place commands for
drawing a picture, called the \emph{cell picture} in the
following. (However, cell pictures are not enclosed in a complete
|{pgfpicture}| environment, they are a bit more light-weight. The main
difference is that cell pictures cannot have layers.) It is not
necessary to specify beforehand how many rows or columns there are
going to be and if a row contains less cell pictures than another
line, empty cells are automatically added as needed.


\subsubsection{Alignment of Cell Pictures}

For each cell picture a bounding box is computed. These bounding boxes
and the origins of the cell pictures determine how the cells are
aligned. Let us start with the rows: Consider the cell pictures on the first
row. Each has a bounding box and somewhere inside this bounding box
the origin of the cell picture can be found (the origin might even lie
outside the bounding box, but let us ignore this problem for the
moment). The cell pictures are then shifted around such that all
origins lie on the same horizontal line. This may make it necessary to
shift some cell pictures upwards and other downwards, but it can be
done and this yields the vertical alignment of the cell pictures this
row. The top of the row is then given by the top of the ``highest''
cell picture in the row, the bottom of the row is given by the bottom
of the lowest cell picture. (To be more precise, the height of the row
is the maximum $y$-value of any of the bounding boxes and the depth of
the row is the negated minimum $y$-value of the bounding boxes).

\begin{codeexample}[]
\begin{tikzpicture}
  [every node/.style={draw=black,anchor=base,font=\huge}]

  \matrix [draw=red]
  {
    \node {a}; \fill[blue] (0,0) circle (2pt); &
    \node {X}; \fill[blue] (0,0) circle (2pt); &
    \node {g}; \fill[blue] (0,0) circle (2pt); \\
  };
\end{tikzpicture}
\end{codeexample}

Each row is aligned in this fashion: For each row the cell pictures
are vertically aligned such that the origins lie on the same
line. Then the second row is placed below the first row such that the
bottom of the first row touches the top of the second row (unless a
|row sep| is used to add a bit of space). Then the bottom of the
second row touches the top of the third row, and so on. Typically,
each row will have an individual height and depth.

\begin{codeexample}[]
\begin{tikzpicture}
  [every node/.style={draw=black,anchor=base}]

  \matrix [draw=red]
  {
    \node {a}; & \node {X}; & \node {g}; \\
    \node {a}; & \node {X}; & \node {g}; \\
  };

  \matrix [row sep=3mm,draw=red] at (0,-2)
  {
    \node {a}; & \node {X}; & \node {g}; \\
    \node {a}; & \node {X}; & \node {g}; \\
  };
\end{tikzpicture}
\end{codeexample}

Let us now have a look at the columns. The rules for how the pictures
on any given column are aligned are very similar to the row
alignment: Consider all cell pictures in the first column. Each is
shifted horizontally such that the origins lie on the same vertical
line. Then, the left end of the column is at the left end of the
bounding box that protrudes furthest to the left. The right end of the
column is at the right end of the bounding box that protrudes furthest
to the left. This fixes the horizontal alignment of the cell pictures
in the first column and the same happens the cell pictures in the
other columns. Then, the right end of the first column touches the
left end of the second column (unless |column sep| is used). The right
end of the second column touches the left end of the third column, and
so on. (Internally, two columns are actually used to achieve the
desired horizontal alignment, but that is only and implementation
detail.) 

\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={draw}]
  \matrix [draw=red]
  {
    \node[left]  {Hallo}; \fill[blue] (0,0) circle (2pt); \\
    \node        {X};     \fill[blue] (0,0) circle (2pt); \\
    \node[right] {g};     \fill[blue] (0,0) circle (2pt); \\
  };
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={draw}]
  \matrix [draw=red,column sep=1cm]
  {
    \node {8}; & \node{1}; & \node {6}; \\
    \node {3}; & \node{5}; & \node {7}; \\
    \node {4}; & \node{9}; & \node {2}; \\
  };
\end{tikzpicture}
\end{codeexample}



\subsubsection{Setting and Adjusting Column and Row Spacing}

There are different ways of setting and adjusting the spacing between
columns and rows. First, you can use the options |column sep| and
|row sep| to set a default spacing for all rows and all
columns. Second, you can add options to the |&| character and the |\\|
command to adjust the spacing between two specific columns or
rows. Additionally, you can specify whether the space between two
columns or rows should be considered between the origins of cells in
the column or row or between their borders. 

\begin{key}{/tikz/column sep=\meta{spacing list}}
  This option sets a default space that is added between every two
  columns. This space can be positive or negative and is zero by
  default. The \meta{spacing list} normally contains a single
  dimension like |2pt|.
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [draw,column sep=1cm,nodes=draw]
  {
    \node(a) {123}; & \node (b) {1};   & \node {1}; \\
    \node    {12};  & \node     {12};  & \node {1}; \\
    \node(c) {1};   & \node (d) {123}; & \node {1}; \\
  };
  \draw [red,thick]  (a.east) -- (a.east |- c)
                     (d.west) -- (d.west |- b);
  \draw [<->,red,thick] (a.east) -- (d.west |- b)
    node [above,midway] {1cm};
\end{tikzpicture}
\end{codeexample}
  More generally, the \meta{spacing list} may contain a whole list of
  numbers, separated by commas, and occurrences of the two key words
  |between origins| and |between borders|. The effect of specifying
  such a list is the following: First, all numbers occurring in the
  list are simply added to compute the final spacing. Second,
  concerning the two keywords, the last occurrence of one of the keywords is
  important. If the last occurrence is |between borders| or if neither
  occurs, then the space is inserted between the two columns
  normally. However, if the last occurs is |between origins|, then the 
  following happens: The distance between the columns is adjusted such
  that the difference between the origins of all the cells in the
  first column (remember that they all lie on straight line) and the
  origins of all the cells in the second column is exactly the given
  distance.

  \emph{The |between origins| option can only be used for columns
    mentioned in the first row, that is, you cannot specify this
    option for columns introduced only in later rows.}
  
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [draw,column sep={1cm,between origins},nodes=draw]
  {
    \node(a) {123}; & \node (b) {1};   & \node {1}; \\
    \node    {12};  & \node     {12};  & \node {1}; \\
    \node    {1};   & \node     {123}; & \node {1}; \\
  };
  \draw [<->,red,thick] (a.center) -- (b.center) node [above,midway] {1cm};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/row sep=\meta{spacing list}}
  This option works like |column sep|, only for rows. Here, too, you
  can specify whether the space is added between the lower end of the
  first row and the upper end of the second row, or whether the space
  is computed between the origins of the two rows.
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [draw,row sep=1cm,nodes=draw]
  {
    \node (a) {123}; & \node {1};   & \node {1}; \\
    \node (b) {12};  & \node {12};  & \node {1}; \\
    \node     {1};   & \node {123}; & \node {1}; \\
  };
  \draw [<->,red,thick] (a.south) -- (b.north) node [right,midway] {1cm};
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [draw,row sep={1cm,between origins},nodes=draw]
  {
    \node (a) {123}; & \node {1};   & \node {1}; \\
    \node (b) {12};  & \node {12};  & \node {1}; \\
    \node     {1};   & \node {123}; & \node {1}; \\
  };
  \draw [<->,red,thick] (a.center) -- (b.center) node [right,midway] {1cm};
\end{tikzpicture}
\end{codeexample}
\end{key}

The row-end command |\\| allows you to provide an optional
argument, which must be a dimension. This dimension will be added to
the list in |row sep|. This means that, firstly, any numbers you list
in this argument will be added as an extra row separation between the
line being ended and the next line and, secondly, you can use the
keywords |between origins| and |between borders| to locally overrule
the standard setting for this line pair.
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [row sep=1mm]
  {
    \draw (0,0) circle (2mm); & \draw (0,0) circle (2mm); \\
    \draw (0,0) circle (2mm); & \draw (0,0) circle (2mm); \\[-1mm]
    \draw (0,0) coordinate (a) circle (2mm); &
    \draw (0,0) circle (2mm); \\[1cm,between origins]
    \draw (0,0) coordinate (b) circle (2mm); &
    \draw (0,0) circle (2mm); \\
  };
  \draw [<->,red,thick] (a.center) -- (b.center) node [right,midway] {1cm};
\end{tikzpicture}
\end{codeexample}

The cell separation character |&| also takes an optional
argument, which must also be a spacing list. This spacing list is
added to the |column sep| having a similar effect as the option for
the |\\| command for rows.

This optional spacing list can only be given the first time
a new column is started (usually in the first row), subsequent usages
of this option in later rows have no effect. 
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [draw,nodes=draw,column sep=1mm]
  {
    \node {8}; &[2mm] \node{1}; &[-1mm] \node {6}; \\
    \node {3}; &      \node{5}; &       \node {7}; \\
    \node {4}; &      \node{9}; &       \node {2}; \\
  };
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [draw,nodes=draw,column sep=1mm]
  {
    \node {8}; &[2mm] \node(a){1}; &[1cm,between origins] \node(b){6}; \\
    \node {3}; &      \node   {5}; &                      \node   {7}; \\
    \node {4}; &      \node   {9}; &                      \node   {2}; \\
  };
  \draw [<->,red,thick] (a.center) -- (b.center) node [above,midway] {11mm};
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [draw,nodes=draw,column sep={1cm,between origins}]
  {
    \node (a) {8}; & \node (b) {1}; &[between borders] \node (c) {6}; \\
    \node     {3}; & \node     {5}; &                  \node     {7}; \\
    \node     {4}; & \node     {9}; &                  \node     {2}; \\
  };
  \draw [<->,red,thick] (a.center) -- (b.center) node [above,midway] {10mm};
  \draw [<->,red,thick] (b.east) -- (c.west) node [above,midway] {10mm};
\end{tikzpicture}
\end{codeexample}




\subsubsection{Cell Styles and Options}

For following style and option are useful for changing the appearance
of the all cell pictures:

\begin{stylekey}{/tikz/every cell=\marg{row}\marg{column} (initially \normalfont empty)}
  This style is installed at the beginning of each cell picture with
  the two parameters being the current \meta{row} and \meta{column} of
  the cell. Note that setting this style to |draw| will \emph{not}
  cause all nodes to be drawn since the |draw| option has to be passed
  to each node individually.

  Inside this style (and inside all cells), the current \meta{row} and
  \meta{column} number are also accessible via the counters
  |\pgfmatrixcurrentrow| and |\pgfmatrixcurrentcolumn|.   
\end{stylekey}

\begin{key}{/tikz/cells=\meta{options}}
  This key adds the \meta{options} to the style |every cell|. It mainly
  just a shorthand for the code
  |every cell/.append style=|\meta{options}.
\end{key}

\begin{key}{/tikz/nodes=\meta{options}}
  This key adds the \meta{options} to the style |every node|. It mainly
  just a shorthand for the code |every node/.append style=|\meta{options}.

  The main use of this option is the install some options for the
  nodes \emph{inside} the matrix that should not apply to the matrix
  \emph{itself}. 

\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [nodes={fill=blue!20,minimum size=5mm}]
  {
    \node {8}; & \node{1}; & \node {6}; \\
    \node {3}; & \node{5}; & \node {7}; \\
    \node {4}; & \node{9}; & \node {2}; \\
  };
\end{tikzpicture}
\end{codeexample}
\end{key}

The next set of styles can be used to change the appearance of certain
rows, columns, or cells. If more than one of these styles is defined,
they are executed in the below order (the |every cell| style is
executed before all of the below).
\begin{stylekey}{/tikz/column \meta{number}}
  This style is used for every cell in column \meta{number}.
\end{stylekey}

\begin{stylekey}{/tikz/every odd column}
  This style is used for every cell in an odd column.
\end{stylekey}

\begin{stylekey}{/tikz/every even column}
  This style is used for every cell in an even column.
\end{stylekey}

\begin{stylekey}{/tikz/row \meta{number}}
  This style is used for every cell in row \meta{number}.
\end{stylekey}

\begin{stylekey}{/tikz/every odd row}
  This style is used for every cell in an odd row.
\end{stylekey}

\begin{stylekey}{/tikz/every even row}
  This style is used for every cell in an even row.
\end{stylekey}

\begin{stylekey}{/tikz/row \meta{row number} column \meta{column number}}
  This style is used for the cell in row \meta{row number} and column
  \meta{column number}.
\end{stylekey}


\begin{codeexample}[]
\begin{tikzpicture}
  [row 1/.style={red},
   column 2/.style={green!50!black},
   row 3 column 3/.style={blue}]
    
  \matrix
  {
    \node {8}; & \node{1}; & \node {6}; \\
    \node {3}; & \node{5}; & \node {7}; \\
    \node {4}; & \node{9}; & \node {2}; \\
  };
\end{tikzpicture}
\end{codeexample}

You can use the |column |\meta{number} option to change the alignment
for different columns.

\begin{codeexample}[]
\begin{tikzpicture}
  [column 1/.style={anchor=base west},
   column 2/.style={anchor=base east},
   column 3/.style={anchor=base}]
  \matrix
  {
    \node {123}; & \node{456}; & \node {789}; \\
    \node {12}; & \node{45}; & \node {78}; \\
    \node {1}; & \node{4}; & \node {7}; \\
  };
\end{tikzpicture}
\end{codeexample}


In many matrices all cell pictures have nearly the same code. For
example, cells typically start with |\node{| and end |};|. The
following options allow you to execute such code in all cells:

\begin{key}{/tikz/execute at begin cell=\meta{code}}
  The code will be executed at the beginning of each nonempty cell.
\end{key}
\begin{key}{/tikz/execute at end cell=\meta{code}}
  The code will be executed at the end of each nonempty cell.
\end{key}
\begin{key}{/tikz/execute at empty cell=\meta{code}}
  The code will be executed inside each empty cell.
\end{key}

\begin{codeexample}[]
\begin{tikzpicture}
  [matrix of nodes/.style={
     execute at begin cell=\node\bgroup,
     execute at end cell=\egroup;%
   }]
  \matrix [matrix of nodes]
  {
    8 & 1 & 6 \\
    3 & 5 & 7 \\
    4 & 9 & 2 \\
  };
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}
  [matrix of nodes/.style={
     execute at begin cell=\node\bgroup,
     execute at end cell=\egroup;,%
     execute at empty cell=\node{--};%
   }]
  \matrix [matrix of nodes]
  {
    8 & 1 &   \\
    3 &   & 7 \\
      &   & 2 \\
  };
\end{tikzpicture}
\end{codeexample}

The |matrix| library defines a number of styles that make use of the
above options.




\subsection{Anchoring a Matrix}

Since matrices are nodes, they can be anchored in the usual fashion
using the |anchor| option. However, there are two ways to influence
this placement further. First, the following option is often useful:

\begin{key}{/tikz/matrix anchor=\meta{anchor}}
  This option has the same effect as |anchor|, but the option applies
  only to the matrix itself, not to the cells inside. If you just say
  |anchor=north| as an option to the matrix node, all nodes inside
  matrix will also have this anchor, unless it is explicitly set
  differently for each node. By comparison, |matrix anchor| sets the
  anchor for the matrix, but for the nodes inside the value of
  |anchor| remain unchanged.

\begin{codeexample}[]
\begin{tikzpicture}
  \matrix [matrix anchor=west] at (0,0)
  {
    \node {123}; \\ % still center anchor
    \node {12}; \\
    \node {1}; \\
  };
  \matrix [anchor=west] at (0,-2)
  {
    \node {123}; \\ % inherited west anchor
    \node {12}; \\
    \node {1}; \\
  };
\end{tikzpicture}
\end{codeexample}
\end{key}

The second way to anchor a matrix is to use \emph{an anchor of a node
  inside the matrix}. For this, the |anchor| option has a special
effect when given as an argument to a matrix:

\begin{key}{/tikz/anchor=\meta{anchor or node.anchor}}
  Normally, the argument of this option refers to anchor of the matrix
  node, which is the node than includes all of the stuff of the
  matrix. However, you can also provide an argument of the form
  \meta{node}|.|\meta{anchor} where \meta{node} must be node defined
  inside the matrix and \meta{anchor} is an anchor of this node. In
  this case, the whole matrix is shifted around in such a way that
  this particular anchor of this particular node lies at the |at|
  position of the matrix. The same is true for |matrix anchor|.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \matrix[matrix anchor=inner node.south,anchor=base,row sep=3mm] at (1,1)
  {
    \node {a}; & \node             {b}; & \node {c}; & \node {d}; \\
    \node {a}; & \node(inner node) {b}; & \node {c}; & \node {d}; \\
    \node {a}; & \node             {b}; & \node {c}; & \node {d}; \\
  };
  \draw (inner node.south) circle (1pt);
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsection{Considerations Concerning Active Characters}

Even though \tikzname\ seems to use |&| to separate cells, \pgfname\ actually
uses a different command to separate cells, namely the command
|\pgfmatrixnextcell| and using a normal |&| character will normally
fail. What happens is that, \tikzname\ makes |&| an active character
and then defines this character to be equal to
|\pgfmatrixnextcell|. In most situations this will work 
nicely, but sometimes |&| cannot be made active; for
instance because the matrix is used in an argument of some macro or
the matrix contains nodes that contain normal |{tabular}|
environments. In this case you can use the following option to avoid
having to type |\pgfmatrixnextcell| each time:

\begin{key}{/tikz/ampersand replacement=\meta{macro name or empty}}
  If a macro name is provided, this macro will be defined to be equal
  to |\pgfmatrixnextcell| inside matrices and |&| will not be made
  active. For instance, you could say |ampersand replacement=\&| and
  then use \& to separate columns as in the following example:
\begin{codeexample}[]
\tikz
  \matrix [ampersand replacement=\&]
  {
    \draw (0,0)   circle (4mm); \& \node[rotate=10] {Hello};        \\
    \draw (0.2,0) circle (2mm); \& \fill[red]   (0,0) circle (3mm); \\
  };
\end{codeexample}
\end{key}


\subsection{Examples}

The following examples are adapted from code by Mark Wibrow. The first
two redraw pictures from Timothy van Zandt's PSTricks documentation: 

{\catcode`\|=12
\begin{codeexample}[]
\begin{tikzpicture} 
  \matrix [matrix of math nodes,row sep=1cm]
  { 
    |(U)| U &[2mm]                       &[8mm]    \\ 
            &      |(XZY)| X \times_Z Y  &      |(X)| X \\ 
            &      |(Y)|   Y             &      |(Z)| Z \\
  }; 
  \begin{scope}[every node/.style={midway,auto,font=\scriptsize}] 
    \draw [double, dashed] (U)   -- node {$x$} (X); 
    \draw                  (X)   -- node {$p$} (X -| XZY.east)
                           (X)   -- node {$f$} (Z)
                                 -- node {$g$} (Y)
                                 -- node {$q$} (XZY)
                                 -- node {$y$} (U);
   \end{scope}
\end{tikzpicture} 
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[>=stealth,->,shorten >=2pt,looseness=.5,auto] 
  \matrix [matrix of math nodes,
           column sep={2cm,between origins},
           row sep={3cm,between origins},
           nodes={circle, draw, minimum size=7.5mm}]
  { 
            & |(A)| A &         \\ 
    |(B)| B & |(E)| E & |(C)| C \\ 
            & |(D)| D           \\
  }; 
  \begin{scope}[every node/.style={font=\small\itshape}]
    \draw (A) to [bend left] (B) node [midway]   {g}; 
    \draw (B) to [bend left] (A) node [midway]   {f}; 
    \draw (D) --             (B) node [midway]   {c}; 
    \draw (E) --             (B) node [midway]   {b}; 
    \draw (E) --             (C) node [near end] {a}; 
    \draw [-,line width=8pt,draw=graphicbackground] 
          (D) to [bend right, looseness=1] (A); 
    \draw (D) to [bend right, looseness=1] (A)
            node [near start] {b} node [near end]   {e}; 
  \end{scope}
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture} 
  \matrix (network)
    [matrix of nodes,%
     nodes in empty cells,
     nodes={outer sep=0pt,circle,minimum size=4pt,draw},
     column sep={1cm,between origins},
     row sep={1cm,between origins}]
  {
                  &                &                 & \\ 
                  &                &                 & \\ 
    |[draw=none]| & |[xshift=1mm]| & |[xshift=-1mm]|   \\
  }; 
  \foreach \a in {1,...,4}{ 
    \draw (network-3-2) -- (network-2-\a); 
    \draw (network-3-3) -- (network-2-\a); 
    \draw [-stealth] ([yshift=5mm]network-1-\a.north) -- (network-1-\a); 
    \foreach \b in {1,...,4} 
      \draw (network-1-\a) -- (network-2-\b); 
  } 
  \draw [stealth-] ([yshift=-5mm]network-3-2.south) -- (network-3-2); 
  \draw [stealth-] ([yshift=-5mm]network-3-3.south) -- (network-3-3); 
\end{tikzpicture} 
\end{codeexample}

The following example is adapted from code written by Kjell Magne
Fauske, which is based on the following paper: K.~Bossley, M.~Brown, 
and C.~Harris, Neurofuzzy identification of an autonomous underwater
vehicle, \emph{International Journal of Systems Science}, 1999, 30, 901--913.

\begin{codeexample}[]
\begin{tikzpicture}
  [auto, 
   decision/.style={diamond, draw=blue, thick, fill=blue!20, 
                    text width=4.5em, text badly centered,
                    inner sep=1pt}, 
   block/.style   ={rectangle, draw=blue, thick, fill=blue!20, 
                    text width=5em, text centered, rounded corners,
                    minimum height=4em},
   line/.style    ={draw, thick, -latex',shorten >=2pt},
   cloud/.style   ={draw=red, thick, ellipse,fill=red!20,
                    minimum height=2em}]
  
  \matrix [column sep=5mm,row sep=7mm]
  {
    % row 1
      \node [cloud] (expert)   {expert}; & 
      \node [block] (init)     {initialize model}; & 
      \node [cloud] (system)   {system}; \\
    % row 2
      & \node [block] (identify) {identify candidate model}; & \\ 
    % row 3
      \node [block] (update)   {update model};  & 
      \node [block] (evaluate) {evaluate candidate models}; & \\ 
    % row 4
      & \node [decision] (decide) {is best candidate}; & \\ 
    % row 5
      & \node [block] (stop)      {stop}; & \\
  }; 
  \begin{scope}[every path/.style=line]
    \path          (init)     -- (identify); 
    \path          (identify) -- (evaluate); 
    \path          (evaluate) -- (decide); 
    \path          (update)   |- (identify); 
    \path          (decide)   -| node [near start] {yes} (update); 
    \path          (decide)   -- node [midway] {no} (stop); 
    \path [dashed] (expert)   -- (init); 
    \path [dashed] (system)   -- (init); 
    \path [dashed] (system)   |- (evaluate); 
  \end{scope}
\end{tikzpicture} 
\end{codeexample}
}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-tikz-paths.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Syntax for Path Specifications}

A \emph{path} is a series of straight and curved line segments. It is
specified following a |\path| command and the specification must
follow a special syntax, which is described in the subsections of the
present section.


\begin{command}{\path\meta{specification}|;|}
  This command is available only inside a |{tikzpicture}| environment.

  The \meta{specification} is a long stream of \emph{path
  operations}. Most of these path operations tell \tikzname\ how the path
  is build. For example, when you write |--(0,0)|, you use a
  \emph{line-to operation} and it means ``continue the path from
  wherever you are to the origin.''

  At any point where \tikzname\ expects a path operation, you can also
  give some graphic options, which is a list of options in brackets,
  such as |[rounded corners]|. These options can have different
  effects:
  \begin{enumerate}
  \item
    Some options take ``immediate'' effect and apply to all subsequent
    path operations on the path. For example, the |rounded corners|
    option will round all following corners, but not the corners
    ``before'' and if the |sharp corners| is given later on the path
    (in a new set of brackets), the rounding effect will end.

\begin{codeexample}[]
\tikz \draw (0,0) -- (1,1)
           [rounded corners] -- (2,0) -- (3,1)
           [sharp corners] -- (3,0) -- (2,1);
\end{codeexample}
    Another example are the transformation options, which also apply
    only to subsequent coordinates.
  \item
    The options that have immediate effect can be ``scoped'' by
    putting part of a path in curly braces. For example, the above
    example could also be written as follows:

\begin{codeexample}[]
\tikz \draw (0,0) -- (1,1)
           {[rounded corners] -- (2,0) -- (3,1)}
           -- (3,0) -- (2,1);
\end{codeexample}
  \item
    Some options only apply to the path as a whole. For example, the
    |color=| option for determining the color used for, say, drawing
    the path always applies to all parts of the path. If several
    different colors are given for different parts of the path, only
    the last one (on the outermost scope) ``wins'':
 
\begin{codeexample}[]
\tikz \draw (0,0) -- (1,1)
           [color=red] -- (2,0) -- (3,1)
           [color=blue] -- (3,0) -- (2,1);
\end{codeexample}

    Most options are of this type. In the above example, we would have
    had to ``split up'' the path into several |\path| commands:
\begin{codeexample}[]
\tikz{\draw (0,0) -- (1,1);
      \draw [color=red] (2,0) -- (3,1);
      \draw [color=blue] (3,0) -- (2,1);}
\end{codeexample}
  \end{enumerate}

  By default, the |\path| command does ``nothing'' with the
  path, it just ``throws it away.'' Thus, if you write
  |\path(0,0)--(1,1);|, nothing is drawn 
  in your picture. The only effect is that the area occupied by the
  picture is (possibly) enlarged so that the path fits inside the
  area. To actually ``do'' something with the path, an option like
  |draw| or |fill| must be given somewhere on the path. Commands like
  |\draw| do this implicitly.
  
  Finally, it is also possible to give \emph{node specifications} on a
  path. Such specifications can come at different locations, but they
  are always allowed when a normal path operation could follow. A node
  specification starts with |node|. Basically, the effect is to
  typeset the node's text as normal \TeX\ text and to place
  it at the ``current location'' on the path. The details are explained
  in Section~\ref{section-nodes}.

  Note, however, that the nodes are \emph{not} part of the path in any
  way. Rather, after everything has been done with the path what is
  specified by the path options (like filling and drawing the path due
  to a |fill| and a |draw| option somewhere in the
  \meta{specification}), the nodes are added in a post-processing
  step.   
  
  The following style influences scopes:
  \begin{stylekey}{/tikz/every path (initially \normalfont empty)}
    This style is installed at the beginning of every path. This can
    be useful for (temporarily) adding, say, the |draw| option to
    everything in a scope.
\begin{codeexample}[]
\begin{tikzpicture}
  [fill=examplefill,          % only sets the color
   every path/.style={draw}]  % all paths are drawn
  \fill  (0,0) rectangle +(1,1);
  \shade (2,0) rectangle +(1,1);
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}

\end{command}




\subsection{The Move-To Operation}

The perhaps simplest operation is the move-to operation, which is
specified by just giving a coordinate where a path operation is
expected.

\begin{pathoperation}[noindex]{}{\meta{coordinate}}
  \index{empty@\protect\meta{empty} path operation}%
  \index{Path operations!empty@\protect\texttt{\meta{empty}}}%
  The move-to operation normally starts a path at a certain
  point. This does not cause a line segment to be created, but it  
  specifies the starting point of the next segment. If a path is
  already under construction, that is, if several segments have
  already been created, a move-to operation will start a new part of the
  path that is not connected to any of the previous segments.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) --(2,0) (0,1) --(2,1);
\end{tikzpicture}
\end{codeexample}

  In the specification |(0,0) --(2,0) (0,1) --(2,1)| two move-to
  operations are specified: |(0,0)| and |(0,1)|. The other two
  operations, namely |--(2,0)| and |--(2,1)| are line-to operations,
  described next.
\end{pathoperation}


\subsection{The Line-To Operation}


\subsubsection{Straight Lines}

\begin{pathoperation}{--}{\meta{coordinate}}
  The line-to operation extends the current path from the current
  point in a straight line to the given coordinate. The ``current
  point'' is the endpoint of the previous drawing operation or the point
  specified by a prior move-to operation.

  You use two minus signs followed by a coordinate in round
  brackets. You can add spaces before and after the~|--|.

  When a line-to operation is used and some path segment has just been
  constructed, for example by another line-to operation, the two line
  segments become joined. This means that if they are drawn, the point
  where they meet is ``joined'' smoothly. To appreciate the difference,
  consider the following two examples: In the left example, the path
  consists of two path segments that are not joined, but that happen to
  share a point, while in the right example a smooth join is shown.

\begin{codeexample}[]
\begin{tikzpicture}[line width=10pt]
  \draw (0,0) --(1,1)  (1,1) --(2,0);
  \draw (3,0) -- (4,1) -- (5,0);
  \useasboundingbox (0,1.5); % make bounding box higher
\end{tikzpicture}
\end{codeexample}

\end{pathoperation}


\subsubsection{Horizontal and Vertical Lines}

Sometimes you want to connect two points via straight lines that are
only horizontal and vertical. For this, you can use two path
construction operations.

{\catcode`\|=12
\begin{pathoperation}[noindex]{-|}{\meta{coordinate}}
  \index{--1@\protect\texttt{-\protect\pgfmanualbar} path operation}%
  \index{Path operations!--1@\protect\texttt{-\protect\pgfmanualbar}}%
  This operation means ``first horizontal, then vertical.''

  \begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) node(a) [draw] {A}  (1,1) node(b) [draw] {B};
  \draw (a.north) |- (b.west);
  \draw[color=red] (a.east) -| (2,1.5) -| (b.north);
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}
\begin{pathoperation}[noindex]{|-}{\meta{coordinate}}
  \index{--2@\protect\texttt{\protect\pgfmanualbar-} path operation}%
  \index{Path operations!--2@\protect\texttt{\protect\pgfmanualbar-}}%
  This operations means  ``first vertical, then horizontal.''
\end{pathoperation}
}


\subsection{The Curve-To Operation}

The curve-to operation allows you to extend a path using a Bézier
curve.

\begin{pathoperation}{..}{\declare{|controls|}\meta{c}\opt{|and|\meta{d}}\declare{|..|\meta{y}}}
  This operation extends the current path from the current
  point, let us call it $x$, via a curve to a the current point~$y$.
  The curve is a cubic Bézier curve. For such a curve, 
  apart from $y$, you also specify two control points $c$ and $d$. The
  idea is that the curve starts at $x$, ``heading'' in the direction
  of~$c$. Mathematically spoken, the tangent of the curve at $x$ goes
  through $c$. Similarly, the curve ends at $y$, ``coming from'' the
  other control point,~$d$. The larger the distance between $x$ and~$c$
  and between $d$ and~$y$, the larger the curve will be.

  If the ``|and|\meta{d}'' part is not given, $d$ is assumed to be
  equal to $c$.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[line width=10pt] (0,0) .. controls (1,1) .. (4,0)
                               .. controls (5,0) and (5,1) .. (4,1);
  \draw[color=gray] (0,0) -- (1,1) -- (4,0) -- (5,0) -- (5,1) -- (4,1);
\end{tikzpicture}
\end{codeexample}

  As with the line-to operation, it makes a difference whether two curves
  are joined because they resulted from consecutive curve-to or line-to
  operations, or whether they just happen to have the same ending:

\begin{codeexample}[]
\begin{tikzpicture}[line width=10pt]
  \draw (0,0) -- (1,1) (1,1) .. controls (1,0) and (2,0) .. (2,0);
  \draw (3,0) -- (4,1) .. controls (4,0) and (5,0) .. (5,0);
  \useasboundingbox (0,1.5); % make bounding box higher
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}


\subsection{The Cycle Operation}

\begin{pathoperation}{--cycle}{}
  This operation adds a straight line from the current
  point to the last point specified by a move-to operation. Note that
  this need not be the beginning of the path. Furthermore, a smooth join
  is created between the first segment created after the last move-to
  operation and the straight line appended by the cycle operation.

  Consider the following example. In the left example, two triangles are
  created using three straight lines, but they are not joined at the
  ends. In the second example cycle operations are used.

\begin{codeexample}[]
\begin{tikzpicture}[line width=10pt]
  \draw (0,0) -- (1,1) -- (1,0) -- (0,0) (2,0) -- (3,1) -- (3,0) -- (2,0);
  \draw (5,0) -- (6,1) -- (6,0) -- cycle (7,0) -- (8,1) -- (8,0) -- cycle;
  \useasboundingbox (0,1.5); % make bounding box higher
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}



\subsection{The Rectangle Operation}

A rectangle can obviously be created using four straight lines and a
cycle operation. However, since rectangles are needed so often, a
special syntax is available for them.

\begin{pathoperation}{rectangle}{\meta{corner}}
  When this operation is used, one corner will be the current point,
  another corner is given by \meta{corner}, which becomes the new
  current point.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) rectangle (1,1);
  \draw (.5,1) rectangle (2,0.5) (3,0) rectangle (3.5,1.5) -- (2,0);
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}


\subsection{Rounding Corners}

All of the path construction operations mentioned up to now are
influenced by the following option:
\begin{key}{/tikz/rounded corners=\meta{inset} (default 4pt)}
  When this option is in force, all corners (places where a line is
  continued either via line-to or a curve-to operation) are replaced by
  little arcs so that the corner becomes smooth. 

\begin{codeexample}[]
\tikz \draw [rounded corners] (0,0) -- (1,1)
           -- (2,0) .. controls (3,1) .. (4,0);
\end{codeexample}

  The \meta{inset} describes how big the corner is. Note that the
  \meta{inset} is \emph{not} scaled along if you use a scaling option
  like |scale=2|. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[color=gray,very thin] (10pt,15pt) circle (10pt);
  \draw[rounded corners=10pt] (0,0) -- (0pt,25pt) -- (40pt,25pt);
\end{tikzpicture}
\end{codeexample}

  You can switch the rounded corners on and off ``in the middle of
  path'' and different corners in the same path can have different
  corner radii:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) [rounded corners=10pt] -- (1,1) -- (2,1)
                     [sharp corners] -- (2,0)
               [rounded corners=5pt] -- cycle;
\end{tikzpicture}
\end{codeexample}

Here is a rectangle with rounded corners:
\begin{codeexample}[]
\tikz \draw[rounded corners=1ex] (0,0) rectangle (20pt,2ex);
\end{codeexample}

  You should be aware, that there are several pitfalls when using this
  option. First, the rounded corner will only be an arc (part of a
  circle) if the angle is $90^\circ$. In other cases, the rounded
  corner will still be round, but ``not as nice.''

  Second, if there are very short line segments in a path, the
  ``rounding'' may cause inadverted effects. In such case it may be
  necessary to temporarily switch off the rounding using
  |sharp corners|. 
\end{key}

\begin{key}{/tikz/sharp corners}
  This options switches off any rounding on subsequent corners of the
  path.   
\end{key}



\subsection{The Circle and Ellipse Operations}

A circle can be approximated well using four Bézier curves. However,
it is difficult to do so correctly. For this reason, a special syntax
is available for adding such an approximation of a circle to the
current path.

\begin{pathoperation}{circle}{|(|\meta{radius}|)|}
  The center of the circle is given by the current point. The new
  current point of the path will remain to be the center of the
  circle.  
\end{pathoperation}

\begin{pathoperation}{ellipse}{|(|\meta{half width}| and |\meta{half height}|)|}
  Note that you can add spaces after |ellipse|, but you have to place
  spaces around |and|.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (1,0) circle (.5cm);
  \draw (3,0) ellipse (1cm and .5cm) -- ++(3,0) circle (.5cm)
    -- ++(2,-.5) circle (.25cm);
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}


\subsection{The Arc Operation}

The \emph{arc operation} allows you to add an arc to the current
path.
\begin{pathoperation}{arc}{|(|\meta{start angle}|:|\meta{end
    angle}|:|\meta{radius}\opt{| and |\meta{half height}}|)|}
  The arc operation adds a part of a circle of the given radius
  between the given angles. The arc will start at the current point
  and will end at the end of the arc.

  \begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) arc (180:90:1cm) -- (2,.5) arc (90:0:1cm);
  \draw (4,0) -- +(30:1cm) arc (30:60:1cm) -- cycle;
  \draw (8,0) arc (0:270:1cm and .5cm) -- cycle;
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (-1,0) -- +(3.5,0);
  \draw (1,0) ++(210:2cm) -- +(30:4cm);
  \draw (1,0) +(0:1cm) arc (0:30:1cm);      
  \draw (1,0) +(180:1cm) arc (180:210:1cm);
  \path (1,0) ++(15:.75cm) node{$\alpha$};
  \path (1,0) ++(15:-.75cm) node{$\beta$};
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}


\subsection{The Grid Operation}

You can add a grid to the current path using the |grid| path
operation. 

\begin{pathoperation}{grid}{\opt{\oarg{options}}\meta{corner}}
  This operations adds a grid filling a rectangle whose two corners
  are given by \meta{corner} and by the previous coordinate. Thus, the
  typical way in which a grid is drawn is |\draw (1,1) grid (3,3);|,
  which yields a grid filling the rectangle whose corners are at
  $(1,1)$ and $(3,3)$. All coordinate transformations apply to the
  grid.

\begin{codeexample}[]
\tikz[rotate=30] \draw[step=1mm] (0,0) grid (2,2);
\end{codeexample}

  The \meta{options}, which are local to the |grid| operation, can be
  used to influence the appearance of the grid. The stepping of the
  grid is governed by the following options: 

\begin{key}{/tikz/step=\meta{number or dimension or coordinate}
    (initially 1cm)}
  Sets the stepping in both the
  $x$ and $y$-direction. If a dimension is provided, this is used
  directly. If a number is provided, this number is interpreted in the
  $xy$-coordinate system. For example, if you provide the number |2|,
  then the $x$-step is twice the $x$-vector and the $y$-step is twice
  the $y$-vector set by the |x=| and |y=| options. Finally, if you
  provide a coordinate, then the $x$-part of this coordinate will be
  used as the $x$-step and the $y$-part will be used as the
  $y$-coordinate.

\begin{codeexample}[]
\begin{tikzpicture}[x=.5cm]
  \draw[thick] (0,0) grid [step=1]     (3,2);
  \draw[red]   (0,0) grid [step=.75cm] (3,2);
\end{tikzpicture}
\begin{tikzpicture}
  \draw        (0,0) circle (1);
  \draw[blue]  (0,0) grid [step=(45:1)] (3,2);
\end{tikzpicture}
\end{codeexample}  

  A complication arises when the $x$- and/or $y$-vector do not point
  along the axes. Because of this, the actual rule for computing the
  $x$-step and the $y$-step is the following: As the $x$- and
  $y$-steps we use the $x$- and $y$-components or the following two
  vectors: The first vector is either $(\meta{x-grid-step-number},0)$
  or $(\meta{x-grid-step-dimension},0\mathrm{pt})$, the second vector
  is  $(0,\meta{y-grid-step-number})$ or
  $(0\mathrm{pt},\meta{x-grid-step-dimension})$. 
\end{key}  

\begin{key}{/tikz/xstep=\meta{dimension or number} (initially 1cm)}
  Sets the stepping in the $x$-direction. 
\begin{codeexample}[]
\tikz \draw (0,0) grid [xstep=.5,ystep=.75] (3,2);
\end{codeexample}
\end{key}

\begin{key}{/tikz/ystep=\meta{dimension or number} (initially 1cm)}
  Sets the stepping in the $y$-direction. 
\end{key}

  It is important to note that the grid is always ``phased'' such that
  it contains the point $(0,0)$ if that point happens to be inside the
  rectangle. Thus, the grid does \emph{not} always have an intersection
  at the corner points; this occurs only if the corner points are
  multiples of the stepping. Note that due to rounding errors, the
  ``last'' lines of a grid may be omitted. In this case, you have to
  add an epsilon to the corner points.

  The following style is useful for drawing grids:
\begin{stylekey}{/tikz/help lines (initially {line width=0.2pt,gray})}
  This style makes lines ``subdued'' by using thin gray lines for
  them. However, this style is not installed automatically and you
  have to say for example:
\begin{codeexample}[]
\tikz \draw[help lines] (0,0) grid (3,3);
\end{codeexample}
\end{stylekey}

\end{pathoperation}



\subsection{The Parabola Operation}

The |parabola| path operation continues the current path with a
parabola. A parabola is a (shifted and scaled) curve defined by the
equation $f(x) = x^2$ and looks like this: \tikz \draw (-1ex,1.5ex)
parabola[parabola height=-1.5ex] +(2ex,0ex);.

\begin{pathoperation}{parabola}{\opt{\oarg{options}|bend|\meta{bend
        coordinate}}\meta{coordinate}}
  This operation adds a parabola through the current point and the
  given \meta{coordinate}. If the |bend| is given, it specifies where
  the bend should go; the \meta{options} can also be used to specify
  where the bend is. By default, the bend is at the old current point. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw               (0,0) rectangle                (1,1.5)
                      (0,0) parabola                 (1,1.5);
  \draw[xshift=1.5cm] (0,0) rectangle                (1,1.5)
                      (0,0) parabola[bend at end]    (1,1.5);
  \draw[xshift=3cm]   (0,0) rectangle                (1,1.5)
                      (0,0) parabola bend (.75,1.75) (1,1.5);
\end{tikzpicture}
\end{codeexample}

  The following options influence parabolas:
\begin{key}{/tikz/bend=\meta{coordinate}}
  Has the same effect as saying |bend|\meta{coordinate} outside the
  \meta{options}. The option specifies that the bend of the parabola
  should be at the given \meta{coordinate}. You have to take care
  yourself that the bend position is a ``valid'' position; which means
  that if there is no parabola of the form $f(x) = a x^2 + b x + c$
  that goes through the old current point, the given bend, and the new
  current point, the result will not be a parabola.

  There is one special property of the \meta{coordinate}: When a
  relative coordinate is given like |+(0,0)|, the position relative
  to which this coordinate is ``flexible.'' More precisely, this
  position lies somewhere on a line from the old current point to the
  new current point. The exact position depends on the next
  option.
\end{key}

\begin{key}{/tikz/bend pos=\meta{fraction}}
  Specifies where the ``previous'' point is relative to which the bend
  is calculated. The previous point will be at the \meta{fraction}th
  part of the line from the old current point to the new current
  point.

  The idea is the following: If you say |bend pos=0| and
  |bend +(0,0)|, the bend will be at the old current point. If you say
  |bend pos=1| and |bend +(0,0)|, the bend will be at the new current
  point. If you say |bend pos=0.5| and |bend +(0,2cm)| the bend will
  be 2cm above the middle of the line between the start and end
  point. This is most useful in situations such as the following:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw (-1,0) parabola[bend pos=0.5] bend +(0,2) +(3,0);
\end{tikzpicture}
\end{codeexample}

  In the above example, the |bend +(0,2)| essentially means ``a
  parabola that is 2cm high'' and |+(3,0)| means ``and 3cm wide.''
  Since this situation arises often, there is a special shortcut
  option:
  \begin{key}{/tikz/parabola height=\meta{dimension}}
    This option has the same effect as
    |[bend pos=0.5,bend={+(0pt,|\meta{dimension}|)}]|. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw (-1,0) parabola[parabola height=2cm] +(3,0);
\end{tikzpicture}
\end{codeexample}
  \end{key}
\end{key}

The following styles are useful shortcuts:
\begin{stylekey}{/tikz/bend at start}
  This places the bend at the start of a
  parabola. It is a shortcut for the following options:
  |bend pos=0,bend={+(0,0)}|.
\end{stylekey}

\begin{stylekey}{/tikz/bend at end}
  This places the bend at the end of a parabola.
\end{stylekey}

\end{pathoperation}


\subsection{The Sine and Cosine Operation}

The |sin| and |cos| operations are similar to the |parabola|
operation. They, too, can be used to draw (parts of) a sine or cosine
curve.

\begin{pathoperation}{sin}{\meta{coordinate}}
  The effect of |sin| is to draw a scaled and shifted version of a sine
  curve in the interval $[0,\pi/2]$. The scaling and shifting is done in
  such a way that the start of the sine curve in the interval is at the
  old current point and that the end of the curve in the interval is at
  \meta{coordinate}. Here is an example that should clarify this:

\begin{codeexample}[]
\tikz \draw (0,0) rectangle (1,1)     (0,0) sin (1,1)
            (2,0) rectangle +(1.57,1) (2,0) sin +(1.57,1);
\end{codeexample}
\end{pathoperation}

\begin{pathoperation}{cos}{\meta{coordinate}}
  This operation works similarly, only a cosine in the interval
  $[0,\pi/2]$ is drawn. By correctly alternating |sin| and |cos|
  operations, you can create a complete sine or cosine curve:

\begin{codeexample}[]
\begin{tikzpicture}[xscale=1.57]
  \draw (0,0) sin (1,1) cos (2,0) sin (3,-1) cos (4,0) sin (5,1);
  \draw[color=red] (0,1.5) cos (1,0) sin (2,-1.5) cos (3,0) sin (4,1.5) cos (5,0);
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}

Note that there is no way to (conveniently) draw an interval on a sine
or cosine curve whose end points are not multiples of $\pi/2$.



\subsection{The Plot Operation}

The |plot| operation can be used to append a line or curve to the path
that goes through a large number of coordinates. These coordinates are
either given in a simple list of coordinates, read from some file, or
they are computed on the fly.

Since the syntax and the behaviour of this command are a bit complex,
they are described in the separated Section~\ref{section-tikz-plots}.

\subsection{The To Path Operation}

The |to| operation is used to add a user-defined path
from the previous coordinate to the following coordinate. When you
write |(a) to (b)|, a straight line is added from |a|
to |b|, exactly as if you had written |(a) -- (b)|. However, if you
write |(a) to [out=135,in=45] (b)| a curve is added to the path,
which leaves at an angle of 135$^\circ$ at |a| and arrives at an angle
of 45$^\circ$ at |b|. This is because the options |in| and |out|
trigger a special path to be used instead of the straight line. 

\begin{pathoperation}{to}{\opt{|[|\meta{options}|]|}
    \opt{\meta{nodes}} |(|\meta{coordinate}|)|}

  This path operation inserts the path current set via the |to path|
  option at the current position. The \meta{options} can be used to
  modify (perhaps implicitly) the |to path| and to setup how the path
  will be rendered. 

  Before the |to path| is inserted, a number of macros are setup that
  can ``help'' the |to path|. These are |\tikztostart|,
  |\tikztotarget|, and |\tikztonodes|; they are explained in the
  following. 
  
  \medskip
  \textbf{Start and Target Coordinates.}\ \ 
  The |to| operation is always followed by a \meta{coordinate}, called
  the target coordinate. The macro |\tikztotarget| is set to this
  coordinate (without the parentheses). There is also a \emph{start
    coordinate}, which is the coordinate preceding the |to|
  operation. This coordinate can be accessed via the macro
  |\tikztostart|. In the following example, for the first |to|, the
  macro |\tikztostart| is |0pt,0pt| and the |\tikztotarget| is
  |0,2|. For the second |to|, the macro |\tikztostart| is |10pt,10pt|
  and |\tikztotarget| is |a|.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  
  \draw      (0,0)       to (0,2);
  \node      (a)         at (2,2) {a};
  \draw[red] (10pt,10pt) to (a);
\end{tikzpicture}
\end{codeexample}


  \medskip
  \textbf{Nodes on tos.}\ \
  It is possible to add nodes to the paths constructed by a |to|
  operation. To do so, you specify the nodes between the |to|
  keyword and the coordinate (if there are options to the |to|
  operation, these come first). The effect of |(a) to node {x} (b)| 
  (typically) is the same as if you had written
  |(a) -- node {x} (b)|, namely that the node is placed on the
  to. This can be used to add labels to tos: 
  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) to node [sloped,above] {x} (3,2);

  \draw (0,0) to[out=90,in=180] node [sloped,above] {x} (3,2);
\end{tikzpicture}
\end{codeexample}

  \medskip
  \textbf{Styles for nodes.}\ \
  In addition to the \meta{options} given after the |to| operation,
  the following style is also set at the beginning of the to path:
  \begin{stylekey}{/tikz/every to (initially \normalfont empty)}
    This style is installed at the beginning of every to. By
    default, it is set to |draw|. 
\begin{codeexample}[]
\tikz[every to/.style={draw,dashed}]
  \path (0,0) to (3,2);
\end{codeexample}
  \end{stylekey}

  \medskip
  \textbf{Options.}\ \ 
  The \meta{options} given with the |to| allow you to influence the
  appearance of the |to path|. Mostly, these options are used to
  change the |to path|. This can be used to change the path from a 
  straight line to, say, a curve.

  The path used is set using the following option:
  \begin{key}{/tikz/to path=\meta{path}}
    Whenever an |to| operation is used, the \meta{path} is
    inserted. More precisely, the following path is added:

    \begin{quote}
      |[every to,|\meta{options}|] |\meta{path}
    \end{quote}
  
    The \meta{options} are the options given to the |to| operation,
    the \meta{path} is the path set by this option |to path|.

    Inside the \meta{path}, different macros are used to reference the
    from- and to-coordinates. In detail, these are:
    \begin{itemize}
    \item \declare{|\tikztostart|} will expand to the from-coordinate
      (without the parentheses).
    \item \declare{|\tikztotarget|} will expand to the to-coordinate.
    \item \declare{|\tikztonodes|} will expand to the nodes between
      the |to| operation and the coordinate. Furthermore, these
      nodes will have the |pos| option set implicitly.      
    \end{itemize}

    Let us have a look at a simple example. The standard straight line
    for an to is achieved by the following \meta{path}:
    \begin{quote}
      |-- (\tikztotarget) \tikztonodes|
    \end{quote}

    Indeed, this is the default setting for the path. When we write
    |(a) to (b)|, the \meta{path} will expand to |(a) -- (b)|, when
    we write
    \begin{quote}
      |(a) to[red] node {x} (b)|
    \end{quote}
    the \meta{path} will expand to
    \begin{quote}
      |(a) -- (b) node[pos] {x}|
    \end{quote}

    It is not possible to specify the path
    \begin{quote}
      |-- \tikztonodes (\tikztotarget)|
    \end{quote}
    since \tikzname\ does not allow one to have a macro after |--|
    that expands to a node.

    Now let us have a look at how we can modify the \meta{path}
    sensibly. The simplest way is to use a curve.
    
\begin{codeexample}[]
\begin{tikzpicture}[to path={
    .. controls +(1,0) and +(1,0) .. (\tikztotarget) \tikztonodes}]

  \node (a) at (0,0) {a};
  \node (b) at (2,1) {b};
  \node (c) at (1,2) {c};
                  
  \draw (a) to node {x} (b)
        (a) to          (c);
\end{tikzpicture}
\end{codeexample}

    Here is another example:

\begin{codeexample}[]
\tikzset{
  my loop/.style={->,to path={
    .. controls +(80:1) and +(100:1) .. (\tikztotarget) \tikztonodes}},
  my state/.style={circle,draw}}
                           
\begin{tikzpicture}[shorten >=2pt]
  \node [my state] (a) at (210:1) {$q_a$};
  \node [my state] (b) at (330:1) {$q_b$};
                  
  \draw (a) to           node[below]       {1} (b)
            to [my loop] node[above right] {0} (b);
\end{tikzpicture}
\end{codeexample}

    \begin{key}{/tikz/execute at begin to=\meta{code}}
      The \meta{code} is executed prior to the to. This can be used to
      draw one or more additional paths or to do additional
      computations.
    \end{key}

    \begin{key}{/tikz/executed at end to=\meta{code}}
      Works like the previous option, only this code is executed after
      the to path has been added.
    \end{key}


    \begin{stylekey}{/tikz/every to (initially \normalfont empty)}
      This style is installed at the beginning of every to.
    \end{stylekey}
  \end{key}
\end{pathoperation}

There are a number of predefined |to path|s, see
Section~\ref{library-to-paths} for a reference.


\subsection{The Let Operation}

The \emph{let operation} is the first of a number of path operations
that do not actually extend that path, but have different, mostly
local, effects.

\begin{pathoperation}{let}{\meta{assignment}
    \opt{|,|\meta{assignment}}%
    \opt{|,|\meta{assignment}\dots}\declare{| in |}}
  When this path operation is encountered, the \meta{assignment}s are 
  evaluated, one by one. This will store coordinate and number in
  special \emph{registers} (which are local to \tikzname, they have
  nothing to do with \TeX\ registers). Subsequently, one can access the
  contents of these registers using the macros |\p|, |\x|, |\y|, and
  |\n|.

  The first kind of permissible \meta{assignment}s have the following
  form:
  \begin{quote}
    |\n|\meta{number register}|={|\meta{formula}|}|
  \end{quote}
  When an assignment has this form, the \meta{formula} is evaluated
  using the |\pgfmathparse| operation. The result stored in the
  \meta{number register}. If the \meta{formula} involves a dimension
  anywhere (as in |2*3cm/2|), then the \meta{number register} stores
  the resulting dimension with a trailing |pt|.  A \meta{number register} can
  be named arbitrarily and is a normal \TeX\  parameter to the |\n|
  macro. Possible names are |{left corner}|, but also just a single
  digit like~|5|.  

  Let us call the path that follows a let operation its
  \emph{body}. Inside the body, the |\n| macro can be used to access
  the register.
  \begin{command}{\n\marg{number register}}
    When this macro is used on the left-hand side of an |=|-sign in a
    let operation, it has no effect and is just there for
    readability. When the macro is used on the right-hand side of an
    |=|-sign or in the body of the let operation, then it expands to
    the value stored in the \meta{number register}. This will either
    be a dimensionless number like |2.0| or a dimension like |5.6pt|.

    For instance, if we say |let \n1={1pt+2pt}, \n2={1+2} in ...|, then
    inside the |...| part the macro |\n1| will expand to |3pt| and
    |\n2| expands to |3|.
  \end{command}

  The second kind of \meta{assignements} have the following form:
  \begin{quote}
    |\p|\meta{point register}|={|\meta{formula}|}|
  \end{quote}
  Point position registers store a single point, consisting
  of an $x$-part and a $y$-part measured in \TeX\ points (|pt|). In
  particular, point registers do not stored nodes or node names.
  Here is an example:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \draw let \p{foo} = (1,1), \p2 = (2,0) in
          (0,0) -- (\p2) -- (\p{foo});
\end{tikzpicture}
\end{codeexample}

  \begin{command}{\p\marg{point register}}
    When this macro is used on the left-hand side of an |=|-sign in a
    let operation, it has no effect and is just there for
    readability. When the macro is used on the right-hand side of an
    |=|-sign or in the body of the let operation, then it expands to
    the $x$-part (measured in \TeX\ points) of the coordinate stored
    in the \meta{register}, followed, by a comma, followed by the
    $y$-part. 

    For instance, if we say |let \p1=(1pt,1pt+2pt) in ...|, then
    inside the |...| part the macro |\p1| will expand to exactly the
    seven characters ``1pt,3pt''. This means that you when you write
    |(\p1)|, this expands to |(1pt,3pt)|, which is presumably exactly
    what you intended.
  \end{command}
  \begin{command}{\x\marg{point register}}
    This macro expand just to the $x$-part of the point
    register. If we say as above, as we did above,
    |let \p1=(1pt,1pt+2pt) in ...|, then
    inside the |...| part the macro |\x1| expands to |1pt|.
  \end{command}
  \begin{command}{\y\marg{point register}}
    Works like |\x|, only for the $y$-part.
  \end{command}
  Note that the above macros are available only inside a let
  operation. 

  Here is an example where let clauses are used to assemble a coordinate
  from the $x$-coordinate of a first point and the $y$-coordinate of a
  second point. Naturally, using the \verb!|-! notation, this could be
  written much more compactly.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \draw    (1,0) coordinate (first point)
        -- (3,2) coordinate (second point);

  \fill[red] let \p1 = (first point),
                 \p2 = (second point) in
               (\x1,\y2) circle (2pt);
\end{tikzpicture}
\end{codeexample}

  Note that the effect of a let operation is local to the body of the
  let operation. If you wish to access a computed coordinate outside
  the body, you must use a |coordinate| path operation:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,2);

  \path % let's define some points:
    let
      \p1        = (1,0),
      \p2        = (3,2),
      \p{center} = ($ (\p1) !.5! (\p2) $) % center
    in
      coordinate (p1) at (\p1)
      coordinate (p2) at (\p2)
      coordinate (center) at (\p{center});
      
  \draw (p1) -- (p2);
  \fill[red] (center) circle (2pt);
\end{tikzpicture}
\end{codeexample}

  For a more useful application of the let operation, let use draw a
  circle that touches a given line:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw [help lines] (0,0) grid (3,3);

  \coordinate (a) at (rnd,rnd);
  \coordinate (b) at (3-rnd,3-rnd);
  \draw (a) -- (b);

  \node (c) at (1,2) {x};

  \draw let \p1 = ($ (a)!(c)!(b) - (c) $),
            \n1 = {veclen(\x1,\y1)}
        in (c) circle (\n1);
\end{tikzpicture}
\end{codeexample}
\end{pathoperation}


\subsection{The Scoping Operation}

When \tikzname\ encounters and opening or a closing brace (|{| or~|}|) at
some point where a path operation should come, it will open or close a
scope. All options that can be applied ``locally'' will be scoped
inside the scope. For example, if you apply a transformation like
|[xshift=1cm]| inside the scoped area, the shifting only applies to
the scope. On the other hand, an option like |color=red| does not have
any effect inside a scope since it can only be applied to the path as
a whole.

Concerning the effect of scopes on relative coordinates,
please see Section~\ref{section-scopes-relative}.


\subsection{The Node and Edge Operations}

There are two more operations that can be found in paths:
|node| and |edge|. The first is used to add a so-called node to a
path. This operation is special in the following sense: It does not 
change the current path in any way. In other words, this operation 
is not really a path operation, but has an effect that is
``external''  to the path. The |edge| operation has similar effect in
that it adds something \emph{after} the main path has been
drawn. However, it works like the |to| operation, that is, it adds a
|to| path to the picture after the main path has been drawn.

Since these operations are quite complex, they are described in the
separate Section~\ref{section-nodes}.  



\subsection{The PGF-Extra Operation}

In some cases you may need to ``do some calculations or some other
stuff'' while a path is constructed. For this, you would like to
suspend the construction of the path and suspend \tikzname's parsing
of the path, you would then like to have some \TeX\ code executed, and
would then like to resume the parsing of the path. This effect can be
achieved using the following path operation |\pgfextra|. Note that
this operation should only be used by real experts and should only be
used deep inside clever macros, not on normal paths.

\begin{command}{\pgfextra\marg{code}}
  This command may only be used inside a \tikzname\ path. There it is
  used like a normal path operation. The construction of the path is
  temporarily suspended and the \meta{code} is executed. Then, the
  path construction is resumed.

\begin{codeexample}[]
\newdimen\mydim
\begin{tikzpicture}
  \mydim=1cm
  \draw (0pt,\mydim) \pgfextra{\mydim=2cm} -- (0pt,\mydim);
\end{tikzpicture}
\end{codeexample}
\end{command}

\begin{command}{\pgfextra \meta{code} \texttt{\char`\\endpgfextra}}
  This is an alternative syntax for the |\pgfextra| command. If the
  code following |\pgfextra| does not start with a brace, the
  \meta{code} is executed until |\endpgfextra| is encountered. What
  actually happens is that |\pgfextra| that is not followed by a brace
  completely shuts down the \tikzname\ parse and |\endpgfextra| is a
  normal macro that restarts the parser.

\begin{codeexample}[]
\newdimen\mydim
\begin{tikzpicture}
  \mydim=1cm
  \draw (0pt,\mydim)
    \pgfextra \mydim=2cm \endpgfextra -- (0pt,\mydim);
\end{tikzpicture}
\end{codeexample}
\end{command}


==> pgfmanual-en-tikz-plots.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Plots of Functions}

\label{section-tikz-plots}

\subsection{When Should One Use \tikzname\ for Generating Plots? }

\label{section-why-pgname-for-plots}

There exist many powerful programs that produce plots, examples are
\textsc{gnuplot} or \textsc{mathematica}. These programs can produce
two different kinds of output: First, they can output a complete plot
picture in a certain format (like \pdf) that includes all low-level
commands necessary for drawing the complete plot (including axes and
labels). Second, they can usually also produce ``just plain data'' in
the form of a long list of coordinates. Most of the powerful programs
consider it a to be ``a bit boring'' to just output tabled data and
very much prefer to produce fancy pictures. Nevertheless, when coaxed,
they can also provide the plain data.

\emph{Note that is often not necessary to use \tikzname\ for plots.}
Programs like \textsc{gnuplot} can produce very sophisticated plots
and it is usually much easier to simply include these plots as a
finished \textsc{pdf} or PostScript graphics.

However, there are a number of reasons why you may wish to invest time
and energy into mastering the \pgfname\ commands for creating plots:

\begin{itemize}
\item
  Virtually all plots produced by ``external programs'' use different
  fonts from the one used in your document.
\item
  Even worse, formulas will look totally different, if they can be
  rendered at all.
\item
  Line width will usually be too large or too small.
\item
  Scaling effects upon inclusion can create a mismatch between sizes
  in the plot and sizes in the text.
\item
  The automatic grid generated by most programs is mostly
  distracting. 
\item
  The automatic ticks generated by most programs are cryptic
  numerics. (Try adding a tick reading ``$\pi$'' at the right point.)
\item
  Most programs make it very easy to create ``chart junk'' in a most
  convenient fashion.  All show, no content.
\item
  Arrows and plot marks will almost never match the arrows used in the
  rest of the document.
\end{itemize}

The above list is not exhaustive, unfortunately.


\subsection{The Plot Path Operation}

The |plot| path operation can be used to append a line or curve to the path
that goes through a large number of coordinates. These coordinates are
either given in a simple list of coordinates, read from some file, or
they are computed on the fly.

The syntax of the |plot| comes in different versions.

\begin{pathoperation}{--plot}{\meta{further arguments}}
  This operation plots the curve through the coordinates specified in
  the \meta{further arguments}. The current (sub)path is simply
  continued, that is, a line-to operation to the first point of the
  curve is implicitly added. The details of the \meta{further
    arguments}  will be explained in a moment.
\end{pathoperation}

\begin{pathoperation}{plot}{\meta{further arguments}}
  This operation plots the curve through the coordinates specified in
  the \meta{further arguments} by first ``moving'' to the first
  coordinate of the curve.
\end{pathoperation}

The \meta{further arguments} are used in three different ways to
specifying the coordinates of the points to be plotted:

\begin{enumerate}
\item
  \opt{|--|}|plot|\oarg{local options}\declare{|coordinates{|\meta{coordinate
    1}\meta{coordinate 2}\dots\meta{coordinate $n$}|}|}
\item
  \opt{|--|}|plot|\oarg{local options}\declare{|file{|\meta{filename}|}|}
\item
  \opt{|--|}|plot|\oarg{local options}\declare{\meta{coordinate expression}}
\item
  \opt{|--|}|plot|\oarg{local options}\declare{|function{|\meta{gnuplot formula}|}|}
\end{enumerate}

These different ways are explained in the following.


\subsection{Plotting Points Given Inline}

In the first two cases, the points are given directly in the \TeX-file
as in the following example:

\begin{codeexample}[]
\tikz \draw plot coordinates {(0,0) (1,1) (2,0) (3,1) (2,1) (10:2cm)};
\end{codeexample}

Here is an example showing the difference between |plot| and |--plot|:

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) -- (1,1) plot coordinates {(2,0)  (4,0)};
  \draw[color=red,xshift=5cm]
        (0,0) -- (1,1) -- plot coordinates {(2,0)  (4,0)};
\end{tikzpicture}
\end{codeexample}


\subsection{Plotting Points Read From an External File}

The second way of specifying points is to put them in an external
file named \meta{filename}. Currently, the only file format that
\tikzname\ allows is the following: Each line of the \meta{filename}
should contain one line starting with two numbers, separated by a
space. Anything following the two numbers on the line is
ignored. Also, lines starting with a |%| or a |#| are ignored as well
as empty lines. (This is exactly the format that \textsc{gnuplot}
produces when you say |set terminal table|.) If necessary, more
formats will be supported in the future, but it is usually easy to
produce a file containing data in this form.

\begin{codeexample}[]
\tikz \draw plot[mark=x,smooth] file {plots/pgfmanual-sine.table};
\end{codeexample}

The file |plots/pgfmanual-sine.table| reads:
\begin{codeexample}[code only]
#Curve 0, 20 points
#x y type
0.00000 0.00000  i
0.52632 0.50235  i
1.05263 0.86873  i
1.57895 0.99997  i
...
9.47368 -0.04889  i
10.00000 -0.54402  i
\end{codeexample}
It was produced from the following source, using |gnuplot|:
\begin{codeexample}[code only]
set terminal table
set output "../plots/pgfmanual-sine.table"
set format "%.5f"
set samples 20
plot [x=0:10] sin(x)
\end{codeexample}

The \meta{local options} of the |plot| operation are local to each
plot and do not affect other plots ``on the same path.'' For example,
|plot[yshift=1cm]| will locally shift the plot 1cm upward. Remember,
however, that most options can only be applied to paths as a
whole. For example, |plot[red]| does not have the effect of making the
plot red. After all, you are trying to ``locally'' make part of the
path red, which is not possible.

\subsection{Plotting a Function}
\label{section-tikz-plot}

When you plot a function, the coordinates of the plot data can be
computed by evaluating a mathematical expression. Since \pgfname\
comes with a mathematical engine, you can specify this expression and
then have \tikzname\ produce the desired coordinates for you,
automatically.

Since this case is quite common when plotting a function, the syntax
is easy: Following the |plot| command and its local options, you
directly provide a \meta{coordinate expression}. It looks like a
normal coordinate, but inside you may use a special macro, which is
|\x| by default, but this can be changed using the |variable|
option. The \meta{coordinate expression} is then evaluated for
different values for |\x| and the resulting coordinates are plotted.

Note that you will often have to put the $x$- or $y$-coordinate inside
braces, namely whenever you use an expression involving a paranthesis.

The following options influence how the \meta{coordinate expression}
is evaluated:
\begin{key}{/tikz/variable=\meta{macro} (initially x)}
  Sets the macro whose value is set to the different values when
  \meta{coordinate expression} is evaluated.
\end{key}

\begin{key}{/tikz/samples=\meta{number} (initially 25)}
  Sets the number of samples used in the plot.
\end{key}

\begin{key}{/tikz/domain=\meta{start}|:|\meta{end} (initially -5:5)}
  Sets the domain between which the samples are taken.
\end{key}

\begin{key}{/tikz/samples at=\meta{sample list}}
  This option specifies a list of positions for which the
  variable should be evaluated. For instance, you can say
  |samples at={1,2,8,9,10}| to have the variable evaluated exactly for
  values $1$, $2$, $8$, $9$, and $10$. You can use the |\foreach|
  syntax, so you can use |...| inside the \meta{sample list}.

  When this option is used, the |samples| and |domain| option are
  overruled. The other ways round, setting either |samples| or
  |domain| will overrule this option.
\end{key}

\begin{codeexample}[]
\begin{tikzpicture}[domain=0:4]
  \draw[very thin,color=gray] (-0.1,-1.1) grid (3.9,3.9);
  
  \draw[->] (-0.2,0) -- (4.2,0) node[right] {$x$};
  \draw[->] (0,-1.2) -- (0,4.2) node[above] {$f(x)$};
  
  \draw[color=red]    plot (\x,\x)             node[right] {$f(x) =x$};
  \draw[color=blue]   plot (\x,{sin(\x r)})    node[right] {$f(x) = \sin x$};
  \draw[color=orange] plot (\x,{0.05*exp(\x)}) node[right] {$f(x) = \frac{1}{20} \mathrm e^x$};
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\tikz \draw[scale=0.5,domain=-3.141:3.141,smooth,variable=\t]
  plot ({\t*sin(\t r)},{\t*cos(\t r)});
\end{codeexample}

\begin{codeexample}[]
\tikz \draw[domain=0:360,smooth,variable=\t]
  plot ({sin(\t)},\t/360,{cos(\t)});
\end{codeexample}


\subsection{Plotting a Function Using Gnuplot}
\label{section-tikz-gnuplot}

Often, you will want to plot points that are given via a function like
$f(x) = x \sin x$. Unfortunately, \TeX\ does not really have enough
computational power to generate the points on such a function
efficiently (it is a text processing program, after all). However,
if you allow it, \TeX\ can try to call external programs that can
easily produce the necessary points. Currently, \tikzname\ knows how to
call \textsc{gnuplot}.

When \tikzname\ encounters your operation
|plot[id=|\meta{id}|] function{x*sin(x)}| for 
the first time, it will create a file called
\meta{prefix}\meta{id}|.gnuplot|, where \meta{prefix} is |\jobname.| by
default, that is, the name of you main |.tex| file. If no \meta{id} is
given, it will be empty, which is alright, but it is better when each
plot has a unique \meta{id} for reasons explained in a moment. Next,
\tikzname\ writes some initialization code into this file followed by
|plot x*sin(x)|. The initialization code sets up things 
such that the |plot| operation will write the coordinates into another
file called \meta{prefix}\meta{id}|.table|. Finally, this table file
is read as if you had said |plot file{|\meta{prefix}\meta{id}|.table}|. 

For the plotting mechanism to work, two conditions must be met:
\begin{enumerate}
\item
  You must have allowed \TeX\ to call external programs. This is often
  switched off by default since this is a security risk (you might,
  without knowing, run a \TeX\ file that calls all sorts of ``bad''
  commands). To enable this ``calling external programs'' a command
  line option must be given to the \TeX\ program. Usually, it is
  called something like |shell-escape| or |enable-write18|. For
  example, for my |pdflatex| the option |--shell-escape| can be
  given.
\item
  You must have installed the |gnuplot| program and \TeX\ must find it
  when compiling your file.
\end{enumerate}

Unfortunately, these conditions will not always be met. Especially if
you pass some source to a coauthor and the coauthor does not have
\textsc{gnuplot} installed, he or she will have trouble compiling your
files.

For this reason, \tikzname\ behaves differently when you compile your
graphic for the second time: If upon reaching
|plot[id=|\meta{id}|] function{...}| the file \meta{prefix}\meta{id}|.table|
already exists \emph{and} if the \meta{prefix}\meta{id}|.gnuplot| file
contains what \tikzname\ thinks that it ``should'' contain, the |.table|
file is immediately read without trying to call a |gnuplot|
program. This approach has the following advantages: 
\begin{enumerate}
\item
  If you pass a bundle of your |.tex| file and all |.gnuplot| and
  |.table| files to someone else, that person can \TeX\ the |.tex|
  file without having to have |gnuplot| installed.
\item
  If the |\write18| feature is switched off for security reasons (a
  good idea), then, upon the first compilation of the |.tex| file, the
  |.gnuplot| will still be generated, but not the |.table|
  file. You can then simply call |gnuplot| ``by hand'' for each
  |.gnuplot| file, which will produce all necessary |.table| files.
\item
  If you change the function that you wish to plot or its
  domain, \tikzname\ will automatically try to regenerate the |.table|
  file.
\item
  If, out of laziness, you do not provide an |id|, the same |.gnuplot|
  will be used for different plots, but this is not a problem since
  the |.table| will automatically be regenerated for each plot
  on-the-fly. \emph{Note: If you intend to share your files with
  someone else, always use an id, so that the file can by typeset
  without having \textsc{gnuplot} installed.} Also, having unique ids
  for each plot will improve compilation speed since no external
  programs need to be called, unless it is really necessary.
\end{enumerate}

When you use |plot function{|\meta{gnuplot formula}|}|, the \meta{gnuplot
  formula} must be given in the |gnuplot| syntax, whose details are
beyond the scope of this manual. Here is the ultra-condensed
essence: Use |x| as the variable and use the C-syntax for normal
plots, use |t| as the variable for parametric plots. Here are some examples:

\begin{codeexample}[]
\begin{tikzpicture}[domain=0:4]
  \draw[very thin,color=gray] (-0.1,-1.1) grid (3.9,3.9);
  
  \draw[->] (-0.2,0) -- (4.2,0) node[right] {$x$};
  \draw[->] (0,-1.2) -- (0,4.2) node[above] {$f(x)$};
  
  \draw[color=red]    plot[id=x]   function{x}           node[right] {$f(x) =x$};
  \draw[color=blue]   plot[id=sin] function{sin(x)}      node[right] {$f(x) = \sin x$};
  \draw[color=orange] plot[id=exp] function{0.05*exp(x)} node[right] {$f(x) = \frac{1}{20} \mathrm e^x$};
\end{tikzpicture}
\end{codeexample}


The plot in influenced by the following options: First, the options
|samples| and |domain| explained earlier. Second, there are some more
specialized options.

\begin{key}{/tikz/parametric=\meta{boolena} (default true)}
  Sets whether the plot is a parametric plot. If true, then |t| must
  be used instead of |x| as the parameter and two comma-separated
  functions must be given in the \meta{gnuplot formula}. An example is
  the following:
\begin{codeexample}[]
\tikz \draw[scale=0.5,domain=-3.141:3.141,smooth]
  plot[parametric,id=parametric-example] function{t*sin(t),t*cos(t)};
\end{codeexample}
\end{key}

\begin{key}{/tikz/id=\meta{id}}
  Sets the identifier of the current plot. This should be a unique
  identifier for each plot (though things will also work if it is not,
  but not as well, see the explanations above). The \meta{id} will be
  part of a filename, so it should not contain anything fancy like |*|
  or |$|.%$
\end{key}

\begin{key}{/tikz/prefix=\meta{prefix}}
  The \meta{prefix} is put before each plot file name. The default is
  |\jobname.|, but 
  if you have many plots, it might be better to use, say |plots/| and
  have all plots placed in a directory. You have to create the
  directory yourself.
\end{key}

\begin{key}{/tikz/raw gnuplot}
  This key causes the \meta{gnuplot formula} to be passed on to
  \textsc{gnuplot} without setting up the samples or the |plot|
  operation. Thus, you could write
\begin{codeexample}[code only]
plot[raw gnuplot,id=raw-example] function{set samples 25; plot sin(x)}
\end{codeexample}
  This can be 
  useful for complicated things that need to be passed to
  \textsc{gnuplot}. However, for really complicated situations you
  should create a special external generating \textsc{gnuplot} file
  and use the |file|-syntax to include the table ``by hand.''
\end{key}

The following styles influence the plot:
\begin{stylekey}{/tikz/every plot (initially \normalfont empyt)}
  This style is installed in each plot, that is, as if you always said
\begin{codeexample}[code only]
  plot[every plot,...]
\end{codeexample}
 This is most useful for globally setting a prefix for all plots by saying:
\begin{codeexample}[code only]
\tikzset{every plot/.style={prefix=plots/}}
\end{codeexample}
\end{stylekey}



\subsection{Placing Marks on the Plot}

As we saw already, it is possible to add \emph{marks} to a plot using
the |mark| option. When this option is used, a copy of the plot
mark is placed on each point of the plot. Note that the marks are
placed \emph{after} the whole path has been drawn/filled/shaded. In
this respect, they are handled like text nodes. 

In detail, the following options govern how marks are drawn:
\begin{key}{/tikz/mark=\meta{mark mnemonic}}
  Sets the mark to a mnemonic that has previously been defined using
  the |\pgfdeclareplotmark|. By default, |*|, |+|, and |x| are available,
  which draw a filled circle, a plus, and a cross as marks. Many more
  marks become available when the library |pgflibraryplotmarks| is
  loaded. Section~\ref{section-plot-marks} lists the available plot
  marks.

  One plot mark is special: the |ball| plot mark is available only
  it \tikzname. The |ball color| determines the balls's color. Do not use
  this option with a large number of marks since it will take very long
  to render in PostScript.
  
  \begin{tabular}{lc}
    Option & Effect \\\hline \vrule height14pt width0pt
    \plotmarkentrytikz{ball}
  \end{tabular}
\end{key}

\begin{key}{/tikz/mark repeat=\meta{r}}
  This option tells \tikzname\ that only every $r$th mark should be
  drawn.
  
\begin{codeexample}[]
\tikz \draw plot[mark=x,mark repeat=3,smooth] file {plots/pgfmanual-sine.table};
\end{codeexample}
\end{key}

\begin{key}{/tikz/mark phase=\meta{p}}
  This option tells \tikzname\ that the first mark to be draw should
  be the $p$th, followed by the $(p+r)$th, then the $(p+2r)$th, and so
  on.
  
\begin{codeexample}[]
\tikz \draw plot[mark=x,mark repeat=3,mark phase=6,smooth] file {plots/pgfmanual-sine.table};
\end{codeexample}
\end{key}

\begin{key}{/tikz/mark indices=\meta{list}}
  This option allows you to specify explicitly the indices at which a
  mark should be placed. Counting starts with 1. You can use the
  |\foreach| syntax, that is, |...| can be used.
    
\begin{codeexample}[]
\tikz \draw plot[mark=x,mark indices={1,4,...,10,11,12,...,16,20},smooth]
  file {plots/pgfmanual-sine.table};
\end{codeexample}
\end{key}

\begin{key}{/tikz/mark size=\meta{dimension}}
  Sets the size of the plot marks. For circular plot marks,
  \meta{dimension} is the radius, for other plot marks
  \meta{dimension} should be about half the width and height.

  This option is not really necessary, since you achieve the same
  effect by specifying |scale=|\meta{factor} as a local option, where
  \meta{factor} is the quotient of the desired size and the default
  size. However, using |mark size| is a bit faster and more natural. 
\end{key}

\begin{key}{/tikz/mark options=\meta{options}}
  These options are applied to marks when they are drawn. For example,
  you can scale (or otherwise transform) the plot mark or set its
  color. 
\begin{codeexample}[]
\tikz \fill[fill=blue!20]
  plot[mark=triangle*,mark options={color=blue,rotate=180}]
    file{plots/pgfmanual-sine.table} |- (0,0);
\end{codeexample}
\end{key}



\subsection{Smooth Plots, Sharp Plots, and Comb Plots}

There are different things the |plot| operation can do with the points
it reads from a file or from the inlined list of points. By default,
it will connect these points by straight lines. However, you can also
use options to change the behavior of |plot|.

\begin{key}{/tikz/sharp plot}
  This is the default and causes the points to be connected by
  straight lines. This option is included only so that you can
  ``switch back'' if you ``globally'' install, say, |smooth|.
\end{key}

\begin{key}{/tikz/smooth}
  This option causes the points on the path to be connected using a
  smooth curve:

\begin{codeexample}[]
\tikz\draw plot[smooth] file{plots/pgfmanual-sine.table};
\end{codeexample}

  Note that the smoothing algorithm is not very intelligent. You will
  get the best results if the bending angles are small, that is, less
  than about $30^\circ$ and, even more importantly, if the distances
  between points are about the same all over the plotting path.
\end{key}

\begin{key}{/tikz/tension=\meta{value}}
  This option influences how ``tight'' the smoothing is. A lower value
  will result in sharper corners, a higher value in more ``round''
  curves. A value of $1$ results in a circle if four points at
  quarter-positions on a circle are given. The default is $0.55$. The
  ``correct'' value depends on the details of plot.
  
\begin{codeexample}[]
\begin{tikzpicture}[smooth cycle]
  \draw                 plot[tension=0.2]
    coordinates{(0,0) (1,1) (2,0) (1,-1)};
  \draw[yshift=-2.25cm] plot[tension=0.5]
    coordinates{(0,0) (1,1) (2,0) (1,-1)};
  \draw[yshift=-4.5cm]  plot[tension=1]
    coordinates{(0,0) (1,1) (2,0) (1,-1)};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/smooth cycle}
  This option causes the points on the path to be connected using a
  closed smooth curve. 

\begin{codeexample}[]
\tikz[scale=0.5]
  \draw plot[smooth cycle] coordinates{(0,0) (1,0) (2,1) (1,2)}
        plot               coordinates{(0,0) (1,0) (2,1) (1,2)} -- cycle;
\end{codeexample}
\end{key}

\begin{key}{/tikz/ycomb}
  This option causes the |plot| operation to interpret the plotting
  points differently. Instead of connecting them, for each point of
  the plot a straight line is added to the path from the $x$-axis to the point,
  resulting in a sort of ``comb'' or ``bar diagram.''

\begin{codeexample}[]
\tikz\draw[ultra thick] plot[ycomb,thin,mark=*] file{plots/pgfmanual-sine.table};
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[ycomb]
  \draw[color=red,line width=6pt]
    plot coordinates{(0,1) (.5,1.2) (1,.6) (1.5,.7) (2,.9)};
  \draw[color=red!50,line width=4pt,xshift=3pt]
    plot coordinates{(0,1.2) (.5,1.3) (1,.5) (1.5,.2) (2,.5)};
\end{tikzpicture}
\end{codeexample}
\end{key}


\begin{key}{/tikz/xcomb}
  This option works like |ycomb| except that the bars are horizontal. 

\begin{codeexample}[]
\tikz \draw plot[xcomb,mark=x] coordinates{(1,0) (0.8,0.2) (0.6,0.4) (0.2,1)};
\end{codeexample}
\end{key}


\begin{key}{/tikz/polar comb}
  This option causes a line from the origin to the point to be added
  to the path for each plot point.

\begin{codeexample}[]
\tikz \draw plot[polar comb,
     mark=pentagon*,mark options={fill=white,draw=red},mark size=4pt]
   coordinates {(0:1cm) (30:1.5cm) (160:.5cm) (250:2cm) (-60:.8cm)};
\end{codeexample}
\end{key}


\begin{key}{/tikz/only marks}
  This option causes only marks to be shown; no path segments are
  added to the actual path. This can be useful for quickly adding some
  marks to a path.

\begin{codeexample}[]
\tikz \draw (0,0) sin (1,1) cos (2,0)
  plot[only marks,mark=x] coordinates{(0,0) (1,1) (2,0) (3,-1)};
\end{codeexample}
\end{key}



==> pgfmanual-en-tikz-scopes.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section[Hierarchical Structures: Package, Environments, Scopes, and Styles]
{Hierarchical Structures:\\
  Package, Environments, Scopes, and Styles}

The present section explains how your files should be structured when
you use \tikzname. On the top level, you need to include the |tikz|
package. In the main text, each graphic needs to be put in a
|{tikzpicture}| environment. Inside these environments, you can use
|{scope}| environments to create internal groups. Inside the scopes
you use |\path| commands to actually draw something. On all levels
(except for the package level), graphic options can be given that
apply to everything within the environment.



\subsection{Loading the Package and the Libraries}

\begin{package}{tikz}
  This package does not have any options.
  
  This will automatically load the \pgfname\ and the |pgffor| package.

  \pgfname\ needs to know what \TeX\ driver you are intending to use. In
  most cases \pgfname\ is clever enough to determine the correct driver
  for you; this is true in particular if you use \LaTeX. Currently, the only
  situation where \pgfname\ cannot know the driver ``by itself'' is when
  you use plain \TeX\ or Con\TeX t together with |dvipdfm|. In this case,
  you have to write |\def\pgfsysdriver{pgfsys-dvipdfm.def}|
  \emph{before} you input |tikz.tex|. 
\end{package}


\begin{command}{\usetikzlibrary\marg{list of libraries}}
  Once \tikzname\ has been loaded, you can use this command to load
  further libraries. The list of libraries should contain the names of
  libraries separated by commas. Instead of curly braces, you can also
  use square brackets, which is something Con\TeX t users will
  like. If you try to load a library a second time, nothing will
  happen. 

  \example |\usetikzlibrary{arrows}|

  The above command will load a whole bunch of extra arrow tip
  definitions.

  What this command does is to load the file
  |tikzlibrary|\meta{library}|.code.tex| for each \meta{library} in
  the \meta{list of libraries}. Thus, to write your own library file,
  all you need to do is to place a file of the appropriate name
  somewhere where \TeX\ can find it. \LaTeX, plain \TeX, and Con\TeX t
  users can then use your library.
\end{command}



\subsection{Creating a Picture}

\subsubsection{Creating a Picture Using an Environment}

The ``outermost'' scope of \tikzname\ is the |{tikzpicture}| 
environment. You may give drawing commands only inside this
environment, giving them outside (as is possible in many other
packages) will result in chaos.

In \tikzname, the way graphics are rendered is strongly influenced by
graphic options. For example, there is an option for setting the color used
for drawing, another for setting the color used for filling, and also
more obscure ones like the option  for setting the prefix used in the
filenames of temporary files written while plotting functions using an
external program. The graphic options are specified in \emph{key
  lists}, see Section~\ref{section-graphic-options} below for
details. All graphic options are local to the |{tikzpicture}| to which
they apply.  

\begin{environment}{{tikzpicture}\opt{\oarg{options}}}
  All \tikzname\ commands should be given inside this
  environment, except for the |\tikzset| command. Unlike other
  packages, it is not possible to use, say, |\pgfpathmoveto| outside
  this environment and doing so will result in chaos. For \tikzname,
  commands like |\path| are only defined inside this environment, so
  there is little chance that you will do something wrong here. 

  When this environment is encountered, the \meta{options} are
  parsed, see Section~\ref{section-graphic-options}. All options given
  here will apply to the whole picture.

  Next, the contents of the environment is processed and the graphic
  commands therein are put into a box. Non-graphic text is suppressed
  as well as possible, but non-\pgfname\ commands inside a
  |{tikzpicture}| environment should not produce any ``output'' since
  this may totally scramble the positioning system of the backend
  drivers. The suppressing of normal text, by the way, is done by
  temporarily switching the font to |\nullfont|. You can, however,
  ``escape back'' to normal \TeX\ typesetting. This happens, for
  example, when you specify a node.

  At the end of the environment, \pgfname\ tries to make a good guess
  at the size of a bounding box of the graphic and
  then resizes the picture box such that the box has this size. To ``make its
  guess,'' everytime \pgfname\ encounters a coordinate, it updates the
  bounding box's size such that it encompasses all these
  coordinates. This will usually give a good 
  approximation of the bounding box, but will not always be
  accurate. First, the line thickness of diagonal lines is not taken
  into account correctly. Second, controls points of a curve often lie far
  ``outside'' the curve and make the bounding box too large. In this
  case, you should use the |[use as bounding box]| option.

  The following key influences the baseline of the resulting
  picture:
  \begin{key}{/tikz/baseline=\meta{dimension or coordinate} (default 0pt)}
    Normally, the lower end of the picture is put on the baseline of
    the surrounding text. For example, when you give the code
    |\tikz\draw(0,0)circle(.5ex);|, \pgfname\ will find out that the
    lower end of the picture is at $-.5\mathrm{ex}$ and that the upper
    end is at $.5\mathrm{ex}$. Then, the lower end will be put on the
    baseline, resulting in the following: \tikz\draw(0,0)circle(.5ex);.

    Using this option, you can specify that the picture should be
    raised or lowered such that the height \meta{dimension} is on the
    baseline. For example, |\tikz[baseline=0pt]\draw(0,0)circle(.5ex);|
    yields \tikz[baseline=0pt]\draw(0,0)circle(.5ex); since, now, the
    baseline is on the height of the $x$-axis.

    This options is often useful for ``inlined'' graphics as in
\begin{codeexample}[]
$A \mathbin{\tikz[baseline] \draw[->>] (0pt,.5ex) -- (3ex,.5ex);} B$
\end{codeexample}

    Instead of a \meta{dimension} you can also provide a coordinate in
    parantheses. Then the effect is to put the baseline on the
    $y$-coordinate that the give \meta{coordinate} has \emph{at the
      end of the picture}. This means that, at the end of the picture,
    the \meta{coordinate} is evaluated and then the baseline is set
    to the $y$-coordinate of the resulting point. This makes it easy
    to reference the $y$-coordinate of, say, the base line of nodes.
\begin{codeexample}[]
Hello
\tikz[baseline=(X.base)]
  \node [cross out,draw] (X) {world.};
\end{codeexample}

\begin{codeexample}[]
Top align:
\tikz[baseline=(current bounding box.north)]
  \draw (0,0) rectangle (1cm,1ex);
\end{codeexample}
  \end{key}

  \begin{key}{/tikz/execute at begin picture=\meta{code}}
    This option causes \meta{code} to be executed
    at the beginning of the picture. This option must be
    given in the argument of the |{tikzpicture}| environment itself
    since this option will not have an effect otherwise. After all,
    the picture has already ``started'' later on. The effect of
    multiply setting this option accumulates.

    This option is mainly used in styles like the |every picture|
    style to execute certain code at the start  of a picture.
  \end{key}

  \begin{key}{/tikz/execute at end picture=\meta{code}}
    This option installs \meta{code} that will be executed
    at the end of the picture. Using this option multiple times will
    cause the code to accumulate. This option must also be given in
    the optional argument of the |{tikzpicture}| environment.

\begin{codeexample}[]
\begin{tikzpicture}[execute at end picture=%
  {
    \begin{pgfonlayer}{background}
      \path[fill=yellow,rounded corners]
        (current bounding box.south west) rectangle
        (current bounding box.north east);
    \end{pgfonlayer}
  }]
  \node at (0,0) {X};
  \node at (2,1) {Y};
\end{tikzpicture}
\end{codeexample}
  \end{key}

  All options ``end'' at the end of the picture. To set an option
  ``globally'' change the following style:
  \begin{stylekey}{/tikz/every picture (initially \normalfont empty)}
    This style is installed at the beginning of each picture.
\begin{codeexample}[code only]
\tikzset{every picture/.style=semithick}
\end{codeexample}
  \end{stylekey}

  Note that you should not use |\tikzset| to set options directly. For
  instance, if you want to use a line width of |1pt| by default, do
  not try to say |\tikzset{line width=1pt}| at the beginning of your
  document. This will not work since the line width is changed in many
  places. Instead, say
\begin{codeexample}[code only]
\tikzset{every picture/.style={line width=1pt}}
\end{codeexample}
  This will have the desired effect.
\end{environment}

In other \TeX\ format, you should use instead the following commands:

\begin{plainenvironment}{{tikzpicture}\opt{\oarg{options}}}
  This is the plain \TeX\ version of the environment.
\end{plainenvironment}

\begin{contextenvironment}{{tikzpicture}\opt{\oarg{options}}}
  This is the Con\TeX t version of the environment.
\end{contextenvironment}


\subsubsection{Creating a Picture Using a Command}

The following two commands are used for ``small'' graphics.

\begin{command}{\tikz\opt{\oarg{options}}\marg{commands}}
  This command places the \meta{commands} inside a
  |{tikzpicture}| environment and adds a semicolon at the end. This is
  just a convenience.

  The \meta{commands} may not contain a paragraph (an empty
  line). This is a precaution to ensure that users really use this
  command only for small graphics.

  \example |\tikz{\draw (0,0) rectangle (2ex,1ex)}| yields
  \tikz{\draw (0,0) rectangle (2ex,1ex);} 
\end{command}


\begin{command}{\tikz\opt{\oarg{options}}\meta{text}|;|}
  If the \meta{text} does not start with an opening brace, the end of
  the \meta{text} is the next semicolon that is encountered.

  \example |\tikz \draw (0,0) rectangle (2ex,1ex);| yields
  \tikz \draw (0,0) rectangle (2ex,1ex);
\end{command}



\subsubsection{Adding a Background}

By default, pictures do not have any background, that is, they are
``transparent'' on all parts on which you do not draw
anything. You may instead wish to have a colored background behind
your picture or a black frame around it or lines above and below it or
some other kind of decoration.

Since backgrounds are often not needed at all, the definition of
styles for adding backgrounds has been put in the library package
|backgrounds|. This package is documented in
Section~\ref{section-tikz-backgrounds}. 


\subsection{Using Scopes to Structure a Picture}

Inside a |{tikzpicture}| environment you can create scopes
using the |{scope}| environment. This environment is available only
inside the |{tikzpicture}| environment, so once more, there is little
chance of doing anything wrong.

\subsubsection{The Scope Environment}

\begin{environment}{{scope}\opt{\oarg{options}}}
  All \meta{options} are local to the \meta{environment
  contents}. Furthermore, the clipping path is also local to the
  environment, that is, any clipping done inside the environment
  ``ends'' at its end.

\begin{codeexample}[]
\begin{tikzpicture}[ultra thick]
  \begin{scope}[red]
    \draw (0mm,10mm) -- (10mm,10mm);
    \draw (0mm,8mm) -- (10mm,8mm);
  \end{scope}
  \draw (0mm,6mm) -- (10mm,6mm);
  \begin{scope}[green]
    \draw (0mm,4mm) -- (10mm,4mm);
    \draw (0mm,2mm) -- (10mm,2mm);
    \draw[blue] (0mm,0mm) -- (10mm,0mm);
  \end{scope}
\end{tikzpicture}
\end{codeexample}
  
  The following style influences scopes:
  \begin{stylekey}{/tikz/every scope (initially \normalfont empty)}
    This style is installed at the beginning of every scope.
  \end{stylekey}

  The following options are useful for scopes:
  \begin{key}{/tikz/execute at begin scope=\meta{code}}
    This option install some code that will be executed
    at the beginning of the scope. This option must be
    given in the argument of the |{scope}| environment.

    The effect applies only to the current scope, not to subscopes.
  \end{key}
  \begin{key}{/tikz/execute at end scope=\meta{code}}
    This option installs some code that will be executed
    at the end of the  current scope. Using this option multiple times
    will  cause the code to accumulate. This option must also be given
    in the optional argument of the |{scope}| environment. 

    Again, the effect applies only to the current scope, not to subscopes.
  \end{key}
\end{environment}

\begin{plainenvironment}{{scope}\opt{\oarg{options}}}
  Plain \TeX\ version of the environment.
\end{plainenvironment}

\begin{contextenvironment}{{scope}\opt{\oarg{options}}}
  Con\TeX t version of the environment.
\end{contextenvironment}


\subsubsection{Shorthand for Scope Environments}

There is a small library that makes using scopes a bit easier:
\begin{tikzlibrary}{scopes}
  This library defines a shorthand for starting and ending |{scope}|
  environments. 
\end{tikzlibrary}
When this library is loaded, the following happens: At certain places
inside a \tikzname\ picture, it is allowed to start a scope just using
a single brace, provided the single brace is followed by options in
square brackets:

\begin{codeexample}[]
\begin{tikzpicture}
  { [ultra thick]
    { [red]
      \draw (0mm,10mm) -- (10mm,10mm);
      \draw (0mm,8mm)  -- (10mm,8mm);
    }
    \draw (0mm,6mm) -- (10mm,6mm);
  }
  { [green]
    \draw (0mm,4mm) -- (10mm,4mm);
    \draw (0mm,2mm) -- (10mm,2mm);
    \draw[blue] (0mm,0mm) -- (10mm,0mm);
  }
\end{tikzpicture}
\end{codeexample}

In the above example, |{ [thick]| actually causes a 
  |\begin{scope}[thick]| to be inserted, and the corresponding closing
    |}| causes an |\end{scope}| to be inserted.

The ``certain places'' where an opening brace has this special meaning
are the following: First, right after the semicolon that ends a path. Second,
right after the end of a scope. Third, right at the beginning of a
scope, which includes the beginning of a picture. Also note that some
square bracket must follow, otherwise the brace is treated as a normal
\TeX\ scope.


\subsubsection{Using Scopes Inside Paths}

The |\path| command, which is described in much more detail in later
sections, also takes graphic options. These options are local to the
path. Furthermore, it is possible to create local scopes within a
path simply by using curly braces as in
\begin{codeexample}[]
\tikz \draw (0,0) -- (1,1)
           {[rounded corners] -- (2,0) -- (3,1)}
           -- (3,0) -- (2,1);
\end{codeexample}

Note that many options apply only to the path as a whole and cannot be
scoped in this way. For example, it is not possible to scope the
|color| of the path. See the explanations in the section on paths for
more details.

Finally, certain elements that you specify in the argument to the
|\path| command also take local options. For example, a node
specification takes options. In this case, the options apply only to
the node, not to the surrounding path.



\subsection{Using Graphic Options}
\label{section-graphic-options}

\subsubsection{How Graphic Options Are Processed}

Many commands and environments of \tikzname\ accept
\emph{options}. These options are so-called \emph{key lists}. To
process the options, the following command is used, which you can also
call yourself. Note that it is usually better not to call this command
directly, since this will ensure that the effect of options are local
to a well-defined scope.

\begin{command}{\tikzset\marg{options}}
  This command will process the \meta{options} using the |\pgfkeys|
  command, documented in detail in Section~\ref{section-keys}, with
  the default path set to |/tikz|. Under normal circumstances, the
  \meta{options} will be lists of comma-separated pairs of the form
  \meta{key}|=|\meta{value}, but more fancy things can happen when you
  use the power of the |pgfkeys| mechanism, see
  Section~\ref{section-keys} once more.

  When a pair \meta{key}|=|\meta{value} is processed, the following
  happens:
  \begin{enumerate}
  \item If the \meta{key} is a full key (starts with a slash) it is
    handled directly as described in Section~\ref{section-keys}.
  \item Otherwise (which is usually the case), it is checked whether
    |/tikz/|\meta{key} is a key and, if so, it is executed.
  \item Otherwise, it is checked whether |/pgf/|\meta{key} is a key
    and, if so, it is executed.
  \item Otherwise, it is checked whether \meta{key} is a color and, if
    so, |color=|\meta{key} is executed.
  \item Otherwise, it is checked whether \meta{key} contains a dash
    and, if so, |arrows=|\meta{key} is executed.
  \item Otherwise, it is checked whether \meta{key} is the name of a
    shape and, if so, |shape=|\meta{key} is executed.
  \item Otherwise, an error message is printed.
  \end{enumerate}

  Note that by the above description, all keys starting with |/tikz|
  and also all keys starting with |/pgf| can be used as \meta{key}s in
  an \meta{options} list.
\end{command}


\subsubsection{Using Styles to Manage How Pictures Look}

There is a way of organizing sets of graphic options ``orthogonally''
to the normal scoping mechanism. For example, you might wish all your
``help lines'' to be drawn in a certain way like, say, gray and thin
(do \emph{not} dash them, that distracts). For this, you can use
\emph{styles}.

A style is a key that, when used, causes a set of graphic options to
be processed. Once a style has been defined, it can be used like any
other key. For example, the predefined |help lines| style, which you
should use for lines in the background like grid lines or construction
lines.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw             (0,0) grid +(2,2);
  \draw[help lines] (2,0) grid +(2,2);
\end{tikzpicture}
\end{codeexample}

Defining styles is also done using options. Suppose we wish to define
a style called |my style| and when this style is used, we want the
draw color to be set to |red| and the fill color be set to
|red!20|. To achieve this, we use the following option:
\begin{codeexample}[code only]
my style/.style={draw=red,fill=red!20}
\end{codeexample}

The meaning of the curious |/.style| is the following: ``The key
|my style| should not be used here but, rather, be defined. So, setup
things such that using the key |my style| will, in the following, have
the same effect as if we had written |draw=red,fill=red!20| instead.''

Returning to the help lines example, suppose we prefer blue help
lines. This could be achieved as follows:
\begin{codeexample}[]
\begin{tikzpicture}[help lines/.style={blue!50,very thin}]
  \draw             (0,0) grid +(2,2);
  \draw[help lines] (2,0) grid +(2,2);
\end{tikzpicture}
\end{codeexample}

Naturally, one of the main ideas behind styles is that they can be
used in different pictures. In this case, we have to use the
|\tikzset| command somewhere at the beginning.
\begin{codeexample}[]
\tikzset{help lines/.style={blue!50,very thin}}
% ...  
\begin{tikzpicture}
  \draw             (0,0) grid +(2,2);
  \draw[help lines] (2,0) grid +(2,2);
\end{tikzpicture}
\end{codeexample}

Since styles are just special cases of |pgfkeys|'s general style
facility, you can actually do quite a bit more. Let us start with
adding options to an already existing style. This is done using
|/.append style| instead of |/.style|:
\begin{codeexample}[]
\begin{tikzpicture}[help lines/.append style=blue!50]
  \draw             (0,0) grid +(2,2);
  \draw[help lines] (2,0) grid +(2,2);
\end{tikzpicture}
\end{codeexample}
In the above example, the option |blue!50| is appended to the style
|help lines|, which now has the same effect as
|black!50,very thin,blue!50|. Note that two colors are set, so the
last one will ``win.'' There also exists a handler called
|/.prefix style| that adds something at the beginning of the style.

Just as normal keys, styles can be parametrized. This means that you
write \meta{style}|=|\meta{value} when you use the style instead of
just \meta{style}. In this case, all occurrences of |#1| in
\meta{style} are replaced by \meta{value}. Here is an example that
shows how this can be used.

\begin{codeexample}[]
\begin{tikzpicture}[outline/.style={draw=#1,thick,fill=#1!50}]
  \node [outline=red]  at (0,1) {red};
  \node [outline=blue] at (0,0) {blue};
\end{tikzpicture}
\end{codeexample}

For parametrized styles you can also set a \emph{default} value using
the |/.default| handler:

\begin{codeexample}[]
\begin{tikzpicture}[outline/.style={draw=#1,thick,fill=#1!50},
                    outline/.default=black]
  \node [outline]      at (0,1) {default};
  \node [outline=blue] at (0,0) {blue};
\end{tikzpicture}
\end{codeexample}

For more details on using and setting styles, see also
Section~\ref{section-keys}. 




==> pgfmanual-en-tikz-shapes.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Nodes and Edges}

\label{section-nodes}

\subsection{Overview}

In the present section, the usage of \emph{nodes} in
\tikzname\ is explained. A node is typically a rectangle or circle or
another simple shape with some text on it. 

Nodes are added to paths using the special path
operation |node|. Nodes \emph{are not part of the path
  itself}. Rather, they are added to the picture after the path has
been drawn. 

In Section~\ref{section-nodes-basic} the basic syntax of the node
operation is explained, followed in Section~\ref{section-nodes-multi}
by the syntax for multi-part nodes, which are nodes that contain
several different text parts. After this, the different options for
the text in nodes are explained. In
Section~\ref{section-nodes-anchors} the concept of \emph{anchors} is
introduced along with their usage. In
Section~\ref{section-nodes-transformations} the different ways
transformations affect nodes are
studied. Sections~\ref{section-nodes-placing-1}
and~\ref{section-nodes-placing-2} are about placing nodes on or next
to straight lines and curves. In
Section~\ref{section-nodes-connecting} it is explained how a node can
be used as a ``pseudo-coordinate.'' Section~\ref{section-nodes-edges}
introduces the |edge| operation, which
works similar to the |to| operation and also similar to the |node|
operation. Finally, Section~\ref{section-nodes-executing} explains the
special |after node path| options.


\subsection{Nodes and Their Shapes}

\label{section-nodes-basic}

In the simplest case, a node is just some text that is
placed at some coordinate. However, a node can also have a border
drawn around it or have a more complex background and
foreground. Indeed, some nodes do not have a text at all, but consist
solely of the background. You can name nodes so that you can reference
their coordinates later in the same picture or, if certain precautions
are taken as explained in Section~\ref{section-cross-picture-tikz},
also in different pictures.

There are no special \TeX\ commands for adding a node to a picture; rather,
there is path operation called |node| for this. Nodes are created
whenever \tikzname\ encounters |node| or |coordinate| at a point on a
path where it would expect a normal path operation (like |-- (1,1)| or
|sin (1,1)|). It is also possible to give node specifications
\emph{inside} certain path operations as explained later.

The node operation is typically followed by some options, which apply
only to the node. Then, you can optionally \emph{name} the node by
providing a name in round braces. Lastly, for the |node| operation you
must provide some label text for the node in curly braces, while for
the |coordinate| operation you may not. The node is placed at the
current position of the path \emph{after the path has been
  drawn}. Thus, all nodes are drawn ``on top'' of the path and
retained until the path is complete. If there are several nodes on a
path, they are drawn on top of the path in the order they are
encountered. 

\begin{codeexample}[]
\tikz \fill[fill=examplefill]
     (0,0) node {first node}
  -- (1,1) node {second node}
  -- (0,2) node {third node};
\end{codeexample}

The syntax for specifying nodes is the following:
\begin{pathoperation}{node}{\opt{|[|\meta{options}|]|}\opt{|(|\meta{name}|)|}%
    \opt{|at(|\meta{coordinate}|)|}\opt{\marg{text}}}
  The effect of |at| is to place the node at the coordinate given
  after |at| and not, as would normally be the case, at the last
  position. The |at| syntax is not available when a node is given
  inside a path operation (it would not make any sense, there).
  
  The |(|\meta{name}|)| is a name for later reference and it is
  optional. You may also add the option |name=|\meta{name} to the
  \meta{option} list; it has the same effect.

  \begin{key}{/tikz/name=\meta{node name}}
    Assigns a name to the node for later reference. Since this is a
    ``high-level'' name (drivers never know of it), you can use spaces,
    number, letters, or whatever you like when naming a node. Thus, you
    can name a node just |1| or perhaps |start of chart| or even
    |y_1|. Your node name should \emph{not} contain any punctuation like
    a dot, a comma, or a colon since these are used to detect what kind
    of coordinate you mean when you reference a node. 
  \end{key}

  \begin{key}{/tikz/alias=\meta{another node name}}
    This option allows you to provide another name for the
    node. Giving this option multiple times will allow you to access
    the node via several aliases. Using the |late options| options,
    you can also assign an alias name to a node at a later point.
  \end{key}

  \begin{key}{/tikz/at=\meta{coordinate}}
    This is another way of specifying ath |at| coordinate. Note that,
    typically, you will have to enclose the \meta{coordinate} in curly
    braces so that a comma inside the \meta{coordinate} does not
    confuse \TeX.
  \end{key}

  The \meta{options} is an optional list of options that \emph{apply
    only to the node} and have no effect outside. The other way round,
  most ``outside'' options also apply to the node, but not all. For
  example, the ``outside'' rotation does not apply to nodes (unless some
  special options are used, sigh). Also, the outside path action, like
  |draw| or |fill|, never applies to the node and must be given in the
  node (unless some special other options are used, deep sigh).

  As mentioned before, we can add a border and even a background to a
  node:  
\begin{codeexample}[]
\tikz \fill[fill=examplefill]
      (0,0) node {first node}
   -- (1,1) node[draw] {second node}
   -- (0,2) node[fill=red!20,draw,double,rounded corners] {third node};
\end{codeexample}

  The ``border'' is actually just a special case of a much more general
  mechanism. Each node has a certain \emph{shape} which, by default, is
  a rectangle. However, we can also ask \tikzname\ to use a circle shape
  instead or an ellipse shape (you have to include |pgflibraryshapes| for
  the latter shape): 

\begin{codeexample}[]
\tikz \fill[fill=examplefill]
      (0,0) node{first node}
   -- (1,1) node[ellipse,draw] {second node}
   -- (0,2) node[circle,fill=red!20] {third node};
\end{codeexample}

  In the future, there might be much more complicated shapes available
  such as, say, a shape for a resistor or a shape for a \textsc{uml}
  class. Unfortunately, creating new shapes is a bit tricky and makes
  it necessary to use the basic layer directly. Life is hard.

  To select the shape of a node, the following option is used:
  \begin{key}{/tikz/shape=\meta{shape name} (initially rectangle)}
    Select the shape either of the current node or, when this option is
    not given inside a node but somewhere outside, the shape of all
    nodes in the current scope.%
    \indexoption{\meta{shape name}}

    Since this option is used often, you can leave out the
    |shape=|. When \tikzname\ encounters an option like |circle|
    that it does not know, it will, after everything else has failed,
    check whether this option is the name of some shape. If so, that
    shape is selected as if you had said |shape=|\meta{shape name}.

    By default, the following shapes are available: |rectangle|,
    |circle|, |coordinate|, and, when the package |pgflibraryshapes| is
    loaded, also |ellipse|. Details of these shapes, like their anchors
    and size options, are discussed in Section~\ref{section-the-shapes}.
  \end{key}
  
  The following styles influences how nodes are rendered:
  \begin{stylekey}{/tikz/every node (initially \normalfont empty)}
    This style is installed at the beginning of every node. 
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={draw}]
  \draw (0,0) node {A} -- (1,1) node {B};
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
  \begin{stylekey}{/tikz/every \meta{shape} node (initially \normalfont empty)}
    These styles are installed at the beginning of a node of a given
    \meta{shape}. For example, |every rectangle node| is used for
    rectangle nodes, and so on.
\begin{codeexample}[]
\begin{tikzpicture}
  [every rectangle node/.style={draw}, 
   every circle node/.style={draw,double}]
  \draw (0,0) node[rectangle] {A} -- (1,1) node[circle] {B};
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
\end{pathoperation}

There is a special syntax for specifying ``light-weighed'' nodes:

\begin{pathoperation}{coordinate}{\opt{|[|\meta{options}|]|}|(|\meta{name}|)|\opt{|at(|\meta{coordinate}|)|}}
  This has the same effect as

  |node[shape=coordinate][|\meta{options}|](|\meta{name}|)at(|\meta{coordinate}|){}|,
  
  where the |at| part might be missing.
\end{pathoperation}

Since nodes are often the only path operation on paths, there are two
special commands for creating paths containing only a node:

\begin{command}{\node}
  Inside |{tikzpicture}| this is an abbreviation for |\path node|.
\end{command}

\begin{command}{\coordinate}
  Inside |{tikzpicture}| this is an abbreviation for |\path coordinate|.
\end{command}


\subsubsection{Predefined Shapes}

\label{section-nodes-predefined}

\label{section-the-shapes}

\pgfname\ and \tikzname\ define three shapes, by default:
\begin{itemize}
\item
  |rectangle|,
\item
  |circle|, and
\item
  |coordinate|.
\end{itemize}
By loading library packages, you can define more shapes like ellipses
or diamonds; see Section~\ref{section-libs-shapes} for the complete
list of shapes. 

\label{section-tikz-coordinate-shape}
The |coordinate| shape is handled in a special way by \tikzname. When
a node |x| whose shape is |coordinate| is used as a coordinate |(x)|,
this has the same effect as if you had said |(x.center)|. None  of the
special ``line shortening rules'' apply in this case. This can be
useful since, normally, the line shortening causes paths to be
segmented and they cannot be used for filling. Here is an example that
demonstrates the difference: 
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={draw}]
  \path[yshift=1.5cm,shape=rectangle]
    (0,0) node(a1){} (1,0) node(a2){}
    (1,1) node(a3){} (0,1) node(a4){};
  \filldraw[fill=examplefill] (a1) -- (a2) -- (a3) -- (a4);
  
  \path[shape=coordinate]
    (0,0) coordinate(b1) (1,0) coordinate(b2)
    (1,1) coordinate(b3) (0,1) coordinate(b4);
  \filldraw[fill=examplefill] (b1) -- (b2) -- (b3) -- (b4);
\end{tikzpicture}
\end{codeexample}



\subsubsection{Common Options: Separations, Margins, Padding and
  Border Rotation}

\label{section-shape-seps}
\label{section-shape-common-options}

The exact behaviour of shapes differs, shapes defined for more
special purposes (like a, say, transistor shape) will have even more
custom behaviors. However, there are some options that apply to most
shapes:

\begin{key}{/pgf/inner sep=\meta{dimension} (initially .3333em)}
  \keyalias{tikz}
  An additional (invisible) separation space of \meta{dimension} will
  be added inside the shape, between the text and the shape's
  background path. The effect is as if you had added appropriate
  horizontal and vertical skips at the beginning and end of the text
  to make it a bit ``larger.''

  For those familiar with \textsc{css}, this is the same as
  \emph{padding}. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0)     node[inner sep=0pt,draw] {tight}
        (0cm,2em) node[inner sep=5pt,draw] {loose}
        (0cm,4em) node[fill=examplefill]   {default};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/inner xsep=\meta{dimension} (initially .3333em)}
  \keyalias{tikz}
  Specifies the inner separation in the $x$-direction, only.
\end{key}

\begin{key}{/pgf/inner ysep=\meta{dimension} (initially .3333em)}
  \keyalias{tikz}
  Specifies the inner separation in the $y$-direction, only.
\end{key}  

\begin{key}{/pgf/outer sep=\meta{dimension} (initially .5\string\pgflinewidth)}
  \keyalias{tikz}
  This option adds an additional (invisible) separation space of
  \meta{dimension} outside the background path. The main effect of
  this option is that all anchors will move a little ``to the
  outside.''

  For those familiar with \textsc{css}, this is same as \emph{margin}.

  The default for this option is half the line width. When the default
  is used and when the background path is draw, the anchors will lie
  exactly on the ``outside border'' of the path (not on the path
  itself). When the shape is filled, but not drawn, this may not be
  desirable. In this case, the |outer sep| should be set to zero
  point. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[line width=5pt]
    (0,0) node[outer sep=0pt,fill=examplefill]     (f) {filled}
    (2,0) node[inner sep=.5\pgflinewidth+2pt,draw] (d) {drawn};

  \draw[->] (1,-1) -- (f);
  \draw[->] (1,-1) -- (d);  
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/outer xsep=\meta{dimension} (initially .5\string\pgflinewidth)}
  \keyalias{tikz}
  Specifies the outer separation in the $x$-direction, only.
\end{key}

\begin{key}{/pgf/outer ysep=\meta{dimension} (initially .5\string\pgflinewidth)}
  \keyalias{tikz}
  Specifies the outer separation in the $y$-direction, only.
\end{key}

\begin{key}{/pgf/minimum height=\meta{dimension} (initially 0pt)}
  \keyalias{tikz}
  This option ensures that the height of the shape (including the
  inner, but ignoring the outer separation) will be at least
  \meta{dimension}. Thus, if the text plus the inner separation is not
  at least as large as \meta{dimension}, the shape will be enlarged 
  appropriately. However, if the text is already larger than
  \meta{dimension}, the shape will not be shrunk.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) node[minimum height=1cm,draw] {1cm}
        (2,0) node[minimum height=0cm,draw] {0cm};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/minimum width=\meta{dimension} (initially 0pt)}
  \keyalias{tikz}
  Same as |minimum height|, only for the width.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0) node[minimum height=2cm,minimum width=3cm,draw] {$3 \times 2$};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/minimum size=\meta{dimension}}
  \keyalias{tikz}
  Sets both the minimum height and width at the same time.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0)  node[minimum size=2cm,draw] {square};
  \draw (0,-2) node[minimum size=2cm,draw,circle] {circle};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/pgf/shape aspect=\meta{aspect ratio}}
  \keyalias{tikz}
  Sets a desired aspect ratio for the shape. For the |diamond| shape,
  this option sets the ratio between width and height of the shape.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw (0,0)  node[shape aspect=1,diamond,draw] {aspect 1};
  \draw (0,-2) node[shape aspect=2,diamond,draw] {aspect 2};
\end{tikzpicture}
\end{codeexample}
\end{key}

\label{section-rotating-shape-borders}

Some shapes (but not all), support a special kind of rotation. This 
rotation affects only the border of a shape and is independent of the 
node contents, but \emph{in addition} to any other transformations.
	
\begin{codeexample}[]
\tikzstyle{every node}=[dart, shape border uses incircle, 
  inner sep=1pt, draw]
\begin{tikzpicture}
  \foreach \a/\b/\c in {A/0/0, B/45/0, C/0/45, D/45/45}
    \node [shape border rotate=\b, rotate=\c] at (\b/36,-\c/36) {\a};
\end{tikzpicture}
\end{codeexample}

There are two types of rotation: restricted and unrestricted. Which 
type of rotation is applied is determined by on how the shape border 
is constructed. If the shape border is contructed using an incircle, 
that is, a circle that tightly fits the node contents (including 
the |inner sep|), then the rotation can be unrestricted. If, however,
the border is constructed using the natural dimensions of the node
contents, the rotation is restricted to integer multiples of 90 
degrees.

Why should there be two kinds of rotation and border construction?
Borders constructed using the natural dimensions of the node contents
provide a much tighter fit to the node contents, but to maintain 
this tight fit, the border rotation must be restricted to integer 
multiples of 90 degrees. By using an incircle, unrestricted rotation
is possible, but the border will not make a very tight fit to the
node contents. 
	
\begin{codeexample}[]
\tikzstyle{every node}=[isosceles triangle, draw]
\begin{tikzpicture}
  \node {abc};
  \node [shape border uses incircle] at (2,0) {abc};
\end{tikzpicture}
\end{codeexample}

There are \pgfname{} keys determine how a shape border is 
contructed, and to specify its rotation.
It should be noted that not all shapes support these keys, so 
reference should be made to the documentation for individual 
shapes. 
	
\begin{key}{/pgf/shape border uses incircle=\opt{\meta{boolean}}
    (default true)}
  \keyalias{tikz}
  Determines if the border of a shape is constructed using the 
  incircle. If no value is given \meta{boolean} will take the default
  value |true|.
\end{key}


\begin{key}{/pgf/shape border rotate=\meta{angle} (initially 0)}
  \keyalias{tikz}
  Rotates the border of a shape independently of the node contents,
  but in addition to any other transformations. If the shape 
  border is not constructed using the incircle, the rotation will be
  rounded to the nearest integer multiple of 90 degrees when the
  shape is drawn. 
\end{key}

Note that if the border of the shape is rotated, 
the compass point anchors, and `text box' anchors (including 
|mid east|, |base west|, and so on), \emph{do not rotate}, but the 
other anchors do:
	
\begin{codeexample}[]
\tikzstyle{every node}=[shape=trapezium, draw, shape border uses incircle]
\begin{tikzpicture}
  \node at (0,0)  (A) {A};
  \node [shape border rotate=30] at (1.5,0) (B) {B};
  \foreach \s/\t in 
    {left side/base east, bottom side/north, bottom left corner/base}{
       \fill[red]  (A.\s) circle(1.5pt) (B.\s) circle(1.5pt);
       \fill[blue] (A.\t) circle(1.5pt) (B.\t) circle(1.5pt);
  }
\end{tikzpicture}
\end{codeexample}

Finally, a somewhat unfortunate side-effect of rotating shape borders 
is that the supporting shapes do not distinguish between 
|outer xsep| and |outer ysep|, and typically, the larger of the 
two values will be used. 




\subsection{Multi-Part Nodes}

\label{section-nodes-multi}

Most nodes just have a single simple text label. However, nodes of a
more complicated shapes might be made up from several \emph{node
  parts}. For example, in automata theory a so-called Moore state has
a state name, drawn in the upper part of the state circle, and an
output text, drawn in the lower part of the state circle. These two
parts are quite independent. Similarly, a \textsc{uml} class shape
would have a name part, a method part, and an attributes
part. Different molecule shape might use parts for the different atoms
to be drawn at the different positions, and so on.

Both \pgfname\ and \tikzname\ support such multipart nodes. On the
lower level, \pgfname\ provides a system for specifying that a shape
consists of several parts. On the \tikzname\ level, you specify the
different node parts by using the following command:

\begin{command}{\nodepart\marg{part name}}
  This command can only be used inside the \meta{text} argument of a
  |node| path operation. It works a little bit like a |\part| command
  in \LaTeX. It will stop the typesetting of whatever node part was
  typeset until now and then start putting all following text into the
  node part named \meta{part name}---until another |\partname| is
  encountered or until the node \meta{text} ends.

\begin{codeexample}[]
\begin{tikzpicture}
  \node [circle split,draw,double,fill=red!20]
  {
    % No \nodepart has been used, yet. So, the following is put in the
    % ``text'' node part by default.
    $q_1$ 
    \nodepart{lower} % Ok, end ``text'' part, start ``output'' part
    $00$
  }; % output part ended.
\end{tikzpicture}
\end{codeexample}

  You will have to lookup which parts are defined by a shape.

  The following styles influences node parts:
  \begin{stylekey}{/tikz/every \meta{part name} node part (initially
      \normalfont empty)}
    This style is installed at the beginning of every node part named
    \meta{part name}. 
\begin{codeexample}[]
\tikz [every lower node part/.style={red}]
  \node [circle split,draw] {$q_1$ \nodepart{lower} $00$};
\end{codeexample}
  \end{stylekey}
\end{command}



\subsection{Options for the Text in  Nodes}

\label{section-nodes-options}

The simplest option for the text in nodes is its color. Normally, this
color is just the last color installed using |color=|, possibly
inherited from another scope. However, it is possible to specificly
set the color used for text using the following option:

\begin{key}{/tikz/text=\meta{color}}
  Sets the color to be used for text labels. A |color=| option
  will immediately override this option.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[red]       (0,0) -- +(1,1) node[above]     {red};
  \draw[text=red]  (1,0) -- +(1,1) node[above]     {red};
  \draw            (2,0) -- +(1,1) node[above,red] {red};
\end{tikzpicture}
\end{codeexample}
\end{key}

Just like the color itself, you may also wish to set the opacity of
the text only. For this, use the option |text opacity| option, which
is detailed in Section~\ref{section-tikz-transparency}.

Next, you may wish to adjust the font used for the text. Use the
following option for this:
\begin{key}{/tikz/font=\meta{font commands}}
  Sets the font used for text labels. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[font=\itshape] (1,0) -- +(1,1) node[above] {italic};
\end{tikzpicture}
\end{codeexample}
  A perhaps more useful example is the following:

\begin{codeexample}[]
\tikz [every text node part/.style={font=\itshape}, 
       every lower node part/.style={font=\footnotesize}]
  \node [circle split,draw] {state \nodepart{lower} output};
\end{codeexample}
\end{key}


Normally, when a node is typeset, all the text you give in the braces
is but in one long line (in an |\hbox|, to be precise) and the node
will become as wide as necessary.

You can change this behaviour using the following options. They allow
you to limit the width of a node (naturally, at the expense of its
height).

\begin{key}{/tikz/text width=\meta{dimension}}
  This option will put the text of a node in a box of the given width
  (more precisely, in a |{minipage}| of this width; for plain \TeX\ a
  rudimentary ``minipage emulation'' is used).

  If the node text is not as wide as \meta{dimension}, it will
  nevertheless be put in a box of this width. If it is larger, line
  breaking will be done.

  By default, when this option is given, a ragged right border will be
  used. This is sensible since, typically, these boxes are narrow and
  justifying the text looks ugly.
\begin{codeexample}[]
\tikz \draw (0,0) node[fill=examplefill,text width=3cm]
  {This is a demonstration text for showing how line breaking works.};  
\end{codeexample}
\end{key}

\begin{key}{/tikz/text justified}
  Causes the text to be justified instead of (right)ragged. Use this
  only with pretty broad nodes.
{%
\hbadness=10000
\begin{codeexample}[]
\tikz \draw (0,0) node[fill=examplefill,text width=3cm,text justified]
  {This is a demonstration text for showing how line breaking works.};  
\end{codeexample}
}
  In the above example, \TeX\ complains (rightfully) about three very
  badly typeset lines. (For this manual I asked \TeX\ to stop
  complaining by using |\hbadness=10000|, but this is a foul deed,
  indeed.) 
\end{key}

\begin{key}{/tikz/text ragged}
  Causes the text to be typeset with a ragged right. This uses the
  original plain \TeX\ definition of a ragged right border, in which
  \TeX\ will try to balance the right border as well as possible. This
  is the default.
\begin{codeexample}[]
\tikz \draw (0,0) node[fill=examplefill,text width=3cm,text ragged]
  {This is a demonstration text for showing how line breaking works.};  
\end{codeexample}
\end{key}

\begin{key}{/tikz/text badly ragged}
  Causes the right border to be ragged in the \LaTeX-style, in which
  no balancing occurs. This looks ugly, but it may be useful for very
  narrow boxes and when you wish to avoid hyphenations.
\begin{codeexample}[]
\tikz \draw (0,0) node[fill=examplefill,text width=3cm,text badly ragged]
  {This is a demonstration text for showing how line breaking works.};  
\end{codeexample}
\end{key}

\begin{key}{/tikz/text centered}
  Centers the text, but tries to balance the lines.
\begin{codeexample}[]
\tikz \draw (0,0) node[fill=examplefill,text width=3cm,text centered]
  {This is a demonstration text for showing how line breaking works.};  
\end{codeexample}
\end{key}

\begin{key}{/tikz/text badly centered}
  Centers the text, without balancing the lines.
\begin{codeexample}[]
\tikz \draw (0,0) node[fill=examplefill,text width=3cm,text badly centered]
  {This is a demonstration text for showing how line breaking works.};  
\end{codeexample}
\end{key}

In addition to changing the width of nodes, you can also change the
height of nodes. This can be done in two ways: First, you can use the
option |minimum height|, which ensures that the height of the whole
node is at least the given height (this option is described in more
detail later). Second, you can use the option |text height|, which
sets the height of the text itself, more precisely, of the \TeX\ text
box of the text. Note that the |text height| typically is not the
height of the shape's box: In addition to the |text height|, an
internal |inner sep| is added as extra space and the text depth is
also taken into account.

I recommend using |minimum size| instead of |text height| except for
special situations.

\begin{key}{/tikz/text height=\meta{dimension}}
  Sets the height of the text boxes in shapes. Thus, when you write
  something like |node {text}|, the |text| is first typeset, resulting
  in some box of a certain height. This height is then replaced by the
  height |text height|. The resulting box is then used to determine
  the size of the shape, which will typically be larger. When you
  write |text height=| without specifying anything, the ``natural''
  size of the text box remains unchanged.
\begin{codeexample}[]
\tikz \node[draw]                  {y};    
\tikz \node[draw,text height=10pt] {y};       
\end{codeexample}
\end{key}

\begin{key}{/tikz/text depth=\meta{dimension}}
  This option works like |text height|, only for the depth of the text
  box. This option is mostly useful when you need to ensure a uniform
  depth of text boxes that need to be aligned. 
\end{key}




\subsection{Positioning Nodes}

\label{section-nodes-anchors}

When you place a node at some coordinate, the node is centered on this
coordinate by default. This is often undesirable and it would be
better to have the node to the right or above the actual coordinate.


\subsubsection{Positioning Nodes Using Anchors}

\pgfname\ uses a so-called anchoring mechanism to give you a very fine
control over the placement. The idea is simple: Imaging a node of
rectangular shape of a certain size. \pgfname\ defines numerous anchor
positions in the shape. For example to upper right corner is called,
well, not ``upper right anchor,'' but the |north east| anchor of the
shape. The center of the shape has an anchor called |center| on top of
it, and so on. Here are some examples (a complete list is given in
Section~\ref{section-the-shapes}).

\medskip\noindent
\begin{tikzpicture}
  \path node[minimum height=2cm,minimum width=5cm,fill=blue!25](x) {Big node};
  \fill (x.north)      circle (2pt) node[above] {|north|}
        (x.north east) circle (2pt) node[above] {|north east|}
        (x.north west) circle (2pt) node[above] {|north west|}
        (x.west) circle (2pt)       node[left]  {|west|}
        (x.east) circle (2pt)       node[right] {|east|}
        (x.base) circle (2pt)       node[below] {|base|};
\end{tikzpicture}

Now, when you place a node at a certain coordinate, you can ask \tikzname\
to place the node shifted around in such a way that a certain
anchor is at the coordinate. In the following example, we ask \tikzname\
to shift the first node such that its  |north east| anchor is at
coordinate |(0,0)| and that the |west| anchor of the second node is at
coordinate |(1,1)|.

\begin{codeexample}[]
\tikz \draw           (0,0) node[anchor=north east] {first node}
            rectangle (1,1) node[anchor=west] {second node};
\end{codeexample}

Since the default anchor is |center|, the default behaviour is to
shift the node in such a way that it is centered on the current
position.

\begin{key}{/tikz/anchor=\meta{anchor name}}
  Causes the node to be shifted such that it's anchor \meta{anchor
  name} lies on the current coordinate.

  The only anchor that is present in all shapes is |center|. However,
  most shapes will at least define anchors in all ``compass
  directions.'' Furthermore, the standard shapes also define a |base|
  anchor, as well as |base west| and |base east|, for placing things on
  the baseline of the text.
  
  The standard shapes also define a |mid| anchor (and |mid west| and
  |mid east|). This anchor is half the height of the character ``x''
  above the base line. This anchor is useful for vertically centering
  multiple nodes that have different heights and depth. Here is an
  example:
\begin{codeexample}[]
\begin{tikzpicture}[scale=3,transform shape]
  % First, center alignment -> wobbles
  \draw[anchor=center] (0,1)  node{x} -- (0.5,1)  node{y} -- (1,1)  node{t};
  % Second, base alignment -> no wobble, but too high
  \draw[anchor=base]   (0,.5) node{x} -- (0.5,.5) node{y} -- (1,.5) node{t};
  % Third, mid alignment
  \draw[anchor=mid]    (0,0)  node{x} -- (0.5,0)  node{y} -- (1,0)  node{t};
\end{tikzpicture}
\end{codeexample}
\end{key}



\subsubsection{Basic Placement Options}

Unfortunately, while perfectly logical, it is often rather
counter-intuitive that in order to place a node \emph{above} a given
point, you need to specify the |south| anchor. For this reason, there
are some useful options that allow you to select the standard anchors
more intuitively:

\begin{key}{/tikz/above=\meta{offset} (default 0pt)}
  Does the same as |anchor=south|. If the \meta{offset} is specified,
  the node is additionally shifted upwards by the given
  \meta{offset}. 
\begin{codeexample}[]
\tikz \fill (0,0) circle (2pt) node[above] {above};
\end{codeexample}
\begin{codeexample}[]
\tikz \fill (0,0) circle (2pt) node[above=2pt] {above};
\end{codeexample}
\end{key}

\begin{key}{/tikz/below=\meta{offset} (default 0pt)}
  Similar to |above|.
\end{key}

\begin{key}{/tikz/left=\meta{offset} (default 0pt)}
  Similar to |above|.
\end{key}

\begin{key}{/tikz/right=\meta{offset} (default 0pt)}
  Similar to |above|.
\end{key}

\begin{key}{/tikz/above left}
  Does the same as |anchor=south east|. Note that giving both |above|
  and |left| options does not have the same effect as |above left|,
  rather only the last |left| ``wins.'' Actually, this option also
  takes an \meta{offset} parameter, but using this parameter without
  using the |positioning| library is deprecated. (The |positioning|
  library changes the meaning of this parameter to something more
  sensible.) 
\begin{codeexample}[]
\tikz \fill (0,0) circle (2pt) node[above left] {above left};
\end{codeexample}
\end{key}

\begin{key}{/tikz/above right}
  Similar to  |above left|.
\begin{codeexample}[]
\tikz \fill (0,0) circle (2pt) node[above right] {above right};
\end{codeexample}
\end{key}

\begin{key}{/tikz/below left}
  Similar to |above left|.
\end{key}
\begin{key}{/tikz/below right}
  Similar to |above left|.
\end{key}

% A second set of options behaves similarly, namely the |above of|,
% |below of|, and so on options. They cause the same anchors to be set
% as the options without |of|, however, their parameter is different:
% You must provide the name of another node. The current node will then
% be placed, say, above this specified node at a distance given by the
% option |node distance|. 
% \begin{key}{/tikz/above of=\meta{node}}
%   This option causes the node to be placed at the distance
%   |node distance| above of \meta{node}. The anchor is |center|.
% \begin{codeexample}[]
% \begin{tikzpicture}[node distance=1cm]
%   \draw[help lines] (0,0) grid (3,2);
%   \node (a)                    {a};
%   \node (b) [above of=a]       {b};
%   \node (c) [above of=b]       {c};
%   \node (d) [right of=c]       {d};
%   \node (e) [below right of=d] {e};
% \end{tikzpicture}
% \end{codeexample}
% \end{key}

% \begin{key}{/tikz/above left of=\meta{node}}
%   Works like |above of|, only the node is now put above and left. The
%   |node distance| is the Euclidean distance between the two nodes, not
%   the $L_1$-distance.
% \end{key}

% \begin{key}{/tikz/above right of=\meta{node}}
%   Works similarly.
% \end{key}
% \begin{key}{/tikz/left of=\meta{node}}
%   Works similarly.
% \end{key}
% \begin{key}{/tikz/right of=\meta{node}}
%   Works similarly.
% \end{key}
% \begin{key}{/tikz/below of=\meta{node}}
%   Works similarly.
% \end{key}
% \begin{key}{/tikz/below left of=\meta{node}}
%   Works similarly.
% \end{key}
% \begin{key}{/tikz/below right of=\meta{node}}
%   Works similarly.
% \end{key}
% \begin{key}{/tikz/node distance=\meta{dimension}}
%   Sets the distance between nodes that are placed using the
%   |... of| options. Note that this distance is the distance between
%   the centers of the nodes, not the distance between their borders. 
% \end{key}



\subsubsection{Advanced Placement Options}

While the standard placement options suffice for simple cases, the
|positioning| library offers more convenient placement options.

\begin{tikzlibrary}{positioning}
  The library defines additional options for placing nodes
  conveniently. It also redefines the standard options like |above| so
  that they give you better control of node placement.
\end{tikzlibrary}

When this library is loaded, the options like |above| or |above left| behave
differently.

\begin{key}{/tikz/above=\opt{\meta{specification}} (default 0pt)}
  With the |positioning| library loaded, the |above| option does not
  take a simple \meta{dimension} as its paramter. Rather, it can
  (also) take a more elaborate \meta{specification} as parameter. This
  \meta{specification} has the following general form: It starts with
  an optional \meta{shifting part} and is followed by an optional
  \meta{of-part}. Let us start with the \meta{shifting part}, which
  can have three forms:
  \begin{enumerate}
  \item It can simply be a \declare{\meta{dimension}} (or a mathematical
    expression that evaluates to a dimension) like |2cm| or
    |3cm/2+4cm|. In this case, the following happens: the node's
    anchor is set to |south| and the node is vertically shifted
    upwards by \meta{dimension}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,2);
  \node at (1,1) [above=2pt+3pt,draw] {above};
\end{tikzpicture}
\end{codeexample}
    This use of the |above| option is the same as if the |positioning|
    library were not loaded.
  \item It can be a \declare{\meta{number}} (that is, any mathematical
    expression that does not include a unit like |pt| or
    |cm|). Examples are |2| or |3+sin(60)|. In this case, the anchor
    is also set to |south| and the node is vertically shifted by
    the vertical component of the coordinate |(0,|\meta{number}|)|.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,2);
  \node at (1,1) [above=.2,draw] {above};
  % south border of the node is now 2mm above (1,1)
\end{tikzpicture}
\end{codeexample}
  \item It can be of the form \declare{\meta{number or
        dimension 1}| and |\meta{number or dimension 2}}. This specification
    does not make particular sense for the |above| option, it is much
    more useful for options like |above left|. The reason it is
    allowed for the |above| option is that it is sometimes
    automatically used, as explained later.

    The effect of this option is the following. First, the point
    |(|\meta{number of dimension 2}|,|\meta{number or dimension 1}|)|
    is computed (note the inversed order), using the normal rules for
    evaluating such a coordinate, yielding some position. Then, the
    node is shifted by the vertical component of this point. The
    anchor is set to |south|.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (2,2);
  \node at (1,1) [above=.2 and 3mm,draw] {above};
  % south border of the node is also 2mm above (1,1)
\end{tikzpicture}
\end{codeexample}
  \end{enumerate}
  The \meta{shifting part} can optionally be followed by a
  \meta{of-part}, which has one of the following forms:
  \begin{enumerate}
  \item The \meta{of-part} can be declare{|of |\meta{coordinate}},
    where\meta{coordinate} is \emph{not} in parentheses and it is
    \emph{not} just a node name. An example would be
    |of somenode.north| or |of 2,3|. In this case, the
    following happens: First, the node's |at| parameter is set to the
    \meta{coordinate}. Second, the node is shifted according to the
    \meta{shift-part}. Third, the anchor is set to |south|. 

    Here is a basic example:
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style=draw]
  \draw[help lines] (0,0) grid (2,2);
  \node (somenode) at (1,1) {some node};
  
  \node [above=5mm of somenode.north east] {\tiny 5mm of somenode.north east};
  \node [above=1cm of somenode.north]      {\tiny 1cm of somenode.north};
\end{tikzpicture}
\end{codeexample}
    As can be seen the |above=5mm of somenode.north east| option does,
    indeed, place the node 5mm above the north east anchor of
    |somenode|. The same effect could have been achieved writing
    |above=5mm| followed by |at=(somenode.north east)|.

    If the \meta{shift-part} is missing, the shift is not zero, but
    rather the value of the |node distance| key is used, see below.
  \item The \meta{of-part} can have be |of |\meta{node name}. An
    example would be |of somenode|. In this case, the following
    usually happens: 
    \begin{itemize}
    \item The anchor is set to |south|.
    \item The node is shifted according to the \meta{shifting part}
      or, if it is missing, according to the value of |node distance|.
    \item The node's |at| parameter is set to \meta{node
        name}|.north|. 
    \end{itemize}
    The net effect of all this is that the new node will be placed in
    such a way that the distance between is south border and
    \meta{node name}'s north border is exactly the given distance.
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style=draw]
  \draw[help lines] (0,0) grid (2,2);
  \node (some node) at (1,1) {some node};
  
  \node (other node) [above=1cm of some node] {\tiny above=1cm of some node};

  \draw [<->] (some node.north) -- (other node.south)
                                node [midway,right,draw=none] {1cm};
\end{tikzpicture}
\end{codeexample}
    It is possible to change the behaviour of this
    \meta{specification} rather drastically, using the following key:
    \begin{key}{/tikz/on grid=\meta{boolean} (initially false)}
      When this key is set to |true|, an \meta{of-part} of the
      current form behaves differently: The anchors set for the
      current node as well as the anchor used for other \meta{node
        name} are set the |center|.

      This has the following effect: When you say
      |above=1cm of somenode| with |on grid| set to true, the new node
      will be placed in such a way that its center is 1cm above the
      center of |somenode|. Repeatedly placing nodes in this way will
      result in nodes that are centered on ``grid coordinate,'' hence
      the name of the option. 
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style=draw]
  \draw[help lines] (0,0) grid (2,3);

  % Not gridded
  \node (a1) at (0,0) {not gridded};
  \node (b1) [above=1cm of a1] {fooy};
  \node (c1) [above=1cm of b1] {a};

  % gridded
  \node (a2) at (2,0) {gridded};
  \node (b2) [on grid,above=1cm of a2] {fooy};
  \node (c2) [on grid,above=1cm of b2] {a};
\end{tikzpicture}
\end{codeexample}
    \end{key}
  \end{enumerate}

  \begin{key}{/tikz/node distance=\meta{shifting part} (initially 1cm and 1cm)}
    The value of this key is used as \meta{shifting part} is used if
    and only if a \meta{of-part} is present, but no \meta{shifting
      part}. 
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style=draw,node distance=5mm]
  \draw[help lines] (0,0) grid (2,3);

  % Not gridded
  \node (a1) at (0,0) {not gridded};
  \node (b1) [above=of a1] {fooy};
  \node (c1) [above=of b1] {a};

  % gridded
  \begin{scope}[on grid]
    \node (a2) at (2,0) {gridded};
    \node (b2) [above=of a2] {fooy};
    \node (c2) [above=of b2] {a};
  \end{scope}
\end{tikzpicture}
\end{codeexample}
  \end{key}
\end{key}

\begin{key}{/tikz/below=\opt{\meta{specification}}}
  This key is redefined in the same manner as |above|.
\end{key}

\begin{key}{/tikz/left=\opt{\meta{specification}}}
  This key is redefined in the same manner as |above|, only all
  vertical shifts are replaced by horizontal shifts.
\end{key}

\begin{key}{/tikz/right=\opt{\meta{specification}}}
  This key is redefined in the same manner as |left|.
\end{key}

\begin{key}{/tikz/above left=\opt{\meta{specification}}}
  This key is also redefined in a manner similar to the above, but
  behaviour of the \meta{shifting part} is more complicated:
  \begin{enumerate}
  \item When the \meta{shifting part} is of the form \meta{number or
      dimension}| and |\meta{number or dimension}, it has
    (essentially) the effect of shifting the node vertically upwards
    by the first \meta{number or dimension} and to the left by the
    second. To be more precise, the coordinate |(|\meta{second number
      or dimension}|,|\meta{first number or dimension}|)| is computed
    and then the node is shifted vertically by the $y$-part of
    the resulting coordinate and horizontally be the negated $x$-part
    of the result. (This is exactly what you expect, except possibly
    when you have used the |x| and |y| options to modify the
    |xy|-coordinate system so that the unit  vectors no longer point
    in the expected directions.)
  \item When the \meta{shifting part} is of the form \meta{number or
      dimension}, the node is shifted by this \meta{number or
      dimension} in the direction of $135^\circ$. This means that
    there is a difference between a \meta{shifting part} of |1cm| and
    of |1cm and 1cm|: In the second case, the node is shifted by 1cm
    upward and 1cm to the left; in the first case it is shifted by
    $\frac{1}{2}\sqrt{2}$cm upward and by the same amount to the
    left. A more mathematical way of phrasing this is the following: A
    plain \meta{dimension} is measured in the $l_2$-norm, while a
    \meta{dimension}| and |\meta{dimension} is measured in the
    $l_1$-norm. 
  \end{enumerate}
  The following example should help to illustrate the difference:
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={draw,circle}]
  \draw[help lines] (0,0) grid (2,5);
  \begin{scope}[node distance=5mm]
    \node (a) at (1,1) {a};
    \node [left=of a] {1};       \node [right=of a] {2};
    \node [above=of a] {3};      \node [below=of a] {4};
    \node [above left=of a] {5}; \node [above right=of a] {6};
    \node [below left=of a] {7}; \node [below right=of a] {8};
  \end{scope}
  \begin{scope}[node distance=5mm and 5mm]
    \node (b) at (1,4) {b};
    \node [left=of b] {1};       \node [right=of b] {2};
    \node [above=of b] {3};      \node [below=of b] {4};
    \node [above left=of b] {5}; \node [above right=of b] {6};
    \node [below left=of b] {7}; \node [below right=of b] {8};
  \end{scope}
\end{tikzpicture}
\end{codeexample}  
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={draw,rectangle}]
  \draw[help lines] (0,0) grid (2,5);
  \begin{scope}[node distance=5mm]
    \node (a) at (1,1) {a};
    \node [left=of a] {1};       \node [right=of a] {2};
    \node [above=of a] {3};      \node [below=of a] {4};
    \node [above left=of a] {5}; \node [above right=of a] {6};
    \node [below left=of a] {7}; \node [below right=of a] {8};
  \end{scope}
  \begin{scope}[node distance=5mm and 5mm]
    \node (b) at (1,4) {b};
    \node [left=of b] {1};       \node [right=of b] {2};
    \node [above=of b] {3};      \node [below=of b] {4};
    \node [above left=of b] {5}; \node [above right=of b] {6};
    \node [below left=of b] {7}; \node [below right=of b] {8};
  \end{scope}
\end{tikzpicture}
\end{codeexample}  
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={draw,rectangle},on grid]
  \draw[help lines] (0,0) grid (4,4);
  \begin{scope}[node distance=1]
    \node (a) at (2,3) {a};
    \node [left=of a] {1};       \node [right=of a] {2};
    \node [above=of a] {3};      \node [below=of a] {4};
    \node [above left=of a] {5}; \node [above right=of a] {6};
    \node [below left=of a] {7}; \node [below right=of a] {8};
  \end{scope}
  \begin{scope}[node distance=1 and 1]
    \node (b) at (2,0) {b};
    \node [left=of b] {1};       \node [right=of b] {2};
    \node [above=of b] {3};      \node [below=of b] {4};
    \node [above left=of b] {5}; \node [above right=of b] {6};
    \node [below left=of b] {7}; \node [below right=of b] {8};
  \end{scope}
\end{tikzpicture}
\end{codeexample}  
\end{key}

\begin{key}{/tikz/below left=\opt{\meta{specification}}}
  Works similar to |above left|.
\end{key}
\begin{key}{/tikz/above left=\opt{\meta{specification}}}
  Works similar to |above left|.
\end{key}
\begin{key}{/tikz/above right=\opt{\meta{specification}}}
  Works similar to |above left|.
\end{key}

The |positioning| package also introduces the following new placement
keys:
\begin{key}{/tikz/base left=\opt{\meta{specification}}}
  This key works like the |left| key, only instead of the |east| anchor,
  the |base east| anchor is used and, when the second form of an
  \meta{of-part} is used, the corresponding |base west| anchor.

  This key is useful for chaining together nodes so that their base
  lines are aligned.
\begin{codeexample}[]
\begin{tikzpicture}[node distance=1ex]
  \draw[help lines] (0,0) grid (3,1);
  \huge
  \node (X) at (0,1)     {X};
  \node (a) [right=of X] {a};
  \node (y) [right=of a] {y};
  
  \node (X) at (0,0)          {X};
  \node (a) [base right=of X] {a};
  \node (y) [base right=of a] {y};
\end{tikzpicture}
\end{codeexample}  
\end{key}
\begin{key}{/tikz/base right=\opt{\meta{specification}}}
  Works like |base left|.
\end{key}
\begin{key}{/tikz/mid left=\opt{\meta{specification}}}
  Works like |base left|, but with |mid east| and |mid west| anchors
  instead of |base east| and |base west|.
\end{key}
\begin{key}{/tikz/mid right=\opt{\meta{specification}}}
  Works like |mid left|.
\end{key}




\subsubsection{Arranging Nodes Using a Chains and Matrices}

The simple |above| and |right| options may not always suffice for
arranging a large number of nodes. For such situations \tikzname\
offers two libraries that make positioning easier: The |chains|
library and the |matrix| library. The first is mostly useful for
creating ``chains of nodes'' and, more generally, ``flows.'' The
second allows you to arrange multiple nodes in rows and columns. These
methods for positioning nodes are described in two separate
Sections~\ref{section-matrices} and~\ref{section-chains}. 


\subsection{Fitting Nodes to a Set of Coordinates}

\label{section-nodes-fitting}

It is sometimes desirable that the size and position of a node is not
given using anchors and size parameters, rather one would sometimes
have a box be placed and be sized such that it ``is just large enough
to contain this, that, and that point.'' This situation typically
arises when a picture has been drawn an, afterwards, parts of the
picture are supposed to be encircled or hilighted.

In this situation the |fit| option from the |fit| library is useful,
see Section~\ref{section-library-fit} for a the details. The idea is
that you may give the |fit| option to a node. The |fit| option expects
a list of coordinates (one after the other without commas) as its
parameter. The effect will be that the node's text area has exactly
the necessary size so that it contains all the given coordinates. Here
is an example:

\begin{codeexample}[]
\begin{tikzpicture}[level distance=8mm]
  \node (root) {root}
    child { node (a) {a} }
    child { node (b) {b}
      child { node (d) {d} }
      child { node (e) {e} } }
    child { node (c) {c} };

  \node[draw=red,inner sep=0pt,thick,ellipse,fit=(root) (b) (d) (e)] {};
  \node[draw=blue,inner sep=0pt,thick,ellipse,fit=(b) (c) (e)] {};
\end{tikzpicture}
\end{codeexample}

If you want to fill the fitted node you will usually have to place it
on a background layer.

\begin{codeexample}[]
\begin{tikzpicture}[level distance=8mm]
  \node (root) {root}
    child { node (a) {a} }
    child { node (b) {b}
      child { node (d) {d} }
      child { node (e) {e} } }
    child { node (c) {c} };

  \begin{pgfonlayer}{background}
    \node[fill=red!20,inner sep=0pt,ellipse,fit=(root) (b) (d) (e)] {};
    \node[fill=blue!20,inner sep=0pt,ellipse,fit=(b) (c) (e)] {};
  \end{pgfonlayer}
\end{tikzpicture}
\end{codeexample}

\subsection{Transformations}

\label{section-nodes-transformations}


It is possible to transform nodes, but, by default, transformations do
not apply to nodes. The reason is that you usually do \emph{not} want
your text to be scaled or rotated even if the main graphic is
transformed. Scaling text is evil, rotating slightly less so.

However, sometimes you \emph{do} wish to transform a node, for
example, it certainly sometimes makes sense to rotate a node by
90 degrees. There are two ways in which you can achieve this:

\begin{enumerate}
\item
  You can use the following option:
  \begin{key}{/tikz/transform shape}
    Causes the current ``external'' transformation matrix to be
    applied to the shape. For example, if you said
    |\tikz[scale=3]| and then say |node[transform shape] {X}|, you
    will get a ``huge'' X in your graphic.
  \end{key}
\item
  You can give transformation option \emph{inside} the option list of
  the node. \emph{These} transformations always apply to the node.
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={draw}]    
  \draw[help lines](0,0) grid (3,2);
  \draw            (1,0) node{A}
                   (2,0) node[rotate=90,scale=1.5] {B};
  \draw[rotate=30] (1,0) node{A}
                   (2,0) node[rotate=90,scale=1.5] {B};
  \draw[rotate=60] (1,0) node[transform shape] {A}
                   (2,0) node[transform shape,rotate=90,scale=1.5] {B};
\end{tikzpicture}
\end{codeexample}
\end{enumerate}




\subsection{Placing Nodes on a Line or Curve Explicitly}

\label{section-nodes-placing-1}

Until now, we always placed node on a coordinate that is mentioned in
the path. Often, however, we wish to place nodes on ``the middle'' of
a line and we do not wish to compute these coordinates ``by hand.''
To facilitate such placements, \tikzname\ allows you to specify that a
certain node should be somewhere ``on'' a line. There are two ways of
specifying this: Either explicitly by using the |pos| option or
implicitly by placing the node ``inside'' a path operation. These two
ways are described in the following.

\label{section-pos-option}

\begin{key}{/tikz/pos=\meta{fraction}}
  When this option is given, the node is not anchored on the last
  coordinate. Rather, it is anchored on some point on the line from
  the previous coordinate to the current point. The \meta{fraction}
  dictates how ``far'' on the line the point should be. A
  \meta{fraction} or 0 is the previous coordinate, 1 is the current
  one, everything else is in between. In particular, 0.5 is the
  middle.  

  Now, what is ``the previous line''? This depends on the previous
  path construction operation.

  In the simplest case, the previous path operation was a ``line-to''
  operation, that is, a  |--|\meta{coordinate} operation:
\begin{codeexample}[]
\tikz \draw (0,0) -- (3,1)
    node[pos=0]{0} node[pos=0.5]{1/2} node[pos=0.9]{9/10};
\end{codeexample}

  The next case is the curve-to operation (the |..| operation). In this
  case, the ``middle'' of the curve, that is, the position |0.5| is
  not necessarily the point at the exact half distance on the
  line. Rather, it is some point at ``time'' 0.5 of a point traveling
  from the start of the curve, where it is at time 0, to the end of
  the curve, which it reaches at time 0.5. The ``speed'' of the point
  depends on the length of the support vectors (the vectors that
  connect the start and end points to the control points). The exact
  math is a bit complicated (depending on your point of view, of
  course); you may wish to consult a good book on computer graphics
  and Bézier curves if you are intrigued. 
\begin{codeexample}[]
  \tikz \draw (0,0) .. controls +(right:3.5cm) and +(right:3.5cm) .. (0,3)
    \foreach \p in {0,0.125,...,1} {node[pos=\p]{\p}};
\end{codeexample}

  Another interesting case are the horizontal/vertical line-to operations
  \verb!|-! and \verb!-|!. For them, the position (or time) |0.5| is
  exactly the corner point.

\begin{codeexample}[]
\tikz \draw (0,0) |- (3,1)
  node[pos=0]{0} node[pos=0.5]{1/2} node[pos=0.9]{9/10};
\end{codeexample}

\begin{codeexample}[]
\tikz \draw (0,0) -| (3,1)
  node[pos=0]{0} node[pos=0.5]{1/2} node[pos=0.9]{9/10};
\end{codeexample}

  For all other path construction operations, \emph{the position
  placement does not work}, currently. This will hopefully change in
  the future (especially for the arc operation).  
\end{key}

\begin{key}{/tikz/auto=\meta{left or right} (default \normalfont is scope's setting)}
  This option causes an anchor positions to be calculated
  automatically according to the following rule. Consider a line
  between to points. If the \meta{direction} is |left|, then the
  anchor is chosen such that the node is to the left of this line. If
  the \meta{direction} is |right|, then the node is to the right of
  this line. Leaving out \meta{direction} causes automatic placement
  to be enabled with the last value of |left| or |right| used. A
  \meta{direction} of |false| disables automatic placement. This
  happens also  whenever an anchor is given explicitly by the
  |anchor| option or by one of the |above|, |below|, etc.\ options.

  This option only has an effect for nodes that are placed on lines or
  curves. 

\begin{codeexample}[]
\begin{tikzpicture}
  [scale=.8,auto=left,every node/.style={circle,fill=blue!20}]
  \node (a) at (-1,-2) {a};
  \node (b) at ( 1,-2) {b};
  \node (c) at ( 2,-1) {c};
  \node (d) at ( 2, 1) {d};
  \node (e) at ( 1, 2) {e};
  \node (f) at (-1, 2) {f};
  \node (g) at (-2, 1) {g};
  \node (h) at (-2,-1) {h};

  \foreach \from/\to in {a/b,b/c,c/d,d/e,e/f,f/g,g/h,h/a}
    \draw [->] (\from) -- (\to)
               node[midway,fill=red!20] {\from--\to};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/swap}
  This option exchanges the roles of |left| and |right| in automatic
  placement. That is, if |left| is the current |auto| placement,
  |right| is set instead and the other way round.
\begin{codeexample}[]
\begin{tikzpicture}[auto]
  \draw[help lines,use as bounding box] (0,-.5) grid (4,5);  

  \draw (0.5,0) .. controls (9,6) and (-5,6) .. (3.5,0)
    \foreach \pos in {0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1}
      {node [pos=\pos,swap,fill=red!20] {\pos}}
    \foreach \pos in {0.025,0.2,0.4,0.6,0.8,0.975}
      {node [pos=\pos,fill=blue!20] {\pos}};
\end{tikzpicture}
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}[shorten >=1pt,node distance=2cm,auto]
  \draw[help lines] (0,0) grid (3,2);

  \node[state] (q_0)                      {$q_0$};
  \node[state] (q_1) [above right of=q_0] {$q_1$};
  \node[state] (q_2) [below right of=q_0] {$q_2$};
  \node[state] (q_3) [below right of=q_1] {$q_3$};

  \path[->] (q_0) edge              node        {0} (q_1)
                  edge              node [swap] {1} (q_2)
            (q_1) edge              node        {1} (q_3)
                  edge [loop above] node        {0} ()
            (q_2) edge              node [swap] {0} (q_3)
                  edge [loop below] node        {1} ();
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/sloped}
  This option causes the node to be rotated such that a horizontal
  line becomes a tangent to the curve. The rotation is normally 
  done in such a way that text is never ``upside down.'' To get
  upside-down text, use can use |[rotate=180]| or
  |[allow upside down]|, see below.
\begin{codeexample}[]
\tikz \draw (0,0) .. controls +(up:2cm) and +(left:2cm) .. (1,3)
    \foreach \p in {0,0.25,...,1} {node[sloped,above,pos=\p]{\p}};
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}[->]
  \draw (0,0)   -- (2,0.5) node[midway,sloped,above] {$x$};
  \draw (2,-.5) -- (0,0)   node[midway,sloped,below] {$y$};
\end{tikzpicture}
\end{codeexample}
\end{key}


\begin{key}{/tikz/allow upside down=\meta{boolean} (default true, initially false)}
  If set to |true|, \tikzname\ will not ``righten'' upside down text. 
\begin{codeexample}[]
\tikz [allow upside down]
  \draw (0,0) .. controls +(up:2cm) and +(left:2cm) .. (1,3)
    \foreach \p in {0,0.25,...,1} {node[sloped,above,pos=\p]{\p}};
\end{codeexample}
\begin{codeexample}[]
\begin{tikzpicture}[->,allow upside down]
  \draw (0,0)   -- (2,0.5) node[midway,sloped,above] {$x$};
  \draw (2,-.5) -- (0,0)   node[midway,sloped,below] {$y$};
\end{tikzpicture}
\end{codeexample}
\end{key}


There exist styles for specifying positions a bit less ``technically'':
\begin{stylekey}{/tikz/midway}
  This has the same effect as |pos=0.5|.
\begin{codeexample}[]
\tikz \draw (0,0) .. controls +(up:2cm) and +(left:3cm) .. (1,5)
       node[at end]          {|at end|}
       node[very near end]   {|very near end|}
       node[near end]        {|near end|}
       node[midway]          {|midway|}
       node[near start]      {|near start|}
       node[very near start] {|very near start|}
       node[at start]        {|at start|};
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/near start}
  Set to |pos=0.25|.
\end{stylekey}

\begin{stylekey}{/tikz/near end}
  Set to |pos=0.75|.
\end{stylekey}

\begin{stylekey}{/tikz/very near start}
  Set to |pos=0.125|.
\end{stylekey}

\begin{stylekey}{/tikz/very near end}
  Set to |pos=0.875|.
\end{stylekey}

\begin{stylekey}{/tikz/at start}
  Set to |pos=0|.
\end{stylekey}

\begin{stylekey}{/tikz/at end}
  Set to |pos=1|.
\end{stylekey}


\subsection{Placing Nodes on a Line or Curve Implicitly}

\label{section-nodes-placing-2}

When you wish to place a node on the line |(0,0) -- (1,1)|,
it is natural to specify the node not following the |(1,1)|, but
``somewhere in the middle.'' This is, indeed, possible and you can
write |(0,0) -- node{a} (1,1)| to place a node midway between |(0,0)| and
|(1,1)|.

What happens is the following: The syntax of the line-to path
operation is actually |--|
\opt{|node|\meta{node specification}}\meta{coordinate}. (It is even
possible to give multiple nodes in this way.) When the optional
|node| is encountered, that is, 
when the |--| is directly followed by |node|, then the
specification(s) are read and ``stored away.'' Then, after the
\meta{coordinate} has finally been reached, they are inserted again,
but with the |pos| option set.

There are two things to note about this: When a node specification is
``stored,'' its catcodes become fixed. This means that you cannot use
overly complicated verbatim text in them. If you really need, say, a
verbatim text, you will have to put it in a normal node following the
coordinate and add the |pos| option.

Second, which |pos| is chosen for the node? The position is inherited
from the surrounding scope. However, this holds only for nodes
specified in this implicit way. Thus, if you add the option
|[near end]| to a scope, this does not mean that \emph{all} nodes given
in this scope will be put on near the end of lines. Only the nodes
for which an implicit |pos| is added will be placed near the
end. Typically, this is what you want. Here are some examples that
should make this clearer:

\begin{codeexample}[]
\begin{tikzpicture}[near end]
  \draw (0cm,4em) -- (3cm,4em) node{A};    
  \draw (0cm,3em) --           node{B}          (3cm,3em);
  \draw (0cm,2em) --           node[midway] {C} (3cm,2em);
  \draw (0cm,1em) -- (3cm,1em) node[midway] {D} ;
\end{tikzpicture}
\end{codeexample}

Like the line-to operation, the curve-to operation |..| also allows you to
specify nodes ``inside'' the operation. After both the first |..| and
also after the second |..| you can place node specifications. Like for
the |--| operation, these will be collected and then reinserted after
the operation with the |pos| option set.


\subsection{The Label and Pin Options}

In addition to the |node| path operation, nodes can also be added
using the |label| and the |pin| option. This is mostly useful
for simple nodes. 

\begin{key}{/tikz/label=\opt{|[|\meta{options}|]|}\meta{angle}|:|\meta{text}}
  When this option is given to a |node| operation, it causes
  \emph{another} node to be added to the path after the current node
  has been finished. This extra node will have the text
  \meta{text}. It is placed according to the following rule: Suppose
  the |node| currently under construction is called |main node| and let us
  call the label node |label node|. Then the anchor of |label node| is
  placed at |main node.|\meta{angle}. The anchor that is chosen
  depends on the \meta{angle}. If the \meta{angle} lies between
  $-3^\circ$ and $+3^\circ$, then the anchor |west| is chosen, which
  causes |label node| to be placed right of the right end
  |main node|. If \meta{angle} lies between $4^\circ$ and $86^\circ$,
  the anchor |south west| is chosen, causing the |label node| to be
  placed above and right of the |main node|; and so on.
\begin{codeexample}[]
\tikz
  \node [circle,draw,label=60:$60^\circ$,label=below:$-90^\circ$] {my circle};
\end{codeexample}

  As can be seen in the above example, instead of specifying
  \meta{angle} as a number, it is also possible to use |left|,
  |right|, |above|, |above left|, and so on.

  You can pass \meta{options} to the node |label node|. For this, you
  provide the options in square brackets before the \meta{angle}. If you
  do so, you need to add braces around the whole argument of the
  |label| option and this is also the case if you have brackets or
  commas or semicolons or anything special in the \meta{text}.
\begin{codeexample}[]
\tikz \node [circle,draw,label={[red]above:X}] {my circle};
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \node [circle,draw,label={[name=label node]above left:$a,b$}] {};
  \draw (label node) -- +(1,1);
\end{tikzpicture}
\end{codeexample}

  If you provide multiple |label| options, then multiple extra label
  nodes are added in the order they are given.

  The following styles influence how labels are drawn:
  \begin{key}{/tikz/label distance=\meta{distance} (initially 0pt)}
    The \meta{distance} is additionally inserted between the main node
    and the label node.
\begin{codeexample}[]
\tikz[label distance=5mm]
  \node [circle,draw,label=right:X,
                     label=above right:Y,
                     label=above:Z]       {my circle};
\end{codeexample}
  \end{key}
  \begin{stylekey}{/tikz/every label (initially \normalfont empty)}
    This style is used in every node created by the |label|
    option. The default is |draw=none,fill=none|.
  \end{stylekey}
\end{key}

\begin{key}{/tikz/pin=\opt{|[|\meta{options}|]|}\meta{angle}|:|\meta{text}}
  This is option is quite similar to the |label| option, but there is
  one difference: In addition to adding a extra node to the picture, 
  it also adds an edge from this node to the main node. This causes
  the node to look like a pin that has been added to the main node: 
\begin{codeexample}[]
\tikz \node [circle,fill=blue!50,minimum size=1cm,pin=60:$q_0$] {};
\end{codeexample}

  The meaning of the \meta{options} and the \meta{angle} and the
  \meta{text} is exactly the same as for the |node| option. Only, the
  options and styles the influence the way pins look are different:
  \begin{key}{/tikz/pin distance=\meta{distance} (initially 3ex)}
    This \meta{distance} is used instead of the |label distance| for
    the distance between the main node and the label node.
\begin{codeexample}[]
\tikz[pin distance=1cm]
  \node [circle,draw,pin=right:X,
                     pin=above right:Y,
                     pin=above:Z]       {my circle};
\end{codeexample}
  \end{key}
  \begin{stylekey}{/tikz/every pin (initially \normalfont draw=none,fill=none)}
    This style is used in every node created by the |pin|
    option.
  \end{stylekey}
  \begin{stylekey}{/tikz/every pin edge (initially help lines)}
    This style is used in every edge created by the |pin| optins.
\begin{codeexample}[]
\tikz [pin distance=15mm,
       every pin edge/.style={<-,shorten <=1pt,decorate,
                              decoration={snake,pre length=4pt}}]
  \node [circle,draw,pin=right:X,
                     pin=above right:Y,
                     pin=above:Z]       {my circle};
\end{codeexample}
  \end{stylekey}

  \begin{key}{/tikz/pin edge=\meta{options} (initially \normalfont empty)}
    This option can be used to set the options that are to be used
    in the edge created by the |pin| option. 
\begin{codeexample}[]
\tikz[pin distance=10mm]
  \node [circle,draw,pin={[pin edge={blue,thick}]right:X},
                     pin=above:Z]       {my circle};
\end{codeexample}
\begin{codeexample}[]
\tikz [every pin edge/.style={},
       initial/.style={pin={[pin distance=5mm,
                             pin edge={<-,shorten <=1pt}]left:start}}]
  \node [circle,draw,initial] {my circle};
\end{codeexample}
  \end{key}
\end{key}


\subsection{Connecting Nodes: Using Nodes as Coordinates}

\label{section-nodes-connecting}

Once you have defined a node and given it a name, you can use this
name to reference it. This can be done in two ways, see also
Section~\ref{section-node-coordinates}. Suppose you have said
|\path(0,0) node(x) {Hello World!};| in order to define a node named |x|. 
\begin{enumerate}
\item
  Once the node |x| has been defined, you can use
  |(x.|\meta{anchor}|)| wherever you would normally use a normal
  coordinate. This will yield the position at which the given
  \meta{anchor} is in the picture. Note that transformations do not
  apply to this coordinate, that is, |(x.north)| will be the northern
  anchor of |x| even if you have said |scale=3| or |xshift=4cm|. This
  is usually what you would expect.
\item
  You can also just use |(x)| as a coordinate. In most cases, this
  gives the same coordinate as |(x.center)|. Indeed, if the |shape| of
  |x| is |coordinate|, then |(x)| and |(x.center)| have exactly the
  same effect.

  However, for most other shapes, some path construction operations like
  |--| try to be ``clever'' when this they are asked to draw a line
  from such a coordinate or to such a coordinate. When you say
  |(x)--(1,1)|, the |--| path operation will not draw a line from the center
  of |x|, but \emph{from the border} of |x| in the direction going
  towards |(1,1)|. Likewise, |(1,1)--(x)| will also have the line
  end on the border in the direction coming from |(1,1)|.

  In addition to |--|, the curve-to path operation |..| and the path
  operations \verb!-|! and \verb!|-! will also handle nodes without
  anchors correctly. Here is an example, see also
  Section~\ref{section-node-coordinates}:
\begin{codeexample}[]
\begin{tikzpicture}
  \path (0,0) node             (x) {Hello World!}
        (3,1) node[circle,draw](y) {$\int_1^2 x \mathrm d x$};

  \draw[->,blue]   (x) -- (y);
  \draw[->,red]    (x) -| node[near start,below] {label} (y);
  \draw[->,orange] (x) .. controls +(up:1cm) and +(left:1cm) .. node[above,sloped] {label} (y);
\end{tikzpicture}
\end{codeexample}
\end{enumerate}




\subsection{Connecting Nodes: Using the Edge Operation}

\label{section-nodes-edges}

The |edge| operation works like a |to| operation that is added after
the main path has been drawn, much like a node is added after the main
path has been drawn. This allows you to have each |edge| to have a
different appearance. As the |node| operation, an |edge| temporarily
suspends the construction of the current path and a new path $p$ is 
constructed. This new path $p$ will be drawn after the main path has
been drawn. Note that $p$ can be totally different from the main
path with respect to its options. Also note that if there are
several |to| and/or |node| operations in the main path, each
creates its own path(s) and they are drawn in the order that they
are encountered on the path.

\begin{pathoperation}{edge}{\opt{|[|\meta{options}|]|}
    \opt{\meta{nodes}} |(|\meta{coordinate}|)|}
  The effect of the |edge| operation is that after the main path the
  following path is added to the picture:
  \begin{quote}
    |\path[every edge,|\meta{options}|] (\tikztostart) |\meta{path}|;|
  \end{quote}
  Here, \meta{path} is the |to path|. Note that, unlike the path added
  by the |to| operation, the |(\tikztostart)| is added before the
  \meta{path} (which is unnecessary for the |to| operation, since this
  coordinate is already part of the main path).

  The |\tikztostart| is the last coordinate on the path just before
  the |edge| operation, just as for the |node| or |to| operations. 
  However, there is one exception to this rule: If the |edge|
  operation is directly preceded by a |node| operation, then this
  just-declared node is the start coordinate (and not, as would
  normally be the case, the coordinate where this just-declared node
  is placed -- a small, but subtle difference). In this regard, |edge|
  differs from both |node| and |to|.
  
  If there are several |edge| operations in a row, the start coordinate
  is the same for all of them as their target coordiantes are not,
  after all, part of the main path. The start coordinate is, thus, the
  coordinate preceding the first |edge| operation. This is
  similar to nodes insofar as the |edge| operation does not modify the
  current path at all. In particular, it does not change the last
  coordinate visited, see the following example:
  
\begin{codeexample}[]
\begin{tikzpicture}
  \node (a) at   (0:1) {$a$};
  \node (b) at  (90:1) {$b$} edge [->]     (a);
  \node (c) at (180:1) {$c$} edge [->]     (a)
                             edge [<-]     (b);
  \node (d) at (270:1) {$d$} edge [->]     (a)
                             edge [dotted] (b)
                             edge [<-]     (c);  
\end{tikzpicture}
\end{codeexample}

  A different way of specifying the above graph using the |edge|
  operation is the following:  

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \name/\angle in {a/0,b/90,c/180,d/270}
    \node (\name) at (\angle:1) {$\name$};

  \path[->] (b) edge (a)
                edge (c)
                edge [-,dotted] (d)
            (c) edge (a)
                edge (d)
            (d) edge (a);
\end{tikzpicture}
\end{codeexample}

  As can be seen, the path of the |edge| operation inherits the
  options from the main path, but you can locally overrule them.

\begin{codeexample}[]
\begin{tikzpicture}
  \foreach \name/\angle in {a/0,b/90,c/180,d/270}
    \node (\name) at (\angle:1.5) {$\name$};

  \path[->] (b) edge            node[above right]  {$5$}     (a)
                edge                                         (c)
                edge [-,dotted] node[below,sloped] {missing} (d)
            (c) edge                                         (a)
                edge                                         (d)
            (d) edge [red]      node[above,sloped] {very}  
                                node[below,sloped] {bad}     (a);
\end{tikzpicture}
\end{codeexample}

  Instead of |every to|, the style |every edge| is installed at the
  beginning of the main path.
  \begin{stylekey}{/tikz/every edge (inititially draw)}
    Executed for each |edge|.
\begin{codeexample}[]
\begin{tikzpicture}[every to/.style={draw,dashed}]
  \path (0,0) to (3,2);
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}
\end{pathoperation}


\subsection{Referencing Nodes Outside the Current Pictures}

\label{section-cross-picture-tikz}

\subsubsection{Referencing a Node in a Different Picture}

It is possible (but not quite trivial) to reference nodes in pictures
other than the current one. This means that you can create a picture
and a node therein and, later, you can draw a line from some other
position to this node. 

To reference nodes in different pictures, proceed as follows:
\begin{enumerate}
\item You need to add the |remember picture| option to all pictures
  that contain nodes that you wish to reference and also to all
  pictures from which you wish to reference a node in another
  picture.
\item You need to add the |overlay| option to paths or to whole
  pictures that contain references to nodes in different
  pictures. (This option switches the computation of the
  bounding box off.)
\item You need to use a driver that supports picture remembering and
  you need to run \TeX\ twice.
\end{enumerate}
(For more details on what is going on behind the scenes, see
Section~\ref{section-cross-pictures-pgf}.)

Let us have a look at the effect of these options.
\begin{key}{/tikz/remember picture=\meta{boolean} (initially false)}
  This option tells \tikzname\ that it should attempt to remember the
  position of the current picture on the page. This attempt may fail
  depending on which backend driver is used. Also, even if remembering
  works, the position may only be available on a second run of \TeX.

  Provided that remebering works, you may consider saying
\begin{codeexample}[code only]
\tikzsytle{every picture}+=[remember picture]
\end{codeexample}
  to make \tikzname\ remember all pictures. This will add one line in
  the |.aux| file for each picture in your document -- which typically
  is not very much. Then, you do not have to worry about remembered
  pictures at all.
\end{key}

\begin{key}{/tikz/overlay}
  This option is mainly intended for use when nodes in other pictures
  are referenced, but you can also use it in other situations. The
  effect of this option is that everything within the current scope is
  not taken into consideration when the bounding box of the current
  picture is computed.

  You need to specify this option on all paths (or at least on all
  parts of paths) that contain a reference to a node in another
  picture. The reason is that, otherwise, \tikzname\ will attempt to
  make the current picture large enough to encompass \emph{the node in
    the other picture}. However, on a second run of \TeX\ this will
  create an even bigger picture, leading to larger and larger
  pictures. Unless you know what you are doing, I suggest specifying
  the |overlay| option with all pictures that contain references to
  other pictures.
\end{key}

Let us now have a look at a few examples. These examples work only if
this document is processed with a driver that supports picture
remembering.
\medskip

\noindent\begin{minipage}{\textwidth}
Inside the current text we place two pictures, containing nodes named
|n1| and |n2|, using
\begin{codeexample}[code only]
\tikz[remember picture] \node[circle,fill=red!50] (n1) {};
\end{codeexample}
which yields \tikz[remember picture] \node[circle,fill=red!50] (n1)
{};, and
\begin{codeexample}[code only]
\tikz[remember picture] \node[fill=blue!50] (n2) {};
\end{codeexample}
yielding the node \tikz[remember picture] \node[fill=blue!50] (n2)
{};. To connect these nodes, we create another picture using the
|overlay| option and also the |remember picture| option.
\begin{codeexample}[]
\begin{tikzpicture}[remember picture,overlay]
  \draw[->,very thick] (n1) -- (n2);
\end{tikzpicture}
\end{codeexample}
Note that the last picture is seemingly empty. What happens is that it
has zero size and contains an arrow that lies well outside its bounds.
As a last example, we connect a node in another picture to the first
two nodes. Here, we provide the |overlay| option only with the line
that we do not wish to count as part of the picture.
\begin{codeexample}[]
\begin{tikzpicture}[remember picture]
  \node (c) [circle,draw] {Big circle};
  
  \draw [overlay,->,very thick,red,opacity=.5]
    (c) to[bend left] (n1) (n1) -| (n2);
\end{tikzpicture}
\end{codeexample}
\end{minipage}


\subsubsection{Referencing the Current Page Node -- Absolute Positioning}

There is a special node called |current page| that can be used to
access the current page. It is a node of shape rectangle whose
|south west| anchor is the lower left corner of the page and whose
|north east| anchor is the upper right corner of the page. While this
node is handled in a special way internally, you can reference it as
if it were defined in some remembered picture other than the current
one. Thus, by giving the |remembered picture| and the |overlay|
options to a picture, you can position nodes \emph{absolutely} on a
page.

The first example places some text in the lower left corner of the
current page:
\begin{codeexample}[]
\begin{tikzpicture}[remember picture,overlay]
  \node [xshift=1cm,yshift=1cm] at (current page.south west)
        [text width=7cm,fill=red!20,rounded corners,above right]
  {
    This is an absolutely positioned text in the
    lower left corner. No shipout-hackery is used.
  };
\end{tikzpicture}
\end{codeexample}

The next example adds a circle in the middle of the page.
\begin{codeexample}[]
\begin{tikzpicture}[remember picture,overlay]
  \draw [line width=1mm,opacity=.25]
    (current page.center) circle (3cm);
\end{tikzpicture}
\end{codeexample}

The final example overlays some text over the page (depending on where
this example is found on the page, the text may also be behind the
page).
\begin{codeexample}[]
\begin{tikzpicture}[remember picture,overlay]
  \node [rotate=60,scale=10,text opacity=0.2]
    at (current page.center) {Example};
\end{tikzpicture}
\end{codeexample}



\subsection{Late Code and Options}

All options given to a node only locally affect this one node. While
this is a blessing in most cases, you may sometimes want to cause
options to have effects ``later'' on. The other way round, you may
sometimes note ``only later'' that some options should be added to the
options of a node. The present section describes ways of achieving
these effects. 


\subsubsection{Executing Code After Nodes}

\label{section-nodes-executing}

It is possible to add a path right after a node using the option
|after node path|. The idea is that a style might use this option to
add some additional stuff to the node that has just been
typeset. Examples of such styles include the |label| option and the
|pin| option. 

\begin{key}{/tikz/after node path=\meta{path}}
  The \meta{path} is added to the main path right after the node, as
  if you had given the path thereafter. This option can only be given
  inside the option list of a node and multiple calls of this option
  accumulate. 

  Inside the \meta{path} you have access to the node that has just
  been created via the macro \declare{|\tikzlastnode|}.
\begin{codeexample}[]
\tikz
  \draw node [draw,after node path={(\tikzlastnode) circle (2cm)}]
    {hello};
\end{codeexample}

  Note that in the above example, if we had written |\path| instead of
  |\draw|, the circle would not have been drawn since the circle is
  part of the main path, not part of the node itself. 
\end{key}

\begin{command}{\tikzaddafternodepathoption\marg{code}}
  This command allows you to specify that the \meta{code} should be
  executed at the beginning of the |after node path| of the current
  node. The code will also be executed immediately, but also again at
  the beginning of an |after node path|.
\end{command}


\subsection{Late Options}

A \emph{late option} for a node is an option that is given a long time
after the node has already been constructed.

\begin{key}{/tikz/late options=\meta{options}}
  This option can be given on a path (but not as an argument to a
  |node| path command). It has the following effect: An already
  \meta{existing node} is determined (in a way to be described in a moment)
  and, then, the \meta{options} are executed in a local scope. Most of
  these options will have no effect since you \emph{cannot change the
    appearance of the node,} that is, you cannot change a red node
  into a green node using late options. However, giving the
  the |after node path| option inside the \meta{options} (directly or
  indirectly) does have the desired effect: The after node path gets
  executed with the |\tikzlastnode| set to the determined node.

  The net effect of all this is that you can provide, say, the |label|
  option inside the \meta{options} to a add a label to a node that has
  already been constructed. Likewise, you can use the |on chain|
  option to make an already \meta{existing node} part of a chain.

  The \meta{existing node} is determined as follows: If the
  |name=|\meta{existing node} option is used inside the
  \meta{options}, then this name is used. Otherwise, if the last
  coordinate on the current path was of the form |(|\meta{existing
    node}|)|, then this \meta{existing node} name is used. Otherwise,
  an error results.

\begin{codeexample}[]
\begin{tikzpicture}
  \node (a) [draw,circle] {Hello};
  \path (a) [late options={label=above:world}];
\end{tikzpicture}
\end{codeexample}  
\end{key}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-tikz-transformations.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Transformations}

\pgfname\ has a powerful transformation mechanism that is similar to
the transformation capabilities of \textsc{metafont}. The present
section explains how you can access it in \tikzname.


\subsection{The Different Coordinate Systems}

It is a long process from  a coordinate like, say, $(1,2)$ or
$(1\mathrm{cm},5\mathrm{pt})$, to the position a point is finally
placed on the display or paper. In order to find out where the point
should go, it is constantly ``transformed,'' which means that it is
mostly shifted around and possibly rotated, slanted, scaled, and
otherwise mutilated. 

In detail, (at least) the following transformations are applied to a
coordinate like $(1,2)$ before a point on the screen is chosen:
\begin{enumerate}
\item
  \pgfname\ interprets a coordinate like $(1,2)$  in its
  $xy$-coordinate system as ``add the current $x$-vector once and the
  current $y$-vector twice to obtain the new point.''
\item
  \pgfname\ applies its coordinate transformation matrix to the
  resulting coordinate. This yields the final position of the point 
  inside the picture.
\item
  The backend driver (like |dvips| or |pdftex|) adds transformation
  commands such the coordinate is shifted to the correct position in
  \TeX's page coordinate system.
\item
  \textsc{pdf} (or PostScript) apply the canvas transformation
  matrix to the point, which can once more change the position on the
  page. 
\item
  The viewer application or the printer applies the device
  transformation matrix to transform the coordinate to its final pixel
  coordinate on the screen or paper.  
\end{enumerate}

In reality, the process is even more involved, but the above should
give the idea: A point is constantly transformed by changes of the
coordinate system.

In \tikzname, you only have access to the first two coordinate systems:
The $xy$-coordinate system and the coordinate transformation matrix
(these will be explained later). \pgfname\ also allows you to change
the canvas transformation matrix, but you have to use commands of
the core layer directly to do so and you ``better know what you are
doing'' when you do this. The moment you start modifying the
canvas matrix, \pgfname\ immediately looses track of all
coordinates and shapes, anchors, and bounding box computations will no
longer work.


\subsection{The XY- and XYZ-Coordinate Systems}
\label{section-xyz}

The first and easiest coordinate systems are \pgfname's $xy$- and
$xyz$-coordinate systems. The idea is very simple: Whenever you
specify a coordinate like |(2,3)| this means $2v_x + 3v_y$, where
$v_x$ is the current \emph{$x$-vector} and $v_y$ is the current
\emph{$y$-vector}. Similarly, the coordinate |(1,2,3)| means $v_x +
2v_y + 3v_z$.

Unlike other packages, \pgfname\ does not insist that $v_x$ actually
has a $y$-component of $0$, that is, that it is a horizontal
vector. Instead, the $x$-vector can point anywhere you
want. Naturally, \emph{normally} you will want the $x$-vector to point
horizontally.

One undesirable effect of this flexibility is that it is not possible
to provide mixed coordinates as in $(1,2\mathrm{pt})$. Life is hard.

To change the $x$-, $y$-, and $z$-vectors, you can use the following
options:

\begin{key}{/tikz/x=\meta{value} (initially 1cm)}
  If \meta{value} is a dimension, the $x$-vector of
  \pgfname's $xyz$-coordinate system is setup to point 
  \meta{value} to the right, that is, to $(\meta{value},0pt)$.

\begin{codeexample}[]
\begin{tikzpicture}
  \draw                  (0,0)   -- +(1,0);
  \draw[x=2cm,color=red] (0,0.1) -- +(1,0);
\end{tikzpicture}
\end{codeexample}    

\begin{codeexample}[]
\tikz \draw[x=1.5cm] (0,0) grid (2,2);
\end{codeexample}    

  The last example shows that the size of steppings in grids, just like
  all other dimensions, are not affected by the $x$-vector. After all,
  the $x$-vector is only used to determine the coordinate of the upper
  right corner of the grid.

  If \meta{value} is a coordinate, the $x$-vector of
  \pgfname's $xyz$-coordinate system to the specified coordinate. If
  \meta{value} contains a comma, it must be put in braces. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw                            (0,0) -- (1,0);
  \draw[x={(2cm,0.5cm)},color=red] (0,0) -- (1,0);
\end{tikzpicture}
\end{codeexample}

  You can use this, for example, to exchange the meaning of the $x$- and
  $y$-coordinate.

\begin{codeexample}[]
\begin{tikzpicture}[smooth]
  \draw plot coordinates{(1,0) (2,0.5) (3,0) (3,1)};
  \draw[x={(0cm,1cm)},y={(1cm,0cm)},color=red]
        plot coordinates{(1,0) (2,0.5) (3,0) (3,1)};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/y=\meta{value} (initially 1cm)}
  Works like the |x=| option, only if \meta{value} is a dimension, the
  resulting vector points to $(0,\meta{value})$.
\end{key}

\begin{key}{/tikz/z=\meta{value} (initially \normalfont$-\sqrt{2}$cm)}
  Works like the |y=| option, but now a dimension is means the point
  $(\meta{value},\meta{value})$.

\begin{codeexample}[]
\begin{tikzpicture}[z=-1cm,->,thick]
  \draw[color=red] (0,0,0) -- (1,0,0);
  \draw[color=blue] (0,0,0) -- (0,1,0);
  \draw[color=orange] (0,0,0) -- (0,0,1);
\end{tikzpicture}
\end{codeexample}
\end{key}



\subsection{Coordinate Transformations}

\pgfname\ and \tikzname\ allow you to specify \emph{coordinate
  transformations}. Whenever you specify a coordinate as in |(1,0)| or
|(1cm,1pt)| or |(30:2cm)|, this coordinate is first
``reduced'' to a position of the form ``$x$ points to the right and
  $y$ points upwards.'' For example, |(1in,5pt)| is reduced to
``$72\frac{72}{100}$ points to the right and 5 points upwards'' and
|(90:100pt)| means ``0pt to the right and 100 points upwards.''

The next step is to apply the current \emph{coordinate transformation
  matrix} to the coordinate. For example, the coordinate
transformation matrix might currently be set such that it adds a
certain constant to the $x$ value. Also, it might be setup such that
it, say, exchanges the $x$ and $y$ value. In general, any
``standard'' transformation like translation, rotation, slanting, or
scaling or any combination thereof is possible. (Internally, \pgfname\
keeps track of a coordinate transformation matrix very much like the
concatenation matrix used by \textsc{pdf} or PostScript.)

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw (0,0) rectangle (1,0.5);
  \begin{scope}[xshift=1cm]
    \draw             [red]    (0,0) rectangle (1,0.5);
    \draw[yshift=1cm] [blue]   (0,0) rectangle (1,0.5);
    \draw[rotate=30]  [orange] (0,0) rectangle (1,0.5);
  \end{scope}
\end{tikzpicture}
\end{codeexample}

The most important aspect of the coordinate transformation matrix is
\emph{that it applies to coordinates only!} In particular, the
coordinate transformation has no effect on things like the line width
or the dash pattern or the shading angle. In certain cases, it is not
immediately clear whether the coordinate transformation matrix
\emph{should} apply to a certain dimension. For example, should the
coordinate transformation matrix apply to grids? (It does.) And what
about the size of arced corners? (It does not.) The general rule is
``If there is no `coordinate' involved, even `indirectly,' the matrix
is not applied.'' However, sometimes, you simply have to try or look
it up in the documentation whether the matrix will be applied.

Setting the matrix cannot be done directly. Rather, all you can do is
to ``add'' another transformation to the current matrix. However, all
transformations are local to the current \TeX-group. All
transformations are added using graphic options, which are described
below.

Transformations apply immediately when they are encountered ``in the
middle of a path'' and they apply only to the coordinates on the path
following the transformation option. 

\begin{codeexample}[]
\tikz \draw (0,0) rectangle (1,0.5) [xshift=2cm] (0,0) rectangle (1,0.5);
\end{codeexample}

A final word of warning: You should refrain from using ``aggressive''
transformations like a scaling of a factor of 10000. The reason is
that all transformations are done using \TeX, which has a fairly low
accuracy. Furthermore, in certain situations it is necessary that
\tikzname\ \emph{inverts} the current transformation matrix and this will
fail if the transformation matrix is badly conditioned or even
singular (if you do not know what singular matrices are, you are blessed).   

\begin{key}{/tikz/shift={\ttfamily\char`\{}\meta{coordinate}{\ttfamily\char`\}}}
  Adds the \meta{coordinate} to all coordinates.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                       (0,0) -- (1,1) -- (1,0);
  \draw[shift={(1,1)},blue]   (0,0) -- (1,1) -- (1,0);
  \draw[shift={(30:1cm)},red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/shift only}
  This option does not take any parameter. Its effect is to cancel all
  current transformations except for the shifting. This means that the
  origin will remain where it is, but any rotation around the origin
  or scaling relative to the origin or skewing will no longer have an
  effect.

  This option is useful in situtations where a complicated
  transformation is used to ``get to a position,'' but you then wish
  to draw something ``normal'' at this position. 

\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                                      (0,0) -- (1,1) -- (1,0);
  \draw[rotate=30,xshift=2cm,blue]           (0,0) -- (1,1) -- (1,0);
  \draw[rotate=30,xshift=2cm,shift only,red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/xshift=\meta{dimension}}
  Adds \meta{dimension} to the $x$ value of all coordinates.  
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                   (0,0) -- (1,1) -- (1,0);
  \draw[xshift=2cm,blue]  (0,0) -- (1,1) -- (1,0);
  \draw[xshift=-10pt,red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/yshift=\meta{dimension}}
  Adds \meta{dimension} to the $y$ value of all coordinates.
\end{key}

\begin{key}{/tikz/scale=\meta{factor}}
  Multiplies all coordinates by the given \meta{factor}. The
  \meta{factor} should not be excessively large in absolute terms or
  very near to zero.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw               (0,0) -- (1,1) -- (1,0);
  \draw[scale=2,blue] (0,0) -- (1,1) -- (1,0);
  \draw[scale=-1,red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/scale around={\ttfamily\char`\{}\meta{factor}|:|\meta{coordinate}{\ttfamily\char`\}}}
  Scales the coordinate system by \meta{factor}, put with the ``origin
  of scaling'' centered on \meta{coordinate} rather than the origin. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                             (0,0) -- (1,1) -- (1,0);
  \draw[scale=2,blue]               (0,0) -- (1,1) -- (1,0);
  \draw[scale around={2:(1,1)},red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/xscale=\meta{factor}}
  Multiplies only the $x$-value of all coordinates by the given
  \meta{factor}. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                (0,0) -- (1,1) -- (1,0);
  \draw[xscale=2,blue] (0,0) -- (1,1) -- (1,0);
  \draw[xscale=-1,red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/yscale=\meta{factor}}
  Multiplies only the $y$-value of all coordinates by \meta{factor}.
\end{key}

\begin{key}{/tikz/xslant=\meta{factor}}
  Slants the coordinate horizontally by the given \meta{factor}:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                (0,0) -- (1,1) -- (1,0);
  \draw[xslant=2,blue] (0,0) -- (1,1) -- (1,0);
  \draw[xslant=-1,red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}


\begin{key}{/tikz/yslant=\meta{factor}}
  Slants the coordinate vertically by the given \meta{factor}:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                (0,0) -- (1,1) -- (1,0);
  \draw[yslant=2,blue] (0,0) -- (1,1) -- (1,0);
  \draw[yslant=-1,red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}


\begin{key}{/tikz/rotate=\meta{degree}}
  Rotates the coordinate system by \meta{degree}:
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                 (0,0) -- (1,1) -- (1,0);
  \draw[rotate=40,blue] (0,0) -- (1,1) -- (1,0);
  \draw[rotate=-20,red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/rotate around={\ttfamily\char`\{}\meta{degree}|:|\meta{coordinate}{\ttfamily\char`\}}}
  Rotates the coordinate system by \meta{degree} around the point
  \meta{coordinate}.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                                (0,0) -- (1,1) -- (1,0);
  \draw[rotate around={40:(1,1)},blue] (0,0) -- (1,1) -- (1,0);
  \draw[rotate around={-20:(1,1)},red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}


\begin{key}{/tikz/cm={\ttfamily\char`\{}\meta{$a$}|,|\meta{$b$}|,|\meta{$c$}|,|\meta{$d$}|,|\meta{coordinate}{\ttfamily\char`\}}}
  applies the following transformation to all coordinates: Let $(x,y)$
  be the coordinate to be transformed and let \meta{coordinate}
  specify the point $(t_x,t_y)$. Then the new coordinate is given by
  $\left(\begin{smallmatrix} a & b \\ c & d\end{smallmatrix}\right)
  \left(\begin{smallmatrix} x \\ y \end{smallmatrix}\right) +
  \left(\begin{smallmatrix} t_x \\ t_y
  \end{smallmatrix}\right)$. Usually, you do not use this option
  directly. 
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                             (0,0) -- (1,1) -- (1,0);
  \draw[cm={1,1,0,1,(0,0)},blue]    (0,0) -- (1,1) -- (1,0);
  \draw[cm={0,1,1,0,(1cm,1cm)},red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/reset cm}
  Completely resets the coordinate transformation matrix to the
  identity matrix. This will destroy not only the transformations
  applied in the current scope, but also all transformations inherited
  from surrounding scopes. Do not use this option, unless you really,
  really know what you are doing.
\end{key}




\subsection{Canvas Transformations}

A \emph{canvas transformation}, see
Section~\ref{section-design-transformations} for details, is best
thought of as a transformation in which the drawing canvas is
stretched or rotated. Imaging writing something on a balloon (the
canvas) and then blowing air into the balloon: Not only does the text
become larger, the thin lines also become larger. In particular, if
you scale the canvas by a factor of two, all lines are twice as
thick.

Canvas transformations should be used with great care. In most
circumstances you do \emph{not} want line widths to change in a
picture as this creates visual inconsistency.

Just as important, when
you use canvas transformations \emph{\pgfname\ looses track of
  positions of nodes and of picture sizes} since it does not take the
effect of canvas transformations into account when it computes
coordinates of nodes (you not, however, rely on this; it may change in
the future).

Finally, not that a canvas transformation always applies to a path as
a whole, it is not possible (as for coordinate transformations) to use
different transformations in different parts of a path.

In short, you should not use canvas transformations unless you really
know what you are doing.

\begin{key}{/tikz/transform canvas=\meta{options}}
  The \meta{options} should contain coordinate transformations options
  like |scale| or |xshift|. Multiple options can be given, their
  effects accumulate in the usual manner. The effect of these
  \meta{options} (immediately) changes the current canvas
  transformation matrix. The coordinate transformation matrix is not
  changed. Tracking of the picture size is (locally) switched off and
  the node coordinate will no longer be correct.
\begin{codeexample}[]
\begin{tikzpicture}
  \draw[help lines] (0,0) grid (3,2);
  \draw                                    (0,0) -- (1,1) -- (1,0);
  \draw[transform canvas={scale=2},blue]   (0,0) -- (1,1) -- (1,0);
  \draw[transform canvas={rotate=180},red] (0,0) -- (1,1) -- (1,0);
\end{tikzpicture}
\end{codeexample}
\end{key}


==> pgfmanual-en-tikz-transparency.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Transparency}

\label{section-tikz-transparency}


\subsection{Overview}

Normally, when you paint something using any of \tikzname's commands
(this includes stroking, filling, shading, patterns, and images), the
newly painted objects totally obscure whatever was painted earlier in
the same area.

You can change this behaviour by using something that can be thought
of as ``(semi)transparent colors.'' Such colors do not completely
obscure the background, rather they blend the background with the new
color. At first sight, using such semitransparent colors might seem quite
straightforward, but the math going on in the background is quite
involved and the correct handling of transparency fills some 64 pages
in the PDF specification. 

In the present section, we start with the different ways of specifying
``how transparent'' newly drawn objects should be. The simplest way is
to just specify a percentage like ``60\% transparent.'' A much more
general way is to use something that I call a \emph{fading,} also
known as a soft mask or a mask.

At the end of the section we adress the problem of creating so-called
\emph{transparency groups}. This problem arises when you paint over a
position several times with a semitransparent color. Sometimes you
want the effect to accumulate, sometimes you do not.

\emph{Note:} Transparency is best supported by the pdf\TeX\
driver. The \textsc{svg} driver also has some support. For PostScript
output, opacity is rendered correctly only with the most recent
versions of GhostScript. Printers and other programs will typically
ignore the opacity setting. 



\subsection{Specifying a Uniform Opacity}

Specifying a stroke and/or fill opacity is quite easy using the
following options.


\begin{key}{/tikz/draw opacity=\meta{value}}
  This option sets ``how transparent'' lines should be. A value of |1|
  means ``fully opaque'' or ``not transparent at all,'' a value of |0|
  means ``fully transparent'' or ``invisible.'' A value of |0.5|
  yields lines that are semitransparent.

  Note that when you use PostScript as your output format,
  this option works only with recent versions of GhostScript.
   
\begin{codeexample}[]
\begin{tikzpicture}[line width=1ex]
  \draw (0,0) -- (3,1);
  \filldraw [fill=examplefill,draw opacity=0.5] (1,0) rectangle (2,1);
\end{tikzpicture}
\end{codeexample}
\end{key}

Note that the |draw opacity| options only sets the opacity of drawn
lines. The opacity of fillings is set using the option
|fill opacity| (documented in Section~\ref{section-fill-opacity}. The
option |opacity| sets both at the same time. 

\begin{key}{/tikz/opacity=\meta{value}}
  Sets both the drawing and filling opacity to \meta{value}.

  The following predefined styles make it easier to use this option:
  \begin{stylekey}{/tikz/transparent}
    Makes everything totally transparent and, hence, invisible.

\begin{codeexample}[]
\tikz{\fill[red]             (0,0)   rectangle (1,0.5);
      \fill[transparent,red] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}

  \begin{stylekey}{/tikz/ultra nearly transparent}
    Makes everything, well, ultra nearly transparent.

\begin{codeexample}[]
\tikz{\fill[red]                      (0,0)   rectangle (1,0.5);
      \fill[ultra nearly transparent] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}

  \begin{stylekey}{/tikz/very nearly transparent}
\begin{codeexample}[]
\tikz{\fill[red]                     (0,0)   rectangle (1,0.5);
      \fill[very nearly transparent] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}

  \begin{stylekey}{/tikz/nearly transparent}
\begin{codeexample}[]
\tikz{\fill[red]                (0,0)   rectangle (1,0.5);
      \fill[nearly transparent] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}

  \begin{stylekey}{/tikz/semitransparent} 
\begin{codeexample}[]
\tikz{\fill[red]             (0,0)   rectangle (1,0.5);
      \fill[semitransparent] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}

  \begin{stylekey}{/tikz/nearly opaque}   
\begin{codeexample}[]
\tikz{\fill[red]           (0,0)   rectangle (1,0.5);
      \fill[nearly opaque] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}
 
  \begin{stylekey}{/tikz/very nearly opaque} 
\begin{codeexample}[]
\tikz{\fill[red]                (0,0)   rectangle (1,0.5);
      \fill[very nearly opaque] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}

  \begin{stylekey}{/tikz/ultra nearly opaque}
\begin{codeexample}[]
\tikz{\fill[red]                 (0,0)   rectangle (1,0.5);
      \fill[ultra nearly opaque] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}

  \begin{stylekey}{/tikz/opaque}
    This yields completely opaque drawings, which is the default.
\begin{codeexample}[]
\tikz{\fill[red]    (0,0)   rectangle (1,0.5);
      \fill[opaque] (0.5,0) rectangle (1.5,0.25); }
\end{codeexample}
  \end{stylekey}
\end{key}


\begin{key}{/tikz/fill opacity=\meta{value}}
  This option sets the opacity of fillings. In addition to filling
  operations, this opacity also applies to text and images.

  Note, again, that when you use PostScript as your output format,
  this option works only with recent versions of GhostScript.
  
\begin{codeexample}[]
\begin{tikzpicture}[thick,fill opacity=0.5]
  \filldraw[fill=red]   (0:1cm)    circle (12mm);
  \filldraw[fill=green] (120:1cm)  circle (12mm);
  \filldraw[fill=blue]  (-120:1cm) circle (12mm);
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \fill[red] (0,0) rectangle (3,2);

  \node                   at (0,0) {\huge A};
  \node[fill opacity=0.5] at (3,2) {\huge B};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/text opacity=\meta{value}}
  Sets the opacity of text labels, overriding the |fill opacity| setting. 
\begin{codeexample}[]
\begin{tikzpicture}[every node/.style={fill,draw}]
  \draw[line width=2mm,blue!50,line cap=round] (0,0) grid (3,2);

  \node[opacity=0.5] at (1.5,2) {Upper node};
  \node[draw opacity=0.8,fill opacity=0.2,text opacity=1]
    at (1.5,0) {Lower node};
\end{tikzpicture}
\end{codeexample}
\end{key}


Note the following effect: If you setup a certain opacity for stroking
or filling and you stroke or fill the same area twice, the effect
accumulates:

\begin{codeexample}[]
\begin{tikzpicture}[fill opacity=0.5]
  \fill[red] (0,0) circle (1);
  \fill[red] (1,0) circle (1);
\end{tikzpicture}
\end{codeexample}

Often, this is exactly what you intend, but not always. You can use
transparency groups, see the end of this section, to change this.


\subsection{Fadings}

For complicated graphics, uniform transparency settings are not always
sufficient. Suppose, for instance, that while you paint a picture, you
want the transparency to vary smoothly from completely opaque to
completely transparent. This is a ``shading-like'' transparency. For
such a form of transparency I will use the term \emph{fading} (as a
noun). They are also known as \emph{soft masks}, \emph{opacity masks},
\emph{masks}, or \emph{soft clips}.


\subsubsection{Creating Fadings}

How do we specify a fading? This is a bit of an art since the
underlying mechanism is quite powerful, but a bit difficult to use.

Let us start with a bit of terminology. A \emph{fading} specifies for
each point of an area to transparency of the point. This transparency
can by any number between 0 and 1. A \emph{fading picture} is a normal
graphic that, in a way to be described in a moment, determines the
transparency of points inside the fading. Each fading has an
underlying fading picture. 

The fading picture is a normal graphic drawn using any of the normal
graphic drawing commands. A fading and its fading picture are related
as follows: Given any point of the fading, the transparency of this
point is determined by the lumonisity of the fading picture at the
same position. The luminosity of a point determines ``how bright'' the
point is. The brighter the point in the fading picture, the more
opaque is the point in the fading. In particular, a white point of the
fading picture is completely opaque in the fading and a black point of
the fading picture is completely transparent in the fading. (The
background of the fading picture is always transparent in the fading
as if the background where black.)

It is rather counter-intuitive that a \emph{white} pixel of the fading
picture will be \emph{opaque} in the fading and a \emph{black} pixel
will be \emph{transparent}. For this reason, \tikzname\ defines a
color called |transparent| that is the same as |black|. The nice thing
about this definition is that the color
|transparent!|\meta{percentage} in the fading picture yields a
pixel that is \meta{percantage} per cent transparent in the fading. 

Turning a fading picture into a normal picture is achieved using the
following commands, which are \emph{only defined in the library},
namely the library |fadings|. So, to use them, you have to say
|\usetikzlibrary{fadings}| first.

\begin{environment}{{tikzfadingfrompicture}\oarg{options}}
  This command works like a |{tikzpicture}|, only the picture is not
  shown, but instead a fading is defined based on this picture. To set
  the name of the picture, use the |name| option (which is normally
  used to set the name of a node).
  \begin{key}{/tikz/name=\marg{name}}
    Use this option with the |{tikzfadingfrompicture}| environment to
    set the name of the fading. You \emph{must} provide this option.
  \end{key}
  
  The following shading is 2cm by 2cm and changes gets more and more
  transparent from left to right, but is 50\% transparent for a large
  circle in the middle.
\begin{codeexample}[]
\begin{tikzfadingfrompicture}[name=fade right]
  \shade[left color=transparent!0,
         right color=transparent!100] (0,0) rectangle (2,2);
  \fill[transparent!50] (1,1) circle (0.7);
\end{tikzfadingfrompicture}

% Now we use the fading in another picture:
\begin{tikzpicture}
  % Background
  \fill [black!20] (-1.2,-1.2) rectangle (1.2,1.2);
  \pattern [pattern=checkerboard,pattern color=black!30]
                   (-1.2,-1.2) rectangle (1.2,1.2);
  
  \fill [path fading=fade right,red] (-1,-1) rectangle (1,1);
\end{tikzpicture}
\end{codeexample}
  In the next example we create a fading picture that contains some
  text. When the fading is used, we only see the shading ``through
  it.'' 
\begin{codeexample}[]
\begin{tikzfadingfrompicture}[name=tikz]
  \node [text=transparent!20]
    {\fontfamily{ptm}\fontsize{45}{45}\bfseries\selectfont Ti\emph{k}Z};
\end{tikzfadingfrompicture}

% Now we use the fading in another picture:
\begin{tikzpicture}
  \fill [black!20] (-2,-1) rectangle (2,1);
  \pattern [pattern=checkerboard,pattern color=black!30]
                   (-2,-1) rectangle (2,1);

  \shade[path fading=tikz,fit fading=false,
         left color=blue,right color=black]
    (-2,-1) rectangle (2,1);
\end{tikzpicture}
\end{codeexample}
\end{environment}

\begin{plainenvironment}{{tikzfadingfrompicture}\oarg{options}}
  The plain\TeX\ version of the environment.
\end{plainenvironment}

\begin{contextenvironment}{{tikzfadingfrompicture}\oarg{options}}
  The Con\TeX t version of the environment.
\end{contextenvironment}

\begin{command}{\tikzfading\oarg{options}}
  This command is used to define a fading similarly to that way a
  shading is defined. In the \meta{options} you should 
  \begin{enumerate}
  \item use the |name=|\meta{name} option to set a name for the fading,
  \item use the |shading| option to set the name of the shading that
    you wish to use,
  \item extra options for setting the colors of the shading (typically
    you will set them to the color |transparent!|\meta{percentage}).
  \end{enumerate}
  Then, a new fading named \meta{name} will be created based on the
  shading.

\begin{codeexample}[]
\tikzfading[name=fade right,
            left color=transparent!0,
            right color=transparent!100]

% Now we use the fading in another picture:
\begin{tikzpicture}
  % Background
  \fill [black!20] (-1.2,-1.2) rectangle (1.2,1.2);
  \path [pattern=checkerboard,pattern color=black!30]
                   (-1.2,-1.2) rectangle (1.2,1.2);

  \fill [red,path fading=fade right] (-1,-1) rectangle (1,1);
\end{tikzpicture}
\end{codeexample}  

\begin{codeexample}[]
\tikzfading[name=fade out,
            inner color=transparent!0,
            outer color=transparent!100]

% Now we use the fading in another picture:
\begin{tikzpicture}
  % Background
  \fill [black!20] (-1.2,-1.2) rectangle (1.2,1.2);
  \path [pattern=checkerboard,pattern color=black!30]
                   (-1.2,-1.2) rectangle (1.2,1.2);

  \fill [blue,path fading=fade out] (-1,-1) rectangle (1,1);
\end{tikzpicture}
\end{codeexample}  
\end{command}



\subsubsection{Fading a Path}

Aa fading specifies for each pixel of a certain area how transparent
this pixel will be. The following options are used to install such a
fading for the current scope or path. 

\pgfdeclarefading{fade down}{%
  \tikzset{top color=pgftransparent!0,bottom color=pgftransparent!100}
  \pgfuseshading{axis}
}
\pgfdeclarefading{fade inside}{%
  \tikzset{inner color=pgftransparent!90,outer color=pgftransparent!30}
  \pgfuseshading{radial}
}

\begin{key}{/tikz/path fading=\meta{name} (default \normalfont scope's setting)}
  This option tells \tikzname\ that the current path should be faded
  with the fading \meta{name}. If no \meta{name} is given, the 
  \meta{name} set for the whole scope is used. Similarly to options
  like |draw| or |fill|, this option is reset for each path, so you
  have to add it to each path that should be faded. You can also
  specify |none| as \meta{name}, in which case fading for the path
  will be switched off in case it has been switched on by previous
  options or styles.
\begin{codeexample}[]
\begin{tikzpicture}[path fading=south]
  % Checker board
  \fill [black!20] (0,0) rectangle (4,3);
  \pattern [pattern=checkerboard,pattern color=black!30]
                   (0,0) rectangle (4,3);

  \fill [color=blue]                   (0.5,1.5) rectangle +(1,1);
  \fill [color=blue,path fading=north] (2.5,1.5) rectangle +(1,1);

  \fill [color=red,path fading]        (1,0.75) ellipse (.75 and .5);
  \fill [color=red]                    (3,0.75) ellipse (.75 and .5);
\end{tikzpicture}
\end{codeexample}

  \begin{key}{/tikz/fit fading=\meta{boolean} (default true, initially true)}
    When set to |true|, the fading is shifted and resized (in exactly
    the same way as a shading) so that is covers the current
    path. When set to |false|, the fading is only shifted so that it
    is centered on the path's center, but it is not resized. This can
    be useful for special-purpose fadings, for instance when you use a
    fading to ``punsh out'' something.
  \end{key}

  \begin{key}{/tikz/fading transform=\meta{transformation options}}
    The \meta{transformation options} are applied to the fading before
    it is used. For instance, if \meta{transformation options} is set
    to |rotate=90|, the fading is rotated by 90 degrees.
\begin{codeexample}[]
\begin{tikzpicture}[path fading=fade down]
  % Checker board
  \fill [black!20] (0,0) rectangle (4,1.5);
  \path [pattern=checkerboard,pattern color=black!30] (0,0) rectangle (4,1.5);

  \fill [red,path fading,fading transform={rotate=90}]
    (1,0.75) ellipse (.75 and .5);
  \fill [red,path fading,fading transform={rotate=30}]
    (3,0.75) ellipse (.75 and .5);
\end{tikzpicture}
\end{codeexample}
  \end{key}
  
  \begin{key}{/tikz/fading angle=\meta{degree}}
    A shortcut for |fading transform={rotate=|\meta{degree}|}|.
  \end{key}

  Note that you can ``fade just about anything.'' In particular, you
  can fade a shading.
  
\begin{codeexample}[]
\begin{tikzpicture}
  % Checker board
  \fill [black!20] (0,0) rectangle (4,4);
  \path [pattern=checkerboard,pattern color=black!30] (0,0) rectangle (4,4);

  \shade [ball color=blue,path fading=south] (2,2) circle (1.8);
\end{tikzpicture}
\end{codeexample}

  The |fade inside| of the following example more transparent in the middle than on the
  outside.

\begin{codeexample}[]
\tikzfading[name=fade inside,
            inner color=transparent!80,
            outer color=transparent!30]    
\begin{tikzpicture}
  % Checker board
  \fill [black!20] (0,0) rectangle (4,4);
  \path [pattern=checkerboard,pattern color=black!30] (0,0) rectangle (4,4);

  \shade [ball color=red] (3,3) circle (0.8);
  \shade [ball color=white,path fading=fade inside] (2,2) circle (1.8);
\end{tikzpicture}
\end{codeexample}

  Note that adding the |path fading| option to a node fades the
  (background) path, not the text itself. To fade the text, you need
  to use a scope fading (see below).
\end{key}

Note that using fadings in conjunction with patterns can create
visually rather pleasing effects:
\begin{codeexample}[]
\tikzfading[name=middle,
            top color=transparent!50,
            bottom color=transparent!50,
            middle color=transparent!20]
\begin{tikzpicture}
  \node      [circle,circular drop shadow,
              pattern=horizontal lines dark blue,
              path fading=south,
              minimum size=3.6cm] {};
  \pattern   [path fading=north,
              pattern=horizontal lines dark gray]
    (0,0) circle (1.8cm);
  \pattern   [path fading=middle,
              pattern=crosshatch dots light steel blue]
    (0,0) circle (1.8cm);
\end{tikzpicture}
\end{codeexample}


\subsubsection{Fading a Scope}

In addtion to fading individual paths, you may also wish to ``fade a
scope,'' that is, you may wish to install a fading that is used
globally to specify the transparency for all objects drawn inside a
scope. This effect can also be thought of as a ``soft clip'' and it
works in a similar way: You add the |scope fading| option to a path in
a scope -- typically the first one -- and then all subsequent drawings
in the scope are faded. You will use a |transparency group| in
conjunction, see the end of this section.

\begin{key}{/tikz/scope fading=\meta{fading}}
  In principle, this key works in excatly the same way as the
  |path fading| key. The only difference is, that the effect of the
  fading will persist after the current path till the end of the
  scope. Thus, the \meta{fading} is applied to all subsequent drawings
  in the current scope, not just to the current path. In this regard,
  the option works very much like the |clip| option. (Note, however,
  that, unlike the |clip| option, fadings to not accumulate unless a
  transparency group is used.)

  The keys |fit fading| and |fading transform| have the same effect as
  for |path fading|. Also that, just as for |path fading|, providing
  the |scope fading| option with a |{scope}| only sets the name of the
  fading to be used. You have to explicitly provide the |scope fading|
  with a path to actually install a fading.
  
\begin{codeexample}[]
\begin{tikzpicture}
  \fill [black!20] (-2,-2) rectangle (2,2);
  \pattern [pattern=checkerboard,pattern color=black!30]
                   (-2,-2) rectangle (2,2);

  % The bounding box of the shading:
  \draw [red] (-50bp,-50bp) rectangle (50bp,50bp);

  \path [scope fading=south,fit fading=false] (0,0);
  % fading is centered at its natural size

  \fill[red]   ( 90:1) circle (1);
  \fill[green] (210:1) circle (1);
  \fill[blue]  (330:1) circle (1);
\end{tikzpicture}
\end{codeexample}

  In the following example we resize the fading to the size of the
  whole picture:
\begin{codeexample}[]
\begin{tikzpicture}
  \fill [black!20] (-2,-2) rectangle (2,2);
  \pattern [pattern=checkerboard,pattern color=black!30]
                   (-2,-2) rectangle (2,2);

  \path [scope fading=south] (-2,-2) rectangle (2,2);

  \fill[red]   ( 90:1) circle (1);
  \fill[green] (210:1) circle (1);
  \fill[blue]  (330:1) circle (1);
\end{tikzpicture}
\end{codeexample}

  Scope fadings are also needed if you wish to fade a node.
\begin{codeexample}[]
\tikz \node [scope fading=south,fading angle=45,text width=3.5cm]
{
  This is some text that will fade out as we go right
  and down. It is pretty hard to achieve this effect in
  other ways.
};    
\end{codeexample}

\end{key}


\subsection{Transparency Groups}

Consider the following cross and sign. They ``look wrong'' because we
can see how they were constructed, while this is not really part of
the desired effect. 

\begin{codeexample}[]
\begin{tikzpicture}[opacity=.5]
  \draw [line width=5mm] (0,0) -- (2,2);
  \draw [line width=5mm] (2,0) -- (0,2);
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \node at (0,0) [forbidden sign,line width=2ex,draw=red,fill=white] {Smoking};

  \node [opacity=.5]
        at (2,0) [forbidden sign,line width=2ex,draw=red,fill=white] {Smoking};
\end{tikzpicture}
\end{codeexample}

Transparency groups are used to render them correctly:

\begin{codeexample}[]
\begin{tikzpicture}[opacity=.5]
  \begin{scope}[transparency group]
    \draw [line width=5mm] (0,0) -- (2,2);
    \draw [line width=5mm] (2,0) -- (0,2);
  \end{scope}
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \node at (0,0) [forbidden sign,line width=2ex,draw=red,fill=white] {Smoking};

  \begin{scope}[opacity=.5,transparency group]
    \node at (2,0) [forbidden sign,line width=2ex,draw=red,fill=white]
      {Smoking};
  \end{scope}
\end{tikzpicture}
\end{codeexample}

\begin{key}{/tikz/transparency group}
  This option can be given to a |scope|. It will have the following
  effect: The scope's contents is stroked/filled
  ``ignoring any outside transparency.'' This means, all previous
  transparency settings are ignored (you can still set transparency
  inside the group, but never mind). For instance, in the forbidden
  sign example, the whole sign is first painted (conceptually) like
  the image on the left hand side. Note that some pixels of the sign
  are painted multiple times (up to three times), but only the last
  color ``wins.''

  Then, when the scope is finished, it is painted as a whole. The  
  \emph{fill} transparency settings are now applied to the resulting
  picutre. For instance, the pixel that has been painted three times
  is just red at the end, so this red color will be blended with
  whatever is ``behind'' the group on the page.

  Note that, depending on the driver, it is possible to directly put
  objects in a transparency group that lie outside the picture. This
  has to do with internal bounding box computations.
  Section~\ref{section-transparency} explains how to sidestep this
  problem.   
\end{key}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual"
%%% End: 


==> pgfmanual-en-tikz-trees.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\section{Making Trees Grow}

\label{section-trees}


\subsection{Introduction to the  Child Operation}

\emph{Trees} are a common way of visualizing hierarchical
structures. A simple tree looks like this:
\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
    child {node {left}}
    child {node {right}
      child {node {child}}
      child {node {child}}
    };
\end{tikzpicture}
\end{codeexample}

Admittedly, in reality trees are more likely to grow \emph{upward} and
not downward as above. You can tell whether the author of a paper is a
mathematician or a computer scientist by looking at the direction
their trees grow. A computer scientist's trees will grow downward
while a mathematician's tree will grow upward. Naturally, the
\emph{correct} way is the mathematician's way, which can be specify as
follows: 
\begin{codeexample}[]
\begin{tikzpicture}
  \node {root} [grow'=up]
    child {node {left}}
    child {node {right}
      child {node {child}}
      child {node {child}}
    };
\end{tikzpicture}
\end{codeexample}

In \tikzname, trees are specified by adding \emph{children} to a
node on a path using the |child| operation:

\begin{pathoperation}{child}{\opt{\oarg{options}}%
    \opt{|foreach|\meta{variables}|in|\marg{values}}\opt{\marg{child path}}} 
  This operation should directly follow a completed |node| operation
  or another |child| operation, although it is permissible that the
  first |child| operation is preceded by options (we will come to
  that).

  When a |node| operation like |node {X}| is followed by |child|,
  \tikzname\ starts counting the number of child nodes that follow the
  original |node {X}|. For this, it scans the input and stores away each
  |child| and its arguments until it reaches a path operation that is
  not a |child|. Note that this will fix the character codes of all
  text inside the child arguments, which means, in essence, that you
  cannot use verbatim text inside the nodes inside a |child|. Sorry. 

  Once the children have been collected and counted, \tikzname\ starts
  generating the child nodes. For each child of a parent node
  \tikzname\ computes an appropriate position where the child is
  placed. For each child, the coordinate system is transformed so that
  the origin is at this position. Then the \meta{child path} is
  drawn. Typically, the child path just consists of a |node|
  specification, which results in a node being drawn at the child's
  position. Finally, an edge is drawn from the first node in the
  \meta{child path} to the parent node.

  The optional |foreach| part (note that there is no backslash before
  |foreach|) allows you to specify multiple children in a single
  |child| command. The idea is the following: A |\foreach| statement
  is (internally) used to iterate over the list of \meta{values}. For
  each value in this list, a new |child| is added to the node. The
  syntax for \meta{variables} and for \meta{values} is the same as for
  the |\foreach| statement, see Section~\ref{section-foreach}. For
  example, when you say 
\begin{codeexample}[code only]
node {root} child [red] foreach \name in {1,2} {node {\name}}
\end{codeexample}
  the effect will be the same as if you had said
\begin{codeexample}[code only]
node {root} child[red] {node {1}} child[ref] {node {2}}
\end{codeexample}
  When you write 
\begin{codeexample}[code only]
node {root} child[\pos] foreach \name/\pos in {1/left,2/right} {node[\pos] {\name}}
\end{codeexample}
  the effect will be the same as for
\begin{codeexample}[code only]
node {root} child[left] {node[left] {1}} child[right] {node[right] {2}}
\end{codeexample}

  You can nest things as in the following example:
\begin{codeexample}[]
\begin{tikzpicture}
  [level distance=4mm,level/.style={sibling distance=8mm/#1}]
  \coordinate
    child foreach \x in {0,1}
      {child foreach \y in {0,1} 
        {child foreach \z in {0,1}}};
\end{tikzpicture}
\end{codeexample}

  The details and options for this operation are described in the rest
  of this present section.
\end{pathoperation}



\subsection{Child Paths and the Child Nodes}

For each |child| of a root node, its \meta{child path} is inserted at
a specific location in the picture (the placement rules are discussed
in Section~\ref{section-tree-placement}). The first node in the
\meta{child path}, if it exists, is special and called the \emph{child
  node}. If there is no first node in the \meta{child path}, that is,
if the \meta{child path} is missing (including the curly braces) or if
it does not start with |node| or with |coordinate|, then an empty
child node of shape |coordinate| is automatically added.

Consider the example |\node {x} child {node {y}} child;|. For the
first child, the \meta{child path} has the child node |node {y}|. For
the second child, no child node is specified and, thus, it is just
|coordinate|.

As for any normal node, you can give the child node a name, shift it 
around, or use options to influence how it is rendered.
\begin{codeexample}[]
\begin{tikzpicture}
  \node[rectangle,draw] {root}
    child {node[circle,draw] (left node) {left}}
    child {node[ellipse,draw] (right node) {right}};
  \draw[dashed,->] (left node) -- (right node);
\end{tikzpicture}
\end{codeexample}

In many cases, the \meta{child path} will just consist of a
specification of a child node and, possibly, children of this child
node. However, the node specification may be followed by arbitrary
other material that will be added to the picture, transformed to the
child's coordinate system. For your convenience, a move-to |(0,0)|
operation is inserted automatically at the beginning of the path. Here
is an example: 

\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
    child {[fill] circle (2pt)}
    child {[fill] circle (2pt)};
\end{tikzpicture}    
\end{codeexample}


At the end of the \meta{child path} you may add a special path
operation called |edge from parent|. If this operation is not given by
yourself somewhere on the path, it will be automatically added at the
end. This option causes a connecting edge from the parent node to the
child node to be added to the path. By giving options to this
operation you can influence how the edge is rendered. Also, nodes
following the |edge from parent| operation will be placed on this
edge, see Section~\ref{section-edge-from-parent} for details.

To sum up:
\begin{enumerate}
\item
  The child path starts with a node specification. If it is not there,
  it is added automatically.
\item
  The child path ends with a |edge from parent| operation, possibly
  followed by nodes to be put on this edge. If the operation is not
  given at the end, it is added automatically.
\end{enumerate}



\subsection{Naming Child Nodes}

Child nodes can be named like any other node using either the |name|
option or the special syntax in which the name of the node is placed
in round parentheses between the |node| operation and the node's
text.

If you do not assign a name to a child node, \tikzname\ will
automatically assign a name as follows: Assume that the name of the
parent node is, say, |parent|. (If you did not assign a
name to the parent, \tikzname\ will do so itself, but that name will
not be user-accessible.) The first child
of |parent| will be named |parent-1|, the second child is named
|parent-2|, and so on.

This naming convention works recursively. If the second child
|parent-2| has children, then the first of these children will be
called |parent-2-1| and the second |parent-2-2| and so on.

If you assign a name to a child node yourself, no name is generated
automatically (the node does not have two names). However, ``counting
continues,'' which means that the third child of |parent| is called
|parent-3| independently of whether you have assigned names to the
first and/or second child of |parent|.

Here is an example:

\begin{codeexample}[]
\begin{tikzpicture}
  \node (root) {root}
    child 
    child {
      child {coordinate (special)}
      child
    };
  \node at (root-1) {root-1};
  \node at (root-2) {root-2};
  \node at (special) {special};
  \node at (root-2-2) {root-2-2};
\end{tikzpicture}
\end{codeexample}

\subsection{Specifying Options for Trees and Children}

Each |child| may have its own \meta{options}, which apply to ``the
whole child,'' including all of its grandchildren. Here is an
example:

\begin{codeexample}[]
\begin{tikzpicture}
  [thick,level 2/.style={sibling distance=10mm}]
  \coordinate
    child[red]   {child child}
    child[green] {child child[blue]};
\end{tikzpicture}
\end{codeexample}

The options of the root node have no effect on the children since
the options of a node are always ``local'' to that node. Because of
this, the edges in the following tree are black, not red.
  
\begin{codeexample}[]
\begin{tikzpicture}[thick]
  \node [red] {root}
    child
    child;
\end{tikzpicture}
\end{codeexample}
  This raises the problem of how to set options for \emph{all}
  children. Naturally, you could always set options for the whole path
  as in |\path [red] node {root} child child;| but this is bothersome
  in some situations. Instead, it is easier to give the options
  \emph{before the first child} as follows:
\begin{codeexample}[]
\begin{tikzpicture}[thick]
  \node [red] {root}
    [green] % option applies to all children
    child
    child;
\end{tikzpicture}
\end{codeexample}

Here is the set of rules:
\begin{enumerate}
\item
  Options for the whole tree are given before the root node.
\item
  Options for the root node are given directly to the |node| operation
  of the root.
\item
  Options for all children can be given between the root node and the
  first child.
\item
  Options applying to a specific child path are given as options to
  the |child| operation.
\item
  Options applying to the node of a child, but not to the whole child
  path, are given as options to the |node| command inside the
  \meta{child path}.
\end{enumerate}

\begin{codeexample}[code only]
\begin{tikzpicture}
  \path
    [...]             % Options apply to the whole tree
    node[...] {root}  % Options apply to the root node only
      [...]           % Options apply to all children
      child[...]      % Options apply to this child and all its children
      {
        node[...] {}  % Options apply to the child node only
        ...
      }
      child[...]      % Options apply to this child and all its children
    ;
\end{tikzpicture}
\end{codeexample}

There are additional styles that influence how children are rendered:
\begin{stylekey}{/tikz/every child (initially \normalfont empty)}
  This style is used at the beginning of each child, as if you had
  given the style's contents as options to the |child| operation.
\end{stylekey}

\begin{stylekey}{/tikz/every child node (initially \normalfont empty)}
  This style is used at the beginning of each child node in addition
  to the |every node| style.
\end{stylekey}

\begin{stylekey}{/tikz/level=\meta{number} (initially \normalfont empty)}
  This style is executed at the beginning of each set of children, where
  \meta{number} is the current level in the current tree. For example,
  when you say |\node {x} child child;|, then |level=1| is
  used before the first |child|. The style or code of this key will be
  passed \meta{number} as its first parameter. If this first |child|
  has children itself, then |level=2| would be used for them.

\begin{codeexample}[]
\begin{tikzpicture}[level/.style={sibling distance=20mm/#1}]
  \node {root}
    child { child child }
    child { child child child };
\end{tikzpicture}
\end{codeexample}
\end{stylekey}

\begin{stylekey}{/tikz/level \meta{number} (initially \normalfont empty)}
  This style is used in addition to the |level| style. So, when you
  say |\node {x} child child;|, then the following key list is
  executed: |level=1,level 1|. 

\begin{codeexample}[]
\begin{tikzpicture}
  [level 1/.style={sibling distance=20mm},
   level 2/.style={sibling distance=5mm}]
  \node {root}
    child { child child }
    child { child child child };
\end{tikzpicture}
\end{codeexample}
\end{stylekey}



\subsection{Placing Child Nodes}

\label{section-tree-placement}

\subsubsection{Basic Idea}

Perhaps the most difficult part in drawing a tree is the correct
layout of the children. Typically, the children have different sizes
and it is not easy to arrange them in such a manner that not too much
space is wasted, the children do not overlap, and they are either 
evenly spaced or their centers are evenly distributed. Calculating
good positions is especially difficult since a good position for the
first child may depend on the size of the last child.

In \tikzname, a comparatively simple approach is taken to placing the
children. In order to compute a child's position, all that is taken
into account is the number of the current child in the list of
children and the number of children in this list. Thus, if a node has
five children, then there is a fixed position for the first child, a
position for the second child, and so on. These positions \emph{do not
  depend on the size of the children} and, hence, children can easily
overlap. However, since you can use options to shift individual
children a bit, this is not as great a problem as it may seem.

Although the placement of the children only depends on their number in
the list of children and the total number of children, everything else
about the placement is highly configurable. You can change the
distance between children (appropriately called the
|sibling distance|) and the distance between levels of the tree. These
distances may change from level to level. The direction in which the
tree grows can be changed globally and for parts of the tree. You can
even specify your own ``growth function'' to arrange children on a
circle or along special lines or curves. 

\subsubsection{Default Growth Function}

The default growth function works as follows: Assume that we are given
a node and five children. These children will be placed on a line with
their centers (or, more generally, with their anchors) spaced apart by
the current |sibling distance|. The line is 
orthogonal to the current \emph{direction of growth}, which is set
with the |grow| and |grow'| option (the latter option reverses the
ordering of the children). The distance from the line to the parent node
is given by the |level distance|.

{\catcode`\|=12
\begin{codeexample}[]
\begin{tikzpicture}
  \path [help lines]
    node (root) {root}
    [grow=-10]
    child {node {1}}
    child {node {2}}
    child {node {3}}
    child {node {4}};

  \draw[|<->|,thick] (root-1.center)
    -- node[above,sloped] {sibling distance} (root-2.center);

  \draw[|<->|,thick] (root.center) 
    -- node[above,sloped] {level distance} +(-10:\tikzleveldistance);
\end{tikzpicture}
\end{codeexample}
}

\begin{key}{/tikz/level distance=\meta{distance} (initially 15mm)}
  This key determines the distance between different levels of the
  tree, more precisely, between the parent and the line 
  on which its children are arranged. When given to a single child,
  this will set the distance for this child only.
 
\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
    [level distance=20mm]
    child
    child {
      [level distance=5mm]
      child
      child
      child
    }
    child[level distance=10mm];  
\end{tikzpicture}
\end{codeexample}
 
\begin{codeexample}[]
\begin{tikzpicture}
  [level 1/.style={level distance=10mm},    
   level 2/.style={level distance=5mm}]    
  \node {root}
    child
    child {
      child
      child[level distance=10mm]
      child
    }
    child;
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/sibling distance=\meta{distance} (initially 15mm)}
  This key specifies the distance between the anchors of the
  children of a parent node.   

\begin{codeexample}[]
\begin{tikzpicture}
  [level distance=4mm,
   level 1/.style={sibling distance=8mm},
   level 2/.style={sibling distance=4mm},
   level 3/.style={sibling distance=2mm}]
  \coordinate
     child {
       child {child child}
       child {child child}
     }
     child {
       child {child child}
       child {child child}
     };
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  [level distance=10mm,
   every node/.style={fill=red!60,circle,inner sep=1pt},
   level 1/.style={sibling distance=20mm,nodes={fill=red!45}},
   level 2/.style={sibling distance=10mm,nodes={fill=red!30}},
   level 3/.style={sibling distance=5mm,nodes={fill=red!25}}]
  \node {31}
     child {node {30}
       child {node {20}
         child {node {5}}
         child {node {4}}
       }
       child {node {10}
         child {node {9}}
         child {node {1}}
       }
     }
     child {node {20}
       child {node {19}
         child {node {1}}
         child[missing]
       }
       child {node {18}}
     };
\end{tikzpicture}
\end{codeexample}
\end{key}  


\begin{key}{/tikz/grow=\meta{direction}}
  This key is used to define the \meta{direction} in which the tree
  will grow. The \meta{direction} can either be an angle in degrees or
  one of the following special text strings: |down|, |up|, |left|,
  |right|, |north|, |south|, |east|, |west|, |north east|,
  |north west|, |south east|, and |south west|. All of these have
  ``their obvious meaning,'' so, say, |south west| is the same as the
  angle $-135^\circ$.

  As a side effect, this option installs the default growth function.

  In addition to setting the direction, this option also has a
  seemingly strange effect: It sets the sibling distance for the
  current level to |0pt|, but leaves the sibling distance for later
  levels unchanged.

  This somewhat strange behaviour has a highly desirable effect: If
  you give this option before the list of children of a node starts,
  the ``current level'' is still the parent level. Each child will be
  on a later level and, hence, the sibling distance will be as
  specified originally. This will cause the children to be neatly
  aligned in a line orthogonal to the given \meta{direction}. However,
  if you give this option locally to a single child, then ``current
  level'' will be the same as the child's level. The zero sibling
  distance will then cause the child to be placed exactly at a point
  at distance |level distance| in the direction
  \meta{direction}. However, the children of the child will be placed
  ``normally'' on a line orthogonal to the \meta{direction}.

  These placement effects are best demonstrated by some examples:
\begin{codeexample}[]
\tikz \node {root} [grow=right] child child;
\end{codeexample}

\begin{codeexample}[]
\tikz \node {root} [grow=south west] child child;
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[level distance=10mm,sibling distance=5mm]
  \node {root}
    [grow=down]
    child
    child
    child[grow=right] {
      child child child
    };  
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}[level distance=2em]
  \node {C}
    child[grow=up]    {node {H}}
    child[grow=left]  {node {H}}
    child[grow=down]  {node {H}}
    child[grow=right] {node {C}
        child[grow=up]    {node {H}}
        child[grow=right] {node {H}}
        child[grow=down]  {node {H}}
      edge from parent[double]
        coordinate (wrong)
    };
  \draw[<-,red] ([yshift=-2mm]wrong) -- +(0,-1)
    node[below]{This is wrong!};  
\end{tikzpicture}
\end{codeexample}

\begin{codeexample}[]
\begin{tikzpicture}
  \node[rectangle,draw] (a) at (0,0) {start node};
  \node[rectangle,draw] (b) at (2,1) {end};

  \draw (a) -- (b)
    node[coordinate,midway] {}
      child[grow=100,<-] {node[above] {the middle is here}};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/grow'=\meta{direction}}
  This key has the same effect as |grow|, only the children are
  arranged in the opposite order.
\end{key}


\subsubsection{Missing Children}

Sometimes one or more of the children of a node are ``missing.'' Such
a missing child will count as a child with respect to the total number
of children and also with respect to the current child count, but it
will not be rendered.

\begin{key}{/tikz/missing=\meta{true or false} (default true)}
  If this option is given to a child, the current child counter is
  increased, but the child is otherwise ignored. In particular, the
  normal contents of the child is completely ignored.

\begin{codeexample}[]
\begin{tikzpicture}[level distance=10mm,sibling distance=5mm]
  \node {root} [grow=down]
    child          { node {1} }
    child          { node {2} }
    child          { node {3} }
    child[missing] { node {4} }
    child          { node {5} }
    child          { node {6} };
\end{tikzpicture}
\end{codeexample}
\end{key}


\subsubsection{Custom Growth Functions}

\begin{key}{/tikz/growth parent anchor=\meta{anchor} (initially center)}
  This key allows you to specify which anchor of the parent node is
  to be used for computing the children's position. For example, when
  there is only one child and the |level distance| is |2cm|, then the
  child node will be placed two centimeters below the \meta{anchor} of
  the parent node. ``Beinng placed'' means that the child node's
  anchor (which is the anchor specified using the |anchor=| option in
  the |node| command of the child) is two centimeters below the parent
  node's \meta{anchor}. 

  In the following example, the two red lines both have length |1cm|.
\begin{codeexample}[]
\begin{tikzpicture}[level distance=1cm]
  \node [rectangle,draw] (a) at (0,0) {root}
  [growth parent anchor=south] child;

  \node [rectangle,draw] (b) at (2,0) {root}
  [growth parent anchor=north east] child;

  \draw [red,thick,dashed] (a.south) -- (a-1);
  \draw [red,thick,dashed] (b.north east) -- (b-1);
\end{tikzpicture}
\end{codeexample}

  In the next example, the top and bottom nodes are aligned at the top
  and the bottom.
\begin{codeexample}[]
\begin{tikzpicture}
  [level distance=2cm,growth parent anchor=north,
   every node/.style={anchor=north,rectangle,draw}    
   every child node/.style={anchor=south}]

  \node at (0,0) {root} child {node {small}};

  \node at (2,0) {big root} child {node {\large big}};
\end{tikzpicture}
\end{codeexample}
\end{key}

\begin{key}{/tikz/growth function=\meta{macro name} (initially
    \normalfont an internal function)}
  This rather low-level option allows you to set a new growth
  function. The \meta{macro name} must be the name of a macro without
  parameters. This macro will be called for each child of a node. The
  initial function is an internal function that corresponds to
  downward growth.

  The effect of executing the macro should be the following: It should
  transform the coordinate system in such a way that the origin
  becomes the place where the current child should be anchored. When
  the macro is called, the current coordinate system will be setup
  such that the anchor of the parent node is in the origin. Thus, in
  each call, the \meta{macro name} must essentially do a shift to the
  child's origin. When the macro is called, the \TeX\ counter
  |\tikznumberofchildren| will be set to the total number of children
  of the parent node and the counter |\tikznumberofcurrentchild| will
  be set to the number of the current child.

  The macro may, in addition to shifting the coordinate system, also
  transform the coordinate system further. For example, it could be
  rotated or scaled.

  Additional growth functions are defined in the library, see 
  Section~\ref{section-tree-library}.
\end{key}



\subsection{Edges From the Parent Node}

\label{section-edge-from-parent}

Every child node is connected to its parent node via a special kind of
edge called the |edge from parent|. This edge is added to the
\meta{child path} when the following path operation is encountered:

\begin{pathoperation}{edge from parent}{\opt{\oarg{options}}}
  This path operation can only be used inside \meta{child paths} and
  should be given at the end, possibly followed by node specifications
  (we will come to that). If a \meta{child path} does not contain this
  operation, it will be added at the end of the \meta{child path}
  automatically.

  This operation has several effects. The most important is that it
  inserts the current ``edge from parent path'' into the child
  path. The edge from parent path can be set using the following
  key:
  \begin{key}{/tikz/edge from parent path=\meta{path} (initially
      \normalfont code shown below)}
    This options allows you to set the edge from parent path to a new
    path. Initially, this path is the following:
\begin{codeexample}[code only]
(\tikzparentnode\tikzparentanchor) -- (\tikzchildnode\tikzchildanchor)      
\end{codeexample}
    The |\tikzparentnode| is a macro that will expand to the name of
    the parent node. This works even when you have not assigned a name
    to the parent node, in this case an internal name is automatically
    generated. The |\tikzchildnode| is a macro that expands to the
    name of the child node. The two |...anchor| macros are empty by
    default. So, what is essentially inserted is just the path segment
    |(\tikzparentnode) -- (\tikzchildnode)|; which is exactly an edge
    from the parent to the child.

    You can modify this edge from parent path to achieve all sorts of
    effects. For example, we could replace the straight line by a
    curve as follows:
\begin{codeexample}[]
\begin{tikzpicture}[edge from parent path=
  {(\tikzparentnode.south) .. controls +(0,-1) and +(0,1)
                           .. (\tikzchildnode.north)}]
  \node {root}
    child {node {left}}
    child {node {right}
      child {node {child}}
      child {node {child}}
    };
\end{tikzpicture}
\end{codeexample}

    Further useful edge from parent paths are defined in the tree
    library, see Section~\ref{section-tree-library}.
  \end{key}

  As said before, the anchors in the default edge from parent path
  are empty. However, you can set them using the following keys:
  \begin{key}{/tikz/child anchor=\meta{anchor} (initially border)}
    Specifies the anchor where the edge from parent meets the child
    node by setting the macro |\tikzchildanchor| to
    |.|\meta{anchor}.
    
    If you specify |border| as the \meta{anchor}, then the macro
    |\tikzchildanchor| is set to the empty string. The effect of
    this is that the edge from the parent will meet the child on the
    border at an automatically calculated position.
\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
    [child anchor=north]
    child {node {left} edge from parent[dashed]}
    child {node {right}
      child {node {child}}
      child {node {child} edge from parent[draw=none]}
    };
\end{tikzpicture}
\end{codeexample}
  \end{key}

  \begin{key}{/tikz/parent anchor=\meta{anchor} (initially border)}
    This option works the same way as the |child anchor|, only for
    the parent.
  \end{key}

  Besides inserting the edge from parent path, the |edge from parent|
  operation has another effect: The \meta{options} are inserted
  directly before the edge from parent path and the following style is
  also installed prior to inserting the path:
  \begin{stylekey}{/tikz/edge from parent (initially draw)}
    This style is inserted right before the edge from parent path and
    before the \meta{options} are inserted. 
\begin{codeexample}[]
\begin{tikzpicture}
  [edge from parent/.style={draw,red,thick}]    
  \node {root}
    child {node {left} edge from parent[dashed]}
    child {node {right}
      child {node {child}}
      child {node {child} edge from parent[draw=none]}
    };
\end{tikzpicture}
\end{codeexample}
  \end{stylekey}

  Note: The \meta{options} inserted before the edge from parent path
  is added \emph{apply to the whole child path}. Thus, it is not
  possible to, say, draw a circle in red as part of the child path and
  then have an edge to parent in blue. However, as always, the child
  node is a node and can be drawn in a totally different way.

  Finally, the |edge from parent| operation has one more effect: It
  causes all nodes \emph{following} the operation to be placed on the
  edge. This is the same effect as if you had added the |pos| option
  to all these nodes, see also Section~\ref{section-pos-option}.

  As an example, consider the following code:
\begin{codeexample}[code only]
\node (root) {} child {node (child) {} edge to parent node {label}};    
\end{codeexample}
  The |edge to parent| operation and the following |node| operation
  will, together, have the same effect as if we had said:
\begin{codeexample}[code only]
(root) -- (child) node [pos=0.5] {label}
\end{codeexample}

  Here is a more complicated example:
\begin{codeexample}[]
\begin{tikzpicture}
  \node {root}
    child {
      node {left}
      edge from parent
        node[left] {a}
        node[right] {b}
    }
    child {
      node {right}
        child {
          node {child}
          edge from parent
            node[left] {c}
        }
        child {node {child}}
      edge from parent
        node[near end] {x}
    };
\end{tikzpicture}
\end{codeexample}

\end{pathoperation}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pgfmanual-pdftex-version"
%%% End: 


==> pgfmanual-en-tutorial-Euclid.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Tutorial: Euclid's Amber Version of the \emph{Elements}}

In this third tutorial we have a look at how \tikzname\ can be used to
draw geometric constructions.

Euclid is currently quite busy writing his new book series, whose
working title is ``Elements'' (Euclid is not quite sure whether this
title will convey the message of the series to future generations
correctly, but he intends to change the title before it goes to the
publisher). Up to know, he wrote down his text and graphics on
papyrus, but his publisher suddenly insists that he must submit in
electronic form. Euclid tries to argue with the publisher that 
electronics will only be discovered thousands of years later, but the
publisher informs him that the use of amber is no longer cutting edge
technology and Euclid will just have to keep up with modern tools.

Slightly disgruntled, Euclid starts converting his papyrus
entitled ``Book I, Proposition I'' to an amber version.  

\subsection{Book I, Proposition I}

The drawing on his papyrus looks like this:\footnote{The text is taken
from the wonderful interactive version of Euclid's Elements by David
E. Joyce, to be found on his website at Clark University.}

\bigskip
\noindent
\begin{tikzpicture}[thick,help lines/.style={thin,draw=black!50}]
  \def\A{\textcolor{input}{$A$}}
  \def\B{\textcolor{input}{$B$}}
  \def\C{\textcolor{output}{$C$}}
  \def\D{$D$}
  \def\E{$E$}
  
  \colorlet{input}{blue!80!black}
  \colorlet{output}{red!70!black}
  \colorlet{triangle}{orange}
  
  \coordinate [label=left:\A]
    (A) at ($ (0,0) + .1*(rand,rand) $);
  \coordinate [label=right:\B]
    (B) at ($ (1.25,0.25) + .1*(rand,rand) $);

  \draw [input] (A) -- (B);
  
  \node [help lines,draw,label=left:\D] (D) at (A) [circle through=(B)] {};
  \node [help lines,draw,label=right:\E] (E) at (B) [circle through=(A)] {};
  
  \coordinate [label=above:\C]
    (C) at (intersection 2 of D and E);

  \draw [output] (A) -- (C);
  \draw [output] (B) -- (C);

  \foreach \point in {A,B,C}
    \fill [black,opacity=.5] (\point) circle (2pt);

  \begin{pgfonlayer}{background}
    \fill[triangle!80] (A) -- (C) -- (B) -- cycle;
  \end{pgfonlayer}
  
  \node [below right,text width=10cm,text justified] at (4,3)
  {
    \small
    \textbf{Proposition I}\par
    \emph{To construct an \textcolor{triangle}{equilateral triangle}
      on a given \textcolor{input}{finite straight line}.}
    \par
    \vskip1em
    Let \A\B\ be the given \textcolor{input}{finite straight line}. It
    is required to construct an \textcolor{triangle}{equilateral
      triangle} on the \textcolor{input}{straight line}~\A\B. 

    Describe the circle \B\C\D\ with center~\A\ and radius \A\B. Again
    describe the circle \A\C\E\ with center~\B\ and radius \B\A. Join the
    \textcolor{output}{straight lines} \C\A\ and \C\B\ from the
    point~\C\ at which the circles cut one another to the points~\A\ and~\B.

    Now, since the point~\A\ is the center of the circle \C\D\B,
    therefore \A\C\ equals \A\B. Again, since the point \B\ is the
    center of the circle \C\A\E, therefore \B\C\ equals \B\A. But
    \A\C\ was proved equal to \A\B, therefore each of the straight
    lines \A\C\ and \B\C\ equals \A\B. And 
    things which equal the same thing also equal one another,
    therefore \A\C\ also equals \B\C. Therefore the three straight
    lines \A\C, \A\B, and \B\C\ equal one another. 
    Therefore the \textcolor{triangle}{triangle} \A\B\C\ is
    equilateral, and it has been  constructed on the given finite
    \textcolor{input}{straight line}~\A\B.  
  };
\end{tikzpicture}
\bigskip

Let us have a look at how Euclid can turn this into \tikzname\ code.

\subsubsection{Setting up the Environment}

As in the previous tutorials, Euclid needs to load \tikzname, together
with some libraries. These libraries are |calc|, |through|, and
|backgrounds|. Depending on which format he uses, Euclid would use one
of the following in the preamble: 

\begin{codeexample}[code only]
% For LaTeX:
\usepackage{tikz}
\usetikzlibrary{calc,through,backgrounds}
\end{codeexample}

\begin{codeexample}[code only]
% For plain TeX:
\input tikz.tex
\usetikzlibrary{calc,through,backgrounds}
\end{codeexample}

\begin{codeexample}[code only]
% For ConTeXt:
\usemodule[tikz]
\usetikzlibrary[calc,through,backgrounds]
\end{codeexample}


\subsubsection{The Line \emph{AB}}

The first part of the picture that Euclid wishes to draw is the line
$AB$. That is easy enough, something like |\draw (0,0) -- (2,1);|
might do. However, Euclid does not wish to reference the two points
$A$ and $B$ as $(0,0)$ and $(2,1)$ subsequently. Rather, he wishes to
just write |A| and |B|. Indeed, the whole point of his book is that
the points $A$ and $B$ can be arbitrary and all other points (like
$C$) are constructed in terms of their positions. It would not do
if Euclid were to write down the coordinates of $C$ explicitly.

So, Euclid starts with defining two coordinates using the
|\coordinate| command:
\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate (A) at (0,0);
  \coordinate (B) at (1.25,0.25);

  \draw[blue] (A) -- (B);
\end{tikzpicture}
\end{codeexample}

That was easy enough. What is missing at this point are the labels for
the coordinates. Euclid does not want them \emph{on} the points, but
next to them. He decides to use the |label| option:
\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:\textcolor{blue}{$A$}]  (A) at (0,0);
  \coordinate [label=right:\textcolor{blue}{$B$}] (B) at (1.25,0.25);

  \draw[blue] (A) -- (B);
\end{tikzpicture}
\end{codeexample}

At this point, Euclid decides that it would be even nicer if the
points $A$ and $B$ were in some sense ``random.'' Then, neither Euclid
nor the reader can make the mistake of taking ``anything for granted''
concerning these position of these points. Euclid is pleased to learn
that there is a |rand| function in \tikzname\ that does exactly what
he needs: It produces a number between $-1$ and $1$. Since \tikzname\
can do a bit of math, Euclid can change the coordinates of the points
as follows:
\begin{codeexample}[code only]
\coordinate [...] (A) at (0+0.1*rand,0+0.1*rand);
\coordinate [...] (B) at (1.25+0.1*rand,0.25+0.1*rand);
\end{codeexample}

This works fine. However, Euclid is not quite satisfied since he would
prefer that the ``main coordinates'' $(0,0)$ and $(1.25,0.25)$ are
``kept separate'' from the perturbation
$0.1(\mathit{rand},\mathit{rand})$. This means, he would like to
specify that coordinate $A$ as ``The point that is at $(0,0)$ plus one
tenth of the vector  $(\mathit{rand},\mathit{rand})$.''

It turns out that the |calc| library allows him to do exactly this
kind of computation. When this library is loaded, you can use special
coordinates that start with |($| and end with |$)| rather than just
|(| and~|)|. Inside these special coordinates you can give a linear
combination of coordinates. (Note that the dollar signs are only
intended to signal that a ``computation'' is going on; no mathematical
typesetting is done.)

The new code for the coordinates is the following:

\begin{codeexample}[code only]
\coordinate [...] (A) at ($ (0,0) + .1*(rand,rand) $);
\coordinate [...] (B) at ($ (1.25,0.25) + .1*(rand,rand) $);
\end{codeexample}

Note that if a coordinate in such a computation has a factor (like
|.1|) you must place a |*| directly before the opening parenthesis of
the coordinate. You can nest such computations.



\subsubsection{The Circle Around \emph{A}}

The first tricky construction is the circle around~$A$. We will see
later how to do this in a very simple manner, but first let us do it
the ``hard'' way.

The idea is the following: We draw a circle around the point $A$ whose
radius is given by the length of the line $AB$. The difficulty lies in
computing the length of this line.

Two ideas ``nearly'' solve this problem: First, we can write
|($ (A) - (B) $)| for the vector that is the difference between $A$
and~$B$. All we need is the length of this vector. Second, given two
numbers $x$ and $y$, one can write |veclen(|$x$|,|$y$|)| inside a
mathematical expression. This gives the value $\sqrt{x^2+y^2}$, which
is exactly the desired length.

The only remaining problem is to access the $x$- and $y$-coordinate of
the vector~$AB$. For this, we need a new concept: the \emph{let
  operation}. A let operation can be given anywhere on a path where a
normal path operation like a line-to or a move-to is expected. The
effect of a let operation is to evaluate some coordinates and to
assign the results to special macros. These macros make it easy to
access the $x$- and $y$-coordinates of the coordinates.

Euclid would write the following:
\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);

  \draw (A) let
              \p1 = ($ (B) - (A) $)
            in
              circle ({veclen(\x1,\y1)});
\end{tikzpicture}
\end{codeexample}

Each assignment in a let operation starts with |\p|, usually followed
by a \meta{digit}. Then comes an equal sign and a coordinate. The
coordinate is evaluated and the result is stored internally. From
then on you can use the following expressions: 
\begin{enumerate}
\item |\x|\meta{digit} yields the $x$-coordinate of the resulting point.
\item |\y|\meta{digit} yields the $y$-coordinate of the resulting
  point.
\item |\p|\meta{digit} yields the same as |\x|\meta{digit}|,\y|\meta{digit}.
\end{enumerate}
You can have multiple assignments in a let operation, just separate
them with commas. In later assignments you can already use the results
of earlier assignments.

Note that |\p1| is not a coordinate in the usual sense. Rather, it
just expands to a string like |10pt,20pt|. So, you cannot write, for
instance, |(\p1.center)| since this would just expand to
|(10pt,20pt.center)|, which makes no sense.

Next, we want to draw both circles at the same time. Each time the
radius is |veclen(\x1,\y1)|. It seems natural to compute this radius
only once. For this, we can also use a let operation: Instead of
writing |\p1 = ...|, we write |\n2 = ...|. Here, ``n'' stands for
``number'' (while ``p'' stands for ``point''). The assignment of a
number should be followed by a number in curly braces.
\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);

  \draw let \p1 = ($ (B) - (A) $),
            \n2 = {veclen(\x1,\y1)}
        in
          (A) circle (\n2)
          (B) circle (\n2);
\end{tikzpicture}
\end{codeexample}
In the above example, you may wonder, what |\n1| would yield? The
answer is that it would be undefined -- the |\p|, |\x|, and |\y|
macros refer to the same logical point, while the |\n| macro has ``its
own namespace.'' We could even have replaced |\n2| in the example by
|\n1| and it would still work. Indeed, the digits following these
macros are just normal \TeX\ parameters. We could also use a longer
name, but then we have to use curly braces:
\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);

  \draw let \p1        = ($ (B) - (A) $),
            \n{radius} = {veclen(\x1,\y1)}
        in
          (A) circle (\n{radius})
          (B) circle (\n{radius});
\end{tikzpicture}
\end{codeexample}

At the beginning of this section it was promised that there is an
easier way to create the desired circle. The trick is to use the
|through| library. As the name suggests, it contains code for creating
shapes that go through a given point.

The option that we are looking for is |circle through|. This option is
given to a \emph{node} and has the following effects: First, it causes
the node's inner and outer separations to be set to zero. Then it sets
the shape of the node to |circle|. Finally, it sets the radius of the
node such that it goes through the parameter given to
|circle through|. This radius is computed in essentially the same way
as above.

\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);

  \node [draw,circle through=(B),label=left:$D$] at (A) {};
\end{tikzpicture}
\end{codeexample}


\subsubsection{The Intersection of the Circles}

Euclid can now draw the line and the circles. The final problem is to
compute the intersection of the two circles. This computation is a bit
involved if you want to do it ``by hand.'' Fortunately, the so-called
intersection coordinate system allows us to specify points as the
intersection of two objects (in order for the following code to work,
the |calc| library must be loaded; it defines the necessary code for
computing the intersection of circles):
\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);

  \node (D) [draw,circle through=(B),label=left:$D$]  at (A) {};
  \node (E) [draw,circle through=(A),label=right:$E$] at (B) {};

  \coordinate [label=above:$C$] (C) at (intersection 2 of D and E);

  \draw [red] (A) -- (C);
  \draw [red] (B) -- (C);
\end{tikzpicture}
\end{codeexample}

We could also have written |intersection 1 of| or just
|intersection of| to get access to the other intersection of the
circles.

Although Euclid does not need it for the current picture, it is just a
small step to computing the bisection of the line $AB$:

\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);

  \node (D) [draw,circle through=(B),label=left:$D$]  at (A) {};
  \node (E) [draw,circle through=(A),label=right:$E$] at (B) {};

  \coordinate [label=above:$C$]  (C)  at (intersection 2 of D and E);
  \coordinate [label=below:$C'$] (C') at (intersection 1 of D and E);

  \draw [red] (C) -- (C');
  \node [fill=red,inner sep=1pt,label=-45:$F$] (F) at (intersection of C--C' and A--B) {};
\end{tikzpicture}
\end{codeexample}



\subsubsection{The Complete Code}

Back to Euclid's code. He introduces a few macros to make life
simpler, like a |\A| macro for typesetting a blue $A$. He also uses the
|background| layer for drawing the triangle behind everything at the
end. 

\begin{codeexample}[]
\begin{tikzpicture}[thick,help lines/.style={thin,draw=black!50}]
  \def\A{\textcolor{input}{$A$}}     \def\B{\textcolor{input}{$B$}}
  \def\C{\textcolor{output}{$C$}}    \def\D{$D$}
  \def\E{$E$}
  
  \colorlet{input}{blue!80!black}    \colorlet{output}{red!70!black}
  \colorlet{triangle}{orange}
  
  \coordinate [label=left:\A]  (A) at ($ (0,0) + .1*(rand,rand) $);
  \coordinate [label=right:\B] (B) at ($ (1.25,0.25) + .1*(rand,rand) $);

  \draw [input] (A) -- (B);
  
  \node [help lines,draw,label=left:\D]   (D) at (A) [circle through=(B)] {};
  \node [help lines,draw,label=right:\E]  (E) at (B) [circle through=(A)] {};
  
  \coordinate [label=above:\C] (C) at (intersection 2 of D and E);

  \draw [output] (A) -- (C) -- (B);

  \foreach \point in {A,B,C}
    \fill [black,opacity=.5] (\point) circle (2pt);

  \begin{pgfonlayer}{background}
    \fill[triangle!80] (A) -- (C) -- (B) -- cycle;
  \end{pgfonlayer}
  
  \node [below right, text width=10cm,text justified] at (4,3) {
    \small\textbf{Proposition I}\par
    \emph{To construct an \textcolor{triangle}{equilateral triangle}
      on a given \textcolor{input}{finite straight line}.}
    \par\vskip1em
    Let \A\B\ be the given \textcolor{input}{finite straight line}.  \dots
  };
\end{tikzpicture}
\end{codeexample}


\subsection{Book I, Proposition II}

The second proposition in the Elements is the following:

\bigskip\noindent
\begin{tikzpicture}[thick,help lines/.style={thin,draw=black!50}]
  \def\A{\textcolor{orange}{$A$}}   \def\B{\textcolor{input}{$B$}}
  \def\C{\textcolor{input}{$C$}}    \def\D{$D$}
  \def\E{$E$}                       \def\F{$F$}
  \def\G{$G$}                       \def\H{$H$}
  \def\K{$K$}                       \def\L{\textcolor{output}{$L$}}
  
  \colorlet{input}{blue!80!black}    \colorlet{output}{red!70!black}
  
  \coordinate [label=left:\A]  (A) at ($ (0,0) + .1*(rand,rand) $);
  \coordinate [label=right:\B] (B) at ($ (1,0.2) + .1*(rand,rand) $);
  \coordinate [label=above:\C] (C) at ($ (1,2) + .1*(rand,rand) $);

  \draw [input] (B) -- (C);
  \draw [help lines] (A) -- (B);

  \coordinate [label=above:\D] (D) at ($ (A)!.5!(B) ! {sin(60)*2} ! 90:(B) $);

  \draw [help lines] (D) -- ($ (D)!3.75!(A) $) coordinate [label=-135:\E] (E);
  \draw [help lines] (D) -- ($ (D)!3.75!(B) $) coordinate [label=-45:\F] (F);

  \node (H) at (B) [help lines,circle through=(C),draw,label=135:\H] {};

  \coordinate [label=right:\G] (G) at (intersection of B--F and H);

  \node (K) at (D) [help lines,circle through=(G),draw,label=135:\K] {};

  \coordinate [label=below:\L] (L) at (intersection of A--E and K);

  \draw [output] (A) -- (L);

  \foreach \point in {A,B,C,D,G,L}
    \fill [black,opacity=.5] (\point) circle (2pt);
  
  \node [below right, text width=9cm,text justified] at (4,4) {
    \small\textbf{Proposition II}\par
    \emph{To place a \textcolor{output}{straight line} equal to a
      given \textcolor{input}{straight line} with 
      one end at a \textcolor{orange}{given point}.} 
    \par\vskip1em
    Let \A\ be the given point, and \B\C\ the given
    \textcolor{input}{straight line}. 
    It is required to place a \textcolor{output}{straight line} equal
    to the given \textcolor{input}{straight line} \B\C\ with one end
    at the point~\A.  

    Join the straight line \A\B\ from the point \A\ to the point \B, and
    construct the equilateral triangle \D\A\B\ on it.
    
    Produce the straight lines \A\E\ and \B\F\ in a straight line with
    \D\A\ and \D\B. Describe the circle \C\G\H\ with center \B\ and
    radius \B\C, and  again, describe the circle \G\K\L\ with center
    \D\ and radius \D\G. 	

    Since the point \B\ is the center of the circle \C\G\H, therefore
    \B\C\ equals \B\G. Again, since the point \D\ is the center of the
    circle \G\K\L, therefore \D\L\ equals \D\G. And in these \D\A\
    equals \D\B, therefore the remainder \A\L\ equals the remainder
    \B\G. But \B\C\ was also proved  equal to \B\G, therefore each of
    the straight lines \A\L\ and \B\C\ equals \B\G. And things which
    equal the same thing also equal one another, therefore \A\L\ also
    equals \B\C. 
    
    Therefore the \textcolor{output}{straight line} \A\L\ equal to the
    given \textcolor{input}{straight line} \B\C\  has been placed with
    one end at the \textcolor{orange}{given point}~\A.  
  };
\end{tikzpicture}




\subsubsection{Using Partway Calculations for the Construction of \emph{D}}

Euclid's construction starts with ``referencing'' Proposition~I for
the construction of the point~$D$. Now, while we could simply repeat the
construction, it seems a bit bothersome that one has to draw all these
circles and do all these complicated constructions.

For this reason, \tikzname\ supports some simplifications. First,
there is a simple syntax for computing a point that is ``partway'' on
a line from $p$ to~$q$: You place these two points in a coordinate
calculation -- remember, they start with |($| and end with |$)| -- and
then combine them using |!|\meta{part}|!|. A \meta{part} of |0| refers
to the \emph{first} coordinate, a \meta{part} of |1| refers to the
second coordinate, and a value in between refers to a point on the
line from $p$ to~$q$. Thus, the syntax is similar to the |xcolor|
syntax for mixing colors.

Here is the computation of the point in the middle of the line $AB$:
\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);
  \node [fill=red,inner sep=1pt,label=below:$X$] (X) at ($ (A)!.5!(B) $) {};
\end{tikzpicture}
\end{codeexample}

The computation of the point $D$ in Euclid's second proposition is a
bit more complicated. It can be expressed as follows: Consider the
line from $X$ to $B$. Suppose we 
rotate this line around $X$ for 90$^\circ$ and then stretch it by a
factor of $\sin(60^\circ)/2$. This yields the desired point~$D$. We
can do the stretching using the partway modifier above, for the
rotation we need a new modifier: the rotation modifier. The idea is
that the second coordinate in a partway computation can be prefixed by
an angle. Then the partway point is computed normally (as if no angle
were given), but the resulting point is rotated by this angle around
the first point.  

\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);
  \node [fill=red,inner sep=1pt,label=below:$X$] (X) at ($ (A)!.5!(B) $) {};
  \node [fill=red,inner sep=1pt,label=above:$D$] (D) at
    ($ (X) ! {sin(60)*2} ! 90:(B) $) {};
  \draw (A) -- (D) -- (B);
\end{tikzpicture}
\end{codeexample}

Finally, it is not necessary to explicitly name the point $X$. Rather,
again like in the |xcolor| package, it is possible to chain partway
modifiers:

\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (1.25,0.25);
  \draw (A) -- (B);
  \node [fill=red,inner sep=1pt,label=above:$D$] (D) at
    ($ (A) ! .5 ! (B) ! {sin(60)*2} ! 90:(B) $) {};
  \draw (A) -- (D) -- (B);
\end{tikzpicture}
\end{codeexample}


\subsubsection{Intersecting a Line and a Circle}

The next step in the construction is to draw a circle around $B$
through $C$, which is easy enough to do using the |circle through|
option. Extending the lines $DA$ and $DB$ can be done using partway
calculations, but this time with a part value outside the range
$[0,1]$: 

\begin{codeexample}[]
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (0.75,0.25);
  \coordinate [label=above:$C$] (C) at (1,1.5);
  \draw (A) -- (B) -- (C);
  \coordinate [label=above:$D$] (D) at
    ($ (A) ! .5 ! (B) ! {sin(60)*2} ! 90:(B) $) {};
  \node (H) [label=135:$H$,draw,circle through=(C)] at (B) {};
  \draw (D) -- ($ (D) ! 3.5 ! (B) $) coordinate [label=below:$F$] (F);
  \draw (D) -- ($ (D) ! 2.5 ! (A) $) coordinate [label=below:$E$] (E);
\end{tikzpicture}
\end{codeexample}

We now face the problem of finding the point $G$, which is the
intersection of the line $BF$ and the circle $H$. One way is to use
yet another variant of the partway computation: Normally, a partway
computation has the form \meta{p}|!|\meta{factor}|!|\meta{q},
resulting in the point $(1-\meta{factor})\meta{p} +
\meta{factor}\meta{q}$. Alternatively, instead of \meta{factor} you
can also use a \meta{dimension} between the points. In this case, you
get the point that is \meta{dimension} removed from \meta{p} on the
straight line to \meta{q}.

We know that the point $G$ is on the way from $B$ to $F$. The distance
is given by the radius of the circle~$H$. Here is the code form
computing $H$:
\begin{codeexample}[pre={
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (0.75,0.25);
  \coordinate [label=above:$C$] (C) at (1,1.5);
  \draw (A) -- (B) -- (C);
  \coordinate [label=above:$D$] (D) at
    ($ (A) ! .5 ! (B) ! {sin(60)*2} ! 90:(B) $) {};
  \node (H) [label=135:$H$,draw,circle through=(C)] at (B) {};
  \draw (D) -- ($ (D) ! 3.5 ! (B) $) coordinate [label=below:$F$] (F);
  \draw (D) -- ($ (D) ! 2.5 ! (A) $) coordinate [label=below:$E$] (E);
},post={\end{tikzpicture}}]
  \path let \p1 = ($ (B) - (C) $) in
    coordinate [label=left:$G$] (G) at ($ (B) ! veclen(\x1,\y1) ! (F) $);
  \fill[red,opacity=.5] (G) circle (2pt);
\end{codeexample}

However, there is a simpler way: As for circles, we can also intersect
a line and a circle using the |intersection| coordinate system:

\begin{codeexample}[pre={
\begin{tikzpicture}
  \coordinate [label=left:$A$]  (A) at (0,0);
  \coordinate [label=right:$B$] (B) at (0.75,0.25);
  \coordinate [label=above:$C$] (C) at (1,1.5);
  \draw (A) -- (B) -- (C);
  \coordinate [label=above:$D$] (D) at
    ($ (A) ! .5 ! (B) ! {sin(60)*2} ! 90:(B) $) {};
  \node (H) [label=135:$H$,draw,circle through=(C)] at (B) {};
  \draw (D) -- ($ (D) ! 3.5 ! (B) $) coordinate [label=below:$F$] (F);
  \draw (D) -- ($ (D) ! 2.5 ! (A) $) coordinate [label=below:$E$] (E);
},post={\end{tikzpicture}}]
  \coordinate [label=left:$G$] (G) at (intersection of B--F and H);
  \fill[red,opacity=.5] (G) circle (2pt);
\end{codeexample}

\subsubsection{The Complete Code}

\begin{codeexample}[]
\begin{tikzpicture}[thick,help lines/.style={thin,draw=black!50}]
  \def\A{\textcolor{orange}{$A$}}   \def\B{\textcolor{input}{$B$}}
  \def\C{\textcolor{input}{$C$}}    \def\D{$D$}
  \def\E{$E$}                       \def\F{$F$}
  \def\G{$G$}                       \def\H{$H$}
  \def\K{$K$}                       \def\L{\textcolor{output}{$L$}}
  
  \colorlet{input}{blue!80!black}    \colorlet{output}{red!70!black}
  
  \coordinate [label=left:\A]  (A) at ($ (0,0) + .1*(rand,rand) $);
  \coordinate [label=right:\B] (B) at ($ (1,0.2) + .1*(rand,rand) $);
  \coordinate [label=above:\C] (C) at ($ (1,2) + .1*(rand,rand) $);

  \draw [input] (B) -- (C);
  \draw [help lines] (A) -- (B);

  \coordinate [label=above:\D] (D) at ($ (A)!.5!(B) ! {sin(60)*2} ! 90:(B) $);

  \draw [help lines] (D) -- ($ (D)!3.75!(A) $) coordinate [label=-135:\E] (E);
  \draw [help lines] (D) -- ($ (D)!3.75!(B) $) coordinate [label=-45:\F] (F);

  \node (H) at (B) [help lines,circle through=(C),draw,label=135:\H] {};

  \coordinate [label=right:\G] (G) at (intersection of B--F and H);

  \node (K) at (D) [help lines,circle through=(G),draw,label=135:\K] {};

  \coordinate [label=below:\L] (L) at (intersection of A--E and K);

  \draw [output] (A) -- (L);

  \foreach \point in {A,B,C,D,G,L}
    \fill [black,opacity=.5] (\point) circle (2pt);

  % \node ...
\end{tikzpicture}
\end{codeexample}

==> pgfmanual-en-tutorial-chains.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Tutorial: Putting a Diagram in Chains}

In this tutorial we have a look at how chains and matrices can be used
to typeset a diagram.

Ilka, who just got tenure for her professorship on Old and
Lovable Programming Languages, has recently dug up a technical report entitled
\emph{The Programming Language Pascal} in the dusty cellar of the
library of her university. Having been created in the good old times
using pens and rules, it looks like this\footnote{The shown diagram was not scanned, but
  rather typeset using \tikzname. The jittering lines were created
  using the |random steps| decoration.}:

\tikzset{
  nonterminal/.style={
    % The shape:
    rectangle,
    % The size:
    minimum size=6mm,
    % The border:
    very thick,           
    draw=red!50!black!50,         % 50% red and 50% black,
                                  % and that mixed with 50% white
    % The filling:
    top color=white,              % a shading that is white at the top...
    bottom color=red!50!black!20, % and something else at the bottom
    % Font
    font=\itshape                 
  },
  terminal/.style={
    % The shape:
    rounded rectangle,
    minimum size=6mm,
    % The rest
    very thick,draw=black!50,
    top color=white,bottom color=black!20,
    font=\ttfamily},
  skip loop/.style={to path={-- ++(0,#1) -| (\tikztotarget)}}
}

{
  \tikzset{terminal/.append style={text height=1.5ex,text depth=.25ex}}
  \tikzset{nonterminal/.append style={text height=1.5ex,text depth=.25ex}}
\medskip
\noindent\begin{tikzpicture}[
  >=latex,thick,
  /pgf/every decoration/.style={/tikz/sharp corners},
  fuzzy/.style={decorate,decoration={random steps,segment length=0.5mm,amplitude=0.15pt}},
  minimum size=6mm,line join=round,line cap=round,
  terminal/.style={rectangle,draw,fill=white,fuzzy,rounded corners=3mm},
  nonterminal/.style={rectangle,draw,fill=white,fuzzy},
  node distance=4mm]

  \ttfamily
  \begin{scope}[start chain,
                every node/.style={on chain},
                terminal/.append style={join=by {->,shorten >=-1pt,fuzzy,decoration={post length=4pt}}},
                nonterminal/.append style={join=by {->,shorten >=-1pt,fuzzy,decoration={post length=4pt}}},
                support/.style={coordinate,join=by fuzzy}]
    \node [support]             (start)        {};
    \node [nonterminal]                        {unsigned integer};
    \node [support]             (after ui)     {};
    \node [terminal]                           {.};
    \node [support]             (after dot)    {};
    \node [terminal]                           {digit};
    \node [support]             (after digit)  {};
    \node [support]             (skip)         {};    
    \node [support]             (before E)     {};
    \node [terminal]                           {E};
    \node [support]             (after E)      {};
    \node [support,xshift=5mm]  (between)      {};
    \node [support,xshift=5mm]  (before last)  {};
    \node [nonterminal]                        {unsigned integer};
    \node [support]             (after last)   {};
    \node [coordinate,join=by ->] (end)          {};
  \end{scope}
  \node (plus)  [terminal,above=of between] {+};
  \node (minus) [terminal,below=of between] {-};

  \begin{scope}[->,decoration={post length=4pt},rounded corners=2mm,every path/.style=fuzzy]
    \draw (after ui)    -- +(0,.7)  -| (skip);
    \draw (after digit) -- +(0,-.7) -| (after dot);
    \draw (before E)    -- +(0,-1.2) -| (after last);
    \draw (after E)     |- (plus);
    \draw (plus)        -| (before last);
    \draw (after E)     |- (minus);
    \draw (minus)       -| (before last);
  \end{scope}
\end{tikzpicture}
\medskip

For her next lecture, Ilka decides to redo this diagram, but this time
perhaps a bit cleaner and perhaps also bit ``cooler.''


\medskip
\noindent\begin{tikzpicture}[point/.style={coordinate},>=stealth',thick,draw=black!50,
                    tip/.style={->,shorten >=1pt},every join/.style={rounded corners},
                    hv path/.style={to path={-| (\tikztotarget)}},
                    vh path/.style={to path={|- (\tikztotarget)}}]
  \matrix[column sep=4mm] {
    % First row:
    & & & & & & &  & & & & \node (plus) [terminal] {+};\\
    % Second row:
    \node (p1) [point]  {}; &    \node (ui1)   [nonterminal] {unsigned integer}; &
    \node (p2) [point]  {}; &    \node (dot)   [terminal]    {.};                &
    \node (p3) [point]  {}; &    \node (digit) [terminal]    {digit};            &
    \node (p4) [point]  {}; &    \node (p5)    [point]  {};                      &
    \node (p6) [point]  {}; &    \node (e)     [terminal]    {E};                &
    \node (p7) [point]  {}; &                                                    &
    \node (p8) [point]  {}; &    \node (ui2)   [nonterminal] {unsigned integer}; &
    \node (p9) [point]  {}; &    \node (p10)   [point]       {};\\
    % Third row:
    & & & & & & &  & & & & \node (minus)[terminal] {-};\\
  };

  { [start chain]
    \chainin (p1);
    \chainin (ui1)   [join=by tip];
    \chainin (p2)    [join];
    \chainin (dot)   [join=by tip];
    \chainin (p3)    [join];
    \chainin (digit) [join=by tip];
    \chainin (p4)    [join];
    { [start branch=digit loop]
      \chainin (p3) [join=by {skip loop=-6mm,tip}];
    }
    \chainin (p5)    [join,join=with p2 by {skip loop=6mm,tip}];
    \chainin (p6)    [join];
    \chainin (e)     [join=by tip];
    \chainin (p7)    [join];
    { [start branch=plus]
      \chainin (plus)  [join=by {vh path,tip}];
      \chainin (p8)    [join=by {hv path,tip}];
    }
    { [start branch=minus]
      \chainin (minus) [join=by {vh path,tip}];
      \chainin (p8)    [join=by {hv path,tip}];
    }
    \chainin (p8)    [join];
    \chainin (ui2)   [join=by tip];
    \chainin (p9)    [join,join=with p6 by {skip loop=-11mm,tip}];
    \chainin (p10)   [join=by tip];
  }
\end{tikzpicture}
}\medskip

Having read the previous tutorials, Ilka knows already how to setup
the environment for her diagram, namely using a |tikzpicture|
environment. She wonders which libraries she will need. She decides
that she will postpone the decision and add the necessary libraries as
needed as she constructs the picture.


\subsection{Styling the Nodes}

The bulk of this tutorial will be about arranging the nodes and
connecting them using chains, but let us start with setting up styles
for the nodes.

There are two kinds of nodes in the diagram, namely what theoreticians
like to call \emph{terminals} and \emph{nonterminals}. For the
terminals, Ilka decides to use a black color, which visually shows
that ``nothing needs to be done about them.'' The nonterminals, which
still need to be ``processed'' further, get a bit of red mixed in.

Ilka starts with the simpler nonterminals, as there are no rounded
corners involved. Naturally, she sets up a style:


\begin{codeexample}[]
\begin{tikzpicture}[
    nonterminal/.style={
      % The shape:
      rectangle,
      % The size:
      minimum size=6mm,
      % The border:
      very thick,           
      draw=red!50!black!50,         % 50% red and 50% black,
                                    % and that mixed with 50% white
      % The filling:
      top color=white,              % a shading that is white at the top...
      bottom color=red!50!black!20, % and something else at the bottom
      % Font
      font=\itshape                 
    }]
  \node [nonterminal] {unsigned integer};
\end{tikzpicture}
\end{codeexample}
Ilka is pretty proud of the use of the |minimum size| option: As the
name suggests, this option ensures that the node is at least 6mm by
6mm, but it will expand in size as necessary to accommodate longer
text. By giving this option to all nodes, they will all have the same
height of 6mm.

Styling the terminals is a bit more difficult because of the round
corners. Ilka has several options how she can achieve them. Once way
is to use the |rounded corners| option. It gets a dimension as
parameter and causes all corners to be replaced by little arcs with
the given dimension as radius. By setting the radius to 3mm, she will
get exactly what she needs: circles, when the shapes are, indeed,
exactly 6mm by 6mm and otherwise half circles on the sides:

\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm,
                    terminal/.style={
                      % The shape:
                      rectangle,minimum size=6mm,rounded corners=3mm,
                      % The rest
                      very thick,draw=black!50,
                      top color=white,bottom color=black!20,
                      font=\ttfamily}]
  \node (dot)   [terminal]                {.};
  \node (digit) [terminal,right=of dot]   {digit};
  \node (E)     [terminal,right=of digit] {E};
\end{tikzpicture}
\end{codeexample}

Another possibility is to use a shape that is specially made for
typesetting rectangles with arcs on the sides (she has to use the
|shapes.misc| library to use it). This shape gives Ilka
much more control over the appearance. For instance, she could have an
arc only on the left side, but she will not need this.
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm,
                    terminal/.style={
                      % The shape:
                      rounded rectangle,
                      minimum size=6mm,
                      % The rest
                      very thick,draw=black!50,
                      top color=white,bottom color=black!20,
                      font=\ttfamily}]
  \node (dot)   [terminal]                {.};
  \node (digit) [terminal,right=of dot]   {digit};
  \node (E)     [terminal,right=of digit] {E};
\end{tikzpicture}
\end{codeexample}
At this point, she notices a problem. The baseline of the text in the
nodes is not aligned:
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm]
  \node (dot)   [terminal]                {.};
  \node (digit) [terminal,right=of dot]   {digit};
  \node (E)     [terminal,right=of digit] {E};

  \draw [help lines] let \p1 = (dot.base),
                         \p2 = (digit.base),
                         \p3 = (E.base)
                     in (-.5,\y1) -- (3.5,\y1)
                        (-.5,\y2) -- (3.5,\y2)
                        (-.5,\y3) -- (3.5,\y3);                     
\end{tikzpicture}
\end{codeexample}
\noindent (Ilka has moved the style definition to the preamble by
saying |\tikzset{terminal/.style=...}|, so that she can use it in all
pictures.)

For the |digit| and the |E| the difference in the baselines is almost
imperceptible, but for the dot the problem is quite severe: It looks
more like a multiplication dot than a period.

Ilka toys with the idea of using the |base right=of...| option rather than
|right=of...| to align the nodes in such a way that the baselines
are all on the same line (the |base right| option places a node
right of something so that the baseline is right of the baseline of
the other object). However, this does not have the desired effect:
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm]
  \node (dot)   [terminal]                {.};
  \node (digit) [terminal,base right=of dot]   {digit};
  \node (E)     [terminal,base right=of digit] {E};
\end{tikzpicture}
\end{codeexample}
The nodes suddenly ``dance around''! There is no hope of changing the
position of text inside a node using anchors. Instead, Ilka must use a
trick: The problem of mismatching baselines is caused by the fact that
|.| and |digit| and |E| all have different heights and depth. If they
all had the same, they would all be positioned vertically in the same
manner. So, all Ilka needs to do is to use the |text height| and
|text depth| options to explicitly specify a height and depth for the
nodes.
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm,
                    text height=1.5ex,text depth=.25ex]
  \node (dot)   [terminal]                {.};
  \node (digit) [terminal,right=of dot]   {digit};
  \node (E)     [terminal,right=of digit] {E};
\end{tikzpicture}
\end{codeexample}



\subsection{Aligning  the Nodes Using Positioning Options}

Ilka now has the ``styling'' of the nodes ready. The next problem is
to place them in the right places. There are several ways to do
this. The most straightforward is to simply explicitly place the nodes
at certain coordinates ``calculated by hand.'' For very simple
graphics this is perfectly alright, but it has several disadvantages:
\begin{enumerate}
\item For more difficult graphics, the calculation may become
  complicated.
\item Changing the text of the nodes may make it necessary to
  recalculate the coordinates.
\item The source code of the graphic is not very clear since the
  relationships between the positions of the nodes are not made
  explicit. 
\end{enumerate}

For these reasons, Ilka decides to try out different ways of arranging
the nodes on the page.

The first method is the use of \emph{positioning options}. To use
them, you need to load the |positioning| library. This gives you
access to advanced implementations of options like |above| or |left|,
since you can now say |above=of some node| in order to place a node
above of |some node|, with the borders separated by |node distance|.

Ilka can use this to draw the place the nodes in a long row:
\tikzset{terminal/.append style={text height=1.5ex,text depth=.25ex}}
\tikzset{nonterminal/.append style={text height=1.5ex,text
    depth=.25ex}}
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm and 5mm]
  \node (ui1)   [nonterminal]                     {unsigned integer};
  \node (dot)   [terminal,right=of ui1]           {.};
  \node (digit) [terminal,right=of dot]           {digit};
  \node (E)     [terminal,right=of digit]         {E};
  \node (plus)  [terminal,above right=of E]       {+};
  \node (minus) [terminal,below right=of E]       {-};
  \node (ui2)   [nonterminal,below right=of plus] {unsigned integer};
\end{tikzpicture}
\end{codeexample}

For the plus and minus nodes, Ilka is a bit startled by their
placements. Shouldn't they be more to the right? The reason they are
placed in that manner is the following: The |north east| anchor of the
|E| node lies at the ``upper start of the right arc,'' which, a bit
unfortunately in this case, happens to be the top of the
node. Likewise, the |south west| anchor of the |+| node is actually at
its bottom and, indeed, the horizontal and vertical distances between
the top of the |E| node and the bottom of the |+| node are both 5mm.

There are several ways of fixing this problem. The
easiest way is to simply add a little bit of horizontal shift by hand:
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm and 5mm]
  \node (E)     [terminal]                                   {E};
  \node (plus)  [terminal,above right=of E,xshift=5mm]       {+};
  \node (minus) [terminal,below right=of E,xshift=5mm]       {-};
  \node (ui2)   [nonterminal,below right=of plus,xshift=5mm] {unsigned integer};
\end{tikzpicture}
\end{codeexample}

A second way is to revert back to the idea of using a normal rectangle
for the terminals, but with rounded corners. Since corner rounding
does not affect anchors, she gets the following result:
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm and 5mm,terminal/.append style={rectangle,rounded corners=3mm}]
  \node (E)     [terminal]                        {E};
  \node (plus)  [terminal,above right=of E]       {+};
  \node (minus) [terminal,below right=of E]       {-};
  \node (ui2)   [nonterminal,below right=of plus] {unsigned integer};
\end{tikzpicture}
\end{codeexample}
A third way is to use matrices, which we will do later.
 
Now that the nodes have been placed, Ilka needs to add
connections. Here, some connections are more difficult than
other. Consider for instance the ``repeat'' line around the
|digit|. One way of describing this line is to say ``it starts a
little to the right of |digit| than goes down and then goes to the
left and finally ends at a point a little to the left of |digit|.''
Ilka can put this into code as follows:
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm and 5mm]
  \node (dot)   [terminal]                        {.};
  \node (digit) [terminal,right=of dot]           {digit};
  \node (E)     [terminal,right=of digit]         {E};

  \path (dot)   edge[->] (digit)  % simple edges
        (digit) edge[->] (E);

  \draw [->]
     % start right of digit.east, that is, at the point that is the
     % linear combination of digit.east and the vector (2mm,0pt). We
     % use the ($ ... $) notation for computing linear combinations
     ($ (digit.east) + (2mm,0) $)  
     % Now go down
     -- ++(0,-.5)
     % And back to the left of digit.west
     -| ($ (digit.west) - (2mm,0) $);
\end{tikzpicture}
\end{codeexample}

Since Ilka needs this ``go up/down then horizontally and than up/down
to a target'' several times, it seems sensible to define a special
\emph{to-path} for this. Whenever the |edge| command is used, it
simply adds the current value of |to path| to the path. So, Ilka can
setup a style that contains the correct path:
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm and 5mm,
    skip loop/.style={to path={-- ++(0,-.5) -| (\tikztotarget)}}]
  \node (dot)   [terminal]                        {.};
  \node (digit) [terminal,right=of dot]           {digit};
  \node (E)     [terminal,right=of digit]         {E};

  \path (dot)   edge[->]           (digit)  % simple edges
        (digit) edge[->]           (E)
        ($ (digit.east) + (2mm,0) $)
                edge[->,skip loop] ($ (digit.west) - (2mm,0) $);
\end{tikzpicture}
\end{codeexample}

Ilka can even go a step further and make her |skip look| style
parametrized. For this, the skip loop's vertical offset is passed as
parameter |#1|. Also, in the following code Ilka specifies the start
and targets differently, namely as the positions that are ``in the
middle between the nodes.''
\begin{codeexample}[]
\begin{tikzpicture}[node distance=5mm and 5mm,
    skip loop/.style={to path={-- ++(0,#1) -| (\tikztotarget)}}]
  \node (dot)   [terminal]                        {.};
  \node (digit) [terminal,right=of dot]           {digit};
  \node (E)     [terminal,right=of digit]         {E};

  \path (dot)   edge[->]                (digit)  % simple edges
        (digit) edge[->]                (E)
        ($ (digit.east)!.5!(E.west) $)
                edge[->,skip loop=-5mm] ($ (digit.west)!.5!(dot.east) $);
\end{tikzpicture}
\end{codeexample}


\subsection{Aligning  the Nodes Using Matrices}

Ilka is still bothered a bit by the placement of the plus and minus
nodes. Somehow, having to add an explicit |xshift| seems too much like
cheating.

A perhaps better way of positioning the nodes is to use a
\emph{matrix}. In \tikzname\ matrices can be used to align quite
arbitrary graphical objects in rows and columns. The syntax is very
similar to the use of arrays and tables in \TeX\ (indeed, internally
\TeX\ tables are used, but a lot of stuff is going on additionally).

In Ilka's graphic, there will be three rows: One row containing only
the plus node, one row containing the main nodes and one row
containing only the minus node.
\begin{codeexample}[]
\begin{tikzpicture}
  \matrix[row sep=1mm,column sep=5mm] {
    % First row:
      & & & & \node [terminal] {+}; & \\
    % Second row:
    \node [nonterminal] {unsigned integer}; &
    \node [terminal]    {.};                &
    \node [terminal]    {digit};            &
    \node [terminal]    {E};                &
                                            &
    \node [nonterminal] {unsigned integer}; \\
    % Third row:
      & & & & \node [terminal] {-}; & \\    
  };
\end{tikzpicture}
\end{codeexample}
That was easy! By toying around with the row and columns separations,
Ilka can achieve all sorts of pleasing arrangements of the nodes.

Ilka now faces the same connecting problem as before. This time, she
has an idea: She adds small nodes (they will be turned into
coordinates later on and be invisible) at all the places
where she would like connections to start and end.
\begin{codeexample}[]
\begin{tikzpicture}[point/.style={circle,inner sep=0pt,minimum size=2pt,fill=red},
                   skip loop/.style={to path={-- ++(0,#1) -| (\tikztotarget)}}]
  \matrix[row sep=1mm,column sep=2mm] {
    % First row:
    & & & & & & &  & & & & \node [terminal] {+};\\
    % Second row:
    \node (p1) [point]  {};                 &    \node [nonterminal] {unsigned integer}; &
    \node (p2) [point]  {};                 &    \node [terminal]    {.};                &
    \node (p3) [point]  {};                 &    \node [terminal]    {digit};            &
    \node (p4) [point]  {};                 &    \node (p5) [point]  {};                 &
    \node (p6) [point]  {};                 &    \node [terminal]    {E};                &
    \node (p7) [point]  {};                 &                                            &
    \node (p8) [point]  {};                 &    \node [nonterminal] {unsigned integer}; &
    \node (p9) [point]  {};                 \\
    % Third row:
    & & & & & & &  & & & & \node [terminal] {-};\\
  };

  \path (p4) edge [->,skip loop=-5mm] (p3)
        (p2) edge [->,skip loop=5mm]  (p6);
\end{tikzpicture}
\end{codeexample}
Now, its only a small step to add all the missing edges.



\subsection{Using Chains}

Matrices allow Ilka to align the nodes nicely, but the connections are
not quite perfect. The problem is that the code does not really
reflect the paths that underlie the diagram.


For this reason, Ilka decides to try out \emph{chains} by including
the |chain| library. Basically, a chain is just a sequence of
(usually) connected nodes. The nodes can already have been constructed
or they can be constructed as the chain is constructed (or these
processes can be mixed).

\subsubsection{Creating a Simple Chain}


Ilka starts with creating a chain from scratch. For this, she starts a
chain using the |start chain| option in a scope. Then, inside the
scope, she uses the |on chain| option on nodes to add them to the
chain.
\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm]
  \node [on chain,nonterminal]  {unsigned integer};
  \node [on chain,terminal]     {.};
  \node [on chain,terminal]     {digit};
  \node [on chain,terminal]     {E};
  \node [on chain,nonterminal]  {unsigned integer};
\end{tikzpicture}
\end{codeexample}
(Ilka will add the plus and minus nodes later.)

As can be seen, the nodes of a chain are placed in a row. This can be
changed, for instance by saying |start chain=going below| we get a
chain where each node is below the previous one.

The next step is to \emph{join} the nodes of the chain. For this, we
add the |join| option to each node. This joins the node with the
previous node (for the first node nothing happens).
\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm]
  \node [on chain,join,nonterminal]  {unsigned integer};
  \node [on chain,join,terminal]     {.};
  \node [on chain,join,terminal]     {digit};
  \node [on chain,join,terminal]     {E};
  \node [on chain,join,nonterminal]  {unsigned integer};
\end{tikzpicture}
\end{codeexample}
In order to get a arrow tip, we redefine the |every join| style. Also,
we move the |join| and |on chain| options to the |every node|
style so that we do not have to repeat them so often.
\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm, every node/.style={on chain,join}, every join/.style={->}]
  \node [nonterminal]  {unsigned integer};
  \node [terminal]     {.};
  \node [terminal]     {digit};
  \node [terminal]     {E};
  \node [nonterminal]  {unsigned integer};
\end{tikzpicture}
\end{codeexample}


\subsubsection{Branching and Joining a Chain}

It is now time to add the plus and minus signs. They obviously
\emph{branch off} the main chain. For this reason, we start a branch
for them using the |start branch| option.
\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm, every node/.style={on chain,join}, every join/.style={->}]
  \node [nonterminal]  {unsigned integer};
  \node [terminal]     {.};
  \node [terminal]     {digit};
  \node [terminal]     {E};
  \begin{scope}[start branch=plus]
    \node (plus)  [terminal,on chain=going above right] {+};
  \end{scope}
  \begin{scope}[start branch=minus]
    \node (minus) [terminal,on chain=going below right] {-};
  \end{scope}
  \node [nonterminal,join=with plus,join=with minus]  {unsigned integer};
\end{tikzpicture}
\end{codeexample}

Let us see, what is going on here. First, the |start branch| begins a
branch, starting with the node last created on the current chain,
which is the |E| node in our case. This is implicitly also the first
node on this branch. A branch is nothing different from a chain, which
is why the plus node is put on this branch using the |on chain|
option. However, this time we specify the placement of the node
explicitly using |going |\meta{direction}. This causes the plus sign
to be placed above and right of the |E| node. It is automatically
joined to its predecessor on the branch by the implicit |join|
option.

When the first branch ends, only the plus node has been added and the
current chain is the original chain once more and we are back to the
|E| node. Now we start a new branch for the minus node. After this
branch, the current chain ens at |E| node once more.

Finally, the rightmost unsigned integer is added to the (main) chain,
which is why it is joined correctly with the |E| node. The two
additional |join| options get a special |with| parameter. This allows
you to join a node with a node other than the predecessor on the
chain. The  |with| should be followed by the name of a node.

Since Ilka will need scopes more often in the following, she includes
the |scopes| library. This allows her to replace |\begin{scope}|
  simply by an opening brace and  |\end{scope}| by the corresponding
closing brace. Also, in the following example we reference
the nodes |plus| and |minus| using
their automatic name: The $i$th node on a chain is called
|chain-|\meta{i}. For a branch \meta{branch}, the $i$th node is called
|chain/|\meta{branch}|-|\meta{i}. The \meta{i} can be replaced by
|begin| and |end| to reference the first and (currently) last node on
the chain.

\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm, every on chain/.style={join}, every join/.style={->}]
  \node [on chain,nonterminal]  {unsigned integer};
  \node [on chain,terminal]     {.};
  \node [on chain,terminal]     {digit};
  \node [on chain,terminal]     {E};
  { [start branch=plus]
    \node (plus)  [terminal,on chain=going above right] {+};
  }
  { [start branch=minus]
    \node (minus) [terminal,on chain=going below right] {-};
  }
  \node [nonterminal,on chain,join=with chain/plus-end,join=with chain/minus-end]  {unsigned integer};
\end{tikzpicture}
\end{codeexample}


The next step is to add intermediate coordinate nodes in the same
manner as Ilka did for the matrix. For them, we change the |join|
style slightly, namely for these nodes we do not want an arrow
tip. This can be achieved either by (locally) changing the
|every join| style or, which is what is done in the below example, by
giving the desired style using |join=by ...|, where |...| is the style
to be used for the join.

\begin{codeexample}[]
\begin{tikzpicture}[start chain,node distance=5mm and 2mm,
                    every node/.style={on chain},    
                    nonterminal/.append style={join=by ->},    
                    terminal/.append style={join=by ->},    
                    point/.style={join=by -,circle,fill=red,minimum size=2pt,inner sep=0pt}]
  \node [point] {};  \node [nonterminal] {unsigned integer};
  \node [point] {};  \node [terminal]    {.};
  \node [point] {};  \node [terminal]    {digit};
  \node [point] {};  \node [point]       {};
  \node [point] {};  \node [terminal]    {E};
  \node [point] {};
  { [node distance=5mm and 1cm] % local change in horizontal distance
    { [start branch=plus]
      \node (plus)  [terminal,on chain=going above right] {+};
    }
    { [start branch=minus]
      \node (minus) [terminal,on chain=going below right] {-};
    }
    \node [point,below right=of plus,join=with chain/plus-end by ->,join=with chain/minus-end by ->] {};
  }
  \node [nonterminal] {unsigned integer};
  \node [point]       {};
\end{tikzpicture}
\end{codeexample}


\subsubsection{Chaining Together Already Positioned Nodes}

The final step is to add the missing arrows. We can also use branches
for them (even though we do not have to, but it is good practice and
they exhibit the structure of the diagram in the code).

Let us start with the repeat loop around the |digit|. This can be
thought of as a branch that starts at the point after the digit and
that ends at the point before the digit. However, we have already
constructed the point before the digit! In such cases, it is possible
to ``chain in'' an already positioned node, using the |\chainin|
command. This command must be followed by a coordinate that contains a
node name and optionally some options. The effect is that the named
node is made part of the current chain.

\begin{codeexample}[pre={\tikzset{node distance=5mm and 2mm,
                    every node/.style={on chain},    
                    terminal/.append style={join=by ->},    
                    point/.style={join=by -,circle,fill=red,minimum size=2pt,inner sep=0pt}}}]
\begin{tikzpicture}[start chain] % plus some styles that are not shown
  \node                [point] {};
  \node (before digit) [point] {};
  \node                [terminal]    {digit};
  \node                [point] {};
  { [start branch=digit loop]
    \chainin (before digit) [join=by {->,skip loop=-5mm}];
  }
  \node                [point] {};
\end{tikzpicture}
\end{codeexample}


\subsubsection{Combined Use of Matrices and Chains}

Ilka's final idea is to combine matrices and chains in the following
manner: She will use a matrix to position the nodes. However, to show
the logical ``flow structure'' inside the diagram, she will create
chains and branches that show what is going on.

Ilka starts with the matrix we had earlier, only with slightly adapted
styles. Then she writes down the main chain and its branches:

\begin{codeexample}[]
\begin{tikzpicture}[point/.style={coordinate},>=stealth',thick,draw=black!50,
                    tip/.style={->,shorten >=1pt},every join/.style={rounded corners},
                    hv path/.style={to path={-| (\tikztotarget)}},
                    vh path/.style={to path={|- (\tikztotarget)}}]
  \matrix[column sep=4mm] {
    % First row:
    & & & & & & &  & & & & \node (plus) [terminal] {+};\\
    % Second row:
    \node (p1) [point]  {}; &    \node (ui1)   [nonterminal] {unsigned integer}; &
    \node (p2) [point]  {}; &    \node (dot)   [terminal]    {.};                &
    \node (p3) [point]  {}; &    \node (digit) [terminal]    {digit};            &
    \node (p4) [point]  {}; &    \node (p5)    [point]  {};                      &
    \node (p6) [point]  {}; &    \node (e)     [terminal]    {E};                &
    \node (p7) [point]  {}; &                                                    &
    \node (p8) [point]  {}; &    \node (ui2)   [nonterminal] {unsigned integer}; &
    \node (p9) [point]  {}; &    \node (p10)   [point]       {};\\
    % Third row:
    & & & & & & &  & & & & \node (minus)[terminal] {-};\\
  };

  { [start chain]
    \chainin (p1);
    \chainin (ui1)   [join=by tip];
    \chainin (p2)    [join];
    \chainin (dot)   [join=by tip];
    \chainin (p3)    [join];
    \chainin (digit) [join=by tip];
    \chainin (p4)    [join];
    { [start branch=digit loop]
      \chainin (p3) [join=by {skip loop=-6mm,tip}];
    }
    \chainin (p5)    [join,join=with p2 by {skip loop=6mm,tip}];
    \chainin (p6)    [join];
    \chainin (e)     [join=by tip];
    \chainin (p7)    [join];
    { [start branch=plus]
      \chainin (plus)  [join=by {vh path,tip}];
      \chainin (p8)    [join=by {hv path,tip}];
    }
    { [start branch=minus]
      \chainin (minus) [join=by {vh path,tip}];
      \chainin (p8)    [join=by {hv path,tip}];
    }
    \chainin (p8)    [join];
    \chainin (ui2)   [join=by tip];
    \chainin (p9)    [join,join=with p6 by {skip loop=-11mm,tip}];
    \chainin (p10)   [join=by tip];
  }
\end{tikzpicture}
\end{codeexample}


==> pgfmanual-en-xxcolor.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Free Documentation License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\section{Extended Color Support}

This section documents the package \texttt{xxcolor}, which is
currently distributed as part of \pgfname. This package extends the
\texttt{xcolor} package, written by Uwe Kern, which in turn extends
the \texttt{color} package. I hope that the commands in
\texttt{xxcolor} will some day migrate to \texttt{xcolor}, such that
this package becomes superfluous.

The main aim of the \texttt{xxcolor} package is to provide an
environment inside which all colors are ``washed out'' or ``dimmed.''
This is useful in numerous situations and must typically be achieved
in a roundabout manner if such an environment is not available.

\begin{environment}{{colormixin}\marg{mix-in specification}}
  The mix-in specification is applied to all colors inside
  the environment. At the beginning of the environment, the mix-in is
  applied to the current color, i.\,e., the color that was in effect
  before the environment started. A mix-in specification is a number
  between 0 and 100 followed by an exclamation mark and a color
  name. When a |\color| command is 
  encountered inside a mix-in environment, the number states what
  percentage of the desired color should be used. The rest is
  ``filled up'' with the color given in the mix-in
  specification. Thus, a mix-in specification like |90!blue|
  will mix in 10\% of blue into everything, whereas |25!white| will
  make everything nearly white.

\begin{codeexample}[width=4cm]
\begin{minipage}{3.5cm}\raggedright
\color{red}Red text,%
\begin{colormixin}{25!white}
  washed-out red text,
  \color{blue} washed-out blue text,
  \begin{colormixin}{25!black}
    dark washed-out blue text,
    \color{green} dark washed-out green text,%
  \end{colormixin}
  back to washed-out blue text,%
\end{colormixin}
and back to red.
\end{minipage}%
\end{codeexample}
\end{environment}

Note that the environment only changes colors that have been installed
using the standard \LaTeX\ |\color| command. In particular,
the colors in images are not changed. There is, however, some support
offered by the commands |\pgfuseimage| and
|\pgfuseshading|. If the first command is invoked 
inside a |colormixin| environment with the parameter, say,
|50!black| on an image with the name |foo|, the command
will first check whether there is also a defined image with the name
|foo.!50!black|. If so, this image is used instead. This allows
you to provide a different image for this case. If you nest
|colormixin| environments, the different mix-ins are all appended. For
example, inside the inner environment of 
the above example, |\pgfuseimage{foo}| would first check whether
there exists an image named |foo.!50!white!25!black|.

\begin{command}{\colorcurrentmixin}
  Expands to the current accumulated mix-in. Each nesting of a
  |colormixin| adds a mix-in to this list.
\begin{codeexample}[]
\begin{minipage}{\linewidth-6pt}\raggedright
\begin{colormixin}{75!white}
  \colorcurrentmixin\ should be ``!75!white''\par
  \begin{colormixin}{75!black}
    \colorcurrentmixin\ should be ``!75!black!75!white''\par
    \begin{colormixin}{50!white}
      \colorcurrentmixin\ should be ``!50!white!75!black!75!white''\par
    \end{colormixin}
  \end{colormixin}
\end{colormixin}
\end{minipage}
\end{codeexample}
\end{command}






==> pgfmath.code.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\input pgfmathcalc.code.tex

==> pgfmath.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\ifx\pgfmathincluded\undefined
\def\pgfmathincluded{}

\edef\pgfmathatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfsys.tex
\input pgfmath.code.tex
\catcode`\@=\pgfmathatcode

\fi

\endinput


==> pgfmathbase.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.
%
% This file provides basic macros for converting between bases.
%
% Version 1.414213 29/9/2007

% \pgfmathbasetodec
%
% Convert a representation of an integer from 
% the spcified base to base 10.
%
% #1 - a macro to store the result.
% #2 - the representation of a number (i.e. not a register)
% #3 - the current base.
%
% e.g.
%
% \pgfmathbasetodec\mynumber{10111}{2}
%
% \mynumber <- 23
%
\def\pgfmathbasetodec#1#2#3{%
	\pgfmath@checknumber{#2}%
	\pgfmath@checkbase{#3}%
	\def\pgfmath@base{#3}%
	\def\pgfmath@macro{#1}%
	\c@pgfmath@counta1\relax%
	\def\pgfmath@reversed{}%
	\expandafter\pgfmathbasetodec@#2\pgfmathbasetodec}
	
\def\pgfmathbasetodec@#1{%
	\ifx\pgfmathbasetodec#1%
		\c@pgfmath@countb0%
		\divide\c@pgfmath@counta by\pgfmath@base\relax%
		\expandafter\pgfmathbasetodec@@%
	\else%
		\edef\pgfmath@reversed{\pgfmath@reversed#1}%
		\expandafter\multiply\expandafter\c@pgfmath@counta\pgfmath@base\relax%
		\expandafter\pgfmathbasetodec@%
	\fi}

\def\pgfmathbasetodec@@{\expandafter\pgfmathbasetodec@@@\pgfmath@reversed\pgfmathbasetodec}
	
\def\pgfmathbasetodec@@@#1{%
	\ifx\pgfmathbasetodec#1\relax%
		\expandafter\edef\pgfmath@macro{\the\c@pgfmath@countb}%
		\let\pgfmath@next\pgfmathbasetodec@@@@%
	\else%
		\chardef\pgfmath@charnum`#1\relax%
		\c@pgfmath@countc\pgfmath@charnum%
		\ifnum\c@pgfmath@countc>96\relax%
			\advance\c@pgfmath@countc-87\relax%
		\else
			\ifnum\c@pgfmath@countc>64\relax%
				\advance\c@pgfmath@countc-55\relax%
			\else
				\advance\c@pgfmath@countc-48\relax%
		\fi\fi%
		\ifnum\c@pgfmath@countc<\pgfmath@base\relax%
			\multiply\c@pgfmath@countc\c@pgfmath@counta\relax%
			\advance\c@pgfmath@countb\c@pgfmath@countc%
			\divide\c@pgfmath@counta by\pgfmath@base\relax%
			\let\pgfmath@next\pgfmathbasetodec@@@%
		\else
			\pgfmath@error{Digit `#1' invalid for base \pgfmath@base}%
			\let\pgfmath@next\relax%
		\fi%	
	\fi%
	\pgfmath@next}
\def\pgfmathbasetodec@@@@{%
	\expandafter\pgfmath@ensurenumberlength\expandafter{\pgfmath@macro}%
}

% \pgfmathdectobase
%
% Convert a representation of an integer from 
% base 10 to the spcified base. Letters for bases
% greater than 10 are in lowercase.
%
% #1 - a macro to store the result.
% #2 - a number in base 10 (in a macro, not a register)
% #3 - the required base.
%
% e.g.
%
% \pgfmathdectobase\mynumber{127}{16}
%
% \mynumber <- 7f
%
\def\pgfmathdectobase#1#2#3{%
	\pgfmath@checknumber{#2}%
	\pgfmath@checkbase{#3}%
	\c@pgfmath@counta#2\relax%
	\def#1{}%
	\pgfmathloop
		\ifnum\c@pgfmath@counta>0\relax%
			\c@pgfmath@countb\c@pgfmath@counta%
			\divide\c@pgfmath@countb#3\relax%
			\multiply\c@pgfmath@countb-#3\relax%
			\advance\c@pgfmath@countb\c@pgfmath@counta%
			\edef#1{\csname pgfmath@lowercase digit@\the\c@pgfmath@countb\endcsname#1}%
			\divide\c@pgfmath@counta#3\relax%
	\repeatpgfmathloop%
	\pgfmath@ensurenumberlength{#1}}

% \pgfmathdectoBase
%
% Convert a representation of an integer from 
% base 10 to the spcified base. Letters for bases
% greater than 10 are in uppercase.
%
% #1 - a macro to store the result.
% #2 - a number in base 10 (in a macro, not a register)
% #3 - the required base.
%
% e.g.
%
% \pgfmathdectoBase\mynumber{127}{16}
%
% \mynumber <- 7F
%	
\def\pgfmathdectoBase#1#2#3{%
	\pgfmath@checkbase{#3}%
	\pgfmath@checknumber{#2}%
	\c@pgfmath@counta#2\relax%
	\def#1{}%
	\pgfmathloop
		\ifnum\c@pgfmath@counta>0\relax%
			\c@pgfmath@countb\c@pgfmath@counta%
			\divide\c@pgfmath@countb#3\relax%
			\multiply\c@pgfmath@countb-#3\relax%
			\advance\c@pgfmath@countb\c@pgfmath@counta%
			\edef#1{\csname pgfmath@uppercase digit@\the\c@pgfmath@countb\endcsname#1}%
			\divide\c@pgfmath@counta#3\relax%
	\repeatpgfmathloop%
	\pgfmath@ensurenumberlength{#1}}

\def\pgfmath@createdigits{%
	\def\pgfmath@digitstyle{lowercase digit}%
	\c@pgfmath@counta0\relax%
	\pgfmath@createdigits@0123456789abcdefghijklmnopqrstuvwxyz\pgfmath@createdigits%
	\def\pgfmath@digitstyle{uppercase digit}%
	\c@pgfmath@counta0\relax%
	\pgfmath@createdigits@0123456789ABCDEFGHIJKLMNOPQRSTUVWXYZ\pgfmath@createdigits}

\def\pgfmath@createdigits@#1{%
	\ifx\pgfmath@createdigits#1\relax%
	\else%
		\expandafter\pgfmath@def\expandafter{\pgfmath@digitstyle}{\the\c@pgfmath@counta}{#1}%
		\advance\c@pgfmath@counta1\relax%
		\expandafter\pgfmath@createdigits@%
	\fi}
\pgfmath@createdigits

% \pgfmathbasetobase
%
% Convert a representation of an integer from 
% between the specified bases. Letters for target
% bases greater than 10 are in lppercase.
%
% #1 - a macro to store the result.
% #2 - a number (in a macro, not a register)
% #3 - the source base.
% #4 - the target base.
%
% e.g.
%
% \pgfmathbasetobase\mynumber{4321}{5}{9}
%
% \mynumber <- 721
%	
\def\pgfmathbasetobase#1#2#3#4{%
	\pgfmathbasetodec{\pgfmath@temp}{#2}{#3}%
	\pgfmathdectobase{#1}{\pgfmath@temp}{#4}
}

% \pgfmathbasetobase
%
% Convert a representation of an integer from 
% between the specified bases. Letters for target
% bases greater than 10 are in uppercase.
%
% #1 - a macro to store the result.
% #2 - a number (in a macro, not a register)
% #3 - the source base.
% #4 - the target base.
%
% e.g.
%
% \pgfmathbasetobase\mynumber{1234}{5}{12}
%
% \mynumber <- 142
%	
\def\pgfmathbasetoBase#1#2#3#4{%
	\pgfmathbasetodec{\pgfmath@temp}{#2}{#3}%
	\pgfmathdectoBase{#1}{\pgfmath@temp}{#4}
}

\def\pgfmath@checkbase#1{%
	\ifnum#1<2\relax%
		\pgfmath@error{Cannot process numbers in base `#1'.}%
	\else%
		\ifnum#1>36\relax%
			\pgfmath@error{Cannot process numbers in base `#1'.}%
	\fi\fi}
	
\def\pgfmath@checknumber#1{%
	\expandafter\pgfmath@checknumber@#1\pgfmath@}
\def\pgfmath@checknumber@#1#2\pgfmath@{%
	\ifx#1-%
		\pgfmath@error{Cannot process negative numbers.}%
	\fi}

% \pgfmath@ensurenumberlength
%
% Internal macro for making a representation of a number have
% a specific length, byt prefixing zeros to the number.
%
% #1 - a macro contatining a representation of an integer.
% #2 - the number of digits to ensure.
%
% e.g.
%
% \foo <- 7FF
%
% \pgfmathsetnumberlength{8}%
% \pgfmath@ensurenumberlength\foo
%
% \foo <- 000007FF
%
\def\pgfmath@ensurenumberlength#1{%
	\def\pgfmath@tempa{#1}%
	\expandafter\c@pgfmath@counta\pgfmath@basenumberlength\relax%
	\expandafter\pgfmath@ensurenumberlength@#1\pgfmath@ensurenumberlength}
\def\pgfmath@ensurenumberlength@#1{%
	\ifx\pgfmath@ensurenumberlength#1\relax%
		\expandafter\pgfmath@ensurenumberlength@@%
	\else%
		\advance\c@pgfmath@counta-1\relax%
		\expandafter\pgfmath@ensurenumberlength@
	\fi}

\def\pgfmath@ensurenumberlength@@{%
	\edef\pgfmath@tempb{\pgfmath@tempa}%
	\pgfmath@ensurenumberlength@@@}
\def\pgfmath@ensurenumberlength@@@{%
	\ifnum\c@pgfmath@counta>0\relax%
		\advance\c@pgfmath@counta-1\relax%
		\edef\pgfmath@tempb{0\pgfmath@tempb}%
		\expandafter\pgfmath@ensurenumberlength@@@%
	\fi%
	\expandafter\edef\pgfmath@tempa{\pgfmath@tempb}}
	
\def\pgfmathsetbasenumberlength#1{\def\pgfmath@basenumberlength{#1}}
\pgfmathsetbasenumberlength{1}%

==> pgfmathcalc.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file loads all the parsing, functions and operator stuff
%
% Version 1.414213 29/9/2007

\input pgfmathutil.code.tex
\input pgfmathparser.code.tex
\input pgfmathoperations.code.tex
\input pgfmathbase.code.tex

% \pgfmathsetlength, \pgfmathaddtolength
%
% #1 = dimension register
% #2 = expression
%
% Description:
%
% These functions work similar to \setlength and \addtolength. Only,
% they allow #2 to contain an expression, which is evaluated before
% assignment. Furthermore, the font is setup before the assignment is
% done, so that dimensions like 1em are evaluated correctly.
%
% If #2 starts with "+", then a simple assignment is done (but the
% font is still setup). This is orders of magnitude faster than a
% parsed assignment.

\def\pgfmathsetlength#1#2{%
	\expandafter\pgfmath@onquick#2\pgfmath@%
	{%
		% Ok, quick version:
		\begingroup%
			\pgfmath@selectfont%
			\pgfmath@x#2\unskip%
			\pgfmath@returnone\pgfmath@x%
		\endgroup%
		#1\pgfmathresult pt\relax%
	}%
	{%
		\pgfmathparse{#2}%
		#1\pgfmathresult pt\relax%
	}%
	\ignorespaces%
}

% \pgfmathaddtolength
%
% Add to #1 the result of evaluating #2.
%
% #1 - a dimension register
% #2 - an expression
%
\def\pgfmathaddtolength#1#2{%
	\expandafter\pgfmath@onquick#2\pgfmath@%
  {%
  	\begingroup%
  		\pgfmath@selectfont%
  		\pgfmath@x#1\relax%
  		\advance\pgfmath@x#2\unskip%
  		\pgfmath@returnone\pgfmath@x%
    \endgroup%
    #1\pgfmathresult pt\relax%
  }%
  {%
  	\pgfmathparse{#2}%
  	\advance#1\pgfmathresult pt\relax%
  }%
  \ignorespaces%
}

% \pgfmathsetcount
%
% Assign #1 the truncated evaluation of #2.
%
% #1 - a count register
% #2 - an expression
%
\def\pgfmathsetcount#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    #1#2\relax%
  }%
  {%
    \pgfmathparse{#2}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1\pgfmathresult\relax\pgfmath@%
  }%
  \ignorespaces%
}

% \pgfmathaddtocount
%
% Add to #1 the truncated evaluation of #2.
%
% #1 - a count register
% #2 - an expression
%
\def\pgfmathaddtocount#1#2{%
  \expandafter\pgfmath@onquick#2\pgfmath@%
  {%
    \advance#1#2\relax%
  }%
  {%
    \edef\pgfmath@addtocounttemp{\the#1}%
    \pgfmathparse{#2}%
    \afterassignment\pgfmath@gobbletilpgfmath@%
    #1\pgfmathresult\relax\pgfmath@%
    \advance#1\pgfmath@addtocounttemp\relax%
  }%
  \ignorespaces%
}

% \pgfmathnewcounter
%
% LaTeX style counter which also works in plain TeX. Defines
% \c@<name> as a count register and also defines \the<name>.
%
% #1 the name of the counter.
%
% Example:
%
% \pgfmathnewcounter{counter}
% \pgfmathsetcounter{counter}{12}
% \thecounter  (same as \the\c@counter)
%
\def\pgfmathnewcounter#1{%
	\expandafter\ifx\csname c@#1\endcsname\relax%
		\def\pgfmath@marshal{\csname newcount\endcsname}% Ha! Who cares about \outer?
		\expandafter\pgfmath@marshal\csname c@#1\endcsname%
		\expandafter\def\csname the#1\endcsname{\expandafter\the\csname c@#1\endcsname}%
	\fi%
}

% \pgfmathsetcounter
%
% Set the counter #1 to the evaluation of #2.
%
% #1 - a counter name
% #2 - an expression
%
\def\pgfmathsetcounter#1#2{%
 	\expandafter\pgfmathsetcount\csname c@#1\endcsname{#2}%
}

% \pgfmathaddtocounter
%
% Add the counter #1 to the evaluation of #2.
%
% #1 - a counter name
% #2 - an expression
%
\def\pgfmathaddtocounter#1#2{%
  \expandafter\pgfmathaddtocount\csname c@#1\endcsname{#2}%
}

% \pgfmathmakecounterglobal
%
% Make the current value of a counter globally defined.
%
% #1 - a (valid) counter name.
%
\def\pgfmath@pgftext{pgf}
\def\pgfmath@tikztext{tikz}
\def\pgfmathmakecounterglobal#1{%
	\pgfmath@ifundefined{c@#1}{}{%
		\expandafter\pgfmath@in@\expandafter{\pgfmath@pgftext}{#1}%
		\ifpgfmath@in@%
		\else%
			\expandafter\pgfmath@in@\expandafter{\pgfmath@tikztext}{#1}%
			\ifpgfmath@in@%
			\else%
				\expandafter\global\csname c@#1\endcsname\csname c@#1\endcsname\relax%
			\fi%
		\fi%
	}%
}

% \pgfmathsetmacro
%
% \edef#1 as the result of evaluating #2.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathsetmacro#1#2{%
	\begingroup%
		\pgfmathsetlength\pgfmath@x{#2}%
		\edef#1{\pgfmath@tonumber{\pgfmath@x}}%
		\pgfmath@smuggleone{#1}%
	\endgroup%
}

% \pgfmathsetlengthmacro
%
% \edef#1 as the result of evaluating #2 with pt.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathsetlengthmacro#1#2{%
	\begingroup%
		\pgfmathsetlength\pgfmath@x{#2}%
		\edef#1{\the\pgfmath@x}%
		\pgfmath@smuggleone{#1}%
	\endgroup%
}

% \pgfmathtruncatemacro
%
% \edef#1 as the truncated result of evaluating #2.
%
% #1 - a macro
% #2 - an expression
%
\def\pgfmathtruncatemacro#1#2{%
	\begingroup%
		\pgfmathsetcount\c@pgfmath@counta{#2}%
		\edef#1{\the\c@pgfmath@counta}%
		\pgfmath@smuggleone{#1}%
	\endgroup%
}

% Check whether a given parameter starts with quick.
%
% The command should be followed by nonempty text, ending with
% \pgfmath@ as a stop-token. Then should follow
%
% #1 - code to execute if text starts with +
% #2 - code to execute if text does not
%
% Example:
%
% \pgfmath@onquick+0pt\pgfmath@{is quick}{is slow}

\def\pgfmath@onquick{%
  \afterassignment\pgfmath@afterquick%
  \let\pgfmath@next=%
}

\def\pgfmath@afterquick#1\pgfmath@{%
  \ifx\pgfmath@next+%
    \expandafter\pgfmath@firstoftwo%
  \else%
    \expandafter\pgfmath@secondoftwo%
  \fi%
}

==> pgfmathoperations.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the mathematical functions and operators.
%
% Version 1.414213 29/9/2007

% This file defines the mathematical functions and operators.
%
% Adding/redefining extra operators/functions:
%
% Each operator/function XXX has two forms:
%
%
% \pgfmathXXX#1...   a public version which evaluates any
%                    arguments passed to it and passes the
%                    results on to...
%
% \pgfmathXXX@#1...  a non-public version which performs 
%                    required calculation on arguments which
%                    must have already been evaluated (i.e.
%                    *without* dimensions).
% 
% If a function XXX is to be included in the parser, it is 
% recommended, for consistency, that where possible, the 
% pgfmathparser file should define the macro \pgfmath@parseXXX.
% The parser should (ideally) then call \pgfmathXXX@.
%
% It is also recommened that all calculations (where necessary)
% take place within a TeX group. \pgfmath@returnone#1 makes and
% expanded version of #1 global and stores this in \pgfmathresult 
% after the group is ended.
%

\input pgfmathtrig.code.tex% Load the trig. stuff.
\input pgfmathrnd.code.tex%  Load the random stuff.


% \pgfmathadd
%
% Add #1 and #2.
%
\def\pgfmathadd#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathadd@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathadd@#1#2{%
  \begingroup%
    \pgfmath@x#1pt%
    \pgfmath@y#2pt%
    \advance\pgfmath@x by\pgfmath@y%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathsubtract
%
% Subtract #2 from #1.
%
\def\pgfmathsubtract#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathsubtract@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathsubtract@#1#2{%
  \begingroup%
    \pgfmath@x#1pt%
    \pgfmath@y#2pt%
    \advance\pgfmath@x-\pgfmath@y%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathmultiply
%
% Multiply #1 by #2.
%
\def\pgfmathmultiply#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathmultiply@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathmultiply@#1#2{%
  \begingroup%
    \pgfmath@x#1pt%
    \pgfmath@y#2pt%
    \pgfmath@x\pgfmath@tonumber{\pgfmath@y}\pgfmath@x%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathdivide
%
% Divide #1 by #2.
%
\def\pgfmathdivide#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathdivide@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathdivide@#1#2{%
  \begingroup%
    \pgfmath@x#1pt%
    \pgfmath@y#2pt%
    \def\pgfmath@sign{}%
		\ifdim\pgfmath@y=0pt\relax%
			\pgfmath@error{You've asked me to divide `#1' by `#2', %
				but I cannot divide any number by `#2'}%				
		\fi%
		\afterassignment\pgfmath@xa%
		\expandafter\c@pgfmath@counta\the\pgfmath@y\relax%
		%
		% If y is an integer, use TeX arithmatic.
		%
		\ifdim\pgfmath@xa=0pt\relax%
			\divide\pgfmath@x\c@pgfmath@counta\relax%
			\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
			\let\pgfmath@next\pgfmathdivide@@@%
		\else%
			%
			% Simple long division.
			%
			\ifdim\pgfmath@x<0pt\relax%
				\def\pgfmath@sign{-}%
				\pgfmath@x-\pgfmath@x%
			\fi%
			\ifdim\pgfmath@y<0pt\relax%
				\edef\pgfmath@sign{\pgfmath@sign-}%
				\pgfmath@y-\pgfmath@y%
			\fi%
			\pgfmath@ya\pgfmath@y%
			\c@pgfmath@counta0\relax%
			\ifdim\pgfmath@x>\pgfmath@ya%
				\ifdim\pgfmath@ya<1638.4pt\relax%
					\pgfmathmultiply@dimenbyten\pgfmath@ya%
					\ifdim\pgfmath@ya>\pgfmath@x%
						\pgfmathdivide@dimenbyten\pgfmath@ya%
						\c@pgfmath@counta0\relax%
					\else%
						\ifdim\pgfmath@ya<1638.4pt\relax%
							\pgfmathmultiply@dimenbyten\pgfmath@ya%
							\ifdim\pgfmath@ya>\pgfmath@x%
								\pgfmathdivide@dimenbyten\pgfmath@ya%
								\c@pgfmath@counta1\relax%
							\else%
								\ifdim\pgfmath@ya<1638.4pt\relax%
									\pgfmathmultiply@dimenbyten\pgfmath@ya%
									\ifdim\pgfmath@ya>\pgfmath@x%
										\pgfmathdivide@dimenbyten\pgfmath@ya%
										\c@pgfmath@counta2\relax%
									\else%
										\ifdim\pgfmath@ya<1638.4pt\relax%
											\pgfmathmultiply@dimenbyten\pgfmath@ya%
											\ifdim\pgfmath@ya>\pgfmath@x%
												\pgfmathdivide@dimenbyten\pgfmath@ya%
												\c@pgfmath@counta3\relax%
											\else%
												\pgfmath@error{The result of `#1/#2' is too big for me}{}%
											\fi%
										\fi%
									\fi%
								\fi%
							\fi%
						\fi%
					\fi%
				\fi%
			\fi%
			%
			% If y < 1pt use reciprocal operation.
			%
			\ifdim\pgfmath@y<1pt\relax%
				\ifdim\pgfmath@y<.00007pt\relax%
					\pgfmath@error{The result of `#1/#2' is too big for me}{}%
				\fi%
				\pgfmathreciprocal@{\pgfmath@tonumber{\pgfmath@y}}%
				\pgfmath@x\pgfmathresult\pgfmath@x%
				\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@x}}%
				\let\pgfmath@next\pgfmathdivide@@@%
			\else%
				\pgfmath@y\pgfmath@ya%
				\def\pgfmathresult{}%
				\let\pgfmath@next\pgfmathdivide@@%
			\fi%
		\fi%
		\pgfmath@next%
}

\def\pgfmathdivide@dimenbyten#1{%
	\edef\pgfmath@temp{\pgfmath@tonumber{#1}}%
	\expandafter\pgfmathdivide@@dimenbyten\pgfmath@temp\@@#1\@@}
\def\pgfmathdivide@@dimenbyten#1.#2\@@#3\@@{%
	\pgfmath@tempcnta#1\relax%
	\divide\pgfmath@tempcnta10\relax%
	\pgfmath@tempcntb\pgfmath@tempcnta%
	\multiply\pgfmath@tempcnta-10\relax%
	\advance\pgfmath@tempcnta#1\relax%
	#3\the\pgfmath@tempcntb.\the\pgfmath@tempcnta#2pt\relax%
}

\def\pgfmathmultiply@dimenbyten#1{%
	\edef\pgfmath@temp{\pgfmath@tonumber{#1}}%
	\expandafter\pgfmathmultiply@@dimenbyten\pgfmath@temp\@@#1\@@}
\def\pgfmathmultiply@@dimenbyten#1.#2#3\@@#4\@@{#4#1#2.#3pt\relax}

\def\pgfmathdivide@@{%
		\ifdim\pgfmath@x>\pgfmath@y%
			\pgfmath@yb6.0\pgfmath@y%
			\ifdim\pgfmath@yb>\pgfmath@x% 6*y
				\advance\pgfmath@yb-\pgfmath@y%
				\advance\pgfmath@yb-\pgfmath@y%
				\ifdim\pgfmath@yb>\pgfmath@x% 4*y
					\advance\pgfmath@yb-\pgfmath@y%
					\advance\pgfmath@yb-\pgfmath@y%
					\ifdim\pgfmath@yb>\pgfmath@x% 2*y
						\advance\pgfmath@yb-\pgfmath@y%
						\ifdim\pgfmath@yb>\pgfmath@x% 1*y
							\c@pgfmath@countb0\relax%
						\else%
							\c@pgfmath@countb1\relax%
						\fi%
					\else%
						\advance\pgfmath@yb\pgfmath@y% 3*y
						\ifdim\pgfmath@yb>\pgfmath@x%
							\c@pgfmath@countb2\relax%
						\else%
							\c@pgfmath@countb3\relax%
						\fi%
					\fi%
				\else%
					\advance\pgfmath@yb\pgfmath@y% 5*y
					\ifdim\pgfmath@yb>\pgfmath@x%
						\c@pgfmath@countb4\relax%
					\else%
						\c@pgfmath@countb5\relax%
					\fi%
				\fi%
			\else%
				\advance\pgfmath@yb\pgfmath@y%
				\advance\pgfmath@yb\pgfmath@y%
				\ifdim\pgfmath@yb>\pgfmath@x% 8*y
					\advance\pgfmath@yb-\pgfmath@y%
					\ifdim\pgfmath@yb>\pgfmath@x% 7*y
						\c@pgfmath@countb6\relax%
					\else%
						\c@pgfmath@countb7\relax%
					\fi%
				\else%
					\advance\pgfmath@yb\pgfmath@y%
					\ifdim\pgfmath@yb>\pgfmath@x% 9*y
						\c@pgfmath@countb8\relax%
					\else%
						\c@pgfmath@countb9\relax%
					\fi%
				\fi%
			\fi%	
		\else%
			\c@pgfmath@countb=0\relax%
		\fi%
		\ifnum\c@pgfmath@countb=0\relax%
			\edef\pgfmathresult{\pgfmathresult0}%
		\else%
			\pgfmath@yb\c@pgfmath@countb\pgfmath@y%
			\advance\pgfmath@x-\pgfmath@yb%	
			\edef\pgfmathresult{\pgfmathresult\the\c@pgfmath@countb}%	
		\fi%
		\pgfmathdivide@dimenbyten\pgfmath@y%
		\ifnum\c@pgfmath@counta=0\relax%
			\edef\pgfmathresult{\pgfmathresult.}%
		\fi%
		\advance\c@pgfmath@counta-1\relax%
		\ifdim\pgfmath@y=0pt\relax%
			\let\pgfmath@next\pgfmathdivide@@@%
		\else%
			\let\pgfmath@next\pgfmathdivide@@%
		\fi%
		\pgfmath@next%
}
		
\def\pgfmathdivide@@@{%
		\pgfmath@x\pgfmath@sign\pgfmathresult pt\relax%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}


% \pgfmathgreaterthan
%
% 1.0 if #1 > #2. Otherwise 0.0
%
\def\pgfmathgreaterthan#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathgreaterthan@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathgreaterthan@#1#2{%
  \begingroup%
    \pgfmath@x#1pt%
    \pgfmath@y#2pt%
    \advance\pgfmath@x-\pgfmath@y%
    \ifdim\pgfmath@x>0pt\relax%
      \pgfmath@x1pt\relax%
    \else%
      \pgfmath@x0pt\relax%
    \fi%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathlessthan
%
% 1.0 if #1< #2. Otherwise 0.0
%
\def\pgfmathlessthan#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathlessthan@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathlessthan@#1#2{%
  \begingroup%
    \pgfmath@x#1pt%
    \pgfmath@y#2pt%
    \advance\pgfmath@x-\pgfmath@y\relax%
    \ifdim\pgfmath@x<0pt\relax%
      \pgfmath@x1pt\relax%
    \else%
      \pgfmath@x0pt\relax%
    \fi%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathequalto
%
% 1.0 if #1 = #2. Otherwise 0.0
%
\def\pgfmathequalto#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathequalto@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathequalto@#1#2{%
  \begingroup%
    \pgfmath@x#1pt%
    \pgfmath@y#2pt%
    \advance\pgfmath@x-\pgfmath@y%
    \ifdim\pgfmath@x=0pt\relax%
      \pgfmath@x1pt\relax%
    \else%
      \pgfmath@x0pt\relax%
    \fi%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathreciprocal
%
% 1 / #1
%
\def\pgfmathreciprocal#1{%
	\pgfmathparse{#1}%
	\pgfmathreciprocal@{\pgfmathresult}}
\def\pgfmathreciprocal@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x=0pt\relax%
			\pgfmath@error{You asked me to calculate `1/#1', but I cannot divide any number by zero}{}%
		\fi%
		\edef\pgfmath@reciprocaltemp{\pgfmath@tonumber{\pgfmath@x}}%
		\expandafter\pgfmathreciprocal@@\pgfmath@reciprocaltemp0000000\pgfmath@}
\def\pgfmathreciprocal@@#1.#2#3#4#5#6#7\pgfmath@{%
		\c@pgfmath@counta#2#3#4#5#6\relax%
		% If the number is an integer, use TeX arithmatic.
		\ifnum\c@pgfmath@counta=0\relax%
			\pgfmath@x1pt\relax%
			\divide\pgfmath@x#1\relax%
		\else%
			\ifnum#1>100\relax%
				\c@pgfmath@counta#1#2#3#4\relax%
				\c@pgfmath@countb1000000000\relax%
				\divide\c@pgfmath@countb\c@pgfmath@counta%
				\c@pgfmath@counta\c@pgfmath@countb%
				\divide\c@pgfmath@counta10000\relax%
				\pgfmath@x\c@pgfmath@counta pt\relax%
				\multiply\c@pgfmath@counta-10000\relax%
				\advance\c@pgfmath@countb\c@pgfmath@counta%
				\pgfmath@y\c@pgfmath@countb pt\relax%
				\divide\pgfmath@y1000000\relax%		
				\advance\pgfmath@x\pgfmath@y%
			\else%
				\c@pgfmath@counta#1#2#3#4#5#6\relax%
				\c@pgfmath@countb1000000000\relax%
				\divide\c@pgfmath@countb\c@pgfmath@counta%
				\c@pgfmath@counta\c@pgfmath@countb%
				\divide\c@pgfmath@counta10000\relax%
				\pgfmath@x\c@pgfmath@counta pt\relax%
				\multiply\c@pgfmath@counta-10000\relax%
				\advance\c@pgfmath@countb\c@pgfmath@counta%
				\pgfmath@y\c@pgfmath@countb pt\relax%
				\pgfmath@y.1\pgfmath@y% Yes! This way is more accurate. Go figure...
				\pgfmath@y.1\pgfmath@y%	
				\pgfmath@y.1\pgfmath@y%	
				\pgfmath@y.1\pgfmath@y%		
				\advance\pgfmath@x\pgfmath@y%
			\fi%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathln
%
% Calculate ln(#1}
%
% This is based on an algorithm due to Rouben Rostamian and
% uses coefficients contributed by Alain Matthes.
%
\def\pgfmathln#1{\pgfmathparse{#1}\pgfmathln@{\pgfmathresult}}
\def\pgfmathln@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x>0pt\else%
			\pgfmath@error{I cannot calculate the logarithm of `#1'}{}%
		\fi%		
		\c@pgfmath@counta0\relax%
		\ifdim\pgfmath@x>2pt\relax%
			\ifdim\pgfmath@x<128pt\relax%
				\ifdim\pgfmath@x<8pt\relax%
					\ifdim\pgfmath@x<4pt\relax%
						\divide\pgfmath@x2\relax%
						\c@pgfmath@counta1\relax%
					\else%
						\divide\pgfmath@x4\relax%
						\c@pgfmath@counta2\relax%
					\fi%
				\else%
					\ifdim\pgfmath@x<32pt\relax%
						\ifdim\pgfmath@x<16pt\relax%
							\divide\pgfmath@x8\relax%
							\c@pgfmath@counta3\relax%
						\else%
							\divide\pgfmath@x16\relax%
							\c@pgfmath@counta4\relax%
						\fi%
					\else%
						\ifdim\pgfmath@x<64pt\relax%
							\divide\pgfmath@x32\relax%
							\c@pgfmath@counta5\relax%
						\else%
							\divide\pgfmath@x64\relax%
							\c@pgfmath@counta6\relax%
						\fi%
					\fi%
				\fi%
			\else%
				\ifdim\pgfmath@x<2048pt\relax%
					\ifdim\pgfmath@x<512pt\relax%
						\ifdim\pgfmath@x<256pt\relax%
							\divide\pgfmath@x128\relax%
							\c@pgfmath@counta7\relax%
						\else%
							\divide\pgfmath@x256\relax%
							\c@pgfmath@counta8\relax%
						\fi%
					\else%
						\ifdim\pgfmath@x<1024pt\relax%
							\divide\pgfmath@x512\relax%
							\c@pgfmath@counta9\relax%
						\else%
							\divide\pgfmath@x1024\relax%
							\c@pgfmath@counta10\relax%
						\fi%
					\fi%
				\else%
					\ifdim\pgfmath@x<8192pt\relax%
						\ifdim\pgfmath@x<4096pt\relax%
							\divide\pgfmath@x2048\relax%
							\c@pgfmath@counta11\relax%
						\else%
							\divide\pgfmath@x4096\relax%
							\c@pgfmath@counta12\relax%
						\fi%
					\else%
						\divide\pgfmath@x8192\relax%
						\c@pgfmath@counta13\relax%
					\fi%
				\fi%
			\fi%	
		\else%
			\ifdim\pgfmath@x<1pt\relax%
				\ifdim\pgfmath@x>0.0078125pt\relax% 2^-7
					\ifdim\pgfmath@x>0.125pt\relax% 2^-3
						\ifdim\pgfmath@x>0.5pt\relax% 2^-1
							\multiply\pgfmath@x2\relax%
							\c@pgfmath@counta-1\relax%
						\else%
							\multiply\pgfmath@x4\relax%
							\c@pgfmath@counta-2\relax%
						\fi%
					\else%
						\ifdim\pgfmath@x>0.03125pt\relax% 2^-5
							\ifdim\pgfmath@x>0.0625pt\relax%
								\multiply\pgfmath@x8\relax%
								\c@pgfmath@counta-3\relax%
							\else%
								\multiply\pgfmath@x16\relax%
								\c@pgfmath@counta-4\relax%
							\fi%
						\else%
							\ifdim\pgfmath@x>0.015625pt\relax% 2^-6
								\multiply\pgfmath@x32\relax%
								\c@pgfmath@counta-5\relax%
							\else%
								\multiply\pgfmath@x64\relax%
								\c@pgfmath@counta-6\relax%
							\fi%
						\fi%
					\fi%
				\else%
					\ifdim\pgfmath@x>0.000244140625pt\relax% 2^-11
						\ifdim\pgfmath@x>0.001953125pt\relax% 2^-9
							\ifdim\pgfmath@x>0.00390625pt\relax% 2^-8
								\multiply\pgfmath@x128\relax%
								\c@pgfmath@counta-7\relax%
							\else%
								\multiply\pgfmath@x256\relax%
								\c@pgfmath@counta-8\relax%
							\fi%
						\else%
							\ifdim\pgfmath@x>0.0009765625pt\relax% 2^-10
								\multiply\pgfmath@x512\relax%
								\c@pgfmath@counta-9\relax%
							\else%
								\multiply\pgfmath@x1024\relax%
								\c@pgfmath@counta-10\relax%
							\fi%
						\fi%
					\else%
						\ifdim\pgfmath@x>0.0001220703125pt\relax% 2^13
							\ifdim\pgfmath@x>0.0002441406256pt\relax% 2^12
								\multiply\pgfmath@x2048\relax%
								\c@pgfmath@counta-11\relax%
							\else%
								\multiply\pgfmath@x4096\relax%
								\c@pgfmath@counta-12\relax%
							\fi%
						\else%
							\multiply\pgfmath@x8192\relax%
							\c@pgfmath@counta-13\relax%
						\fi%
					\fi%
				\fi%
			\fi%	
		\fi%
		%
		% Use A+(B+(C+(D+(E+F*x)*x)*x)*x)*x
		%
		% where:
		% A = -2.787927935
		% B =  5.047861502
		% C = -3.489886985
		% D =  1.589480044
		% E = -.4025153233
		% F =  0.04300521312
		%
		\edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@x}}%
		\pgfmath@x0.04300521312\pgfmath@x%
		\advance\pgfmath@x-.4025153233pt\relax%
		\pgfmath@x\pgfmath@temp\pgfmath@x%
		\advance\pgfmath@x1.589480044pt\relax%
		\pgfmath@x\pgfmath@temp\pgfmath@x%
		\advance\pgfmath@x-3.489886985pt\relax%
		\pgfmath@x\pgfmath@temp\pgfmath@x%
		\advance\pgfmath@x5.047861502pt\relax%
		\pgfmath@x\pgfmath@temp\pgfmath@x%
		\advance\pgfmath@x-2.787927935pt\relax%
		\advance\pgfmath@x\c@pgfmath@counta pt\relax%
		\pgfmath@x0.6931471806\pgfmath@x%	
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}
	
% \pgfmathabs
%
% Calculate |#1|
%
\def\pgfmathabs#1{%
	\pgfmathparse{#1}%
	\pgfmathabsolute@{\pgfmathresult}}
\def\pgfmathabs@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
	\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathmod
%
% Calculate #1 mod #2.
%
\def\pgfmathmod#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathmod@{\pgfmathresult}{\pgfmath@arg}%
}
\def\pgfmathmod@#1#2{%
  \begingroup%
    \pgfmath@xa#1pt%
    \pgfmath@xb#2pt%
    \pgfmath@x\pgfmath@xa%
    \c@pgfmath@counta\pgfmath@xa%
    \c@pgfmath@countb\pgfmath@xb%
    \divide\c@pgfmath@counta\c@pgfmath@countb%
    \multiply\pgfmath@xb\c@pgfmath@counta%
    \advance\pgfmath@x-\pgfmath@xb%
    \pgfmath@returnone\pgfmath@x%
  \endgroup%
}

% \pgfmathsqrt
%
% Square-root of #1.
%
%
\def\pgfmathsqrt#1{\pgfmathparse{#1}\pgfmathsqrt@{\pgfmathresult}}
\def\pgfmathsqrt@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@error{I cannot calculate the square-root of the negative number `#1'}{}%
		\else%
			\ifdim\pgfmath@x<10pt\relax%
				\def\pgfmath@zeros{0}%
				\def\pgfmath@targetiterations{1}%
			\else%
				\ifdim\pgfmath@x<100pt\relax%
					\def\pgfmath@zeros{}%
					\def\pgfmath@targetiterations{1}%
				\else%
					\ifdim\pgfmath@x<1000pt\relax%
						\def\pgfmath@zeros{0}%
						\def\pgfmath@targetiterations{2}%
					\else%
						\ifdim\pgfmath@x<10000pt\relax%
							\def\pgfmath@zeros{}%
							\def\pgfmath@targetiterations{2}%
					\else%
							\def\pgfmath@zeros{0}%
							\def\pgfmath@targetiterations{3}%
		\fi\fi\fi\fi\fi%
		\edef\pgfmath@temp{\pgfmath@zeros\pgfmath@tonumber{\pgfmath@x}}%
		\expandafter\pgfmath@sqrt@\pgfmath@temp\pgfmath@%
}
\def\pgfmath@sqrt@#1.#2\pgfmath@{\pgfmath@@sqrt@#1#2\pgfmath@empty\pgfmath@empty\pgfmath@}

\def\pgfmath@@sqrt@#1#2{%
		\c@pgfmath@countb#1#2\relax%
		\ifnum\c@pgfmath@countb>35\relax%
			\ifnum\c@pgfmath@countb>63\relax%
				\ifnum\c@pgfmath@countb>80\relax%
					\c@pgfmath@counta9\relax%
				\else%
					\c@pgfmath@counta8\relax%
				\fi%
			\else%
				\ifnum\c@pgfmath@countb>48\relax%
					\c@pgfmath@counta7\relax%
				\else%
					\c@pgfmath@counta6\relax%
				\fi%
			\fi%
		\else%
			\ifnum\c@pgfmath@countb>15\relax%
				\ifnum\c@pgfmath@countb>24\relax%
					\c@pgfmath@counta5\relax%
				\else%
					\c@pgfmath@counta4\relax%
				\fi%
			\else%
				\ifnum\c@pgfmath@countb>3\relax%
					\ifnum\c@pgfmath@countb>8\relax%
						\c@pgfmath@counta3\relax%
					\else%
						\c@pgfmath@counta2\relax%
					\fi%
				\else%
					\ifnum\c@pgfmath@countb>0\relax%
						\c@pgfmath@counta1\relax%
					\else%
						\c@pgfmath@counta0\relax%
					\fi%
				\fi%
			\fi%
		\fi%
		\edef\pgfmath@root{\the\c@pgfmath@counta}%
		\edef\pgfmath@rootspecial{\the\c@pgfmath@counta}%
		\multiply\c@pgfmath@counta-\c@pgfmath@counta\relax%
		\advance\c@pgfmath@counta#1#2\relax%
		\edef\pgfmath@remainder{\the\c@pgfmath@counta}%
		\pgfmath@@@sqrt@%
}

\def\pgfmath@@@sqrt@#1#2{%
		\ifx\pgfmath@empty#1%
			\edef\pgfmath@remainder{\pgfmath@remainder00}%
			\def\pgfmath@tokens{\pgfmath@empty\pgfmath@empty}%
		\else%
			\ifx\pgfmath@empty#2%
				\edef\pgfmath@remainder{\pgfmath@remainder#10}%
				\def\pgfmath@tokens{\pgfmath@empty\pgfmath@empty}%
			\else%
				\edef\pgfmath@remainder{\pgfmath@remainder#1#2}%
				\def\pgfmath@tokens{}%
		\fi\fi%
		\c@pgfmath@counta\pgfmath@rootspecial\relax%
		\multiply\c@pgfmath@counta20\relax%
		\c@pgfmath@countb\c@pgfmath@counta%
		\multiply\c@pgfmath@countb6\relax%
		\advance\c@pgfmath@countb36\relax%
		\c@pgfmath@countc\c@pgfmath@counta\relax%
		\multiply\c@pgfmath@countc2\relax%
		\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax% 
			\advance\c@pgfmath@countb-\c@pgfmath@countc%
			\advance\c@pgfmath@countb-20\relax%
			\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
				\advance\c@pgfmath@countb-\c@pgfmath@countc%
				\advance\c@pgfmath@countb-12\relax%
				\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
					\advance\c@pgfmath@countb-\c@pgfmath@counta%
					\advance\c@pgfmath@countb-3\relax%
					\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
						\def\pgfmath@digit{0}%
					\else%
						\def\pgfmath@digit{1}%
					\fi%
				\else%
					\advance\c@pgfmath@countb\c@pgfmath@counta%
					\advance\c@pgfmath@countb5\relax%
					\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
						\def\pgfmath@digit{2}%
					\else%
						\def\pgfmath@digit{3}%
					\fi%
				\fi%
			\else%
				\advance\c@pgfmath@countb\c@pgfmath@counta%
				\advance\c@pgfmath@countb9\relax%
				\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
					\def\pgfmath@digit{4}%
				\else%
					\def\pgfmath@digit{5}%
				\fi%
			\fi%
		\else%
			\advance\c@pgfmath@countb\c@pgfmath@countc%
			\advance\c@pgfmath@countb28\relax%
			\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
				\advance\c@pgfmath@countb-\c@pgfmath@counta%
				\advance\c@pgfmath@countb-15\relax%
				\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
					\def\pgfmath@digit{6}%
				\else%
					\def\pgfmath@digit{7}%
				\fi%
			\else%
				\advance\c@pgfmath@countb\c@pgfmath@counta%
				\advance\c@pgfmath@countb17\relax%
				\ifnum\c@pgfmath@countb>\pgfmath@remainder\relax%
					\def\pgfmath@digit{8}%
				\else%
					\def\pgfmath@digit{9}%
				\fi%
			\fi%
		\fi%
		\edef\pgfmath@rootspecial{\pgfmath@rootspecial\pgfmath@digit}%
		\advance\c@pgfmath@counta\pgfmath@digit\relax%
		\multiply\c@pgfmath@counta-\pgfmath@digit\relax%
		\advance\c@pgfmath@counta\pgfmath@remainder\relax%
		\edef\pgfmath@remainder{\the\c@pgfmath@counta}%
		\c@pgfmath@counta\pgfmath@targetiterations\relax%
		\advance\c@pgfmath@counta-1\relax%
		\edef\pgfmath@targetiterations{\the\c@pgfmath@counta}%
		\ifnum\c@pgfmath@counta=0\relax%
			\edef\pgfmath@root{\pgfmath@root.\pgfmath@digit}%
		\else%
			\edef\pgfmath@root{\pgfmath@root\pgfmath@digit}%
		\fi%
		\ifnum\c@pgfmath@counta=-4\relax% -n+1 digits of precision.
			\let\pgfmath@next\pgfmath@sqrt@end%
		\else%
			\let\pgfmath@next\pgfmath@@@sqrt@%
		\fi%
		\expandafter\pgfmath@next\pgfmath@tokens%
}

\def\pgfmath@sqrt@end#1\pgfmath@{%
		\edef\pgfmathresult{\pgfmath@root}%
		\pgfmath@smuggleone\pgfmathresult%
	\endgroup}

% \pgfmathpow
%
% Calculates #1 ^ #2
%
\def\pgfmathpow#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathpow@{\pgfmathresult}{\pgfmath@arg}}
\def\pgfmathpow@#1#2{%
  \begingroup%
    \pgfmath@xa#1pt%
    \pgfmath@xb#2pt%
    \afterassignment\pgfmath@x%
		\expandafter\c@pgfmath@counta\the\pgfmath@xb\relax%
		\ifnum\c@pgfmath@counta<0\relax%
			\c@pgfmath@counta-\c@pgfmath@counta%
			\pgfmathreciprocal@{#1}%
			\pgfmath@xa\pgfmathresult pt\relax%
		\fi
		\ifdim\pgfmath@x=0pt\relax%
			\pgfmath@x1pt\relax%
			\pgfmathloop%
				\ifnum\c@pgfmath@counta>0\relax%
					\ifodd\c@pgfmath@counta%
						\pgfmath@x\pgfmath@tonumber{\pgfmath@x}\pgfmath@xa%
					\fi
					\ifnum\c@pgfmath@counta>1\relax%
						\pgfmath@xa\pgfmath@tonumber{\pgfmath@xa}\pgfmath@xa%
					\fi%
					\divide\c@pgfmath@counta2\relax%
			\repeatpgfmathloop%
		\else%
			\pgfmathln@{#1}%
			\pgfmath@x\pgfmathresult pt\relax%
			\pgfmath@x\pgfmath@tonumber{\pgfmath@xb}\pgfmath@x%
			\pgfmathexp@{\pgfmath@tonumber{\pgfmath@x}}%
			\pgfmath@x\pgfmathresult pt\relax%
		\fi%
		\pgfmath@returnone\pgf@x%
	\endgroup%
}

% \pgfmathround
% 
% Asymmetric Half-up rounding.
%
\def\pgfmathround#1{\pgfmathparse{#1}\pgfmathround@{\pgfmathresult}}
\def\pgfmathround@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\afterassignment\pgfmath@xa%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		\pgfmath@xb\pgfmath@x%
		\ifdim\pgfmath@xb<0pt\relax%
			\ifdim\pgfmath@xa<0.5pt\relax%
			\else%
				\advance\c@pgfmath@counta-1\relax%
			\fi%
		\else%
			\ifdim\pgfmath@xa<0.5pt\relax%
			\else%
				\advance\c@pgfmath@counta1\relax%
			\fi%
		\fi%
		\pgfmath@returnone\the\c@pgfmath@counta pt%
	\endgroup%
}%

% \pgfmathfloor
% 
% Floor function.
%
\def\pgfmathfloor#1{\pgfmathparse{#1}\pgfmathfloor@{\pgfmathresult}}
\def\pgfmathfloor@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\pgfmath@x\c@pgfmath@counta pt\relax%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathceil
% 
% Ceiling function.
%
\def\pgfmathceil#1{\pgfmathparse{#1}\pgfmathceil@{\pgfmathresult}}
\def\pgfmathceil@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\pgfmath@y\pgfmath@x%
		\advance\pgfmath@y-\c@pgfmath@counta pt\relax%
		\pgfmath@x\c@pgfmath@counta pt\relax%
		\ifdim\pgfmath@y>0pt\relax%
			\advance\pgfmath@x1pt\relax%
		\fi%
	\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathexp
%
% A Maclaurens expansion for e^#1.
% 0 <= #1 < ln(16384).
%
\def\pgfmathexp#1{\pgfmathparse{#1}\pgfmathexp@{\pgfmathresult}}
\def\pgfmathexp@#1{%
	\begingroup%
		\edef\pgfmath@arg{#1}%
		\pgfmath@x1pt\relax%
		\pgfmath@xa1pt\relax%
		\pgfmath@xb\pgfmath@x%
		\pgfmathloop%
			\pgfmath@xc\pgfmathcounter pt\relax%
			\c@pgfmath@counta\pgfmath@xc%
			\divide\c@pgfmath@counta65536\relax%
			\pgfmath@xc1pt\relax%
			\divide\pgfmath@xc\c@pgfmath@counta%
			\pgfmath@xa\pgfmath@tonumber{\pgfmath@xc}\pgfmath@xa%
			\expandafter\pgfmath@xa\pgfmath@arg\pgfmath@xa%
			\advance\pgfmath@x\pgfmath@xa%
			\ifdim\pgfmath@x=\pgfmath@xb%
			\else%
				\pgfmath@xb\pgfmath@x%
		\repeatpgfmathloop%
	\pgfmath@returnone\pgfmath@x%
	\endgroup%
}



% \pgfmathvectorlength
%
% Calcluate the Eulidean length of a 2D vector.
%
% This based on polynomial approximation co-efficents
% contributed by Rouben Rostamian.
%
% #1 - the x component of the vector.
% #2 - the y component of the vector.
%
\def\pgfmathveclen#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathveclen@{\pgfmathresult}{\pgfmath@arg}%
}
\def\pgfmathveclen@#1#2{%
  \begingroup%
    \pgfmath@x#1pt\relax%
    \pgfmath@y#2pt\relax%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\ifdim\pgfmath@y<0pt\relax%
			\pgfmath@y-\pgfmath@y%
		\fi%
		\ifdim\pgfmath@x=0pt\relax%
			\pgfmath@x\pgfmath@y%
		\else%
			\ifdim\pgfmath@y=0pt\relax%
			\else%
				\ifdim\pgfmath@x>\pgfmath@y%
					\pgfmath@xa\pgfmath@x%
					\pgfmath@x\pgfmath@y%
					\pgfmath@y\pgfmath@xa%
				\fi%
				% We use a scaling factor to reduce errors.
				\ifdim\pgfmath@y>10000pt\relax%
					\c@pgfmath@counta1500\relax%
				\else%
					\ifdim\pgfmath@y>1000pt\relax%
						\c@pgfmath@counta150\relax%
					\else%
						\ifdim\pgfmath@y>100pt\relax%
							\c@pgfmath@counta50\relax%
						\else%
							\c@pgfmath@counta1\relax%
						\fi%
					\fi%
				\fi%
				\divide\pgfmath@x\c@pgfmath@counta\relax%
				\divide\pgfmath@y\c@pgfmath@counta\relax%
				\pgfmathreciprocal@{\pgfmath@tonumber{\pgfmath@y}}%
				\pgfmath@x\pgfmathresult\pgfmath@x%
				\pgfmath@xa\pgfmath@tonumber{\pgfmath@x}\pgfmath@x%
				\edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@xa}}%
				%
				% Use A+x^2*(B+x^2*(C+x^2*(D+E*x^2))) 
				% where
				% A = +1.000012594
				% B = +0.4993615349 
				% C = -0.1195159052
				% D = +0.04453994279
				% E = -0.01019210944
				%
				\pgfmath@x-0.01019210944\pgfmath@xa%
				\advance\pgfmath@x0.04453994279pt\relax%
				\pgfmath@x\pgfmath@temp\pgfmath@x%
				\advance\pgfmath@x-0.1195159052pt\relax%
				\pgfmath@x\pgfmath@temp\pgfmath@x%
				\advance\pgfmath@x0.4993615349pt\relax%
				\pgfmath@x\pgfmath@temp\pgfmath@x%
				\advance\pgfmath@x1.000012594pt\relax%
				\ifdim\pgfmath@y<0pt\relax%
					\pgfmath@y-\pgfmath@y%
				\fi%
				\pgfmath@x\pgfmath@tonumber{\pgfmath@y}\pgfmath@x%
				% Invert the scaling factor.
				\multiply\pgfmath@x\c@pgfmath@counta\relax%
			\fi%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathmax
%
% Return the maximum of #1 or #2
%
\def\pgfmathmax#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathmax@{\pgfmathresult}{\pgfmath@arg}}%
\def\pgfmathmax@#1#2{%
  \begingroup
    \pgfmath@x#1pt%
    \pgfmath@y#2pt\relax%
    \ifdim\pgfmath@x>\pgfmath@y%
      \pgfmath@returnone\pgfmath@x%
    \else%
      \pgfmath@returnone\pgfmath@y%
    \fi%
  \endgroup
}

% \pgfmathmax
%
% Return the minimim of #1 or #2
%
\def\pgfmathmin#1#2{%
	\edef\pgfmath@marshal{%
		\noexpand\pgfmathparse{#2}
		\noexpand\let\noexpand\pgfmath@arg\noexpand\pgfmathresult%
		\noexpand\pgfmathparse{#1}%
	}%
	\pgfmath@marshal%
	\pgfmathmin@{\pgfmathresult}{\pgfmath@arg}}%
\def\pgfmathmin@#1#2{%
  \begingroup
    \pgfmath@x#1pt%
    \pgfmath@y#2pt%
    \relax%
    \ifdim\pgfmath@x<\pgfmath@y%
      \pgfmath@returnone\pgfmath@x%
    \else%
      \pgfmath@returnone\pgfmath@y%
    \fi%
  \endgroup%
}

% \pgfmathscientific
%
% Return the value of #1e#2
%
% e.g. \pgfmathscientific{1.23456789123}{4}
%
% defines \pgfmathresult as 12345.67891
%
% NB These arguments *are not parsed*, as the long mantissa would be lost.
%
\def\pgfmathscientific#1#2{%
	\begingroup%
		\edef\pgfmath@sci@exponent{#2}%
		\pgfmath@x#1pt\relax%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
			\edef\pgfmath@sci@sign{-}%
			\edef\pgfmath@temp{\pgfmath@gobbleone#1}%
		\else%
			\edef\pgfmath@sci@sign{+}%
			\edef\pgfmath@temp{#1}%
		\fi%
		\expandafter\pgfmath@scientific@@\pgfmath@temp00000000000\pgfmath@}

\def\pgfmath@scientific@@#1.#2#3#4#5#6{%
		\edef\pgfmath@sci@int{#1}%
		\edef\pgfmath@sci@mantissaA{#2#3#4#5#6}%
		\pgfmath@scientific@@@}
	
\def\pgfmath@scientific@@@#1#2#3#4#5#6\pgfmath@{%
		\edef\pgfmath@sci@mantissaB{#1#2#3#4#5}%
		\c@pgfmath@counta\pgfmath@sci@exponent\relax%
		\c@pgfmath@countb\c@pgfmath@counta%
		\ifnum\c@pgfmath@counta<0\relax%
			\c@pgfmath@counta-\c@pgfmath@counta%
		\fi%
		\pgfmathpow@{10}{\the\c@pgfmath@counta}%
		\afterassignment\pgfmath@gobbletilpgfmath@
		\c@pgfmath@countc\pgfmathresult\relax\pgfmath@
		\edef\pgfmath@sci@factor{\the\c@pgfmath@countc}%
		\ifnum\c@pgfmath@countb<0\relax%
			% xE-y: easy...
			\pgfmath@x\pgfmath@sci@int.\pgfmath@sci@mantissaA pt\relax%
			\divide\pgfmath@x\pgfmath@sci@factor\relax%
		\else%
			% xE+y: 
			% Must do this way so as not lose digits in a long mantissa. Sigh...
			\c@pgfmath@counta\pgfmath@sci@int%
			\c@pgfmath@countb\pgfmath@sci@mantissaA%
			\multiply\c@pgfmath@counta\pgfmath@sci@factor\relax%
			\multiply\c@pgfmath@countb\pgfmath@sci@factor\relax%
			\c@pgfmath@countc\c@pgfmath@countb%
			\divide\c@pgfmath@countb100000\relax%
			\advance\c@pgfmath@counta\c@pgfmath@countb%
			\multiply\c@pgfmath@countb100000\relax%
			\advance\c@pgfmath@countc-\c@pgfmath@countb%
			\c@pgfmath@countb\pgfmath@sci@mantissaB\relax%
			\multiply\c@pgfmath@countb\pgfmath@sci@factor\relax%
			\divide\c@pgfmath@countb100000\relax%
			\advance\c@pgfmath@countc\c@pgfmath@countb%
			\advance\c@pgfmath@countc100000\relax%
			\edef\pgfmath@sci@result{\pgfmath@sci@sign\the\c@pgfmath@counta.\expandafter\pgfmath@gobbleone\the\c@pgfmath@countc pt}%
			\pgfmath@x\pgfmath@sci@result\relax%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup}





% *** The following commands DO NOT WORK without the rest of PGF ***
%
% (a dumping ground for stuff that doesn't really belong anywhere else)
	
% \pgfmathanglebetweenpoints
%
% Define \pgfmathresult as the angle between points #1 and #2
% Should get the quadrants right as well.
%
\def\pgfmathanglebetweenpoints#1#2{%
	\begingroup%
		\pgf@process{\pgfpointdiff{#1}{#2}}%
		%
		% First approximate the angle of the external point...
		%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\pgf@xb\pgf@x%
		\pgf@yb\pgf@y%
		\ifdim\pgf@xa<0pt\relax%
			\pgf@xa-\pgf@xa%
		\fi%
		\ifdim\pgf@ya<0pt\relax%
			\pgf@ya-\pgf@ya%
		\fi%
		\ifdim\pgf@ya>\pgf@xa%
			\pgf@x\pgf@xa%
			\pgf@y\pgf@ya%
		\else%
			\pgf@x\pgf@ya%
			\pgf@y\pgf@xa%
		\fi%
		\ifdim\pgf@y=0pt\relax%
			\pgf@x0pt%
		\else%
			\pgfmathreciprocal@{\pgfmath@tonumber{\pgf@y}}%
			\pgf@x\pgfmathresult\pgf@x%
		\fi%
		\multiply\pgf@x1000\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgf@counta\the\pgf@x\relax\pgfmath@%
		\expandafter\pgf@x\csname pgfmath@atan@\the\c@pgf@counta\endcsname pt\relax%
		\ifdim\pgfmath@ya>\pgfmath@xa\relax%
			\pgf@x-\pgf@x%
			\advance\pgf@x90pt%
		\fi%
		\ifdim\pgf@xb<0pt%
			\ifdim\pgf@yb>0pt%
				\pgf@x-\pgf@x%
			\fi%
			\advance\pgf@x180pt\relax%
		\else%
			\ifdim\pgf@yb<0pt%
			\pgf@x-\pgf@x%
			\advance\pgf@x360pt\relax%
		\fi\fi%
		\pgfmath@returnone\pgf@x%
	\endgroup%
}

%
% \pgfmathrotatepointaround
%
% Rotate point #1 about point #2 by #3 degrees.
%
\def\pgfmathrotatepointaround#1#2#3{%
	\pgf@process{%
		\pgf@process{#2}%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\pgf@xb\pgf@x%
		\pgf@yb\pgf@y%
		\pgf@process{#1}%
		\advance\pgf@x-\pgf@xa%
		\advance\pgf@y-\pgf@ya%
		\pgfmathsetmacro\angle{#3}%
		\pgfmathsin@{\angle}%
		\let\sineangle\pgfmathresult%
		\pgfmathcos@{\angle}%
		\let\cosineangle\pgfmathresult%
		\pgf@xa\cosineangle\pgf@x%
		\advance\pgf@xa-\sineangle\pgf@y%
		\pgf@ya\sineangle\pgf@x%
		\advance\pgf@ya\cosineangle\pgf@y%
		\pgf@x\pgf@xb%
		\pgf@y\pgf@yb%
		\advance\pgf@x\pgf@xa%
		\advance\pgf@y\pgf@ya%
	}%
}

% \pgfmathanglebetweenlines
%
% Calculate the clockwise angle between a line from point #1
% to point #2 and a line from #3 to point #4.
%
\def\pgfmathanglebetweenlines#1#2#3#4{%
	\begingroup%
		\pgfmathanglebetweenpoints{#1}{#2}%
		\let\firstangle\pgfmathresult%
		\pgfmathanglebetweenpoints{#3}{#4}%
		\let\secondangle\pgfmathresult%
		\ifdim\firstangle pt>\secondangle pt\relax%
			\pgfmathadd@{\secondangle}{360}%
			\let\secondangle\pgfmathresult%
		\fi%
		\pgfmathsubtract@{\secondangle}{\firstangle}%
		\pgfmath@smuggleone\pgfmathresult%
	\endgroup%
}

% \pgfmathpointreflectalongaxis
%
% Reflects point #2 around an axis centered on #2 at an angle #3.
%
\def\pgfmathreflectpointalongaxis#1#2#3{%
	\pgf@process{%
		\pgfmathanglebetweenpoints{#2}{#1}%
		\pgfmath@tempdima\pgfmathresult pt\relax%
		\pgfmathparse{#3}%
		\advance\pgfmath@tempdima-\pgfmathresult pt\relax%
		\pgfmath@tempdima-2.0\pgfmath@tempdima%
		\pgfmathrotatepointaround{#1}{#2}{\pgfmath@tonumber{\pgfmath@tempdima}}%
	}%
}


% \pgfmathpointintersectionoflineandarc 
%
% A bit experimental at the moment:
%
% Locates the point where a line crosses an eliptical arc. If the line
% does not cross the arc, a meaningless point will result.
%
% #1 the point of the line on the "convex" side of the arc.
% #2 the point of the line on the "concave" side of the arc.
% #3 the center of the eliptical arc.
% #4 start angle of the arc.
% #5 end angle of the arc.
% #6 radii of the arc.
%
\def\pgfmathpointintersectionoflineandarc#1#2#3#4#5#6{%
	\pgf@process{%
		%
		% Get the required angle.
		%
		\pgfmathanglebetweenpoints{#2}{#1}%
		\let\x\pgfmathresult%
		%
		% Get the radii of the arc.
		%
		\pgfmath@in@{and }{#6}%
	  \ifpgfmath@in@%
	    \pgf@polar@#6\@@%
	  \else%
	    \pgf@polar@#6 and #6\@@%
	  \fi%
	  \edef\xarcradius{\the\pgf@x}%
	  \edef\yarcradius{\the\pgf@y}% 
	   %
	  % Get the start and end angles of the arc...
	  % 
	  \pgfmathsetmacro\s{#4}%
	  \pgfmathsetmacro\e{#5}%
	  %
	  % ...and also with rounding.
	  %
	  \pgfmathmod@{\s}{360}%
	  \ifdim\pgfmathresult pt<0pt\relax%
	  	\pgfmathadd@{\pgfmathresult}{360}%
	  \fi%
	  \let\ss\pgfmathresult%
	  \pgfmathmod@{\e}{360}%
	  \ifdim\pgfmathresult pt<0pt\relax%
	  	\pgfmathadd@{\pgfmathresult}{360}%
	  \fi%
	  \let\ee\pgfmathresult%
	  %
	  % Hackery for when arc straddles zero.
	  %
	  \ifdim\ee pt<\ss pt\relax%
	  	\pgfmathadd@{\x}{180}%
	  	\pgfmathmod@{\pgfmathresult}{360}%
	  	\let\x\pgfmathresult%
	  \fi%
	  \def\m{360}% Measure of nearness.
		\pgfmathadd@{\s}{\e}%
		\pgfmathdivide@{\pgfmathresult}{2}%
		\let\n\pgfmathresult% The best estimate (default to middle of arc).
		\pgfmathloop%
			\pgfmathadd@{\s}{\e}%
			\pgfmathdivide@{\pgfmathresult}{2}%
			\let\p\pgfmathresult%
			\ifdim\p pt=\s pt\relax% 
			\else%
				\pgfmathanglebetweenpoints{#2}{%
					\pgfpointadd{#3}{%
						\pgf@x\xarcradius\relax%
						\pgfmathcos@{\p}%
						\pgf@x\pgfmathresult\pgf@x%
						\pgf@y\yarcradius\relax%
						\pgfmathsin@{\p}%
						\pgf@y\pgfmathresult\pgf@y%
					}%
				}%
				%
			  % Hackery for when arc straddles zero.
			  %
				\ifdim\ee pt<\ss pt\relax%
			  	\pgfmathadd@{\pgfmathresult}{180}%
			  	\pgfmathmod@{\pgfmathresult}{360}%
			  \fi%
				\let\q\pgfmathresult%
				%
				% More hackery...
				%
				\ifdim\x pt>335pt\relax%
					\ifdim\q pt<45pt\relax%
						\pgfmathadd@{\q}{360}%
						\let\q\pgfmathresult%
					\fi%
				\fi%
				\ifdim\x pt=\q pt% Found it!
						\pgfmathbreakloop% Breaks after current iteration is complete.
					\else
						\ifdim\x pt<\q pt\relax%
							\let\e\p%
						\else%
							\let\s\p%
						\fi%
					\fi%
					\pgfmathsubtract@{\x}{\q}%
					\pgfmathabs@{\pgfmathresult}%
					%
					% Save the estimate if it is better than any previous estimate.
					%
					\ifdim\pgfmathresult pt<\m pt\relax%
						\let\m\pgfmathresult%
						\let\n\p%
					\fi%				
		\repeatpgfmathloop%
		\pgfpointadd{#3}{\pgfpointpolar{\n}{\xarcradius and \yarcradius}}%
	}%
}

% \pgfmathangleonellipse
% 
% Find the angle corresponding to a point on the border of an ellispe.
%
% #1 - the point on the border.
% #2 - the radii of the ellipse.
%
\def\pgfmathangleonellipse#1#2{%
	\begingroup%
		\pgfmath@in@{and }{#2}%
	  \ifpgfmath@in@%
	    \pgf@polar@#2\@@%
	  \else%
	    \pgf@polar@#2 and #2\@@%
	  \fi%
	  \pgf@xa\pgf@x%
	  \pgf@ya\pgf@y%
	  \pgf@process{#1}% 
	  \ifdim\pgf@x=0pt\relax%
			\pgfutil@tempdima1pt\relax%
		\else%
			\pgfutil@tempdima\pgf@x%
			\pgfmathdivide@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgfutil@tempdima}}%
			\pgfutil@tempdima\pgfmathresult pt\relax%
		\fi%
		\ifdim\pgf@y=0pt\relax%
			\pgfutil@tempdima1pt\relax%
		\else%
			\pgfmathdivide@{\pgfmath@tonumber{\pgf@y}}{\pgfmath@tonumber{\pgf@ya}}%
			\pgfutil@tempdima\pgfmathresult\pgfutil@tempdima%
			\pgfmathatan@{\pgfmath@tonumber{\pgfutil@tempdima}}%
		\fi%
		%
		\pgfutil@tempdima\pgfmathresult pt\relax%
		\ifdim\pgfutil@tempdima<0pt\relax%
  		\advance\pgfutil@tempdima360pt\relax%
  	\fi%
		\ifdim\pgf@x<0pt\relax%
			\ifdim\pgf@y=0pt\relax%
				\pgfutil@tempdima180pt\relax%
			\else%
				\ifdim\pgf@y<0pt\relax%
					\advance\pgfutil@tempdima180pt\relax%
				\else%
					\advance\pgfutil@tempdima-180pt\relax%
				\fi%
			\fi%
		\else%
			\ifdim\pgf@x=0pt\relax%
				\ifdim\pgf@y<0pt\relax%
					\pgfutil@tempdima270pt\relax%
				\else%
					\pgfutil@tempdima90pt\relax%
				\fi%
			\else%
				\ifdim\pgf@y=0pt\relax%
					\pgfutil@tempdima0pt\relax%
				\fi%
			\fi%				
		\fi%
		\pgfmath@returnone\pgfutil@tempdima%
	\endgroup%
}

==> pgfmathparser.code.tex <==
% Copyright 2007 Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file parses/evaluates a decimal expression.
%
% Version 1.414213 29/9/2007

% \pgfmathparse, \pgfmathqparse
%
% Evaluates a decimal expression.
%
% #1 - the expression.
%
% returns
%
% x = the result as a dimension.
%
% E.g.
% \pgfmathparse{3pt*2cm+1.5}
% \pgfmathqparse{3pt*2cm+1.5pt}
%
% Every number in \pgfmathqparse *must*
% specify a unit.
%
\newif\ifpgfmath@quickparse

\def\pgfmathparse{%
	\pgfmath@quickparsefalse%
	\pgfmathparse@}

\def\pgfmathqparse{%
	\pgfmath@quickparsetrue%
	\pgfmathparse@}
		
\def\pgfmath@calcreal#1{#1}%
\def\pgfmath@calcminof#1#2{min(#1,#2)}%
\def\pgfmath@calcmaxof#1#2{max(#1,#2)}%
\def\pgfmath@calcratio#1#2{#1/#2}%

\def\pgfmathparse@#1{%
  \begingroup%    
    % Reinstall correct font, so that dimensions like 1em are correct
    \pgfmath@selectfont%
    \let\real\pgfmath@calcreal%
    \let\minof\pgfmath@calcminof%
    \let\maxof\pgfmath@calcmaxof%
    \let\ratio\pgfmath@calcratio%
    \edef\pgfmath@temp{#1}%
    \pgfmath@resetparsingparameters%
    \global\pgfmathunitsdeclaredfalse%
    \ifpgfmath@quickparse%
      \let\pgfmath@parseoperand\pgfmath@quickparseoperand%
    \else%
      \let\pgfmath@parseoperand\pgfmath@parseoperand%
    \fi%
    \let\pgfmath@parsepostgroup\pgfmath@parseoperator%
    \expandafter\pgfmath@parse@\pgfmath@temp @@@@@@@@@@@\pgfmath@empty}


% \pgfmath@resetparsingparameters
%
% Reset the stack at the begining of the parse/group.
%
\def\pgfmath@resetparsingparameters{%
	\pgfmath@stack{\pgfmath@empty\pgfmath@empty\pgfmath@empty\pgfmath@empty}%
	\def\pgfmath@stacknextoperator{\pgfmath@empty}% Will not work with \let
}
% \pgfmath@parse@
%
% Start parsing. Expect one of
% 1) the end of the parse
% 2) the start of a group
% 3) a (possible) operand.
%
\def\pgfmath@parse@#1{%
	\def\pgfmath@token{}%
	\ifx#1@%
		\let\pgfmath@parsenext\pgfmath@endparse%
	\else%
		\ifx#1(%
			\let\pgfmath@parsenext\pgfmath@startparsegroup%
		\else%
			\edef\pgfmath@token{#1}%
			\let\pgfmath@parsenext\pgfmath@parseoperand%
	\fi\fi%
	\pgfmath@parsenext%
}

% If no TeX units are declared *at any point* in the parse
% the result is scaled by \pgfmathresultunitscale.
\newif\ifpgfmathunitsdeclared
\def\pgfmathsetresultunitscale#1{\def\pgfmathresultunitscale{#1}}
\def\pgfmathresultunitscale{1}

% \pgfmath@endparse
%
% Everything stops here.
%
\def\pgfmath@endparse#1\pgfmath@empty{%
    \pgfmath@processalloperations%
    \pgfmath@stackpop{\pgfmathresult}%
    \begingroup%
      \ifpgfmathunitsdeclared%
        \pgfmath@x1pt\relax%
      \else%
        \afterassignment\pgfmath@gobbletilpgfmath@%
        \pgfmath@x\pgfmathresultunitscale pt\relax\pgfmath@%
      \fi%
      \expandafter\pgfmath@x\pgfmathresult\pgfmath@x%
      \pgfmath@returnone\pgfmath@x%
    \endgroup%
    \pgfmath@smuggleone{\pgfmathresult}%
  \endgroup%
  \ignorespaces%
}

% \pgfmath@startparsegroup
%
% When opening ( is scanned start a new group.
%
\def\pgfmath@startparsegroup{%
	\begingroup%
		\let\pgfmath@parsepostgroup\pgfmath@parseoperator%
		\pgfmath@resetparsingparameters%
		\pgfmath@parse@}

% \pgfmath@endparsegroup
%
% When closing ) is scanned, processes all waiting
% operations (within the group) and close the group.
%
\def\pgfmath@endparsegroup{%
		\pgfmath@processalloperations%
		\pgfmath@stackpop{\pgfmathresult}%
		\expandafter\pgfmath@x\pgfmathresult pt\relax%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
	\pgfmath@parsepostgroup%
}

% \pgfmath@parseoperator
%
% An operator is expected here. 
% Or the end of the parse or parse group.
% 
\def\pgfmath@parseoperator#1{%
	\def\pgfmath@token{}%
	% Push the operand in \pgfmathresult on to the stack. 
	\expandafter\pgfmath@stackpushoperand\expandafter{\pgfmathresult}%
	\ifx#1@%
		\let\pgfmath@parsenext\pgfmath@endparse%
	\else%
		\ifx#1+%
			\let\pgfmath@parsenext\pgfmath@parseadd%
		\else%
			\ifx#1-%
				\let\pgfmath@parsenext\pgfmath@parsesubtract%
			\else%
				\ifx#1*%
					\let\pgfmath@parsenext\pgfmath@parsemultiply%
				\else%
					\ifx#1/%
						\let\pgfmath@parsenext\pgfmath@parsedivide%
					\else
						\ifx#1)%
							\let\pgfmath@parsenext\pgfmath@endparsegroup%
						\else%
							\ifx#1r%
								\let\pgfmath@parsenext\pgfmath@parseradians%
							\else%
								\ifx#1>%
									\let\pgfmath@parsenext\pgfmath@parsegreaterthan%
								\else%
									\ifx#1<%
										\let\pgfmath@parsenext\pgfmath@parselessthan%
									\else%
										\if#1=%
											\let\pgfmath@parsenext\pgfmath@parseequalto%
										\else%
											\if#1^%
												\let\pgfmath@parsenext\pgfmath@parsepower%
											\else%
												\pgfmath@error{Unknown operator `#1'}%
												\let\pgfmath@parsenext\relax%
	\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi%
	\pgfmath@parsenext%
}

% Use a \toks register as a stack.
\newtoks\pgfmath@stack

% \pgfmath@stackpushoperator
% 
% Push an operator (actually its macro e.g., \pgfmathadd@)
% on to the stack. And keep track of it using the macro
% \pgfmath@stacknextoperator.
%
\def\pgfmath@stackpushoperator#1{%
	\edef\pgfmath@temp{\noexpand#1\the\pgfmath@stack}%
	\expandafter\pgfmath@stack\expandafter{\pgfmath@temp}%
	\def\pgfmath@stacknextoperator{#1}}% <- Must \def. Cannot \let.

% \pgfmath@stackpushoperand
%
% Push an operand (i.e. a number) on the stack. It is
% put within a TeX group to make popping a lot simpler.
%
\def\pgfmath@stackpushoperand#1{%
	\edef\pgfmath@temp{{#1}\the\pgfmath@stack}%
	\expandafter\pgfmath@stack\expandafter{\pgfmath@temp}%
}

% \pgfmath@stackpeek
%
% Peek (i.e. without removal) at the top of the stack.
%
\def\pgfmath@stackpeek{\expandafter\pgfmath@stackpeek@\the\pgfmath@stack\pgfmath@}
\def\pgfmath@stackpeek@#1#2\pgfmath@{#1}%

% \pgfmath@stackpop
%
% Pop (i.e. remove) the top of the stack into #1.
%
\def\pgfmath@stackpop#1{\expandafter\pgfmath@stackpop@\expandafter#1\the\pgfmath@stack\pgfmath@}
\def\pgfmath@stackpop@#1#2#3\pgfmath@{\edef#1{#2}\pgfmath@stack{#3}}%

% \pgfmath@stackpopoperation
%
% Remove and perform an operation from the stack.
%
\def\pgfmath@stackpopoperation{%
	\expandafter\pgfmath@stackpopoperation@\the\pgfmath@stack\pgfmath@%
}
\def\pgfmath@stackpopoperation@#1#2#3#4#5\pgfmath@{%
	\ifx\pgfmath@empty#1\relax%
			\pgfmath@stack{\pgfmath@empty\pgfmath@empty\pgfmath@empty\pgfmath@empty}%
	\else%
		\ifx\pgfmath@empty#2\relax%
			\pgfmath@stack{{#1}\pgfmath@empty\pgfmath@empty\pgfmath@empty\pgfmath@empty}%
		\else%
			#2{#3}{#1}%
			\pgfmath@stack{#4#5}%
			\expandafter\pgfmath@stackpushoperand\expandafter{\pgfmathresult}%
	\fi\fi%
	\def\pgfmath@stacknextoperator{#4}}

% \pgfmath@processalloperations
%
% Process all operation in the stack. The 
% overall result is at the top of the stack.
%
\def\pgfmath@processalloperations{%
	\expandafter\pgfmath@in@\pgfmath@stacknextoperator{\pgfmath@empty}%
	\ifpgfmath@in@%
		\let\pgfmath@processnext\relax%		
	\else%
		\pgfmath@stackpopoperation%
		\let\pgfmath@processnext\pgfmath@processalloperations%
	\fi%
	\pgfmath@processnext}

% \pgfmath@processoperationsuntil
%
% Process operations in the stack, until the specified
% operation/s is/are encountered. The overall result is 
% at the top of the stack.
%
\def\pgfmath@processoperationsuntil#1{%
	\expandafter\pgfmath@in@\pgfmath@stacknextoperator{#1\pgfmath@empty}%
	\ifpgfmath@in@%
		\let\pgfmath@processnext\pgfmath@processoperationsuntil@end%		
	\else%
		\pgfmath@stackpopoperation%
		\let\pgfmath@processnext\pgfmath@processoperationsuntil%
	\fi%
	\pgfmath@processnext{#1}}
\def\pgfmath@processoperationsuntil@end#1{}


% OK. Now the operators are parsed.
% These correspond to the + - / * ^ < > = operators and r (postfix) function.
%
\def\pgfmath@parseadd{%	
	% If no operator has been assigned (i.e. + is the first operator scanned),
	% do nothing, except add addition to the stack.
	\ifx\pgfmath@stacknextoperator\pgfmath@empty%
	\else%
		% Empty the process stack up to any inequalities.
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@}%
	\fi%
	\pgfmath@stackpushoperator{\pgfmathadd@}%
	\pgfmath@parse@}
	
\def\pgfmath@parsesubtract{%	
	% If no operator has been assigned (i.e. - is the first operator scanned),
	% do nothing, except add subtract to the stack.
	\ifx\pgfmath@stacknextoperator\pgfmath@empty%
	\else%
		% Empty the process stack up to any inequalities.
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@}%
	\fi%
	\pgfmath@stackpushoperator{\pgfmathsubtract@}%
	\pgfmath@parse@}
	
\def\pgfmath@parsemultiply{%
	% If no operator has been assigned (i.e. * is the first operator scanned),
	% do nothing, except push multiply onto the stack.
	\ifx\pgfmath@stacknextoperator\pgfmath@empty%
	\else%
		% Process all operations up to inequalites or addition/subtraction
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@%
			\pgfmathadd@\pgfmathsubtract@}%
	\fi%
	\pgfmath@stackpushoperator{\pgfmathmultiply@}%
	\pgfmath@parse@}
	
\def\pgfmath@parsedivide{%
	% If no operator has been assigned (i.e. / is the first operator scanned),
	% do nothing, except push divide onto the stack.
	\ifx\pgfmath@stacknextoperator\pgfmath@empty%
	\else%
		% Process all operations up to inequalites or addition/subtraction
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@%
			\pgfmathadd@\pgfmathsubtract@}%
	\fi%
	\pgfmath@stackpushoperator{\pgfmathdivide@}%
	\pgfmath@parse@}

\def\pgfmath@parsegreaterthan{%
	% On scanning an equality/inequality operator everything up to
	% (but not including) the operator is evaluated... 
	\pgfmath@processalloperations%
	% ...and the operation pushed onto the stack.
	\pgfmath@stackpushoperator{\pgfmathgreaterthan@}%
	\pgfmath@parse@}

\def\pgfmath@parselessthan{%
	\pgfmath@processalloperations%
	\pgfmath@stackpushoperator{\pgfmathlessthan@}%
	\pgfmath@parse@}

\def\pgfmath@parseequalto={%
	\pgfmath@processalloperations%
	\pgfmath@stackpushoperator{\pgfmathequalto@}%
	\pgfmath@parse@}

\def\pgfmath@parsepower{%
	% Easy, just push power onto the stack.
	\pgfmath@stackpushoperator{\pgfmathpow@}%
	\pgfmath@parse@}

\def\pgfmath@parseradians{%
	% r is a post-fix function...
	\ifx\pgfmath@primaryoperation\pgfmath@empty%
	\else%
		\pgfmath@processoperationsuntil{\pgfmathequalto@\pgfmathlessthan@\pgfmathgreaterthan@%
			\pgfmathadd@\pgfmathsubtract@}%
	\fi%	
	\pgfmath@stackpop{\pgfmath@temp}%
	\pgfmathdeg@{\pgfmath@temp}%
	% ...so processing returns to \pgfmath@parseoperator
	\pgfmath@parseoperator}
	
\newcount\c@pgfmath@parsecounta
\newcount\c@pgfmath@parsecountb
\newcount\c@pgfmath@parsecountc
\newdimen\pgfmath@parsex

% \pgfmath@quickparseoperand
%
% An operand can *only* be a dimension.
%
\def\pgfmath@quickparseoperand{%
	\afterassignment\pgfmath@quickparseoperand@%
	\pgfmath@parsex\pgfmath@token}
\def\pgfmath@quickparseoperand@{%
	\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
	\pgfmath@parseoperator%
}
	
% \pgfmath@parseoperand
%
% An operand can be an ASCII number (with or without dimensions, with
% or without a decimal point), a TeX register (count, dimen or skip,
% which may have expanded with \the), or a function e.g. sin(X).
%
% It is assumed that after \edef-ing, the only unexpanded tokens are registers. 
%
\def\pgfmath@parseoperand{%
	\def\pgfmath@sign{}%
	\expandafter\pgfmath@parseoperandsign\pgfmath@token}
\def\pgfmath@parseoperandsign#1{%
	\pgfmath@in@#1{-+}% 
	\ifpgfmath@in@
		% Gobble multiple signs.
		\edef\pgfmath@sign{\pgfmath@sign#1}%
		\expandafter\pgfmath@parseoperandsign%
	\else%
		\expandafter\pgfmath@parsenumberorfunction\expandafter#1%
	\fi%
}

\newif\ifpgfmath@dimen@

\def\pgfmath@ifregisterdimen@#1\pgfmath@{%
	\pgfmath@in@{p}{#1}%
	\ifpgfmath@in@%
		\pgfmath@dimen@true%
	\else%
		\pgfmath@dimen@false%
	\fi} 			

\def\pgfmath@parsenumberorfunction#1{%
  \let\pgfmath@parsenext\pgfmath@parsenumberorfunction@simple%
  \ifx#1\wd\let\pgfmath@parsenext\pgfmath@boxdimen\fi%
  \ifx#1\ht\let\pgfmath@parsenext\pgfmath@boxdimen\fi%
  \ifx#1\dp\let\pgfmath@parsenext\pgfmath@boxdimen\fi%
  \pgfmath@parsenext#1%
}

\def\pgfmath@boxdimen#1#2{%
  \pgfmath@parsex=\pgfmath@sign#1#2%
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
  \global\pgfmathunitsdeclaredtrue% a dimension has units 
  \pgfmath@parseoperator%
}

\def\pgfmath@parsenumberorfunction@simple#1{%	
	\expandafter\ifcat#1\relax%
		% So, a TeX register.
		\afterassignment\pgfmath@ifregisterdimen@%
		\pgfmath@parsex\pgfmath@sign#1pt\relax\pgfmath@%
		\ifpgfmath@dimen@% 
			% A dimension! So stop scanning operand here.
			\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
         \global\pgfmathunitsdeclaredtrue% a dimension has units
			\def\pgfmath@temp{}%
			\let\pgfmath@parsenext\pgfmath@parseoperator%
		\else%
			% A count! Expand it, but carry on as usual as it might
			% be immediately followed by a dimension.
			\ifdim\pgfmath@parsex<0pt\relax%
				\edef\pgfmath@sign{\pgfmath@sign-}%
				\pgfmath@parsex-\pgfmath@parsex%
			\fi%
			\edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@parsex}}%
			\let\pgfmath@parsenext\pgfmath@parsenumberorfunction@%
		\fi%
	\else%
		% Could be a number or a function...?
		\edef\pgfmath@temp{#1}%
		\let\pgfmath@parsenext\pgfmath@parsenumberorfunction@%
	\fi%
	\expandafter\pgfmath@parsenext\pgfmath@temp%
}%

\def\pgfmath@parsenumberorfunction@#1{%
	\ifx#1(% It might be a group e.g. -(1+2)...
		\let\pgfmath@parsenext\pgfmath@parseoperandgroup%
	\else%
		\pgfmath@in@{#1}{.0123456789}% 
		\ifpgfmath@in@% ... or a number...
			\let\pgfmath@parsenext\pgfmath@parsenumber%
		\else% ... or a function.
			\let\pgfmath@parsenext\pgfmath@parsefunction%
		\fi%
	\fi%
	\pgfmath@parsenext#1%
}%

\def\pgfmath@parseoperandgroup({%
	\let\pgfmath@postparsegroup\pgfmath@@parseoperandgroup%
	\pgfmath@startparsegroup%
}

\def\pgfmath@@parseoperandgroup{%
	\let\pgfmath@postparsegroup\pgfmath@parseoperator%
	\edef\pgfmathresult{\pgfmath@sign\pgfmathresult}%
	\pgfmath@parseoperator%
}

\def\pgfmath@parsenumber{% 
	% Consider the number 3.14159
	% 3 is parsed by assignment to a, then '.' is absorbed and 14159
	% parsed by assignement to b (actually b=114159, see below). 
	\c@pgfmath@parsecountc0\relax%
	\afterassignment\pgfmath@parsedecimalpoint%
	\c@pgfmath@parsecounta0}

\def\pgfmath@parsedecimalpoint#1{%
	\ifx#1.% Is there a decimal point? If not, see if there are any units.
		\let\pgfmath@parsenext\pgfmath@parsemantissa%
	\else%
		\c@pgfmath@parsecountb10\relax% The first digit of b is gobbled (see below). 
		\let\pgfmath@parsenext\pgfmath@parseunits%
	\fi%
	\pgfmath@parsenext#1}



% We would like to assign the following number (which is the mantisse)
% to a number. However, for a very long mantisse as in 3.141592653589793238462643
% this will fail since the number becomes too large.
%
% Because of this, we have to do some ``magic'': We scan 9 tokens and
% then do an assignment with a guard after 9 tokens so that the
% assigment cannot fail.
%
\def\pgfmath@parsemantissa.#1#2#3#4#5#6#7#8#9{%
  \afterassignment\pgfmath@checkforguard%    
  % Consider the number: 2.005
  % 2 is assigned to a, but b will be assigned 5, which is *not right*. 
  % So using 1 here hereresults in  b=1005. The first digit is then  
  % gobbled later, when expanded with \the.
  \c@pgfmath@parsecountb1#1#2#3#4#5#6#7#8#9\relax}%

\def\pgfmath@checkforguard{%
  \pgfmath@ifnextchar\relax%
  {%
    % Ok, this is a looong mantisse. Start gobbling all following
    % numbers
    \pgfmath@gobblemantisse%
  }%
  {%
    \pgfmath@removeguard%
  }%
}

\def\pgfmath@gobblemantisse\relax#1#2#3#4#5#6#7#8#9{%
  \afterassignment\pgfmath@checkforguard%
  \c@pgfmath@parsecountc0#1#2#3#4#5#6#7#8#9\relax% these digits are ignored
}

\def\pgfmath@removeguard#1\relax{\pgfmath@parseunits#1}

 
\def\pgfmath@parseunits#1{%
  % Here the extra first digit in b is gobbled. 
  \edef\pgfmath@resulttemp{%
    \pgfmath@sign\the\c@pgfmath@parsecounta.\expandafter\pgfmath@gobbleone\the\c@pgfmath@parsecountb}%
  % Check whether #1 is a \dp, \wd, or \ht
  \let\pgfmath@parsenext=\pgfmath@parseunits@simple%
  \ifx#1\wd\let\pgfmath@parsenext=\pgfmath@parseunits@boxdimen\fi%
  \ifx#1\ht\let\pgfmath@parsenext=\pgfmath@parseunits@boxdimen\fi%
  \ifx#1\dp\let\pgfmath@parsenext=\pgfmath@parseunits@boxdimen\fi%
  \pgfmath@parsenext#1%
}

\def\pgfmath@parseunits@boxdimen#1#2{%
  \pgfmath@parsex=\pgfmath@sign#1#2%
  \pgfmath@parsex\pgfmath@resulttemp\pgfmath@parsex%
  \edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
  \global\pgfmathunitsdeclaredtrue% a dimension has units 
  \pgfmath@parseoperator%
}

\def\pgfmath@parseunits@simple#1{%
	% Now check if #1 is actually a register.
	\ifcat#1\relax%
		\afterassignment\pgfmath@ifregisterdimen@%
		\pgfmath@parsex#1pt\relax\pgfmath@%
		\pgfmath@parsex\pgfmath@resulttemp\pgfmath@parsex%
		\ifpgfmath@dimen@% If it's a dimen stop scanning operand here.
      \global\pgfmathunitsdeclaredtrue% a dimension has units
			\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
			\let\pgfmath@parsenext\pgfmath@parseoperator%
		\else
			\edef\pgfmath@resulttemp{\pgfmath@tonumber{\pgfmath@parsex}}%
			\let\pgfmath@parsenext\pgfmath@parseunits@%
		\fi%
		\expandafter\pgfmath@parsenext%
	\else%
		\expandafter\pgfmath@parseunits@\expandafter#1%
	\fi}

\def\pgfmath@parseunits@#1#2{%
	% Check if #1 is an operator, or the character `@' indicating the end of the parse.
	\pgfmath@in@#1{@+-*/^r<>=()}%
	\ifpgfmath@in@%
		\edef\pgfmath@tokens{#1#2}%
		\edef\pgfmathresult{\pgfmath@resulttemp}%
		\let\pgfmath@parsenext\pgfmath@parseoperator%
	\else%
		\pgfmath@in@#1{Ee}% e+0X
		\ifpgfmath@in@%
			% Oh no! It might be and em or an ex...
			\pgfmath@in@#2{mx}%
			\ifpgfmath@in@%
				\global\pgfmathunitsdeclaredtrue%
				\pgfmath@parsex\pgfmath@resulttemp#1#2\relax%
				\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
				\edef\pgfmath@tokens{}%
				\let\pgfmath@parsenext\pgfmath@parseoperator%
			\else%
				\edef\pgfmath@tokens{#2}%
				\let\pgfmath@parsenext\pgfmath@parsescientific%
			\fi%
		\else
			% Anything else *should* be a TeX unit.
			\global\pgfmathunitsdeclaredtrue%
			\pgfmath@parsex\pgfmath@resulttemp#1#2\relax%
			\edef\pgfmathresult{\pgfmath@tonumber{\pgfmath@parsex}}%
			\edef\pgfmath@tokens{}%
			\let\pgfmath@parsenext\pgfmath@parseoperator%
	\fi\fi%
	\expandafter\pgfmath@parsenext\pgfmath@tokens%
}

% Parse 'Scientific' notation in the form xEyy
%
\def\pgfmath@parsescientific{%
	\afterassignment\pgfmath@parsescientific@%
	\c@pgfmath@parsecounta}

\def\pgfmath@parsescientific@{%
	\edef\pgfmath@parsesci@temp{\pgfmath@resulttemp\the\c@pgfmath@parsecountc}%
	\expandafter\pgfmathscientific\expandafter{\pgfmath@parsesci@temp}%
		{\the\c@pgfmath@parsecounta}%
	\edef\pgfmath@resulttemp{\pgfmathresult}%
	\pgfmath@parseunits@}

% Functions parsed (not calculated) here are:
%
% round(X)         'half-up' rounding.
% floor(X)         floor function.
% ciel(X)          ceiling function.
% abs(X)           absolute function.
%
% exp(X)           e^X (0 <= X <~= 9.7).
% ln(X)            logarithm of X.
% pow(X,Y)         X^Y,
%
% sin(X)           sine function.
% cos(X)           cosine function.
% tan(X)           tan function.
% asin(X)          arcsine of X (in radians)    -1 <= X <= 1
% acos(X)          arccosine of X (in radians)  -1 <= X <= 1
% atan(X)          arctangent of X (in radians) -1 <= X <= 1
% veclen(X,Y)      the length Z where Z^2 = X^2 + Y^2
% mod(X,Y)         X modulo Y
% max(X,Y)         the maximum of X or Y
% min(X,Y)         the minimum of X or Y
%
% NB veclen, mod, max, and min *cannot* be nested.
%
% deg(X)           converts X to degrees (X in radians)
% rad(X)           converts X to radians (X in degrees)
%
% rnd              generate pseudo-random number X (0 <= X <= 1).
% rand             generate pseudo-random number X (1 <= X <= -1).
% sqrt(X)          square root.
% 
% pi               the constant PI.

\def\pgfmath@parsefunction{%
	\def\pgfmath@parsedfunctionname{}%
	\futurelet\pgfmath@parsetoken\pgfmath@parsefunction@@}
\def\pgfmath@parsefunction@@#1{%
	\pgfmath@in@#1{()@+-*/^<>=}% A function name ends with one of these...
	\ifpgfmath@in@%
		\let\pgfmath@parsefunctionnext\pgfmath@parsefunction@end%
	\else%
		\ifx\pgfmath@parsetoken\pgfmath@sptoken% ...or a space.
			\let\pgfmath@parsefunctionnext\pgfmath@parsefunction@end%
		\else%
			\let\pgfmath@parsefunctionnext\pgfmath@parsefunction@continue%
	\fi\fi%
	\pgfmath@parsefunctionnext#1}

\def\pgfmath@parsefunction@end#1{%
	\expandafter\ifx\csname pgfmath@parsefunction@\pgfmath@parsedfunctionname\endcsname\relax%
		\pgfmath@reportunknownfunction%
		\let\pgfmath@parsefunctionnext\relax%
	\else%
		\let\pgfmath@parsefunctionnext\pgfmath@executeparsefunction@%
	\fi%
	\pgfmath@parsefunctionnext#1}

\def\pgfmath@parsefunction@continue#1{%
	\edef\pgfmath@parsedfunctionname{\pgfmath@parsedfunctionname#1}%
	\futurelet\pgfmath@parsetoken\pgfmath@parsefunction@@}
	
\def\pgfmath@executeparsefunction@{\csname pgfmath@parsefunction@\pgfmath@parsedfunctionname\endcsname}
		
		
\def\pgfmath@reportunknownfunction{%
	\pgfmath@error{Unknown function `\pgfmath@parsedfunctionname'}{}%
}

% \pgfmath@postfunction
% 
% In scanning a function e.g. sin(40), we subvert the normal parsing 
% group mechanism by messing around with \pgfmath@parsepostgroup, so 
% that after scanning ), the parser doesn't scan for an operator, but 
% returns to the macros scanning the function. 
% Here the mechanism is restored, and the value of the function is 
% stored along with the approprate sign, which was saved earlier.
%
\def\pgfmath@postfunction{%
	\let\pgfmath@parsepostgroup\pgfmath@parseoperator%
	\edef\pgfmathresult{\pgfmath@sign\pgfmathresult}%
	\pgfmath@parseoperator}
	

% \pgfmath@parsefunction@abs
%
\def\pgfmath@parsefunction@abs{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@abs@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@abs@{%	
	\expandafter\pgfmathabs@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@sqrt
%
\def\pgfmath@parsefunction@sqrt{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@sqrt@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@sqrt@{%	
	\expandafter\pgfmathsqrt@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@round
%
\def\pgfmath@parsefunction@round{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@round@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@round@{%	
	\expandafter\pgfmathround@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@floor
%
\def\pgfmath@parsefunction@floor{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@floor@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@floor@{%	
	\expandafter\pgfmathfloor@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@ceil
%
\def\pgfmath@parsefunction@ceil{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@ceil@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@ceil@{%	
	\expandafter\pgfmathceil@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@sin
%
\def\pgfmath@parsefunction@sin{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@sin@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@sin@{%	
	\expandafter\pgfmathsin@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@cos
%
\def\pgfmath@parsefunction@cos{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@cos@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@cos@{%	
	\expandafter\pgfmathcos@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@asin
%
\def\pgfmath@parsefunction@asin{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@asin@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@asin@{%	
	\expandafter\pgfmathasin@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@acos
%
\def\pgfmath@parsefunction@acos{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@acos@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@acos@{%	
	\expandafter\pgfmathacos@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction}

% \pgfmath@parsefunction@atan
%
\def\pgfmath@parsefunction@atan{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@atan@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@atan@{%	
	\expandafter\pgfmathatan@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@tan
%
\def\pgfmath@parsefunction@tan{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@tan@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@tan@{%	
	\expandafter\pgfmathtan@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@cot
%
\def\pgfmath@parsefunction@cot{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@cot@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@cot@{%	
	\expandafter\pgfmathcot@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@sec
%
\def\pgfmath@parsefunction@sec{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@sec@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@sec@{%	
	\expandafter\pgfmathsec@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@cosec
%
\def\pgfmath@parsefunction@cosec{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@cosec@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@cosec@{%	
	\expandafter\pgfmathcosec@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@rad
%
\def\pgfmath@parsefunction@rad{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@rad@%
	\pgfmath@parse@}
\def\pgfmath@parsefunction@rad@{%
	\expandafter\pgfmathrad@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction}%
	
% \pgfmath@parsefunction@rad
%
\def\pgfmath@parsefunction@deg{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@deg@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@deg@{%
	\expandafter\pgfmathdeg@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction}%
	
% \pgfmath@parsefunction@rnd
%
\def\pgfmath@parsefunction@rnd{%
	\expandafter\pgfmathrnd%
	\expandafter\pgfmath@postfunction}
			
% \pgfmath@parsefunction@rand
%
\def\pgfmath@parsefunction@rand{%
	\expandafter\pgfmathrand%
	\expandafter\pgfmath@postfunction}%
			
% \pgfmath@parsefunction@exp
%
\def\pgfmath@parsefunction@exp{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@exp@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@exp@{%	
	\expandafter\pgfmathexp@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@ln
%
\def\pgfmath@parsefunction@ln{%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@ln@%
	\expandafter\pgfmath@parse@}
\def\pgfmath@parsefunction@ln@{%	
	\expandafter\pgfmathln@\expandafter{\pgfmathresult}%
	\pgfmath@postfunction%
}
	
% \pgfmath@parsefunction@pi
%
\def\pgfmath@parsefunction@pi{%
	\pgfmathpi%
	\pgfmath@postfunction%
}

% \pgfmath@parsefunction@veclen
%
\def\pgfmath@parsefunction@veclen{%
	\expandafter\pgfmath@parsefunction@veclen@}
\def\pgfmath@parsefunction@veclen@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@veclen@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@veclen@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathveclen@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}

% \pgfmath@parsefunction@mod 
%
\def\pgfmath@parsefunction@mod{%
	\expandafter\pgfmath@parsefunction@mod@}
\def\pgfmath@parsefunction@mod@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@mod@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@mod@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathmod@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}

% \pgfmath@parsefunction@max
%
\def\pgfmath@parsefunction@max{%
	\expandafter\pgfmath@parsefunction@max@}
\def\pgfmath@parsefunction@max@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@max@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@max@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathmax@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}	

% \pgfmath@parsefunction@min 
%
\def\pgfmath@parsefunction@min{%
	\expandafter\pgfmath@parsefunction@min@}
\def\pgfmath@parsefunction@min@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@min@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@min@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathmin@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}
	
% \pgfmath@parsefunction@pow 
%
\def\pgfmath@parsefunction@pow{%
	\expandafter\pgfmath@parsefunction@pow@}
\def\pgfmath@parsefunction@pow@(#1,{%
	\pgfmathparse@{#1}\edef\pgfmath@firstoperand{\pgfmathresult}%
	\let\pgfmath@parsepostgroup\pgfmath@parsefunction@pow@@
	\pgfmath@startparsegroup}
\def\pgfmath@parsefunction@pow@@{%
	\edef\pgfmath@secondoperand{\pgfmathresult}%
	\pgfmathpow@{\pgfmath@firstoperand}{\pgfmath@secondoperand}%
	\pgfmath@postfunction}	

==> pgfmathrnd.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the pesudorandom numbers.
%
% Version 1.414213 29/9/2007

% Pseudo-random number generation.
%
% See:
% \book@{pressetal1992,
%    author    = {William H. Press and Brian P. Flannery and Saul A. 
%                 Teukolsky and William T. Vetterling}, 
%    title     = {Numerical Recipies in C},
%    edition   = {Second},
%    publisher = {Cambridge University Press}
% }
%
% See also, the documentation for the lcg package by Erich Janka:
% (http://www.ctan.org/tex-archive/macros/latex/contrib/lcg/lcg.pdf)
%
\def\pgfmath@rnd@m{2147483647}% LaTeX Maximum.

\begingroup
\c@pgfmath@counta=\time%
\multiply\c@pgfmath@counta by\year%
\xdef\pgfmath@rnd@z{\the\c@pgfmath@counta}% The seed. 
\endgroup

% \pgfmathsetseed
%
% Explictly set the seed for the generator
%   
% #1 -> the new seed.
%
\def\pgfmathsetseed#1{\pgfmathparse{#1}\expandafter\pgfmath@setseed\pgfmathresult\relax}%
\def\pgfmath@setseed#1.#2\relax{\def\pgfmath@rnd@z{#1}}%  

% Alternative paramaters - see Press et al (1992) p278-279, 
% for discussion.
%
% a=16807 q=127773 r=2836
% a=48271 q=4488   r=3399
%
\def\pgfmath@rnd@a{69621}
\def\pgfmath@rnd@r{23902}
\def\pgfmath@rnd@q{30845}

% \pgfmathgeneratepseudorandomnumber
% 
% A linear congruency generator for generating
% pseudo-random numbers. Generates numbers in
% the range 1 - 2^31-1.
%
\def\pgfmathgeneratepseudorandomnumber{%
	\begingroup%
		\c@pgfmath@counta=\pgfmath@rnd@z%
		\c@pgfmath@countb=\pgfmath@rnd@z%
		\c@pgfmath@countc=\pgfmath@rnd@q%
		\divide\c@pgfmath@counta by\c@pgfmath@countc%
		\multiply\c@pgfmath@counta by-\c@pgfmath@countc%
		\advance\c@pgfmath@counta by\c@pgfmath@countb
		\c@pgfmath@countc=\pgfmath@rnd@a%
		\multiply\c@pgfmath@counta by\c@pgfmath@countc%
		\c@pgfmath@countc=\pgfmath@rnd@q%
		\divide\c@pgfmath@countb by\c@pgfmath@countc%
		\c@pgfmath@countc=\pgfmath@rnd@r%
		\multiply\c@pgfmath@countb by\c@pgfmath@countc%
		\advance\c@pgfmath@counta by-\c@pgfmath@countb%
		\ifnum\c@pgfmath@counta<0\relax%
			\c@pgfmath@countb=\pgfmath@rnd@m%
			\advance\c@pgfmath@counta by\c@pgfmath@countb%
		\fi%
		\xdef\pgfmath@rnd@z{\the\c@pgfmath@counta}%
	\endgroup%
	\edef\pgfmathresult{\pgfmath@rnd@z}%
}

% \pgfmathrnd
%
% Generates a pseudo-random number between 0 and 1.
%
\def\pgfmathrnd{%
	\begingroup%
		\pgfmathgeneratepseudorandomnumber%
		\c@pgfmath@counta\pgfmathresult%
		\c@pgfmath@countb\c@pgfmath@counta%
		\divide\c@pgfmath@countb100001\relax% To get one.
		\multiply\c@pgfmath@countb-100001\relax%
		\advance\c@pgfmath@countb\c@pgfmath@counta%
		\advance\c@pgfmath@countb1000000\relax%
		\expandafter\pgfmathrnd@\the\c@pgfmath@countb\pgfmath@%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

\def\pgfmathrnd@#1#2#3\pgfmath@{%
	\edef\pgfmath@temp{#2.#3}%
	\pgfmath@x=\pgfmath@temp pt\relax%
}%

% \pgfmathrand
%
% Generates a pseudo-random number between -1 and 1.
%
\def\pgfmathrand{%
	\begingroup%
		\pgfmathgeneratepseudorandomnumber%
		\c@pgfmath@counta\pgfmathresult%
		\c@pgfmath@countb\c@pgfmath@counta%
		\divide\c@pgfmath@countb200001\relax%
		\multiply\c@pgfmath@countb-200001\relax%
		\advance\c@pgfmath@countb\c@pgfmath@counta%
		\advance\c@pgfmath@countb-100000\relax%
		\ifnum\c@pgfmath@countb<0\relax%
			\advance\c@pgfmath@countb-1000000\relax%
		\else%
			\advance\c@pgfmath@countb1000000\relax%
		\fi%
		\expandafter\pgfmathrand@\the\c@pgfmath@countb\pgfmath@%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

\def\pgfmathrand@#1#2#3#4\pgfmath@{%
	\ifx#1-%
		\edef\pgfmath@temp{-#3.#4}%
	\else%
		\edef\pgfmath@temp{#2.#3#4}%
	\fi%
	\pgfmath@x=\pgfmath@temp pt\relax%
}%

% \pgfmathrandominteger
%
% Return a 'randomly' selected integer in the range #2 - #3 (inclusive).
%
% #1 - a macro to store the integer (not a count register).
% #2 - the lower limit of the range.
% #3 - the upper limit of the range.
%
\def\pgfmathrandominteger#1#2#3{%
	\begingroup%
		\pgfmathgeneratepseudorandomnumber%
		\c@pgfmath@counta#2\relax%
		\c@pgfmath@countb#3\relax%
		\c@pgfmath@countc\c@pgfmath@countb%
		% OK. Maybe #2 > #3.
		\ifnum\c@pgfmath@counta>\c@pgfmath@countb\relax%
			\c@pgfmath@countc\c@pgfmath@countb%
			\c@pgfmath@countb\c@pgfmath@counta%
			\c@pgfmath@counta\c@pgfmath@countc%
		\fi%
		\advance\c@pgfmath@countc1\relax%
		\advance\c@pgfmath@countc-\c@pgfmath@counta%
		\c@pgfmath@counta\pgfmathresult\relax%
		\c@pgfmath@countb\c@pgfmath@counta%
		\divide\c@pgfmath@countb\c@pgfmath@countc%
		\multiply\c@pgfmath@countb-\c@pgfmath@countc%
		\advance\c@pgfmath@counta\c@pgfmath@countb%
		\advance\c@pgfmath@counta#2\relax%
		\edef\pgfmathresult{\the\c@pgfmath@counta}%
		\pgfmath@smuggleone{\pgfmathresult}%
	\endgroup%
	\edef#1{\pgfmathresult}%
}

% \pgfmathdeclarerandomlist
%
% Create a list to be used with \pgfmathrandomelement.
%
% #1 - the name of the list
% #2 - a list of comma separated elements.
%
\def\pgfmathdeclarerandomlist#1#2{%
	\def\pgfmath@randomlistname{#1}%
	\begingroup%
		\c@pgfmath@counta=1\relax%
		% {} is a possible random element so (locally) 
		% redefine \pgfmath@empty.
		\def\pgfmath@empty{pgfmath@empty}% 
		\expandafter\pgfmath@scanrandomlist#2{pgfmath@empty}}
\def\pgfmath@scanrandomlist#1{%
	\def\pgfmath@scanneditem{#1}%
	\ifx\pgfmath@scanneditem\pgfmath@empty%
		\advance\c@pgfmath@counta-1\relax%
		\expandafter\xdef\csname pgfmath@randomlist@\pgfmath@randomlistname\endcsname{\the\c@pgfmath@counta}%
		\endgroup%	
	\else%
		\expandafter\gdef\csname pgfmath@randomlist@\pgfmath@randomlistname @\the\c@pgfmath@counta\endcsname{#1}%
		\advance\c@pgfmath@counta1\relax%
		\expandafter\pgfmath@scanrandomlist%
	\fi}

% \pgfmathrandomitem
%
% Return a 'randomly' selected element from a list.
%
% #1 - a macro to store the item.
% #2 - the name of the list.
%
\def\pgfmathrandomitem#1#2{%
	\pgfmath@ifundefined{pgfmath@randomlist@#2}{\pgfmath@error{Unknown random list `#2'}}{%
		\edef\pgfmath@randomlistlength{\csname pgfmath@randomlist@#2\endcsname}%
		\pgfmathrandominteger{\pgfmath@randomtemp}{1}{\pgfmath@randomlistlength}%
		\def#1{\csname pgfmath@randomlist@#2@\pgfmath@randomtemp\endcsname}}}

==> pgfmathtrig.code.tex <==
% Copyright 2007 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file defines the trigonometric functions/operations.
%
% Much of this file is based on ideas and code (particularly 
% the old \pgfcoremath.code.tex) due to Till Tantau.
%
% Version 1.414213 29/9/2007

% \pgfmathpi
%
\def\pgfmathpi{\edef\pgfmathresult{\pgfmath@pi}}
\def\pgfmath@pi{3.14159}

% \pgfmathradians 
% (for comptability with 1.18 beta, will be deprecated)
% 
% Convert #1 from radians to degrees (accurate to 1 deg).
%
\def\pgfmathradians#1{%
	\pgfmathparse{#1}%
	\pgfmathradians@{\pgfmathresult}}
\def\pgfmathradians@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@x57.29577\pgfmath@x\relax% 57.29577 = 360/(2*pi)
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathdeg
% 
% Convert #1 from radians to degrees.
%
\def\pgfmathdeg#1{%
	\pgfmathparse{#1}%
	\pgfmathdeg@{\pgfmathresult}}
\def\pgfmathdeg@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@x57.29577\pgfmath@x\relax% 57.29577 = 360/(2*pi)
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathrad
% 
% Convert #1 from degrees to radians.
%
\def\pgfmathrad#1{%
	\pgfmathparse{#1}%
	\pgfmathrad@{\pgfmathresult}}
\def\pgfmathrad@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@x3.14159\pgfmath@x% 
		\divide\pgfmath@x180\relax%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}%

% \pgfmathsin
% 
% Calculate the sine of #1 (in degrees).
%
\def\pgfmathsin#1{%
	\pgfmathparse{#1}%
	\pgfmathsin@{\pgfmathresult}}
\def\pgfmathsin@#1{%
	% Let #1 = a.b
	% Then sin(#1) \approx (1-b)*sin(a) + b*sin(a+1)
	%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\advance\pgfmath@x-90pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@
		\divide\c@pgfmath@counta360\relax%
		\multiply\c@pgfmath@counta-360\relax%
		\advance\pgfmath@x\c@pgfmath@counta pt\relax%
		\ifdim\pgfmath@x<0pt\relax\pgfmath@x-\pgfmath@x\fi%
		\ifdim\pgfmath@x<180pt\relax%
		\else
			\pgfmath@x-\pgfmath@x%
			\advance\pgfmath@x360pt\relax%
		\fi%
		% Now 0 <= x < 179. So split x into integer and decimal...
		%
		\afterassignment\pgfmath@xa%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		%
		% ...if #1 is an integer, don't do anything fancy.
		\ifdim\pgfmath@xa=0pt%
			\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname pt\relax%
		\else%
			\pgfmath@x-\pgfmath@xa%
			\advance\pgfmath@x1pt\relax%
			\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@x%
			\advance\c@pgfmath@counta1\relax%
			\expandafter\advance\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@xa%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup
}

% \pgfmathcos
% 
% Calculate the cosine of #1 (in degrees).
%
\def\pgfmathcos#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathcos@\expandafter{\pgfmathresult}}
\def\pgfmathcos@#1{%
	% Let x = a.b
	% Then cos(x) \approx (1-b)*cos(a) + b*cos(a+1)
	%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@% 
		\divide\c@pgfmath@counta360\relax%
		\multiply\c@pgfmath@counta-360\relax%
		\advance\pgfmath@x\c@pgfmath@counta pt\relax%
		\ifdim\pgfmath@x<0pt\relax\pgfmath@x-\pgfmath@x\fi%
		\ifdim\pgfmath@x<180pt\relax%
		\else%
			\pgfmath@x-\pgfmath@x%
			\advance\pgfmath@x360pt\relax%
		\fi%
		% Now 0 <= x < 179. So split x into integer and decimal...
		%
		\afterassignment\pgfmath@xa%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		%
		% ...if #1 is an integer, don't do anything fancy.
		\ifdim\pgfmath@xa=0pt%
			\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname pt%
		\else%
			\pgfmath@x-\pgfmath@xa%
			\advance\pgfmath@x1pt\relax%
			\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@x%
			\advance\c@pgfmath@counta1\relax%
			\ifnum\c@pgfmath@counta=181\relax\c@pgfmath@counta179\relax\fi%
			\expandafter\advance\expandafter\pgfmath@x\csname pgfmath@cos@\the\c@pgfmath@counta\endcsname\pgfmath@xa%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathsincos
% 
% Calculate the sin and cosine of #1 (in degrees).
%
\def\pgfmathsincos#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathsincos@\expandafter{\pgfmathresult}}
\def\pgfmathsincos@#1{%
	\edef\pgfmath@temparg{#1}%
	\pgfmathsin@{\pgfmath@temparg}\edef\pgfmathresulty{\pgfmathresult}%
	\pgfmathcos@{\pgfmath@temparg}\edef\pgfmathresultx{\pgfmathresult}%
}

% \pgfmathtan
% 
% Calculate the tangent of #1 (in degrees).
%
\def\pgfmathtan#1{%
	\pgfmathparse{#1}%
	\pgfmathtan@{\pgfmathresult}}
\def\pgfmathtan@#1{%
	\begingroup%
		\edef\pgfmath@temparg{#1}%
		\pgfmathcos@{\pgfmath@temparg}%
		\expandafter\pgfmathreciprocal@\expandafter{\pgfmathresult}%
		\edef\pgfmath@tantemp{\pgfmathresult}%
		\pgfmathsin@{\pgfmath@temparg}%
		\pgfmath@x\pgfmathresult pt\relax%
		\pgfmath@x\pgfmath@tantemp\pgfmath@x%
		\ifdim\pgfmath@x<0pt\relax%
			\c@pgfmath@countb-1\relax%
		\else%
			\c@pgfmath@countb1\relax%
		\fi%
		% Adjust to 4 decimal places. This gets rid of some annoyingly tiny errors.
		\afterassignment\pgfmath@x%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		\ifdim\pgfmath@x<.0001pt\relax%
			\pgfmath@x0pt\relax%
		\fi%
		\advance\pgfmath@x\c@pgfmath@counta pt%
		\multiply\pgfmath@x\c@pgfmath@countb%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathcosec
% 
% Calculate the cosec of #1 (in degrees).
%
\def\pgfmathcosec#1{%
	\pgfmathparse{#1}%
	\pgfmathcosec@{\pgfmathresult}}
\def\pgfmathcosec@#1{%
	\expandafter\pgfmathsin@\expandafter{#1}%
	\pgfmathreciprocal@{\pgfmathresult}%
}

% \pgfmathsec
% 
% Calculate the sec of #1 (in degrees).
%
\def\pgfmathsec#1{%
	\pgfmathparse{#1}%
	\pgfmathsec@{\pgfmathresult}}
\def\pgfmathsec@#1{%
	\expandafter\pgfmathcos@\expandafter{#1}%
	\pgfmathreciprocal@{\pgfmathresult}%
}

% \pgfmathcot
% 
% Calculate the cotangent of #1 (in degrees).
%
\def\pgfmathcot#1{%
	\pgfmathparse{#1}%
	\pgfmathcot@{\pgfmathresult}}
\def\pgfmathcot@#1{%
	\begingroup%
		\edef\pgfmath@temparg{#1}%
		\pgfmathsin@{\pgfmath@temparg}%
		\expandafter\pgfmathreciprocal@\expandafter{\pgfmathresult}%
		\edef\pgfmath@tantemp{\pgfmathresult}%
		\pgfmathcos@{\pgfmath@temparg}%
		\pgfmath@x\pgfmathresult pt\relax%
		\pgfmath@x\pgfmath@tantemp\pgfmath@x%
		\ifdim\pgfmath@x<0pt\relax%
			\c@pgfmath@countb-1\relax%
		\else%
			\c@pgfmath@countb1\relax%
		\fi%
		% Adjust to 4 decimal places. This gets rid of some annoyingly tiny errors.
		\afterassignment\pgfmath@x%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax%
		\ifdim\pgfmath@x<.0001pt\relax%
			\pgfmath@x0pt\relax%
		\fi%
		\advance\pgfmath@x\c@pgfmath@counta pt%
		\multiply\pgfmath@x\c@pgfmath@countb%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathasin
%
% The asin of #1
%
\def\pgfmathasin#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathasin@\expandafter{\pgfmathresult}}
\def\pgfmathasin@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@xa\pgfmath@x%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@x1000\pgfmath@x%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\pgfmath@x-\csname pgfmath@acos@\the\c@pgfmath@counta\endcsname pt\relax%
		\advance\pgfmath@x90pt\relax%
		\ifdim\pgfmath@xa<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathacos
%
% The acos of #1
%	
\def\pgfmathacos#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathacos@\expandafter{\pgfmathresult}}
\def\pgfmathacos@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@xa\pgfmath@x%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@x1000\pgfmath@x%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\expandafter\pgfmath@x\csname pgfmath@acos@\the\c@pgfmath@counta\endcsname pt\relax%
		\ifdim\pgfmath@xa<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

% \pgfmathasin
%
% The atan of #1
%
\def\pgfmathatan#1{%
	\pgfmathparse{#1}%
	\expandafter\pgfmathatan@\expandafter{\pgfmathresult}}
\def\pgfmathatan@#1{%
	\begingroup%
		\expandafter\pgfmath@x#1pt\relax%
		\pgfmath@xa\pgfmath@x%
		\ifdim\pgfmath@x<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@xb\pgfmath@x%
		\ifdim\pgfmath@x>1pt\relax%
			\edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@x}}%
			\pgfmathreciprocal@{\pgfmath@temp}%
			\pgfmath@x\pgfmathresult pt\relax%
		\fi%
		\pgfmath@x1000\pgfmath@x%
		\afterassignment\pgfmath@gobbletilpgfmath@%
		\expandafter\c@pgfmath@counta\the\pgfmath@x\relax\pgfmath@%
		\ifdim\pgfmath@xb>1pt\relax%
			\expandafter\pgfmath@x\expandafter-\csname pgfmath@atan@\the\c@pgfmath@counta\endcsname pt\relax%
			\advance\pgfmath@x90pt%
		\else%
			\expandafter\pgfmath@x\csname pgfmath@atan@\the\c@pgfmath@counta\endcsname pt\relax%
		\fi%
		\ifdim\pgfmath@xa<0pt\relax%
			\pgfmath@x-\pgfmath@x%
		\fi%
		\pgfmath@returnone\pgfmath@x%
	\endgroup%
}

	
\def\pgfmath@def#1#2#3{\expandafter\def\csname pgfmath@#1@#2\endcsname{#3}}
\pgfmath@def{cos}{0}{1.00000}		\pgfmath@def{cos}{1}{0.99985}
\pgfmath@def{cos}{2}{0.99939}		\pgfmath@def{cos}{3}{0.99863}
\pgfmath@def{cos}{4}{0.99756}		\pgfmath@def{cos}{5}{0.99619}
\pgfmath@def{cos}{6}{0.99452}		\pgfmath@def{cos}{7}{0.99255}
\pgfmath@def{cos}{8}{0.99027}		\pgfmath@def{cos}{9}{0.98769}
\pgfmath@def{cos}{10}{0.98481}		\pgfmath@def{cos}{11}{0.98163}
\pgfmath@def{cos}{12}{0.97815}		\pgfmath@def{cos}{13}{0.97437}
\pgfmath@def{cos}{14}{0.97030}		\pgfmath@def{cos}{15}{0.96593}
\pgfmath@def{cos}{16}{0.96126}		\pgfmath@def{cos}{17}{0.95630}
\pgfmath@def{cos}{18}{0.95106}		\pgfmath@def{cos}{19}{0.94552}
\pgfmath@def{cos}{20}{0.93969}		\pgfmath@def{cos}{21}{0.93358}
\pgfmath@def{cos}{22}{0.92718}		\pgfmath@def{cos}{23}{0.92050}
\pgfmath@def{cos}{24}{0.91355}		\pgfmath@def{cos}{25}{0.90631}
\pgfmath@def{cos}{26}{0.89879}		\pgfmath@def{cos}{27}{0.89101}
\pgfmath@def{cos}{28}{0.88295}		\pgfmath@def{cos}{29}{0.87462}
\pgfmath@def{cos}{30}{0.86603}		\pgfmath@def{cos}{31}{0.85717}
\pgfmath@def{cos}{32}{0.84805}		\pgfmath@def{cos}{33}{0.83867}
\pgfmath@def{cos}{34}{0.82904}		\pgfmath@def{cos}{35}{0.81915}
\pgfmath@def{cos}{36}{0.80902}		\pgfmath@def{cos}{37}{0.79864}
\pgfmath@def{cos}{38}{0.78801}		\pgfmath@def{cos}{39}{0.77715}
\pgfmath@def{cos}{40}{0.76604}		\pgfmath@def{cos}{41}{0.75471}
\pgfmath@def{cos}{42}{0.74314}		\pgfmath@def{cos}{43}{0.73135}
\pgfmath@def{cos}{44}{0.71934}		\pgfmath@def{cos}{45}{0.70711}
\pgfmath@def{cos}{46}{0.69466}		\pgfmath@def{cos}{47}{0.68200}
\pgfmath@def{cos}{48}{0.66913}		\pgfmath@def{cos}{49}{0.65606}
\pgfmath@def{cos}{50}{0.64279}		\pgfmath@def{cos}{51}{0.62932}
\pgfmath@def{cos}{52}{0.61566}		\pgfmath@def{cos}{53}{0.60182}
\pgfmath@def{cos}{54}{0.58779}		\pgfmath@def{cos}{55}{0.57358}
\pgfmath@def{cos}{56}{0.55919}		\pgfmath@def{cos}{57}{0.54464}
\pgfmath@def{cos}{58}{0.52992}		\pgfmath@def{cos}{59}{0.51504}
\pgfmath@def{cos}{60}{0.50000}		\pgfmath@def{cos}{61}{0.48481}
\pgfmath@def{cos}{62}{0.46947}		\pgfmath@def{cos}{63}{0.45399}
\pgfmath@def{cos}{64}{0.43837}		\pgfmath@def{cos}{65}{0.42262}
\pgfmath@def{cos}{66}{0.40674}		\pgfmath@def{cos}{67}{0.39073}
\pgfmath@def{cos}{68}{0.37461}		\pgfmath@def{cos}{69}{0.35837}
\pgfmath@def{cos}{70}{0.34202}		\pgfmath@def{cos}{71}{0.32557}
\pgfmath@def{cos}{72}{0.30902}		\pgfmath@def{cos}{73}{0.29237}
\pgfmath@def{cos}{74}{0.27564}		\pgfmath@def{cos}{75}{0.25882}
\pgfmath@def{cos}{76}{0.24192}		\pgfmath@def{cos}{77}{0.22495}
\pgfmath@def{cos}{78}{0.20791}		\pgfmath@def{cos}{79}{0.19081}
\pgfmath@def{cos}{80}{0.17365}		\pgfmath@def{cos}{81}{0.15643}
\pgfmath@def{cos}{82}{0.13917}		\pgfmath@def{cos}{83}{0.12187}
\pgfmath@def{cos}{84}{0.10453}		\pgfmath@def{cos}{85}{0.08716}
\pgfmath@def{cos}{86}{0.06976}		\pgfmath@def{cos}{87}{0.05234}
\pgfmath@def{cos}{88}{0.03490}		\pgfmath@def{cos}{89}{0.01745}
\pgfmath@def{cos}{90}{0.00000}		\pgfmath@def{cos}{91}{-0.01745}
\pgfmath@def{cos}{92}{-0.03490}		\pgfmath@def{cos}{93}{-0.05234}
\pgfmath@def{cos}{94}{-0.06976}		\pgfmath@def{cos}{95}{-0.08716}
\pgfmath@def{cos}{96}{-0.10453}		\pgfmath@def{cos}{97}{-0.12187}
\pgfmath@def{cos}{98}{-0.13917}		\pgfmath@def{cos}{99}{-0.15643}
\pgfmath@def{cos}{100}{-0.17365}		\pgfmath@def{cos}{101}{-0.19081}
\pgfmath@def{cos}{102}{-0.20791}		\pgfmath@def{cos}{103}{-0.22495}
\pgfmath@def{cos}{104}{-0.24192}		\pgfmath@def{cos}{105}{-0.25882}
\pgfmath@def{cos}{106}{-0.27564}		\pgfmath@def{cos}{107}{-0.29237}
\pgfmath@def{cos}{108}{-0.30902}		\pgfmath@def{cos}{109}{-0.32557}
\pgfmath@def{cos}{110}{-0.34202}		\pgfmath@def{cos}{111}{-0.35837}
\pgfmath@def{cos}{112}{-0.37461}		\pgfmath@def{cos}{113}{-0.39073}
\pgfmath@def{cos}{114}{-0.40674}		\pgfmath@def{cos}{115}{-0.42262}
\pgfmath@def{cos}{116}{-0.43837}		\pgfmath@def{cos}{117}{-0.45399}
\pgfmath@def{cos}{118}{-0.46947}		\pgfmath@def{cos}{119}{-0.48481}
\pgfmath@def{cos}{120}{-0.50000}		\pgfmath@def{cos}{121}{-0.51504}
\pgfmath@def{cos}{122}{-0.52992}		\pgfmath@def{cos}{123}{-0.54464}
\pgfmath@def{cos}{124}{-0.55919}		\pgfmath@def{cos}{125}{-0.57358}
\pgfmath@def{cos}{126}{-0.58779}		\pgfmath@def{cos}{127}{-0.60182}
\pgfmath@def{cos}{128}{-0.61566}		\pgfmath@def{cos}{129}{-0.62932}
\pgfmath@def{cos}{130}{-0.64279}		\pgfmath@def{cos}{131}{-0.65606}
\pgfmath@def{cos}{132}{-0.66913}		\pgfmath@def{cos}{133}{-0.68200}
\pgfmath@def{cos}{134}{-0.69466}		\pgfmath@def{cos}{135}{-0.70711}
\pgfmath@def{cos}{136}{-0.71934}		\pgfmath@def{cos}{137}{-0.73135}
\pgfmath@def{cos}{138}{-0.74314}		\pgfmath@def{cos}{139}{-0.75471}
\pgfmath@def{cos}{140}{-0.76604}		\pgfmath@def{cos}{141}{-0.77715}
\pgfmath@def{cos}{142}{-0.78801}		\pgfmath@def{cos}{143}{-0.79864}
\pgfmath@def{cos}{144}{-0.80902}		\pgfmath@def{cos}{145}{-0.81915}
\pgfmath@def{cos}{146}{-0.82904}		\pgfmath@def{cos}{147}{-0.83867}
\pgfmath@def{cos}{148}{-0.84805}		\pgfmath@def{cos}{149}{-0.85717}
\pgfmath@def{cos}{150}{-0.86603}		\pgfmath@def{cos}{151}{-0.87462}
\pgfmath@def{cos}{152}{-0.88295}		\pgfmath@def{cos}{153}{-0.89101}
\pgfmath@def{cos}{154}{-0.89879}		\pgfmath@def{cos}{155}{-0.90631}
\pgfmath@def{cos}{156}{-0.91355}		\pgfmath@def{cos}{157}{-0.92050}
\pgfmath@def{cos}{158}{-0.92718}		\pgfmath@def{cos}{159}{-0.93358}
\pgfmath@def{cos}{160}{-0.93969}		\pgfmath@def{cos}{161}{-0.94552}
\pgfmath@def{cos}{162}{-0.95106}		\pgfmath@def{cos}{163}{-0.95630}
\pgfmath@def{cos}{164}{-0.96126}		\pgfmath@def{cos}{165}{-0.96593}
\pgfmath@def{cos}{166}{-0.97030}		\pgfmath@def{cos}{167}{-0.97437}
\pgfmath@def{cos}{168}{-0.97815}		\pgfmath@def{cos}{169}{-0.98163}
\pgfmath@def{cos}{170}{-0.98481}		\pgfmath@def{cos}{171}{-0.98769}
\pgfmath@def{cos}{172}{-0.99027}		\pgfmath@def{cos}{173}{-0.99255}
\pgfmath@def{cos}{174}{-0.99452}		\pgfmath@def{cos}{175}{-0.99619}
\pgfmath@def{cos}{176}{-0.99756}		\pgfmath@def{cos}{177}{-0.99863}
\pgfmath@def{cos}{178}{-0.99939}		\pgfmath@def{cos}{179}{-0.99985}
\pgfmath@def{cos}{180}{-1.00000}	   \pgfmath@def{cos}{181}{-0.99985}

\pgfmath@def{cosfrac}{0}{1.00000}		\pgfmath@def{cosfrac}{1}{0.99995}
\pgfmath@def{cosfrac}{2}{0.99980}		\pgfmath@def{cosfrac}{3}{0.99955}
\pgfmath@def{cosfrac}{4}{0.99920}		\pgfmath@def{cosfrac}{5}{0.99875}
\pgfmath@def{cosfrac}{6}{0.99820}		\pgfmath@def{cosfrac}{7}{0.99755}
\pgfmath@def{cosfrac}{8}{0.99681}		\pgfmath@def{cosfrac}{9}{0.99597}
\pgfmath@def{cosfrac}{10}{0.99503}		\pgfmath@def{cosfrac}{11}{0.99400}
\pgfmath@def{cosfrac}{12}{0.99287}		\pgfmath@def{cosfrac}{13}{0.99165}
\pgfmath@def{cosfrac}{14}{0.99034}		\pgfmath@def{cosfrac}{15}{0.98893}
\pgfmath@def{cosfrac}{16}{0.98744}		\pgfmath@def{cosfrac}{17}{0.98585}
\pgfmath@def{cosfrac}{18}{0.98418}		\pgfmath@def{cosfrac}{19}{0.98242}
\pgfmath@def{cosfrac}{20}{0.98058}		\pgfmath@def{cosfrac}{21}{0.97865}
\pgfmath@def{cosfrac}{22}{0.97664}		\pgfmath@def{cosfrac}{23}{0.97455}
\pgfmath@def{cosfrac}{24}{0.97238}		\pgfmath@def{cosfrac}{25}{0.97014}
\pgfmath@def{cosfrac}{26}{0.96782}		\pgfmath@def{cosfrac}{27}{0.96542}
\pgfmath@def{cosfrac}{28}{0.96296}		\pgfmath@def{cosfrac}{29}{0.96042}
\pgfmath@def{cosfrac}{30}{0.95782}		\pgfmath@def{cosfrac}{31}{0.95515}
\pgfmath@def{cosfrac}{32}{0.95242}		\pgfmath@def{cosfrac}{33}{0.94962}
\pgfmath@def{cosfrac}{34}{0.94677}		\pgfmath@def{cosfrac}{35}{0.94385}
\pgfmath@def{cosfrac}{36}{0.94088}		\pgfmath@def{cosfrac}{37}{0.93786}
\pgfmath@def{cosfrac}{38}{0.93478}		\pgfmath@def{cosfrac}{39}{0.93165}
\pgfmath@def{cosfrac}{40}{0.92847}		\pgfmath@def{cosfrac}{41}{0.92525}
\pgfmath@def{cosfrac}{42}{0.92198}		\pgfmath@def{cosfrac}{43}{0.91866}
\pgfmath@def{cosfrac}{44}{0.91531}		\pgfmath@def{cosfrac}{45}{0.91192}
\pgfmath@def{cosfrac}{46}{0.90849}		\pgfmath@def{cosfrac}{47}{0.90502}
\pgfmath@def{cosfrac}{48}{0.90152}		\pgfmath@def{cosfrac}{49}{0.89799}
\pgfmath@def{cosfrac}{50}{0.89442}		\pgfmath@def{cosfrac}{51}{0.89083}
\pgfmath@def{cosfrac}{52}{0.88721}		\pgfmath@def{cosfrac}{53}{0.88357}
\pgfmath@def{cosfrac}{54}{0.87990}		\pgfmath@def{cosfrac}{55}{0.87621}
\pgfmath@def{cosfrac}{56}{0.87250}		\pgfmath@def{cosfrac}{57}{0.86877}
\pgfmath@def{cosfrac}{58}{0.86503}		\pgfmath@def{cosfrac}{59}{0.86126}
\pgfmath@def{cosfrac}{60}{0.85749}		\pgfmath@def{cosfrac}{61}{0.85370}
\pgfmath@def{cosfrac}{62}{0.84990}		\pgfmath@def{cosfrac}{63}{0.84609}
\pgfmath@def{cosfrac}{64}{0.84227}		\pgfmath@def{cosfrac}{65}{0.83844}
\pgfmath@def{cosfrac}{66}{0.83460}		\pgfmath@def{cosfrac}{67}{0.83077}
\pgfmath@def{cosfrac}{68}{0.82692}		\pgfmath@def{cosfrac}{69}{0.82308}
\pgfmath@def{cosfrac}{70}{0.81923}		\pgfmath@def{cosfrac}{71}{0.81538}
\pgfmath@def{cosfrac}{72}{0.81153}		\pgfmath@def{cosfrac}{73}{0.80768}
\pgfmath@def{cosfrac}{74}{0.80384}		\pgfmath@def{cosfrac}{75}{0.80000}
\pgfmath@def{cosfrac}{76}{0.79616}		\pgfmath@def{cosfrac}{77}{0.79232}
\pgfmath@def{cosfrac}{78}{0.78850}		\pgfmath@def{cosfrac}{79}{0.78468}
\pgfmath@def{cosfrac}{80}{0.78086}		\pgfmath@def{cosfrac}{81}{0.77706}
\pgfmath@def{cosfrac}{82}{0.77326}		\pgfmath@def{cosfrac}{83}{0.76948}
\pgfmath@def{cosfrac}{84}{0.76570}		\pgfmath@def{cosfrac}{85}{0.76193}
\pgfmath@def{cosfrac}{86}{0.75818}		\pgfmath@def{cosfrac}{87}{0.75444}
\pgfmath@def{cosfrac}{88}{0.75071}		\pgfmath@def{cosfrac}{89}{0.74699}
\pgfmath@def{cosfrac}{90}{0.74329}		\pgfmath@def{cosfrac}{91}{0.73960}
\pgfmath@def{cosfrac}{92}{0.73593}		\pgfmath@def{cosfrac}{93}{0.73227}
\pgfmath@def{cosfrac}{94}{0.72862}		\pgfmath@def{cosfrac}{95}{0.72499}
\pgfmath@def{cosfrac}{96}{0.72138}		\pgfmath@def{cosfrac}{97}{0.71779}
\pgfmath@def{cosfrac}{98}{0.71421}		\pgfmath@def{cosfrac}{99}{0.71065}
\pgfmath@def{cosfrac}{100}{0.70710}	

% Oh No! Some really loooooong tables.
\pgfmath@def{atan}{0}{0.00000}		\pgfmath@def{atan}{1}{0.05729}
\pgfmath@def{atan}{2}{0.11459}		\pgfmath@def{atan}{3}{0.17188}
\pgfmath@def{atan}{4}{0.22918}		\pgfmath@def{atan}{5}{0.28647}
\pgfmath@def{atan}{6}{0.34377}		\pgfmath@def{atan}{7}{0.40106}
\pgfmath@def{atan}{8}{0.45835}		\pgfmath@def{atan}{9}{0.51564}
\pgfmath@def{atan}{10}{0.57293}		\pgfmath@def{atan}{11}{0.63022}
\pgfmath@def{atan}{12}{0.68751}		\pgfmath@def{atan}{13}{0.74480}
\pgfmath@def{atan}{14}{0.80208}		\pgfmath@def{atan}{15}{0.85937}
\pgfmath@def{atan}{16}{0.91665}		\pgfmath@def{atan}{17}{0.97393}
\pgfmath@def{atan}{18}{1.03121}		\pgfmath@def{atan}{19}{1.08848}
\pgfmath@def{atan}{20}{1.14576}		\pgfmath@def{atan}{21}{1.20303}
\pgfmath@def{atan}{22}{1.26030}		\pgfmath@def{atan}{23}{1.31757}
\pgfmath@def{atan}{24}{1.37483}		\pgfmath@def{atan}{25}{1.43209}
\pgfmath@def{atan}{26}{1.48935}		\pgfmath@def{atan}{27}{1.54661}
\pgfmath@def{atan}{28}{1.60386}		\pgfmath@def{atan}{29}{1.66111}
\pgfmath@def{atan}{30}{1.71835}		\pgfmath@def{atan}{31}{1.77560}
\pgfmath@def{atan}{32}{1.83284}		\pgfmath@def{atan}{33}{1.89007}
\pgfmath@def{atan}{34}{1.94730}		\pgfmath@def{atan}{35}{2.00453}
\pgfmath@def{atan}{36}{2.06175}		\pgfmath@def{atan}{37}{2.11897}
\pgfmath@def{atan}{38}{2.17619}		\pgfmath@def{atan}{39}{2.23340}
\pgfmath@def{atan}{40}{2.29061}		\pgfmath@def{atan}{41}{2.34781}
\pgfmath@def{atan}{42}{2.40500}		\pgfmath@def{atan}{43}{2.46220}
\pgfmath@def{atan}{44}{2.51938}		\pgfmath@def{atan}{45}{2.57657}
\pgfmath@def{atan}{46}{2.63374}		\pgfmath@def{atan}{47}{2.69092}
\pgfmath@def{atan}{48}{2.74808}		\pgfmath@def{atan}{49}{2.80524}
\pgfmath@def{atan}{50}{2.86240}		\pgfmath@def{atan}{51}{2.91955}
\pgfmath@def{atan}{52}{2.97669}		\pgfmath@def{atan}{53}{3.03383}
\pgfmath@def{atan}{54}{3.09097}		\pgfmath@def{atan}{55}{3.14809}
\pgfmath@def{atan}{56}{3.20521}		\pgfmath@def{atan}{57}{3.26232}
\pgfmath@def{atan}{58}{3.31943}		\pgfmath@def{atan}{59}{3.37653}
\pgfmath@def{atan}{60}{3.43363}		\pgfmath@def{atan}{61}{3.49071}
\pgfmath@def{atan}{62}{3.54779}		\pgfmath@def{atan}{63}{3.60487}
\pgfmath@def{atan}{64}{3.66193}		\pgfmath@def{atan}{65}{3.71899}
\pgfmath@def{atan}{66}{3.77604}		\pgfmath@def{atan}{67}{3.83308}
\pgfmath@def{atan}{68}{3.89012}		\pgfmath@def{atan}{69}{3.94715}
\pgfmath@def{atan}{70}{4.00417}		\pgfmath@def{atan}{71}{4.06118}
\pgfmath@def{atan}{72}{4.11819}		\pgfmath@def{atan}{73}{4.17518}
\pgfmath@def{atan}{74}{4.23217}		\pgfmath@def{atan}{75}{4.28915}
\pgfmath@def{atan}{76}{4.34612}		\pgfmath@def{atan}{77}{4.40308}
\pgfmath@def{atan}{78}{4.46004}		\pgfmath@def{atan}{79}{4.51698}
\pgfmath@def{atan}{80}{4.57392}		\pgfmath@def{atan}{81}{4.63084}
\pgfmath@def{atan}{82}{4.68776}		\pgfmath@def{atan}{83}{4.74467}
\pgfmath@def{atan}{84}{4.80157}		\pgfmath@def{atan}{85}{4.85846}
\pgfmath@def{atan}{86}{4.91534}		\pgfmath@def{atan}{87}{4.97221}
\pgfmath@def{atan}{88}{5.02907}		\pgfmath@def{atan}{89}{5.08592}
\pgfmath@def{atan}{90}{5.14276}		\pgfmath@def{atan}{91}{5.19959}
\pgfmath@def{atan}{92}{5.25641}		\pgfmath@def{atan}{93}{5.31322}
\pgfmath@def{atan}{94}{5.37002}		\pgfmath@def{atan}{95}{5.42681}
\pgfmath@def{atan}{96}{5.48359}		\pgfmath@def{atan}{97}{5.54035}
\pgfmath@def{atan}{98}{5.59711}		\pgfmath@def{atan}{99}{5.65385}
\pgfmath@def{atan}{100}{5.71059}		\pgfmath@def{atan}{101}{5.76731}
\pgfmath@def{atan}{102}{5.82402}		\pgfmath@def{atan}{103}{5.88072}
\pgfmath@def{atan}{104}{5.93741}		\pgfmath@def{atan}{105}{5.99409}
\pgfmath@def{atan}{106}{6.05075}		\pgfmath@def{atan}{107}{6.10741}
\pgfmath@def{atan}{108}{6.16405}		\pgfmath@def{atan}{109}{6.22068}
\pgfmath@def{atan}{110}{6.27729}		\pgfmath@def{atan}{111}{6.33390}
\pgfmath@def{atan}{112}{6.39049}		\pgfmath@def{atan}{113}{6.44707}
\pgfmath@def{atan}{114}{6.50364}		\pgfmath@def{atan}{115}{6.56019}
\pgfmath@def{atan}{116}{6.61673}		\pgfmath@def{atan}{117}{6.67326}
\pgfmath@def{atan}{118}{6.72978}		\pgfmath@def{atan}{119}{6.78628}
\pgfmath@def{atan}{120}{6.84277}		\pgfmath@def{atan}{121}{6.89924}
\pgfmath@def{atan}{122}{6.95571}		\pgfmath@def{atan}{123}{7.01216}
\pgfmath@def{atan}{124}{7.06859}		\pgfmath@def{atan}{125}{7.12501}
\pgfmath@def{atan}{126}{7.18142}		\pgfmath@def{atan}{127}{7.23781}
\pgfmath@def{atan}{128}{7.29419}		\pgfmath@def{atan}{129}{7.35056}
\pgfmath@def{atan}{130}{7.40691}		\pgfmath@def{atan}{131}{7.46324}
\pgfmath@def{atan}{132}{7.51957}		\pgfmath@def{atan}{133}{7.57587}
\pgfmath@def{atan}{134}{7.63217}		\pgfmath@def{atan}{135}{7.68844}
\pgfmath@def{atan}{136}{7.74471}		\pgfmath@def{atan}{137}{7.80095}
\pgfmath@def{atan}{138}{7.85719}		\pgfmath@def{atan}{139}{7.91340}
\pgfmath@def{atan}{140}{7.96961}		\pgfmath@def{atan}{141}{8.02579}
\pgfmath@def{atan}{142}{8.08196}		\pgfmath@def{atan}{143}{8.13812}
\pgfmath@def{atan}{144}{8.19426}		\pgfmath@def{atan}{145}{8.25038}
\pgfmath@def{atan}{146}{8.30649}		\pgfmath@def{atan}{147}{8.36258}
\pgfmath@def{atan}{148}{8.41866}		\pgfmath@def{atan}{149}{8.47472}
\pgfmath@def{atan}{150}{8.53076}		\pgfmath@def{atan}{151}{8.58679}
\pgfmath@def{atan}{152}{8.64280}		\pgfmath@def{atan}{153}{8.69879}
\pgfmath@def{atan}{154}{8.75477}		\pgfmath@def{atan}{155}{8.81073}
\pgfmath@def{atan}{156}{8.86667}		\pgfmath@def{atan}{157}{8.92260}
\pgfmath@def{atan}{158}{8.97851}		\pgfmath@def{atan}{159}{9.03440}
\pgfmath@def{atan}{160}{9.09027}		\pgfmath@def{atan}{161}{9.14613}
\pgfmath@def{atan}{162}{9.20197}		\pgfmath@def{atan}{163}{9.25779}
\pgfmath@def{atan}{164}{9.31359}		\pgfmath@def{atan}{165}{9.36938}
\pgfmath@def{atan}{166}{9.42515}		\pgfmath@def{atan}{167}{9.48090}
\pgfmath@def{atan}{168}{9.53663}		\pgfmath@def{atan}{169}{9.59235}
\pgfmath@def{atan}{170}{9.64804}		\pgfmath@def{atan}{171}{9.70372}
\pgfmath@def{atan}{172}{9.75938}		\pgfmath@def{atan}{173}{9.81502}
\pgfmath@def{atan}{174}{9.87064}		\pgfmath@def{atan}{175}{9.92624}
\pgfmath@def{atan}{176}{9.98182}		\pgfmath@def{atan}{177}{10.03739}
\pgfmath@def{atan}{178}{10.09294}		\pgfmath@def{atan}{179}{10.14846}
\pgfmath@def{atan}{180}{10.20397}		\pgfmath@def{atan}{181}{10.25946}
\pgfmath@def{atan}{182}{10.31493}		\pgfmath@def{atan}{183}{10.37037}
\pgfmath@def{atan}{184}{10.42580}		\pgfmath@def{atan}{185}{10.48121}
\pgfmath@def{atan}{186}{10.53660}		\pgfmath@def{atan}{187}{10.59197}
\pgfmath@def{atan}{188}{10.64732}		\pgfmath@def{atan}{189}{10.70265}
\pgfmath@def{atan}{190}{10.75796}		\pgfmath@def{atan}{191}{10.81325}
\pgfmath@def{atan}{192}{10.86852}		\pgfmath@def{atan}{193}{10.92377}
\pgfmath@def{atan}{194}{10.97900}		\pgfmath@def{atan}{195}{11.03420}
\pgfmath@def{atan}{196}{11.08939}		\pgfmath@def{atan}{197}{11.14456}
\pgfmath@def{atan}{198}{11.19970}		\pgfmath@def{atan}{199}{11.25483}
\pgfmath@def{atan}{200}{11.30993}		\pgfmath@def{atan}{201}{11.36501}
\pgfmath@def{atan}{202}{11.42007}		\pgfmath@def{atan}{203}{11.47511}
\pgfmath@def{atan}{204}{11.53013}		\pgfmath@def{atan}{205}{11.58512}
\pgfmath@def{atan}{206}{11.64010}		\pgfmath@def{atan}{207}{11.69505}
\pgfmath@def{atan}{208}{11.74998}		\pgfmath@def{atan}{209}{11.80489}
\pgfmath@def{atan}{210}{11.85977}		\pgfmath@def{atan}{211}{11.91464}
\pgfmath@def{atan}{212}{11.96948}		\pgfmath@def{atan}{213}{12.02430}
\pgfmath@def{atan}{214}{12.07910}		\pgfmath@def{atan}{215}{12.13388}
\pgfmath@def{atan}{216}{12.18863}		\pgfmath@def{atan}{217}{12.24336}
\pgfmath@def{atan}{218}{12.29807}		\pgfmath@def{atan}{219}{12.35275}
\pgfmath@def{atan}{220}{12.40741}		\pgfmath@def{atan}{221}{12.46205}
\pgfmath@def{atan}{222}{12.51667}		\pgfmath@def{atan}{223}{12.57126}
\pgfmath@def{atan}{224}{12.62583}		\pgfmath@def{atan}{225}{12.68038}
\pgfmath@def{atan}{226}{12.73490}		\pgfmath@def{atan}{227}{12.78940}
\pgfmath@def{atan}{228}{12.84388}		\pgfmath@def{atan}{229}{12.89833}
\pgfmath@def{atan}{230}{12.95276}		\pgfmath@def{atan}{231}{13.00717}
\pgfmath@def{atan}{232}{13.06155}		\pgfmath@def{atan}{233}{13.11590}
\pgfmath@def{atan}{234}{13.17024}		\pgfmath@def{atan}{235}{13.22455}
\pgfmath@def{atan}{236}{13.27883}		\pgfmath@def{atan}{237}{13.33309}
\pgfmath@def{atan}{238}{13.38733}		\pgfmath@def{atan}{239}{13.44154}
\pgfmath@def{atan}{240}{13.49573}		\pgfmath@def{atan}{241}{13.54989}
\pgfmath@def{atan}{242}{13.60403}		\pgfmath@def{atan}{243}{13.65814}
\pgfmath@def{atan}{244}{13.71223}		\pgfmath@def{atan}{245}{13.76630}
\pgfmath@def{atan}{246}{13.82034}		\pgfmath@def{atan}{247}{13.87435}
\pgfmath@def{atan}{248}{13.92834}		\pgfmath@def{atan}{249}{13.98230}
\pgfmath@def{atan}{250}{14.03624}		\pgfmath@def{atan}{251}{14.09015}
\pgfmath@def{atan}{252}{14.14404}		\pgfmath@def{atan}{253}{14.19790}
\pgfmath@def{atan}{254}{14.25174}		\pgfmath@def{atan}{255}{14.30555}
\pgfmath@def{atan}{256}{14.35933}		\pgfmath@def{atan}{257}{14.41309}
\pgfmath@def{atan}{258}{14.46682}		\pgfmath@def{atan}{259}{14.52053}
\pgfmath@def{atan}{260}{14.57421}		\pgfmath@def{atan}{261}{14.62787}
\pgfmath@def{atan}{262}{14.68149}		\pgfmath@def{atan}{263}{14.73510}
\pgfmath@def{atan}{264}{14.78867}		\pgfmath@def{atan}{265}{14.84222}
\pgfmath@def{atan}{266}{14.89575}		\pgfmath@def{atan}{267}{14.94924}
\pgfmath@def{atan}{268}{15.00271}		\pgfmath@def{atan}{269}{15.05615}
\pgfmath@def{atan}{270}{15.10957}		\pgfmath@def{atan}{271}{15.16296}
\pgfmath@def{atan}{272}{15.21632}		\pgfmath@def{atan}{273}{15.26966}
\pgfmath@def{atan}{274}{15.32297}		\pgfmath@def{atan}{275}{15.37625}
\pgfmath@def{atan}{276}{15.42950}		\pgfmath@def{atan}{277}{15.48273}
\pgfmath@def{atan}{278}{15.53593}		\pgfmath@def{atan}{279}{15.58910}
\pgfmath@def{atan}{280}{15.64224}		\pgfmath@def{atan}{281}{15.69536}
\pgfmath@def{atan}{282}{15.74845}		\pgfmath@def{atan}{283}{15.80151}
\pgfmath@def{atan}{284}{15.85454}		\pgfmath@def{atan}{285}{15.90755}
\pgfmath@def{atan}{286}{15.96052}		\pgfmath@def{atan}{287}{16.01347}
\pgfmath@def{atan}{288}{16.06640}		\pgfmath@def{atan}{289}{16.11929}
\pgfmath@def{atan}{290}{16.17215}		\pgfmath@def{atan}{291}{16.22499}
\pgfmath@def{atan}{292}{16.27780}		\pgfmath@def{atan}{293}{16.33058}
\pgfmath@def{atan}{294}{16.38333}		\pgfmath@def{atan}{295}{16.43605}
\pgfmath@def{atan}{296}{16.48875}		\pgfmath@def{atan}{297}{16.54142}
\pgfmath@def{atan}{298}{16.59405}		\pgfmath@def{atan}{299}{16.64666}
\pgfmath@def{atan}{300}{16.69924}		\pgfmath@def{atan}{301}{16.75179}
\pgfmath@def{atan}{302}{16.80431}		\pgfmath@def{atan}{303}{16.85680}
\pgfmath@def{atan}{304}{16.90927}		\pgfmath@def{atan}{305}{16.96170}
\pgfmath@def{atan}{306}{17.01411}		\pgfmath@def{atan}{307}{17.06648}
\pgfmath@def{atan}{308}{17.11883}		\pgfmath@def{atan}{309}{17.17114}
\pgfmath@def{atan}{310}{17.22343}		\pgfmath@def{atan}{311}{17.27569}
\pgfmath@def{atan}{312}{17.32792}		\pgfmath@def{atan}{313}{17.38012}
\pgfmath@def{atan}{314}{17.43228}		\pgfmath@def{atan}{315}{17.48442}
\pgfmath@def{atan}{316}{17.53653}		\pgfmath@def{atan}{317}{17.58861}
\pgfmath@def{atan}{318}{17.64066}		\pgfmath@def{atan}{319}{17.69268}
\pgfmath@def{atan}{320}{17.74467}		\pgfmath@def{atan}{321}{17.79663}
\pgfmath@def{atan}{322}{17.84855}		\pgfmath@def{atan}{323}{17.90045}
\pgfmath@def{atan}{324}{17.95232}		\pgfmath@def{atan}{325}{18.00416}
\pgfmath@def{atan}{326}{18.05596}		\pgfmath@def{atan}{327}{18.10774}
\pgfmath@def{atan}{328}{18.15949}		\pgfmath@def{atan}{329}{18.21120}
\pgfmath@def{atan}{330}{18.26289}		\pgfmath@def{atan}{331}{18.31454}
\pgfmath@def{atan}{332}{18.36616}		\pgfmath@def{atan}{333}{18.41775}
\pgfmath@def{atan}{334}{18.46931}		\pgfmath@def{atan}{335}{18.52084}
\pgfmath@def{atan}{336}{18.57234}		\pgfmath@def{atan}{337}{18.62381}
\pgfmath@def{atan}{338}{18.67525}		\pgfmath@def{atan}{339}{18.72665}
\pgfmath@def{atan}{340}{18.77803}		\pgfmath@def{atan}{341}{18.82937}
\pgfmath@def{atan}{342}{18.88068}		\pgfmath@def{atan}{343}{18.93196}
\pgfmath@def{atan}{344}{18.98321}		\pgfmath@def{atan}{345}{19.03443}
\pgfmath@def{atan}{346}{19.08562}		\pgfmath@def{atan}{347}{19.13677}
\pgfmath@def{atan}{348}{19.18789}		\pgfmath@def{atan}{349}{19.23898}
\pgfmath@def{atan}{350}{19.29004}		\pgfmath@def{atan}{351}{19.34107}
\pgfmath@def{atan}{352}{19.39206}		\pgfmath@def{atan}{353}{19.44303}
\pgfmath@def{atan}{354}{19.49396}		\pgfmath@def{atan}{355}{19.54486}
\pgfmath@def{atan}{356}{19.59572}		\pgfmath@def{atan}{357}{19.64656}
\pgfmath@def{atan}{358}{19.69736}		\pgfmath@def{atan}{359}{19.74813}
\pgfmath@def{atan}{360}{19.79887}		\pgfmath@def{atan}{361}{19.84958}
\pgfmath@def{atan}{362}{19.90025}		\pgfmath@def{atan}{363}{19.95089}
\pgfmath@def{atan}{364}{20.00150}		\pgfmath@def{atan}{365}{20.05208}
\pgfmath@def{atan}{366}{20.10262}		\pgfmath@def{atan}{367}{20.15313}
\pgfmath@def{atan}{368}{20.20361}		\pgfmath@def{atan}{369}{20.25406}
\pgfmath@def{atan}{370}{20.30447}		\pgfmath@def{atan}{371}{20.35485}
\pgfmath@def{atan}{372}{20.40520}		\pgfmath@def{atan}{373}{20.45551}
\pgfmath@def{atan}{374}{20.50579}		\pgfmath@def{atan}{375}{20.55604}
\pgfmath@def{atan}{376}{20.60626}		\pgfmath@def{atan}{377}{20.65644}
\pgfmath@def{atan}{378}{20.70659}		\pgfmath@def{atan}{379}{20.75670}
\pgfmath@def{atan}{380}{20.80679}		\pgfmath@def{atan}{381}{20.85684}
\pgfmath@def{atan}{382}{20.90685}		\pgfmath@def{atan}{383}{20.95684}
\pgfmath@def{atan}{384}{21.00678}		\pgfmath@def{atan}{385}{21.05670}
\pgfmath@def{atan}{386}{21.10658}		\pgfmath@def{atan}{387}{21.15643}
\pgfmath@def{atan}{388}{21.20625}		\pgfmath@def{atan}{389}{21.25603}
\pgfmath@def{atan}{390}{21.30578}		\pgfmath@def{atan}{391}{21.35549}
\pgfmath@def{atan}{392}{21.40517}		\pgfmath@def{atan}{393}{21.45482}
\pgfmath@def{atan}{394}{21.50444}		\pgfmath@def{atan}{395}{21.55402}
\pgfmath@def{atan}{396}{21.60356}		\pgfmath@def{atan}{397}{21.65307}
\pgfmath@def{atan}{398}{21.70255}		\pgfmath@def{atan}{399}{21.75200}
\pgfmath@def{atan}{400}{21.80140}		\pgfmath@def{atan}{401}{21.85078}
\pgfmath@def{atan}{402}{21.90012}		\pgfmath@def{atan}{403}{21.94943}
\pgfmath@def{atan}{404}{21.99870}		\pgfmath@def{atan}{405}{22.04794}
\pgfmath@def{atan}{406}{22.09715}		\pgfmath@def{atan}{407}{22.14632}
\pgfmath@def{atan}{408}{22.19546}		\pgfmath@def{atan}{409}{22.24456}
\pgfmath@def{atan}{410}{22.29362}		\pgfmath@def{atan}{411}{22.34266}
\pgfmath@def{atan}{412}{22.39166}		\pgfmath@def{atan}{413}{22.44062}
\pgfmath@def{atan}{414}{22.48955}		\pgfmath@def{atan}{415}{22.53845}
\pgfmath@def{atan}{416}{22.58731}		\pgfmath@def{atan}{417}{22.63613}
\pgfmath@def{atan}{418}{22.68492}		\pgfmath@def{atan}{419}{22.73368}
\pgfmath@def{atan}{420}{22.78240}		\pgfmath@def{atan}{421}{22.83109}
\pgfmath@def{atan}{422}{22.87974}		\pgfmath@def{atan}{423}{22.92836}
\pgfmath@def{atan}{424}{22.97694}		\pgfmath@def{atan}{425}{23.02549}
\pgfmath@def{atan}{426}{23.07400}		\pgfmath@def{atan}{427}{23.12248}
\pgfmath@def{atan}{428}{23.17092}		\pgfmath@def{atan}{429}{23.21933}
\pgfmath@def{atan}{430}{23.26770}		\pgfmath@def{atan}{431}{23.31604}
\pgfmath@def{atan}{432}{23.36434}		\pgfmath@def{atan}{433}{23.41261}
\pgfmath@def{atan}{434}{23.46084}		\pgfmath@def{atan}{435}{23.50904}
\pgfmath@def{atan}{436}{23.55720}		\pgfmath@def{atan}{437}{23.60532}
\pgfmath@def{atan}{438}{23.65341}		\pgfmath@def{atan}{439}{23.70147}
\pgfmath@def{atan}{440}{23.74949}		\pgfmath@def{atan}{441}{23.79747}
\pgfmath@def{atan}{442}{23.84542}		\pgfmath@def{atan}{443}{23.89334}
\pgfmath@def{atan}{444}{23.94122}		\pgfmath@def{atan}{445}{23.98906}
\pgfmath@def{atan}{446}{24.03687}		\pgfmath@def{atan}{447}{24.08464}
\pgfmath@def{atan}{448}{24.13238}		\pgfmath@def{atan}{449}{24.18008}
\pgfmath@def{atan}{450}{24.22774}		\pgfmath@def{atan}{451}{24.27537}
\pgfmath@def{atan}{452}{24.32296}		\pgfmath@def{atan}{453}{24.37052}
\pgfmath@def{atan}{454}{24.41804}		\pgfmath@def{atan}{455}{24.46553}
\pgfmath@def{atan}{456}{24.51298}		\pgfmath@def{atan}{457}{24.56040}
\pgfmath@def{atan}{458}{24.60778}		\pgfmath@def{atan}{459}{24.65512}
\pgfmath@def{atan}{460}{24.70243}		\pgfmath@def{atan}{461}{24.74970}
\pgfmath@def{atan}{462}{24.79693}		\pgfmath@def{atan}{463}{24.84413}
\pgfmath@def{atan}{464}{24.89130}		\pgfmath@def{atan}{465}{24.93842}
\pgfmath@def{atan}{466}{24.98551}		\pgfmath@def{atan}{467}{25.03257}
\pgfmath@def{atan}{468}{25.07959}		\pgfmath@def{atan}{469}{25.12657}
\pgfmath@def{atan}{470}{25.17352}		\pgfmath@def{atan}{471}{25.22043}
\pgfmath@def{atan}{472}{25.26731}		\pgfmath@def{atan}{473}{25.31414}
\pgfmath@def{atan}{474}{25.36095}		\pgfmath@def{atan}{475}{25.40771}
\pgfmath@def{atan}{476}{25.45444}		\pgfmath@def{atan}{477}{25.50114}
\pgfmath@def{atan}{478}{25.54780}		\pgfmath@def{atan}{479}{25.59442}
\pgfmath@def{atan}{480}{25.64100}		\pgfmath@def{atan}{481}{25.68755}
\pgfmath@def{atan}{482}{25.73406}		\pgfmath@def{atan}{483}{25.78054}
\pgfmath@def{atan}{484}{25.82698}		\pgfmath@def{atan}{485}{25.87338}
\pgfmath@def{atan}{486}{25.91975}		\pgfmath@def{atan}{487}{25.96608}
\pgfmath@def{atan}{488}{26.01237}		\pgfmath@def{atan}{489}{26.05863}
\pgfmath@def{atan}{490}{26.10485}		\pgfmath@def{atan}{491}{26.15103}
\pgfmath@def{atan}{492}{26.19718}		\pgfmath@def{atan}{493}{26.24329}
\pgfmath@def{atan}{494}{26.28937}		\pgfmath@def{atan}{495}{26.33541}
\pgfmath@def{atan}{496}{26.38141}		\pgfmath@def{atan}{497}{26.42737}
\pgfmath@def{atan}{498}{26.47330}		\pgfmath@def{atan}{499}{26.51919}
\pgfmath@def{atan}{500}{26.56505}		\pgfmath@def{atan}{501}{26.61086}
\pgfmath@def{atan}{502}{26.65665}		\pgfmath@def{atan}{503}{26.70239}
\pgfmath@def{atan}{504}{26.74810}		\pgfmath@def{atan}{505}{26.79377}
\pgfmath@def{atan}{506}{26.83941}		\pgfmath@def{atan}{507}{26.88500}
\pgfmath@def{atan}{508}{26.93057}		\pgfmath@def{atan}{509}{26.97609}
\pgfmath@def{atan}{510}{27.02158}		\pgfmath@def{atan}{511}{27.06703}
\pgfmath@def{atan}{512}{27.11244}		\pgfmath@def{atan}{513}{27.15782}
\pgfmath@def{atan}{514}{27.20316}		\pgfmath@def{atan}{515}{27.24846}
\pgfmath@def{atan}{516}{27.29373}		\pgfmath@def{atan}{517}{27.33896}
\pgfmath@def{atan}{518}{27.38415}		\pgfmath@def{atan}{519}{27.42931}
\pgfmath@def{atan}{520}{27.47443}		\pgfmath@def{atan}{521}{27.51951}
\pgfmath@def{atan}{522}{27.56455}		\pgfmath@def{atan}{523}{27.60956}
\pgfmath@def{atan}{524}{27.65453}		\pgfmath@def{atan}{525}{27.69947}
\pgfmath@def{atan}{526}{27.74437}		\pgfmath@def{atan}{527}{27.78923}
\pgfmath@def{atan}{528}{27.83405}		\pgfmath@def{atan}{529}{27.87884}
\pgfmath@def{atan}{530}{27.92359}		\pgfmath@def{atan}{531}{27.96830}
\pgfmath@def{atan}{532}{28.01297}		\pgfmath@def{atan}{533}{28.05761}
\pgfmath@def{atan}{534}{28.10221}		\pgfmath@def{atan}{535}{28.14678}
\pgfmath@def{atan}{536}{28.19130}		\pgfmath@def{atan}{537}{28.23579}
\pgfmath@def{atan}{538}{28.28025}		\pgfmath@def{atan}{539}{28.32466}
\pgfmath@def{atan}{540}{28.36904}		\pgfmath@def{atan}{541}{28.41338}
\pgfmath@def{atan}{542}{28.45769}		\pgfmath@def{atan}{543}{28.50196}
\pgfmath@def{atan}{544}{28.54619}		\pgfmath@def{atan}{545}{28.59038}
\pgfmath@def{atan}{546}{28.63454}		\pgfmath@def{atan}{547}{28.67865}
\pgfmath@def{atan}{548}{28.72274}		\pgfmath@def{atan}{549}{28.76678}
\pgfmath@def{atan}{550}{28.81079}		\pgfmath@def{atan}{551}{28.85476}
\pgfmath@def{atan}{552}{28.89869}		\pgfmath@def{atan}{553}{28.94259}
\pgfmath@def{atan}{554}{28.98645}		\pgfmath@def{atan}{555}{29.03027}
\pgfmath@def{atan}{556}{29.07405}		\pgfmath@def{atan}{557}{29.11780}
\pgfmath@def{atan}{558}{29.16151}		\pgfmath@def{atan}{559}{29.20519}
\pgfmath@def{atan}{560}{29.24882}		\pgfmath@def{atan}{561}{29.29242}
\pgfmath@def{atan}{562}{29.33598}		\pgfmath@def{atan}{563}{29.37951}
\pgfmath@def{atan}{564}{29.42299}		\pgfmath@def{atan}{565}{29.46644}
\pgfmath@def{atan}{566}{29.50986}		\pgfmath@def{atan}{567}{29.55323}
\pgfmath@def{atan}{568}{29.59657}		\pgfmath@def{atan}{569}{29.63987}
\pgfmath@def{atan}{570}{29.68314}		\pgfmath@def{atan}{571}{29.72636}
\pgfmath@def{atan}{572}{29.76955}		\pgfmath@def{atan}{573}{29.81270}
\pgfmath@def{atan}{574}{29.85582}		\pgfmath@def{atan}{575}{29.89890}
\pgfmath@def{atan}{576}{29.94194}		\pgfmath@def{atan}{577}{29.98494}
\pgfmath@def{atan}{578}{30.02791}		\pgfmath@def{atan}{579}{30.07084}
\pgfmath@def{atan}{580}{30.11373}		\pgfmath@def{atan}{581}{30.15658}
\pgfmath@def{atan}{582}{30.19940}		\pgfmath@def{atan}{583}{30.24218}
\pgfmath@def{atan}{584}{30.28492}		\pgfmath@def{atan}{585}{30.32763}
\pgfmath@def{atan}{586}{30.37030}		\pgfmath@def{atan}{587}{30.41293}
\pgfmath@def{atan}{588}{30.45552}		\pgfmath@def{atan}{589}{30.49808}
\pgfmath@def{atan}{590}{30.54060}		\pgfmath@def{atan}{591}{30.58308}
\pgfmath@def{atan}{592}{30.62553}		\pgfmath@def{atan}{593}{30.66794}
\pgfmath@def{atan}{594}{30.71031}		\pgfmath@def{atan}{595}{30.75264}
\pgfmath@def{atan}{596}{30.79494}		\pgfmath@def{atan}{597}{30.83720}
\pgfmath@def{atan}{598}{30.87942}		\pgfmath@def{atan}{599}{30.92160}
\pgfmath@def{atan}{600}{30.96375}		\pgfmath@def{atan}{601}{31.00586}
\pgfmath@def{atan}{602}{31.04794}		\pgfmath@def{atan}{603}{31.08997}
\pgfmath@def{atan}{604}{31.13197}		\pgfmath@def{atan}{605}{31.17393}
\pgfmath@def{atan}{606}{31.21586}		\pgfmath@def{atan}{607}{31.25775}
\pgfmath@def{atan}{608}{31.29960}		\pgfmath@def{atan}{609}{31.34141}
\pgfmath@def{atan}{610}{31.38319}		\pgfmath@def{atan}{611}{31.42493}
\pgfmath@def{atan}{612}{31.46663}		\pgfmath@def{atan}{613}{31.50829}
\pgfmath@def{atan}{614}{31.54992}		\pgfmath@def{atan}{615}{31.59151}
\pgfmath@def{atan}{616}{31.63306}		\pgfmath@def{atan}{617}{31.67458}
\pgfmath@def{atan}{618}{31.71606}		\pgfmath@def{atan}{619}{31.75750}
\pgfmath@def{atan}{620}{31.79891}		\pgfmath@def{atan}{621}{31.84028}
\pgfmath@def{atan}{622}{31.88161}		\pgfmath@def{atan}{623}{31.92290}
\pgfmath@def{atan}{624}{31.96416}		\pgfmath@def{atan}{625}{32.00538}
\pgfmath@def{atan}{626}{32.04656}		\pgfmath@def{atan}{627}{32.08771}
\pgfmath@def{atan}{628}{32.12882}		\pgfmath@def{atan}{629}{32.16989}
\pgfmath@def{atan}{630}{32.21092}		\pgfmath@def{atan}{631}{32.25192}
\pgfmath@def{atan}{632}{32.29288}		\pgfmath@def{atan}{633}{32.33381}
\pgfmath@def{atan}{634}{32.37469}		\pgfmath@def{atan}{635}{32.41554}
\pgfmath@def{atan}{636}{32.45636}		\pgfmath@def{atan}{637}{32.49713}
\pgfmath@def{atan}{638}{32.53787}		\pgfmath@def{atan}{639}{32.57857}
\pgfmath@def{atan}{640}{32.61924}		\pgfmath@def{atan}{641}{32.65987}
\pgfmath@def{atan}{642}{32.70046}		\pgfmath@def{atan}{643}{32.74101}
\pgfmath@def{atan}{644}{32.78153}		\pgfmath@def{atan}{645}{32.82201}
\pgfmath@def{atan}{646}{32.86246}		\pgfmath@def{atan}{647}{32.90286}
\pgfmath@def{atan}{648}{32.94323}		\pgfmath@def{atan}{649}{32.98357}
\pgfmath@def{atan}{650}{33.02386}		\pgfmath@def{atan}{651}{33.06412}
\pgfmath@def{atan}{652}{33.10435}		\pgfmath@def{atan}{653}{33.14453}
\pgfmath@def{atan}{654}{33.18468}		\pgfmath@def{atan}{655}{33.22479}
\pgfmath@def{atan}{656}{33.26487}		\pgfmath@def{atan}{657}{33.30491}
\pgfmath@def{atan}{658}{33.34491}		\pgfmath@def{atan}{659}{33.38488}
\pgfmath@def{atan}{660}{33.42481}		\pgfmath@def{atan}{661}{33.46470}
\pgfmath@def{atan}{662}{33.50455}		\pgfmath@def{atan}{663}{33.54437}
\pgfmath@def{atan}{664}{33.58416}		\pgfmath@def{atan}{665}{33.62390}
\pgfmath@def{atan}{666}{33.66361}		\pgfmath@def{atan}{667}{33.70328}
\pgfmath@def{atan}{668}{33.74292}		\pgfmath@def{atan}{669}{33.78252}
\pgfmath@def{atan}{670}{33.82208}		\pgfmath@def{atan}{671}{33.86161}
\pgfmath@def{atan}{672}{33.90110}		\pgfmath@def{atan}{673}{33.94055}
\pgfmath@def{atan}{674}{33.97997}		\pgfmath@def{atan}{675}{34.01935}
\pgfmath@def{atan}{676}{34.05869}		\pgfmath@def{atan}{677}{34.09800}
\pgfmath@def{atan}{678}{34.13727}		\pgfmath@def{atan}{679}{34.17650}
\pgfmath@def{atan}{680}{34.21570}		\pgfmath@def{atan}{681}{34.25486}
\pgfmath@def{atan}{682}{34.29398}		\pgfmath@def{atan}{683}{34.33307}
\pgfmath@def{atan}{684}{34.37212}		\pgfmath@def{atan}{685}{34.41114}
\pgfmath@def{atan}{686}{34.45012}		\pgfmath@def{atan}{687}{34.48906}
\pgfmath@def{atan}{688}{34.52797}		\pgfmath@def{atan}{689}{34.56684}
\pgfmath@def{atan}{690}{34.60567}		\pgfmath@def{atan}{691}{34.64447}
\pgfmath@def{atan}{692}{34.68323}		\pgfmath@def{atan}{693}{34.72195}
\pgfmath@def{atan}{694}{34.76064}		\pgfmath@def{atan}{695}{34.79930}
\pgfmath@def{atan}{696}{34.83791}		\pgfmath@def{atan}{697}{34.87649}
\pgfmath@def{atan}{698}{34.91504}		\pgfmath@def{atan}{699}{34.95354}
\pgfmath@def{atan}{700}{34.99202}		\pgfmath@def{atan}{701}{35.03045}
\pgfmath@def{atan}{702}{35.06885}		\pgfmath@def{atan}{703}{35.10721}
\pgfmath@def{atan}{704}{35.14554}		\pgfmath@def{atan}{705}{35.18383}
\pgfmath@def{atan}{706}{35.22209}		\pgfmath@def{atan}{707}{35.26031}
\pgfmath@def{atan}{708}{35.29849}		\pgfmath@def{atan}{709}{35.33664}
\pgfmath@def{atan}{710}{35.37475}		\pgfmath@def{atan}{711}{35.41282}
\pgfmath@def{atan}{712}{35.45086}		\pgfmath@def{atan}{713}{35.48886}
\pgfmath@def{atan}{714}{35.52683}		\pgfmath@def{atan}{715}{35.56476}
\pgfmath@def{atan}{716}{35.60266}		\pgfmath@def{atan}{717}{35.64052}
\pgfmath@def{atan}{718}{35.67834}		\pgfmath@def{atan}{719}{35.71613}
\pgfmath@def{atan}{720}{35.75388}		\pgfmath@def{atan}{721}{35.79160}
\pgfmath@def{atan}{722}{35.82928}		\pgfmath@def{atan}{723}{35.86692}
\pgfmath@def{atan}{724}{35.90453}		\pgfmath@def{atan}{725}{35.94211}
\pgfmath@def{atan}{726}{35.97965}		\pgfmath@def{atan}{727}{36.01715}
\pgfmath@def{atan}{728}{36.05461}		\pgfmath@def{atan}{729}{36.09204}
\pgfmath@def{atan}{730}{36.12944}		\pgfmath@def{atan}{731}{36.16680}
\pgfmath@def{atan}{732}{36.20412}		\pgfmath@def{atan}{733}{36.24141}
\pgfmath@def{atan}{734}{36.27866}		\pgfmath@def{atan}{735}{36.31588}
\pgfmath@def{atan}{736}{36.35306}		\pgfmath@def{atan}{737}{36.39021}
\pgfmath@def{atan}{738}{36.42732}		\pgfmath@def{atan}{739}{36.46440}
\pgfmath@def{atan}{740}{36.50144}		\pgfmath@def{atan}{741}{36.53844}
\pgfmath@def{atan}{742}{36.57541}		\pgfmath@def{atan}{743}{36.61234}
\pgfmath@def{atan}{744}{36.64924}		\pgfmath@def{atan}{745}{36.68611}
\pgfmath@def{atan}{746}{36.72293}		\pgfmath@def{atan}{747}{36.75973}
\pgfmath@def{atan}{748}{36.79648}		\pgfmath@def{atan}{749}{36.83321}
\pgfmath@def{atan}{750}{36.86989}		\pgfmath@def{atan}{751}{36.90654}
\pgfmath@def{atan}{752}{36.94316}		\pgfmath@def{atan}{753}{36.97974}
\pgfmath@def{atan}{754}{37.01629}		\pgfmath@def{atan}{755}{37.05280}
\pgfmath@def{atan}{756}{37.08928}		\pgfmath@def{atan}{757}{37.12572}
\pgfmath@def{atan}{758}{37.16212}		\pgfmath@def{atan}{759}{37.19849}
\pgfmath@def{atan}{760}{37.23483}		\pgfmath@def{atan}{761}{37.27113}
\pgfmath@def{atan}{762}{37.30740}		\pgfmath@def{atan}{763}{37.34363}
\pgfmath@def{atan}{764}{37.37982}		\pgfmath@def{atan}{765}{37.41598}
\pgfmath@def{atan}{766}{37.45211}		\pgfmath@def{atan}{767}{37.48820}
\pgfmath@def{atan}{768}{37.52426}		\pgfmath@def{atan}{769}{37.56028}
\pgfmath@def{atan}{770}{37.59627}		\pgfmath@def{atan}{771}{37.63222}
\pgfmath@def{atan}{772}{37.66814}		\pgfmath@def{atan}{773}{37.70402}
\pgfmath@def{atan}{774}{37.73987}		\pgfmath@def{atan}{775}{37.77568}
\pgfmath@def{atan}{776}{37.81146}		\pgfmath@def{atan}{777}{37.84720}
\pgfmath@def{atan}{778}{37.88291}		\pgfmath@def{atan}{779}{37.91859}
\pgfmath@def{atan}{780}{37.95423}		\pgfmath@def{atan}{781}{37.98983}
\pgfmath@def{atan}{782}{38.02540}		\pgfmath@def{atan}{783}{38.06094}
\pgfmath@def{atan}{784}{38.09644}		\pgfmath@def{atan}{785}{38.13191}
\pgfmath@def{atan}{786}{38.16734}		\pgfmath@def{atan}{787}{38.20274}
\pgfmath@def{atan}{788}{38.23811}		\pgfmath@def{atan}{789}{38.27344}
\pgfmath@def{atan}{790}{38.30873}		\pgfmath@def{atan}{791}{38.34399}
\pgfmath@def{atan}{792}{38.37922}		\pgfmath@def{atan}{793}{38.41441}
\pgfmath@def{atan}{794}{38.44957}		\pgfmath@def{atan}{795}{38.48469}
\pgfmath@def{atan}{796}{38.51979}		\pgfmath@def{atan}{797}{38.55484}
\pgfmath@def{atan}{798}{38.58986}		\pgfmath@def{atan}{799}{38.62485}
\pgfmath@def{atan}{800}{38.65980}		\pgfmath@def{atan}{801}{38.69472}
\pgfmath@def{atan}{802}{38.72961}		\pgfmath@def{atan}{803}{38.76446}
\pgfmath@def{atan}{804}{38.79928}		\pgfmath@def{atan}{805}{38.83406}
\pgfmath@def{atan}{806}{38.86881}		\pgfmath@def{atan}{807}{38.90353}
\pgfmath@def{atan}{808}{38.93821}		\pgfmath@def{atan}{809}{38.97285}
\pgfmath@def{atan}{810}{39.00747}		\pgfmath@def{atan}{811}{39.04205}
\pgfmath@def{atan}{812}{39.07659}		\pgfmath@def{atan}{813}{39.11111}
\pgfmath@def{atan}{814}{39.14558}		\pgfmath@def{atan}{815}{39.18003}
\pgfmath@def{atan}{816}{39.21444}		\pgfmath@def{atan}{817}{39.24882}
\pgfmath@def{atan}{818}{39.28316}		\pgfmath@def{atan}{819}{39.31747}
\pgfmath@def{atan}{820}{39.35175}		\pgfmath@def{atan}{821}{39.38599}
\pgfmath@def{atan}{822}{39.42020}		\pgfmath@def{atan}{823}{39.45438}
\pgfmath@def{atan}{824}{39.48852}		\pgfmath@def{atan}{825}{39.52263}
\pgfmath@def{atan}{826}{39.55670}		\pgfmath@def{atan}{827}{39.59074}
\pgfmath@def{atan}{828}{39.62475}		\pgfmath@def{atan}{829}{39.65873}
\pgfmath@def{atan}{830}{39.69267}		\pgfmath@def{atan}{831}{39.72658}
\pgfmath@def{atan}{832}{39.76045}		\pgfmath@def{atan}{833}{39.79429}
\pgfmath@def{atan}{834}{39.82810}		\pgfmath@def{atan}{835}{39.86188}
\pgfmath@def{atan}{836}{39.89562}		\pgfmath@def{atan}{837}{39.92933}
\pgfmath@def{atan}{838}{39.96300}		\pgfmath@def{atan}{839}{39.99665}
\pgfmath@def{atan}{840}{40.03025}		\pgfmath@def{atan}{841}{40.06383}
\pgfmath@def{atan}{842}{40.09737}		\pgfmath@def{atan}{843}{40.13088}
\pgfmath@def{atan}{844}{40.16436}		\pgfmath@def{atan}{845}{40.19781}
\pgfmath@def{atan}{846}{40.23122}		\pgfmath@def{atan}{847}{40.26459}
\pgfmath@def{atan}{848}{40.29794}		\pgfmath@def{atan}{849}{40.33125}
\pgfmath@def{atan}{850}{40.36453}		\pgfmath@def{atan}{851}{40.39778}
\pgfmath@def{atan}{852}{40.43099}		\pgfmath@def{atan}{853}{40.46417}
\pgfmath@def{atan}{854}{40.49732}		\pgfmath@def{atan}{855}{40.53044}
\pgfmath@def{atan}{856}{40.56352}		\pgfmath@def{atan}{857}{40.59657}
\pgfmath@def{atan}{858}{40.62959}		\pgfmath@def{atan}{859}{40.66257}
\pgfmath@def{atan}{860}{40.69553}		\pgfmath@def{atan}{861}{40.72845}
\pgfmath@def{atan}{862}{40.76133}		\pgfmath@def{atan}{863}{40.79419}
\pgfmath@def{atan}{864}{40.82701}		\pgfmath@def{atan}{865}{40.85980}
\pgfmath@def{atan}{866}{40.89256}		\pgfmath@def{atan}{867}{40.92528}
\pgfmath@def{atan}{868}{40.95798}		\pgfmath@def{atan}{869}{40.99064}
\pgfmath@def{atan}{870}{41.02326}		\pgfmath@def{atan}{871}{41.05586}
\pgfmath@def{atan}{872}{41.08842}		\pgfmath@def{atan}{873}{41.12095}
\pgfmath@def{atan}{874}{41.15345}		\pgfmath@def{atan}{875}{41.18592}
\pgfmath@def{atan}{876}{41.21836}		\pgfmath@def{atan}{877}{41.25076}
\pgfmath@def{atan}{878}{41.28313}		\pgfmath@def{atan}{879}{41.31547}
\pgfmath@def{atan}{880}{41.34777}		\pgfmath@def{atan}{881}{41.38005}
\pgfmath@def{atan}{882}{41.41229}		\pgfmath@def{atan}{883}{41.44450}
\pgfmath@def{atan}{884}{41.47668}		\pgfmath@def{atan}{885}{41.50882}
\pgfmath@def{atan}{886}{41.54094}		\pgfmath@def{atan}{887}{41.57302}
\pgfmath@def{atan}{888}{41.60507}		\pgfmath@def{atan}{889}{41.63709}
\pgfmath@def{atan}{890}{41.66908}		\pgfmath@def{atan}{891}{41.70103}
\pgfmath@def{atan}{892}{41.73296}		\pgfmath@def{atan}{893}{41.76485}
\pgfmath@def{atan}{894}{41.79671}		\pgfmath@def{atan}{895}{41.82854}
\pgfmath@def{atan}{896}{41.86034}		\pgfmath@def{atan}{897}{41.89210}
\pgfmath@def{atan}{898}{41.92383}		\pgfmath@def{atan}{899}{41.95554}
\pgfmath@def{atan}{900}{41.98721}		\pgfmath@def{atan}{901}{42.01885}
\pgfmath@def{atan}{902}{42.05046}		\pgfmath@def{atan}{903}{42.08203}
\pgfmath@def{atan}{904}{42.11358}		\pgfmath@def{atan}{905}{42.14509}
\pgfmath@def{atan}{906}{42.17657}		\pgfmath@def{atan}{907}{42.20802}
\pgfmath@def{atan}{908}{42.23944}		\pgfmath@def{atan}{909}{42.27083}
\pgfmath@def{atan}{910}{42.30219}		\pgfmath@def{atan}{911}{42.33352}
\pgfmath@def{atan}{912}{42.36481}		\pgfmath@def{atan}{913}{42.39607}
\pgfmath@def{atan}{914}{42.42731}		\pgfmath@def{atan}{915}{42.45851}
\pgfmath@def{atan}{916}{42.48968}		\pgfmath@def{atan}{917}{42.52082}
\pgfmath@def{atan}{918}{42.55193}		\pgfmath@def{atan}{919}{42.58300}
\pgfmath@def{atan}{920}{42.61405}		\pgfmath@def{atan}{921}{42.64507}
\pgfmath@def{atan}{922}{42.67605}		\pgfmath@def{atan}{923}{42.70701}
\pgfmath@def{atan}{924}{42.73793}		\pgfmath@def{atan}{925}{42.76882}
\pgfmath@def{atan}{926}{42.79968}		\pgfmath@def{atan}{927}{42.83051}
\pgfmath@def{atan}{928}{42.86131}		\pgfmath@def{atan}{929}{42.89208}
\pgfmath@def{atan}{930}{42.92282}		\pgfmath@def{atan}{931}{42.95353}
\pgfmath@def{atan}{932}{42.98421}		\pgfmath@def{atan}{933}{43.01485}
\pgfmath@def{atan}{934}{43.04547}		\pgfmath@def{atan}{935}{43.07605}
\pgfmath@def{atan}{936}{43.10661}		\pgfmath@def{atan}{937}{43.13713}
\pgfmath@def{atan}{938}{43.16763}		\pgfmath@def{atan}{939}{43.19809}
\pgfmath@def{atan}{940}{43.22853}		\pgfmath@def{atan}{941}{43.25893}
\pgfmath@def{atan}{942}{43.28930}		\pgfmath@def{atan}{943}{43.31964}
\pgfmath@def{atan}{944}{43.34996}		\pgfmath@def{atan}{945}{43.38024}
\pgfmath@def{atan}{946}{43.41049}		\pgfmath@def{atan}{947}{43.44071}
\pgfmath@def{atan}{948}{43.47090}		\pgfmath@def{atan}{949}{43.50106}
\pgfmath@def{atan}{950}{43.53119}		\pgfmath@def{atan}{951}{43.56130}
\pgfmath@def{atan}{952}{43.59137}		\pgfmath@def{atan}{953}{43.62141}
\pgfmath@def{atan}{954}{43.65142}		\pgfmath@def{atan}{955}{43.68140}
\pgfmath@def{atan}{956}{43.71135}		\pgfmath@def{atan}{957}{43.74127}
\pgfmath@def{atan}{958}{43.77116}		\pgfmath@def{atan}{959}{43.80102}
\pgfmath@def{atan}{960}{43.83086}		\pgfmath@def{atan}{961}{43.86066}
\pgfmath@def{atan}{962}{43.89043}		\pgfmath@def{atan}{963}{43.92017}
\pgfmath@def{atan}{964}{43.94988}		\pgfmath@def{atan}{965}{43.97957}
\pgfmath@def{atan}{966}{44.00922}		\pgfmath@def{atan}{967}{44.03884}
\pgfmath@def{atan}{968}{44.06844}		\pgfmath@def{atan}{969}{44.09800}
\pgfmath@def{atan}{970}{44.12754}		\pgfmath@def{atan}{971}{44.15704}
\pgfmath@def{atan}{972}{44.18652}		\pgfmath@def{atan}{973}{44.21597}
\pgfmath@def{atan}{974}{44.24538}		\pgfmath@def{atan}{975}{44.27477}
\pgfmath@def{atan}{976}{44.30413}		\pgfmath@def{atan}{977}{44.33346}
\pgfmath@def{atan}{978}{44.36276}		\pgfmath@def{atan}{979}{44.39203}
\pgfmath@def{atan}{980}{44.42127}		\pgfmath@def{atan}{981}{44.45048}
\pgfmath@def{atan}{982}{44.47966}		\pgfmath@def{atan}{983}{44.50882}
\pgfmath@def{atan}{984}{44.53794}		\pgfmath@def{atan}{985}{44.56704}
\pgfmath@def{atan}{986}{44.59610}		\pgfmath@def{atan}{987}{44.62514}
\pgfmath@def{atan}{988}{44.65415}		\pgfmath@def{atan}{989}{44.68313}
\pgfmath@def{atan}{990}{44.71208}		\pgfmath@def{atan}{991}{44.74100}
\pgfmath@def{atan}{992}{44.76989}		\pgfmath@def{atan}{993}{44.79876}
\pgfmath@def{atan}{994}{44.82759}		\pgfmath@def{atan}{995}{44.85640}
\pgfmath@def{atan}{996}{44.88517}		\pgfmath@def{atan}{997}{44.91392}
\pgfmath@def{atan}{998}{44.94264}		\pgfmath@def{atan}{999}{44.97133}
\pgfmath@def{atan}{1000}{45.00000}		
	
\pgfmath@def{acos}{0}{90.00000}		\pgfmath@def{acos}{1}{89.94270}
\pgfmath@def{acos}{2}{89.88540}		\pgfmath@def{acos}{3}{89.82811}
\pgfmath@def{acos}{4}{89.77081}		\pgfmath@def{acos}{5}{89.71352}
\pgfmath@def{acos}{6}{89.65622}		\pgfmath@def{acos}{7}{89.59892}
\pgfmath@def{acos}{8}{89.54162}		\pgfmath@def{acos}{9}{89.48433}
\pgfmath@def{acos}{10}{89.42703}		\pgfmath@def{acos}{11}{89.36973}
\pgfmath@def{acos}{12}{89.31243}		\pgfmath@def{acos}{13}{89.25513}
\pgfmath@def{acos}{14}{89.19783}		\pgfmath@def{acos}{15}{89.14053}
\pgfmath@def{acos}{16}{89.08322}		\pgfmath@def{acos}{17}{89.02592}
\pgfmath@def{acos}{18}{88.96862}		\pgfmath@def{acos}{19}{88.91131}
\pgfmath@def{acos}{20}{88.85400}		\pgfmath@def{acos}{21}{88.79670}
\pgfmath@def{acos}{22}{88.73939}		\pgfmath@def{acos}{23}{88.68208}
\pgfmath@def{acos}{24}{88.62476}		\pgfmath@def{acos}{25}{88.56745}
\pgfmath@def{acos}{26}{88.51014}		\pgfmath@def{acos}{27}{88.45282}
\pgfmath@def{acos}{28}{88.39550}		\pgfmath@def{acos}{29}{88.33818}
\pgfmath@def{acos}{30}{88.28086}		\pgfmath@def{acos}{31}{88.22354}
\pgfmath@def{acos}{32}{88.16622}		\pgfmath@def{acos}{33}{88.10889}
\pgfmath@def{acos}{34}{88.05156}		\pgfmath@def{acos}{35}{87.99423}
\pgfmath@def{acos}{36}{87.93690}		\pgfmath@def{acos}{37}{87.87957}
\pgfmath@def{acos}{38}{87.82223}		\pgfmath@def{acos}{39}{87.76489}
\pgfmath@def{acos}{40}{87.70755}		\pgfmath@def{acos}{41}{87.65021}
\pgfmath@def{acos}{42}{87.59286}		\pgfmath@def{acos}{43}{87.53552}
\pgfmath@def{acos}{44}{87.47817}		\pgfmath@def{acos}{45}{87.42081}
\pgfmath@def{acos}{46}{87.36346}		\pgfmath@def{acos}{47}{87.30610}
\pgfmath@def{acos}{48}{87.24874}		\pgfmath@def{acos}{49}{87.19138}
\pgfmath@def{acos}{50}{87.13401}		\pgfmath@def{acos}{51}{87.07664}
\pgfmath@def{acos}{52}{87.01927}		\pgfmath@def{acos}{53}{86.96190}
\pgfmath@def{acos}{54}{86.90452}		\pgfmath@def{acos}{55}{86.84714}
\pgfmath@def{acos}{56}{86.78975}		\pgfmath@def{acos}{57}{86.73237}
\pgfmath@def{acos}{58}{86.67497}		\pgfmath@def{acos}{59}{86.61758}
\pgfmath@def{acos}{60}{86.56018}		\pgfmath@def{acos}{61}{86.50278}
\pgfmath@def{acos}{62}{86.44538}		\pgfmath@def{acos}{63}{86.38797}
\pgfmath@def{acos}{64}{86.33056}		\pgfmath@def{acos}{65}{86.27314}
\pgfmath@def{acos}{66}{86.21572}		\pgfmath@def{acos}{67}{86.15830}
\pgfmath@def{acos}{68}{86.10087}		\pgfmath@def{acos}{69}{86.04344}
\pgfmath@def{acos}{70}{85.98601}		\pgfmath@def{acos}{71}{85.92857}
\pgfmath@def{acos}{72}{85.87113}		\pgfmath@def{acos}{73}{85.81368}
\pgfmath@def{acos}{74}{85.75623}		\pgfmath@def{acos}{75}{85.69877}
\pgfmath@def{acos}{76}{85.64131}		\pgfmath@def{acos}{77}{85.58385}
\pgfmath@def{acos}{78}{85.52638}		\pgfmath@def{acos}{79}{85.46891}
\pgfmath@def{acos}{80}{85.41143}		\pgfmath@def{acos}{81}{85.35395}
\pgfmath@def{acos}{82}{85.29646}		\pgfmath@def{acos}{83}{85.23897}
\pgfmath@def{acos}{84}{85.18147}		\pgfmath@def{acos}{85}{85.12397}
\pgfmath@def{acos}{86}{85.06646}		\pgfmath@def{acos}{87}{85.00895}
\pgfmath@def{acos}{88}{84.95144}		\pgfmath@def{acos}{89}{84.89392}
\pgfmath@def{acos}{90}{84.83639}		\pgfmath@def{acos}{91}{84.77886}
\pgfmath@def{acos}{92}{84.72132}		\pgfmath@def{acos}{93}{84.66378}
\pgfmath@def{acos}{94}{84.60623}		\pgfmath@def{acos}{95}{84.54868}
\pgfmath@def{acos}{96}{84.49112}		\pgfmath@def{acos}{97}{84.43355}
\pgfmath@def{acos}{98}{84.37598}		\pgfmath@def{acos}{99}{84.31841}
\pgfmath@def{acos}{100}{84.26083}		\pgfmath@def{acos}{101}{84.20324}
\pgfmath@def{acos}{102}{84.14564}		\pgfmath@def{acos}{103}{84.08805}
\pgfmath@def{acos}{104}{84.03044}		\pgfmath@def{acos}{105}{83.97283}
\pgfmath@def{acos}{106}{83.91521}		\pgfmath@def{acos}{107}{83.85759}
\pgfmath@def{acos}{108}{83.79996}		\pgfmath@def{acos}{109}{83.74232}
\pgfmath@def{acos}{110}{83.68468}		\pgfmath@def{acos}{111}{83.62703}
\pgfmath@def{acos}{112}{83.56938}		\pgfmath@def{acos}{113}{83.51171}
\pgfmath@def{acos}{114}{83.45405}		\pgfmath@def{acos}{115}{83.39637}
\pgfmath@def{acos}{116}{83.33869}		\pgfmath@def{acos}{117}{83.28100}
\pgfmath@def{acos}{118}{83.22330}		\pgfmath@def{acos}{119}{83.16560}
\pgfmath@def{acos}{120}{83.10789}		\pgfmath@def{acos}{121}{83.05018}
\pgfmath@def{acos}{122}{82.99245}		\pgfmath@def{acos}{123}{82.93472}
\pgfmath@def{acos}{124}{82.87698}		\pgfmath@def{acos}{125}{82.81924}
\pgfmath@def{acos}{126}{82.76149}		\pgfmath@def{acos}{127}{82.70373}
\pgfmath@def{acos}{128}{82.64596}		\pgfmath@def{acos}{129}{82.58819}
\pgfmath@def{acos}{130}{82.53040}		\pgfmath@def{acos}{131}{82.47261}
\pgfmath@def{acos}{132}{82.41482}		\pgfmath@def{acos}{133}{82.35701}
\pgfmath@def{acos}{134}{82.29920}		\pgfmath@def{acos}{135}{82.24138}
\pgfmath@def{acos}{136}{82.18355}		\pgfmath@def{acos}{137}{82.12571}
\pgfmath@def{acos}{138}{82.06786}		\pgfmath@def{acos}{139}{82.01001}
\pgfmath@def{acos}{140}{81.95215}		\pgfmath@def{acos}{141}{81.89428}
\pgfmath@def{acos}{142}{81.83640}		\pgfmath@def{acos}{143}{81.77851}
\pgfmath@def{acos}{144}{81.72062}		\pgfmath@def{acos}{145}{81.66272}
\pgfmath@def{acos}{146}{81.60480}		\pgfmath@def{acos}{147}{81.54688}
\pgfmath@def{acos}{148}{81.48895}		\pgfmath@def{acos}{149}{81.43102}
\pgfmath@def{acos}{150}{81.37307}		\pgfmath@def{acos}{151}{81.31511}
\pgfmath@def{acos}{152}{81.25715}		\pgfmath@def{acos}{153}{81.19917}
\pgfmath@def{acos}{154}{81.14119}		\pgfmath@def{acos}{155}{81.08320}
\pgfmath@def{acos}{156}{81.02520}		\pgfmath@def{acos}{157}{80.96719}
\pgfmath@def{acos}{158}{80.90917}		\pgfmath@def{acos}{159}{80.85114}
\pgfmath@def{acos}{160}{80.79310}		\pgfmath@def{acos}{161}{80.73505}
\pgfmath@def{acos}{162}{80.67699}		\pgfmath@def{acos}{163}{80.61893}
\pgfmath@def{acos}{164}{80.56085}		\pgfmath@def{acos}{165}{80.50276}
\pgfmath@def{acos}{166}{80.44466}		\pgfmath@def{acos}{167}{80.38656}
\pgfmath@def{acos}{168}{80.32844}		\pgfmath@def{acos}{169}{80.27031}
\pgfmath@def{acos}{170}{80.21218}		\pgfmath@def{acos}{171}{80.15403}
\pgfmath@def{acos}{172}{80.09587}		\pgfmath@def{acos}{173}{80.03770}
\pgfmath@def{acos}{174}{79.97953}		\pgfmath@def{acos}{175}{79.92134}
\pgfmath@def{acos}{176}{79.86314}		\pgfmath@def{acos}{177}{79.80493}
\pgfmath@def{acos}{178}{79.74671}		\pgfmath@def{acos}{179}{79.68848}
\pgfmath@def{acos}{180}{79.63024}		\pgfmath@def{acos}{181}{79.57198}
\pgfmath@def{acos}{182}{79.51372}		\pgfmath@def{acos}{183}{79.45545}
\pgfmath@def{acos}{184}{79.39716}		\pgfmath@def{acos}{185}{79.33886}
\pgfmath@def{acos}{186}{79.28056}		\pgfmath@def{acos}{187}{79.22224}
\pgfmath@def{acos}{188}{79.16391}		\pgfmath@def{acos}{189}{79.10556}
\pgfmath@def{acos}{190}{79.04721}		\pgfmath@def{acos}{191}{78.98885}
\pgfmath@def{acos}{192}{78.93047}		\pgfmath@def{acos}{193}{78.87208}
\pgfmath@def{acos}{194}{78.81368}		\pgfmath@def{acos}{195}{78.75527}
\pgfmath@def{acos}{196}{78.69685}		\pgfmath@def{acos}{197}{78.63841}
\pgfmath@def{acos}{198}{78.57997}		\pgfmath@def{acos}{199}{78.52151}
\pgfmath@def{acos}{200}{78.46304}		\pgfmath@def{acos}{201}{78.40455}
\pgfmath@def{acos}{202}{78.34606}		\pgfmath@def{acos}{203}{78.28755}
\pgfmath@def{acos}{204}{78.22903}		\pgfmath@def{acos}{205}{78.17050}
\pgfmath@def{acos}{206}{78.11195}		\pgfmath@def{acos}{207}{78.05339}
\pgfmath@def{acos}{208}{77.99482}		\pgfmath@def{acos}{209}{77.93624}
\pgfmath@def{acos}{210}{77.87764}		\pgfmath@def{acos}{211}{77.81903}
\pgfmath@def{acos}{212}{77.76041}		\pgfmath@def{acos}{213}{77.70178}
\pgfmath@def{acos}{214}{77.64313}		\pgfmath@def{acos}{215}{77.58447}
\pgfmath@def{acos}{216}{77.52579}		\pgfmath@def{acos}{217}{77.46711}
\pgfmath@def{acos}{218}{77.40841}		\pgfmath@def{acos}{219}{77.34969}
\pgfmath@def{acos}{220}{77.29096}		\pgfmath@def{acos}{221}{77.23222}
\pgfmath@def{acos}{222}{77.17347}		\pgfmath@def{acos}{223}{77.11470}
\pgfmath@def{acos}{224}{77.05591}		\pgfmath@def{acos}{225}{76.99712}
\pgfmath@def{acos}{226}{76.93831}		\pgfmath@def{acos}{227}{76.87948}
\pgfmath@def{acos}{228}{76.82064}		\pgfmath@def{acos}{229}{76.76179}
\pgfmath@def{acos}{230}{76.70292}		\pgfmath@def{acos}{231}{76.64404}
\pgfmath@def{acos}{232}{76.58515}		\pgfmath@def{acos}{233}{76.52624}
\pgfmath@def{acos}{234}{76.46731}		\pgfmath@def{acos}{235}{76.40837}
\pgfmath@def{acos}{236}{76.34942}		\pgfmath@def{acos}{237}{76.29045}
\pgfmath@def{acos}{238}{76.23147}		\pgfmath@def{acos}{239}{76.17247}
\pgfmath@def{acos}{240}{76.11346}		\pgfmath@def{acos}{241}{76.05443}
\pgfmath@def{acos}{242}{75.99538}		\pgfmath@def{acos}{243}{75.93632}
\pgfmath@def{acos}{244}{75.87725}		\pgfmath@def{acos}{245}{75.81816}
\pgfmath@def{acos}{246}{75.75906}		\pgfmath@def{acos}{247}{75.69994}
\pgfmath@def{acos}{248}{75.64080}		\pgfmath@def{acos}{249}{75.58165}
\pgfmath@def{acos}{250}{75.52248}		\pgfmath@def{acos}{251}{75.46330}
\pgfmath@def{acos}{252}{75.40410}		\pgfmath@def{acos}{253}{75.34489}
\pgfmath@def{acos}{254}{75.28566}		\pgfmath@def{acos}{255}{75.22641}
\pgfmath@def{acos}{256}{75.16715}		\pgfmath@def{acos}{257}{75.10787}
\pgfmath@def{acos}{258}{75.04857}		\pgfmath@def{acos}{259}{74.98926}
\pgfmath@def{acos}{260}{74.92993}		\pgfmath@def{acos}{261}{74.87059}
\pgfmath@def{acos}{262}{74.81123}		\pgfmath@def{acos}{263}{74.75185}
\pgfmath@def{acos}{264}{74.69245}		\pgfmath@def{acos}{265}{74.63304}
\pgfmath@def{acos}{266}{74.57361}		\pgfmath@def{acos}{267}{74.51417}
\pgfmath@def{acos}{268}{74.45471}		\pgfmath@def{acos}{269}{74.39523}
\pgfmath@def{acos}{270}{74.33573}		\pgfmath@def{acos}{271}{74.27621}
\pgfmath@def{acos}{272}{74.21668}		\pgfmath@def{acos}{273}{74.15713}
\pgfmath@def{acos}{274}{74.09757}		\pgfmath@def{acos}{275}{74.03798}
\pgfmath@def{acos}{276}{73.97838}		\pgfmath@def{acos}{277}{73.91876}
\pgfmath@def{acos}{278}{73.85912}		\pgfmath@def{acos}{279}{73.79946}
\pgfmath@def{acos}{280}{73.73979}		\pgfmath@def{acos}{281}{73.68010}
\pgfmath@def{acos}{282}{73.62039}		\pgfmath@def{acos}{283}{73.56066}
\pgfmath@def{acos}{284}{73.50091}		\pgfmath@def{acos}{285}{73.44115}
\pgfmath@def{acos}{286}{73.38136}		\pgfmath@def{acos}{287}{73.32156}
\pgfmath@def{acos}{288}{73.26174}		\pgfmath@def{acos}{289}{73.20190}
\pgfmath@def{acos}{290}{73.14204}		\pgfmath@def{acos}{291}{73.08216}
\pgfmath@def{acos}{292}{73.02226}		\pgfmath@def{acos}{293}{72.96235}
\pgfmath@def{acos}{294}{72.90241}		\pgfmath@def{acos}{295}{72.84246}
\pgfmath@def{acos}{296}{72.78248}		\pgfmath@def{acos}{297}{72.72249}
\pgfmath@def{acos}{298}{72.66248}		\pgfmath@def{acos}{299}{72.60244}
\pgfmath@def{acos}{300}{72.54239}		\pgfmath@def{acos}{301}{72.48232}
\pgfmath@def{acos}{302}{72.42223}		\pgfmath@def{acos}{303}{72.36212}
\pgfmath@def{acos}{304}{72.30198}		\pgfmath@def{acos}{305}{72.24183}
\pgfmath@def{acos}{306}{72.18166}		\pgfmath@def{acos}{307}{72.12147}
\pgfmath@def{acos}{308}{72.06125}		\pgfmath@def{acos}{309}{72.00102}
\pgfmath@def{acos}{310}{71.94077}		\pgfmath@def{acos}{311}{71.88049}
\pgfmath@def{acos}{312}{71.82019}		\pgfmath@def{acos}{313}{71.75988}
\pgfmath@def{acos}{314}{71.69954}		\pgfmath@def{acos}{315}{71.63918}
\pgfmath@def{acos}{316}{71.57880}		\pgfmath@def{acos}{317}{71.51840}
\pgfmath@def{acos}{318}{71.45798}		\pgfmath@def{acos}{319}{71.39754}
\pgfmath@def{acos}{320}{71.33707}		\pgfmath@def{acos}{321}{71.27658}
\pgfmath@def{acos}{322}{71.21608}		\pgfmath@def{acos}{323}{71.15555}
\pgfmath@def{acos}{324}{71.09499}		\pgfmath@def{acos}{325}{71.03442}
\pgfmath@def{acos}{326}{70.97382}		\pgfmath@def{acos}{327}{70.91321}
\pgfmath@def{acos}{328}{70.85257}		\pgfmath@def{acos}{329}{70.79190}
\pgfmath@def{acos}{330}{70.73122}		\pgfmath@def{acos}{331}{70.67051}
\pgfmath@def{acos}{332}{70.60978}		\pgfmath@def{acos}{333}{70.54903}
\pgfmath@def{acos}{334}{70.48826}		\pgfmath@def{acos}{335}{70.42746}
\pgfmath@def{acos}{336}{70.36664}		\pgfmath@def{acos}{337}{70.30579}
\pgfmath@def{acos}{338}{70.24493}		\pgfmath@def{acos}{339}{70.18404}
\pgfmath@def{acos}{340}{70.12312}		\pgfmath@def{acos}{341}{70.06218}
\pgfmath@def{acos}{342}{70.00122}		\pgfmath@def{acos}{343}{69.94024}
\pgfmath@def{acos}{344}{69.87923}		\pgfmath@def{acos}{345}{69.81820}
\pgfmath@def{acos}{346}{69.75714}		\pgfmath@def{acos}{347}{69.69606}
\pgfmath@def{acos}{348}{69.63496}		\pgfmath@def{acos}{349}{69.57383}
\pgfmath@def{acos}{350}{69.51268}		\pgfmath@def{acos}{351}{69.45150}
\pgfmath@def{acos}{352}{69.39030}		\pgfmath@def{acos}{353}{69.32908}
\pgfmath@def{acos}{354}{69.26783}		\pgfmath@def{acos}{355}{69.20655}
\pgfmath@def{acos}{356}{69.14525}		\pgfmath@def{acos}{357}{69.08393}
\pgfmath@def{acos}{358}{69.02258}		\pgfmath@def{acos}{359}{68.96120}
\pgfmath@def{acos}{360}{68.89980}		\pgfmath@def{acos}{361}{68.83837}
\pgfmath@def{acos}{362}{68.77692}		\pgfmath@def{acos}{363}{68.71544}
\pgfmath@def{acos}{364}{68.65394}		\pgfmath@def{acos}{365}{68.59241}
\pgfmath@def{acos}{366}{68.53086}		\pgfmath@def{acos}{367}{68.46928}
\pgfmath@def{acos}{368}{68.40767}		\pgfmath@def{acos}{369}{68.34604}
\pgfmath@def{acos}{370}{68.28438}		\pgfmath@def{acos}{371}{68.22269}
\pgfmath@def{acos}{372}{68.16098}		\pgfmath@def{acos}{373}{68.09924}
\pgfmath@def{acos}{374}{68.03748}		\pgfmath@def{acos}{375}{67.97568}
\pgfmath@def{acos}{376}{67.91386}		\pgfmath@def{acos}{377}{67.85202}
\pgfmath@def{acos}{378}{67.79014}		\pgfmath@def{acos}{379}{67.72824}
\pgfmath@def{acos}{380}{67.66631}		\pgfmath@def{acos}{381}{67.60436}
\pgfmath@def{acos}{382}{67.54237}		\pgfmath@def{acos}{383}{67.48036}
\pgfmath@def{acos}{384}{67.41832}		\pgfmath@def{acos}{385}{67.35626}
\pgfmath@def{acos}{386}{67.29416}		\pgfmath@def{acos}{387}{67.23204}
\pgfmath@def{acos}{388}{67.16988}		\pgfmath@def{acos}{389}{67.10770}
\pgfmath@def{acos}{390}{67.04550}		\pgfmath@def{acos}{391}{66.98326}
\pgfmath@def{acos}{392}{66.92099}		\pgfmath@def{acos}{393}{66.85870}
\pgfmath@def{acos}{394}{66.79637}		\pgfmath@def{acos}{395}{66.73402}
\pgfmath@def{acos}{396}{66.67164}		\pgfmath@def{acos}{397}{66.60923}
\pgfmath@def{acos}{398}{66.54679}		\pgfmath@def{acos}{399}{66.48432}
\pgfmath@def{acos}{400}{66.42182}		\pgfmath@def{acos}{401}{66.35929}
\pgfmath@def{acos}{402}{66.29673}		\pgfmath@def{acos}{403}{66.23414}
\pgfmath@def{acos}{404}{66.17152}		\pgfmath@def{acos}{405}{66.10887}
\pgfmath@def{acos}{406}{66.04619}		\pgfmath@def{acos}{407}{65.98348}
\pgfmath@def{acos}{408}{65.92074}		\pgfmath@def{acos}{409}{65.85796}
\pgfmath@def{acos}{410}{65.79516}		\pgfmath@def{acos}{411}{65.73233}
\pgfmath@def{acos}{412}{65.66946}		\pgfmath@def{acos}{413}{65.60657}
\pgfmath@def{acos}{414}{65.54364}		\pgfmath@def{acos}{415}{65.48068}
\pgfmath@def{acos}{416}{65.41769}		\pgfmath@def{acos}{417}{65.35467}
\pgfmath@def{acos}{418}{65.29161}		\pgfmath@def{acos}{419}{65.22853}
\pgfmath@def{acos}{420}{65.16541}		\pgfmath@def{acos}{421}{65.10226}
\pgfmath@def{acos}{422}{65.03908}		\pgfmath@def{acos}{423}{64.97586}
\pgfmath@def{acos}{424}{64.91261}		\pgfmath@def{acos}{425}{64.84933}
\pgfmath@def{acos}{426}{64.78602}		\pgfmath@def{acos}{427}{64.72267}
\pgfmath@def{acos}{428}{64.65929}		\pgfmath@def{acos}{429}{64.59588}
\pgfmath@def{acos}{430}{64.53244}		\pgfmath@def{acos}{431}{64.46896}
\pgfmath@def{acos}{432}{64.40544}		\pgfmath@def{acos}{433}{64.34190}
\pgfmath@def{acos}{434}{64.27832}		\pgfmath@def{acos}{435}{64.21470}
\pgfmath@def{acos}{436}{64.15105}		\pgfmath@def{acos}{437}{64.08737}
\pgfmath@def{acos}{438}{64.02365}		\pgfmath@def{acos}{439}{63.95990}
\pgfmath@def{acos}{440}{63.89611}		\pgfmath@def{acos}{441}{63.83229}
\pgfmath@def{acos}{442}{63.76844}		\pgfmath@def{acos}{443}{63.70455}
\pgfmath@def{acos}{444}{63.64062}		\pgfmath@def{acos}{445}{63.57666}
\pgfmath@def{acos}{446}{63.51266}		\pgfmath@def{acos}{447}{63.44863}
\pgfmath@def{acos}{448}{63.38456}		\pgfmath@def{acos}{449}{63.32045}
\pgfmath@def{acos}{450}{63.25631}		\pgfmath@def{acos}{451}{63.19213}
\pgfmath@def{acos}{452}{63.12792}		\pgfmath@def{acos}{453}{63.06367}
\pgfmath@def{acos}{454}{62.99938}		\pgfmath@def{acos}{455}{62.93506}
\pgfmath@def{acos}{456}{62.87070}		\pgfmath@def{acos}{457}{62.80630}
\pgfmath@def{acos}{458}{62.74187}		\pgfmath@def{acos}{459}{62.67740}
\pgfmath@def{acos}{460}{62.61289}		\pgfmath@def{acos}{461}{62.54834}
\pgfmath@def{acos}{462}{62.48376}		\pgfmath@def{acos}{463}{62.41913}
\pgfmath@def{acos}{464}{62.35447}		\pgfmath@def{acos}{465}{62.28977}
\pgfmath@def{acos}{466}{62.22504}		\pgfmath@def{acos}{467}{62.16026}
\pgfmath@def{acos}{468}{62.09545}		\pgfmath@def{acos}{469}{62.03059}
\pgfmath@def{acos}{470}{61.96570}		\pgfmath@def{acos}{471}{61.90077}
\pgfmath@def{acos}{472}{61.83580}		\pgfmath@def{acos}{473}{61.77079}
\pgfmath@def{acos}{474}{61.70574}		\pgfmath@def{acos}{475}{61.64065}
\pgfmath@def{acos}{476}{61.57552}		\pgfmath@def{acos}{477}{61.51035}
\pgfmath@def{acos}{478}{61.44514}		\pgfmath@def{acos}{479}{61.37988}
\pgfmath@def{acos}{480}{61.31459}		\pgfmath@def{acos}{481}{61.24926}
\pgfmath@def{acos}{482}{61.18389}		\pgfmath@def{acos}{483}{61.11847}
\pgfmath@def{acos}{484}{61.05302}		\pgfmath@def{acos}{485}{60.98752}
\pgfmath@def{acos}{486}{60.92199}		\pgfmath@def{acos}{487}{60.85641}
\pgfmath@def{acos}{488}{60.79078}		\pgfmath@def{acos}{489}{60.72512}
\pgfmath@def{acos}{490}{60.65941}		\pgfmath@def{acos}{491}{60.59367}
\pgfmath@def{acos}{492}{60.52787}		\pgfmath@def{acos}{493}{60.46204}
\pgfmath@def{acos}{494}{60.39616}		\pgfmath@def{acos}{495}{60.33025}
\pgfmath@def{acos}{496}{60.26428}		\pgfmath@def{acos}{497}{60.19828}
\pgfmath@def{acos}{498}{60.13223}		\pgfmath@def{acos}{499}{60.06613}
\pgfmath@def{acos}{500}{60.00000}		\pgfmath@def{acos}{501}{59.93381}
\pgfmath@def{acos}{502}{59.86759}		\pgfmath@def{acos}{503}{59.80132}
\pgfmath@def{acos}{504}{59.73500}		\pgfmath@def{acos}{505}{59.66864}
\pgfmath@def{acos}{506}{59.60224}		\pgfmath@def{acos}{507}{59.53579}
\pgfmath@def{acos}{508}{59.46929}		\pgfmath@def{acos}{509}{59.40275}
\pgfmath@def{acos}{510}{59.33617}		\pgfmath@def{acos}{511}{59.26953}
\pgfmath@def{acos}{512}{59.20285}		\pgfmath@def{acos}{513}{59.13613}
\pgfmath@def{acos}{514}{59.06936}		\pgfmath@def{acos}{515}{59.00254}
\pgfmath@def{acos}{516}{58.93568}		\pgfmath@def{acos}{517}{58.86876}
\pgfmath@def{acos}{518}{58.80180}		\pgfmath@def{acos}{519}{58.73480}
\pgfmath@def{acos}{520}{58.66774}		\pgfmath@def{acos}{521}{58.60064}
\pgfmath@def{acos}{522}{58.53349}		\pgfmath@def{acos}{523}{58.46629}
\pgfmath@def{acos}{524}{58.39905}		\pgfmath@def{acos}{525}{58.33175}
\pgfmath@def{acos}{526}{58.26441}		\pgfmath@def{acos}{527}{58.19702}
\pgfmath@def{acos}{528}{58.12957}		\pgfmath@def{acos}{529}{58.06208}
\pgfmath@def{acos}{530}{57.99454}		\pgfmath@def{acos}{531}{57.92695}
\pgfmath@def{acos}{532}{57.85931}		\pgfmath@def{acos}{533}{57.79162}
\pgfmath@def{acos}{534}{57.72388}		\pgfmath@def{acos}{535}{57.65608}
\pgfmath@def{acos}{536}{57.58824}		\pgfmath@def{acos}{537}{57.52035}
\pgfmath@def{acos}{538}{57.45240}		\pgfmath@def{acos}{539}{57.38441}
\pgfmath@def{acos}{540}{57.31636}		\pgfmath@def{acos}{541}{57.24826}
\pgfmath@def{acos}{542}{57.18010}		\pgfmath@def{acos}{543}{57.11190}
\pgfmath@def{acos}{544}{57.04364}		\pgfmath@def{acos}{545}{56.97533}
\pgfmath@def{acos}{546}{56.90697}		\pgfmath@def{acos}{547}{56.83855}
\pgfmath@def{acos}{548}{56.77008}		\pgfmath@def{acos}{549}{56.70156}
\pgfmath@def{acos}{550}{56.63298}		\pgfmath@def{acos}{551}{56.56435}
\pgfmath@def{acos}{552}{56.49567}		\pgfmath@def{acos}{553}{56.42693}
\pgfmath@def{acos}{554}{56.35813}		\pgfmath@def{acos}{555}{56.28928}
\pgfmath@def{acos}{556}{56.22038}		\pgfmath@def{acos}{557}{56.15141}
\pgfmath@def{acos}{558}{56.08240}		\pgfmath@def{acos}{559}{56.01333}
\pgfmath@def{acos}{560}{55.94420}		\pgfmath@def{acos}{561}{55.87501}
\pgfmath@def{acos}{562}{55.80577}		\pgfmath@def{acos}{563}{55.73647}
\pgfmath@def{acos}{564}{55.66712}		\pgfmath@def{acos}{565}{55.59770}
\pgfmath@def{acos}{566}{55.52823}		\pgfmath@def{acos}{567}{55.45871}
\pgfmath@def{acos}{568}{55.38912}		\pgfmath@def{acos}{569}{55.31947}
\pgfmath@def{acos}{570}{55.24977}		\pgfmath@def{acos}{571}{55.18001}
\pgfmath@def{acos}{572}{55.11019}		\pgfmath@def{acos}{573}{55.04030}
\pgfmath@def{acos}{574}{54.97036}		\pgfmath@def{acos}{575}{54.90036}
\pgfmath@def{acos}{576}{54.83030}		\pgfmath@def{acos}{577}{54.76018}
\pgfmath@def{acos}{578}{54.69000}		\pgfmath@def{acos}{579}{54.61976}
\pgfmath@def{acos}{580}{54.54945}		\pgfmath@def{acos}{581}{54.47909}
\pgfmath@def{acos}{582}{54.40866}		\pgfmath@def{acos}{583}{54.33817}
\pgfmath@def{acos}{584}{54.26762}		\pgfmath@def{acos}{585}{54.19701}
\pgfmath@def{acos}{586}{54.12633}		\pgfmath@def{acos}{587}{54.05559}
\pgfmath@def{acos}{588}{53.98479}		\pgfmath@def{acos}{589}{53.91392}
\pgfmath@def{acos}{590}{53.84299}		\pgfmath@def{acos}{591}{53.77199}
\pgfmath@def{acos}{592}{53.70093}		\pgfmath@def{acos}{593}{53.62981}
\pgfmath@def{acos}{594}{53.55862}		\pgfmath@def{acos}{595}{53.48736}
\pgfmath@def{acos}{596}{53.41604}		\pgfmath@def{acos}{597}{53.34466}
\pgfmath@def{acos}{598}{53.27320}		\pgfmath@def{acos}{599}{53.20168}
\pgfmath@def{acos}{600}{53.13010}		\pgfmath@def{acos}{601}{53.05844}
\pgfmath@def{acos}{602}{52.98672}		\pgfmath@def{acos}{603}{52.91494}
\pgfmath@def{acos}{604}{52.84308}		\pgfmath@def{acos}{605}{52.77115}
\pgfmath@def{acos}{606}{52.69916}		\pgfmath@def{acos}{607}{52.62710}
\pgfmath@def{acos}{608}{52.55497}		\pgfmath@def{acos}{609}{52.48276}
\pgfmath@def{acos}{610}{52.41049}		\pgfmath@def{acos}{611}{52.33815}
\pgfmath@def{acos}{612}{52.26574}		\pgfmath@def{acos}{613}{52.19326}
\pgfmath@def{acos}{614}{52.12070}		\pgfmath@def{acos}{615}{52.04808}
\pgfmath@def{acos}{616}{51.97538}		\pgfmath@def{acos}{617}{51.90261}
\pgfmath@def{acos}{618}{51.82976}		\pgfmath@def{acos}{619}{51.75685}
\pgfmath@def{acos}{620}{51.68386}		\pgfmath@def{acos}{621}{51.61080}
\pgfmath@def{acos}{622}{51.53766}		\pgfmath@def{acos}{623}{51.46445}
\pgfmath@def{acos}{624}{51.39117}		\pgfmath@def{acos}{625}{51.31781}
\pgfmath@def{acos}{626}{51.24437}		\pgfmath@def{acos}{627}{51.17086}
\pgfmath@def{acos}{628}{51.09728}		\pgfmath@def{acos}{629}{51.02361}
\pgfmath@def{acos}{630}{50.94987}		\pgfmath@def{acos}{631}{50.87606}
\pgfmath@def{acos}{632}{50.80216}		\pgfmath@def{acos}{633}{50.72819}
\pgfmath@def{acos}{634}{50.65414}		\pgfmath@def{acos}{635}{50.58001}
\pgfmath@def{acos}{636}{50.50580}		\pgfmath@def{acos}{637}{50.43152}
\pgfmath@def{acos}{638}{50.35715}		\pgfmath@def{acos}{639}{50.28270}
\pgfmath@def{acos}{640}{50.20818}		\pgfmath@def{acos}{641}{50.13357}
\pgfmath@def{acos}{642}{50.05888}		\pgfmath@def{acos}{643}{49.98411}
\pgfmath@def{acos}{644}{49.90926}		\pgfmath@def{acos}{645}{49.83432}
\pgfmath@def{acos}{646}{49.75930}		\pgfmath@def{acos}{647}{49.68420}
\pgfmath@def{acos}{648}{49.60902}		\pgfmath@def{acos}{649}{49.53375}
\pgfmath@def{acos}{650}{49.45839}		\pgfmath@def{acos}{651}{49.38296}
\pgfmath@def{acos}{652}{49.30743}		\pgfmath@def{acos}{653}{49.23182}
\pgfmath@def{acos}{654}{49.15613}		\pgfmath@def{acos}{655}{49.08035}
\pgfmath@def{acos}{656}{49.00448}		\pgfmath@def{acos}{657}{48.92852}
\pgfmath@def{acos}{658}{48.85248}		\pgfmath@def{acos}{659}{48.77634}
\pgfmath@def{acos}{660}{48.70012}		\pgfmath@def{acos}{661}{48.62381}
\pgfmath@def{acos}{662}{48.54741}		\pgfmath@def{acos}{663}{48.47092}
\pgfmath@def{acos}{664}{48.39434}		\pgfmath@def{acos}{665}{48.31767}
\pgfmath@def{acos}{666}{48.24091}		\pgfmath@def{acos}{667}{48.16405}
\pgfmath@def{acos}{668}{48.08710}		\pgfmath@def{acos}{669}{48.01006}
\pgfmath@def{acos}{670}{47.93293}		\pgfmath@def{acos}{671}{47.85570}
\pgfmath@def{acos}{672}{47.77838}		\pgfmath@def{acos}{673}{47.70096}
\pgfmath@def{acos}{674}{47.62345}		\pgfmath@def{acos}{675}{47.54585}
\pgfmath@def{acos}{676}{47.46814}		\pgfmath@def{acos}{677}{47.39034}
\pgfmath@def{acos}{678}{47.31244}		\pgfmath@def{acos}{679}{47.23445}
\pgfmath@def{acos}{680}{47.15635}		\pgfmath@def{acos}{681}{47.07816}
\pgfmath@def{acos}{682}{46.99987}		\pgfmath@def{acos}{683}{46.92147}
\pgfmath@def{acos}{684}{46.84298}		\pgfmath@def{acos}{685}{46.76439}
\pgfmath@def{acos}{686}{46.68569}		\pgfmath@def{acos}{687}{46.60690}
\pgfmath@def{acos}{688}{46.52800}		\pgfmath@def{acos}{689}{46.44899}
\pgfmath@def{acos}{690}{46.36989}		\pgfmath@def{acos}{691}{46.29068}
\pgfmath@def{acos}{692}{46.21136}		\pgfmath@def{acos}{693}{46.13194}
\pgfmath@def{acos}{694}{46.05241}		\pgfmath@def{acos}{695}{45.97278}
\pgfmath@def{acos}{696}{45.89304}		\pgfmath@def{acos}{697}{45.81319}
\pgfmath@def{acos}{698}{45.73323}		\pgfmath@def{acos}{699}{45.65317}
\pgfmath@def{acos}{700}{45.57299}		\pgfmath@def{acos}{701}{45.49271}
\pgfmath@def{acos}{702}{45.41231}		\pgfmath@def{acos}{703}{45.33180}
\pgfmath@def{acos}{704}{45.25118}		\pgfmath@def{acos}{705}{45.17045}
\pgfmath@def{acos}{706}{45.08961}		\pgfmath@def{acos}{707}{45.00865}
\pgfmath@def{acos}{708}{44.92757}		\pgfmath@def{acos}{709}{44.84638}
\pgfmath@def{acos}{710}{44.76508}		\pgfmath@def{acos}{711}{44.68366}
\pgfmath@def{acos}{712}{44.60212}		\pgfmath@def{acos}{713}{44.52046}
\pgfmath@def{acos}{714}{44.43869}		\pgfmath@def{acos}{715}{44.35680}
\pgfmath@def{acos}{716}{44.27478}		\pgfmath@def{acos}{717}{44.19265}
\pgfmath@def{acos}{718}{44.11039}		\pgfmath@def{acos}{719}{44.02802}
\pgfmath@def{acos}{720}{43.94552}		\pgfmath@def{acos}{721}{43.86289}
\pgfmath@def{acos}{722}{43.78014}		\pgfmath@def{acos}{723}{43.69727}
\pgfmath@def{acos}{724}{43.61427}		\pgfmath@def{acos}{725}{43.53115}
\pgfmath@def{acos}{726}{43.44790}		\pgfmath@def{acos}{727}{43.36452}
\pgfmath@def{acos}{728}{43.28101}		\pgfmath@def{acos}{729}{43.19737}
\pgfmath@def{acos}{730}{43.11360}		\pgfmath@def{acos}{731}{43.02970}
\pgfmath@def{acos}{732}{42.94567}		\pgfmath@def{acos}{733}{42.86151}
\pgfmath@def{acos}{734}{42.77721}		\pgfmath@def{acos}{735}{42.69278}
\pgfmath@def{acos}{736}{42.60821}		\pgfmath@def{acos}{737}{42.52351}
\pgfmath@def{acos}{738}{42.43867}		\pgfmath@def{acos}{739}{42.35370}
\pgfmath@def{acos}{740}{42.26858}		\pgfmath@def{acos}{741}{42.18333}
\pgfmath@def{acos}{742}{42.09793}		\pgfmath@def{acos}{743}{42.01240}
\pgfmath@def{acos}{744}{41.92672}		\pgfmath@def{acos}{745}{41.84090}
\pgfmath@def{acos}{746}{41.75493}		\pgfmath@def{acos}{747}{41.66882}
\pgfmath@def{acos}{748}{41.58257}		\pgfmath@def{acos}{749}{41.49617}
\pgfmath@def{acos}{750}{41.40962}		\pgfmath@def{acos}{751}{41.32292}
\pgfmath@def{acos}{752}{41.23607}		\pgfmath@def{acos}{753}{41.14908}
\pgfmath@def{acos}{754}{41.06193}		\pgfmath@def{acos}{755}{40.97463}
\pgfmath@def{acos}{756}{40.88717}		\pgfmath@def{acos}{757}{40.79956}
\pgfmath@def{acos}{758}{40.71180}		\pgfmath@def{acos}{759}{40.62388}
\pgfmath@def{acos}{760}{40.53580}		\pgfmath@def{acos}{761}{40.44756}
\pgfmath@def{acos}{762}{40.35916}		\pgfmath@def{acos}{763}{40.27061}
\pgfmath@def{acos}{764}{40.18189}		\pgfmath@def{acos}{765}{40.09300}
\pgfmath@def{acos}{766}{40.00396}		\pgfmath@def{acos}{767}{39.91474}
\pgfmath@def{acos}{768}{39.82537}		\pgfmath@def{acos}{769}{39.73582}
\pgfmath@def{acos}{770}{39.64611}		\pgfmath@def{acos}{771}{39.55622}
\pgfmath@def{acos}{772}{39.46617}		\pgfmath@def{acos}{773}{39.37594}
\pgfmath@def{acos}{774}{39.28554}		\pgfmath@def{acos}{775}{39.19496}
\pgfmath@def{acos}{776}{39.10421}		\pgfmath@def{acos}{777}{39.01328}
\pgfmath@def{acos}{778}{38.92218}		\pgfmath@def{acos}{779}{38.83089}
\pgfmath@def{acos}{780}{38.73942}		\pgfmath@def{acos}{781}{38.64777}
\pgfmath@def{acos}{782}{38.55594}		\pgfmath@def{acos}{783}{38.46392}
\pgfmath@def{acos}{784}{38.37171}		\pgfmath@def{acos}{785}{38.27932}
\pgfmath@def{acos}{786}{38.18673}		\pgfmath@def{acos}{787}{38.09396}
\pgfmath@def{acos}{788}{38.00100}		\pgfmath@def{acos}{789}{37.90784}
\pgfmath@def{acos}{790}{37.81448}		\pgfmath@def{acos}{791}{37.72093}
\pgfmath@def{acos}{792}{37.62719}		\pgfmath@def{acos}{793}{37.53324}
\pgfmath@def{acos}{794}{37.43909}		\pgfmath@def{acos}{795}{37.34474}
\pgfmath@def{acos}{796}{37.25019}		\pgfmath@def{acos}{797}{37.15542}
\pgfmath@def{acos}{798}{37.06046}		\pgfmath@def{acos}{799}{36.96528}
\pgfmath@def{acos}{800}{36.86989}		\pgfmath@def{acos}{801}{36.77429}
\pgfmath@def{acos}{802}{36.67848}		\pgfmath@def{acos}{803}{36.58245}
\pgfmath@def{acos}{804}{36.48621}		\pgfmath@def{acos}{805}{36.38974}
\pgfmath@def{acos}{806}{36.29305}		\pgfmath@def{acos}{807}{36.19615}
\pgfmath@def{acos}{808}{36.09901}		\pgfmath@def{acos}{809}{36.00165}
\pgfmath@def{acos}{810}{35.90406}		\pgfmath@def{acos}{811}{35.80625}
\pgfmath@def{acos}{812}{35.70820}		\pgfmath@def{acos}{813}{35.60991}
\pgfmath@def{acos}{814}{35.51139}		\pgfmath@def{acos}{815}{35.41263}
\pgfmath@def{acos}{816}{35.31364}		\pgfmath@def{acos}{817}{35.21440}
\pgfmath@def{acos}{818}{35.11491}		\pgfmath@def{acos}{819}{35.01518}
\pgfmath@def{acos}{820}{34.91520}		\pgfmath@def{acos}{821}{34.81497}
\pgfmath@def{acos}{822}{34.71449}		\pgfmath@def{acos}{823}{34.61375}
\pgfmath@def{acos}{824}{34.51276}		\pgfmath@def{acos}{825}{34.41150}
\pgfmath@def{acos}{826}{34.30999}		\pgfmath@def{acos}{827}{34.20821}
\pgfmath@def{acos}{828}{34.10616}		\pgfmath@def{acos}{829}{34.00385}
\pgfmath@def{acos}{830}{33.90126}		\pgfmath@def{acos}{831}{33.79840}
\pgfmath@def{acos}{832}{33.69526}		\pgfmath@def{acos}{833}{33.59184}
\pgfmath@def{acos}{834}{33.48814}		\pgfmath@def{acos}{835}{33.38416}
\pgfmath@def{acos}{836}{33.27989}		\pgfmath@def{acos}{837}{33.17533}
\pgfmath@def{acos}{838}{33.07047}		\pgfmath@def{acos}{839}{32.96532}
\pgfmath@def{acos}{840}{32.85988}		\pgfmath@def{acos}{841}{32.75413}
\pgfmath@def{acos}{842}{32.64807}		\pgfmath@def{acos}{843}{32.54171}
\pgfmath@def{acos}{844}{32.43504}		\pgfmath@def{acos}{845}{32.32806}
\pgfmath@def{acos}{846}{32.22076}		\pgfmath@def{acos}{847}{32.11314}
\pgfmath@def{acos}{848}{32.00520}		\pgfmath@def{acos}{849}{31.89693}
\pgfmath@def{acos}{850}{31.78833}		\pgfmath@def{acos}{851}{31.67939}
\pgfmath@def{acos}{852}{31.57012}		\pgfmath@def{acos}{853}{31.46051}
\pgfmath@def{acos}{854}{31.35056}		\pgfmath@def{acos}{855}{31.24026}
\pgfmath@def{acos}{856}{31.12961}		\pgfmath@def{acos}{857}{31.01860}
\pgfmath@def{acos}{858}{30.90724}		\pgfmath@def{acos}{859}{30.79551}
\pgfmath@def{acos}{860}{30.68341}		\pgfmath@def{acos}{861}{30.57095}
\pgfmath@def{acos}{862}{30.45811}		\pgfmath@def{acos}{863}{30.34489}
\pgfmath@def{acos}{864}{30.23128}		\pgfmath@def{acos}{865}{30.11729}
\pgfmath@def{acos}{866}{30.00291}		\pgfmath@def{acos}{867}{29.88813}
\pgfmath@def{acos}{868}{29.77294}		\pgfmath@def{acos}{869}{29.65736}
\pgfmath@def{acos}{870}{29.54136}		\pgfmath@def{acos}{871}{29.42494}
\pgfmath@def{acos}{872}{29.30810}		\pgfmath@def{acos}{873}{29.19084}
\pgfmath@def{acos}{874}{29.07315}		\pgfmath@def{acos}{875}{28.95502}
\pgfmath@def{acos}{876}{28.83645}		\pgfmath@def{acos}{877}{28.71743}
\pgfmath@def{acos}{878}{28.59796}		\pgfmath@def{acos}{879}{28.47803}
\pgfmath@def{acos}{880}{28.35763}		\pgfmath@def{acos}{881}{28.23677}
\pgfmath@def{acos}{882}{28.11542}		\pgfmath@def{acos}{883}{27.99360}
\pgfmath@def{acos}{884}{27.87128}		\pgfmath@def{acos}{885}{27.74847}
\pgfmath@def{acos}{886}{27.62516}		\pgfmath@def{acos}{887}{27.50134}
\pgfmath@def{acos}{888}{27.37700}		\pgfmath@def{acos}{889}{27.25214}
\pgfmath@def{acos}{890}{27.12675}		\pgfmath@def{acos}{891}{27.00082}
\pgfmath@def{acos}{892}{26.87434}		\pgfmath@def{acos}{893}{26.74731}
\pgfmath@def{acos}{894}{26.61973}		\pgfmath@def{acos}{895}{26.49157}
\pgfmath@def{acos}{896}{26.36283}		\pgfmath@def{acos}{897}{26.23351}
\pgfmath@def{acos}{898}{26.10359}		\pgfmath@def{acos}{899}{25.97306}
\pgfmath@def{acos}{900}{25.84193}		\pgfmath@def{acos}{901}{25.71017}
\pgfmath@def{acos}{902}{25.57778}		\pgfmath@def{acos}{903}{25.44475}
\pgfmath@def{acos}{904}{25.31106}		\pgfmath@def{acos}{905}{25.17671}
\pgfmath@def{acos}{906}{25.04169}		\pgfmath@def{acos}{907}{24.90598}
\pgfmath@def{acos}{908}{24.76958}		\pgfmath@def{acos}{909}{24.63247}
\pgfmath@def{acos}{910}{24.49464}		\pgfmath@def{acos}{911}{24.35608}
\pgfmath@def{acos}{912}{24.21678}		\pgfmath@def{acos}{913}{24.07672}
\pgfmath@def{acos}{914}{23.93588}		\pgfmath@def{acos}{915}{23.79427}
\pgfmath@def{acos}{916}{23.65185}		\pgfmath@def{acos}{917}{23.50863}
\pgfmath@def{acos}{918}{23.36457}		\pgfmath@def{acos}{919}{23.21967}
\pgfmath@def{acos}{920}{23.07391}		\pgfmath@def{acos}{921}{22.92728}
\pgfmath@def{acos}{922}{22.77975}		\pgfmath@def{acos}{923}{22.63132}
\pgfmath@def{acos}{924}{22.48195}		\pgfmath@def{acos}{925}{22.33164}
\pgfmath@def{acos}{926}{22.18036}		\pgfmath@def{acos}{927}{22.02810}
\pgfmath@def{acos}{928}{21.87483}		\pgfmath@def{acos}{929}{21.72053}
\pgfmath@def{acos}{930}{21.56518}		\pgfmath@def{acos}{931}{21.40876}
\pgfmath@def{acos}{932}{21.25124}		\pgfmath@def{acos}{933}{21.09260}
\pgfmath@def{acos}{934}{20.93281}		\pgfmath@def{acos}{935}{20.77185}
\pgfmath@def{acos}{936}{20.60969}		\pgfmath@def{acos}{937}{20.44630}
\pgfmath@def{acos}{938}{20.28165}		\pgfmath@def{acos}{939}{20.11570}
\pgfmath@def{acos}{940}{19.94844}		\pgfmath@def{acos}{941}{19.77982}
\pgfmath@def{acos}{942}{19.60981}		\pgfmath@def{acos}{943}{19.43837}
\pgfmath@def{acos}{944}{19.26546}		\pgfmath@def{acos}{945}{19.09105}
\pgfmath@def{acos}{946}{18.91509}		\pgfmath@def{acos}{947}{18.73754}
\pgfmath@def{acos}{948}{18.55835}		\pgfmath@def{acos}{949}{18.37748}
\pgfmath@def{acos}{950}{18.19487}		\pgfmath@def{acos}{951}{18.01047}
\pgfmath@def{acos}{952}{17.82423}		\pgfmath@def{acos}{953}{17.63609}
\pgfmath@def{acos}{954}{17.44598}		\pgfmath@def{acos}{955}{17.25385}
\pgfmath@def{acos}{956}{17.05962}		\pgfmath@def{acos}{957}{16.86322}
\pgfmath@def{acos}{958}{16.66457}		\pgfmath@def{acos}{959}{16.46359}
\pgfmath@def{acos}{960}{16.26020}		\pgfmath@def{acos}{961}{16.05430}
\pgfmath@def{acos}{962}{15.84580}		\pgfmath@def{acos}{963}{15.63459}
\pgfmath@def{acos}{964}{15.42057}		\pgfmath@def{acos}{965}{15.20360}
\pgfmath@def{acos}{966}{14.98357}		\pgfmath@def{acos}{967}{14.76033}
\pgfmath@def{acos}{968}{14.53374}		\pgfmath@def{acos}{969}{14.30364}
\pgfmath@def{acos}{970}{14.06986}		\pgfmath@def{acos}{971}{13.83221}
\pgfmath@def{acos}{972}{13.59049}		\pgfmath@def{acos}{973}{13.34447}
\pgfmath@def{acos}{974}{13.09392}		\pgfmath@def{acos}{975}{12.83856}
\pgfmath@def{acos}{976}{12.57811}		\pgfmath@def{acos}{977}{12.31225}
\pgfmath@def{acos}{978}{12.04060}		\pgfmath@def{acos}{979}{11.76278}
\pgfmath@def{acos}{980}{11.47834}		\pgfmath@def{acos}{981}{11.18676}
\pgfmath@def{acos}{982}{10.88748}		\pgfmath@def{acos}{983}{10.57984}
\pgfmath@def{acos}{984}{10.26309}		\pgfmath@def{acos}{985}{9.93636}
\pgfmath@def{acos}{986}{9.59863}		\pgfmath@def{acos}{987}{9.24870}
\pgfmath@def{acos}{988}{8.88512}		\pgfmath@def{acos}{989}{8.50614}
\pgfmath@def{acos}{990}{8.10961}		\pgfmath@def{acos}{991}{7.69281}
\pgfmath@def{acos}{992}{7.25224}		\pgfmath@def{acos}{993}{6.78328}
\pgfmath@def{acos}{994}{6.27958}		\pgfmath@def{acos}{995}{5.73196}
\pgfmath@def{acos}{996}{5.12640}		\pgfmath@def{acos}{997}{4.43922}
\pgfmath@def{acos}{998}{3.62430}		\pgfmath@def{acos}{999}{2.56255}
\pgfmath@def{acos}{1000}{0.00000}

==> pgfmathutil.code.tex <==
% Copyright 2007 Mark Wibrow
%
% but subject to the LaTeX Project Public License 
% (http://www.latex-project.org/lppl.txt)
%
% and the GNU Public License 
% (http://www.gnu.org/licenses/gpl.txt)
%

% This file defines utilities common to the \pgfmath files.
%
% Version 1.414213 29/9/2007

\def\pgfmathincluded{}

% \pgfmath@ensureregister
%
% Ensure a control sequence exists as a TeX count/dimen register.
%
% #1 - count or dimen.
% #2 - a control sequence.
%
\newbox\pgfmath@box%
\def\pgfmath@ensureregister#1#2{%
	\setbox\pgfmath@box\hbox\bgroup% In case #2 is a defined macro. Unlikely, but you never know...
		\afterassignment\pgfmath@@ensureregister%
		\noexpand#20.0pt\let\pgfmath@temp\relax\relax\pgfmath@#2#1\pgfmath@}

\def\pgfmath@@ensureregister#1#2\pgfmath@#3#4#5\pgfmath@{%
	\egroup%
	\ifx#4c% 
		\ifx#1.% Already a count register.
		\else%
			\csname newcount\endcsname#3% This gets round \outer in plain TeX.
		\fi%
	\else%
		\ifx#4d% 
			\ifx\let#1% Already a dimen register.
			\else%
				\csname newdimen\endcsname#3%
			\fi%
		\fi%
	\fi%
}

% Check registers exist. If not, create them. 
%
\pgfmath@ensureregister{dimen}{\pgf@x}
\pgfmath@ensureregister{dimen}{\pgf@xa}
\pgfmath@ensureregister{dimen}{\pgf@xb}
\pgfmath@ensureregister{dimen}{\pgf@xc}

\pgfmath@ensureregister{dimen}{\pgf@y}
\pgfmath@ensureregister{dimen}{\pgf@ya}
\pgfmath@ensureregister{dimen}{\pgf@yb}
\pgfmath@ensureregister{dimen}{\pgf@yc}

\pgfmath@ensureregister{dimen}{\pgfutil@tempdima}
\pgfmath@ensureregister{dimen}{\pgfutil@tempdimb}

\pgfmath@ensureregister{count}{\c@pgf@counta}
\pgfmath@ensureregister{count}{\c@pgf@countb}
\pgfmath@ensureregister{count}{\c@pgf@countc}
\pgfmath@ensureregister{count}{\c@pgf@countd}

\pgfmath@ensureregister{count}{\pgfutil@tempcnta}
\pgfmath@ensureregister{count}{\pgfutil@tempcntb}

% Alias for \pgfmath.
%
\let\pgfmath@x\pgf@x
\let\pgfmath@xa\pgf@xa
\let\pgfmath@xb\pgf@xb
\let\pgfmath@xc\pgf@xc

\let\pgfmath@y\pgf@y
\let\pgfmath@ya\pgf@ya
\let\pgfmath@yb\pgf@yb
\let\pgfmath@yc\pgf@yc

\let\pgfmath@tempdima\pgfutil@tempdima
\let\pgfmath@tempdima\pgfutil@tempdima

\let\c@pgfmath@counta\c@pgf@counta
\let\c@pgfmath@countb\c@pgf@countb
\let\c@pgfmath@countc\c@pgf@countc
\let\c@pgfmath@countd\c@pgf@countd

\let\pgfmath@tempcnta\pgfutil@tempcnta
\let\pgfmath@tempcntb\pgfutil@tempcntb

% Now check if pgfutil and pgf@sys stuff exists. If it does, fine.
% Just \let pgfmath versions. If not, define pgfmath versions (Arghhh). 
%

% \...ifnextchar
%
\ifx\pgfutil@ifnextchar\pgfmath@undefined%
	\long\def\pgfmath@ifnextchar#1#2#3{%
  \let\pgfmath@reserved@d#1%
  \def\pgfmath@reserved@a{#2}%
  \def\pgfmath@reserved@b{#3}%
  \futurelet\pgfmath@let@token\pgfmath@ifnch}
	\def\pgfmath@ifnch{%
	  \ifx\pgfmath@let@token\pgfmath@sptoken%
	    \let\pgfmath@reserved@c\pgfmath@xifnch%
	  \else%
	    \ifx\pgfmath@let@token\pgfmath@reserved@d%
	      \let\pgfmath@reserved@c\pgfmath@reserved@a%
	    \else%
	      \let\pgfmath@reserved@c\pgfmath@reserved@b%
	    \fi%
	  \fi%
	  \pgfmath@reserved@c}
	{%
	  \def\:{\global\let\pgfmath@sptoken= } \:
	  \def\:{\pgfmath@xifnch} \expandafter\gdef\: {\futurelet\pgfmath@let@token\pgfmath@ifnch}
	}%
\else%
	\let\pgfmath@ifnextchar\pgfutil@ifnextchar%
	% Still need to define \pgfmath@sptoken (cannot \let).
	{%
		\def\:{\global\let\pgfmath@sptoken= } \:
	}%
\fi%

% \...ifundefined
%
\ifx\pgfutil@ifundefined\pgfmath@undefined%
	\long\def\pgfmath@ifundefined#1{%
	  \expandafter\ifx\csname#1\endcsname\relax%
	    \expandafter\pgfmath@firstoftwo%
	  \else%
	    \expandafter\pgfmath@secondoftwo%
	  \fi}%
\else%
	\let\pgfmath@ifundefined\pgfutil@ifundefined%
\fi%

% \...selectfont
%
\ifx\pgfutil@selectfont\pgfmath@undefined%
	\ifx\selectfont\pgfmath@undefined%
		\let\pgfmath@selectfont\rm% Plain TeX and ConTeXt.
	\else%
		\let\pgfmath@selectfont\selectfont% LaTeX.
	\fi%
\else%
	\let\pgfmath@selectfont\pgfutil@selectfont%
\fi%

% New definition easier than fussing around with let.
%
\newif\ifpgfmath@in@
\def\pgfmath@in@#1#2{%
 \def\pgfmath@in@@##1#1##2##3\pgfmath@in@@{%
  \ifx\pgfmath@in@##2\pgfmath@in@false\else\pgfmath@in@true\fi}%
 \pgfmath@in@@#2#1\pgfmath@in@\pgfmath@in@@}


% \...tonumber
%
\ifx\pgf@sys@tonumber\pgfmath@undefined%
  {\catcode`\p=12\catcode`\t=12\gdef\Pgf@geT#1pt{#1}}
	\def\pgfmath@tonumber#1{\expandafter\Pgf@geT\the#1}
\else%
	\let\pgfmath@tonumber\pgf@sys@tonumber%
\fi%


% \PackageWarning and \PackageError
%
\ifx\PackageWarning\pgfmath@undefined
	\def\pgfmath@PackageWarning#1#2{\immediate\write-1{Package #1: Warning! #2.}}%
\else%
	\let\pgfmath@PackageWarning\PackageWarning%
\fi%
\ifx\PackageError\pgfmath@undefined
	\def\pgfmath@PackageError#1#2#3{\immediate\write-1{Package #1: Error! #2.}}%
\else%
	\let\pgfmath@PackageError\PackageError%
\fi%

\def\pgfmath@error#1#2{\pgfmath@PackageError{PGF Math}{#1}{#2}}
\def\pgfmath@warning#1{\pgfmath@PackageWarning{PGF Math}{#1}}

% \pgfmath@pt
%
% Needed to test for 'pt' resulting from expansion using \the.
%
{\catcode`\p=12\catcode`\t=12\gdef\PgfmaTh@PT{pt}}		
\edef\pgfmath@pt{\PgfmaTh@PT}%

% \pgfmath@empty
%
% A handy macro.
%
\def\pgfmath@empty{}

\def\pgfmath@firstoftwo#1#2{#1}
\def\pgfmath@secondoftwo#1#2{#2}

% \pgfmath@gobbletilpgfmath@
%
% Gobble stream until \pgfmath@ {which is undefined}.
% 
\def\pgfmath@gobbletilpgfmath@#1\pgfmath@{}
\def\pgfmath@gobbleone#1{}%


% \pgfmathloop
%
% A version of the standard TeX and LaTeX
% \loop, with an additional macro \pgfmathcounter
% (which is *not* a TeX counter) which keeps
% track of the iterations.
%
\newif\ifpgfmathcontinueloop
\def\pgfmathloop#1\repeatpgfmathloop{%
	\def\pgfmathcounter{1}%
	\def\pgfmath@iterate{%
		#1\relax%
		{% Do this inside a group, just in case...
			\c@pgfmath@counta\pgfmathcounter%
			\advance\c@pgfmath@counta1\relax%
			\xdef\pgfmathloop@temp{\the\c@pgfmath@counta}%
		}%	
		\edef\pgfmathcounter{\pgfmathloop@temp}%
		\expandafter\pgfmath@iterate\fi}%
	\pgfmath@iterate\let\pgfmath@iterate\relax}
\let\repeatpgfmathloop\fi
\def\pgfmathbreakloop{\let\pgfmath@iterate\relax}%

% \pgfmath@returnone
%
% \edef \pfgmathresult to the value of #1 after the end
% of a group, which *must directly follow*.
%
% #1 - a dimension representing a number or dimension.
%
% Changed by TT: made faster and simpler since it is used
% *heavily*. #1 must be something that can be assigned to a
% dimension. 
%
\def\pgfmath@returnone#1\endgroup{%
  \pgfmath@x#1%
  \edef\pgfmath@temp{\pgfmath@tonumber{\pgfmath@x}}%
  \expandafter\endgroup\expandafter\def\expandafter\pgfmathresult\expandafter{\pgfmath@temp}%
}


% \pgfmath@returntwo
%
% Removed by TT: not used.


% \pgfmath@smuggleone
%
% Smuggle a macro outside a group.
%
% Changed by TT: Speedup by insisting, that smuggleone is directly
% followed by \endgroup
%
\def\pgfmath@smuggleone#1\endgroup{%
  \expandafter\endgroup\expandafter\def\expandafter#1\expandafter{#1}}  


==> pgfmoduledecorations.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% The following naming conventions are (more or less) observed:
%
% `decorated'  : the path that is being decorated.
% `decoration' : any path created/left by the automaton
% `decorate'   : generic use where distinction is probably unimportant
%                (e.g. internal macros).



% These should be moved.
%
\def\pgfgetpath#1{\pgfsyssoftpath@getcurrentpath{#1}}
\def\pgfsetpath#1{\pgfsyssoftpath@setcurrentpath{#1}}


% Required registers.
%
\newdimen\pgfdecoratedcompleteddistance
\newdimen\pgfdecoratedremainingdistance
\newdimen\pgfdecoratedinputsegmentcompleteddistance
\newdimen\pgfdecoratedinputsegmentremainingdistance
\newdimen\pgf@decorate@distancetomove

\newcount\pgf@decorate@repeatstate


% Extra options used in all libraries

\newdimen\pgfdecorationsegmentamplitude
\newdimen\pgfdecorationsegmentlength
\pgfdecorationsegmentamplitude2.5pt
\pgfdecorationsegmentlength10pt
\def\pgfdecorationsegmentangle{45}
\def\pgfdecorationsegmentaspect{0.5}
\def\pgfmetadecorationsegmentamplitude{2.5pt}  
\def\pgfmetadecorationsegmentlength{1cm}

\pgfkeys{%
  /pgf/decoration/.code={\pgfkeys{/pgf/decoration/.cd,#1}},
  /pgf/decoration/.cd,
  amplitude/.code={\pgfmathsetlength\pgfdecorationsegmentamplitude{#1}},
  meta-amplitude/.store in=\pgfmetadecorationsegmentamplitude,
  segment length/.code={\pgfmathsetlength\pgfdecorationsegmentlength{#1}},
  meta-segment length/.store in=\pgfmetadecorationsegmentlength,
  angle/.code={\pgfmathparse{#1}\let\pgfdecorationsegmentangle\pgfmathresult},
  aspect/.code={\pgfmathparse{#1}\let\pgfdecorationsegmentaspect\pgfmathresult},
  start radius/.initial=2.5pt,
  end radius/.initial=2.5pt,
  radius/.style={start radius=#1,end radius=#1},
  path has corners/.is if=pgfdecoratepathhascorners
} 
\newif\ifpgfdecoratepathhascorners


% Declare a decoration
%
% #1 = name of the decoration
% #2 = initial state
% #3 = states
%
% This command declares a new decoration for later use.
% Inside the code of #3 the command \state may be used. This command
% will only be defined while #3 is executed.
%
% Example:
%
% \pgfdeclaredecoration{zigzag}{q}
% {
%   \state{q}[width=10pt]
%   {
%     \pgfpathlineto{\pgfpoint{2.5pt}{2.5pt}}
%     \pgfpathlineto{\pgfpoint{7.5pt}{-2.5pt}}
%     \pgfpathlineto{\pgfpoint{10pt}{0pt}}
%   }
%   \state{final}
%   {
%     \pgfpathlineto{\pgfpointdecoratedpathlast}
%   }
% }

\long\def\pgfdeclaredecoration#1#2#3{%
  \let\pgf@mod@dec@next=\pgf@mod@dec@firstofone%
  \pgfifmetadecoration{#1}{%
    \PackageError{pgf}{You cannot declare a decoration of the same
      name as a meta-decoration}{}%
    \let\pgf@mod@dec@next=\pgfutil@gobble%
  }{}%
  \pgf@mod@dec@next
  {%
    \def\pgf@decorate@name{#1}%
    \pgfutil@namedef{pgf@decorate@@#1@initial}{#2}%
    \let\pgf@orig@state\state%
    \let\state\pgf@decorate@state
    #3%
    \let\state\pgf@orig@state%
  }%
}

\def\pgf@decorate@state#1{\pgfutil@ifnextchar[{\pgf@decorate@@start#1}{\pgf@decorate@@start#1[]}}%}
\def\pgf@decorate@@start#1[#2]#3{%
  \pgfutil@namedef{pgf@decorate@@\pgf@decorate@name @#1@options}{#2}%
  \pgfutil@namedef{pgf@decorate@@\pgf@decorate@name @#1@code}{#3}%
}
\long\def\pgf@mod@dec@firstofone#1{#1}


% Test whether something is a decoration
%
% #1 = name
% #2 = if-code
% #3 = else-code
%
% Example:
%
% \pgfifdecoration{zigzag}{Exists}{Does not exist}

\def\pgfifdecoration#1#2#3{\pgfutil@ifundefined{pgf@decorate@@#1@initial}{#3}{#2}}



% Declare a meta decoration
%
% #1 = name of the meta decoration
% #2 = initial state
% #3 = states
%
% This command declares a new meta decoration for later use.
% Inside the code of #3 the command \state may be used.

\long\def\pgfdeclaremetadecoration#1#2#3{%
  \let\pgf@mod@dec@next=\pgf@mod@dec@firstofone%
  \pgfifdecoration{#1}{%
    \PackageError{pgf}{You cannot declare a meta-decoration of the
      same name as a decoration}{}%
    \let\pgf@mod@dec@next=\pgfutil@gobble%
  }{}%
  \pgf@mod@dec@next{%
    \def\pgf@metadecoration@name{#1}%
    \pgfutil@namedef{pgf@metadecoration@@#1@initial}{#2}%
    \let\pgf@orig@state\state%
    \let\state\pgf@metadecoration@state
    #3%
    \let\state\pgf@orig@state%
  }%
}

\def\pgf@metadecoration@state#1{\pgfutil@ifnextchar[{\pgf@metadecoration@@state#1}{\pgf@metadecoration@@state#1[]}}%}
\def\pgf@metadecoration@@state#1[#2]#3{%
  \pgfutil@namedef{pgf@metadecoration@@\pgf@metadecoration@name @#1@options}{#2}%
  \pgfutil@namedef{pgf@metadecoration@@\pgf@metadecoration@name @#1@code}{#3}%
}


% Test whether something is a meta-decoration
%
% #1 = name
% #2 = if-code
% #3 = else-code
%
% Example:
%
% \pgfifmetadecoration{zigzag}{Exists}{Does not exist}

\def\pgfifmetadecoration#1#2#3{\pgfutil@ifundefined{pgf@metadecoration@@#1@initial}{#3}{#2}}





\let\pgfdecoratebeforecode\pgfutil@empty
\let\pgfdecorateaftercode\pgfutil@empty

% \pgfdecoratepath
%
% Decorate a path.
%
% \pgfdecoratebeforecode and \pgfdecorateaftercode can be used to 
% execute code before and after the decoration.
% 
% #1 - the name of the decoration.
% #2 - a (non-empty) path specification.
%
% Example:
%
%	\pgfdeclaredecoration{circles}{red circles}{
%		\state{red circles}[width=10pt, repeat state=2, next state=blue circles]
%		{
%			\pgfmathparse{round(rnd*100)}
%			\pgfsetstrokecolor{red!\pgfmathresult!brown}
%			\pgfsetfillcolor{orange!\pgfmathresult!yellow}
%			\pgfpathcircle{\pgfpointorigin}{2.5pt}
%			\pgfusepath{stroke,fill}
%		}
%		\state{blue circles}[width=10pt, repeat state=1, next state=red circles]
%		{
%			\pgfmathparse{round(rnd*100)}
%			\pgfsetstrokecolor{blue!\pgfmathresult!gray}
%			\pgfsetfillcolor{blue!\pgfmathresult!white}
%			\pgfpathcircle{\pgfpointorigin}{2.5pt}
%			\pgfusepath{stroke,fill}
%		}
%		\state{final}{}
%	}	
%	
%	\pgfpicture
%		\pgfdecoratepath{circles}
%		{
%			\pgfpathmoveto{\pgfpointorigin}
%			\pgfpathcurveto{\pgfpoint{0cm}{3cm}}{\pgfpoint{4cm}{0cm}}{\pgfpoint{4cm}{3cm}}
%		}
%	\endpgfpicture
%
\long\def\pgfdecoratepath#1#2{%
	\pgfdecoration{{#1}{\pgfdecoratedpathlength}{\pgfdecoratebeforecode}{\pgfdecorateaftercode}}%
	#2%
	\endpgfdecoration}




% \pgfdecoratecurrentpath
%
% Decorate the current/existing path, but (unavoidably) destroys it.
% 
% \pgfdecoratebeforecode and \pgfdecorateaftercode can be used to 
% execute code before and after the decoration.
%
% #1 - the name of the decoration.
%
% Example:
%
%	\pgfdeclaredecoration{stars}{move}{
%		\state{move}[width=7.5pt, next state=star]{}
%	  \state{star}[width=7.5pt, next state=move]
%	  {
%	  	\pgfmathparse{round(rnd*100)}
%	  	\pgfsetfillcolor{yellow!\pgfmathresult!orange}
%	    \pgfsetstrokecolor{yellow!\pgfmathresult!red}
%	    \pgfmathparse{rnd*.75+.25}
%	    \pgftransformscale{\pgfmathresult}
%	    \pgfnode{star}{center}{}{}{\pgfusepath{stroke,fill}}
%	  }
%	  \state{final}
%	  {
%	  	\pgfpathmoveto{\pgfpointdecoratedpathlast}
%	  }
%	}
%
%	\pgfpicture
%		\pgfpathmoveto{\pgfpointorigin}
%		\pgfpathcurveto{\pgfqpoint{0cm}{2cm}}{\pgfqpoint{3cm}{2cm}}{\pgfqpoint{3cm}{0cm}}
%		\pgfpathcurveto{\pgfqpoint{3cm}{-3cm}}{\pgfqpoint{0cm}{0cm}}{\pgfqpoint{0cm}{-3cm}}
%		\pgfpathcurveto{\pgfqpoint{0cm}{-5cm}}{\pgfqpoint{3cm}{-5cm}}{\pgfqpoint{3cm}{-3cm}}
%		\pgfdecoratecurrentpath{stars}
%	\endpgfpicture
%
\def\pgfdecoratecurrentpath#1{%
	\pgfgetpath\pgf@decorate@currentpath%
	\pgfsetpath\pgfutil@empty%
	\pgfdecoration{{#1}{\pgfdecoratedpathlength}{\pgfdecoratebeforecode}{\pgfdecorateaftercode}}%
		\pgfsetpath\pgf@decorate@currentpath%
	\endpgfdecoration}




% Environment \pgfdecoration \endpgfdecoration
%
% Decorates a path with multiple decorations.
%
% Definitions:
%
% `existing path' 
%		- any unsed path exsiting prior to the environment.
%
% `decorated path'
% 	- the path that is being decorated.
%
%	`decoration path'
%		- any unused path left by the decoration automaton.
%
% The action of the environment is as follows:
%
%	1. Any existing path is saved.
%	2. Construction commands are executed forming the decorated path.
%	3. If the first command in the decorated path is not a `move to',
%    the last known position from the exisiting path is inserted.
%	4. The saved existing path is reinstalled. 
%	5. The decoration automaton is executed along the decorated path.
%  
% Parameters:
%
% #1 - a comma separated list of decoration specifications.
% 
% A decoration specification takes the format:
%
% {<name>}{<distance>}{<before code>}{<after code>}
%
% The decoration <name> is applied to a section of the decorated
% path from the last point on the decorated path the decoration 
% automaton reached to <distance> from that point.
% 
% When <distance>} is parsed, the dimension 
% \pgfdecoratedreminingdistance holds the distance remaining on the
% entire decorated path, and the macro \pgfdecoratedpathlength holds
% the total length of the entire decorated path. 
% After <distance> is parsed, both are set to to the value of 
% <distance> for the automaton to decorate current section of the 
% decorated path.
%
% <before code> is executed just before the decoration automaton
% starts and <after code> is executed just after the automaton stops.
% If <before code> or <after code> are empty, they can be omitted.
%	The macros \pgfdecoratedpathfirst and \pgfdecoratedpathlast
% will be set up as the first and last points on the current section
% of the decorated path.
%
% When the environment exits, the following macros will be set up:
%
%	\pgfdecorateexistingpath
%	  - the existing path.
%
%	\pgfdecoratedpath
%	  - the decorated path.
%
%	\pgfdecorationpath
%	  - any unused decoration path.
%
%	\pgfpointdecoratedpathlast 
%   - the last point on the decorated path.
%
% Examples (require pgfdecorations library):
%
%	\pgfpicture
%	\pgfdecoration
%		{
%			{lineto}{\pgfdecoratedpathlength/3},
%			{zigzag}{\pgfdecoratedpathlength/3},
%			{lineto}{\pgfdecoratedpathlength/3}
%		}
%		\pgfpathmoveto{\pgfpointorigin}
%		\pgfpathcurveto{\pgfpoint{0cm}{4cm}}{\pgfpoint{5cm}{0cm}}{\pgfpoint{5cm}{4cm}}
%	\endpgfdecoration
%	\pgfusepath{stroke}
%	\endpgfpicture 
%	
%	
%	\pgfpicture
%	\pgfdecoration
%		{
%			{lineto}{\pgfdecoratedpathlength/5}{}{\pgfusepath{stroke}},
%			{zigzag}{\pgfdecoratedpathlength/5}
%				{
%					\pgfpathmoveto{\pgfpointdecoratedpathfirst}
%				}
%				{
%					\pgfsetstrokecolor{red}
%					\pgfusepath{stroke}
%				},
%			{lineto}{\pgfdecoratedpathlength/5}
%			  {
%			  	\pgfpathmoveto{\pgfpointdecoratedpathfirst}
%			  }
%			  {
%			  	\pgfsetstrokecolor{black}
%			  	\pgfusepath{stroke}
%			  },
%			{zigzag}{\pgfdecoratedpathlength/5}
%				{
%					\pgfpathmoveto{\pgfpointdecoratedpathfirst}
%				}
%				{
%					\pgfsetstrokecolor{red}
%					\pgfusepath{stroke}
%				},
%			{lineto}{\pgfdecoratedpathlength/5}
%				{
%			  	\pgfpathmoveto{\pgfpointdecoratedpathfirst}
%			  }
%			  {
%			  	\pgfsetstrokecolor{black}
%			  	\pgfusepath{stroke}
%			  }
%		}
%		\pgfpathmoveto{\pgfpointorigin}
%		\pgfpathcurveto{\pgfpoint{0cm}{4cm}}{\pgfpoint{5cm}{0cm}}{\pgfpoint{5cm}{4cm}}
%	\endpgfdecoration
%	
%	\endpgfpicture 
%	
%	
%	
%	\pgfdeclaredecoration{polygons}{move}{
%		\state{move}[width=7.5pt, next state=polygon]{}
%	  \state{polygon}[width=7.5pt, next state=move]
%	  {
%	  	\pgfmathparse{round(rnd*100)}
%	  	\pgfsetfillcolor{green!\pgfmathresult!yellow}
%	    \pgfsetstrokecolor{green!\pgfmathresult!brown}
%	    \pgfnode{regular polygon}{center}{}{}{\pgfusepath{stroke,fill}}
%	  }
%	  \state{final}
%	  {
%	  	\pgfpathmoveto{\pgfpointdecoratedpathlast}
%	  }
%	}
%	
%	\pgfpicture
%	\pgfdecoration
%		{
%			{polygons}{45pt},
%			{lineto}{30pt}
%				{\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%				{				
%					\pgfsetstrokecolor{yellow!50!orange}
%					\pgfusepath{stroke}	
%				},
%			{polygons}{45pt},
%			{lineto}{30pt}
%				{\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%				{				
%					\pgfsetstrokecolor{green!50!blue}
%					\pgfusepath{stroke}	
%				},
%			{polygons}{\pgfdecoratedremainingdistance}
%		}
%		\pgfpathmoveto{\pgfpointorigin}
%		\pgfpathcurveto{\pgfpoint{0cm}{4cm}}{\pgfpoint{5cm}{0cm}}{\pgfpoint{5cm}{4cm}}
%	\endpgfdecoration
%	\endpgfpicture
%	
%	
%	\pgfpicture
%	  \pgfpathmoveto{\pgfpointorigin}
%	  \pgfpathcurveto{\pgfpoint{0cm}{4cm}}{\pgfpoint{5cm}{0cm}}{\pgfpoint{5cm}{4cm}}
%	  \pgfgetpath\temppath
%		\pgfsetstrokecolor{red}
%	  \pgfusepath{stroke}
%	  
%	  \pgfset{decoration text={Here is some text all the way along this curve!}}
%	  \pgfdecoration{{text}{\pgfdecoratedremainingdistance}}
%	    \pgfsetpath\temppath
%	  \endpgfdecoration
%	\endpgfpicture
%
\def\pgfdecoration#1{%
  \begingroup%
    \def\pgf@decorate@decorationlist{#1}%
    \pgf@decoration@env%		
}

\def\endpgfdecoration{%
    \pgf@decoration@endenv%
    \ifx\pgfdecoratedpath\pgfutil@empty%
    \else%
      % 
      % Perform the decoration(s).
      % 
      \pgf@decorate@for\pgf@temp:=\pgf@decorate@decorationlist\do{%
        \ifx\pgf@temp\pgfutil@empty%
        \else%
          \expandafter\pgf@decorate@invoke\expandafter{\pgf@temp}%
        \fi%
      }%
    \fi%
    \pgfgetpath\pgfdecorationpath%
    % 
    % Take stuff outside the group.
    % 
    \global\let\pgf@decorate@decorationpathtemp\pgfdecorationpath%
    \global\let\pgf@decorate@decoratedpathtemp\pgfdecoratedpath%
    \global\let\pgf@decorate@existingpathtemp\pgfdecorateexistingpath%
    \global\let\pgfpoint@decorated@pathlasttemp\pgfpoint@decorated@pathlast%
  \endgroup%
  % 
  % Are we in LaTeX?
  % 
  \pgfutil@ifnextchar\@checkend{\aftergroup\pgf@decorate@installmacrosatend}%
  {\pgf@decorate@installmacrosatend}%
}


% Enviroment \pgfmetadecoration \endpgfmetadecoration
%
% Decorate a path with decoration automatons!
%
% Example:
%
%	\pgfdeclaremetadecoration{fancy line}{line to}{
%	  \state{line to}[width=1cm, next state=zigzag]
%	  {
%	    \decoration{lineto}
%	    \beforedecoration{\pgfpathmoveto{\pgfpointdecoratedpathfirst}}	
%	    \afterdecoration
%	    {
%	      \pgfsetstrokecolor{black}
%	      \pgfusepath{stroke}			
%	    }
%	  }
%	  \state{zigzag}[width=2cm, next state=line to]
%	  {
%	    \decoration{zigzag}	
%	    \beforedecoration{\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%	    \afterdecoration
%	    {
%	      \pgfsetstrokecolor{red}
%	      \pgfusepath{stroke}	
%	    }
%	  }
%	  \state{final}
%	  {
%	    \decoration{lineto}
%	    \beforedecoration{\pgfpathmoveto{\pgfpointdecoratedpathfirst}}
%	    \afterdecoration
%	    {
%	      \pgfsetstrokecolor{black}
%	      \pgfusepath{stroke}			
%	    }
%	  }
%	}
%	
%	\pgfpicture
%		\pgfmetadecoration{fancy line}
%			\pgfpathmoveto{\pgfpointorigin}
%			\pgfpathcurveto{\pgfqpoint{0cm}{2cm}}{\pgfqpoint{3cm}{2cm}}{\pgfqpoint{3cm}{0cm}}
%			\pgfpathcurveto{\pgfqpoint{3cm}{-3cm}}{\pgfqpoint{0cm}{0cm}}{\pgfqpoint{0cm}{-3cm}}
%			\pgfpathcurveto{\pgfqpoint{0cm}{-5cm}}{\pgfqpoint{3cm}{-5cm}}{\pgfqpoint{3cm}{-3cm}}
%		\endpgfmetadecoration
%	\endpgfpicture
%
\def\pgfmetadecoration#1{%
	\begingroup%
		\let\decoration\pgf@metadecoration@decoration%
		\let\beforedecoration\pgf@metadecoration@beforedecoration%
		\let\afterdecoration\pgf@metadecoration@afterdecoration%
		\def\pgf@metadecoration@name{#1}%
		\pgf@decoration@env%
}

\def\endpgfmetadecoration{%
		\pgf@decoration@endenv%
		\ifx\pgfdecoratedpath\pgfutil@empty%
		\else%
			\let\pgfmetadecoratedpathlength\pgf@decorate@totalpathlength%
			\def\pgfmetadecoratedinputsegmentremainingdistance{\pgfdecoratedremainingdistance}%
			\def\pgfmetadecoratedinputsegmentcompleteddistance{\pgfdecoratedcompleteddistance}%
    	%
			% Perform the meta decoration...
			%
			\expandafter\let\expandafter\pgf@metadecoration@current@state%
	  	\csname pgf@metadecoration@@\pgf@metadecoration@name @initial\endcsname%
	  	\pgf@metadecoration@run%
			%
			% ..until the final state.
			%
			\let\pgf@decorate@tempname\pgfutil@empty%
		  \let\pgf@decorate@tempbefore\pgfutil@empty%
		  \let\pgf@decorate@tempafter\pgfutil@empty%
  		\csname pgf@metadecoration@@\pgf@metadecoration@name @\pgf@metadecoration@current@state @code\endcsname%
  		\ifx\pgf@decorate@tempname\pgfutil@empty%
  			\def\pgf@decorate@tempname{moveto}
  		\fi%
			\pgf@decorate@invoke{%
				{\pgf@decorate@tempname}{\pgfdecoratedremainingdistance}%
				{\pgf@decorate@tempbefore}{\pgf@decorate@tempafter}%
			}%   		
		\fi%
		\pgfgetpath\pgfdecorationpath%
		%
	  % Take stuff outside the group.
	  %
	 	\global\let\pgf@decorate@decorationpathtemp\pgfdecorationpath%
	  \global\let\pgf@decorate@decoratedpathtemp\pgfdecoratedpath%
	  \global\let\pgf@decorate@existingpathtemp\pgfdecorateexistingpath%
	  \global\let\pgfpoint@decorated@pathlasttemp\pgfpoint@decorated@pathlast%
	\endgroup%
	%
	% Are we in LaTeX?
	% 
	\pgfutil@ifnextchar\@checkend{\aftergroup\pgf@decorate@installmacrosatend}%
		{\pgf@decorate@installmacrosatend}%
}






% Internal macro for the decoration enironment.
%
\def\pgf@decoration@env{%
  \pgfgetpath\pgfdecorateexistingpath%
  \pgfsetpath\pgfutil@empty%
  \let\pgfdecorationpath\pgfutil@empty%
  \let\pgfdecoratedpath\pgfutil@empty%
  \let\pgfpoint@decorated@pathlast\pgfpointorigin%
  \edef\pgfpoint@decorate@existingpathlast{\pgf@x\the\pgf@path@lastx\pgf@y\the\pgf@path@lasty}%			
  % 
  % Begin a group so transformations don't mess things up.
  % 
  \bgroup%	
}

\def\pgf@decoration@endenv{%
  \egroup%        
  \pgftransformreset%
  % 
  % Save the existing soft path and restore the existing path.
  % 
  \pgfgetpath\pgfdecoratedpath%
  \pgfsetpath\pgfdecorateexistingpath%
  % 
  \ifx\pgfdecoratedpath\pgfutil@empty%
    \PackageError{PGF}{I cannot decorate an empty path}{}%
  \else%
    %   
    % Remove special round tokens and get points.
    % 
    \pgfprocessround{\pgfdecoratedpath}{\pgfdecoratedpath}%
    % 
    % Parse the soft path into a series of decorated input segment objects.
    % 
    \pgf@decorate@parsesoftpath{\pgfdecoratedpath}{\pgf@decorate@inputsegmentobjects}%
    % 
    \let\pgf@decorated@remainingdistance\pgf@decorate@totalpathlength%
    % 
    \let\pgfpoint@decorated@totalpathfirst\pgfpoint@decorated@firstparsed%
    \let\pgfpoint@decorated@totalpathlast\pgfpoint@decorate@lastnonmovetoparsed%
    % 
    \let\pgfpoint@decorated@pathfirst\pgfpoint@decorated@totalpathfirst
    \let\pgfpoint@decorated@pathlast\pgfpoint@decorated@totalpathlast%
    % 
    % Set up the first input segment.
    % 
    \let\pgf@decorate@currentinputsegmentobjects\pgf@decorate@inputsegmentobjects%
    \let\pgf@decorate@transformtoinputsegment\pgfutil@empty%
    \pgf@decorate@getnextinputsegmentobject\pgf@decorate@nextinputsegmentobject%
    \pgf@decorate@processnextinputsegmentobject%
    \pgf@decorate@distancetomove0pt\relax%
    %
    % Setup further options
    %
    \pgfkeys{/pgf/every decoration/.try}%
  \fi%
}%		





\def\pgf@decorate@installmacrosatend{%
	\let\pgfdecorationpath\pgf@decorate@decorationpathtemp%
  \let\pgfdecoratedpath\pgf@decorate@decoratedpathtemp%
  \let\pgfdecorateexistingpath\pgf@decorate@existingpathtemp%
  \let\pgfpoint@decorated@pathlast\pgfpoint@decorated@pathlasttemp%
}

\let\pgfdecorationpath\pgfutil@empty
\let\pgfdecoratedpath\pgfutil@empty
\let\pgfdecorateexisitingpath\pgfutil@empty

\let\pgfpoint@decorated@pathlast\pgfpointorigin



% A version of \pgfutil@for which doesn't expand each value in #3.
%
\def\pgf@decorate@for#1:=#2\do#3{%
	\def\pgf@decorate@for@var{#1}%
	\def\pgf@decorate@for@action{#3}%
	\expandafter\pgf@decorate@@for#2,\pgf@stop,}
	
\def\pgf@decorate@@for#1,{%
	\ifx#1\pgf@stop%
		\expandafter\let\pgf@decorate@for@var\pgfutil@empty%
	\else%
		\expandafter\def\pgf@decorate@for@var{#1}%
		\pgf@decorate@for@action%
		\expandafter\pgf@decorate@@for%
	\fi%
}


% Invoke a decoration.
%
% #1 - {<name>}{<distance>}{<before code>}{<after code>}
%
\def\pgf@decorate@invoke#1{%
	\pgf@decorate@@invoke#1\pgf@decorate@invoke\pgf@decorate@invoke\pgf@decorate@invoke\pgf@stop}
	
\def\pgf@decorate@@invoke#1#2#3#4#5\pgf@stop{%
	\pgfutil@ifundefined{pgf@decorate@@#1@initial}%
	{%
		\PackageError{PGF}{Unknown decoration `#1'}{}%
	}%
	{%
		\def\pgf@decorate@name{#1}%
		\ifx\pgf@decorate@invoke#3%
			\let\pgf@decorate@beforecode\pgfutil@empty%
		\else%
			\def\pgf@decorate@beforecode{#3}%
		\fi%
		\ifx\pgf@decorate@invoke#4%
			\let\pgf@decorate@aftercode\pgfutil@empty%
		\else%
			\def\pgf@decorate@aftercode{#4}%
		\fi%
		%
		% Make remaining distance and the decorated path length `public'.
		%
		\pgfdecoratedremainingdistance\pgf@decorated@remainingdistance\relax%
		\let\pgfdecoratedpathlength\pgf@decorate@totalpathlength%
		%
		\pgfmathsetlength\pgf@xa{#2}%
		\ifdim\pgf@xa>\pgf@decorated@remainingdistance\relax%
			\pgf@xa\pgf@decorated@remainingdistance\relax%
		\fi%
		\edef\pgf@decorate@currentpathlength{\the\pgf@xa}%
		%
		% Calculate the distance remaining to the end of the entire path.
		%
		\pgf@xa-\pgf@decorate@currentpathlength\relax%
		\advance\pgf@xa\pgf@decorated@remainingdistance\relax%
		\edef\pgf@decorated@remainingdistance{\the\pgf@xa}%
		%
		% Set up the macros and distances for the current section
		% of the decorated path.
		%
		\let\pgfdecoratedpathlength\pgf@decorate@currentpathlength%
		\pgfdecoratedremainingdistance\pgfdecoratedpathlength\relax%
		\pgfdecoratedcompleteddistance0pt\relax%
		%
		% Execute user-defined code beore decoration.
		%
		\pgf@decorate@beforecode%
		%
		% Run the decoration...
		%
	  \expandafter\let\expandafter\pgf@decorate@current@state%
	  	\csname pgf@decorate@@\pgf@decorate@name @initial\endcsname%
	  \pgf@decorate@run%
	  %
	  % ...until the final state.
	  %
	  \ifdim\pgf@decorated@remainingdistance<1pt\relax% Should be =0pt, but need to control for inaccuracies.
	  	\let\pgfpoint@decorated@pathlast\pgfpoint@decorated@totalpathlast%
	  \else%
	  	%
	  	% Set up \pgfpoint@decorated@pathlast if the end of
	  	% the total decorated path has not been reached.
	  	%
		  {%
		  	\pgf@decorate@movealonginputsegment{\the\pgfdecoratedremainingdistance}%
		  	\pgf@decorate@transformtoinputsegment%
		  	\pgfpointorigin%
		  	\pgf@pos@transform{\pgf@x}{\pgf@y}%
		  	\global\pgf@x\pgf@x%
		  	\global\pgf@y\pgf@y%
		  }%
		  \edef\pgfpoint@decorated@pathlast{\pgf@x\the\pgf@x\pgf@y\the\pgf@y}%
		\fi%  	
	  {%
	  	\pgftransformreset%
	  	\pgf@decorate@transformtoinputsegment%
	    \pgf@decorate@additionaltransform%
	    \csname pgf@decorate@@\pgf@decorate@name @final@code\endcsname%
	  }%
	  \pgf@decorate@movealonginputsegment{\the\pgfdecoratedremainingdistance}%
	  %
	  % Execute user-defined code after decoration.
	  %
	  \pgf@decorate@aftercode%	
	  %
	  % Update the input segment objects.
	  %
	  \let\pgf@decorate@additionaltransform\pgfutil@empty%
	  \let\pgf@decorate@inputsegmentobjects\pgf@decorate@inputsegmentobjects@aftersplit%
	  \let\pgfpoint@decorated@pathfirst\pgfpoint@decorated@pathlast%
	 }%
}



\let\pgf@decorate@transformtoinputsegment\pgfutil@empty%
\let\pgf@decorate@additionaltransform\pgfutil@empty%


% \pgfpointdecoratedpathfirst
%
\def\pgfpointdecoratedpathfirst{%
	{%
		\pgftransforminvert%
		\pgfpoint@decorated@pathfirst%
		\pgf@pos@transform{\pgf@x}{\pgf@y}%
		\global\pgf@x\pgf@x%
		\global\pgf@y\pgf@y%
	}%
}%

% \pgfpointdecoratedpathlast
%
\def\pgfpointdecoratedpathlast{%
	{%
		\pgftransforminvert%
		\pgfpoint@decorated@pathlast%
		\pgf@pos@transform{\pgf@x}{\pgf@y}%
		\global\pgf@x\pgf@x%
		\global\pgf@y\pgf@y%
	}%
}%

% \pgfpointdecoratedinputsegmentfirst
%
% The first point of the current sub-path. 
%
\def\pgfpointdecoratedinputsegmentfirst{%
	{%
		\pgftransforminvert%
		\pgf@decorate@inputsegment@first%
		\pgf@pos@transform{\pgf@x}{\pgf@y}%
		\global\pgf@x\pgf@x%
		\global\pgf@y\pgf@y%
	}%
}%	

% \pgfpointdecoratedinputsegmentlast
%
% The final point of the current sub-path. 
%
\def\pgfpointdecoratedinputsegmentlast{%
	{%
		\pgftransforminvert%
		\pgf@decorate@inputsegment@last%
		\pgf@pos@transform{\pgf@x}{\pgf@y}%
		\global\pgf@x\pgf@x%
		\global\pgf@y\pgf@y%
	}%
}%


\def\pgf@final@text{final}

% Run a normal decoration.
%
\def\pgf@decorate@run{%
	\let\pgf@decorate@next\pgf@decorate@do@state%
  \ifx\pgf@decorate@current@state\pgf@final@text%
    \let\pgf@decorate@next\relax%
  \fi%
  \pgf@decorate@next%  
}

\def\pgf@decorate@do@state{%
  \let\pgf@decorate@next\relax%
  \let\pgf@decorate@next@state\pgf@decorate@current@state%
  %
  % Get the options.
  %
  \let\pgf@decorate@persistent@pre=\relax%
  \let\pgf@decorate@persistent@post=\relax%
  \expandafter\expandafter\expandafter\pgf@decorate@setter
  \expandafter\expandafter\expandafter{\csname pgf@decorate@@\pgf@decorate@name @\pgf@decorate@current@state @options\endcsname}%
  \ifx\pgf@decorate@next\relax%
    \let\pgf@decorate@next\pgf@decorate@do@code%
  \fi%
  \pgf@decorate@next%
}

\def\pgf@decorate@setter{\pgfqkeys{/pgf/decoration automaton}}

\pgf@decorate@repeatstate-1\relax

\def\pgf@decorate@do@code{%
  %
  % Execute code.
  %
  \pgf@decorate@persistent@pre%
  {%
    \pgftransformreset%
    \pgf@decorate@transformtoinputsegment%
    \pgf@decorate@additionaltransform%
    \csname pgf@decorate@@\pgf@decorate@name @\pgf@decorate@current@state @code\endcsname%
  }%
  \pgf@decorate@persistent@post%
  \pgf@decorate@movealongpath{\pgf@decorate@width}%
  %
  % Next iteration.
  %
  \ifnum\pgf@decorate@repeatstate>0\relax%
  	\advance\pgf@decorate@repeatstate-1\relax%
  \else%
  	\pgf@decorate@repeatstate-1\relax%
  	\let\pgf@decorate@current@state\pgf@decorate@next@state%
  \fi%
  \pgf@decorate@run%
}

\pgfkeys{
  /pgf/decoration automaton/width/.code=\def\pgf@decorate@width{#1}\pgf@decorate@switch@if#1 to final\pgf@stop,%
  /pgf/decoration automaton/switch if less than/.code=\pgf@decorate@switch@if#1\pgf@stop,%
  /pgf/decoration automaton/switch if input segment less than/.code=\pgf@decorate@switch@ifinputsegment#1\pgf@stop,%
  /pgf/decoration automaton/next state/.store in=\pgf@decorate@next@state,%
  /pgf/decoration automaton/persistent precomputation/.store in=\pgf@decorate@persistent@pre,%
  /pgf/decoration automaton/persistent postcomputation/.store in=\pgf@decorate@persistent@post,%
  /pgf/decoration automaton/repeat state/.code={%
    \ifnum\pgf@decorate@repeatstate=-1\relax%
      \pgfmathsetcount\pgf@decorate@repeatstate{#1}%
    \fi%
  },%
  /pgf/decoration automaton/if input segment is closepath/.code={%
    \ifpgf@decorate@is@closepath@%
      \pgfkeysalso{#1}%
    \fi%
  },
  /pgf/decoration automaton/auto end on length/.code=\pgf@decorate@auto@end{#1},
  /pgf/decoration automaton/auto corner on length/.code=\pgf@decorate@auto@corner{#1},
}

\def\pgf@decorate@auto@end#1{%
  \ifx\pgf@decorate@next\relax%
    \pgfmathsetlength\pgf@x{#1}%
    \ifpgf@decorate@is@closepath@%
      \ifdim\pgfdecoratedremainingdistance>\pgf@x%
        \ifdim\pgfdecoratedinputsegmentremainingdistance>\pgf@x%
        \else%
          \pgfpathclose%
          \pgf@decorate@movealongpath{\pgfdecoratedinputsegmentremainingdistance}%
          \pgf@decorate@repeatstate-1\relax%
          \let\pgf@decorate@next\pgf@decorate@run%
        \fi%
      \else%
        \pgfpathclose%
        \def\pgf@decorate@current@state{final}%
        \def\pgf@decorate@width{\pgfdecoratedremainingdistance}
        \pgf@decorate@repeatstate-1\relax%
        \let\pgf@decorate@next\pgf@decorate@run%
      \fi%
    \else%
      \ifdim\pgfdecoratedremainingdistance>\pgf@x%
      \else%
        {%
          \pgftransformreset%
          \pgf@decorate@transformtoinputsegment%
          \pgf@decorate@additionaltransform%
          \pgfpathlineto{\pgfpoint{\pgfdecoratedremainingdistance}{0pt}}
        }%
        \def\pgf@decorate@current@state{final}%
        \def\pgf@decorate@width{\pgfdecoratedremainingdistance}
        \pgf@decorate@repeatstate-1\relax%
        \let\pgf@decorate@next\pgf@decorate@run%
      \fi%
    \fi%
  \fi%
}

\def\pgf@decorate@auto@corner#1{%
  \ifpgfdecoratepathhascorners%
    \ifx\pgf@decorate@next\relax%
      \pgfmathsetlength\pgf@x{#1}%
      \ifdim\pgfdecoratedinputsegmentremainingdistance>\pgf@x%
      \else%
        {%
          \pgftransformreset%
          \pgf@decorate@transformtoinputsegment%
          \pgf@decorate@additionaltransform%
          \pgfpathlineto{\pgfqpoint{\pgfdecoratedinputsegmentremainingdistance}{0pt}}
        }%
        \pgf@decorate@movealongpath{\pgfdecoratedinputsegmentremainingdistance}%
        \pgf@decorate@repeatstate-1\relax%
        \let\pgf@decorate@next\pgf@decorate@run%
      \fi%
    \fi%
  \fi%
}

\def\pgf@decorate@switch@if#1to #2\pgf@stop{%
  \ifx\pgf@decorate@next\relax%
    \ifdim\pgfdecoratedremainingdistance=0pt\relax%
      \def\pgf@decorate@current@state{#2}%
      \pgf@decorate@repeatstate-1\relax%
      \let\pgf@decorate@next\pgf@decorate@run%
    \else%
      \pgfmathsetlength\pgf@x{#1}%
      \ifdim\pgfdecoratedremainingdistance<\pgf@x%
        \def\pgf@decorate@current@state{#2}%
        \pgf@decorate@repeatstate-1\relax%
        \let\pgf@decorate@next\pgf@decorate@run%
      \fi%
    \fi%
  \fi%
}

\def\pgf@decorate@switch@ifinputsegment#1to #2\pgf@stop{%
  \ifx\pgf@decorate@next\relax%
    \pgfmathsetlength\pgf@x{#1}%
    \ifdim\pgfdecoratedinputsegmentremainingdistance<\pgf@x%
      \def\pgf@decorate@current@state{#2}%
      \pgf@decorate@repeatstate-1\relax%
      \let\pgf@decorate@next\pgf@decorate@run%
    \fi%
  \fi%
}




% \pgfsetdecorationsegmenttransformation
%
% Set the additional transform for each decoration state.
%
% Example:
%
% \pgfsetdecorationsegmenttransformation{\pgftransformyshift{5pt}}
%
\def\pgfsetdecorationsegmenttransformation#1{\def\pgf@decorate@additionaltransform{#1}}
\let\pgf@decorate@additionaltransform\pgfutil@empty%




\def\pgf@metadecoration@decoration#1{%
	\edef\pgf@decorate@tempname{#1}%
}
\def\pgf@metadecoration@beforedecoration#1{%
	\def\pgf@decorate@tempbefore{#1}%
}
\def\pgf@metadecoration@afterdecoration#1{%
	\def\pgf@decorate@tempafter{#1}%
}


\def\pgf@final@text{final}

% Run a meta decoration.
%
\def\pgf@metadecoration@run{%
	\let\pgf@metadecoration@next\pgf@metadecoration@do@state%
  \ifx\pgf@metadecoration@current@state\pgf@final@text%
    \let\pgf@metadecoration@next\relax%
  \fi%
  \pgf@metadecoration@next%  
}

\def\pgf@metadecoration@do@state{%
	\let\pgf@metadecoration@next\relax%
  \let\pgf@metadecoration@next@state\pgf@metadecoration@current@state%
  %
  % Set up some macros.
  %
  \let\pgfmetadecoratedremainingdistance\pgf@decorated@remainingdistance%
  \pgf@x-\pgfmetadecoratedremainingdistance\relax%
  \advance\pgf@x\pgf@decorate@totalpathlength\relax%
  \edef\pgfmetadecoratedcompleteddistance{\the\pgf@x}%
  %
  % Get the options.
  %
  \expandafter\expandafter\expandafter\pgf@metadecoration@setter
  \expandafter\expandafter\expandafter{\csname pgf@metadecoration@@\pgf@metadecoration@name @\pgf@metadecoration@current@state @options\endcsname}%
  \ifx\pgf@metadecoration@next\relax%
    \let\pgf@metadecoration@next\pgf@metadecoration@do@code%
  \fi%
  \pgf@metadecoration@next%
}

\def\pgf@metadecoration@do@code{%
	%
  % Execute code.
  %
  \let\pgf@decorate@tempname\pgfutil@empty%
  \let\pgf@decorate@tempbefore\pgfutil@empty%
  \let\pgf@decorate@tempafter\pgfutil@empty%
  \let\pgfpointmetadecoratedpathfirst\pgfpointdecoratedpathfirst%
  \let\pgfpointmetadecoratedpathlast\pgfpointdecoratedpathlast%
  \csname pgf@metadecoration@@\pgf@metadecoration@name @\pgf@metadecoration@current@state @code\endcsname%
  \ifx\pgf@decorate@tempname\pgfutil@empty%
		\def\pgf@decorate@tempname{moveto}
	\fi%
  \pgf@decorate@invoke{%
  	{\pgf@decorate@tempname}{\pgf@metadecoration@width}%
  	{\pgf@decorate@tempbefore}{\pgf@decorate@tempafter}%
  }%
  %
  % Next iteration.
  %
  \let\pgf@metadecoration@current@state\pgf@metadecoration@next@state%
  \pgf@metadecoration@run%
}

\def\pgf@metadecoration@setter{\pgfqkeys{/pgf/meta-decoration automaton}}

\pgfkeys{
  /pgf/meta-decoration automaton/width/.code=\def\pgf@metadecoration@width{#1}\pgf@metadecoration@switch@if#1 to final\pgf@stop,%
  /pgf/meta-decoration automaton/switch if less than/.code=\pgf@metadecoration@switch@if#1\pgf@stop,%
  /pgf/meta-decoration automaton/switch if input segment less than/.code=\pgf@metadecoration@switch@ifinputsegment#1\pgf@stop,%
  /pgf/meta-decoration automaton/next state/.store in=\pgf@metadecoration@next@state,%
}

\def\pgf@metadecoration@switch@if#1to #2\pgf@stop{%
  \ifx\pgf@metadecoration@next\relax%
  	\pgfmathsetlength\pgf@x{#1}%
    \ifdim\pgf@decorated@remainingdistance<\pgf@x%
      \def\pgf@metadecoration@current@state{#2}%
      \let\pgf@metadecoration@next\pgf@metadecoration@run%
    \fi%
  \fi%
}

\def\pgf@metadecoration@switch@ifinputsegment#1to #2\pgf@stop{%
  \ifx\pgf@metadecoration@next\relax%
  	\pgfmathsetlength\pgf@x{#1}%
    \ifdim\pgfdecoratedinputsegmentremainingdistance<\pgf@x%
      \def\pgf@metadecoration@current@state{#2}%
      \let\pgf@metadecoration@next\pgf@metadecoration@run%
    \fi%
  \fi%
}



% Move along the path by a specified distance.
%
\def\pgf@decorate@movealongpath#1{%
	\pgfmathsetlength\pgf@decorate@distancetomove{#1}%
	\advance\pgfdecoratedcompleteddistance\pgf@decorate@distancetomove%
	\advance\pgfdecoratedremainingdistance-\pgf@decorate@distancetomove%
	\pgf@decorate@@movealongpath%
}
\def\pgf@decorate@@movealongpath{%
  \advance\pgfdecoratedinputsegmentcompleteddistance\pgf@decorate@distancetomove%
  \advance\pgfdecoratedinputsegmentremainingdistance-\pgf@decorate@distancetomove%
  \ifdim\pgfdecoratedinputsegmentremainingdistance>0pt\relax%
    \let\pgf@next\pgf@decorate@@@movealongpath%
  \else%
    \pgf@decorate@distancetomove-\pgfdecoratedinputsegmentremainingdistance%
    \pgf@decorate@processnextinputsegmentobject%
    \ifx\pgf@decorate@currentinputsegmentobjects\pgfutil@empty%
      \pgfdecoratedremainingdistance0pt\relax%
      \let\pgf@next\relax%
    \else%
      \let\pgf@next\pgf@decorate@@movealongpath%
    \fi%
  \fi%
  \pgf@next%
}

\def\pgf@decorate@@@movealongpath{%
	%
	% Move along input segment for real.
	%
	\pgf@decorate@movealonginputsegment{\the\pgf@decorate@distancetomove}%
	\pgf@decorate@distancetomove0pt\relax%
	%
	% Grrr. Hacking to control some inaccuracies.
	%
	\ifdim\pgf@decorate@inputsegmenttime pt>1pt\relax%
		\let\pgf@decorate@inputsegmenttimetemp\pgf@decorate@inputsegmenttime%
		\pgf@decorate@processnextinputsegmentobject%
		\pgf@x\pgf@decorate@inputsegmenttimetemp pt\relax%
		\advance\pgf@x-1pt\relax%
		\edef\pgf@decorate@inputsegmenttime{\pgfmath@tonumber{\pgf@x}}%
		\ifx\pgf@decorate@currentinputsegmentobjects\pgfutil@empty%
			\pgfdecoratedremainingdistance0pt\relax%
		\fi%
	\fi%
}

% Return the next input segment object in a macro 
%
\def\pgf@decorate@getnextinputsegmentobject#1{%
	\ifx\pgf@decorate@currentinputsegmentobjects\pgfutil@empty%
		\let\pgf@next\relax%
	\else%
		\def\pgf@decorate@temp{#1}%
		\let\pgf@next\pgf@decorate@@getnextinputsegmentobject%
	\fi%
	\pgf@next%
}
\def\pgf@decorate@@getnextinputsegmentobject{%
	\expandafter\pgf@decorate@@@getnextinputsegmentobject\pgf@decorate@currentinputsegmentobjects\pgf@stop}
\def\pgf@decorate@@@getnextinputsegmentobject#1#2\pgf@stop{%
	\expandafter\def\pgf@decorate@temp{#1}%
	\def\pgf@decorate@currentinputsegmentobjects{#2}}

% Process the next input segment object.
%
\def\pgf@decorate@processnextinputsegmentobject{%
	%
	\let\pgf@decorate@currentinputsegmentobject\pgf@decorate@nextinputsegmentobject%
	\pgf@decorate@getnextinputsegmentobject\pgf@decorate@nextinputsegmentobject%
	% 
	% If the current input segment object is a moveto, execute the 
	% object macro and get the next input segment object.
	%
	\expandafter\pgfutil@in@\expandafter\pgf@decorate@inputsegmentobject@moveto%
		\expandafter{\pgf@decorate@currentinputsegmentobject}%
	\ifpgfutil@in@%
		\pgf@decorate@currentinputsegmentobject%
		\let\pgf@decorate@currentinputsegmentobject\pgf@decorate@nextinputsegmentobject%
		\pgf@decorate@getnextinputsegmentobject\pgf@decorate@nextinputsegmentobject%
		\relax%
	\fi%
	%
        \pgf@decorate@is@closepath@false%
	\pgf@decorate@currentinputsegmentobject%
	%
	% Teensy hack in case a path goes nowhere.
	%
	\ifdim\pgfdecoratedinputsegmentlength=0pt\relax%
		\def\pgfdecoratedinputsegmentlength{0.05pt}% Arbitrary choice >0pt.
	\fi%
	\pgfdecoratedinputsegmentremainingdistance\pgfdecoratedinputsegmentlength\relax%
	\pgfdecoratedinputsegmentcompleteddistance0pt\relax%
	\def\pgf@decorate@inputsegmenttime{0}%
	\pgfmathanglebetweenpoints{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
	\let\pgfdecoratedangle\pgfmathresult%	
}


%
% Input segment objects
%

\newif\ifpgf@decorate@is@closepath@%


% Input segment object moveto.
%
\def\pgf@decorate@inputsegmentobject@moveto#1{%
	\pgfpathmoveto{#1}%
	\def\pgf@decorate@inputsegment@first{#1}%
	\def\pgf@decorate@inputsegment@supporta{#1}%
	\def\pgf@decorate@inputsegment@supportb{#1}%
	\def\pgf@decorate@inputsegment@last{#1}%
	\edef\pgf@decorate@lastmoveto{#1}%
	\def\pgfdecoratedinputsegmentlength{0pt}%
	\let\pgf@decorate@splitinputsegmentobject\pgf@decorate@splitinputsegmentobject@move%
}

% Input segment object lineto.
%
\def\pgf@decorate@inputsegmentobject@lineto#1#2#3{%
	\def\pgfdecoratedinputsegmentlength{#1}%
	\def\pgf@decorate@inputsegment@first{#2}%
	%
	% OK, lines don't need supports, but this means angle calculations 
	% do not have to be done individually for each object.
	%
	\def\pgf@decorate@inputsegment@supporta{#3}%
	\def\pgf@decorate@inputsegment@supportb{#2}%
	\def\pgf@decorate@inputsegment@last{#3}%	
	%
	\let\pgf@decorate@movealonginputsegment\pgf@decorate@movealonginputsegment@line%
	\let\pgf@decorate@transformtoinputsegment\pgf@decorate@transformtoinputsegment@line%
	\let\pgf@decorate@splitinputsegmentobject\pgf@decorate@splitinputsegmentobject@line%
}

% Input segment object curveto.
%
\def\pgf@decorate@inputsegmentobject@curveto#1#2#3#4#5{%
	\def\pgfdecoratedinputsegmentlength{#1}%
	\def\pgf@decorate@inputsegment@first{#2}%
	\def\pgf@decorate@inputsegment@supporta{#3}%
	\def\pgf@decorate@inputsegment@supportb{#4}%
	\def\pgf@decorate@inputsegment@last{#5}%	
	%
	\let\pgf@decorate@movealonginputsegment\pgf@decorate@movealonginputsegment@curve%
	\let\pgf@decorate@transformtoinputsegment\pgf@decorate@transformtoinputsegment@curve%
	\let\pgf@decorate@splitinputsegmentobject\pgf@decorate@splitinputsegmentobject@curve%
}

% Input segment object closepath.
%
% Treated like a lineto, but flag that it is a closepath.
%
\def\pgf@decorate@inputsegmentobject@closepath#1#2#3{%
  \pgf@decorate@is@closepath@true%
  %
  \def\pgfdecoratedinputsegmentlength{#1}%
  \def\pgf@decorate@inputsegment@first{#2}%
  \def\pgf@decorate@inputsegment@supporta{#3}%
  \def\pgf@decorate@inputsegment@supportb{#2}%
  \def\pgf@decorate@inputsegment@last{#3}%	
  % 
  \let\pgf@decorate@movealonginputsegment\pgf@decorate@movealonginputsegment@line%
  \let\pgf@decorate@transformtoinputsegment\pgf@decorate@transformtoinputsegment@line%
  \let\pgf@decorate@splitinputsegmentobject\pgf@decorate@splitinputsegmentobject@line%
}

% Input segment object endofinputsegments.
%
\def\pgf@decorate@inputsegmentobject@endofinputsegments{}




% This macro controls how the automaton moves along a line sub-path
%
\def\pgf@decorate@movealonginputsegment@line#1{}% Nothing special needed.

% This macro controls how the automaton moves along a curve sub-path.
%
\def\pgf@decorate@movealonginputsegment@curve#1{%
	\ifdim#1=0pt\relax%
	\else%
		\pgfpointcurveattime{\pgf@decorate@inputsegmenttime}%
			{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
			{\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
		\pgf@xa\pgf@x%
		\pgf@ya\pgf@y%
		\pgf@xb\pgf@decorate@inputsegmenttime pt\relax%
		%
		% Reduce the initial time step, depending on the length 
		% of the path. To do: Optimise this step (should also depend on #1).
		%
		\ifdim\pgf@decorate@currentpathlength<128pt\relax%
			\pgf@yb.03125pt\relax%
		\else%
			\ifdim\pgf@decorate@currentpathlength<512pt\relax%
				\pgf@yb.015625pt\relax%
			\else%
				\ifdim\pgf@decorate@currentpathlength<2048pt\relax%
					\pgf@yb.00390625pt\relax%
				\else%
					\pgf@yb.0009765625pt\relax%
				\fi%
			\fi%
		\fi%
		\c@pgf@counta1\relax%
		\pgfutil@tempdima0pt\relax%
		\pgfmathloop%
			\advance\pgf@xb\c@pgf@counta\pgf@yb%
			%
			% We would like to use \pgfpointcurveattime. However, we must not
			% overuse \pgf@process or \pgfmath stuff within this loop,
			% otherwise we increase the chances of save stack overflow. 
			%
			\edef\pgf@decorate@temp{%
				\pgf@xa\the\pgf@xa%
				\pgf@xb\the\pgf@xb%
				\pgf@ya\the\pgf@ya%
				\pgf@yb\the\pgf@yb%
			}%	
			%
			\pgfpoint@decorate@curveattime{\pgfmath@tonumber{\pgf@xb}}%
				{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
				{\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
			%
			\pgf@decorate@temp%
			%
			\pgf@xc\pgf@xa%
			\pgf@yc\pgf@ya%
			\pgf@xa\pgf@x%
			\pgf@ya\pgf@y%
			\advance\pgf@x-\pgf@xc%
			\advance\pgf@y-\pgf@yc%
			\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
			\pgfutil@tempdimb\pgfmathresult pt\relax%
			\advance\pgfutil@tempdima\c@pgf@counta\pgfutil@tempdimb%
			\ifnum\c@pgf@counta>0\relax%
				\ifdim\pgfutil@tempdima>#1\relax%
					\c@pgf@counta-\c@pgf@counta%
					\pgf@yb.5\pgf@yb%
				\fi%
			\else%
				\ifdim\pgfutil@tempdima<#1\relax%
					\c@pgf@counta-\c@pgf@counta%
					\pgf@yb.5\pgf@yb%
				\fi%
			\fi%
			\ifdim\pgf@yb=0pt\relax% *Should* be OK.
			\else%
		\repeatpgfmathloop%
		\edef\pgf@decorate@inputsegmenttime{\pgfmath@tonumber{\pgf@xb}}%
		%
		% Now calculate the angle at the new time on the curve.
		%
		% We can use \pgfpointcurveattime safely here.
		%
		\pgfpointcurveattime{\pgf@decorate@inputsegmenttime}%
			{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
			{\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
		\edef\pgf@marshal{%
			\noexpand\pgfmathanglebetweenpoints%
				{\pgf@x\the\pgf@xb\pgf@y\pgf@yb}%
				{\pgf@x\the\pgf@xa\pgf@y\pgf@ya}%
		}%
		\pgf@marshal%
		\let\pgfdecoratedangle\pgfmathresult%
	\fi%
}

% \pgfpoint@decorate@curveattime
%
% A `quick' version of \pgfpointcurveattime
%
% No parsing and no use of \pgf@process. 
% This prevents save stack build up when used inside a loop.
%
\def\pgfpoint@decorate@curveattime#1#2#3#4#5{%
  \edef\pgf@time@s{#1}%
  \pgf@x-\pgf@time@s pt\relax%
  \advance\pgf@x1pt\relax%
  \edef\pgf@time@t{\pgf@sys@tonumber{\pgf@x}}%
  #5\relax%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  #4\relax%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  #3\relax%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  #2\relax%
  % First iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  \pgf@xb=\pgf@time@t\pgf@xb\advance\pgf@xb by\pgf@time@s\pgf@xc%
  \pgf@yb=\pgf@time@t\pgf@yb\advance\pgf@yb by\pgf@time@s\pgf@yc%
  % Second iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
  \pgf@xa=\pgf@time@t\pgf@xa\advance\pgf@xa by\pgf@time@s\pgf@xb%
  \pgf@ya=\pgf@time@t\pgf@ya\advance\pgf@ya by\pgf@time@s\pgf@yb%
  % Save x/y
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  % Third iteration:
  \pgf@x=\pgf@time@t\pgf@x\advance\pgf@x by\pgf@time@s\pgf@xa%
  \pgf@y=\pgf@time@t\pgf@y\advance\pgf@y by\pgf@time@s\pgf@ya%
}


% Applies the necessary transform for a line sub-path.
%
\def\pgf@decorate@transformtoinputsegment@line{%
	\pgftransformshift{%
		\pgfpointadd{\pgf@decorate@inputsegment@first}%
			{\pgfpointpolar{\pgfdecoratedangle}{\pgfdecoratedinputsegmentcompleteddistance}}%
	}%
	\pgftransformrotate{\pgfdecoratedangle}%
}

% Applies the necessary transform for a curve sub-path.
%
\def\pgf@decorate@transformtoinputsegment@curve{%
	\pgfslopedattimetrue%
	\pgfallowupsidedownattimetrue%
	\pgftransformcurveattime{\pgf@decorate@inputsegmenttime}%
		{\pgf@decorate@inputsegment@first}{\pgf@decorate@inputsegment@supporta}%
		{\pgf@decorate@inputsegment@supportb}{\pgf@decorate@inputsegment@last}%
}





%	\pgf@decorate@parsesoftpath
%	
%	Parses an instance of a soft path into intermediate line and curve
%	sub-path objects which the decoration automaton can use to traverse 
% the decorated path. 
%	
%	The soft path should be well formed and only contain `primative' 
%	soft path tokens, that is: moveto, lineto, curvetosupporta, 
%	curvetosupportb, curveto, rectcorner, rectsize, and closepath.
%	(i.e., all specialround tokens should have removed using 
%	\pgfprocessround)
%	
%	The overall length of the path is also calculated and returned
%	in the macro \pgfdecoratedpathlength. 
%	
%	Parameters:
%	
%	#1 - a macro containing a well formed soft path.
%	#2 - a macro to store the intermediate sub-path representations.
%
%	Example:
%	
%	\pgfpathmoveto{\pgfpointorigin}
%	\pgfpathlineto{\pgfpoint{0pt}{12pt}}
%	\pgfpathlineto{\pgfpoint{12pt}{0pt}}
%	\pgfgetpath\softpath
%	
%	\pgf@decorate@parsesoftpath{\softpath}{\parsedsoftpath}{}
%	
%	results in:
%	
%	\parsedsoftpath ->
%	  {\pgf@decorate@inputsegmentobject@lineto{12pt}{\pgf@x 0pt\pgf@y 0pt}{\pgf@x 0pt\pgf@y 12pt}}
%	  {\pgf@decorate@inputsegmentobject@lineto{12pt}{\pgf@x 0pt\pgf@y 12pt}{\pgf@x 12pt\pgf@y 12pt}}
%	
%	\pgfdecoratedpathlength ->
%	  24pt
%

\def\pgf@decorate@parsesoftpath#1#2{%
	\def\pgf@decorate@inputsegmentobjectsmacro{#2}%
	\let\pgf@decorate@inputsegmentobjects\pgfutil@empty%
	\pgfutil@tempdima0pt\relax%
	\let\pgfpoint@decorate@lastparsed\pgfpoint@decorate@existingpathlast%
	\let\pgfpoint@decorate@lastnonmovetoparsed\pgfpoint@origin%
	\let\pgf@decorate@queueinputsegmentobject\pgfutil@empty%
	\let\pgfpoint@decorated@firstparsed\pgfutil@empty%
	\expandafter\pgf@decorate@@parsesoftpath#1\pgf@stop%
}

\def\pgf@decorate@@parsesoftpath#1{%
	\ifx#1\pgf@stop%
		\let\pgf@decorate@queueinputsegmentobject\pgfutil@empty% <- removes final moveto (may not be desirable).
		\pgf@decorate@addtoinputsegmentobjects{\pgf@decorate@inputsegmentobject@endofinputsegments}%
		\pgf@decorate@addtoinputsegmentobjects{\pgf@decorate@inputsegmentobject@endofinputsegments}%
		\expandafter\let\pgf@decorate@inputsegmentobjectsmacro\pgf@decorate@inputsegmentobjects%
		\edef\pgf@decorate@totalpathlength{\the\pgfutil@tempdima}%
		\let\pgf@next\relax%
	\else%
		\ifx#1\pgfsyssoftpath@movetotoken%
			\let\pgf@next\pgf@decorate@parsemoveto%
		\else%
			\ifx#1\pgfsyssoftpath@linetotoken%
				\let\pgf@next\pgf@decorate@parselineto%
			\else%
				\ifx#1\pgfsyssoftpath@curvetosupportatoken%
					\let\pgf@next\pgf@decorate@parsecurveto%
				\else%
					\ifx#1\pgfsyssoftpath@closepathtoken%
						\let\pgf@next\pgf@decorate@parseclosepath%
					\else%
						\ifx#1\pgfsyssoftpath@rectcornertoken%
							\let\pgf@next\pgf@decorate@parserect%
						\else%
							\PackageError{PGF}{Unrecognised soft path token `#1'}{}%
						\fi%
					\fi%
				\fi%
			\fi%
		\fi%
	\fi%
	\pgf@next}


\def\pgf@decorate@addtoinputsegmentobjects#1{%
	%
	% If there is an input segment object waiting (i.e. a moveto), insert it here.
	%
	\ifx\pgf@decorate@queueinputsegmentobject\pgfutil@empty%
	\else%
		\let\pgf@decorate@temp\pgf@decorate@queueinputsegmentobject%
		\let\pgf@decorate@queueinputsegmentobject\pgfutil@empty%
		\expandafter\pgf@decorate@addtoinputsegmentobjects\expandafter{\pgf@decorate@temp}%
	\fi%
	\ifx\pgfpoint@decorated@firstparsed\pgfutil@empty%
		#1%
		\let\pgfpoint@decorated@firstparsed\pgf@decorate@inputsegment@first%
	\fi%
	\expandafter\def\expandafter\pgf@decorate@inputsegmentobjects\expandafter%
		{\pgf@decorate@inputsegmentobjects{#1}}%
}

%	Convert \pgfsyssoftpath@movetotoken{<X>}{<Y>} into the following
% representation:
%	
%	\pgf@decorate@inputsegmentobject@moveto{\pgf@x X\pgf@y Y}
%
%	The moveto input segment object is not added immediately, so that
%	only the last of multiple movetos is inserted.
%	
\def\pgf@decorate@parsemoveto#1#2{%
	\def\pgf@decorate@queueinputsegmentobject{\pgf@decorate@inputsegmentobject@moveto{\pgf@x#1\pgf@y#2}}%
	\def\pgfpoint@decorate@lastparsed{\pgf@x#1\pgf@y#2}%
	\pgf@decorate@@parsesoftpath%
}

% Convert \pgfsyssoftpath@linetotoken{<X>}{<Y>} into the following
% representation:
%
% \pgf@decorate@inputsegmentobject@lineto{<length>}{\pgf@x <Last X> \pgf@y <Last Y}{\pgf@x <X> \pgf@y <Y>}
%
\def\pgf@decorate@parselineto#1#2{%
	\pgf@decorate@linelength{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}%
	\advance\pgfutil@tempdima\pgfmathresult pt\relax%
	\edef\pgf@decorate@temp{%
		\noexpand\pgf@decorate@inputsegmentobject@lineto{\pgfmathresult pt}{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}%
	}%
	\edef\pgfpoint@decorate@lastparsed{\pgf@x#1\pgf@y#2}%
	\let\pgfpoint@decorate@lastnonmovetoparsed\pgfpoint@decorate@lastparsed%
	\expandafter\pgf@decorate@addtoinputsegmentobjects\expandafter{\pgf@decorate@temp}%
	\pgf@decorate@@parsesoftpath%
}
	
% Convert \pgfsyssoftpath@curvetosupportatoken{<Xa>}{<Ya>}...etc
% into the following representation:
%
% \pgf@decorate@inputsegmentobject@curveto{<length>}{\pgf@x <Last X> \pgf@y <Last Y}
%		{\pgf@x <Xa> \pgf@y <Ya>}{\pgf@x <Xb> \pgf@y <Yb>}{\pgf@x <X> \pgf@y <Y>}
%
\def\pgf@decorate@parsecurveto#1#2\pgfsyssoftpath@curvetosupportbtoken#3#4\pgfsyssoftpath@curvetotoken#5#6{%
	\pgf@decorate@curvelength{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}{\pgf@x#3\pgf@y#4}{\pgf@x#5\pgf@y#6}%
	\advance\pgfutil@tempdima\pgfmathresult pt\relax%
	\edef\pgf@decorate@temp{%
		\noexpand\pgf@decorate@inputsegmentobject@curveto{\pgfmathresult pt}{\pgfpoint@decorate@lastparsed}%
			{\pgf@x#1\pgf@y#2}{\pgf@x#3\pgf@y#4}{\pgf@x#5\pgf@y#6}%
	}%
	\expandafter\pgf@decorate@addtoinputsegmentobjects\expandafter{\pgf@decorate@temp}%
	\edef\pgfpoint@decorate@lastparsed{\pgf@x#5\pgf@y#6}%
	\let\pgfpoint@decorate@lastnonmovetoparsed\pgfpoint@decorate@lastparsed%
	\pgf@decorate@@parsesoftpath%
}


\def\pgf@decorate@parseclosepath#1#2{%
	\pgf@decorate@linelength{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}%
	\advance\pgfutil@tempdima\pgfmathresult pt\relax%
	\edef\pgf@decorate@temp{%
		\noexpand\pgf@decorate@inputsegmentobject@closepath{\pgfmathresult pt}{\pgfpoint@decorate@lastparsed}{\pgf@x#1\pgf@y#2}%
	}%
	\expandafter\pgf@decorate@addtoinputsegmentobjects\expandafter{\pgf@decorate@temp}%
	\edef\pgfpoint@decorate@lastparsed{\pgf@x#1\pgf@y#2}%
	\let\pgfpoint@decorate@lastnonmovetoparsed\pgfpoint@decorate@lastparsed%
	\pgf@decorate@@parsesoftpath%
}

% Convert \pgfsyssoftpath@rectcornertoken{<X>}{<Y>}\pgfsyssoftpath@rectsizetoken{<Xa>}{<Ya>}
% into either (clockwise)
%
% \pgf@decorate@inputsegmentobject@moveto{<X>}{<Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 1>}{\pgf@x <X> \pgf@y <Y>}{\pgf@x <X> \pgf@y <Ya+Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 2>}{\pgf@x <X> \pgf@y <Ya+Y>}{\pgf@x <Xa+X> \pgf@y <Ya+Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 1>}{\pgf@x <Xa+X> \pgf@y <Ya+X>}{\pgf@x <Xa+X> \pgf@y <Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 2>}{\pgf@x <Xa+X> \pgf@y <Y>}{\pgf@x <X> \pgf@y <Y>}
% \pgf@decorate@inputsegmentobject@moveto{<Xa>}{<Ya>}
%
% ...or (anti-clockwise)
%
% \pgf@decorate@inputsegmentobject@moveto{<X>}{<Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 2>}{\pgf@x <X> \pgf@y <Y>}{\pgf@x <Xa+X> \pgf@y <Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 1>}{\pgf@x <Xa+X> \pgf@y <Y>}{\pgf@x <Xa+X> \pgf@y <Ya+Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 2>}{\pgf@x <Xa+X> \pgf@y <Ya+Y>}{\pgf@x <X> \pgf@y <Ya+Y>}
% \pgf@decorate@inputsegmentobject@lineto{<length 1>}{\pgf@x <X> \pgf@y <Ya+Y>}{\pgf@x <X> \pgf@y <Y>}
% \pgf@decorate@inputsegmentobject@moveto{<Xa>}{<Ya>}
%
\newif\ifpgfdecoraterectangleclockwise
\def\pgf@decorate@parserect#1#2\pgfsyssoftpath@rectsizetoken#3#4{%
	%
	% Subvert \pgf@decorate@parsesoftpath so parsing macros will
	% return here instead of continuing to parse the soft path.
	%
	\let\pgf@decorate@orig@@parsesoftpath\pgf@decorate@@parsesoftpath%
	\let\pgf@decorate@@parsesoftpath\relax%
	\pgf@decorate@parsemoveto{#1}{#2}%
	\pgf@xa#1\relax%
	\pgf@ya#2\relax%
	\ifpgfdecoraterectangleclockwise%	
		\advance\pgf@ya#4%
		\pgf@yb\pgf@ya%
		\edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
		\expandafter\pgf@decorate@parselineto\pgf@temp%
		\advance\pgf@xa#3%
		\pgf@xb\pgf@xa%
		\edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
		\expandafter\pgf@decorate@parselineto\pgf@temp%
		\advance\pgf@ya-#4%
		\edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
		\expandafter\pgf@decorate@parselineto\pgf@temp%
		\advance\pgf@xa-#3%
		\edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
		\expandafter\pgf@decorate@parseclosepath\pgf@temp%
	\else%
		\advance\pgf@xa#3%
		\edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
		\pgf@xb\pgf@xa%
		\expandafter\pgf@decorate@parselineto\pgf@temp%
		\advance\pgf@ya#4%
		\pgf@yb\pgf@ya%
		\edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
		\expandafter\pgf@decorate@parselineto\pgf@temp%
		\advance\pgf@xa-#3%
		\edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
		\expandafter\pgf@decorate@parselineto\pgf@temp%
		\advance\pgf@ya-#4%
		\edef\pgf@temp{{\the\pgf@xa}{\the\pgf@ya}}%
		\expandafter\pgf@decorate@parseclosepath\pgf@temp%
	\fi%	
	%
	% Restore the parsing.
	%
	\let\pgf@decorate@@parsesoftpath\pgf@decorate@orig@@parsesoftpath%
	\edef\pgf@marshal{\noexpand\pgf@decorate@parsemoveto{\the\pgf@xb}{\the\pgf@yb}}%
	\pgf@marshal%
}




% \pgf@decorate@linelength
%
% Define \pgfmathresult as the distance between #1 and #2 (without units).
%
\def\pgf@decorate@linelength#1#2{%
	\pgf@process{\pgfpointdiff{#1}{#2}}%
	\pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
}

% \pgf@decorate@curvelength
%
% Define \pgfmathresult as the length (without units) of the cubic 
% bezier described by #1,#2,#3 and #4.
%
% To approximate the length of the curve P (sort of) use:
% 
% curveLength(P,q)
% 	Q = subdivideLeft(P);
%		R = subdivideRight(P);
%   return curveLength'(Q,q) + curveLength'(R,q);
%
% curveLength'(P,q)
%		<P1,P2,P3,P4> <- P;
%   P' = P4 - P1;
%   x = P'.x();
%		y = P'.y();
%   if (x < q) && (y < q)
%			return |P'|;
%		else%
%  		Q = subdivideLeft(P);
%			R = subdivideRight(P);
%     return curveLength'(Q,q) + curveLength'(R,q);
%  
% Where q is some small value (`tolerance').
% 
\newif\ifpgf@decorate@subdivide
\def\pgf@decorate@curvelength#1#2#3#4{%
	%
	% Always begin with a subdivision in case #1 = #4.
	%
	\begingroup%
		\pgf@decorate@recursive@subdividecurve@left{#1}{#2}{#3}{#4}%
		\pgfutil@tempdimb\pgfmathresult pt\relax%
		\pgf@decorate@recursive@subdividecurve@right{#1}{#2}{#3}{#4}%
		\advance\pgfutil@tempdimb\pgfmathresult pt\relax%
		\pgfmath@returnone\pgfutil@tempdimb%
	\endgroup%
}
	
\def\pgf@decorate@@curvelength#1#2#3#4{%
	\begingroup%
		\pgf@decorate@curvecordlength{#1}{#2}{#3}{#4}%
		\ifpgf@decorate@subdivide%
			\pgf@decorate@recursive@subdividecurve@left{#1}{#2}{#3}{#4}%
			\pgfutil@tempdimb\pgfmathresult pt\relax%
			\pgf@decorate@recursive@subdividecurve@right{#1}{#2}{#3}{#4}%
			\advance\pgfutil@tempdimb\pgfmathresult pt\relax%
			\expandafter\pgfmath@returnone\expandafter\pgfutil@tempdimb%
		\else%
			\expandafter\pgfmath@returnone\expandafter\pgfmathresult\expandafter p\expandafter t\expandafter%
		\fi%
	\endgroup%
}

\def\pgf@decorate@curvelength@tolerance{1pt}

\def\pgf@decorate@curvecordlength#1#2#3#4{%
	% 
	% Calculate the curve cord vector.
	%
	#4\relax%
	\pgf@xa\pgf@x\pgf@ya\pgf@y%
	#1\relax%
	\advance\pgf@xa-\pgf@x%
	\advance\pgf@ya-\pgf@y%
	\ifdim\pgf@xa<0pt\relax\pgf@xa-\pgf@xa\fi%
	\ifdim\pgf@ya<0pt\relax\pgf@ya-\pgf@ya\fi%
	%
	% Always subdivide, unless...
	%
	\pgf@decorate@subdividetrue%
	%
	% The cord vector is small.
	%
	\ifdim\pgf@xa<\pgf@decorate@curvelength@tolerance\relax%
		\ifdim\pgf@ya<\pgf@decorate@curvelength@tolerance\relax%
			\pgfmathveclen@{\pgfmath@tonumber{\pgf@xa}}{\pgfmath@tonumber{\pgf@ya}}%
			\pgf@decorate@subdividefalse%
		\fi%		
	\fi%
}

\def\pgf@decorate@recursive@subdividecurve@left#1#2#3#4{%
	{%
		%
		% The left curve (from t=0 to t=.5) 
		%
		#1\relax%
		\pgfutil@tempdima\pgf@x%
		\pgfutil@tempdimb\pgf@y%
		\pgf@xa.5\pgf@x\pgf@ya.5\pgf@y%
		\pgf@xb.25\pgf@x\pgf@yb.25\pgf@y%
		\pgf@xc.125\pgf@x\pgf@yc.125\pgf@y%
		#2\relax%
		\advance\pgf@xa.5\pgf@x\advance\pgf@ya.5\pgf@y%
		\advance\pgf@xb.5\pgf@x\advance\pgf@yb.5\pgf@y%
		\advance\pgf@xc.375\pgf@x\advance\pgf@yc.375\pgf@y%
		#3\relax%
		\advance\pgf@xb.25\pgf@x\advance\pgf@yb.25\pgf@y%
		\advance\pgf@xc.375\pgf@x\advance\pgf@yc.375\pgf@y%
		#4\relax%
		\advance\pgf@xc.125\pgf@x\advance\pgf@yc.125\pgf@y%
		\xdef\pgf@marshal{%
			\noexpand\pgf@decorate@@curvelength%
				{\pgf@x\the\pgfutil@tempdima\pgf@y\the\pgfutil@tempdimb}%
				{\pgf@x\the\pgf@xa\pgf@y\the\pgf@ya}{\pgf@x\the\pgf@xb\pgf@y\the\pgf@yb}
					{\pgf@x\the\pgf@xc\pgf@y\the\pgf@yc}%
		}%
	}%
	\pgf@marshal%
}

\def\pgf@decorate@recursive@subdividecurve@right#1#2#3#4{%
	{%
		%
		% The right curve (from t=0.5 to t=1) 
		%
		#1\relax%
		\pgfutil@tempdima.125\pgf@x\pgfutil@tempdimb.125\pgf@y%
		#2\relax%
		\advance\pgfutil@tempdima.375\pgf@x\advance\pgfutil@tempdimb.375\pgf@y%
		\pgf@xa.25\pgf@x\pgf@ya.25\pgf@y%
		#3\relax%
		\advance\pgfutil@tempdima.375\pgf@x\advance\pgfutil@tempdimb.375\pgf@y%
		\advance\pgf@xa.5\pgf@x\advance\pgf@ya.5\pgf@y%
		\pgf@xb.5\pgf@x\pgf@yb.5\pgf@y%
		#4\relax%
		\advance\pgfutil@tempdima.125\pgf@x\advance\pgfutil@tempdimb.125\pgf@y%
		\advance\pgf@xa.25\pgf@x\advance\pgf@ya.25\pgf@y%
		\advance\pgf@xb.5\pgf@x\advance\pgf@yb.5\pgf@y%
		\pgf@xc\pgf@x\pgf@yc\pgf@y%
		\xdef\pgf@marshal{%
			\noexpand\pgf@decorate@@curvelength%
				{\pgf@x\the\pgfutil@tempdima\pgf@y\the\pgfutil@tempdimb}%
				{\pgf@x\the\pgf@xa\pgf@y\the\pgf@ya}{\pgf@x\the\pgf@xb\pgf@y\the\pgf@yb}
					{\pgf@x\the\pgf@xc\pgf@y\the\pgf@yc}%
		}%
	}%
	\pgf@marshal%
}


\let\startpgfdecoration=\pgfdecoration
\let\stoppgfdecoration=\endpgfdecoration

\let\startpgfmetadecoration=\pgfmetadecoration
\let\stoppgfmetadecoration=\endpgfmetadecoration



%
% Predefined decorations
%


% Simple decorations. 

\pgfdeclaredecoration{lineto}{initial}{
  \state{initial}[switch if input segment less than=\pgfdecoratedremainingdistance to input segment,
                  width=\pgfdecoratedremainingdistance]
  {
  }
  \state{input segment}[width=\pgfdecoratedinputsegmentlength,next state=initial]
  {
    \pgfpathlineto{\pgfpointdecoratedinputsegmentlast}
  }
  
  \state{final}{\pgfpathlineto{\pgfpointdecoratedpathlast}}
}

\pgfdeclaredecoration{moveto}{initial}{
  \state{initial}[width=\pgfdecoratedremainingdistance]{}
  \state{final}{\pgfpathmoveto{\pgfpointdecoratedpathlast}}
}

% This decorations curves to the end along the line.

\pgfdeclaredecoration{curveto}{initial}{
  \state{initial}[width=\pgfdecoratedinputsegmentlength/100]
  {
    \pgfpathlineto{\pgfpointorigin}
  }
  \state{final}{\pgfpathlineto{\pgfpointdecoratedpathlast}}
}




% Compatibility with old "snakes":

\let\pgfsnakeremainingdistance=\pgfdecoratedremainingdistance
\let\pgfsnakecompleteddistance=\pgfdecoratedcompleteddistance
\def\pgfsnakeangle{\pgfdecoratedangle}
\let\pgfdeclaresnake=\pgfdeclaredecoration
\let\pgfsetsnakesegmenttransformation=\pgfsetdecorationsegmenttransformation
\def\pgfpathsnakesto#1#2{%
  \edef\pgf@temp{#1}%
  \expandafter\pgfdecoration\expandafter{\pgf@temp}%
    \pgfpathlineto{#2}%
  \endpgfdecoration%
}
\def\pgfpathsnaketo#1#2{\pgfpathsnakesto{{#1}{\pgfsnakeremainingdistance}}{#2}}
\def\pgfpathsnakealongvector#1#2#3{%
  \pgf@process{#3}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgfmathparse{#2}%
  \pgf@xa=\pgfmathresult\pgf@xa%
  \pgf@ya=\pgfmathresult\pgf@ya%
  \advance\pgf@xa by\pgf@path@lastx%
  \advance\pgf@ya by\pgf@path@lasty%
  \edef\pgf@snake@lib@temp{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \pgfpathsnaketo{#1}{\pgf@snake@lib@temp}%
}

\let\pgfsnakesegmentamplitude=\pgfdecorationsegmentamplitude
\let\pgfsnakesegmentlength=\pgfdecorationsegmentlength
\def\pgfsnakesegmentangle{\pgfdecorationsegmentangle}
\def\pgfsnakesegmentobjectlength{\pgfkeysvalueof{/pgf/decoration/shape start width}}
\def\pgfsnakesegmentaspect{\pgfdecorationsegmentaspect}

\pgfset{%
  /pgf/segment amplitude/.style={/pgf/decoration={amplitude=#1,shape height=2*#1}},
  /pgf/segment length/.style={/pgf/decoration={segment length=#1}},
  /pgf/segment angle/.style={/pgf/decoration={angle=#1}},
  /pgf/segment aspect/.style={/pgf/decoration={aspect=#1}},
  /pgf/segment object length/.style={/pgf/decoration={shape width=#1,radius=#1}}}



\endinput

==> pgfmodulematrix.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/modules/pgfmodulematrix.code.tex,v 1.1 2008/01/15 10:27:34 tantau Exp $

\usepgfmodule{shapes}

\newif\ifpgfmatrix
\newif\ifpgf@matrix@correct@call

\newif\ifpgf@matrix@fixed

\newcount\pgfmatrixcurrentrow

\newcount\pgfmatrixcurrentcolumn
\newcount\pgf@matrix@numberofcolumns

\let\pgf@matrix@cell=\pgfnodeparttextbox % alias
\let\pgf@matrix@box=\pgf@matrix@cell % alias


% Sets the default row or column sep
%
% #1 = default row or column sep list
%
% Description:
%
% Sets the macro \pgfmatrixrowsep or \pgfmatrixcolumnsep to #1.
%
% Example:
%
% \pgfsetmatrixrowsep{5pt}

\def\pgfsetmatrixrowsep#1{\def\pgfmatrixrowsep{#1}}
\def\pgfsetmatrixcolumnsep#1{\def\pgfmatrixcolumnsep{#1}}

\def\pgfmatrixrowsep{0pt}
\def\pgfmatrixcolumnsep{0pt}



% The pgfmatrix command creates a node that contains a matrix. Like
% the \pgfnode command, it is to be used inside a pgfpicture
% environment. 
%
% #1 = shape type
% #2 = anchor
% #3 = name for later reference
% #4 = path usage command
% #5 = inner shift
% #6 = startup code
% #7 = the matrix code (may contain verbatim stuff)
%
% Description:
%
% This command creates a node that contains a matrix. For 
% each cell of the matrix, drawing commands may be given. These
% commands will create a cell picture and a bounding box is computed
% for each cell picture. The cell picture is then placed inside the
% cell. The position inside the cell is computed according to the
% following rules: 
%
% 1. In each column, the origins of the cell pictures are all on a
%    vertical line.
% 2. In each row, the origins of the cell pictures are all on a
%    horizontal line.
% 3. All cells in the same row have the same height and depth.
% 4. All cells in the same column have the same width.
% 5. The size of cells are chosen minimal such that the boxes fit into
%    the cells and still meet the above requirement.
%
% Next, the whole resulting matrix, which is given as #7, is placed
% inside a node whose name is given as #3, whose shape is #1, and
% whose anchor is #1. This means that the resulting node is shifted
% such that the given anchor lies at the origin. Then, as for a normal
% node, the #4 path usage command is used for the node. 
%
% The parameter #5 is an additional negative shift for the node. Normally, such
% a shift could be given beforehand (that is, the shift could be
% preapplied to the current transformation matrix). However, when #5
% is evaluated, you can refer to temporary positions of nodes inside
% the matrix. In detail, the following happens: When the matrix has
% been typeset, all nodes in the matrix temporarily get assigned their
% positions in the matrix box. The origin of this coordinate system is
% at the left baseline end of the matrix box, which corresponds to the
% text anchor. The position #5 is then interpreted inside this
% coordinate system and then used for shifting. 
%
% The idea behind using the parameter #5 is the following: If you
% specify "text" as anchor #2 and specify \pgfpointanchor{inner
% node}{some anchor} for parameter #5, where inner node is a node that
% is created in the matrix, then the whole matrix will be shifted such
% that inner node.some anchor lies at the origin of the whole picture.
%
% At the beginning and at the end of each cell, the macros
% \pgfmatrixbegincode and \pgfmatrixendcode are called. Inside these
% macros you can use \pgfmatrixcurrentcolumn and \pgfmatrixcurrentrow
% to access the current row and column.
%
% Before each column except for the first, an extra space given by the
% macro \pgfmatrixcolumnsep is added. Additionally, an extra space
% given by the optional argument of the \pgfmatrixnextcell commands in
% the first line are added, which may vary between columns. Between
% rows, an extra space given by the macro \pgfmatrixrowsep is
% added. You can also change this value for each row by using a \gdef.
%
%
% Lines are ended using the command \pgfmatrixendrow. The command \\
% is \let to be the same, but \\ is sometimes overridden by, say,
% minipage, so it's good to have \pgfmatrixendrow as a "fallback". 
%
% Inside the matrix, \\ must be used to end every line ***including
% the last***. You can pass an optional parameter to \\ as in \\[2pt]
% to give an additional space after this particular line.
%
% The usage of \\ at the end of the matrix is imporant since this
% command is used to find the end of the matrix. What happens is that
% \\ followed by a closing brace ends the matrix. 
%
% Inside the matrix, you must use \pgfmatrixnextcell to separate
% columns. The reason is that two columns are used internally for
% every single column shown. The macro \pgfmatrixnextcell is yields
% (more or less) two && (and some further trickery).
%
% The parameter #6 is executed at the beginning of the matrix
% group. It is inside the protecting group of the matrix, but outside
% the matrix itself. It can be used for different purposes: 1) It can be
% used to simplify the next cell macro. 2) It can be used to issue an
% \aftergroup command. 3) It can be used to setup local settings. For
% example, by setting #6 to \let\&=\pgfmatrixnextcell you can use \&
% instead of \pgfmatrixnextcell. You can also set the catcode of & to
% active.
%
%
% Example:
%
% \begin{tikzpicture}
%
%   \draw (0,0) circle (1mm);  % b.north will lie on the center of this circle
%
%   \pgfmatrix{rectangle}{text}{mymatrix}{\pgfusepath{}}{\pgfpointanchor{b}{north}}{\let\&=\pgfmatrixnextcell}
%   {
%     \draw (0,0) circle (1cm); \& \node (a) [draw] {Hallo}; \\
%     \node (b) [draw] {Welt};  \& \draw (0,0) circle (5mm); \\
%   }
%
%   \draw [->] (a) -- (b);
%
% \end{tikzpicture}

\def\pgfmatrix#1#2#3#4#5#6{%
  \ifpgfmatrix%
    \PackageError{pgf}{You cannot nest pgfmatrix environments, yet}{}
  \fi%
  \bgroup%  
    #6%
    \def\pgf@matrix@par@shape{#1}%
    \def\pgf@matrix@par@anchor{#2}%
    \def\pgf@matrix@par@name{#3}%
    \def\pgf@matrix@par@usage{#4}%
    \def\pgf@matrix@par@shift{#5}%
    % the matrix must have a name:
    \ifx\pgf@matrix@par@name\pgfutil@empty%
      \def\pgf@matrix@par@name{pgf@matrix@internal}%
    \fi%
    \pgfmatrixcurrentrow=0\relax%
    \pgfmatrixcurrentcolumn=0\relax%
    \pgf@matrix@numberofcolumns=0\relax%
    \let\\=\pgfmatrixendrow%
    \tabskip=0pt%
    \offinterlineskip%
    \pgfmatrixtrue%
    \let\pgf@matrix@node@list=\pgfutil@empty%
    \expandafter\let\csname pgf@matrix@column@finish@1\endcsname=\pgfutil@empty%
    \let\pgf@matrix@row@finish=\pgfutil@empty%
    % 
    % Get rid of bgroup
    %
    \afterassignment\pgf@matrix@cont\let\pgf@next=%
}
\def\pgf@matrix@cont{%  
    \setbox\pgf@matrix@box=\hbox\bgroup\vbox\bgroup%
    \halign\bgroup%
    \pgf@matrix@init@row%
    \pgf@matrix@step@column%
    {%
      \pgf@matrix@startcell%
      ##%
      \pgf@matrix@endcell%
    }%
    &%
    ##\pgf@matrix@padding&&%
    \pgf@matrix@step@column%
    {%
      \pgf@matrix@startcell%
      ##%
      \pgf@matrix@endcell%
    }&%
    ##\pgf@matrix@padding%
    \cr%
}

\def\pgf@end@matrix{%
      \egroup\egroup%
    \egroup%
    %
    % If there are named nodes, we must adjust their coordinates.
    %
    \ifx\pgf@matrix@node@list\pgfutil@empty%
    \else%
      % Ok, this means we got a lot of work to do...
      \pgf@matrix@compute@origin%
      \pgf@matrix@shift@nodes@initial%
    \fi%
    %
    % Compute additional shift
    %
    \pgftransformresetnontranslations%
    \pgftransformshift{\pgf@process{\pgftransformreset\pgf@matrix@par@shift\pgf@x=-\pgf@x\pgf@y=-\pgf@y}}%
    %
    % Create node
    %
    \pgfmultipartnode{\pgf@matrix@par@shape}{\pgf@matrix@par@anchor}{\pgf@matrix@par@name}{\pgf@matrix@par@usage}%
    %
    % If there are named nodes, we must adjust their coordinates, again.
    %
    \ifx\pgf@matrix@node@list\pgfutil@empty%
    \else%
      {%
        \pgftransformreset%
        \pgf@process{\pgfpointanchor{\pgf@matrix@par@name}{text}}%
        \xdef\pgf@matrix@offset{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
        \pgf@matrix@shift@nodes@secondary{\pgf@matrix@offset}%
      }%
    \fi%
}




% Ending a cell
%
% #1 = (optional) spacing between previous and next column. This
%      parameter only has an effect in the first row.
%
% Description:
%
% This command ends a cell of a matrix.
%
% Example:
%
% \pgfmatrix{rectangle}{text}{mymatrix}{\pgfusepath{}}{\pgfpointanchor{b}{north}}{}
% {
%   \draw (0,0) circle (1cm); \pgfmatrixnextcell[1cm] \node (a) [draw] {Hallo}; \\
%   \node (b) [draw] {Welt};  \pgfmatrixnextcell \draw (0,0) circle (5mm); \\
% }

\def\pgfmatrixnextcell{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end%
  \pgfutil@ifnextchar[{\pgf@matrix@cell@cont}{\pgf@matrix@cell@cont[0pt]}}%}

\def\pgf@matrix@cell@cont[#1]{%
  \ifnum\pgfmatrixcurrentcolumn<\pgf@matrix@numberofcolumns%
  \else%
  {%
    \global\pgf@matrix@fixedfalse%
    \pgf@x=0pt%
    \pgf@matrix@addtolength{\pgf@x}{\pgfmatrixcolumnsep}%
    \pgf@matrix@addtolength{\pgf@x}{#1}%
    \ifpgf@matrix@fixed%
      \expandafter\pgfutil@g@addto@macro\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname%
        {\global\pgf@picmaxx=0pt}%
    \fi%
    \advance\pgfmatrixcurrentcolumn by1\relax % only temporary for the following:
    \expandafter\xdef\csname pgf@matrix@column@sep@\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@x}%
    \ifpgf@matrix@fixed%
      \expandafter\gdef\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname{\global\pgf@picminx=0pt}%
    \else%
      \expandafter\global\expandafter\let\csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname=\pgfutil@empty%
    \fi%
  }%
  \fi%
  &\pgf@matrix@correct@calltrue&%
}%


\def\pgf@matrix@fixed@text{between origins}
\def\pgf@matrix@natural@text{between borders}

\def\pgf@matrix@addtolength#1#2{\edef\pgf@temp{#2}\expandafter\pgf@matrix@addtolength@\expandafter#1#2,\pgf@stop}
\def\pgf@matrix@addtolength@#1#2,#3\pgf@stop{%
  \def\pgf@temp{#2}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \ifx\pgf@temp\pgf@matrix@fixed@text%
      \global\pgf@matrix@fixedtrue%
    \else%
      \ifx\pgf@temp\pgf@matrix@natural@text%
        \global\pgf@matrix@fixedfalse%
      \else%
        \pgfmathaddtolength{#1}{#2}%
      \fi%
    \fi%
  \fi%
  \def\pgf@temp{#3}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \pgf@matrix@addtolength@#1#3\pgf@stop%
  \fi%
}



% Init a line

\def\pgf@matrix@init@row{%
  \relax%
  \global\advance\pgfmatrixcurrentrow by 1\relax%
  \global\pgfmatrixcurrentcolumn=0\relax%
  \expandafter\gdef\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname{0pt}%
  \expandafter\gdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{0pt}%
}



% Step the row column number

\def\pgf@matrix@step@column{%
  \relax%
  \global\advance\pgfmatrixcurrentcolumn by1\relax%
}



% Start a cell

\def\pgf@matrix@startcell{%
  %
  % Step 1: Init the list of nodes for this cell
  %
  \let\pgf@nodecallback=\pgf@matrix@nodecallback%
  %
  % Step 2: Setup the bounding box
  %
  \pgfinterruptboundingbox%
  %
  % Step 3: Reset the transformation matrix
  %
  \pgftransformreset%
  %
  % Step 4: Collect everything in a cell box
  %
  \setbox\pgf@matrix@cell=\hbox\bgroup\bgroup%
    \pgfsys@beginpicture%
    \normalbaselines%
    % Find out whether the cell is empty:
    \pgfutil@ifnextchar\let%
    {% ok, candidate, check following symbol
      \afterassignment\pgf@matrix@empty@check\let\pgf@matrix@temp=% get rid of \let
    }%
    {% no, not empty
      \pgf@matrix@empty@cell@false%
      \pgfmatrixbegincode%
    }%
}

\def\pgf@matrix@empty@check{\futurelet\pgf@matrix@check@token\pgf@matrix@empty@check@cont}
\def\pgf@matrix@empty@check@cont{%
  \ifx\pgf@matrix@check@token\pgf@matrix@signal@cell@end%
    \pgf@matrix@empty@cell@true%
    \expandafter%
    \pgfmatrixemptycode%
    \expandafter%
    \let% reinserted
  \else%
    \pgf@matrix@empty@cell@false%
    \expandafter%
    \pgfmatrixbegincode%
    \expandafter
    \let% reinserted
  \fi%
}   

\newif\ifpgf@matrix@empty@cell@


% End a  cell

\def\pgf@matrix@endcell{%
    \ifpgf@matrix@empty@cell@%
    \else%
      \expandafter\pgfmatrixendcode%
    \fi
    \pgfsys@endpicture%
    \csname pgf@matrix@column@finish@\the\pgfmatrixcurrentcolumn\endcsname%
    \pgf@matrix@row@finish%
  \egroup\egroup%
  % Special case of the empty picture
  \ifdim\pgf@picmaxx=-16000pt\relax%
    \pgf@picmaxx=0pt\relax%
    \pgf@picminx=0pt\relax%
    \pgf@picmaxy=0pt\relax%
    \pgf@picminy=0pt\relax%
  \fi%
  %
  % Step 5: Horizontal gap
  %
  \ifnum\pgfmatrixcurrentcolumn>1\relax%
    \pgf@y=\csname pgf@matrix@column@sep@\the\pgfmatrixcurrentcolumn\endcsname\relax%
    \advance\pgf@picminx by-\pgf@y%
  \fi%
  % 
  % Step 6: Protocol and adjust height and depth
  %
  % Step 6.1: Protocol...
  %
  \ifdim\pgf@picmaxy>\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname%
    \expandafter\xdef\csname pgf@matrix@maxy\the\pgfmatrixcurrentrow\endcsname{\the\pgf@picmaxy}%
  \fi%  
  \ifdim\pgf@picminy<\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname%
    \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@picminy}%
  \fi%  
  %
  % Step 6.2: and setup.
  %  
  \ht\pgf@matrix@cell=\pgf@picmaxy%
  \dp\pgf@matrix@cell=-\pgf@picminy%
  %
  % Step 7: Protocol and adjust left and right width
  %
  % Step 7.1: Protocol...
  %
  \ifnum\pgfmatrixcurrentcolumn>\pgf@matrix@numberofcolumns\relax%
    \expandafter\xdef\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picmaxx}%
    \expandafter\xdef\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picminx}%
    \global\pgf@matrix@numberofcolumns=\pgfmatrixcurrentcolumn\relax%
  \else%
    \ifdim\pgf@picmaxx>\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname%
      \expandafter\xdef\csname pgf@matrix@maxx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picmaxx}%
    \fi%  
    \ifdim\pgf@picminx<\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname%
      \expandafter\xdef\csname pgf@matrix@minx\the\pgfmatrixcurrentcolumn\endcsname{\the\pgf@picminx}%
    \fi%  
  \fi%
  %
  % Step 7.2: and setup.
  %  
  \xdef\pgf@matrix@paddingskip{\the\pgf@picmaxx}%
  % 
  % Step 8: Put in the box now
  %
  \hfil\hskip-\pgf@picminx%
  \wd\pgf@matrix@cell=0pt%
  \box\pgf@matrix@cell%
  %
  % Step 9: End bounding box
  \endpgfinterruptboundingbox%
}

% Default code for the start and end code
\let\pgfmatrixbegincode=\relax
\let\pgfmatrixendcode=\relax
\let\pgfmatrixemptycode=\relax


% The following callback is called for every node that is produced
% inside a cell

\def\pgf@matrix@nodecallback#1{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \xdef\pgf@matrix@node@list{\pgf@matrix@node@list,{#1}}%
    \expandafter\xdef\csname pgf@matrix@node@location@#1\endcsname{{\the\pgfmatrixcurrentrow}{\the\pgfmatrixcurrentcolumn}}%
  \fi%
}



% Padding code

\def\pgf@matrix@padding{%
  \ifpgf@matrix@correct@call%
  \else%
    \PackageError{pgfbasematrix}{Single ampersand used with wrong
      catcode}{}%
  \fi%
  \hskip\pgf@matrix@paddingskip\hfil%
}


% Compute the real positions of the origins

% We must now compute the real positions of the origins of all the
% small pictures. To this end, we need to compute prefix sums. After
% the procedure is done, the minx and the maxy will contain the origin
% positions. 

\def\pgf@matrix@compute@origin{%
  %
  % Inverse prefix sum on the vertical positions
  %
  {%
    \ifnum\pgfmatrixcurrentrow>0\relax%
      \expandafter\gdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{0pt}%
    \fi
    \c@pgf@counta=\pgfmatrixcurrentrow\relax%
    \loop%
    \ifnum\c@pgf@counta>1\relax%
      \pgf@y=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by\csname pgf@matrix@maxy\the\c@pgf@counta\endcsname\relax
      \advance\c@pgf@counta by-1\relax%
      \pgf@ya=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by-\pgf@ya\relax%
      \expandafter\xdef\csname pgf@matrix@miny\the\c@pgf@counta\endcsname{\the\pgf@y}%
    \repeat%
  }%
  %
  % Prefix sum on the horizontal positions
  %
  {%
    \ifnum\pgf@matrix@numberofcolumns>0\relax%
      \pgf@x=\csname pgf@matrix@minx1\endcsname\relax%
      \pgf@x=-\pgf@x%
      \expandafter\xdef\csname pgf@matrix@minx1\endcsname{\the\pgf@x}%
    \fi
    \c@pgf@counta=1\relax%
    \loop%
    \ifnum\c@pgf@counta<\pgf@matrix@numberofcolumns\relax%
      \pgf@x=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by\csname pgf@matrix@maxx\the\c@pgf@counta\endcsname\relax%
      \advance\c@pgf@counta by1\relax%
      \pgf@xa=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by-\pgf@xa\relax%
      \expandafter\xdef\csname pgf@matrix@minx\the\c@pgf@counta\endcsname{\the\pgf@x}%
    \repeat%
  }%
}


% Shift the nodes to their origins

% The following procedure shifts all nodes in
% \pgf@matrix@node@list to their location inside a temporary
% picture. This picture will later be shifted again to its final
% position in the real picture.

\def\pgf@matrix@shift@nodes@initial{%
  {%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{%
          \pgf@x=\csname pgf@matrix@minx%
            \expandafter\expandafter\expandafter\pgfutil@secondoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          \pgf@y=\csname pgf@matrix@miny%
            \expandafter\expandafter\expandafter\pgfutil@firstoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          }%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
  }%
}


% The second shifting, done in the following procedure, shifts all
% nodes to their real positions inside the real picture.

\def\pgf@matrix@shift@nodes@secondary#1{%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{#1}%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
}


% End of line
\def\pgfmatrixendrow{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end%
  &\pgf@matrix@correct@calltrue%
  \global\pgf@matrix@fixedfalse%
  \pgf@y=0pt%
  \pgf@matrix@addtolength\pgf@y{\pgfmatrixrowsep}%
  \pgfutil@ifnextchar[{\pgfmatrixendrow@skip}{\pgf@matrix@finish@line}%
}

\def\pgf@matrix@signal@cell@end{\pgf@matrix@signal@cell@end}
% exact definition does not matter, only needs to be unique.

\def\pgfmatrixendrow@skip[#1]{%
  \pgf@matrix@addtolength\pgf@y{#1}%
  \pgf@matrix@finish@line%
}

\def\pgf@matrix@finish@line{%
  \global\pgf@y=\pgf@y%
  \pgf@ya=-\pgf@y%
  \global\advance\pgf@ya by\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname%
  \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@ya}%
  \pgfutil@ifnextchar\egroup{\cr\pgf@end@matrix}{\pgf@matrix@no@eom@found}%
}

\def\pgf@matrix@eom@found{%
  \cr%
  \pgf@end@matrix%
}

\def\pgf@matrix@no@eom@found{%
  \cr%
  \noalign{\vskip\pgf@y%
  \ifpgf@matrix@fixed%
    \vskip\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname% unskip
    \vskip\pgf@y%
    \pgf@y=-\pgf@y%
    \expandafter\xdef\csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname{\the\pgf@y}%
    \gdef\pgf@matrix@row@finish{\global\pgf@picmaxy=0pt}%
  \else%
    \global\let\pgf@matrix@row@finish=\pgfutil@empty%
  \fi%
  }%
}


\endinput


==> pgfmoduleplot.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/modules/pgfmoduleplot.code.tex,v 1.1 2008/01/15 10:27:34 tantau Exp $


% PGF's plotting interface works as follows:
%
% In order to plot something, two things need to be done. First, you
% need to provide the coordinates (obviously) of the points that
% should be plotted. The coordinates are given via a long stream of
% commands. These commands are \pgfplotstreamstart, which is
% given exactly once at the beginning, \pgfplotstreampoint, of which there
% are numerous in the middle, \pgfplotstreamspecial, of which there may be
% numerous in the middle, and \pgfplotstreamend, which must be given
% at the end. Between these commands arbitrary other commands may be
% given. Here is an example:
%
% ...
% \pgfplotstreamstart
% \pgfplotstreampoint{\pgfpointxy{0}{0}}
% \pgfplotstreampoint{\pgfpointxy{1}{1}}
% \pgfplotstreampoint{\pgfpointxy{2}{4}}
% \relax
% \pgfplotstreampoint{\pgfpointxy{3}{9}}
% \pgfplotstreamspecial{some handler-dependent special stuff}
% \pgfplotstreamend
%
% By themselves, the \pgfplotstreamxxxx commands do not do anything by
% default. Rather, the ``use'' such a stream, you must first install a
% stream handler. For example, the ``lineto'' handler will simply
% translate every \pgfplotstreampoint into a \pgfpathlineto.
%
% Example:
%
% \pgfpathmoveto{\pgfpointorigin}
%
% \pgfplothandlerlineto
% \pgfplotstreamstart
% \pgfplotstreampoint{\pgfpointxy{0}{0}}
% \pgfplotstreampoint{\pgfpointxy{1}{1}}
% \pgfplotstreampoint{\pgfpointxy{2}{4}}
% \relax
% \pgfplotstreampoint{\pgfpointxy{3}{9}}
% \pgfplotstreamend


% The stream commands actually call their ``internal'' versions, which
% are set by the handlers:
\def\pgfplotstreamstart{\pgf@plotstreamstart}
\def\pgfplotstreampoint#1{\gdef\pgfplotlastpoint{#1}\pgf@plotstreampoint{#1}}
\def\pgfplotstreamspecial{\pgf@plotstreamspecial}
\def\pgfplotstreamend{\pgf@plotstreamend}




% Sets the action taken for the first point of a plot to a lineto.
%
% Description:
%
% For certain handlers it makes sense either the start a plot by
% moving to the first point of the plot or to do a lineto to that
% first point. Using this command this action can be set to a lineto. 
%
% Example:
%
% \pgfsetlinetofirstplotpoint

\def\pgfsetlinetofirstplotpoint{\let\pgf@plot@first@action=\pgfpathlineto}


% Sets the action taken for the first point of a plot to a moveto.
%
% Example:
%
% \pgfsetmovetofirstplotpoint

\def\pgfsetmovetofirstplotpoint{\let\pgf@plot@first@action=\pgfpathmoveto}

\let\pgf@plot@first@action=\pgfpathmoveto



%
% Handlers
%


% This handler converts each plot stream command into a lineto
% command, except for the first, which is converted to the action that
% has previously been specified using \pgfsetlinetofirstplotpoint or
% \pgfsetmovetofirstplotpoint. 
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotxyfile{mytable}

\def\pgfplothandlerlineto{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgf@plot@line@handler%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}

\def\pgf@plot@line@handler#1{%
  \pgf@plot@first@action{#1}%
  \global\let\pgf@plotstreampoint=\pgfpathlineto%
}



% More handlers are defined in pgflibraryplothandlers





% This handler discards the plot.
%
% Example:
%
% \pgfplothandlerdiscard
% \pgfplotxyfile{mytable}

\def\pgfplothandlerdiscard{%
  \def\pgf@plotstreamstart{%
    \global\let\pgf@plotstreampoint=\pgfutil@gobble%
    \global\let\pgf@plotstreamspecial=\pgfutil@gobble%
    \global\let\pgf@plotstreamend=\relax%
  }%
}




% This handler records each plot stream command to a macro. This is
% useful if plot commands are difficult to generate and need to be
% ``recylced'' later on.
%
% Example:
%
% \pgfplothandlerrecord{\myplot}
% \pgfplotxyfile{mytable}  % stored in \myplot now
% \pgfplothandlerline
% \myplot
% \pgftransformxshift{1cm}
% \myplot

\def\pgfplothandlerrecord#1{%
  \def\pgf@plot@recordto{#1}%
  \gdef#1{\pgfplotstreamstart}%
  \def\pgf@plotstreamstart{%
    \gdef\pgf@plotstreampoint####1{\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreampoint{####1}}}%
    \gdef\pgf@plotstreamspecial####1{\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamspecial{####1}}}%
    \gdef\pgf@plotstreamend{\expandafter\gdef\expandafter#1\expandafter{#1\pgfplotstreamend}}%
  }%
}



% Read a plot stream from a file and plot it.
%
% #1 = file from which to read things
%
% File format:
%
% Each line of the file should begin with two numbers separated by a
% space. Such a line with number #1 and #2 is converted to a
% \pgfplotstreampoint{\pgfpointxy{#1}{#2}}. Extra characters following
% on the line are ignored.
%
% Lines starting with ``%'' and ``#'' are ignored.
%
% Example:
%
% \pgfplotxyfile{tableformgnuplot.dat}

\def\pgfplotxyfile#1{%
  \begingroup%
    \pgfplotstreamstart%
    \openin1=#1
    \ifeof1
      \PackageWarning{pgf}{Plot data file `#1' not found.}
     \else
      \catcode`\#=14
      \pgf@readxyfile%
    \fi
    \pgfplotstreamend%    
  \endgroup%
}

\let\pgf@savedpar=\par%
\def\pgf@partext{\par}
\def\pgf@readxyfile{%
  \read1 to \pgf@temp%
  \let\par=\pgf@savedpar%
  \edef\pgf@temp{\pgf@temp}%
  \ifx\pgf@temp\pgfutil@empty%
  \else\ifx\pgf@temp\pgf@partext%
  \else%
    \expandafter\pgf@parsexyline\pgf@temp\pgf@stop%
  \fi\fi%
  \ifeof1\else\expandafter\pgf@readxyfile\fi%
}

\def\pgf@parsexyline#1 #2 #3\pgf@stop{%
  \pgfplotstreampoint{\pgfpointxy{#1}{#2}}%
}





% Read a plot stream from a file and plot it.
%
% #1 = file from which to read things
%
% File format:
%
% Like xy, except that each line contains three numbers, which are
% converted to xyz coordiantes.
%
% Example:
%
% \pgfplotxyfile{tableformgnuplot.dat}

\def\pgfplotxyzfile#1{%
  \begingroup%
    \pgfplotstreamstart%
    \openin1=#1
    \ifeof1
      \PackageWarning{pgf}{Plot data file `#1' not found.}
    \else
      \catcode`\#=14
      \pgf@readxyzfile%
    \fi
    \pgfplotstreamend%    
  \endgroup%
}

\def\pgf@readxyzfile{%
  \read1 to \pgf@temp%
  \ifx\pgf@temp\pgfutil@empty%
  \else\ifx\pgf@temp\pgf@partext%
  \else%
    \expandafter\pgf@parsexyzline\pgf@temp\pgf@stop%
  \fi\fi%
  \ifeof1\else\expandafter\pgf@readxyzfile\fi%
}

\def\pgf@parsexyzline#1 #2 #3 #4\pgf@stop{%
  \pgfplotstreampoint{\pgfpointxyz{#1}{#2}{#3}}%
}




% Render a function using gnuplot.
%
% #1 = filename prefix for .gnuplot and .table files (optional,
%      default is \jobname)
% #2 = gnuplot function text
%
% Description:
%
% This command will write a file called #1.gnuplot that sets up
% some gnuplot commands to write output to a file called
% #1.table. Then it calls gnuplot (using the \write18 mechanism)
% to execute the file. Then it reads #2.table using \pgfplotxyfile.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotgnuplot[\jobname]{plot [x=0:5] x*sin(x)}

{
  \catcode`\%=12
  \catcode`\"=12
  \xdef\pgf@gnuplot@head#1{set terminal table; set output "#1.table"; set format "%.5f"}
}

\newwrite\pgf@plotwrite
\newif\ifpgf@resample@plot

\def\pgfplotgnuplot{\pgfutil@ifnextchar[{\pgf@plotgnuplot}{\pgf@plotgnuplot[\jobname]}}%}
\def\pgf@plotgnuplot[#1]#2{%
  \pgf@resample@plottrue%
  % Check, whether it is up-to-date
  \openin\pgfutil@inputcheck=#1.gnuplot
  \ifeof\pgfutil@inputcheck%
  \else%
    \read\pgfutil@inputcheck to\pgf@temp% ignored
    \read\pgfutil@inputcheck to\pgf@plot@line%
    \edef\pgf@plot@code{#2\space}%
    \ifx\pgf@plot@code\pgf@plot@line%
      \openin\pgfutil@inputcheck=#1.table
      \ifeof\pgfutil@inputcheck%
      \else%
        \pgf@resample@plotfalse%
      \fi%
    \fi%
  \fi
  \ifpgf@resample@plot%  
    \immediate\openout\pgf@plotwrite=#1.gnuplot
    \immediate\write\pgf@plotwrite{\pgf@gnuplot@head{#1}}%
    \immediate\write\pgf@plotwrite{#2}%
    \immediate\closeout\pgf@plotwrite%
    \immediate\write18{gnuplot #1.gnuplot}
  \fi%
  \pgfplotxyfile{#1.table}
}



% This producer handler plots a function using pgf's mathematical engine.
%
% #1 = variable
% #2 = domain for the variable
% #3 = point, typically defined in terms of the value of the variable
%
% Description:
%
% This producer will iterate the variable #1 over all variables in #2
% (using the \foreach statement). For each value, a plot coordinate
% #3  is created.
%
% Note that this command is pretty slow.
%
% Example:
%
% \pgfplothandlerlineto
% \pgfplotfunction{\x}{0,0.1,...,3.141}{\pgfpointxy{\x}{sin(\x)}}

\def\pgfplotfunction#1#2#3{%
  \pgfplotstreamstart%
  \foreach#1in{#2}%
  {%
    \pgf@process{#3}%
    \edef\pgf@marshal{\noexpand\pgfplotstreampoint{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
    \pgf@marshal%
  }
  \pgfplotstreamend%
}




\endinput


==> pgfmoduleshapes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/modules/pgfmoduleshapes.code.tex,v 1.4 2008/02/13 15:10:06 tantau Exp $



\newbox\pgfnodeparttextbox


% Creates a node
%
% #1 = shape type
% #2 = anchor
% #3 = name for later reference
% #4 = path usage command
%
% Description:
%
% This command draws a shape that has previously been defined using
% \pgfdeclareshape. The shape is shifted such that the anchor is at
% the origin. In order to transform the whole shape, you should setup
% pgf's transformation matrix prior to calling this command.
%
% When this command is called, the shape-specific TeX boxes of the
% node must have been setup correctly.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{1cm}}
% \pgfmultipartnode{rectangle}{center}{hellonode}{\pgfusepath{stroke}}

\def\pgfmultipartnode#1#2#3#4{%
  \pgfutil@ifundefined{pgf@sh@s@#1}%
  {\PackageError{pgf}{Unknown shape ``#1''}{}}%
  {%
    {%
      \let\pgf@sh@savedmacros=\pgfutil@empty% MW
      \let\pgf@sh@savedpoints=\pgfutil@empty%
      \csname pgf@sh@s@#1\endcsname%
      \pgf@sh@savedpoints%
      \pgf@sh@savedmacros% MW
      \pgftransformshift{%
        \pgf@sh@reanchor{#1}{#2}%
        \pgf@x=-\pgf@x%
        \pgf@y=-\pgf@y%
      }%
      \expandafter\pgfsavepgf@process\csname pgf@sh@sa@#3\endcsname{%
      	\pgf@sh@reanchor{#1}{#2}%
      }%
      % Save the saved points and the transformation matrix
      \edef\pgf@test{#3}%
      \ifx\pgf@test\pgfutil@empty%
      \else%
        \expandafter\xdef\csname pgf@sh@ns@#3\endcsname{#1}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@np@#3\endcsname}%
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedpoints}%
        \edef\pgf@sh@@temp{\noexpand\gdef\expandafter\noexpand\csname pgf@sh@ma@#3\endcsname}% MW
        \expandafter\pgf@sh@@temp\expandafter{\pgf@sh@savedmacros}% MW
        \pgfgettransform\pgf@temp
        \expandafter\xdef\csname pgf@sh@nt@#3\endcsname{\pgf@temp}%
        \expandafter\xdef\csname pgf@sh@pi@#3\endcsname{\pgfpictureid}%
      \fi%
      \pgfutil@ifundefined{pgf@sh@bbg@#1}{}
      {{\pgfscope\csname pgf@sh@bbg@#1\endcsname\endpgfscope}}%
      \pgfutil@ifundefined{pgf@sh@bg@#1}{}%
      {\csname pgf@sh@bg@#1\endcsname#4}%
      \pgfutil@ifundefined{pgf@sh@fbg@#1}{}
      {{\pgfscope\csname pgf@sh@fbg@#1\endcsname\endpgfscope}}%
      {%
        \expandafter\pgfutil@for\expandafter\pgf@shape@com\expandafter:\expandafter=\csname pgf@sh@boxes@#1\endcsname\do{%
          {%
            \pgftransformshift{\pgf@sh@reanchor{#1}{\pgf@shape@com}}%
            \expandafter\pgfqboxsynced\expandafter{\csname pgfnodepart\pgf@shape@com box\endcsname}%
          }%
        }%
      }%
      \pgfutil@ifundefined{pgf@sh@bfg@#1}{}%
      {{\pgfscope\csname pgf@sh@bfg@#1\endcsname\endpgfscope}}%
      \pgfutil@ifundefined{pgf@sh@fg@#1}{}%
      {\csname pgf@sh@fg@#1\endcsname#4}%
      \pgfutil@ifundefined{pgf@sh@ffg@#1}{}%
      {{\pgfscope\csname pgf@sh@ffg@#1\endcsname\endpgfscope}}%
      \pgf@nodecallback{#3}%
    }%
  }%
}


\def\pgf@shift@node#1#2{%
  % This internal command shifts the recorded coordinates for node #1
  % by the vector #2. It is used to
  % correct the position of the node if the recorded coordinate
  % happens to be wrong
  {%
    \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
    \pgf@process{#2}%
    \advance\pgf@pt@x by\pgf@x%
    \advance\pgf@pt@y by\pgf@y%
    \pgfgettransform{\pgf@temp}%
    \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  }%
}

\let\pgf@nodecallback=\pgfutil@gobble



% Creates a node
%
% #1 = shape type
% #2 = anchor
% #3 = normal TeX text
% #4 = name for later reference
% #5 = path usage command
%
% Description:
%
% This command draws a shape that has previously been defined using
% \pgfdeclareshape. The shape is shifted such that the anchor is at
% the origin. In order to transform the whole shape, you should setup
% pgf's transformation matrix prior to calling this command.
%
% Example:
%
% \pgftransformshift{\pgfpoint{1cm}{1cm}}
% \pgfnode{rectangle}{center}{Hello}{hellonode}{\pgfusepath{stroke}}

\def\pgfnode#1#2#3#4#5{%
  {%
    \setbox\pgfnodeparttextbox=\hbox%
    {%
      \pgfinterruptpicture%
        {#3}%
      \endpgfinterruptpicture%
    }%
    \pgfmultipartnode{#1}{#2}{#4}{#5}%
  }
}  

% Alias a node
%
% #1 = new node name
% #2 = existing node name
%
% Description:
%
% This command allows you to subsequently access the node #2 using the
% name #1.
%
% Example:
%
% \pgfnode{rectangle}{center}{Hallo}{hellonode}{}
% \pgfnodealias{mynode}{hellonode}

\def\pgfnodealias#1#2{%
  \pgf@node@gnamelet{pgf@sh@ns@#1}{pgf@sh@ns@#2}%
  \pgf@node@gnamelet{pgf@sh@np@#1}{pgf@sh@np@#2}%
  \pgf@node@gnamelet{pgf@sh@nt@#1}{pgf@sh@nt@#2}%
  \pgf@node@gnamelet{pgf@sh@pi@#1}{pgf@sh@pi@#2}%
  \pgf@node@gnamelet{pgf@sh@ma@#1}{pgf@sh@ma@#2}%
}
\def\pgf@node@gnamelet#1#2{%
  \expandafter\let\expandafter\pgf@temp\csname #2\endcsname%
  \expandafter\global\expandafter\let\csname #1\endcsname=\pgf@temp%
}


\def\pgf@sh@resavedanchor#1#2{%
  \pgf@process{#2}%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedpoints{%
      \noexpand\def\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    }}%
  \pgf@sh@marshal%
}


\def\pgf@sh@resaveddimen#1#2{%
  {#2\global\pgf@x=\pgf@x}%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedpoints{%
      \noexpand\def\noexpand#1{\the\pgf@x}%
    }}%
  \pgf@sh@marshal%
}

% MW
\newtoks\toks@savedmacro
\def\pgf@sh@resavedmacro#1#2{%
	\let#1\pgfutil@empty%
	\def\addtosavedmacro##1{%
		\expandafter\def\expandafter\pgf@sh@addtomacro@temp\expandafter{#1\noexpand\def\noexpand##1{##1}}%
		\expandafter\toks@savedmacro\expandafter{\pgf@sh@addtomacro@temp}%
		\expandafter\def\expandafter#1\expandafter{\the\toks@savedmacro}%
	}%
  #2\relax%
  \edef\pgf@sh@marshal{%
    \noexpand\pgfutil@g@addto@macro\noexpand\pgf@sh@savedmacros{%
      \noexpand\def\noexpand#1{#1}%
    }}%
  \pgf@sh@marshal%
}

% Invoke an anchor
\def\pgf@sh@reanchor#1#2{%
  \pgfutil@ifundefined{pgf@anchor@#1@#2}%
  {%
    \pgfmathsetcounter{pgf@counta}{#2}%
    \csname pgf@anchor@#1@border\endcsname{\pgfqpointpolar{\c@pgf@counta}{1pt}}%
  }%
  {\csname pgf@anchor@#1@#2\endcsname}%
}



% Retrieves an anchor of a shape
%
% #1 = name
% #2 = anchor or a number (corresponding to a degree)
%
% Description:
%
% This command yields a point at the anchor of the given named shape.
%
% Example:
%
% \pgfshape{rectangle}{center}{Hello}{hellonode}{\pgfusepath[stroke]}
% \pgfpathmoveto{\pgfpointanchor{hellonode}{center}}

\def\pgfpointanchor#1#2{%
  % Ok, check whether #1 is known!
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {\PackageError{pgf}{No shape named #1 is known}{}%
    \pgfpointorigin}%
  {%
    \pgf@process{%
      % MW install special macros
      \csname pgf@sh@ma@#1\endcsname% MW
      % install special coordinates
      \csname pgf@sh@np@#1\endcsname
      \pgf@sh@reanchor{\csname pgf@sh@ns@#1\endcsname}{#2}%
      {%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgf@pos@transform{\pgf@x}{\pgf@y}%
        \global\pgf@x=\pgf@x%
        \global\pgf@y=\pgf@y%
      }%
      % Add inter picture transformation
      \pgf@shape@interpictureshift{#1}%
      % Undo current transformation
      \pgftransforminvert%
      \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }%
}

\def\pgf@shape@interpictureshift#1{%
  \expandafter\ifx\csname pgf@sh@pi@#1\endcsname\pgfpictureid%
  \else%
    \pgfsys@getposition{\csname pgf@sh@pi@#1\endcsname}\pgf@shape@original@pos%
    \pgfsys@getposition{\pgfpictureid}\pgf@shape@current@pos%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgfpointorigin\pgf@shape@current@pos}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \pgf@process{\pgfpointorigin\pgf@shape@original@pos}%
    \advance\pgf@xa by\pgf@x%
    \advance\pgf@ya by\pgf@y%
    \pgf@x=\pgf@xa%
    \pgf@y=\pgf@ya%
  \fi%
}



% Retrieves a border point of a shape
%
% #1 = name
% #2 = another point
%
% Description:
%
% This command yields a point on the border of the shape that is on a
% straight line from the center to the point #2.
%
% Example:
%
% \pgfshape{rectangle}{center}{Hello}{hellonode}{\pgfusepath[stroke]}
% \pgfpathmoveto{\pgfpointshapeborder{hellonode}{\pgfpoint{2cm}{1cm}}
% \pgfpathlineto{\pgfpoint{2cm}{1cm}}
% \pgfusepath{stroke}

\def\pgfpointshapeborder#1#2{%
  % Ok, check whether #1 is known!
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {\PackageError{pgf}{No shape named #1 is known}{}%
    \pgfpointorigin}%
  {%
    \pgf@process{%
      % MW install special macros
      \csname pgf@sh@ma@#1\endcsname% MW
      % install special coordinates
      \csname pgf@sh@np@#1\endcsname%
      {%
        \pgf@process{\pgfpointtransformed{#2}}%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgftransforminvert%
        \pgf@pos@transform{\pgf@x}{\pgf@y}%
        \pgf@xa=\pgf@x%
        \pgf@ya=\pgf@y%
        \pgf@process{\csname pgf@anchor@\csname pgf@sh@ns@#1\endcsname @center\endcsname}%
        \pgf@process{\pgf@shape@interpictureshift{#1}}%%
        \advance\pgf@xa by-\pgf@x%
        \advance\pgf@ya by-\pgf@y%
        \csname pgf@anchor@\csname pgf@sh@ns@#1\endcsname @border\endcsname{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
        \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
        \pgf@pos@transform{\pgf@x}{\pgf@y}%
        \global\pgf@x=\pgf@x%
        \global\pgf@y=\pgf@y%
      }%
      % Add inter picture transformation
      \pgf@shape@interpictureshift{#1}%
      % Undo current transformation
      \pgftransforminvert%
      \pgf@pos@transform{\pgf@x}{\pgf@y}%
    }%
  }%
}



% Declares a shape type
%
% #1 = shape type
% #2 = shape specification
%
% Description:
%
% This command declares a new shape type. The shape specification
% should contain the following commands:
%
% - \savedanchor
%   This command takes two arguments: a name and some code. The point
%   specified by the code (the \pgf@x and \pgf@y values resulting from
%   executing the code, to be precise), will be stored under the given
%   name. Whenever, later on, an anchor is invoked these stored points
%   will be available. The \saveddimen works like \savedanchor, only a
%   single dimension is stored (taken from \pgf@x).
%   When a savedanchor is calculated, the height/width/depth of the
%   boxes mentioned in \nodeparts can be used.
%
% - \anchor
%   Specifies an anchor. This command takes two arguments: an anchor
%   name and some code for computing the anchor. When the anchor
%   computation starts, all shape points and shape dimension will be
%   setup.
%
% - \anchorborder
%   This command should compute a point on the border of the
%   shape. When the code is called, \pgf@x and \pgf@y will have been
%   preinitialised with a direction.
%
% - \behindbackgroundpath
%   Some things to be draw behind everything.
%
% - \backgroundpath
%   A path that is drawn behind the main box. How this path is used
%   depends on how \pgfshape is called.
%
% - \beforebackgroundpath
%   Some things to be draw before the background path, but behind the
%   main box.
%
% - \behindforegroundpath
%   Some things to be draw on top of the main box.
%
% - \foregroundpath
%   A path that is drawn on top of all of the above. How this path is
%   used depends on how \pgfshape is called.
%
% - \beforeforegroundpath
%   Some things to be draw before everything.
%
% - \nodeparts
%   List of node parts that make up the shape. For each entry XYZ in
%   the list there must be a box named \pgfnodepartXYZbox (possibly
%   ``redirected'' to some different box using \let). Each such box
%   will be placed at the anchor XYZ.
%   By default, \nodeparts is just {text}. Thus, there will be one
%   node part box named \pgfnodeparttextbox and this node will be
%   placed at the anchor text. 
%   
%
% Example:
%
% See the definition of rectangle, below.

\long\def\pgfdeclareshape#1#2{%
  {
    \def\shape@name{#1}
    \let\savedanchor=\pgf@sh@savedanchor
    \let\saveddimen=\pgf@sh@saveddimen
    \let\savedmacro=\pgf@sh@savedmacro% MW
    \let\anchor=\pgf@sh@anchor
    \let\anchorborder=\pgf@sh@anchorborder
    \let\behindbackgroundpath=\pgf@sh@behindbgpath
    \let\backgroundpath=\pgf@sh@bgpath
    \let\beforebackgroundpath=\pgf@sh@beforebgpath
    \let\behindforegroundpath=\pgf@sh@behindfgpath
    \let\foregroundpath=\pgf@sh@fgpath
    \let\beforeforegroundpath=\pgf@sh@beforefgpath
    \let\nodeparts=\pgf@sh@boxes
    \let\inheritsavedanchors=\pgf@sh@inheritsavedanchors
    \let\inheritanchor=\pgf@sh@inheritanchor
    \let\inheritanchorborder=\pgf@sh@inheritanchorborder
    \let\inheritbehindbackgroundpath=\pgf@sh@inheritbehindbgpath
    \let\inheritbackgroundpath=\pgf@sh@inheritbgpath
    \let\inheritbeforebackgroundpath=\pgf@sh@inheritbeforebgpath
    \let\inheritbehindforegroundpath=\pgf@sh@inheritbehindfgpath
    \let\inheritforegroundpath=\pgf@sh@inheritfgpath
    \let\inheritbeforeforegroundpath=\pgf@sh@inheritbeforefgpath
    \let\inheritnodeparts=\pgf@sh@inheritboxes
    \anchorborder{\csname pgf@anchor@#1@center\endcsname}%
    \anchor{text}{\pgfpointorigin}%
    \nodeparts{text}%
    \expandafter\global\expandafter\let\csname pgf@sh@s@\shape@name\endcsname=\pgfutil@empty%
    #2
  }
}

\def\pgf@sh@savedanchor#1#2{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\shape@name\endcsname{\pgf@sh@resavedanchor{#1}{#2}}}
\def\pgf@sh@saveddimen#1#2{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\shape@name\endcsname{\pgf@sh@resaveddimen{#1}{#2}}}
 \def\pgf@sh@savedmacro#1#2{% MW
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\shape@name\endcsname{\pgf@sh@resavedmacro{#1}{#2}}}% MW
\def\pgf@sh@anchor#1#2{\expandafter\gdef\csname pgf@anchor@\shape@name @#1\endcsname{#2}}
\def\pgf@sh@anchorborder#1{\expandafter\gdef\csname pgf@anchor@\shape@name @border\endcsname##1{\pgf@process{##1}#1}}
\long\def\pgf@sh@behindbgpath#1{\expandafter\gdef\csname pgf@sh@bbg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@bgpath#1{\expandafter\gdef\csname pgf@sh@bg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@beforebgpath#1{\expandafter\gdef\csname pgf@sh@fbg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@behindfgpath#1{\expandafter\gdef\csname pgf@sh@bfg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@fgpath#1{\expandafter\gdef\csname pgf@sh@fg@\shape@name\endcsname{#1}}
\long\def\pgf@sh@beforefgpath#1{\expandafter\gdef\csname pgf@sg@ffg@\shape@name\endcsname{#1}}
\def\pgf@sh@boxes#1{\expandafter\gdef\csname pgf@sh@boxes@\shape@name\endcsname{#1}}

\def\pgf@sh@inheritsavedanchors[from=#1]{%
  \expandafter\pgfutil@g@addto@macro\csname pgf@sh@s@\shape@name\endcsname{\csname pgf@sh@s@#1\endcsname}}
  
 \def\pgf@sh@inheritanchor[from=#1]#2{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@anchor@\shape@name @#2\endcsname=\expandafter\noexpand\csname
    pgf@anchor@#1@#2\endcsname}%
  \pgf@marshal%
}
\def\pgf@sh@inheritanchorborder[from=#1]{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@anchor@\shape@name @border\endcsname=\expandafter\noexpand\csname
    pgf@anchor@#1@border\endcsname}%
  \pgf@marshal%
}
\def\pgf@sh@inheritor#1#2{%
  \edef\pgf@marshal{\global\let\expandafter\noexpand\csname
    pgf@sh@#1@\shape@name\endcsname=\expandafter\noexpand\csname
    pgf@sh@#1@#2\endcsname}%
  \pgf@marshal%
}
\def\pgf@sh@inheritbehindbgpath[from=#1]{\pgf@sh@inheritor{bbg}{#1}}
\def\pgf@sh@inheritbgpath[from=#1]{\pgf@sh@inheritor{bg}{#1}}
\def\pgf@sh@inheritbeforebgpath[from=#1]{\pgf@sh@inheritor{fbg}{#1}}
\def\pgf@sh@inheritbehindfgpath[from=#1]{\pgf@sh@inheritor{bfg}{#1}}
\def\pgf@sh@inheritfgpath[from=#1]{\pgf@sh@inheritor{fg}{#1}}
\def\pgf@sh@inheritbeforefgpath[from=#1]{\pgf@sh@inheritor{ffg}{#1}}
\def\pgf@sh@inheritboxes[from=#1]{\pgf@sh@inheritor{boxes}{#1}}



% 
% Coordinate. This shape is special: It is only used to reference a
% point for later usage. Nothing is drawn, all anchors are identical
% to the center. 
%

\pgfdeclareshape{coordinate}
{
  \savedanchor\centerpoint{%
    % x
    \pgf@x=.5\wd\pgfnodeparttextbox%
    % y
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by -.5\dp\pgfnodeparttextbox%
  }
  
  \anchor{center}{\centerpoint}
  \anchor{north}{\centerpoint}
  \anchor{north west}{\centerpoint}
  \anchor{north east}{\centerpoint}
  \anchor{center}{\centerpoint}
  \anchor{west}{\centerpoint}
  \anchor{east}{\centerpoint}
  \anchor{mid}{\centerpoint}
  \anchor{mid west}{\centerpoint}
  \anchor{mid east}{\centerpoint}
  \anchor{base}{\centerpoint}
  \anchor{base west}{\centerpoint}
  \anchor{base east}{\centerpoint}
  \anchor{south}{\centerpoint}
  \anchor{south west}{\centerpoint}
  \anchor{south east}{\centerpoint}
  \anchorborder{\centerpoint}

  \nodeparts{}% no text
}


% Value keys for shapes:
%
% /pgf/inner xsep     : recommended inner x separation
% /pgf/inner ysep     : recommended inner y separation
% /pgf/outer xsep     : recommended outer x separation
% /pgf/outer ysep     : recommended outer y separation
% /pgf/minimum width  : recommended minimum width
% /pgf/minimum height : recommended minimum height

\pgfset{
  inner xsep/.initial     =.3333em,
  inner ysep/.initial     =.3333em,
  inner sep/.style        ={/pgf/inner xsep=#1,/pgf/inner ysep=#1},
  outer xsep/.initial     =.5\pgflinewidth,
  outer ysep/.initial     =.5\pgflinewidth,
  outer sep/.style        ={/pgf/outer xsep=#1,/pgf/outer ysep=#1},
  minimum width/.initial  =1pt,
  minimum height/.initial =1pt,
  minimum size/.style     ={/pgf/minimum width=#1,/pgf/minimum height=#1},
}

% Keys for rotating the shape border.
% (may not be supported by all shapes)
%
% /pgf/shape border uses incircle : Calculate the shape border using the incircle 
%                                   around the node contents (+inner sep).
%						
% /pgf/shape border rotate        : Angle of independent border rotation.

\newif\ifpgfshapeborderusesincircle
\pgfkeys{/pgf/shape border uses incircle/.is if=pgfshapeborderusesincircle}
\pgfkeys{/pgf/shape border rotate/.initial=0}

% 
% Rectangle
%

\pgfdeclareshape{rectangle}
{
  \savedanchor\northeast{%
    % Calculate x
    %
    % First, is width < minimum width?
    \pgf@x=\the\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@x by 2\pgf@xc%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
    \ifdim\pgf@x<\pgf@xb%
      % yes, too small. Enlarge...
      \pgf@x=\pgf@xb%
    \fi%
    % Now, calculate right border: .5\wd\pgfnodeparttextbox + .5 \pgf@x + outer sep
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
    \advance\pgf@x by\pgf@xa%
    % Calculate y
    %
    % First, is height+depth < minimum height?
    \pgf@y=\ht\pgfnodeparttextbox%
    \advance\pgf@y by\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@y by 2\pgf@yc%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
    \ifdim\pgf@y<\pgf@yb%
      % yes, too small. Enlarge...
      \pgf@y=\pgf@yb%
    \fi%
    % Now, calculate upper border: .5\ht-.5\dp + .5 \pgf@y + outer sep
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
    \advance\pgf@y by.5\ht\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
    \advance\pgf@y by\pgf@ya%
  }
    
  \savedanchor\southwest{%
      % Calculate x
      %
      % First, is width < minimum width?
      \pgf@x=\wd\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/pgf/inner xsep}}%
      \advance\pgf@x by 2\pgf@xc%
      \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/minimum width}}%
      \ifdim\pgf@x<\pgf@xb%
        % yes, too small. Enlarge...
        \pgf@x=\pgf@xb%
      \fi%
      % Now, calculate left border: .5\wd\pgfnodeparttextbox - .5 \pgf@x - outer sep
      \pgf@x=-.5\pgf@x%
      \advance\pgf@x by.5\wd\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/outer xsep}}%
      \advance\pgf@x by-\pgf@xa%
      % Calculate y
      %
      % First, is height+depth < minimum height?
      \pgf@y=\ht\pgfnodeparttextbox%
      \advance\pgf@y by\dp\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@yc{\pgfkeysvalueof{/pgf/inner ysep}}%
      \advance\pgf@y by 2\pgf@yc%
      \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/minimum height}}%
      \ifdim\pgf@y<\pgf@yb%
        % yes, too small. Enlarge...
        \pgf@y=\pgf@yb%
      \fi%
       % Now, calculate upper border: .5\ht-.5\dp - .5 \pgf@y - outer sep
      \pgf@y=-.5\pgf@y%
      \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
      \advance\pgf@y by.5\ht\pgfnodeparttextbox%
      \pgfmathsetlength\pgf@ya{\pgfkeysvalueof{/pgf/outer ysep}}%
      \advance\pgf@y by-\pgf@ya%
  }

  %
  % Anchors
  % 
  \anchor{center}{
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \pgf@y=.5\pgf@y%
    \advance\pgf@x by \pgf@xa%
    \advance\pgf@y by \pgf@ya%
  }
  \anchor{mid}{\pgf@anchor@rectangle@center\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base}{\pgf@anchor@rectangle@center\pgf@y=0pt}
  \anchor{north}{
    \pgf@process{\southwest}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\northeast}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
  }
  \anchor{south}{
    \pgf@process{\northeast}%
    \pgf@xa=.5\pgf@x%
    \pgf@process{\southwest}%
    \pgf@x=.5\pgf@x%
    \advance\pgf@x by \pgf@xa%
  }
  \anchor{west}{
    \pgf@process{\northeast}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\southwest}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
  }
  \anchor{mid west}{\southwest\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base west}{\southwest\pgf@y=0pt}
  \anchor{north west}{
    \southwest
    \pgf@xa=\pgf@x
    \northeast
    \pgf@x=\pgf@xa}
  \anchor{south west}{\southwest}
  \anchor{east}{%
    \pgf@process{\southwest}%
    \pgf@ya=.5\pgf@y%
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
    \advance\pgf@y by \pgf@ya%
  }
  \anchor{mid east}{\northeast\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base east}{\northeast\pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{south east}{
    \northeast
    \pgf@xa=\pgf@x
    \southwest
    \pgf@x=\pgf@xa
  }
  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }

  %
  % Background path
  %
  \backgroundpath{
    \pgfpathrectanglecorners
    {\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}
    {\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
  }
}



% Special  current bounding box  rectangle:
\expandafter\def\csname pgf@sh@ns@current bounding box\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current bounding box\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@picminx}{\pgf@picminy}}%
  \def\northeast{\pgfqpoint{\pgf@picmaxx}{\pgf@picmaxy}}%
}
\expandafter\def\csname pgf@sh@nt@current bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
\expandafter\def\csname pgf@sh@pi@current bounding box\endcsname{\pgfpictureid}


% Special  current path bounding box  rectangle:
\expandafter\def\csname pgf@sh@ns@current path bounding box\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current path bounding box\endcsname{%
  \def\southwest{\pgfqpoint{\pgf@pathminx}{\pgf@pathminy}}%
  \def\northeast{\pgfqpoint{\pgf@pathmaxx}{\pgf@pathmaxy}}%
}
\expandafter\def\csname pgf@sh@nt@current path bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
\expandafter\def\csname pgf@sh@pi@current path bounding box\endcsname{\pgfpictureid}


% Special  current page bounding box rectangle:
\expandafter\def\csname pgf@sh@ns@current page\endcsname{rectangle}
\expandafter\def\csname pgf@sh@np@current page\endcsname{%
  \def\southwest{\pgfqpoint{0pt}{0pt}}%
  \def\northeast{\pgfqpoint{\paperwidth}{\paperheight}}%
}
\expandafter\def\csname pgf@sh@nt@current page\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
\expandafter\def\csname pgf@sh@pi@current page\endcsname{pgfpageorigin}


% Special scope bounding box rectangle:
\pgfkeys{/pgf/local bounding box/.code={%
    \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
    \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
      \def\southwest{\pgfqpoint{\csname pgf@lbb@minx@#1\endcsname}{\csname pgf@lbb@miny@#1\endcsname}}%
      \def\northeast{\pgfqpoint{\csname pgf@lbb@maxx@#1\endcsname}{\csname pgf@lbb@maxy@#1\endcsname}}%
    }
    \expandafter\gdef\csname pgf@sh@nt@#1\endcsname{{1}{0}{0}{1}{0pt}{0pt}}
    \expandafter\gdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}
    \expandafter\gdef\csname pgf@lbb@maxx@#1\endcsname{-16000pt}%
    \expandafter\gdef\csname pgf@lbb@minx@#1\endcsname{16000pt}%
    \expandafter\gdef\csname pgf@lbb@maxy@#1\endcsname{-16000pt}%
    \expandafter\gdef\csname pgf@lbb@miny@#1\endcsname{16000pt}%
    \pgf@size@hookedtrue%
    \expandafter\def\expandafter\pgf@path@size@hook\expandafter{\pgf@path@size@hook\pgf@lbb@do{#1}}
  }%
}
\def\pgf@lbb@do#1{%
  \ifdim\pgf@size@hook@x<\csname pgf@lbb@minx@#1\endcsname\expandafter\xdef\csname pgf@lbb@minx@#1\endcsname{\the\pgf@size@hook@x}\fi%
  \ifdim\pgf@size@hook@x>\csname pgf@lbb@maxx@#1\endcsname\expandafter\xdef\csname pgf@lbb@maxx@#1\endcsname{\the\pgf@size@hook@x}\fi%
  \ifdim\pgf@size@hook@y<\csname pgf@lbb@miny@#1\endcsname\expandafter\xdef\csname pgf@lbb@miny@#1\endcsname{\the\pgf@size@hook@y}\fi%
  \ifdim\pgf@size@hook@y>\csname pgf@lbb@maxy@#1\endcsname\expandafter\xdef\csname pgf@lbb@maxy@#1\endcsname{\the\pgf@size@hook@y}\fi%
}

%
% Circle
%

\pgfdeclareshape{circle}
%
% Draws a circle around the text
%
{
  \savedanchor\centerpoint{%
    \pgf@x=.5\wd\pgfnodeparttextbox%
    \pgf@y=.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by-.5\dp\pgfnodeparttextbox%
  }
    
  \saveddimen\radius{%
    % 
    % Caculate ``height radius''
    % 
    \pgf@ya=.5\ht\pgfnodeparttextbox%
    \advance\pgf@ya by.5\dp\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@yb{\pgfkeysvalueof{/pgf/inner ysep}}%
    \advance\pgf@ya by\pgf@yb%
    % 
    % Caculate ``width radius''
    % 
    \pgf@xa=.5\wd\pgfnodeparttextbox%
    \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/inner xsep}}%
    \advance\pgf@xa by\pgf@xb%
    % 
    % Calculate length of radius vector:
    % 
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \ifdim\pgf@x>\pgf@y%
        \c@pgf@counta=\pgf@x%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@xa=16\pgf@xa\relax%
          \divide\pgf@xa by\c@pgf@counta%
          \pgf@xa=16\pgf@xa\relax%
        \fi%
      \else%
        \c@pgf@counta=\pgf@y%
        \ifnum\c@pgf@counta=0\relax%
        \else%
          \divide\c@pgf@counta by 255\relax%
          \pgf@ya=16\pgf@ya\relax%
          \divide\pgf@ya by\c@pgf@counta%
          \pgf@xa=16\pgf@ya\relax%
        \fi%
    \fi%
    \pgf@x=\pgf@xa%
    % 
    % If necessary, adjust radius so that the size requirements are
    % met: 
    % 
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/minimum width}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/minimum height}}%  
    \ifdim\pgf@x<.5\pgf@xb%
        \pgf@x=.5\pgf@xb%
    \fi%
    \ifdim\pgf@x<.5\pgf@yb%
        \pgf@x=.5\pgf@yb%
    \fi%
    % 
    % Now, add larger of outer sepearations.
    % 
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgf@x by\pgf@yb%
    \else%
      \advance\pgf@x by\pgf@xb%
    \fi%
  }

  %
  % Anchors
  % 
  \anchor{center}{\centerpoint}
  \anchor{mid}{\centerpoint\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base}{\centerpoint\pgf@y=0pt}
  \anchor{north}{\centerpoint\advance\pgf@y by\radius}
  \anchor{south}{\centerpoint\advance\pgf@y by-\radius}
  \anchor{west}{\centerpoint\advance\pgf@x by-\radius}
  \anchor{east}{\centerpoint\advance\pgf@x by\radius}
  \anchor{mid west}{\centerpoint\advance\pgf@x by-\radius\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{mid east}{\centerpoint\advance\pgf@x by\radius\pgfmathsetlength\pgf@y{.5ex}}
  \anchor{base west}{\centerpoint\advance\pgf@x by-\radius\pgf@y=0pt}
  \anchor{base east}{\centerpoint\advance\pgf@x by\radius\pgf@y=0pt}
  \anchor{north west}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@xa
  }
  \anchor{south west}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by-0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@xa
  }
  \anchor{north east}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by0.707107\pgf@xa
  }
  \anchor{south east}{
    \centerpoint
    \pgf@xa=\radius
    \advance\pgf@x by0.707107\pgf@xa
    \advance\pgf@y by-0.707107\pgf@xa
  }
  \anchorborder{
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderellipse
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
      {\noexpand\pgfqpoint{\radius}{\radius}}%
    }%
    \pgf@marshal%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \centerpoint%
    \advance\pgf@x by\pgf@xa%
    \advance\pgf@y by\pgf@ya%
  }

  %
  % Background path
  %
  \backgroundpath{
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
  }
}





\endinput


==> pgfmodulesnakes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/modules/pgfmodulesnakes.code.tex,v 1.2 2008/01/17 20:09:17 tantau Exp $

\PackageWarning{pgf}{Snakes have been superseded by decorations. Use
the module decorations instead of snakes}

\usepgfmodule{decorations}

\endinput



\newdimen\pgfsnakeremainingdistance
\newdimen\pgfsnakecompleteddistance


% Creates a new pgf snake
%
% #1 = snake name
% #1 = initial state
% #3 = states of the snake
%
%
% This command declares a new snake for later use. The second
% parameter specifies the states of the snake, see also the
% description of pgfpathsnake.
%
% Inside the code of #3 the command \state may be used. This command
% will only be defined while #3 is executed.
%
% Example:
%
% \pgfdeclaresnake{zig zag}{one zig zag}
% {
%   \state{one zig zag}[width=10pt]
%   {
%     \pgfpathlineto{\pgfpoint{2.5pt}{2.5pt}}
%     \pgfpathlineto{\pgfpoint{7.5pt}{-2.5pt}}
%     \pgfpathlineto{\pgfpoint{10pt}{0pt}}
%   }
%   \state{final}
%   {
%     \pgfpathlineto{\pgfpoint{\pgfsnakeremainingdistance}{0pt}}
%   }
% }

\long\def\pgfdeclaresnake#1#2#3{%
  \def\pgf@snake@name{#1}%
  \pgfutil@namedef{pgf@snake@@#1@initial}{#2}%
  \let\pgf@orig@state=\state%
  \let\state=\pgf@snake@state
  #3
  \let\state=\pgf@orig@state%
}


% Sets the additional transformation applied to every segment of a snake
%
% #1 = transformation
%
% Example:
%
% \pgfsetsnakesegmenttransformation{\pgftransformyshift{5pt}}

\def\pgfsetsnakesegmenttransformation#1{\def\pgf@snakeadditionaltransform{#1}}
\pgfsetsnakesegmenttransformation{}


% Declares a new state
%
% #1 = state name
% #2 = options
% #3 = path element
%
% Description:
%
% When a snake is drawn and the current state is #1, the following
% happens. First, the options are executed, which will possible change
% the state. If that does not happen, the path element is added to the
% path and the coordinate system is translated by the path element's
% width (which is specified using the width option).
%
% Example:
%
% \state{initial}[width=10pt]
% {
%   \pgfpathlineto{\pgfpoint{2.5pt}{2.5pt}}
%   \pgfpathlineto{\pgfpoint{7.5pt}{-2.5pt}}
%   \pgfpathlineto{\pgfpoint{10pt}{0pt}}
% }

\def\pgf@snake@state#1{\pgfutil@ifnextchar[{\pgf@@snake@start#1}{\pgf@@snake@start#1[]}}%}
\def\pgf@@snake@start#1[#2]#3{%
  \pgfutil@namedef{pgf@snake@@\pgf@snake@name @#1@options}{#2}%
  \pgfutil@namedef{pgf@snake@@\pgf@snake@name @#1@code}{#3}%
}



% Use multiple snakes
%
% #1 = list of snake names/length pairs
% #2 = point to which the snake leads
%
% This operation uses the snakes in parameter #1 to get to the point
% #4. The parameter #1 should contain pairs consisting of a snake name
% and a length for which this snake should be used. When the length is
% computed, the dimensions \pgfsnakeremainingdistance and
% \pgfsnakecompleteddistance will have been set to the length of the
% total distance to #2 that has already been covered/that still needs
% to be covered.
%
% Example:
%
% \pgfpathsnakesto{{lineto}{1cm},{zig zag}{\pgfsnakeremainingdistance}}{\pgfpoint{2cm}{3cm}}

\def\pgfpathsnakesto#1#2{%
  \begingroup%
    % compute target vector
    \pgfpointtransformed{#2}%
    \advance\pgf@x by-\pgf@path@lastx%
    \advance\pgf@y by-\pgf@path@lasty%
    %
    % MW: Calculate the angle of the snake.
    %
    \edef\pgf@marshal{%
    	\noexpand\pgfmathanglebetweenpoints{\noexpand\pgfpointorigin}{%
    		\noexpand\pgf@x\the\pgf@x\noexpand\pgf@y\the\pgf@y}%
    }%
    \pgf@marshal%
    \let\pgfsnakeangle\pgfmathresult%
    %
    % MW: Use this instead for length (?). More accurate and only a few operations slower.
    %
    \pgfmathveclen@{\pgfmath@tonumber{\pgf@x}}{\pgfmath@tonumber{\pgf@y}}%
    \pgfsnakeremainingdistance\pgfmathresult pt\relax%
    %
    % Ok, now normalize the vector...
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgfpointnormalised{}}%
    % ok, now computer length (arghh...)
    % In theory that's easy: divide the larger of the values x or y by
    % the normalized x or y. Well...
    %
    % First, make xa and ya positive:
   % \ifdim\pgf@xa<0pt%
%      \pgf@xa=-\pgf@xa%
%    \fi%
%    \ifdim\pgf@ya<0pt%
%      \pgf@ya=-\pgf@ya%
%    \fi%
%    % Now do division:
%    \ifdim\pgf@xa>\pgf@ya%
%      \c@pgf@counta=\pgf@x%
%      \ifnum\c@pgf@counta=0\relax%
%      \else%
%        \divide\c@pgf@counta by 255\relax%
%        \pgf@xa=16\pgf@xa\relax%
%        \divide\pgf@xa by\c@pgf@counta%
%        \pgf@xa=16\pgf@xa\relax%
%      \fi%
%    \else%
%      \c@pgf@counta=\pgf@y%
%      \ifnum\c@pgf@counta=0\relax%
%      \else%
%        \divide\c@pgf@counta by 255\relax%
%        \pgf@ya=16\pgf@ya\relax%
%        \divide\pgf@ya by\c@pgf@counta%
%        \pgf@xa=16\pgf@ya\relax%
%      \fi%
%    \fi%
%    % Make positive:
%    \ifdim\pgf@xa<0pt%
%      \pgf@xa=-\pgf@xa%
%    \fi%
%    % Ok, now we draw things...
    \edef\pgf@list{#1}%
%   \pgfsnakeremainingdistance=\pgf@xa%
    \pgfsnakecompleteddistance=0pt%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgfutil@for\pgf@temp:=\pgf@list\do{%
      \ifx\pgf@temp\pgfutil@empty%
      \else%
        \expandafter\pgf@snake@invoke\pgf@temp%
      \fi%
    }%
  \endgroup%
}

\def\pgf@snake@invoke#1#2{%
  \pgfmathsetlength\pgf@xa{#2}%
  {%
    \edef\pgf@marshal{\noexpand\pgfpathsnakealongvector{#1}{\the\pgf@xa}{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}}%
    \pgf@marshal%
  }%
  \advance\pgfsnakecompleteddistance by\pgf@xa%
  \advance\pgfsnakeremainingdistance by-\pgf@xa%
}

% Use a snake
%
% #1 = snake name
% #2 = point to which the snake leads
%
% This operation mainly computes \pgfpathsnakealongvector for a vector
% appropriately choosen. See \pgfpathsnakealongvector for details.
%
% Example:
%
% \pgfpathsnaketo{zig zag}{\pgfpoint{2cm}{3cm}}

\def\pgfpathsnaketo#1#2{\pgfpathsnakesto{{#1}{\pgfsnakeremainingdistance}}{#2}}



% Use a snake
%
% #1 = snake name
% #2 = length of the snake
% #3 = vector along which the snake grows, should have unit length.
%
% This command draws a snake (more precisely, it adds a snake to the
% path). This works as follows:
%
% First, the coordinate system is transformed such that the vector #3
% points to the right.
%
% Next, the state `initial' of the snake is entered. Unless the
% options of this state cause it to switch to another state, the path
% element is added to the path. Then, the coordinate system is
% translated by the width of the path element as specified in the
% width option of the path element. The dimensions
% \pgfsnakeremainingdistance and \pgfsnakecompleteddistance are
% updated. 
%
% The process ends when the state `final' is entered. The code of the
% final state is executed and the process stops.
%
% Example:
%
% \pgfpathsnakealongvector{zig zag}{100pt}{\pgfpolar{30}{1pt}}

\def\pgfpathsnakealongvector#1#2#3{%
  \pgfutil@ifundefined{pgf@snake@@#1@initial}{\PackageError{pgf}{Undefined snake ``#1''}{}}
  { 
  \begingroup% keep things local
    \pgftransformreset%
    \pgf@pt@x=\pgf@path@lastx% evil trickery to transform to the last point
    \pgf@pt@y=\pgf@path@lasty%
    \pgf@process{#3}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@xb=-\pgf@y%
    \pgf@yb=\pgf@x%
    \pgftransformcm
      {\pgf@sys@tonumber{\pgf@xa}}{\pgf@sys@tonumber{\pgf@ya}}
      {\pgf@sys@tonumber{\pgf@xb}}{\pgf@sys@tonumber{\pgf@yb}}
      {\pgfpointorigin}%
    % Now, setup the automaton
    \expandafter\let\expandafter\pgf@snake@current@state\expandafter=\csname pgf@snake@@#1@initial\endcsname%
    \def\pgf@snake@name{#1}%  
    \pgfsnakecompleteddistance=0pt%  
    \pgfmathsetlength\pgfsnakeremainingdistance{#2}%
    \pgf@snake@run%
    % Last step:
    {%
      \pgftransformxshift{\pgfsnakecompleteddistance}%
      \pgf@snakeadditionaltransform%
      \csname pgf@snake@@#1@final@code\endcsname%
    }%
  \endgroup%
  }%
}

\def\pgf@final@text{final}

\def\pgf@snake@run{%
  \let\pgf@snake@next=\pgf@snake@do@state%
  \ifx\pgf@snake@current@state\pgf@final@text%
    \let\pgf@snake@next=\relax%
  \fi%
  \pgf@snake@next%  
}

\def\pgf@snake@do@state{%
  \let\pgf@snake@next=\relax%
  \let\pgf@snake@next@state=\pgf@snake@current@state%
  % execute options
  \expandafter\expandafter\expandafter\pgf@snakes@setter
  \expandafter\expandafter\expandafter{\csname pgf@snake@@\pgf@snake@name @\pgf@snake@current@state @options\endcsname}%
  \ifx\pgf@snake@next\relax%
    \let\pgf@snake@next=\pgf@snake@do@code%
  \fi%
  \pgf@snake@next%
}
\def\pgf@snakes@setter{%
  \pgfqkeys{/pgf/snakes}%
}

\def\pgf@snake@do@code{%
  % Ok, execute code:
  {%
    \pgftransformxshift{\pgfsnakecompleteddistance}%
    \pgf@snakeadditionaltransform%
    \csname pgf@snake@@\pgf@snake@name @\pgf@snake@current@state @code\endcsname%
  }%
  % next, do transformation and update
  \pgfmathsetlength{\pgf@xa}{\pgf@snake@width}%
  \advance\pgfsnakeremainingdistance by-\pgf@xa%
  \advance\pgfsnakecompleteddistance by\pgf@xa%
  % Next iteration:
  \let\pgf@snake@current@state=\pgf@snake@next@state%
  \pgf@snake@run%
}

\pgfkeys{
  /pgf/snakes/width/.code=\def\pgf@snake@width{#1}\pgf@snake@switch@if#1 to final\pgf@stop,%
  /pgf/snakes/switch if less than/.code=\pgf@snake@switch@if#1\pgf@stop,%
  /pgf/snakes/next state/.store in=\pgf@snake@next@state%
}

\def\pgf@snake@switch@if#1to #2\pgf@stop{%
  \ifx\pgf@snake@next\relax%
    \pgfmathsetlength\pgf@x{#1}%
    \ifdim\pgfsnakeremainingdistance<\pgf@x%
      \def\pgf@snake@current@state{#2}%
      \let\pgf@snake@next=\pgf@snake@run%
    \fi%
  \fi%
}



% lineto snake
%
% This snake simply adds a straight line. This snake is mainly useful
% in conjunction with other snakes.

\pgfdeclaresnake{lineto}{final}
{
  \state{final}
  { \pgfpathlineto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}} }
}



% moveto snake
%
% This snake simply jumps to the end. This snake, too, is mainly
% useful in conjunction with other snakes.

\pgfdeclaresnake{moveto}{final}
{
  \state{final}
  { \pgfpathmoveto{\pgfqpoint{\pgfsnakeremainingdistance}{0pt}} }
}



\endinput


==> pgfrcs.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.



% The purpose of this file is to define the command
% \ProvidesPackageRCS, which should be followed by an RCS id
% string. This command will also be available in plain TeX, where it
% prints out a message to the log.


\def\pgfversion{2.00}
\def\pgftypesetversion{\oldstylenums{2}.\oldstylenums{00}}


\ifx\pgfrcsloaded\undefined
\def\pgfrcsloaded{}

\edef\pgfrcsatcode{\the\catcode`\@}
\catcode`\@=11

% Get date and version from RCS Ids
\def\pgf@parseid $#1: #2.#3,v #4 #5/#6/#7 #8${%
  \pgf@parsercsfile$#2/$
  \def\pgf@rcssuffix{#3}
  \def\pgf@rcsrevision{#4}
  \def\pgf@rcsdate{#5/#6/#7}
}
\def\pgf@parsercsfile$#1/#2${
  \def\pgf@temp{#2}
  \ifx\pgf@temp\pgfutil@empty
    \def\pgf@rcsfile{#1}
  \else
    \pgf@parsercsfile$#2$
  \fi}

\def\ProvidesFileRCS{%
  \def\pgfrcs@marshal{\ProvidesFile{\pgf@rcsfile.\pgf@rcssuffix}}%
  \pgfrcs@parserest%
}

\def\ProvidesPackageRCS{%
  \def\pgfrcs@marshal{\ProvidesPackage{\pgf@rcsfile}}%
  \pgfrcs@parserest%
}

\def\pgfrcs@parserest{%
  \def\pgf@rcsadditional{}%
  \afterassignment\pgfrcs@checkforoptional\let\next=}

\def\pgfrcs@checkforoptional{%
  \ifx\next[%
    \let\next=\pgfrcs@getoptional%
  \else
    \let\next=\pgfrcs@package%
  \fi%
  \next}%}

\def\pgfrcs@getoptional#1] ${%
  \def\pgf@rcsadditional{#1}%
  \pgfrcs@package%
}

\def\pgfrcs@package#1${
  \pgf@parseid $#1$
  \pgfrcs@marshal[\pgf@rcsdate\space\pgf@rcsadditional\space(rcs-revision \pgf@rcsrevision)]
}

\def\ProvidesClassRCS $#1$ [#2]{%
  \pgf@parseid $#1$
  \ProvidesClass{\pgf@rcsfile}[\pgf@rcsdate\space#2\space (rcs-revision \pgf@rcsrevision)]
}

\ifx\ProvidesPackage\@undefined
  % plain tex
  \def\ProvidesPackage#1[#2]{\wlog{Loading package #1 version #2.}}
\fi

\ifx\ProvidesFile\@undefined
  % plain tex
  \def\ProvidesFile#1[#2]{\wlog{Loading file #1 version #2.}}
\fi

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/utilities/pgfrcs.code.tex,v 1.21 2008/02/20 11:00:42 tantau Exp $

\catcode`\@=\pgfrcsatcode

\fi



==> pgfrcs.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


\ifx\pgfrcsincluded\undefined
\def\pgfrcsincluded{}

\edef\pgfrcsatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfutil-common.tex
\input pgfutil-plain.def

\input pgfrcs.code.tex

\catcode`\@=\pgfrcsatcode

\fi

\endinput


==> pgfsys.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/systemlayer/pgfsys.code.tex,v 1.31 2008/02/07 19:25:41 tantau Exp $


% Load key mechanism
\input pgfkeys.code.tex

% "pgf" is a family
\pgfkeys{/pgf/.is family}
\def\pgfset{\pgfqkeys{/pgf}}

%
% The following conversion functions are used to convert from TeX
% dimensions to postscript/pdf points.
% 
{\catcode`\p=12\catcode`\t=12\gdef\Pgf@geT#1pt{#1}}

\def\pgf@sys@tonumber#1{\expandafter\Pgf@geT\the#1}

\def\pgf@sys@bp@correct#1{#1=0.99627#1}

\def\pgf@sys@bp#1{%
  {%
    \pgf@x=#1\relax%
    \pgf@x=0.99627\pgf@x%
    \edef\temp{\expandafter\Pgf@geT\the\pgf@x\space}%
    \toks@\expandafter\expandafter\expandafter{\expandafter\pgfsysprotocol@currentprotocol\temp}%
    \xdef\pgfsysprotocol@currentprotocol{\the\toks@}%
  }%
}
\def\pgf@sys@pt#1{%
  {%
    \pgf@x=#1\relax%
    \edef\temp{\expandafter\Pgf@geT\the\pgf@x\space}%
    \toks@\expandafter\expandafter\expandafter{\expandafter\pgfsysprotocol@currentprotocol\temp}%
    \xdef\pgfsysprotocol@currentprotocol{\the\toks@}%
  }%
}


% internal dimensions that are always present when pgsys is loaded.
\newdimen\pgf@x
\newdimen\pgf@y
\newdimen\pgf@xa
\newdimen\pgf@ya
\newdimen\pgf@xb
\newdimen\pgf@yb
\newdimen\pgf@xc
\newdimen\pgf@yc

% internal counters that are alwyas present when pgfsys is loaded
\newcount\c@pgf@counta
\newcount\c@pgf@countb
\newcount\c@pgf@countc
\newcount\c@pgf@countd


% The following \if decides, whether even-odd filling and clipping is
% to be used or normal the non-zero winding number rule. See the
% pdf-documentation for details on what these rules are.

\newif\ifpgfsys@eorule



% In the following dummy definitions of the pgf system commands are
% given. The individual drivers must overwrite these definitions,
% preferably all of them. If some system command is used that has not
% been overwritten, the command fails with a warning.
%
% In some cases, some pgf system commands are just shorthands for a
% series of more complicated commands. In this case, a default
% implementation is given in this file, but a driver may choose to
% overwrite this default implementation with a more effecient
% version. For example, a closestroke is the same as a closepath
% followed by a stroking, but in pdf there is a special shorthand for
% this. So, the pdf driver overwrites \pgfsys@closestroke, while the
% postscript driver does not.
%
% The commands for which default implementations are available are
% given at the end.

\def\pgf@sys@fail#1{%
  \expandafter\ifx\csname pgf@sys@fail@#1\endcsname\pgfutil@empty%
  \else%
    \expandafter\global\expandafter\let\csname pgf@sys@fail@#1\endcsname=\pgfutil@empty%
    \PackageWarning{pgf}{%
      Your graphic driver \pgfsysdriver\space does not support #1. This warning is given only once}%
  \fi%
}



\def\pgfsys@invoke{\pgf@sys@fail{invoking specials}}
% This command is used whenever some literal text needs to be inserted
% into the resulting .pdf, .ps, or .dvi file. Note that most
% \pgfsys@xxxx commands will not directly call this command, but,
% rather, use the protocolling mechanism to record their literal
% text. It is then left to the discretion of the protocolling
% mechansim to insert the literal text at some appropriate, later
% time. 
%
% This command should only be called when \pgfsys@beginpicture has
% been called previously and when the picture has not been suspended
% using \pgfsys@beginhbox.


\def\pgfsys@outerinvoke{\pgfsys@invoke}
% This command can be used to insert protocolled graphic commands
% outside any picture. This is extremely dangerous, but sometimes
% useful. By default, this command does the same as inside pictures. 



%
%
% Path construction commands
%
%

\def\pgfsys@moveto#1#2{\pgf@sys@fail{path constructions}}
% This command is used to start a path at a specific point (#1bp,#2bp)
% or to move the current point of the current path to (#1bp,#2bp)
% without drawing anything upon stroking (the current path is
% `interrupted'). 
%
% Here (and in the following) the coordinates are in TeX's big points
% (bp), unless the coordinate system has been scaled. A big point is
% 1/72 inches. Note that TeX's point pt is 1/72.27 inches.
%
% Example:
%
% \pgfsys@moveto{10}{10}
% \pgfsys@lineto{0}{0}
% \pgfsys@stroke
%
% This will draw a line from (10bp,10bp) to the origin of the picture.

\def\pgfsys@lineto#1#2{\pgf@sys@fail{path constructions}}
% Continue the current path to (#1bp,#2bp) with a line.

\def\pgfsys@curveto#1#2#3#4#5#6{\pgf@sys@fail{path constructions}}
% Continue the current path with a bezier curver to (#5bp,#6bp). The
% control points of the curve are at (#1bp,#2bp) and (#3bp,#4bp).

\def\pgfsys@rect#1#2#3#4{\pgf@sys@fail{path constructions}}
% Append a rectangle to the current path whose lower left corner is at
% (#1bp,#2bp) and whose width/height is given by (#3bp,#4bp).
%
% This command can be `mapped back' to moveto and lineto commands, but
% it is included since pdf has a special, quick version of this command.

\def\pgfsys@closepath{\pgf@sys@fail{path constructions}}
% Close the current path. This results in joining the current point of
% the path with the point specified by the last moveto
% operation. Typically, this is preferable over using lineto to the
% last point specified by a moveto, since the line starting at this
% point and the line ending at this point will be smoothly joined by
% closepath. 
%
% Example:
%
% \pgfsys@moveto{0}{0}
% \pgfsys@lineto{10}{10}
% \pgfsys@lineto{0}{10}
% \pgfsys@closepath
% \pgfsys@stroke
%
% versus
%
% \pgfsys@moveto{0}{0}
% \pgfsys@lineto{10}{10}
% \pgfsys@lineto{0}{10}
% \pgfsys@lineto{0}{0}
% \pgfsys@stroke
% 
% The difference between the above will be that in the second triangle
% the corner at the origin will be wrong; it will just be the overlay
% of two lines going in different directions, not a sharp pointed
% corner.






%
%
% Stroking and filling commands
%
%

\def\pgfsys@stroke{\pgf@sys@fail{path usage}}
% Stroke the current path (as if it were drawn with a pen). A number
% of so-called graphic state parameters influence this, which can be
% set in different ways:
%
% - linewidth
%   The `thickness' of the line. A width of 0 is the thinnest width
%   renderable on the device. On a high-resolution printer this may
%   become invisible and should be avoided. A good choice is 0.4pt,
%   which is the default.
%
% - stroke color
%   This special color is used for stroking. If it is not set, the
%   current color is used.
%
% - cap
%   The cap describes how the endings of lines a drawn. A round cap
%   adds a little half circle to these endings. A butt cap ends the
%   lines exactly at the end (or start) point without anything
%   added. A rectangular cap ends the lines like the butt cap, but the
%   lines protrude over the endpoint by the line thickness. (See also
%   the pdf or postscript manual). If the path has been closed, no cap
%   is drawn.
%
% - join
%   This describes how a bend (a join) in a path is rendered. A round
%   join draws bends using small arcs. A bevel join just draws the two
%   lines and then fills the join minimally so that it becomes
%   convex. A miter join extends the lines so that they form a single
%   sharp corner, but only up to a certain miter limit. (See the pdf
%   or postscript manual once more).
%
% - dash
%   The line may be dashed according to a dashing pattern.
%
% - clipping area
%   If a clipping area is established, only those parts of the path
%   that are inside the clipping area will be drawn.
%
% In addition to stroking a path, the path may also be used for
% clipping after it has been stroked. This will happen if the
% \pgfsys@clipnext is used prior to this command, see there for
% details.

\def\pgfsys@fill{\pgf@sys@fail{path usage}}
% This command fills the area surrounded by the current path. If the
% path has not yet been closed, it is closed prior to filling. The
% path itself is not stroked. For self-intersecting paths or paths
% consisting of multiple parts, the nonzero winding number rule is
% used to determine whether a point is inside or outside the
% path, except if \ifpgfsys@eorule holds -- in which case the even-odd
% rule should be used. (See the pdf or postscript manual for details.) 
%
% The following graphic state parameters influence the filling:
%
% - fill color
%   If the fill color is not especially set, the current color is
%   used. 
%
% - clipping area
%   If a clipping area is established, only those parts of the filling
%   area that are inside the clipping area will be drawn.
%
% In addition to filling the path, the path will also be used for
% clipping if \pgfsys@clipnext is used prior to this command.

\def\pgfsys@fillstroke{\pgf@sys@fail{path usage}}
% First, the path is filled, then the path is stroked. If the fill and
% stroke colors are the same (or if they are not specified and the
% current color is used), this yields almost the same as a
% \pgfsys@fill. However, due to the line thickness of the stroked
% path, the fillstroked area will be slightly larger.
%
% In addition to stroking and filling the path, the path will also be
% used for clipping if \pgfsys@clipnext is used prior to this command.

\def\pgfsys@clipnext{\pgf@sys@fail{path usage}}
% This command should be issued after a path has been constructed, but
% before it has been stroked and/or filled or discarded. When the
% command is used, the next stroking/filling/discarding command will
% first be executed normally. Then, afterwards, the just-used path
% will be used for subsequent clipping. If there has already been a
% clipping region, this region is intersected with the new clipping
% path (the clipping cannot get bigger). The nonzero winding number
% rule is used to determine whether a point is inside or outside the
% clipping area or the even-odd rule, depending on whether
% \ifpgfsys@eorule holds.

\def\pgfsys@discardpath{\pgf@sys@fail{path usage}}
% Normally, this command should `throw away' the current path.
% However, after \pgfsys@clipnext has been called, the current path
% should subsequently be used for clipping. See \pgfsys@clipnext for
% details. 





%
%
% Stroking options
%
%
\def\pgfsys@setlinewidth#1{\pgf@sys@fail{setting the line width}}
% Sets the width of lines, when stroked, to #1bp.

\def\pgfsys@buttcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a butt cap. See \pgfsys@stroke.

\def\pgfsys@roundcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a round cap. See \pgfsys@stroke.

\def\pgfsys@rectcap{\pgf@sys@fail{setting the line cap}}
% Sets the cap to a rectangular cap. See \pgfsys@stroke.

\def\pgfsys@miterjoin{\pgf@sys@fail{setting the line join}}
% Sets the join to a miter join. See \pgfsys@stroke.

\def\pgfsys@setmiterlimit#1{\pgf@sys@fail{setting the line cap}}
% Sets the miter limit of lines to #1. See the pdf or postscript
% documentation.

\def\pgfsys@roundjoin{\pgf@sys@fail{setting the line cap}}
% Sets the join to a round join. See \pgfsys@stroke.

\def\pgfsys@beveljoin{\pgf@sys@fail{setting the line cap}}
% Sets the join to a bevel join. See \pgfsys@stroke.

\def\pgfsys@setdash#1#2{\pgf@sys@fail{setting the dashing pattern}}
% Sets the dashing patter. #1 should be a list of lengths given in big
% points (bp) separated by spaces. #2 should be a single value given
% in bp.
%
% The list of values in #1 is used to determine the lengths of the
% `on' phases of the dashing and of the `off' phases. For example, if
% #1 is `3 4', then the dashing pattern is `3bp on followed by 4bp
% off, followed by 3bp on, followed by 4bp off, and so on'. A pattern
% of `.5 4 3 1.5' means `.5bp on, 4bp off, 3bp on, 1.5bp off, .5bp on,
% ...'. If the number of entries is odd, the last one is used twice,
% so `3' means `3bp on, 3bp off, 3bp on, 3bp off,...'. An empty list
% means `always on'.
%
% The second argument determines the `phase' of the pattern. For
% example, for a pattern of `3 4' and a phase of `1', the pattern
% would start: `2bp on, 4bp off, 3bp on, 4bp off, 3bp on, 4bp off...'.





%
%
% Color stuff
%
%

\def\pgfsys@color@rgb@stroke#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given rgb tuple
% (numbers between 0 and 1). 
%
% Example: Make stroked text dark red: \pgfsys@color@rgb@stroke{0.5}{0}{0}
%
% The special stroking color is only used if the stroking color has
% been set since the last \pgfutil@color command. Thus, each \pgfutil@color command
% should reset both the stroking and filling colors.

\def\pgfsys@color@rgb@fill#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given rgb tuple
% (numbers between 0 and 1). This color may be different from the
% stroking color.

\def\pgfsys@color@rgb#1#2#3{\pgfsys@color@rgb@stroke{#1}{#2}{#3}\pgfsys@color@rgb@fill{#1}{#2}{#3}}
% Sets the color used for filling and stroking operations. This is a
% ``low-level'' version of the \pgfutil@color command. It is currently only
% used by the plain tex version to support colors.

\def\pgfsys@color@cmyk@stroke#1#2#3#4{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given cymk tuple
% (numbers between 0 and 1). 

\def\pgfsys@color@cmyk@fill#1#2#3#4{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given cymk tuple
% (numbers between 0 and 1). 

\def\pgfsys@color@cmyk#1#2#3#4{\pgfsys@color@cmyk@stroke{#1}{#2}{#3}{#4}\pgfsys@color@cmyk@fill{#1}{#2}{#3}{#4}}
% Sets the color used for filling and stroking operations.

\def\pgfsys@color@cmy@stroke#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given cym tuple
% (numbers between 0 and 1). 

\def\pgfsys@color@cmy@fill#1#2#3{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given cym tuple
% (numbers between 0 and 1). 

\def\pgfsys@color@cmy#1#2#3{\pgfsys@color@cmy@stroke{#1}{#2}{#3}\pgfsys@color@cmy@fill{#1}{#2}{#3}}
% Sets the color used for filling and stroking operations.

\def\pgfsys@color@gray@stroke#1{\pgf@sys@fail{color}}
% Sets the color used for stroking operations to the given gray level 
% (number between 0 and 1). 

\def\pgfsys@color@gray@fill#1{\pgf@sys@fail{color}}
% Sets the color used for filling operations to the given gray level 
% (number between 0 and 1). 

\def\pgfsys@color@gray#1{\pgfsys@color@gray@stroke{#1}\pgfsys@color@gray@fill{#1}}
% Sets the color used for filling and stroking operations.

\newif\ifpgfsys@color@reset@inorder
% This if decides whether the color resetting of the
% \pgfsys@color@reset command may assume that all color commands are
% given ``in order.'' This means that this command will not be called,
% say, at the beginning of a box that is later inserted at a point
% where a fill color was actively set. This may allow the command to
% produce more compact code when it ``knows'' that no special fill or
% stroke color has been set.
\pgfsys@color@reset@inordertrue


\def\pgfsys@color@reset{}
% This command will be called when the \pgfutil@color command is used. It
% should purge any internal settings of stroking and filling
% color. After this call, till the next use of a command like
% \pgfsys@color@rgb@fill, the current color installed by the \pgfutil@color
% command should be used.

\def\pgfsys@color@unstacked#1{}
% This slightly obscure command causes the color stack to be
% tricked. When called, this command should set the current color to
% #1 without causing any change in the color stack. 



%
%
% Coordinate system transformations
%
%

\def\pgfsys@transformcm#1#2#3#4#5#6{\pgf@sys@fail{transformations}}
% Perform a concatenation of the low-level current transformation
% matrix with the matrix given by the values #1 to #6. The
% transformation matrix is a transformation on a homogeneous
% 2D-coordinate system. See the pdf or postscript manual for details. 




%
%
% Graphic state saving and restoring.
%
%

\def\pgfsys@beginscope{\pgf@sys@fail{scoping}}
% Saves the current graphic state on a graphic state stack. All
% changes to the graphic state parameters mentioned for \pgfsys@stroke
% and \pgfsys@fill will be local to the current graphic state and will
% the old values will be restored after endscope is used.
%
% WARNING: pdf and postscript differ with respect to the question of
% whether the current path is part of the graphic state or not. For
% this reason, you should never use this command unless the path is
% currently empty. For example, it might be a good idea to use
% discardpath prior to calling this command. 

\def\pgfsys@endscope{\pgf@sys@fail{scoping}}
% Restores the last saved graphic state.




%
%
% Special commands
%
%

\def\pgfsys@imagesuffixlist{}
% A list of suffixes, separated by `:', that will be tried when
% searching for an image.



%
%
% Transparency
%
%

\def\pgfsys@stroke@opacity#1{\pgf@sys@fail{opacity}}
% Sets the opacity of stroking operations. 1 means fully opaque, 0
% means fully transparent.

\def\pgfsys@fill@opacity#1{\pgf@sys@fail{opacity}}
% Sets the opacity of filling operations. 1 means fully opaque, 0
% means fully transparent.

\def\pgfsys@transparencygroupfrombox#1{\pgf@sys@fail{transparency groups}}
% This takes a TeX box and converts it into a transparency
% group. This means that any transparency settings apply to the box as
% a whole. For instance, if a box contains two overlapping black
% circles and you draw them normally with 50% transparency, then the
% overlap will be darker than the rest. By comparison, if the circles
% are part of a transparency group, the overlap will get the same
% color as the rest.

\def\pgfsys@definemask{\pgf@sys@fail{image masks}}
% This command declares a mask for usage with images. It works similar
% to \pgfsys@defineimage: Certain macros are set when the command is
% called. The result should be to set the macro \pgf@mask to a pdf
% object count that can subsequently be used as a soft mask. The
% following macros will be set when this command is invoked:
%
% - \pgf@filename
%   File name of the mask to be defined.
%
% - \pgf@maskmatte
%   The so-called matte of the mask (see the pdf documentation for
%   details). The matte is a color specification consisting of 1, 3 or
%   4 numbers between 0 and 1. The number of numbers depends on the
%   number of color channels in the image (not in the mask!). It will
%   be assumed that the image has been preblended with this color.

\def\pgfsys@fadingfrombox#1#2{\pgf@sys@fail{fadings}}
% Declares an fading named #1. The parameter #2 must be a
% box. Its contents luminosity determines the opacity of the resulting
% mask. 

\def\pgfsys@usefading#1#2#3#4#5#6#7{\pgf@sys@fail{fadings}}
% Installs a previously declared fading #1 in the current graphics
% state. Parameters #2 to #7 specify a transformation cm that should
% be applied to the mask before it is used.



%
%
% Shading commands
%
%

\def\pgfsys@horishading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Declares a horizontal shading for later use. The effect of this
% command should be the definition of a macro called `@pgfshading#1!'
% (or \csname @pdfshading#1!\endcsname, to be precise). When invoked,
% this new macro should insert a shading at the current position.
%
% #1 is the name of the shading, which is also used in the output
% macro name. #2 is the height of the shading and must be given as a
% TeX dimension like `2cm' or `10pt'. #3 is a shading color
% specification as specified in the pgfuserguide. The shading
% specification implicitly fixes the width of the shading. 
%
% When `@pgfshading#1!' is invoked, it should insert a box of height
% #2 and the width implicit in the shading declaration.

\def\pgfsys@vertshading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Like horishading, only for vertical shadings. This time, the height
% of the shading is implicit in #3 and the width is given as #2.

\def\pgfsys@radialshading#1#2#3{\pgf@sys@fail{shadings}\pgf@sys@noshading{#1}}
% Declares a radial shading. Like the previous macros, this command
% should setup the macro `@pgfshading#1!', which upon invocation
% should insert a radial shading whose size is implicit in #3. 
%
% The parameter #2 is a pgf point specification if the starting point
% of the shading. See the pgfuserguide for details.

\def\pgfsys@functionalshading#1#2#3#4{\pgf@sys@fail{shadings (functional)}\pgf@sys@noshading{#1}}
% Declares a shading using a PostScript-like function that provides a
% color for each point. Like the previous macros, this command
% should setup the macro `@pgfshading#1!' so that it will produce a
% box containing the desired shading.
%
% Parameter #1 is the name of the shading. Parameter #4 is a
% Postscript-like function (type 4 function of the PDF specification)
% as described in Section 3.9.4 of the PDF Specification version 1.7.
% Parameter #2 and #3 are pgf point specifications that specifies the
% lower left and upper right coordinate.
%
% When function #4 is evaluated, the coordinate of the current
% point will be on the (virtual) PostScript stack in bp units. After
% the function has been evaluated, the stack should consist of three
% numbers (not integers! - the Apple PDF renderer is broken in this
% regard, so add cvr's at the end if needed) that represent the red,
% green, and blue components of the color.
%
% A buggy #4 will result is *totally unpredictable chaos* during
% rendering. 

\def\pgf@sys@noshading#1{\expandafter\global\expandafter\let\csname @pgfshading#1!\endcsname=\pgfutil@empty}




%
%
% Pattern stuff
%
%

\def\pgfsys@declarepattern#1#2#3#4#5#6#7#8#9{\pgf@sys@fail{patterns}}
% This command declares a new colored or uncolored pattern. Uncolored
% patterns have no inherent color, the color is provided when they are
% set. Colored patters have an inherent color.
% #1       = name of the pattern (must be a plain suffix for use in
%            postscript/pdf/etc.) 
% #2 to #5 = four coordinates describing the corners of a bounding box
%            of pattern cells
% #6       = x-step
% #7       = y-step
% #8       = pattern code
% #9       = 0 if uncolored patter, 1 if colored pattern.

\def\pgfsys@setpatternuncolored#1#2#3#4{\pgf@sys@fail{patterns}}
% Sets an uncolored pattern #1 as filling color. The numbers #2, #3,
% #4 must be an rgb-value to be used as the color of the pattern.

\def\pgfsys@setpatterncolored#1{\pgf@sys@fail{patterns}}
% Sets an colored pattern #1 as filling color.


%
%
% Page size stuff
%
%
\def\pgfsys@papersize#1#2{\pgf@sys@fail{papersize}}
% This command sets the paper size in a portable way.
% #1 = width
% #2 = height



%
%
% Position tracking commands
%
%

% Marks the current position on the page. This position can later be
% referenced using \pgfsys@getposition
\def\pgfsys@markposition#1{\pgf@sys@fail{marking the current position}}

% Sets #2 to a pgfpoint macro that returns the position #1 is
% returned in a coordinate system where the x-axis goes right and the
% y-axis goes up. The origin of this coordinate system may or may not
% lie in the lower left corner; you should shift the coordinate system
% to the position "pgfpageorigin" to make sure that the origin is at
% the lower left corner. Typically, getting this position
% requires two runs of TeX. On the first run, the macro will be set to
% \relax, indicating that the position is not available. 
%
% If #1 is set to the special position "pgfpageorigin", the position
% of the the lower left page corner is returned. 

\def\pgfsys@getposition#1#2{\let#2=\relax}



%
%
% Commands having a default implementation. These commands only need
% not be implemented by drivers if this results in a better
% preformance. 
%
%


\def\pgfsys@shadingoutsidepgfpicture#1{%
  #1%
}
% This command gets the definition of a shading (@pgfshadingxxxx!) as
% an argument and should insert this shading into the normal text.
%
% This command has a default implementation.


\def\pgfsys@shadinginsidepgfpicture#1{%
  \pgf@makehbox{#1}%
  \setbox\pgf@hbox=\hbox{\hskip-.5\wd\pgf@hbox\lower.5\ht\pgf@hbox\hbox{\box\pgf@hbox}}%
  \pgfqbox{\pgf@hbox}%
}
% This command works like \pgfsys@shadingoutsidepgfpicture, only it is
% called when a shading should be inserted inside a picture. This
% command should insert the shading centered on the origin (which will
% typically have been low-level translated somewhere else.)
%
% This command has a default implementation.





\def\pgfsys@closestroke{\pgfsys@closepath\pgfsys@stroke}
% This command should have the same effect as first closing the path
% and then stroking it.


\def\pgfsys@transformshift#1#2{\pgfsys@transformcm{1}{0}{0}{1}{#1}{#2}}
% This command will change the origin of the low-level coordinate
% system to (#1bp,#2bp).

\def\pgfsys@transformxyscale#1#2{\pgfsys@transformcm{#1}{0}{0}{#2}{0bp}{0bp}}
% This command will scale the low-level coordinate system (and
% everything that is drawn) by a factor of #1 in x-directed and #2 in
% y-direction. Note that this applies to everything, including
% lines. So a scaled line will have a different width and may even
% have a different width when going along the x-axis and when going
% along the y-axis, if the scaling is different in these directions.

\def\pgfsys@hbox#1{%
  \pgfsys@beginscope%
    \setbox#1=\hbox{\box#1}%
    \wd#1=0pt%
    \ht#1=0pt%
    \dp#1=0pt%
    \box#1%
  \pgfsys@endscope%
}
% Called to insert a TeX hbox into a pgfpicture. 

\def\pgfsys@hboxsynced#1{%
  {\pgfsys@beginscope\pgflowlevelsynccm\pgfsys@hbox#1\pgfsys@endscope}%
}
% Called to insert a TeX hbox into a pgfpicture, but with the current
% coordinate transformation matrix synced with the canvas
% transformation matrix. 
%
% In essence, this command does the same as if you first said
% \pgflowlevelsynccm and then \pgfsys@hbox. However, a driver may
% choose to use a ``TeX-translation'' for the translation part of the
% transformation cm. This will ensure that hyperlinks ``survive'' at
% least translations. 

\def\pgfsys@beginpicture{}
% Called at the beginning of a pgfpicture. Used to setup things.

\def\pgfsys@endpicture{}
% Called at the end of a pgfpicture. 

\def\pgfsys@typesetpicturebox#1{%
  \pgfmathsetlength\pgf@x{\pgf@shift@baseline}%
  \advance\pgf@x by-\pgf@picminy\relax%
  \advance\pgf@picmaxy by-\pgf@picminy\relax% maxy is now the height
  \advance\pgf@picmaxx by-\pgf@picminx\relax% maxx is now the width
  \setbox#1=\hbox{\hskip-\pgf@picminx\lower\pgf@picminy\box#1}%
  \ht#1=\pgf@picmaxy%
  \wd#1=\pgf@picmaxx%
  \dp#1=0pt%
  \leavevmode\raise-\pgf@x\box#1%
}
% Called after a picture has been typeset in box #1. This
% command should insert the box into the normal TeX code. The box #1
% will still be a ``raw'' box that contains only the \special's. The
% job of this command is to resize and shift this box according to the
% baseline shift and the size of the box.
%
% This command has a default implementation.

\def\pgfsys@beginpurepicture{\pgfsys@beginpicture}
% This version of the beginpicture command can be used for pictures
% that are guaranteed not to contain any hboxes. In this case, a
% driver might provide a more compact version of the command.

\def\pgfsys@endpurepicture{\pgfsys@endpicture}
% Called at the end of a ``pure'' pgfpicture.

\def\pgfsys@defineimage{%
  \ifx\pgf@imagewidth\pgfutil@empty\else\edef\pgf@imagewidth{width=\pgf@imagewidth,}\fi%
  \ifx\pgf@imageheight\pgfutil@empty\else\edef\pgf@imageheight{height=\pgf@imageheight,}\fi%
  \ifx\pgf@imagepage\pgfutil@empty\else\edef\pgf@imagepage{page=\pgf@imagepage,}\fi%
  \edef\pgf@image{\noexpand\includegraphics[\pgf@imageheight\pgf@imagewidth]{\pgf@filename}}%
}
% Called, when an image should be defined. 
%
% This command does not take any parameters. Instead, certain macros
% will be preinstalled with appropriate values when this command is
% invoked. These are:
%
% - \pgf@filename
%   File name of the image to be defined.
%
% - \pgf@imagewidth
%   Will be set to the desired (scaled) width of the image.
%
% - \pgf@imageheight
%   Will be set to the desired (scaled) height of the image.
%
%   If this macro and also the height macro are empty, the image
%   should have its `natural' size.
%
%   If exactly only of them is specified, the undefined value the
%   image is scaled so that the aspect ratio is kept.
%
%   If both are set, the image is scaled in both directions
%   independently, possibly changing the aspect ratio.
%
%
% The following macros presumable mostly make sense for drivers that
% can handle pdf: 
%
% - \pgf@imagepage
%   The desired page number to be extracted from a multi-page
%   `image'. 
%
% - \pgf@imagemask
%   If set, it will be set to `/SMask x 0 R', where x is the pdf
%   object number of a soft mask to be applied to the image.
%
% - \pgf@imageinterpolate
%   If set, it will be set to `/Interpolate true' or  `/Interpolate
%   false', indicating whether the image should be interpolated in
%   pdf. 
%
%
% The command should now setup the macro \pgf@image such that calling
% this macro will result in typesetting the image. Thus, \pgf@image is
% the `return value' of the command.


\def\pgfsys@defobject#1#2#3#4{%
  \pgfsysprotocol@getcurrentprotocol\pgfsys@temp%
  {%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedtrue%
    #4%
    \pgfsysprotocol@getcurrentprotocol\pgfsys@@temp%
    \expandafter\global\expandafter\let\csname #1\endcsname=\pgfsys@@temp%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgfsys@temp%
}
% Declares an object for later use. The idea is that the object can be
% precached in some way and then be rendered more quickly when used
% several times. For example, an arrow head might be defined and
% prerendered in this way.
%
% The parameter #1 is the name for later use. #2 and #3 are pgf points
% specifying a bounding box for the object. #4 is the code for the
% object. The code may only contain protocollable code.


\def\pgfsys@useobject#1#2{%
  \pgfsysprotocol@getcurrentprotocol\pgfsys@temp%
  {%
    \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
    \pgfsysprotocol@bufferedfalse%
    #2%
    \expandafter\pgfsysprotocol@setcurrentprotocol\csname #1\endcsname%
    \pgfsysprotocol@invokecurrentprotocol%
  }%
  \pgfsysprotocol@setcurrentprotocol\pgfsys@temp%
}
% Renders a previously declared object. The first parameter is the
% name of the the object. The second parameter is extra code that
% should be executed right *before* the object is rendered. Typically,
% this will be some transformation code. 


\def\pgfsys@begininvisible{\pgfsys@transformcm{1}{0}{0}{1}{2000bp}{2000bp}}
% Between this command and the closing endinvisible, all output should
% be suppressed. Nothing should be drawn at all, which includes all
% paths, images and shadings.

\def\pgfsys@endinvisible{\pgfsys@transformcm{1}{0}{0}{1}{-2000bp}{-2000bp}}
% Ends the invisibilty section, unless invisibility blocks have been
% nested. In this case, only the `last' one restores visibility.


\def\pgfsys@atbegindocument{}
% This command will be executed at the begin of the document. If for
% whatever reason this is not done, you may wish to execute this
% command yourself. It will setup certain specials that need to be
% inserted into the resulting .pdf/.ps/.xxx file.





% Discern the driver:
\input pgf.cfg

\PackageInfo{pgfsys}{Driver file for pgf: \pgfsysdriver}
\pgfutil@InputIfFileExists{\pgfsysdriver}{}{%
  \PackageError{pgfsys}{Driver file ``\pgfsysdriver'' not found.}{}}



% This will insert always-present-specials at the beginning of the
% code. 
\AtBeginDocument{
  \pgfsys@atbegindocument
  \let\pgfsys@atbegindocument=\pgfutil@empty
}



% Read aux file in plain and context mode:

\pgfutil@aux@read@hook


\endinput


==> pgfsys.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file is pgfsys.tex

\ifx\pgfsysincluded\undefined
\def\pgfsysincluded{}

\edef\pgfsysatcode{\the\catcode`\@}
\catcode`\@=11

\input pgfrcs.tex

\input pgfsys.code.tex
\input pgfsyssoftpath.code.tex
\input pgfsysprotocol.code.tex

\catcode`\@=\pgfsysatcode\relax

\fi

\endinput


==> pgfsysprotocol.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/systemlayer/pgfsysprotocol.code.tex,v 1.4 2006/10/16 22:32:59 tantau Exp $



% This package provides the pgf system protcol layer. Protocolling is
% used to record a bunch of graphic operations so that they can be
% reused quickly at a later point.
%
% Basically, all ``recordable'' \pgfsys@xxxx commands call
% \pgfsysprotocol@protocol for their protocolable literal
% specials. The literal text will either be stored in the current
% protocol. At a later point (actually, normally this happens
% immediately afterwards), the accumulated protocolled text is invoked
% using pgfsys@invokeprotocol.



\let\pgfsysprotocol@currentprotocol=\pgfutil@empty
\newif\ifpgfsysprotocol@buffered


% Add to the protocol buffered
\def\pgfsysprotocol@literalbuffered#1{%
  \edef\pgfsysprotocol@temp{{#1\space}}%
  \expandafter\pgfutil@g@addto@macro\expandafter\pgfsysprotocol@currentprotocol\pgfsysprotocol@temp%
}

% Add to the protocol
\def\pgfsysprotocol@literal#1{%
  \pgfsysprotocol@literalbuffered{#1}%
  \ifpgfsysprotocol@buffered%
  \else%
    \pgfsysprotocol@flushcurrentprotocol%
  \fi%
}

% Getting and setting the current protocol
\def\pgfsysprotocol@getcurrentprotocol#1{%
  \let#1=\pgfsysprotocol@currentprotocol%
}

\def\pgfsysprotocol@setcurrentprotocol#1{%
  \global\let\pgfsysprotocol@currentprotocol=#1%
}


% Invoking the current protocol
\def\pgfsysprotocol@invokecurrentprotocol{%
  \ifx\pgfsysprotocol@currentprotocol\pgfutil@empty%
  \else%
    \expandafter\pgfsys@invoke\expandafter{\pgfsysprotocol@currentprotocol}%
  \fi%
}

\def\pgfsysprotocol@flushcurrentprotocol{%
  \pgfsysprotocol@invokecurrentprotocol%
  \pgfsysprotocol@setcurrentprotocol\pgfutil@empty%
}


\endinput


==> pgfsyssoftpath.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS $Header: /cvsroot/pgf/pgf/generic/pgf/systemlayer/pgfsyssoftpath.code.tex,v 1.6 2008/01/23 13:15:28 tantau Exp $


% This package provides the pgf system path abstraction layer. This
% layer is used to construct paths first ``abstractly.'' These
% abstract paths can still be modified, before they are ``made
% concrete.'' 
%
% An abstract path consists of a sequence of basic building blocks,
% each of which is a tuple consisting of two numbers (specifying a
% coordinate) and a token. Possible tokens are:
%
% 1. moveto
% 2. lineto
% 3. rectcorner
% 4. rectsize
% 5. curvetosupporta
% 6. curvetosupportb
% 7. curveto
% 8. closepath
% 9. specialround
%
% A curveto must always be preceeded by a curvetosupporta and a
% curvetosupportb. A non-empty path must always begin with a
% moveto. The coordinates of a closepath are non-specified, currently, 
% but they might be set to the coordinate of the path segment start,
% in the future.


% Access to the current path:
%
% Lots of stuff is added to the current path and it can get very long
% (containing literally tens of thousands of tokens). For such macros,
% adding things using a simple "g@addtomacro" takes more and more
% time, resulting in quadratic runtime. To avoid this, ideally, one
% would collect things in an array and then use a divide and conquer
% merger. A simple intermediate solution is the following, implemented
% here: We have the path and two buffers. New tokens are added to the
% first buffer, which is quite small. When it overflow, its contents
% is added to the second buffer, which is large. If that buffer
% overflow, the contents is finally added to the main path (which can
% have arbitrary length). Whenever the main path is set or read, the
% buffers are flushed.
%
% Because of this buffering, it is imperative that the main path is
% accessed only vie appropriate interface macros.



% The current path
\let\pgfsyssoftpath@thepath=\pgfutil@empty
\let\pgfsyssoftpath@bigbuffer=\pgfutil@empty
\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty
\newcount\pgfsyssoftpath@smallbuffer@items
\newcount\pgfsyssoftpath@bigbuffer@items

\def\pgfsyssoftpath@flushbuffers{%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfsyssoftpath@thepath%
  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
    \expandafter\expandafter\expandafter\pgfsyssoftpath@thepath%
    \expandafter\pgfsyssoftpath@bigbuffer\pgfsyssoftpath@smallbuffer}%
  \global\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty
  \global\let\pgfsyssoftpath@bigbuffer=\pgfutil@empty
  \global\pgfsyssoftpath@bigbuffer@items0\relax%
  \global\pgfsyssoftpath@smallbuffer@items0\relax%
}

% Getting and setting the current path
\def\pgfsyssoftpath@getcurrentpath#1{%
  \pgfsyssoftpath@flushbuffers%
  \let#1=\pgfsyssoftpath@thepath%
}

\def\pgfsyssoftpath@setcurrentpath#1{%
  \global\let\pgfsyssoftpath@thepath=#1%
  \global\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty
  \global\let\pgfsyssoftpath@bigbuffer=\pgfutil@empty
  \global\pgfsyssoftpath@bigbuffer@items0\relax%
  \global\pgfsyssoftpath@smallbuffer@items0\relax%
}


% Invoking the current path (slightly optimized)
\def\pgfsyssoftpath@invokecurrentpath{%
  \pgfsyssoftpath@thepath%
  \pgfsyssoftpath@bigbuffer%
  \pgfsyssoftpath@smallbuffer%
}

\def\pgfsyssoftpath@flushcurrentpath{%
  \pgfsyssoftpath@invokecurrentpath%
  \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
}

% Add an item at the end
\def\pgfsyssoftpath@addtocurrentpath#1{%
  \global\advance\pgfsyssoftpath@smallbuffer@items by1\relax%
  \ifnum\pgfsyssoftpath@smallbuffer@items<40\relax% good number?
    \expandafter\gdef\expandafter\pgfsyssoftpath@smallbuffer\expandafter{\pgfsyssoftpath@smallbuffer#1}%
  \else%
    \pgfsyssoftpath@smalloverflow{#1}%
  \fi%
}
\def\pgfsyssoftpath@smalloverflow#1{%
  \global\advance\pgfsyssoftpath@bigbuffer@items by1\relax%
  \ifnum\pgfsyssoftpath@smallbuffer@items<30\relax% good number?
    \expandafter\expandafter\expandafter\gdef%
    \expandafter\expandafter\expandafter\pgfsyssoftpath@bigbuffer%
    \expandafter\expandafter\expandafter{\expandafter\pgfsyssoftpath@bigbuffer\pgfsyssoftpath@smallbuffer#1}%
    \global\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty%
    \global\pgfsyssoftpath@smallbuffer@items0\relax%
  \else%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gdef%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfsyssoftpath@thepath%
    \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
      \expandafter\expandafter\expandafter\pgfsyssoftpath@thepath
      \expandafter\pgfsyssoftpath@bigbuffer\pgfsyssoftpath@smallbuffer#1}%
    \global\let\pgfsyssoftpath@smallbuffer=\pgfutil@empty
    \global\let\pgfsyssoftpath@bigbuffer=\pgfutil@empty
    \global\pgfsyssoftpath@bigbuffer@items0\relax%
    \global\pgfsyssoftpath@smallbuffer@items0\relax%
  \fi%
}



\def\pgfsyssoftpath@lastmoveto{{0pt}{0pt}}

\newif\ifpgfsyssoftpathmovetorelevant
\pgfsyssoftpathmovetorelevanttrue

% Add a moveto element to the current path
\def\pgfsyssoftpath@moveto#1#2{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@movetotoken{#1}{#2}%
  }}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\pgfsyssoftpath@temp%
  \ifpgfsyssoftpathmovetorelevant%
    \xdef\pgfsyssoftpath@lastmoveto{{#1}{#2}}%
  \fi%
}

% Add a lineto element to the current path
\def\pgfsyssoftpath@lineto#1#2{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@linetotoken{#1}{#2}%
  }}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\pgfsyssoftpath@temp%
}

% Add curveto elements to the current path
\def\pgfsyssoftpath@curveto#1#2#3#4#5#6{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@curvetosupportatoken{#1}{#2}%
    \noexpand\pgfsyssoftpath@curvetosupportbtoken{#3}{#4}%
    \noexpand\pgfsyssoftpath@curvetotoken{#5}{#6}%
  }}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\pgfsyssoftpath@temp%
}

% Add rectanlge elements to the current path
\def\pgfsyssoftpath@rect#1#2#3#4{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@rectcornertoken{#1}{#2}%
    \noexpand\pgfsyssoftpath@rectsizetoken{#3}{#4}%
  }}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\pgfsyssoftpath@temp%
}

% Add closepath element to the current path
\def\pgfsyssoftpath@closepath{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@closepathtoken\pgfsyssoftpath@lastmoveto%
  }}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\pgfsyssoftpath@temp%
}

% Add special element to the current path
\def\pgfsyssoftpath@specialround#1#2{%
  \edef\pgfsyssoftpath@temp{{%
    \noexpand\pgfsyssoftpath@specialroundtoken{#1}{#2}%
  }}%
  \expandafter\pgfsyssoftpath@addtocurrentpath\pgfsyssoftpath@temp%
}

% Marshallers
\def\pgfsyssoftpath@movetotoken#1#2{\pgfsys@moveto{#1}{#2}}
\def\pgfsyssoftpath@linetotoken#1#2{\pgfsys@lineto{#1}{#2}}
\def\pgfsyssoftpath@rectcornertoken#1#2#3#4#5{\pgfsys@rect{#1}{#2}{#4}{#5}} % #3 = \pgfsyssoftpath@rectsizetoken
\def\pgfsyssoftpath@curvetosupportatoken#1#2#3#4#5#6#7#8{\pgfsys@curveto{#1}{#2}{#4}{#5}{#7}{#8}}
\def\pgfsyssoftpath@closepathtoken#1#2{\pgfsys@closepath}
\let\pgfsyssoftpath@specialroundtoken=\pgfutil@gobbletwo


\endinput

%%% Local Variables: 
%%% mode: latex
%%% End: 


==> pgfutil-common.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% 
% This file provides utitiliy commands that are used throughout pgf.
%
% For most commands, the definition of these commands is just given
% below. We cannot use the LaTeX definition of these commands since
% LaTeX may not be the current format and since LaTeX packages tend to
% redefine these commands.
%
% For some commands the actual definition of the format (like latex or
% context) is to be preferred over the generic definition below. In
% this case, the definition of the format is installed when the file
% pgfutil-XXXX.tex is read, where XXXX is the format name (latex,
% plain, or context). 



\catcode`\@=11\relax


% Simple stuff

\long\def\pgfutil@ifundefined#1{%
  \expandafter\ifx\csname#1\endcsname\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}
\def\pgfutil@firstofone#1{#1}
\def\pgfutil@firstoftwo#1#2{#1}
\def\pgfutil@secondoftwo#1#2{#2}
\def\pgfutil@empty{}
\def\pgfutil@gobble#1{}
\def\pgfutil@gobbletwo#1#2{}
\def\pgfutil@namedef#1{\expandafter\def\csname #1\endcsname}
\def\pgfutil@namelet#1{\expandafter\pgfutil@@namelet\csname#1\endcsname}
\def\pgfutil@@namelet#1#2{\expandafter\let\expandafter#1\csname#2\endcsname}
\long\def\pgfutil@g@addto@macro#1#2{%
  \begingroup
    \toks@\expandafter{#1#2}%
    \xdef#1{\the\toks@}%
 \endgroup}
\newif\ifpgfutil@tempswa

% pgfutil@ifnextchar

\long\def\pgfutil@ifnextchar#1#2#3{%
  \let\pgfutil@reserved@d=#1%
  \def\pgfutil@reserved@a{#2}%
  \def\pgfutil@reserved@b{#3}%
  \futurelet\pgfutil@let@token\pgfutil@ifnch}
\def\pgfutil@ifnch{%
  \ifx\pgfutil@let@token\pgfutil@sptoken
    \let\pgfutil@reserved@c\pgfutil@xifnch
  \else
    \ifx\pgfutil@let@token\pgfutil@reserved@d
      \let\pgfutil@reserved@c\pgfutil@reserved@a
    \else
      \let\pgfutil@reserved@c\pgfutil@reserved@b
    \fi
  \fi
  \pgfutil@reserved@c}
{%
  \def\:{\global\let\pgfutil@sptoken= } \:
  \def\:{\pgfutil@xifnch} \expandafter\gdef\: {\futurelet\pgfutil@let@token\pgfutil@ifnch}
}

% pgfutil@in@

\newif\ifpgfutil@in@
\def\pgfutil@in@#1#2{%
 \def\pgfutil@in@@##1#1##2##3\pgfutil@in@@{%
  \ifx\pgfutil@in@##2\pgfutil@in@false\else\pgfutil@in@true\fi}%
 \pgfutil@in@@#2#1\pgfutil@in@\pgfutil@in@@}


% pgfutil@for

\def\pgfutil@nnil{\pgfutil@nil}
\def\pgfutil@fornoop#1\@@#2#3{}
\long\def\pgfutil@for#1:=#2\do#3{%
  \expandafter\def\expandafter\pgfutil@fortmp\expandafter{#2}%
  \ifx\pgfutil@fortmp\pgfutil@empty \else
    \expandafter\pgfutil@forloop#2,\pgfutil@nil,\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\pgfutil@nnil \else
       #5\def#4{#2}\ifx #4\pgfutil@nnil \else#5\pgfutil@iforloop #3\@@#4{#5}\fi\fi}
\long\def\pgfutil@iforloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@iforloop\fi#2\@@#3{#4}}
\def\pgfutil@tfor#1:={\pgfutil@tf@r#1 }
\long\def\pgfutil@tf@r#1#2\do#3{\def\pgfutil@fortmp{#2}\ifx\pgfutil@fortmp\space\else
    \pgfutil@tforloop#2\pgfutil@nil\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@tforloop#1#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@tforloop\fi#2\@@#3{#4}}


% pgfutil@IfFileExists

\chardef\pgfutil@inputcheck0
\def\pgfutil@IfFileExists#1#2#3{%
  \openin\pgfutil@inputcheck#1 %
  \ifeof\pgfutil@inputcheck
     #3\relax
  \else
    #2\relax
  \fi
  \closein\pgfutil@inputcheck}

\def\pgfutil@InputIfFileExists#1#2#3{\pgfutil@IfFileExists{#1}{\input #1\relax#2}{#3}}%


% aux-read-hook

\let\pgfutil@aux@read@hook=\relax


% Tokens for the end of the typesetting -- they will be added at the
% end of every job (hopefully...).

\newtoks\pgfutil@everybye


\endinput


==> t-pgf.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgf.


\ifx\pgfdefined\undefined
\let\pgfdefined=\relax

\input t-pgfcor.tex

\usepgfmodule[shapes,plot]

%\input t-pgfbsn.tex
%\input t-pgfbde.tex
%\input t-pgfbma.tex

\fi

\endinput

==> t-pgfbim.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfbaseimage.

\PackageWarning{pgf}{This module is obsolete and no longer needed}

\endinput

==> t-pgfbla.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfbaselayers.

\PackageWarning{pgf}{This module is obsolete and no longer needed}

\endinput

==> t-pgfbma.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfbasematrix.

\PackageWarning{pgf}{This module is obsolete. Use \string\usepgfmodule[matrix] instead}

\usepgfmodule[matrix]

\endinput

==> t-pgfbpl.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfbaseplot.

\PackageWarning{pgf}{This module is obsolete. Use \string\usepgfmodule[plot] instead}

\usepgfmodule[plot]


\endinput

==> t-pgfbpt.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfbasepatterns.

\PackageWarning{pgf}{This module is obsolete and no longer needed}

\endinput

==> t-pgfbsh.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfbaseshapes.

\PackageWarning{pgf}{This module is obsolete. Use \string\usepgfmodule[shapes] instead}

\usepgfmodule[shapes]

\endinput

==> t-pgfbsn.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfbasesnakes.

\PackageWarning{pgf}{This module is obsolete. Use \string\usepgfmodule[decorations] instead}

\usepgfmodule[decorations]


\endinput

==> t-pgfcal.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% ConTeXt module pgfcalendar.

\ifx\pgfcalendardefined\undefined
\let\pgfcalendardefined=\relax

\input t-pgfrcs.tex

\edef\pgfcalendaratcode{\the\catcode`\@}
\edef\pgfcalendarbarcode{\the\catcode`\|}
\catcode`\@=11
\catcode`\|=12

\input pgfcalendar.code.tex

\catcode`\@=\pgfcalendaratcode
\catcode`\|=\pgfcalendarbarcode

\fi

\endinput

==> t-pgfcor.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfcore.


\ifx\pgfcoredefined\undefined
\let\pgfcoredefined=\relax

\input t-pgfsys.tex

\edef\pgfcoreatcode{\the\catcode`\@}
\edef\pgfcorebarcode{\the\catcode`\|}
\edef\pgfcoreexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input pgfcore.code.tex

\catcode`\@=\pgfcoreatcode
\catcode`\|=\pgfcorebarcode
\catcode`\!=\pgfcoreexclaimcode

\let\startpgfpicture=\pgfpicture
\let\stoppgfpicture=\endpgfpicture

\let\startpgfscope=\pgfscope
\let\stoppgfscope=\endpgfscope

\let\startpgflowlevelscope=\pgflowlevelscope
\let\stoppgflowlevelscope=\endpgflowlevelscope

\let\startpgfinterruptpath=\pgfinterruptpath
\let\stoppgfinterruptpath=\endpgfinterruptpath

\let\startpgfinterruptpicture=\pgfinterruptpicture
\let\stoppgfinterruptpicture=\endpgfinterruptpicture

\let\startpgfinterruptboundingbox=\pgfinterruptboundinbox
\let\stoppgfinterruptboudingbox=\endpgfinterruptboundingbox

\fi

\endinput

==> t-pgffor.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% ConTeXt module pgffor.

\ifx\pgffordefined\undefined
\let\pgffordefined=\relax

\input t-pgfrcs.tex

\edef\pgfforatcode{\the\catcode`\@}
\edef\pgfforbarcode{\the\catcode`\|}
\catcode`\@=11
\catcode`\|=12

\input pgffor.code.tex

\catcode`\@=\pgfforatcode
\catcode`\|=\pgfforbarcode

\fi

\endinput

==> t-pgfkey.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% ConTeXt module pgfkeys.

\ifx\pgfkeysdefined\undefined
\let\pgfkeysdefined=\relax

\edef\pgfkeysatcode{\the\catcode`\@}
\edef\pgfkeysbarcode{\the\catcode`\|}
\catcode`\@=11
\catcode`\|=12

\input pgfkeys.code.tex

\catcode`\@=\pgfkeysatcode
\catcode`\|=\pgfkeysbarcode

\fi

\endinput

==> t-pgfmat.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfmath.

\ifx\pgfmathdefined\undefined
\let\pgfmathdefined=\relax

\edef\pgfmathatcode{\the\catcode`\@}
\edef\pgfmathbarcode{\the\catcode`\|}
\edef\pgfmathexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input pgfmath.code.tex

\catcode`\@=\pgfmathatcode
\catcode`\|=\pgfmathbarcode
\catcode`\!=\pgfmathexclaimcode

\fi

\endinput

==> t-pgfmod.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.



% ConTeXt module pgfmodules.

% This module defines the correct names for the context modules. 
%
% This is necessary because context cuts down all module names to 6
% characters.
%
% One starts to wonder whether context was already used in the Apollo
% missions... 

\ifx\pgfmoddefined\undefined
\let\pgfmoddefined=\relax

\definefilesynonym [pgfmath]             [pgfmat]
\definefilesynonym [pgfkeys]             [pgfkey]

\definefilesynonym [pgfcore]             [pgfcor]

\definefilesynonym [pgfbasesnakes]       [pgfbsn]
\definefilesynonym [pgfbaseshapes]       [pgfbsh]
\definefilesynonym [pgfbaseplots]        [pgfbpl]
\definefilesynonym [pgfbaselayers]       [pgfbla]
\definefilesynonym [pgfbaseimage]        [pgfbim]
\definefilesynonym [pgfbasepatterns]     [pgfbpt]
\definefilesynonym [pgfbasematrix]       [pgfbma]
\definefilesynonym [pgfbasetransparency] [pgfbtr]

\definefilesynonym [pgfcalendar]         [pgfcal]


\fi

\endinput

==> t-pgfrcs.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% ConTeXt module pgfrcs.

\ifx\pgfrcsdefined\undefined
\let\pgfrcsdefined=\relax

\input t-pgfmod.tex

\edef\pgfrcsatcode{\the\catcode`\@}
\edef\pgfrcsbarcode{\the\catcode`\|}
\edef\pgfrcsexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input pgfutil-common.tex
\input pgfutil-context.def

\input pgfrcs.code.tex

\catcode`\@=\pgfrcsatcode
\catcode`\|=\pgfrcsbarcode
\catcode`\!=\pgfrcsexclaimcode

\fi

\endinput

==> t-pgfsys.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module pgfsys.

\ifx\pgfsysdefined\undefined
\let\pgfsysdefined=\relax

\input t-pgfrcs.tex

\edef\pgfsysatcode{\the\catcode`\@}
\edef\pgfsysbarcode{\the\catcode`\|}
\edef\pgfsysexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input pgfsys.code.tex
\input pgfsyssoftpath.code.tex
\input pgfsysprotocol.code.tex

\catcode`\@=\pgfsysatcode
\catcode`\|=\pgfsysbarcode
\catcode`\!=\pgfsysexclaimcode

\fi

\endinput

==> t-tikz.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% ConTeXt module tikz.

% \input xkeyval.tex   % no longer used/needed

\input t-pgf.tex
\input t-pgffor.tex

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input tikz.code.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

\let\starttikzpicture=\tikzpicture
\let\stoptikzpicture=\endtikzpicture

\endinput

==> tikz.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesPackageRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/tikz.code.tex,v 1.27 2008/02/13 19:48:11 tantau Exp $


% Always-present libraries:

\usepgflibrary{plothandlers}

% TikZ is a key family
\pgfkeys{/tikz/.is family}

\def\tikzset{\pgfqkeys{/tikz}}


\newdimen\tikz@lastx
\newdimen\tikz@lasty
\newdimen\tikz@lastxsaved
\newdimen\tikz@lastysaved

\newdimen\tikzleveldistance
\newdimen\tikzsiblingdistance

\newbox\tikz@figbox
\newbox\tikz@tempbox

\newcount\tikztreelevel
\newcount\tikznumberofchildren
\newcount\tikznumberofcurrentchild

\newcount\tikz@fig@count

\newif\iftikz@node@is@a@label
\newif\iftikz@snaked
\newif\iftikz@decoratepath

\let\tikz@options=\pgfutil@empty
\def\tikz@addoption#1{\expandafter\def\expandafter\tikz@options\expandafter{\tikz@options#1}}
\def\tikz@addmode#1{\expandafter\def\expandafter\tikz@mode\expandafter{\tikz@mode#1}}
\def\tikz@addtransform#1{%
  \ifx\tikz@transform\relax%
    #1%
  \else%
    \expandafter\def\expandafter\tikz@transform\expandafter{\tikz@transform#1}%
  \fi%
}



% TikZ options:

% This command is supported for compatibility only:

\def\tikzoption#1{\pgfutil@ifnextchar[{\tikzoption@opt{#1}}{\tikzoption@noopt{#1}}}%}

\def\tikzoption@opt#1[#2]#3{\pgfkeysdef{/tikz/#1}{#3}\pgfkeyssetvalue{/tikz/#1/.@def}{#2}}
\def\tikzoption@noopt#1#2{\pgfkeysdef{/tikz/#1}{#2}\pgfkeyssetvalue{/tikz/#1/.@def}{\pgfkeysvaluerequired}}

% Baseline options
\tikzoption{baseline}[0pt]{\pgfutil@ifnextchar({\tikz@baseline@coordinate}{\tikz@baseline@simple}#1\@nil}%)
\def\tikz@baseline@simple#1\@nil{\pgfsetbaseline{#1}}
\def\tikz@baseline@coordinate#1\@nil{\pgfsetbaselinepointlater{\tikz@scan@one@point\pgfutil@firstofone#1}}

% Draw options
\tikzoption{line width}{\tikz@semiaddlinewidth{#1}}%

\def\tikz@semiaddlinewidth#1{\tikz@addoption{\pgfsetlinewidth{#1}}\pgfmathsetlength\pgflinewidth{#1}}

\tikzoption{cap}{\tikz@addoption{\csname pgfset#1cap\endcsname}}
\tikzoption{join}{\tikz@addoption{\csname pgfset#1join\endcsname}}
\tikzoption{line cap}{\tikz@addoption{\csname pgfset#1cap\endcsname}}
\tikzoption{line join}{\tikz@addoption{\csname pgfset#1join\endcsname}}
\tikzoption{miter limit}{\tikz@addoption{\pgfsetmiterlimit{#1}}}

\tikzoption{dash pattern}{% syntax: on 2pt off 3pt on 4pt ...
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
    \def\tikz@dashpattern{}%
    \tikz@addoption{\pgfsetdash{}{0pt}}%
  \else%
    \def\tikz@dashpattern{}%
    \expandafter\tikz@scandashon\pgfutil@gobble#1o\@nil%
    \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
    \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
  \fi}
\tikzoption{dash phase}{%
  \def\tikz@dashphase{#1}%
  \edef\tikz@temp{{\tikz@dashpattern}{\noexpand\tikz@dashphase}}%
  \expandafter\tikz@addoption\expandafter{\expandafter\pgfsetdash\tikz@temp}%
}%
\def\tikz@dashphase{0pt}

\def\tikz@scandashon n#1o{%
  \expandafter\def\expandafter\tikz@dashpattern\expandafter{\tikz@dashpattern{#1}}%
  \pgfutil@ifnextchar\@nil{\pgfutil@gobble}{\tikz@scandashoff}}
\def\tikz@scandashoff ff#1o{%
  \expandafter\def\expandafter\tikz@dashpattern\expandafter{\tikz@dashpattern{#1}}%
  \pgfutil@ifnextchar\@nil{\pgfutil@gobble}{\tikz@scandashon}}

\tikzoption{draw opacity}{\tikz@addoption{\pgfsetstrokeopacity{#1}}}

% Double draw options
\tikzoption{double}[]{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@doublefalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \def\tikz@double@color{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@doubletrue}%
  \fi}
\tikzoption{double distance}{%
  \pgfmathsetlength{\pgf@x}{#1}%
  \edef\tikz@double@width@distance{\the\pgf@x}%
  \tikz@addmode{\tikz@mode@doubletrue}}

\def\tikz@double@width@distance{0.6pt}
\def\tikz@double@color{white}

% Fill options

\tikzoption{even odd rule}[]{\tikz@addoption{\pgfseteorule}}
\tikzoption{nonzero rule}[]{\tikz@addoption{\pgfsetnonzerorule}}

\tikzoption{fill opacity}{\tikz@addoption{\pgfsetfillopacity{#1}}}


% Joined fill/draw options

\tikzoption{opacity}{\tikz@addoption{\pgfsetstrokeopacity{#1}\pgfsetfillopacity{#1}}}


% Main color options
\tikzoption{color}{%
  \tikz@addoption{%
    \ifx\tikz@fillcolor\pgfutil@empty%
      \ifx\tikz@strokecolor\pgfutil@empty%
      \else%
        \pgfsys@color@reset@inorderfalse%
        \let\tikz@strokecolor\pgfutil@empty%
        \let\tikz@fillcolor\pgfutil@empty%
      \fi%
    \else%
      \pgfsys@color@reset@inorderfalse%
      \let\tikz@strokecolor\pgfutil@empty%
      \let\tikz@fillcolor\pgfutil@empty%
    \fi%
    \pgfutil@colorlet{tikz@color}{#1}%
    \pgfutil@colorlet{.}{tikz@color}%
    \pgfsetcolor{.}%
    \pgfsys@color@reset@inordertrue%
  }%
  \def\tikz@textcolor{#1}}



% Rounding options
\tikzoption{rounded corners}[4pt]{\pgfsetcornersarced{\pgfpoint{#1}{#1}}}
\tikzoption{sharp corners}[]{\pgfsetcornersarced{\pgfpointorigin}}



% Coordinate options
\tikzoption{x}{\tikz@handle@vec{\pgfsetxvec}{\tikz@handle@x}#1\relax}
\tikzoption{y}{\tikz@handle@vec{\pgfsetyvec}{\tikz@handle@y}#1\relax}
\tikzoption{z}{\tikz@handle@vec{\pgfsetzvec}{\tikz@handle@z}#1\relax}

\def\tikz@handle@vec#1#2{\pgfutil@ifnextchar({\tikz@handle@coordinate#1}{\tikz@handle@single#2}}
\def\tikz@handle@coordinate#1{\tikz@scan@one@point#1}
\def\tikz@handle@single#1#2\relax{#1{#2}}
\def\tikz@handle@x#1{\pgfsetxvec{\pgfpoint{#1}{0pt}}}
\def\tikz@handle@y#1{\pgfsetyvec{\pgfpoint{0pt}{#1}}}
\def\tikz@handle@z#1{\pgfsetzvec{\pgfpoint{#1}{#1}}}


% Transformation options
\tikzoption{scale}{\tikz@addtransform{\pgftransformscale{#1}}}
\tikzoption{scale around}{\tikz@addtransform{\def\tikz@aroundaction{\pgftransformscale}\tikz@doaround{#1}}}
\tikzoption{xscale}{\tikz@addtransform{\pgftransformxscale{#1}}}
\tikzoption{xslant}{\tikz@addtransform{\pgftransformxslant{#1}}}
\tikzoption{yscale}{\tikz@addtransform{\pgftransformyscale{#1}}}
\tikzoption{yslant}{\tikz@addtransform{\pgftransformyslant{#1}}}
\tikzoption{rotate}{\tikz@addtransform{\pgftransformrotate{#1}}}
\tikzoption{rotate around}{\tikz@addtransform{\def\tikz@aroundaction{\pgftransformrotate}\tikz@doaround{#1}}}
\def\tikz@doaround#1{%
  \edef\tikz@temp{#1}% get rid of active stuff
  \expandafter\tikz@doparseA\tikz@temp%
}%
\def\tikz@doparseA#1:{%
  \def\tikz@temp@rot{#1}%
  \tikz@scan@one@point\tikz@doparseB%
}
\def\tikz@doparseB#1{%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@aroundaction{\tikz@temp@rot}%
  \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
}

\tikzoption{shift}{\tikz@addtransform{\tikz@scan@one@point\pgftransformshift#1\relax}}
\tikzoption{xshift}{\tikz@addtransform{\pgftransformxshift{#1}}}
\tikzoption{yshift}{\tikz@addtransform{\pgftransformyshift{#1}}}
\tikzoption{cm}{\tikz@addtransform{\tikz@parse@cm#1\relax}}
\tikzoption{reset cm}[]{\tikz@addtransform{\pgftransformreset}}
\tikzoption{shift only}[]{\tikz@addtransform{\pgftransformresetnontranslations}}

\def\tikz@parse@cm#1,#2,#3,#4,{%
  \def\tikz@p@cm{{#1}{#2}{#3}{#4}}%
  \tikz@scan@one@point\tikz@parse@cmA}
\def\tikz@parse@cmA#1{%
  \expandafter\pgftransformcm\tikz@p@cm{#1}%
}

\tikzset{transform canvas/.code=%
  {%
    \tikz@addoption
    {%
      {%
        \pgftransformreset%
        \let\tikz@transform=\relax%
        \tikzset{#1}%
        \pgflowlevelsynccm%
      }%
      \pgf@relevantforpicturesizefalse%
    }%
  }%
}


% Grid options
\tikzoption{xstep}{\def\tikz@grid@x{#1}}
\tikzoption{ystep}{\def\tikz@grid@y{#1}}
\tikzoption{step}{\tikz@handle@vec{\tikz@step@point}{\tikz@step@single}#1\relax}
\def\tikz@step@single#1{\def\tikz@grid@x{#1}\def\tikz@grid@y{#1}}
\def\tikz@step@point#1{\pgf@process{#1}\edef\tikz@grid@x{\the\pgf@x}\edef\tikz@grid@y{\the\pgf@y}}

\def\tikz@grid@x{1cm}
\def\tikz@grid@y{1cm}


% Current point updates
\newif\iftikz@current@point@local
\tikzset{current point is local/.is if=tikz@current@point@local}

% Path usage options
\newif\iftikz@mode@double
\newif\iftikz@mode@fill
\newif\iftikz@mode@draw
\newif\iftikz@mode@clip
\newif\iftikz@mode@boundary
\newif\iftikz@mode@shade
\newif\iftikz@mode@fade@path
\newif\iftikz@mode@fade@scope
\let\tikz@mode=\pgfutil@empty

\def\tikz@nonetext{none}

\tikzoption{path only}[]{\let\tikz@mode=\pgfutil@empty}
\tikzoption{shade}[]{\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{fill}[]{%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fillfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetfillcolor{#1}}%
      \def\tikz@fillcolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@filltrue}%
  \fi%
}
\tikzoption{draw}[]{%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@drawfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetstrokecolor{#1}}%
      \def\tikz@strokecolor{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@drawtrue}%
  \fi%
}
\tikzoption{clip}[]{\tikz@addmode{\tikz@mode@cliptrue}}
\tikzoption{use as bounding box}[]{\tikz@addmode{\tikz@mode@boundarytrue}}

\tikzoption{save path}{\tikz@addmode{\pgfsyssoftpath@getcurrentpath#1\global\let#1=#1}}

\let\tikz@fillcolor=\pgfutil@empty
\let\tikz@strokecolor=\pgfutil@empty


% Pattern options
\tikzset{pattern/.code=\PackageError{tikz}{You need to say \string\usetikzlibrary{patterns}}{},
         pattern color/.style=pattern}


% Shading options
\tikzset{path fading/.code={
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fade@pathfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \def\tikz@path@fading{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@fade@pathtrue}%
  \fi%
  },
  path fading/.default=, 
  scope fading/.code={
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fade@scopefalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \def\tikz@scope@fading{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@fade@scopetrue}%
  \fi%
  },
  scope fading/.default=}
\tikzset{fit fading/.is if=tikz@fade@adjust}
\tikzset{fading transform/.store in=\tikz@fade@transform}
\tikzset{fading angle/.style={fading transform={rotate=#1}}}

\newif\iftikz@fade@adjust
\tikz@fade@adjusttrue
\let\tikz@fade@transform\pgfutil@empty

\pgfutil@colorlet{transparent}{pgftransparent}
\def\tikz@do@fade@transform{\let\tikz@transform=\relax\expandafter\tikzset\expandafter{\tikz@fade@transform}}



% Transparency groups
\newif\iftikz@transparency@group
\tikzset{/tikz/transparency group/.is if=tikz@transparency@group}


% Shading options
\tikzoption{shading}{\def\tikz@shading{#1}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{shading angle}{\def\tikz@shade@angle{#1}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{top color}{%
  \pgfutil@colorlet{tikz@axis@top}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{0}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{bottom color}{%
  \pgfutil@colorlet{tikz@axis@bottom}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{0}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{middle color}{%
  \pgfutil@colorlet{tikz@axis@middle}{#1}%
  \def\tikz@shading{axis}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{left color}{%
  \pgfutil@colorlet{tikz@axis@top}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{90}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{right color}{%
  \pgfutil@colorlet{tikz@axis@bottom}{#1}%
  \pgfutil@colorlet{tikz@axis@middle}{tikz@axis@top!50!tikz@axis@bottom}%
  \def\tikz@shading{axis}\def\tikz@shade@angle{90}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{ball color}{\pgfutil@colorlet{tikz@ball}{#1}\def\tikz@shading{ball}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{inner color}{\pgfutil@colorlet{tikz@radial@inner}{#1}\def\tikz@shading{radial}\tikz@addmode{\tikz@mode@shadetrue}}
\tikzoption{outer color}{\pgfutil@colorlet{tikz@radial@outer}{#1}\def\tikz@shading{radial}\tikz@addmode{\tikz@mode@shadetrue}}

\def\tikz@shading{axis}
\def\tikz@shade@angle{0}

\pgfdeclareverticalshading[tikz@axis@top,tikz@axis@middle,tikz@axis@bottom]{axis}{100bp}{%
  color(0bp)=(tikz@axis@bottom);
  color(25bp)=(tikz@axis@bottom);
  color(50bp)=(tikz@axis@middle);
  color(75bp)=(tikz@axis@top);
  color(100bp)=(tikz@axis@top)}

\pgfutil@colorlet{tikz@axis@top}{gray}
\pgfutil@colorlet{tikz@axis@middle}{gray!50!white}
\pgfutil@colorlet{tikz@axis@bottom}{white}

\pgfdeclareradialshading[tikz@ball]{ball}{\pgfqpoint{-10bp}{10bp}}{%
 color(0bp)=(tikz@ball!15!white);
 color(9bp)=(tikz@ball!75!white);
 color(18bp)=(tikz@ball!70!black);
 color(25bp)=(tikz@ball!50!black);
 color(50bp)=(black)}

\pgfutil@colorlet{tikz@ball}{blue}

\pgfdeclareradialshading[tikz@radial@inner,tikz@radial@outer]{radial}{\pgfpointorigin}{%
 color(0bp)=(tikz@radial@inner);
 color(25bp)=(tikz@radial@outer);
 color(50bp)=(tikz@radial@outer)}

\pgfutil@colorlet{tikz@radial@inner}{gray}
\pgfutil@colorlet{tikz@radial@outer}{white}


% Pin options
\tikzoption{pin}{\pgfutil@ifnextchar[{\tikz@parse@pin}{\tikz@parse@pin[]}#1\pgf@nil}
\tikzoption{pin distance}{\def\tikz@pin@distance{#1}}
\tikzoption{pin edge}{\def\tikz@pin@edge@style{#1}}

\tikzoption{tikz@pin@post}[]{%
  \tikz@compute@direction{\tikz@label@angle}{\tikz@pin@distance}%
  \global\let\tikz@pin@edge@style@smuggle=\tikz@pin@edge@style%
}
\tikzoption{tikz@pre@pin@edge}[]{\def\pgf@marshal{\tikzstyle{tikz@pin@options}=}
  \expandafter\pgf@marshal\expandafter[\tikz@pin@edge@style@smuggle]%
}

\def\tikz@pin@distance{3ex}
\def\tikz@pin@edge@style{}

\def\tikz@parse@pin[#1]#2:#3\pgf@nil{%
  \tikz@add@after@node@path{%
    \bgroup
      [current point is local=true]
      \pgfextra{\let\tikz@save@last@node=\tikzlastnode}%
      node [every pin,tikz@label@angle=#2,#1,at=(\tikzlastnode.\tikz@label@angle),%
            after node path={(\tikz@save@last@node) edge[every pin edge,tikz@pre@pin@edge,tikz@pin@options] (\tikzlastnode)},
            tikz@pin@post]
        {#3}
    \egroup%
  }
}


% Label and pin options

\tikzoption{label}{\pgfutil@ifnextchar[{\tikz@parse@label}{\tikz@parse@label[]}#1\pgf@nil}
\tikzoption{label distance}{\def\tikz@label@distance{#1}}

\tikzoption{tikz@label@angle}{\def\tikz@label@angle{#1}\csname tikz@label@angle@is@#1\endcsname}

\tikzoption{tikz@label@post}[]{\tikz@compute@direction{\tikz@label@angle}{\tikz@label@distance}}

\def\tikz@label@distance{0pt}

\def\tikz@parse@label[#1]#2:#3\pgf@nil{%
  \tikz@add@after@node@path{
    \bgroup
    \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name}%
    node
    [every label,%
    tikz@label@angle=#2,%
    #1,%
    at=(\tikzlastnode.\tikz@label@angle),tikz@label@post]%
    {#3}%
    \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}%
    \egroup%
  }
}

\expandafter\def\csname tikz@label@angle@is@right\endcsname{\def\tikz@label@angle{0}}
\expandafter\def\csname tikz@label@angle@is@above right\endcsname{\def\tikz@label@angle{45}}
\expandafter\def\csname tikz@label@angle@is@above\endcsname{\def\tikz@label@angle{90}}
\expandafter\def\csname tikz@label@angle@is@above left\endcsname{\def\tikz@label@angle{135}}
\expandafter\def\csname tikz@label@angle@is@left\endcsname{\def\tikz@label@angle{180}}
\expandafter\def\csname tikz@label@angle@is@below left\endcsname{\def\tikz@label@angle{225}}
\expandafter\def\csname tikz@label@angle@is@below\endcsname{\def\tikz@label@angle{270}}
\expandafter\def\csname tikz@label@angle@is@below right\endcsname{\def\tikz@label@angle{315}}

\def\tikz@compute@direction#1#2{%
  \let\tikz@do@auto@anchor=\relax
  \c@pgf@counta=#1\relax%
  \ifnum\c@pgf@counta<0\relax
    \advance\c@pgf@counta by 360\relax%
  \fi%
  \ifnum\c@pgf@counta>359\relax
    \advance\c@pgf@counta by-360\relax%
  \fi%
  \ifnum\c@pgf@counta<4\relax%
    \def\tikz@anchor{west}%
  \else\ifnum\c@pgf@counta<87\relax%
    \def\tikz@anchor{south west}%
  \else\ifnum\c@pgf@counta<94\relax%
    \def\tikz@anchor{south}%
  \else\ifnum\c@pgf@counta<177\relax%
    \def\tikz@anchor{south east}%
  \else\ifnum\c@pgf@counta<184\relax%
    \def\tikz@anchor{east}%
  \else\ifnum\c@pgf@counta<267\relax%
    \def\tikz@anchor{north east}%
  \else\ifnum\c@pgf@counta<274\relax%
    \def\tikz@anchor{north}%
  \else\ifnum\c@pgf@counta<357\relax%
    \def\tikz@anchor{north west}%
  \else%
    \def\tikz@anchor{west}%
  \fi\fi\fi\fi\fi\fi\fi\fi%
  \tikz@addtransform{\pgftransformshift{\pgfpointpolar{#1}{#2}}}%  
}



% General node options
\tikzoption{name}{\edef\tikz@fig@name{#1}}

\tikzoption{at}{\tikz@scan@one@point\tikz@set@at#1}
\def\tikz@set@at#1{\def\tikz@node@at{#1}}%

\tikzoption{shape}{\edef\tikz@shape{#1}}

\tikzoption{nodes}{\tikzstyle{every node}+=[#1]}

\tikzset{alias/.code={\tikz@fig@mustbenamed\expandafter\def\expandafter\tikz@alias\expandafter{\tikz@alias\pgfnodealias{#1}{\tikz@fig@name}}}}

\tikzoption{after node path}{\tikz@add@after@node@path{#1}}%
\def\tikz@add@after@node@path#1{\expandafter\def\expandafter\tikz@after@node\expandafter{\tikz@after@node#1}}

\def\tikzaddafternodepathoption#1{%
  #1%
  \expandafter\def\expandafter\tikz@afternodepathoptions\expandafter{\tikz@afternodepathoptions#1}}

\let\tikz@afternodepathoptions=\pgfutil@empty

\tikzoption{anchor}{\def\tikz@anchor{#1}\let\tikz@do@auto@anchor=\relax}

\tikzoption{left}[]{\def\tikz@anchor{east}\tikz@possibly@transform{x}{-}{#1}}
\tikzoption{right}[]{\def\tikz@anchor{west}\tikz@possibly@transform{x}{}{#1}}
\tikzoption{above}[]{\def\tikz@anchor{south}\tikz@possibly@transform{y}{}{#1}}
\tikzoption{below}[]{\def\tikz@anchor{north}\tikz@possibly@transform{y}{-}{#1}}
\tikzoption{above left}[]%
  {\def\tikz@anchor{south east}%
    \tikz@possibly@transform{x}{-}{#1}\tikz@possibly@transform{y}{}{#1}}
\tikzoption{above right}[]%
  {\def\tikz@anchor{south west}%
    \tikz@possibly@transform{x}{}{#1}\tikz@possibly@transform{y}{}{#1}}
\tikzoption{below left}[]%
  {\def\tikz@anchor{north east}%
    \tikz@possibly@transform{x}{-}{#1}\tikz@possibly@transform{y}{-}{#1}}
\tikzoption{below right}[]%
  {\def\tikz@anchor{north west}%
    \tikz@possibly@transform{x}{}{#1}\tikz@possibly@transform{y}{-}{#1}}

\tikzoption{node distance}{\def\tikz@node@distance{#1}}
\def\tikz@node@distance{1cm}

% The following are deprecated:
\tikzoption{above of}{\tikz@of{#1}{90}}%
\tikzoption{below of}{\tikz@of{#1}{-90}}%
\tikzoption{left of}{\tikz@of{#1}{180}}%
\tikzoption{right of}{\tikz@of{#1}{0}}%
\tikzoption{above left of}{\tikz@of{#1}{135}}%
\tikzoption{below left of}{\tikz@of{#1}{-135}}%
\tikzoption{above right of}{\tikz@of{#1}{45}}%
\tikzoption{below right of}{\tikz@of{#1}{-45}}%
\def\tikz@of#1#2{%
  \def\tikz@anchor{center}%
  \let\tikz@do@auto@anchor=\relax%
  \tikz@addtransform{%
    \expandafter\tikz@extract@node@dist\tikz@node@distance and\pgf@stop%
    \pgftransformshift{\pgfpointpolar{#2}{\tikz@extracted@node@distance}}}%
  \def\tikz@node@at{\pgfpointanchor{#1}{center}}}
\def\tikz@extract@node@dist#1and#2\pgf@stop{%
  \def\tikz@extracted@node@distance{#1}}  


\tikzoption{transform shape}[true]{%
  \csname tikz@fullytransformed#1\endcsname%
  \iftikz@fullytransformed%
    \pgfresetnontranslationattimefalse%
  \else%
    \pgfresetnontranslationattimetrue%
  \fi%
}

\newif\iftikz@fullytransformed
\pgfresetnontranslationattimetrue%

\def\tikz@anchor{center}%
\def\tikz@shape{rectangle}%

\def\tikz@possibly@transform#1#2#3{%
  \let\tikz@do@auto@anchor=\relax%
  \def\tikz@test{#3}%
  \ifx\tikz@test\pgfutil@empty%
  \else%
    \pgfmathsetlength{\pgf@x}{#3}%
    \pgf@x=#2\pgf@x\relax%
    \edef\tikz@marshal{\noexpand\tikz@addtransform{%
        \expandafter\noexpand\csname  pgftransform#1shift\endcsname{\the\pgf@x}}}% 
    \tikz@marshal%
  \fi%
}


% Inter-picture options
\tikzoption{remember picture}[true]{\csname pgfrememberpicturepositiononpage#1\endcsname}
\tikzoption{overlay}[]{\pgf@relevantforpicturesizefalse}



% Line/curve label placement options
\tikzoption{sloped}[true]{\csname pgfslopedattime#1\endcsname}
\tikzoption{allow upside down}[true]{\csname pgfallowupsidedownattime#1\endcsname}

\tikzoption{pos}{\edef\tikz@time{#1}}

\tikzoption{auto}[]{\csname tikz@install@auto@anchor@#1\endcsname}
\tikzoption{swap}[]{%
  \def\tikz@temp{left}%
  \ifx\tikz@auto@anchor@direction\tikz@temp%
    \def\tikz@auto@anchor@direction{right}%
  \else%
    \def\tikz@auto@anchor@direction{left}%
  \fi%
}

\def\tikz@time{.5}

\def\tikz@install@auto@anchor@{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on}
\def\tikz@install@auto@anchor@false{\let\tikz@do@auto@anchor=\relax}
\def\tikz@install@auto@anchor@left{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on\def\tikz@auto@anchor@direction{left}}
\def\tikz@install@auto@anchor@right{\let\tikz@do@auto@anchor=\tikz@auto@anchor@on\def\tikz@auto@anchor@direction{right}}

\let\tikz@do@auto@anchor=\relax%

\def\tikz@auto@anchor@on{\csname tikz@auto@anchor@\tikz@auto@anchor@direction\endcsname}

\def\tikz@auto@anchor@left{\tikz@auto@pre\tikz@auto@anchor\tikz@auto@post}
\def\tikz@auto@anchor@right{\tikz@auto@pre\tikz@auto@anchor@prime\tikz@auto@post}

\def\tikz@auto@anchor@direction{left}

% Text options
\tikzoption{text}{\def\tikz@textcolor{#1}}
\tikzoption{font}{\def\tikz@textfont{#1}}
\tikzoption{text opacity}{\def\tikz@textopacity{#1}}
\tikzoption{text width}{\def\tikz@text@width{#1}}
\tikzoption{text height}{\def\tikz@text@height{#1}}
\tikzoption{text depth}{\def\tikz@text@depth{#1}}
\tikzoption{text ragged}[]%
{\def\tikz@text@action{\raggedright\rightskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}}
\tikzoption{text badly ragged}[]{\def\tikz@text@action{\raggedright\relax}}
\tikzoption{text ragged left}[]%
{\def\tikz@text@action{\raggedleft\leftskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}}
\tikzoption{text badly ragged left}[]{\def\tikz@text@action{\raggedleft\relax}}
\tikzoption{text justified}[]{\def\tikz@text@action{\leftskip\z@\rightskip\z@\relax}}
\tikzoption{text centered}[]{\def\tikz@text@action{%
  \leftskip\z@ plus2em%
  \rightskip\z@ plus2em%
  \spaceskip.3333em \xspaceskip.5em%
  \parfillskip=0pt%
  \let\\=\@centercr% for latex
  \relax}}
\tikzoption{text badly centered}[]%
{\def\tikz@text@action{%
  \let\\=\@centercr% for latex
  \parfillskip=0pt%
  \rightskip\@flushglue%
  \leftskip\@flushglue\relax}}

\let\tikz@text@width=\pgfutil@empty
\let\tikz@text@height=\pgfutil@empty
\let\tikz@text@depth=\pgfutil@empty
\let\tikz@textcolor=\pgfutil@empty
\let\tikz@textfont=\pgfutil@empty
\let\tikz@textopacity=\pgfutil@empty

\def\tikz@text@action{\raggedright\rightskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}





% Arrow options
\tikzoption{arrows}{\tikz@processarrows{#1}}

\tikzoption{>}{%
  \tikz@set@pointed{\csname pgf@arrows@invert#1\endcsname}{#1}%
  \expandafter\tikz@processarrows\expandafter{\tikz@current@arrows}%
}

\tikzoption{shorten <}{\pgfsetshortenstart{#1}}
\tikzoption{shorten >}{\pgfsetshortenend{#1}}

\def\tikz@set@pointed#1#2{%
  \pgfutil@ifundefined{pgf@arrow@code@tikze@>@#2}
  {%
    \pgfarrowsdeclarealias{tikzs@<@#2}{tikze@>@#2}{#1}{#2}%
    \pgfarrowsdeclarereversed{tikzs@>@#2}{tikze@<@#2}{#1}{#2}%
    \pgfarrowsdeclarecombine*{tikz@|<@#2}{tikz@>|@#2}{#1}{#2}{|}{|}%
    \pgfarrowsdeclaredouble[\pgflinewidth]{tikzs@<<@#2}{tikze@>>@#2}{#1}{#2}%<<
    \pgfarrowsdeclarereversed{tikzs@>>@#2}{tikze@<<@#2}{tikzs@<<@#2}{tikze@>>@#2}%<<
  }{}%
  \pgfutil@namedef{tikz@special@arrow@start<}{tikzs@<@#2}%
  \pgfutil@namedef{tikz@special@arrow@end>}{tikze@>@#2}%
  \pgfutil@namedef{tikz@special@arrow@start>}{tikzs@>@#2}%
  \pgfutil@namedef{tikz@special@arrow@end<}{tikze@<@#2}%
  \pgfutil@namedef{tikz@special@arrow@start|<}{tikz@|<@#2}%
  \pgfutil@namedef{tikz@special@arrow@end>|}{tikz@>|@#2}%
  \pgfutil@namedef{tikz@special@arrow@start<<}{tikzs@<<@#2}%
  \pgfutil@namedef{tikz@special@arrow@end>>}{tikze@>>@#2}%<<
  \pgfutil@namedef{tikz@special@arrow@start>>}{tikzs@<<@#2}%<<
  \pgfutil@namedef{tikz@special@arrow@end<<}{tikze@>>@#2}%<<
}

\def\tikz@processarrows#1{%
  \def\tikz@current@arrows{#1}%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
  \else%
    \tikz@@processarrows#1\@nil
  \fi%
}
\def\tikz@@processarrows#1-#2\@nil{%
  \expandafter\ifx\csname tikz@special@arrow@start#1\endcsname\relax%
    \pgfsetarrowsstart{#1}
  \else%
    \pgfsetarrowsstart{\csname tikz@special@arrow@start#1\endcsname}%
  \fi%
  \expandafter\ifx\csname tikz@special@arrow@end#2\endcsname\relax%
    \pgfsetarrowsend{#2}
  \else%
    \pgfsetarrowsend{\csname tikz@special@arrow@end#2\endcsname}%
  \fi%
}

\tikz@set@pointed{\pgf@arrows@invertto}{to}
\def\tikz@current@arrows{-}

% Parabola options
\tikzoption{bend}{\tikz@scan@one@point\tikz@set@parabola@bend#1\relax}%
\tikzoption{bend pos}{\def\tikz@parabola@bend@factor{#1}}
\tikzoption{parabola height}{%
  \def\tikz@parabola@bend@factor{.5}%
  \def\tikz@parabola@bend{\pgfpointadd{\pgfpoint{0pt}{#1}}{\tikz@last@position@saved}}}

\def\tikz@parabola@bend{\tikz@last@position@saved}
\def\tikz@parabola@bend@factor{0}

\def\tikz@set@parabola@bend#1{\def\tikz@parabola@bend{#1}}

% Axis options
\tikzoption{domain}{\def\tikz@plot@domain{#1}\expandafter\tikz@plot@samples@recalc\tikz@plot@domain\relax}
\tikzoption{range}{\def\tikz@plot@range{#1}}

% Plot options
\tikzoption{smooth}[]{\let\tikz@plot@handler=\pgfplothandlercurveto}
\tikzoption{smooth cycle}[]{\let\tikz@plot@handler=\pgfplothandlerclosedcurve}
\tikzoption{sharp plot}[]{\let\tikz@plot@handler\pgfplothandlerlineto}

\tikzoption{tension}{\pgfsetplottension{#1}}

\tikzoption{xcomb}[]{\let\tikz@plot@handler=\pgfplothandlerxcomb}
\tikzoption{ycomb}[]{\let\tikz@plot@handler=\pgfplothandlerycomb}
\tikzoption{polar comb}[]{\let\tikz@plot@handler=\pgfplothandlerpolarcomb}

\tikzoption{raw gnuplot}[true]{\csname tikz@plot@raw@gnuplot#1\endcsname}
\tikzoption{prefix}{\def\tikz@plot@prefix{#1}}
\tikzoption{id}{\def\tikz@plot@id{#1}}

\tikzoption{samples}{\def\tikz@plot@samples{#1}\expandafter\tikz@plot@samples@recalc\tikz@plot@domain\relax}
\tikzoption{samples at}{\def\tikz@plot@samplesat{#1}}
\tikzoption{parametric}[true]{\csname tikz@plot@parametric#1\endcsname}

\tikzoption{variable}{\def\tikz@plot@var{#1}}

\tikzoption{only marks}[]{\let\tikz@plot@handler\pgfplothandlerdiscard}

\tikzoption{mark}{\def\tikz@plot@mark{#1}}
\tikzoption{mark options}{\def\tikz@plot@mark@options{#1}}
\tikzoption{mark size}{\pgfsetplotmarksize{#1}}

\tikzoption{mark indices}{\def\tikz@mark@list{#1}}
\tikzoption{mark phase}{\pgfsetplotmarkphase{#1}}
\tikzoption{mark repeat}{\pgfsetplotmarkrepeat{#1}}

\let\tikz@mark@list=\pgfutil@empty

\let\tikz@plot@mark@options=\pgfutil@empty

\let\tikz@plot@handler=\pgfplothandlerlineto
\let\tikz@plot@mark=\pgfutil@empty

\def\tikz@plot@samples{25}
\def\tikz@plot@domain{-5:5}
\def\tikz@plot@var{\x}
\def\tikz@plot@samplesat{-5,-4.6,...,5}
\def\tikz@plot@samples@recalc#1:#2\relax{%
  \pgfmathparse{#1}%
  \let\tikz@temp@start=\pgfmathresult%
  \pgfmathparse{#2}%
  \let\tikz@temp@end=\pgfmathresult%
  \pgfmathparse{\tikz@temp@start+(\tikz@temp@end-\tikz@temp@start)/\tikz@plot@samples}%
  \edef\tikz@plot@samplesat{\tikz@temp@start,\pgfmathresult,...,\tikz@temp@end}%
}


\def\tikz@plot@prefix{\jobname.}
\def\tikz@plot@id{pgf-plot}

\newif\iftikz@plot@parametric
\newif\iftikz@plot@raw@gnuplot


% To options
\tikzoption{to path}{\def\tikz@to@path{#1}}

\def\tikz@to@path{-- (\tikztotarget) \tikztonodes}



% Tree options
\newif\iftikz@child@missing
\pgfkeys{/tikz/missing/.is if=tikz@child@missing}

\tikzoption{edge from parent path}{\def\tikz@edge@to@parent@path{#1}}

\tikzoption{parent anchor}{\def\tikzparentanchor{.#1}\ifx\tikzparentanchor\tikz@border@text\let\tikzparentanchor\pgfutil@empty\fi}
\tikzoption{child anchor}{\def\tikzchildanchor{.#1}\ifx\tikzchildanchor\tikz@border@text\let\tikzchildanchor\pgfutil@empty\fi}

\tikzoption{level distance}{\pgfmathsetlength\tikzleveldistance{#1}}
\tikzoption{sibling distance}{\pgfmathsetlength\tikzsiblingdistance{#1}}

\tikzoption{growth function}{\let\tikz@grow=#1}
\tikzoption{growth parent anchor}{\def\tikz@growth@anchor{#1}}
\tikzoption{grow}{\tikz@set@growth{#1}\edef\tikz@special@level{\the\tikztreelevel}}%
\tikzoption{grow'}{\tikz@set@growth{#1}\tikz@swap@growth\edef\tikz@special@level{\the\tikztreelevel}}%

\def\tikz@growth@anchor{center}

\def\tikz@special@level{-1}% never

\def\tikz@swap@growth{%
  % Swap left and right
  \let\tikz@temp=\tikz@angle@grow@right%
  \let\tikz@angle@grow@right=\tikz@angle@grow@left%
  \let\tikz@angle@grow@left=\tikz@temp%
}%

\def\tikz@set@growth#1{%
  \let\tikz@grow=\tikz@grow@direction%
  \expandafter\ifx\csname tikz@grow@direction@#1\endcsname\relax%
    \c@pgf@counta=#1\relax%
  \else%
    \c@pgf@counta=\csname tikz@grow@direction@#1\endcsname%
  \fi%
  \edef\tikz@angle@grow{\the\c@pgf@counta}%
  \advance\c@pgf@counta by-90\relax%
  \edef\tikz@angle@grow@left{\the\c@pgf@counta}%
  \advance\c@pgf@counta by180\relax%
  \edef\tikz@angle@grow@right{\the\c@pgf@counta}%
}

\def\tikz@border@text{.border}
\let\tikzparentanchor=\pgfutil@empty
\let\tikzchildanchor=\pgfutil@empty
\def\tikz@edge@to@parent@path{(\tikzparentnode\tikzparentanchor) -- (\tikzchildnode\tikzchildanchor)}

\tikzleveldistance=15mm
\tikzsiblingdistance=15mm

\def\tikz@grow@direction@down{-90}
\def\tikz@grow@direction@up{90}
\def\tikz@grow@direction@left{180}
\def\tikz@grow@direction@right{0}

\def\tikz@grow@direction@south{-90}
\def\tikz@grow@direction@north{90}
\def\tikz@grow@direction@west{180}
\def\tikz@grow@direction@east{0}

\expandafter\def\csname tikz@grow@direction@north east\endcsname{45}
\expandafter\def\csname tikz@grow@direction@north west\endcsname{135}
\expandafter\def\csname tikz@grow@direction@south east\endcsname{-45}
\expandafter\def\csname tikz@grow@direction@south west\endcsname{-135}

\def\tikz@grow@direction{%
  \pgftransformshift{\pgfpointpolar{\tikz@angle@grow}{\tikzleveldistance}}%
  \ifnum\tikztreelevel=\tikz@special@level%
  \else%
    \pgf@xc=.5\tikzsiblingdistance%
    \c@pgf@counta=\tikznumberofchildren%
    \advance\c@pgf@counta by1\relax%
    \pgfutil@tempdima=\c@pgf@counta\pgf@xc%
    \pgftransformshift{\pgfpointpolar{\tikz@angle@grow@left}{\pgfutil@tempdima}}%
    \pgftransformshift{\pgfpointpolar{\tikz@angle@grow@right}{\tikznumberofcurrentchild\tikzsiblingdistance}}%
  \fi%
}

\tikzset{grow=down}


% Snakes are in a lib:
\tikzset{snake/.code=\PackageError{tikz}{You need to say \string\usetikzlibrary{snakes}}{}}

% Decorations
\tikzset{decorate/.code=\PackageError{tikz}{You need to load a  decoration library}{}}

% Matrix options
\usepgfmodule{matrix}

\tikzoption{matrix}[true]{\csname tikz@is@matrix#1\endcsname}

\tikzoption{matrix anchor}{\def\tikz@matrix@anchor{#1}}

\tikzoption{column sep}{\def\pgfmatrixcolumnsep{#1}}
\tikzoption{row sep}{\def\pgfmatrixrowsep{#1}}

\tikzoption{cells}{\tikzstyle{every cell}+=[#1]}

\tikzoption{ampersand replacement}{\def\tikz@ampersand@replacement{#1}}

\newif\iftikz@is@matrix
\let\tikz@matrix@anchor=\pgfutil@empty
\let\tikz@ampersand@replacement=\pgfutil@empty


% Execute option
\tikzoption{execute at begin picture}{\expandafter\def\expandafter\tikz@atbegin@picture\expandafter{\tikz@atbegin@picture#1}}
\tikzoption{execute at end picture}{\expandafter\def\expandafter\tikz@atend@picture\expandafter{\tikz@atend@picture#1}}
\tikzoption{execute at begin scope}{\expandafter\def\expandafter\tikz@atbegin@scope\expandafter{\tikz@atbegin@scope#1}}
\tikzoption{execute at end scope}{\expandafter\def\expandafter\tikz@atend@scope\expandafter{\tikz@atend@scope#1}}
\tikzoption{execute at begin to}{\expandafter\def\expandafter\tikz@atbegin@to\expandafter{\tikz@atbegin@to#1}}
\tikzoption{execute at end to}{\expandafter\def\expandafter\tikz@atend@to\expandafter{\tikz@atend@to#1}}
\tikzoption{execute at begin node}{\expandafter\def\expandafter\tikz@atbegin@node\expandafter{\tikz@atbegin@node#1}}
\tikzoption{execute at end node}{\expandafter\def\expandafter\tikz@atend@node\expandafter{\tikz@atend@node#1}}
\tikzoption{execute at begin cell}{\expandafter\def\expandafter\tikz@atbegin@cell\expandafter{\tikz@atbegin@cell#1}}
\tikzoption{execute at end cell}{\expandafter\def\expandafter\tikz@atend@cell\expandafter{\tikz@atend@cell#1}}
\tikzoption{execute at empty cell}{\expandafter\def\expandafter\tikz@at@emptycell\expandafter{\tikz@at@emptycell#1}}

\let\tikz@atbegin@picture=\pgfutil@empty
\let\tikz@atend@picture=\pgfutil@empty
\let\tikz@atbegin@scope=\pgfutil@empty
\let\tikz@atend@scope=\pgfutil@empty
\let\tikz@atbegin@to=\pgfutil@empty
\let\tikz@atend@to=\pgfutil@empty
\let\tikz@atbegin@node=\pgfutil@empty
\let\tikz@atend@node=\pgfutil@empty
\let\tikz@atbegin@cell=\pgfutil@empty
\let\tikz@atend@cell=\pgfutil@empty
\let\tikz@at@emptycell=\pgfutil@empty


% Pre and post actions
\tikzset{preaction/.code=\expandafter\def\expandafter\tikz@preactions\expandafter{\tikz@preactions\tikz@extra@preaction{#1}}}
\tikzset{postaction/.code=\expandafter\def\expandafter\tikz@postactions\expandafter{\tikz@postactions\tikz@extra@postaction{#1}}}
\let\tikz@preactions=\pgfutil@empty
\let\tikz@postactions=\pgfutil@empty

% Styles
\tikzoption{set style}{\tikzstyle#1}

% Handled in a special way.
\def\tikzstyle{\pgfutil@ifnextchar\bgroup\tikz@style@parseA\tikz@style@parseB}
\def\tikz@style@parseB#1={\tikz@style@parseA{#1}=}
\def\tikz@style@parseA#1#2=#3[#4]{% check for an optional argument
  \pgfutil@in@[{#2}%]
  \ifpgfutil@in@%
    \tikz@style@parseC{#1}#2={#4}%
  \else%
    \tikz@style@parseD{#1}#2={#4}%
  \fi%
}%

\def\tikz@style@parseC#1[#2]#3=#4{%
  \pgfkeys{/tikz/#1/.default={#2}}%
  \pgfutil@in@+{#3}%
  \ifpgfutil@in@%
    \pgfkeys{/tikz/#1/.append style={#4}}%
  \else%
    \pgfkeys{/tikz/#1/.style={#4}}%
  \fi}
\def\tikz@style@parseD#1#2=#3{%
  \pgfutil@in@+{#2}%
  \ifpgfutil@in@%
    \pgfkeys{/tikz/#1/.append style={#3}}%
  \else%
    \pgfkeys{/tikz/#1/.style={#3}}%
  \fi}


%
%
% Predefined styles
%
%

\tikzstyle{help lines}=              [color=gray,line width=0.2pt]

\tikzstyle{every picture}=           []
\tikzstyle{every path}=              []
\tikzstyle{every scope}=             []
\tikzstyle{every plot}=              []
\tikzstyle{every node}=              []
\tikzstyle{every child}=             []
\tikzstyle{every child node}=        []
\tikzstyle{every to}=                []
\tikzstyle{every cell}=              []
\tikzstyle{every matrix}=            []
\tikzstyle{every edge}=              [draw]
\tikzstyle{every label}=             [draw=none,fill=none]
\tikzstyle{every pin}=               [draw=none,fill=none]
\tikzstyle{every pin edge}=          [help lines]

\tikzstyle{ultra thin}=              [line width=0.1pt]
\tikzstyle{very thin}=               [line width=0.2pt]
\tikzstyle{thin}=                    [line width=0.4pt]
\tikzstyle{semithick}=               [line width=0.6pt]
\tikzstyle{thick}=                   [line width=0.8pt]
\tikzstyle{very thick}=              [line width=1.2pt]
\tikzstyle{ultra thick}=             [line width=1.6pt]

\tikzstyle{solid}=                   [dash pattern=]
\tikzstyle{dotted}=                  [dash pattern=on \pgflinewidth off 2pt]
\tikzstyle{densely dotted}=          [dash pattern=on \pgflinewidth off 1pt]
\tikzstyle{loosely dotted}=          [dash pattern=on \pgflinewidth off 4pt]
\tikzstyle{dashed}=                  [dash pattern=on 3pt off 3pt]
\tikzstyle{densely dashed}=          [dash pattern=on 3pt off 2pt]
\tikzstyle{loosely dashed}=          [dash pattern=on 3pt off 6pt]

\tikzstyle{transparent}=             [opacity=0]
\tikzstyle{ultra nearly transparent}=[opacity=0.05]
\tikzstyle{very nearly transparent}= [opacity=0.1]
\tikzstyle{nearly transparent}=      [opacity=0.25]
\tikzstyle{semitransparent}=         [opacity=0.5]
\tikzstyle{nearly opaque}=           [opacity=0.75]
\tikzstyle{very nearly opaque}=      [opacity=0.9]
\tikzstyle{ultra nearly opaque}=     [opacity=0.95]
\tikzstyle{opaque}=                  [opacity=1]

\tikzstyle{at start}=                [pos=0]
\tikzstyle{very near start}=         [pos=0.125]
\tikzstyle{near start}=              [pos=0.25]
\tikzstyle{midway}=                  [pos=0.5]
\tikzstyle{near end}=                [pos=0.75]
\tikzstyle{very near end}=           [pos=0.875]
\tikzstyle{at end}=                  [pos=1]

\tikzstyle{bend at start}=           [bend pos=0,bend={+(0,0)}]
\tikzstyle{bend at end}=             [bend pos=1,bend={+(0,0)}]

\tikzstyle{edge from parent}=        [draw]



%
% Setting keys
%

\pgfkeys{/tikz/style/.style=#1}

\pgfkeys{/tikz/.unknown/.code=%
  % Is it a pgf key?
  \let\tikz@key\pgfkeyscurrentname% 
  \pgfkeys{/pgf/\tikz@key/.try={#1}}%
  \ifpgfkeyssuccess%
  \else%
    \expandafter\pgfutil@in@\expandafter!\expandafter{\tikz@key}%
    \ifpgfutil@in@%
      % this is a color!
      \expandafter\tikz@addoption\expandafter{\expandafter\pgfutil@color\expandafter{\tikz@key}}%
      \edef\tikz@textcolor{\tikz@key}%
    \else%
      \pgfutil@doifcolorelse{\tikz@key}
      { %     
        \expandafter\tikz@addoption\expandafter{\expandafter\pgfutil@color\expandafter{\tikz@key}}%
        \edef\tikz@textcolor{\tikz@key}%
      }%
      {%
        % Ok, second chance: This might be an arrow specification:
        \expandafter\pgfutil@in@\expandafter-\expandafter{\tikz@key}
        \ifpgfutil@in@%
          % Ah, an arrow spec!
          \expandafter\tikz@processarrows\expandafter{\tikz@key}%
        \else%
          % Ok, third chance: A shape!
          \expandafter\ifx\csname pgf@sh@s@\tikz@key\endcsname\relax%
            \pgfkeys{/errors/unknown key={/tikz/\tikz@key}{#1}}%
          \else%
            \edef\tikz@shape{\tikz@key}%
          \fi%
        \fi%
      }%
    \fi%
  \fi%
}


%
% Main TikZ Environment
%

\def\tikzpicture{\pgfutil@ifnextchar[\tikz@picture{\tikz@picture[]}}%}
\def\tikz@picture[#1]{%
  \pgfpicture%
  \let\tikz@atbegin@picture=\pgfutil@empty%
  \let\tikz@atend@picture=\pgfutil@empty%
  \let\tikz@transform=\relax%
  \tikz@installcommands\scope[every picture,#1]%
  \expandafter\tikz@atbegin@picture%
  \tikz@lib@scope@check%
}
\def\endtikzpicture{%
    \tikz@atend@picture%
    \global\let\pgf@shift@baseline=\pgf@baseline%
    \global\let\pgf@remember@smuggle=\ifpgfrememberpicturepositiononpage%
    \endscope%
    \let\pgf@baseline=\pgf@shift@baseline%
    \let\ifpgfrememberpicturepositiononpage=\pgf@remember@smuggle%
  \endpgfpicture}
  

% Inlined picture
%
% #1 - some code to be put in a tikzpicture environment.
%
% If the command is not followed by braces, everything up to the next
% semicolon is used as argument.
%
% Example:
%
% The rectangle \tikz{\draw (0,0) rectangle (1em,1ex)} has width 1em and
% height 1ex.

\def\tikz{\pgfutil@ifnextchar[{\tikz@opt}{\tikz@opt[]}}
\def\tikz@opt[#1]{\tikzpicture[#1]\pgfutil@ifnextchar\bgroup{\tikz@}{\tikz@@}}
\def\tikz@#1{#1\endtikzpicture}
\def\tikz@@{%
  \let\tikz@next=\tikz@collectnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@next=\tikz@collectactivesemicolon%
  \fi%
  \tikz@next}
\def\tikz@collectnormalsemicolon#1;{#1;\endtikzpicture}
{
  \catcode`\;=\active
  \gdef\tikz@collectactivesemicolon#1;{#1;\endtikzpicture}
}



%
% Environment for scoping graphic state settings
%
\def\tikz@scope@env{\pgfutil@ifnextchar[\tikz@@scope@env{\tikz@@scope@env[]}}
\def\tikz@@scope@env[#1]{%
  \pgfscope%
  \begingroup%
  \let\tikz@atbegin@scope=\pgfutil@empty%
  \let\tikz@atend@scope=\pgfutil@empty%
  \let\tikz@options=\pgfutil@empty%
  \let\tikz@mode=\pgfutil@empty%
  \tikz@transparency@groupfalse%
  \tikzset{every scope/.try,#1}%
  \tikz@options%
  \iftikz@transparency@group\pgftransparencygroup\fi%
  \expandafter\tikz@atbegin@scope%
  \tikz@lib@scope@check%
}
\def\endtikz@scope@env{%
  \tikz@atend@scope%
  \iftikz@transparency@group\endpgftransparencygroup\fi%
  \endgroup%
  \endpgfscope%
  \tikz@lib@scope@check%
}

%
% Install the abbreviated commands
%
\def\tikz@installcommands{%
  \ifnum\the\catcode`\;=\active\relax\expandafter\let\expandafter\tikz@origsemi\expandafter=\tikz@activesemicolon\fi%
  \ifnum\the\catcode`\:=\active\relax\expandafter\let\expandafter\tikz@origcolon\expandafter=\tikz@activecolon\fi%
  \ifnum\the\catcode`\|=\active\relax\expandafter\let\expandafter\tikz@origbar\expandafter=\tikz@activebar\fi%
  \let\tikz@origscope=\scope%
  \let\tikz@origendscope=\endscope%
  \let\tikz@origstartscope=\startscope%
  \let\tikz@origstopscope=\stopscope%
  \let\tikz@origpath=\path%
  \let\tikz@origagainpath=\againpath%
  \let\tikz@origdraw=\draw%
  \let\tikz@origpattern=\pattern%
  \let\tikz@origfill=\fill%
  \let\tikz@origfilldraw=\filldraw%
  \let\tikz@origshade=\shade%
  \let\tikz@origshadedraw=\shadedraw%
  \let\tikz@origclip=\clip%
  \let\tikz@origuseasboundingbox=\useasboundingbox%
  \let\tikz@orignode=\node%
  \let\tikz@origcoordinate=\coordinate%
  \let\tikz@origmatrix=\matrix%
  \let\tikz@origcalendar=\calendar%
  %
  \tikz@deactivatthings%
  %
  \let\scope=\tikz@scope@env%
  \let\endscope=\endtikz@scope@env%
  \let\startscope=\scope%
  \let\stopscope=\endscope%
  \let\path=\tikz@command@path%
  \let\againpath=\tikz@command@againpath%
  %
  \def\draw{\path[draw]}
  \def\pattern{\path[pattern]}
  \def\fill{\path[fill]}
  \def\filldraw{\path[fill,draw]}
  \def\shade{\path[shade]}
  \def\shadedraw{\path[shade,draw]}
  \def\clip{\path[clip]}
  \def\useasboundingbox{\path[use as bounding box]}
  \def\node{\tikz@path@overlay{node}}
  \def\coordinate{\tikz@path@overlay{coordinate}}
  \def\matrix{\tikz@path@overlay{node[matrix]}}
  \def\calendar{\tikz@lib@cal@calendar}%
}
\ifx\tikz@lib@cal@calendar\@undefined
\def\tikz@lib@cal@calendar{\PackageError{tikz}{You need to load the calendar library}{}}
\fi

\def\tikz@path@overlay#1{%
  \let\tikz@signal@path=\tikz@signal@path% for detection at begin of matrix cell
  \pgfutil@ifnextchar<{\tikz@path@overlayed{#1}}{\path #1}}
\def\tikz@path@overlayed#1<#2>{\path<#2> #1}

\def\tikz@uninstallcommands{%
  \ifnum\the\catcode`\;=\active\relax\expandafter\let\tikz@activesemicolon=\tikz@origsemi\fi%
  \ifnum\the\catcode`\:=\active\relax\expandafter\let\tikz@activecolon=\tikz@origcolon\fi%
  \ifnum\the\catcode`\|=\active\relax\expandafter\let\tikz@activebar=\tikz@origbar\fi%
  \let\scope=\tikz@origscope%
  \let\endscope=\tikz@origendscope%
  \let\startscope=\tikz@origstartscope%
  \let\stopscope=\tikz@origstopscope%
  \let\path=\tikz@origpath%
  \let\againpath=\tikz@origagainpath%
  \let\draw=\tikz@origdraw%
  \let\pattern=\tikz@origpattern%
  \let\fill=\tikz@origfill%
  \let\filldraw=\tikz@origfilldraw%
  \let\shade=\tikz@origshade%
  \let\shadedraw=\tikz@origshadedraw%
  \let\clip=\tikz@origclip%
  \let\useasboundingbox=\tikz@origuseasboundingbox%
  \let\node=\tikz@orignode%
  \let\coordinate=\tikz@origcoordinate%
  \let\matrix=\tikz@origmatrix%
  \let\calendar=\tikz@origcalendar%
}


{
  \catcode`\;=12
  \gdef\tikz@nonactivesemicolon{;}
  \catcode`\:=12
  \gdef\tikz@nonactivecolon{:}
  \catcode`\|=12
  \gdef\tikz@nonactivebar{|}
  \catcode`\;=\active
  \catcode`\:=\active
  \catcode`\|=\active
  \catcode`\"=\active
  \gdef\tikz@activesemicolon{;}%
  \gdef\tikz@activecolon{:}%
  \gdef\tikz@activebar{|}%
  \gdef\tikz@activequotes{"}%
  \gdef\tikz@deactivatthings{%
    \def;{\tikz@nonactivesemicolon}
    \def:{\tikz@nonactivecolon}
    \def|{\tikz@nonactivebar}
  }
}





% Constructs a path and draws/fills them according to the current
% settings.  

\def\tikz@command@path{%
  \let\tikz@signal@path=\tikz@signal@path% for detection at begin of matrix cell
  \pgfutil@ifnextchar[{\tikz@check@earg}%]
  {\pgfutil@ifnextchar<{\tikz@doopt}{\tikz@@command@path}}}
\def\tikz@signal@path{\tikz@signal@path}%
\def\tikz@check@earg[#1]{%
  \pgfutil@ifnextchar<{\tikz@swap@args[#1]}{\tikz@@command@path[#1]}}
\def\tikz@swap@args[#1]<#2>{\tikz@command@path<#2>[#1]}

\def\tikz@doopt{%
  \let\tikz@next=\tikz@eargnormalsemicolon%
  \ifnum\the\catcode`\;=\active\relax%
    \let\tikz@next=\tikz@eargactivesemicolon%
  \fi%
  \tikz@next}
\long\def\tikz@eargnormalsemicolon<#1>#2;{\only<#1>{\tikz@@command@path#2;}}
{
  \catcode`\;=\active
  \long\global\def\tikz@eargactivesemicolon<#1>#2;{\only<#1>{\tikz@@command@path#2;}}
}

\def\tikz@@command@path{%
  \edef\tikzscope@linewidth{\the\pgflinewidth}%
  \begingroup%
    \let\tikz@options=\pgfutil@empty%
    \let\tikz@mode=\pgfutil@empty%
    \let\tikz@moveto@waiting=\relax%
    \let\tikz@timer=\relax%
    \let\tikz@collected@onpath=\pgfutil@empty%
    \let\tikz@preactions=\pgfutil@empty%
    \let\tikz@postactions=\pgfutil@empty%
    \tikz@snakedfalse%
    \tikz@decoratepathfalse%
    \tikz@node@is@a@labelfalse%
    \tikz@expandcount=1000\relax%
    \tikz@lastx=0pt%
    \tikz@lasty=0pt%
    \tikz@lastxsaved=0pt%
    \tikz@lastysaved=0pt%
    \tikzset{every path/.try}%
    \tikz@scan@next@command%
}
\def\tikz@scan@next@command{%
  \ifx\tikz@collected@onpath\pgfutil@empty%
  \else%
    \tikz@invoke@collected@onpath%
  \fi%
  \afterassignment\tikz@handle\let\@let@token=%
}
\newcount\tikz@expandcount

% Central dispatcher for commands
\def\tikz@handle{%
  \let\@next=\tikz@expand%
  \ifx\@let@token(%)
    \let\@next=\tikz@movetoabs%
  \else%
    \ifx\@let@token+%
      \let\@next=\tikz@movetorel%
    \else%
      \ifx\@let@token-%
        \let\@next=\tikz@lineto%
      \else%
        \ifx\@let@token.%
          \let\@next=\tikz@dot%
        \else%
          \ifx\@let@token r%
            \let\@next=\tikz@rect%
          \else%
            \ifx\@let@token n%
              \let\@next=\tikz@fig%
            \else%
              \ifx\@let@token[%]
                \let\@next=\tikz@parse@options%
              \else%
                \ifx\@let@token c%
                  \let\@next=\tikz@cchar%
                \else%
                  \ifx\@let@token\bgroup%
                    \let\@next=\tikz@beginscope%
                  \else%
                    \ifx\@let@token\egroup%
                      \let\@next=\tikz@endscope%
                    \else%
                      \ifx\@let@token;%
                        \let\@next=\tikz@finish%
                      \else%
                        \let\@next=\tikz@handle@more%
                      \fi%
                    \fi%
                  \fi%
                \fi%
              \fi%
            \fi%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \@next%
}

% Continued...
\def\tikz@handle@more{%
  \ifx\@let@token a%
    \let\@next=\tikz@arcA%
  \else%
    \ifx\@let@token e%
      \let\@next=\tikz@e@char%
    \else%
      \ifx\@let@token g%
        \let\@next=\tikz@grid%
      \else%
        \ifx\@let@token s%
           \let\@next=\tikz@sine%
        \else%
          \ifx\@let@token |%
             \let\@next=\tikz@vh@lineto%
          \else%
            \ifx\@let@token p%
              \let\@next=\tikz@pchar%
              \pgfsetmovetofirstplotpoint%
            \else%
              \ifx\@let@token t%
                \let\@next=\tikz@to%
              \else%
                \ifx\@let@token\pgfextra%
                  \let\@next=\tikz@extra%
                \else%
                  \ifx\@let@token\foreach%
                    \let\@next=\tikz@foreach%
                  \else%
                    \ifx\@let@token\pgf@stop%
                      \let\@next=\relax%
                    \else%
                      \ifx\@let@token\par%
                        \let\@next=\tikz@scan@next@command%
                      \else%
                        \ifx\@let@token d%
                          \let\@next=\tikz@decoration%
                        \else%
                          \ifx\@let@token l%
                            \let\@next=\tikz@let@command%
                          \else%
                            \let\@next=\tikz@expand%
                          \fi%      
                        \fi%      
                      \fi%      
                    \fi%      
                  \fi%      
                \fi%      
              \fi%      
            \fi%  
          \fi%  
        \fi%
      \fi%
    \fi%
  \fi%
  \@next%
}

\def\tikz@pchar{\pgfutil@ifnextchar l{\tikz@plot}{\tikz@parabola}}
\def\tikz@cchar{%
  \pgfutil@ifnextchar i{\tikz@circle}%
  {\pgfutil@ifnextchar h{\tikz@children}{\tikz@cochar}}}%
\def\tikz@cochar o{%
  \pgfutil@ifnextchar o{\tikz@coordinate}{\tikz@cosine}}
\def\tikz@e@char{%
  \pgfutil@ifnextchar l{\tikz@ellipse}{\tikz@@e@char}}%
\def\tikz@@e@char dge{%
  \pgfutil@ifnextchar f{\tikz@edgetoparent}{\tikz@edge@plain}}%


\def\tikz@finish{%
  % Rendering pipeline 
  % 
  % Step 1: Decorate path
  % 
  \iftikz@decoratepath%
    \tikz@lib@dec@decorate@path%
  \fi%
  % 
  % Step 1: Preactions
  % 
  \pgfsyssoftpath@getcurrentpath\tikz@actions@path%
  \edef\tikz@restorepathsize{%
    \global\pgf@pathmaxx=\the\pgf@pathmaxx%
    \global\pgf@pathmaxy=\the\pgf@pathmaxy%
    \global\pgf@pathminx=\the\pgf@pathminx%
    \global\pgf@pathminy=\the\pgf@pathminy%
  }%
  \tikz@preactions%
  %
  % Reset modes
  %
  \tikz@mode@fillfalse%
  \tikz@mode@drawfalse%
  \tikz@mode@doublefalse%
  \tikz@mode@clipfalse%
  \tikz@mode@boundaryfalse%
  \tikz@mode@fade@pathfalse%
  \tikz@mode@fade@scopefalse%
  \edef\tikz@pathextend{%
    {\noexpand\pgfqpoint{\the\pgf@pathminx}{\the\pgf@pathminy}}%
    {\noexpand\pgfqpoint{\the\pgf@pathmaxx}{\the\pgf@pathmaxy}}%
  }%
  \tikz@mode% installs the mode settings
  % Path fading counts as an option:
  \iftikz@mode@fade@path%
    \tikz@addoption{%
      \iftikz@fade@adjust%
        \pgfsetfadingforcurrentpath{\tikz@path@fading}{\tikz@do@fade@transform}%
      \else%
        \pgfsetfading{\tikz@path@fading}{\tikz@do@fade@transform}%
      \fi%
      \tikz@mode@fade@pathfalse% no more fading...
    }%
  \fi%
  % Rendering pipeline 
  %
  % Step 2: Install scope fading
  %
  \iftikz@mode@fade@scope%
    \iftikz@fade@adjust%
      \pgfsetfadingforcurrentpath{\tikz@scope@fading}{\tikz@do@fade@transform}%
    \else%
      \pgfsetfading{\tikz@scope@fading}{\tikz@do@fade@transform}%
    \fi%
    \tikz@mode@fade@scopefalse%
  \fi%
  %
  % Step 3: Setup options
  % 
  \ifx\tikz@options\pgfutil@empty%
  \else%
    \pgfsys@beginscope%
      \begingroup%
      \tikz@options%
  \fi%
  % 
  % Step 4: Do a fill if shade follows.
  %
  \iftikz@mode@fill%
    \iftikz@mode@shade%
      \pgfsyssoftpath@getcurrentpath\tikz@temppath
      \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
      \pgfsyssoftpath@setcurrentpath\tikz@temppath%
      \pgfsyssoftpath@invokecurrentpath%
      \pgfsys@fill%
      \tikz@mode@fillfalse% no more filling...
    \fi%
  \fi%
  % 
  % Step 5: Do a shade if necessary.
  %
  \iftikz@mode@shade%
    \pgfsyssoftpath@getcurrentpath\tikz@temppath
    \pgfprocessround{\tikz@temppath}{\tikz@temppath}% change the path
    \pgfsyssoftpath@setcurrentpath\tikz@temppath%
    \pgfshadepath{\tikz@shading}{\tikz@shade@angle}%
    \tikz@mode@shadefalse% no more shading...
  \fi%
  % 
  % Step 6: Double stroke, if necessary
  %
  \iftikz@mode@draw%
    \iftikz@mode@double%
      % Change line width
      \begingroup%
        \pgfsys@beginscope%
          \pgf@x=2\pgflinewidth%
          \advance\pgf@x by\tikz@double@width@distance%
          \pgflinewidth=\pgf@x%
          \pgfsetlinewidth{\the\pgflinewidth}%
    \fi%
  \fi%
  % 
  % Step 7: Do stroke/fill/clip as needed
  %
  \edef\tikz@temp{\noexpand\pgfusepath{%
    \iftikz@mode@fill fill,\fi%
    \iftikz@mode@draw draw,\fi%
    \iftikz@mode@clip clip,\fi%
    }}%
  \tikz@temp%
  \tikz@mode@fillfalse% no more filling
  % 
  % Step 8: Double stroke, if necessary
  %
  \iftikz@mode@draw%
    \iftikz@mode@double%
          \pgfsyssoftpath@setcurrentpath\pgf@last@used@path% reinstall
          \pgf@x=\tikz@double@width@distance%
          \pgfsetlinewidth{\the\pgf@x}%
          \pgfsetstrokecolor{\tikz@double@color}%
          \pgfsyssoftpath@flushcurrentpath%
          \pgfsys@stroke%
        \pgfsys@endscope%
        \ifpgf@drawarrows% set in pgfusepath...
          \pgf@add@arrows@as@needed%
        \fi%
      \endgroup%
    \fi%
  \fi%
  \tikz@mode@drawfalse% no more stroking
  %
  % Step 9: Postactions
  %
  \tikz@postactions%
  % 
  % Step 10: Add labels and nodes
  %
  \box\tikz@figbox%
  %
  % Step 11: Close option brace
  %
  \ifx\tikz@options\pgfutil@empty%
  \else%
      \endgroup%
    \pgfsys@endscope%
    \iftikz@mode@clip%
      \PackageError{tikz}{Extra options not allowed for clipping path command.}{}%
    \fi%
  \fi%
  \iftikz@mode@clip%
    \aftergroup\pgf@relevantforpicturesizefalse%
  \fi%
  \iftikz@mode@boundary%
    \aftergroup\pgf@relevantforpicturesizefalse%
  \fi%
  \endgroup%
  \global\pgflinewidth=\tikzscope@linewidth%
  \tikz@lib@scope@check%
}
\let\tikz@lib@scope@check\pgfutil@empty% this is a hook for the scopes library

% Extra actions

\def\tikz@extra@preaction#1{%
  {%
    \pgfsys@beginscope%
      \setbox\tikz@figbox=\box\voidb@x%
      \path[#1];% do extra path
      \pgfsyssoftpath@setcurrentpath\tikz@actions@path% restore
      \tikz@restorepathsize%
    \pgfsys@endscope%
  }%
}

\def\tikz@extra@postaction#1{%
  {%
    \pgfsys@beginscope%
      \setbox\tikz@figbox=\box\voidb@x%
      \tikz@restorepathsize%
      \path[#1]\pgfextra{\pgfsyssoftpath@setcurrentpath\tikz@actions@path};% do extra path
      \pgf@resetpathsizes%
    \pgfsys@endscope%
  }%
}



\def\tikz@skip#1{\tikz@scan@next@command#1}
\def\tikz@expand{%
  \advance\tikz@expandcount by -1%
  \ifnum\tikz@expandcount<0\relax%
    \PackageError{tikz}{Giving up on this path. Did you forget a semicolon?}{}%
    \let\@next=\tikz@finish%
  \else%
    \let\@next=\tikz@@expand
  \fi%
  \@next}

\def\tikz@@expand{%
  \expandafter\tikz@scan@next@command\@let@token}



% Syntax for scopes: 
% {scoped path commands}

\def\tikz@beginscope{\begingroup\tikz@scan@next@command}
\def\tikz@endscope{%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
    \xdef\tikz@scope@save@lastx{\the\tikz@lastx}%
    \xdef\tikz@scope@save@lasty{\the\tikz@lasty}%
  \iftikz@current@point@local%
    \endgroup%
  \else%
      \xdef\tikz@scope@save@lastxsaved{\the\tikz@lastxsaved}%
      \xdef\tikz@scope@save@lastysaved{\the\tikz@lastysaved}%
    \endgroup%
    \tikz@lastxsaved=\tikz@scope@save@lastxsaved%
    \tikz@lastysaved=\tikz@scope@save@lastysaved%
  \fi%
  \tikz@lastx=\tikz@scope@save@lastx%
  \tikz@lasty=\tikz@scope@save@lasty%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \tikz@scan@next@command}


% Syntax for pgfextra: 
% \pgfextra {normal tex text}
% \pgfextra normal tex text \endpgfextra

\def\tikz@extra{\pgfutil@ifnextchar\bgroup\tikz@@extra\relax}
\long\def\tikz@@extra#1{#1\tikz@scan@next@command}
\let\endpgfextra=\tikz@scan@next@command

\def\pgfextra{pgfextra}


% Syntax for \foreach: 
% \foreach \var in {list} {path text}
%
% Example:
%
% \draw (0,0) \foreach \x in {1,2,3} {-- (\x,0) circle (1cm)} -- (5,5);

\def\tikz@foreach{%
  \def\pgffor@beginhook{\setbox\tikz@figbox=\box\tikz@tempbox\expandafter\tikz@scan@next@command\pgfutil@firstofone}%
  \def\pgffor@endhook{\pgfextra{%
      \xdef\tikz@foreach@save@lastx{\the\tikz@lastx}%
      \xdef\tikz@foreach@save@lasty{\the\tikz@lasty}%
      \xdef\tikz@foreach@save@lastxsaved{\the\tikz@lastxsaved}%
      \xdef\tikz@foreach@save@lastysaved{\the\tikz@lastysaved}%
      \global\setbox\tikz@tempbox=\copy\tikz@figbox\pgfutil@gobble}}%
  \def\pgffor@afterhook{%
    \tikz@lastx=\tikz@foreach@save@lastx%
    \tikz@lasty=\tikz@foreach@save@lasty%
    \tikz@lastxsaved=\tikz@foreach@save@lastxsaved%
    \tikz@lastysaved=\tikz@foreach@save@lastysaved%
    \setbox\tikz@figbox=\box\tikz@tempbox\tikz@scan@next@command}%
  \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \foreach}

  
% Syntax for againpath: 
% \againpath \somepathname

\def\tikz@command@againpath#1{%
  \pgfextra{%
    \pgfsyssoftpath@getcurrentpath\tikz@temp%
    \expandafter\pgfutil@g@addto@macro\expandafter\tikz@temp\expandafter{#1}%
    \pgfsyssoftpath@setcurrentpath\tikz@temp%
  }
}




%
% When this if is set, a just-scanned point is a shape and its border
% position still needs to be determined, depending on subsequent
% commands. 
%

\newif\iftikz@shapeborder


% Syntax for moveto: 
% <point>
\def\tikz@movetoabs{\tikz@moveto(}
\def\tikz@movetorel{\tikz@moveto+}
\def\tikz@moveto{%
  \tikz@scan@one@point{\tikz@@moveto}}
\def\tikz@@moveto#1{%
  \tikz@make@last@position{#1}%
  \iftikz@shapeborder%
    % ok, the moveto will have to wait. flag that we have a moveto in
    % wainting:
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%
  \else%
    \pgfpathmoveto{\tikz@last@position}%
    \let\tikz@moveto@waiting=\relax%
  \fi%
  \tikz@scan@next@command%
}

\let\tikz@moveto@waiting=\relax % normally, nothing is waiting...

\def\tikz@flush@moveto{%
  \ifx\tikz@moveto@waiting\relax%
  \else%
    \pgfpathmoveto{\tikz@last@position}%
  \fi%
  \let\tikz@moveto@waiting=\relax%
}


\def\tikz@flush@moveto@toward#1#2#3{%
  % #1 = a point towards which the last moveto should be corrected
  % #2 = a dimension to which the corrected x-coordinate should be stored
  % #3 = a dimension for the corrected y-coordinate
  \ifx\tikz@moveto@waiting\relax%
    % do nothing
  \else%
    \pgf@process{\pgfpointshapeborder{\tikz@moveto@waiting}{#1}}%
    #2=\pgf@x%
    #3=\pgf@y%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \pgfpathmoveto{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi%
  \let\tikz@moveto@waiting=\relax%
}


%
% Collecting labels on the path 
%

\def\tikz@collect@coordinate@onpath#1coordinate{%
  \pgfutil@ifnextchar[{\tikz@@collect@coordinate@opt#1}{\tikz@@collect@coordinate@opt#1[]}}%}
\def\tikz@@collect@coordinate@opt#1[#2]{%
  \pgfutil@ifnextchar({\tikz@@collect@coordinate#1[#2]}{%
  \tikz@collect@label@onpath#1node[shape=coordinate,#2]{}}}%}
\def\tikz@@collect@coordinate#1[#2](#3){%
  \tikz@collect@label@onpath#1node[shape=coordinate,#2](#3){}}

\def\tikz@collect@label@onpath#1node{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath node}%
  \tikz@collect@label@scan#1}

\def\tikz@collect@label@scan#1{%  
  \pgfutil@ifnextchar({\tikz@collect@paran#1}%
  {\pgfutil@ifnextchar[{\tikz@collect@options#1}%
    {\pgfutil@ifnextchar\bgroup{\tikz@collect@arg#1}%
      {#1}}}%
}%}}

\def\tikz@collect@paran#1(#2){%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath(#2)}%
  \tikz@collect@label@scan#1%
}
\def\tikz@collect@options#1[#2]{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath[#2]}%
  \tikz@collect@label@scan#1%
}
\def\tikz@collect@arg#1#2{%
  \expandafter\def\expandafter\tikz@collected@onpath\expandafter{\tikz@collected@onpath{#2}}%
  #1%
}


\def\tikz@invoke@collected@onpath{%
  \tikz@node@is@a@labeltrue%
  \let\tikz@temp=\tikz@collected@onpath%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \expandafter\tikz@scan@next@command\tikz@temp\pgf@stop%
  \tikz@node@is@a@labelfalse%
}




% Syntax for lineto: 
% -- <point>

\def\tikz@lineto{%
  \pgfutil@ifnextchar |%
  {\expandafter\tikz@hv@lineto\pgfutil@gobble}%
  {\expandafter\pgfutil@ifnextchar\tikz@activebar{\expandafter\tikz@hv@lineto\pgfutil@gobble}%
    {\expandafter\tikz@lineto@mid\pgfutil@gobble}}}
\def\tikz@lineto@mid{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@lineto@mid}%
  {%
    \pgfutil@ifnextchar c{\tikz@close}{%
      \pgfutil@ifnextchar p{\pgfsetlinetofirstplotpoint\expandafter\tikz@plot\pgfutil@gobble}%
        {\tikz@scan@one@point{\tikz@@lineto}}}}}
\def\tikz@@lineto#1{%
  % Record the starting point for later labels on the path:
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}
  \iftikz@shapeborder%
    % ok, target is a shape. recalculate end
    \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\tikz@last@position}}%
    \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
    \tikz@flush@moveto@toward{\tikz@last@position}\pgf@x\pgf@y%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \tikz@make@last@position{#1}%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%    
  \else%
    % target is a reasonable point...
    % Record the starting point for later labels on the path:
    \tikz@make@last@position{#1}%
    \tikz@flush@moveto@toward{\tikz@last@position}\pgf@x\pgf@y%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \fi%
  \let\tikz@timer=\tikz@timer@line%
  \tikz@scan@next@command%
}

% snake or lineto?
\def\tikz@path@lineto#1{%
  \iftikz@snaked%
    {
      \pgfsyssoftpathmovetorelevantfalse%
      \pgfpathsnakesto{\tikz@presnake,{\tikz@snake}{\tikz@mainsnakelength}{\noexpand\tikz@snake@install@trans}{},\tikz@postsnake}{#1}%
    }
  \else%
    \pgfpathlineto{#1}%
  \fi%
}

% snake or lineto?
\def\tikz@path@close#1{%
  \iftikz@snaked%
    {%
      \pgftransformreset%
      \pgfpathsnakesto{\tikz@presnake,{\tikz@snake}{\tikz@mainsnakelength}{\noexpand\tikz@snake@install@trans}{},\tikz@postsnake}{#1}%
    }%
  \fi%
  \pgfpathclose%
}


% Syntax for lineto horizontal/vertical: 
% -| <point>

\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar n
  {\tikz@collect@label@onpath\tikz@hv@lineto}
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@hv@lineto}%
    {\tikz@scan@one@point{\tikz@@hv@lineto}}}}
\def\tikz@@hv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@yc=\tikz@lasty%
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@x\pgf@yc%
  \iftikz@shapeborder%
    % ok, target is a shape. have to work now:
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yc}}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@yc}}%
      \tikz@path@lineto{\tikz@last@position}%
      \xdef\tikz@timer@end@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%    
  \else%
    \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@yc}}%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
  \fi%
  \let\tikz@timer=\tikz@timer@hvline%
  \tikz@scan@next@command%
}

% Syntax for lineto vertical/horizontal: 
% |- <point>

\def\tikz@vh@lineto-{\tikz@vh@lineto@next}
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar n
  {\tikz@collect@label@onpath\tikz@vh@lineto@next}
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@vh@lineto@next}%
    {\tikz@scan@one@point\tikz@@vh@lineto}}}
\def\tikz@@vh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx%
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@y%
  \iftikz@shapeborder%
    % ok, target is a shape. have to work now:
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xc}{\tikz@lasty}}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \tikz@path@lineto{\pgfqpoint{\pgf@xc}{\tikz@lasty}}%
      \tikz@path@lineto{\tikz@last@position}%
      \xdef\tikz@timer@end@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%    
  \else%
    \tikz@path@lineto{\pgfqpoint{\pgf@xc}{\tikz@lasty}}%
    \tikz@path@lineto{\tikz@last@position}%
    \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \fi%
  \let\tikz@timer=\tikz@timer@vhline%
  \tikz@scan@next@command%
}

% Syntax for cycle: 
% -- cycle
\def\tikz@close c{%
  \pgfutil@ifnextchar o{\tikz@collect@coordinate@onpath\tikz@lineto@mid c}% oops, a coordinate
  {\tikz@@close c}}%
\def\tikz@@close cycle{%
  \tikz@flush@moveto%
  \tikz@path@close{\expandafter\pgfpoint\pgfsyssoftpath@lastmoveto}%
  \def\pgfstrokehook{}%
  \let\tikz@timer=\@undefined%
  \tikz@scan@next@command%
}


% Syntax for options: 
% [options]
\def\tikz@parse@options#1]{%
  \tikzset{#1}%
  \tikz@lib@dec@hook% for decorations...
  \tikz@scan@next@command%
}
\let\tikz@lib@dec@hook=\relax

% Syntax for edges:
% edge [options] (coordinate)
% edge [options] node {node text} (coordinate)
\def\tikz@edge@plain{%
  \begingroup%
    \tikz@to@use@whom%
    \let\tikz@to@or@edge@function=\tikz@do@edge%
    \tikz@to@or@edge}

% Syntax for to paths:
% to [options] (coordinate)
% to [options] node {node text} (coordinate)
\def\tikz@to o{%
  \tikz@to@use@last@coordinate%
  \let\tikz@to@or@edge@function=\tikz@do@to%
  \tikz@to@or@edge}
  
\def\tikz@to@or@edge{\pgfutil@ifnextchar[\tikz@@to@or@edge{\tikz@@to@or@edge[]}}%}
\def\tikz@@to@or@edge[#1]{%
  \def\tikz@@to@local@options{[#1]}%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \tikz@@to@collect%
}
\def\tikz@@to@collect{%
  \pgfutil@ifnextchar(\tikz@@to@or@edge@coordinate
  {\pgfutil@ifnextchar n{\tikz@collect@label@onpath\tikz@@to@collect}%
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@@to@collect}
      {\PackageError{tikz}{( expected}{}%}
        \tikz@@to@or@edge@coordinate()}}}%
}

\def\tikz@@to@or@edge@coordinate({%
  \pgfutil@ifnextchar${%$
    % Ok, parse directly
    \tikz@scan@one@point\tikz@@to@or@edge@math(%
  }{%
    \pgfutil@ifnextchar[{%]
      \tikz@scan@one@point\tikz@@to@or@edge@math(%
    }{%
      \tikz@@to@or@edge@@coordinate(%
    }%
  }%
}
\def\tikz@@to@or@edge@math#1{% 
  \pgf@process{#1}%
  \edef\tikztotarget{\the\pgf@x,\the\pgf@y}%
  \tikz@to@or@edge@function%
}

\def\tikz@@to@or@edge@@coordinate(#1){%
  \def\tikztotarget{#1}%
  \tikz@to@or@edge@function%
}

\def\tikz@do@edge{%
  \setbox\tikz@figbox=\hbox\bgroup%
    \unhbox\tikz@figbox%
    \hbox\bgroup
      \bgroup%
        \pgfinterruptpath%
          \pgfscope%
            \let\tikz@transform=\pgfutil@empty%
            \let\tikz@options=\pgfutil@empty%
            \let\tikz@tonodes=\tikz@collected@onpath%
            \def\tikztonodes{{\pgfextra{\tikz@node@is@a@labeltrue}\tikz@tonodes}}%
            \let\tikz@collected@onpath=\pgfutil@empty%
            \tikz@options%
            \tikz@transform%            
            % Typeset node:
            \tikz@atbegin@to%
            \path[style=every edge]\tikz@@to@local@options(\tikztostart)\tikz@to@path;%
            \tikz@atend@to%
          \endpgfscope%
        \endpgfinterruptpath%
      \egroup
    \egroup%
  \egroup%
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%  
  \tikz@scan@next@command%  
}

\def\tikz@do@to{%
  \let\tikz@tonodes=\tikz@collected@onpath%
  \def\tikztonodes{{\pgfextra{\tikz@node@is@a@labeltrue}\tikz@tonodes}}%
  \let\tikz@collected@onpath=\pgfutil@empty%
  \tikz@scan@next@command%
  \pgfextra{\tikz@atbegin@to}%
  [style=every to]\tikz@@to@local@options\tikz@to@path%
  \pgfextra{\tikz@atend@to}%
}


\def\tikz@to@use@last@coordinate{%
  \iftikz@shapeborder%
    \edef\tikztostart{\tikz@shapeborder@name}%
  \else%
    \edef\tikztostart{\the\tikz@lastx,\the\tikz@lasty}%
  \fi%
}
\def\tikz@to@use@last@fig@name{%
  \edef\tikztostart{\tikz@to@last@fig@name}%
}



% Syntax for edge from parent: 
% edge from parent [options]
\def\tikz@edgetoparent from parent{\pgfutil@ifnextchar[\tikz@@edgetoparent{\tikz@@edgetoparent[]}}%}
\def\tikz@@edgetoparent[#1]{%
  \let\tikz@edge@to@parent@needed=\pgfutil@empty%
  \tikz@node@is@a@labeltrue%
  \tikz@scan@next@command [style=edge from parent,#1] \tikz@edge@to@parent@path%
}


% Syntax for bezier curves
% .. controls(point) and (point) .. (target)
% .. controls(point) .. (target) 
% .. (target) % currently not supported

\def\tikz@dot.{\tikz@@dot}%
\def\tikz@@dot{%
  \pgfutil@ifnextchar n%
  {\tikz@collect@label@onpath\tikz@@dot}%
  {\pgfutil@ifnextchar c{\tikz@curveto@double}{\tikz@curveto@auto}}}

\def\tikz@curveto@double co{%
  \pgfutil@ifnextchar o{\tikz@collect@coordinate@onpath\tikz@@dot co}
  {\tikz@cureveto@@double}}
\def\tikz@cureveto@@double ntrols#1{%
  \tikz@scan@one@point\tikz@curveA#1%
}
\def\tikz@curveA#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  {%
    \tikz@make@last@position{#1}%
    \xdef\tikz@curve@first{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  }%
  \pgfutil@ifnextchar a
  {\tikz@curveBand}%
  {\let\tikz@curve@second\tikz@curve@first\tikz@curveCdots}%
}
\def\tikz@curveBand and{%
  \tikz@scan@one@point\tikz@curveB%
}
\def\tikz@curveB#1{%
  \def\tikz@curve@second{#1}%
  \tikz@curveCdots}
\def\tikz@curveCdots{%
  \afterassignment\tikz@curveCdot\let\@next=}
\def\tikz@curveCdot.{%
  \ifx\@next.%
  \else%
    \PackageError{tikz}{Dot expected}{}%
  \fi%
  \tikz@updatecurrenttrue%
  \tikz@curveCcheck%
}
\def\tikz@curveCcheck{%
  \pgfutil@ifnextchar n%
  {\tikz@collect@label@onpath\tikz@curveCcheck}
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@curveCcheck}
    {\tikz@scan@one@point\tikz@curveC}}%
}
\def\tikz@curveC#1{%
  \tikz@make@last@position{#1}%
  \edef\tikz@curve@third{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  {%
    \tikz@lastxsaved=\tikz@lastx%
    \tikz@lastysaved=\tikz@lasty%
    \tikz@make@last@position{\tikz@curve@second}%
    \xdef\tikz@curve@second{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  }%
  %
  % Start recalculating things in case start and end are shapes.
  %
  % First, the start:
  \ifx\tikz@moveto@waiting\relax%
  \else%
    \pgf@process{\pgfpointshapeborder{\tikz@moveto@waiting}{\tikz@curve@first}}%
    \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \pgfpathmoveto{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi%
  \let\tikz@timer@cont@one=\tikz@curve@first%
  \let\tikz@timer@cont@two=\tikz@curve@second%    
  % Second, the end:
  \iftikz@shapeborder%
    % ok, target is a shape. recalculate third
    {%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\tikz@curve@second}}%
      \tikz@make@last@position{\pgfqpoint{\pgf@x}{\pgf@y}}%
      \edef\tikz@curve@third{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \pgfpathcurveto{\tikz@curve@first}{\tikz@curve@second}{\tikz@curve@third}%
      \global\let\tikz@timer@end@temp=\tikz@curve@third% move out of group
    }%
    \let\tikz@timer@end=\tikz@timer@end@temp%
    \edef\tikz@moveto@waiting{\tikz@shapeborder@name}%    
  \else%
    \pgfpathcurveto{\tikz@curve@first}{\tikz@curve@second}{\tikz@curve@third}%
    \let\tikz@timer@end=\tikz@curve@third
    \let\tikz@moveto@waiting=\relax%
  \fi%
  \let\tikz@timer=\tikz@timer@curve%  
  \tikz@scan@next@command%
}


% Syntax for rectangles: 
% rectangle <corner point> 
\def\tikz@rect ectangle{%
  \tikz@flush@moveto%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \tikz@@rect}%
\def\tikz@@rect{%
  \pgfutil@ifnextchar n
  {\tikz@collect@label@onpath\tikz@@rect}
  {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\tikz@@rect}%
    {
      \pgf@xa=\tikz@lastx\relax%
      \pgf@ya=\tikz@lasty\relax%
      \tikz@scan@one@point\tikz@rectB}}}
\def\tikz@rectB#1{%
  \tikz@make@last@position{#1}%
  \edef\tikz@timer@end{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \let\tikz@timer=\tikz@timer@line%  
  \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \tikz@path@lineto{\pgfqpoint{\pgf@xa}{\tikz@lasty}}%
  \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \tikz@path@lineto{\pgfqpoint{\tikz@lastx}{\pgf@ya}}%
  \iftikz@snaked% 
    \tikz@path@lineto{\pgfqpoint{\pgf@xa}{\pgf@ya}}%
  \fi%
  \pgfpathclose%
  \pgfpathmoveto{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  \def\pgfstrokehook{}%
  \tikz@scan@next@command%
}



% Syntax for grids: 
% grid <corner point> 
\def\tikz@grid rid{%
  \tikz@flush@moveto%
  \pgf@xa=\tikz@lastx\relax%
  \pgf@ya=\tikz@lasty\relax%
  \pgfutil@ifnextchar[{\tikz@gridA}{\tikz@gridA[]}}%}
\def\tikz@gridA[#1]{%
  \def\tikz@grid@options{#1}%
  \tikz@scan@one@point\tikz@gridB}%
\def\tikz@gridB#1{%
  \tikz@make@last@position{#1}%
  {%
    \expandafter\tikzset\expandafter{\tikz@grid@options}
    \tikz@checkunit{\tikz@grid@x}%
    \iftikz@isdimension%
      \pgf@process{\pgfpoint{\tikz@grid@x}{0pt}}%
    \else%
      \pgf@process{\pgfpointxy{\tikz@grid@x}{0}}%
    \fi%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \tikz@checkunit{\tikz@grid@y}%
    \iftikz@isdimension%
      \pgf@process{\pgfpoint{0pt}{\tikz@grid@y}}%
    \else%
      \pgf@process{\pgfpointxy{0}{\tikz@grid@y}}%
    \fi%
    \advance\pgf@xb by\pgf@x%
    \advance\pgf@yb by\pgf@y%
    \pgfpathgrid[stepx=\pgf@xb,stepy=\pgf@yb]%
      {\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}%
  }
  \tikz@scan@next@command%
}



% Syntax for plot: 
% plot [local options] ...    % starts with a moveto
% -- plot [local options] ... % starts with a lineto
\def\tikz@plot lot{%
  \tikz@flush@moveto%
  \pgfutil@ifnextchar[{\tikz@@plot}{\tikz@@plot[]}}%}
\def\tikz@@plot[#1]{%
  \begingroup%
    \let\tikz@options=\pgfutil@empty%
    \tikzset{every plot/.try}%
    \tikzset{#1}%
    \pgfutil@ifnextchar f{\tikz@plot@f}%
    {\pgfutil@ifnextchar c{\tikz@plot@scan@points}%
      {\pgfutil@ifnextchar ({\tikz@plot@expression}{%
      \PackageError{tikz}{Cannot parse this plotting data}{}%
       \endgroup}}}}
\def\tikz@plot@f f{\pgfutil@ifnextchar i{\tikz@plot@file}{\tikz@plot@function}}

\def\tikz@plot@file ile#1{\def\tikz@plot@data{\pgfplotxyfile{#1}}\tikz@@@plot}%
\def\tikz@plot@scan@points coordinates#1{%
  \pgfplothandlerrecord\tikz@plot@data%
  \pgfplotstreamstart%
  \pgfutil@ifnextchar\pgf@stop{\pgfplotstreamend\expandafter\tikz@@@plot\pgfutil@gobble}
  {\tikz@scan@one@point\tikz@plot@next@point}%
  #1\pgf@stop%
}
\def\tikz@plot@next@point#1{%
  \pgfplotstreampoint{#1}%
  \pgfutil@ifnextchar\pgf@stop{\pgfplotstreamend\expandafter\tikz@@@plot\pgfutil@gobble}%
  {\tikz@scan@one@point\tikz@plot@next@point}%
}  
\def\tikz@plot@function unction#1{%
  \def\tikz@plot@filename{\tikz@plot@prefix\tikz@plot@id}%  
  \iftikz@plot@raw@gnuplot%
    \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{#1}}%
  \else%
    \iftikz@plot@parametric%   
      \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{%
          set samples \tikz@plot@samples;
          set parametric;
          plot [t=\tikz@plot@domain] #1}}%
    \else%
      \def\tikz@plot@data{\pgfplotgnuplot[\tikz@plot@filename]{%
          set samples \tikz@plot@samples;
          plot [x=\tikz@plot@domain] #1}}%
    \fi%
  \fi%
  \tikz@@@plot%
}

\def\tikz@plot@no@resample{%
  \pgfutil@IfFileExists{\tikz@plot@filename.table}%
  {\def\tikz@plot@data{\pgfplotxyfile{\tikz@plot@filename.table}}}%
  {}%
}

\def\tikz@plot@expression(#1){%
  \edef\tikz@plot@data{\noexpand\pgfplotfunction{\expandafter\noexpand\tikz@plot@var}{\tikz@plot@samplesat}}%
  \expandafter\def\expandafter\tikz@plot@data\expandafter{\tikz@plot@data{\tikz@scan@one@point\pgfutil@firstofone(#1)}}%
  \tikz@@@plot%
}

\def\tikz@@@plot{%
    \def\pgfplotlastpoint{\pgfpointorigin}%
    \tikz@plot@handler%
    \tikz@plot@data%
    \global\let\tikz@@@temp=\pgfplotlastpoint%
    \ifx\tikz@plot@mark\pgfutil@empty%
    \else%
      % Marks are drawn after the path.
      \setbox\tikz@figbox=\hbox{%
        \unhbox\tikz@figbox%
        \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \let\tikz@options=\pgfutil@empty%
              \let\tikz@transform=\pgfutil@empty%
              \expandafter\tikzset\expandafter{\tikz@plot@mark@options}%
              \tikz@options%
              \ifx\tikz@mark@list\pgfutil@empty%
                \pgfplothandlermark{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}%
              \else
                \pgfplothandlermarklisted{\tikz@transform\pgfuseplotmark{\tikz@plot@mark}}{\tikz@mark@list}%
              \fi
              \tikz@plot@data%
            \endpgfscope
          \endpgfinterruptpath%
        }}%
      }%
    \fi%
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%  
  \tikz@make@last@position{\tikz@@@temp}%  
  \tikz@scan@next@command%
}


\pgfdeclareplotmark{ball}
{%
  \def\tikz@shading{ball}%
  \shade (0,0) circle (\pgfplotmarksize);%
}




% Syntax for cosine curves:
% cos <end of quarter-period>
\def\tikz@cosine s{\tikz@scan@one@point\tikz@@cosine}
\def\tikz@@cosine#1{%
  \tikz@flush@moveto%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\tikz@lastx%
  \advance\pgf@yc by-\tikz@lasty%
  \advance\tikz@lastx by\pgf@xc%
  \advance\tikz@lasty by\pgf@yc%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@updatecurrenttrue%
  \pgfpathcosine{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@scan@next@command%
}

% Syntax for sine curves:
% sin <end of quarter-period>
\def\tikz@sine in{\tikz@scan@one@point\tikz@@sine}
\def\tikz@@sine#1{%
  \tikz@flush@moveto%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\tikz@lastx%
  \advance\pgf@yc by-\tikz@lasty%
  \advance\tikz@lastx by\pgf@xc%
  \advance\tikz@lasty by\pgf@yc%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@updatecurrenttrue%
  \pgfpathsine{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
  \tikz@scan@next@command%
}

% Syntax for parabolas: 
% parabola[options] bend <coordinate> <coordinate>
\def\tikz@parabola arabola{%
  \pgfutil@ifnextchar[{\tikz@parabola@options}{\tikz@parabola@options[]}}%}

\def\tikz@parabola@options[#1]{%
  \def\tikz@parabola@option{#1}%
  \pgfutil@ifnextchar b{\tikz@parabola@scan@bend}{\tikz@scan@one@point\tikz@parabola@semifinal}}
\def\tikz@parabola@scan@bend bend{\tikz@scan@one@point\tikz@parabola@scan@bendB}
\def\tikz@parabola@scan@bendB#1{%
  \def\tikz@parabola@bend{#1}%
  \tikz@scan@one@point\tikz@parabola@semifinal%
}
\def\tikz@parabola@semifinal#1{%
  \tikz@flush@moveto%
  % Save original start:
  \pgf@xb=\tikz@lastx%
  \pgf@yb=\tikz@lasty%
  \tikz@make@last@position{#1}%
  \pgf@xc=\tikz@lastx%
  \pgf@yc=\tikz@lasty%
  \begingroup% now calculate bend:
    \expandafter\tikzset\expandafter{\tikz@parabola@option}%
    \tikz@lastxsaved=\tikz@parabola@bend@factor\tikz@lastx%
    \tikz@lastysaved=\tikz@parabola@bend@factor\tikz@lasty%
    \advance\tikz@lastxsaved by\pgf@xb%
    \advance\tikz@lastysaved by\pgf@yb%
    \advance\tikz@lastxsaved by-\tikz@parabola@bend@factor\pgf@xb%
    \advance\tikz@lastysaved by-\tikz@parabola@bend@factor\pgf@yb%
    \expandafter\tikz@make@last@position\expandafter{\tikz@parabola@bend}%
    % Calculate delta from bend
    \advance\pgf@xc by-\tikz@lastx%
    \advance\pgf@yc by-\tikz@lasty%
    % Ok, now calculate delta to bend
    \advance\tikz@lastx by-\pgf@xb%
    \advance\tikz@lasty by-\pgf@yb%
    \xdef\tikz@parabola@b{{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}}%
  \endgroup%
  \expandafter\pgfpathparabola\tikz@parabola@b%
  \tikz@scan@next@command%
}


% Syntax for circles:
% circle (radius)
%
% Syntax for ellipses:
% ellipse (x-radius and y-radius)
%
% radii can be dimensionless, then they are in the xy-system
\def\tikz@circle ircle{\tikz@flush@moveto\tikz@@circle}
\def\tikz@ellipse llipse{\tikz@flush@moveto\tikz@@circle}
\def\tikz@@circle{%
  \pgfutil@ifnextchar(\tikz@@@circle{%)
    \advance\tikz@expandcount by -1%
    \ifnum\tikz@expandcount<0\relax%
      \let\@next=\tikz@@circle@scangiveup%
    \else%
      \let\@next=\tikz@@circle@scanexpand%
    \fi%
    \@next%
  }%
}
\def\tikz@@circle@scanexpand{\expandafter\tikz@@circle}
\def\tikz@@circle@scangiveup#1{\PackageError{tikz}{Cannot parse this radius}{}#1{\tikz@scan@next@command}}
\def\tikz@@@circle(#1){%
  \pgfutil@in@{ and }{#1}%
  \ifpgfutil@in@%
    \tikz@@ellipseB(#1)%
  \else%
    \tikz@@ellipseB({#1} and {#1})%
  \fi%
  \tikz@scan@next@command%
}
\def\tikz@@ellipseB(#1 and #2){%
  \pgfmathparse{#1}%
  \let\tikz@ellipse@x=\pgfmathresult%
  \ifpgfmathunitsdeclared%
    \pgfmathparse{#2}%
    \let\tikz@ellipse@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \pgfpathellipse{\tikz@last@position}{%
        \pgfqpoint{\tikz@ellipse@x pt}{0pt}}{\pgfpoint{0pt}{\tikz@ellipse@y pt}}%
    \else%
      \PackageError{tikz}{You cannot mix dimensions and dimensionless values in an ellipse}{}%
    \fi%
  \else%
    \pgfmathparse{#2}%
    \let\tikz@ellipse@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \PackageError{tikz}{You cannot mix dimensions and dimensionless values in an ellipse}{}%
    \else%
      \pgfpathellipse{\tikz@last@position}{%
        \pgfpointxy{\tikz@ellipse@x}{0}}{\pgfpointxy{0}{\tikz@ellipse@y}}%
    \fi%
  \fi%
}

% Syntax 1 for arcs:
% arc (start angle:end angle:radius)
%
% Syntax 2 for arcs:
% arc (start angle:end angle:x-radius and y-radius)
%
% radius can be dimensionless, then the arc is in the xy-coordinate system
\def\tikz@arcA rc{%
  \tikz@flush@moveto%
  \pgfutil@ifnextchar({\tikz@@arcto}{\expandafter\tikz@arcA\expandafter r\expandafter c}}

\def\tikz@@arcto(#1){%
  \edef\tikz@temp{(#1)}%
   \expandafter\tikz@@@arcto@check@slashand\tikz@temp%
}

\def\tikz@@@arcto@check@slashand(#1:#2:#3){%
  \pgfutil@in@{ and }{#3}%
  \ifpgfutil@in@% 
    \tikz@parse@arc@and(#1:#2:#3)%
  \else%
    \tikz@parse@arc@and(#1:#2:{#3} and {#3})%
  \fi%
}

\def\tikz@parse@arc@and(#1:#2:#3 and #4){%
  \pgfmathparse{#3}%
  \let\tikz@arc@x=\pgfmathresult%
  \ifpgfmathunitsdeclared%
    \pgfmathparse{#4}%
    \let\tikz@arc@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \tikz@@@arcfinal{\pgfpatharc{#1}{#2}{\tikz@arc@x pt and \tikz@arc@y pt}}
      {\pgfpointpolar{#1}{\tikz@arc@x pt and \tikz@arc@y pt}}
      {\pgfpointpolar{#2}{\tikz@arc@x pt and \tikz@arc@y pt}}%
    \else%
      \PackageError{tikz}{You cannot mix dimensions and dimensionless values in an arc}{}%
    \fi%
  \else%
    \pgfmathparse{#4}%
    \let\tikz@arc@y=\pgfmathresult%
    \ifpgfmathunitsdeclared%
      \PackageError{tikz}{You cannot mix dimensions and dimensionless values in an arc}{}%
    \else%
      \tikz@@@arcfinal{\pgfpatharcaxes{#1}{#2}{\pgfpointxy{\tikz@arc@x}{0}}{\pgfpointxy{0}{\tikz@arc@y}}}
      {\pgfpointpolarxy{#1}{\tikz@arc@x and \tikz@arc@y}}{\pgfpointpolarxy{#2}{\tikz@arc@x and \tikz@arc@y}}%
     \fi%
  \fi%
}

\def\tikz@@@arcfinal#1#2#3{%
  #1%
  \pgf@process{#2}%
  \advance\tikz@lastx by-\pgf@x%
  \advance\tikz@lasty by-\pgf@y%
  \pgf@process{#3}%
  \advance\tikz@lastx by\pgf@x%
  \advance\tikz@lasty by\pgf@y%
  \tikz@lastxsaved=\tikz@lastx%
  \tikz@lastysaved=\tikz@lasty%
  \tikz@scan@next@command%
}


% Syntax for coordinates:
% coordinate[options] (coordinate name) at (point)
% where ``at (point)'' is optional
\def\tikz@coordinate ordinate{%
  \pgfutil@ifnextchar[{\tikz@@coordinate@opt}{\tikz@@coordinate@opt[]}}
\def\tikz@@coordinate@opt[#1]{%
  \pgfutil@ifnextchar({\tikz@@coordinate[#1]}
  {\tikz@fig ode[shape=coordinate,#1]{}}}%}
\def\tikz@@coordinate[#1](#2){%
  \pgfutil@ifnextchar a{\tikz@@coordinate@at[#1](#2)}
  {\tikz@fig ode[shape=coordinate,#1](#2){}}}
\def\tikz@@coordinate@at[#1](#2)at#3({%
  \def\tikz@coordinate@caller{\tikz@fig ode[shape=coordinate,#1](#2)at}%
  \tikz@scan@one@point\tikz@@coordinate@at@math(%
}
\def\tikz@@coordinate@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@temp{(\the\pgf@x,\the\pgf@y)}%
  \expandafter\tikz@coordinate@caller\tikz@temp{}%
}
  


% Syntax for nodes:
% node[options] (node name) {label text}
%
% all of [options], (node name) and {label text} are optional. There
% can be multiple options before the label text as in
% node[draw] (a) [rotate=10] {text}
%
% A label text always ``ends'' the node.
\def\tikz@fig ode{%
  \edef\tikz@save@line@width{\the\pgflinewidth}%
  \begingroup%
  \let\tikz@fig@name=\pgfutil@empty%
    \begingroup%
      \tikz@is@matrixfalse%
      \let\nodepart=\tikz@nodepart%
      \let\tikz@options=\pgfutil@empty%
      \let\tikz@after@node=\pgfutil@empty%
      \let\tikz@afternodepathoptions=\pgfutil@empty%
      \let\tikz@transform=\pgfutil@empty%
      \let\tikz@mode=\pgfutil@empty%
      \tikz@decoratepathfalse%
      \let\tikz@preactions=\pgfutil@empty%
      \let\tikz@postactions=\pgfutil@empty%
      \let\tikz@alias=\pgfutil@empty%
      \def\tikz@node@at{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
      \iftikz@node@is@a@label%
      \else%
        \let\tikz@time=\pgfutil@empty%
      \fi%
      \tikz@node@reset@hook%
      \tikzset{every node/.try}%
      \tikz@@scan@fig}%
\def\tikz@@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
  {\pgfutil@ifnextchar({\tikz@fig@scan@name}
    {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
      {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
      {\PackageError{tikz}{A node must have a (possibly empty) label text}{}%
       \tikz@fig@main{}}}}}}%}}
\def\tikz@fig@scan@at at{%
  \tikz@scan@one@point\tikz@@fig@scan@at}
\def\tikz@@fig@scan@at#1{%
  \def\tikz@node@at{#1}\tikz@@scan@fig}%
\def\tikz@fig@scan@name(#1){\edef\tikz@fig@name{#1}\tikz@@scan@fig}%
\def\tikz@fig@scan@options[#1]{\tikzset{#1}\tikz@@scan@fig}%
\let\tikz@node@reset@hook=\pgfutil@empty%
\let\tikz@node@begin@hook=\pgfutil@empty%
\def\tikz@fig@main{\afterassignment\tikz@@fig@main\let\next=}
\def\tikz@@fig@main{%
    \pgfutil@ifundefined{pgf@sh@s@\tikz@shape}%
    {\PackageError{tikz}%
      {Unknown shape ``\tikz@shape.'' Using ``rectangle'' instead}{}%
      \def\tikz@shape{rectangle}}%
    {}%
    \tikzset{every \tikz@shape\space node/.try}%
    \tikz@node@begin@hook%
    \iftikz@is@matrix%
      \let\tikz@next=\tikz@do@matrix%
    \else%
      \let\tikz@next=\tikz@do@fig%
    \fi%
    \tikz@next%  
}
\def\tikz@do@fig{%  
    \setbox\pgfnodeparttextbox=\hbox%
      \bgroup%
        \tikzset{every text node part/.try}%
        \ifx\tikz@textopacity\pgfutil@empty%
        \else%
          \pgfsetfillopacity{\tikz@textopacity}%
          \pgfsetstrokeopacity{\tikz@textopacity}%
        \fi%
        \pgfinterruptpicture%
          \tikz@textfont%  
          \ifx\tikz@text@width\pgfutil@empty%
          \else%
            \begingroup%
              \pgfutil@minipage[t]{\tikz@text@width}%
                \tikz@text@action%
          \fi%
          \tikz@atbegin@node%
          \bgroup%
            \aftergroup\unskip%
            \ifx\tikz@textcolor\pgfutil@empty%
            \else%
              \pgfutil@colorlet{.}{\tikz@textcolor}%
            \fi%
            \pgfsetcolor{.}%
            \setbox\tikz@figbox=\box\voidb@x%
            \tikz@uninstallcommands%
            \aftergroup\tikz@fig@collectresetcolor%
            \ignorespaces%
}
\def\tikz@fig@collectresetcolor{%
  \pgfutil@ifnextchar\reset@color%
  {\reset@color\afterassignment\tikz@fig@collectresetcolor\let\tikz@temp=}%
  {\tikz@fig@boxdone}%
}
\def\tikz@fig@boxdone{%
            \tikz@atend@node%
          \ifx\tikz@text@width\pgfutil@empty%
          \else%
              \pgfutil@endminipage%
            \endgroup%
          \fi%
        \endpgfinterruptpicture%
      \egroup%
    \pgfutil@ifnextchar c{\tikz@fig@mustbenamed\tikz@fig@continue}%
    {\pgfutil@ifnextchar[{\tikz@fig@mustbenamed\tikz@fig@continue}%
      {\pgfutil@ifnextchar t{\tikz@fig@mustbenamed\tikz@fig@continue}
        {\pgfutil@ifnextchar e{\tikz@fig@mustbenamed\tikz@fig@continue}
          {\ifx\tikz@after@node\pgfutil@empty\expandafter\tikz@fig@continue\else\expandafter\tikz@fig@mustbenamed\expandafter\tikz@fig@continue\fi}}}}}%}

\def\tikz@do@matrix{%
    \tikzset{every matrix/.try}%
    \tikz@node@transformations%
    \tikz@fig@mustbenamed%
    \setbox\tikz@figbox=\hbox\bgroup%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox\bgroup\bgroup%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\voidb@x%
              \let\tikzmatrixname=\tikz@fig@name%
              \edef\tikz@m@anchor{\ifx\tikz@matrix@anchor\pgfutil@empty\tikz@anchor\else\tikz@matrix@anchor\fi}%
              \expandafter\pgfutil@in@\expandafter{\expandafter.\expandafter}\expandafter{\tikz@m@anchor}%
              \ifpgfutil@in@%
                \expandafter\tikz@matrix@split\tikz@m@anchor\relax%
              \else%
                \def\tikz@matrix@shift{\pgfpointorigin}%  
              \fi%
              \let\tikz@transform=\relax%
              \pgfmatrix%
              {\tikz@shape}%
              {\tikz@m@anchor}%
              {\tikz@fig@name}%
              {%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
              {\tikz@matrix@shift}%
              {%
                \tikz@matrix@make@active@ampersand%
                \def\pgfmatrixbegincode{%
                  \pgfsys@beginscope%
                  \tikz@common@matrix@code%
                  \tikz@atbegin@cell%
                }%
                \def\tikz@common@matrix@code{%
                  \let\tikz@options=\pgfutil@empty%
                  \let\tikz@mode=\pgfutil@empty%
                  \tikzset{every cell/.try={\the\pgfmatrixcurrentrow}{\the\pgfmatrixcurrentcolumn}}%
                  \tikzset{column \the\pgfmatrixcurrentcolumn/.try}%
                  \ifodd\pgfmatrixcurrentcolumn%
                    \tikzset{every odd column/.try}%
                  \else%
                    \tikzset{every even column/.try}%
                  \fi%
                  \tikzset{row \the\pgfmatrixcurrentrow/.try}%
                  \ifodd\pgfmatrixcurrentrow%
                    \tikzset{every odd row/.try}%
                  \else%
                    \tikzset{every even row/.try}%
                  \fi%
                  \tikzset{row \the\pgfmatrixcurrentrow\space column \the\pgfmatrixcurrentcolumn/.try}%
                  \tikz@options%
                }%
                \def\pgfmatrixendcode{%
                  \tikz@atend@cell%
                  \pgfsys@endscope%
                }%
                \def\pgfmatrixemptycode{%
                  \pgfsys@beginscope%
                  \tikz@common@matrix@code%
                  \tikz@at@emptycell%
                  \pgfsys@endscope%
                }%
                \aftergroup\tikz@do@matrix@cont}%
              \bgroup%
}
\def\tikz@do@matrix@cont{%            
            \endpgfscope
          \endpgfinterruptpath%
      \egroup\egroup%
    \egroup%
    %
    \tikz@node@finish%
}

{%
  \catcode`\&=13
  \gdef\tikz@matrix@make@active@ampersand{%
    \ifx\tikz@ampersand@replacement\pgfutil@empty%
      \catcode`\&=13%
      \let&=\pgfmatrixnextcell%
    \else%
      \expandafter\let\tikz@ampersand@replacement=\pgfmatrixnextcell%
    \fi%
  }%
}%


\def\tikz@matrix@split#1.#2\relax{%
  \def\tikz@m@anchor{text}%
  \def\tikz@matrix@shift{\pgfpointanchor{#1}{#2}}%
}
  
\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    % Node transformation
    %
    \tikz@node@transformations
    %
    \setbox\tikz@figbox=\hbox{%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\voidb@x%
              \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
            \endpgfscope
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}


\def\tikz@fig@mustbenamed{%
  \ifx\tikz@fig@name\pgfutil@empty%
    % Assign a dummy name
    \global\advance\tikz@fig@count by1\relax
    \edef\tikz@fig@name{tikz@f@\the\tikz@fig@count}%
  \fi%
}

\def\tikz@node@transformations{
  % 
  % Possibly, we are ``online''
  % 
  \ifx\tikz@time\pgfutil@empty%
    \pgftransformshift{\tikz@node@at}%
    \iftikz@fullytransformed%
    \else%
      \pgftransformresetnontranslations%
    \fi%
  \else%
    \tikz@do@auto@anchor%
    \tikz@timer%
  \fi%
  % Invoke local transformations
  \tikz@transform%
}

\def\tikz@node@finish{%  
    \global\let\tikz@last@fig@name=\tikz@fig@name%
    \global\let\tikz@after@node@smuggle=\tikz@after@node%
    \global\let\tikz@afternodepathoptions@smuggle=\tikz@afternodepathoptions%
    % shift box outside group
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup\endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%
  \pgflinewidth=\tikz@save@line@width%
  \let\tikz@to@last@fig@name=\tikz@last@fig@name%
  \let\tikz@to@use@whom=\tikz@to@use@last@fig@name%
  \let\tikzlastnode=\tikz@last@fig@name%
  \ifx\tikz@after@node@smuggle\pgfutil@empty%
  \else%
    \tikz@scan@next@command{\pgfextra{\tikz@afternodepathoptions@smuggle}\tikz@after@node@smuggle}\pgf@stop%
  \fi%
  \tikz@scan@next@command%
}
\let\tikz@fig@continue@orig=\tikz@fig@continue



% Syntax for parts of  nodes:
% node ... {... \nodepart{name} ... \nodepart{name} ...}

\def\tikz@nodepart#1{%
  \tikz@atend@node%
  \unskip%
  \gdef\tikz@nodepart@name{#1}%
  \global\let\tikz@fig@continue=\tikz@nodepart@continue%
  \pgfutil@ifnextchar x{\egroup\relax}{\egroup\relax}% gobble spaces
}
\def\tikz@nodepart@continue{%
  \global\let\tikz@fig@continue=\tikz@fig@continue@orig%
  % Now start new box:
   \expandafter\setbox\csname pgfnodepart\tikz@nodepart@name box\endcsname=\hbox%
      \bgroup%
        \tikzset{every \tikz@nodepart@name\space node part/.try}%
        \pgfinterruptpicture%
          \tikz@textfont%  
          \ifx\tikz@text@width\pgfutil@empty%
          \else%
            \begingroup%
              \pgfutil@minipage[t]{\tikz@text@width}%
                \tikz@text@action%
          \fi%
          \bgroup%
            \aftergroup\unskip%
            \ifx\tikz@textcolor\pgfutil@empty%
            \else%
              \pgfutil@colorlet{.}{\tikz@textcolor}%
            \fi%
            \pgfsetcolor{.}%
            \setbox\tikz@figbox=\box\voidb@x%
            \tikz@uninstallcommands%
            \tikz@atbegin@node%
            \aftergroup\tikz@fig@collectresetcolor%
            \ignorespaces%
}

%
% "late" options can be used to "redo" a node
%
\tikzset{late options/.code=\tikz@late@options{#1}}
\def\tikz@late@options#1{%
  % Do a "virtual" node:
  \begingroup%
    \iftikz@shapeborder%
      \let\tikz@fig@name=\tikz@shapeborder@name%
    \else%
      \let\tikz@fig@name=\pgfutil@empty%
    \fi%
    \tikz@is@matrixfalse%
    \let\tikz@options=\pgfutil@empty%
    \let\tikz@after@node=\pgfutil@empty%
    \let\tikz@afternodepathoptions=\pgfutil@empty%
    \let\tikz@alias=\pgfutil@empty%
    \let\tikz@transform=\pgfutil@empty%
    \tikz@decoratepathfalse%
    \tikz@node@reset@hook%
    \tikzset{every node/.try,#1}%
    \ifx\tikz@fig@name\pgfutil@empty%
      \PackageError{tikz}{Late options must reference some existing
        node}{}%
    \fi%
    \tikz@node@begin@hook%
    \tikz@alias%
    \global\let\tikz@last@fig@name=\tikz@fig@name%
    \global\let\tikz@after@node@smuggle=\tikz@after@node%
    \global\let\tikz@afternodepathoptions@smuggle=\tikz@afternodepathoptions%
  \endgroup%
  \let\tikz@to@last@fig@name=\tikz@last@fig@name%
  \let\tikz@to@use@whom=\tikz@to@use@last@fig@name%
  \let\tikzlastnode=\tikz@last@fig@name%
  \ifx\tikz@after@node@smuggle\pgfutil@empty%
  \else%
    \tikz@scan@next@command{\pgfextra{\tikz@afternodepathoptions@smuggle}\tikz@after@node@smuggle}\pgf@stop%
  \fi%
}


% Auto placement

\def\tikz@auto@pre{%
  \begingroup
    \pgfresetnontranslationattimefalse
    \pgfslopedattimetrue%
    \pgfallowupsidedownattimetrue%
    \tikz@timer%
    \pgf@x=\pgf@pt@aa pt% 
    \pgf@y=\pgf@pt@ab pt%
    \pgfpointnormalised{}%
}

\def\tikz@auto@post{%
    \global\let\tikz@anchor@smuggle=\tikz@anchor%
  \endgroup%
  \let\tikz@anchor=\tikz@anchor@smuggle%
}

\def\tikz@auto@anchor{%
    \ifdim\pgf@x>0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{south east}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{south west}%
      \else
        \def\tikz@anchor{south}%
      \fi\fi%
    \else\ifdim\pgf@x<-0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{north east}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{north west}%
      \else
        \def\tikz@anchor{north}%
      \fi\fi%
    \else%
      \ifdim\pgf@y>0pt%
        \def\tikz@anchor{east}%
      \else%
        \def\tikz@anchor{west}%
      \fi%
    \fi\fi%
}

\def\tikz@auto@anchor@prime{%
    \ifdim\pgf@x>0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{north west}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{north east}%
      \else
        \def\tikz@anchor{north}%
      \fi\fi%
    \else\ifdim\pgf@x<-0.05pt%
      \ifdim\pgf@y>0.05pt%
        \def\tikz@anchor{south west}%
      \else\ifdim\pgf@y<-0.05pt%
        \def\tikz@anchor{south east}%
      \else
        \def\tikz@anchor{south}%
      \fi\fi%
    \else%
      \ifdim\pgf@y>0pt%
        \def\tikz@anchor{west}%
      \else%
        \def\tikz@anchor{east}%
      \fi%
    \fi\fi%
}




% Syntax for trees:
% node {...} child [options] {...} child [options] {...} ...
% node {...} child [options] foreach \var in {list} [options] {...} ...

\def\tikz@children{%
  % Start collecting the children:
  \let\tikz@children@list=\pgfutil@empty%
  \tikznumberofchildren=0\relax%
  \tikz@collect@children c}

\def\tikz@collect@children{\pgfutil@ifnextchar c{\tikz@collect@children@cchar}{\tikz@children@collected}}
\def\tikz@collect@children@cchar c{\pgfutil@ifnextchar h{\tikz@collect@child}{\tikz@children@collected c}}
\def\tikz@collect@child hild{\pgfutil@ifnextchar[{\tikz@collect@childA}{\tikz@collect@childA[]}}%}
\def\tikz@collect@childA[#1]{\pgfutil@ifnextchar f{\tikz@collect@children@foreach[#1]}{\tikz@collect@childB[#1]}}
\def\tikz@collect@childB[#1]{%
  \advance\tikznumberofchildren by1\relax
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list \tikz@childnode[#1]}%
  \pgfutil@ifnextchar\bgroup{\tikz@collect@child@code}{\tikz@collect@child@code{}}}
\def\tikz@collect@child@code#1{%
  \expandafter\def\expandafter\tikz@children@list\expandafter{\tikz@children@list{#1}}%
  \tikz@collect@children%
}
\def\tikz@collect@children@foreach[#1]foreach#2in#3{%
  \pgfutil@ifnextchar\bgroup{\tikz@collect@children@foreachA{#1}{#2}{#3}}{\tikz@collect@children@foreachA{#1}{#2}{#3}{}}}
\def\tikz@collect@children@foreachA#1#2#3#4{%
  \expandafter\def\expandafter\tikz@children@list\expandafter
    {\tikz@children@list\tikz@childrennodes[#1]{#2}{#3}{#4}}%
  \c@pgf@counta=\tikznumberofchildren%
  \foreach#2in{#3}%
  {%
    \global\advance\c@pgf@counta by1\relax%
  }%
  \tikznumberofchildren=\c@pgf@counta%
  \tikz@collect@children%
}
\long\def\tikz@children@collected{%
  \begingroup%
    \advance\tikztreelevel by 1\relax%
    \let\tikz@options=\pgfutil@empty%
    \let\tikz@transform=\pgfutil@empty%
    \tikzset{level/.try=\the\tikztreelevel,level \the\tikztreelevel/.try}%
    \tikz@transform%            
    \let\tikzparentnode=\tikz@last@fig@name%
    % Transform to center of node
    \pgftransformshift{\pgfpointanchor{\tikzparentnode}{\tikz@growth@anchor}}%
    \tikznumberofcurrentchild=0\relax%
    \tikz@children@list%
    \global\setbox\tikz@tempbox=\copy\tikz@figbox%
  \endgroup%
  \setbox\tikz@figbox=\box\tikz@tempbox%  
  \tikz@scan@next@command%
}


% Syntax for children:
%
% child [all children options] foreach \var in {values} [child options] {...}
\def\tikz@childrennodes[#1]#2#3#4{%
  \c@pgf@counta=\tikznumberofcurrentchild\relax%
  \setbox\tikz@tempbox=\box\tikz@figbox%
  \foreach#2in{#3}{%
    \tikznumberofcurrentchild=\c@pgf@counta\relax%
    \setbox\tikz@figbox=\box\tikz@tempbox%
    \tikz@childnode[#1]{#4}%
    % we must now make the current child number and the figbox survive
    % the group
    \global\c@pgf@counta=\tikznumberofcurrentchild\relax%
    \global\setbox\tikz@tempbox=\box\tikz@figbox%
  }%
  \tikznumberofcurrentchild=\c@pgf@counta\relax%
  \setbox\tikz@figbox=\box\tikz@tempbox%
}


% Syntax for child:
%
% child
%
% child[options]
%
% child[options] {node (name) {child node text} ...
%   edge from parent[options] node {label text} node {label text}}

\def\tikz@childnode[#1]#2{%
  \advance\tikznumberofcurrentchild by1\relax%
  {\tikzset{every child/.try,#1}\expandafter}%
  \iftikz@child@missing%
  \else%
  \setbox\tikz@figbox=\hbox\bgroup%
    \unhbox\tikz@figbox%
    \hbox\bgroup\bgroup%
        \pgfinterruptpath%
          \pgfscope%
            \let\tikz@transform=\pgfutil@empty%
            \tikzset{every child/.try,#1}%
            \tikz@options%
            \tikz@transform%            
            \tikz@grow%
            % Typeset node:
            \edef\tikz@parent@node@name{[name=\tikzparentnode-\the\tikznumberofcurrentchild,style=every child node]}%
            \def\tikz@child@node@text{[shape=coordinate]{}}
            \tikz@parse@child@node#2\pgf@stop%
            \expandafter\expandafter\expandafter\node
            \expandafter\tikz@parent@node@name
              \tikz@child@node@text
              \pgfextra{\global\let\tikz@childnode@name=\tikz@last@fig@name};%
            \let\tikzchildnode=\tikz@childnode@name%
            {%
              \def\tikz@edge@to@parent@needed{edge from parent}
              \ifx\tikz@child@node@rest\pgfutil@empty%
                \path edge from parent;%
              \else%
                \path (0,0) \tikz@child@node@rest \tikz@edge@to@parent@needed;%
              \fi%
            }%
        \endpgfscope%
      \endpgfinterruptpath%
    \egroup\egroup%
  \egroup%
  \fi%
}

\def\tikz@parse@child@node{%
  \pgfutil@ifnextchar n{\tikz@parse@child@node@n}%
  {\pgfutil@ifnextchar c{\tikz@parse@child@node@c}%
    {\tikz@parse@child@node@rest}}}
\def\tikz@parse@child@node@rest#1\pgf@stop{\def\tikz@child@node@rest{#1}}
\def\tikz@parse@child@node@c c{\pgfutil@ifnextchar o{\tikz@parse@child@node@co}{\tikz@parse@child@node@rest c}}
\def\tikz@parse@child@node@co o{\pgfutil@ifnextchar o{\tikz@parse@child@node@coordinate}{\tikz@parse@child@node@rest co}}
\def\tikz@parse@child@node@coordinate ordinate{%
  \pgfutil@ifnextchar ({\tikz@@parse@child@node@coordinate}{%
    \def\tikz@child@node@text{[shape=coordinate]{}}%
    \tikz@parse@child@node@rest}}%}
\def\tikz@@parse@child@node@coordinate(#1){%
  \pgfutil@ifnextchar a{\tikz@p@c@n@c@at(#1)}{%
    \def\tikz@child@node@text{[shape=coordinate,name=#1]{}}%
    \tikz@parse@child@node@rest}}
\def\tikz@p@c@n@c@at(#1)at#2({%
  \def\tikz@child@node@text@pre{[shape=coordinate,name=#1]at}%
  \tikz@scan@one@point\tikz@p@c@n@c@at@math(%
}
\def\tikz@p@c@n@c@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@marshal{(\the\pgf@x,\the\pgf@y){}}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\tikz@child@node@text%
  \expandafter\expandafter\expandafter{\expandafter\tikz@child@node@text@pre\tikz@marshal}%
  \tikz@parse@child@node@rest%
}
\def\tikz@parse@child@node@n node{%
  \let\tikz@child@node@text=\pgfutil@empty%
  \tikz@p@c@s}%
\def\tikz@p@c@s{%
  \pgfutil@ifnextchar a{\tikz@p@c@s@at}
  {\pgfutil@ifnextchar ({\tikz@p@c@s@paran}
    {\pgfutil@ifnextchar [{\tikz@p@c@s@bra}
      {\pgfutil@ifnextchar \bgroup{\tikz@p@c@s@group}
        {\PackageError{tikz}{Cannot parse this node}{}}}}}}%}}
\def\tikz@p@c@s@at at#1({%
  \tikz@scan@one@point\tikz@p@c@s@at@math(%
}
\def\tikz@p@c@s@at@math#1{%
  \pgf@process{#1}%
  \edef\tikz@marshal{ at(\the\pgf@x,\the\pgf@y)}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\tikz@child@node@text%
  \expandafter\expandafter\expandafter{\expandafter\tikz@child@node@text\tikz@marshal}
  \tikz@p@c@s}
\def\tikz@p@c@s@paran(#1){%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text(#1)}
  \tikz@p@c@s}
\def\tikz@p@c@s@bra[#1]{%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text[#1]}
  \tikz@p@c@s}
\def\tikz@p@c@s@group#1{%
  \expandafter\def\expandafter\tikz@child@node@text\expandafter{\tikz@child@node@text{#1}}
  \tikz@parse@child@node@rest}



% 
% Syntax for decorated subpaths:
%
% decorate [option] { subpath }
%
\def\tikz@decoration ecorate{%
  \pgfutil@ifnextchar[{\tikz@lib@decoration}{\tikz@lib@decoration[]}%]
}

\def\tikz@lib@decoration[#1]#2{\PackageError{tikz}{You need to load a decoration library}{}}

% The decorate path command:
\def\tikz@lib@dec@decorate@path{\PackageError{tikz}{You need to load a decoration library}{}}



% 
% Syntax for let :
%
% let \p1 = (coordinate), \p2 = (coordinate),... in 
%
\def\tikz@let@command et#1in{%
  \PackageError{tikz}{You need to say \string\usetikzlibrary{calc} to use the let command}{}%
}



%
% Timers
% 

\def\tikz@timer@line{%
  \pgftransformlineattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@end}%
}

\def\tikz@timer@vhline{%
  \ifdim\tikz@time pt<0.5pt% first half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%    
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
    \tikz@marshal%
  \else% second half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \advance\pgf@xb by-1pt%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \tikz@marshal%
  \fi%
}

\def\tikz@timer@hvline{%
  \ifdim\tikz@time pt<0.5pt% first half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%    
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
    \tikz@marshal%
  \else% second half
    \pgf@process{\tikz@timer@start}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@timer@end}%
    \pgf@xb=\tikz@time pt%
    \pgf@xb=2\pgf@xb%
    \advance\pgf@xb by-1pt%
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@end}}%
    \tikz@marshal%
  \fi%
}

\def\tikz@timer@curve{%
  \pgftransformcurveattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@cont@one}{\tikz@timer@cont@two}{\tikz@timer@end}%
}



%
% Coordinate systems
% 

\def\tikzdeclarecoordinatesystem#1#2{%
  \expandafter\def\csname tikz@parse@cs@#1\endcsname(##1){%
    \pgf@process{%
      #2%
      \global\let\tikz@smubble@b=\tikz@shapeborder@name%
    }%
    \let\tikz@shapeborder@name=\tikz@smubble@b%
    \edef\tikz@return@coordinate{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
}
\def\tikzaliascoordinatesystem#1#2{%
  \edef\pgf@marshal{\noexpand\let\expandafter\noexpand\csname
    tikz@parse@cs@#1\endcsname=\expandafter\noexpand\csname
    tikz@parse@cs@#2\endcsname}%
  \pgf@marshal%
}


% Default coodinate systems:

\tikzdeclarecoordinatesystem{canvas}
{%
  \tikzset{cs/.cd,x=0pt,y=0pt,#1}%
  \pgfpoint{\tikz@cs@x}{\tikz@cs@y}%
}

\tikzdeclarecoordinatesystem{canvas polar}
{%
  \tikzset{cs/.cd,angle=0,radius=0cm,#1}%
  \pgfpointpolar{\tikz@cs@angle}{\tikz@cs@xradius and \tikz@cs@yradius}%
}

\tikzdeclarecoordinatesystem{xyz}
{%
  \tikzset{cs/.cd,x=0,y=0,z=0,#1}%
  \pgfpointxyz{\tikz@cs@x}{\tikz@cs@y}{\tikz@cs@z}%
}

\tikzdeclarecoordinatesystem{xyz polar}
{%
  \tikzset{cs/.cd,angle=0,radius=0,#1}%
  \pgfpointpolarxy{\tikz@cs@angle}{\tikz@cs@xradius and \tikz@cs@yradius}%
}
\tikzaliascoordinatesystem{xy polar}{xyz polar}


\tikzdeclarecoordinatesystem{node}
{%
  \tikzset{cs/.cd,name=,anchor=none,angle=none,#1}%
  \ifx\tikz@cs@anchor\tikz@nonetext%
    \ifx\tikz@cs@angle\tikz@nonetext%
      \expandafter\ifx\csname pgf@sh@ns@\tikz@cs@node\endcsname\tikz@coordinate@text%
      \else
        \aftergroup\tikz@shapebordertrue%
        \edef\tikz@shapeborder@name{\tikz@cs@node}%
      \fi%
      \pgfpointanchor{\tikz@cs@node}{center}%
    \else%
      \pgfpointanchor{\tikz@cs@node}{\tikz@cs@angle}%
    \fi%
  \else%
    \pgfpointanchor{\tikz@cs@node}{\tikz@cs@anchor}%
  \fi%
}

% Intersection coordinates
\tikzset{cs/first line/.code=\def\tikz@cs@line@a{#1}\def\tikz@cs@type@a{line}}
\tikzset{cs/second line/.code=\def\tikz@cs@line@b{#1}\def\tikz@cs@type@b{line}}

\tikzset{cs/first node/.code=\tikz@cs@unpack{\tikz@cs@node@a}{\tikz@cs@type@a}{#1}}
\tikzset{cs/second node/.code=\tikz@cs@unpack{\tikz@cs@node@b}{\tikz@cs@type@b}{#1}}

\def\tikz@cs@unpack#1#2#3{%
  \expandafter\ifx\csname pgf@sh@ns@#3\endcsname\relax%
    \PackageError{tikz}{Undefined node ``#3''}{}%
  \else%
    \def#1{#3}%
    \edef#2{\csname pgf@sh@ns@#3\endcsname}%
  \fi%
}

\tikzset{cs/solution/.initial=1}

\tikzset{cs/horizontal line through/.store in=\tikz@cs@hori@line}
\tikzset{cs/vertical line through/.store in=\tikz@cs@vert@line}

\tikzdeclarecoordinatesystem{intersection}
{%
  \tikzset{cs/.cd,#1}%
  \expandafter\ifx\csname tikz@intersect@\tikz@cs@type@a @and@\tikz@cs@type@b\endcsname\relax%
    \PackageError{tikz}{I do not know how to compute the intersection
    of a \tikz@cs@type@a and a \tikz@cs@type@b. Try saying
    \string\usetikzlibrary{calc}}{}%
    \pgfpointorigin%
  \else%
    \csname tikz@intersect@\tikz@cs@type@a @and@\tikz@cs@type@b\endcsname%
  \fi%
}

\def\tikz@intersect@line@and@line{%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@line\tikz@cs@line@a%
  \pgf@xa=\pgf@xc%
  \pgf@ya=\pgf@yc%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@line\tikz@cs@line@b%
  \edef\pgf@marshal{%
    {\noexpand\pgfpointintersectionoflines%
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}}%
  \pgf@marshal%
}

\def\tikz@parse@line#1--{%
  \pgf@process{#1}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \tikz@scan@one@point\pgf@process%
}


\tikzdeclarecoordinatesystem{perpendicular}
{%
  \tikzset{cs/.cd,#1}%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@intersection@a\tikz@cs@hori@line%
  \expandafter\tikz@scan@one@point\expandafter\tikz@parse@intersection@b\tikz@cs@vert@line%
  \pgfqpoint{\the\pgf@xb}{\the\pgf@ya}
}

\tikzdeclarecoordinatesystem{barycentric}
{%
  {%
    \pgf@xa=0pt% point
    \pgf@ya=0pt%
    \pgf@xb=0pt% sum
    \tikz@bary@dolist#1,=,%
    \pgfmathparse{1/\the\pgf@xb}%
    \global\pgf@x=\pgfmathresult\pgf@xa%
    \global\pgf@y=\pgfmathresult\pgf@ya%
  }%
}

\def\tikz@bary@dolist#1=#2,{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
  \else
    \pgf@process{\pgfpointanchor{#1}{center}}%
    \pgfmathparse{#2}%
    \advance\pgf@xa by\pgfmathresult\pgf@x%
    \advance\pgf@ya by\pgfmathresult\pgf@y%
    \advance\pgf@xb by\pgfmathresult pt%
    \expandafter\tikz@bary@dolist%
  \fi%
}

\tikzset{cs/x/.store in=\tikz@cs@x}
\tikzset{cs/y/.store in=\tikz@cs@y}
\tikzset{cs/z/.store in=\tikz@cs@z}
\tikzset{cs/angle/.store in=\tikz@cs@angle}
\tikzset{cs/x radius/.store in=\tikz@cs@xradius}
\tikzset{cs/y radius/.store in=\tikz@cs@yradius}
\tikzset{cs/radius/.style={/tikz/cs/x radius=#1,/tikz/cs/y radius=#1}}
\tikzset{cs/name/.store in=\tikz@cs@node}
\tikzset{cs/anchor/.store in=\tikz@cs@anchor}





%
% Coordinate management
%


% Last position visited
\def\tikz@last@position{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}
\def\tikz@last@position@saved{\pgfqpoint{\tikz@lastxsaved}{\tikz@lastysaved}}

% Make given point the last position visited
\def\tikz@make@last@position#1{%
  \pgf@process{#1}%
  \tikz@lastx=\pgf@x\relax%
  \tikz@lasty=\pgf@y\relax%
  \iftikz@updatecurrent%
    \tikz@lastxsaved=\pgf@x\relax%
    \tikz@lastysaved=\pgf@y\relax%
  \fi%
  \tikz@updatecurrenttrue%
}

\newif\iftikz@updatecurrent
\tikz@updatecurrenttrue



% Scanner: Scans a point or a relative point. 
% It then calls the first parameter with the argument set to an
% appropriate pgf command representing that point.

\def\tikz@scan@one@point#1{%
  \let\tikz@to@use@whom=\tikz@to@use@last@coordinate%
  \tikz@shapeborderfalse%
  \pgfutil@ifnextchar+{\tikz@scan@relative#1}{\tikz@scan@absolute#1}}
\def\tikz@scan@absolute#1{%
  \pgfutil@ifnextchar({\tikz@scan@@absolute#1}%)
  {%
    \advance\tikz@expandcount by -1%
    \ifnum\tikz@expandcount<0\relax%
      \let\@next=\tikz@@scangiveup%
    \else%
      \let\@next=\tikz@@scanexpand%
    \fi%
    \@next{#1}%
  }%
}
\def\tikz@@scanexpand#1{\expandafter\tikz@scan@one@point\expandafter#1}
\def\tikz@@scangiveup#1{\PackageError{tikz}{Cannot parse this coordinate}{}#1{\pgfpointorigin}}
\def\tikz@scan@@absolute#1({%
  \pgfutil@ifnextchar[% uhoh... options!
  {\def\tikz@scan@point@recall{#1}\tikz@scan@options}%
  {\tikz@@@scan@@absolute#1(}%
}

\def\tikz@scan@options[#1]#2{%
  \def\tikz@scan@point@options{#1}%
  \tikz@@@scan@@absolute\tikz@scan@handle@options(#2%
}

\def\tikz@scan@handle@options#1{%
  {%
    % Ok, compute point with options set and zero transformation
    % matrix:
    \pgftransformreset%
    \let\tikz@transform=\pgfutil@empty%
    \expandafter\tikzset\expandafter{\tikz@scan@point@options}%
    \tikz@transform%
    \pgf@process{\pgfpointtransformed{#1}}%
    \xdef\tikz@marshal{\expandafter\noexpand\tikz@scan@point@recall{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  }%
  \tikz@marshal%  
}

\def\tikz@@@scan@@absolute#1({%
  \pgfutil@ifnextchar{$}%$
  {\tikz@parse@calculator#1(}
  {\tikz@scan@no@calculator#1(}%
}
\def\tikz@scan@no@calculator#1(#2){%
  \edef\tikz@temp{(#2)}%
  \expandafter\tikz@@scan@@no@calculator\expandafter#1\tikz@temp%
}
\def\tikz@@scan@@no@calculator#1(#2){%
  \pgfutil@in@{cs:}{#2}%
  \ifpgfutil@in@%
    \let\@next\tikz@parse@coordinatesystem%
  \else%
    \pgfutil@in@{intersection }{#2}%
    \ifpgfutil@in@%
      \let\@next\tikz@parse@intersection%
    \else%
      \pgfutil@in@|{#2}%
      \ifpgfutil@in@
        \pgfutil@in@{-|}{#2}%
        \ifpgfutil@in@
          \let\@next\tikz@parse@hv%
        \else%
          \let\@next\tikz@parse@vh%
        \fi%
      \else%
        \pgfutil@in@:{#2}%
        \ifpgfutil@in@
          \let\@next\tikz@parse@polar%
        \else%
          \pgfutil@in@,{#2}%
          \ifpgfutil@in@%      
            \let\@next\tikz@parse@regular%
          \else%
            \let\@next\tikz@parse@node%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \@next#1(#2)%
}

\def\tikz@parse@calculator#1($#2$){%
  \PackageError{tikz}{You need to say \string\usetikzlibrary{calc} for
    coordinate calculation}{}%
  #1{\pgfpointorigin}%
}

\def\tikz@parse@coordinatesystem#1(#2 cs:#3){%
  \let\tikz@return@coordinate=\pgfpointorigin%
  \pgfutil@ifundefined{tikz@parse@cs@#2}
  {\PackageError{tikz}{Unknown coordinate system '#2'}{}}
  {\csname tikz@parse@cs@#2\endcsname(#3)}%
  \expandafter#1\expandafter{\tikz@return@coordinate}%
}


\newif\iftikz@isdimension
\def\tikz@checkunit#1{%
  \pgfmathparse{#1}%
  \let\iftikz@isdimension=\ifpgfmathunitsdeclared%
}

\def\tikz@parse@polar#1(#2:#3){%
  \pgfutil@ifundefined{tikz@polar@dir@#2}
  {\tikz@@parse@polar#1(#2:#3)}
  {\tikz@@parse@polar#1(\csname tikz@polar@dir@#2\endcsname:#3)}%
}
\def\tikz@@parse@polar#1(#2:#3){%
  \pgfutil@in@{ and }{#3}%
  \ifpgfutil@in@%
    \edef\tikz@args{(#2:#3)}%
  \else%
    \edef\tikz@args{(#2:#3 and #3)}%
  \fi%
  \expandafter\tikz@@@parse@polar\expandafter#1\tikz@args%
}
\def\tikz@@@parse@polar#1(#2:#3 and #4){%
  \tikz@checkunit{#3}%
  \iftikz@isdimension%
    \tikz@checkunit{#4}%
    \iftikz@isdimension%
      \def\tikz@next{#1{\pgfpointpolar{#2}{#3 and #4}}}%
    \else%
      \PackageError{tikz}{You cannot mix dimension and dimensionless values for polar coordinates}{}
      \def\tikz@next{#1{\pgfpointorigin}}%
    \fi%
  \else%
    \tikz@checkunit{#4}%
    \iftikz@isdimension%
      \PackageError{tikz}{You cannot mix dimension and dimensionless values for polar coordinates}{}
      \def\tikz@next{#1{\pgfpointorigin}}%
    \else%
      \def\tikz@next{#1{\pgfpointpolarxy{#2}{#3 and #4}}}%
    \fi%
  \fi%
  \tikz@next%
}
\def\tikz@polar@dir@up{90}
\def\tikz@polar@dir@down{-90}
\def\tikz@polar@dir@left{180}
\def\tikz@polar@dir@right{0}
\def\tikz@polar@dir@north{90}
\def\tikz@polar@dir@south{-90}
\def\tikz@polar@dir@east{0}
\def\tikz@polar@dir@west{180}
\expandafter\def\csname tikz@polar@dir@north east\endcsname{45}
\expandafter\def\csname tikz@polar@dir@north west\endcsname{135}
\expandafter\def\csname tikz@polar@dir@south east\endcsname{-45}
\expandafter\def\csname tikz@polar@dir@south west\endcsname{-135}


% MW: 
% Check to see if the y-coordinate is inside {}. If it is, scan it and
% reinsert it into the stream inside an extra group. 
%
\def\tikz@parse@regular#1(#2,{%
	\pgfutil@ifnextchar\bgroup{\tikz@@parse@regular#1{#2}}{\tikz@@@parse@regular#1{#2}}%
}
\def\tikz@@parse@regular#1#2#3{\tikz@@@parse@regular#1{#2}{{#3}}}%


% Originally \def\tikz@parse@regular#1(#2,#3){%
%
\def\tikz@@@parse@regular#1#2#3){%
  \pgfutil@in@,{#3}%
  \ifpgfutil@in@%  
    \tikz@parse@splitxyz{#1}{#2}#3,%
  \else%
    \tikz@checkunit{#2}%
    \iftikz@isdimension%
      \tikz@checkunit{#3}%
      \iftikz@isdimension%
        \def\@next{#1{\pgfpoint{#2}{#3}}}%
      \else%
        \def\@next{#1{\pgfpointadd{\pgfpoint{#2}{0pt}}{\pgfpointxy{0}{#3}}}}%
      \fi%
    \else%
      \tikz@checkunit{#3}%
      \iftikz@isdimension%
        \def\@next{#1{\pgfpointadd{\pgfpoint{0pt}{#3}}{\pgfpointxy{#2}{0}}}}%
      \else%
        \def\@next{#1{\pgfpointxy{#2}{#3}}}%
      \fi%
    \fi%
  \fi%
  \@next%
}

\def\tikz@parse@splitxyz#1#2#3,#4,{%
  \def\@next{#1{\pgfpointxyz{#2}{#3}{#4}}}%
}

\def\tikz@coordinate@text{coordinate}

\def\tikz@parse@node#1(#2){%
  \pgfutil@in@.{#2}% Ok, flag this
  \ifpgfutil@in@
    \tikz@calc@anchor#2\tikz@stop%
  \else%
    \tikz@calc@anchor#2.center\tikz@stop% to be on the save side, in
                                % case iftikz@shapeborder is ignored...
    \expandafter\ifx\csname pgf@sh@ns@#2\endcsname\tikz@coordinate@text%
    \else
      \tikz@shapebordertrue%
      \def\tikz@shapeborder@name{#2}%
    \fi%
  \fi%
  \edef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \tikz@marshal%
}

\def\tikz@calc@anchor#1.#2\tikz@stop{%
  \pgfpointanchor{#1}{#2}%
}


\def\tikz@parse@hv#1(#2){%
  \pgfutil@in@{ -| }{#2}%
  \ifpgfutil@in@%
    \let\tikz@next=\tikz@parse@hvboth%
  \else%
    \pgfutil@in@{ -|}{#2}%
    \ifpgfutil@in@%
      \let\tikz@next=\tikz@parse@hvleft%
    \else%
      \pgfutil@in@{-| }{#2}%
      \ifpgfutil@in@%
        \let\tikz@next=\tikz@parse@hvright%
      \else%
        \let\tikz@next=\tikz@parse@hvdone%
      \fi%
    \fi%
  \fi%
  \tikz@next#1(#2)}
\def\tikz@parse@hvboth#1(#2 -| #3){\tikz@parse@vhdone#1(#3|-#2)}
\def\tikz@parse@hvleft#1(#2 -|#3){\tikz@parse@vhdone#1(#3|-#2)}
\def\tikz@parse@hvright#1(#2-| #3){\tikz@parse@vhdone#1(#3|-#2)}
\def\tikz@parse@hvdone#1(#2-|#3){\tikz@parse@vhdone#1(#3|-#2)}

\def\tikz@parse@vh#1(#2){%
  \pgfutil@in@{ |- }{#2}%
  \ifpgfutil@in@%
    \let\tikz@next=\tikz@parse@vhboth%
  \else%
    \pgfutil@in@{ |-}{#2}%
    \ifpgfutil@in@%
      \let\tikz@next=\tikz@parse@vhleft%
    \else%
      \pgfutil@in@{|- }{#2}%
      \ifpgfutil@in@%
        \let\tikz@next=\tikz@parse@vhright%
      \else%
        \let\tikz@next=\tikz@parse@vhdone%
      \fi%
    \fi%
  \fi%
  \tikz@next#1(#2)}
\def\tikz@parse@vhboth#1(#2 |- #3){\tikz@parse@vhdone#1(#2|-#3)}
\def\tikz@parse@vhleft#1(#2 |-#3){\tikz@parse@vhdone#1(#2|-#3)}
\def\tikz@parse@vhright#1(#2|- #3){\tikz@parse@vhdone#1(#2|-#3)}
\def\tikz@parse@vhdone#1(#2|-#3){%
  {%
    \tikz@@@scan@@absolute\tikz@parse@vh@mid(#2)%
    \tikz@@@scan@@absolute\tikz@parse@vh@end(#3)%
    \xdef\tikz@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}}%
  }%
  \tikz@marshal%
}
\def\tikz@parse@vh@mid#1{\pgf@process{#1}\pgf@xa=\pgf@x}
\def\tikz@parse@vh@end#1{\pgf@process{#1}\pgf@ya=\pgf@y}

\def\tikz@parse@intersection#1(intersection{%
  \pgfutil@ifnextchar o{%
    \tikz@parse@main@intersection#1 1%
  }{%
    \tikz@parse@main@intersection#1%
  }%
}
\def\tikz@parse@main@intersection#1#2of #3 and #4){%
  \tikzset{cs/solution=#2}%
  \pgfutil@in@{--}{#3}%
  \ifpgfutil@in@%
    \tikz@reparse@line{first}#3\pgf@stop%
  \else%
    \tikzset{cs/first node=#3}%
  \fi%
  \pgfutil@in@{--}{#4}%
  \ifpgfutil@in@%
    \tikz@reparse@line{second}#4\pgf@stop%
  \else%
    \tikzset{cs/second node=#4}%
  \fi%
  \tikz@parse@cs@intersection()% advanced hackery...
  \edef\pgf@marshal{\noexpand#1{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \pgf@marshal%
}
\def\tikz@reparse@line#1#2--#3\pgf@stop{%
  \tikzset{cs/#1 line={(#2)--(#3)}}%
}


\def\tikz@parse@intersection@a#1{\pgf@process{#1}\pgf@xa=\pgf@x\pgf@ya=\pgf@y}
\def\tikz@parse@intersection@b#1{\pgf@process{#1}\pgf@xb=\pgf@x\pgf@yb=\pgf@y}

\def\tikz@scan@relative#1+{%
  \pgfutil@ifnextchar+{\tikz@scan@plusplus#1}{\tikz@scan@oneplus#1}}

\def\tikz@scan@plusplus#1+{%
  \def\tikz@doafter{#1}%
  \tikz@scan@absolute\tikz@add%
}
\def\tikz@add#1{%
  \tikz@doafter{\pgfpointadd{#1}{\tikz@last@position@saved}}%
}
\def\tikz@scan@oneplus#1{%
  \def\tikz@doafter{#1}%
  \tikz@updatecurrentfalse%
  \tikz@scan@absolute\tikz@add%
} 



% Loading further libraries

% Include a library file.
%
% #1 = List of names of library file.
%  
% Description:
%
% This command includes a list of TikZ library files. For each file X in the
% list, the file tikzlibraryX.code.tex is included, provided this has
% not been done earlier. 
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usetikzlibrary{arrows}
% \usetikzlibrary[patterns,topaths]

\def\usetikzlibrary{\pgfutil@ifnextchar[{\use@tikzlibrary}{\use@@tikzlibrary}}%}
\def\use@tikzlibrary[#1]{\use@@tikzlibrary{#1}}
\def\use@@tikzlibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\ifx\csname tikz@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\global\expandafter\let\csname tikz@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname tikz@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname tikz@library@#1@barcode\endcsname{\the\catcode`\|}
      \catcode`\@=11
      \catcode`\|=12
      \input tikzlibrary\pgf@temp.code.tex
      \catcode`\@=\csname tikz@library@#1@atcode\endcsname
      \catcode`\|=\csname tikz@library@#1@barcode\endcsname
    \fi%
  }%
}


% Always-present libraries:

\usetikzlibrary{topaths}




\endinput


==> tikz.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

% This file is tikz.tex

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

%\input xkeyval.tex % no longer used/needed

\input pgf.tex
\input pgffor.tex
\input tikz.code.tex

\catcode`\@=\tikzatcode

\endinput


==> tikzlibrary3d.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary3d.code.tex,v 1.1 2008/01/09 17:57:15 tantau Exp $



% New coordinate systems:

\tikzdeclarecoordinatesystem{xyz cylindrical}
{%
  \pgfset{/tikz/cs/.cd,angle=0,radius=0,z=0,#1}%
  \pgfpointcylindrical{\tikz@cs@angle}{\tikz@cs@radius}{\tikz@cs@z}%
}

\tikzdeclarecoordinatesystem{xyz spherical}
{%
  \pgfset{/tikz/cs/.cd,angle=0,radius=0,latitude=0,longitude=0,#1}%
  \pgfpointspherical{\tikz@cs@angle}{\tikz@cs@latitude}{\tikz@cs@radius}%
}

\pgfset{/tikz/cs/longitude/.store in=\tikz@cs@angle}
\pgfset{/tikz/cs/latitude/.store in=\tikz@cs@latitude}


% Options for transforming into a plane:

\tikzoption{plane origin}{\def\tikz@plane@origin{\tikz@scan@one@point\pgfutil@firstofone#1}}
\tikzoption{plane x}{\def\tikz@plane@x{\tikz@scan@one@point\pgfutil@firstofone#1}}
\tikzoption{plane y}{\def\tikz@plane@y{\tikz@scan@one@point\pgfutil@firstofone#1}}

\let\tikz@plane@origin=\pgfpointorigin
\def\tikz@plain@x{\pgfpointxy{1}{0}}
\def\tikz@plain@y{\pgfpointxy{0}{1}}

\tikzoption{canvas is plane}[]{
  \tikz@canvas@is@plane
}
\tikzoption{canvas is xy plane at z}{%
  \tikz@addtransform{\pgftransformshift{\pgfpointxyz{0}{0}{#1}}}%
}
\tikzoption{canvas is yx plane at z}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{0}{0}{#1}}%
  \def\tikz@plane@x{\pgfpointxyz{0}{1}{#1}}%
  \def\tikz@plane@y{\pgfpointxyz{1}{0}{#1}}%
  \tikz@canvas@is@plane
}
\tikzoption{canvas is xz plane at y}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{0}{#1}{0}}%
  \def\tikz@plane@x{\pgfpointxyz{1}{#1}{0}}%
  \def\tikz@plane@y{\pgfpointxyz{0}{#1}{1}}%
  \tikz@canvas@is@plane
}
\tikzoption{canvas is zx plane at y}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{0}{#1}{0}}%
  \def\tikz@plane@x{\pgfpointxyz{0}{#1}{1}}%
  \def\tikz@plane@y{\pgfpointxyz{1}{#1}{0}}%
  \tikz@canvas@is@plane
}
\tikzoption{canvas is yz plane at x}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{#1}{0}{0}}%
  \def\tikz@plane@x{\pgfpointxyz{#1}{1}{0}}%
  \def\tikz@plane@y{\pgfpointxyz{#1}{0}{1}}%
  \tikz@canvas@is@plane
}
\tikzoption{canvas is zy plane at x}[]{%
  \def\tikz@plane@origin{\pgfpointxyz{#1}{0}{0}}%
  \def\tikz@plane@x{\pgfpointxyz{#1}{0}{1}}%
  \def\tikz@plane@y{\pgfpointxyz{#1}{1}{0}}%
  \tikz@canvas@is@plane
}



% Transformation code

\def\tikz@canvas@is@plane{
  \pgf@process{\tikz@plane@x}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\tikz@plane@y}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \pgf@process{\tikz@plane@origin}%
  \edef\pgf@marshal{\noexpand\tikz@addtransform{%
      \noexpand\pgftransformtriangle
      {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      \noexpand\pgftransformscale{0.035146}%
      \noexpand\pgfsetxvec{\noexpand\pgfpoint{1cm}{0cm}}%
      \noexpand\pgfsetyvec{\noexpand\pgfpoint{0cm}{1cm}}%
      \noexpand\pgfsetzvec{\noexpand\pgfpoint{0cm}{0cm}}%
    }}%
  \pgf@marshal%
}

                                    
\endinput


==> tikzlibraryarrows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryarrows.code.tex,v 1.1 2008/01/09 17:57:15 tantau Exp $

\usepgflibrary{arrows}

\endinput


==> tikzlibraryautomata.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryautomata.code.tex,v 1.2 2008/02/14 10:31:22 tantau Exp $


% Styles for states:

\tikzstyle{every state}=           []

\tikzstyle{state without output}=  [circle,draw,minimum size=2.5em,every state]
\tikzstyle{state with output}=     [circle split,draw,minimum size=2.5em,every state]

\tikzstyle{accepting by arrow}=    [after node path=
{
  {
    [to path=
    {
      [->,double=none,every accepting by arrow]
      --
      ([shift=(\tikz@accepting@angle:\tikz@accepting@distance)]\tikztostart.\tikz@accepting@angle)
          node [shape=rectangle,anchor=\tikz@accepting@anchor] {\tikz@accepting@text}
      }]
    edge ()
  }
}]
\tikzstyle{every accepting by arrow}=[]
\tikzstyle{accepting by double}= [double,outer sep=.5\pgflinewidth+.3pt] % .3pt is half double width distance

\tikzstyle{initial by arrow}=   [after node path=
{
  {
    [to path=
    {
      [->,double=none,every initial by arrow]
      ([shift=(\tikz@initial@angle:\tikz@initial@distance)]\tikztostart.\tikz@initial@angle)
          node [shape=rectangle,anchor=\tikz@initial@anchor] {\tikz@initial@text}
        -- (\tikztostart)}]
    edge ()
  }
}]
\tikzstyle{every initial by arrow}=[]

\tikzstyle{initial by diamond}=[shape=diamond]


\tikzoption{initial text}{\tikzaddafternodepathoption{\def\tikz@initial@text{#1}}}
\tikzoption{accepting text}{\tikzaddafternodepathoption{\def\tikz@accepting@text{#1}}}

\tikzoption{initial where}{\tikzaddafternodepathoption{\csname tikz@initial@compute@#1\endcsname}}
\tikzoption{accepting where}{\tikzaddafternodepathoption{\csname tikz@accepting@compute@#1\endcsname}}

\tikzoption{initial distance}{\tikzaddafternodepathoption{\def\tikz@initial@distance{#1}}}
\tikzoption{accepting distance}{\tikzaddafternodepathoption{\def\tikz@accepting@distance{#1}}}

\def\tikz@initial@text{start}
\def\tikz@accepting@text{}

\def\tikz@initial@distance{3ex}
\def\tikz@accepting@distance{3ex}

\def\tikz@initial@compute@above{\def\tikz@initial@angle{90}\def\tikz@initial@anchor{south}}
\def\tikz@initial@compute@below{\def\tikz@initial@angle{270}\def\tikz@initial@anchor{north}}
\def\tikz@initial@compute@left{\def\tikz@initial@angle{180}\def\tikz@initial@anchor{east}}
\def\tikz@initial@compute@right{\def\tikz@initial@angle{0}\def\tikz@initial@anchor{west}}

\def\tikz@initial@angle{180}
\def\tikz@initial@anchor{east}

\def\tikz@accepting@compute@above{\def\tikz@accepting@angle{90}\def\tikz@accepting@anchor{south}}
\def\tikz@accepting@compute@below{\def\tikz@accepting@angle{270}\def\tikz@accepting@anchor{north}}
\def\tikz@accepting@compute@left{\def\tikz@accepting@angle{180}\def\tikz@accepting@anchor{east}}
\def\tikz@accepting@compute@right{\def\tikz@accepting@angle{0}\def\tikz@accepting@anchor{west}}

\def\tikz@accepting@angle{0}
\def\tikz@accepting@anchor{west}


\tikzstyle{initial above}=        [initial by arrow,initial where=above]
\tikzstyle{initial below}=        [initial by arrow,initial where=below]
\tikzstyle{initial left}=         [initial by arrow,initial where=left]
\tikzstyle{initial right}=        [initial by arrow,initial where=right]

\tikzstyle{accepting above}=      [accepting by arrow,accepting where=above]
\tikzstyle{accepting below}=      [accepting by arrow,accepting where=below]
\tikzstyle{accepting left}=       [accepting by arrow,accepting where=left]
\tikzstyle{accepting right}=      [accepting by arrow,accepting where=right]


% Defaults:

\tikzstyle{state}=                [state without output]
\tikzstyle{accepting}=            [accepting by double]
\tikzstyle{initial}=              [initial by arrow]



\endinput


==> tikzlibrarybackgrounds.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarybackgrounds.code.tex,v 1.1 2008/01/09 17:57:15 tantau Exp $


% Layers

\pgfdeclarelayer{background}
\pgfsetlayers{background,main}


% Main style

\tikzstyle{background rectangle}= [draw]
\tikzstyle{background top}=       [draw]
\tikzstyle{background bottom}=    [draw]
\tikzstyle{background left}=      [draw]
\tikzstyle{background right}=     [draw]
\tikzstyle{background grid}=      [help lines,draw]

\tikzoption{inner frame sep}{\def\tikz@framexsep{#1}\def\tikz@frameysep{#1}}
\tikzoption{inner frame xsep}{\def\tikz@framexsep{#1}}
\tikzoption{inner frame ysep}{\def\tikz@frameysep{#1}}
\def\tikz@framexsep{1ex}
\def\tikz@frameysep{1ex}

\tikzoption{outer frame sep}{\def\tikz@outerframexsep{#1}\def\tikz@outerframeysep{#1}}
\tikzoption{outer frame xsep}{\def\tikz@outerframexsep{#1}}
\tikzoption{outer frame ysep}{\def\tikz@outerframeysep{#1}}
\def\tikz@outerframexsep{0ex}
\def\tikz@outerframeysep{0ex}


% Looseness

\tikzstyle{loose background}=     [inner frame sep=2ex]
\tikzstyle{tight background}=     [inner frame sep=0ex]



% Showing background styles

\tikzstyle{framed}=                   [style=show background rectangle]
\tikzstyle{gridded}=                  [style=show background grid]

\tikzstyle{show background rectangle}=[execute at end picture=\tikz@background@framed]
\tikzstyle{show background top}=      [execute at end picture=\tikz@background@top]
\tikzstyle{show background bottom}=   [execute at end picture=\tikz@background@bottom]
\tikzstyle{show background left}=     [execute at end picture=\tikz@background@left]
\tikzstyle{show background right}=    [execute at end picture=\tikz@background@right]
\tikzstyle{show background grid}=     [execute at end picture=\tikz@background@grid]


% Implementation

\def\tikz@background@save{%
  \pgftransformreset%
  \ifx\tikz@bg@minx\@undefined%
    \pgf@xb=\pgf@picminx%
    \pgf@yb=\pgf@picminy%
    \pgf@xc=\pgf@picmaxx%
    \pgf@yc=\pgf@picmaxy%
    \pgfmathsetlength{\pgf@x}{\tikz@framexsep}%
    \pgfmathsetlength{\pgf@y}{\tikz@frameysep}%
    \advance\pgf@xb by-\pgf@x%
    \advance\pgf@yb by-\pgf@y%
    \advance\pgf@xc by\pgf@x%
    \advance\pgf@yc by\pgf@y%
    \edef\tikz@bg@minx{\the\pgf@xb}%
    \edef\tikz@bg@miny{\the\pgf@yb}%
    \edef\tikz@bg@maxx{\the\pgf@xc}%
    \edef\tikz@bg@maxy{\the\pgf@yc}%
    \pgfmathsetlength{\pgf@x}{\tikz@outerframexsep}%
    \pgfmathsetlength{\pgf@y}{\tikz@outerframeysep}%
    \advance\pgf@xb by-\pgf@x%
    \advance\pgf@yb by-\pgf@y%
    \advance\pgf@xc by\pgf@x%
    \advance\pgf@yc by\pgf@y%
    \edef\tikz@bg@outerminx{\the\pgf@xb}%
    \edef\tikz@bg@outerminy{\the\pgf@yb}%
    \edef\tikz@bg@outermaxx{\the\pgf@xc}%
    \edef\tikz@bg@outermaxy{\the\pgf@yc}%
  \fi%
}

\def\tikz@background@framed{%
  \tikz@background@save%
  \pgfonlayer{background}
    \path[style=background rectangle] (\tikz@bg@minx,\tikz@bg@miny) rectangle (\tikz@bg@maxx,\tikz@bg@maxy);
  \endpgfonlayer
}

\def\tikz@background@top{%
  \tikz@background@save%
  \pgfonlayer{background}
    \path[style=background top] (\tikz@bg@outerminx,\tikz@bg@maxy) -- (\tikz@bg@outermaxx,\tikz@bg@maxy);
  \endpgfonlayer
}

\def\tikz@background@bottom{%
  \tikz@background@save%
  \pgfonlayer{background}
    \path[style=background bottom] (\tikz@bg@outerminx,\tikz@bg@miny) -- (\tikz@bg@outermaxx,\tikz@bg@miny);
  \endpgfonlayer
}

\def\tikz@background@left{%
  \tikz@background@save%
  \pgfonlayer{background}
    \path[style=background left] (\tikz@bg@minx,\tikz@bg@outerminy) -- (\tikz@bg@minx,\tikz@bg@outermaxy);
  \endpgfonlayer
}

\def\tikz@background@right{%
  \tikz@background@save%
  \pgfonlayer{background}
    \path[style=background right] (\tikz@bg@maxx,\tikz@bg@outerminy) -- (\tikz@bg@maxx,\tikz@bg@outermaxy);
  \endpgfonlayer
}

\def\tikz@background@grid{%
  \tikz@background@save%
  \pgfonlayer{background}
    \path[style=background grid] (\tikz@bg@minx,\tikz@bg@miny) grid (\tikz@bg@maxx,\tikz@bg@maxy);
  \endpgfonlayer
}

                                    
\endinput


==> tikzlibrarycalc.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarycalc.code.tex,v 1.5 2008/02/04 17:19:55 tantau Exp $

%
%
% Part I: The let path command
% 
%


%
% Syntax: let \p{name1} = (coord), \p{name2} = (coord), ... in ...
%
% Currently (this may get more fancy in the future), the (coord)s are
% evaluated one by one. If the first evaluates to, say, (10pt,20pt),
% the macro \p{name1} is set to "10pt,20pt" (without parantheses), the
% macro \x{name1} is set to "10pt" and the macro \y{name1} is set to
% "20pt". 
%
% If you use a number for {name}, you need no parantheses, so you
% could write:
%
% \draw let
%         \p1 = (1,1),
%         \p2 = ($ 2.5*(3,2) $)
%       in
%         (\x1,\x2) -- (\y1,\y2);

\def\tikz@let@command et{%
  \let\p=\tikz@cc@dop%
  \let\x=\tikz@cc@dox%
  \let\y=\tikz@cc@doy%
  \let\n=\tikz@cc@don%
  \pgfutil@ifnextchar i{\tikz@cc@stop@let}{\tikz@cc@handle@line}%
}
\def\tikz@cc@handle@line{%
  \pgfutil@ifnextchar\p{%
    \tikz@cc@handle@coor%
  }{%
    \pgfutil@ifnextchar\n{%
      \tikz@cc@handle@num%
    }{%
      \PackageError{tikz}{``\string\p'' or ``\string\n'' expected}{}%
    }%
  }%
}
\def\tikz@cc@handle@num\n#1#2=#3{%
  \pgfmathparse{#3}%
  \expandafter\edef\csname tikz@cc@n@#1\endcsname{\pgfmathresult\ifpgfmathunitsdeclared pt\fi}
  \pgfutil@ifnextchar,{\tikz@cc@handle@nextline}{\tikz@cc@stop@let}%
}
\def\tikz@cc@handle@coor\p#1#2={%
  \def\tikz@cc@coord@name{#1}%
  \tikz@scan@one@point\tikz@cc@dolet%
}
\def\tikz@cc@dolet#1{%
  \pgf@process{#1}%
  \expandafter\edef\csname tikz@cc@p@\tikz@cc@coord@name\endcsname{\the\pgf@x,\the\pgf@y}%
  \expandafter\edef\csname tikz@cc@x@\tikz@cc@coord@name\endcsname{\the\pgf@x}%
  \expandafter\edef\csname tikz@cc@y@\tikz@cc@coord@name\endcsname{\the\pgf@y}%
  \pgfutil@ifnextchar,{\tikz@cc@handle@nextline}{\tikz@cc@stop@let}%
}
\def\tikz@cc@handle@nextline,{%
  \tikz@cc@handle@line%
}
\def\tikz@cc@stop@let in{%
  \tikz@scan@next@command%
}%

\def\tikz@cc@dop#1{\csname tikz@cc@p@#1\endcsname}
\def\tikz@cc@dox#1{\csname tikz@cc@x@#1\endcsname}
\def\tikz@cc@doy#1{\csname tikz@cc@y@#1\endcsname}
\def\tikz@cc@don#1{\csname tikz@cc@n@#1\endcsname}



%
%
% Part II: The ($...$) parser
%
%

\def\tikz@parse@calculator#1(${%$
  \def\tikz@cc@command{#1}%
  \begingroup%
    %
    % Parse main computation. It's a series of optional factors in front
    % of coordiantes.
    % 
    \pgf@xa=0pt% We accumulate the result in here.
    \pgf@ya=0pt%
    \tikz@cc@parse+% 
}

\def\tikz@cc@parse{%
  \pgfutil@ifnextchar${%$
    % Ok, we found the end...
    \tikz@cc@end%
  }
  {\pgfutil@ifnextchar+{%
      % Ok, we found a coordinate...
      \tikz@cc@add%
    }{%
      \pgfutil@ifnextchar-{%
        \tikz@cc@sub%
      }{%
        \PackageError{tikz}{+ or - expected}{}%
        \tikz@cc@end$%$
      }%
    }%
  }%
}

%
% The end is reached with $
%
\def\tikz@cc@end$#1){%$
    \xdef\tikz@marshal{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
  \endgroup%
  \expandafter\tikz@cc@command\expandafter{\tikz@marshal}%
}


%
% Another coordinate with +/-, possibly with a factor
%
\def\tikz@cc@add+{%
  \def\tikz@cc@factor{1}%
  \tikz@cc@factororcoordinate%
}
\def\tikz@cc@sub-{%
  \def\tikz@cc@factor{-1}%
  \tikz@cc@factororcoordinate%
}

%
% Check for a factor: If we see a (, its a coordinate...
% 
\def\tikz@cc@factororcoordinate{%
  \pgfutil@ifnextchar({%)
    % Ok, found coordinate
    \tikz@cc@coordinate%
  }{%
    \tikz@cc@parse@factor%
  }%
}

%
% ... otherwise it's a factor. It ends at ...*(
%
\def\tikz@cc@parse@factor#1*({%
  \pgfmathparse{#1*\tikz@cc@factor}%
  \let\tikz@cc@factor=\pgfmathresult%
  \tikz@cc@coordinate(%)
}

\def\tikz@cc@coordinate{%
  \tikz@scan@absolute\tikz@cc@after@coordinate%
}
\def\tikz@cc@after@coordinate#1{%
  \pgf@process{#1}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \tikz@cc@mid@checks%
}


%
% A coordinate can be followed by !...!(...)
%

\def\tikz@cc@mid@checks{
  \pgfutil@ifnextchar!{%
    \tikz@cc@mid%
  }{%
    \advance\pgf@xa by\tikz@cc@factor\pgf@xb%
    \advance\pgf@ya by\tikz@cc@factor\pgf@yb%
    \tikz@cc@parse% continue
  }%
}

\def\tikz@cc@mid!{%
  \pgfutil@ifnextchar({%
    \tikz@scan@one@point\tikz@cc@project%
  }{%
    \tikz@cc@mid@num%
  }%
}

%
% Partway case: (coord a)!number!(coord b)
%
% Returns the position that is at <number> fraction on the way from a
% to b. This, (a)!0!(b) is (a), (a)!.5!(b) is the middle and (a)!1!(b)
% is (b)
%
\def\tikz@cc@mid@num#1!{%
  \pgfmathparse{#1}%
  \ifpgfmathunitsdeclared%
    \let\tikz@cc@mid@unit=\pgfmathresult%
    \expandafter\tikz@cc@scan@rot\expandafter\tikz@cc@after@unit%
  \else%
    \let\tikz@cc@mid@factor=\pgfmathresult%
    \pgfmathparse{1-\tikz@cc@mid@factor}%
    \let\tikz@cc@mid@factor@one=\pgfmathresult%
    \expandafter\tikz@cc@scan@rot\expandafter\tikz@cc@after@num%
  \fi%
}

\def\tikz@cc@after@num#1{%
  \pgf@process{#1}%
  \pgf@xb=\tikz@cc@mid@factor@one\pgf@xb%
  \pgf@yb=\tikz@cc@mid@factor@one\pgf@yb%
  \advance\pgf@xb by\tikz@cc@mid@factor\pgf@x%
  \advance\pgf@yb by\tikz@cc@mid@factor\pgf@y%
  \tikz@cc@mid@checks%
}



%
% Distance case: (coord a)!dimension!(coord b)
%
% Returns the position that is at <dimension> removed from (coord a)
% in the direction of (coord b).
%

\def\tikz@cc@after@unit#1{%
  \pgf@process{#1}%
  \advance\pgf@x by-\pgf@xb%
  \advance\pgf@y by-\pgf@yb%
  \pgf@process{\pgfpointnormalised{}}%
  \advance\pgf@xb by\tikz@cc@mid@unit\pgf@x%
  \advance\pgf@yb by\tikz@cc@mid@unit\pgf@y%
  \tikz@cc@mid@checks%
}

%
% Projection case: (a)!(p)!(b)
%
% Projection of p on line from a to b
%
\def\tikz@cc@project#1{%
  \pgf@process{#1}%
  % Save in c
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \expandafter\tikz@cc@scan@rot\expandafter\tikz@cc@after@project\tikz@cc@scan@ex%
}

\def\tikz@cc@scan@ex!{}

\def\tikz@cc@after@project#1{%
  \pgf@process{#1}%
  % Ok, now we need to project (xc,yc) on the line (xb,xc) to (x,y)
  \advance\pgf@x by-\pgf@xb%
  \advance\pgf@y by-\pgf@yb%
  \advance\pgf@xc by-\pgf@xb%
  \advance\pgf@yc by-\pgf@yb%
  \pgf@process{\pgfpointnormalised{}}%
  % Scalar product
  \pgf@xc=\pgf@sys@tonumber{\pgf@xc}\pgf@x%
  \advance\pgf@xc by\pgf@sys@tonumber{\pgf@yc}\pgf@y%
  % and add
  \advance\pgf@xb by\pgf@sys@tonumber{\pgf@xc}\pgf@x%
  \advance\pgf@yb by\pgf@sys@tonumber{\pgf@xc}\pgf@y%
  \tikz@cc@mid@checks%
}

%
% Rotational scanner: radius:(x)
%

\def\tikz@cc@scan@rot#1{%
  \pgfutil@ifnextchar({%)
    \tikz@scan@one@point#1% normal
  }%
  {
    \def\tikz@cc@scan@rot@cmd{#1}
    \tikz@cc@scan@one@rot%
  }%
}

\def\tikz@cc@scan@one@rot#1:{%
  \def\tikz@cc@scan@rot@angle{#1}%
  \tikz@scan@one@point\tikz@cc@handle@rot%
}

\def\tikz@cc@handle@rot#1{%
  \pgf@process{#1}%
  % Ok, now we need to rotate x/y around xb/xb by ...rot@angle
  {%
    \pgftransformreset%
    % Save them...
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgftransformshift{\pgfqpoint{\pgf@xb}{\pgf@yb}}%
    \pgftransformrotate{\tikz@cc@scan@rot@angle}%
    \pgftransformshift{\pgfqpoint{-\pgf@xb}{-\pgf@yb}}%
    \pgfpointtransformed{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
    \expandafter
  }%
  \edef\tikz@marshal{\noexpand\tikz@cc@scan@rot@cmd{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \tikz@marshal%
}




%
%
% Part III: Calculation coordinate systems
% 
%

% Tangent cs: Keys are a node and a point. Depending on the type of
% node, the appropriate tanent computation should be done.

\tikzdeclarecoordinatesystem{tangent}
{%
  \tikzset{cs/.cd,#1}%
  \expandafter\ifx\csname tikz@tangent@\tikz@cs@type\endcsname\relax%
    \PackageError{tikz}{I do not know how to compute the tangent to 
    a \tikz@cs@type}{}%
    \pgfpointorigin%
  \else%
    \expandafter\tikz@scan@one@point\expandafter\tikz@lib@do@tangent\tikz@cs@point%  
  \fi%
}

\tikzset{cs/node/.code=\tikz@cs@unpack{\tikz@cs@node}{\tikz@cs@type}{#1}}
\tikzset{cs/point/.store in=\tikz@cs@point}

\def\tikz@lib@do@tangent{\csname tikz@tangent@\tikz@cs@type\endcsname}

\def\tikz@tangent@coordinate#1{%
  \pgfpointanchor{\tikz@cs@node}{center}%
}

\def\tikz@tangent@circle#1{%
  {%
    % Step 1: Compute the transformed position of the input:
    \pgf@process{\pgfpointtransformed{#1}}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    %
    % Step 2: Compute vector from center of circle to transformed #1
    %
    \pgf@process{\pgfpointtransformed{\pgfpointanchor{\tikz@cs@node}{center}}}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    %
    % Step 2: Reset transformations, they distract...
    %
    \pgftransformreset%
    %
    % Step 3: Transform to the center of the circle.
    %
    \pgftransformshift{\pgfpointanchor{\tikz@cs@node}{center}}%
    %
    % Step 4: Compute the radius
    %
    \pgf@process{\pgfpointanchor{\tikz@cs@node}{east}}%
    \pgf@xc=\pgf@x%
    %
    % Now, (xa,ya) is a point. Compute the tangent from this point to
    % a circle around the origin of radius xc.
    %
    % acos(radius/veclen(xa,ya)) is the angle of the tangent.
    \pgfmathparse{veclen(\the\pgf@xa,\the\pgf@ya)}
    \pgfmathparse{acos(\the\pgf@xc/\pgfmathresult)}
    \ifnum\pgfkeysvalueof{/tikz/cs/solution}>1\relax%
      \pgfmathsubtract{0}{\pgfmathresult}%
    \fi%
    \let\tikz@lib@temp=\pgfmathresult%
    %
    % Now \pgfmathparse contains the desired angle. Use this to
    % compute the correct position on the circle...
    %
    % But, first, rotate to the point.
    \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    \pgf@ya=-\pgf@y%
    \pgftransformcm{\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}{\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}{\pgfpointorigin}%
    % Finally, rotate...
    \pgf@process{\pgfpointtransformed{\pgfpointpolar{\tikz@lib@temp}{\the\pgf@xc}}}%
    %
    % Ok, undo transformations...
  }%
  % \pgf@x, \pgf@y have been smuggled outside by \pgf@process
  {%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{}}%
  }%
}


% Implementation of intersections


\def\tikz@intersect@circle@and@circle{%
  {%
    \pgftransformreset% transformations only confuse us, here...
    %
    % Compute origin and radius of first circle
    %
    \pgf@process{\pgfpointanchor{\tikz@cs@node@a}{center}}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\pgfpointanchor{\tikz@cs@node@a}{east}}%
    \advance\pgf@x by-\pgf@xa%
    \pgf@xc=\pgf@x% ok, pgf@xc is first radius, (xa,ya) is center
    %
    % Compute origin and radius of second circle
    %
    \pgf@process{\pgfpointanchor{\tikz@cs@node@b}{center}}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{\pgfpointanchor{\tikz@cs@node@b}{east}}%
    \advance\pgf@x by-\pgf@xb%
    \pgf@yc=\pgf@x% \pgf@yc is second radius, (xb,yb) is center
    %
    \pgf@process{%
      \pgfpointintersectionofcircles{\pgfqpoint{\pgf@xa}{\pgf@ya}}{\pgfqpoint{\pgf@xb}{\pgf@yb}}{\pgf@xc}{\pgf@yc}{\pgfkeysvalueof{/tikz/cs/solution}}%
    }%
  }%
  % \pgf@x, \pgf@y have been smuggled outside by \pgf@process,
  % reinstall transformations...
  {%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{}}%
  }%
}


\def\tikz@intersect@line@and@circle{%
  {%
    %
    % Step 1: Get line
    %
    \expandafter\tikz@scan@one@point\expandafter\tikz@parse@line\tikz@cs@line@a%
    \pgf@process{\pgfpointtransformed{}}%
    \pgf@xb=\pgf@x%
    \pgf@yb=\pgf@y%
    \pgf@process{\pgfpointtransformed{\pgfqpoint{\pgf@xc}{\pgf@yc}}}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    %
    % Step 2: Subtract center of circle
    %
    \pgf@process{\pgfpointtransformed{\pgfpointanchor{\tikz@cs@node@b}{center}}}%
    \advance\pgf@xa by-\pgf@x%
    \advance\pgf@ya by-\pgf@y%
    \advance\pgf@xb by-\pgf@x%
    \advance\pgf@yb by-\pgf@y%
    %
    % Step 3: Reset transformations, they distract...
    %
    \pgftransformreset%
    %
    % Step 4: Transform to the center of the circle.
    %
    \pgftransformshift{\pgfpointanchor{\tikz@cs@node@b}{center}}%
    %
    % Step 5: Compute the radius
    %
    \pgf@process{\pgfpointanchor{\tikz@cs@node@b}{east}}%
    \edef\tikz@lib@saved@radius{\pgf@sys@tonumber{\pgf@x}}%
    %
    % Step 6: Compute projection of origin on line (xa,ya) -- (xb,yb),
    % store in (xa,ya)
    \pgf@x=\pgf@xb%
    \pgf@y=\pgf@yb%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@process{\pgfpointnormalised{}}%
    % Scalar product
    \pgf@xc=\pgf@sys@tonumber{\pgf@xa}\pgf@x%
    \advance\pgf@xc by\pgf@sys@tonumber{\pgf@ya}\pgf@y%
    \pgf@xc=-\pgf@xc%
    % and add
    \advance\pgf@xa by\pgf@sys@tonumber{\pgf@xc}\pgf@x%
    \advance\pgf@ya by\pgf@sys@tonumber{\pgf@xc}\pgf@y%
    % 
    % Now, we have a triangle with a right angle at (xa,ya). The
    % second point of the triangle is the origin. The third point is
    % sought. 
    % Save x/y
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    % Square radius
    \pgf@xb=\tikz@lib@saved@radius pt%
    %
    % First, make numbers smaller, in case they are too large
    %
    \c@pgf@counta=1\relax%
    \loop%
    \ifdim\pgf@xb>50pt%
      \multiply\c@pgf@counta by2\relax%
      \divide\pgf@xa by2\relax%
      \divide\pgf@ya by2\relax%
      \divide\pgf@xb by2\relax%
    \repeat%
    \pgf@xb=\pgf@sys@tonumber{\pgf@xb}\pgf@xb%
    % Subtract xa^2 + ya^2
    \pgf@yb=\pgf@sys@tonumber{\pgf@xa}\pgf@xa%
    \advance\pgf@xb by-\pgf@yb%
    \pgf@yb=\pgf@sys@tonumber{\pgf@ya}\pgf@ya%
    \advance\pgf@xb by-\pgf@yb%
    % Square root
    \ifdim\pgf@xb<0pt%
      \pgf@xb=0pt%
    \fi%
    \pgfmathsqrt@{\pgf@sys@tonumber{\pgf@xb}}%
    \pgfmathmultiply@{\pgfmathresult}{\the\c@pgf@counta}%
    \multiply\pgf@xa by\c@pgf@counta\relax%
    \multiply\pgf@ya by\c@pgf@counta\relax%
    \ifnum\pgfkeysvalueof{/tikz/cs/solution}>1\relax%
      \pgfmathsubtract{0}{\pgfmathresult}%
    \fi%
    % Ok, now add things...
    \advance\pgf@xa by \pgfmathresult\pgf@xc%
    \advance\pgf@ya by \pgfmathresult\pgf@yc%
    \pgf@process{\pgfpointtransformed{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
    % Ok, undo transformations...
  }%
  % \pgf@x, \pgf@y have been smuggled outside by \pgf@process
  {%
    \pgftransforminvert%
    \pgf@process{\pgfpointtransformed{}}%
  }%
}

\def\tikz@intersect@circle@and@line{%
  % Swap
  {%
    \let\tikz@cs@node@b=\tikz@cs@node@a%
    \let\tikz@cs@line@a=\tikz@cs@line@b%
    \tikz@intersect@line@and@circle%
  }%
}



==> tikzlibrarycalendar.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarycalendar.code.tex,v 1.1 2008/01/09 17:57:15 tantau Exp $


\pgfutil@usemodule{pgfcalendar}


%
% General options (these options affect all calendars typeset unsind \calendar):
%
% Start, end, and code executed for each current date
%

\tikzoption{dates}{\tikz@lib@cal@parse#1\relax}
\def\tikz@lib@cal@parse#1to#2\relax{%
  \def\tikz@lib@cal@start{#1}
  \def\tikz@lib@cal@end{#2}%
}
\tikzoption{execute at begin day scope}{\expandafter\def\expandafter\tikz@atbegin@day\expandafter{\tikz@atbegin@day#1}}
\tikzoption{execute at end day scope}{%
  \def\pgf@temp{#1}%
  \expandafter\expandafter\expandafter\def%
  \expandafter\expandafter\expandafter\tikz@atend@day%
  \expandafter\expandafter\expandafter{\expandafter\pgf@temp\tikz@atend@day}}
\tikzoption{execute before day scope}{\expandafter\def\expandafter\tikz@before@day\expandafter{\tikz@before@day#1}}
\tikzoption{execute after day scope}{\expandafter\def\expandafter\tikz@after@day\expandafter{\tikz@after@day#1}}

\let\tikz@atbegin@day=\pgfutil@empty
\let\tikz@atend@day=\pgfutil@empty
\let\tikz@before@day=\pgfutil@empty
\let\tikz@after@day=\pgfutil@empty



% 
% Options affecting some calendars:
%

%
% Shifts and skips
%

% Shift between days 

\tikzoption{day xshift}{\def\tikz@lib@cal@xshift{#1}}
\tikzoption{day yshift}{\def\tikz@lib@cal@yshift{#1}}

\def\tikz@lib@cal@yshift{3ex}
\def\tikz@lib@cal@xshift{3.5ex}


% Shift between months

\tikzoption{month xshift}{\def\tikz@lib@cal@month@xshift{#1}}
\tikzoption{month yshift}{\def\tikz@lib@cal@month@yshift{#1}}

\def\tikz@lib@cal@month@yshift{9ex}
\def\tikz@lib@cal@month@xshift{9ex}




% Templates for typesetting days, month, years

\tikzoption{day code}{\def\tikzdaycode{#1}}
\tikzoption{day text}{\def\tikzdaytext{#1}}
\tikzoption{days}{\tikzstyle{every day}+=[#1]}
\tikzstyle{every day}=[anchor=base east]

\tikzoption{month code}{\def\tikzmonthcode{#1}}
\tikzoption{month text}{\def\tikzmonthtext{#1}}
\tikzstyle{every month}=[]

\tikzoption{year code}{\def\tikzyearcode{#1}}
\tikzoption{year text}{\def\tikzyeartext{#1}}
\tikzstyle{every year}=[]

\def\tikzdaycode{\node[name=\pgfcalendarsuggestedname,every day]{\tikzdaytext};}
\def\tikzmonthcode{\node[every month]{\tikzmonthtext};}
\def\tikzyearcode{\node[every year]{\tikzyeartext};}

\def\tikzdaytext{\%d-}
\def\tikzmonthtext{\%mt}
\def\tikzyeartext{\%y0}


% Internal option for storing the "width" of a calendar as a number of
% days 

\tikzoption{tikz@lib@cal@width}{\def\tikz@lib@cal@width{#1}}

\def\tikz@lib@cal@width{1}

%
% Days on a line
%

\tikzstyle{day list downward}=[%
  execute before day scope={
    \ifdate{day of month=1}{\ifdate{equals=\pgfcalendarbeginiso}{}
      {%
        % On first of month, except when first date in calendar.
        \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@month@yshift}%
        \pgftransformyshift{-\pgf@y}
      }%
    }{}%
  },  
  execute after day scope={\pgfmathsetlength{\pgf@y}{\tikz@lib@cal@yshift}\pgftransformyshift{-\pgf@y}},
  tikz@lib@cal@width=1
]
\tikzstyle{day list upward}=[%
  execute before day scope={
    \ifdate{day of month=1}{\ifdate{equals=\pgfcalendarbeginiso}{}
      {%
        % On first of month, except when first date in calendar.
        \pgftransformyshift{\tikz@lib@cal@month@yshift}%
      }%
    }{}%
  },  
  execute after day scope={\pgftransformyshift\tikz@lib@cal@yshift},
  tikz@lib@cal@width=1
]
\tikzstyle{day list right}=[%
  execute before day scope={
    \ifdate{day of month=1}{\ifdate{equals=\pgfcalendarbeginiso}{}
      {%
        % On first of month, except when first date in calendar.
        \pgftransformxshift{\tikz@lib@cal@month@xshift}%
      }%
    }{}%
  },  
  execute after day scope={\pgftransformxshift\tikz@lib@cal@xshift},
  tikz@lib@cal@width=30% not quite right, but close enough in most cases...
]

\tikzstyle{day list left}=[%
  execute before day scope={
    \ifdate{day of month=1}{\ifdate{equals=\pgfcalendarbeginiso}{}
      {%
        % On first of month, except when first date in calendar.
        \pgfmathsetlength{\pgf@x}{\tikz@lib@cal@month@xshift}
        \pgftransformxshift{-\pgf@x}%
      }%
    }{}%
  },  
  execute after day scope={
    \pgfmathsetlength{\pgf@x}{\tikz@lib@cal@xshift}
    \pgftransformxshift{-\pgf@x}%
  },
  tikz@lib@cal@width=30% not quite right, but close enough in most cases...
]



%
% Week list
%

\tikzstyle{week list}=[%
  execute before day scope={%
    \ifdate{day of month=1}{\ifdate{equals=\pgfcalendarbeginiso}{}
      {%
        % On first of month, except when first date in calendar.
        \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@month@yshift}%
        \pgftransformyshift{-\pgf@y}
      }%
    }{}%
  }, 
  execute at begin day scope={%
    \pgfmathsetlength\pgf@x{\tikz@lib@cal@xshift}%
    \pgf@x=\pgfcalendarcurrentweekday\pgf@x%
    \pgftransformxshift{\pgf@x}%
  },
  execute after day scope={%
    \ifdate{Sunday}{%
      \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@yshift}%
      \pgftransformyshift{-\pgf@y}
    }{}%
  },
  tikz@lib@cal@width=7
]



%
% Month list
%

\tikzstyle{month list}=[%
  execute before day scope={%
    \ifdate{day of month=1}{\ifdate{equals=\pgfcalendarbeginiso}{}
      {%
        % On first of month, except when first date in calendar.
        \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@month@yshift}%
        \pgftransformyshift{-\pgf@y}
      }%
    }{}%
    \ifdate{day of month=1}
    {%
      \edef\tikz@lib@cal@month@list@start{\pgfcalendarcurrentweekday}%
    }{}%
    \ifdate{equals=\pgfcalendarbeginiso}%
    {%
      % Computer day of week for start of month
      {%
        \c@pgf@counta=\pgfcalendarcurrentjulian%
        \advance\c@pgf@counta by-\pgfcalendarcurrentday%
        \advance\c@pgf@counta by1\relax%
        \pgfcalendarjuliantoweekday{\c@pgf@counta}{\c@pgf@countb}%
        \xdef\pgf@temp{\the\c@pgf@countb}%
      }%
      \let\tikz@lib@cal@month@list@start=\pgf@temp%
    }{}%
  }, 
  execute at begin day scope={%
    \pgfmathsetlength\pgf@xa{\tikz@lib@cal@xshift}%
    \pgf@xb=\pgfcalendarcurrentday\pgf@xa%
    \advance\pgf@xb by\tikz@lib@cal@month@list@start\pgf@xa%
    \advance\pgf@xb by-\pgf@xa\relax%
    \pgftransformxshift{\pgf@xb}%
  },
  tikz@lib@cal@width=37
]




%
% Month labels
%

\tikzstyle{month label left}=[%
  execute before day scope={\ifdate{day of month=1}{\tikzmonthcode}{}},
  every month/.append style={anchor=base east,xshift=-3.5ex}
]

\tikzstyle{month label left vertical}=[%
  execute before day scope={\ifdate{day of month=1}{\tikzmonthcode}{}},
  every month/.append style={anchor=base east,xshift=-4.5ex,yshift=2.25ex,rotate=90}
]
  
\tikzstyle{month label right}=[%
execute before day scope={\ifdate{day of month=1}{%
    {%
      \pgfmathsetlength{\pgf@xa}{\tikz@lib@cal@xshift}%
      \pgftransformxshift{\tikz@lib@cal@width\pgf@xa}%
      \pgftransformxshift{-\pgf@xa}%
      \tikzmonthcode%
    }}{}},
  every month/.append style={anchor=base west,xshift=1ex}
]

\tikzstyle{month label right vertical}=[%
  execute before day scope={\ifdate{day of month=1}{%
    {%
      \pgfmathsetlength{\pgf@xa}{\tikz@lib@cal@xshift}%
      \pgftransformxshift{\tikz@lib@cal@width\pgf@xa}%
      \pgftransformxshift{-\pgf@xa}%
      \tikzmonthcode%
    }}{}},
  every month/.append style={anchor=base west,xshift=2ex,yshift=2.25ex,rotate=-90}
]

\tikzstyle{month label above centered}=[%
  execute before day scope={%
    \ifdate{day of month=1}{%
      {
        \pgfmathsetlength{\pgf@xa}{\tikz@lib@cal@xshift}%
        \pgf@xb=\tikz@lib@cal@width\pgf@xa%
        \advance\pgf@xb by-\pgf@xa%
        \pgf@xb=.5\pgf@xb%
        \pgftransformxshift{\pgf@xb}%
        \pgftransformxshift{-1.5ex}%
        \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@yshift}%
        \pgftransformyshift{1.25\pgf@y}
        \tikzmonthcode%
      }
    }{}},
  every month/.append style={anchor=base}
]
  
\tikzstyle{month label above left}=[%
  execute before day scope={%
    \ifdate{day of month=1}{%
      {
        \pgftransformxshift{-3.25ex}%
        \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@yshift}%
        \pgftransformyshift{1.25\pgf@y}
        \tikzmonthcode%
      }
    }{}},
  every month/.append style={anchor=base west}
]



\tikzstyle{month label above right}=[%
  execute before day scope={%
    \ifdate{day of month=1}{%
      {
        \pgfmathsetlength{\pgf@xa}{\tikz@lib@cal@xshift}%
        \pgf@xb=\tikz@lib@cal@width\pgf@xa%
        \advance\pgf@xb by-\pgf@xa%
        \pgftransformxshift{\pgf@xb}%
        \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@yshift}%
        \pgftransformyshift{1.25\pgf@y}
        \tikzmonthcode%
      }
    }{}},
  every month/.append style={anchor=base east}
]
  
\tikzstyle{month label below centered}=[%
  execute before day scope={%
    \ifdate{day of month=1}{%
      {
        \pgfmathsetlength{\pgf@xa}{\tikz@lib@cal@xshift}%
        \pgf@xb=\tikz@lib@cal@width\pgf@xa%
        \advance\pgf@xb by-\pgf@xa%
        \pgf@xb=.5\pgf@xb%
        \pgftransformxshift{\pgf@xb}%
        \pgftransformxshift{-1.5ex}%
        \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@yshift}%
        \pgftransformyshift{-1.25\pgf@y}
        \tikzmonthcode%
      }
    }{}},
  every month/.append style={anchor=base}
]
  
\tikzstyle{month label below left}=[%
  execute before day scope={%
    \ifdate{day of month=1}{%
      {
        \pgftransformxshift{-3.25ex}%
        \pgfmathsetlength{\pgf@y}{\tikz@lib@cal@yshift}%
        \pgftransformyshift{-1.25\pgf@y}
        \tikzmonthcode%
      }
    }{}},
  every month/.append style={anchor=base west}
]



%
% Code of the actual \calendar command (tikz.code.tex contains \let\calendar=\tikz@lib@cal@calendar):
%

\def\tikz@lib@cal@calendar{%
  \begingroup%
    \let\tikz@lib@cal@ifs=\pgfutil@empty%
    \tikz@expandcount=1000\relax%
    \tikzset{name=,at={(0,0)}}%
    \let\%=\pgfcalendarshorthand%
    \tikzset{every calendar/.try}%
    \tikz@lib@cal@scanner%
}

\def\tikz@lib@cal@scanner{%
  \afterassignment\tikz@lib@cal@handle\let\@let@token=%
}

\def\tikz@lib@cal@handle{%
  \let\@next=\tikz@lib@cal@expand%
  \ifx\@let@token;%
    \let\@next=\tikz@lib@cal@stop%
  \else%
    \ifx\@let@token(%)
      \let\@next=\tikz@lib@cal@name%
    \else%
      \ifx\@let@token a%
        \let\@next=\tikz@lib@cal@at%
      \else%
        \ifx\@let@token[%
          \let\@next=\tikz@lib@cal@option%
        \else%
          \ifx\@let@token i%
            \let\@next=\tikz@lib@cal@if%
          \fi%
        \fi%
      \fi%
    \fi%
  \fi%
  \@next%
}
\def\tikz@lib@cal@expand{%
  \advance\tikz@expandcount by -1%
  \ifnum\tikz@expandcount<0\relax%
    \PackageError{tikz}{Giving up on this calendar}{}%
    \let\@next=\tikz@lib@cal@end%
  \else%
    \let\@next=\tikz@lib@cal@@expand
  \fi%
  \@next}

\def\tikz@lib@cal@@expand{\expandafter\tikz@lib@cal@scanner\@let@token}


\def\tikz@lib@cal@name#1){%
  \tikzset{name=#1}%
  \tikz@lib@cal@scanner%
}
\def\tikz@lib@cal@at t#1(#2){%
  \tikzset{at={(#2)}}%
  \tikz@lib@cal@scanner%
}
\def\tikz@lib@cal@option#1]{%
  \tikzset{#1}%
  \tikz@lib@cal@scanner%
}
\def\tikz@lib@cal@if f#1(#2){%
  \pgfutil@ifnextchar[{\tikz@lib@cal@if@opt{#2}}{\tikz@lib@cal@if@code{#2}}}%}

\def\tikz@lib@cal@if@opt#1[#2]{\tikz@lib@cal@if@code{#1}{\tikzset{#2}}}
\def\tikz@lib@cal@if@code#1#2{%
  \pgfutil@ifnextchar e{\tikz@lib@cal@if@else{#1}{#2}}{\tikz@lib@cal@if@else{#1}{#2}else{}}}

\def\tikz@lib@cal@if@else#1#2else{%
  \pgfutil@ifnextchar[{\tikz@lib@cal@if@else@opt{#1}{#2}}{\tikz@lib@cal@if@else@code{#1}{#2}}}%}
\def\tikz@lib@cal@if@else@opt#1#2[#3]{\tikz@lib@cal@if@else@code{#1}{#2}{\tikzset{#3}}}
\def\tikz@lib@cal@if@else@code#1#2#3{%
  \expandafter\def\expandafter\tikz@lib@cal@ifs\expandafter{\tikz@lib@cal@ifs\ifdate{#1}{#2}{#3}}%
  \tikz@lib@cal@scanner%
}
\def\tikz@lib@cal@stop{%
    \pgftransformshift{\tikz@node@at}%
    \expandafter\pgfcalendar\expandafter{\tikz@fig@name}{\tikz@lib@cal@start}{\tikz@lib@cal@end}%
    {%
      \tikz@before@day%  
      \scope%
        \tikz@atbegin@day%
        \tikz@lib@cal@ifs%
        \tikzdaycode%
        \tikz@atend@day%
      \endscope%
      \tikz@after@day%  
    }%
  \endgroup%
}

\tikzoption{if}{%
  \let\tikz@lib@cal@scanner@orig=\tikz@lib@cal@scanner%
  \let\tikz@lib@cal@scanner=\relax%
  \tikz@lib@cal@if f#1\relax%
  \let\tikz@lib@cal@scanner=\tikz@lib@cal@scanner@orig}



\endinput


==> tikzlibrarychains.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarychains.code.tex,v 1.4 2008/02/12 23:41:59 tantau Exp $

\tikzset{start chain/.default=,
         start chain/.code={%
    \tikz@lib@chain@parse{#1}%
    \ifx\tikz@lib@chain@name\pgfutil@empty%
      \def\tikz@lib@chain@name{chain}%
    \fi%
    \ifx\tikz@lib@chain@direction\relax%
      \let\tikz@lib@chain@direction=\tikz@lib@chain@default@direction%
    \fi%
    \expandafter\ifx\csname tikz@lib@chain@active@\tikz@lib@chain@name\endcsname\relax%
      \expandafter\let\csname tikz@lib@chain@active@\tikz@lib@chain@name\endcsname=\pgfutil@empty% does not matter
      \expandafter\global\expandafter\let\csname tikz@lib@chain@exists@\tikz@lib@chain@name\endcsname=\pgfutil@empty% does not matter
      % Setup chain parameters
      \expandafter\gdef\csname tikz@lib@chain@count@\tikz@lib@chain@name\endcsname{0}%
      \expandafter\global\expandafter\let\csname tikz@lib@chain@dir@\tikz@lib@chain@name\endcsname\tikz@lib@chain@direction%
      \let\tikz@lib@current@chain=\tikz@lib@chain@name%
      \let\chainin=\tikz@lib@chainin%
    \else%
      \PackageError{tikz}{Chain ``\tikz@lib@chain@name'' is already active}{}%
    \fi%
  },
  continue chain/.default=,
  continue chain/.code={%
    \tikz@lib@chain@parse{#1}%
    \ifx\tikz@lib@chain@name\pgfutil@empty%
      \let\tikz@lib@chain@name\tikz@lib@current@chain%
    \fi%
    \expandafter\ifx\csname tikz@lib@chain@exists@\tikz@lib@chain@name\endcsname\relax%
      \PackageError{tikz}{Unknown chain ``#1''}{}%
    \else%
      \let\tikz@lib@current@chain=\tikz@lib@chain@name%
      \expandafter\let\csname tikz@lib@chain@active@\tikz@lib@chain@name\endcsname=\pgfutil@empty% does not matter
      \ifx\tikz@lib@chain@direction\relax%
        % Just restart...
      \else%
        % Setup chain parameters
        \expandafter\global\expandafter\let\csname tikz@lib@chain@dir@\tikz@lib@chain@name\endcsname\tikz@lib@chain@direction%
      \fi%
    \fi%
  },
  join/.code=\tikz@lib@parse@join{#1},
  join/.default={}% 
}

\def\tikz@lib@chain@parse#1{%
  \pgfutil@in@{going }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@chain@going#1\pgf@stop%
  \else%
    \pgfutil@in@{placed }{#1}%
    \ifpgfutil@in@%
      \tikz@lib@chain@positioning#1\pgf@stop%
    \else%
      \def\tikz@lib@chain@name{#1}%
      \let\tikz@lib@chain@direction\relax%
    \fi%
  \fi%
}

\def\tikz@lib@chain@going#1going #2\pgf@stop{%
  \def\tikz@lib@chain@name{#1}%
  \ifx\tikz@lib@chain@name\pgfutil@empty%
  \else%
    \tikz@lib@chain@strip#1\pgf@stop%%
  \fi%
  \tikz@lib@chain@is@goingtrue%
  \def\tikz@lib@chain@direction{%
    \ifx\tikzchainprevious\pgfutil@empty%
    \else%
      \tikz@lib@chain@place{#2}%
    \fi%
  }%  
}

\def\tikz@lib@chain@positioning#1placed #2\pgf@stop{%
  \def\tikz@lib@chain@name{#1}%
  \ifx\tikz@lib@chain@name\pgfutil@empty%
  \else%
    \tikz@lib@chain@strip#1\pgf@stop%%
  \fi%
  \tikz@lib@chain@is@goingfalse%
  \def\tikz@lib@chain@direction{\tikz@lib@chain@place{#2}}%
}
\newif\iftikz@lib@chain@is@going


\tikzset{/tikz/chain default direction/.code=%
  {%
    \tikz@lib@chain@parse{#1}%
    \let\tikz@lib@chain@default@direction=\tikz@lib@chain@direction%
  },%
  /tikz/chain default direction=going right
}

\def\tikz@lib@current@chain{chain}

\pgfutil@g@addto@macro\tikz@node@reset@hook{\let\tikz@lib@chain@caller=\relax}
\pgfutil@g@addto@macro\tikz@node@begin@hook{\tikz@lib@chain@caller}

\tikzset{
  on chain/.default=,
  on chain/.code=\tikz@lib@on@chain{#1}%
}
\def\tikz@lib@on@chain#1{%    
  \tikz@lib@chain@parse{#1}%
  \ifx\tikz@lib@chain@name\pgfutil@empty%
    \let\tikz@lib@chain@name\tikz@lib@current@chain%
  \fi%
  \expandafter\ifx\csname tikz@lib@chain@exists@\tikz@lib@chain@name\endcsname\relax%
    \PackageError{tikz}{Unknown chain ``\tikz@lib@chain@name''}{}%
  \else%
    \c@pgf@counta\csname tikz@lib@chain@count@\tikz@lib@chain@name\endcsname\relax%
    \ifnum\c@pgf@counta=0\relax%
      \global\let\tikzchainprevious=\pgfutil@empty%
    \else
      \xdef\tikzchainprevious{\tikz@lib@chain@name-\the\c@pgf@counta}%
    \fi%
    \advance\c@pgf@counta by1\relax%
    \xdef\tikzchaincount{\the\c@pgf@counta}%
    \ifx\tikz@lib@chain@direction\relax%
      \csname tikz@lib@chain@dir@\tikz@lib@chain@name\endcsname% use default
    \else%
      \tikz@lib@chain@direction%
    \fi%
    \edef\tikz@lib@chain@caller{\noexpand\tikz@lib@chain@last@found{\tikz@lib@chain@name}}%
  \fi%
}
\def\tikz@lib@chain@last@found#1{%
  % Increase the count and set name, if necessary.
  \c@pgf@counta\csname tikz@lib@chain@count@#1\endcsname\relax%
  \advance\c@pgf@counta by1\relax%
  \xdef\tikzchaincurrent{#1-\the\c@pgf@counta}%
  \expandafter\xdef\csname tikz@lib@chain@count@#1\endcsname{\the\c@pgf@counta}%
  \ifnum\c@pgf@counta=1\relax%
    \tikzset{alias/.expanded=#1-begin} % Define pseudostart
  \fi%    
  \tikzset{alias/.expanded=#1-end} % Define pseudostart
  \tikzset{alias/.expanded=#1-\the\c@pgf@counta} % Define pseudostart
  \tikz@lib@chain@direction%
  \tikzset{every on chain/.try}%
}


\def\tikz@lib@chain@place#1{%
  \pgfutil@in@{=}{#1}%
  \ifpgfutil@in@%
    \tikzset{#1}%
  \else%
    \tikzset{#1=of \tikzchainprevious}%
  \fi%
}

\def\tikz@lib@chain@strip#1 \pgf@stop{%
  \def\tikz@lib@chain@name{#1}%
}

\def\tikz@lib@parse@join#1{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
    \tikz@lib@parse@join@by by \pgf@stop%
  \else%
    \pgfutil@in@{with }{#1}%
    \ifpgfutil@in@%
      \pgfutil@in@{by }{#1}%
      \ifpgfutil@in@%
        \tikz@lib@parse@join@with@by#1\pgf@stop%
      \else%
        \tikz@lib@parse@join@with@by#1 by \pgf@stop%
      \fi%
    \else%
      \tikz@lib@parse@join@by#1\pgf@stop%
    \fi%
  \fi%
}
\def\tikz@lib@parse@join@with@by with #1 by #2\pgf@stop{%
  \tikzset{after node path={(#1)edge[every join,#2](\tikzchaincurrent)}}%
}
\def\tikz@lib@parse@join@by by #1\pgf@stop{%
  \tikzset{after node path={\ifx\tikzchainprevious\pgfutil@empty\else (\tikzchainprevious)edge[every join,#1](\tikzchaincurrent)\fi}}%
}
\tikzset{every join/.style=}


\def\tikz@lib@chainin#1(#2){\pgfutil@ifnextchar[{\tikz@lib@chainin@{#2}}{\tikz@lib@chainin@{#2}[]}}%]
\def\tikz@lib@chainin@#1[#2]{\path[late options={name=#1,on chain,every chain in/.try,#2}]}


%
% Branches
%

\tikzset{start branch/.code={%
    % save last node on current chain:
    \let\tikz@lib@save@current\tikz@lib@current@chain%
    \pgfkeysalso{/tikz/start chain/.expand once=\tikz@lib@current@chain/#1}%
    \path[late options={name=\tikz@lib@save@current-end,on chain}];%
  }%
}
\tikzset{continue branch/.style={continue chain/.expand once=\tikz@lib@current@chain/#1}}

\endinput


==> tikzlibrarydecorations.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgfmodule{decorations}

% Define the basic decoration stuff for tikz. Load more libraries to
% "actually use" decorations

\tikzset{decorate/.is if=tikz@decoratepath,
  /pgf/decoration/name/.store in=\tikz@decoration@name,
  /pgf/decoration/.unknown/.code=%
    \pgfifdecoration{\pgfkeyscurrentname}{\edef\tikz@decoration@name{\pgfkeyscurrentname}}
    {\pgfifmetadecoration{\pgfkeyscurrentname}{\edef\tikz@decoration@name{\pgfkeyscurrentname}}
    {\pgfkeys{/errors/unknown
        key={/pgf/decoration/\pgfkeyscurrentname}{#1}}}},%
  /pgf/decoration/raise/.code={\def\tikz@dec@shift{\pgftransformyshift{#1}}\tikz@dec@trans},
  /pgf/decoration/mirror/.code={%
    \csname if#1\endcsname
      \def\tikz@dec@mirror{\pgftransformyscale{-1}}%
    \else%
      \let\tikz@dec@mirror=\relax%
    \fi%
    \tikz@dec@trans%  
  },
  /pgf/decoration/mirror/.default=true,  
  /pgf/decoration/transform/.code={%
    {%
      \pgftransformreset%
      \def\tikz@transform{}%
      \pgfkeysalso{/tikz/.cd, #1}%
      \expandafter\gdef\expandafter\tikz@g@temptransform\expandafter{\tikz@transform}%
    }%
    \let\tikz@dec@user@transform=\tikz@g@temptransform%
    \tikz@dec@trans%
  },%
  /pgf/decoration/pre/.initial=lineto,
  /pgf/decoration/post/.initial=lineto,
  /pgf/decoration/pre length/.initial=0pt,
  /pgf/decoration/post length/.initial=0pt,
}

\let\tikz@decoration@name=\tikz@nonetext

\def\tikz@dec@trans{\pgfsetdecorationsegmenttransformation{\tikz@dec@user@transform\tikz@dec@mirror\tikz@dec@shift}}
\let\tikz@dec@user@transform=\relax
\let\tikz@dec@shift=\relax
\let\tikz@dec@mirror=\relax

\pgfdeclaremetadecoration{tikz@internal}{pre}{
  \state{pre}[width=\pgfkeysvalueof{/pgf/decoration/pre length}, next state=main]
  {
    \decoration{\pgfkeysvalueof{/pgf/decoration/pre}}
  }
  \state{main}[width=\pgfmetadecoratedremainingdistance-\pgfkeysvalueof{/pgf/decoration/post length}, next state=final]
  {
    \decoration{\tikz@decoration@name}
  }
  \state{final}
  {
    \decoration{\pgfkeysvalueof{/pgf/decoration/post}}
  }
}


\newif\iftikz@metadecoration

\def\tikz@lib@dec@addtomacro#1#2{\expandafter\def\expandafter#1\expandafter{#1#2}}

\def\tikz@lib@decoration[#1]{%
  \begingroup%
    % Just to be on the save side...
    %
    % Now, let's parse the options:
    \tikzset{#1}%
    %
    \ifx\tikz@decoration@name\tikz@nonetext%
    % Ok, let's forget about this decoration stuff...
    \else
      \expandafter\tikz@lib@do@dec%
    \fi%
      % Now, we expect a brace.
      \pgfutil@ifnextchar\bgroup{%
        \begingroup%
          \aftergroup\tikz@enddecoration%
          \afterassignment\tikz@scan@next@command%
          \let\tikz@lib@next% gobble \bgroup%
      }%
      {%
        \PackageError{tikz}{A decoration must begin with a brace}{}%
        \tikz@enddecoration%
      }%
}
\def\tikz@lib@do@dec{%
  % Ok, now what?
  \pgfifmetadecoration{\tikz@decoration@name}%
  {\expandafter\pgfmetadecoration\expandafter{\tikz@decoration@name}}%
  {%
    \pgfifdecoration{\tikz@decoration@name}%
    {\tikz@lib@dec@startdecoration}%
    {\PackageError{tikz}{Unknown (meta-)decoration '\tikz@decoration@name'. Perhaps you
        misspelled it?}{}}%
  }%
  \ifx\pgfdecorateexistingpath\pgfutil@empty%
    \pgfpathmoveto{\pgfqpoint{\the\tikz@lastxsaved}{\the\tikz@lastysaved}}%
  \fi%
}

\def\tikz@enddecoration{%
    \ifx\tikz@decoration@name\tikz@nonetext%
    % ignore this.
    \else
      % Ok, now what?
      \iftikz@metadecoration%
        \endpgfmetadecoration%
      \else%
        \tikz@lib@dec@stopdecoration%
      \fi%
    \fi
  \endgroup%
}


\def\tikz@lib@dec@decorate@path{%
  \ifx\tikz@decoration@name\tikz@nonetext%
  \else%
    \pgfgetpath\tikz@lib@dec@currentpath%
    \pgfsetpath\pgfutil@empty%
    \pgfifmetadecoration{\tikz@decoration@name}
    {   
      \expandafter\pgfmetadecoration\expandafter{\tikz@decoration@name}%
        \pgfsetpath\tikz@lib@dec@currentpath%
      \endpgfmetadecoration%
    }
    {
      \pgfifdecoration{\tikz@decoration@name}
      {
        \tikz@lib@dec@startdecoration%
          \pgfsetpath\tikz@lib@dec@currentpath%
        \tikz@lib@dec@stopdecoration%
      }
      {
        \PackageError{tikz}{Unknown (meta-)decoration '\tikz@decoration@name'. Perhaps
          you misspelled it?}{}
      }
    }
  \fi%
}

\def\tikz@lib@dec@zpttext{0pt}

\newif\iftikz@lib@dec@temp
\def\tikz@lib@dec@startdecoration{%
  \pgfkeysgetvalue{/pgf/decoration/pre length}{\tikz@lib@pre}%
  \pgfkeysgetvalue{/pgf/decoration/post length}{\tikz@lib@post}%
  \tikz@lib@dec@tempfalse%
  \ifx\tikz@lib@pre\tikz@lib@dec@zpttext%
    \ifx\tikz@lib@post\tikz@lib@dec@zpttext%
    \else%
      \tikz@lib@dec@temptrue%
    \fi%
  \else%
    \tikz@lib@dec@temptrue%
  \fi%
  \iftikz@lib@dec@temp%
    \pgfmetadecoration{tikz@internal}%
  \else%
    \expandafter\pgfdecoration\expandafter{\expandafter{\tikz@decoration@name}{\pgfdecoratedpathlength}{}{}}%
  \fi%
}

\def\tikz@lib@dec@stopdecoration{%
  \iftikz@lib@dec@temp%
    \endpgfmetadecoration%
  \else%
    \endpgfdecoration%
  \fi%
}


\endinput


==> tikzlibrarydecorations.footprints.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{decorations}
\usepgflibrary{decorations.footprints}

\endinput


==> tikzlibrarydecorations.fractals.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{decorations}
\usepgflibrary{decorations.fractals}

\endinput


==> tikzlibrarydecorations.markings.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{decorations}
\usepgflibrary{decorations.markings}

% Upgrade \arrow command
\def\pgf@lib@dec@doarrowhead{%
  \pgfutil@ifnextchar[{\tikz@lib@dec@doarrowhead}{\tikz@lib@dec@doarrowhead[]}%]
}
\def\tikz@lib@dec@doarrowhead[#1]#2{%
  \scope[#1]
    \pgf@lib@dec@arrowhead{1}{#2}%
  \endscope
}
\def\pgf@lib@dec@doarrowheadrev{%
  \pgfutil@ifnextchar[{\tikz@lib@dec@doarrowheadrev}{\tikz@lib@dec@doarrowheadrev[]}%]
}
\def\tikz@lib@dec@doarrowheadrev[#1]#2{%
  \scope[#1]
    \pgf@lib@dec@arrowhead{-1}{#2}%
  \endscope
}

\endinput


==> tikzlibrarydecorations.pathmorphing.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{decorations}
\usepgflibrary{decorations.pathmorphing}

\endinput


==> tikzlibrarydecorations.pathreplacing.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{decorations}
\usepgflibrary{decorations.pathreplacing}

\endinput


==> tikzlibrarydecorations.shapes.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{decorations}
\usepgflibrary{decorations.shapes}

\endinput


==> tikzlibrarydecorations.text.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usetikzlibrary{decorations}
\usepgflibrary{decorations.text}

\endinput


==> tikzlibraryer.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryer.code.tex,v 1.2 2008/02/20 11:00:42 tantau Exp $

\usetikzlibrary{shapes.geometric}

% Styles for entity types:

\tikzstyle{every entity}=           []
\tikzstyle{entity}=                 [rectangle,draw,
                                     minimum height=2\baselineskip,
                                     minimum width=4\baselineskip,every entity]


% Styles for relationship types:

\tikzstyle{every relationship}=     []
\tikzstyle{relationship}=           [diamond,draw,
                                     minimum size=1.5\baselineskip,
                                     inner sep=1pt,
                                     every relationship]


% Styles for relationship types:

\tikzstyle{every attribute}=        []
\tikzstyle{attribute}=              [minimum size=1.5\baselineskip,ellipse,draw,every attribute]
\tikzstyle{key attribute}=          [font=\itshape,attribute]




\endinput


==> tikzlibraryfadings.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryfadings.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\usepgflibrary{fadings}

%
% Environments for creating fadings
%

\def\tikzfadingfrompicture{%
  \begingroup%
    \setbox\pgfpic=\hbox\bgroup%
      \tikzpicture%
}
\def\endtikzfadingfrompicture{%
        \global\let\tikz@smuggle=\tikz@fig@name%
      \endtikzpicture
    \egroup%
    \pgfdeclarefading{\tikz@smuggle}{\box\pgfpic}%
  \endgroup%
}

\let\starttikzfadingfrompicture=\tikzfadingfrompicture
\let\stopttikzfadingfrompicture=\endtikzfadingfrompicture

\def\tikzfading[#1]{%
  {%
    \setbox\pgfpic=\hbox{%
      \tikzset{#1}%
      \global\let\tikz@smuggle=\tikz@fig@name%
      \tikz{%
        \useasboundingbox(0,0) (100bp,100bp);
        \node at (50bp,50bp) [rotate=\tikz@shade@angle]
        {\pgfuseshading{\tikz@shading}};
      }%
    }%
    \pgfdeclarefading{\tikz@smuggle}{\box\pgfpic}%    
  }%
}

==> tikzlibraryfit.code.tex <==
% Copyright 2007 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryfit.code.tex,v 1.2 2008/02/06 22:18:29 tantau Exp $

\pgfkeys{/tikz/fit/.code=\tikz@lib@fit{#1}}

\def\tikz@lib@fit#1{%
  \pgf@xb=-16000pt\relax%
  \pgf@xa=16000pt\relax%
  \pgf@yb=-16000pt\relax%
  \pgf@ya=16000pt\relax%
  % Now iterate over the coordinates
  \tikz@lib@fit@scan#1\pgf@stop%
  % Now, let's see what has happend
  \ifdim\pgf@xa>\pgf@xa%
    % Nothing... Ok, let's just ignore this.
  \else%
    % Ok, compute center and width and height
    \pgf@x=\pgf@xb%
    \advance\pgf@x by-\pgf@xa%
    \pgf@y=\pgf@yb%
    \advance\pgf@y by-\pgf@ya%
    \advance\pgf@xa by.5\pgf@x%
    \advance\pgf@ya by.5\pgf@y%
    \edef\tikz@node@at{\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}%
    \pgfkeysalso{/tikz/anchor=center,/tikz/text centered}%
    \pgfkeysalso{/tikz/text width/.expanded=\the\pgf@x}%
    \pgf@x=\pgf@y%
    \pgf@y=.5\pgf@y%
    \pgfkeysalso{
      /tikz/text height/.expanded=\the\pgf@y-.5\dp\pgfnodeparttextbox,
      /tikz/text depth/.expanded=\the\pgf@x-\noexpand\the\ht\pgfnodeparttextbox}%
    \pgfkeysalso{every fit/.try}%
  \fi%
}

\def\tikz@lib@fit@scan{%
  \pgfutil@ifnextchar\pgf@stop{\pgfutil@gobble}
  {\tikz@scan@one@point\tikz@lib@fit@scan@handle}}

\def\tikz@lib@fit@scan@handle#1{%
  \iftikz@shapeborder%
    % Ok, fit all four external anchors, if they exist
    \tikz@lib@fit@adjust{\pgfpointanchor{\tikz@shapeborder@name}{west}}%
    \tikz@lib@fit@adjust{\pgfpointanchor{\tikz@shapeborder@name}{east}}%
    \tikz@lib@fit@adjust{\pgfpointanchor{\tikz@shapeborder@name}{north}}%
    \tikz@lib@fit@adjust{\pgfpointanchor{\tikz@shapeborder@name}{south}}%
  \else%
    \tikz@lib@fit@adjust{#1}%
  \fi%
  \tikz@lib@fit@scan%
}

\def\tikz@lib@fit@adjust#1{%
  \pgf@process{#1}%
  \ifdim\pgf@x<\pgf@xa%
    \pgf@xa=\pgf@x%
  \fi%
  \ifdim\pgf@y<\pgf@ya%
    \pgf@ya=\pgf@y%
  \fi%
  \ifdim\pgf@x>\pgf@xb%
    \pgf@xb=\pgf@x%
  \fi%
  \ifdim\pgf@y>\pgf@yb%
    \pgf@yb=\pgf@y%
  \fi%
}

\endinput


==> tikzlibraryfolding.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryfolding.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $


%
% Length of a standard line in a folding
% 

\tikzoption{folding line length}{\pgfmathsetlength\tikz@lib@fold@length{#1}}
\newdimen\tikz@lib@fold@length
\tikz@lib@fold@length=2cm


\def\tikz@lib@fold@pentagon#1#2#3#4#5#6{%
  \begin{scope}[xshift=.5\tikz@lib@fold@length,yshift=0.68819\tikz@lib@fold@length]
    #1
  \end{scope}
  \begin{scope}[shift={(108:\tikz@lib@fold@length)},shift={(36:\tikz@lib@fold@length)},rotate=-36]
    #2
  \end{scope}
  \begin{scope}[xshift=\tikz@lib@fold@length,shift={(72:\tikz@lib@fold@length)},rotate=-108]
    #3
  \end{scope}
  \begin{scope}[xshift=\tikz@lib@fold@length,rotate=180]
    #4
  \end{scope}
  \begin{scope}[rotate=108]
    #5
  \end{scope}
  \begin{scope}[shift={(108:\tikz@lib@fold@length)},rotate=36]
    #6
  \end{scope}
}


\def\tikz@lib@fold@path{\draw[every fold](0,0) -- (\tikz@lib@fold@length,0pt);}
\def\tikz@lib@fold@cut@path{\draw[every cut](0,0) -- (\tikz@lib@fold@length,0pt);}
\def\tikz@lib@fold@ear@path{
  \draw[every fold](0,0) -- (\tikz@lib@fold@length,0pt);
  \draw[every cut] (0,0) -- (.5\tikz@lib@fold@length,.2\tikz@lib@fold@length) --(\tikz@lib@fold@length,0pt);}

\tikzstyle{every cut}=[]
\tikzstyle{every fold}=[help lines]

\tikzoption{face 1}{\def\tikz@lib@fold@face@A{#1}}
\tikzoption{face 2}{\def\tikz@lib@fold@face@B{#1}}
\tikzoption{face 3}{\def\tikz@lib@fold@face@C{#1}}
\tikzoption{face 4}{\def\tikz@lib@fold@face@D{#1}}
\tikzoption{face 5}{\def\tikz@lib@fold@face@E{#1}}
\tikzoption{face 6}{\def\tikz@lib@fold@face@F{#1}}
\tikzoption{face 7}{\def\tikz@lib@fold@face@G{#1}}
\tikzoption{face 8}{\def\tikz@lib@fold@face@H{#1}}
\tikzoption{face 9}{\def\tikz@lib@fold@face@I{#1}}
\tikzoption{face 10}{\def\tikz@lib@fold@face@J{#1}}
\tikzoption{face 11}{\def\tikz@lib@fold@face@K{#1}}
\tikzoption{face 12}{\def\tikz@lib@fold@face@L{#1}}

\let\tikz@lib@fold@face@A=\pgfutil@empty
\let\tikz@lib@fold@face@B=\pgfutil@empty
\let\tikz@lib@fold@face@C=\pgfutil@empty
\let\tikz@lib@fold@face@D=\pgfutil@empty
\let\tikz@lib@fold@face@E=\pgfutil@empty
\let\tikz@lib@fold@face@F=\pgfutil@empty
\let\tikz@lib@fold@face@G=\pgfutil@empty
\let\tikz@lib@fold@face@H=\pgfutil@empty
\let\tikz@lib@fold@face@I=\pgfutil@empty
\let\tikz@lib@fold@face@J=\pgfutil@empty
\let\tikz@lib@fold@face@K=\pgfutil@empty
\let\tikz@lib@fold@face@L=\pgfutil@empty

\def\tikzfoldingdodecahedron#1[#2]#3;{%
  \begingroup%
    \tikzset{#2}%
    \tikz@lib@fold@pentagon{\tikz@lib@fold@face@A}
    {
      \tikz@lib@fold@pentagon{\tikz@lib@fold@face@B}
      {
        \tikz@lib@fold@pentagon{\tikz@lib@fold@face@C}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@path}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@ear@path}
      }
      {\tikz@lib@fold@ear@path}
      {\tikz@lib@fold@path}
      {\tikz@lib@fold@ear@path}
      {\tikz@lib@fold@ear@path}
    }
    {
      \tikz@lib@fold@pentagon{\tikz@lib@fold@face@D}
      {
        \tikz@lib@fold@pentagon{\tikz@lib@fold@face@E}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@path}{\tikz@lib@fold@cut@path}{\tikz@lib@fold@ear@path}
      }
      {\tikz@lib@fold@ear@path}
      {\tikz@lib@fold@path}
      {\tikz@lib@fold@cut@path}
      {\tikz@lib@fold@cut@path}
    }
    {
      \tikz@lib@fold@pentagon{\tikz@lib@fold@face@F}
      {
        \tikz@lib@fold@pentagon{\tikz@lib@fold@face@G}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@path}{\tikz@lib@fold@cut@path}{\tikz@lib@fold@ear@path}
      }
      {\tikz@lib@fold@ear@path}
      {\tikz@lib@fold@path}
      {\tikz@lib@fold@cut@path}
      {\tikz@lib@fold@cut@path}
    }
    {
      \tikz@lib@fold@pentagon{\tikz@lib@fold@face@H}
      {
        \tikz@lib@fold@pentagon{\tikz@lib@fold@face@I}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@ear@path}{\tikz@lib@fold@path}{\tikz@lib@fold@cut@path}{\tikz@lib@fold@ear@path}
      }
      {\tikz@lib@fold@ear@path}
      {\tikz@lib@fold@path}
      {\tikz@lib@fold@cut@path}
      {\tikz@lib@fold@cut@path}
    }
    {
      \tikz@lib@fold@pentagon{\tikz@lib@fold@face@J}
      {
        \tikz@lib@fold@pentagon{\tikz@lib@fold@face@K}
        {\tikz@lib@fold@cut@path}
        {\tikz@lib@fold@cut@path}
        {\tikz@lib@fold@path}
        {\tikz@lib@fold@cut@path}
        {
          \tikz@lib@fold@pentagon{\tikz@lib@fold@face@L}{\tikz@lib@fold@cut@path}{\tikz@lib@fold@cut@path}{\tikz@lib@fold@path}{\tikz@lib@fold@cut@path}{\tikz@lib@fold@cut@path}
        }
      }
      {\tikz@lib@fold@cut@path}
      {\tikz@lib@fold@path}
      {\tikz@lib@fold@cut@path}
      {\tikz@lib@fold@cut@path}
    }
  \endgroup
}
  



==> tikzlibrarymatrix.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarymatrix.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $


% A matrix of nodes contains a node in each cell.

\tikzstyle{matrix of nodes}=[%
   matrix,%
   cells={anchor=base},%
   nodes={%
     execute at begin node=,%
     execute at end node=,
     name=\tikzmatrixname-\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn%
   },
   execute at begin cell=\tikz@lib@matrix@start@cell,%
   execute at end cell=\tikz@lib@matrix@end@cell,%
   execute at empty cell=\tikz@lib@matrix@empty@cell
]

\def\tikz@lib@matrix@empty@cell{\iftikz@lib@matrix@empty\node{};\fi}

\newif\iftikz@lib@matrix@plain

\def\tikz@lib@matrix@start@cell{%
  \pgfutil@ifnextchar|{\tikz@lib@matrix@with@options}{\tikz@lib@matrix@normal@start@cell}}

\def\tikz@lib@matrix@with@options|#1|{\tikz@lib@matrix@plainfalse\node#1\bgroup\tikz@lib@matrix@startup}


\def\tikz@lib@matrix@normal@start@cell{\pgfutil@ifnextchar\let{\tikz@lib@matrix@check}{\tikz@lib@matrix@plainfalse\node\bgroup\tikz@lib@matrix@startup}}%

\def\tikz@lib@matrix@check#1{% evil hackery to find out about start of path
  \pgfutil@ifnextchar\tikz@signal@path{\tikz@lib@matrix@plaintrue\let}{\tikz@lib@matrix@plainfalse\node\bgroup\tikz@lib@matrix@startup\let}%
}
  
\def\tikz@lib@matrix@end@cell{%
  \iftikz@lib@matrix@plain%
  \else%
    \expandafter\egroup\expandafter;%
  \fi%    
}

\def\tikz@lib@matrix@startup{%
  \pgfutil@ifnextchar\bgroup{%
    % Save meaning of \\:
    \let\tikz@lib@matrix@saved@eol=\\%
    % Now smuggle meaning inside following group.
    \let\\=\pgfmatrixendrow%
    \afterassignment\tikz@lib@matrix@smuggle%
    \let\tikz@next}
  {\let\\=\pgfmatrixendrow}%
}
\def\tikz@lib@matrix@smuggle{%
  \bgroup%
  \let\\=\tikz@lib@matrix@saved@eol%
}


% Fill empty nodes in a matrix of nodes

\newif\iftikz@lib@matrix@empty

\tikzoption{nodes in empty cells}[true]{\csname tikz@lib@matrix@empty#1\endcsname}


% Same as a matrix of nodes, but switch on math mode in each cell
\tikzstyle{matrix of math nodes}=[%
  matrix of nodes,
  nodes={%
   execute at begin node=$,%
   execute at end node=$%
  }%
]



% Provide a delimiter

\tikzoption{left delimiter}{\tikz@add@after@node@path{\tikz@delimiter%
    {south east}%
    {south west}%
    {every delimiter,every left delimiter}%
    {south}%
    {north}%
    {#1}%
    {.}%
    {\pgf@y}}}

\tikzoption{right delimiter}{\tikz@add@after@node@path{\tikz@delimiter%
    {south west}%
    {south east}%
    {every delimiter,every right delimiter}%
    {south}%
    {north}%
    {.}%
    {#1}%
    {\pgf@y}}}

\tikzoption{above delimiter}{\tikz@add@after@node@path{\tikz@delimiter%
    {south east}%
    {north west}%
    {every delimiter,every above delimiter,rotate=-90}%
    {west}%
    {east}%
    {#1}%
    {.}%
    {\pgf@x}}}

\tikzoption{below delimiter}{\tikz@add@after@node@path{\tikz@delimiter%
    {south west}%
    {south west}%
    {every delimiter,every below delimiter,rotate=-90}%
    {west}%
    {east}%
    {.}%
    {#1}%
    {\pgf@x}}}

\def\tikz@delimiter#1#2#3#4#5#6#7#8{%
  \bgroup
    \pgfextra{\let\tikz@save@last@fig@name=\tikz@last@fig@name}%
    node[outer sep=0pt,inner sep=0pt,draw=none,fill=none,anchor=#1,at=(\tikz@last@fig@name.#2),#3]
    {%
      {\nullfont\pgf@process{\pgfpointdiff{\pgfpointanchor{\tikz@last@fig@name}{#4}}{\pgfpointanchor{\tikz@last@fig@name}{#5}}}}%
      $\left#6\vcenter{\hrule height .5#8 depth .5#8 width0pt}\right#7$%
    }
    \pgfextra{\global\let\tikz@last@fig@name=\tikz@save@last@fig@name}%
  \egroup%
}

\tikzstyle{every delimiter}=[]
\tikzstyle{every left delimiter}=[]
\tikzstyle{every right delimiter}=[]
\tikzstyle{every above delimiter}=[]
\tikzstyle{every below delimiter}=[]

\endinput


==> tikzlibrarymindmap.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarymindmap.code.tex,v 1.5 2008/02/10 16:29:07 tantau Exp $


\usetikzlibrary{trees,decorations}


% A decoration for connecting circle nodes
%
% Parameters: start radius, end radius, amplitude, angle

\pgfdeclaredecoration{circle connection bar}{initial}
{
  \state{initial}[width=0pt,next state=bar]
  {
    {
    \pgftransformxshift{-\pgfkeysvalueof{/pgf/decoration/start radius}}%
    \pgfpathmoveto{\pgfpointpolar{\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}}
    \pgfpatharc{\pgfdecorationsegmentangle}{-\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}
    \pgfutil@tempcnta=-\pgfdecorationsegmentangle\relax
    \advance\pgfutil@tempcnta by90\relax
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/decoration/start radius}}
    \pgfmathsetlength\pgfutil@tempdimb{\pgfdecorationsegmentamplitude}
    \pgfpathcurveto
    {\pgfpointadd
      {\pgfpointpolar{-\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}}
      {\pgfpointpolar{\the\pgfutil@tempcnta}{.25\pgfutil@tempdima}}}
    {\pgfqpoint{1.25\pgfutil@tempdima}{-.5\pgfutil@tempdimb}}
    {\pgfqpoint{1.5\pgfutil@tempdima}{-.5\pgfutil@tempdimb}}
    \pgfpathlineto{\pgfpoint{1.5\pgfutil@tempdima}{.5\pgfutil@tempdimb}}
    \pgfutil@tempcnta=\pgfdecorationsegmentangle\relax
    \advance\pgfutil@tempcnta by-90\relax
    \pgfpathcurveto
    {\pgfpoint{1.25\pgfutil@tempdima}{.5\pgfutil@tempdimb}}
    {\pgfpointadd
      {\pgfpointpolar{\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}}
      {\pgfpointpolar{\the\pgfutil@tempcnta}{.25\pgfutil@tempdima}}}
    {\pgfpointpolar{\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/start radius}}}
    \pgfpathclose
    }
  }
  \state{bar}[width=0pt,next state=end]
  {
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/decoration/start radius}}%
    \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/decoration/end radius}}%
    \pgfmathsetlength\pgf@xc{\pgfdecorationsegmentamplitude}%
    \pgfpathrectangle
    {\pgfqpoint{.5\pgfutil@tempdima}{-.5\pgf@xc}}
    {\pgfpoint{\pgfdecoratedremainingdistance+-.5\pgfutil@tempdimb+-.5\pgfutil@tempdima}{\pgf@xc}}
  }
  \state{end}[width=0pt,next state=final]
  {
    {
    \pgftransformxshift{\pgfdecoratedremainingdistance}%
    \pgftransformxscale{-1}%
    \pgftransformxshift{-\pgfkeysvalueof{/pgf/decoration/end radius}}%
    \pgfpathmoveto{\pgfpointpolar{\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/end radius}}}
    \pgfpatharc{\pgfdecorationsegmentangle}{-\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/end radius}}
    \pgfutil@tempcnta=-\pgfdecorationsegmentangle\relax
    \advance\pgfutil@tempcnta by90\relax
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/decoration/end radius}}
    \pgfmathsetlength\pgfutil@tempdimb{\pgfdecorationsegmentamplitude}%
    \pgfpathcurveto
    {\pgfpointadd
      {\pgfpointpolar{-\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/end radius}}}
      {\pgfpointpolar{\the\pgfutil@tempcnta}{.25\pgfutil@tempdima}}}
    {\pgfqpoint{1.25\pgfutil@tempdima}{-.5\pgfutil@tempdimb}}
    {\pgfqpoint{1.5\pgfutil@tempdima}{-.5\pgfutil@tempdimb}}
    \pgfpathlineto{\pgfpoint{1.5\pgfutil@tempdima}{.5\pgfutil@tempdimb}}
    \pgfutil@tempcnta=\pgfdecorationsegmentangle\relax
    \advance\pgfutil@tempcnta by-90\relax
    \pgfpathcurveto
    {\pgfpoint{1.25\pgfutil@tempdima}{.5\pgfutil@tempdimb}}
    {\pgfpointadd
      {\pgfpointpolar{\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/end radius}}}
      {\pgfpointpolar{\the\pgfutil@tempcnta}{.25\pgfutil@tempdima}}}
    {\pgfpointpolar{\pgfdecorationsegmentangle}{\pgfkeysvalueof{/pgf/decoration/end radius}}}
    \pgfpathclose
    }
  }
  \state{final}
  {}
}



\pgfkeys{/pgf/decoration/angle=20}

% To paths for connecting circle nodes

\tikzstyle{circle connection bar}=
[to path={
  \pgfextra{\tikz@compute@circle@radii\tikz@compute@segmentamplitude}
  [fill=\tikz@concept@color,draw=none]
  [every circle connection bar]
  decorate [decoration=circle connection bar]
  { -- (\tikztotarget) \tikztonodes}
}]
\tikzstyle{every circle connection bar}=[]

\def\tikz@compute@circle@radii{%
  \pgf@process{\pgfpointtransformed{\pgfpointanchor{\tikztostart}{center}}}%
  \pgf@xa=\pgf@x%
  \pgf@process{\pgfpointtransformed{\pgfpointanchor{\tikztostart}{west}}}%
  \advance\pgf@xa by-\pgf@x%
  \pgfkeys{/pgf/decoration/start radius/.expanded=\the\pgf@xa}%
  \pgf@process{\pgfpointtransformed{\pgfpointanchor{\tikztotarget}{center}}}%
  \pgf@xa=\pgf@x%
  \pgf@process{\pgfpointtransformed{\pgfpointanchor{\tikztotarget}{west}}}%
  \advance\pgf@xa by-\pgf@x%
  \pgfkeys{/pgf/decoration/end radius/.expanded=\the\pgf@xa}%
}
\def\tikz@compute@segmentamplitude{%
  \pgf@x=\pgfkeysvalueof{/pgf/decoration/start radius}\relax%
  \ifdim\pgf@x>\pgfkeysvalueof{/pgf/decoration/end radius}\relax%
    \pgf@x=\pgfkeysvalueof{/pgf/decoration/end radius}\relax%
  \fi%
  \pgf@x=.175\pgf@x\relax%
  \edef\pgfdecorationsegmentamplitude{\the\pgf@x}%
}


% Switch color in a mindmap

\tikzoption{circle connection bar switch color}{\tikz@parse@switch#1\pgf@unique}
\def\tikz@parse@switch from (#1) to (#2)\pgf@unique{%
  \def\tikz@to@path{%
    \pgfextra{%
      \pgfutil@colorlet{tikz@switch@from}{#1}%
      \pgfutil@colorlet{tikz@switch@to}{#2}%
      \tikz@compute@circle@radii\tikz@compute@segmentamplitude%
      \tikz@compute@rotation%
    }
    [fill=none,draw=none]
    [every circle connection bar]
    decorate [decoration=circle connection bar]
    {-- (\tikztotarget) \tikztonodes} 
    [shading=tikz@shade@bar]
  }
}

\tikzoption{concept color}{%
  \let\tikz@old@concept@color=\tikz@concept@color%
  \def\tikz@edge@to@parent@path{
    (\tikzparentnode)
    to[circle connection bar switch color=from (\tikz@old@concept@color) to (#1)]
    (\tikzchildnode)}
  \def\tikz@concept@color{#1}%
}

\pgfdeclarehorizontalshading[tikz@switch@from,tikz@switch@to]{tikz@shade@bar}{100bp}{%
  color(0pt)=(tikz@switch@from);
  color(50bp)=(tikz@switch@from);
  color(55bp)=(tikz@switch@to);
  color(100bp)=(tikz@switch@to)}

\def\tikz@compute@rotation{%
  \pgf@process{\pgfpointnormalised{\pgfpointdiff{\pgfpointanchor{\tikztostart}{center}}{\pgfpointanchor{\tikztotarget}{center}}}}%
  \pgf@ya=-\pgf@y%
  \edef\pgf@marshal{%
    \noexpand\pgfsetadditionalshadetransform{%
      \noexpand\pgftransformcm
      {\pgf@sys@tonumber{\pgf@x}}{\pgf@sys@tonumber{\pgf@y}}%
      {\pgf@sys@tonumber{\pgf@ya}}{\pgf@sys@tonumber{\pgf@x}}%
      {\noexpand\pgfpointorigin}%
    }%
  }%
  \pgf@marshal%
}




% A concept node

\tikzstyle{concept}=          [circle,fill=\tikz@concept@color,draw=\tikz@concept@color,every concept]
\tikzstyle{every concept}=    []

\def\tikz@concept@color{black}

\tikzstyle{tikz@concept@setting}=[edge from parent path={(\tikzparentnode) to [circle connection bar] (\tikzchildnode)}]
\tikzstyle{tikz@concept@color@set}=[]


\tikzstyle{extra concept}=     [concept color=black!50,level 2 concept,concept,every extra concept]
\tikzstyle{every extra concept}=[]

\tikzstyle{concept connection}=[line width=1mm,shorten <=2mm,shorten >=2mm,cap=round,draw=black!50]


% A mindmap

\tikzstyle{mindmap}=
  [fill,draw,very thick,outer sep=0pt,inner sep=1pt,%
   every child/.append style={style=tikz@concept@setting,style=tikz@concept@color@set},%
   root concept,
   level 1/.append style={level 1 concept},
   level 2/.append style={level 2 concept},
   level 3/.append style={level 3 concept},
   level 4/.append style={level 4 concept},
   text centered,%       
   segment angle=20,
   style=every mindmap,
  ]
\tikzstyle{every mindmap}=[]


\tikzstyle{root concept}=   [minimum size=4cm,text width=3.5cm,font=\pgfutil@font@large]
\tikzstyle{level 1 concept}=[minimum size=2.25cm,
                             level distance=5cm,
                             text width=2cm,
                             sibling angle=60,
                             font=\pgfutil@font@small]
\tikzstyle{level 2 concept}=[minimum size=1.75cm,%
                             level distance=2.9cm,%
                             text width=1.5cm,%
                             sibling angle=60,%
                             font=\pgfutil@font@footnotesize]
\tikzstyle{level 3 concept}=[minimum size=1.15cm,%
                             text width=1cm,%
                             level distance=2.4cm,%
                             sibling angle=30,%
                             font=\pgfutil@font@tiny]
\tikzstyle{level 4 concept}=[minimum size=0.9cm,%
                             text width=0.7cm,
                             level distance=1.85cm,%
                             sibling angle=30,%
                             font=\pgfutil@font@tiny]
  
\tikzstyle{large mindmap}=
  [%
  root concept/.style={minimum size=5.6cm,text width=4.5cm,font=\pgfutil@font@Large},
  level 1 concept/.style={%
    minimum size=3.2cm,
    level distance=7cm,
    text width=2.8cm,
    sibling angle=60,
    font=},%
  level 2 concept/.style={%
    minimum size=2.45cm,%
    level distance=4cm,%
    text width=2.2cm,%
    sibling angle=60,%
    font=\pgfutil@font@small%
    },%
  level 3 concept/.style={%
    minimum size=1.63cm,%
    text width=1.4cm,%
    level distance=3.38cm,%
    sibling angle=30,%
    font=\pgfutil@font@scriptsize},%
  level 4 concept/.style={%
    minimum size=1.27cm,%
    text width=1cm,
    level distance=2.60cm,%
    sibling angle=30,%
    font=\pgfutil@font@tiny},%
  mindmap,%
  line width=2pt
  ]
  
\tikzstyle{huge mindmap}=
  [%
  root concept/.style={minimum size=8cm,text width=7cm,font=\pgfutil@font@huge},
  level 1 concept/.style={%
    minimum size=4.5cm,
    level distance=10cm,
    text width=4cm,
    sibling angle=60,
    font=\pgfutil@font@large},%
  level 2 concept/.style={%
    minimum size=3.5cm,%
    level distance=5.8cm,%
    text width=3cm,%
    sibling angle=60,%
    font=%
    },%
  level 3 concept/.style={%
    minimum size=2.3cm,%
    text width=2cm,%
    level distance=4.8cm,%
    sibling angle=30,%
    font=\pgfutil@font@footnotesize},%
  level 4 concept/.style={%
    minimum size=1.7cm,%
    text width=1.4cm,
    level distance=3.7cm,%
    sibling angle=30,%
    font=\pgfutil@font@scriptsize},%
  mindmap,%
  line width=3pt
  ]
  

% Annotations

\tikzstyle{annotation}=[shape=rectangle,
                        minimum size=0pt,
                        text width=3.5cm,
                        outer sep=1.5mm,
                        inner sep=1mm,
                        text badly ragged,
                        rounded corners,
                        font=\pgfutil@font@tiny,
                        every annotation]
\tikzstyle{every annotation}=[]



\endinput



==> tikzlibrarypatterns.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarypatterns.code.tex,v 1.2 2008/01/15 10:27:34 tantau Exp $

\usepgflibrary{patterns}

\tikzoption{pattern color}{\edef\tikz@pattern@color{#1}}
\tikzoption{pattern}[]{%
  \edef\tikz@temp{#1}%
  \ifx\tikz@temp\tikz@nonetext%
    \tikz@addmode{\tikz@mode@fillfalse}%
  \else%
    \ifx\tikz@temp\pgfutil@empty%
    \else%
      \tikz@addoption{\pgfsetfillpattern{#1}{\tikz@pattern@color}}%
      \def\tikz@pattern{#1}%
    \fi%
    \tikz@addmode{\tikz@mode@filltrue}%
  \fi%
}
\def\tikz@pattern@color{black}
\def\tikz@pattern{dots}

\endinput


==> tikzlibrarypetri.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarypetri.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $


% Styles for places:

\tikzstyle{every place}=           []
\tikzstyle{place}=                 [circle,draw,inner sep=0pt,
                                    minimum size=5ex,
                                    every place]


% Styles for transition:

\tikzstyle{every transition}=      []
\tikzstyle{transition}=            [rectangle,draw,inner sep=0pt,
                                    minimum size=4mm,
                                    every transition]


% Styles for relationship types:

\tikzstyle{pre}=                   [<-,shorten <=1pt]
\tikzstyle{post}=                  [->,shorten >=1pt]
\tikzstyle{pre and post}=          [<->,shorten >=1pt,shorten <=1pt]



% Styles for marks:

\tikzstyle{every token}=           []
\tikzstyle{token}=                 [fill=black,draw=none,circle,
                                    inner sep=0.5pt,minimum size=1ex,
                                    text=white,font=\pgfutil@font@tiny,every token]

\tikzoption{token distance}{\def\tikz@token@distance{#1}}
\def\tikz@token@distance{1.5ex}

\tikzstyle{children are tokens}=   [growth function=\tikz@grow@tokens,edge from parent path=]

\tikzoption{tokens}{%
  \ifnum#1>0\relax%
    \tikz@add@after@node@path{%
     {[children are tokens]child foreach \tikz@dummy in {1,...,#1} {node[token]{}}}}%
  \fi}

\tikzoption{colored tokens}{%
  \tikz@add@after@node@path{%
    {[children are tokens]child foreach \tikz@child@color in {#1} {node[token,\tikz@child@color]{}}}}%
  }

\tikzoption{structured tokens}{%
  \tikz@add@after@node@path{%
    {[children are tokens]child foreach \tikz@child@name in {#1} {node[token]{\tikz@child@name}}}}%
  }


\def\tikz@grow@tokens{%
  \pgfmathsetlength{\pgf@xa}{\tikz@token@distance}%
  \pgfmathsetlength{\pgf@ya}{\tikz@token@distance}%
  \pgf@xc=0pt%
  \pgf@yc=0pt%
  \csname tikz@grow@tokens@placer@\the\tikznumberofchildren @\the\tikznumberofcurrentchild\endcsname%
  \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
}

\def\tikz@def@grow@tokens#1#2#3#4{%
  \expandafter\def\csname tikz@grow@tokens@placer@#1@#2\endcsname{%
    \pgf@xc=#3\pgf@xa%
    \pgf@yc=#4\pgf@ya}%
}


% Single token
\tikz@def@grow@tokens{1}{1}{0}{0}

% Two tokens
\tikz@def@grow@tokens{2}{1}{-.5}{0}
\tikz@def@grow@tokens{2}{2}{.5}{0}

% Three tokens
\tikz@def@grow@tokens{3}{1}{0} {0.57}
\tikz@def@grow@tokens{3}{2}{-.5}{-.306025}
\tikz@def@grow@tokens{3}{3}{.5} {-.306025}

% Four tokens
\tikz@def@grow@tokens{4}{1}{-.5}{.5}
\tikz@def@grow@tokens{4}{2}{.5}{.5}
\tikz@def@grow@tokens{4}{3}{-.5}{-.5}
\tikz@def@grow@tokens{4}{4}{.5}{-.5}

% Five tokens
\tikz@def@grow@tokens{5}{1}{0}{.85}
\tikz@def@grow@tokens{5}{2}{-0.808398}{0.26266}
\tikz@def@grow@tokens{5}{3}{0.808398}{0.26266}
\tikz@def@grow@tokens{5}{4}{-0.499617}{-0.687664}
\tikz@def@grow@tokens{5}{5}{0.499617}{-0.687664}

% Six tokens
\tikz@def@grow@tokens{6}{1}{-1}{.5}
\tikz@def@grow@tokens{6}{2}{0}{.5}
\tikz@def@grow@tokens{6}{3}{1}{.5}
\tikz@def@grow@tokens{6}{4}{-1}{-.5}
\tikz@def@grow@tokens{6}{5}{0}{-.5}
\tikz@def@grow@tokens{6}{6}{1}{-.5}

% Seven tokens
\tikz@def@grow@tokens{7}{1}{0}{1}
\tikz@def@grow@tokens{7}{2}{-1}{.5}
\tikz@def@grow@tokens{7}{3}{0}{0}
\tikz@def@grow@tokens{7}{4}{1}{.5}
\tikz@def@grow@tokens{7}{5}{-1}{-.5}
\tikz@def@grow@tokens{7}{6}{0}{-1}
\tikz@def@grow@tokens{7}{7}{1}{-.5}

% Eight tokens
\tikz@def@grow@tokens{8}{1}{-.5}{1}
\tikz@def@grow@tokens{8}{2}{.5}{1}
\tikz@def@grow@tokens{8}{3}{-1}{0}
\tikz@def@grow@tokens{8}{4}{0}{0}
\tikz@def@grow@tokens{8}{5}{1}{0}
\tikz@def@grow@tokens{8}{6}{-1}{-1}
\tikz@def@grow@tokens{8}{7}{0}{-1}
\tikz@def@grow@tokens{8}{8}{1}{-1}

% Eight tokens
\tikz@def@grow@tokens{9}{1}{-1}{1}
\tikz@def@grow@tokens{9}{2}{0}{1}
\tikz@def@grow@tokens{9}{3}{1}{1}
\tikz@def@grow@tokens{9}{4}{-1}{0}
\tikz@def@grow@tokens{9}{5}{0}{0}
\tikz@def@grow@tokens{9}{6}{1}{0}
\tikz@def@grow@tokens{9}{7}{-1}{-1}
\tikz@def@grow@tokens{9}{8}{0}{-1}
\tikz@def@grow@tokens{9}{9}{1}{-1}


\endinput


==> tikzlibraryplothandlers.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryplothandlers.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\usepgflibrary{plothandlers}

\endinput


==> tikzlibraryplotmarks.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryplotmarks.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\usepgflibrary{plotmarks}

\endinput


==> tikzlibrarypositioning.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarypositioning.code.tex,v 1.5 2008/02/12 23:41:59 tantau Exp $


\tikzset{above/.code=\tikz@lib@place@handle@{#1}{south}{0}{1}{north}{1}}
\tikzset{above left/.code=\tikz@lib@place@handle@{#1}{south east}{-1}{1}{north west}{0.707106781}}
\tikzset{above right/.code=\tikz@lib@place@handle@{#1}{south west}{1}{1}{north east}{0.707106781}}
\tikzset{base left/.code =\tikz@lib@place@handle@{#1}{base east}{-1}{0}{base west}{1}}
\tikzset{base right/.code=\tikz@lib@place@handle@{#1}{base west}{1}{0}{base east}{1}}
\tikzset{below/.code=\tikz@lib@place@handle@{#1}{north}{0}{-1}{south}{1}}
\tikzset{below left/.code=\tikz@lib@place@handle@{#1}{north east}{-1}{-1}{south west}{0.707106781}}
\tikzset{below right/.code=\tikz@lib@place@handle@{#1}{north west}{1}{-1}{south east}{0.707106781}}
\tikzset{left/.code =\tikz@lib@place@handle@{#1}{east}{-1}{0}{west}{1}}
\tikzset{mid left/.code =\tikz@lib@place@handle@{#1}{mid east}{-1}{0}{base west}{1}}
\tikzset{mid right/.code=\tikz@lib@place@handle@{#1}{mid west}{1}{0}{base east}{1}}
\tikzset{right/.code=\tikz@lib@place@handle@{#1}{west}{1}{0}{east}{1}}

\newif\iftikz@lib@ignore@size

% Hook into resets:
\pgfutil@g@addto@macro\tikz@node@reset@hook{\tikz@addtransform{\tikz@lib@pos@call}\let\tikz@lib@pos@call=\relax}

\tikzset{on grid/.is if=tikz@lib@ignore@size}

\tikzset{node distance=1cm and 1cm}

\def\tikz@lib@place@handle@#1#2#3#4#5#6{%
  \def\tikz@anchor{#2}%
  \edef\tikz@temp{#1}%
  \def\tikz@lib@place@single@factor{#6}%
  \expandafter\tikz@lib@place@handle@@\expandafter{\tikz@temp}{#3}{#4}{#5}%
}
\def\tikz@lib@place@handle@@#1#2#3#4{%
  \pgfutil@in@{of }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@of#1\tikz@stop{#4}%
  \else%
    \edef\tikz@lib@place@nums{#1}%
  \fi%
  \ifx\tikz@lib@place@nums\pgfutil@empty%
    % Ok, nothing to do, we have set the anchor and we are happy...
  \else%
    \expandafter\tikz@lib@place@parse@nums\expandafter{\tikz@lib@place@nums}%
    \pgf@x=#2\pgf@x%
    \pgf@y=#3\pgf@y%
    \edef\tikz@lib@pos@call{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \fi%
}

\def\tikz@lib@place@parse@nums#1{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@parse@nums@#1\tikz@stop%
  \else%
    \tikz@lib@place@parse@nums@#1and#1\tikz@stop%
    \pgf@x=\tikz@lib@place@single@factor\pgf@x%
    \pgf@y=\tikz@lib@place@single@factor\pgf@y%
  \fi
}
\def\tikz@lib@place@parse@nums@#1and#2\tikz@stop{%
  \pgfmathparse{#2}%
  \ifpgfmathunitsdeclared%
    \pgf@xa=\pgfmathresult pt%
    \pgf@ya=0pt%
  \else%
    \let\tikz@lib@temp=\pgfmathresult%
    \pgf@process{\pgfpointxy{\tikz@lib@temp}{0}}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
  \fi%
  \pgfmathparse{#1}%
  \ifpgfmathunitsdeclared%
    \advance\pgf@ya by\pgfmathresult pt%
  \else%
    \let\tikz@lib@temp=\pgfmathresult%
    \pgf@process{\pgfpointxy{0}{\tikz@lib@temp}}%
    \advance\pgf@xa by\pgf@x%
    \advance\pgf@ya by\pgf@y%
  \fi%
  \pgf@x=\pgf@xa%
  \pgf@y=\pgf@ya%
}

\def\tikz@lib@place@of#1of #2\tikz@stop#3{%
  \def\tikz@temp{#1}%
  \ifx\tikz@temp\pgfutil@empty%
    \tikz@lib@place@of@{\tikz@node@distance}{#2}{#3}%
  \else%
    \tikz@lib@place@of@{#1}{#2}{#3}%
  \fi%
}
\def\tikz@lib@place@of@#1#2#3{%
  \tikz@scan@one@point\tikz@lib@place@remember(#2)%
  \iftikz@shapeborder%
    % Ok, this is relative to a border.
    \iftikz@lib@ignore@size%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{center}}%
      \def\tikz@anchor{center}%
    \else%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{#3}}%
    \fi%
  \fi%
  \edef\tikz@lib@place@nums{#1}%
}
\def\tikz@lib@place@remember#1{\def\tikz@node@at{#1}}



\endinput


==> tikzlibraryscopes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryscopes.code.tex,v 1.1 2008/02/08 01:18:38 tantau Exp $

% Redefine the after command hook...

\def\tikz@lib@scope@check{%
  \pgfutil@ifnextchar\par{%
    \afterassignment\tikz@lib@scope@check\let\tikz@next%
  }%
  {\pgfutil@ifnextchar\bgroup{%gotcha
      \afterassignment\tikz@lib@scope@gotcha\let\tikz@next%
    }%
    {}%
  }
}

\def\tikz@lib@scope@gotcha{%
  \pgfutil@ifnextchar[{%]
    \tikz@lib@scope@action%
  }{%
    % false alarm
    \bgroup%
  }%  
}
\def\tikz@lib@scope@action[#1]{%
  \scope[#1]\bgroup\aftergroup\endscope%
  \tikz@lib@scope@check%
}

\endinput


==> tikzlibraryshadows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshadows.code.tex,v 1.3 2008/01/13 15:30:04 tantau Exp $

\usetikzlibrary{fadings}


% General options
\tikzset{
  /tikz/shadow scale/.initial=1,
  /tikz/shadow xshift/.initial=0pt,
  /tikz/shadow yshift/.initial=0pt,
}

% Basic shadow style
\tikzset{
  general shadow/.style={
    preaction={
      #1,
      transform canvas={
        scale around=\pgfkeysvalueof{/tikz/shadow scale}:(current path bounding box.center),
        shift={(\pgfkeysvalueof{/tikz/shadow xshift},\pgfkeysvalueof{/tikz/shadow yshift})}
      },
    }
  },
  every shadow/.style={}
}



%
% Adds a simple drop shadow to a path
%

\tikzset{
  /tikz/drop shadow/.style={
    general shadow={%
      shadow scale=1,
      shadow xshift=.5ex,
      shadow yshift=-.5ex,
      opacity=.5,
      fill=black!50,
      every shadow,
      #1
    }
  }
}


%
% Adds a circular drop shadow to a path
%

\tikzset{
  /tikz/circular drop shadow/.style={
    general shadow={%
      shadow scale=1.1,
      shadow xshift=.3ex,
      shadow yshift=-.3ex,
      fill=black!50,
      path fading={circle with fuzzy edge 15 percent},
      every shadow,
      #1
    }
  }
}



%
% Adds a circular glow to a path
%

\tikzset{
  /tikz/circular glow/.style={
    general shadow={%
      shadow scale=1.25,
      shadow xshift=0pt,
      shadow yshift=0pt,
      fill=black!50,
      path fading={circle with fuzzy edge 15 percent},
      every shadow,
      #1,
    }
  }
}





%
% Adds a "copy" version of the path behind it.
%

\tikzset{
  /tikz/copy shadow/.style={
    general shadow={%
      /utils/exec={\let\tikz@lib@shadow@fill=\tikz@fillcolor\let\tikz@lib@shadow@draw=\tikz@strokecolor},
      shadow scale=1,
      shadow xshift=.5ex,
      shadow yshift=.5ex,
      fill=\tikz@lib@shadow@fill,
      draw=\tikz@lib@shadow@draw,
      every shadow,
      #1
    }
  }
}


%
% Adds two "copies" of the path behind it.
%

\tikzset{
  /tikz/double copy shadow/.style={
    general shadow={%
      /utils/exec={\let\tikz@lib@shadow@fill=\tikz@fillcolor\let\tikz@lib@shadow@draw=\tikz@strokecolor},
      shadow scale=1,
      shadow xshift=.5ex,
      shadow yshift=.5ex,
      fill=\tikz@lib@shadow@fill,
      draw=\tikz@lib@shadow@draw,
      #1,
      shadow xshift/.expanded=2*\pgfkeysvalueof{/tikz/shadow xshift},
      shadow yshift/.expanded=2*\pgfkeysvalueof{/tikz/shadow yshift},
    },
    general shadow={%
      /utils/exec={\let\tikz@lib@shadow@fill=\tikz@fillcolor\let\tikz@lib@shadow@draw=\tikz@strokecolor},
      shadow scale=1,
      shadow xshift=.5ex,
      shadow yshift=.5ex,
      fill=\tikz@lib@shadow@fill,
      draw=\tikz@lib@shadow@draw,
      #1,
    },
  }
}



==> tikzlibraryshapes.arrows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshapes.arrows.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\usepgflibrary{shapes.arrows}

\pgfkeys{/tikz/arrow box arrows/.code={\pgf@lib@arrowbox@parsearrows{#1}}}

\endinput


==> tikzlibraryshapes.callouts.code.tex <==
% Copyright 2006 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\usepgflibrary{shapes.callouts}

\pgfkeys{/tikz/callout absolute pointer/.code={%
	\tikz@scan@one@point\tikz@lib@callout@checkforplus#1\relax%
	}%
}

\def\tikz@lib@callout@checkforplus#1{%
	\pgfutil@ifnextchar+{\def\tikz@lib@callout@originalpoint{#1}\tikz@lib@callout@scan@relative}%
		{\pgf@lib@callout@makeabsolutepointer{#1}}}%

\def\tikz@lib@callout@scan@relative+{%
	\pgfutil@ifnextchar+{\tikz@lib@callout@scan@plusplus}{\tikz@lib@callout@scan@plus}}
\def\tikz@lib@callout@scan@plusplus+{\tikz@scan@one@point\tikz@lib@callout@add}
\def\tikz@lib@callout@scan@plus{\tikz@scan@one@point\tikz@lib@callout@add}
\def\tikz@lib@callout@add#1{%
	\expandafter\pgf@lib@callout@makeabsolutepointer\expandafter{%
		\expandafter\pgfpointadd\expandafter{\tikz@lib@callout@originalpoint}{#1}}%
}%

\pgfkeys{/tikz/callout relative pointer/.code={%
		\tikz@scan@one@point\pgf@lib@callout@makerelativepointer#1\relax%
	}%
}

\endinput

==> tikzlibraryshapes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshapes.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes.misc}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shapes.arrows}
\usetikzlibrary{shapes.callouts}
\usetikzlibrary{shapes.multipart}

\endinput


==> tikzlibraryshapes.gates.logic.IEC.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshapes.gates.logic.IEC.code.tex,v 1.3 2008/01/27 11:39:49 vibrovski Exp $

\usepgflibrary{shapes.gates.logic.IEC}

\tikzset{%
  use IEC style logic gates/.code={%
  	\tikzset{%
			and gate/.style={shape=and gate IEC},
			nand gate/.style={shape=nand gate IEC},
			or gate/.style={shape=or gate IEC},
			nor gate/.style={shape=nor gate IEC},
			xor gate/.style={shape=xor gate IEC},
			xnor gate/.style={shape=xnor gate IEC},
			not gate/.style={shape=not gate IEC},
			buffer gate/.style={shape=buffer gate IEC},
			and gate symbol/.style={and gate IEC symbol={##1}},
			nand gate symbol/.style={nand gate IEC symbol={##1}},
			or gate symbol/.style={or gate IEC symbol={##1}},
			nor gate symbol/.style={nor gate IEC symbol={##1}},
			xor gate symbol/.style={xor gate IEC symbol={##1}},
			xnor gate symbol/.style={xnor gate IEC symbol={##1}},
			not gate symbol/.style={not gate IEC symbol={##1}},
			buffer gate symbol/.style={buffer gate IEC symbol={##1}},
			logic gate symbol align/.style={/pgf/logic gate IEC symbol align={##1}},
			logic gate symbol color/.style={/pgf/logic gate IEC symbol color={##1}}
		}%
	}%
}
\endinput




==> tikzlibraryshapes.gates.logic.US.code.tex <==
% Copyright 2008 by Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshapes.gates.logic.US.code.tex,v 1.1 2008/01/25 08:26:00 vibrovski Exp $

\usepgflibrary{shapes.gates.logic.US}

\tikzset{%
   use US style logic gates/.code={%
  	\tikzset{%
			and gate/.style={shape=and gate US},
			nand gate/.style={shape=nand gate US},
			or gate/.style={shape=or gate US},
			nor gate/.style={shape=nor gate US},
			xor gate/.style={shape=xor gate US},
			xnor gate/.style={shape=xnor gate US},
			not gate/.style={shape=not gate US},
			buffer gate/.style={shape=buffer gate US}
		}%
	},
	use CDH style logic gates/.code={%
  	\tikzset{%
			and gate/.style={shape=and gate CDH},
			nand gate/.style={shape=nand gate CDH},
			or gate/.style={shape=or gate US},
			nor gate/.style={shape=nor gate US},
			xor gate/.style={shape=xor gate US},
			xnor gate/.style={shape=xnor gate US},
			not gate/.style={shape=not gate US},
			buffer gate/.style={shape=buffer gate US}
		}
	}
}
\endinput


==> tikzlibraryshapes.geometric.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshapes.geometric.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\usepgflibrary{shapes.geometric}

\endinput


==> tikzlibraryshapes.misc.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshapes.misc.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\usepgflibrary{shapes.misc}

\endinput


==> tikzlibraryshapes.multipart.code.tex <==
% Copyright 2007 by Till Tantau and Mark Wibrow
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshapes.multipart.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\usepgflibrary{shapes.multipart}

\pgfkeys{/tikz/rectangle split/parts/.code={%
	\pgfkeys{/pgf/rectangle split parts=#1}%
	}%
}

\pgfkeys{/tikz/rectangle split use custom fill/.code={%
	\pgfkeys{/pgf/rectangle split use custom fill=#1}%
	\pgfkeys{/tikz/fill=none}}%
}

\pgfkeys{/tikz/rectangle split draw splits/.is if=pgfrectanglesplitdrawsplits}

\pgfkeys{/tikz/rectangle split part align/.code={%
		\pgfkeys{/pgf/rectangle split part align={#1}}%
	}%
}%

\pgfkeys{/tikz/rectangle split part fill/.code={%
		\pgfkeys{/pgf/rectangle split part fill={#1}}%
	}%
}%

\endinput


==> tikzlibraryshapes.symbols.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryshapes.symbols.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $

\pgfkeysifdefined{/tikz/shape border uses incircle}{}{%
	\pgfkeys{/tikz/shape border uses incircle/.is if=pgfshapeborderusesincircle}}
	
\usepgflibrary{shapes.symbols}

\endinput


==> tikzlibrarysnakes.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarysnakes.code.tex,v 1.6 2008/02/05 13:08:05 tantau Exp $

\PackageWarning{tikz}{Snakes have been superseded by
decorations. Please use the decoration libraries instead of the snakes
library}

\usetikzlibrary{decorations.pathmorphing,decorations.pathreplacing,decorations.shapes}


% Old snakes stuff:

\tikzoption{snake}[]{%
  \def\tikz@@snake{#1}%
  \ifx\tikz@@snake\pgfutil@empty%
    \tikz@snakedtrue%
  \else%
    \ifx\tikz@@snake\tikz@nonetext%
      \tikz@snakedfalse%
    \else%
      \tikz@snakedtrue%
      \let\tikz@snake=\tikz@@snake%
    \fi%
  \fi}

\tikzoption{raise snake}{\def\pgf@snake@raise{\pgftransformyshift{#1}}}
\tikzoption{mirror snake}[true]{%
  \csname if#1\endcsname
    \def\pgf@snake@mirror{\pgftransformyscale{-1}}%
  \else%
    \let\pgf@snake@mirror=\pgfutil@empty%
  \fi
}

\tikzoption{gap before snake}{\def\tikz@presnake{{moveto}{#1}{\noexpand\tikz@snake@install@trans}{}}}
\tikzoption{line before snake}{\def\tikz@presnake{{lineto}{#1}{\noexpand\tikz@snake@install@trans}{}}}

\tikzoption{gap after snake}{\def\tikz@postsnake{{moveto}{#1}{\noexpand\tikz@snake@install@trans}{}}\def\tikz@mainsnakelength{\pgfsnakeremainingdistance-#1}}
\tikzoption{line after snake}{\def\tikz@postsnake{{lineto}{#1}{\noexpand\tikz@snake@install@trans}{}}\def\tikz@mainsnakelength{\pgfsnakeremainingdistance-#1}}

\tikzoption{gap around snake}{%
  \def\tikz@presnake{{moveto}{#1}{\noexpand\tikz@snake@install@trans}{}}%
  \def\tikz@postsnake{{moveto}{#1}{\noexpand\tikz@snake@install@trans}{}}%
  \def\tikz@mainsnakelength{\pgfsnakeremainingdistance-#1}%
}
\tikzoption{line around snake}{%
  \def\tikz@presnake{{lineto}{#1}{\noexpand\tikz@snake@install@trans}{}}%
  \def\tikz@postsnake{{lineto}{#1}{\noexpand\tikz@snake@install@trans}{}}%
  \def\tikz@mainsnakelength{\pgfsnakeremainingdistance-#1}%
}
\let\pgf@snake@mirror=\pgfutil@empty
\let\pgf@snake@raise=\pgfutil@empty

\def\tikz@snake@install@trans{\pgfsetsnakesegmenttransformation{\pgf@snake@mirror\pgf@snake@raise}}

\def\tikz@snake{zigzag}

\let\tikz@presnake=\pgfutil@empty
\let\tikz@postsnake=\pgfutil@empty
\def\tikz@mainsnakelength{\pgfsnakeremainingdistance}


\tikzstyle{snake triangles 45}=      [snake=triangles,segment object length=2.41421356\pgfsnakesegmentamplitude]
\tikzstyle{snake triangles 60}=      [snake=triangles,segment object length=1.73205081\pgfsnakesegmentamplitude]
\tikzstyle{snake triangles 90}=      [snake=triangles,segment object length=\pgfsnakesegmentamplitude]



\endinput


==> tikzlibrarythrough.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarythrough.code.tex,v 1.1 2008/02/03 19:37:27 tantau Exp $



\tikzset{circle through/.code={%
    \pgfkeysalso{shape=circle,inner sep=0pt,outer sep=0pt}%
    % Save transformations (correct?)
    \pgfgettransform{\tikz@lib@saved@transform}%
    \tikz@scan@one@point\tikz@lib@circle@through#1%
  }}

\def\tikz@lib@circle@through#1{%
  \tikz@addoption{%
    {%
      \pgfsettransform{\tikz@lib@saved@transform}%
      \pgf@process{\pgfpointtransformed{#1}}%
      \pgf@xa=\pgf@x%
      \pgf@ya=\pgf@y%
      \pgf@process{\pgfpointtransformed{\tikz@node@at}}%
      \advance\pgf@xa by-\pgf@x%
      \advance\pgf@ya by-\pgf@y%
      \pgfmathparse{2*veclen(\the\pgf@xa,\the\pgf@ya)}%
      \global\let\tikz@lib@circle@size=\pgfmathresult%
    }%
    \pgfset{/pgf/minimum size/.expanded=\tikz@lib@circle@size}%
  }%
}

==> tikzlibrarytopaths.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarytopaths.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $


% Straight to

\tikzstyle{line to}=                 [to path={-- (\tikztotarget) \tikztonodes}]


% Curved to

\tikzstyle{every curve to}=          []
\tikzstyle{curve to}=                [to path=\tikz@to@curve@path]

\tikzoption{bend angle}{\def\tikz@to@bend{#1}}

\tikzoption{bend left}[]{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \def\tikz@to@bend{#1}%
  \fi%
  \let\tikz@to@out=\tikz@to@bend%
  \c@pgf@counta=180\relax%
  \advance\c@pgf@counta by-\tikz@to@out\relax%
  \edef\tikz@to@in{\the\c@pgf@counta}%
  \tikz@to@switch@on%
  \tikz@to@relativetrue%
}

\tikzoption{bend right}[]{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty%
  \else%
    \def\tikz@to@bend{#1}%
  \fi%
  % Now, negate
  \c@pgf@counta=\tikz@to@bend\relax%
  \c@pgf@counta=-\c@pgf@counta\relax%
  \edef\tikz@to@out{\the\c@pgf@counta}%
  \c@pgf@counta=180\relax%
  \advance\c@pgf@counta by-\tikz@to@out\relax%
  \edef\tikz@to@in{\the\c@pgf@counta}%
  \tikz@to@switch@on%
  \tikz@to@relativetrue%
}

\tikzoption{relative}[true]{\csname tikz@to@relative#1\endcsname}
\newif\iftikz@to@relative
\tikz@to@relativefalse

\tikzoption{in}{\def\tikz@to@in{#1}\tikz@to@switch@on}
\tikzoption{out}{\def\tikz@to@out{#1}\tikz@to@switch@on}

\tikzoption{in looseness}{\tikz@to@set@in@looseness{#1}}
\tikzoption{out looseness}{\tikz@to@set@out@looseness{#1}}
\tikzoption{looseness}{\tikz@to@set@in@looseness{#1}\tikz@to@set@out@looseness{#1}}

\tikzoption{in control}{\tikz@to@set@in@control{#1}}
\tikzoption{out control}{\tikz@to@set@out@control{#1}}
\tikzoption{controls}{\tikz@to@parse@controls#1\pgf@stop}

\tikzoption{in min distance}{\tikz@to@set@distances{#1}{}{}{}}
\tikzoption{in max distance}{\tikz@to@set@distances{}{#1}{}{}}
\tikzoption{in distance}{\tikz@to@set@distances{#1}{#1}{}{}}
\tikzoption{out min distance}{\tikz@to@set@distances{}{}{#1}{}}
\tikzoption{out max distance}{\tikz@to@set@distances{}{}{}{#1}}
\tikzoption{out distance}{\tikz@to@set@distances{}{}{#1}{#1}}
\tikzoption{min distance}{\tikz@to@set@distances{#1}{}{#1}{}}
\tikzoption{max distance}{\tikz@to@set@distances{}{#1}{}{#1}}
\tikzoption{distance}{\tikz@to@set@distances{#1}{#1}{#1}{#1}}

\def\tikz@to@set@distances#1#2#3#4{%
  \tikz@to@setifnotempy{#1}{\tikz@to@in@min}{\let\tikz@to@end@compute=\tikz@to@end@compute@looseness}%
  \tikz@to@setifnotempy{#2}{\tikz@to@in@max}{\let\tikz@to@end@compute=\tikz@to@end@compute@looseness}%
  \tikz@to@setifnotempy{#3}{\tikz@to@out@min}{\let\tikz@to@start@compute=\tikz@to@start@compute@looseness}%
  \tikz@to@setifnotempy{#4}{\tikz@to@out@max}{\let\tikz@to@start@compute=\tikz@to@start@compute@looseness}%
  \tikz@to@switch@on%
}

\def\tikz@to@setifnotempy#1#2#3{%
  \def\pgf@temp{#1}%
  \ifx\pgf@temp\pgfutil@empty\else\def#2{#1}#3\fi%
}


\def\tikz@to@set@in@looseness#1{%
  \def\tikz@to@in@looseness{#1}%
  \let\tikz@to@end@compute=\tikz@to@end@compute@looseness%
  \tikz@to@switch@on%
}
\def\tikz@to@set@out@looseness#1{%
  \def\tikz@to@out@looseness{#1}%
  \let\tikz@to@start@compute=\tikz@to@start@compute@looseness%
  \tikz@to@switch@on%
}

\def\tikz@to@parse@controls#1and#2\pgf@stop{\tikz@to@set@in@control{#2}\tikz@to@set@out@control{#1}}

\def\tikz@to@set@in@control#1{%
  \def\tikz@to@in@control{#1}%
  \let\tikz@to@end@compute=\tikz@to@end@compute@control%
  \tikz@to@switch@on%
}
\def\tikz@to@set@out@control#1{%
  \def\tikz@to@out@control{#1}%
  \let\tikz@to@start@compute=\tikz@to@start@compute@control%
  \tikz@to@switch@on%
}


\def\tikz@to@bend{30}

\def\tikz@to@out{45}
\def\tikz@to@in{135}

\def\tikz@to@out@looseness{1}
\def\tikz@to@in@looseness{1}

\def\tikz@to@in@min{0pt}
\def\tikz@to@in@max{10000pt}
\def\tikz@to@out@min{0pt}
\def\tikz@to@out@max{10000pt}

\def\tikz@to@switch@on{\let\tikz@to@path=\tikz@to@curve@path}

\def\tikz@to@curve@path{%
  [every curve to]
  \pgfextra{\iftikz@to@relative\tikz@to@compute@relative\else\tikz@to@compute\fi}
  \tikz@computed@path
  \tikztonodes%
}

\def\tikz@to@modify#1#2{%
  \pgfutil@ifundefined{pgf@sh@ns@#1}
  {}%
  {\edef#1{#1.#2}}
}%

\def\tikz@to@compute{%
  \let\tikz@tofrom=\tikztostart%
  \let\tikz@toto=\tikztotarget%
  \tikz@to@modify\tikz@tofrom\tikz@to@out%
  \tikz@to@modify\tikz@toto\tikz@to@in%
  \ifx\tikz@to@start@compute\tikz@to@start@compute@looseness%
    \tikz@to@compute@distance%
  \else%
    \ifx\tikz@from@start@compute\tikz@to@start@compute@looseness%  
      \tikz@to@compute@distance%
    \fi%
  \fi%
  \tikz@to@start@compute%
  \tikz@to@end@compute%
  \edef\tikz@computed@path{.. controls \tikz@computed@start and \tikz@computed@end .. (\tikz@toto)}
}

\def\tikz@to@compute@distance{\tikz@scan@one@point\tikz@@to@compute@distance(\tikz@tofrom)}
\def\tikz@@to@compute@distance#1{%
  \def\tikz@first@point{#1}%
  \tikz@scan@one@point\tikz@@@to@compute@distance(\tikz@toto)}
\def\tikz@@@to@compute@distance#1{%
  \def\tikz@second@point{#1}%
  \tikz@to@compute@distance@main%
}
\def\tikz@to@compute@distance@main{%
  \pgf@process{\pgfpointdiff{\tikz@first@point}{\tikz@second@point}}%
  \ifdim\pgf@x<0pt\pgf@xa=-\pgf@x\else\pgf@xa=\pgf@x\fi%
  \ifdim\pgf@y<0pt\pgf@ya=-\pgf@y\else\pgf@ya=\pgf@y\fi%
  % 
  % Calculate length of second to first vector:
  % 
  \pgf@process{\pgfpointnormalised{\pgfqpoint{\pgf@xa}{\pgf@ya}}}%
  \ifdim\pgf@x>\pgf@y%
    \c@pgf@counta=\pgf@x%
    \ifnum\c@pgf@counta=0\relax%
    \else%
      \divide\c@pgf@counta by 255\relax%
      \pgf@xa=16\pgf@xa\relax%
      \divide\pgf@xa by\c@pgf@counta%
      \pgf@xa=16\pgf@xa\relax%
    \fi%
  \else%
    \c@pgf@counta=\pgf@y%
    \ifnum\c@pgf@counta=0\relax%
    \else%
      \divide\c@pgf@counta by 255\relax%
      \pgf@ya=16\pgf@ya\relax%
      \divide\pgf@ya by\c@pgf@counta%
      \pgf@xa=16\pgf@ya\relax%
    \fi%
  \fi%
  \pgf@x=0.3915\pgf@xa%
  \pgf@xa=\tikz@to@out@looseness\pgf@x%
  \pgf@xb=\tikz@to@in@looseness\pgf@x%
  % Adjust as necessary
  \pgfmathsetlength{\pgf@ya}{\tikz@to@out@min}
  \ifdim\pgf@xa<\pgf@ya%
    \pgf@xa=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@out@max}
  \ifdim\pgf@xa>\pgf@ya%
    \pgf@xa=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@in@min}
  \ifdim\pgf@xb<\pgf@ya%
    \pgf@xb=\pgf@ya%
  \fi%
  \pgfmathsetlength{\pgf@ya}{\tikz@to@in@max}
  \ifdim\pgf@xb>\pgf@ya%
    \pgf@xb=\pgf@ya%
  \fi%
}

\def\tikz@to@start@compute@looseness{%
  \edef\tikz@computed@start{([shift=(\tikz@to@out:\the\pgf@xa)]\tikz@tofrom)}%
}
\def\tikz@to@end@compute@looseness{%
  \edef\tikz@computed@end{([shift=(\tikz@to@in:\the\pgf@xb)]\tikz@toto)}%
}
\def\tikz@to@start@compute@control{%
  \let\tikz@computed@start=\tikz@to@out@control%
}
\def\tikz@to@end@compute@control{%
  \let\tikz@computed@end=\tikz@to@in@control%
}

\let\tikz@to@start@compute=\tikz@to@start@compute@looseness%
\let\tikz@to@end@compute=\tikz@to@end@compute@looseness%




% Relative curves

\def\tikz@to@compute@relative{%
  \tikz@scan@one@point\tikz@@to@compute@relative(\tikztostart)%
}
\def\tikz@@to@compute@relative#1{%
  \def\tikz@tofrom{#1}%
  \tikz@scan@one@point\tikz@@@to@compute@relative(\tikztotarget)%
}
\def\tikz@@@to@compute@relative#1{%
  \def\tikz@toto{#1}%
  \begingroup
    % 
    % Adjust start and target so that they lie on the border in the
    % rotated coordinate system.
    %  
    \pgfutil@ifundefined{pgf@sh@ns@\tikztostart}
    {%
      \let\tikz@first@point=\tikz@tofrom%
      \let\tikz@tostart@tikz=\pgfutil@empty
    }%
    {%
      % Start computation of new start.
      {%
        \tikz@tofrom%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        {%
          \pgftransformreset%
          \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
          \pgftransformrotate{\tikz@to@out}%
          \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
          \pgf@process{\pgfpointtransformed{\tikz@toto}}%
        }%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        \pgfpointshapeborder{\tikztostart}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
        \xdef\tikz@tofrom@smuggle{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      }%
      \let\tikz@first@point=\tikz@tofrom@smuggle%
      \tikz@first@point%
      \edef\tikz@tostart@tikz{(\the\pgf@x,\the\pgf@y)}%
    }%
    \pgfutil@ifundefined{pgf@sh@ns@\tikztotarget}
    {%
      \let\tikz@second@point=\tikz@toto%
    }%
    {%
      % Start computation of new target.
      {%
        \tikz@toto%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        {%
          \pgftransformreset%
          \pgftransformshift{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
          \pgftransformrotate{180}%
          \pgftransformrotate{\tikz@to@in}%
          \pgftransformshift{\pgfqpoint{-\pgf@xc}{-\pgf@yc}}%
          \pgf@process{\pgfpointtransformed{\tikz@tofrom}}%
        }%
        \pgf@xc=\pgf@x%
        \pgf@yc=\pgf@y%
        \pgfpointshapeborder{\tikztotarget}{\pgfqpoint{\pgf@xc}{\pgf@yc}}%
        \xdef\tikz@toto@smuggle{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}
      }%
      \let\tikz@second@point=\tikz@toto@smuggle%
    }%
    \tikz@second@point%
    \edef\tikz@totarget@tikz{(\the\pgf@x,\the\pgf@y)}%
    %
    % Compute distances
    %
    \tikz@to@compute@distance@main%
    \edef\tikz@to@first@distance{\the\pgf@xa}%
    \edef\tikz@to@second@distance{\the\pgf@xb}%
    %
    % Next step: Establish a transformed coordinate system so that the (modified)
    % start is at the origin and the (modified) target is at (1,0)
    %
    \pgftransformreset%
    \pgf@process{\tikz@first@point}%
    \pgf@xa=\pgf@x%
    \pgf@ya=\pgf@y%
    \pgf@process{\tikz@second@point}%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgfpointnormalised{}%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgf@xb=-\pgf@x%
    \pgf@yb=-\pgf@y%
    %
    % Now compute the control points.
    %
    {%
      \pgftransformshift{\tikz@first@point}%
      \pgftransformcm{\pgf@sys@tonumber\pgf@xc}{\pgf@sys@tonumber\pgf@yc}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xc}%
                      {\pgfpointorigin}%
      \pgf@process{\pgfpointtransformed{\pgfpointpolar{\tikz@to@out}{\tikz@to@first@distance}}}%
      \xdef\tikz@computed@start{(\the\pgf@x,\the\pgf@y)}%
    }
    {%
      \pgftransformshift{\tikz@second@point}%
      \pgftransformcm{\pgf@sys@tonumber\pgf@xc}{\pgf@sys@tonumber\pgf@yc}{\pgf@sys@tonumber\pgf@yb}{\pgf@sys@tonumber\pgf@xc}%
                      {\pgfpointorigin}%
      \pgf@process{\pgfpointtransformed{\pgfpointpolar{\tikz@to@in}{\tikz@to@second@distance}}}%
      \xdef\tikz@computed@end{(\the\pgf@x,\the\pgf@y)}%
    }
    \xdef\tikz@computed@path{
      \tikz@tostart@tikz
      .. controls \tikz@computed@start and \tikz@computed@end ..
      \tikz@totarget@tikz}%
  \endgroup
}



% Loops

\tikzstyle{loop}=                    [to path={
  \pgfextra{\let\tikztotarget=\tikztostart}
  [looseness=8,min distance=5mm,every loop]
  \tikz@to@curve@path
  }]

\tikzstyle{every loop}=              [->,shorten >=1pt]

\tikzstyle{loop right}=              [right,out=15,in=-15,loop]
\tikzstyle{loop above}=              [above,out=105,in=75,loop]
\tikzstyle{loop left}=               [left,out=195,in=165,loop]
\tikzstyle{loop below}=              [below,out=285,in=255,loop]





\endinput


==> tikzlibrarytrees.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibrarytrees.code.tex,v 1.1 2008/01/09 17:57:16 tantau Exp $



%
% Three point growth
%

\tikzoption{grow via three points}{\let\tikz@grow=\tikz@grow@three\tikz@parse@three#1}

\def\tikz@parse@three one child at#1(#2)#3and two children at#4(#5)#6and#7(#8){%
  \def\tikz@tree@one@child{\tikz@scan@one@point\pgf@process(#2)}
  \def\tikz@tree@left@child{\tikz@scan@one@point\pgf@process(#5)}
  \def\tikz@tree@right@child{\tikz@scan@one@point\pgf@process(#8)}
}

\def\tikz@grow@three{%
  \pgf@process{\tikz@tree@one@child}%
  \pgf@xa=\pgf@x%
  \pgf@ya=\pgf@y%
  \pgf@process{\tikz@tree@left@child}%
  \pgf@xb=\pgf@x%
  \pgf@yb=\pgf@y%
  \advance\pgf@xb by-\pgf@xa%
  \advance\pgf@yb by-\pgf@ya%
  \pgf@process{\tikz@tree@right@child}%
  \pgf@xc=\pgf@x%
  \pgf@yc=\pgf@y%
  \advance\pgf@xc by-\pgf@xa%
  \advance\pgf@yc by-\pgf@ya%
  \advance\pgf@xc by-\pgf@xb%
  \advance\pgf@yc by-\pgf@yb%
  \advance\tikznumberofchildren by-1\relax%
  \pgf@xb=\tikznumberofchildren\pgf@xb\relax%
  \pgf@yb=\tikznumberofchildren\pgf@yb\relax%
  \advance\tikznumberofcurrentchild by-1\relax%
  \pgf@xc=\tikznumberofcurrentchild\pgf@xc\relax%
  \pgf@yc=\tikznumberofcurrentchild\pgf@yc\relax%
  \advance\pgf@xa by\pgf@xb%
  \advance\pgf@xa by\pgf@xc%
  \advance\pgf@ya by\pgf@yb%
  \advance\pgf@ya by\pgf@yc%
  \edef\pgf@temp{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}}%
  \pgf@temp%
}

%
% Circle grow
%

\tikzstyle{grow cyclic}=[growth function=\tikz@grow@circle]

\tikzset{sibling angle/.initial=20}

\def\tikz@grow@circle{%
  \pgftransformrotate{%
    (\pgfkeysvalueof{/tikz/sibling angle})*(-.5-.5*\tikznumberofchildren+\tikznumberofcurrentchild)}%
  \pgftransformxshift{\the\tikzleveldistance}%
}

\tikzoption{counterclockwise from}{\let\tikz@grow=\tikz@grow@circle@from\def\tikz@grow@circle@from@start{#1}}

\def\tikz@grow@circle@from{%
  \pgftransformshift{\pgfpointpolar{\tikz@grow@circle@from@start+(\pgfkeysvalueof{/tikz/sibling angle})*(\tikznumberofcurrentchild-1)}{\the\tikzleveldistance}}%
}

\tikzoption{clockwise from}{\let\tikz@grow=\tikz@grow@circle@from@\def\tikz@grow@circle@from@start{#1}}

\def\tikz@grow@circle@from@{%
  \pgftransformshift{\pgfpointpolar{\tikz@grow@circle@from@start-(\pgfkeysvalueof{/tikz/sibling angle})*(\tikznumberofcurrentchild-1)}{\the\tikzleveldistance}}%
}



%
% Connections
%

\tikzstyle{edge from parent fork down}=
  [edge from parent path={(\tikzparentnode\tikzparentanchor) -- +(0pt,-.5\tikzleveldistance)  -| (\tikzchildnode\tikzchildanchor)}]

\tikzstyle{edge from parent fork up}=
  [edge from parent path={(\tikzparentnode\tikzparentanchor) -- +(0pt,.5\tikzleveldistance)  -| (\tikzchildnode\tikzchildanchor)}]

\tikzstyle{edge from parent fork left}=
  [edge from parent path={(\tikzparentnode\tikzparentanchor) -- +(-.5\tikzleveldistance,0pt) |- (\tikzchildnode\tikzchildanchor)}]

\tikzstyle{edge from parent fork right}=
  [edge from parent path={(\tikzparentnode\tikzparentanchor) -- +(.5\tikzleveldistance,0pt) |- (\tikzchildnode\tikzchildanchor)}]


                                    
\endinput

